Estimating a scalar log-concave random variable, using a silence set based probabilistic sampling

We study the probabilistic sampling of a random variable, in which the variable is sampled only if it falls outside a given set, which is called the silence set. This helps us to understand optimal event-based sampling for the special case of IID random processes, and also to understand the design of a sub-optimal scheme for other cases. We consider the design of this probabilistic sampling for a scalar, log-concave random variable, to minimize either the mean square estimation error, or the mean absolute estimation error. We show that the optimal silence interval: (i) is essentially unique, and (ii) is the limit of an iterative procedure of centering. Further we show through numerical experiments that super-level intervals seem to be remarkably near-optimal for mean square estimation. Finally we use the Gauss inequality for scalar unimodal densities, to show that probabilistic sampling gives a mean square distortion that is less than a third of the distortion incurred by periodic sampling, if the average sampling rate is between 0.3 and 0.9 samples per tick.

==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5MeanZero.tex <==
-0.5 0.0357096718032
-0.49501 0.0356957014811
-0.49002 0.035654141861
-0.48503 0.0355833107285
-0.48004 0.0354868727149
-0.47505 0.0353657503028
-0.47006 0.0352208407726
-0.46507 0.035050480076
-0.46008 0.0348606258829
-0.45509 0.0346470654179
-0.4501 0.0344131475513
-0.44511 0.0341596645629
-0.44012 0.0338873907074
-0.43513 0.0335970831281
-0.43014 0.0332894827051
-0.42515 0.0329653148425
-0.42016 0.0326252901998
-0.41517 0.0322701053713
-0.41018 0.0319004435171
-0.40519 0.0315191081323
-0.4002 0.0311224550134
-0.39521 0.0307132991706
-0.39022 0.0302943005252
-0.38523 0.0298619965793
-0.38024 0.0294210141005
-0.37525 0.0289699310506
-0.37026 0.0285093407334
-0.36527 0.0280398271148
-0.36028 0.027561965127
-0.35529 0.0270780877172
-0.3503 0.0265851817304
-0.34531 0.026087292803
-0.34032 0.0255831955046
-0.33533 0.0250750409994
-0.33034 0.0245600828864
-0.32535 0.0240420377708
-0.32036 0.0235197997076
-0.31537 0.0229953420706
-0.31038 0.0224676198838
-0.30539 0.0219371245321
-0.3004 0.0214043408729
-0.29541 0.0208710688198
-0.29042 0.0203363860774
-0.28543 0.019800759024
-0.28044 0.0192646479418
-0.27545 0.0187296839708
-0.27046 0.0181962086045
-0.26547 0.0176623469261
-0.26048 0.0171307841004
-0.25549 0.016601847343
-0.2505 0.0160748582496
-0.24551 0.0155502388288
-0.24052 0.0150293393468
-0.23553 0.0145115700257
-0.23054 0.013997337362
-0.22555 0.0134878770113
-0.22056 0.0129826853741
-0.21557 0.0124829243033
-0.21058 0.0119881464314
-0.20559 0.0114994417478
-0.2006 0.0110164176686
-0.19561 0.0105400943439
-0.19062 0.0100701323706
-0.18563 0.00960689513739
-0.18064 0.00915186176945
-0.17565 0.00870361946153
-0.17066 0.0082636113945
-0.16567 0.0078321006529
-0.16068 0.0074088962756
-0.15569 0.00699433455055
-0.1507 0.00658914782242
-0.14571 0.00619358832894
-0.14072 0.00580755339879
-0.13573 0.0054316915739
-0.13074 0.0050659407226
-0.12575 0.00471089622214
-0.12076 0.00436653390563
-0.11577 0.00403339873151
-0.11078 0.0037117266427
-0.10579 0.00340154641113
-0.1008 0.00310314608086
-0.09581 0.00281714874658
-0.09082 0.00254342382787
-0.08583 0.00228224692999
-0.08084 0.0020340107241
-0.07585 0.00179893652876
-0.07086 0.0015771495973
-0.06587 0.0013689897389
-0.06088 0.00117460230049
-0.05589 0.000994295151312
-0.0509 0.000828280214379
-0.04591 0.000676727912836
-0.04092 0.000539905899612
-0.03593 0.000418021213985
-0.03094 0.000311261505507
-0.02595 0.00021986221305
-0.02096 0.000144017004764
-0.01597 8.39485205566e-05
-0.01098 3.98423138112e-05
-0.00599 1.1904058059e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt2.tex <==
-0.5 0.0111111111111
-0.497763932023 0.0111094665008
-0.495527864045 0.011104619582
-0.493291796068 0.0110966978116
-0.49105572809 0.011085824842
-0.488819660113 0.0110721206167
-0.486583592135 0.011055701463
-0.484347524158 0.0110366801833
-0.48211145618 0.011015166145
-0.479875388203 0.0109912653673
-0.477639320225 0.0109650806076
-0.475403252248 0.0109367114452
-0.47316718427 0.0109062543632
-0.470931116293 0.0108738028296
-0.468695048315 0.0108394473754
-0.466458980338 0.010803275672
-0.46422291236 0.0107653726066
-0.461986844383 0.0107258203555
-0.459750776405 0.0106846984571
-0.457514708428 0.0106420838814
-0.45527864045 0.0105980511
-0.453042572473 0.0105526721529
-0.450806504495 0.0105060167145
-0.448570436518 0.0104581521585
-0.44633436854 0.0104091436204
-0.444098300563 0.0103590540593
-0.441862232585 0.0103079443181
-0.439626164608 0.0102558731822
-0.43739009663 0.0102028974369
-0.435154028653 0.0101490719235
-0.432917960675 0.0100944495938
-0.430681892698 0.010039081564
-0.42844582472 0.0099830171667
-0.426209756743 0.00992630400159
-0.423973688765 0.0098689879855
-0.421737620788 0.00981111340076
-0.41950155281 0.00975272294256
-0.417265484833 0.00969385776513
-0.415029416855 0.0096345575268
-0.412793348878 0.00957486043391
-0.4105572809 0.00951480328367
-0.408321212923 0.00945442150592
-0.406085144945 0.00939374920388
-0.403849076968 0.00933281919382
-0.40161300899 0.00927166304374
-0.399376941013 0.00921031111111
-0.397140873035 0.0091487925796
-0.394904805058 0.00908713549483
-0.39266873708 0.00902536679928
-0.390432669103 0.00896351236622
-0.388196601125 0.00890159703279
-0.385960533148 0.00883964463219
-0.38372446517 0.00877767802503
-0.381488397193 0.00871571912982
-0.379252329215 0.00865378895273
-0.377016261238 0.00859190761641
-0.37478019326 0.00853009438819
-0.372544125283 0.00846836770737
-0.370308057305 0.00840674521192
-0.368071989328 0.00834524376427
-0.36583592135 0.00828387947657
-0.363599853373 0.00822266773514
-0.361363785395 0.00816162322424
-0.359127717418 0.00810075994926
-0.35689164944 0.00804009125921
-0.354655581463 0.00797962986851
-0.352419513485 0.0079193878783
-0.350183445508 0.00785937679707
-0.34794737753 0.00779960756066
-0.345711309553 0.00774009055178
-0.343475241575 0.0076808356189
-0.341239173598 0.00762185209462
-0.33900310562 0.00756314881351
-0.336767037643 0.0075047341294
-0.334530969665 0.00744661593221
-0.332294901688 0.00738880166424
-0.33005883371 0.00733129833601
-0.327822765733 0.00727411254161
-0.325586697755 0.00721725047359
-0.323350629778 0.00716071793744
-0.3211145618 0.00710452036557
-0.318878493823 0.00704866283093
-0.316642425845 0.00699315006018
-0.314406357868 0.00693798644648
-0.31217028989 0.00688317606185
-0.309934221913 0.00682872266922
-0.307698153935 0.00677462973403
-0.305462085958 0.0067209004355
-0.30322601798 0.00666753767759
-0.300989950003 0.00661454409956
-0.298753882025 0.00656192208619
-0.296517814048 0.00650967377777
-0.29428174607 0.00645780107966
-0.292045678093 0.00640630567159
-0.289809610115 0.00635518901673
-0.287573542138 0.00630445237032
-0.28533747416 0.00625409678818
-0.283101406183 0.00620412313482
-0.280865338205 0.00615453209139
-0.278629270228 0.00610532416327
-0.27639320225 0.0060564996875
-0.273629270228 0.00599668050619
-0.270865338205 0.00593745368025
-0.268101406183 0.00587882534014
-0.26533747416 0.00582080154918
-0.262573542138 0.00576338831695
-0.259809610115 0.00570659161176
-0.257045678093 0.00565041737206
-0.25428174607 0.00559487151696
-0.251517814048 0.0055399599558
-0.248753882025 0.0054856885968
-0.245989950003 0.00543206335492
-0.24322601798 0.00537909015881
-0.240462085958 0.00532677495699
-0.237698153935 0.00527512372325
-0.234934221913 0.00522414246127
-0.23217028989 0.00517383720853
-0.229406357868 0.0051242140395
-0.226642425845 0.00507527906813
-0.223878493823 0.0050270384497
-0.2211145618 0.00497949838199
-0.218350629778 0.00493266510588
-0.215586697755 0.00488654490525
-0.212822765733 0.00484114410638
-0.21005883371 0.00479646907672
-0.207294901688 0.00475252622311
-0.204530969665 0.00470932198941
-0.201767037643 0.00466686285373
-0.19900310562 0.00462515532492
-0.196239173598 0.00458420593875
-0.193475241575 0.00454402125347
-0.190711309553 0.00450460784488
-0.18794737753 0.00446597230091
-0.185183445508 0.0044281212158
-0.182419513485 0.00439106118361
-0.179655581463 0.00435479879143
-0.17689164944 0.00431934061204
-0.174127717418 0.00428469319601
-0.171363785395 0.00425086306345
-0.168599853373 0.0042178566952
-0.16583592135 0.00418568052351
-0.163071989328 0.00415434092226
-0.160308057305 0.00412384419666
-0.157544125283 0.00409419657242
-0.15478019326 0.00406540418441
-0.152016261238 0.00403747306476
-0.149252329215 0.00401040913042
-0.146488397193 0.00398421817016
-0.14372446517 0.00395890583091
-0.140960533148 0.00393447760356
-0.138196601125 0.00391093880813
-0.135432669103 0.00388829457823
-0.13266873708 0.00386654984485
-0.129904805058 0.0038457093195
-0.127140873035 0.00382577747652
-0.124376941013 0.00380675853468
-0.12161300899 0.00378865643795
-0.118849076968 0.00377147483545
-0.116085144945 0.00375521706045
-0.113321212923 0.00373988610856
-0.1105572809 0.00372548461483
-0.107793348878 0.00371201482994
-0.105029416855 0.00369947859528
-0.102265484833 0.00368787731692
-0.09950155281 0.00367721193841
-0.0967376207875 0.00366748291238
-0.093973688765 0.00365869017089
-0.0912097567425 0.0036508330943
-0.08844582472 0.00364391047894
-0.0856818926975 0.0036379205031
-0.082917960675 0.00363286069162
-0.0801540286525 0.00362872787879
-0.07739009663 0.00362551816955
-0.0746261646075 0.00362322689894
-0.071862232585 0.00362184858964
-0.0690983005625 0.00362137690761
-0.06633436854 0.00362180461564
-0.0635704365175 0.00362312352478
-0.060806504495 0.00362532444348
-0.0580425724725 0.00362839712448
-0.05527864045 0.00363233020915
-0.0525147084275 0.00363711116929
-0.049750776405 0.00364272624627
-0.0469868443825 0.00364916038733
-0.04422291236 0.00365639717898
-0.0414589803375 0.00366441877727
-0.038695048315 0.00367320583493
-0.0359311162925 0.00368273742514
-0.03316718427 0.00369299096179
-0.0304032522475 0.00370394211608
-0.027639320225 0.0037155647294
-0.0248753882025 0.00372783072212
-0.02211145618 0.00374070999836
-0.0193475241575 0.00375417034632
-0.016583592135 0.00376817733423
-0.0138196601125 0.00378269420152
-0.01105572809 0.00379768174511
-0.0082917960675 0.00381309820066
-0.005527864045 0.00382889911843
-0.0027639320225 0.00384503723367
0.0 0.00386146233122
0.00725403330759 0.00390529001642
0.0145080666152 0.00394990838629
0.0217620999228 0.0039953375494
0.0290161332303 0.00404159828771
0.0362701665379 0.00408871208499
0.0435241998455 0.00413670115661
0.0507782331531 0.00418558848097
0.0580322664607 0.00423539783252
0.0652862997683 0.00428615381651
0.0725403330759 0.00433788190567
0.0797943663834 0.00439060847876
0.087048399691 0.00444436086129
0.0943024329986 0.00449916736844
0.101556466306 0.0045550573504
0.108810499614 0.00461206124017
0.116064532921 0.00467021060414
0.123318566229 0.00472953819553
0.130572599537 0.00479007801091
0.137826632844 0.00485186535003
0.145080666152 0.00491493687917
0.152334699459 0.00497933069825
0.159588732767 0.00504508641202
0.166842766074 0.00511224520559
0.174096799382 0.00518084992455
0.18135083269 0.00525094516014
0.188604865997 0.0053225773398
0.195858899305 0.00539579482345
0.203112932612 0.005470648006
0.21036696592 0.00554718942659
0.217620999228 0.005625473885
0.224875032535 0.00570555856586
0.232129065843 0.00578750317135
0.23938309915 0.0058713700629
0.246637132458 0.00595722441281
0.253891165765 0.00604513436656
0.261145199073 0.00613517121669
0.268399232381 0.00622740958923
0.275653265688 0.00632192764383
0.282907298996 0.00641880728886
0.290161332303 0.00651813441257
0.297415365611 0.00661999913212
0.304669398919 0.0067244960618
0.311923432226 0.00683172460258
0.319177465534 0.0069417892546
0.326431498841 0.00705479995532
0.333685532149 0.00717087244539
0.340939565457 0.00729012866535
0.348193598764 0.00741269718613
0.355447632072 0.00753871367684
0.362701665379 0.00766832141393
0.369955698687 0.00780167183599
0.377209731994 0.00793892514921
0.384463765302 0.00808025098922
0.39171779861 0.00822582914566
0.398971831917 0.00837585035663
0.406225865225 0.00853051718143
0.413479898532 0.00869004496092
0.42073393184 0.00885466287622
0.427987965148 0.00902461511819
0.435241998455 0.00920016218181
0.442496031763 0.00938158230199
0.44975006507 0.00956917304951
0.457004098378 0.0097632531094
0.464258131685 0.00996416426728
0.471512164993 0.0101722736337
0.478766198301 0.0103879761414
0.486020231608 0.0106116973583
0.493274264916 0.010843896663
0.500528298223 0.0110850708437
0.507782331531 0.0113357581892
0.515036364839 0.0115965431559
0.522290398146 0.0118680617121
0.529544431454 0.012151007483
0.536798464761 0.0124461388459
0.544052498069 0.0127542871612
0.551306531376 0.0130763663671
0.558560564684 0.0134133842236
0.565814597992 0.0137664555655
0.573068631299 0.0141368180177
0.580322664607 0.0145258507579
0.587576697914 0.0149350970807
0.594830731222 0.0153662917494
0.60208476453 0.0158213944447
0.609338797837 0.0163026310673
0.616592831145 0.0168125452882
0.623846864452 0.0173540636692
0.63110089776 0.0179305790438
0.638354931067 0.0185460589298
0.645608964375 0.0192051889847
0.652862997683 0.0199135667241
0.66011703099 0.0206779694095
0.667371064298 0.0215067351164
0.674625097605 0.0224103236415
0.681879130913 0.0234021777335
0.689133164221 0.0245001183598
0.696387197528 0.0257287709573
0.703641230836 0.0271242204071
0.710895264143 0.0287443665483
0.718149297451 0.0306987457151


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt4.tex <==
-0.5 0.0234601434715
-0.495 0.0234524350944
-0.49 0.0234299939278
-0.485 0.0233938105277
-0.48 0.0233448298184
-0.475 0.0232839529822
-0.47 0.0232120392859
-0.465 0.0231299078452
-0.46 0.0230383393279
-0.455 0.0229380775985
-0.45 0.022829831306
-0.445 0.0227142754148
-0.44 0.0225920526825
-0.435 0.0224637750844
-0.43 0.0223300251868
-0.425 0.0221913574706
-0.42 0.0220482996065
-0.415 0.0219013536829
-0.41 0.0217509973887
-0.405 0.0215976851513
-0.4 0.0214418492312
-0.395 0.0212839007757
-0.39 0.0211242308312
-0.385 0.0209632113168
-0.38 0.0208011959588
-0.375 0.0206385211892
-0.37 0.0204755070073
-0.365 0.0203124578073
-0.36 0.0201496631716
-0.355 0.0199873986314
-0.35 0.0198259263959
-0.345 0.0196654960505
-0.34 0.019506345225
-0.335 0.0193487002338
-0.33 0.0191927766873
-0.325 0.0190387800764
-0.32 0.0188869063312
-0.315 0.0187373423541
-0.31 0.0185902665282
-0.305 0.0184458492019
-0.3 0.0183042531506
-0.295 0.018165634016
-0.29 0.0180301407236
-0.285 0.0178979158792
-0.28 0.0177690961451
-0.275 0.0176438125967
-0.27 0.0175221910593
-0.265 0.0174043524269
-0.26 0.0172904129624
-0.255 0.0171804845802
-0.25 0.0170746751114
-0.245 0.0169730885529
-0.24 0.0168758252987
-0.235 0.0167829823565
-0.23 0.0166946535478
-0.225 0.0166109296921
-0.22 0.0165318987767
-0.215 0.016457646111
-0.21 0.0163882544655
-0.205 0.0163238041968
-0.2 0.0162643733572
-0.195 0.01621003779
-0.19 0.0161608712102
-0.185 0.0161169452701
-0.18 0.0160783296103
-0.175 0.0160450918962
-0.17 0.0160172978388
-0.165 0.0159950112001
-0.16 0.0159782937835
-0.155 0.0159672054079
-0.15 0.0159618038648
-0.145 0.0159621448602
-0.14 0.015968281937
-0.135 0.0159802663819
-0.13 0.0159981471116
-0.125 0.0160219705413
-0.12 0.0160517804326
-0.115 0.0160876177208
-0.11 0.0161295203203
-0.105 0.0161775229075
-0.1 0.01623165668
-0.095 0.0162919490909
-0.09 0.0163584235571
-0.085 0.0164310991403
-0.08 0.0165099901989
-0.075 0.0165951060106
-0.07 0.0166864503624
-0.065 0.0167840211078
-0.06 0.0168878096887
-0.055 0.0169978006206
-0.05 0.0171139709389
-0.045 0.0172362896046
-0.04 0.0173647168667
-0.035 0.0174992035799
-0.03 0.0176396904754
-0.025 0.0177861073809
-0.02 0.0179383723899
-0.015 0.0180963909751
-0.01 0.0182600550461
-0.005 0.018429241946
0.0 0.018603813387
0.0040455488499 0.0187481435215
0.00809109769979 0.0188943885223
0.0121366465497 0.0190425865365
0.0161821953996 0.0191927767638
0.0202277442495 0.0193449994945
0.0242732930994 0.019499296149
0.0283188419493 0.0196557093197
0.0323643907992 0.0198142828141
0.0364099396491 0.0199750617006
0.040455488499 0.0201380923557
0.0445010373489 0.0203034225145
0.0485465861988 0.0204711013224
0.0525921350487 0.0206411793904
0.0566376838986 0.020813708852
0.0606832327485 0.0209887434244
0.0647287815983 0.0211663384708
0.0687743304482 0.0213465510681
0.0728198792981 0.0215294400759
0.076865428148 0.0217150662107
0.0809109769979 0.0219034921229
0.0849565258478 0.0220947824786
0.0890020746977 0.0222890040454
0.0930476235476 0.0224862257824
0.0970931723975 0.0226865189364
0.101138721247 0.022889957142
0.105184270097 0.023096616528
0.109229818947 0.0233065758296
0.113275367797 0.0235199165076
0.117320916647 0.0237367228734
0.121366465497 0.0239570822223
0.125412014347 0.0241810849743
0.129457563197 0.0244088248233
0.133503112047 0.0246403988958
0.137548660896 0.0248759079189
0.141594209746 0.0251154563989
0.145639758596 0.025359152812
0.149685307446 0.0256071098057
0.153730856296 0.0258594444151
0.157776405146 0.0261162782923
0.161821953996 0.0263777379515
0.165867502846 0.0266439550314
0.169913051696 0.0269150665746
0.173958600546 0.0271912153276
0.178004149395 0.0274725500622
0.182049698245 0.0277592259193
0.186095247095 0.028051404779
0.190140795945 0.0283492556581
0.194186344795 0.0286529551378
0.198231893645 0.0289626878244
0.202277442495 0.0292786468468
0.206322991345 0.0296010343939
0.210368540195 0.0299300622952
0.214414089045 0.0302659526509
0.218459637894 0.0306089385147
0.222505186744 0.0309592646361
0.226550735594 0.0313171882682
0.230596284444 0.0316829800486
0.234641833294 0.0320569249608
0.238687382144 0.0324393233866
0.242732930994 0.0328304922597
0.246778479844 0.0332307663326
0.250824028694 0.033640499571
0.254869577543 0.034060066692
0.258915126393 0.0344898648651
0.262960675243 0.0349303155969
0.267006224093 0.0353818668261
0.271051772943 0.0358449952565
0.275097321793 0.0363202089651
0.279142870643 0.0368080503243
0.283188419493 0.0373090992876
0.287233968343 0.0378239770961
0.291279517193 0.0383533504753
0.295325066042 0.0388979364055
0.299370614892 0.0394585075654
0.303416163742 0.0400358985726
0.307461712592 0.0406310131717
0.311507261442 0.0412448325549
0.315552810292 0.0418784250481
0.319598359142 0.0425329574528
0.323643907992 0.0432097084149
0.327689456842 0.0439100842927
0.331735005692 0.0446356381388
0.335780554541 0.0453880926021
0.339826103391 0.0461693678204
0.343871652241 0.04698161575
0.347917201091 0.0478272629181
0.351962749941 0.0487090643735
0.356008298791 0.0496301728009
0.360053847641 0.050594228603
0.364099396491 0.0516054796788
0.368144945341 0.0526689444661
0.37219049419 0.0537906401498
0.37623604304 0.0549779130514
0.38028159189 0.056239937365
0.38432714074 0.0575885091384
0.38837268959 0.0590394022105
0.39241823844 0.0606149212715
0.39646378729 0.0623494701753
0.40050933614 0.0643052457837


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt5.tex <==
-0.5 0.0325395998849
-0.495 0.032532352819
-0.49 0.032511236032
-0.485 0.0324771572588
-0.48 0.0324309869027
-0.475 0.0323735594678
-0.47 0.032305674947
-0.465 0.0322281001658
-0.46 0.0321415700832
-0.455 0.032046789051
-0.45 0.0319444320333
-0.445 0.0318351457856
-0.44 0.0317195499965
-0.435 0.0315982383917
-0.43 0.0314717798016
-0.425 0.0313407191939
-0.42 0.031205578672
-0.415 0.0310668584398
-0.41 0.0309250377344
-0.405 0.0307805757267
-0.4 0.0306339123923
-0.395 0.0304854693521
-0.39 0.0303356506841
-0.385 0.0301848437072
-0.38 0.0300334197375
-0.375 0.0298817348192
-0.37 0.0297301304283
-0.365 0.0295789341523
-0.36 0.029428460346
-0.355 0.0292790107633
-0.35 0.0291308751659
-0.345 0.0289843319115
-0.34 0.0288396485183
-0.335 0.0286970822113
-0.33 0.0285568804464
-0.325 0.0284192814159
-0.32 0.0282845145357
-0.315 0.0281528009128
-0.31 0.0280243537964
-0.305 0.0278993790109
-0.3 0.0277780753729
-0.295 0.0276606350916
-0.29 0.0275472441539
-0.285 0.0274380826941
-0.28 0.0273333253492
-0.275 0.0272331415999
-0.27 0.0271376960978
-0.265 0.027047148979
-0.26 0.0269616561656
-0.255 0.0268813696537
-0.25 0.0268064377897
-0.245 0.0267370055353
-0.24 0.0266732147199
-0.235 0.0266152042831
-0.23 0.0265631105057
-0.225 0.0265170672309
-0.22 0.0264772060747
-0.215 0.0264436566266
-0.21 0.0264165466414
-0.205 0.0263960022211
-0.2 0.0263821479876
-0.195 0.0263751072474
-0.19 0.0263750021472
-0.185 0.0263819538213
-0.18 0.0263960825313
-0.175 0.0264175077977
-0.17 0.0264463485244
-0.165 0.0264827231151
-0.16 0.0265267495837
-0.155 0.0265785456575
-0.15 0.0266382288735
-0.145 0.0267059166693
-0.14 0.0267817264679
-0.135 0.0268657757565
-0.13 0.0269581821611
-0.125 0.027059063516
-0.12 0.027168537929
-0.115 0.0272867238432
-0.11 0.0274137400961
-0.105 0.027549705976
-0.1 0.0276947412777
-0.095 0.0278489663569
-0.09 0.0280125021861
-0.085 0.0281854704122
-0.08 0.0283679934177
-0.075 0.0285601943864
-0.07 0.0287621973778
-0.065 0.0289741274093
-0.06 0.0291961105519
-0.055 0.0294282740403
-0.05 0.0296707464022
-0.045 0.0299236576114
-0.04 0.0301871392673
-0.035 0.0304613248093
-0.03 0.0307463497711
-0.025 0.0310423520822
-0.02 0.0313494724273
-0.015 0.0316678546718
-0.01 0.0319976463671
-0.005 0.03233899935
0.0 0.0326920704511
0.00275255128608 0.0328907757948
0.00550510257217 0.0330916680619
0.00825765385825 0.0332947851691
0.0110102051443 0.0335001659774
0.0137627564304 0.0337078503237
0.0165153077165 0.0339178790536
0.0192678590026 0.0341302940561
0.0220204102887 0.0343451382994
0.0247729615748 0.0345624558681
0.0275255128608 0.0347822920026
0.0302780641469 0.0350046931398
0.033030615433 0.0352297069562
0.0357831667191 0.0354573824121
0.0385357180052 0.0356877697987
0.0412882692913 0.0359209207868
0.0440408205773 0.0361568884786
0.0467933718634 0.0363957274609
0.0495459231495 0.0366374938615
0.0522984744356 0.0368822454086
0.0550510257217 0.0371300414926
0.0578035770078 0.037380943231
0.0605561282939 0.0376350135373
0.0633086795799 0.0378923171924
0.066061230866 0.0381529209205
0.0688137821521 0.0384168934685
0.0715663334382 0.0386843056901
0.0743188847243 0.0389552306336
0.0770714360104 0.0392297436353
0.0798239872964 0.0395079224179
0.0825765385825 0.0397898471935
0.0853290898686 0.0400756007739
0.0880816411547 0.0403652686859
0.0908341924408 0.0406589392939
0.0935867437269 0.0409567039295
0.0963392950129 0.0412586570292
0.099091846299 0.0415648962799
0.101844397585 0.0418755227733
0.104596948871 0.0421906411708
0.107349500157 0.0425103598773
0.110102051443 0.0428347912275
0.112854602729 0.0431640516835
0.115607154016 0.0434982620459
0.118359705302 0.0438375476785
0.121112256588 0.0441820387491
0.123864807874 0.0445318704858
0.12661735916 0.044887183453
0.129369910446 0.0452481238452
0.132122461732 0.0456148438041
0.134875013018 0.0459875017575
0.137627564304 0.0463662627854
0.14038011559 0.0467512990127
0.143132666876 0.0471427900336
0.145885218162 0.04754092337
0.148637769449 0.0479458949663
0.151390320735 0.0483579097264
0.154142872021 0.0487771820951
0.156895423307 0.0492039366907
0.159647974593 0.0496384089931
0.162400525879 0.0500808460943
0.165153077165 0.0505315075179
0.167905628451 0.0509906661164
0.170658179737 0.0514586090557
0.173410731023 0.051935638896
0.176163282309 0.0524220747847
0.178915833595 0.0529182537717
0.181668384882 0.0534245322673
0.184420936168 0.0539412876595
0.187173487454 0.0544689201151
0.18992603874 0.0550078545907
0.192678590026 0.0555585430852
0.195431141312 0.0561214671712
0.198183692598 0.0566971408504
0.200936243884 0.0572861137867
0.20368879517 0.0578889749817
0.206441346456 0.0585063569716
0.209193897742 0.0591389406419
0.211946449028 0.0597874607793
0.214699000315 0.0604527125079
0.217451551601 0.0611355587962
0.220204102887 0.0618369392681
0.222956654173 0.0625578806189
0.225709205459 0.0632995090227
0.228461756745 0.0640630650385
0.231214308031 0.0648499216881
0.233966859317 0.0656616066088
0.236719410603 0.0664998295211
0.239471961889 0.0673665167387
0.242224513175 0.0682638551795
0.244977064461 0.0691943494693
0.247729615748 0.0701608975228
0.250482167034 0.0711668929459
0.25323471832 0.0722163676928
0.255987269606 0.0733141976103
0.258739820892 0.0744664112086
0.261492372178 0.0756806787875
0.264244923464 0.0769671435293
0.26699747475 0.0783399782161
0.269750026036 0.0798207621553
0.272502577322 0.0814479436577


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt6.tex <==
-0.5 0.0449051370549
-0.495 0.0448984914013
-0.49 0.0448791403218
-0.485 0.0448479380993
-0.48 0.0448057072552
-0.475 0.0447532397166
-0.47 0.0446912979491
-0.465 0.0446206160563
-0.46 0.044541900848
-0.455 0.0444558328756
-0.45 0.0443630674383
-0.445 0.0442642355583
-0.44 0.0441599449284
-0.435 0.0440507808307
-0.43 0.0439373070284
-0.425 0.0438200666312
-0.42 0.0436995829346
-0.415 0.043576360235
-0.41 0.0434508846199
-0.405 0.0433236247347
-0.4 0.0431950325274
-0.395 0.0430655439703
-0.39 0.0429355797609
-0.385 0.0428055460021
-0.38 0.0426758348622
-0.375 0.0425468252152
-0.37 0.0424188832631
-0.365 0.0422923631396
-0.36 0.0421676074963
-0.355 0.0420449480723
-0.35 0.0419247062471
-0.345 0.0418071935785
-0.34 0.041692712325
-0.335 0.0415815559537
-0.33 0.0414740096346
-0.325 0.0413703507216
-0.32 0.0412708492204
-0.315 0.0411757682449
-0.31 0.0410853644617
-0.305 0.0409998885234
-0.3 0.0409195854922
-0.295 0.0408446952531
-0.29 0.0407754529183
-0.285 0.0407120892226
-0.28 0.0406548309113
-0.275 0.0406039011203
-0.27 0.04055951975
-0.265 0.040521903832
-0.26 0.040491267892
-0.255 0.0404678243065
-0.25 0.0404517836559
-0.245 0.0404433550749
-0.24 0.0404427465996
-0.235 0.040450165513
-0.23 0.0404658186899
-0.225 0.0404899129414
-0.22 0.0405226553611
-0.215 0.0405642536722
-0.21 0.0406149165783
-0.205 0.0406748541187
-0.2 0.0407442780279
-0.195 0.0408234021036
-0.19 0.0409124425814
-0.185 0.0410116185201
-0.18 0.0411211521986
-0.175 0.0412412695261
-0.17 0.0413722004674
-0.165 0.0415141794869
-0.16 0.0416674460122
-0.155 0.0418322449213
-0.15 0.0420088270558
-0.145 0.0421974497636
-0.14 0.0423983774758
-0.135 0.0426118823208
-0.13 0.0428382447809
-0.125 0.0430777543979
-0.12 0.0433307105312
-0.115 0.0435974231786
-0.11 0.0438782138638
-0.105 0.044173416603
-0.1 0.0444833789571
-0.095 0.0448084631836
-0.09 0.0451490474991
-0.085 0.0455055274674
-0.08 0.045878317531
-0.075 0.0462678527038
-0.07 0.0466745904476
-0.065 0.0470990127582
-0.06 0.0475416284904
-0.055 0.0480029759558
-0.05 0.0484836258333
-0.045 0.0489841844389
-0.04 0.0495052974093
-0.035 0.0500476538631
-0.03 0.0506119911142
-0.025 0.0511991000293
-0.02 0.0518098311322
-0.015 0.0524451015857
-0.01 0.0531059032017
-0.005 0.0537933116638
0.0 0.0545084971875
0.001583592135 0.0547405136537
0.00316718427 0.0549744957342
0.004750776405 0.0552104718459
0.00633436854001 0.0554484710314
0.00791796067501 0.0556885229783
0.00950155281001 0.0559306580392
0.011085144945 0.0561749072525
0.01266873708 0.0564213023644
0.014252329215 0.0566698758509
0.01583592135 0.0569206609422
0.017419513485 0.0571736916467
0.01900310562 0.0574290027765
0.020586697755 0.0576866299748
0.02217028989 0.0579466097434
0.023753882025 0.0582089794715
0.02533747416 0.058473777467
0.026921066295 0.0587410429876
0.02850465843 0.0590108162746
0.030088250565 0.0592831385871
0.0316718427 0.0595580522394
0.033255434835 0.0598356006384
0.03483902697 0.0601158283238
0.036422619105 0.0603987810105
0.03800621124 0.0606845056321
0.039589803375 0.0609730503875
0.04117339551 0.0612644647891
0.042756987645 0.0615587997144
0.04434057978 0.061856107459
0.045924171915 0.0621564417936
0.04750776405 0.0624598580231
0.049091356185 0.0627664130496
0.05067494832 0.0630761654383
0.052258540455 0.063389175487
0.05384213259 0.0637055053004
0.055425724725 0.064025218867
0.05700931686 0.0643483821423
0.058592908995 0.0646750631353
0.06017650113 0.0650053320008
0.061760093265 0.0653392611375
0.0633436854001 0.0656769252918
0.0649272775351 0.0660184016678
0.0665108696701 0.0663637700446
0.0680944618051 0.066713112901
0.0696780539401 0.0670665155487
0.0712616460751 0.0674240662735
0.0728452382101 0.0677858564867
0.0744288303451 0.0681519808868
0.0760124224801 0.0685225376321
0.0775960146151 0.0688976285264
0.0791796067501 0.069277359217
0.0807631988851 0.0696618394082
0.0823467910201 0.0700511830908
0.0839303831551 0.0704455087886
0.0855139752901 0.070844939825
0.0870975674251 0.0712496046101
0.0886811595601 0.0716596369521
0.0902647516951 0.0720751763937
0.0918483438301 0.072496368578
0.0934319359651 0.0729233656459
0.0950155281001 0.0733563266689
0.0965991202351 0.0737954181214
0.0981827123701 0.0742408143976
0.0997663045051 0.0746926983773
0.10134989664 0.075151262048
0.102933488775 0.0756167071894
0.10451708091 0.0760892461289
0.106100673045 0.0765691025783
0.10768426518 0.0770565125619
0.109267857315 0.0775517254489
0.11085144945 0.078055005108
0.112435041585 0.078566631199
0.11401863372 0.0790869006261
0.115602225855 0.079616129178
0.11718581799 0.080154653386
0.118769410125 0.0807028326394
0.12035300226 0.0812610516041
0.121936594395 0.081829723002
0.12352018653 0.0824092908234
0.125103778665 0.0830002340601
0.1266873708 0.0836030710735
0.128270962935 0.08421836474
0.12985455507 0.0848467285599
0.131438147205 0.0854888339714
0.13302173934 0.0861454191898
0.134605331475 0.086817300002
0.13618892361 0.0875053831043
0.137772515745 0.0882106827994
0.13935610788 0.0889343422161
0.140939700015 0.0896776607422
0.14252329215 0.0904421302023
0.144106884285 0.0912294836963
0.14569047642 0.0920417633837
0.147274068555 0.0928814177883
0.14885766069 0.0937514474165
0.150441252825 0.0946556345539
0.15202484496 0.0955989322035
0.153608437095 0.0965881897149
0.15519202923 0.0976337204033
0.156775621365 0.0987536749614


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt8.tex <==
-0.5 0.0852206031035
-0.495527864045 0.0852171448302
-0.49105572809 0.0852071622872
-0.486583592135 0.0851912326502
-0.48211145618 0.0851699185346
-0.477639320225 0.0851437685197
-0.47316718427 0.0851133176647
-0.468695048315 0.0850790880155
-0.46422291236 0.0850415891041
-0.459750776405 0.0850013184403
-0.45527864045 0.0849587619956
-0.450806504495 0.0849143946809
-0.44633436854 0.0848686808174
-0.441862232585 0.0848220746014
-0.43739009663 0.084775020564
-0.432917960675 0.0847279540248
-0.42844582472 0.0846813015418
-0.423973688765 0.0846354813565
-0.41950155281 0.0845909038357
-0.415029416855 0.0845479719095
-0.4105572809 0.0845070815069
-0.406085144945 0.0844686219895
-0.40161300899 0.0844329765832
-0.397140873035 0.0844005228091
-0.39266873708 0.0843716329138
-0.388196601125 0.0843466743002
-0.38372446517 0.0843260099596
-0.379252329215 0.0843099989043
-0.37478019326 0.0842989966043
-0.370308057305 0.0842933554259
-0.36583592135 0.0842934250754
-0.361363785395 0.0842995530471
-0.35689164944 0.0843120850781
-0.352419513485 0.0843313656099
-0.34794737753 0.084357738258
-0.343475241575 0.0843915462916
-0.33900310562 0.0844331331239
-0.334530969665 0.0844828428139
-0.33005883371 0.0845410205837
-0.325586697755 0.084608013349
-0.3211145618 0.0846841702691
-0.316642425845 0.0847698433146
-0.31217028989 0.0848653878571
-0.307698153935 0.0849711632828
-0.30322601798 0.0850875336319
-0.298753882025 0.0852148682683
-0.29428174607 0.0853535425801
-0.289809610115 0.0855039387171
-0.28533747416 0.0856664463677
-0.280865338205 0.0858414635787
-0.27639320225 0.086029397625
-0.271921066295 0.0862306659316
-0.26744893034 0.0864456970559
-0.262976794385 0.0866749317358
-0.25850465843 0.0869188240107
-0.254032522475 0.0871778424241
-0.24956038652 0.0874524713162
-0.245088250565 0.0877432122181
-0.24061611461 0.0880505853575
-0.236143978655 0.0883751312909
-0.2316718427 0.0887174126755
-0.227199706745 0.0890780162001
-0.22272757079 0.0894575546926
-0.218255434835 0.0898566694279
-0.21378329888 0.0902760326619
-0.209311162925 0.0907163504207
-0.20483902697 0.0911783655817
-0.200366891015 0.0916628612847
-0.19589475506 0.0921706647222
-0.191422619105 0.092702651364
-0.18695048315 0.093259749681
-0.182478347195 0.0938429464471
-0.17800621124 0.094453292711
-0.173534075285 0.0950919105499
-0.16906193933 0.0957600007376
-0.164589803375 0.0964588514916
-0.16011766742 0.0971898484954
-0.155645531465 0.0979544864418
-0.15117339551 0.0987543823992
-0.146701259555 0.0995912913802
-0.1422291236 0.10046712459
-0.137756987645 0.101383970963
-0.13328485169 0.102344122778
-0.128812715735 0.103350106374
-0.12434057978 0.104404719318
-0.119868443825 0.105511075859
-0.11539630787 0.106672663141
-0.110924171915 0.107893411635
-0.10645203596 0.109177784693
-0.101979900005 0.11053089436
-0.09750776405 0.11195865411
-0.093035628095 0.113467984976
-0.08856349214 0.11506710148
-0.084091356185 0.11676592172
-0.07961922023 0.118576680323
-0.075147084275 0.120514894188
-0.07067494832 0.122600993828
-0.066202812365 0.124863359653
-0.06173067641 0.12734486272
-0.057258540455 0.130121048943


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5equalAreas.tex <==
-0.5 0.0325395998849
-0.49501 0.0325271248953
-0.49002 0.0324903225052
-0.48503 0.0324301010943
-0.48004 0.0323473366933
-0.47505 0.0322428749138
-0.47006 0.0321175327517
-0.46507 0.031972100273
-0.46008 0.0318073421887
-0.45509 0.0316239993296
-0.4501 0.031422790025
-0.44511 0.0312044113946
-0.44012 0.0309695405575
-0.43513 0.030718835765
-0.43014 0.0304529374632
-0.42515 0.0301724692875
-0.42016 0.0298780389965
-0.41517 0.0295702393477
-0.41018 0.0292496489185
-0.40519 0.0289168328772
-0.4002 0.0285723437066
-0.39521 0.0282167218831
-0.39022 0.0278504965145
-0.38523 0.0274741859386
-0.38024 0.0270882982858
-0.37525 0.0266933320074
-0.37026 0.0262897763715
-0.36527 0.025878111929
-0.36028 0.0254588109518
-0.35529 0.0250323378435
-0.3503 0.0245991495261
-0.34531 0.0241596958027
-0.34032 0.0237144196983
-0.33533 0.0232637577799
-0.33034 0.0228081404572
-0.32535 0.0223479922645
-0.32036 0.0218837321263
-0.31537 0.0214157736053
-0.31038 0.0209445251365
-0.30539 0.0204703902457
-0.3004 0.0199937677556
-0.29541 0.0195150519777
-0.29042 0.0190346328938
-0.28543 0.0185528963248
-0.28044 0.0180702240898
-0.27545 0.0175869941547
-0.27046 0.017103580771
-0.26547 0.0166203546067
-0.26048 0.0161376828682
-0.25549 0.0156559294138
-0.2505 0.015175454861
-0.24551 0.0146966166857
-0.24052 0.0142197693157
-0.23553 0.013745264217
-0.23054 0.0132734499757
-0.22555 0.0128046723728
-0.22056 0.0123392744555
-0.21557 0.0118775966022
-0.21058 0.0114199765841
-0.20559 0.0109667496221
-0.2006 0.0105182484395
-0.19561 0.0100748033114
-0.19062 0.00963674211043
-0.18563 0.00920439034909
-0.18064 0.00877807121919
-0.17565 0.00835810562837
-0.17066 0.00794481223393
-0.16567 0.0075385074742
-0.16068 0.00713950559753
-0.15569 0.00674811868916
-0.1507 0.00636465669606
-0.14571 0.00598942744987
-0.14072 0.00562273668813
-0.13573 0.00526488807386
-0.13074 0.00491618321367
-0.12575 0.00457692167447
-0.12076 0.00424740099893
-0.11577 0.00392791671971
-0.11078 0.00361876237264
-0.10579 0.00332022950894
-0.1008 0.00303260770644
-0.09581 0.00275618458005
-0.09082 0.00249124579142
-0.08583 0.00223807505797
-0.08084 0.00199695416121
-0.07585 0.00176816295455
-0.07086 0.00155197937066
-0.06587 0.00134867942823
-0.06088 0.00115853723848
-0.05589 0.000981825011233
-0.0509 0.000818813060701
-0.04591 0.000669769810997
-0.04092 0.000534961801418
-0.03593 0.000414653691538
-0.03094 0.000309108266132
-0.02595 0.000218586439968
-0.02096 0.000143347262501
-0.01597 8.36479224892e-05
-0.01098 3.97437525512e-05
-0.00599 1.18882337026e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5equalSides.tex <==
-0.5 0.0555555555556
-0.49501 0.0549576285556
-0.49002 0.0543426805787
-0.48503 0.053711649361
-0.48004 0.0530654464779
-0.47505 0.0524049581703
-0.47006 0.0517310461405
-0.46507 0.0510445483209
-0.46008 0.0503462796151
-0.45509 0.0496370326124
-0.4501 0.0489175782782
-0.44511 0.0481886666193
-0.44012 0.0474510273267
-0.43513 0.0467053703962
-0.43014 0.0459523867271
-0.42515 0.0451927487009
-0.42016 0.0444271107396
-0.41517 0.0436561098458
-0.41018 0.0428803661238
-0.40519 0.0421004832835
-0.4002 0.0413170491272
-0.39521 0.0405306360201
-0.39022 0.0397418013453
-0.38523 0.0389510879435
-0.38024 0.0381590245382
-0.37525 0.037366126147
-0.37026 0.0365728944793
-0.36527 0.035779818321
-0.36028 0.034987373907
-0.35529 0.0341960252809
-0.3503 0.0334062246439
-0.34531 0.0326184126924
-0.34032 0.0318330189437
-0.33533 0.031050462053
-0.33034 0.0302711501189
-0.32535 0.0294954809801
-0.32036 0.0287238425023
-0.31537 0.0279566128564
-0.31038 0.0271941607874
-0.30539 0.0264368458759
-0.3004 0.0256850187905
-0.29541 0.024939021533
-0.29042 0.0241991876756
-0.28543 0.0234658425916
-0.28044 0.0227393036777
-0.27545 0.0220198805712
-0.27046 0.0213078753588
-0.26547 0.0206035827809
-0.26048 0.0199072904282
-0.25549 0.0192192789331
-0.2505 0.0185398221558
-0.24551 0.0178691873636
-0.24052 0.0172076354063
-0.23553 0.0165554208851
-0.23054 0.0159127923176
-0.22555 0.0152799922973
-0.22056 0.0146572576485
-0.21557 0.0140448195769
-0.21058 0.0134429038156
-0.20559 0.0128517307671
-0.2006 0.0122715156407
-0.19561 0.0117024685867
-0.19062 0.011144794826
-0.18563 0.0105986947764
-0.18064 0.0100643641752
-0.17565 0.0095419941985
-0.17066 0.0090317715766
-0.16567 0.00853387870672
-0.16068 0.0080484937622
-0.15569 0.00757579079878
-0.1507 0.00711593985783
-0.14571 0.00666910706674
-0.14072 0.00623545473651
-0.13573 0.00581514145661
-0.13074 0.00540832218731
-0.12575 0.00501514834931
-0.12076 0.00463576791108
-0.11577 0.00427032547368
-0.11078 0.00391896235333
-0.10579 0.00358181666174
-0.1008 0.00325902338422
-0.09581 0.0029507144557
-0.09082 0.00265701883471
-0.08583 0.00237806257538
-0.08084 0.00211396889746
-0.07585 0.00186485825455
-0.07086 0.00163084840043
-0.06587 0.00141205445371
-0.06088 0.00120858896069
-0.05589 0.00102056195663
-0.0509 0.000848081025347
-0.04591 0.000691251357327
-0.04092 0.000550175806224
-0.03593 0.000424954943955
-0.03094 0.000315687114333
-0.02595 0.000222468485315
-0.02096 0.000145393099901
-0.01597 8.45529257169e-05
-0.01098 4.00379033271e-05
-0.00599 1.19359933043e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceA0pt5B1pt5levelSets.tex <==
-0.5 0.180555555556
-0.49501 0.18045642652
-0.49002 0.180166279471
-0.48503 0.179695586175
-0.48004 0.179054324186
-0.47505 0.178252004682
-0.47006 0.177297698473
-0.46507 0.176200060344
-0.46008 0.174967351824
-0.45509 0.173607462522
-0.4501 0.172127930113
-0.44511 0.170535959091
-0.44012 0.168838438348
-0.43513 0.167041957692
-0.43014 0.165152823357
-0.42515 0.163177072579
-0.42016 0.161120487306
-0.41517 0.158988607095
-0.41018 0.15678674126
-0.40519 0.154519980304
-0.4002 0.1521932067
-0.39521 0.149811105053
-0.39022 0.147378171687
-0.38523 0.144898723693
-0.38024 0.142376907472
-0.37525 0.139816706805
-0.37026 0.137221950481
-0.36527 0.13459631951
-0.36028 0.131943353948
-0.35529 0.12926645935
-0.3503 0.126568912888
-0.34531 0.123853869138
-0.34032 0.121124365573
-0.33533 0.118383327762
-0.33034 0.115633574306
-0.32535 0.11287782152
-0.32036 0.110118687873
-0.31537 0.107358698212
-0.31038 0.104600287767
-0.30539 0.101845805964
-0.3004 0.0990975200379
-0.29541 0.0963576184836
-0.29042 0.0936282143268
-0.28543 0.0909113482433
-0.28044 0.0882089915256
-0.27545 0.0855230489096
-0.27046 0.0828553612665
-0.26547 0.0802077081692
-0.26048 0.0775818103375
-0.25549 0.074979331971
-0.2505 0.0724018829742
-0.24551 0.0698510210792
-0.24052 0.067328253873
-0.23553 0.0648350407321
-0.23054 0.0623727946708
-0.22555 0.0599428841075
-0.22056 0.0575466345518
-0.21557 0.0551853302184
-0.21058 0.0528602155693
-0.20559 0.0505724967901
-0.2006 0.0483233432017
-0.19561 0.0461138886121
-0.19062 0.0439452326098
-0.18563 0.0418184418027
-0.18064 0.0397345510055
-0.17565 0.0376945643761
-0.17066 0.0356994565056
-0.16567 0.0337501734631
-0.16068 0.0318476337972
-0.15569 0.0299927294968
-0.1507 0.0281863269131
-0.14571 0.0264292676437
-0.14072 0.0247223693819
-0.13573 0.0230664267314
-0.13074 0.0214622119895
-0.12575 0.0199104758988
-0.12076 0.018411948369
-0.11577 0.016967339172
-0.11078 0.0155773386083
-0.10579 0.0142426181489
-0.1008 0.0129638310518
-0.09581 0.0117416129558
-0.09082 0.0105765824512
-0.08583 0.0094693416285
-0.08084 0.00842047660799
-0.07585 0.007430558048
-0.07086 0.0065001416352
-0.06587 0.00562976855655
-0.06088 0.00481996595385
-0.05589 0.00407124736181
-0.0509 0.00338411313013
-0.04591 0.00275905083033
-0.04092 0.002196535648
-0.03593 0.00169703076093
-0.03094 0.0012609877039
-0.02595 0.000888846720458
-0.02096 0.00058103710238
-0.01597 0.000337977517188
-0.01098 0.00016007632428
-0.00599 4.77318800925e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularEqualAreas.tex <==
-0.450442616461 0.0582998243664
-0.449561731229 0.0579839015579
-0.448680845996 0.0579005571713
-0.447799960763 0.0578157053666
-0.44691907553 0.0577296835335
-0.446038190297 0.0574087522934
-0.445157305064 0.0573210582147
-0.444276419831 0.0572326209376
-0.443395534598 0.0569104249306
-0.442514649365 0.0568208619054
-0.441633764132 0.0567307436728
-0.440752878899 0.0564078801507
-0.439871993666 0.0563169260519
-0.438991108433 0.0562255291476
-0.438110223201 0.0559023557026
-0.437229337968 0.0558103107638
-0.436348452735 0.0557178999941
-0.435467567502 0.0553946637433
-0.434586682269 0.0553017397487
-0.433705797036 0.0552085069128
-0.432824911803 0.0548853929078
-0.43194402657 0.0547917498667
-0.431063141337 0.0546978423782
-0.430182256104 0.0543749965519
-0.429301370871 0.0542807610059
-0.428420485638 0.0539583552082
-0.427539600405 0.0538638385338
-0.426658715173 0.0537691138772
-0.42577782994 0.0534471654643
-0.424896944707 0.0533522197334
-0.424016059474 0.0532570925427
-0.423135174241 0.0529356917285
-0.422254289008 0.0528403946525
-0.421373403775 0.0527449388171
-0.420492518542 0.0524241638191
-0.419611633309 0.052328582423
-0.418730748076 0.0520084616255
-0.417849862843 0.0519127815757
-0.41696897761 0.0518169744425
-0.416088092377 0.0514975909307
-0.415207207145 0.0514017209627
-0.414326321912 0.0513057398645
-0.413445436679 0.0509871505309
-0.412564551446 0.0508911385476
-0.411683666213 0.0505733088942
-0.41080278098 0.0504772859115
-0.409921895747 0.0503811748732
-0.409041010514 0.0500642235227
-0.408160125281 0.0499681283426
-0.407279240048 0.0498719570545
-0.406398354815 0.0495559280912
-0.405517469582 0.0494597970825
-0.404636584349 0.0491446100388
-0.403755699117 0.0490485347832
-0.402874813884 0.0489524011253
-0.401993928651 0.0486382033149
-0.401113043418 0.048542146493
-0.400232158185 0.0482288341786
-0.399351272952 0.0481328676714
-0.398470387719 0.0480368580525
-0.397589502486 0.0477245939588
-0.396708617253 0.0476286930869
-0.39582773202 0.0473173533155
-0.394946846787 0.0472215730668
-0.394065961554 0.0471257630643
-0.393185076321 0.0468155241593
-0.392304191089 0.0467198510649
-0.391423305856 0.0464105714312
-0.390542420623 0.04631504581
-0.38966153539 0.0462195022176
-0.388780650157 0.0459113708818
-0.387899764924 0.045815989278
-0.387018879691 0.0455088489429
-0.386137994458 0.0454136388033
-0.385257109225 0.0453184211709
-0.384376223992 0.0450124722094
-0.383495338759 0.0449174390774
-0.382614453526 0.0446125101335
-0.381733568293 0.0445176700599
-0.380852683061 0.0444228318776
-0.379971797828 0.0441191336951
-0.379090912595 0.0440245003557
-0.378210027362 0.0437218488928
-0.377329142129 0.0436274281726
-0.376448256896 0.0435330177991
-0.375567371663 0.0432316333262
-0.37468648643 0.0431374462855
-0.373805601197 0.042837133237
-0.372924715964 0.042743176633
-0.372043830731 0.0424439447799
-0.371162945498 0.0423502254707
-0.370282060265 0.0422565270983
-0.369401175033 0.0419586089236
-0.3685202898 0.0418651572966
-0.367639404567 0.0415683426384
-0.366758519334 0.0414751440622
-0.365877634101 0.0411794418073
-0.364996748868 0.0410865023836
-0.364115863635 0.0409935932011
-0.363234978402 0.0406992468269
-0.362354093169 0.0406066052028
-0.361473207936 0.0403133915556
-0.360592322703 0.0402210231305
-0.35971143747 0.0401286908864
-0.358830552237 0.0398368605929
-0.357949667005 0.0397448093149
-0.357068781772 0.0394541308395
-0.356187896539 0.03936236576
-0.355307011306 0.0390728467772
-0.354426126073 0.038981372976
-0.35354524084 0.0388899429399
-0.352664355607 0.0386018433957
-0.351783470374 0.038510711627
-0.350902585141 0.0382237891437
-0.350021699908 0.0381329603744
-0.349140814675 0.0378472220488
-0.348259929442 0.0377567008806
-0.347379044209 0.0376662302649
-0.346498158977 0.0373819445656
-0.345617273744 0.0372917878748
-0.344736388511 0.0370087025815
-0.343855503278 0.0369188641184
-0.342974618045 0.0366369858234
-0.342093732812 0.0365474697776
-0.341212847579 0.0364580103897
-0.340331962346 0.0361776153913
-0.339451077113 0.0360884841709
-0.33857019188 0.0358093112638
-0.337689306647 0.0357205121411
-0.336808421414 0.0354425674735
-0.335927536181 0.0353541042803
-0.335046650949 0.0350773938804
-0.334165765716 0.034989270354
-0.333284880483 0.0349012105167
-0.33240399525 0.0346260199208
-0.331523110017 0.034538304869
-0.330642224784 0.0342643623391
-0.329761339551 0.0341769955914
-0.328880454318 0.0339043067739
-0.327999569085 0.0338172917655
-0.327118683852 0.033730345317
-0.326237798619 0.0334592022891
-0.325356913386 0.0333726122771
-0.324476028153 0.0331027358813
-0.323595142921 0.0330165055482
-0.322714257688 0.0327479010889
-0.321833372455 0.0326620336032
-0.320952487222 0.0323947062911
-0.320071601989 0.0323092047499
-0.319190716756 0.032223777436
-0.318309831523 0.0319580271366
-0.31742894629 0.0318729699922
-0.316548061057 0.031608508756
-0.315667175824 0.0315238247127
-0.314786290591 0.0312606574507
-0.313905405358 0.0311763493763
-0.313024520125 0.0309144809168
-0.312143634893 0.0308305516174
-0.31126274966 0.0307467016017
-0.310381864427 0.0304864389304
-0.309500979194 0.0304029715083
-0.308620093961 0.0301440186735
-0.307739208728 0.0300609365076
-0.306858323495 0.0298032980724
-0.305977438262 0.0297206037699
-0.305096553029 0.0294642842237
-0.304215667796 0.0293819803383
-0.303334782563 0.029126984099
-0.30245389733 0.0290450731317
-0.301573012097 0.0289632469441
-0.300692126865 0.0287098889489
-0.299811241632 0.0286284590721
-0.298930356399 0.0283764344707
-0.298049471166 0.0282954032845
-0.297168585933 0.0280447162638
-0.2962877007 0.0279640861006
-0.295406815467 0.0277147407831
-0.294525930234 0.0276345139292
-0.293645045001 0.0275543758383
-0.292764159768 0.0273066930718
-0.291883274535 0.0272269613832
-0.291002389302 0.0269806297249
-0.290121504069 0.026901306618
-0.289240618837 0.0266563299823
-0.288359733604 0.0265774175948
-0.287478848371 0.0263337998382
-0.286597963138 0.0262553002669
-0.285717077905 0.0260130451887
-0.284836192672 0.0259349604909
-0.283955307439 0.0258569689265
-0.283074422206 0.0256164040292
-0.282193536973 0.0255388301117
-0.28131265174 0.0252996365516
-0.280431766507 0.0252224822461
-0.279550881274 0.0249846636381
-0.278669996041 0.0249079308732
-0.277789110809 0.0246714907804
-0.276908225576 0.0245951814493
-0.276027340343 0.0243601233838
-0.27514645511 0.0242842393453
-0.274265569877 0.0240505667693
-0.273384684644 0.0239751098486
-0.272503799411 0.0238997506106
-0.271622914178 0.0236677981647
-0.270742028945 0.023592868495
-0.269861143712 0.0233623094192
-0.268980258479 0.0232878110644
-0.268099373246 0.0230586486592
-0.267218488013 0.022984583335
-0.266337602781 0.0227568208548
-0.265456717548 0.0226831902468
-0.264575832315 0.0224568309012
-0.263694947082 0.0223836366653
-0.262814061849 0.0221586836196
-0.261933176616 0.0220859273828
-0.261052291383 0.0220132727989
-0.26017140615 0.0217900671202
-0.259290520917 0.0217178527108
-0.258409635684 0.0214960605279
-0.257528750451 0.0214242878529
-0.256647865218 0.0212039121876
-0.255766979985 0.0211325827798
-0.254886094753 0.0209136266131
-0.25400520952 0.0208427419795
-0.253124324287 0.0206252082522
-0.252243439054 0.0205547698742
-0.251362553821 0.0203386614874
-0.250481668588 0.0202686708212
-0.249600783355 0.0201987852877
-0.248719898122 0.0199844491148
-0.247839012889 0.0199150132321
-0.246958127656 0.0197021089869
-0.246077242423 0.0196331241529
-0.24519635719 0.0194216546082
-0.244315471957 0.0193531221977
-0.243434586725 0.0191430900895
-0.242553701492 0.0190750114545
-0.241672816259 0.0188664194826
-0.240791931026 0.0187987959525
-0.239911045793 0.018591646781
-0.23903016056 0.0185244796638
-0.238149275327 0.0183187759217
-0.237268390094 0.0182520665035
-0.236387504861 0.0181854657271
-0.235506619628 0.0179815603313
-0.234625734395 0.0179154189583
-0.233744849162 0.0177129649523
-0.232863963929 0.0176472842191
-0.231983078697 0.0174462841175
-0.231102193464 0.0173810652404
-0.230221308231 0.0171815215253
-0.229340422998 0.017116765701
-0.228459537765 0.0169186808217
-0.227578652532 0.0168543892277
-0.226697767299 0.0166577656017
-0.225816882066 0.0165939393964
-0.224935996833 0.0163987794098
-0.2240551116 0.016335419733
-0.223174226367 0.0161417257406
-0.222293341134 0.0160788337142
-0.221412455901 0.0160160537504
-0.220531570669 0.0158241847679
-0.219650685436 0.0157618739327
-0.218769800203 0.0155714762742
-0.21788891497 0.0155096356468
-0.217008029737 0.0153207115661
-0.216127144504 0.0152593422088
-0.215246259271 0.0150718939302
-0.214365374038 0.0150109968884
-0.213484488805 0.0148250266073
-0.212603603572 0.0147646029099
-0.211722718339 0.0145801127932
-0.210841833106 0.0145201634528
-0.209960947873 0.0143371556391
-0.209080062641 0.0142776816524
-0.208199177408 0.0140961582524
-0.207318292175 0.0140371606005
-0.206437406942 0.0138571236975
-0.205556521709 0.0137986033458
-0.204675636476 0.0137401982947
-0.203794751243 0.013562012895
-0.20291386601 0.013504086409
-0.202032980777 0.0133273922126
-0.201152095544 0.0132699452216
-0.200271210311 0.0130947442222
-0.199390325078 0.0130377776414
-0.198509439846 0.0128640718065
-0.197628554613 0.0128075865368
-0.19674766938 0.0126353778083
-0.195866784147 0.0125793747365
-0.194985898914 0.0124086650306
-0.194105013681 0.0123531450297
-0.193224128448 0.0121839362374
-0.192343243215 0.0121289001666
-0.191462357982 0.011961194154
-0.190581472749 0.0119066428592
-0.189700587516 0.0117404414677
-0.188819702283 0.0116863757816
-0.18793881705 0.0115216808281
-0.187057931818 0.0114681015702
-0.186177046585 0.011414640597
-0.185296161352 0.0112518228248
-0.184415276119 0.0111988493465
-0.183534390886 0.0110375421083
-0.182653505653 0.0109850569143
-0.18177262042 0.0108252619477
-0.180891735187 0.010773265815
-0.180010849954 0.0106149848343
-0.179129964721 0.0105634785279
-0.178249079488 0.0104067132242
-0.177368194255 0.0103556974968
-0.176487309022 0.0102004495386
-0.17560642379 0.0101499251312
-0.174725538557 0.00999619616413
-0.173844653324 0.00994616380614
-0.172963768091 0.0097939554536
-0.172082882858 0.0097444158628
-0.171201997625 0.00959372972599
-0.170321112392 0.00954468360885
-0.169440227159 0.00939552126703
-0.168559341926 0.00934696931883
-0.167678456693 0.00919933232949
-0.16679757146 0.00915127523446
-0.165916686227 0.00910333910415
-0.165035800994 0.00895760356506
-0.164154915762 0.00891016317228
-0.163274030529 0.00876595648782
-0.162393145296 0.00871901249133
-0.161512260063 0.00857633614819
-0.16063137483 0.0085298891962
-0.159750489597 0.0083887446602
-0.158869604364 0.00834279539052
-0.157988719131 0.00820318410677
-0.157107833898 0.00815773314693
-0.156226948665 0.00801965654001
-0.155346063432 0.00797470450742
-0.154465178199 0.00783816398157
-0.153584292966 0.00779371148363
-0.152703407734 0.0076587084229
-0.151822522501 0.00761475605711
-0.150941637268 0.00748129182556
-0.150060752035 0.00743784017968
-0.149179866802 0.00730591612152
-0.148298981569 0.00726296577364
-0.147418096336 0.0071325832134
-0.146537211103 0.0070901347321
-0.14565632587 0.0069612949748
-0.144775440637 0.00691934891924
-0.143894555404 0.00687752617066
-0.143013670171 0.00675061017056
-0.142132784938 0.00670929056516
-0.141251899706 0.00658392029317
-0.140371014473 0.00654310436846
-0.13949012924 0.006419281066
-0.138609244007 0.00637896935045
-0.137728358774 0.00625669424009
-0.136847473541 0.00621688725324
-0.135966588308 0.00609616153882
-0.135085703075 0.00605685979136
-0.134204817842 0.00593768465814
-0.133323932609 0.00589888865202
-0.132443047376 0.00578126526681
-0.131562162143 0.00574297549535
-0.13068127691 0.00562690500664
-0.129800391678 0.00558912195459
-0.128919506445 0.00547460549267
-0.128038621212 0.00543732963634
-0.127157735979 0.00532436831344
-0.126276850746 0.00528760012075
-0.125395965513 0.00517619503118
-0.12451508028 0.00513993496177
-0.123634195047 0.005030087182
-0.122753309814 0.00499433568732
-0.121872424581 0.00488604627612
-0.120991539348 0.0048508037995
-0.120110654115 0.00474407379807
-0.119229768882 0.0047093407748
-0.11834888365 0.00460417120686
-0.117467998417 0.00456994806428
-0.116587113184 0.00453585046721
-0.115706227951 0.00443262709375
-0.114825342718 0.00439903992077
-0.113944457485 0.00429737926399
-0.113063572252 0.0042643029242
-0.112182687019 0.00416420595089
-0.111301801786 0.00413164084572
-0.110420916553 0.00403310850564
-0.10954003132 0.00400105502889
-0.108659146087 0.00390408825489
-0.107778260854 0.00387254679282
-0.106897375622 0.00377714650097
-0.106016490389 0.00374611743231
-0.105135605156 0.00365228452197
-0.104254719923 0.00362176821808
-0.10337383469 0.00352950357197
-0.102492949457 0.00349950039681
-0.101612064224 0.00340880488116
-0.100731178991 0.00337931519143
-0.0998502937581 0.00329018965601
-0.0989694085252 0.00326121380116
-0.0980885232923 0.00317365907941
-0.0972076380594 0.00314519740171
-0.0963267528264 0.00305921431081
-0.0954458675935 0.00303126714543
-0.0945649823606 0.00294685648638
-0.0936840971277 0.00291942416144
-0.0928032118948 0.00283658671913
-0.0919223266618 0.00280966955573
-0.0910414414289 0.00272840609907
-0.090160556196 0.00270200441137
-0.0892796709631 0.00262231569329
-0.0883987857301 0.00259642978856
-0.0875179004972 0.00251831654617
-0.0866370152643 0.00249294672483
-0.0857561300314 0.00246770425496
-0.0848752447984 0.00239155623511
-0.0839943595655 0.00236683022643
-0.0831134743326 0.00229225931186
-0.0822325890997 0.00226805004921
-0.0813517038668 0.00219505692522
-0.0804708186338 0.00217136468674
-0.0795899334009 0.00209995002309
-0.078709048168 0.0020767750803
-0.0778281629351 0.00200693953126
-0.0769472777021 0.00198428214909
-0.0760663924692 0.0019160263535
-0.0751855072363 0.00189388679035
-0.0743046220034 0.0018272113717
-0.0734237367704 0.00180558987946
-0.0725428515375 0.00174049544593
-0.0716619663046 0.00171939227004
-0.0707810810717 0.00165587941458
-0.0699001958388 0.00163529479405
-0.0690193106058 0.00157336409443
-0.0681384253729 0.00155329826189
-0.06725754014 0.00149295028074
-0.0663766549071 0.00147340346249
-0.0654957696741 0.00141463874737
-0.0646148844412 0.0013956111634
-0.0637339992083 0.00133843024686
-0.0628531139754 0.00131992211088
-0.0619722287425 0.00126432551049
-0.0610913435095 0.00124633702999
-0.0602104582766 0.00119232524841
-0.0593295730437 0.00117485662464
-0.0584486878108 0.00112243014966
-0.0575678025778 0.00110548157773
-0.0566869173449 0.0010546408823
-0.055806032112 0.00103821255118
-0.0549251468791 0.000988958093485
-0.0540442616461 0.000973050186007
-0.0531633764132 0.000925382409497
-0.0522824911803 0.000909995102428
-0.0514016059474 0.000894736423917
-0.0505207207145 0.000849047899899
-0.0496398354815 0.00083431004002
-0.0487589502486 0.000790209157196
-0.0478780650157 0.000775992278877
-0.0469971797828 0.000733479432477
-0.0461162945498 0.000719783692655
-0.0452354093169 0.000678859263346
-0.044354524084 0.000665684812992
-0.0434736388511 0.000626349166911
-0.0425927536181 0.00061369615105
-0.0417118683852 0.000575949639841
-0.0408309831523 0.00056381819758
-0.0399500979194 0.000527661158425
-0.0390692126865 0.00051605142297
-0.0381883274535 0.000481484178621
-0.0373074422206 0.000470396277297
-0.0364265569877 0.000437419136107
-0.0355456717548 0.000426853190383
-0.0346647865218 0.000395466446333
-0.0337839012889 0.000385422571835
-0.032903016056 0.000355626504561
-0.0320221308231 0.000346104811092
-0.0311412455901 0.000317899685913
-0.0302603603572 0.000308900277471
-0.0293794751243 0.000282286345411
-0.0284985898914 0.000273809320202
-0.0276177046585 0.000248786818016
-0.0267368194255 0.000240832268473
-0.0258559341926 0.000217401418666
-0.0249750489597 0.000209969431459
-0.0240941637268 0.000188130442307
-0.0232132784938 0.000181221098359
-0.0223323932609 0.000160974163931
-0.021451508028 0.000154587538429
-0.0205706227951 0.000135932838603
-0.0196897375622 0.00013006900101
-0.0188088523292 0.000113006701486
-0.0179279670963 0.000107665715554
-0.0170470818634 9.2195967874e-05
-0.0161661966305 8.73778916484e-05
-0.0152853113975 7.35008332104e-05
-0.0144044261646 6.92057190432e-05
-0.0135235409317 6.50398791563e-05
-0.0126426556988 5.31493676672e-05
-0.0117617704658 4.95065486174e-05
-0.0108808852329 3.9208987648e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularEqualSides.tex <==
-0.450442616461 0.062598021111
-0.449561731229 0.0623963165375
-0.448680845996 0.0621923022804
-0.447799960763 0.0619869529256
-0.44691907553 0.0617806193854
-0.446038190297 0.06157350596
-0.445157305064 0.0613657514445
-0.444276419831 0.0611574584025
-0.443395534598 0.0609487068038
-0.442514649365 0.0607395613814
-0.441633764132 0.0605300760049
-0.440752878899 0.0603202964691
-0.439871993666 0.0601102623689
-0.438991108433 0.0599000084128
-0.438110223201 0.0596895653757
-0.437229337968 0.0594789608085
-0.436348452735 0.0592682195794
-0.435467567502 0.0590573642953
-0.434586682269 0.0588464156351
-0.433705797036 0.0586353926179
-0.432824911803 0.0584243128209
-0.43194402657 0.0582131925588
-0.431063141337 0.0580020470342
-0.430182256104 0.057790890462
-0.429301370871 0.057579736177
-0.428420485638 0.0573685967238
-0.427539600405 0.0571574839357
-0.426658715173 0.0569464090016
-0.42577782994 0.0567353825253
-0.424896944707 0.0565244145769
-0.424016059474 0.0563135147378
-0.423135174241 0.056102692141
-0.422254289008 0.0558919555065
-0.421373403775 0.055681313173
-0.420492518542 0.055470773126
-0.419611633309 0.0552603430233
-0.418730748076 0.0550500302181
-0.417849862843 0.0548398417793
-0.41696897761 0.0546297845104
-0.416088092377 0.0544198649666
-0.415207207145 0.05421008947
-0.414326321912 0.0540004641242
-0.413445436679 0.0537909948267
-0.412564551446 0.0535816872813
-0.411683666213 0.0533725470088
-0.41080278098 0.0531635793571
-0.409921895747 0.0529547895103
-0.409041010514 0.0527461824977
-0.408160125281 0.0525377632015
-0.407279240048 0.0523295363641
-0.406398354815 0.0521215065953
-0.405517469582 0.0519136783785
-0.404636584349 0.0517060560764
-0.403755699117 0.0514986439372
-0.402874813884 0.0512914460993
-0.401993928651 0.0510844665962
-0.401113043418 0.0508777093614
-0.400232158185 0.0506711782323
-0.399351272952 0.0504648769546
-0.398470387719 0.0502588091857
-0.397589502486 0.0500529784986
-0.396708617253 0.0498473883852
-0.39582773202 0.0496420422592
-0.394946846787 0.0494369434594
-0.394065961554 0.0492320952526
-0.393185076321 0.049027500836
-0.392304191089 0.0488231633399
-0.391423305856 0.04861908583
-0.390542420623 0.04841527131
-0.38966153539 0.0482117227233
-0.388780650157 0.0480084429555
-0.387899764924 0.047805434836
-0.387018879691 0.0476027011403
-0.386137994458 0.0474002445913
-0.385257109225 0.0471980678613
-0.384376223992 0.0469961735736
-0.383495338759 0.046794564304
-0.382614453526 0.046593242582
-0.381733568293 0.0463922108929
-0.380852683061 0.0461914716784
-0.379971797828 0.0459910273383
-0.379090912595 0.0457908802317
-0.378210027362 0.045591032678
-0.377329142129 0.0453914869584
-0.376448256896 0.0451922453166
-0.375567371663 0.0449933099599
-0.37468648643 0.0447946830605
-0.373805601197 0.0445963667561
-0.372924715964 0.0443983631511
-0.372043830731 0.0442006743173
-0.371162945498 0.0440033022949
-0.370282060265 0.0438062490931
-0.369401175033 0.0436095166911
-0.3685202898 0.043413107039
-0.367639404567 0.0432170220581
-0.366758519334 0.043021263642
-0.365877634101 0.0428258336569
-0.364996748868 0.0426307339427
-0.364115863635 0.0424359663133
-0.363234978402 0.0422415325576
-0.362354093169 0.0420474344395
-0.361473207936 0.0418536736988
-0.360592322703 0.0416602520521
-0.35971143747 0.0414671711927
-0.358830552237 0.0412744327914
-0.357949667005 0.0410820384972
-0.357068781772 0.0408899899374
-0.356187896539 0.0406982887183
-0.355307011306 0.0405069364258
-0.354426126073 0.0403159346253
-0.35354524084 0.0401252848628
-0.352664355607 0.0399349886649
-0.351783470374 0.0397450475392
-0.350902585141 0.0395554629748
-0.350021699908 0.0393662364429
-0.349140814675 0.0391773693966
-0.348259929442 0.0389888632717
-0.347379044209 0.038800719487
-0.346498158977 0.0386129394444
-0.345617273744 0.0384255245296
-0.344736388511 0.0382384761121
-0.343855503278 0.0380517955454
-0.342974618045 0.0378654841678
-0.342093732812 0.0376795433023
-0.341212847579 0.037493974257
-0.340331962346 0.0373087783252
-0.339451077113 0.0371239567859
-0.33857019188 0.0369395109042
-0.337689306647 0.036755441931
-0.336808421414 0.0365717511037
-0.335927536181 0.0363884396465
-0.335046650949 0.0362055087701
-0.334165765716 0.0360229596726
-0.333284880483 0.0358407935392
-0.33240399525 0.0356590115427
-0.331523110017 0.0354776148436
-0.330642224784 0.0352966045905
-0.329761339551 0.0351159819198
-0.328880454318 0.0349357479565
-0.327999569085 0.0347559038141
-0.327118683852 0.0345764505946
-0.326237798619 0.0343973893892
-0.325356913386 0.034218721278
-0.324476028153 0.0340404473303
-0.323595142921 0.0338625686048
-0.322714257688 0.03368508615
-0.321833372455 0.0335080010039
-0.320952487222 0.0333313141944
-0.320071601989 0.0331550267396
-0.319190716756 0.0329791396477
-0.318309831523 0.0328036539173
-0.31742894629 0.0326285705374
-0.316548061057 0.0324538904878
-0.315667175824 0.0322796147388
-0.314786290591 0.032105744252
-0.313905405358 0.0319322799796
-0.313024520125 0.0317592228652
-0.312143634893 0.0315865738437
-0.31126274966 0.0314143338415
-0.310381864427 0.0312425037762
-0.309500979194 0.0310710845573
-0.308620093961 0.0309000770862
-0.307739208728 0.0307294822558
-0.306858323495 0.0305593009514
-0.305977438262 0.0303895340501
-0.305096553029 0.0302201824214
-0.304215667796 0.030051246927
-0.303334782563 0.0298827284211
-0.30245389733 0.0297146277503
-0.301573012097 0.0295469457539
-0.300692126865 0.029379683264
-0.299811241632 0.0292128411052
-0.298930356399 0.0290464200955
-0.298049471166 0.0288804210453
-0.297168585933 0.0287148447585
-0.2962877007 0.0285496920321
-0.295406815467 0.0283849636562
-0.294525930234 0.0282206604143
-0.293645045001 0.0280567830834
-0.292764159768 0.0278933324339
-0.291883274535 0.0277303092298
-0.291002389302 0.0275677142288
-0.290121504069 0.0274055481823
-0.289240618837 0.0272438118356
-0.288359733604 0.0270825059276
-0.287478848371 0.0269216311914
-0.286597963138 0.0267611883542
-0.285717077905 0.026601178137
-0.284836192672 0.0264416012552
-0.283955307439 0.0262824584184
-0.283074422206 0.0261237503303
-0.282193536973 0.0259654776893
-0.28131265174 0.0258076411878
-0.280431766507 0.0256502415131
-0.279550881274 0.0254932793468
-0.278669996041 0.0253367553652
-0.277789110809 0.0251806702393
-0.276908225576 0.0250250246346
-0.276027340343 0.0248698192118
-0.27514645511 0.024715054626
-0.274265569877 0.0245607315274
-0.273384684644 0.0244068505613
-0.272503799411 0.0242534123678
-0.271622914178 0.024100417582
-0.270742028945 0.0239478668344
-0.269861143712 0.0237957607503
-0.268980258479 0.0236440999505
-0.268099373246 0.023492885051
-0.267218488013 0.0233421166629
-0.266337602781 0.023191795393
-0.265456717548 0.0230419218433
-0.264575832315 0.0228924966112
-0.263694947082 0.0227435202897
-0.262814061849 0.0225949934674
-0.261933176616 0.0224469167283
-0.261052291383 0.0222992906521
-0.26017140615 0.0221521158144
-0.259290520917 0.0220053927862
-0.258409635684 0.0218591221343
-0.257528750451 0.0217133044215
-0.256647865218 0.0215679402063
-0.255766979985 0.021423030043
-0.254886094753 0.021278574482
-0.25400520952 0.0211345740695
-0.253124324287 0.0209910293478
-0.252243439054 0.0208479408551
-0.251362553821 0.0207053091259
-0.250481668588 0.0205631346905
-0.249600783355 0.0204214180756
-0.248719898122 0.0202801598039
-0.247839012889 0.0201393603943
-0.246958127656 0.0199990203622
-0.246077242423 0.0198591402189
-0.24519635719 0.0197197204724
-0.244315471957 0.0195807616267
-0.243434586725 0.0194422641823
-0.242553701492 0.0193042286362
-0.241672816259 0.0191666554817
-0.240791931026 0.0190295452087
-0.239911045793 0.0188928983034
-0.23903016056 0.0187567152488
-0.238149275327 0.0186209965243
-0.237268390094 0.0184857426058
-0.236387504861 0.018350953966
-0.235506619628 0.0182166310741
-0.234625734395 0.018082774396
-0.233744849162 0.0179493843945
-0.232863963929 0.0178164615288
-0.231983078697 0.017684006255
-0.231102193464 0.0175520190261
-0.230221308231 0.0174205002918
-0.229340422998 0.0172894504986
-0.228459537765 0.0171588700898
-0.227578652532 0.0170287595058
-0.226697767299 0.0168991191837
-0.225816882066 0.0167699495577
-0.224935996833 0.0166412510588
-0.2240551116 0.0165130241151
-0.223174226367 0.0163852691515
-0.222293341134 0.0162579865903
-0.221412455901 0.0161311768505
-0.220531570669 0.0160048403483
-0.219650685436 0.015878977497
-0.218769800203 0.015753588707
-0.21788891497 0.0156286743858
-0.217008029737 0.0155042349383
-0.216127144504 0.0153802707662
-0.215246259271 0.0152567822686
-0.214365374038 0.0151337698418
-0.213484488805 0.0150112338795
-0.212603603572 0.0148891747723
-0.211722718339 0.0147675929084
-0.210841833106 0.0146464886732
-0.209960947873 0.0145258624494
-0.209080062641 0.0144057146171
-0.208199177408 0.0142860455535
-0.207318292175 0.0141668556337
-0.206437406942 0.0140481452296
-0.205556521709 0.013929914711
-0.204675636476 0.0138121644449
-0.203794751243 0.0136948947956
-0.20291386601 0.0135781061252
-0.202032980777 0.0134617987931
-0.201152095544 0.0133459731563
-0.200271210311 0.0132306295691
-0.199390325078 0.0131157683835
-0.198509439846 0.0130013899492
-0.197628554613 0.0128874946131
-0.19674766938 0.0127740827199
-0.195866784147 0.012661154612
-0.194985898914 0.0125487106292
-0.194105013681 0.012436751109
-0.193224128448 0.0123252763867
-0.192343243215 0.012214286795
-0.191462357982 0.0121037826644
-0.190581472749 0.0119937643232
-0.189700587516 0.0118842320972
-0.188819702283 0.01177518631
-0.18793881705 0.011666627283
-0.187057931818 0.0115585553354
-0.186177046585 0.0114509707839
-0.185296161352 0.0113438739431
-0.184415276119 0.0112372651256
-0.183534390886 0.0111311446415
-0.182653505653 0.0110255127988
-0.18177262042 0.0109203699035
-0.180891735187 0.0108157162592
-0.180010849954 0.0107115521675
-0.179129964721 0.0106078779278
-0.178249079488 0.0105046938375
-0.177368194255 0.0104020001916
-0.176487309022 0.0102997972834
-0.17560642379 0.0101980854037
-0.174725538557 0.0100968648417
-0.173844653324 0.0099961358841
-0.172963768091 0.0098958988158
-0.172082882858 0.00979615391957
-0.171201997625 0.00969690147619
-0.170321112392 0.00959814176441
-0.169440227159 0.00949987506099
-0.168559341926 0.00940210164068
-0.167678456693 0.00930482177625
-0.16679757146 0.0092080357385
-0.165916686227 0.0091117437963
-0.165035800994 0.00901594621652
-0.164154915762 0.00892064326412
-0.163274030529 0.00882583520213
-0.162393145296 0.00873152229165
-0.161512260063 0.00863770479189
-0.16063137483 0.00854438296013
-0.159750489597 0.0084515570518
-0.158869604364 0.00835922732041
-0.157988719131 0.00826739401763
-0.157107833898 0.00817605739325
-0.156226948665 0.00808521769524
-0.155346063432 0.00799487516968
-0.154465178199 0.00790503006086
-0.153584292966 0.00781568261123
-0.152703407734 0.00772683306143
-0.151822522501 0.00763848165028
-0.150941637268 0.00755062861482
-0.150060752035 0.0074632741903
-0.149179866802 0.00737641861018
-0.148298981569 0.00729006210616
-0.147418096336 0.00720420490817
-0.146537211103 0.0071188472444
-0.14565632587 0.00703398934127
-0.144775440637 0.00694963142348
-0.143894555404 0.006865773714
-0.143013670171 0.00678241643407
-0.142132784938 0.00669955980323
-0.141251899706 0.00661720403928
-0.140371014473 0.00653534935837
-0.13949012924 0.00645399597492
-0.138609244007 0.00637314410169
-0.137728358774 0.00629279394974
-0.136847473541 0.0062129457285
-0.135966588308 0.00613359964569
-0.135085703075 0.00605475590741
-0.134204817842 0.00597641471811
-0.133323932609 0.00589857628059
-0.132443047376 0.00582124079602
-0.131562162143 0.00574440846394
-0.13068127691 0.00566807948229
-0.129800391678 0.00559225404736
-0.128919506445 0.00551693235387
-0.128038621212 0.00544211459493
-0.127157735979 0.00536780096204
-0.126276850746 0.00529399164515
-0.125395965513 0.00522068683258
-0.12451508028 0.00514788671113
-0.123634195047 0.00507559146598
-0.122753309814 0.0050038012808
-0.121872424581 0.00493251633766
-0.120991539348 0.0048617368171
-0.120110654115 0.00479146289813
-0.119229768882 0.0047216947582
-0.11834888365 0.00465243257324
-0.117467998417 0.00458367651765
-0.116587113184 0.0045154267643
-0.115706227951 0.00444768348456
-0.114825342718 0.0043804468483
-0.113944457485 0.00431371702386
-0.113063572252 0.00424749417809
-0.112182687019 0.00418177847636
-0.111301801786 0.00411657008255
-0.110420916553 0.00405186915903
-0.10954003132 0.00398767586673
-0.108659146087 0.00392399036509
-0.107778260854 0.00386081281208
-0.106897375622 0.00379814336421
-0.106016490389 0.00373598217654
-0.105135605156 0.00367432940268
-0.104254719923 0.00361318519477
-0.10337383469 0.00355254970354
-0.102492949457 0.00349242307825
-0.101612064224 0.00343280546675
-0.100731178991 0.00337369701545
-0.0998502937581 0.00331509786934
-0.0989694085252 0.00325700817199
-0.0980885232923 0.00319942806555
-0.0972076380594 0.00314235769076
-0.0963267528264 0.00308579718697
-0.0954458675935 0.00302974669211
-0.0945649823606 0.0029742063427
-0.0936840971277 0.00291917627391
-0.0928032118948 0.00286465661947
-0.0919223266618 0.00281064751175
-0.0910414414289 0.00275714908174
-0.090160556196 0.00270416145906
-0.0892796709631 0.00265168477192
-0.0883987857301 0.0025997191472
-0.0875179004972 0.00254826471039
-0.0866370152643 0.00249732158563
-0.0857561300314 0.00244688989569
-0.0848752447984 0.002396969762
-0.0839943595655 0.00234756130464
-0.0831134743326 0.00229866464231
-0.0822325890997 0.00225027989241
-0.0813517038668 0.00220240717097
-0.0804708186338 0.00215504659269
-0.0795899334009 0.00210819827093
-0.078709048168 0.00206186231775
-0.0778281629351 0.00201603884384
-0.0769472777021 0.00197072795859
-0.0760663924692 0.00192592977007
-0.0751855072363 0.00188164438503
-0.0743046220034 0.0018378719089
-0.0734237367704 0.0017946124458
-0.0725428515375 0.00175186609854
-0.0716619663046 0.00170963296864
-0.0707810810717 0.0016679131563
-0.0699001958388 0.00162670676043
-0.0690193106058 0.00158601387864
-0.0681384253729 0.00154583460725
-0.06725754014 0.00150616904128
-0.0663766549071 0.00146701727447
-0.0654957696741 0.00142837939927
-0.0646148844412 0.00139025550686
-0.0637339992083 0.00135264568712
-0.0628531139754 0.00131555002867
-0.0619722287425 0.00127896861884
-0.0610913435095 0.0012429015437
-0.0602104582766 0.00120734888804
-0.0593295730437 0.00117231073539
-0.0584486878108 0.00113778716802
-0.0575678025778 0.00110377826691
-0.0566869173449 0.00107028411182
-0.055806032112 0.00103730478121
-0.0549251468791 0.00100484035232
-0.0540442616461 0.000972890901111
-0.0531633764132 0.000941456502304
-0.0522824911803 0.000910537229369
-0.0514016059474 0.000880133154526
-0.0505207207145 0.000850244348751
-0.0496398354815 0.000820870881777
-0.0487589502486 0.000792012822093
-0.0478780650157 0.000763670236951
-0.0469971797828 0.000735843192365
-0.0461162945498 0.000708531753111
-0.0452354093169 0.000681735982734
-0.044354524084 0.000655455943544
-0.0434736388511 0.000629691696622
-0.0425927536181 0.00060444330182
-0.0417118683852 0.000579710817761
-0.0408309831523 0.000555494301847
-0.0399500979194 0.00053179381025
-0.0390692126865 0.000508609397925
-0.0381883274535 0.000485941118604
-0.0373074422206 0.000463789024798
-0.0364265569877 0.000442153167803
-0.0355456717548 0.000421033597697
-0.0346647865218 0.000400430363344
-0.0337839012889 0.000380343512392
-0.032903016056 0.00036077309128
-0.0320221308231 0.000341719145232
-0.0311412455901 0.000323181718267
-0.0302603603572 0.00030516085319
-0.0293794751243 0.000287656591603
-0.0284985898914 0.000270668973899
-0.0276177046585 0.000254198039267
-0.0267368194255 0.000238243825691
-0.0258559341926 0.000222806369953
-0.0249750489597 0.000207885707633
-0.0240941637268 0.000193481873109
-0.0232132784938 0.000179594899559
-0.0223323932609 0.000166224818963
-0.021451508028 0.0001533716621
-0.0205706227951 0.000141035458555
-0.0196897375622 0.000129216236715
-0.0188088523292 0.000117914023768
-0.0179279670963 0.000107128845713
-0.0170470818634 9.68607273482e-05
-0.0161661966305 8.71096922827e-05
-0.0152853113975 7.78757629304e-05
-0.0144044261646 6.9158960513e-05
-0.0135235409317 6.09593050604e-05
-0.0126426556988 5.32768154112e-05
-0.0117617704658 4.61115092129e-05
-0.0108808852329 3.94634029229e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularLevelSets.tex <==
-0.450442616461 0.12309389097
-0.450442616461 0.123093890969
-0.450442616461 0.123093890962
-0.450442616461 0.123093890945
-0.450442616461 0.123093890912
-0.450442616461 0.123093890857
-0.450442616461 0.123093890776
-0.450442616461 0.123093890662
-0.450442616461 0.12309389051
-0.450442616461 0.123093890315
-0.450442616461 0.123093890072
-0.450442616461 0.123093889775
-0.450442616461 0.123093889419
-0.450442616461 0.123093888998
-0.450442616461 0.123093888507
-0.450442616461 0.123093887941
-0.450442616461 0.123093887294
-0.450442616461 0.123093886561
-0.450442616461 0.123093885737
-0.450442616461 0.123093884815
-0.450442616461 0.123093883791
-0.450442616461 0.12309388266
-0.450442616461 0.123093881415
-0.450442616461 0.123093880052
-0.450442616461 0.123093878566
-0.450442616461 0.12309387695
-0.450442616461 0.123093875199
-0.450442616461 0.123093873309
-0.450442616461 0.123093871273
-0.450442616461 0.123093869086
-0.450442616461 0.123093866743
-0.450442616461 0.123093864239
-0.450442616461 0.123093861568
-0.450442616461 0.123093858725
-0.450442616461 0.123093855704
-0.450442616461 0.1230938525
-0.450442616461 0.123093849107
-0.450442616461 0.123093845521
-0.450442616461 0.123093841736
-0.450442616461 0.123093837746
-0.450442616461 0.123093833546
-0.450442616461 0.12309382913
-0.450442616461 0.123093824494
-0.450442616461 0.123093819632
-0.450442616461 0.123093814539
-0.450442616461 0.123093809209
-0.450442616461 0.123093803636
-0.450442616461 0.123093797816
-0.450442616461 0.123093791743
-0.450442616461 0.123093785411
-0.450442616461 0.123093778816
-0.450442616461 0.123093771952
-0.450442616461 0.123093764813
-0.450442616461 0.123093757394
-0.450442616461 0.12309374969
-0.450442616461 0.123093741695
-0.450442616461 0.123093733405
-0.450442616461 0.123093724813
-0.450442616461 0.123093715914
-0.450442616461 0.123093706703
-0.450442616461 0.123093697174
-0.450442616461 0.123093687322
-0.450442616461 0.123093677143
-0.450442616461 0.123093666629
-0.450442616461 0.123093655776
-0.450442616461 0.123093644579
-0.450442616461 0.123093633033
-0.450442616461 0.123093621131
-0.450442616461 0.123093608868
-0.450442616461 0.123093596239
-0.450442616461 0.12309358324
-0.450442616461 0.123093569863
-0.450442616461 0.123093556104
-0.450442616461 0.123093541958
-0.450442616461 0.123093527419
-0.450442616461 0.123093512482
-0.450442616461 0.123093497141
-0.450442616461 0.123093481392
-0.450442616461 0.123093465228
-0.450442616461 0.123093448644
-0.450442616461 0.123093431635
-0.450442616461 0.123093414196
-0.450442616461 0.123093396321
-0.450442616461 0.123093378005
-0.450442616461 0.123093359242
-0.450442616461 0.123093340027
-0.450442616461 0.123093320355
-0.450442616461 0.12309330022
-0.450442616461 0.123093279617
-0.450442616461 0.12309325854
-0.450442616461 0.123093236985
-0.450442616461 0.123093214945
-0.450442616461 0.123093192416
-0.450442616461 0.123093169392
-0.450442616461 0.123093145868
-0.450442616461 0.123093121838
-0.450442616461 0.123093097297
-0.450442616461 0.12309307224
-0.450442616461 0.12309304666
-0.450442616461 0.123093020554
-0.450442616461 0.123092993915
-0.450442616461 0.123092966738
-0.450442616461 0.123092939018
-0.450442616461 0.123092910749
-0.450442616461 0.123092881926
-0.450442616461 0.123092852544
-0.450442616461 0.123092822597
-0.450442616461 0.12309279208
-0.450442616461 0.123092760987
-0.450442616461 0.123092729313
-0.450442616461 0.123092697054
-0.450442616461 0.123092664202
-0.450442616461 0.123092630754
-0.450442616461 0.123092596703
-0.450442616461 0.123092562045
-0.450442616461 0.123092526773
-0.450442616461 0.123092490884
-0.450442616461 0.12309245437
-0.450442616461 0.123092417227
-0.450442616461 0.12309237945
-0.450442616461 0.123092341032
-0.450442616461 0.12309230197
-0.450442616461 0.123092262257
-0.450442616461 0.123092221888
-0.450442616461 0.123092180857
-0.450442616461 0.12309213916
-0.450442616461 0.123092096791
-0.450442616461 0.123092053744
-0.450442616461 0.123092010014
-0.450442616461 0.123091965597
-0.450442616461 0.123091920486
-0.450442616461 0.123091874676
-0.450442616461 0.123091828161
-0.450442616461 0.123091780937
-0.450442616461 0.123091732998
-0.450442616461 0.123091684339
-0.450442616461 0.123091634954
-0.450442616461 0.123091584838
-0.450442616461 0.123091533986
-0.450442616461 0.123091482392
-0.450442616461 0.12309143005
-0.450442616461 0.123091376957
-0.450442616461 0.123091323105
-0.450442616461 0.12309126849
-0.450442616461 0.123091213107
-0.450442616461 0.12309115695
-0.450442616461 0.123091100013
-0.450442616461 0.123091042292
-0.450442616461 0.123090983781
-0.450442616461 0.123090924475
-0.450442616461 0.123090864368
-0.450442616461 0.123090803455
-0.450442616461 0.12309074173
-0.450442616461 0.123090679189
-0.450442616461 0.123090615825
-0.450442616461 0.123090551635
-0.450442616461 0.123090486611
-0.450442616461 0.123090420749
-0.450442616461 0.123090354044
-0.450442616461 0.12309028649
-0.450442616461 0.123090218082
-0.450442616461 0.123090148814
-0.450442616461 0.123090078681
-0.450442616461 0.123090007678
-0.450442616461 0.123089935799
-0.450442616461 0.12308986304
-0.450442616461 0.123089789394
-0.450442616461 0.123089714857
-0.450442616461 0.123089639422
-0.450442616461 0.123089563085
-0.450442616461 0.123089485841
-0.450442616461 0.123089407683
-0.450442616461 0.123089328607
-0.450442616461 0.123089248608
-0.450442616461 0.123089167679
-0.450442616461 0.123089085816
-0.450442616461 0.123089003013
-0.450442616461 0.123088919265
-0.450442616461 0.123088834567
-0.450442616461 0.123088748913
-0.450442616461 0.123088662297
-0.450442616461 0.123088574716
-0.450442616461 0.123088486162
-0.450442616461 0.123088396631
-0.450442616461 0.123088306118
-0.450442616461 0.123088214617
-0.450442616461 0.123088122123
-0.450442616461 0.12308802863
-0.450442616461 0.123087934134
-0.450442616461 0.123087838628
-0.450442616461 0.123087742108
-0.450442616461 0.123087644568
-0.450442616461 0.123087546003
-0.450442616461 0.123087446407
-0.450442616461 0.123087345776
-0.450442616461 0.123087244103
-0.450442616461 0.123087141384
-0.450442616461 0.123087037612
-0.450442616461 0.123086932784
-0.450442616461 0.123086826893
-0.450442616461 0.123086719934
-0.450442616461 0.123086611903
-0.450442616461 0.123086502792
-0.450442616461 0.123086392598
-0.450442616461 0.123086281314
-0.450442616461 0.123086168936
-0.450442616461 0.123086055459
-0.450442616461 0.123085940876
-0.450442616461 0.123085825182
-0.450442616461 0.123085708373
-0.450442616461 0.123085590442
-0.450442616461 0.123085471386
-0.450442616461 0.123085351197
-0.450442616461 0.123085229871
-0.450442616461 0.123085107403
-0.450442616461 0.123084983787
-0.450442616461 0.123084859017
-0.450442616461 0.12308473309
-0.450442616461 0.123084605998
-0.450442616461 0.123084477738
-0.450442616461 0.123084348303
-0.450442616461 0.123084217689
-0.450442616461 0.123084085889
-0.450442616461 0.123083952899
-0.450442616461 0.123083818714
-0.450442616461 0.123083683327
-0.450442616461 0.123083546734
-0.450442616461 0.12308340893
-0.450442616461 0.123083269908
-0.450442616461 0.123083129665
-0.450442616461 0.123082988193
-0.450442616461 0.123082845489
-0.450442616461 0.123082701547
-0.450442616461 0.123082556361
-0.450442616461 0.123082409926
-0.450442616461 0.123082262237
-0.450442616461 0.123082113289
-0.450442616461 0.123081963075
-0.450442616461 0.123081811592
-0.450442616461 0.123081658834
-0.450442616461 0.123081504794
-0.450442616461 0.123081349469
-0.450442616461 0.123081192852
-0.450442616461 0.123081034939
-0.450442616461 0.123080875723
-0.450442616461 0.123080715201
-0.450442616461 0.123080553366
-0.450442616461 0.123080390213
-0.450442616461 0.123080225737
-0.450442616461 0.123080059932
-0.450442616461 0.123079892794
-0.450442616461 0.123079724316
-0.450442616461 0.123079554494
-0.450442616461 0.123079383323
-0.450442616461 0.123079210796
-0.450442616461 0.123079036909
-0.450442616461 0.123078861657
-0.450442616461 0.123078685033
-0.450442616461 0.123078507034
-0.450442616461 0.123078327653
-0.450442616461 0.123078146885
-0.450442616461 0.123077964725
-0.450442616461 0.123077781168
-0.450442616461 0.123077596208
-0.450442616461 0.12307740984
-0.450442616461 0.123077222059
-0.450442616461 0.123077032859
-0.450442616461 0.123076842235
-0.450442616461 0.123076650182
-0.450442616461 0.123076456695
-0.450442616461 0.123076261768
-0.450442616461 0.123076065396
-0.450442616461 0.123075867573
-0.450442616461 0.123075668295
-0.450442616461 0.123075467556
-0.450442616461 0.123075265351
-0.450442616461 0.123075061675
-0.450442616461 0.123074856521
-0.450442616461 0.123074649886
-0.450442616461 0.123074441763
-0.450442616461 0.123074232148
-0.450442616461 0.123074021034
-0.450442616461 0.123073808418
-0.450442616461 0.123073594293
-0.450442616461 0.123073378654
-0.450442616461 0.123073161496
-0.450442616461 0.123072942814
-0.450442616461 0.123072722602
-0.450442616461 0.123072500856
-0.450442616461 0.123072277569
-0.450442616461 0.123072052737
-0.450442616461 0.123071826354
-0.450442616461 0.123071598415
-0.450442616461 0.123071368915
-0.450442616461 0.123071137848
-0.450442616461 0.123070905209
-0.450442616461 0.123070670994
-0.450442616461 0.123070435196
-0.450442616461 0.12307019781
-0.450442616461 0.123069958831
-0.450442616461 0.123069718254
-0.450442616461 0.123069476074
-0.450442616461 0.123069232285
-0.450442616461 0.123068986882
-0.450442616461 0.12306873986
-0.450442616461 0.123068491213
-0.450442616461 0.123068240936
-0.450442616461 0.123067989025
-0.450442616461 0.123067735472
-0.450442616461 0.123067480275
-0.450442616461 0.123067223426
-0.450442616461 0.123066964922
-0.450442616461 0.123066704755
-0.450442616461 0.123066442923
-0.450442616461 0.123066179418
-0.450442616461 0.123065914236
-0.450442616461 0.123065647372
-0.450442616461 0.12306537882
-0.450442616461 0.123065108575
-0.450442616461 0.123064836632
-0.450442616461 0.123064562985
-0.450442616461 0.12306428763
-0.450442616461 0.12306401056
-0.450442616461 0.123063731772
-0.450442616461 0.123063451258
-0.450442616461 0.123063169016
-0.450442616461 0.123062885038
-0.450442616461 0.12306259932
-0.450442616461 0.123062311856
-0.450442616461 0.123062022641
-0.450442616461 0.123061731671
-0.450442616461 0.123061438939
-0.450442616461 0.123061144441
-0.450442616461 0.123060848171
-0.450442616461 0.123060550124
-0.450442616461 0.123060250295
-0.450442616461 0.123059948678
-0.450442616461 0.123059645269
-0.450442616461 0.123059340062
-0.450442616461 0.123059033051
-0.450442616461 0.123058724232
-0.450442616461 0.123058413599
-0.450442616461 0.123058101148
-0.450442616461 0.123057786872
-0.450442616461 0.123057470766
-0.450442616461 0.123057152826
-0.450442616461 0.123056833046
-0.450442616461 0.123056511421
-0.450442616461 0.123056187946
-0.450442616461 0.123055862615
-0.450442616461 0.123055535423
-0.450442616461 0.123055206365
-0.450442616461 0.123054875436
-0.450442616461 0.12305454263
-0.450442616461 0.123054207943
-0.450442616461 0.123053871368
-0.450442616461 0.123053532901
-0.450442616461 0.123053192537
-0.450442616461 0.12305285027
-0.450442616461 0.123052506095
-0.450442616461 0.123052160008
-0.450442616461 0.123051812001
-0.450442616461 0.123051462071
-0.450442616461 0.123051110213
-0.450442616461 0.12305075642
-0.450442616461 0.123050400688
-0.450442616461 0.123050043011
-0.450442616461 0.123049683385
-0.450442616461 0.123049321804
-0.450442616461 0.123048958263
-0.450442616461 0.123048592756
-0.450442616461 0.123048225279
-0.450442616461 0.123047855826
-0.450442616461 0.123047484392
-0.450442616461 0.123047110972
-0.450442616461 0.123046735561
-0.450442616461 0.123046358152
-0.450442616461 0.123045978742
-0.450442616461 0.123045597325
-0.450442616461 0.123045213896
-0.450442616461 0.123044828449
-0.450442616461 0.123044440979
-0.450442616461 0.123044051482
-0.450442616461 0.123043659951
-0.450442616461 0.123043266382
-0.450442616461 0.12304287077
-0.450442616461 0.123042473108
-0.450442616461 0.123042073393
-0.450442616461 0.123041671619
-0.450442616461 0.123041267781
-0.450442616461 0.123040861872
-0.450442616461 0.12304045389
-0.450442616461 0.123040043827
-0.450442616461 0.123039631679
-0.450442616461 0.123039217441
-0.450442616461 0.123038801107
-0.450442616461 0.123038382673
-0.450442616461 0.123037962132
-0.450442616461 0.123037539481
-0.450442616461 0.123037114713
-0.450442616461 0.123036687824
-0.450442616461 0.123036258808
-0.450442616461 0.12303582766
-0.450442616461 0.123035394375
-0.450442616461 0.123034958948
-0.450442616461 0.123034521373
-0.450442616461 0.123034081646
-0.450442616461 0.123033639761
-0.450442616461 0.123033195713
-0.450442616461 0.123032749497
-0.450442616461 0.123032301107
-0.450442616461 0.123031850539
-0.450442616461 0.123031397787
-0.450442616461 0.123030942846
-0.450442616461 0.123030485711
-0.450442616461 0.123030026377
-0.450442616461 0.123029564839
-0.450442616461 0.12302910109
-0.450442616461 0.123028635127
-0.450442616461 0.123028166944
-0.450442616461 0.123027696536
-0.450442616461 0.123027223898
-0.450442616461 0.123026749024
-0.450442616461 0.123026271909
-0.450442616461 0.123025792549
-0.450442616461 0.123025310938
-0.450442616461 0.12302482707
-0.450442616461 0.123024340941
-0.450442616461 0.123023852546
-0.450442616461 0.123023361878
-0.450442616461 0.123022868934
-0.450442616461 0.123022373708
-0.450442616461 0.123021876195
-0.450442616461 0.12302137639
-0.450442616461 0.123020874287
-0.450442616461 0.123020369881
-0.450442616461 0.123019863168
-0.450442616461 0.123019354142
-0.450442616461 0.123018842797
-0.450442616461 0.123018329129
-0.450442616461 0.123017813133
-0.450442616461 0.123017294803
-0.450442616461 0.123016774135
-0.450442616461 0.123016251122
-0.450442616461 0.123015725761
-0.450442616461 0.123015198045
-0.450442616461 0.12301466797
-0.450442616461 0.12301413553
-0.450442616461 0.123013600721
-0.450442616461 0.123013063537
-0.450442616461 0.123012523973
-0.450442616461 0.123011982024
-0.450442616461 0.123011437685
-0.450442616461 0.123010890951
-0.450442616461 0.123010341816
-0.450442616461 0.123009790275
-0.450442616461 0.123009236323
-0.450442616461 0.123008679956
-0.450442616461 0.123008121167
-0.450442616461 0.123007559952
-0.450442616461 0.123006996306
-0.450442616461 0.123006430224
-0.450442616461 0.123005861699
-0.450442616461 0.123005290729
-0.450442616461 0.123004717306
-0.450442616461 0.123004141426
-0.450442616461 0.123003563084
-0.450442616461 0.123002982275
-0.450442616461 0.123002398993
-0.450442616461 0.123001813234
-0.450442616461 0.123001224992
-0.450442616461 0.123000634262
-0.450442616461 0.12300004104
-0.450442616461 0.122999445319
-0.450442616461 0.122998847096
-0.450442616461 0.122998246364
-0.450442616461 0.122997643118
-0.450442616461 0.122997037354
-0.450442616461 0.122996429067
-0.450442616461 0.122995818251
-0.450442616461 0.122995204901
-0.450442616461 0.122994589011
-0.450442616461 0.122993970578
-0.450442616461 0.122993349596
-0.450442616461 0.122992726059
-0.450442616461 0.122992099963
-0.450442616461 0.122991471302
-0.450442616461 0.122990840072
-0.450442616461 0.122990206267
-0.450442616461 0.122989569882
-0.450442616461 0.122988930912
-0.450442616461 0.122988289352
-0.450442616461 0.122987645197
-0.450442616461 0.122986998441
-0.450442616461 0.122986349081
-0.450442616461 0.122985697109
-0.450442616461 0.122985042522
-0.450442616461 0.122984385315
-0.450442616461 0.122983725481
-0.450442616461 0.122983063017
-0.450442616461 0.122982397917
-0.450442616461 0.122981730175
-0.450442616461 0.122981059788
-0.450442616461 0.122980386749
-0.450442616461 0.122979711054
-0.450442616461 0.122979032698
-0.450442616461 0.122978351674
-0.450442616461 0.12297766798
-0.450442616461 0.122976981608
-0.450442616461 0.122976292555
-0.450442616461 0.122975600815
-0.450442616461 0.122974906383
-0.450442616461 0.122974209254
-0.450442616461 0.122973509423
-0.450442616461 0.122972806884
-0.450442616461 0.122972101633
-0.450442616461 0.122971393665
-0.450442616461 0.122970682975
-0.450442616461 0.122969969556
-0.450442616461 0.122969253406
-0.450442616461 0.122968534517
-0.450442616461 0.122967812886
-0.450442616461 0.122967088507
-0.450442616461 0.122966361375
-0.450442616461 0.122965631485
-0.450442616461 0.122964898833
-0.450442616461 0.122964163412
-0.450442616461 0.122963425217
-0.450442616461 0.122962684245
-0.450442616461 0.122961940489
-0.450442616461 0.122961193945
-0.450442616461 0.122960444608
-0.450442616461 0.122959692472
-0.450442616461 0.122958937532
-0.450442616461 0.122958179784
-0.450442616461 0.122957419222
-0.450442616461 0.122956655841
-0.450442616461 0.122955889637
-0.450442616461 0.122955120603
-0.450442616461 0.122954348736
-0.450442616461 0.12295357403
-0.450442616461 0.12295279648
-0.450442616461 0.122952016081
-0.450442616461 0.122951232827
-0.450442616461 0.122950446715
-0.450442616461 0.122949657738
-0.450442616461 0.122948865892
-0.450442616461 0.122948071172
-0.450442616461 0.122947273572
-0.450442616461 0.122946473088
-0.450442616461 0.122945669715
-0.450442616461 0.122944863447
-0.450442616461 0.122944054279
-0.450442616461 0.122943242207
-0.450442616461 0.122942427226
-0.450442616461 0.12294160933
-0.450442616461 0.122940788514
-0.450442616461 0.122939964773
-0.450442616461 0.122939138103
-0.450442616461 0.122938308498
-0.450442616461 0.122937475953
-0.450442616461 0.122936640463
-0.450442616461 0.122935802023
-0.450442616461 0.122934960629
-0.450442616461 0.122934116274
-0.450442616461 0.122933268955
-0.450442616461 0.122932418666
-0.450442616461 0.122931565402
-0.450442616461 0.122930709157
-0.450442616461 0.122929849928
-0.450442616461 0.122928987708
-0.450442616461 0.122928122494
-0.450442616461 0.122927254279
-0.450442616461 0.12292638306
-0.450442616461 0.12292550883
-0.450442616461 0.122924631585
-0.450442616461 0.12292375132
-0.450442616461 0.122922868029
-0.450442616461 0.122921981709
-0.450442616461 0.122921092353
-0.450442616461 0.122920199957
-0.450442616461 0.122919304516
-0.450442616461 0.122918406025
-0.450442616461 0.122917504479
-0.450442616461 0.122916599872
-0.450442616461 0.1229156922
-0.450442616461 0.122914781458
-0.450442616461 0.12291386764
-0.450442616461 0.122912950743
-0.450442616461 0.12291203076
-0.450442616461 0.122911107687
-0.450442616461 0.122910181518
-0.450442616461 0.12290925225
-0.450442616461 0.122908319876
-0.450442616461 0.122907384392
-0.450442616461 0.122906445793
-0.450442616461 0.122905504073
-0.450442616461 0.122904559229
-0.450442616461 0.122903611254
-0.450442616461 0.122902660144
-0.450442616461 0.122901705894
-0.450442616461 0.122900748499
-0.450442616461 0.122899787954
-0.450442616461 0.122898824253
-0.450442616461 0.122897857393
-0.450442616461 0.122896887368
-0.450442616461 0.122895914172
-0.450442616461 0.122894937801
-0.450442616461 0.122893958251
-0.450442616461 0.122892975515
-0.450442616461 0.12289198959
-0.450442616461 0.12289100047
-0.450442616461 0.122890008149
-0.450442616461 0.122889012624
-0.450442616461 0.122888013889
-0.450442616461 0.12288701194
-0.450442616461 0.12288600677
-0.450442616461 0.122884998376
-0.450442616461 0.122883986752
-0.450442616461 0.122882971893
-0.450442616461 0.122881953795
-0.450442616461 0.122880932452
-0.450442616461 0.12287990786
-0.450442616461 0.122878880013
-0.450442616461 0.122877848907
-0.450442616461 0.122876814536
-0.450442616461 0.122875776896
-0.450442616461 0.122874735982
-0.450442616461 0.122873691788
-0.450442616461 0.12287264431
-0.450442616461 0.122871593543
-0.450442616461 0.122870539482
-0.450442616461 0.122869482121
-0.450442616461 0.122868421457
-0.450442616461 0.122867357484
-0.450442616461 0.122866290196
-0.450442616461 0.12286521959
-0.450442616461 0.12286414566
-0.450442616461 0.122863068402
-0.450442616461 0.122861987809
-0.450442616461 0.122860903878
-0.450442616461 0.122859816603
-0.450442616461 0.12285872598
-0.450442616461 0.122857632004
-0.450442616461 0.122856534669
-0.450442616461 0.122855433971
-0.450442616461 0.122854329904
-0.450442616461 0.122853222465
-0.450442616461 0.122852111647
-0.450442616461 0.122850997446
-0.450442616461 0.122849879857
-0.450442616461 0.122848758876
-0.450442616461 0.122847634496
-0.450442616461 0.122846506714
-0.450442616461 0.122845375524
-0.450442616461 0.122844240922
-0.450442616461 0.122843102902
-0.450442616461 0.12284196146
-0.450442616461 0.12284081659
-0.450442616461 0.122839668289
-0.450442616461 0.12283851655
-0.450442616461 0.122837361369
-0.450442616461 0.122836202741
-0.450442616461 0.122835040661
-0.450442616461 0.122833875124
-0.450442616461 0.122832706125
-0.450442616461 0.12283153366
-0.450442616461 0.122830357724
-0.450442616461 0.122829178311
-0.450442616461 0.122827995416
-0.450442616461 0.122826809036
-0.450442616461 0.122825619164
-0.450442616461 0.122824425796
-0.450442616461 0.122823228928
-0.450442616461 0.122822028553
-0.450442616461 0.122820824668
-0.450442616461 0.122819617267
-0.450442616461 0.122818406345
-0.450442616461 0.122817191899
-0.450442616461 0.122815973921
-0.450442616461 0.122814752409
-0.450442616461 0.122813527357
-0.450442616461 0.122812298759
-0.450442616461 0.122811066612
-0.450442616461 0.12280983091
-0.450442616461 0.122808591648
-0.450442616461 0.122807348822
-0.450442616461 0.122806102427
-0.450442616461 0.122804852457
-0.450442616461 0.122803598908
-0.450442616461 0.122802341775
-0.450442616461 0.122801081053
-0.450442616461 0.122799816737
-0.450442616461 0.122798548823
-0.450442616461 0.122797277305
-0.450442616461 0.122796002179
-0.450442616461 0.122794723439
-0.450442616461 0.122793441082
-0.450442616461 0.122792155101
-0.450442616461 0.122790865493
-0.450442616461 0.122789572251
-0.450442616461 0.122788275372
-0.450442616461 0.122786974851
-0.450442616461 0.122785670682
-0.450442616461 0.122784362862
-0.450442616461 0.122783051384
-0.450442616461 0.122781736244
-0.450442616461 0.122780417437
-0.450442616461 0.122779094959
-0.450442616461 0.122777768805
-0.450442616461 0.122776438969
-0.450442616461 0.122775105447
-0.450442616461 0.122773768234
-0.450442616461 0.122772427325
-0.450442616461 0.122771082715
-0.450442616461 0.1227697344
-0.450442616461 0.122768382374
-0.450442616461 0.122767026633
-0.450442616461 0.122765667172
-0.450442616461 0.122764303986
-0.450442616461 0.12276293707
-0.450442616461 0.12276156642
-0.450442616461 0.12276019203
-0.450442616461 0.122758813896
-0.450442616461 0.122757432013
-0.450442616461 0.122756046376
-0.450442616461 0.12275465698
-0.450442616461 0.12275326382
-0.450442616461 0.122751866892
-0.450442616461 0.122750466191
-0.450442616461 0.122749061712
-0.450442616461 0.122747653449
-0.450442616461 0.122746241399
-0.450442616461 0.122744825557
-0.450442616461 0.122743405916
-0.450442616461 0.122741982474
-0.450442616461 0.122740555225
-0.450442616461 0.122739124164
-0.450442616461 0.122737689286
-0.450442616461 0.122736250587
-0.450442616461 0.122734808061
-0.450442616461 0.122733361704
-0.450442616461 0.122731911512
-0.450442616461 0.122730457478
-0.450442616461 0.122728999599
-0.450442616461 0.12272753787
-0.450442616461 0.122726072286
-0.450442616461 0.122724602841
-0.450442616461 0.122723129532
-0.450442616461 0.122721652354
-0.450442616461 0.1227201713
-0.450442616461 0.122718686368
-0.450442616461 0.122717197552
-0.450442616461 0.122715704847
-0.450442616461 0.122714208248
-0.450442616461 0.122712707751
-0.450442616461 0.122711203351
-0.450442616461 0.122709695043
-0.450442616461 0.122708182823
-0.450442616461 0.122706666684
-0.450442616461 0.122705146624
-0.450442616461 0.122703622636
-0.450442616461 0.122702094717
-0.450442616461 0.12270056286
-0.450442616461 0.122699027063
-0.450442616461 0.122697487319
-0.450442616461 0.122695943624
-0.450442616461 0.122694395973
-0.450442616461 0.122692844362
-0.450442616461 0.122691288785
-0.450442616461 0.122689729238
-0.450442616461 0.122688165717
-0.450442616461 0.122686598216
-0.450442616461 0.12268502673
-0.450442616461 0.122683451255
-0.450442616461 0.122681871786
-0.450442616461 0.122680288318
-0.450442616461 0.122678700847
-0.450442616461 0.122677109368
-0.450442616461 0.122675513875
-0.450442616461 0.122673914365
-0.450442616461 0.122672310832
-0.450442616461 0.122670703272
-0.450442616461 0.12266909168
-0.450442616461 0.122667476051
-0.450442616461 0.12266585638
-0.450442616461 0.122664232663
-0.450442616461 0.122662604895
-0.450442616461 0.122660973071
-0.450442616461 0.122659337187
-0.450442616461 0.122657697237
-0.450442616461 0.122656053217
-0.450442616461 0.122654405122
-0.450442616461 0.122652752948
-0.450442616461 0.122651096689
-0.450442616461 0.122649436342
-0.450442616461 0.1226477719
-0.450442616461 0.12264610336
-0.450442616461 0.122644430717
-0.450442616461 0.122642753965
-0.450442616461 0.122641073101
-0.450442616461 0.12263938812
-0.450442616461 0.122637699016
-0.450442616461 0.122636005785
-0.450442616461 0.122634308423
-0.450442616461 0.122632606924
-0.450442616461 0.122630901284
-0.450442616461 0.122629191498
-0.450442616461 0.122627477562
-0.450442616461 0.12262575947
-0.450442616461 0.122624037218
-0.450442616461 0.122622310802
-0.450442616461 0.122620580216
-0.450442616461 0.122618845455
-0.450442616461 0.122617106516
-0.450442616461 0.122615363394
-0.450442616461 0.122613616082
-0.450442616461 0.122611864578
-0.450442616461 0.122610108877
-0.450442616461 0.122608348972
-0.450442616461 0.122606584861
-0.450442616461 0.122604816537
-0.450442616461 0.122603043997
-0.450442616461 0.122601267236
-0.450442616461 0.122599486249
-0.450442616461 0.122597701031
-0.450442616461 0.122595911578
-0.450442616461 0.122594117884
-0.450442616461 0.122592319946
-0.450442616461 0.122590517758
-0.450442616461 0.122588711316
-0.450442616461 0.122586900616
-0.450442616461 0.122585085651
-0.450442616461 0.122583266419
-0.450442616461 0.122581442913
-0.450442616461 0.12257961513
-0.450442616461 0.122577783065
-0.450442616461 0.122575946712
-0.450442616461 0.122574106068
-0.450442616461 0.122572261127
-0.450442616461 0.122570411886
-0.450442616461 0.122568558338
-0.450442616461 0.12256670048
-0.450442616461 0.122564838308
-0.450442616461 0.122562971815
-0.450442616461 0.122561100998
-0.450442616461 0.122559225852
-0.450442616461 0.122557346372
-0.450442616461 0.122555462553
-0.450442616461 0.122553574392
-0.450442616461 0.122551681882
-0.450442616461 0.122549785021
-0.450442616461 0.122547883802
-0.450442616461 0.122545978221
-0.450442616461 0.122544068274
-0.450442616461 0.122542153955
-0.450442616461 0.122540235261
-0.450442616461 0.122538312187
-0.450442616461 0.122536384727
-0.450442616461 0.122534452878
-0.450442616461 0.122532516634
-0.450442616461 0.122530575992
-0.450442616461 0.122528630945
-0.450442616461 0.12252668149
-0.450442616461 0.122524727623
-0.450442616461 0.122522769337
-0.450442616461 0.122520806629
-0.450442616461 0.122518839495
-0.450442616461 0.122516867929
-0.450442616461 0.122514891926
-0.450442616461 0.122512911483
-0.450442616461 0.122510926594
-0.450442616461 0.122508937255
-0.450442616461 0.122506943461
-0.450442616461 0.122504945208
-0.450442616461 0.122502942491
-0.450442616461 0.122500935305
-0.450442616461 0.122498923646
-0.450442616461 0.122496907509
-0.450442616461 0.12249488689
-0.450442616461 0.122492861783
-0.450442616461 0.122490832185
-0.450442616461 0.12248879809
-0.450442616461 0.122486759494
-0.450442616461 0.122484716392
-0.450442616461 0.12248266878
-0.450442616461 0.122480616653
-0.450442616461 0.122478560007
-0.450442616461 0.122476498836
-0.450442616461 0.122474433137
-0.450442616461 0.122472362904
-0.450442616461 0.122470288133
-0.450442616461 0.12246820882
-0.450442616461 0.12246612496
-0.450442616461 0.122464036547
-0.450442616461 0.122461943579
-0.450442616461 0.122459846049
-0.450442616461 0.122457743954
-0.450442616461 0.122455637288
-0.450442616461 0.122453526048
-0.450442616461 0.122451410228
-0.450442616461 0.122449289824
-0.450442616461 0.122447164832
-0.450442616461 0.122445035247
-0.450442616461 0.122442901063
-0.450442616461 0.122440762278
-0.450442616461 0.122438618885
-0.450442616461 0.122436470881
-0.450442616461 0.12243431826
-0.450442616461 0.122432161019
-0.450442616461 0.122429999152
-0.450442616461 0.122427832656
-0.450442616461 0.122425661525
-0.450442616461 0.122423485755
-0.450442616461 0.122421305342
-0.450442616461 0.12241912028
-0.450442616461 0.122416930565
-0.450442616461 0.122414736193
-0.450442616461 0.122412537159
-0.450442616461 0.122410333459
-0.450442616461 0.122408125087
-0.450442616461 0.12240591204
-0.450442616461 0.122403694313
-0.450442616461 0.1224014719
-0.450442616461 0.122399244799
-0.450442616461 0.122397013003
-0.450442616461 0.122394776509
-0.450442616461 0.122392535312
-0.450442616461 0.122390289408
-0.450442616461 0.122388038791
-0.450442616461 0.122385783457
-0.450442616461 0.122383523402
-0.450442616461 0.122381258622
-0.450442616461 0.122378989111
-0.450442616461 0.122376714865
-0.450442616461 0.122374435879
-0.450442616461 0.12237215215
-0.450442616461 0.122369863672
-0.450442616461 0.122367570441
-0.450442616461 0.122365272452
-0.450442616461 0.122362969701
-0.450442616461 0.122360662183
-0.450442616461 0.122358349894
-0.450442616461 0.122356032829
-0.450442616461 0.122353710984
-0.450442616461 0.122351384354
-0.450442616461 0.122349052934
-0.450442616461 0.122346716721
-0.450442616461 0.122344375709
-0.450442616461 0.122342029894
-0.450442616461 0.122339679271
-0.450442616461 0.122337323836
-0.450442616461 0.122334963585
-0.450442616461 0.122332598512
-0.450442616461 0.122330228614
-0.450442616461 0.122327853886
-0.450442616461 0.122325474323
-0.450442616461 0.122323089921
-0.450442616461 0.122320700675
-0.450442616461 0.122318306581
-0.450442616461 0.122315907634
-0.450442616461 0.12231350383
-0.450442616461 0.122311095164
-0.450442616461 0.122308681632
-0.450442616461 0.122306263228
-0.450442616461 0.12230383995
-0.450442616461 0.122301411792
-0.450442616461 0.122298978749
-0.450442616461 0.122296540818
-0.450442616461 0.122294097993
-0.450442616461 0.122291650271
-0.450442616461 0.122289197646
-0.450442616461 0.122286740115
-0.450442616461 0.122284277672
-0.450442616461 0.122281810313
-0.450442616461 0.122279338034
-0.450442616461 0.12227686083
-0.450442616461 0.122274378697
-0.450442616461 0.12227189163
-0.450442616461 0.122269399625
-0.450442616461 0.122266902677
-0.450442616461 0.122264400782
-0.450442616461 0.122261893935
-0.450442616461 0.122259382132
-0.450442616461 0.122256865368
-0.450442616461 0.12225434364
-0.450442616461 0.122251816941
-0.450442616461 0.122249285269
-0.450442616461 0.122246748617
-0.450442616461 0.122244206983
-0.450442616461 0.122241660361
-0.450442616461 0.122239108748
-0.450442616461 0.122236552138
-0.450442616461 0.122233990526
-0.450442616461 0.12223142391
-0.450442616461 0.122228852284
-0.450442616461 0.122226275643
-0.450442616461 0.122223693983
-0.450442616461 0.122221107301
-0.450442616461 0.12221851559
-0.450442616461 0.122215918848
-0.450442616461 0.122213317068
-0.450442616461 0.122210710248
-0.450442616461 0.122208098382
-0.450442616461 0.122205481467
-0.450442616461 0.122202859496
-0.450442616461 0.122200232467
-0.450442616461 0.122197600375
-0.450442616461 0.122194963215
-0.450442616461 0.122192320982
-0.450442616461 0.122189673673
-0.450442616461 0.122187021283
-0.450442616461 0.122184363807
-0.450442616461 0.122181701242
-0.450442616461 0.122179033582
-0.450442616461 0.122176360823
-0.450442616461 0.122173682961
-0.450442616461 0.122170999991
-0.450442616461 0.122168311909
-0.450442616461 0.12216561871
-0.450442616461 0.122162920391
-0.450442616461 0.122160216945
-0.450442616461 0.122157508371
-0.450442616461 0.122154794661
-0.450442616461 0.122152075813
-0.450442616461 0.122149351822
-0.450442616461 0.122146622684
-0.450442616461 0.122143888393
-0.450442616461 0.122141148946
-0.450442616461 0.122138404339
-0.450442616461 0.122135654566
-0.450442616461 0.122132899623
-0.450442616461 0.122130139507
-0.450442616461 0.122127374212
-0.450442616461 0.122124603734
-0.450442616461 0.122121828069
-0.450442616461 0.122119047212
-0.450442616461 0.122116261159
-0.450442616461 0.122113469905
-0.450442616461 0.122110673447
-0.450442616461 0.12210787178
-0.450442616461 0.122105064898
-0.450442616461 0.122102252799
-0.450442616461 0.122099435477
-0.450442616461 0.122096612929
-0.450442616461 0.122093785149
-0.450442616461 0.122090952134
-0.450442616461 0.122088113878
-0.450442616461 0.122085270378
-0.450442616461 0.122082421629
-0.450442616461 0.122079567627
-0.450442616461 0.122076708368
-0.450442616461 0.122073843846
-0.450442616461 0.122070974058
-0.450442616461 0.122068099
-0.450442616461 0.122065218666
-0.450442616461 0.122062333053
-0.450442616461 0.122059442156
-0.450442616461 0.122056545971
-0.450442616461 0.122053644493
-0.450442616461 0.122050737718
-0.450442616461 0.122047825642
-0.450442616461 0.12204490826
-0.450442616461 0.122041985568
-0.450442616461 0.122039057562
-0.450442616461 0.122036124237
-0.450442616461 0.122033185588
-0.450442616461 0.122030241612
-0.450442616461 0.122027292305
-0.450442616461 0.122024337661
-0.450442616461 0.122021377676
-0.450442616461 0.122018412346
-0.450442616461 0.122015441667
-0.450442616461 0.122012465635
-0.450442616461 0.122009484244
-0.450442616461 0.122006497491
-0.450442616461 0.122003505372
-0.450442616461 0.122000507881
-0.450442616461 0.121997505015
-0.450442616461 0.121994496769
-0.450442616461 0.121991483139
-0.450442616461 0.121988464121
-0.450442616461 0.121985439709
-0.450442616461 0.121982409901
-0.450442616461 0.121979374691
-0.450442616461 0.121976334076
-0.450442616461 0.12197328805
-0.450442616461 0.12197023661
-0.450442616461 0.121967179751
-0.450442616461 0.121964117469
-0.450442616461 0.12196104976
-0.450442616461 0.121957976619
-0.450442616461 0.121954898042
-0.450442616461 0.121951814024
-0.450442616461 0.121948724562
-0.450442616461 0.12194562965
-0.450442616461 0.121942529285
-0.450442616461 0.121939423463
-0.450442616461 0.121936312178
-0.450442616461 0.121933195428
-0.450442616461 0.121930073206
-0.450442616461 0.12192694551
-0.450442616461 0.121923812334
-0.450442616461 0.121920673675
-0.450442616461 0.121917529528
-0.450442616461 0.121914379888
-0.450442616461 0.121911224753
-0.450442616461 0.121908064116
-0.450442616461 0.121904897974
-0.450442616461 0.121901726323
-0.450442616461 0.121898549159
-0.450442616461 0.121895366476
-0.450442616461 0.121892178271
-0.450442616461 0.12188898454
-0.450442616461 0.121885785277
-0.450442616461 0.12188258048
-0.450442616461 0.121879370142
-0.450442616461 0.121876154262
-0.450442616461 0.121872932833
-0.450442616461 0.121869705852
-0.450442616461 0.121866473314
-0.450442616461 0.121863235215
-0.450442616461 0.121859991552
-0.450442616461 0.121856742318
-0.450442616461 0.121853487512
-0.450442616461 0.121850227127
-0.450442616461 0.121846961159
-0.450442616461 0.121843689606
-0.450442616461 0.121840412461
-0.450442616461 0.121837129721
-0.450442616461 0.121833841382
-0.450442616461 0.12183054744
-0.450442616461 0.121827247889
-0.450442616461 0.121823942726
-0.450442616461 0.121820631947
-0.450442616461 0.121817315547
-0.450442616461 0.121813993523
-0.450442616461 0.121810665869
-0.450442616461 0.121807332581
-0.450442616461 0.121803993656
-0.450442616461 0.121800649089
-0.450442616461 0.121797298875
-0.450442616461 0.121793943011
-0.450442616461 0.121790581493
-0.450442616461 0.121787214315
-0.450442616461 0.121783841474
-0.450442616461 0.121780462966
-0.450442616461 0.121777078786
-0.450442616461 0.12177368893
-0.450442616461 0.121770293393
-0.450442616461 0.121766892173
-0.450442616461 0.121763485263
-0.450442616461 0.121760072661
-0.450442616461 0.121756654361
-0.450442616461 0.12175323036
-0.450442616461 0.121749800654
-0.450442616461 0.121746365237
-0.450442616461 0.121742924106
-0.450442616461 0.121739477257
-0.450442616461 0.121736024686
-0.450442616461 0.121732566388
-0.450442616461 0.121729102358
-0.450442616461 0.121725632594
-0.450442616461 0.12172215709
-0.450442616461 0.121718675842
-0.450442616461 0.121715188846
-0.450442616461 0.121711696099
-0.450442616461 0.121708197595
-0.450442616461 0.12170469333
-0.450442616461 0.121701183301
-0.450442616461 0.121697667502
-0.450442616461 0.121694145931
-0.450442616461 0.121690618582
-0.450442616461 0.121687085451
-0.450442616461 0.121683546535
-0.450442616461 0.121680001829
-0.450442616461 0.121676451328
-0.450442616461 0.121672895029
-0.450442616461 0.121669332927
-0.450442616461 0.121665765019
-0.450442616461 0.121662191299
-0.450442616461 0.121658611765
-0.450442616461 0.121655026411
-0.450442616461 0.121651435233
-0.450442616461 0.121647838227
-0.450442616461 0.12164423539
-0.450442616461 0.121640626716
-0.450442616461 0.121637012202
-0.450442616461 0.121633391844
-0.450442616461 0.121629765636
-0.450442616461 0.121626133576
-0.450442616461 0.121622495659
-0.450442616461 0.12161885188
-0.450442616461 0.121615202236
-0.450442616461 0.121611546722
-0.450442616461 0.121607885335
-0.450442616461 0.121604218069
-0.450442616461 0.121600544922
-0.450442616461 0.121596865888
-0.450442616461 0.121593180963
-0.450442616461 0.121589490144
-0.450442616461 0.121585793426
-0.450442616461 0.121582090805
-0.450442616461 0.121578382277
-0.450442616461 0.121574667838
-0.450442616461 0.121570947483
-0.450442616461 0.121567221208
-0.450442616461 0.12156348901
-0.450442616461 0.121559750883
-0.450442616461 0.121556006825
-0.450442616461 0.12155225683
-0.450442616461 0.121548500895
-0.450442616461 0.121544739015
-0.450442616461 0.121540971186
-0.450442616461 0.121537197405
-0.450442616461 0.121533417666
-0.450442616461 0.121529631967
-0.450442616461 0.121525840302
-0.450442616461 0.121522042667
-0.450442616461 0.121518239059
-0.450442616461 0.121514429473
-0.450442616461 0.121510613906
-0.450442616461 0.121506792352
-0.450442616461 0.121502964808
-0.450442616461 0.12149913127
-0.450442616461 0.121495291734
-0.450442616461 0.121491446195
-0.450442616461 0.121487594649
-0.450442616461 0.121483737092
-0.450442616461 0.121479873521
-0.450442616461 0.12147600393
-0.450442616461 0.121472128316
-0.450442616461 0.121468246675
-0.450442616461 0.121464359003
-0.450442616461 0.121460465295
-0.450442616461 0.121456565547
-0.450442616461 0.121452659756
-0.450442616461 0.121448747916
-0.450442616461 0.121444830025
-0.450442616461 0.121440906077
-0.450442616461 0.12143697607
-0.450442616461 0.121433039997
-0.450442616461 0.121429097857
-0.450442616461 0.121425149644
-0.450442616461 0.121421195354
-0.450442616461 0.121417234983
-0.450442616461 0.121413268528
-0.450442616461 0.121409295983
-0.450442616461 0.121405317346
-0.450442616461 0.121401332611
-0.450442616461 0.121397341775
-0.450442616461 0.121393344834
-0.450442616461 0.121389341783
-0.450442616461 0.121385332619
-0.450442616461 0.121381317337
-0.450442616461 0.121377295933
-0.450442616461 0.121373268403
-0.450442616461 0.121369234744
-0.450442616461 0.12136519495
-0.450442616461 0.121361149019
-0.450442616461 0.121357096945
-0.450442616461 0.121353038725
-0.450442616461 0.121348974355
-0.450442616461 0.12134490383
-0.450442616461 0.121340827147
-0.450442616461 0.121336744301
-0.450442616461 0.121332655289
-0.450442616461 0.121328560106
-0.450442616461 0.121324458748
-0.450442616461 0.121320351212
-0.450442616461 0.121316237492
-0.450442616461 0.121312117586
-0.450442616461 0.121307991488
-0.450442616461 0.121303859196
-0.450442616461 0.121299720704
-0.450442616461 0.121295576009
-0.450442616461 0.121291425106
-0.450442616461 0.121287267993
-0.450442616461 0.121283104664
-0.450442616461 0.121278935115
-0.450442616461 0.121274759343
-0.450442616461 0.121270577344
-0.450442616461 0.121266389112
-0.450442616461 0.121262194646
-0.450442616461 0.121257993939
-0.450442616461 0.121253786989
-0.450442616461 0.121249573791
-0.450442616461 0.121245354341
-0.450442616461 0.121241128635
-0.450442616461 0.121236896669
-0.450442616461 0.121232658439
-0.450442616461 0.121228413942
-0.450442616461 0.121224163172
-0.450442616461 0.121219906126
-0.450442616461 0.1212156428
-0.450442616461 0.12121137319
-0.450442616461 0.121207097292
-0.450442616461 0.121202815101
-0.450442616461 0.121198526614
-0.450442616461 0.121194231827
-0.450442616461 0.121189930736
-0.450442616461 0.121185623336
-0.450442616461 0.121181309625
-0.450442616461 0.121176989596
-0.450442616461 0.121172663248
-0.450442616461 0.121168330575
-0.450442616461 0.121163991573
-0.450442616461 0.121159646239
-0.450442616461 0.121155294569
-0.450442616461 0.121150936558
-0.450442616461 0.121146572203
-0.450442616461 0.121142201499
-0.450442616461 0.121137824443
-0.450442616461 0.121133441031
-0.450442616461 0.121129051258
-0.450442616461 0.12112465512
-0.450442616461 0.121120252614
-0.450442616461 0.121115843735
-0.450442616461 0.12111142848
-0.450442616461 0.121107006845
-0.450442616461 0.121102578825
-0.450442616461 0.121098144416
-0.450442616461 0.121093703615
-0.450442616461 0.121089256417
-0.450442616461 0.121084802819
-0.450442616461 0.121080342817
-0.450442616461 0.121075876406
-0.450442616461 0.121071403583
-0.450442616461 0.121066924343
-0.450442616461 0.121062438683
-0.450442616461 0.121057946599
-0.450442616461 0.121053448086
-0.450442616461 0.12104894314
-0.450442616461 0.121044431759
-0.450442616461 0.121039913937
-0.450442616461 0.121035389671
-0.450442616461 0.121030858957
-0.450442616461 0.12102632179
-0.450442616461 0.121021778167
-0.450442616461 0.121017228085
-0.450442616461 0.121012671538
-0.450442616461 0.121008108522
-0.450442616461 0.121003539035
-0.450442616461 0.120998963072
-0.450442616461 0.120994380629
-0.450442616461 0.120989791702
-0.450442616461 0.120985196287
-0.450442616461 0.12098059438
-0.450442616461 0.120975985977
-0.450442616461 0.120971371074
-0.450442616461 0.120966749668
-0.450442616461 0.120962121754
-0.450442616461 0.120957487328
-0.450442616461 0.120952846387
-0.450442616461 0.120948198926
-0.450442616461 0.120943544942
-0.450442616461 0.120938884431
-0.450442616461 0.120934217387
-0.450442616461 0.120929543809
-0.450442616461 0.120924863691
-0.450442616461 0.120920177031
-0.450442616461 0.120915483823
-0.450442616461 0.120910784064
-0.450442616461 0.12090607775
-0.450442616461 0.120901364877
-0.450442616461 0.120896645441
-0.450442616461 0.120891919438
-0.450442616461 0.120887186864
-0.450442616461 0.120882447716
-0.450442616461 0.120877701989
-0.450442616461 0.12087294968
-0.450442616461 0.120868190784
-0.450442616461 0.120863425298
-0.450442616461 0.120858653218
-0.450442616461 0.120853874539
-0.450442616461 0.120849089259
-0.450442616461 0.120844297372
-0.450442616461 0.120839498875
-0.450442616461 0.120834693764
-0.450442616461 0.120829882036
-0.450442616461 0.120825063686
-0.450442616461 0.12082023871
-0.450442616461 0.120815407104
-0.450442616461 0.120810568865
-0.450442616461 0.120805723989
-0.450442616461 0.120800872472
-0.450442616461 0.120796014309
-0.450442616461 0.120791149498
-0.450442616461 0.120786278033
-0.450442616461 0.120781399912
-0.450442616461 0.120776515129
-0.450442616461 0.120771623682
-0.450442616461 0.120766725567
-0.450442616461 0.120761820779
-0.450442616461 0.120756909315
-0.450442616461 0.12075199117
-0.450442616461 0.120747066342
-0.450442616461 0.120742134825
-0.450442616461 0.120737196617
-0.450442616461 0.120732251712
-0.450442616461 0.120727300108
-0.450442616461 0.120722341801
-0.450442616461 0.120717376786
-0.450442616461 0.12071240506
-0.450442616461 0.120707426618
-0.450442616461 0.120702441458
-0.450442616461 0.120697449574
-0.450442616461 0.120692450964
-0.450442616461 0.120687445623
-0.450442616461 0.120682433547
-0.450442616461 0.120677414733
-0.450442616461 0.120672389177
-0.450442616461 0.120667356875
-0.450442616461 0.120662317822
-0.450442616461 0.120657272016
-0.450442616461 0.120652219452
-0.450442616461 0.120647160126
-0.450442616461 0.120642094035
-0.450442616461 0.120637021174
-0.450442616461 0.12063194154
-0.450442616461 0.120626855129
-0.450442616461 0.120621761937
-0.450442616461 0.120616661961
-0.450442616461 0.120611555195
-0.450442616461 0.120606441638
-0.450442616461 0.120601321284
-0.450442616461 0.120596194129
-0.450442616461 0.120591060171
-0.450442616461 0.120585919405
-0.450442616461 0.120580771827
-0.450442616461 0.120575617434
-0.450442616461 0.120570456221
-0.450442616461 0.120565288185
-0.450442616461 0.120560113322
-0.450442616461 0.120554931628
-0.450442616461 0.120549743099
-0.450442616461 0.120544547731
-0.450442616461 0.120539345522
-0.450442616461 0.120534136466
-0.450442616461 0.120528920559
-0.450442616461 0.120523697799
-0.450442616461 0.120518468182
-0.450442616461 0.120513231702
-0.450442616461 0.120507988358
-0.450442616461 0.120502738144
-0.450442616461 0.120497481057
-0.450442616461 0.120492217093
-0.450442616461 0.120486946248
-0.450442616461 0.120481668519
-0.450442616461 0.120476383902
-0.450442616461 0.120471092392
-0.450442616461 0.120465793987
-0.450442616461 0.120460488682
-0.450442616461 0.120455176473
-0.450442616461 0.120449857357
-0.450442616461 0.12044453133
-0.450442616461 0.120439198387
-0.450442616461 0.120433858526
-0.450442616461 0.120428511742
-0.450442616461 0.120423158032
-0.450442616461 0.120417797392
-0.450442616461 0.120412429818
-0.450442616461 0.120407055306
-0.450442616461 0.120401673852
-0.450442616461 0.120396285453
-0.450442616461 0.120390890104
-0.450442616461 0.120385487803
-0.450442616461 0.120380078545
-0.450442616461 0.120374662326
-0.450442616461 0.120369239143
-0.450442616461 0.120363808992
-0.450442616461 0.120358371869
-0.450442616461 0.12035292777
-0.450442616461 0.120347476691
-0.450442616461 0.12034201863
-0.450442616461 0.120336553581
-0.450442616461 0.120331081541
-0.450442616461 0.120325602507
-0.450442616461 0.120320116474
-0.450442616461 0.120314623439
-0.450442616461 0.120309123398
-0.450442616461 0.120303616348
-0.450442616461 0.120298102284
-0.450442616461 0.120292581202
-0.450442616461 0.1202870531
-0.450442616461 0.120281517973
-0.450442616461 0.120275975817
-0.450442616461 0.120270426629
-0.450442616461 0.120264870404
-0.450442616461 0.12025930714
-0.450442616461 0.120253736832
-0.450442616461 0.120248159477
-0.450442616461 0.120242575071
-0.450442616461 0.12023698361
-0.450442616461 0.12023138509
-0.450442616461 0.120225779507
-0.450442616461 0.120220166859
-0.450442616461 0.12021454714
-0.450442616461 0.120208920348
-0.450442616461 0.120203286479
-0.450442616461 0.120197645528
-0.450442616461 0.120191997492
-0.450442616461 0.120186342368
-0.450442616461 0.120180680151
-0.450442616461 0.120175010838
-0.450442616461 0.120169334425
-0.450442616461 0.120163650909
-0.450442616461 0.120157960285
-0.450442616461 0.12015226255
-0.450442616461 0.1201465577
-0.450442616461 0.120140845732
-0.450442616461 0.120135126641
-0.450442616461 0.120129400424
-0.450442616461 0.120123667078
-0.450442616461 0.120117926598
-0.450442616461 0.12011217898
-0.450442616461 0.120106424222
-0.450442616461 0.120100662319
-0.450442616461 0.120094893268
-0.450442616461 0.120089117064
-0.450442616461 0.120083333705
-0.450442616461 0.120077543186
-0.450442616461 0.120071745504
-0.450442616461 0.120065940654
-0.450442616461 0.120060128634
-0.450442616461 0.12005430944
-0.450442616461 0.120048483067
-0.450442616461 0.120042649513
-0.450442616461 0.120036808773
-0.450442616461 0.120030960844
-0.450442616461 0.120025105721
-0.450442616461 0.120019243402
-0.450442616461 0.120013373883
-0.450442616461 0.120007497159
-0.450442616461 0.120001613228
-0.450442616461 0.119995722085
-0.450442616461 0.119989823727
-0.450442616461 0.11998391815
-0.450442616461 0.11997800535
-0.450442616461 0.119972085324
-0.450442616461 0.119966158068
-0.450442616461 0.119960223578
-0.450442616461 0.119954281851
-0.450442616461 0.119948332883
-0.450442616461 0.11994237667
-0.450442616461 0.119936413209
-0.450442616461 0.119930442495
-0.450442616461 0.119924464526
-0.450442616461 0.119918479297
-0.450442616461 0.119912486805
-0.450442616461 0.119906487046
-0.450442616461 0.119900480016
-0.450442616461 0.119894465713
-0.450442616461 0.119888444131
-0.450442616461 0.119882415267
-0.450442616461 0.119876379119
-0.450442616461 0.119870335681
-0.450442616461 0.119864284951
-0.450442616461 0.119858226925
-0.450442616461 0.119852161598
-0.450442616461 0.119846088968
-0.450442616461 0.119840009031
-0.450442616461 0.119833921782
-0.450442616461 0.119827827219
-0.450442616461 0.119821725338
-0.450442616461 0.119815616135
-0.450442616461 0.119809499606
-0.450442616461 0.119803375748
-0.450442616461 0.119797244557
-0.450442616461 0.119791106029
-0.450442616461 0.119784960161
-0.450442616461 0.119778806949
-0.450442616461 0.11977264639
-0.450442616461 0.11976647848
-0.450442616461 0.119760303214
-0.450442616461 0.11975412059
-0.450442616461 0.119747930604
-0.450442616461 0.119741733252
-0.450442616461 0.119735528531
-0.450442616461 0.119729316436
-0.450442616461 0.119723096965
-0.450442616461 0.119716870113
-0.450442616461 0.119710635878
-0.450442616461 0.119704394255
-0.450442616461 0.11969814524
-0.450442616461 0.119691888831
-0.450442616461 0.119685625022
-0.450442616461 0.119679353812
-0.450442616461 0.119673075196
-0.450442616461 0.11966678917
-0.450442616461 0.119660495732
-0.450442616461 0.119654194876
-0.450442616461 0.119647886601
-0.450442616461 0.119641570901
-0.450442616461 0.119635247773
-0.450442616461 0.119628917215
-0.450442616461 0.119622579221
-0.450442616461 0.11961623379
-0.450442616461 0.119609880916
-0.450442616461 0.119603520596
-0.450442616461 0.119597152827
-0.450442616461 0.119590777605
-0.450442616461 0.119584394926
-0.450442616461 0.119578004787
-0.450442616461 0.119571607185
-0.450442616461 0.119565202115
-0.450442616461 0.119558789574
-0.450442616461 0.119552369559
-0.450442616461 0.119545942065
-0.450442616461 0.119539507089
-0.450442616461 0.119533064628
-0.450442616461 0.119526614678
-0.450442616461 0.119520157235
-0.450442616461 0.119513692296
-0.450442616461 0.119507219857
-0.450442616461 0.119500739915
-0.450442616461 0.119494252466
-0.450442616461 0.119487757506
-0.450442616461 0.119481255032
-0.450442616461 0.11947474504
-0.450442616461 0.119468227526
-0.450442616461 0.119461702488
-0.450442616461 0.119455169921
-0.450442616461 0.119448629822
-0.450442616461 0.119442082187
-0.450442616461 0.119435527013
-0.450442616461 0.119428964295
-0.450442616461 0.119422394032
-0.450442616461 0.119415816218
-0.450442616461 0.11940923085
-0.450442616461 0.119402637925
-0.450442616461 0.11939603744
-0.450442616461 0.119389429389
-0.450442616461 0.119382813771
-0.450442616461 0.119376190582
-0.450442616461 0.119369559817
-0.450442616461 0.119362921473
-0.450442616461 0.119356275547
-0.450442616461 0.119349622036
-0.450442616461 0.119342960935
-0.450442616461 0.11933629224
-0.450442616461 0.11932961595
-0.450442616461 0.119322932059
-0.450442616461 0.119316240564
-0.450442616461 0.119309541463
-0.450442616461 0.11930283475
-0.450442616461 0.119296120423
-0.450442616461 0.119289398478
-0.450442616461 0.119282668912
-0.450442616461 0.11927593172
-0.450442616461 0.1192691869
-0.450442616461 0.119262434448
-0.450442616461 0.11925567436
-0.450442616461 0.119248906633
-0.450442616461 0.119242131263
-0.450442616461 0.119235348247
-0.450442616461 0.11922855758
-0.450442616461 0.119221759261
-0.450442616461 0.119214953284
-0.450442616461 0.119208139647
-0.450442616461 0.119201318345
-0.450442616461 0.119194489376
-0.450442616461 0.119187652736
-0.450442616461 0.119180808421
-0.450442616461 0.119173956428
-0.450442616461 0.119167096754
-0.450442616461 0.119160229393
-0.450442616461 0.119153354344
-0.450442616461 0.119146471603
-0.450442616461 0.119139581166
-0.450442616461 0.119132683029
-0.450442616461 0.119125777189
-0.450442616461 0.119118863643
-0.450442616461 0.119111942387
-0.450442616461 0.119105013417
-0.450442616461 0.11909807673
-0.450442616461 0.119091132322
-0.450442616461 0.119084180191
-0.450442616461 0.119077220332
-0.450442616461 0.119070252741
-0.450442616461 0.119063277416
-0.450442616461 0.119056294353
-0.450442616461 0.119049303548
-0.450442616461 0.119042304997
-0.450442616461 0.119035298698
-0.450442616461 0.119028284647
-0.450442616461 0.11902126284
-0.450442616461 0.119014233274
-0.450442616461 0.119007195945
-0.450442616461 0.119000150849
-0.450442616461 0.118993097984
-0.450442616461 0.118986037346
-0.450442616461 0.11897896893
-0.450442616461 0.118971892735
-0.450442616461 0.118964808755
-0.450442616461 0.118957716988
-0.450442616461 0.118950617431
-0.450442616461 0.118943510079
-0.450442616461 0.118936394929
-0.450442616461 0.118929271978
-0.450442616461 0.118922141222
-0.450442616461 0.118915002658
-0.450442616461 0.118907856282
-0.450442616461 0.118900702091
-0.450442616461 0.118893540081
-0.450442616461 0.118886370249
-0.450442616461 0.118879192591
-0.450442616461 0.118872007104
-0.450442616461 0.118864813784
-0.450442616461 0.118857612628
-0.450442616461 0.118850403632
-0.450442616461 0.118843186794
-0.450442616461 0.118835962108
-0.450442616461 0.118828729572
-0.450442616461 0.118821489183
-0.450442616461 0.118814240937
-0.450442616461 0.11880698483
-0.450442616461 0.118799720859
-0.450442616461 0.11879244902
-0.450442616461 0.118785169311
-0.450442616461 0.118777881727
-0.450442616461 0.118770586265
-0.450442616461 0.118763282922
-0.450442616461 0.118755971694
-0.450442616461 0.118748652578
-0.450442616461 0.11874132557
-0.450442616461 0.118733990667
-0.450442616461 0.118726647865
-0.450442616461 0.11871929716
-0.450442616461 0.118711938551
-0.450442616461 0.118704572032
-0.450442616461 0.1186971976
-0.450442616461 0.118689815253
-0.450442616461 0.118682424986
-0.450442616461 0.118675026796
-0.450442616461 0.11866762068
-0.450442616461 0.118660206634
-0.450442616461 0.118652784655
-0.450442616461 0.118645354739
-0.450442616461 0.118637916882
-0.450442616461 0.118630471083
-0.450442616461 0.118623017336
-0.450442616461 0.118615555638
-0.450442616461 0.118608085987
-0.450442616461 0.118600608378
-0.450442616461 0.118593122809
-0.450442616461 0.118585629275
-0.450442616461 0.118578127773
-0.450442616461 0.118570618301
-0.450442616461 0.118563100853
-0.450442616461 0.118555575428
-0.450442616461 0.118548042021
-0.450442616461 0.118540500629
-0.450442616461 0.118532951249
-0.450442616461 0.118525393878
-0.450442616461 0.118517828511
-0.450442616461 0.118510255145
-0.450442616461 0.118502673777
-0.450442616461 0.118495084404
-0.450442616461 0.118487487022
-0.450442616461 0.118479881628
-0.450442616461 0.118472268217
-0.450442616461 0.118464646788
-0.450442616461 0.118457017336
-0.450442616461 0.118449379858
-0.450442616461 0.118441734351
-0.450442616461 0.11843408081
-0.450442616461 0.118426419234
-0.450442616461 0.118418749618
-0.450442616461 0.118411071958
-0.450442616461 0.118403386252
-0.450442616461 0.118395692497
-0.450442616461 0.118387990687
-0.450442616461 0.118380280822
-0.450442616461 0.118372562895
-0.450442616461 0.118364836906
-0.450442616461 0.118357102849
-0.450442616461 0.118349360722
-0.450442616461 0.118341610521
-0.450442616461 0.118333852243
-0.450442616461 0.118326085885
-0.450442616461 0.118318311442
-0.450442616461 0.118310528912
-0.450442616461 0.118302738291
-0.450442616461 0.118294939576
-0.450442616461 0.118287132764
-0.450442616461 0.11827931785
-0.450442616461 0.118271494832
-0.450442616461 0.118263663707
-0.450442616461 0.11825582447
-0.450442616461 0.118247977118
-0.450442616461 0.118240121649
-0.450442616461 0.118232258058
-0.450442616461 0.118224386343
-0.450442616461 0.118216506499
-0.450442616461 0.118208618524
-0.450442616461 0.118200722414
-0.450442616461 0.118192818166
-0.450442616461 0.118184905776
-0.450442616461 0.118176985241
-0.450442616461 0.118169056557
-0.450442616461 0.118161119722
-0.450442616461 0.118153174732
-0.450442616461 0.118145221583
-0.450442616461 0.118137260272
-0.450442616461 0.118129290796
-0.450442616461 0.118121313151
-0.450442616461 0.118113327334
-0.450442616461 0.118105333342
-0.450442616461 0.118097331171
-0.450442616461 0.118089320817
-0.450442616461 0.118081302279
-0.450442616461 0.118073275551
-0.450442616461 0.118065240631
-0.450442616461 0.118057197515
-0.450442616461 0.118049146201
-0.450442616461 0.118041086684
-0.450442616461 0.118033018961
-0.450442616461 0.118024943029
-0.450442616461 0.118016858885
-0.450442616461 0.118008766525
-0.450442616461 0.118000665946
-0.450442616461 0.117992557144
-0.450442616461 0.117984440117
-0.450442616461 0.11797631486
-0.450442616461 0.117968181371
-0.450442616461 0.117960039645
-0.450442616461 0.117951889681
-0.450442616461 0.117943731474
-0.450442616461 0.11793556502
-0.450442616461 0.117927390318
-0.450442616461 0.117919207362
-0.450442616461 0.117911016151
-0.450442616461 0.117902816681
-0.450442616461 0.117894608947
-0.450442616461 0.117886392948
-0.450442616461 0.117878168679
-0.450442616461 0.117869936137
-0.450442616461 0.11786169532
-0.450442616461 0.117853446223
-0.450442616461 0.117845188843
-0.450442616461 0.117836923177
-0.450442616461 0.117828649221
-0.450442616461 0.117820366973
-0.450442616461 0.117812076429
-0.450442616461 0.117803777585
-0.450442616461 0.117795470439
-0.450442616461 0.117787154986
-0.450442616461 0.117778831224
-0.450442616461 0.11777049915
-0.450442616461 0.117762158759
-0.450442616461 0.117753810048
-0.450442616461 0.117745453015
-0.450442616461 0.117737087656
-0.450442616461 0.117728713968
-0.450442616461 0.117720331947
-0.450442616461 0.11771194159
-0.450442616461 0.117703542893
-0.450442616461 0.117695135854
-0.450442616461 0.117686720469
-0.450442616461 0.117678296734
-0.450442616461 0.117669864647
-0.450442616461 0.117661424204
-0.450442616461 0.117652975402
-0.450442616461 0.117644518237
-0.450442616461 0.117636052706
-0.450442616461 0.117627578806
-0.450442616461 0.117619096534
-0.450442616461 0.117610605886
-0.450442616461 0.117602106858
-0.450442616461 0.117593599449
-0.450442616461 0.117585083653
-0.450442616461 0.117576559469
-0.450442616461 0.117568026892
-0.450442616461 0.117559485919
-0.450442616461 0.117550936548
-0.450442616461 0.117542378774
-0.450442616461 0.117533812595
-0.450442616461 0.117525238007
-0.450442616461 0.117516655006
-0.450442616461 0.117508063591
-0.450442616461 0.117499463756
-0.450442616461 0.1174908555
-0.450442616461 0.117482238818
-0.450442616461 0.117473613708
-0.450442616461 0.117464980166
-0.450442616461 0.117456338188
-0.450442616461 0.117447687772
-0.450442616461 0.117439028914
-0.450442616461 0.117430361612
-0.450442616461 0.11742168586
-0.450442616461 0.117413001658
-0.450442616461 0.117404309
-0.450442616461 0.117395607884
-0.450442616461 0.117386898306
-0.450442616461 0.117378180264
-0.450442616461 0.117369453754
-0.450442616461 0.117360718772
-0.450442616461 0.117351975316
-0.450442616461 0.117343223382
-0.450442616461 0.117334462967
-0.450442616461 0.117325694067
-0.450442616461 0.117316916679
-0.450442616461 0.117308130801
-0.450442616461 0.117299336428
-0.450442616461 0.117290533558
-0.450442616461 0.117281722186
-0.450442616461 0.117272902311
-0.450442616461 0.117264073929
-0.450442616461 0.117255237035
-0.450442616461 0.117246391628
-0.450442616461 0.117237537704
-0.450442616461 0.117228675259
-0.450442616461 0.117219804291
-0.450442616461 0.117210924796
-0.450442616461 0.11720203677
-0.450442616461 0.117193140211
-0.450442616461 0.117184235115
-0.450442616461 0.117175321479
-0.450442616461 0.1171663993
-0.450442616461 0.117157468575
-0.450442616461 0.117148529299
-0.450442616461 0.117139581471
-0.450442616461 0.117130625086
-0.450442616461 0.117121660142
-0.450442616461 0.117112686635
-0.450442616461 0.117103704562
-0.450442616461 0.117094713919
-0.450442616461 0.117085714704
-0.450442616461 0.117076706914
-0.450442616461 0.117067690544
-0.450442616461 0.117058665592
-0.450442616461 0.117049632054
-0.450442616461 0.117040589928
-0.450442616461 0.117031539209
-0.450442616461 0.117022479895
-0.450442616461 0.117013411983
-0.450442616461 0.117004335469
-0.450442616461 0.11699525035
-0.450442616461 0.116986156623
-0.450442616461 0.116977054284
-0.450442616461 0.11696794333
-0.450442616461 0.116958823759
-0.450442616461 0.116949695566
-0.450442616461 0.116940558749
-0.450442616461 0.116931413304
-0.450442616461 0.116922259228
-0.450442616461 0.116913096518
-0.450442616461 0.116903925171
-0.450442616461 0.116894745183
-0.450442616461 0.116885556552
-0.450442616461 0.116876359273
-0.450442616461 0.116867153344
-0.450442616461 0.116857938761
-0.450442616461 0.116848715522
-0.450442616461 0.116839483623
-0.450442616461 0.11683024306
-0.450442616461 0.116820993831
-0.450442616461 0.116811735933
-0.450442616461 0.116802469361
-0.450442616461 0.116793194114
-0.450442616461 0.116783910187
-0.450442616461 0.116774617578
-0.450442616461 0.116765316283
-0.450442616461 0.116756006299
-0.450442616461 0.116746687622
-0.450442616461 0.116737360251
-0.450442616461 0.11672802418
-0.450442616461 0.116718679408
-0.450442616461 0.116709325931
-0.450442616461 0.116699963746
-0.450442616461 0.116690592849
-0.450442616461 0.116681213237
-0.450442616461 0.116671824908
-0.450442616461 0.116662427857
-0.450442616461 0.116653022083
-0.450442616461 0.11664360758
-0.450442616461 0.116634184347
-0.450442616461 0.11662475238
-0.450442616461 0.116615311676
-0.450442616461 0.116605862232
-0.450442616461 0.116596404044
-0.450442616461 0.116586937109
-0.450442616461 0.116577461424
-0.450442616461 0.116567976987
-0.450442616461 0.116558483792
-0.450442616461 0.116548981839
-0.450442616461 0.116539471122
-0.450442616461 0.11652995164
-0.450442616461 0.116520423389
-0.450442616461 0.116510886365
-0.450442616461 0.116501340566
-0.450442616461 0.116491785988
-0.450442616461 0.116482222628
-0.450442616461 0.116472650483
-0.450442616461 0.116463069549
-0.450442616461 0.116453479825
-0.450442616461 0.116443881305
-0.450442616461 0.116434273988
-0.450442616461 0.11642465787
-0.450442616461 0.116415032947
-0.450442616461 0.116405399217
-0.450442616461 0.116395756677
-0.450442616461 0.116386105322
-0.450442616461 0.116376445151
-0.450442616461 0.116366776159
-0.450442616461 0.116357098345
-0.450442616461 0.116347411703
-0.450442616461 0.116337716232
-0.450442616461 0.116328011928
-0.450442616461 0.116318298789
-0.450442616461 0.116308576809
-0.450442616461 0.116298845988
-0.450442616461 0.116289106321
-0.450442616461 0.116279357805
-0.450442616461 0.116269600437
-0.450442616461 0.116259834214
-0.450442616461 0.116250059133
-0.450442616461 0.11624027519
-0.450442616461 0.116230482383
-0.450442616461 0.116220680708
-0.450442616461 0.116210870162
-0.450442616461 0.116201050742
-0.450442616461 0.116191222445
-0.450442616461 0.116181385267
-0.450442616461 0.116171539205
-0.450442616461 0.116161684257
-0.450442616461 0.116151820419
-0.450442616461 0.116141947687
-0.450442616461 0.11613206606
-0.450442616461 0.116122175533
-0.450442616461 0.116112276103
-0.450442616461 0.116102367767
-0.450442616461 0.116092450523
-0.450442616461 0.116082524367
-0.450442616461 0.116072589295
-0.450442616461 0.116062645305
-0.450442616461 0.116052692393
-0.450442616461 0.116042730557
-0.450442616461 0.116032759792
-0.450442616461 0.116022780097
-0.450442616461 0.116012791468
-0.450442616461 0.116002793901
-0.450442616461 0.115992787394
-0.450442616461 0.115982771943
-0.450442616461 0.115972747545
-0.450442616461 0.115962714197
-0.450442616461 0.115952671897
-0.450442616461 0.11594262064
-0.450442616461 0.115932560423
-0.450442616461 0.115922491244
-0.450442616461 0.1159124131
-0.450442616461 0.115902325987
-0.450442616461 0.115892229901
-0.450442616461 0.115882124841
-0.450442616461 0.115872010802
-0.450442616461 0.115861887782
-0.450442616461 0.115851755778
-0.450442616461 0.115841614785
-0.450442616461 0.115831464802
-0.450442616461 0.115821305825
-0.450442616461 0.115811137851
-0.450442616461 0.115800960877
-0.450442616461 0.115790774899
-0.450442616461 0.115780579915
-0.450442616461 0.115770375921
-0.450442616461 0.115760162915
-0.450442616461 0.115749940892
-0.450442616461 0.115739709851
-0.450442616461 0.115729469787
-0.450442616461 0.115719220698
-0.450442616461 0.115708962581
-0.450442616461 0.115698695432
-0.450442616461 0.115688419248
-0.450442616461 0.115678134027
-0.450442616461 0.115667839765
-0.450442616461 0.115657536458
-0.450442616461 0.115647224105
-0.450442616461 0.115636902701
-0.450442616461 0.115626572243
-0.450442616461 0.115616232729
-0.450442616461 0.115605884155
-0.450442616461 0.115595526519
-0.450442616461 0.115585159816
-0.450442616461 0.115574784045
-0.450442616461 0.115564399201
-0.450442616461 0.115554005282
-0.450442616461 0.115543602285
-0.450442616461 0.115533190206
-0.450442616461 0.115522769042
-0.450442616461 0.115512338791
-0.450442616461 0.115501899449
-0.450442616461 0.115491451012
-0.450442616461 0.115480993479
-0.450442616461 0.115470526845
-0.450442616461 0.115460051108
-0.450442616461 0.115449566265
-0.450442616461 0.115439072312
-0.450442616461 0.115428569246
-0.450442616461 0.115418057064
-0.450442616461 0.115407535764
-0.450442616461 0.115397005341
-0.450442616461 0.115386465794
-0.450442616461 0.115375917118
-0.450442616461 0.115365359311
-0.450442616461 0.115354792369
-0.450442616461 0.11534421629
-0.450442616461 0.11533363107
-0.450442616461 0.115323036707
-0.450442616461 0.115312433196
-0.450442616461 0.115301820536
-0.450442616461 0.115291198722
-0.450442616461 0.115280567752
-0.450442616461 0.115269927623
-0.450442616461 0.115259278332
-0.450442616461 0.115248619875
-0.450442616461 0.11523795225
-0.450442616461 0.115227275453
-0.450442616461 0.115216589481
-0.450442616461 0.115205894331
-0.450442616461 0.11519519
-0.450442616461 0.115184476485
-0.450442616461 0.115173753783
-0.450442616461 0.115163021891
-0.450442616461 0.115152280806
-0.450442616461 0.115141530524
-0.450442616461 0.115130771042
-0.450442616461 0.115120002358
-0.450442616461 0.115109224468
-0.450442616461 0.115098437369
-0.450442616461 0.115087641058
-0.450442616461 0.115076835533
-0.450442616461 0.115066020789
-0.450442616461 0.115055196824
-0.450442616461 0.115044363635
-0.450442616461 0.115033521219
-0.450442616461 0.115022669572
-0.450442616461 0.115011808691
-0.450442616461 0.115000938574
-0.450442616461 0.114990059217
-0.450442616461 0.114979170618
-0.450442616461 0.114968272773
-0.450442616461 0.114957365678
-0.450442616461 0.114946449332
-0.450442616461 0.11493552373
-0.450442616461 0.114924588871
-0.450442616461 0.11491364475
-0.450442616461 0.114902691365
-0.450442616461 0.114891728712
-0.450442616461 0.114880756789
-0.450442616461 0.114869775592
-0.450442616461 0.114858785119
-0.450442616461 0.114847785366
-0.450442616461 0.11483677633
-0.450442616461 0.114825758008
-0.450442616461 0.114814730397
-0.450442616461 0.114803693494
-0.450442616461 0.114792647296
-0.450442616461 0.1147815918
-0.450442616461 0.114770527003
-0.450442616461 0.114759452901
-0.450442616461 0.114748369492
-0.450442616461 0.114737276773
-0.450442616461 0.114726174739
-0.450442616461 0.11471506339
-0.450442616461 0.11470394272
-0.450442616461 0.114692812728
-0.450442616461 0.11468167341
-0.450442616461 0.114670524764
-0.450442616461 0.114659366785
-0.450442616461 0.114648199471
-0.450442616461 0.114637022819
-0.450442616461 0.114625836826
-0.450442616461 0.114614641489
-0.450442616461 0.114603436804
-0.450442616461 0.11459222277
-0.450442616461 0.114580999381
-0.450442616461 0.114569766637
-0.450442616461 0.114558524532
-0.450442616461 0.114547273066
-0.450442616461 0.114536012233
-0.450442616461 0.114524742032
-0.450442616461 0.114513462459
-0.450442616461 0.114502173511
-0.450442616461 0.114490875186
-0.450442616461 0.114479567479
-0.450442616461 0.114468250389
-0.450442616461 0.114456923911
-0.450442616461 0.114445588043
-0.450442616461 0.114434242782
-0.450442616461 0.114422888125
-0.450442616461 0.114411524069
-0.450442616461 0.11440015061
-0.450442616461 0.114388767746
-0.450442616461 0.114377375474
-0.450442616461 0.11436597379
-0.450442616461 0.114354562691
-0.450442616461 0.114343142175
-0.450442616461 0.114331712238
-0.450442616461 0.114320272878
-0.450442616461 0.11430882409
-0.450442616461 0.114297365873
-0.450442616461 0.114285898223
-0.450442616461 0.114274421138
-0.450442616461 0.114262934613
-0.450442616461 0.114251438646
-0.450442616461 0.114239933234
-0.450442616461 0.114228418375
-0.450442616461 0.114216894064
-0.450442616461 0.114205360299
-0.450442616461 0.114193817076
-0.450442616461 0.114182264394
-0.450442616461 0.114170702248
-0.450442616461 0.114159130635
-0.450442616461 0.114147549554
-0.450442616461 0.114135959
-0.450442616461 0.11412435897
-0.450442616461 0.114112749462
-0.450442616461 0.114101130472
-0.450442616461 0.114089501998
-0.450442616461 0.114077864036
-0.450442616461 0.114066216584
-0.450442616461 0.114054559637
-0.450442616461 0.114042893194
-0.450442616461 0.114031217252
-0.450442616461 0.114019531806
-0.450442616461 0.114007836854
-0.450442616461 0.113996132394
-0.450442616461 0.113984418422
-0.450442616461 0.113972694934
-0.450442616461 0.113960961929
-0.450442616461 0.113949219402
-0.450442616461 0.113937467352
-0.450442616461 0.113925705774
-0.450442616461 0.113913934667
-0.450442616461 0.113902154026
-0.450442616461 0.113890363848
-0.450442616461 0.113878564132
-0.450442616461 0.113866754873
-0.450442616461 0.113854936069
-0.450442616461 0.113843107717
-0.450442616461 0.113831269813
-0.450442616461 0.113819422355
-0.450442616461 0.113807565339
-0.450442616461 0.113795698763
-0.450442616461 0.113783822624
-0.450442616461 0.113771936918
-0.450442616461 0.113760041642
-0.450442616461 0.113748136794
-0.450442616461 0.11373622237
-0.450442616461 0.113724298368
-0.450442616461 0.113712364784
-0.450442616461 0.113700421615
-0.450442616461 0.113688468859
-0.450442616461 0.113676506511
-0.450442616461 0.11366453457
-0.450442616461 0.113652553033
-0.450442616461 0.113640561895
-0.450442616461 0.113628561155
-0.450442616461 0.113616550809
-0.450442616461 0.113604530853
-0.450442616461 0.113592501286
-0.450442616461 0.113580462105
-0.450442616461 0.113568413305
-0.450442616461 0.113556354884
-0.450442616461 0.113544286839
-0.450442616461 0.113532209167
-0.450442616461 0.113520121866
-0.450442616461 0.113508024931
-0.450442616461 0.11349591836
-0.450442616461 0.11348380215
-0.450442616461 0.113471676298
-0.450442616461 0.113459540801
-0.450442616461 0.113447395655
-0.450442616461 0.113435240859
-0.450442616461 0.113423076408
-0.450442616461 0.1134109023
-0.450442616461 0.113398718532
-0.450442616461 0.113386525101
-0.450442616461 0.113374322003
-0.450442616461 0.113362109237
-0.450442616461 0.113349886798
-0.450442616461 0.113337654684
-0.450442616461 0.113325412891
-0.450442616461 0.113313161417
-0.450442616461 0.113300900259
-0.450442616461 0.113288629414
-0.450442616461 0.113276348878
-0.450442616461 0.113264058649
-0.450442616461 0.113251758723
-0.450442616461 0.113239449098
-0.450442616461 0.113227129771
-0.450442616461 0.113214800738
-0.450442616461 0.113202461997
-0.450442616461 0.113190113544
-0.450442616461 0.113177755378
-0.450442616461 0.113165387493
-0.450442616461 0.113153009888
-0.450442616461 0.11314062256
-0.450442616461 0.113128225505
-0.450442616461 0.113115818721
-0.450442616461 0.113103402204
-0.450442616461 0.113090975952
-0.450442616461 0.113078539961
-0.450442616461 0.113066094229
-0.450442616461 0.113053638752
-0.450442616461 0.113041173528
-0.450442616461 0.113028698553
-0.450442616461 0.113016213825
-0.450442616461 0.11300371934
-0.450442616461 0.112991215096
-0.450442616461 0.112978701089
-0.450442616461 0.112966177317
-0.450442616461 0.112953643776
-0.450442616461 0.112941100463
-0.450442616461 0.112928547376
-0.450442616461 0.112915984511
-0.450442616461 0.112903411866
-0.450442616461 0.112890829437
-0.450442616461 0.112878237222
-0.450442616461 0.112865635217
-0.450442616461 0.112853023419
-0.450442616461 0.112840401826
-0.450442616461 0.112827770434
-0.450442616461 0.112815129241
-0.450442616461 0.112802478243
-0.450442616461 0.112789817438
-0.450442616461 0.112777146822
-0.450442616461 0.112764466392
-0.450442616461 0.112751776146
-0.450442616461 0.11273907608
-0.450442616461 0.112726366192
-0.450442616461 0.112713646478
-0.450442616461 0.112700916935
-0.450442616461 0.112688177561
-0.450442616461 0.112675428352
-0.450442616461 0.112662669306
-0.450442616461 0.112649900419
-0.450442616461 0.112637121689
-0.450442616461 0.112624333111
-0.450442616461 0.112611534685
-0.450442616461 0.112598726406
-0.450442616461 0.112585908271
-0.450442616461 0.112573080278
-0.450442616461 0.112560242423
-0.450442616461 0.112547394703
-0.450442616461 0.112534537117
-0.450442616461 0.112521669659
-0.450442616461 0.112508792328
-0.450442616461 0.11249590512
-0.450442616461 0.112483008033
-0.450442616461 0.112470101064
-0.450442616461 0.112457184209
-0.450442616461 0.112444257465
-0.450442616461 0.11243132083
-0.450442616461 0.1124183743
-0.450442616461 0.112405417873
-0.450442616461 0.112392451545
-0.450442616461 0.112379475314
-0.450442616461 0.112366489176
-0.450442616461 0.112353493129
-0.450442616461 0.11234048717
-0.450442616461 0.112327471295
-0.450442616461 0.112314445501
-0.450442616461 0.112301409786
-0.450442616461 0.112288364147
-0.450442616461 0.11227530858
-0.450442616461 0.112262243083
-0.450442616461 0.112249167652
-0.450442616461 0.112236082285
-0.450442616461 0.112222986979
-0.450442616461 0.11220988173
-0.450442616461 0.112196766536
-0.450442616461 0.112183641393
-0.450442616461 0.112170506299
-0.450442616461 0.112157361251
-0.450442616461 0.112144206245
-0.450442616461 0.112131041279
-0.450442616461 0.11211786635
-0.450442616461 0.112104681455
-0.450442616461 0.11209148659
-0.450442616461 0.112078281752
-0.450442616461 0.11206506694
-0.450442616461 0.112051842149
-0.450442616461 0.112038607377
-0.450442616461 0.112025362621
-0.450442616461 0.112012107878
-0.450442616461 0.111998843144
-0.450442616461 0.111985568417
-0.450442616461 0.111972283694
-0.450442616461 0.111958988971
-0.450442616461 0.111945684247
-0.450442616461 0.111932369517
-0.450442616461 0.111919044779
-0.450442616461 0.11190571003
-0.450442616461 0.111892365267
-0.450442616461 0.111879010487
-0.450442616461 0.111865645687
-0.450442616461 0.111852270863
-0.450442616461 0.111838886014
-0.450442616461 0.111825491135
-0.450442616461 0.111812086224
-0.450442616461 0.111798671278
-0.450442616461 0.111785246295
-0.450442616461 0.11177181127
-0.450442616461 0.111758366201
-0.450442616461 0.111744911085
-0.450442616461 0.111731445919
-0.450442616461 0.1117179707
-0.450442616461 0.111704485426
-0.450442616461 0.111690990092
-0.450442616461 0.111677484696
-0.450442616461 0.111663969236
-0.450442616461 0.111650443707
-0.450442616461 0.111636908108
-0.450442616461 0.111623362434
-0.450442616461 0.111609806684
-0.450442616461 0.111596240854
-0.450442616461 0.111582664941
-0.450442616461 0.111569078943
-0.450442616461 0.111555482855
-0.450442616461 0.111541876676
-0.450442616461 0.111528260402
-0.450442616461 0.11151463403
-0.450442616461 0.111500997557
-0.450442616461 0.111487350981
-0.450442616461 0.111473694298
-0.450442616461 0.111460027505
-0.450442616461 0.111446350599
-0.450442616461 0.111432663578
-0.450442616461 0.111418966438
-0.450442616461 0.111405259176
-0.450442616461 0.11139154179
-0.450442616461 0.111377814276
-0.450442616461 0.111364076632
-0.450442616461 0.111350328853
-0.450442616461 0.111336570939
-0.450442616461 0.111322802884
-0.450442616461 0.111309024687
-0.450442616461 0.111295236345
-0.450442616461 0.111281437854
-0.450442616461 0.111267629211
-0.450442616461 0.111253810414
-0.450442616461 0.11123998146
-0.450442616461 0.111226142345
-0.450442616461 0.111212293066
-0.450442616461 0.111198433621
-0.450442616461 0.111184564007
-0.450442616461 0.11117068422
-0.450442616461 0.111156794258
-0.450442616461 0.111142894117
-0.450442616461 0.111128983795
-0.450442616461 0.111115063289
-0.450442616461 0.111101132595
-0.450442616461 0.111087191711
-0.450442616461 0.111073240633
-0.450442616461 0.11105927936
-0.450442616461 0.111045307886
-0.450442616461 0.111031326211
-0.450442616461 0.11101733433
-0.450442616461 0.111003332241
-0.450442616461 0.110989319941
-0.450442616461 0.110975297427
-0.450442616461 0.110961264695
-0.450442616461 0.110947221743
-0.450442616461 0.110933168568
-0.450442616461 0.110919105167
-0.450442616461 0.110905031536
-0.450442616461 0.110890947673
-0.450442616461 0.110876853575
-0.450442616461 0.11086274924
-0.450442616461 0.110848634662
-0.450442616461 0.110834509841
-0.450442616461 0.110820374773
-0.450442616461 0.110806229454
-0.450442616461 0.110792073883
-0.450442616461 0.110777908055
-0.450442616461 0.110763731969
-0.450442616461 0.11074954562
-0.450442616461 0.110735349006
-0.450442616461 0.110721142124
-0.450442616461 0.110706924972
-0.450442616461 0.110692697545
-0.450442616461 0.110678459841
-0.450442616461 0.110664211857
-0.450442616461 0.110649953591
-0.450442616461 0.110635685038
-0.450442616461 0.110621406196
-0.450442616461 0.110607117063
-0.450442616461 0.110592817634
-0.450442616461 0.110578507908
-0.450442616461 0.11056418788
-0.450442616461 0.110549857549
-0.450442616461 0.110535516911
-0.450442616461 0.110521165963
-0.450442616461 0.110506804702
-0.450442616461 0.110492433125
-0.450442616461 0.11047805123
-0.450442616461 0.110463659012
-0.450442616461 0.11044925647
-0.450442616461 0.1104348436
-0.450442597657 0.110420418279
-0.450442509572 0.11040597481
-0.450442349433 0.110391512871
-0.450442117239 0.110377032455
-0.450441812989 0.110362533553
-0.450441436685 0.110348016156
-0.450440988325 0.110333480257
-0.450440467909 0.110318925846
-0.450439875438 0.110304352915
-0.45043921091 0.110289761457
-0.450438474326 0.110275151462
-0.450437665686 0.110260522923
-0.450436784988 0.11024587583
-0.450435832232 0.110231210176
-0.450434807418 0.110216525952
-0.450433710546 0.110201823149
-0.450432541615 0.11018710176
-0.450431300624 0.110172361776
-0.450429987572 0.110157603189
-0.45042860246 0.11014282599
-0.450427145286 0.110128030172
-0.45042561605 0.110113215725
-0.450424014751 0.110098382641
-0.450422341389 0.110083530912
-0.450420595962 0.11006866053
-0.450418778469 0.110053771486
-0.45041688891 0.110038863773
-0.450414927284 0.110023937381
-0.45041289359 0.110008992302
-0.450410787826 0.109994028528
-0.450408609993 0.109979046052
-0.450406360089 0.109964044864
-0.450404038112 0.109949024956
-0.450401644062 0.109933986319
-0.450399177937 0.109918928947
-0.450396639737 0.10990385283
-0.45039402946 0.109888757959
-0.450391347105 0.109873644328
-0.45038859267 0.109858511927
-0.450385766154 0.109843360748
-0.450382867557 0.109828190783
-0.450379896876 0.109813002024
-0.45037685411 0.109797794462
-0.450373739257 0.109782568089
-0.450370552317 0.109767322898
-0.450367293287 0.109752058878
-0.450363962167 0.109736776023
-0.450360558954 0.109721474325
-0.450357083646 0.109706153774
-0.450353536243 0.109690814363
-0.450349916742 0.109675456083
-0.450346225141 0.109660078926
-0.45034246144 0.109644682885
-0.450338625636 0.10962926795
-0.450334717727 0.109613834114
-0.450330737711 0.109598381367
-0.450326685587 0.109582909704
-0.450322561352 0.109567419113
-0.450318365005 0.109551909589
-0.450314096543 0.109536381122
-0.450309755965 0.109520833704
-0.450305343269 0.109505267328
-0.450300858451 0.109489681984
-0.450296301511 0.109474077665
-0.450291672445 0.109458454363
-0.450286971252 0.109442812069
-0.45028219793 0.109427150775
-0.450277352476 0.109411470473
-0.450272434887 0.109395771154
-0.450267445162 0.109380052812
-0.450262383298 0.109364315437
-0.450257249293 0.109348559021
-0.450252043144 0.109332783557
-0.450246764848 0.109316989035
-0.450241414404 0.109301175449
-0.450235991808 0.109285342789
-0.450230497058 0.109269491048
-0.450224930151 0.109253620217
-0.450219291085 0.109237730289
-0.450213579857 0.109221821254
-0.450207796464 0.109205893106
-0.450201940904 0.109189945836
-0.450196013172 0.109173979436
-0.450190013268 0.109157993897
-0.450183941188 0.109141989212
-0.450177796928 0.109125965372
-0.450171580486 0.10910992237
-0.450165291859 0.109093860197
-0.450158931045 0.109077778846
-0.450152498039 0.109061678307
-0.450145992838 0.109045558574
-0.450139415441 0.109029419637
-0.450132765843 0.10901326149
-0.450126044041 0.108997084123
-0.450119250032 0.108980887528
-0.450112383813 0.108964671699
-0.450105445381 0.108948436626
-0.450098434731 0.108932182301
-0.450091351862 0.108915908717
-0.450084196769 0.108899615865
-0.450076969448 0.108883303738
-0.450069669897 0.108866972326
-0.450062298112 0.108850621623
-0.450054854089 0.108834251621
-0.450047337825 0.10881786231
-0.450039749317 0.108801453683
-0.450032088559 0.108785025733
-0.45002435555 0.10876857845
-0.450016550285 0.108752111828
-0.45000867276 0.108735625857
-0.450000722971 0.108719120531
-0.449992700915 0.10870259584
-0.449984606588 0.108686051778
-0.449976439986 0.108669488335
-0.449968201105 0.108652905505
-0.449959889941 0.108636303278
-0.44995150649 0.108619681647
-0.449943050748 0.108603040604
-0.449934522711 0.108586380141
-0.449925922375 0.108569700251
-0.449917249735 0.108553000924
-0.449908504788 0.108536282153
-0.449899687529 0.10851954393
-0.449890797954 0.108502786247
-0.449881836058 0.108486009096
-0.449872801839 0.10846921247
-0.44986369529 0.10845239636
-0.449854516408 0.108435560757
-0.449845265188 0.108418705655
-0.449835941625 0.108401831046
-0.449826545716 0.108384936921
-0.449817077456 0.108368023272
-0.44980753684 0.108351090092
-0.449797923864 0.108334137372
-0.449788238522 0.108317165105
-0.44977848081 0.108300173282
-0.449768650725 0.108283161897
-0.449758748259 0.10826613094
-0.44974877341 0.108249080404
-0.449738726172 0.108232010281
-0.449728606541 0.108214920563
-0.449718414511 0.108197811243
-0.449708150077 0.108180682311
-0.449697813235 0.108163533762
-0.449687403979 0.108146365585
-0.449676922305 0.108129177774
-0.449666368208 0.108111970321
-0.449655741682 0.108094743218
-0.449645042722 0.108077496457
-0.449634271323 0.108060230029
-0.44962342748 0.108042943928
-0.449612511188 0.108025638145
-0.449601522441 0.108008312673
-0.449590461234 0.107990967503
-0.449579327561 0.107973602628
-0.449568121418 0.10795621804
-0.449556842799 0.107938813731
-0.449545491698 0.107921389693
-0.449534068111 0.107903945918
-0.44952257203 0.107886482399
-0.449511003452 0.107868999128
-0.449499362369 0.107851496096
-0.449487648778 0.107833973296
-0.449475862671 0.10781643072
-0.449464004044 0.107798868361
-0.44945207289 0.10778128621
-0.449440069203 0.10776368426
-0.449427992979 0.107746062502
-0.449415844211 0.10772842093
-0.449403622893 0.107710759535
-0.449391329019 0.107693078309
-0.449378962583 0.107675377245
-0.44936652358 0.107657656335
-0.449354012003 0.107639915571
-0.449341427846 0.107622154945
-0.449328771104 0.107604374449
-0.449316041769 0.107586574077
-0.449303239837 0.107568753819
-0.449290365299 0.107550913668
-0.449277418152 0.107533053616
-0.449264398387 0.107515173656
-0.449251305999 0.10749727378
-0.449238140982 0.10747935398
-0.449224903328 0.107461414249
-0.449211593033 0.107443454578
-0.449198210088 0.107425474959
-0.449184754488 0.107407475386
-0.449171226226 0.10738945585
-0.449157625296 0.107371416343
-0.449143951691 0.107353356859
-0.449130205404 0.107335277388
-0.449116386429 0.107317177924
-0.449102494759 0.107299058458
-0.449088530387 0.107280918983
-0.449074493307 0.107262759492
-0.449060383511 0.107244579976
-0.449046200992 0.107226380427
-0.449031945745 0.107208160839
-0.449017617762 0.107189921203
-0.449003217035 0.107171661512
-0.448988743559 0.107153381758
-0.448974197326 0.107135081932
-0.448959578328 0.107116762029
-0.448944886559 0.107098422039
-0.448930122012 0.107080061956
-0.448915284679 0.107061681771
-0.448900374554 0.107043281476
-0.448885391628 0.107024861065
-0.448870335895 0.10700642053
-0.448855207348 0.106987959862
-0.448840005978 0.106969479054
-0.448824731779 0.106950978099
-0.448809384744 0.106932456989
-0.448793964864 0.106913915716
-0.448778472132 0.106895354272
-0.44876290654 0.106876772651
-0.448747268082 0.106858170843
-0.448731556749 0.106839548842
-0.448715772534 0.10682090664
-0.448699915429 0.10680224423
-0.448683985427 0.106783561603
-0.448667982519 0.106764858752
-0.448651906697 0.10674613567
-0.448635757955 0.106727392348
-0.448619536284 0.10670862878
-0.448603241676 0.106689844957
-0.448586874123 0.106671040873
-0.448570433617 0.106652216519
-0.448553920151 0.106633371887
-0.448537333716 0.106614506971
-0.448520674304 0.106595621762
-0.448503941906 0.106576716254
-0.448487136516 0.106557790438
-0.448470258124 0.106538844306
-0.448453306722 0.106519877852
-0.448436282303 0.106500891068
-0.448419184857 0.106481883946
-0.448402014376 0.106462856478
-0.448384770852 0.106443808657
-0.448367454277 0.106424740476
-0.448350064642 0.106405651927
-0.448332601939 0.106386543002
-0.448315066159 0.106367413694
-0.448297457293 0.106348263995
-0.448279775333 0.106329093897
-0.44826202027 0.106309903394
-0.448244192095 0.106290692477
-0.448226290801 0.10627146114
-0.448208316377 0.106252209374
-0.448190268816 0.106232937172
-0.448172148108 0.106213644526
-0.448153954244 0.106194331429
-0.448135687217 0.106174997874
-0.448117347015 0.106155643853
-0.448098933632 0.106136269358
-0.448080447057 0.106116874382
-0.448061887282 0.106097458918
-0.448043254297 0.106078022957
-0.448024548094 0.106058566493
-0.448005768663 0.106039089517
-0.447986915994 0.106019592024
-0.44796799008 0.106000074004
-0.44794899091 0.10598053545
-0.447929918475 0.105960976356
-0.447910772766 0.105941396713
-0.447891553773 0.105921796514
-0.447872261487 0.105902175751
-0.447852895899 0.105882534418
-0.447833456999 0.105862872507
-0.447813944777 0.105843190009
-0.447794359223 0.105823486918
-0.447774700329 0.105803763227
-0.447754968085 0.105784018927
-0.447735162481 0.105764254012
-0.447715283506 0.105744468474
-0.447695331152 0.105724662305
-0.447675305408 0.105704835498
-0.447655206266 0.105684988046
-0.447635033713 0.105665119942
-0.447614787742 0.105645231177
-0.447594468342 0.105625321744
-0.447574075502 0.105605391636
-0.447553609214 0.105585440846
-0.447533069466 0.105565469366
-0.447512456249 0.105545477189
-0.447491769552 0.105525464307
-0.447471009366 0.105505430713
-0.44745017568 0.105485376399
-0.447429268484 0.105465301359
-0.447408287767 0.105445205584
-0.447387233519 0.105425089068
-0.44736610573 0.105404951803
-0.44734490439 0.105384793781
-0.447323629487 0.105364614996
-0.447302281012 0.105344415439
-0.447280858954 0.105324195104
-0.447259363302 0.105303953983
-0.447237794046 0.105283692069
-0.447216151175 0.105263409354
-0.447194434678 0.105243105831
-0.447172644545 0.105222781493
-0.447150780765 0.105202436333
-0.447128843326 0.105182070342
-0.44710683222 0.105161683514
-0.447084747433 0.105141275841
-0.447062588956 0.105120847316
-0.447040356777 0.105100397932
-0.447018050886 0.105079927682
-0.446995671271 0.105059436557
-0.446973217922 0.105038924551
-0.446950690827 0.105018391656
-0.446928089974 0.104997837866
-0.446905415354 0.104977263172
-0.446882666955 0.104956667568
-0.446859844765 0.104936051045
-0.446836948773 0.104915413598
-0.446813978968 0.104894755218
-0.446790935338 0.104874075899
-0.446767817872 0.104853375632
-0.446744626559 0.104832654411
-0.446721361387 0.104811912228
-0.446698022344 0.104791149077
-0.446674609419 0.104770364949
-0.4466511226 0.104749559838
-0.446627561876 0.104728733737
-0.446603927235 0.104707886637
-0.446580218665 0.104687018532
-0.446556436154 0.104666129415
-0.446532579691 0.104645219277
-0.446508649263 0.104624288113
-0.44648464486 0.104603335915
-0.446460566468 0.104582362675
-0.446436414076 0.104561368386
-0.446412187673 0.104540353042
-0.446387887245 0.104519316634
-0.44636351278 0.104498259156
-0.446339064268 0.1044771806
-0.446314541695 0.104456080959
-0.446289945049 0.104434960226
-0.446265274318 0.104413818394
-0.44624052949 0.104392655455
-0.446215710553 0.104371471403
-0.446190817493 0.104350266229
-0.446165850299 0.104329039927
-0.446140808958 0.10430779249
-0.446115693458 0.104286523911
-0.446090503786 0.104265234181
-0.44606523993 0.104243923295
-0.446039901877 0.104222591245
-0.446014489614 0.104201238023
-0.445989003129 0.104179863623
-0.445963442408 0.104158468037
-0.44593780744 0.104137051258
-0.445912098212 0.104115613279
-0.445886314709 0.104094154093
-0.445860456921 0.104072673693
-0.445834524833 0.104051172071
-0.445808518433 0.10402964922
-0.445782437707 0.104008105134
-0.445756282644 0.103986539804
-0.445730053229 0.103964953225
-0.445703749449 0.103943345388
-0.445677371292 0.103921716287
-0.445650918744 0.103900065914
-0.445624391792 0.103878394263
-0.445597790422 0.103856701325
-0.445571114622 0.103834987095
-0.445544364377 0.103813251565
-0.445517539675 0.103791494728
-0.445490640502 0.103769716576
-0.445463666845 0.103747917103
-0.445436618689 0.103726096301
-0.445409496022 0.103704254164
-0.44538229883 0.103682390684
-0.445355027099 0.103660505854
-0.445327680815 0.103638599668
-0.445300259965 0.103616672117
-0.445272764535 0.103594723195
-0.445245194512 0.103572752895
-0.44521754988 0.10355076121
-0.445189830627 0.103528748132
-0.445162036738 0.103506713655
-0.4451341682 0.103484657771
-0.445106224998 0.103462580474
-0.445078207119 0.103440481756
-0.445050114548 0.103418361611
-0.445021947271 0.10339622003
-0.444993705274 0.103374057008
-0.444965388543 0.103351872537
-0.444936997063 0.10332966661
-0.44490853082 0.103307439221
-0.4448799898 0.103285190361
-0.444851373989 0.103262920024
-0.444822683371 0.103240628203
-0.444793917933 0.103218314891
-0.44476507766 0.10319598008
-0.444736162537 0.103173623765
-0.44470717255 0.103151245937
-0.444678107685 0.10312884659
-0.444648967925 0.103106425717
-0.444619753258 0.103083983311
-0.444590463667 0.103061519364
-0.444561099139 0.10303903387
-0.444531659658 0.103016526822
-0.444502145209 0.102993998213
-0.444472555778 0.102971448035
-0.44444289135 0.102948876282
-0.444413151909 0.102926282947
-0.44438333744 0.102903668023
-0.444353447929 0.102881031502
-0.44432348336 0.102858373379
-0.444293443718 0.102835693645
-0.444263328988 0.102812992294
-0.444233139154 0.102790269319
-0.444202874202 0.102767524712
-0.444172534115 0.102744758468
-0.444142118879 0.102721970579
-0.444111628478 0.102699161038
-0.444081062896 0.102676329838
-0.444050422119 0.102653476972
-0.444019706129 0.102630602433
-0.443988914913 0.102607706214
-0.443958048454 0.102584788309
-0.443927106736 0.102561848711
-0.443896089744 0.102538887411
-0.443864997462 0.102515904404
-0.443833829874 0.102492899683
-0.443802586965 0.102469873241
-0.443771268717 0.10244682507
-0.443739875117 0.102423755164
-0.443708406146 0.102400663516
-0.44367686179 0.102377550119
-0.443645242032 0.102354414966
-0.443613546857 0.10233125805
-0.443581776247 0.102308079365
-0.443549930188 0.102284878903
-0.443518008662 0.102261656658
-0.443486011653 0.102238412622
-0.443453939145 0.102215146789
-0.443421791121 0.102191859152
-0.443389567566 0.102168549703
-0.443357268462 0.102145218437
-0.443324893793 0.102121865346
-0.443292443543 0.102098490424
-0.443259917695 0.102075093663
-0.443227316233 0.102051675056
-0.443194639138 0.102028234598
-0.443161886396 0.10200477228
-0.443129057989 0.101981288096
-0.4430961539 0.10195778204
-0.443063174113 0.101934254104
-0.44303011861 0.101910704281
-0.442996987375 0.101887132565
-0.442963780391 0.101863538949
-0.44293049764 0.101839923426
-0.442897139105 0.101816285989
-0.44286370477 0.101792626632
-0.442830194617 0.101768945346
-0.442796608629 0.101745242127
-0.442762946789 0.101721516967
-0.442729209079 0.101697769858
-0.442695395483 0.101674000795
-0.442661505982 0.101650209771
-0.442627540559 0.101626396778
-0.442593499197 0.101602561809
-0.442559381878 0.101578704859
-0.442525188585 0.10155482592
-0.4424909193 0.101530924986
-0.442456574005 0.101507002049
-0.442422152683 0.101483057104
-0.442387655317 0.101459090142
-0.442353081887 0.101435101157
-0.442318432376 0.101411090144
-0.442283706767 0.101387057094
-0.442248905042 0.101363002001
-0.442214027182 0.101338924858
-0.44217907317 0.101314825659
-0.442144042987 0.101290704396
-0.442108936615 0.101266561063
-0.442073754037 0.101242395654
-0.442038495234 0.101218208161
-0.442003160187 0.101193998578
-0.441967748879 0.101169766898
-0.441932261292 0.101145513114
-0.441896697406 0.10112123722
-0.441861057203 0.101096939208
-0.441825340665 0.101072619073
-0.441789547774 0.101048276807
-0.44175367851 0.101023912403
-0.441717732856 0.100999525855
-0.441681710792 0.100975117157
-0.441645612301 0.100950686301
-0.441609437362 0.10092623328
-0.441573185957 0.100901758089
-0.441536858069 0.10087726072
-0.441500453676 0.100852741167
-0.441463972762 0.100828199422
-0.441427415306 0.10080363548
-0.44139078129 0.100779049334
-0.441354070694 0.100754440976
-0.4413172835 0.1007298104
-0.441280419689 0.1007051576
-0.44124347924 0.100680482569
-0.441206462136 0.1006557853
-0.441169368356 0.100631065787
-0.441132197882 0.100606324022
-0.441094950693 0.100581559999
-0.441057626771 0.100556773712
-0.441020226096 0.100531965154
-0.440982748648 0.100507134318
-0.440945194408 0.100482281198
-0.440907563356 0.100457405786
-0.440869855473 0.100432508076
-0.440832070739 0.100407588063
-0.440794209134 0.100382645738
-0.440756270638 0.100357681095
-0.440718255232 0.100332694128
-0.440680162895 0.100307684831
-0.440641993608 0.100282653195
-0.44060374735 0.100257599216
-0.440565424102 0.100232522885
-0.440527023844 0.100207424197
-0.440488546554 0.100182303146
-0.440449992214 0.100157159723
-0.440411360803 0.100131993923
-0.4403726523 0.10010680574
-0.440333866686 0.100081595166
-0.440295003939 0.100056362195
-0.44025606404 0.10003110682
-0.440217046968 0.100005829035
-0.440177952702 0.0999805288331
-0.440138781223 0.0999552062079
-0.440099532508 0.0999298611527
-0.440060206538 0.0999044936609
-0.440020803292 0.099879103726
-0.43998132275 0.0998536913414
-0.439941764889 0.0998282565005
-0.43990212969 0.0998027991968
-0.439862417132 0.0997773194236
-0.439822627193 0.0997518171745
-0.439782759853 0.0997262924429
-0.43974281509 0.0997007452222
-0.439702792884 0.0996751755059
-0.439662693213 0.0996495832874
-0.439622516056 0.0996239685603
-0.439582261392 0.0995983313179
-0.4395419292 0.0995726715537
-0.439501519458 0.0995469892612
-0.439461032145 0.0995212844338
-0.439420467239 0.0994955570651
-0.439379824719 0.0994698071485
-0.439339104563 0.0994440346775
-0.43929830675 0.0994182396455
-0.439257431259 0.0993924220461
-0.439216478066 0.0993665818728
-0.439175447152 0.099340719119
-0.439134338493 0.0993148337782
-0.439093152069 0.099288925844
-0.439051887856 0.0992629953098
-0.439010545834 0.0992370421692
-0.43896912598 0.0992110664156
-0.438927628273 0.0991850680426
-0.438886052689 0.0991590470436
-0.438844399208 0.0991330034123
-0.438802667806 0.0991069371421
-0.438760858462 0.0990808482265
-0.438718971154 0.0990547366591
-0.438677005858 0.0990286024334
-0.438634962553 0.099002445543
-0.438592841216 0.0989762659813
-0.438550641825 0.0989500637419
-0.438508364357 0.0989238388184
-0.43846600879 0.0988975912043
-0.438423575101 0.0988713208932
-0.438381063267 0.0988450278785
-0.438338473265 0.098818712154
-0.438295805073 0.098792373713
-0.438253058668 0.0987660125493
-0.438210234027 0.0987396286563
-0.438167331127 0.0987132220276
-0.438124349945 0.0986867926568
-0.438081290458 0.0986603405375
-0.438038152643 0.0986338656632
-0.437994936477 0.0986073680276
-0.437951641937 0.0985808476242
-0.437908268999 0.0985543044466
-0.43786481764 0.0985277384883
-0.437821287836 0.0985011497431
-0.437777679565 0.0984745382045
-0.437733992803 0.098447903866
-0.437690227526 0.0984212467213
-0.437646383711 0.0983945667641
-0.437602461334 0.0983678639878
-0.437558460372 0.0983411383861
-0.4375143808 0.0983143899527
-0.437470222596 0.0982876186812
-0.437425985735 0.0982608245651
-0.437381670193 0.0982340075981
-0.437337275947 0.0982071677739
-0.437292802972 0.098180305086
-0.437248251245 0.0981534195281
-0.437203620741 0.0981265110939
-0.437158911436 0.0980995797769
-0.437114123307 0.0980726255708
-0.437069256328 0.0980456484694
-0.437024310476 0.0980186484661
-0.436979285726 0.0979916255547
-0.436934182054 0.0979645797289
-0.436888999435 0.0979375109822
-0.436843737846 0.0979104193084
-0.43679839726 0.0978833047011
-0.436752977655 0.097856167154
-0.436707479004 0.0978290066608
-0.436661901284 0.0978018232151
-0.436616244469 0.0977746168107
-0.436570508536 0.0977473874411
-0.436524693458 0.0977201351001
-0.436478799211 0.0976928597814
-0.436432825771 0.0976655614786
-0.436386773111 0.0976382401855
-0.436340641207 0.0976108958958
-0.436294430034 0.0975835286031
-0.436248139567 0.0975561383012
-0.43620176978 0.0975287249838
-0.436155320648 0.0975012886445
-0.436108792146 0.0974738292771
-0.436062184248 0.0974463468753
-0.436015496929 0.0974188414329
-0.435968730164 0.0973913129435
-0.435921883926 0.0973637614008
-0.43587495819 0.0973361867987
-0.435827952931 0.0973085891308
-0.435780868122 0.0972809683909
-0.435733703738 0.0972533245727
-0.435686459754 0.0972256576699
-0.435639136142 0.0971979676763
-0.435591732878 0.0971702545857
-0.435544249935 0.0971425183918
-0.435496687288 0.0971147590882
-0.435449044909 0.0970869766689
-0.435401322773 0.0970591711276
-0.435353520854 0.097031342458
-0.435305639125 0.0970034906538
-0.435257677561 0.0969756157089
-0.435209636134 0.0969477176171
-0.435161514818 0.096919796372
-0.435113313586 0.0968918519676
-0.435065032413 0.0968638843974
-0.435016671272 0.0968358936555
-0.434968230135 0.0968078797354
-0.434919708976 0.0967798426311
-0.434871107769 0.0967517823364
-0.434822426486 0.0967236988449
-0.434773665101 0.0966955921505
-0.434724823586 0.0966674622471
-0.434675901915 0.0966393091284
-0.43462690006 0.0966111327882
-0.434577817995 0.0965829332203
-0.434528655692 0.0965547104186
-0.434479413125 0.0965264643769
-0.434430090264 0.096498195089
-0.434380687085 0.0964699025487
-0.434331203558 0.0964415867499
-0.434281639656 0.0964132476864
-0.434231995353 0.0963848853519
-0.43418227062 0.0963564997404
-0.434132465429 0.0963280908457
-0.434082579754 0.0962996586616
-0.434032613566 0.0962712031821
-0.433982566838 0.0962427244008
-0.433932439541 0.0962142223117
-0.433882231648 0.0961856969086
-0.43383194313 0.0961571481855
-0.43378157396 0.0961285761361
-0.43373112411 0.0960999807543
-0.433680593551 0.096071362034
-0.433629982256 0.096042719969
-0.433579290195 0.0960140545533
-0.433528517341 0.0959853657807
-0.433477663665 0.0959566536451
-0.433426729139 0.0959279181403
-0.433375713734 0.0958991592603
-0.433324617422 0.0958703769989
-0.433273440174 0.09584157135
-0.433222181961 0.0958127423076
-0.433170842755 0.0957838898655
-0.433119422527 0.0957550140176
-0.433067921248 0.0957261147579
-0.433016338889 0.0956971920802
-0.432964675421 0.0956682459784
-0.432912930815 0.0956392764465
-0.432861105041 0.0956102834784
-0.432809198072 0.0955812670679
-0.432757209877 0.0955522272091
-0.432705140428 0.0955231638958
-0.432652989694 0.095494077122
-0.432600757647 0.0954649668815
-0.432548444257 0.0954358331685
-0.432496049495 0.0954066759766
-0.432443573331 0.0953774953
-0.432391015735 0.0953482911326
-0.432338376678 0.0953190634682
-0.432285656129 0.0952898123009
-0.43223285406 0.0952605376246
-0.43217997044 0.0952312394332
-0.432127005239 0.0952019177208
-0.432073958428 0.0951725724812
-0.432020829976 0.0951432037085
-0.431967619852 0.0951138113965
-0.431914328028 0.0950843955394
-0.431860954473 0.095054956131
-0.431807499155 0.0950254931653
-0.431753962046 0.0949960066364
-0.431700343114 0.0949664965381
-0.43164664233 0.0949369628645
-0.431592859661 0.0949074056096
-0.431538995079 0.0948778247673
-0.431485048552 0.0948482203317
-0.431431020049 0.0948185922967
-0.43137690954 0.0947889406564
-0.431322716994 0.0947592654047
-0.43126844238 0.0947295665357
-0.431214085667 0.0946998440433
-0.431159646823 0.0946700979217
-0.431105125818 0.0946403281647
-0.431050522621 0.0946105347664
-0.4309958372 0.0945807177209
-0.430941069524 0.0945508770221
-0.430886219562 0.0945210126641
-0.430831287282 0.0944911246409
-0.430776272652 0.0944612129466
-0.430721175642 0.0944312775752
-0.43066599622 0.0944013185207
-0.430610734353 0.0943713357772
-0.43055539001 0.0943413293386
-0.43049996316 0.0943112991992
-0.43044445377 0.0942812453529
-0.430388861809 0.0942511677937
-0.430333187244 0.0942210665157
-0.430277430043 0.0941909415131
-0.430221590175 0.0941607927798
-0.430165667607 0.0941306203099
-0.430109662307 0.0941004240975
-0.430053574243 0.0940702041367
-0.429997403381 0.0940399604215
-0.429941149691 0.094009692946
-0.429884813138 0.0939794017043
-0.429828393691 0.0939490866905
-0.429771891317 0.0939187478986
-0.429715305983 0.0938883853228
-0.429658637657 0.0938579989572
-0.429601886306 0.0938275887958
-0.429545051896 0.0937971548327
-0.429488134395 0.0937666970621
-0.429431133769 0.093736215478
-0.429374049986 0.0937057100746
-0.429316883013 0.093675180846
-0.429259632816 0.0936446277862
-0.429202299361 0.0936140508895
-0.429144882616 0.0935834501499
-0.429087382548 0.0935528255615
-0.429029799122 0.0935221771185
-0.428972132304 0.093491504815
-0.428914382063 0.0934608086451
-0.428856548363 0.093430088603
-0.42879863117 0.0933993446828
-0.428740630452 0.0933685768786
-0.428682546174 0.0933377851847
-0.428624378303 0.093306969595
-0.428566126803 0.0932761301039
-0.428507791642 0.0932452667054
-0.428449372784 0.0932143793936
-0.428390870196 0.0931834681628
-0.428332283843 0.0931525330072
-0.428273613692 0.0931215739208
-0.428214859706 0.0930905908978
-0.428156021853 0.0930595839325
-0.428097100097 0.093028553019
-0.428038094404 0.0929974981514
-0.427979004739 0.0929664193239
-0.427919831068 0.0929353165308
-0.427860573355 0.0929041897662
-0.427801231565 0.0928730390243
-0.427741805663 0.0928418642992
-0.427682295616 0.0928106655853
-0.427622701386 0.0927794428766
-0.42756302294 0.0927481961674
-0.427503260241 0.0927169254519
-0.427443413255 0.0926856307242
-0.427383481946 0.0926543119787
-0.427323466279 0.0926229692094
-0.427263366217 0.0925916024107
-0.427203181726 0.0925602115767
-0.42714291277 0.0925287967017
-0.427082559313 0.0924973577798
-0.427022121319 0.0924658948054
-0.426961598752 0.0924344077726
-0.426900991577 0.0924028966756
-0.426840299757 0.0923713615087
-0.426779523256 0.0923398022662
-0.426718662038 0.0923082189423
-0.426657716067 0.0922766115312
-0.426596685306 0.0922449800271
-0.426535569719 0.0922133244244
-0.426474369269 0.0921816447172
-0.426413083921 0.0921499408998
-0.426351713637 0.0921182129666
-0.42629025838 0.0920864609116
-0.426228718115 0.0920546847293
-0.426167092803 0.0920228844139
-0.426105382409 0.0919910599596
-0.426043586895 0.0919592113607
-0.425981706225 0.0919273386115
-0.42591974036 0.0918954417063
-0.425857689264 0.0918635206393
-0.4257955529 0.0918315754048
-0.42573333123 0.0917996059972
-0.425671024217 0.0917676124107
-0.425608631823 0.0917355946396
-0.425546154012 0.0917035526782
-0.425483590744 0.0916714865208
-0.425420941983 0.0916393961616
-0.425358207691 0.0916072815951
-0.425295387829 0.0915751428155
-0.425232482361 0.0915429798172
-0.425169491248 0.0915107925943
-0.425106414451 0.0914785811413
-0.425043251933 0.0914463454525
-0.424980003656 0.0914140855222
-0.424916669581 0.0913818013447
-0.424853249669 0.0913494929143
-0.424789743884 0.0913171602254
-0.424726152185 0.0912848032724
-0.424662474534 0.0912524220494
-0.424598710893 0.091220016551
-0.424534861223 0.0911875867713
-0.424470925485 0.0911551327049
-0.42440690364 0.0911226543459
-0.424342795649 0.0910901516889
-0.424278601474 0.091057624728
-0.424214321074 0.0910250734577
-0.424149954412 0.0909924978724
-0.424085501446 0.0909598979664
-0.424020962139 0.090927273734
-0.423956336451 0.0908946251696
-0.423891624342 0.0908619522677
-0.423826825773 0.0908292550225
-0.423761940703 0.0907965334285
-0.423696969094 0.0907637874801
-0.423631910906 0.0907310171715
-0.423566766097 0.0906982224972
-0.42350153463 0.0906654034517
-0.423436216463 0.0906325600292
-0.423370811556 0.0905996922241
-0.423305319869 0.090566800031
-0.423239741363 0.0905338834441
-0.423174075996 0.0905009424579
-0.423108323728 0.0904679770667
-0.423042484518 0.0904349872651
-0.422976558327 0.0904019730473
-0.422910545113 0.0903689344078
-0.422844444835 0.0903358713411
-0.422778257453 0.0903027838415
-0.422711982926 0.0902696719035
-0.422645621213 0.0902365355214
-0.422579172272 0.0902033746898
-0.422512636063 0.090170189403
-0.422446012544 0.0901369796555
-0.422379301674 0.0901037454418
-0.422312503412 0.0900704867562
-0.422245617716 0.0900372035931
-0.422178644545 0.0900038959472
-0.422111583856 0.0899705638127
-0.422044435609 0.0899372071842
-0.421977199761 0.089903826056
-0.421909876271 0.0898704204228
-0.421842465096 0.0898369902788
-0.421774966195 0.0898035356186
-0.421707379525 0.0897700564366
-0.421639705045 0.0897365527274
-0.421571942711 0.0897030244853
-0.421504092482 0.0896694717049
-0.421436154315 0.0896358943806
-0.421368128168 0.0896022925069
-0.421300013997 0.0895686660783
-0.421231811761 0.0895350150893
-0.421163521416 0.0895013395343
-0.42109514292 0.0894676394079
-0.42102667623 0.0894339147045
-0.420958121302 0.0894001654186
-0.420889478093 0.0893663915448
-0.420820746561 0.0893325930776
-0.420751926662 0.0892987700113
-0.420683018353 0.0892649223406
-0.420614021589 0.08923105006
-0.420544936329 0.089197153164
-0.420475762527 0.089163231647
-0.420406500141 0.0891292855037
-0.420337149126 0.0890953147285
-0.420267709439 0.0890613193159
-0.420198181036 0.0890272992605
-0.420128563872 0.0889932545568
-0.420058857904 0.0889591851994
-0.419989063087 0.0889250911827
-0.419919179377 0.0888909725014
-0.41984920673 0.0888568291499
-0.419779145101 0.0888226611228
-0.419708994445 0.0887884684146
-0.419638754719 0.0887542510199
-0.419568425876 0.0887200089333
-0.419498007873 0.0886857421493
-0.419427500665 0.0886514506625
-0.419356904206 0.0886171344673
-0.419286218451 0.0885827935585
-0.419215443356 0.0885484279305
-0.419144578874 0.0885140375779
-0.419073624961 0.0884796224953
-0.419002581571 0.0884451826773
-0.418931448659 0.0884107181184
-0.418860226179 0.0883762288132
-0.418788914086 0.0883417147563
-0.418717512333 0.0883071759423
-0.418646020875 0.0882726123658
-0.418574439665 0.0882380240214
-0.418502768658 0.0882034109036
-0.418431007808 0.0881687730071
-0.418359157068 0.0881341103265
-0.418287216391 0.0880994228563
-0.418215185733 0.0880647105911
-0.418143065045 0.0880299735257
-0.418070854283 0.0879952116545
-0.417998553397 0.0879604249722
-0.417926162343 0.0879256134735
-0.417853681073 0.0878907771528
-0.41778110954 0.0878559160049
-0.417708447698 0.0878210300245
-0.417635695498 0.087786119206
-0.417562852894 0.0877511835441
-0.417489919839 0.0877162230335
-0.417416896285 0.0876812376688
-0.417343782184 0.0876462274447
-0.417270577489 0.0876111923557
-0.417197282153 0.0875761323966
-0.417123896126 0.0875410475619
-0.417050419363 0.0875059378464
-0.416976851814 0.0874708032446
-0.416903193432 0.0874356437513
-0.416829444168 0.087400459361
-0.416755603975 0.0873652500686
-0.416681672803 0.0873300158685
-0.416607650605 0.0872947567555
-0.416533537331 0.0872594727242
-0.416459332934 0.0872241637693
-0.416385037364 0.0871888298856
-0.416310650573 0.0871534710676
-0.416236172512 0.08711808731
-0.416161603132 0.0870826786076
-0.416086942383 0.087047244955
-0.416012190217 0.0870117863469
-0.415937346584 0.086976302778
-0.415862411435 0.086940794243
-0.415787384721 0.0869052607366
-0.415712266391 0.0868697022534
-0.415637056396 0.0868341187882
-0.415561754687 0.0867985103357
-0.415486361213 0.0867628768906
-0.415410875924 0.0867272184476
-0.415335298771 0.0866915350015
-0.415259629704 0.0866558265468
-0.415183868671 0.0866200930784
-0.415108015623 0.086584334591
-0.41503207051 0.0865485510793
-0.41495603328 0.086512742538
-0.414879903883 0.0864769089618
-0.414803682268 0.0864410503455
-0.414727368385 0.0864051666838
-0.414650962183 0.0863692579715
-0.414574463609 0.0863333242033
-0.414497872615 0.0862973653739
-0.414421189147 0.0862613814781
-0.414344413155 0.0862253725106
-0.414267544587 0.0861893384662
-0.414190583392 0.0861532793396
-0.414113529518 0.0861171951256
-0.414036382914 0.086081085819
-0.413959143527 0.0860449514144
-0.413881811305 0.0860087919067
-0.413804386198 0.0859726072907
-0.413726868151 0.0859363975611
-0.413649257114 0.0859001627126
-0.413571553033 0.0858639027402
-0.413493755857 0.0858276176384
-0.413415865532 0.0857913074022
-0.413337882007 0.0857549720262
-0.413259805228 0.0857186115053
-0.413181635142 0.0856822258344
-0.413103371697 0.085645815008
-0.41302501484 0.0856093790212
-0.412946564516 0.0855729178685
-0.412868020674 0.085536431545
-0.412789383259 0.0854999200453
-0.412710652219 0.0854633833642
-0.412631827498 0.0854268214966
-0.412552909045 0.0853902344373
-0.412473896805 0.0853536221811
-0.412394790724 0.0853169847228
-0.412315590748 0.0852803220572
-0.412236296823 0.0852436341792
-0.412156908894 0.0852069210835
-0.412077426908 0.085170182765
-0.411997850811 0.0851334192186
-0.411918180546 0.085096630439
-0.41183841606 0.085059816421
-0.411758557299 0.0850229771597
-0.411678604207 0.0849861126496
-0.411598556728 0.0849492228858
-0.411518414809 0.0849123078631
-0.411438178394 0.0848753675762
-0.411357847428 0.0848384020202
-0.411277421855 0.0848014111897
-0.411196901619 0.0847643950796
-0.411116286666 0.0847273536849
-0.411035576939 0.0846902870004
-0.410954772382 0.0846531950209
-0.410873872941 0.0846160777414
-0.410792878557 0.0845789351566
-0.410711789176 0.0845417672614
-0.410630604742 0.0845045740508
-0.410549325197 0.0844673555196
-0.410467950485 0.0844301116627
-0.410386480549 0.084392842475
-0.410304915334 0.0843555479513
-0.410223254781 0.0843182280865
-0.410141498835 0.0842808828756
-0.410059647438 0.0842435123134
-0.409977700532 0.0842061163948
-0.409895658061 0.0841686951147
-0.409813519968 0.0841312484681
-0.409731286194 0.0840937764498
-0.409648956682 0.0840562790547
-0.409566531374 0.0840187562777
-0.409484010213 0.0839812081138
-0.40940139314 0.0839436345579
-0.409318680098 0.0839060356048
-0.409235871028 0.0838684112496
-0.409152965872 0.0838307614871
-0.409069964571 0.0837930863122
-0.408986867068 0.0837553857199
-0.408903673302 0.0837176597051
-0.408820383217 0.0836799082627
-0.408736996752 0.0836421313878
-0.408653513848 0.0836043290751
-0.408569934448 0.0835665013197
-0.40848625849 0.0835286481165
-0.408402485917 0.0834907694604
-0.408318616668 0.0834528653464
-0.408234650684 0.0834149357695
-0.408150587905 0.0833769807246
-0.408066428271 0.0833390002066
-0.407982171724 0.0833009942106
-0.407897818201 0.0832629627314
-0.407813367644 0.083224905764
-0.407728819991 0.0831868233035
-0.407644175184 0.0831487153448
-0.40755943316 0.0831105818828
-0.407474593859 0.0830724229125
-0.407389657221 0.0830342384289
-0.407304623185 0.0829960284271
-0.40721949169 0.0829577929018
-0.407134262674 0.0829195318483
-0.407048936076 0.0828812452614
-0.406963511835 0.0828429331361
-0.406877989889 0.0828045954674
-0.406792370178 0.0827662322504
-0.406706652638 0.08272784348
-0.406620837208 0.0826894291512
-0.406534923827 0.082650989259
-0.406448912431 0.0826125237985
-0.40636280296 0.0825740327646
-0.40627659535 0.0825355161523
-0.406190289539 0.0824969739567
-0.406103885464 0.0824584061729
-0.406017383063 0.0824198127957
-0.405930782272 0.0823811938202
-0.405844083029 0.0823425492415
-0.405757285271 0.0823038790546
-0.405670388935 0.0822651832545
-0.405583393956 0.0822264618362
-0.405496300272 0.0821877147948
-0.405409107819 0.0821489421253
-0.405321816534 0.0821101438228
-0.405234426351 0.0820713198822
-0.405146937208 0.0820324702988
-0.40505934904 0.0819935950674
-0.404971661784 0.0819546941831
-0.404883875373 0.0819157676411
-0.404795989745 0.0818768154363
-0.404708004835 0.0818378375638
-0.404619920577 0.0817988340186
-0.404531736906 0.081759804796
-0.404443453759 0.0817207498908
-0.404355071069 0.0816816692982
-0.404266588772 0.0816425630132
-0.404178006801 0.0816034310309
-0.404089325092 0.0815642733465
-0.404000543578 0.0815250899549
-0.403911662195 0.0814858808513
-0.403822680875 0.0814466460307
-0.403733599553 0.0814073854882
-0.403644418163 0.081368099219
-0.403555136638 0.081328787218
-0.403465754911 0.0812894494805
-0.403376272917 0.0812500860015
-0.403286690589 0.081210696776
-0.403197007859 0.0811712817993
-0.403107224661 0.0811318410664
-0.403017340927 0.0810923745724
-0.40292735659 0.0810528823124
-0.402837271583 0.0810133642815
-0.402747085838 0.080973820475
-0.402656799288 0.0809342508877
-0.402566411864 0.080894655515
-0.402475923499 0.0808550343519
-0.402385334124 0.0808153873935
-0.402294643672 0.080775714635
-0.402203852074 0.0807360160715
-0.402112959262 0.0806962916981
-0.402021965166 0.08065654151
-0.401930869718 0.0806167655024
-0.401839672849 0.0805769636702
-0.401748374491 0.0805371360088
-0.401656974573 0.0804972825131
-0.401565473027 0.0804574031785
-0.401473869783 0.080417498
-0.401382164771 0.0803775669728
-0.401290357921 0.0803376100921
-0.401198449165 0.0802976273529
-0.401106438431 0.0802576187505
-0.401014325649 0.0802175842801
-0.40092211075 0.0801775239368
-0.400829793662 0.0801374377157
-0.400737374315 0.080097325612
-0.400644852639 0.080057187621
-0.400552228562 0.0800170237378
-0.400459502013 0.0799768339575
-0.400366672921 0.0799366182754
-0.400273741215 0.0798963766866
-0.400180706823 0.0798561091863
-0.400087569674 0.0798158157698
-0.399994329695 0.0797754964321
-0.399900986816 0.0797351511686
-0.399807540963 0.0796947799743
-0.399713992065 0.0796543828445
-0.399620340049 0.0796139597745
-0.399526584843 0.0795735107593
-0.399432726374 0.0795330357942
-0.399338764569 0.0794925348745
-0.399244699356 0.0794520079953
-0.399150530661 0.0794114551518
-0.39905625841 0.0793708763393
-0.398961882531 0.079330271553
-0.39886740295 0.079289640788
-0.398772819594 0.0792489840397
-0.398678132388 0.0792083013033
-0.398583341258 0.0791675925739
-0.39848844613 0.0791268578469
-0.39839344693 0.0790860971174
-0.398298343584 0.0790453103807
-0.398203136017 0.079004497632
-0.398107824153 0.0789636588666
-0.398012407919 0.0789227940797
-0.397916887239 0.0788819032666
-0.397821262037 0.0788409864225
-0.397725532239 0.0788000435426
-0.397629697769 0.0787590746223
-0.397533758551 0.0787180796567
-0.397437714509 0.0786770586412
-0.397341565568 0.078636011571
-0.39724531165 0.0785949384413
-0.397148952681 0.0785538392475
-0.397052488582 0.0785127139848
-0.396955919279 0.0784715626485
-0.396859244693 0.0784303852338
-0.396762464748 0.078389181736
-0.396665579367 0.0783479521505
-0.396568588473 0.0783066964724
-0.396471491988 0.0782654146971
-0.396374289834 0.0782241068199
-0.396276981934 0.078182772836
-0.396179568209 0.0781414127408
-0.396082048583 0.0781000265295
-0.395984422975 0.0780586141974
-0.395886691309 0.0780171757399
-0.395788853506 0.0779757111522
-0.395690909486 0.0779342204296
-0.395592859171 0.0778927035675
-0.395494702482 0.0778511605612
-0.39539643934 0.077809591406
-0.395298069664 0.0777679960971
-0.395199593377 0.0777263746299
-0.395101010397 0.0776847269998
-0.395002320646 0.077643053202
-0.394903524042 0.0776013532319
-0.394804620506 0.0775596270847
-0.394705609958 0.0775178747559
-0.394606492317 0.0774760962408
-0.394507267501 0.0774342915346
-0.394407935431 0.0773924606328
-0.394308496026 0.0773506035307
-0.394208949203 0.0773087202236
-0.394109294882 0.0772668107068
-0.39400953298 0.0772248749757
-0.393909663418 0.0771829130257
-0.393809686111 0.0771409248521
-0.393709600979 0.0770989104503
-0.393609407938 0.0770568698155
-0.393509106908 0.0770148029433
-0.393408697804 0.0769727098289
-0.393308180545 0.0769305904677
-0.393207555047 0.076888444855
-0.393106821227 0.0768462729863
-0.393005979002 0.0768040748569
-0.392905028288 0.0767618504622
-0.392803969002 0.0767195997976
-0.392702801061 0.0766773228583
-0.392601524379 0.07663501964
-0.392500138873 0.0765926901378
-0.392398644458 0.0765503343472
-0.39229704105 0.0765079522636
-0.392195328564 0.0764655438823
-0.392093506916 0.0764231091988
-0.39199157602 0.0763806482085
-0.391889535791 0.0763381609067
-0.391787386143 0.0762956472889
-0.391685126992 0.0762531073505
-0.39158275825 0.0762105410868
-0.391480279833 0.0761679484933
-0.391377691654 0.0761253295654
-0.391274993627 0.0760826842985
-0.391172185664 0.076040012688
-0.39106926768 0.0759973147294
-0.390966239588 0.075954590418
-0.390863101301 0.0759118397492
-0.39075985273 0.0758690627186
-0.39065649379 0.0758262593215
-0.390553024391 0.0757834295534
-0.390449444447 0.0757405734097
-0.39034575387 0.0756976908858
-0.39024195257 0.0756547819771
-0.390138040461 0.0756118466792
-0.390034017453 0.0755688849874
-0.389929883457 0.0755258968972
-0.389825638385 0.0754828824041
-0.389721282147 0.0754398415034
-0.389616814654 0.0753967741907
-0.389512235817 0.0753536804614
-0.389407545546 0.0753105603109
-0.389302743751 0.0752674137348
-0.389197830341 0.0752242407284
-0.389092805227 0.0751810412873
-0.388987668319 0.0751378154068
-0.388882419525 0.0750945630826
-0.388777058754 0.07505128431
-0.388671585916 0.0750079790845
-0.388566000919 0.0749646474016
-0.388460303672 0.0749212892568
-0.388354494083 0.0748779046455
-0.38824857206 0.0748344935633
-0.388142537512 0.0747910560056
-0.388036390346 0.0747475919679
-0.387930130469 0.0747041014457
-0.387823757789 0.0746605844345
-0.387717272213 0.0746170409298
-0.387610673648 0.0745734709271
-0.387503962001 0.0745298744219
-0.387397137179 0.0744862514097
-0.387290199087 0.074442601886
-0.387183147632 0.0743989258463
-0.387075982719 0.0743552232861
-0.386968704255 0.0743114942009
-0.386861312145 0.0742677385863
-0.386753806295 0.0742239564377
-0.386646186609 0.0741801477507
-0.386538452992 0.0741363125208
-0.38643060535 0.0740924507435
-0.386322643586 0.0740485624144
-0.386214567605 0.074004647529
-0.386106377311 0.0739607060828
-0.385998072608 0.0739167380713
-0.3858896534 0.0738727434901
-0.38578111959 0.0738287223347
-0.385672471081 0.0737846746007
-0.385563707776 0.0737406002836
-0.385454829578 0.073696499379
-0.38534583639 0.0736523718823
-0.385236728114 0.0736082177892
-0.385127504653 0.0735640370952
-0.385018165908 0.0735198297959
-0.384908711781 0.0734755958867
-0.384799142173 0.0734313353634
-0.384689456986 0.0733870482213
-0.384579656122 0.0733427344562
-0.38446973948 0.0732983940636
-0.384359706962 0.073254027039
-0.384249558468 0.0732096333779
-0.384139293898 0.0731652130761
-0.384028913153 0.0731207661291
-0.383918416132 0.0730762925323
-0.383807802734 0.0730317922815
-0.383697072859 0.0729872653722
-0.383586226407 0.0729427118
-0.383475263275 0.0728981315605
-0.383364183363 0.0728535246493
-0.38325298657 0.0728088910619
-0.383141672793 0.0727642307939
-0.38303024193 0.072719543841
-0.38291869388 0.0726748301988
-0.382807028539 0.0726300898628
-0.382695245805 0.0725853228287
-0.382583345576 0.0725405290921
-0.382471327748 0.0724957086486
-0.382359192217 0.0724508614937
-0.382246938881 0.0724059876231
-0.382134567634 0.0723610870325
-0.382022078375 0.0723161597174
-0.381909470997 0.0722712056735
-0.381796745396 0.0722262248963
-0.381683901469 0.0721812173816
-0.381570939109 0.0721361831249
-0.381457858211 0.0720911221219
-0.381344658671 0.0720460343682
-0.381231340382 0.0720009198594
-0.381117903238 0.0719557785912
-0.381004347134 0.0719106105592
-0.380890671963 0.0718654157591
-0.380776877618 0.0718201941865
-0.380662963993 0.0717749458371
-0.380548930979 0.0717296707064
-0.380434778471 0.0716843687902
-0.38032050636 0.0716390400841
-0.380206114538 0.0715936845838
-0.380091602898 0.0715483022848
-0.379976971331 0.071502893183
-0.379862219729 0.0714574572739
-0.379747347982 0.0714119945533
-0.379632355981 0.0713665050167
-0.379517243618 0.0713209886598
-0.379402010783 0.0712754454784
-0.379286657366 0.0712298754681
-0.379171183257 0.0711842786246
-0.379055588345 0.0711386549435
-0.37893987252 0.0710930044205
-0.378824035672 0.0710473270514
-0.378708077689 0.0710016228318
-0.378591998459 0.0709558917574
-0.378475797872 0.0709101338238
-0.378359475816 0.0708643490269
-0.378243032178 0.0708185373622
-0.378126466846 0.0707726988255
-0.378009779707 0.0707268334125
-0.37789297065 0.0706809411189
-0.37777603956 0.0706350219403
-0.377658986324 0.0705890758725
-0.377541810829 0.0705431029113
-0.377424512961 0.0704971030522
-0.377307092605 0.0704510762911
-0.377189549647 0.0704050226236
-0.377071883974 0.0703589420455
-0.376954095468 0.0703128345525
-0.376836184017 0.0702667001403
-0.376718149503 0.0702205388046
-0.376599991812 0.0701743505411
-0.376481710827 0.0701281353457
-0.376363306433 0.070081893214
-0.376244778512 0.0700356241418
-0.376126126947 0.0699893281247
-0.376007351623 0.0699430051586
-0.375888452421 0.0698966552392
-0.375769429224 0.0698502783621
-0.375650281914 0.0698038745233
-0.375531010373 0.0697574437184
-0.375411614482 0.0697109859431
-0.375292094123 0.0696645011933
-0.375172449177 0.0696179894647
-0.375052679525 0.0695714507529
-0.374932785046 0.0695248850539
-0.374812765622 0.0694782923634
-0.374692621133 0.069431672677
-0.374572351457 0.0693850259907
-0.374451956474 0.0693383523001
-0.374331436064 0.0692916516011
-0.374210790105 0.0692449238893
-0.374090018476 0.0691981691607
-0.373969121054 0.0691513874109
-0.373848097719 0.0691045786357
-0.373726948347 0.069057742831
-0.373605672816 0.0690108799924
-0.373484271003 0.0689639901159
-0.373362742785 0.0689170731972
-0.373241088039 0.068870129232
-0.37311930664 0.0688231582162
-0.372997398465 0.0687761601456
-0.372875363389 0.0687291350159
-0.372753201288 0.0686820828231
-0.372630912036 0.0686350035628
-0.372508495509 0.0685878972308
-0.372385951581 0.0685407638231
-0.372263280126 0.0684936033354
-0.372140481018 0.0684464157634
-0.37201755413 0.0683992011031
-0.371894499337 0.0683519593503
-0.37177131651 0.0683046905006
-0.371648005523 0.0682573945501
-0.371524566248 0.0682100714945
-0.371400998557 0.0681627213296
-0.371277302322 0.0681153440513
-0.371153477414 0.0680679396554
-0.371029523705 0.0680205081377
-0.370905441065 0.067973049494
-0.370781229365 0.0679255637202
-0.370656888475 0.0678780508122
-0.370532418266 0.0678305107658
-0.370407818606 0.0677829435768
-0.370283089365 0.067735349241
-0.370158230412 0.0676877277544
-0.370033241616 0.0676400791127
-0.369908122845 0.0675924033118
-0.369782873967 0.0675447003477
-0.369657494851 0.067496970216
-0.369531985362 0.0674492129128
-0.369406345369 0.0674014284338
-0.369280574739 0.0673536167749
-0.369154673337 0.067305777932
-0.36902864103 0.0672579119009
-0.368902477684 0.0672100186776
-0.368776183165 0.0671620982579
-0.368649757337 0.0671141506376
-0.368523200065 0.0670661758127
-0.368396511214 0.0670181737791
-0.368269690648 0.0669701445325
-0.368142738231 0.0669220880689
-0.368015653826 0.0668740043843
-0.367888437297 0.0668258934744
-0.367761088507 0.0667777553351
-0.367633607318 0.0667295899624
-0.367505993592 0.0666813973522
-0.367378247192 0.0666331775003
-0.367250367978 0.0665849304026
-0.367122355812 0.0665366560551
-0.366994210555 0.0664883544537
-0.366865932068 0.0664400255942
-0.36673752021 0.0663916694726
-0.366608974842 0.0663432860848
-0.366480295823 0.0662948754267
-0.366351483012 0.0662464374941
-0.366222536268 0.0661979722831
-0.366093455449 0.0661494797896
-0.365964240414 0.0661009600094
-0.36583489102 0.0660524129385
-0.365705407125 0.0660038385728
-0.365575788586 0.0659552369083
-0.36544603526 0.0659066079409
-0.365316147002 0.0658579516664
-0.36518612367 0.065809268081
-0.365055965118 0.0657605571804
-0.364925671202 0.0657118189606
-0.364795241777 0.0656630534176
-0.364664676698 0.0656142605473
-0.364533975818 0.0655654403456
-0.364403138992 0.0655165928086
-0.364272166074 0.0654677179321
-0.364141056915 0.0654188157121
-0.36400981137 0.0653698861446
-0.363878429291 0.0653209292255
-0.363746910528 0.0652719449508
-0.363615254936 0.0652229333164
-0.363483462363 0.0651738943183
-0.363351532663 0.0651248279525
-0.363219465684 0.0650757342149
-0.363087261278 0.0650266131016
-0.362954919294 0.0649774646084
-0.362822439581 0.0649282887314
-0.36268982199 0.0648790854665
-0.362557066367 0.0648298548097
-0.362424172562 0.064780596757
-0.362291140423 0.0647313113044
-0.362157969797 0.0646819984479
-0.362024660532 0.0646326581834
-0.361891212474 0.064583290507
-0.361757625469 0.0645338954146
-0.361623899363 0.0644844729022
-0.361490034003 0.0644350229658
-0.361356029234 0.0643855456015
-0.361221884899 0.0643360408051
-0.361087600845 0.0642865085728
-0.360953176914 0.0642369489006
-0.360818612951 0.0641873617844
-0.360683908798 0.0641377472202
-0.360549064299 0.0640881052041
-0.360414079296 0.064038435732
-0.360278953631 0.0639887388001
-0.360143687147 0.0639390144042
-0.360008279683 0.0638892625405
-0.359872731081 0.063839483205
-0.359737041181 0.0637896763936
-0.359601209824 0.0637398421024
-0.359465236849 0.0636899803274
-0.359329122096 0.0636400910647
-0.359192865403 0.0635901743104
-0.359056466608 0.0635402300603
-0.358919925549 0.0634902583106
-0.358783242065 0.0634402590573
-0.358646415993 0.0633902322965
-0.358509447168 0.0633401780242
-0.358372335427 0.0632900962364
-0.358235080607 0.0632399869292
-0.358097682543 0.0631898500986
-0.357960141069 0.0631396857407
-0.357822456021 0.0630894938516
-0.357684627232 0.0630392744273
-0.357546654537 0.0629890274639
-0.357408537769 0.0629387529573
-0.35727027676 0.0628884509038
-0.357131871343 0.0628381212993
-0.356993321351 0.06278776414
-0.356854626614 0.0627373794218
-0.356715786964 0.0626869671409
-0.356576802232 0.0626365272933
-0.356437672248 0.0625860598752
-0.356298396841 0.0625355648826
-0.356158975842 0.0624850423115
-0.356019409079 0.0624344921581
-0.35587969638 0.0623839144184
-0.355739837575 0.0623333090885
-0.355599832489 0.0622826761646
-0.355459680951 0.0622320156427
-0.355319382787 0.0621813275189
-0.355178937824 0.0621306117893
-0.355038345886 0.06207986845
-0.354897606801 0.062029097497
-0.354756720391 0.0619782989266
-0.354615686483 0.0619274727348
-0.354474504899 0.0618766189177
-0.354333175463 0.0618257374714
-0.354191697999 0.061774828392
-0.354050072328 0.0617238916757
-0.353908298273 0.0616729273185
-0.353766375656 0.0616219353166
-0.353624304297 0.061570915666
-0.353482084018 0.061519868363
-0.353339714638 0.0614687934037
-0.353197195977 0.0614176907841
-0.353054527854 0.0613665605003
-0.352911710088 0.0613154025486
-0.352768742498 0.061264216925
-0.352625624901 0.0612130036258
-0.352482357114 0.0611617626469
-0.352338938955 0.0611104939846
-0.352195370238 0.061059197635
-0.352051650781 0.0610078735942
-0.351907780399 0.0609565218584
-0.351763758906 0.0609051424237
-0.351619586117 0.0608537352863
-0.351475261845 0.0608023004423
-0.351330785904 0.060750837888
-0.351186158107 0.0606993476193
-0.351041378266 0.0606478296325
-0.350896446192 0.0605962839238
-0.350751361698 0.0605447104893
-0.350606124593 0.0604931093252
-0.350460734688 0.0604414804276
-0.350315191794 0.0603898237927
-0.350169495718 0.0603381394167
-0.35002364627 0.0602864272957
-0.349877643258 0.060234687426
-0.34973148649 0.0601829198037
-0.349585175773 0.0601311244249
-0.349438710913 0.0600793012859
-0.349292091717 0.0600274503828
-0.349145317989 0.0599755717119
-0.348998389536 0.0599236652692
-0.348851306162 0.0598717310511
-0.34870406767 0.0598197690536
-0.348556673864 0.059767779273
-0.348409124547 0.0597157617055
-0.348261419522 0.0596637163473
-0.348113558589 0.0596116431945
-0.347965541551 0.0595595422434
-0.347817368207 0.0595074134901
-0.347669038359 0.059455256931
-0.347520551806 0.0594030725621
-0.347371908346 0.0593508603797
-0.347223107779 0.05929862038
-0.347074149902 0.0592463525593
-0.346925034512 0.0591940569136
-0.346775761407 0.0591417334394
-0.346626330383 0.0590893821327
-0.346476741234 0.0590370029897
-0.346326993758 0.0589845960068
-0.346177087747 0.0589321611802
-0.346027022996 0.058879698506
-0.345876799298 0.0588272079805
-0.345726416447 0.0587746895999
-0.345575874234 0.0587221433605
-0.34542517245 0.0586695692585
-0.345274310888 0.0586169672901
-0.345123289338 0.0585643374516
-0.344972107588 0.0585116797392
-0.34482076543 0.0584589941492
-0.34466926265 0.0584062806778
-0.344517599038 0.0583535393213
-0.344365774382 0.0583007700758
-0.344213788467 0.0582479729377
-0.34406164108 0.0581951479033
-0.343909332007 0.0581422949687
-0.343756861033 0.0580894141302
-0.343604227942 0.0580365053842
-0.343451432519 0.0579835687268
-0.343298474546 0.0579306041543
-0.343145353806 0.057877611663
-0.342992070081 0.0578245912491
-0.342838623153 0.057771542909
-0.342685012803 0.0577184666388
-0.342531238809 0.057665362435
-0.342377300953 0.0576122302937
-0.342223199012 0.0575590702112
-0.342068932766 0.0575058821838
-0.341914501991 0.0574526662079
-0.341759906465 0.0573994222796
-0.341605145964 0.0573461503953
-0.341450220263 0.0572928505512
-0.341295129138 0.0572395227437
-0.341139872364 0.057186166969
-0.340984449713 0.0571327832234
-0.340828860958 0.0570793715033
-0.340673105873 0.0570259318049
-0.340517184229 0.0569724641246
-0.340361095798 0.0569189684586
-0.340204840348 0.0568654448032
-0.340048417651 0.0568118931548
-0.339891827476 0.0567583135096
-0.33973506959 0.0567047058641
-0.339578143762 0.0566510702144
-0.339421049758 0.0565974065569
-0.339263787346 0.0565437148879
-0.33910635629 0.0564899952038
-0.338948756356 0.0564362475008
-0.338790987308 0.0563824717753
-0.338633048909 0.0563286680236
-0.338474940923 0.0562748362421
-0.338316663112 0.056220976427
-0.338158215238 0.0561670885747
-0.33799959706 0.0561131726816
-0.33784080834 0.0560592287439
-0.337681848837 0.0560052567581
-0.337522718309 0.0559512567203
-0.337363416515 0.0558972286271
-0.337203943211 0.0558431724747
-0.337044298154 0.0557890882595
-0.336884481101 0.0557349759778
-0.336724491806 0.055680835626
-0.336564330023 0.0556266672004
-0.336403995507 0.0555724706975
-0.336243488009 0.0555182461134
-0.336082807283 0.0554639934446
-0.33592195308 0.0554097126876
-0.33576092515 0.0553554038385
-0.335599723243 0.0553010668938
-0.335438347108 0.0552467018498
-0.335276796495 0.055192308703
-0.33511507115 0.0551378874497
-0.33495317082 0.0550834380862
-0.334791095253 0.0550289606089
-0.334628844192 0.0549744550143
-0.334466417382 0.0549199212987
-0.334303814568 0.0548653594584
-0.334141035493 0.0548107694899
-0.333978079898 0.0547561513895
-0.333814947525 0.0547015051536
-0.333651638115 0.0546468307786
-0.333488151408 0.054592128261
-0.333324487143 0.054537397597
-0.333160645058 0.0544826387831
-0.332996624891 0.0544278518157
-0.332832426379 0.0543730366912
-0.332668049257 0.0543181934059
-0.33250349326 0.0542633219563
-0.332338758124 0.0542084223388
-0.33217384358 0.0541534945498
-0.332008749363 0.0540985385857
-0.331843475203 0.0540435544429
-0.331678020833 0.0539885421178
-0.331512385981 0.0539335016069
-0.331346570377 0.0538784329065
-0.331180573751 0.0538233360131
-0.331014395829 0.053768210923
-0.330848036338 0.0537130576328
-0.330681495004 0.0536578761388
-0.330514771553 0.0536026664374
-0.330347865708 0.0535474285252
-0.330180777194 0.0534921623984
-0.330013505732 0.0534368680536
-0.329846051044 0.0533815454872
-0.329678412852 0.0533261946956
-0.329510590874 0.0532708156753
-0.32934258483 0.0532154084226
-0.329174394439 0.0531599729341
-0.329006019417 0.0531045092061
-0.328837459481 0.0530490172352
-0.328668714347 0.0529934970177
-0.328499783728 0.0529379485502
-0.328330667339 0.052882371829
-0.328161364892 0.0528267668507
-0.3279918761 0.0527711336116
-0.327822200673 0.0527154721083
-0.327652338322 0.0526597823371
-0.327482288755 0.0526040642947
-0.32731205168 0.0525483179773
-0.327141626806 0.0524925433815
-0.326971013838 0.0524367405038
-0.326800212481 0.0523809093406
-0.326629222441 0.0523250498884
-0.326458043421 0.0522691621436
-0.326286675123 0.0522132461028
-0.326115117248 0.0521573017624
-0.325943369499 0.0521013291189
-0.325771431573 0.0520453281687
-0.32559930317 0.0519892989084
-0.325426983989 0.0519332413345
-0.325254473724 0.0518771554434
-0.325081772073 0.0518210412316
-0.32490887873 0.0517648986956
-0.324735793389 0.0517087278319
-0.324562515743 0.0516525286369
-0.324389045483 0.0515963011073
-0.324215382301 0.0515400452395
-0.324041525885 0.0514837610299
-0.323867475926 0.0514274484752
-0.323693232111 0.0513711075717
-0.323518794126 0.051314738316
-0.323344161658 0.0512583407046
-0.323169334391 0.0512019147341
-0.322994312008 0.0511454604009
-0.322819094193 0.0510889777015
-0.322643680627 0.0510324666324
-0.32246807099 0.0509759271903
-0.322292264963 0.0509193593715
-0.322116262223 0.0508627631726
-0.321940062447 0.0508061385902
-0.321763665313 0.0507494856207
-0.321587070496 0.0506928042607
-0.321410277669 0.0506360945068
-0.321233286505 0.0505793563554
-0.321056096677 0.050522589803
-0.320878707856 0.0504657948463
-0.320701119711 0.0504089714817
-0.320523331911 0.0503521197059
-0.320345344123 0.0502952395152
-0.320167156015 0.0502383309063
-0.319988767251 0.0501813938758
-0.319810177495 0.0501244284201
-0.319631386411 0.0500674345358
-0.319452393661 0.0500104122194
-0.319273198906 0.0499533614676
-0.319093801804 0.0498962822769
-0.318914202015 0.0498391746438
-0.318734399197 0.0497820385648
-0.318554393004 0.0497248740366
-0.318374183093 0.0496676810557
-0.318193769117 0.0496104596187
-0.318013150729 0.0495532097221
-0.317832327581 0.0494959313625
-0.317651299322 0.0494386245364
-0.317470065601 0.0493812892405
-0.317288626068 0.0493239254713
-0.317106980368 0.0492665332254
-0.316925128147 0.0492091124993
-0.31674306905 0.0491516632897
-0.316560802718 0.0490941855931
-0.316378328795 0.0490366794061
-0.316195646921 0.0489791447253
-0.316012756735 0.0489215815473
-0.315829657875 0.0488639898686
-0.315646349978 0.0488063696859
-0.315462832679 0.0487487209958
-0.315279105614 0.0486910437947
-0.315095168415 0.0486333380794
-0.314911020714 0.0485756038464
-0.314726662141 0.0485178410924
-0.314542092326 0.0484600498139
-0.314357310897 0.0484022300075
-0.314172317479 0.0483443816699
-0.313987111699 0.0482865047976
-0.313801693181 0.0482285993872
-0.313616061546 0.0481706654355
-0.313430216417 0.0481127029389
-0.313244157414 0.0480547118941
-0.313057884154 0.0479966922977
-0.312871396257 0.0479386441463
-0.312684693336 0.0478805674366
-0.312497775007 0.0478224621652
-0.312310640884 0.0477643283286
-0.312123290578 0.0477061659236
-0.311935723699 0.0476479749467
-0.311747939857 0.0475897553946
-0.31155993866 0.0475315072639
-0.311371719713 0.0474732305512
-0.311183282621 0.0474149252532
-0.310994626989 0.0473565913665
-0.310805752418 0.0472982288878
-0.310616658508 0.0472398378137
-0.310427344859 0.0471814181408
-0.310237811069 0.0471229698658
-0.310048056733 0.0470644929853
-0.309858081448 0.047005987496
-0.309667884805 0.0469474533945
-0.309477466397 0.0468888906775
-0.309286825815 0.0468302993416
-0.309095962646 0.0467716793835
-0.30890487648 0.0467130307999
-0.3087135669 0.0466543535874
-0.308522033493 0.0465956477426
-0.308330275841 0.0465369132622
-0.308138293525 0.046478150143
-0.307946086124 0.0464193583815
-0.307753653218 0.0463605379744
-0.307560994383 0.0463016889184
-0.307368109194 0.0462428112102
-0.307174997225 0.0461839048465
-0.306981658047 0.0461249698238
-0.306788091232 0.046066006139
-0.306594296348 0.0460070137886
-0.306400272962 0.0459479927694
-0.30620602064 0.0458889430781
-0.306011538946 0.0458298647113
-0.305816827442 0.0457707576657
-0.305621885689 0.045711621938
-0.305426713246 0.0456524575249
-0.305231309672 0.045593264423
-0.30503567452 0.0455340426292
-0.304839807347 0.0454747921401
-0.304643707703 0.0454155129523
-0.30444737514 0.0453562050626
-0.304250809208 0.0452968684677
-0.304054009452 0.0452375031643
-0.30385697542 0.045178109149
-0.303659706655 0.0451186864187
-0.303462202699 0.04505923497
-0.303264463093 0.0449997547995
-0.303066487375 0.0449402459042
-0.302868275083 0.0448807082805
-0.302669825752 0.0448211419254
-0.302471138915 0.0447615468354
-0.302272214103 0.0447019230073
-0.302073050847 0.0446422704378
-0.301873648675 0.0445825891237
-0.301674007113 0.0445228790616
-0.301474125685 0.0444631402484
-0.301274003914 0.0444033726807
-0.30107364132 0.0443435763552
-0.300873037424 0.0442837512687
-0.300672191741 0.044223897418
-0.300471103786 0.0441640147997
-0.300269773074 0.0441041034107
-0.300068199114 0.0440441632476
-0.299866381418 0.0439841943071
-0.299664319492 0.0439241965861
-0.299462012842 0.0438641700813
-0.299259460972 0.0438041147894
-0.299056663383 0.0437440307072
-0.298853619575 0.0436839178314
-0.298650329046 0.0436237761587
-0.298446791292 0.043563605686
-0.298243005806 0.04350340641
-0.298038972081 0.0434431783275
-0.297834689606 0.0433829214351
-0.29763015787 0.0433226357298
-0.297425376357 0.0432623212081
-0.297220344552 0.043201977867
-0.297015061936 0.0431416057031
-0.296809527989 0.0430812047133
-0.296603742188 0.0430207748942
-0.296397704009 0.0429603162428
-0.296191412925 0.0428998287557
-0.295984868408 0.0428393124298
-0.295778069925 0.0427787672617
-0.295571016946 0.0427181932484
-0.295363708933 0.0426575903865
-0.29515614535 0.0425969586728
-0.294948325657 0.0425362981043
-0.294740249312 0.0424756086775
-0.294531915772 0.0424148903894
-0.294323324491 0.0423541432367
-0.294114474919 0.0422933672161
-0.293905366506 0.0422325623246
-0.2936959987 0.0421717285589
-0.293486370945 0.0421108659157
-0.293276482684 0.042049974392
-0.293066333358 0.0419890539845
-0.292855922403 0.0419281046899
-0.292645249256 0.0418671265051
-0.29243431335 0.041806119427
-0.292223114117 0.0417450834523
-0.292011650984 0.0416840185778
-0.291799923379 0.0416229248003
-0.291587930724 0.0415618021167
-0.291375672442 0.0415006505238
-0.291163147951 0.0414394700184
-0.290950356668 0.0413782605972
-0.290737298008 0.0413170222572
-0.290523971382 0.0412557549952
-0.290310376199 0.0411944588079
-0.290096511866 0.0411331336923
-0.289882377788 0.041071779645
-0.289667973366 0.0410103966631
-0.289453298 0.0409489847432
-0.289238351085 0.0408875438823
-0.289023132017 0.0408260740771
-0.288807640187 0.0407645753245
-0.288591874984 0.0407030476214
-0.288375835795 0.0406414909645
-0.288159522002 0.0405799053508
-0.287942932987 0.0405182907771
-0.287726068129 0.0404566472401
-0.287508926804 0.0403949747368
-0.287291508384 0.0403332732641
-0.28707381224 0.0402715428187
-0.28685583774 0.0402097833975
-0.286637584248 0.0401479949974
-0.286419051128 0.0400861776152
-0.286200237737 0.0400243312479
-0.285981143434 0.0399624558921
-0.285761767571 0.0399005515449
-0.285542109501 0.039838618203
-0.28532216857 0.0397766558634
-0.285101944125 0.0397146645229
-0.284881435508 0.0396526441784
-0.284660642059 0.0395905948267
-0.284439563114 0.0395285164648
-0.284218198007 0.0394664090894
-0.283996546069 0.0394042726975
-0.283774606628 0.039342107286
-0.283552379008 0.0392799128517
-0.283329862533 0.0392176893914
-0.283107056519 0.0391554369022
-0.282883960284 0.0390931553809
-0.282660573141 0.0390308448243
-0.282436894398 0.0389685052294
-0.282212923363 0.038906136593
-0.281988659339 0.0388437389121
-0.281764101626 0.0387813121835
-0.281539249522 0.0387188564041
-0.281314102321 0.0386563715708
-0.281088659314 0.0385938576806
-0.280862919789 0.0385313147302
-0.280636883029 0.0384687427167
-0.280410548316 0.038406141637
-0.280183914928 0.0383435114878
-0.27995698214 0.0382808522662
-0.279729749223 0.038218163969
-0.279502215445 0.0381554465932
-0.279274380071 0.0380927001357
-0.279046242362 0.0380299245934
-0.278817801575 0.0379671199631
-0.278589056966 0.0379042862419
-0.278360007784 0.0378414234266
-0.278130653279 0.0377785315142
-0.277900992693 0.0377156105016
-0.277671025267 0.0376526603857
-0.277440750239 0.0375896811634
-0.277210166842 0.0375266728317
-0.276979274305 0.0374636353875
-0.276748071855 0.0374005688277
-0.276516558714 0.0373374731493
-0.276284734101 0.0372743483491
-0.276052597233 0.0372111944242
-0.27582014732 0.0371480113715
-0.275587383569 0.0370847991879
-0.275354305186 0.0370215578703
-0.275120911371 0.0369582874157
-0.27488720132 0.0368949878211
-0.274653174226 0.0368316590834
-0.274418829277 0.0367683011995
-0.27418416566 0.0367049141664
-0.273949182554 0.036641497981
-0.273713879137 0.0365780526404
-0.273478254582 0.0365145781414
-0.273242308059 0.036451074481
-0.273006038732 0.0363875416561
-0.272769445763 0.0363239796638
-0.272532528309 0.036260388501
-0.272295285523 0.0361967681647
-0.272057716554 0.0361331186518
-0.271819820546 0.0360694399592
-0.27158159664 0.0360057320841
-0.271343043973 0.0359419950232
-0.271104161677 0.0358782287737
-0.270864948879 0.0358144333324
-0.270625404704 0.0357506086964
-0.27038552827 0.0356867548627
-0.270145318692 0.0356228718281
-0.269904775081 0.0355589595898
-0.269663896543 0.0354950181446
-0.269422682179 0.0354310474896
-0.269181131087 0.0353670476217
-0.26893924236 0.035303018538
-0.268697015086 0.0352389602354
-0.268454448347 0.0351748727109
-0.268211541224 0.0351107559616
-0.267968292791 0.0350466099843
-0.267724702116 0.0349824347762
-0.267480768266 0.0349182303341
-0.267236490301 0.0348539966552
-0.266991867275 0.0347897337364
-0.26674689824 0.0347254415746
-0.266501582242 0.034661120167
-0.266255918321 0.0345967695105
-0.266009905513 0.0345323896022
-0.26576354285 0.0344679804389
-0.265516829358 0.0344035420179
-0.265269764058 0.034339074336
-0.265022345966 0.0342745773902
-0.264774574093 0.0342100511777
-0.264526447444 0.0341454956954
-0.264277965022 0.0340809109403
-0.26402912582 0.0340162969095
-0.26377992883 0.0339516536
-0.263530373036 0.0338869810087
-0.263280457419 0.0338222791329
-0.263030180952 0.0337575479693
-0.262779542604 0.0336927875152
-0.262528541339 0.0336279977675
-0.262277176116 0.0335631787232
-0.262025445886 0.0334983303795
-0.261773349596 0.0334334527333
-0.261520886189 0.0333685457816
-0.261268054599 0.0333036095216
-0.261014853757 0.0332386439502
-0.260761282587 0.0331736490645
-0.260507340008 0.0331086248615
-0.260253024933 0.0330435713384
-0.259998336268 0.0329784884921
-0.259743272914 0.0329133763196
-0.259487833767 0.0328482348181
-0.259232017716 0.0327830639847
-0.258975823644 0.0327178638162
-0.258719250428 0.0326526343099
-0.258462296938 0.0325873754627
-0.25820496204 0.0325220872718
-0.257947244592 0.0324567697341
-0.257689143446 0.0323914228468
-0.257430657448 0.0323260466069
-0.257171785437 0.0322606410115
-0.256912526247 0.0321952060577
-0.256652878705 0.0321297417425
-0.25639284163 0.032064248063
-0.256132413837 0.0319987250162
-0.255871594131 0.0319331725993
-0.255610381314 0.0318675908093
-0.255348774179 0.0318019796434
-0.255086771512 0.0317363390985
-0.254824372095 0.0316706691717
-0.254561574699 0.0316049698602
-0.254298378092 0.0315392411611
-0.254034781031 0.0314734830713
-0.25377078227 0.0314076955881
-0.253506380553 0.0313418787085
-0.253241574619 0.0312760324295
-0.252976363197 0.0312101567484
-0.252710745012 0.0311442516621
-0.252444718779 0.0310783171678
-0.252178283206 0.0310123532626
-0.251911436996 0.0309463599435
-0.251644178842 0.0308803372078
-0.251376507429 0.0308142850524
-0.251108421437 0.0307482034744
-0.250839919535 0.0306820924711
-0.250571000388 0.0306159520395
-0.25030166265 0.0305497821767
-0.250031904968 0.0304835828798
-0.249761725982 0.0304173541459
-0.249491124323 0.0303510959722
-0.249220098614 0.0302848083558
-0.248948647471 0.0302184912937
-0.248676769499 0.0301521447831
-0.248404463298 0.0300857688212
-0.248131727458 0.030019363405
-0.24785856056 0.0299529285317
-0.247584961178 0.0298864641984
-0.247310927877 0.0298199704022
-0.247036459211 0.0297534471402
-0.246761553729 0.0296868944097
-0.246486209969 0.0296203122076
-0.24621042646 0.0295537005312
-0.245934201724 0.0294870593777
-0.245657534272 0.029420388744
-0.245380422605 0.0293536886274
-0.245102865219 0.029286959025
-0.244824860596 0.029220199934
-0.244546407212 0.0291534113514
-0.244267503531 0.0290865932745
-0.24398814801 0.0290197457004
-0.243708339094 0.0289528686262
-0.243428075221 0.0288859620491
-0.243147354817 0.0288190259662
-0.242866176299 0.0287520603747
-0.242584538074 0.0286850652718
-0.242302438538 0.0286180406546
-0.24201987608 0.0285509865202
-0.241736849075 0.0284839028659
-0.24145335589 0.0284167896888
-0.241169394881 0.028349646986
-0.240884964394 0.0282824747547
-0.240600062763 0.0282152729921
-0.240314688313 0.0281480416953
-0.240028839358 0.0280807808616
-0.239742514199 0.028013490488
-0.239455711129 0.0279461705719
-0.239168428429 0.0278788211102
-0.238880664369 0.0278114421003
-0.238592417205 0.0277440335392
-0.238303685186 0.0276765954243
-0.238014466547 0.0276091277526
-0.237724759512 0.0275416305213
-0.237434562293 0.0274741037276
-0.23714387309 0.0274065473688
-0.236852690093 0.0273389614419
-0.236561011477 0.0272713459442
-0.236268835407 0.0272037008729
-0.235976160036 0.0271360262252
-0.235682983503 0.0270683219982
-0.235389303935 0.0270005881892
-0.235095119448 0.0269328247953
-0.234800428143 0.0268650318138
-0.234505228111 0.0267972092418
-0.234209517426 0.0267293570766
-0.233913294154 0.0266614753153
-0.233616556342 0.0265935639552
-0.23331930203 0.0265256229935
-0.233021529239 0.0264576524273
-0.232723235981 0.0263896522539
-0.23242442025 0.0263216224706
-0.232125080029 0.0262535630744
-0.231825213286 0.0261854740626
-0.231524817976 0.0261173554325
-0.231223892039 0.0260492071813
-0.230922433399 0.0259810293061
-0.230620439969 0.0259128218043
-0.230317909643 0.0258445846729
-0.230014840305 0.0257763179093
-0.22971122982 0.0257080215107
-0.229407076041 0.0256396954742
-0.229102376802 0.0255713397972
-0.228797129925 0.0255029544769
-0.228491333215 0.0254345395104
-0.228184984461 0.0253660948951
-0.227878081438 0.0252976206281
-0.227570621902 0.0252291167067
-0.227262603595 0.0251605831281
-0.226954024242 0.0250920198896
-0.226644881552 0.0250234269885
-0.226335173215 0.0249548044219
-0.226024896907 0.024886152187
-0.225714050285 0.0248174702813
-0.22540263099 0.0247487587018
-0.225090636646 0.0246800174459
-0.224778064856 0.0246112465107
-0.22446491321 0.0245424458936
-0.224151179277 0.0244736155918
-0.223836860608 0.0244047556026
-0.223521954737 0.0243358659232
-0.223206459178 0.0242669465508
-0.222890371427 0.0241979974828
-0.222573688962 0.0241290187164
-0.22225640924 0.0240600102488
-0.221938529699 0.0239909720774
-0.221620047759 0.0239219041993
-0.221300960819 0.0238528066119
-0.220981266258 0.0237836793124
-0.220660961435 0.0237145222981
-0.220340043689 0.0236453355663
-0.220018510337 0.0235761191142
-0.219696358677 0.0235068729392
-0.219373585985 0.0234375970384
-0.219050189515 0.0233682914092
-0.218726166501 0.0232989560489
-0.218401514154 0.0232295909547
-0.218076229664 0.0231601961239
-0.217750310196 0.0230907715538
-0.217423752897 0.0230213172418
-0.217096554887 0.022951833185
-0.216768713266 0.0228823193807
-0.216440225108 0.0228127758264
-0.216111087465 0.0227432025192
-0.215781297366 0.0226735994564
-0.215450851814 0.0226039666354
-0.215119747789 0.0225343040534
-0.214787982245 0.0224646117077
-0.214455552113 0.0223948895957
-0.214122454296 0.0223251377147
-0.213788685675 0.0222553560618
-0.213454243103 0.0221855446346
-0.213119123405 0.0221157034302
-0.212783323384 0.0220458324459
-0.212446839814 0.0219759316791
-0.21210966944 0.0219060011272
-0.211771808984 0.0218360407873
-0.211433255135 0.0217660506568
-0.21109400456 0.021696030733
-0.210754053892 0.0216259810133
-0.210413399738 0.021555901495
-0.210072038677 0.0214857921754
-0.209729967256 0.0214156530517
-0.209387181994 0.0213454841214
-0.20904367938 0.0212752853817
-0.20869945587 0.0212050568301
-0.208354507893 0.0211347984637
-0.208008831844 0.02106451028
-0.207662424087 0.0209941922762
-0.207315280955 0.0209238444498
-0.206967398746 0.020853466798
-0.206618773728 0.0207830593181
-0.206269402135 0.0207126220076
-0.205919280166 0.0206421548637
-0.205568403987 0.0205716578838
-0.205216769731 0.0205011310652
-0.204864373492 0.0204305744053
-0.204511211333 0.0203599879015
-0.204157279278 0.020289371551
-0.203802573317 0.0202187253512
-0.203447089401 0.0201480492994
-0.203090823445 0.0200773433931
-0.202733771327 0.0200066076296
-0.202375928886 0.0199358420061
-0.202017291921 0.0198650465202
-0.201657856193 0.019794221169
-0.201297617425 0.0197233659501
-0.200936571296 0.0196524808607
-0.200574713447 0.0195815658982
-0.200212039477 0.01951062106
-0.199848544942 0.0194396463435
-0.199484225357 0.0193686417459
-0.199119076193 0.0192976072647
-0.198753092878 0.0192265428972
-0.198386270795 0.0191554486409
-0.198018605283 0.019084324493
-0.197650091635 0.019013170451
-0.197280725098 0.0189419865123
-0.196910500874 0.0188707726741
-0.196539414114 0.0187995289339
-0.196167459923 0.0187282552891
-0.195794633359 0.018656951737
-0.195420929429 0.0185856182751
-0.195046343088 0.0185142549007
-0.194670869244 0.0184428616111
-0.194294502751 0.0183714384039
-0.193917238412 0.0182999852763
-0.193539070976 0.0182285022258
-0.193159995138 0.0181569892497
-0.192780005541 0.0180854463455
-0.19239909677 0.0180138735106
-0.192017263355 0.0179422707422
-0.191634499768 0.0178706380379
-0.191250800426 0.0177989753951
-0.190866159684 0.0177272828111
-0.19048057184 0.0176555602833
-0.19009403113 0.0175838078091
-0.189706531729 0.017512025386
-0.189318067752 0.0174402130113
-0.188928633247 0.0173683706825
-0.188538222201 0.017296498397
-0.188146828535 0.0172245961522
-0.187754446104 0.0171526639454
-0.187361068696 0.0170807017741
-0.186966690029 0.0170087096358
-0.186571303756 0.0169366875278
-0.186174903455 0.0168646354475
-0.185777482637 0.0167925533925
-0.185379034738 0.01672044136
-0.18497955312 0.0166482993475
-0.184579031072 0.0165761273525
-0.184177461806 0.0165039253723
-0.183774838457 0.0164316934045
-0.183371154083 0.0163594314463
-0.182966401659 0.0162871394953
-0.182560574083 0.0162148175489
-0.182153664168 0.0161424656046
-0.181745664644 0.0160700836596
-0.181336568157 0.0159976717116
-0.180926367265 0.0159252297579
-0.18051505444 0.0158527577959
-0.180102622064 0.0157802558232
-0.179689062427 0.015707723837
-0.179274367728 0.015635161835
-0.178858530072 0.0155625698145
-0.178441541469 0.015489947773
-0.17802339383 0.015417295708
-0.17760407897 0.0153446136168
-0.177183588601 0.0152719014969
-0.176761914334 0.0151991593458
-0.176339047677 0.0151263871609
-0.17591498003 0.0150535849397
-0.175489702687 0.0149807526797
-0.175063206833 0.0149078903783
-0.174635483538 0.0148349980329
-0.174206523763 0.0147620756411
-0.17377631835 0.0146891232002
-0.173344858026 0.0146161407078
-0.172912133396 0.0145431281613
-0.172478134945 0.0144700855581
-0.172042853032 0.0143970128958
-0.171606277891 0.0143239101719
-0.171168399626 0.0142507773837
-0.170729208212 0.0141776145288
-0.170288693487 0.0141044216046
-0.169846845155 0.0140311986086
-0.169403652781 0.0139579455383
-0.168959105789 0.0138846623912
-0.168513193458 0.0138113491647
-0.16806590492 0.0137380058564
-0.167617229158 0.0136646324636
-0.167167155003 0.013591228984
-0.166715671128 0.0135177954149
-0.166262766049 0.0134443317539
-0.165808428121 0.0133708379984
-0.165352645532 0.013297314146
-0.164895406303 0.0132237601941
-0.164436698282 0.0131501761402
-0.163976509144 0.0130765619819
-0.163514826383 0.0130029177166
-0.163051637311 0.0129292433417
-0.162586929055 0.0128555388549
-0.162120688551 0.0127818042536
-0.16165290254 0.0127080395353
-0.161183557567 0.0126342446976
-0.160712639974 0.0125604197378
-0.160240135894 0.0124865646536
-0.159766031253 0.0124126794424
-0.159290311759 0.0123387641017
-0.1588129629 0.0122648186291
-0.158333969939 0.0121908430221
-0.15785331791 0.0121168372781
-0.157370991611 0.0120428013947
-0.1568869756 0.0119687353694
-0.156401254189 0.0118946391998
-0.155913811441 0.0118205128832
-0.155424631159 0.0117463564174
-0.154933696886 0.0116721697997
-0.154440991895 0.0115979530277
-0.153946499184 0.0115237060989
-0.15345020147 0.0114494290109
-0.152952081184 0.0113751217612
-0.15245212046 0.0113007843473
-0.151950301131 0.0112264167667
-0.151446604722 0.011152019017
-0.15094101244 0.0110775910957
-0.150433505171 0.0110031330003
-0.149924063468 0.0109286447284
-0.149412667542 0.0108541262775
-0.14889929726 0.0107795776452
-0.148383932127 0.0107049988289
-0.147866551287 0.0106303898263
-0.147347133506 0.0105557506349
-0.146825657166 0.0104810812521
-0.146302100255 0.0104063816756
-0.145776440355 0.010331651903
-0.145248654634 0.0102568919316
-0.144718719834 0.0101821017592
-0.144186612258 0.0101072813833
-0.143652307763 0.0100324308013
-0.143115781742 0.00995755001092
-0.142577009116 0.00988263900965
-0.142035964319 0.00980769779506
-0.141492621287 0.00973272636469
-0.14094695344 0.00965772471612
-0.140398933673 0.00958269284691
-0.139848534335 0.00950763075461
-0.13929572722 0.00943253843679
-0.138740483546 0.00935741589101
-0.138182773943 0.00928226311485
-0.13762256843 0.00920708010586
-0.137059836403 0.00913186686163
-0.136494546614 0.00905662337971
-0.135926667151 0.00898134965769
-0.135356165419 0.00890604569313
-0.13478300812 0.00883071148361
-0.134207161232 0.00875534702671
-0.133628589983 0.00867995232001
-0.133047258831 0.00860452736107
-0.132463131441 0.0085290721475
-0.131876170655 0.00845358667686
-0.131286338471 0.00837807094674
-0.130693596011 0.00830252495472
-0.130097903497 0.00822694869839
-0.129499220219 0.00815134217535
-0.128897504504 0.00807570538317
-0.128292713682 0.00800003831945
-0.127684804059 0.00792434098177
-0.127073730874 0.00784861336774
-0.126459448265 0.00777285547495
-0.125841909235 0.00769706730099
-0.125221065604 0.00762124884346
-0.124596867974 0.00754540009996
-0.123969265682 0.00746952106809
-0.123338206755 0.00739361174545
-0.122703637861 0.00731767212965
-0.122065504258 0.00724170221828
-0.121423749745 0.00716570200895
-0.120778316603 0.00708967149928
-0.120129145538 0.00701361068686
-0.119476175619 0.00693751956931
-0.118819344219 0.00686139814424
-0.118158586939 0.00678524640926
-0.117493837545 0.00670906436199
-0.11682502789 0.00663285200004
-0.116152087837 0.00655660932103
-0.115474945175 0.00648033632257
-0.114793525533 0.00640403300229
-0.114107752289 0.00632769935781
-0.11341754647 0.00625133538674
-0.112722826655 0.00617494108672
-0.112023508862 0.00609851645536
-0.111319506437 0.00602206149029
-0.110610729931 0.00594557618915
-0.109897086973 0.00586906054955
-0.109178482135 0.00579251456914
-0.108454816787 0.00571593824553
-0.107725988946 0.00563933157637
-0.10699189311 0.00556269455929
-0.106252420089 0.00548602719193
-0.105507456824 0.00540932947191
-0.104756886184 0.00533260139689
-0.104000586764 0.0052558429645
-0.103238432662 0.00517905417238
-0.102470293239 0.00510223501818
-0.10169603287 0.00502538549954
-0.100915510668 0.0049485056141
-0.100128580196 0.00487159535951
-0.0993350891559 0.00479465473342
-0.0985348790534 0.00471768373348
-0.0977277848384 0.00464068235733
-0.0969136345188 0.00456365060265
-0.0960922487443 0.00448658846706
-0.0952634403573 0.00440949594824
-0.0944270139079 0.00433237304383
-0.0935827651296 0.0042552197515
-0.0927304803714 0.0041780360689
-0.0918699359823 0.00410082199369
-0.0910008976426 0.00402357752354
-0.0901231196364 0.00394630265611
-0.0892363440595 0.00386899738906
-0.0883402999548 0.00379166172006
-0.0874347023668 0.00371429564678
-0.086519251307 0.00363689916688
-0.0855936306179 0.00355947227803
-0.0846575067247 0.00348201497791
-0.0837105272605 0.00340452726419
-0.0827523195475 0.00332700913454
-0.081782488918 0.00324946058663
-0.0808006168518 0.00317188161815
-0.0798062589056 0.00309427222677
-0.0787989424058 0.00301663241017
-0.0777781638696 0.00293896216604
-0.0767433861153 0.00286126149204
-0.0756940350149 0.00278353038587
-0.0746294958318 0.00270576884521
-0.0735491090786 0.00262797686775
-0.072452165815 0.00255015445118
-0.0713379022904 0.00247230159317
-0.0702054938162 0.00239441829143
-0.0690540477281 0.00231650454365
-0.0678825952669 0.00223856034751
-0.0666900821681 0.00216058570071
-0.0654753576995 0.00208258060094
-0.0642371618227 0.00200454504591
-0.0629741100698 0.00192647903332
-0.0616846756173 0.00184838256085
-0.0603671678962 0.00177025562621
-0.0590197068824 0.00169209822711
-0.05764019195 0.00161391036124
-0.0562262638138 0.00153569202631
-0.0547752575874 0.00145744322003
-0.0532841442828 0.0013791639401
-0.0517494570698 0.00130085418424
-0.0501671971407 0.00122251395015
-0.048532711832 0.00114414323555
-0.0468405342995 0.00106574203814
-0.0450841687961 0.00098731035564
-0.0432557971315 0.000908848185769
-0.0413458677718 0.00083035552624
-0.0393425045594 0.000751832374772
-0.0372306276483 0.000673278729085
-0.0349905943368 0.000594694586898
-0.0325959941691 0.000516079945934
-0.0300098494929 0.000437434803916
-0.0271775345492 0.000358759158568
-0.0240120967147 0.000280053007616
-0.0203587396461 0.000201316348789
-0.0158842959616 0.000122549179813


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularMeanZero.tex <==
-0.450442616461 0.0590073193873
-0.449561731229 0.05892590042
-0.448680845996 0.0586060482466
-0.447799960763 0.058520782129
-0.44691907553 0.0584343392036
-0.446038190297 0.0581117702745
-0.445157305064 0.0580236436336
-0.444276419831 0.0579347690681
-0.443395534598 0.0576109158272
-0.442514649365 0.0575209066343
-0.441633764132 0.0574303384114
-0.440752878899 0.0571058008867
-0.439871993666 0.0570143892828
-0.438991108433 0.0569225315914
-0.438110223201 0.0565976690237
-0.437229337968 0.0565051566626
-0.436348452735 0.0564122755598
-0.435467567502 0.0560873361998
-0.434586682269 0.0559939358661
-0.433705797036 0.0559002240555
-0.432824911803 0.0555753938021
-0.43194402657 0.0554812662598
-0.431063141337 0.0551567830968
-0.430182256104 0.0550622973043
-0.429301370871 0.0549675696923
-0.428420485638 0.054643425936
-0.427539600405 0.0545484122656
-0.426658715173 0.0544531884667
-0.42577782994 0.0541294904994
-0.424896944707 0.0540340409752
-0.424016059474 0.0537108860431
-0.423135174241 0.0536152464278
-0.422254289008 0.0535194391298
-0.421373403775 0.0531968753871
-0.420492518542 0.053100924622
-0.419611633309 0.0527789923738
-0.418730748076 0.0526829263319
-0.417849862843 0.0525867258664
-0.41696897761 0.0522655013098
-0.416088092377 0.0521692230084
-0.415207207145 0.0518487024015
-0.414326321912 0.0517523693038
-0.413445436679 0.0516559287175
-0.412564551446 0.0513362122703
-0.411683666213 0.0512397478125
-0.41080278098 0.0511431896421
-0.409921895747 0.0508243273187
-0.409041010514 0.0507277731537
-0.408160125281 0.0504097077145
-0.407279240048 0.0503131750713
-0.406398354815 0.0499959271471
-0.405517469582 0.0498994324947
-0.404636584349 0.0498028716275
-0.403755699117 0.0494865805185
-0.402874813884 0.0493900800425
-0.401993928651 0.0490746524154
-0.401113043418 0.0489782266017
-0.400232158185 0.048881750824
-0.399351272952 0.0485673421651
-0.398470387719 0.0484709605414
-0.397589502486 0.0481574561341
-0.396708617253 0.0480611811848
-0.39582773202 0.0479648704075
-0.394946846787 0.0476524402067
-0.394065961554 0.047556253257
-0.393185076321 0.0472447638685
-0.392304191089 0.0471487118442
-0.391423305856 0.0470526364158
-0.390542420623 0.0467422708274
-0.38966153539 0.0466463455629
-0.388780650157 0.0463369538752
-0.387899764924 0.0462411886977
-0.387018879691 0.0459327837345
-0.386137994458 0.0458371881496
-0.385257109225 0.0457415843165
-0.384376223992 0.0454343654149
-0.383495338759 0.0453389442539
-0.382614453526 0.0450327412089
-0.381733568293 0.0449375113056
-0.380852683061 0.0446323355141
-0.379971797828 0.0445373051232
-0.379090912595 0.0444422794714
-0.378210027362 0.0441383446896
-0.377329142129 0.0440435299211
-0.376448256896 0.0437406483572
-0.375567371663 0.0436460519895
-0.37468648643 0.0433442338833
-0.373805601197 0.0432498631662
-0.372924715964 0.0431555084476
-0.372043830731 0.0428549803928
-0.371162945498 0.0427608613156
-0.370282060265 0.0424614200925
-0.369401175033 0.0423675433047
-0.3685202898 0.0420691981961
-0.367639404567 0.0419755701249
-0.366758519334 0.0418819679092
-0.365877634101 0.0415849570307
-0.364996748868 0.0414916123885
-0.364115863635 0.0411957188425
-0.363234978402 0.0411026377022
-0.362354093169 0.0408078699675
-0.361473207936 0.0407150580731
-0.360592322703 0.040622280734
-0.35971143747 0.0403288873389
-0.358830552237 0.0402363871569
-0.357949667005 0.0399441389694
-0.357068781772 0.0398519212693
-0.356187896539 0.039560826083
-0.355307011306 0.0394688960334
-0.354426126073 0.0391789614615
-0.35354524084 0.0390873240819
-0.352664355607 0.0389957310839
-0.351783470374 0.0387072177321
-0.350902585141 0.0386159243097
-0.350021699908 0.0383285889986
-0.349140814675 0.0382375998305
-0.348259929442 0.0379514496058
-0.347379044209 0.0378607692426
-0.346498158977 0.0377701399636
-0.345617273744 0.0374854438689
-0.344736388511 0.0373951296481
-0.343855503278 0.0371116347689
-0.342974618045 0.0370216398636
-0.342093732812 0.0367393527494
-0.341212847579 0.036649681306
-0.340331962346 0.0363686083732
-0.339451077113 0.0362792644316
-0.33857019188 0.0359994119686
-0.337689306647 0.0359103994662
-0.336808421414 0.0358214473359
-0.335927536181 0.0355430964131
-0.335046650949 0.0354544811207
-0.334165765716 0.0351773650608
-0.333284880483 0.0350890903079
-0.33240399525 0.0348132149904
-0.331523110017 0.0347252843888
-0.330642224784 0.0344506555828
-0.329761339551 0.0343630726578
-0.328880454318 0.0342755566813
-0.327999569085 0.0340024642184
-0.327118683852 0.0339153007417
-0.326237798619 0.0336434679899
-0.325356913386 0.0335566603382
-0.324476028153 0.033286092713
-0.323595142921 0.0331996441349
-0.322714257688 0.0329303469553
-0.321833372455 0.0328442606257
-0.320952487222 0.0325762391171
-0.320071601989 0.0324905181391
-0.319190716756 0.032404871171
-0.318309831523 0.0321384248437
-0.31742894629 0.032053147461
-0.316548061057 0.0317879887527
-0.315667175824 0.0317030838928
-0.314786290591 0.0314392177285
-0.313905405358 0.031354688265
-0.313024520125 0.0310921194869
-0.312143634893 0.0310079682318
-0.31126274966 0.0307467016017
-0.310381864427 0.0306629313068
-0.309500979194 0.0305792411646
-0.308620093961 0.0303195848675
-0.307739208728 0.0302362794285
-0.306858323495 0.0299779361585
-0.305977438262 0.0298950180354
-0.305096553029 0.0296379922953
-0.304215667796 0.0295554640471
-0.303334782563 0.029299760268
-0.30245389733 0.029217624401
-0.301573012097 0.0289632469441
-0.300692126865 0.0288815059142
-0.299811241632 0.0287998504157
-0.298930356399 0.0285471152857
-0.298049471166 0.0284658579536
-0.297168585933 0.0282144590999
-0.2962877007 0.0281336022717
-0.295406815467 0.0278835438296
-0.294525930234 0.0278030897966
-0.293645045001 0.0275543758383
-0.292764159768 0.0274743268473
-0.291883274535 0.0272269613832
-0.291002389302 0.0271473196375
-0.290121504069 0.026901306618
-0.289240618837 0.0268220742783
-0.288359733604 0.0267429330225
-0.287478848371 0.0264985967806
-0.286597963138 0.0264198678485
-0.285717077905 0.0261768930574
-0.284836192672 0.0260985785112
-0.283955307439 0.0258569689265
-0.283074422206 0.0257790707893
-0.282193536973 0.0255388301117
-0.28131265174 0.0254613503693
-0.280431766507 0.0252224822461
-0.279550881274 0.0251454228474
-0.278669996041 0.0249079308732
-0.277789110809 0.0248312937313
-0.276908225576 0.0247547524827
-0.276027340343 0.0245189684423
-0.27514645511 0.0244428520233
-0.274265569877 0.0242084523174
-0.273384684644 0.0241327625576
-0.272503799411 0.0238997506106
-0.271622914178 0.0238244893067
-0.270742028945 0.023592868495
-0.269861143712 0.0235180374116
-0.268980258479 0.0232878110644
-0.268099373246 0.0232134119348
-0.267218488013 0.022984583335
-0.266337602781 0.0229106178617
-0.265456717548 0.0226831902468
-0.264575832315 0.0226096601026
-0.263694947082 0.0225362306486
-0.262814061849 0.0223105434937
-0.261933176616 0.0222375516076
-0.261052291383 0.0220132727989
-0.26017140615 0.0219407200836
-0.259290520917 0.0217178527108
-0.258409635684 0.0216457407417
-0.257528750451 0.0214242878529
-0.256647865218 0.0213526181783
-0.255766979985 0.0211325827798
-0.254886094753 0.0210613569216
-0.25400520952 0.0208427419795
-0.253124324287 0.0207719614338
-0.252243439054 0.0205547698742
-0.251362553821 0.0204844361115
-0.250481668588 0.0202686708212
-0.249600783355 0.0201987852877
-0.248719898122 0.0201290050728
-0.247839012889 0.0199150132321
-0.246958127656 0.019845683171
-0.246077242423 0.0196331241529
-0.24519635719 0.0195642456338
-0.244315471957 0.0193531221977
-0.243434586725 0.0192846965857
-0.242553701492 0.0190750114545
-0.241672816259 0.0190070400922
-0.240791931026 0.0187987959525
-0.239911045793 0.0187312801604
-0.23903016056 0.0185244796638
-0.238149275327 0.0184574207407
-0.237268390094 0.0182520665035
-0.236387504861 0.0181854657271
-0.235506619628 0.0179815603313
-0.234625734395 0.0179154189583
-0.233744849162 0.0177129649523
-0.232863963929 0.0176472842191
-0.231983078697 0.0175817131479
-0.231102193464 0.0173810652404
-0.230221308231 0.0173159564446
-0.229340422998 0.017116765701
-0.228459537765 0.0170521203693
-0.227578652532 0.0168543892277
-0.226697767299 0.0167902085299
-0.225816882066 0.0165939393964
-0.224935996833 0.0165302244834
-0.2240551116 0.016335419733
-0.223174226367 0.0162721717374
-0.222293341134 0.0160788337142
-0.221412455901 0.0160160537504
-0.220531570669 0.0158241847679
-0.219650685436 0.0157618739327
-0.218769800203 0.0155714762742
-0.21788891497 0.0155096356468
-0.217008029737 0.0153207115661
-0.216127144504 0.0152593422088
-0.215246259271 0.0151980861386
-0.214365374038 0.0150109968884
-0.213484488805 0.014950213485
-0.212603603572 0.0147646029099
-0.211722718339 0.0147042931957
-0.210841833106 0.0145201634528
-0.209960947873 0.0144603284341
-0.209080062641 0.0142776816524
-0.208199177408 0.0142183223198
-0.207318292175 0.0140371606005
-0.206437406942 0.0139782779288
-0.205556521709 0.0137986033458
-0.204675636476 0.0137401982947
-0.203794751243 0.013562012895
-0.20291386601 0.013504086409
-0.202032980777 0.0133273922126
-0.201152095544 0.0132699452216
-0.200271210311 0.0130947442222
-0.199390325078 0.0130377776414
-0.198509439846 0.0128640718065
-0.197628554613 0.0128075865368
-0.19674766938 0.0126353778083
-0.195866784147 0.0125793747365
-0.194985898914 0.0125234885762
-0.194105013681 0.0123531450297
-0.193224128448 0.012297742225
-0.192343243215 0.0121289001666
-0.191462357982 0.0120739815717
-0.190581472749 0.0119066428592
-0.189700587516 0.0118522093149
-0.188819702283 0.0116863757816
-0.18793881705 0.0116324281155
-0.187057931818 0.0114681015702
-0.186177046585 0.011414640597
-0.185296161352 0.0112518228248
-0.184415276119 0.0111988493465
-0.183534390886 0.0110375421083
-0.182653505653 0.0109850569143
-0.18177262042 0.0108252619477
-0.180891735187 0.010773265815
-0.180010849954 0.0106149848343
-0.179129964721 0.0105634785279
-0.178249079488 0.0104067132242
-0.177368194255 0.0103556974968
-0.176487309022 0.0102004495386
-0.17560642379 0.0101499251312
-0.174725538557 0.00999619616413
-0.173844653324 0.00994616380614
-0.172963768091 0.00989625152897
-0.172082882858 0.0097444158628
-0.171201997625 0.00969499657991
-0.170321112392 0.00954468360885
-0.169440227159 0.00949575802258
-0.168559341926 0.00934696931883
-0.167678456693 0.00929853812041
-0.16679757146 0.00915127523446
-0.165916686227 0.00910333910415
-0.165035800994 0.00895760356506
-0.164154915762 0.00891016317228
-0.163274030529 0.00876595648782
-0.162393145296 0.00871901249133
-0.161512260063 0.00857633614819
-0.16063137483 0.0085298891962
-0.159750489597 0.0083887446602
-0.158869604364 0.00834279539052
-0.157988719131 0.00820318410677
-0.157107833898 0.00815773314693
-0.156226948665 0.00801965654001
-0.155346063432 0.00797470450742
-0.154465178199 0.00783816398157
-0.153584292966 0.00779371148363
-0.152703407734 0.0076587084229
-0.151822522501 0.00761475605711
-0.150941637268 0.00748129182556
-0.150060752035 0.00743784017968
-0.149179866802 0.00730591612152
-0.148298981569 0.00726296577364
-0.147418096336 0.00722013838791
-0.146537211103 0.0070901347321
-0.14565632587 0.00704780938699
-0.144775440637 0.00691934891924
-0.143894555404 0.00687752617066
-0.143013670171 0.00675061017056
-0.142132784938 0.00670929056516
-0.141251899706 0.00658392029317
-0.140371014473 0.00654310436846
-0.13949012924 0.006419281066
-0.138609244007 0.00637896935045
-0.137728358774 0.00625669424009
-0.136847473541 0.00621688725324
-0.135966588308 0.00609616153882
-0.135085703075 0.00605685979136
-0.134204817842 0.00593768465814
-0.133323932609 0.00589888865202
-0.132443047376 0.00578126526681
-0.131562162143 0.00574297549535
-0.13068127691 0.00562690500664
-0.129800391678 0.00558912195459
-0.128919506445 0.00547460549267
-0.128038621212 0.00543732963634
-0.127157735979 0.00532436831344
-0.126276850746 0.00528760012075
-0.125395965513 0.00517619503118
-0.12451508028 0.00513993496177
-0.123634195047 0.005030087182
-0.122753309814 0.00499433568732
-0.121872424581 0.00488604627612
-0.120991539348 0.0048508037995
-0.120110654115 0.00481568661281
-0.119229768882 0.0047093407748
-0.11834888365 0.00467473317055
-0.117467998417 0.00456994806428
-0.116587113184 0.00453585046721
-0.115706227951 0.00443262709375
-0.114825342718 0.00439903992077
-0.113944457485 0.00429737926399
-0.113063572252 0.0042643029242
-0.112182687019 0.00416420595089
-0.111301801786 0.00413164084572
-0.110420916553 0.00403310850564
-0.10954003132 0.00400105502889
-0.108659146087 0.00390408825489
-0.107778260854 0.00387254679282
-0.106897375622 0.00377714650097
-0.106016490389 0.00374611743231
-0.105135605156 0.00365228452197
-0.104254719923 0.00362176821808
-0.10337383469 0.00352950357197
-0.102492949457 0.00349950039681
-0.101612064224 0.00340880488116
-0.100731178991 0.00337931519143
-0.0998502937581 0.00329018965601
-0.0989694085252 0.00326121380116
-0.0980885232923 0.00317365907941
-0.0972076380594 0.00314519740171
-0.0963267528264 0.00305921431081
-0.0954458675935 0.00303126714543
-0.0945649823606 0.00294685648638
-0.0936840971277 0.00291942416144
-0.0928032118948 0.00283658671913
-0.0919223266618 0.00280966955573
-0.0910414414289 0.00272840609907
-0.090160556196 0.00270200441137
-0.0892796709631 0.00262231569329
-0.0883987857301 0.00259642978856
-0.0875179004972 0.00257067114904
-0.0866370152643 0.00249294672483
-0.0857561300314 0.00246770425496
-0.0848752447984 0.00239155623511
-0.0839943595655 0.00236683022643
-0.0831134743326 0.00229225931186
-0.0822325890997 0.00226805004921
-0.0813517038668 0.00219505692522
-0.0804708186338 0.00217136468674
-0.0795899334009 0.00209995002309
-0.078709048168 0.0020767750803
-0.0778281629351 0.00200693953126
-0.0769472777021 0.00198428214909
-0.0760663924692 0.0019160263535
-0.0751855072363 0.00189388679035
-0.0743046220034 0.0018272113717
-0.0734237367704 0.00180558987946
-0.0725428515375 0.00174049544593
-0.0716619663046 0.00171939227004
-0.0707810810717 0.00165587941458
-0.0699001958388 0.00163529479405
-0.0690193106058 0.00157336409443
-0.0681384253729 0.00155329826189
-0.06725754014 0.00149295028074
-0.0663766549071 0.00147340346249
-0.0654957696741 0.00141463874737
-0.0646148844412 0.0013956111634
-0.0637339992083 0.00133843024686
-0.0628531139754 0.00131992211088
-0.0619722287425 0.00126432551049
-0.0610913435095 0.00124633702999
-0.0602104582766 0.00119232524841
-0.0593295730437 0.00117485662464
-0.0584486878108 0.00112243014966
-0.0575678025778 0.00110548157773
-0.0566869173449 0.0010546408823
-0.055806032112 0.00103821255118
-0.0549251468791 0.000988958093485
-0.0540442616461 0.000973050186007
-0.0531633764132 0.000925382409497
-0.0522824911803 0.000909995102428
-0.0514016059474 0.000894736423917
-0.0505207207145 0.000849047899899
-0.0496398354815 0.00083431004002
-0.0487589502486 0.000790209157196
-0.0478780650157 0.000775992278877
-0.0469971797828 0.000733479432477
-0.0461162945498 0.000719783692655
-0.0452354093169 0.000678859263346
-0.044354524084 0.000665684812992
-0.0434736388511 0.000626349166911
-0.0425927536181 0.00061369615105
-0.0417118683852 0.000575949639841
-0.0408309831523 0.00056381819758
-0.0399500979194 0.000527661158425
-0.0390692126865 0.00051605142297
-0.0381883274535 0.000481484178621
-0.0373074422206 0.000470396277297
-0.0364265569877 0.000437419136107
-0.0355456717548 0.000426853190383
-0.0346647865218 0.000395466446333
-0.0337839012889 0.000385422571835
-0.032903016056 0.000355626504561
-0.0320221308231 0.000346104811092
-0.0311412455901 0.000317899685913
-0.0302603603572 0.000308900277471
-0.0293794751243 0.000282286345411
-0.0284985898914 0.000273809320202
-0.0276177046585 0.000248786818016
-0.0267368194255 0.000240832268473
-0.0258559341926 0.000217401418666
-0.0249750489597 0.000209969431459
-0.0240941637268 0.000188130442307
-0.0232132784938 0.000181221098359
-0.0223323932609 0.000160974163931
-0.021451508028 0.000154587538429
-0.0205706227951 0.000135932838603
-0.0196897375622 0.00013006900101
-0.0188088523292 0.000113006701486
-0.0179279670963 0.000107665715554
-0.0170470818634 9.2195967874e-05
-0.0161661966305 8.73778916484e-05
-0.0152853113975 7.35008332104e-05
-0.0144044261646 6.92057190432e-05
-0.0135235409317 5.69214731108e-05
-0.0126426556988 5.31493676672e-05
-0.0117617704658 4.95065486174e-05
-0.0108808852329 3.9208987648e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularProb0pt2.tex <==
-0.450442616461 0.00571066117218
-0.449995759368 0.00570759889139
-0.449548902275 0.00570027636448
-0.449102045182 0.00569721866103
-0.448655188089 0.00569209411223
-0.448208330995 0.00568478374297
-0.447761473902 0.00568126593488
-0.447314616809 0.00567541097007
-0.446867759716 0.00567019710223
-0.446420902622 0.00566257191538
-0.445974045529 0.00565851988146
-0.445527188436 0.00565199993758
-0.445080331343 0.00564898038458
-0.444633474249 0.00564345338303
-0.444186617156 0.00563839185952
-0.443739760063 0.00563080727676
-0.44329290297 0.00562662576773
-0.442846045876 0.00562285553824
-0.442399188783 0.00561653250602
-0.44195233169 0.00561060485351
-0.441505474597 0.00560505957072
-0.441058617504 0.00559988449744
-0.44061176041 0.00559506822404
-0.440164903317 0.00559060000815
-0.439718046224 0.00558356098891
-0.439271189131 0.00557976575973
-0.438824332037 0.00557339455379
-0.438377474944 0.00557023583524
-0.437930617851 0.00556449779659
-0.437483760758 0.00555906773713
-0.437036903664 0.00555393811821
-0.436590046571 0.00554910170811
-0.436143189478 0.00554455155844
-0.435696332385 0.00553743366724
-0.435249475291 0.00553344311915
-0.434802618198 0.00552688597104
-0.434355761105 0.00552343019809
-0.433908904012 0.00551740986398
-0.433462046919 0.00551165291251
-0.433015189825 0.00550895975018
-0.432568332732 0.00550370653302
-0.432121475639 0.00549870092404
-0.431674618546 0.00549393796895
-0.431227761452 0.00548663490731
-0.430780904359 0.00548234992973
-0.430334047266 0.00547829354115
-0.429887190173 0.00547170434907
-0.429440333079 0.00546809891805
-0.428993475986 0.00546196615802
-0.428546618893 0.0054587947694
-0.4280997618 0.00545310196025
-0.427652904706 0.00544762670303
-0.427206047613 0.00544236515832
-0.42675919052 0.00543731356908
-0.426312333427 0.00543246825725
-0.425865476334 0.00542782562047
-0.42541861924 0.0054233821291
-0.424971762147 0.00541913432333
-0.424524905054 0.00541507881053
-0.424078047961 0.00540854710611
-0.423631190867 0.00540487336563
-0.423184333774 0.00540138212447
-0.422737476681 0.00539542641069
-0.422290619588 0.00538966119761
-0.421843762494 0.00538671304787
-0.421396905401 0.00538131269324
-0.420950048308 0.00537609391998
-0.420503191215 0.00537105385519
-0.420056334122 0.00536879071031
-0.419609477028 0.0053640924819
-0.419162619935 0.00535956461264
-0.418715762842 0.00535262482257
-0.418268905749 0.00534843678723
-0.417822048655 0.00534441115266
-0.417375191562 0.00534054534395
-0.416928334469 0.00533683682404
-0.416481477376 0.00533073933319
-0.416034620282 0.00532734510139
-0.415587763189 0.00532157135847
-0.415140906096 0.00531848170624
-0.414694049003 0.00531302214932
-0.414247191909 0.00530771977302
-0.413800334816 0.00530507295956
-0.413353477723 0.00530007090868
-0.41290662063 0.00529521924909
-0.412459763537 0.0052905157768
-0.412012906443 0.00528595831581
-0.41156604935 0.00528154471744
-0.411119192257 0.00527727285971
-0.410672335164 0.0052731406468
-0.41022547807 0.00526914600842
-0.409778620977 0.0052652868993
-0.409331763884 0.00526156129866
-0.408884906791 0.00525554571937
-0.408438049697 0.00525208837471
-0.407991192604 0.00524875861865
-0.407544335511 0.00524315465575
-0.407097478418 0.00524008152285
-0.406650621324 0.00523474481262
-0.406203764231 0.00523192076665
-0.405756907138 0.00522684385869
-0.405310050045 0.00522189771552
-0.404863192952 0.00521708053527
-0.404416335858 0.00521473992372
-0.403969478765 0.00521016812692
-0.403522621672 0.00520572000142
-0.403075764579 0.00520139382031
-0.402628907485 0.00519718787456
-0.402182050392 0.00519310047277
-0.401735193299 0.00518912994081
-0.401288336206 0.0051852746216
-0.400841479112 0.00518153287481
-0.400394622019 0.00517790307656
-0.399947764926 0.00517210633968
-0.399500907833 0.00516870283733
-0.399054050739 0.00516540650681
-0.398607193646 0.00515996013071
-0.398160336553 0.00515688067876
-0.39771347946 0.00515390376055
-0.397266622367 0.00514879381339
-0.396819765273 0.00514602462642
-0.39637290818 0.00514113382215
-0.395926051087 0.0051363539694
-0.395479193994 0.00513388884296
-0.3950323369 0.00512931931208
-0.394585479807 0.00512485638031
-0.394138622714 0.00512268227998
-0.393691765621 0.00511842108992
-0.393244908527 0.00511426226407
-0.392798051434 0.00511020441532
-0.392351194341 0.00510624616884
-0.391904337248 0.00510238616199
-0.391457480155 0.0050986230441
-0.391010623061 0.00509495547636
-0.390563765968 0.00509138213165
-0.390116908875 0.00508790169441
-0.389670051782 0.0050845128605
-0.389223194688 0.00507910967187
-0.388776337595 0.00507590734069
-0.388329480502 0.00507279276419
-0.387882623409 0.00506768151511
-0.387435766315 0.00506474583245
-0.386988909222 0.00506189415328
-0.386542052129 0.00505706354983
-0.386095195036 0.0050543833463
-0.385648337942 0.00504973608966
-0.385201480849 0.00504722251655
-0.384754623756 0.00504275378698
-0.384307766663 0.00504040207899
-0.38386090957 0.00503610713508
-0.383414052476 0.00503190089957
-0.382967195383 0.00502778221181
-0.38252033829 0.00502574735935
-0.382073481197 0.00502179319455
-0.381626624103 0.00501792315447
-0.38117976701 0.00501413611479
-0.380732909917 0.00501043096004
-0.380286052824 0.00500680658348
-0.37983919573 0.00500326188706
-0.379392338637 0.0049997957813
-0.378945481544 0.00499640718522
-0.378498624451 0.00499309502629
-0.378051767357 0.00498985824029
-0.377604910264 0.00498669577128
-0.377158053171 0.00498360657152
-0.376711196078 0.00497868447053
-0.376264338985 0.00497574576543
-0.375817481891 0.00497287722955
-0.375370624798 0.00497007784708
-0.374923767705 0.00496546974227
-0.374476910612 0.00496281269652
-0.374030053518 0.00495835904389
-0.373583196425 0.00495584034287
-0.373136339332 0.00495153715945
-0.372689482239 0.00494915287102
-0.372242625145 0.00494499623259
-0.371795768052 0.00494274248353
-0.371348910959 0.00493872852366
-0.370902053866 0.00493660149862
-0.370455196772 0.00493272640773
-0.370008339679 0.00492892284965
-0.369561482586 0.00492518988714
-0.369114625493 0.00492331206799
-0.3686677684 0.00491971051029
-0.368220911306 0.00491617678258
-0.367774054213 0.00491270997433
-0.36732719712 0.00490930918159
-0.366880340027 0.00490597350685
-0.366433482933 0.00490270205908
-0.36598662584 0.00489949395364
-0.365539768747 0.0048963483122
-0.365092911654 0.00489326426278
-0.36464605456 0.0048902409396
-0.364199197467 0.00488727748313
-0.363752340374 0.00488437303999
-0.363305483281 0.00488152676291
-0.362858626188 0.00487873781072
-0.362411769094 0.00487432424174
-0.361964912001 0.00487165434563
-0.361518054908 0.00486903927996
-0.361071197815 0.00486481785313
-0.360624340721 0.00486231688725
-0.360177483628 0.00485986831019
-0.359730626535 0.00485583161829
-0.359283769442 0.00485349228868
-0.358836912348 0.00484957701186
-0.358390055255 0.00484734374676
-0.357943198162 0.00484354669621
-0.357496341069 0.0048414163572
-0.357049483975 0.00483773438782
-0.356602626882 0.00483570388043
-0.356155769789 0.00483213389032
-0.355708912696 0.00482862216197
-0.355262055603 0.00482673909336
-0.354815198509 0.00482333476379
-0.354368341416 0.00481998641826
-0.353921484323 0.00481824404434
-0.35347462723 0.00481499861087
-0.353027770136 0.00481180692992
-0.352580913043 0.00480866826523
-0.35213405595 0.00480558188552
-0.351687198857 0.00480254706445
-0.351240341763 0.00479956308058
-0.35079348467 0.00479662921738
-0.350346627577 0.00479374476315
-0.349899770484 0.00479090901102
-0.34945291339 0.00478812125895
-0.349006056297 0.00478538080963
-0.348559199204 0.00478268697052
-0.348112342111 0.0047800390538
-0.347665485018 0.00477743637634
-0.347218627924 0.00477487825967
-0.346771770831 0.00477236402996
-0.346324913738 0.00476845693124
-0.345878056645 0.00476603514333
-0.345431199551 0.00476365524001
-0.344984342458 0.00475990051177
-0.344537485365 0.00475760906096
-0.344090628272 0.0047553575329
-0.343643771178 0.0047517491885
-0.343196914085 0.00474958220362
-0.342750056992 0.00474745321954
-0.342303199899 0.00474398539015
-0.341856342805 0.00474193711862
-0.341409485712 0.00473856197349
-0.340962628619 0.00473659189797
-0.340515771526 0.00473330690265
-0.340068914433 0.00473141254055
-0.339622057339 0.00472821519395
-0.339175200246 0.00472506403845
-0.338728343153 0.00472328193037
-0.33828148606 0.0047202147249
-0.337834628966 0.00471719186619
-0.337387771873 0.00471551658619
-0.33694091478 0.00471257405175
-0.336494057687 0.0047096740557
-0.336047200593 0.00470681600015
-0.3356003435 0.00470399929108
-0.335153486407 0.0047024946017
-0.334706629314 0.00469975232076
-0.334259772221 0.00469704963666
-0.333812915127 0.00469438597079
-0.333366058034 0.00469176074836
-0.332919200941 0.00468917339836
-0.332472343848 0.00468662335353
-0.332025486754 0.00468411005036
-0.331578629661 0.00468163292906
-0.331131772568 0.00467919143358
-0.330684915475 0.00467678501153
-0.330238058381 0.00467441311423
-0.329791201288 0.00467207519663
-0.329344344195 0.00466858319661
-0.328897487102 0.0046663179923
-0.328450630008 0.00466408514455
-0.328003772915 0.00466188412278
-0.327556915822 0.00465971439996
-0.327110058729 0.00465641976064
-0.326663201636 0.00465431739395
-0.326216344542 0.00465224475646
-0.325769487449 0.00464906464421
-0.325322630356 0.00464705622487
-0.324875773263 0.00464507599639
-0.324428916169 0.00464200567626
-0.323982059076 0.00464008659003
-0.323535201983 0.00463708898321
-0.32308834489 0.0046352290159
-0.322641487796 0.00463339474083
-0.322194630703 0.00463049922728
-0.32174777361 0.00462764092266
-0.321300916517 0.00462589323059
-0.320854059423 0.00462310156755
-0.32040720233 0.0046214070849
-0.319960345237 0.00461868009187
-0.319513488144 0.00461598781254
-0.319066631051 0.0046143726328
-0.318619773957 0.00461174210403
-0.318172916864 0.00460914482803
-0.317726059771 0.00460760469344
-0.317279202678 0.0046050663057
-0.316832345584 0.00460255973801
-0.316385488491 0.00460008451549
-0.315938631398 0.00459863999168
-0.315491774305 0.00459621992165
-0.315044917211 0.00459382980117
-0.314598060118 0.00459146916757
-0.314151203025 0.00458913756124
-0.313704345932 0.00458683452553
-0.313257488838 0.00458455960681
-0.312810631745 0.00458231235442
-0.312363774652 0.00458009232067
-0.311916917559 0.00457789906083
-0.311470060466 0.00457573213314
-0.311023203372 0.00457359109874
-0.310576346279 0.00457147552171
-0.310129489186 0.00456938496907
-0.309682632093 0.00456731901071
-0.309235774999 0.00456527721943
-0.308788917906 0.00456325917092
-0.308342060813 0.00456126444374
-0.30789520372 0.00455929261931
-0.307448346626 0.00455645798531
-0.307001489533 0.00455453663902
-0.30655463244 0.00455263694549
-0.306107775347 0.00455075849744
-0.305660918253 0.00454803925918
-0.30521406116 0.00454620796321
-0.304767204067 0.00454439669629
-0.304320346974 0.00454176107764
-0.303873489881 0.00453999452062
-0.303426632787 0.00453824680109
-0.302979775694 0.00453569109032
-0.302532918601 0.00453398568764
-0.302086061508 0.00453148317529
-0.301639204414 0.0045298185134
-0.301192347321 0.00452736758809
-0.300745490228 0.00452574211232
-0.300298633135 0.00452334118373
-0.299851776041 0.00452175336063
-0.299404918948 0.00451940085932
-0.298958061855 0.00451784917652
-0.298511204762 0.00451554355381
-0.298064347669 0.00451402651991
-0.297617490575 0.00451176624775
-0.297170633482 0.00450953094955
-0.296723776389 0.00450806596295
-0.296276919296 0.00450587374978
-0.295830062202 0.00450370537153
-0.295383205109 0.00450228915695
-0.294936348016 0.00450016164367
-0.294489490923 0.00449805684876
-0.294042633829 0.00449597440103
-0.293595776736 0.00449391393172
-0.293148919643 0.00449257561358
-0.29270206255 0.0044905523929
-0.292255205456 0.00448855007102
-0.291808348363 0.00448656828893
-0.29136149127 0.00448460669002
-0.290914634177 0.00448266492011
-0.290467777084 0.00448074262736
-0.29002091999 0.00447883946236
-0.289574062897 0.00447695507807
-0.289127205804 0.0044750891298
-0.288680348711 0.00447324127524
-0.288233491617 0.00447141117444
-0.287786634524 0.00446959848979
-0.287339777431 0.00446780288602
-0.286892920338 0.00446602403021
-0.286446063244 0.00446426159175
-0.285999206151 0.00446251524237
-0.285552349058 0.0044607846561
-0.285105491965 0.00445906950928
-0.284658634871 0.00445736948056
-0.284211777778 0.00445509362959
-0.283764920685 0.004453428248
-0.283318063592 0.00445177702158
-0.282871206499 0.00445013963808
-0.282424349405 0.00444851578751
-0.281977492312 0.00444634131808
-0.281530635219 0.00444474891526
-0.281083778126 0.00444316911622
-0.280636921032 0.00444105372059
-0.280190063939 0.00443950349306
-0.279743206846 0.00443796496019
-0.279296349753 0.0044359057588
-0.278849492659 0.00443439496078
-0.278402635566 0.0044323734143
-0.277955778473 0.00443088914001
-0.27750892138 0.00442941508486
-0.277062064286 0.00442744505054
-0.276615207193 0.0044259957477
-0.2761683501 0.00442406027925
-0.275721493007 0.00442263456067
-0.275274635914 0.00442073244707
-0.27482777882 0.00441932916176
-0.274380921727 0.00441745920878
-0.273934064634 0.00441560747372
-0.273487207541 0.00441423825283
-0.273040350447 0.00441241690539
-0.272593493354 0.00441106730115
-0.272146636261 0.00440927518867
-0.271699779168 0.00440749981429
-0.271252922074 0.00440618009527
-0.270806064981 0.00440443224466
-0.270359207888 0.00440270026615
-0.269912350795 0.00440098387073
-0.269465493702 0.00439970186216
-0.269018636608 0.00439801075711
-0.268571779515 0.00439633439328
-0.268124922422 0.00439467248967
-0.267678065329 0.00439302476721
-0.267231208235 0.00439178516526
-0.266784351142 0.00439016002521
-0.266337494049 0.00438854825428
-0.265890636956 0.00438694958128
-0.265443779862 0.004385363737
-0.264996922769 0.00438379045416
-0.264550065676 0.00438222946744
-0.264103208583 0.00438068051343
-0.263656351489 0.00437914333066
-0.263209494396 0.00437761765961
-0.262762637303 0.00437610324264
-0.26231578021 0.00437459982406
-0.261868923117 0.00437310715008
-0.261422066023 0.00437162496881
-0.26097520893 0.00437015303028
-0.260528351837 0.00436869108639
-0.260081494744 0.00436723889097
-0.25963463765 0.00436579619971
-0.259187780557 0.00436436277019
-0.258740923464 0.00436293836188
-0.258294066371 0.0043615227361
-0.257847209277 0.00435982258548
-0.257400352184 0.00435842848352
-0.256953495091 0.00435704244559
-0.256506637998 0.00435566424045
-0.256059780904 0.00435429363873
-0.255612923811 0.00435266062123
-0.255166066718 0.00435130914413
-0.254719209625 0.00434996457956
-0.254272352532 0.00434837074822
-0.253825495438 0.00434704390153
-0.253378638345 0.00434572329288
-0.252931781252 0.00434416645858
-0.252484924159 0.00434286219358
-0.252038067065 0.00434156350839
-0.251591209972 0.00434004153015
-0.251144352879 0.00433875784666
-0.250697495786 0.00433725945352
-0.250250638692 0.00433598988561
-0.249803781599 0.00433472483166
-0.249356924506 0.00433325781848
-0.248910067413 0.00433200559141
-0.248463210319 0.00433055986657
-0.248016353226 0.00432931961549
-0.247569496133 0.00432789427903
-0.24712263904 0.00432666516703
-0.246675781947 0.00432525933282
-0.246228924853 0.00432386512204
-0.24578206776 0.00432265333251
-0.245335210667 0.0043212773064
-0.244888353574 0.00432007461023
-0.24444149648 0.00431871591683
-0.243994639387 0.0043173677396
-0.243547782294 0.00431617932643
-0.243100925201 0.00431484721528
-0.242654068107 0.00431352497329
-0.242207211014 0.00431221238342
-0.241760353921 0.00431104166005
-0.241313496828 0.00430974348497
-0.240866639735 0.00430845433499
-0.240419782641 0.00430717399966
-0.239972925548 0.00430601788786
-0.239526068455 0.00430475036933
-0.239079211362 0.00430349105825
-0.238632354268 0.00430223975074
-0.238185497175 0.00430099624453
-0.237738640082 0.00429976033898
-0.237291782989 0.00429862262341
-0.236844925895 0.00429739722219
-0.236398068802 0.00429617884384
-0.235951211709 0.00429496729419
-0.235504354616 0.00429376238069
-0.235057497522 0.00429256391238
-0.234610640429 0.00429137169992
-0.234163783336 0.00429018555555
-0.233716926243 0.00428900529312
-0.23327006915 0.00428783072806
-0.232823212056 0.00428666167738
-0.232376354963 0.0042854979597
-0.23192949787 0.0042843393952
-0.231482640777 0.00428318580565
-0.231035783683 0.00428203701439
-0.23058892659 0.00428089284633
-0.230142069497 0.00427975312795
-0.229695212404 0.00427859465608
-0.22924835531 0.00427746717745
-0.228801498217 0.0042763436227
-0.228354641124 0.00427522382454
-0.227907784031 0.00427410761724
-0.227460926937 0.00427299483661
-0.227014069844 0.00427188527901
-0.226560041705 0.00427076215863
-0.226106013565 0.00426965167546
-0.225651985425 0.00426853077109
-0.225197957285 0.00426743745325
-0.224743929146 0.00426631812279
-0.224289901006 0.00426524121342
-0.223835872866 0.00426412282872
-0.223381844727 0.00426306158471
-0.222927816587 0.00426194353152
-0.222473788447 0.00426089722342
-0.222019760308 0.00425986189195
-0.221565732168 0.0042587468133
-0.221111704028 0.00425772531847
-0.220657675889 0.00425660906533
-0.220203647749 0.0042556007116
-0.219749619609 0.00425448271766
-0.21929559147 0.0042534868229
-0.21884156333 0.00425250057652
-0.21838753519 0.0042513824309
-0.21793350705 0.0042504076146
-0.217479478911 0.00424944189349
-0.217025450771 0.00424832230581
-0.216571422631 0.00424736701564
-0.216117394492 0.00424624349528
-0.215663366352 0.00424529800697
-0.215209338212 0.00424436073487
-0.214755310073 0.00424323375215
-0.214301281933 0.00424230533189
-0.213847253793 0.00424138461373
-0.213393225654 0.00424047141915
-0.212939197514 0.00423934021002
-0.212485169374 0.00423843462526
-0.212031141235 0.00423753606919
-0.211577113095 0.00423639870169
-0.211123084955 0.0042355068731
-0.210669056815 0.0042346215926
-0.210215028676 0.00423374269274
-0.209761000536 0.00423259759048
-0.209306972396 0.00423172426545
-0.208852944257 0.00423085685936
-0.208398916117 0.00422999521103
-0.207944887977 0.00422884049211
-0.207490859838 0.00422798331628
-0.207036831698 0.0042271314552
-0.206582803558 0.00422628475388
-0.206128775419 0.00422544305883
-0.205674747279 0.00422427535595
-0.205220719139 0.00422343680992
-0.204766691 0.00422260285028
-0.20431266286 0.00422177332966
-0.20385863472 0.00422094810223
-0.20340460658 0.00422012702363
-0.202950578441 0.0042189414243
-0.202496550301 0.00421812199533
-0.202042522161 0.00421730632267
-0.201588494022 0.004216494268
-0.201134465882 0.00421568569448
-0.200680437742 0.00421488046678
-0.200226409603 0.00421407845104
-0.199772381463 0.0042132795149
-0.199318353323 0.00421206643151
-0.198864325184 0.00421126729404
-0.198410297044 0.00421047087946
-0.197956268904 0.00420967706131
-0.197502240764 0.00420888571457
-0.197048212625 0.00420809671571
-0.196594184485 0.00420730994263
-0.196140156345 0.0042065252747
-0.195686128206 0.00420574259274
-0.195232100066 0.004204961779
-0.194778071926 0.00420418271719
-0.194324043787 0.00420340529244
-0.193870015647 0.00420262939134
-0.193415987507 0.00420185490189
-0.192961959368 0.00420108171353
-0.192507931228 0.00420030971713
-0.192053903088 0.00419953880496
-0.191599874949 0.00419876887073
-0.191145846809 0.00419799980955
-0.190691818669 0.00419723151794
-0.190237790529 0.00419646389386
-0.18978376239 0.00419569683662
-0.18932973425 0.00419493024698
-0.18887570611 0.00419416402706
-0.188421677971 0.0041933980804
-0.187967649831 0.00419263231191
-0.187513621691 0.0041918666279
-0.187059593552 0.00419110093606
-0.186605565412 0.00419033514545
-0.186151537272 0.00419014651998
-0.185697509133 0.00418938531456
-0.185243480993 0.004188623714
-0.184789452853 0.00418786163287
-0.184335424714 0.00418709898706
-0.183881396574 0.00418633569386
-0.183427368434 0.00418557167187
-0.182973340294 0.00418480684108
-0.182519312155 0.0041846582872
-0.182065284015 0.00418389639898
-0.181611255875 0.00418313343812
-0.181157227736 0.00418236932996
-0.180703199596 0.0041816040012
-0.180249171456 0.00418083737984
-0.179795143317 0.00418006939523
-0.179341115177 0.00417995033559
-0.178887087037 0.00417918398907
-0.178433058898 0.0041784160434
-0.177979030758 0.0041776464332
-0.177525002618 0.00417687509439
-0.177070974479 0.00417677515482
-0.176616946339 0.00417600458316
-0.176162918199 0.00417523206664
-0.175708890059 0.00417445754643
-0.17525486192 0.00417437190258
-0.17480083378 0.00417359748674
-0.17434680564 0.00417282086651
-0.173892777501 0.00417204198818
-0.173438749361 0.00417196896901
-0.172984721221 0.00417118957353
-0.172530693082 0.00417040773466
-0.172076664942 0.00416962340382
-0.171622636802 0.00416956142015
-0.171168608663 0.00416877599145
-0.170714580523 0.00416798790073
-0.170260552383 0.00416793426191
-0.169806524243 0.00416714464825
-0.169352496104 0.00416635221385
-0.168898467964 0.00416630605647
-0.168444439824 0.00416551169664
-0.167990411685 0.00416471436858
-0.167536383545 0.00416467486293
-0.167082355405 0.00416387522936
-0.166628327266 0.00416307249126
-0.166174299126 0.00416303884106
-0.165720270986 0.0041622334396
-0.165266242847 0.0041614248084
-0.164812214707 0.00416139625061
-0.164358186567 0.00416058462029
-0.163904158428 0.00416056031311
-0.163450130288 0.00415974545056
-0.162996102148 0.00415892716332
-0.162542074008 0.00415890671721
-0.162088045869 0.00415808489844
-0.161634017729 0.00415806785753
-0.161179989589 0.00415724229826
-0.16072596145 0.00415641314954
-0.16027193331 0.00415639882892
-0.15981790517 0.00415556567641
-0.159363877031 0.00415555397563
-0.158909848891 0.00415471663422
-0.158455820751 0.00415470724258
-0.158001792612 0.00415386553665
-0.157547764472 0.00415385815291
-0.157093736332 0.00415301191624
-0.156639708193 0.00415216185564
-0.156185680053 0.00415215532432
-0.155731651913 0.0041513005334
-0.155277623773 0.00415129533089
-0.154823595634 0.00415043566678
-0.154369567494 0.00415043152459
-0.153915539354 0.00414956685367
-0.153461511215 0.00414956351253
-0.153007483075 0.00414956197733
-0.152553454935 0.00414869092028
-0.152099426796 0.00414868978153
-0.151645398656 0.00414781339173
-0.151191370516 0.00414781241313
-0.150737342377 0.00414693058903
-0.150283314237 0.00414692954339
-0.149829286097 0.00414604219248
-0.149375257958 0.00414604086166
-0.148921229818 0.00414514790046
-0.148467201678 0.00414514607537
-0.148013173538 0.00414514524572
-0.147559145399 0.00414424490985
-0.147105117259 0.00414424325613
-0.146651089119 0.00414333710831
-0.14619706098 0.0041433344438
-0.14574303284 0.00414333244222
-0.1452890047 0.00414241857857
-0.144834976561 0.0041424152698
-0.144380948421 0.00414149544794
-0.143926920281 0.00414149066737
-0.143472892142 0.00414148624492
-0.143018864002 0.00414055844874
-0.142564835862 0.0041405522911
-0.142110807722 0.00414054631519
-0.141656779583 0.00413961040958
-0.141202751443 0.00413960245471
-0.140748723303 0.00413959451495
-0.140294695164 0.00413865039401
-0.139840667024 0.00413864025103
-0.139386638884 0.00413862996629
-0.138932610745 0.0041376775531
-0.138478582605 0.00413766486021
-0.138024554465 0.00413765187835
-0.137570526326 0.00413763854949
-0.137116498186 0.00413667554905
-0.136662470046 0.00413665954678
-0.136208441907 0.00413664306307
-0.135754413767 0.00413567167044
-0.135300385627 0.00413565235304
-0.134846357487 0.00413563242932
-0.134392329348 0.00413561184862
-0.133938301208 0.00413462976387
-0.133484273068 0.0041346061433
-0.133030244929 0.00413458175345
-0.132576216789 0.00413455654785
-0.132122188649 0.0041335637845
-0.13166816051 0.00413353536618
-0.13121413237 0.00413350603228
-0.13076010423 0.0041334757405
-0.130306076091 0.00413344444957
-0.129852047951 0.00413243873363
-0.129398019811 0.00413240404392
-0.128943991672 0.00413236827067
-0.128489963532 0.0041323313767
-0.128035935392 0.00413229332585
-0.127581907252 0.00413127482895
-0.127127879113 0.00413123324432
-0.126673850973 0.00413119043368
-0.126219822833 0.00413114636494
-0.125765794694 0.00413110100702
-0.125311766554 0.00413105432984
-0.124857738414 0.00413002105043
-0.124403710275 0.0041299707309
-0.123949682135 0.00412991904107
-0.123495653995 0.00412986595487
-0.123041625856 0.00412981144722
-0.122587597716 0.00412975549403
-0.122133569576 0.00412969807221
-0.121679541437 0.00412864836631
-0.121225513297 0.00412858725509
-0.120771485157 0.00412852464499
-0.120317457017 0.00412846051686
-0.119863428878 0.00412839485253
-0.119409400738 0.0041283276348
-0.118955372598 0.00412825884747
-0.118501344459 0.00412818847528
-0.118047316319 0.00412811650396
-0.117593288179 0.00412804292022
-0.11713926004 0.00412796771173
-0.1166852319 0.0041278908671
-0.11623120376 0.00412781237595
-0.115777175621 0.00412673525694
-0.115323147481 0.0041266531867
-0.114869119341 0.00412656947743
-0.114415091201 0.00412648412255
-0.113961063062 0.00412639711642
-0.113507034922 0.00412630845436
-0.113053006782 0.00412621813265
-0.112598978643 0.00412612614849
-0.112144950503 0.00412603250004
-0.111690922363 0.00412593718639
-0.111236894224 0.00412584020759
-0.110782866084 0.0041257415646
-0.110328837944 0.00412564125933
-0.109874809805 0.00412553929463
-0.109420781665 0.00412543567426
-0.108966753525 0.00412533040292
-0.108512725386 0.00412522348624
-0.108058697246 0.00412511493077
-0.107604669106 0.00412500474396
-0.107150640966 0.00412489293422
-0.106696612827 0.00412477951085
-0.106242584687 0.00412565998657
-0.105788556547 0.00412554293713
-0.105334528408 0.0041254242748
-0.104880500268 0.00412530401257
-0.104426472128 0.00412518216429
-0.103972443989 0.00412505874475
-0.103518415849 0.00412493376963
-0.103064387709 0.0041248072555
-0.10261035957 0.00412467921984
-0.10215633143 0.00412454968104
-0.10170230329 0.00412441865834
-0.101248275151 0.0041242861719
-0.100794247011 0.00412514055726
-0.100340218871 0.00412500438493
-0.0998861907315 0.00412486678221
-0.0994321625918 0.00412472777282
-0.0989781344521 0.00412458738135
-0.0985241063124 0.00412444563327
-0.0980700781727 0.00412430255493
-0.097616050033 0.00412415817355
-0.0971620218933 0.00412499346075
-0.0967079937536 0.00412484547551
-0.096253965614 0.00412469624183
-0.0957999374743 0.0041245457904
-0.0953459093346 0.0041243941528
-0.0948918811949 0.00412424136148
-0.0944378530552 0.00412506151877
-0.0939838249155 0.00412490524284
-0.0935297967758 0.00412474788344
-0.0930757686361 0.00412458947644
-0.0926217404965 0.00412443005858
-0.0921677123568 0.00412426966742
-0.0917136842171 0.004125074359
-0.0912596560774 0.00412491066519
-0.0908056279377 0.00412474608381
-0.090351599798 0.0041245806558
-0.0898975716583 0.00412537445175
-0.0894435435186 0.00412520585498
-0.0889895153789 0.0041250365075
-0.0885354872393 0.00412486645363
-0.0880814590996 0.00412469573852
-0.0876274309599 0.00412547619286
-0.0871734028202 0.00412530253106
-0.0867193746805 0.00412512831651
-0.0862653465408 0.00412495359768
-0.0858113184011 0.00412572304372
-0.0853572902614 0.00412554557316
-0.0849032621217 0.0041253677168
-0.0844492339821 0.00412612844872
-0.0839952058424 0.00412594798816
-0.0835411777027 0.00412576726772
-0.083087149563 0.00412558634156
-0.0826331214233 0.0041263361092
-0.0821790932836 0.0041261528205
-0.0817250651439 0.00412596946181
-0.0812710370042 0.00412671055151
-0.0808170088646 0.00412652501261
-0.0803629807249 0.00412633954673
-0.0799089525852 0.00412615421366
-0.0794549244455 0.00412688454837
-0.0790008963058 0.00412669732267
-0.0785468681661 0.00412651038243
-0.0780928400264 0.0041272321986
-0.0776388118867 0.00412704358227
-0.077184783747 0.00412685541123
-0.0767307556074 0.00412756880002
-0.0762767274677 0.00412737918395
-0.075822699328 0.00412808617533
-0.0753686711883 0.0041278952549
-0.0749146430486 0.0041277050515
-0.0744606149089 0.00412840378321
-0.0740065867692 0.00412821253049
-0.0735525586295 0.00412802217353
-0.0730985304898 0.00412871279564
-0.0726445023502 0.00412852165865
-0.0721904742105 0.00412920603838
-0.0717364460708 0.00412901428746
-0.0712824179311 0.00412882373527
-0.0708283897914 0.00412950027056
-0.0703743616517 0.00412930939725
-0.069920333512 0.00412997983132
-0.0694663053723 0.00412978881866
-0.0690122772326 0.00412959932692
-0.068558249093 0.00413026224178
-0.0681042209533 0.00413007292674
-0.0676501928136 0.00413072992152
-0.0671961646739 0.00413054098043
-0.0667421365342 0.00413119212534
-0.0662881083945 0.0041310037616
-0.0658340802548 0.0041308173955
-0.0653800521151 0.00413146155635
-0.0649260239755 0.00413127611572
-0.0644719958358 0.00413191466316
-0.0640179676961 0.00413173036662
-0.0635639395564 0.00413236339286
-0.0631099114167 0.00413218046508
-0.062655883277 0.00413280806859
-0.0622018551373 0.00413262674028
-0.0617478269976 0.00413324902571
-0.0612937988579 0.00413306953355
-0.0608397707183 0.00413368661177
-0.0603857425786 0.0041335091984
-0.0599317144389 0.00413412118642
-0.0594776862992 0.00413394610042
-0.0590236581595 0.00413455312138
-0.0585696300198 0.00413438061722
-0.0581156018801 0.00413498280036
-0.0576615737404 0.0041348131384
-0.0572075456007 0.00413541061903
-0.0567535174611 0.00413524406544
-0.0562994893214 0.00413583698492
-0.0558454611817 0.0041356738117
-0.055391433042 0.00413626231741
-0.0549374049023 0.00413684664824
-0.0544833767626 0.00413668704763
-0.0540293486229 0.00413726716426
-0.0535753204832 0.00413711161842
-0.0531212923436 0.0041376876832
-0.0526672642039 0.00413753648427
-0.0522132360642 0.00413810866548
-0.0517592079245 0.00413867682995
-0.0513051797848 0.00413853058306
-0.0508511516451 0.00413909509487
-0.0503971235054 0.00413895391941
-0.0499430953657 0.00413951496157
-0.049489067226 0.00414007211775
-0.0490350390864 0.0041399369308
-0.0485810109467 0.00414049087035
-0.048126982807 0.00414036151463
-0.0476729546673 0.00414091243513
-0.0472189265276 0.00414145961902
-0.0467648983879 0.00414133734122
-0.0463108702482 0.00414188178093
-0.0458568421085 0.00414176612899
-0.0454028139688 0.00414230803646
-0.0449487858292 0.00414284637512
-0.0444947576895 0.0041427389428
-0.0440407295498 0.00414327504569
-0.0435867014101 0.00414380768258
-0.0431326732704 0.00414370916147
-0.0426786451307 0.00414423987194
-0.042224616991 0.00414476722576
-0.0417705888513 0.00414467832598
-0.0413165607117 0.00414520407549
-0.040862532572 0.00414572658421
-0.0404085044323 0.00414564803428
-0.0399544762926 0.00414616927349
-0.0395004481529 0.00414668739421
-0.0390464200132 0.00414661994088
-0.0385923918735 0.00414713713949
-0.0381383637338 0.00414765134834
-0.0376843355941 0.00414816260085
-0.0372303074545 0.00414810940308
-0.0367762793148 0.00414862019502
-0.0363222511751 0.00414912816787
-0.0358682230354 0.00414908784937
-0.0354141948957 0.00414959573813
-0.034960166756 0.00415010095132
-0.0345061386163 0.00415060352736
-0.0340521104766 0.00415057983653
-0.0335980823369 0.00415108282863
-0.0331440541973 0.00415158333549
-0.0326900260576 0.00415208139835
-0.0322359979179 0.00415207573168
-0.0317819697782 0.00415257473254
-0.0313279416385 0.00415307144961
-0.0308739134988 0.00415356592692
-0.0304198853591 0.00415357972263
-0.0299658572194 0.00415407568145
-0.0295118290798 0.00415456956893
-0.0290578009401 0.00415506143187
-0.0286037728004 0.00415509616948
-0.0281497446607 0.00415559007881
-0.027695716521 0.00415608214016
-0.0272416883813 0.00415657240308
-0.0267876602416 0.0041570609178
-0.0263336321019 0.00415712249822
-0.0258796039622 0.00415761377973
-0.0254255758226 0.00415810349969
-0.0249715476829 0.00415859171104
-0.0245175195432 0.00415907846742
-0.0240634914035 0.00415956382314
-0.0236094632638 0.00415965954835
-0.0231554351241 0.00416014856633
-0.0227014069844 0.00416063638226
-0.0222473788447 0.00416112305311
-0.021793350705 0.00416160863655
-0.0213393225654 0.00416209319089
-0.0208852944257 0.00416222655556
-0.020431266286 0.0041627157143
-0.0199772381463 0.00416320405435
-0.0195232100066 0.00416369163667
-0.0190691818669 0.00416417852288
-0.0186151537272 0.00416466477527
-0.0181611255875 0.00416515045679
-0.0177070974479 0.00416533125242
-0.0172530693082 0.00416582268544
-0.0167990411685 0.00416631377152
-0.0163450130288 0.00416680457621
-0.0158909848891 0.0041672951657
-0.0154369567494 0.00416778560682
-0.0149829286097 0.00416827596706
-0.01452890047 0.00416876631457
-0.0140748723303 0.00416925671813
-0.0136208441907 0.00416950407061
-0.013166816051 0.00417000177371
-0.0127127879113 0.00417049977389
-0.0122587597716 0.00417099814246
-0.0118047316319 0.00417149695138
-0.0113507034922 0.00417199627322
-0.0108966753525 0.00417249618123
-0.0104426472128 0.00417299674926
-0.00998861907315 0.00417349805179
-0.00953459093346 0.00417400016395
-0.00908056279377 0.00417450316149
-0.00862653465408 0.00417500712078
-0.00817250651439 0.00417551211883
-0.0077184783747 0.00417601823325
-0.00726445023502 0.0041765255423
-0.00681042209533 0.00417689857732
-0.00635639395564 0.00417741594721
-0.00590236581595 0.00417793478042
-0.00544833767626 0.00417845515762
-0.00499430953657 0.00417897716011
-0.00454028139688 0.00417950086979
-0.0040862532572 0.00418002636918
-0.00363222511751 0.00418055374142
-0.00317819697782 0.00418108307022
-0.00272416883813 0.00418161443994
-0.00227014069844 0.00418214793551
-0.00181611255875 0.00418268364249
-0.00136208441907 0.00418322164701
-0.000908056279377 0.00418376203584
-0.000454028139689 0.0041843048963
0.0 0.00418485031635
0.00103039649401 0.00418609806914
0.00206079298802 0.00418736072153
0.00309118948202 0.00418860596906
0.00412158597603 0.00418988326625
0.00515198247004 0.00419117858488
0.00618237896405 0.00419249305621
0.00721277545806 0.00419382783151
0.00824317195206 0.00419518408205
0.00927356844607 0.00419641670052
0.0103039649401 0.00419780020699
0.0113343614341 0.0041992086753
0.0123647579281 0.00420064335749
0.0133951544221 0.00420188081545
0.0144255509161 0.0042033518812
0.0154559474101 0.00420485289236
0.0164863439041 0.00420610000208
0.0175167403981 0.00420764460294
0.0185471368921 0.0042092230655
0.0195775333862 0.00421048980254
0.0206079298802 0.00421211943599
0.0216383263742 0.00421378703268
0.0226687228682 0.0042150839487
0.0236991193622 0.0042168106737
0.0247295158562 0.00421812660131
0.0257599123502 0.00421991787403
0.0267903088442 0.00422125773491
0.0278207053382 0.00422260035708
0.0288511018322 0.00422448803479
0.0298814983262 0.00422586215399
0.0309118948202 0.0042278285312
0.0319422913142 0.0042292395075
0.0329726878083 0.00423065950703
0.0340030843023 0.00423274396929
0.0350334807963 0.00423420905236
0.0360638772903 0.00423568715562
0.0370942737843 0.00423790340573
0.0381246702783 0.00423943521932
0.0391550667723 0.00424098425347
0.0401854632663 0.00424255190605
0.0412158597603 0.00424495835471
0.0422462562543 0.00424659175289
0.0432766527483 0.00424824824291
0.0443070492423 0.0042499293148
0.0453374457363 0.00425163648184
0.0463678422304 0.00425337128063
0.0473982387244 0.00425513527109
0.0484286352184 0.00425693003655
0.0494590317124 0.0042587571837
0.0504894282064 0.00426061834271
0.0515198247004 0.00426251516719
0.0525502211944 0.00426444933424
0.0535806176884 0.00426642254452
0.0546110141824 0.00426843652223
0.0556414106764 0.00427049301517
0.0566718071704 0.00427259379474
0.0577022036644 0.00427474065601
0.0587326001585 0.00427693541772
0.0597629966525 0.00427790418202
0.0607933931465 0.00428017364511
0.0618237896405 0.00428249647916
0.0628541861345 0.00428487459868
0.0638845826285 0.00428730994198
0.0649149791225 0.00428839352674
0.0659453756165 0.00429092193841
0.0669757721105 0.00429351340784
0.0680061686045 0.00429467608688
0.0690365650985 0.00429737213347
0.0700669615925 0.00429858724406
0.0710973580865 0.00430139570606
0.0721277545806 0.00430427739853
0.0731581510746 0.00430559959316
0.0741885475686 0.00430860595929
0.0752189440626 0.00430999967318
0.0762493405566 0.00431313905523
0.0772797370506 0.00431461223662
0.0783101335446 0.00431789318004
0.0793405300386 0.0043194539872
0.0803709265326 0.00432104684668
0.0814013230266 0.00432454204311
0.0824317195206 0.00432623503886
0.0834621160146 0.00432796627747
0.0844925125086 0.00433169575796
0.0855229090027 0.00433354012457
0.0865533054967 0.00433542916957
0.0875837019907 0.00433736505252
0.0886140984847 0.00434142931752
0.0896444949787 0.00434349632572
0.0906748914727 0.00434561693676
0.0917052879667 0.00434779342153
0.0927356844607 0.00435002807907
0.0937660809547 0.00435232323663
0.0947964774487 0.0043546812497
0.0958268739427 0.00435710450209
0.0968572704367 0.00436192400503
0.0978876669308 0.00436451677181
0.0989180634248 0.0043647899584
0.0999484599188 0.00436749857342
0.100978856413 0.00437028477269
0.102009252907 0.00437315111069
0.103039649401 0.0043761001705
0.104070045895 0.00437913456384
0.105100442389 0.00438225693112
0.106130838883 0.00438546994145
0.107161235377 0.0043861241682
0.108191631871 0.00438949374555
0.109222028365 0.00439296204506
0.110252424859 0.00439653185212
0.111282821353 0.00439742091365
0.112313217847 0.00440116896171
0.113343614341 0.0044050269503
0.114374010835 0.00440611169133
0.115404407329 0.00441016475675
0.116434803823 0.00441138218955
0.117465200317 0.00441564179422
0.118495596811 0.00441700310416
0.119525993305 0.0044214809565
0.120556389799 0.00442299758383
0.121586786293 0.00442770563902
0.122617182787 0.00442938927968
0.123647579281 0.0044343397404
0.124677975775 0.00443620234688
0.125708372269 0.00443814123142
0.126738768763 0.00444346144611
0.127769165257 0.00444559761546
0.128799561751 0.00444781922885
0.129829958245 0.00445012937718
0.130860354739 0.00445597560455
0.131890751233 0.00445850832026
0.132921147727 0.00446113913839
0.133951544221 0.00446387128566
0.134981940715 0.00446670802316
0.136012337209 0.00446965264642
0.137042733703 0.00447270848549
0.138073130197 0.00447587890496
0.139103526691 0.00447916730404
0.140133923185 0.00448257711662
0.141164319679 0.0044861118113
0.142194716173 0.00448977489148
0.143225112667 0.00449356989537
0.144255509161 0.0044975003961
0.145285905655 0.00450157000172
0.146316302149 0.00450578235527
0.147346698643 0.00450610921598
0.148377095137 0.00451058075635
0.149407491631 0.00451520611413
0.150437888125 0.00451998907412
0.151468284619 0.00452075036998
0.152498681113 0.00452582237188
0.153529077607 0.00453106347712
0.154559474101 0.004532180101
0.155589870595 0.00453773337492
0.156620267089 0.00453909302378
0.157650663583 0.00454497421167
0.158681060077 0.00454659251288
0.159711456571 0.00455281766055
0.160741853065 0.00455471055325
0.161772249559 0.00455672705256
0.162802646053 0.0045634797441
0.163833042547 0.00456579526831
0.164863439041 0.00456824669962
0.165893835535 0.00457556457574
0.166924232029 0.00457834018098
0.167954628523 0.00458126435881
0.168985025017 0.00458434139327
0.170015421511 0.0045875756102
0.171045818005 0.00459097137728
0.172076214499 0.00459949798702
0.173106610993 0.00460327028799
0.174137007487 0.00460721754436
0.175167403981 0.00461134429046
0.176197800475 0.00461565510282
0.177228196969 0.00461498841532
0.178258593463 0.00461964085955
0.179288989957 0.0046244913107
0.180319386451 0.00462954451628
0.181349782945 0.00463480526632
0.182380179439 0.00464027839345
0.183410575933 0.00464055813847
0.184440972427 0.00464643004904
0.185471368921 0.00465252905729
0.186501765415 0.00465332605554
0.187532161909 0.00465985357632
0.188562558403 0.00466100621189
0.189592954897 0.00466798249155
0.190623351391 0.00467521127334
0.191653747885 0.00467695670433
0.192684144379 0.00467888186583
0.193714540873 0.00468681785826
0.194744937367 0.0046891606644
0.195775333862 0.00469760834141
0.196805730356 0.00470039021934
0.19783612685 0.00470337852828
0.198866523344 0.00470657874504
0.199896919838 0.00471607426204
0.200927316332 0.00471975751132
0.201957712826 0.00472366942079
0.20298810932 0.00472781566758
0.204018505814 0.00473220197956
0.205048902308 0.00473683413541
0.206079298802 0.00474171796471
0.207109695296 0.00474685934799
0.20814009179 0.00475226421683
0.209170488284 0.00475793855392
0.210200884778 0.00476388839317
0.211231281272 0.00476357275984
0.212261677766 0.00477004921311
0.21329207426 0.00477681957889
0.214322470754 0.00478389009846
0.215352867248 0.0047845475945
0.216383263742 0.00479219466335
0.217413660236 0.00479335444332
0.21844405673 0.00480160367764
0.219474453224 0.00480329159061
0.220504849718 0.00481216904403
0.221535246212 0.00481441139286
0.222565642706 0.00482394355769
0.2235960392 0.00482676710041
0.224626435694 0.00482986927841
0.225656832188 0.00484041285996
0.226687228682 0.00484413724197
0.227717625176 0.00484816104864
0.22874802167 0.00485249133431
0.229778418164 0.00485713521396
0.230808814658 0.00486209986329
0.231839211152 0.00486739251879
0.232869607646 0.00487302047788
0.23390000414 0.00487899109895
0.234930400634 0.00488531180146
0.235960797128 0.00489199006604
0.236991193622 0.00489903343452
0.238021590116 0.00490644951006
0.23905198661 0.00490651677806
0.240082383104 0.00491465746311
0.241112779598 0.00492319407844
0.242143176092 0.00492427207575
0.243173572586 0.00493358044475
0.24420396908 0.00493535695264
0.245234365574 0.0049454691817
0.246264762068 0.0049479767594
0.247295158562 0.00495892547715
0.248325555056 0.00496219722548
0.24935595155 0.00496584103777
0.250386348044 0.00497808514686
0.251416744538 0.00498254385917
0.252447141032 0.00498740039828
0.253477537526 0.00499266351332
0.25450793402 0.00499834202546
0.255538330514 0.00500444482795
0.256568727008 0.00501098088627
0.257599123502 0.00501795923816
0.258629519996 0.00502538899374
0.25965991649 0.0050332793356
0.260690312984 0.00504163951887
0.261720709478 0.00504176692197
0.262751105972 0.00505105055929
0.263781502466 0.00506083232809
0.26481189896 0.00506227535741
0.265842295454 0.00507303809281
0.266872691948 0.00507539167405
0.267903088442 0.0050871745415
0.268933484936 0.00509047852267
0.26996388143 0.00509425008208
0.270994277924 0.00510761617226
0.272024674418 0.00511239920453
0.273055070912 0.00511768086859
0.274085467406 0.0051234717165
0.2751158639 0.00512978238491
0.276146260394 0.00513662359513
0.277176656888 0.00514400615325
0.278207053382 0.00515194095022
0.279237449876 0.00516043896192
0.28026784637 0.00516951124927
0.281298242864 0.00517916895828
0.282328639358 0.00517981430306
0.283359035852 0.00519063261718
0.284389432346 0.00520207043906
0.28541982884 0.00520439664018
0.286450225334 0.00521706443198
0.287480621828 0.00522055495818
0.288511018322 0.0052246230205
0.289541414816 0.00523920296795
0.29057181131 0.00524450803394
0.291602207804 0.0052504276225
0.292632604298 0.00525697430651
0.293663000792 0.00526416075735
0.294693397286 0.00527199974501
0.29572379378 0.00528050413815
0.296754190274 0.00528968690418
0.297784586768 0.00529956110937
0.298814983262 0.00531013991888
0.299845379756 0.00531107185864
0.30087577625 0.0053230564452
0.301906172744 0.00533578591072
0.302936569238 0.00533877765713
0.303966965732 0.00535299491404
0.304997362226 0.00535741473065
0.30602775872 0.0053625477218
0.307058155214 0.00537908054078
0.308088551708 0.00538572768119
0.309118948202 0.00539313182831
0.310149344696 0.005401307885
0.31117974119 0.00541027086799
0.312210137684 0.00542003590794
0.313240534178 0.00543061824949
0.314270930672 0.00543105767048
0.315301327166 0.00544327832955
0.31633172366 0.00545636294005
0.317362120154 0.00545922285431
0.318392516648 0.00547404082498
0.319422913142 0.00547858074934
0.320453309636 0.00549519679207
0.32148370613 0.005501482893
0.322514102624 0.00550864579081
0.323544499118 0.00551670265635
0.324574895612 0.00552567079088
0.325605292106 0.00553556762617
0.326635688601 0.00554641072455
0.327666085095 0.0055582177789
0.328696481589 0.00557100661278
0.329726878083 0.00557318385005
0.330757274577 0.00558794957552
0.331787671071 0.00559205720748
0.332818067565 0.0056088738553
0.333848464059 0.00561498762881
0.334878860553 0.0056221124662
0.335909257047 0.0056302680364
0.336939653541 0.00565137415582
0.337970050035 0.00566169138924
0.339000446529 0.00567309893261
0.340030843023 0.00567359622408
0.341061239517 0.00568720569272
0.342091636011 0.00570196702825
0.343122032505 0.00570576021637
0.344152428999 0.00572284896296
0.345182825493 0.00572893287294
0.346213221987 0.00573617488976
0.347243618481 0.00575689656314
0.348274014975 0.0057665613474
0.349304411469 0.00577745153639
0.350334807963 0.00578959001773
0.351365204457 0.00580299984723
0.352395600951 0.00580521274351
0.353425997445 0.00582119779518
0.354456393939 0.00583852476816
0.355486790433 0.00584461310202
0.356517186927 0.0058520167401
0.357547583421 0.00587344116488
0.358577979915 0.00588358884803
0.359608376409 0.00589512791604
0.360638772903 0.00590808424506
0.361669169397 0.00590965709337
0.362699565891 0.00592549076875
0.363729962385 0.00594282091998
0.364760358879 0.00594874003045
0.365790755373 0.00596910904931
0.366821151867 0.00597805141308
0.367851548361 0.00598852991306
0.368881944855 0.00600057339764
0.369912341349 0.00601421092758
0.370942737843 0.00602947177589
0.371973134337 0.0060463854277
0.373003530831 0.00605177137455
0.374033927325 0.00607204769315
0.375064323819 0.00608079090916
0.376094720313 0.00609124316255
0.377125116807 0.00610343662505
0.378155513301 0.00611740370558
0.379185909795 0.00613317705002
0.380216306289 0.00615078954107
0.381246702783 0.00617027429799
0.382277099277 0.00617816606171
0.383307495771 0.00618793667457
0.384337892265 0.00621318208534
0.385368288759 0.00622684747002
0.386398685253 0.00624249874337
0.387429081747 0.00624652401516
0.388459478241 0.00626622847942
0.389489874735 0.00627432377152
0.390520271229 0.00629823173655
0.391550667723 0.0063105510552
0.392581064217 0.00632502716967
0.393611460711 0.00634170010664
0.394641857205 0.0063606101849
0.395672253699 0.0063679303792
0.396702650193 0.00639141230677
0.397733046687 0.0064033369006
0.398763443181 0.00641761547538
0.399793839675 0.00643429203351
0.400824236169 0.00645341090058
0.401854632663 0.00647501672487
0.402885029157 0.00648511749553
0.403915425651 0.00649775140931
0.404945822145 0.00651296648055
0.405976218639 0.00653081108053
0.407006615133 0.00655133393687
0.408037011627 0.00657458413309
0.409067408121 0.00658644699407
0.410097804615 0.00660109877815
0.411128201109 0.00661859225863
0.412158597603 0.0066389806013
0.413188994097 0.00666231736382
0.414219390591 0.0066744010826
0.415249787085 0.00670378175349
0.416280183579 0.00672198828358
0.417310580073 0.00672903090706
0.418340976567 0.00675356040678
0.419371373061 0.00676701563615
0.420401769555 0.00679810750046
0.421432166049 0.00681822054304
0.422462562543 0.00682738026062
0.423492959037 0.00685437899418
0.424523355531 0.00687053189821
0.425553752025 0.00689027647612
0.426584148519 0.00691368120023
0.427614545013 0.0069263961125
0.428644941507 0.00695732212498
0.429675338001 0.00697768565811
0.430705734495 0.00700197975484
0.431736130989 0.00701583515347
0.432766527483 0.00703376309651
0.433796923977 0.00705584314474
0.434827320471 0.0070821554776
0.435857716965 0.0071127808923
0.436888113459 0.00713334482037
0.437918509953 0.00715838750667
0.438948906447 0.00717354049923
0.439979302941 0.00719335140202
0.441009699435 0.00721791257323
0.442040095929 0.00724731710739
0.443070492423 0.00726721833805
0.444100888917 0.00729216544961
0.445131285411 0.00732225833068
0.446161681905 0.0073431797937
0.447192078399 0.00736947021267
0.448222474893 0.00738683903676
0.449252871387 0.00742420291997
0.450283267881 0.00743851871898
0.451313664375 0.00747305854846
0.452344060869 0.0074992121308
0.453374457363 0.00753147372833
0.454404853857 0.00755566271107
0.455435250351 0.00758624954105
0.456465646845 0.00760910342286
0.45749604334 0.00763866645821
0.458526439834 0.0076608640886
0.459556836328 0.00769010507885
0.460587232822 0.00772653761558
0.461617629316 0.00775618255752
0.46264802581 0.00777928738483
0.463678422304 0.00781017651108
0.464708818798 0.00784901729319
0.465739215292 0.00788198846684
0.466769611786 0.00790938060334
0.46780000828 0.00794540854728
0.468830404774 0.00797639573156
0.469860801268 0.00800267203447
0.470891197762 0.00803835567877
0.471921594256 0.00806993711825
0.47295199075 0.00811145832987
0.473982387244 0.00814953260391
0.475012783738 0.00818456408998
0.476043180232 0.00821697669488
0.477073576726 0.00824721510943
0.47810397322 0.00828910598323
0.479134369714 0.00832963763895
0.480164766208 0.0083693137655
0.481195162702 0.00840866274248
0.482225559196 0.00844823891473
0.48325595569 0.00848862393555
0.484286352184 0.00851754575139
0.485316748678 0.00856150322694
0.486347145172 0.00860819745036
0.487377541666 0.00864574603813
0.48840793816 0.00868769430285
0.489438334654 0.00873483674677
0.490468731148 0.00878800821208
0.491499127642 0.00883596165527
0.492529524136 0.00888001262669
0.49355992063 0.00892156511764
0.494590317124 0.00897382762246
0.495620713618 0.00902638664686
0.496651110112 0.00908093151749
0.497681506606 0.00912804994735
0.4987119031 0.00918126558648
0.499742299594 0.00923184691219
0.500772696088 0.00929332053098
0.501803092582 0.00934733499526
0.502833489076 0.00940816097262
0.50386388557 0.0094696183205
0.504894282064 0.00952698430899
0.505924678558 0.00959597042699
0.506955075052 0.00966469923528
0.507985471546 0.00972491524908
0.50901586804 0.00979766837394
0.510046264534 0.00987321451509
0.511076661028 0.00995056745588
0.512107057522 0.0100277116256
0.513137454016 0.0101097681891
0.51416785051 0.0102008222931


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularProb0pt4.tex <==
-0.450442616461 0.0190678050482
-0.445938190297 0.0189785640243
-0.441433764132 0.0188953393677
-0.436929337968 0.018807677442
-0.432424911803 0.0187252000057
-0.427920485638 0.0186404308269
-0.423416059474 0.0185629538579
-0.418911633309 0.0184841282819
-0.414407207145 0.0184038922786
-0.40990278098 0.018332810222
-0.405398354815 0.0182608938879
-0.400893928651 0.0181880004089
-0.396389502486 0.0181139887751
-0.391885076321 0.0180509410584
-0.387380650157 0.017987248081
-0.382876223992 0.0179227552259
-0.378371797828 0.0178573186597
-0.373867371663 0.017790806084
-0.369362945498 0.0177371316154
-0.364858519334 0.0176828198446
-0.360354093169 0.0176277358775
-0.355849667005 0.0175717572359
-0.35134524084 0.0175301482533
-0.346840814675 0.0174723564609
-0.342336388511 0.0174293399039
-0.337831962346 0.0173856094984
-0.333327536181 0.0173410625235
-0.328823110017 0.017295608068
-0.324318683852 0.0172491668573
-0.319814257688 0.0172190028194
-0.315309831523 0.0171881996276
-0.310805405358 0.0171388543879
-0.306300979194 0.0171062988592
-0.301796553029 0.0170728857946
-0.297292126865 0.0170385589752
-0.2927877007 0.0170218752045
-0.288283274535 0.0169857543819
-0.283778848371 0.0169675299866
-0.279274422206 0.0169294549468
-0.274769996041 0.0169095100052
-0.270265569877 0.0168887232742
-0.265761143712 0.0168670639079
-0.261256717548 0.0168445105453
-0.256752291383 0.0168406719263
-0.252247865218 0.0168163659354
-0.247743439054 0.0168108910186
-0.243239012889 0.016784797353
-0.238734586725 0.0167776260908
-0.23423016056 0.016769615945
-0.229725734395 0.0167607631129
-0.225221308231 0.016751072514
-0.220716882066 0.0167405576576
-0.216212455901 0.0167292405098
-0.211708029737 0.016717151359
-0.207203603572 0.0167239715765
-0.202699177408 0.0167103753713
-0.198194751243 0.0167155988214
-0.193690325078 0.0167200166814
-0.189185898914 0.0167236549622
-0.184681472749 0.0167265479359
-0.180177046585 0.0167287380338
-0.17567262042 0.0167302757437
-0.171168194255 0.0167312195057
-0.166663768091 0.0167500551242
-0.162159341926 0.0167498080718
-0.157654915762 0.0167671663509
-0.153150489597 0.0167659989877
-0.148646063432 0.0167821237015
-0.144141637268 0.0167976115035
-0.139637211103 0.0168125328606
-0.135132784938 0.0168269663739
-0.130628358774 0.0168409987036
-0.126123932609 0.0168547244905
-0.121619506445 0.0168839610868
-0.11711508028 0.016897042801
-0.112610654115 0.0169101361748
-0.108106227951 0.0169380008851
-0.103601801786 0.0169653629736
-0.0990973756215 0.0169923256329
-0.0945929494569 0.0170190007826
-0.0900885232923 0.017045509021
-0.0855840971277 0.0170719795727
-0.0810796709631 0.0170985502349
-0.0765752447984 0.0171253673201
-0.0720708186338 0.0171637377618
-0.0675663924692 0.0171910327041
-0.0630619663046 0.0172292074234
-0.05855754014 0.0172576241905
-0.0540531139754 0.0172962383911
-0.0495486878108 0.0173350620572
-0.0450442616461 0.0173742714821
-0.0405398354815 0.0174140527652
-0.0360354093169 0.0174614662608
-0.0315309831523 0.0175024063356
-0.0270265569877 0.0175445266386
-0.0225221308231 0.017593126625
-0.0180177046585 0.0176421342619
-0.0135132784938 0.0176879586022
-0.00900885232923 0.0177391014801
-0.00450442616461 0.0177913600887
0.0 0.0178449909125
0.00267562914178 0.0178787479844
0.00535125828356 0.0179114524473
0.00802688742534 0.0179457036842
0.0107025165671 0.0179798247884
0.0133781457089 0.0180148068453
0.0160537748507 0.0180505961263
0.0187294039925 0.01808656076
0.0214050331342 0.0181229037686
0.024080662276 0.0181614979509
0.0267562914178 0.018199228449
0.0294319205596 0.0182375466046
0.0321075497014 0.0182765259373
0.0347831788432 0.01831624215
0.0374588079849 0.0183567731373
0.0401344371267 0.0183981989944
0.0428100662685 0.0184406020246
0.0454856954103 0.0184840667475
0.0481613245521 0.0185286799056
0.0508369536938 0.018574530471
0.0535125828356 0.0186151665795
0.0561882119774 0.0186633366223
0.0588638411192 0.018705589573
0.061539470261 0.0187564647881
0.0642150994027 0.0188007325183
0.0668907285445 0.0188547189767
0.0695663576863 0.0189014215159
0.0722419868281 0.0189492774295
0.0749176159699 0.0190085254045
0.0775932451116 0.0190594895895
0.0802688742534 0.0191119592648
0.0829445033952 0.0191660585202
0.085620132537 0.0192219146198
0.0882957616788 0.0192796580109
0.0909713908206 0.0193394223322
0.0936470199623 0.0193880928809
0.0963226491041 0.0194518775817
0.0989982782459 0.0195039548529
0.101673907388 0.0195723480208
0.104349536529 0.0196284493376
0.107025165671 0.0197020680074
0.109700794813 0.019762841984
0.112376423955 0.0198259835169
0.115052053097 0.0198916718231
0.117727682238 0.0199600905348
0.12040331138 0.0200314277071
0.123078940522 0.0201058758242
0.125754569664 0.0201651162611
0.128430198805 0.0202459744383
0.131105827947 0.020311198547
0.133781457089 0.0203993198833
0.136457086231 0.020471430912
0.139132715373 0.020547132923
0.141808344514 0.0206266768076
0.144483973656 0.0207103194199
0.147159602798 0.0207983235767
0.14983523194 0.0208909580541
0.152510861082 0.0209659885984
0.155186490223 0.0210454766871
0.157862119365 0.0211530020632
0.160537748507 0.0212427361327
0.163213377649 0.021337905955
0.16588900679 0.0214388572233
0.168564635932 0.0215213492733
0.171240265074 0.0216346337404
0.173915894216 0.0217295952652
0.176591523358 0.0218312549447
0.179267152499 0.0219400498131
0.181942781641 0.0220564269879
0.184618410783 0.0221545456112
0.187294039925 0.0222607088999
0.189969669066 0.0223754581775
0.192645298208 0.0224993475957
0.19532092735 0.0226329440808
0.197996556492 0.0227495167406
0.200672185634 0.0228766987807
0.203347814775 0.023015176913
0.206023443917 0.0231379733756
0.208699073059 0.0232733562881
0.211374702201 0.0234221577398
0.214050331342 0.0235852297753
0.216725960484 0.0237078594957
0.219401589626 0.0238745062025
0.222077218768 0.0240307328776
0.22475284791 0.0242055292342
0.227428477051 0.0243727744177
0.230104106193 0.0245344081784
0.232779735335 0.0247195615934
0.235455364477 0.0249034052279
0.238130993619 0.0250888874032
0.24080662276 0.0253050267927
0.243482251902 0.025504079742
0.246157881044 0.0257167568602
0.248833510186 0.0259484355994
0.251509139327 0.0261828273346
0.254184768469 0.0264305772979
0.256860397611 0.0266848099308
0.259536026753 0.0269486721568
0.262211655895 0.0272408403591
0.264887285036 0.0275684132642


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularProb0pt6.tex <==
-0.450442616461 0.0401952228333
-0.445938190297 0.0400978410914
-0.441433764132 0.0400271957691
-0.436929337968 0.0399380533696
-0.432424911803 0.0398347561322
-0.427920485638 0.0397488820821
-0.423416059474 0.0396822236035
-0.418911633309 0.0396068878979
-0.414407207145 0.0395237558989
-0.40990278098 0.0394335316262
-0.405398354815 0.0393661252638
-0.400893928651 0.0392927450181
-0.396389502486 0.0392431880159
-0.391885076321 0.0391884485209
-0.387380650157 0.039128813551
-0.382876223992 0.039064542513
-0.378371797828 0.0389958734295
-0.373867371663 0.0389524820071
-0.369362945498 0.0389050980223
-0.364858519334 0.0388538924716
-0.360354093169 0.0388284554186
-0.355849667005 0.0387700607446
-0.35134524084 0.0387376782981
-0.346840814675 0.0387020076326
-0.342336388511 0.0386924650621
-0.337831962346 0.0386505357957
-0.333327536181 0.0386348654534
-0.328823110017 0.0386162623561
-0.324318683852 0.0385948288471
-0.319814257688 0.0385706703006
-0.315309831523 0.0385727748123
-0.310805405358 0.0385433950358
-0.306300979194 0.0385402970866
-0.301796553029 0.0385346949717
-0.297292126865 0.0385266869966
-0.2927877007 0.0385447075603
-0.288283274535 0.0385320663264
-0.283778848371 0.0385453927505
-0.279274422206 0.0385564484975
-0.274769996041 0.038565332429
-0.270265569877 0.0385997445358
-0.265761143712 0.0386044324747
-0.261256717548 0.0386345186519
-0.256752291383 0.0386625063205
-0.252247865218 0.0386885008164
-0.247743439054 0.0387126146571
-0.243239012889 0.0387614218678
-0.238734586725 0.0387819210293
-0.23423016056 0.0388269227565
-0.229725734395 0.0388700900209
-0.225221308231 0.0389115482526
-0.220716882066 0.0389767215609
-0.216212455901 0.0390149140068
-0.211708029737 0.0390765865988
-0.207203603572 0.0391365844085
-0.202699177408 0.0391950522452
-0.198194751243 0.0392760826008
-0.193690325078 0.0393316693912
-0.189185898914 0.0394095559272
-0.184681472749 0.0394859652653
-0.180177046585 0.0395610693601
-0.17567262042 0.0396350504938
-0.171168194255 0.0397301827392
-0.166663768091 0.039823923305
-0.162159341926 0.0399164689927
-0.157654915762 0.0400080283283
-0.153150489597 0.0401195325935
-0.148646063432 0.0402297898439
-0.144141637268 0.04033903037
-0.139637211103 0.0404474977766
-0.135132784938 0.0405554489275
-0.130628358774 0.0406820251048
-0.126123932609 0.0408078776796
-0.121619506445 0.0409513913518
-0.11711508028 0.0410762889609
-0.112610654115 0.0412186827868
-0.108106227951 0.0413777115803
-0.103601801786 0.0415195101206
-0.0990973756215 0.0416778452585
-0.0945929494569 0.0418361906776
-0.0900885232923 0.0420102221325
-0.0855840971277 0.04218426022
-0.0810796709631 0.0423587459317
-0.0765752447984 0.0425481752008
-0.0720708186338 0.0427381752188
-0.0675663924692 0.0429424596992
-0.0630619663046 0.0431475441213
-0.05855754014 0.0433540034369
-0.0540531139754 0.0435863530832
-0.0495486878108 0.043808139673
-0.0450442616461 0.0440546760936
-0.0405398354815 0.0443027940506
-0.0360354093169 0.044553272217
-0.0315309831523 0.0448168584293
-0.0270265569877 0.0451027886562
-0.0225221308231 0.0453913653913
-0.0180177046585 0.045683596779
-0.0135132784938 0.0459973736456
-0.00900885232923 0.0463316499462
-0.00450442616461 0.04667011909
0.0 0.0470288360191
0.00041620897761 0.0470657071424
0.000832417955221 0.0470952875379
0.00124862693283 0.0471322301157
0.00166483591044 0.0471619436269
0.00208104488805 0.0471989623856
0.00249725386566 0.0472360048196
0.00291346284327 0.0472659126493
0.00332967182088 0.0473030385093
0.00374588079849 0.0473401919533
0.0041620897761 0.0473773743465
0.00457829875371 0.0474075475645
0.00499450773132 0.0474448230751
0.00541071670893 0.0474821313936
0.00582692568655 0.0475194738655
0.00624313466416 0.0475568518301
0.00665934364177 0.0475873745463
0.00707555261938 0.047624857624
0.00749176159699 0.0476623799668
0.0079079705746 0.0476999428863
0.00832417955221 0.0477375476858
0.00874038852982 0.0477751956599
0.00915659750743 0.047812888094
0.00957280648504 0.0478506262635
0.00998901546265 0.0478884114336
0.0104052244403 0.0479262448587
0.0108214334179 0.0479641277815
0.0112376423955 0.0480020614331
0.0116538513731 0.0480400470316
0.0120700603507 0.0480780857821
0.0124862693283 0.0481161788757
0.0129024783059 0.0481607884204
0.0133186872835 0.0481989664964
0.0137348962611 0.0482372025774
0.0141511052388 0.0482754977897
0.0145673142164 0.0483138532418
0.014983523194 0.048358590975
0.0153997321716 0.048397043828
0.0158159411492 0.0484355602969
0.0162321501268 0.0484803782828
0.0166483591044 0.0485189992118
0.017064568082 0.0485576869233
0.0174807770596 0.0486025967012
0.0178969860372 0.0486413954468
0.0183131950149 0.0486863621698
0.0187294039925 0.048725276125
0.0191456129701 0.0487703044454
0.0195618219477 0.0488153500959
0.0199780309253 0.0488544317242
0.0203942399029 0.0488995454227
0.0208104488805 0.0489446796545
0.0212266578581 0.0489839369631
0.0216428668357 0.049029144746
0.0220590758134 0.0490743757165
0.022475284791 0.049119630653
0.0228914937686 0.0491649102522
0.0233077027462 0.049210215126
0.0237239117238 0.0492555457966
0.0241401207014 0.0493009026925
0.024556329679 0.0493462861438
0.0249725386566 0.0493916963774
0.0253887476342 0.0494371335118
0.0258049566118 0.0494825975517
0.0262211655895 0.0495336351528
0.0266373745671 0.0495791231495
0.0270535835447 0.0496246372264
0.0274697925223 0.0496756297334
0.0278860014999 0.0497211644466
0.0283022104775 0.0497721106855
0.0287184194551 0.0498230138481
0.0291346284327 0.0498685560129
0.0295508374103 0.0499194030205
0.0299670463879 0.0499702002616
0.0303832553656 0.0500209446947
0.0307994643432 0.0500716328809
0.0312156733208 0.0501222609578
0.0316318822984 0.0501728246107
0.032048091276 0.0502283689803
0.0324643002536 0.0502787482048
0.0328805092312 0.0503340074203
0.0332967182088 0.0503841748368
0.0337129271864 0.0504391142343
0.0341291361641 0.0504938523472
0.0345453451417 0.050548375902
0.0349615541193 0.0506026702129
0.0353777630969 0.050661360032
0.0357939720745 0.0507150850193
0.0362101810521 0.0507730332877
0.0366263900297 0.0508305321614
0.0370425990073 0.0508875461456
0.0374588079849 0.0509482964442
0.0378750169625 0.0510082873703
0.0382912259402 0.0510674484074
0.0387074349178 0.0511296230308
0.0391236438954 0.0511905251093
0.039539852873 0.0512536194591
0.0399560618506 0.0513181530808
0.0403722708282 0.0513831137158
0.0407884798058 0.0514470786388
0.0412046887834 0.0515147344064


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceCircularProb0pt8.tex <==
-0.450442616461 0.071606609885
-0.447766086434 0.0715901797583
-0.445089556407 0.0715535566331
-0.44241302638 0.0715413622323
-0.439736496353 0.0714823885228
-0.437059966326 0.0714888981808
-0.434383436299 0.0714513087249
-0.431706906272 0.071443997138
-0.429030376245 0.0714307550277
-0.426353846218 0.0714120795796
-0.423677316191 0.0713883846321
-0.421000786164 0.0713964194978
-0.418324256137 0.0713636136456
-0.41564772611 0.071362948301
-0.412971196083 0.0713582571657
-0.410294666056 0.0713497474672
-0.407618136029 0.0713376070236
-0.404941606002 0.0713579067179
-0.402265075975 0.0713389136791
-0.399588545948 0.0713524801149
-0.396912015921 0.0713628355122
-0.394235485894 0.0713701002784
-0.391558955867 0.0713743876034
-0.38888242584 0.0714111376365
-0.386205895813 0.0714096819345
-0.383529365786 0.0714406790073
-0.380852835759 0.0714338574125
-0.378176305732 0.0714594516513
-0.375499775705 0.0714824119645
-0.372823245678 0.0715028135809
-0.370146715651 0.0715553070736
-0.367470185624 0.0715706899911
-0.364793655597 0.0716180668335
-0.36211712557 0.0716286964429
-0.359440595543 0.0716712053928
-0.356764065516 0.071711307737
-0.354087535489 0.0717490594471
-0.351411005462 0.0718182325989
-0.348734475435 0.0718513149519
-0.346057945408 0.0718822074408
-0.343381415381 0.0719442763288
-0.340704885354 0.0720039825943
-0.338028355327 0.0720613713492
-0.3353518253 0.0721164875579
-0.332675295273 0.072169376094
-0.329998765246 0.0722526753259
-0.327322235219 0.0723010915547
-0.324645705192 0.0723797003813
-0.321969175165 0.0724559457962
-0.319292645138 0.0725298656082
-0.316616115111 0.072601497926
-0.313939585084 0.0726708811728
-0.311263055057 0.0727695321191
-0.30858652503 0.0728343643769
-0.305909995003 0.0729281976904
-0.303233464976 0.0730195861964
-0.300556934949 0.0731085625432
-0.297880404922 0.0732257568876
-0.295203874895 0.0733098245856
-0.292527344868 0.0734218019376
-0.289850814841 0.0735311181462
-0.287174284814 0.0736377999449
-0.284497754787 0.0737715100324
-0.28182122476 0.0738728040229
-0.279144694733 0.0740007707798
-0.276468164706 0.0741257939487
-0.273791634679 0.0742478929383
-0.271115104652 0.0743670873
-0.268438574625 0.0745117584623
-0.265762044597 0.0746531124782
-0.26308551457 0.074791158306
-0.260408984543 0.0749535658159
-0.257732454516 0.075084780674
-0.255055924489 0.0752670474639
-0.252379394462 0.0754181100286
-0.249702864435 0.0755920267792
-0.247026334408 0.0757616057021
-0.244349804381 0.0759268193272
-0.241673274354 0.0761134563914
-0.238996744327 0.0762950834994
-0.2363202143 0.076471642517
-0.233643684273 0.0766679814216
-0.230967154246 0.0768830611348
-0.228290624219 0.0770915244425
-0.225614094192 0.0772932273973
-0.222937564165 0.0775350445906
-0.220261034138 0.0777451147581
-0.217584504111 0.0779925171219
-0.214907974084 0.0782298595369
-0.212231444057 0.0784785505786
-0.20955491403 0.0787366712419
-0.206878384003 0.0790228020806
-0.204201853976 0.0792923625436
-0.201525323949 0.0795832638995
-0.198848793922 0.0798899201525
-0.196172263895 0.0802055173486
-0.193495733868 0.080521544501
-0.190819203841 0.0808738542822
-0.188142673814 0.0812334627178
-0.185466143787 0.0816232718214


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceEqualAreas.tex <==
-4.5 0.13656204421
-4.49551 0.136561861464
-4.49102 0.136561676614
-4.48653 0.136561489637
-4.48204 0.136561300509
-4.47755 0.136561109205
-4.47306 0.136560915701
-4.46857 0.136560719972
-4.46408 0.136560521993
-4.45959 0.136560321738
-4.4551 0.136560119181
-4.45061 0.136559914297
-4.44612 0.136559707059
-4.44163 0.13655949744
-4.43714 0.136559285415
-4.43265 0.136559070954
-4.42816 0.136558854032
-4.42367 0.136558634619
-4.41918 0.136558412689
-4.41469 0.136558188213
-4.4102 0.136557961161
-4.40571 0.136557731505
-4.40122 0.136557499216
-4.39673 0.136557264263
-4.39224 0.136557026617
-4.38775 0.136556786248
-4.38326 0.136556543124
-4.37877 0.136556297215
-4.37428 0.136556048489
-4.36979 0.136555796915
-4.3653 0.136555542461
-4.36081 0.136555285093
-4.35632 0.13655502478
-4.35183 0.136554761488
-4.34734 0.136554495183
-4.34285 0.136554225833
-4.33836 0.136553953402
-4.33387 0.136553677856
-4.32938 0.136553399159
-4.32489 0.136553117278
-4.3204 0.136552832175
-4.31591 0.136552543815
-4.31142 0.13655225216
-4.30693 0.136551957175
-4.30244 0.136551658822
-4.29795 0.136551357062
-4.29346 0.136551051858
-4.28897 0.136550743171
-4.28448 0.136550430962
-4.27999 0.136550115192
-4.2755 0.13654979582
-4.27101 0.136549472807
-4.26652 0.136549146111
-4.26203 0.136548815692
-4.25754 0.136548481507
-4.25305 0.136548143515
-4.24856 0.136547801672
-4.24407 0.136547455936
-4.23958 0.136547106264
-4.23509 0.136546752611
-4.2306 0.136546394933
-4.22611 0.136546033184
-4.22162 0.13654566732
-4.21713 0.136545297294
-4.21264 0.136544923061
-4.20815 0.136544544572
-4.20366 0.13654416178
-4.19917 0.136543774639
-4.19468 0.136543383098
-4.19019 0.136542987109
-4.1857 0.136542586622
-4.18121 0.136542181587
-4.17672 0.136541771954
-4.17223 0.136541357671
-4.16774 0.136540938687
-4.16325 0.136540514949
-4.15876 0.136540086404
-4.15427 0.136539652999
-4.14978 0.13653921468
-4.14529 0.136538771391
-4.1408 0.136538323079
-4.13631 0.136537869686
-4.13182 0.136537411157
-4.12733 0.136536947434
-4.12284 0.13653647846
-4.11835 0.136536004177
-4.11386 0.136535524525
-4.10937 0.136535039445
-4.10488 0.136534548876
-4.10039 0.136534052759
-4.0959 0.13653355103
-4.09141 0.136533043629
-4.08692 0.136532530492
-4.08243 0.136532011556
-4.07794 0.136531486756
-4.07345 0.136530956028
-4.06896 0.136530419305
-4.06447 0.136529876522
-4.05998 0.136529327612
-4.05549 0.136528772506
-4.051 0.136528211137
-4.04651 0.136527643434
-4.04202 0.136527069329
-4.03753 0.136526488749
-4.03304 0.136525901625
-4.02855 0.136525307883
-4.02406 0.13652470745
-4.01957 0.136524100253
-4.01508 0.136523486217
-4.01059 0.136522865266
-4.0061 0.136522237324
-4.00161 0.136521602315
-3.99712 0.13652096016
-3.99263 0.136520310781
-3.98814 0.136519654097
-3.98365 0.13651899003
-3.97916 0.136518318496
-3.97467 0.136517639415
-3.97018 0.136516952703
-3.96569 0.136516258276
-3.9612 0.13651555605
-3.95671 0.136514845938
-3.95222 0.136514127854
-3.94773 0.136513401711
-3.94324 0.13651266742
-3.93875 0.136511924891
-3.93426 0.136511174035
-3.92977 0.136510414759
-3.92528 0.136509646972
-3.92079 0.136508870579
-3.9163 0.136508085488
-3.91181 0.136507291602
-3.90732 0.136506488825
-3.90283 0.13650567706
-3.89834 0.136504856208
-3.89385 0.136504026171
-3.88936 0.136503186846
-3.88487 0.136502338134
-3.88038 0.136501479931
-3.87589 0.136500612133
-3.8714 0.136499734636
-3.86691 0.136498847333
-3.86242 0.136497950119
-3.85793 0.136497042883
-3.85344 0.136496125518
-3.84895 0.136495197912
-3.84446 0.136494259954
-3.83997 0.136493311531
-3.83548 0.136492352529
-3.83099 0.136491382833
-3.8265 0.136490402326
-3.82201 0.13648941089
-3.81752 0.136488408407
-3.81303 0.136487394756
-3.80854 0.136486369816
-3.80405 0.136485333464
-3.79956 0.136484285576
-3.79507 0.136483226027
-3.79058 0.136482154689
-3.78609 0.136481071436
-3.7816 0.136479976137
-3.77711 0.136478868662
-3.77262 0.136477748879
-3.76813 0.136476616654
-3.76364 0.136475471852
-3.75915 0.136474314338
-3.75466 0.136473143973
-3.75017 0.136471960618
-3.74568 0.136470764133
-3.74119 0.136469554375
-3.7367 0.136468331201
-3.73221 0.136467094466
-3.72772 0.136465844022
-3.72323 0.136464579723
-3.71874 0.136463301418
-3.71425 0.136462008956
-3.70976 0.136460702184
-3.70527 0.136459380948
-3.70078 0.136458045091
-3.69629 0.136456694457
-3.6918 0.136455328885
-3.68731 0.136453948214
-3.68282 0.136452552283
-3.67833 0.136451140926
-3.67384 0.136449713977
-3.66935 0.13644827127
-3.66486 0.136446812633
-3.66037 0.136445337896
-3.65588 0.136443846886
-3.65139 0.136442339428
-3.6469 0.136440815346
-3.64241 0.13643927446
-3.63792 0.13643771659
-3.63343 0.136436141554
-3.62894 0.136434549168
-3.62445 0.136432939246
-3.61996 0.1364313116
-3.61547 0.13642966604
-3.61098 0.136428002374
-3.60649 0.136426320408
-3.602 0.136424619947
-3.59751 0.136422900792
-3.59302 0.136421162744
-3.58853 0.136419405601
-3.58404 0.136417629158
-3.57955 0.13641583321
-3.57506 0.136414017547
-3.57057 0.136412181961
-3.56608 0.136410326237
-3.56159 0.136408450162
-3.5571 0.136406553518
-3.55261 0.136404636087
-3.54812 0.136402697646
-3.54363 0.136400737972
-3.53914 0.136398756839
-3.53465 0.136396754018
-3.53016 0.13639472928
-3.52567 0.13639268239
-3.52118 0.136390613114
-3.51669 0.136388521214
-3.5122 0.136386406449
-3.50771 0.136384268577
-3.50322 0.136382107352
-3.49873 0.136379922527
-3.49424 0.136377713852
-3.48975 0.136375481073
-3.48526 0.136373223936
-3.48077 0.136370942183
-3.47628 0.136368635553
-3.47179 0.136366303782
-3.4673 0.136363946606
-3.46281 0.136361563755
-3.45832 0.136359154958
-3.45383 0.136356719941
-3.44934 0.136354258428
-3.44485 0.136351770138
-3.44036 0.136349254789
-3.43587 0.136346712096
-3.43138 0.13634414177
-3.42689 0.136341543521
-3.4224 0.136338917055
-3.41791 0.136336262074
-3.41342 0.136333578278
-3.40893 0.136330865364
-3.40444 0.136328123027
-3.39995 0.136325350957
-3.39546 0.136322548841
-3.39097 0.136319716365
-3.38648 0.13631685321
-3.38199 0.136313959053
-3.3775 0.13631103357
-3.37301 0.136308076433
-3.36852 0.13630508731
-3.36403 0.136302065866
-3.35954 0.136299011763
-3.35505 0.136295924658
-3.35056 0.136292804208
-3.34607 0.136289650064
-3.34158 0.136286461872
-3.33709 0.136283239279
-3.3326 0.136279981925
-3.32811 0.136276689448
-3.32362 0.13627336148
-3.31913 0.136269997653
-3.31464 0.136266597592
-3.31015 0.136263160921
-3.30566 0.136259687257
-3.30117 0.136256176218
-3.29668 0.136252627413
-3.29219 0.13624904045
-3.2877 0.136245414934
-3.28321 0.136241750463
-3.27872 0.136238046634
-3.27423 0.136234303037
-3.26974 0.136230519262
-3.26525 0.13622669489
-3.26076 0.136222829503
-3.25627 0.136218922675
-3.25178 0.136214973978
-3.24729 0.136210982978
-3.2428 0.136206949238
-3.23831 0.136202872317
-3.23382 0.136198751768
-3.22933 0.136194587142
-3.22484 0.136190377983
-3.22035 0.136186123833
-3.21586 0.136181824227
-3.21137 0.136177478698
-3.20688 0.136173086772
-3.20239 0.136168647972
-3.1979 0.136164161816
-3.19341 0.136159627818
-3.18892 0.136155045485
-3.18443 0.136150414322
-3.17994 0.136145733826
-3.17545 0.136141003493
-3.17096 0.136136222811
-3.16647 0.136131391263
-3.16198 0.13612650833
-3.15749 0.136121573485
-3.153 0.136116586197
-3.14851 0.136111545929
-3.14402 0.13610645214
-3.13953 0.136101304284
-3.13504 0.136096101809
-3.13055 0.136090844157
-3.12606 0.136085530765
-3.12157 0.136080161065
-3.11708 0.136074734484
-3.11259 0.136069250442
-3.1081 0.136063708356
-3.10361 0.136058107634
-3.09912 0.13605244768
-3.09463 0.136046727893
-3.09014 0.136040947666
-3.08565 0.136035106385
-3.08116 0.13602920343
-3.07667 0.136023238177
-3.07218 0.136017209995
-3.06769 0.136011118246
-3.0632 0.136004962288
-3.05871 0.13599874147
-3.05422 0.135992455139
-3.04973 0.135986102631
-3.04524 0.135979683278
-3.04075 0.135973196407
-3.03626 0.135966641337
-3.03177 0.13596001738
-3.02728 0.135953323843
-3.02279 0.135946560025
-3.0183 0.135939725219
-3.01381 0.135932818712
-3.00932 0.135925839783
-3.00483 0.135918787705
-3.00034 0.135911661744
-2.99585 0.13590446116
-2.99136 0.135897185204
-2.98687 0.135889833121
-2.98238 0.135882404149
-2.97789 0.13587489752
-2.9734 0.135867312456
-2.96891 0.135859648174
-2.96442 0.135851903884
-2.95993 0.135844078786
-2.95544 0.135836172075
-2.95095 0.135828182938
-2.94646 0.135820110553
-2.94197 0.135811954092
-2.93748 0.135803712718
-2.93299 0.135795385588
-2.9285 0.13578697185
-2.92401 0.135778470644
-2.91952 0.135769881102
-2.91503 0.135761202348
-2.91054 0.135752433498
-2.90605 0.135743573661
-2.90156 0.135734621935
-2.89707 0.135725577413
-2.89258 0.135716439177
-2.88809 0.135707206302
-2.8836 0.135697877854
-2.87911 0.135688452891
-2.87462 0.13567893046
-2.87013 0.135669309604
-2.86564 0.135659589352
-2.86115 0.135649768727
-2.85666 0.135639846743
-2.85217 0.135629822404
-2.84768 0.135619694706
-2.84319 0.135609462636
-2.8387 0.135599125169
-2.83421 0.135588681275
-2.82972 0.135578129911
-2.82523 0.135567470026
-2.82074 0.135556700561
-2.81625 0.135545820445
-2.81176 0.135534828597
-2.80727 0.135523723929
-2.80278 0.135512505342
-2.79829 0.135501171725
-2.7938 0.13548972196
-2.78931 0.135478154917
-2.78482 0.135466469458
-2.78033 0.135454664432
-2.77584 0.135442738679
-2.77135 0.13543069103
-2.76686 0.135418520303
-2.76237 0.135406225307
-2.75788 0.135393804841
-2.75339 0.135381257691
-2.7489 0.135368582634
-2.74441 0.135355778436
-2.73992 0.135342843853
-2.73543 0.135329777626
-2.73094 0.13531657849
-2.72645 0.135303245166
-2.72196 0.135289776364
-2.71747 0.135276170782
-2.71298 0.135262427109
-2.70849 0.13524854402
-2.704 0.135234520178
-2.69951 0.135220354238
-2.69502 0.135206044838
-2.69053 0.135191590609
-2.68604 0.135176990167
-2.68155 0.135162242117
-2.67706 0.135147345051
-2.67257 0.135132297549
-2.66808 0.13511709818
-2.66359 0.1351017455
-2.6591 0.135086238051
-2.65461 0.135070574364
-2.65012 0.135054752956
-2.64563 0.135038772334
-2.64114 0.135022630987
-2.63665 0.135006327397
-2.63216 0.134989860029
-2.62767 0.134973227336
-2.62318 0.134956427757
-2.61869 0.134939459718
-2.6142 0.134922321634
-2.60971 0.134905011902
-2.60522 0.134887528909
-2.60073 0.134869871027
-2.59624 0.134852036613
-2.59175 0.134834024012
-2.58726 0.134815831553
-2.58277 0.134797457554
-2.57828 0.134778900316
-2.57379 0.134760158125
-2.5693 0.134741229256
-2.56481 0.134722111967
-2.56032 0.134702804502
-2.55583 0.13468330509
-2.55134 0.134663611945
-2.54685 0.134643723267
-2.54236 0.134623637241
-2.53787 0.134603352035
-2.53338 0.134582865805
-2.52889 0.134562176688
-2.5244 0.134541282808
-2.51991 0.134520182273
-2.51542 0.134498873175
-2.51093 0.134477353591
-2.50644 0.134455621582
-2.50195 0.134433675192
-2.49746 0.13441151245
-2.49297 0.134389131368
-2.48848 0.134366529942
-2.48399 0.134343706154
-2.4795 0.134320657966
-2.47501 0.134297383325
-2.47052 0.134273880161
-2.46603 0.134250146388
-2.46154 0.134226179902
-2.45705 0.134201978583
-2.45256 0.134177540294
-2.44807 0.13415286288
-2.44358 0.134127944169
-2.43909 0.134102781971
-2.4346 0.13407737408
-2.43011 0.13405171827
-2.42562 0.134025812301
-2.42113 0.13399965391
-2.41664 0.133973240821
-2.41215 0.133946570738
-2.40766 0.133919641345
-2.40317 0.133892450311
-2.39868 0.133864995284
-2.39419 0.133837273895
-2.3897 0.133809283756
-2.38521 0.13378102246
-2.38072 0.133752487581
-2.37623 0.133723676676
-2.37174 0.133694587279
-2.36725 0.133665216909
-2.36276 0.133635563064
-2.35827 0.133605623222
-2.35378 0.133575394843
-2.34929 0.133544875366
-2.3448 0.133514062211
-2.34031 0.133482952778
-2.33582 0.133451544448
-2.33133 0.13341983458
-2.32684 0.133387820515
-2.32235 0.133355499573
-2.31786 0.133322869053
-2.31337 0.133289926234
-2.30888 0.133256668374
-2.30439 0.133223092712
-2.2999 0.133189196465
-2.29541 0.133154976829
-2.29092 0.133120430978
-2.28643 0.133085556068
-2.28194 0.13305034923
-2.27745 0.133014807578
-2.27296 0.132978928199
-2.26847 0.132942708164
-2.26398 0.13290614452
-2.25949 0.132869234291
-2.255 0.132831974481
-2.25051 0.132794362072
-2.24602 0.132756394022
-2.24153 0.13271806727
-2.23704 0.132679378729
-2.23255 0.132640325294
-2.22806 0.132600903833
-2.22357 0.132561111195
-2.21908 0.132520944205
-2.21459 0.132480399664
-2.2101 0.132439474351
-2.20561 0.132398165024
-2.20112 0.132356468415
-2.19663 0.132314381234
-2.19214 0.132271900168
-2.18765 0.13222902188
-2.18316 0.13218574301
-2.17867 0.132142060175
-2.17418 0.132097969966
-2.16969 0.132053468953
-2.1652 0.13200855368
-2.16071 0.131963220669
-2.15622 0.131917466416
-2.15173 0.131871287394
-2.14724 0.131824680052
-2.14275 0.131777640814
-2.13826 0.131730166079
-2.13377 0.131682252223
-2.12928 0.131633895596
-2.12479 0.131585092524
-2.1203 0.131535839308
-2.11581 0.131486132225
-2.11132 0.131435967525
-2.10683 0.131385341435
-2.10234 0.131334250155
-2.09785 0.131282689863
-2.09336 0.131230656707
-2.08887 0.131178146814
-2.08438 0.131125156282
-2.07989 0.131071681187
-2.0754 0.131017717576
-2.07091 0.130963261472
-2.06642 0.130908308873
-2.06193 0.13085285575
-2.05744 0.130796898047
-2.05295 0.130740431685
-2.04846 0.130683452556
-2.04397 0.130625956527
-2.03948 0.13056793944
-2.03499 0.130509397109
-2.0305 0.130450325322
-2.02601 0.130390719842
-2.02152 0.130330576403
-2.01703 0.130269890715
-2.01254 0.130208658459
-2.00805 0.130146875293
-2.00356 0.130084536844
-1.99907 0.130021638716
-1.99458 0.129958176483
-1.99009 0.129894145694
-1.9856 0.129829541872
-1.98111 0.12976436051
-1.97662 0.129698597078
-1.97213 0.129632247015
-1.96764 0.129565305736
-1.96315 0.129497768627
-1.95866 0.129429631048
-1.95417 0.129360888331
-1.94968 0.129291535781
-1.94519 0.129221568677
-1.9407 0.129150982269
-1.93621 0.12907977178
-1.93172 0.129007932406
-1.92723 0.128935459317
-1.92274 0.128862347653
-1.91825 0.128788592528
-1.91376 0.12871418903
-1.90927 0.128639132216
-1.90478 0.12856341712
-1.90029 0.128487038745
-1.8958 0.128409992068
-1.89131 0.128332272039
-1.88682 0.12825387358
-1.88233 0.128174791585
-1.87784 0.128095020922
-1.87335 0.12801455643
-1.86886 0.127933392921
-1.86437 0.127851525182
-1.85988 0.127768947969
-1.85539 0.127685656012
-1.8509 0.127601644015
-1.84641 0.127516906653
-1.84192 0.127431438575
-1.83743 0.127345234401
-1.83294 0.127258288725
-1.82845 0.127170596115
-1.82396 0.12708215111
-1.81947 0.126992948221
-1.81498 0.126902981936
-1.81049 0.126812246711
-1.806 0.126720736979
-1.80151 0.126628447144
-1.79702 0.126535371585
-1.79253 0.126441504651
-1.78804 0.126346840668
-1.78355 0.126251373933
-1.77906 0.126155098718
-1.77457 0.126058009267
-1.77008 0.125960099799
-1.76559 0.125861364505
-1.7611 0.125761797553
-1.75661 0.125661393081
-1.75212 0.125560145203
-1.74763 0.125458048008
-1.74314 0.125355095558
-1.73865 0.125251281888
-1.73416 0.125146601011
-1.72967 0.125041046911
-1.72518 0.124934613549
-1.72069 0.124827294859
-1.7162 0.124719084752
-1.71171 0.124609977113
-1.70722 0.124499965801
-1.70273 0.124389044653
-1.69824 0.12427720748
-1.69375 0.124164448068
-1.68926 0.124050760181
-1.68477 0.123936137556
-1.68028 0.123820573909
-1.67579 0.123704062932
-1.6713 0.123586598291
-1.66681 0.123468173632
-1.66232 0.123348782576
-1.65783 0.123228418721
-1.65334 0.123107075643
-1.64885 0.122984746897
-1.64436 0.122861426012
-1.63987 0.122737106499
-1.63538 0.122611781844
-1.63089 0.122485445513
-1.6264 0.12235809095
-1.62191 0.122229711579
-1.61742 0.122100300803
-1.61293 0.121969852002
-1.60844 0.121838358539
-1.60395 0.121705813754
-1.59946 0.121572210969
-1.59497 0.121437543487
-1.59048 0.12130180459
-1.58599 0.121164987541
-1.5815 0.121027085586
-1.57701 0.120888091951
-1.57252 0.120747999845
-1.56803 0.120606802459
-1.56354 0.120464492967
-1.55905 0.120321064524
-1.55456 0.120176510271
-1.55007 0.12003082333
-1.54558 0.119883996809
-1.54109 0.119736023799
-1.5366 0.119586897376
-1.53211 0.119436610601
-1.52762 0.11928515652
-1.52313 0.119132528166
-1.51864 0.118978718558
-1.51415 0.118823720699
-1.50966 0.118667527583
-1.50517 0.118510132188
-1.50068 0.118351527481
-1.49619 0.118191706419
-1.4917 0.118030661944
-1.48721 0.11786838699
-1.48272 0.117704874481
-1.47823 0.117540117328
-1.47374 0.117374108435
-1.46925 0.117206840696
-1.46476 0.117038306998
-1.46027 0.116868500218
-1.45578 0.116697413226
-1.45129 0.116525038885
-1.4468 0.116351370053
-1.44231 0.116176399579
-1.43782 0.11600012031
-1.43333 0.115822525087
-1.42884 0.115643606744
-1.42435 0.115463358115
-1.41986 0.115281772029
-1.41537 0.115098841313
-1.41088 0.114914558792
-1.40639 0.114728917288
-1.4019 0.114541909625
-1.39741 0.114353528625
-1.39292 0.114163767111
-1.38843 0.113972617908
-1.38394 0.11378007384
-1.37945 0.113586127737
-1.37496 0.11339077243
-1.37047 0.113194000755
-1.36598 0.112995805551
-1.36149 0.112796179663
-1.357 0.112595115943
-1.35251 0.112392607248
-1.34802 0.112188646445
-1.34353 0.111983226405
-1.33904 0.111776340011
-1.33455 0.111567980156
-1.33006 0.111358139742
-1.32557 0.111146811683
-1.32108 0.110933988906
-1.31659 0.110719664348
-1.3121 0.110503830963
-1.30761 0.110286481719
-1.30312 0.110067609598
-1.29863 0.1098472076
-1.29414 0.109625268741
-1.28965 0.109401786056
-1.28516 0.1091767526
-1.28067 0.108950161445
-1.27618 0.108722005688
-1.27169 0.108492278444
-1.2672 0.108260972854
-1.26271 0.108028082081
-1.25822 0.107793599314
-1.25373 0.107557517766
-1.24924 0.107319830681
-1.24475 0.107080531326
-1.24026 0.106839613
-1.23577 0.106597069032
-1.23128 0.106352892781
-1.22679 0.106107077639
-1.2223 0.105859617033
-1.21781 0.105610504422
-1.21332 0.105359733301
-1.20883 0.105107297204
-1.20434 0.104853189701
-1.19985 0.104597404403
-1.19536 0.104339934961
-1.19087 0.104080775066
-1.18638 0.103819918455
-1.18189 0.103557358908
-1.1774 0.10329309025
-1.17291 0.103027106354
-1.16842 0.102759401141
-1.16393 0.102489968582
-1.15944 0.102218802698
-1.15495 0.101945897563
-1.15046 0.101671247307
-1.14597 0.101394846112
-1.14148 0.101116688218
-1.13699 0.100836767924
-1.1325 0.100555079589
-1.12801 0.100271617632
-1.12352 0.099986376536
-1.11903 0.099699350848
-1.11454 0.0994105351814
-1.11005 0.099119924217
-1.10556 0.0988275127052
-1.10107 0.0985332954674
-1.09658 0.0982372673977
-1.09209 0.0979394234647
-1.0876 0.0976397587133
-1.08311 0.0973382682665
-1.07862 0.097034947327
-1.07413 0.0967297911791
-1.06964 0.096422795191
-1.06515 0.096113954816
-1.06066 0.0958032655949
-1.05617 0.0954907231578
-1.05168 0.0951763232262
-1.04719 0.0948600616149
-1.0427 0.0945419342341
-1.03821 0.0942219370913
-1.03372 0.0939000662937
-1.02923 0.0935763180504
-1.02474 0.0932506886742
-1.02025 0.092923174584
-1.01576 0.0925937723073
-1.01127 0.0922624784819
-1.00678 0.0919292898591
-1.00229 0.0915942033052
-0.9978 0.0912572158042
-0.99331 0.0909183244607
-0.98882 0.0905775265015
-0.98433 0.0902348192789
-0.97984 0.0898902002729
-0.97535 0.0895436670938
-0.97086 0.089195217485
-0.96637 0.0888448493254
-0.96188 0.0884925606325
-0.95739 0.088138349565
-0.9529 0.0877822144255
-0.94841 0.0874241536636
-0.94392 0.0870641658786
-0.93943 0.0867022498227
-0.93494 0.0863384044038
-0.93045 0.0859726286886
-0.92596 0.0856049219059
-0.92147 0.0852352834497
-0.91698 0.084863712882
-0.91249 0.0844902099368
-0.908 0.0841147745229
-0.90351 0.0837374067276
-0.89902 0.0833581068197
-0.89453 0.0829768752535
-0.89004 0.0825937126722
-0.88555 0.0822086199114
-0.88106 0.0818215980029
-0.87657 0.0814326481783
-0.87208 0.081041771873
-0.86759 0.0806489707301
-0.8631 0.080254246604
-0.85861 0.0798576015649
-0.85412 0.0794590379024
-0.84963 0.0790585581301
-0.84514 0.0786561649892
-0.84065 0.0782518614536
-0.83616 0.0778456507336
-0.83167 0.0774375362805
-0.82718 0.0770275217915
-0.82269 0.0766156112136
-0.8182 0.0762018087489
-0.81371 0.075786118859
-0.80922 0.0753685462699
-0.80473 0.074949095977
-0.80024 0.0745277732499
-0.79575 0.0741045836379
-0.79126 0.0736795329746
-0.78677 0.0732526273834
-0.78228 0.0728238732833
-0.77779 0.0723932773934
-0.7733 0.0719608467394
-0.76881 0.0715265886586
-0.76432 0.0710905108056
-0.75983 0.0706526211588
-0.75534 0.0702129280253
-0.75085 0.0697714400479
-0.74636 0.0693281662105
-0.74187 0.0688831158447
-0.73738 0.068436298636
-0.73289 0.0679877246302
-0.7284 0.06753740424
-0.72391 0.0670853482516
-0.71942 0.0666315678317
-0.71493 0.0661760745338
-0.71044 0.0657188803059
-0.70595 0.0652599974969
-0.70146 0.0647994388644
-0.69697 0.0643372175817
-0.69248 0.0638733472452
-0.68799 0.0634078418824
-0.6835 0.0629407159591
-0.67901 0.0624719843874
-0.67452 0.0620016625338
-0.67003 0.061529766227
-0.66554 0.0610563117664
-0.66105 0.0605813159301
-0.65656 0.0601047959836
-0.65207 0.0596267696884
-0.64758 0.0591472553105
-0.64309 0.0586662716296
-0.6386 0.0581838379478
-0.63411 0.0576999740987
-0.62962 0.0572147004572
-0.62513 0.0567280379482
-0.62064 0.0562400080566
-0.61615 0.055750632837
-0.61166 0.0552599349234
-0.60717 0.0547679375392
-0.60268 0.0542746645073
-0.59819 0.0537801402606
-0.5937 0.0532843898522
-0.58921 0.052787438966
-0.58472 0.0522893139277
-0.58023 0.0517900417153
-0.57574 0.0512896499703
-0.57125 0.0507881670089
-0.56676 0.0502856218334
-0.56227 0.0497820441435
-0.55778 0.0492774643481
-0.55329 0.0487719135771
-0.5488 0.0482654236931
-0.54431 0.047758027304
-0.53982 0.0472497577747
-0.53533 0.0467406492399
-0.53084 0.0462307366165
-0.52635 0.0457200556164
-0.52186 0.0452086427595
-0.51737 0.0446965353862
-0.51288 0.0441837716714
-0.50839 0.0436703906373
-0.5039 0.0431564321669
-0.49941 0.0426419370179
-0.49492 0.0421269468365
-0.49043 0.0416115041709
-0.48594 0.0410956524861
-0.48145 0.0405794361776
-0.47696 0.0400629005862
-0.47247 0.0395460920123
-0.46798 0.0390290577305
-0.46349 0.0385118460048
-0.459 0.0379945061034
-0.45451 0.0374770883138
-0.45002 0.0369596439581
-0.44553 0.0364422254084
-0.44104 0.0359248861023
-0.43655 0.0354076805588
-0.43206 0.0348906643937
-0.42757 0.034373894336
-0.42308 0.0338574282434
-0.41859 0.0333413251191
-0.4141 0.0328256451277
-0.40961 0.0323104496117
-0.40512 0.0317958011081
-0.40063 0.0312817633648
-0.39614 0.0307684013577
-0.39165 0.0302557813073
-0.38716 0.0297439706957
-0.38267 0.0292330382838
-0.37818 0.0287230541281
-0.37369 0.0282140895981
-0.3692 0.0277062173936
-0.36471 0.0271995115621
-0.36022 0.0266940475162
-0.35573 0.026189902051
-0.35124 0.0256871533617
-0.34675 0.0251858810614
-0.34226 0.0246861661986
-0.33777 0.0241880912749
-0.33328 0.0236917402628
-0.32879 0.0231971986235
-0.3243 0.0227045533247
-0.31981 0.0222138928582
-0.31532 0.0217253072582
-0.31083 0.0212388881186
-0.30634 0.0207547286113
-0.30185 0.0202729235037
-0.29736 0.0197935691766
-0.29287 0.019316763642
-0.28838 0.018842606561
-0.28389 0.0183711992613
-0.2794 0.0179026447547
-0.27491 0.0174370477553
-0.27042 0.0169745146964
-0.26593 0.0165151537484
-0.26144 0.016059074836
-0.25695 0.0156063896554
-0.25246 0.0151572116917
-0.24797 0.014711656236
-0.24348 0.0142698404023
-0.23899 0.0138318831442
-0.2345 0.0133979052717
-0.23001 0.0129680294682
-0.22552 0.012542380306
-0.22103 0.0121210842636
-0.21654 0.0117042697408
-0.21205 0.0112920670755
-0.20756 0.0108846085584
-0.20307 0.0104820284497
-0.19858 0.0100844629931
-0.19409 0.00969205043192
-0.1896 0.00930493102332
-0.18511 0.00892324705308
-0.18062 0.00854714284991
-0.17613 0.0081767647995
-0.17164 0.00781226135833
-0.16715 0.00745378306717
-0.16266 0.00710148256426
-0.15817 0.00675551459829
-0.15368 0.00641603604091
-0.14919 0.00608320589903
-0.1447 0.00575718532678
-0.14021 0.00543813763703
-0.13572 0.00512622831269
-0.13123 0.00482162501751
-0.12674 0.0045244976066
-0.12225 0.00423501813653
-0.11776 0.00395336087503
-0.11327 0.0036797023103
-0.10878 0.00341422115987
-0.10429 0.0031570983791
-0.0998 0.00290851716916
-0.09531 0.00266866298468
-0.09082 0.00243772354081
-0.08633 0.00221588881994
-0.08184 0.00200335107791
-0.07735 0.00180030484968
-0.07286 0.00160694695464
-0.06837 0.00142347650128
-0.06388 0.00125009489149
-0.05939 0.00108700582427
-0.0549 0.00093441529892
-0.05041 0.000792531617761
-0.04592 0.000661565388262
-0.04143 0.000541729524667
-0.03694 0.000433239249058
-0.03245 0.000336312091872
-0.02796 0.000251167891858
-0.02347 0.000178028795467
-0.01898 0.000117119255675
-0.01449 6.86660302318e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceEqualSides.tex <==
-4.5 0.537366491512
-4.49551 0.53727746771
-4.49102 0.537188038527
-4.48653 0.537098202323
-4.48204 0.537007957453
-4.47755 0.53691730227
-4.47306 0.536826235117
-4.46857 0.536734754335
-4.46408 0.53664285826
-4.45959 0.536550545219
-4.4551 0.536457813539
-4.45061 0.536364661538
-4.44612 0.536271087529
-4.44163 0.536177089823
-4.43714 0.536082666721
-4.43265 0.535987816523
-4.42816 0.535892537521
-4.42367 0.535796828002
-4.41918 0.53570068625
-4.41469 0.53560411054
-4.4102 0.535507099145
-4.40571 0.535409650331
-4.40122 0.535311762359
-4.39673 0.535213433485
-4.39224 0.53511466196
-4.38775 0.535015446028
-4.38326 0.53491578393
-4.37877 0.5348156739
-4.37428 0.534715114167
-4.36979 0.534614102955
-4.3653 0.534512638482
-4.36081 0.534410718963
-4.35632 0.534308342604
-4.35183 0.534205507608
-4.34734 0.534102212172
-4.34285 0.533998454488
-4.33836 0.533894232742
-4.33387 0.533789545116
-4.32938 0.533684389785
-4.32489 0.533578764918
-4.3204 0.533472668683
-4.31591 0.533366099236
-4.31142 0.533259054734
-4.30693 0.533151533324
-4.30244 0.53304353315
-4.29795 0.53293505235
-4.29346 0.532826089056
-4.28897 0.532716641396
-4.28448 0.532606707492
-4.27999 0.532496285459
-4.2755 0.53238537341
-4.27101 0.532273969448
-4.26652 0.532162071675
-4.26203 0.532049678186
-4.25754 0.531936787069
-4.25305 0.531823396409
-4.24856 0.531709504284
-4.24407 0.531595108767
-4.23958 0.531480207926
-4.23509 0.531364799824
-4.2306 0.531248882516
-4.22611 0.531132454055
-4.22162 0.531015512487
-4.21713 0.530898055851
-4.21264 0.530780082184
-4.20815 0.530661589515
-4.20366 0.530542575869
-4.19917 0.530423039263
-4.19468 0.530302977713
-4.19019 0.530182389225
-4.1857 0.530061271803
-4.18121 0.529939623444
-4.17672 0.529817442139
-4.17223 0.529694725875
-4.16774 0.529571472634
-4.16325 0.529447680389
-4.15876 0.529323347113
-4.15427 0.529198470768
-4.14978 0.529073049316
-4.14529 0.528947080709
-4.1408 0.528820562896
-4.13631 0.52869349382
-4.13182 0.528565871419
-4.12733 0.528437693625
-4.12284 0.528308958365
-4.11835 0.52817966356
-4.11386 0.528049807127
-4.10937 0.527919386977
-4.10488 0.527788401013
-4.10039 0.527656847137
-4.0959 0.527524723243
-4.09141 0.527392027221
-4.08692 0.527258756952
-4.08243 0.527124910317
-4.07794 0.526990485188
-4.07345 0.526855479433
-4.06896 0.526719890915
-4.06447 0.526583717489
-4.05998 0.526446957007
-4.05549 0.526309607317
-4.051 0.526171666258
-4.04651 0.526033131666
-4.04202 0.525894001372
-4.03753 0.5257542732
-4.03304 0.52561394497
-4.02855 0.525473014495
-4.02406 0.525331479586
-4.01957 0.525189338045
-4.01508 0.525046587671
-4.01059 0.524903226257
-4.0061 0.52475925159
-4.00161 0.524614661454
-3.99712 0.524469453624
-3.99263 0.524323625874
-3.98814 0.524177175969
-3.98365 0.524030101671
-3.97916 0.523882400736
-3.97467 0.523734070915
-3.97018 0.523585109954
-3.96569 0.523435515593
-3.9612 0.523285285568
-3.95671 0.523134417608
-3.95222 0.522982909437
-3.94773 0.522830758777
-3.94324 0.522677963341
-3.93875 0.522524520838
-3.93426 0.522370428973
-3.92977 0.522215685444
-3.92528 0.522060287946
-3.92079 0.521904234167
-3.9163 0.52174752179
-3.91181 0.521590148494
-3.90732 0.521432111953
-3.90283 0.521273409834
-3.89834 0.521114039801
-3.89385 0.520953999512
-3.88936 0.52079328662
-3.88487 0.520631898773
-3.88038 0.520469833613
-3.87589 0.520307088779
-3.8714 0.520143661904
-3.86691 0.519979550615
-3.86242 0.519814752536
-3.85793 0.519649265285
-3.85344 0.519483086473
-3.84895 0.519316213711
-3.84446 0.519148644599
-3.83997 0.518980376738
-3.83548 0.518811407719
-3.83099 0.518641735132
-3.8265 0.51847135656
-3.82201 0.518300269582
-3.81752 0.51812847177
-3.81303 0.517955960695
-3.80854 0.51778273392
-3.80405 0.517608789005
-3.79956 0.517434123504
-3.79507 0.517258734967
-3.79058 0.517082620939
-3.78609 0.516905778959
-3.7816 0.516728206565
-3.77711 0.516549901286
-3.77262 0.516370860648
-3.76813 0.516191082173
-3.76364 0.516010563378
-3.75915 0.515829301774
-3.75466 0.51564729487
-3.75017 0.515464540168
-3.74568 0.515281035167
-3.74119 0.515096777359
-3.7367 0.514911764235
-3.73221 0.514725993279
-3.72772 0.51453946197
-3.72323 0.514352167785
-3.71874 0.514164108195
-3.71425 0.513975280667
-3.70976 0.513785682662
-3.70527 0.513595311638
-3.70078 0.513404165049
-3.69629 0.513212240345
-3.6918 0.513019534968
-3.68731 0.512826046361
-3.68282 0.512631771959
-3.67833 0.512436709193
-3.67384 0.512240855491
-3.66935 0.512044208277
-3.66486 0.511846764969
-3.66037 0.511648522982
-3.65588 0.511449479727
-3.65139 0.51124963261
-3.6469 0.511048979034
-3.64241 0.510847516396
-3.63792 0.510645242091
-3.63343 0.510442153509
-3.62894 0.510238248036
-3.62445 0.510033523053
-3.61996 0.50982797594
-3.61547 0.509621604069
-3.61098 0.509414404811
-3.60649 0.509206375532
-3.602 0.508997513594
-3.59751 0.508787816357
-3.59302 0.508577281173
-3.58853 0.508365905395
-3.58404 0.508153686369
-3.57955 0.507940621438
-3.57506 0.507726707942
-3.57057 0.507511943217
-3.56608 0.507296324594
-3.56159 0.507079849403
-3.5571 0.506862514967
-3.55261 0.506644318609
-3.54812 0.506425257646
-3.54363 0.506205329392
-3.53914 0.505984531158
-3.53465 0.50576286025
-3.53016 0.505540313974
-3.52567 0.505316889628
-3.52118 0.505092584511
-3.51669 0.504867395915
-3.5122 0.50464132113
-3.50771 0.504414357445
-3.50322 0.504186502142
-3.49873 0.503957752502
-3.49424 0.503728105803
-3.48975 0.503497559317
-3.48526 0.503266110317
-3.48077 0.50303375607
-3.47628 0.502800493842
-3.47179 0.502566320893
-3.4673 0.502331234482
-3.46281 0.502095231866
-3.45832 0.501858310298
-3.45383 0.501620467026
-3.44934 0.501381699299
-3.44485 0.501142004361
-3.44036 0.500901379453
-3.43587 0.500659821814
-3.43138 0.500417328679
-3.42689 0.500173897283
-3.4224 0.499929524856
-3.41791 0.499684208626
-3.41342 0.499437945818
-3.40893 0.499190733655
-3.40444 0.498942569358
-3.39995 0.498693450145
-3.39546 0.498443373231
-3.39097 0.49819233583
-3.38648 0.497940335151
-3.38199 0.497687368405
-3.3775 0.497433432796
-3.37301 0.497178525529
-3.36852 0.496922643805
-3.36403 0.496665784825
-3.35954 0.496407945785
-3.35505 0.496149123881
-3.35056 0.495889316306
-3.34607 0.495628520252
-3.34158 0.495366732908
-3.33709 0.495103951462
-3.3326 0.494840173099
-3.32811 0.494575395002
-3.32362 0.494309614355
-3.31913 0.494042828337
-3.31464 0.493775034126
-3.31015 0.4935062289
-3.30566 0.493236409834
-3.30117 0.492965574101
-3.29668 0.492693718874
-3.29219 0.492420841323
-3.2877 0.492146938617
-3.28321 0.491872007924
-3.27872 0.491596046411
-3.27423 0.491319051243
-3.26974 0.491041019583
-3.26525 0.490761948594
-3.26076 0.490481835438
-3.25627 0.490200677274
-3.25178 0.489918471263
-3.24729 0.489635214562
-3.2428 0.489350904329
-3.23831 0.489065537719
-3.23382 0.488779111888
-3.22933 0.488491623991
-3.22484 0.488203071181
-3.22035 0.487913450611
-3.21586 0.487622759433
-3.21137 0.487330994799
-3.20688 0.487038153861
-3.20239 0.486744233767
-3.1979 0.486449231668
-3.19341 0.486153144714
-3.18892 0.485855970053
-3.18443 0.485557704835
-3.17994 0.485258346207
-3.17545 0.484957891317
-3.17096 0.484656337313
-3.16647 0.484353681344
-3.16198 0.484049920555
-3.15749 0.483745052096
-3.153 0.483439073113
-3.14851 0.483131980754
-3.14402 0.482823772166
-3.13953 0.482514444498
-3.13504 0.482203994897
-3.13055 0.481892420511
-3.12606 0.481579718489
-3.12157 0.48126588598
-3.11708 0.480950920133
-3.11259 0.480634818098
-3.1081 0.480317577024
-3.10361 0.479999194064
-3.09912 0.479679666367
-3.09463 0.479358991087
-3.09014 0.479037165376
-3.08565 0.478714186388
-3.08116 0.478390051277
-3.07667 0.478064757199
-3.07218 0.477738301309
-3.06769 0.477410680766
-3.0632 0.477081892728
-3.05871 0.476751934354
-3.05422 0.476420802805
-3.04973 0.476088495243
-3.04524 0.475755008831
-3.04075 0.475420340734
-3.03626 0.475084488117
-3.03177 0.474747448149
-3.02728 0.474409217998
-3.02279 0.474069794834
-3.0183 0.47372917583
-3.01381 0.47338735816
-3.00932 0.473044338999
-3.00483 0.472700115525
-3.00034 0.472354684917
-2.99585 0.472008044357
-2.99136 0.471660191027
-2.98687 0.471311122112
-2.98238 0.470960834801
-2.97789 0.470609326282
-2.9734 0.470256593748
-2.96891 0.469902634393
-2.96442 0.469547445412
-2.95993 0.469191024005
-2.95544 0.468833367373
-2.95095 0.468474472719
-2.94646 0.468114337251
-2.94197 0.467752958177
-2.93748 0.467390332708
-2.93299 0.46702645806
-2.9285 0.46666133145
-2.92401 0.466294950097
-2.91952 0.465927311226
-2.91503 0.465558412061
-2.91054 0.465188249834
-2.90605 0.464816821775
-2.90156 0.46444412512
-2.89707 0.464070157109
-2.89258 0.463694914984
-2.88809 0.46331839599
-2.8836 0.462940597375
-2.87911 0.462561516394
-2.87462 0.462181150302
-2.87013 0.461799496358
-2.86564 0.461416551827
-2.86115 0.461032313974
-2.85666 0.460646780073
-2.85217 0.460259947397
-2.84768 0.459871813225
-2.84319 0.45948237484
-2.8387 0.45909162953
-2.83421 0.458699574586
-2.82972 0.458306207302
-2.82523 0.45791152498
-2.82074 0.457515524922
-2.81625 0.457118204437
-2.81176 0.456719560838
-2.80727 0.456319591442
-2.80278 0.455918293573
-2.79829 0.455515664555
-2.7938 0.455111701721
-2.78931 0.454706402407
-2.78482 0.454299763954
-2.78033 0.453891783709
-2.77584 0.453482459021
-2.77135 0.453071787247
-2.76686 0.452659765749
-2.76237 0.452246391893
-2.75788 0.45183166305
-2.75339 0.451415576597
-2.7489 0.450998129917
-2.74441 0.450579320398
-2.73992 0.450159145432
-2.73543 0.449737602419
-2.73094 0.449314688763
-2.72645 0.448890401875
-2.72196 0.44846473917
-2.71747 0.44803769807
-2.71298 0.447609276004
-2.70849 0.447179470404
-2.704 0.446748278711
-2.69951 0.446315698371
-2.69502 0.445881726835
-2.69053 0.445446361562
-2.68604 0.445009600017
-2.68155 0.444571439671
-2.67706 0.444131878
-2.67257 0.443690912489
-2.66808 0.443248540629
-2.66359 0.442804759917
-2.6591 0.442359567856
-2.65461 0.441912961957
-2.65012 0.441464939738
-2.64563 0.441015498723
-2.64114 0.440564636443
-2.63665 0.440112350436
-2.63216 0.439658638249
-2.62767 0.439203497434
-2.62318 0.43874692555
-2.61869 0.438288920165
-2.6142 0.437829478853
-2.60971 0.437368599197
-2.60522 0.436906278786
-2.60073 0.436442515216
-2.59624 0.435977306093
-2.59175 0.435510649029
-2.58726 0.435042541644
-2.58277 0.434572981567
-2.57828 0.434101966432
-2.57379 0.433629493883
-2.5693 0.433155561574
-2.56481 0.432680167163
-2.56032 0.432203308318
-2.55583 0.431724982717
-2.55134 0.431245188044
-2.54685 0.430763921991
-2.54236 0.43028118226
-2.53787 0.429796966561
-2.53338 0.429311272613
-2.52889 0.428824098143
-2.5244 0.428335440885
-2.51991 0.427845298586
-2.51542 0.427353668999
-2.51093 0.426860549885
-2.50644 0.426365939016
-2.50195 0.425869834172
-2.49746 0.425372233142
-2.49297 0.424873133725
-2.48848 0.424372533729
-2.48399 0.423870430971
-2.4795 0.423366823277
-2.47501 0.422861708482
-2.47052 0.422355084432
-2.46603 0.421846948982
-2.46154 0.421337299996
-2.45705 0.420826135349
-2.45256 0.420313452923
-2.44807 0.419799250613
-2.44358 0.419283526323
-2.43909 0.418766277964
-2.4346 0.418247503462
-2.43011 0.41772720075
-2.42562 0.41720536777
-2.42113 0.416682002478
-2.41664 0.416157102837
-2.41215 0.415630666822
-2.40766 0.415102692418
-2.40317 0.414573177619
-2.39868 0.414042120432
-2.39419 0.413509518874
-2.3897 0.412975370971
-2.38521 0.412439674761
-2.38072 0.411902428294
-2.37623 0.411363629628
-2.37174 0.410823276833
-2.36725 0.410281367993
-2.36276 0.409737901198
-2.35827 0.409192874553
-2.35378 0.408646286172
-2.34929 0.408098134182
-2.3448 0.407548416719
-2.34031 0.406997131933
-2.33582 0.406444277985
-2.33133 0.405889853045
-2.32684 0.405333855297
-2.32235 0.404776282936
-2.31786 0.404217134169
-2.31337 0.403656407215
-2.30888 0.403094100304
-2.30439 0.402530211677
-2.2999 0.401964739591
-2.29541 0.40139768231
-2.29092 0.400829038113
-2.28643 0.400258805292
-2.28194 0.399686982149
-2.27745 0.399113566999
-2.27296 0.398538558171
-2.26847 0.397961954003
-2.26398 0.39738375285
-2.25949 0.396803953076
-2.255 0.39622255306
-2.25051 0.395639551191
-2.24602 0.395054945874
-2.24153 0.394468735525
-2.23704 0.393880918574
-2.23255 0.393291493462
-2.22806 0.392700458646
-2.22357 0.392107812594
-2.21908 0.391513553789
-2.21459 0.390917680724
-2.2101 0.390320191909
-2.20561 0.389721085866
-2.20112 0.389120361131
-2.19663 0.388518016253
-2.19214 0.387914049794
-2.18765 0.387308460332
-2.18316 0.386701246457
-2.17867 0.386092406773
-2.17418 0.385481939898
-2.16969 0.384869844466
-2.1652 0.384256119122
-2.16071 0.383640762527
-2.15622 0.383023773357
-2.15173 0.3824051503
-2.14724 0.381784892061
-2.14275 0.381162997358
-2.13826 0.380539464923
-2.13377 0.379914293506
-2.12928 0.379287481867
-2.12479 0.378659028784
-2.1203 0.37802893305
-2.11581 0.377397193472
-2.11132 0.376763808871
-2.10683 0.376128778086
-2.10234 0.375492099969
-2.09785 0.374853773389
-2.09336 0.374213797228
-2.08887 0.373572170387
-2.08438 0.372928891779
-2.07989 0.372283960335
-2.0754 0.371637375003
-2.07091 0.370989134742
-2.06642 0.370339238533
-2.06193 0.369687685369
-2.05744 0.36903447426
-2.05295 0.368379604233
-2.04846 0.367723074332
-2.04397 0.367064883616
-2.03948 0.366405031161
-2.03499 0.365743516059
-2.0305 0.365080337422
-2.02601 0.364415494374
-2.02152 0.36374898606
-2.01703 0.36308081164
-2.01254 0.362410970292
-2.00805 0.361739461212
-2.00356 0.361066283611
-1.99907 0.36039143672
-1.99458 0.359714919787
-1.99009 0.359036732077
-1.9856 0.358356872874
-1.98111 0.357675341479
-1.97662 0.356992137212
-1.97213 0.356307259411
-1.96764 0.355620707432
-1.96315 0.35493248065
-1.95866 0.354242578458
-1.95417 0.353551000268
-1.94968 0.352857745512
-1.94519 0.35216281364
-1.9407 0.351466204121
-1.93621 0.350767916444
-1.93172 0.350067950116
-1.92723 0.349366304666
-1.92274 0.348662979641
-1.91825 0.347957974608
-1.91376 0.347251289156
-1.90927 0.34654292289
-1.90478 0.34583287544
-1.90029 0.345121146454
-1.8958 0.3444077356
-1.89131 0.34369264257
-1.88682 0.342975867073
-1.88233 0.342257408842
-1.87784 0.341537267631
-1.87335 0.340815443215
-1.86886 0.340091935389
-1.86437 0.339366743974
-1.85988 0.338639868809
-1.85539 0.337911309758
-1.8509 0.337181066706
-1.84641 0.33644913956
-1.84192 0.335715528252
-1.83743 0.334980232735
-1.83294 0.334243252987
-1.82845 0.333504589008
-1.82396 0.332764240822
-1.81947 0.332022208477
-1.81498 0.331278492045
-1.81049 0.330533091623
-1.806 0.329786007332
-1.80151 0.329037239317
-1.79702 0.328286787749
-1.79253 0.327534652824
-1.78804 0.326780834763
-1.78355 0.326025333814
-1.77906 0.325268150249
-1.77457 0.324509284368
-1.77008 0.323748736497
-1.76559 0.322986506988
-1.7611 0.322222596221
-1.75661 0.321457004602
-1.75212 0.320689732567
-1.74763 0.319920780577
-1.74314 0.319150149123
-1.73865 0.318377838723
-1.73416 0.317603849926
-1.72967 0.316828183309
-1.72518 0.316050839476
-1.72069 0.315271819064
-1.7162 0.314491122738
-1.71171 0.313708751195
-1.70722 0.312924705161
-1.70273 0.312138985394
-1.69824 0.311351592683
-1.69375 0.310562527847
-1.68926 0.309771791741
-1.68477 0.308979385249
-1.68028 0.308185309288
-1.67579 0.307389564811
-1.6713 0.306592152801
-1.66681 0.305793074277
-1.66232 0.304992330291
-1.65783 0.304189921931
-1.65334 0.303385850319
-1.64885 0.302580116614
-1.64436 0.30177272201
-1.63987 0.300963667737
-1.63538 0.300152955061
-1.63089 0.299340585289
-1.6264 0.298526559762
-1.62191 0.29771087986
-1.61742 0.296893547002
-1.61293 0.296074562648
-1.60844 0.295253928294
-1.60395 0.294431645478
-1.59946 0.29360771578
-1.59497 0.292782140818
-1.59048 0.291954922255
-1.58599 0.291126061793
-1.5815 0.290295561178
-1.57701 0.289463422201
-1.57252 0.288629646695
-1.56803 0.287794236536
-1.56354 0.286957193648
-1.55905 0.286118519999
-1.55456 0.285278217603
-1.55007 0.28443628852
-1.54558 0.28359273486
-1.54109 0.282747558777
-1.5366 0.281900762478
-1.53211 0.281052348215
-1.52762 0.280202318293
-1.52313 0.279350675067
-1.51864 0.278497420941
-1.51415 0.277642558373
-1.50966 0.276786089874
-1.50517 0.275928018006
-1.50068 0.275068345388
-1.49619 0.27420707469
-1.4917 0.273344208642
-1.48721 0.272479750026
-1.48272 0.271613701684
-1.47823 0.270746066514
-1.47374 0.269876847474
-1.46925 0.26900604758
-1.46476 0.268133669908
-1.46027 0.267259717597
-1.45578 0.266384193846
-1.45129 0.265507101917
-1.4468 0.264628445136
-1.44231 0.263748226894
-1.43782 0.262866450645
-1.43333 0.261983119913
-1.42884 0.261098238285
-1.42435 0.260211809418
-1.41986 0.25932383704
-1.41537 0.258434324945
-1.41088 0.257543277
-1.40639 0.256650697145
-1.4019 0.255756589391
-1.39741 0.254860957825
-1.39292 0.253963806605
-1.38843 0.253065139971
-1.38394 0.252164962234
-1.37945 0.251263277787
-1.37496 0.250360091102
-1.37047 0.24945540673
-1.36598 0.248549229304
-1.36149 0.247641563539
-1.357 0.246732414235
-1.35251 0.245821786277
-1.34802 0.244909684635
-1.34353 0.243996114366
-1.33904 0.243081080617
-1.33455 0.242164588625
-1.33006 0.241246643716
-1.32557 0.240327251309
-1.32108 0.239406416919
-1.31659 0.238484146152
-1.3121 0.237560444713
-1.30761 0.236635318404
-1.30312 0.235708773124
-1.29863 0.234780814876
-1.29414 0.233851449762
-1.28965 0.232920683986
-1.28516 0.23198852386
-1.28067 0.231054975799
-1.27618 0.230120046327
-1.27169 0.229183742076
-1.2672 0.228246069789
-1.26271 0.227307036321
-1.25822 0.22636664864
-1.25373 0.225424913829
-1.24924 0.224481839088
-1.24475 0.223537431735
-1.24026 0.222591699208
-1.23577 0.221644649066
-1.23128 0.220696288991
-1.22679 0.219746626791
-1.2223 0.218795670399
-1.21781 0.217843427877
-1.21332 0.216889907417
-1.20883 0.215935117343
-1.20434 0.214979066112
-1.19985 0.214021762314
-1.19536 0.213063214681
-1.19087 0.212103432081
-1.18638 0.211142423521
-1.18189 0.210180198155
-1.1774 0.209216765278
-1.17291 0.208252134333
-1.16842 0.207286314911
-1.16393 0.206319316755
-1.15944 0.205351149758
-1.15495 0.204381823968
-1.15046 0.20341134959
-1.14597 0.202439736988
-1.14148 0.201466996686
-1.13699 0.200493139369
-1.1325 0.19951817589
-1.12801 0.198542117267
-1.12352 0.197564974686
-1.11903 0.196586759507
-1.11454 0.195607483261
-1.11005 0.194627157656
-1.10556 0.193645794578
-1.10107 0.192663406091
-1.09658 0.191680004445
-1.09209 0.190695602072
-1.0876 0.189710211592
-1.08311 0.188723845815
-1.07862 0.187736517743
-1.07413 0.18674824057
-1.06964 0.185759027689
-1.06515 0.184768892692
-1.06066 0.183777849372
-1.05617 0.182785911725
-1.05168 0.181793093956
-1.04719 0.180799410476
-1.0427 0.179804875911
-1.03821 0.178809505098
-1.03372 0.177813313095
-1.02923 0.176816315174
-1.02474 0.175818526833
-1.02025 0.174819963794
-1.01576 0.173820642006
-1.01127 0.172820577648
-1.00678 0.171819787132
-1.00229 0.170818287106
-0.9978 0.169816094454
-0.99331 0.168813226305
-0.98882 0.167809700029
-0.98433 0.166805533244
-0.97984 0.165800743816
-0.97535 0.164795349866
-0.97086 0.163789369769
-0.96637 0.162782822157
-0.96188 0.161775725925
-0.95739 0.160768100231
-0.9529 0.1597599645
-0.94841 0.158751338428
-0.94392 0.157742241984
-0.93943 0.156732695411
-0.93494 0.155722719233
-0.93045 0.154712334255
-0.92596 0.153701561569
-0.92147 0.152690422552
-0.91698 0.151678938876
-0.91249 0.150667132504
-0.908 0.149655025699
-0.90351 0.148642641024
-0.89902 0.147630001346
-0.89453 0.146617129837
-0.89004 0.145604049983
-0.88555 0.14459078558
-0.88106 0.143577360743
-0.87657 0.142563799906
-0.87208 0.141550127825
-0.86759 0.140536369584
-0.8631 0.139522550596
-0.85861 0.138508696607
-0.85412 0.1374948337
-0.84963 0.136480988295
-0.84514 0.135467187156
-0.84065 0.134453457396
-0.83616 0.133439826472
-0.83167 0.132426322199
-0.82718 0.131412972745
-0.82269 0.130399806637
-0.8182 0.129386852768
-0.81371 0.128374140394
-0.80922 0.127361699142
-0.80473 0.126349559011
-0.80024 0.125337750377
-0.79575 0.124326303997
-0.79126 0.123315251008
-0.78677 0.122304622935
-0.78228 0.121294451693
-0.77779 0.12028476959
-0.7733 0.119275609329
-0.76881 0.118267004017
-0.76432 0.117258987159
-0.75983 0.11625159267
-0.75534 0.115244854875
-0.75085 0.114238808511
-0.74636 0.113233488733
-0.74187 0.112228931114
-0.73738 0.111225171653
-0.73289 0.110222246776
-0.7284 0.109220193335
-0.72391 0.108219048621
-0.71942 0.107218850358
-0.71493 0.106219636711
-0.71044 0.105221446289
-0.70595 0.104224318147
-0.70146 0.103228291789
-0.69697 0.102233407174
-0.69248 0.101239704716
-0.68799 0.100247225289
-0.6835 0.0992560102288
-0.67901 0.0982661013386
-0.67452 0.0972775408896
-0.67003 0.0962903716253
-0.66554 0.0953046367645
-0.66105 0.0943203800042
-0.65656 0.0933376455228
-0.65207 0.092356477983
-0.64758 0.091376922535
-0.64309 0.0903990248191
-0.6386 0.0894228309689
-0.63411 0.0884483876142
-0.62962 0.0874757418838
-0.62513 0.086504941408
-0.62064 0.0855360343222
-0.61615 0.0845690692687
-0.61166 0.0836040954002
-0.60717 0.0826411623819
-0.60268 0.0816803203945
-0.59819 0.0807216201366
-0.5937 0.0797651128273
-0.58921 0.0788108502087
-0.58472 0.0778588845483
-0.58023 0.0769092686415
-0.57574 0.0759620558139
-0.57125 0.0750172999233
-0.56676 0.0740750553627
-0.56227 0.0731353770615
-0.55778 0.0721983204885
-0.55329 0.0712639416534
-0.5488 0.0703322971091
-0.54431 0.0694034439533
-0.53982 0.0684774398311
-0.53533 0.0675543429359
-0.53084 0.0666342120118
-0.52635 0.0657171063552
-0.52186 0.064803085816
-0.51737 0.0638922107996
-0.51288 0.0629845422683
-0.50839 0.0620801417423
-0.5039 0.0611790713017
-0.49941 0.0602813935869
-0.49492 0.0593871718006
-0.49043 0.0584964697081
-0.48594 0.0576093516388
-0.48145 0.0567258824871
-0.47696 0.0558461277128
-0.47247 0.0549701533423
-0.46798 0.0540980259688
-0.46349 0.0532298127531
-0.459 0.0523655814242
-0.45451 0.0515054002792
-0.45002 0.0506493381838
-0.44553 0.0497974645725
-0.44104 0.0489498494487
-0.43655 0.0481065633841
-0.43206 0.0472676775193
-0.42757 0.0464332635631
-0.42308 0.045603393792
-0.41859 0.0447781410499
-0.4141 0.0439575787477
-0.40961 0.0431417808621
-0.40512 0.0423308219349
-0.40063 0.0415247770723
-0.39614 0.0407237219435
-0.39165 0.0399277327796
-0.38716 0.0391368863723
-0.38267 0.0383512600723
-0.37818 0.0375709317879
-0.37369 0.0367959799832
-0.3692 0.0360264836761
-0.36471 0.0352625224363
-0.36022 0.0345041763835
-0.35573 0.0337515261847
-0.35124 0.0330046530522
-0.34675 0.0322636387407
-0.34226 0.0315285655448
-0.33777 0.0307995162958
-0.33328 0.0300765743594
-0.32879 0.0293598236319
-0.3243 0.0286493485373
-0.31981 0.0279452340234
-0.31532 0.0272475655589
-0.31083 0.026556429129
-0.30634 0.0258719112316
-0.30185 0.0251940988736
-0.29736 0.0245230795661
-0.29287 0.0238589413206
-0.28838 0.0232017726439
-0.28389 0.0225516625335
-0.2794 0.021908700473
-0.27491 0.0212729764265
-0.27042 0.0206445808338
-0.26593 0.0200236046047
-0.26144 0.0194101391137
-0.25695 0.0188042761937
-0.25246 0.0182061081307
-0.24797 0.017615727657
-0.24348 0.0170332279456
-0.23899 0.016458702603
-0.2345 0.015892245663
-0.23001 0.0153339515797
-0.22552 0.0147839152202
-0.22103 0.0142422318579
-0.21654 0.0137089971646
-0.21205 0.0131843072029
-0.20756 0.0126682584189
-0.20307 0.0121609476336
-0.19858 0.0116624720348
-0.19409 0.0111729291692
-0.1896 0.0106924169331
-0.18511 0.0102210335644
-0.18062 0.0097588776329
-0.17613 0.00930604803158
-0.17164 0.00886264396709
-0.16715 0.0084287649502
-0.16266 0.00800451078603
-0.15817 0.00758998156407
-0.15368 0.00718527764802
-0.14919 0.00679049966546
-0.1447 0.0064057484972
-0.14021 0.00603112526657
-0.13572 0.00566673132843
-0.13123 0.00531266825801
-0.12674 0.00496903783947
-0.12225 0.0046359420544
-0.11776 0.00431348306997
-0.11327 0.00400176322698
-0.10878 0.00370088502767
-0.10429 0.0034109511233
-0.0998 0.00313206430157
-0.09531 0.00286432747383
-0.09082 0.00260784366209
-0.08633 0.00236271598578
-0.08184 0.0021290476484
-0.07735 0.00190694192387
-0.07286 0.00169650214277
-0.06837 0.00149783167832
-0.06388 0.00131103393219
-0.05939 0.00113621232009
-0.0549 0.000973470257211
-0.05041 0.000822911143396
-0.04592 0.000684638348192
-0.04143 0.000558755195664
-0.03694 0.000445364949028
-0.03245 0.000344570795099
-0.02796 0.000256475828546
-0.02347 0.000181183035956
-0.01898 0.000118795279714
-0.01449 6.94152817088e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceLevelSets.tex <==
-4.5 0.555464043873
-4.49551 0.555462979559
-4.49102 0.555461903038
-4.48653 0.555460814172
-4.48204 0.555459712821
-4.47755 0.555458598844
-4.47306 0.555457472101
-4.46857 0.555456332446
-4.46408 0.555455179734
-4.45959 0.555454013818
-4.4551 0.55545283455
-4.45061 0.555451641779
-4.44612 0.555450435353
-4.44163 0.555449215119
-4.43714 0.555447980922
-4.43265 0.555446732603
-4.42816 0.555445470005
-4.42367 0.555444192967
-4.41918 0.555442901326
-4.41469 0.555441594919
-4.4102 0.55544027358
-4.40571 0.555438937141
-4.40122 0.555437585432
-4.39673 0.555436218283
-4.39224 0.555434835519
-4.38775 0.555433436966
-4.38326 0.555432022447
-4.37877 0.555430591782
-4.37428 0.555429144791
-4.36979 0.55542768129
-4.3653 0.555426201095
-4.36081 0.555424704019
-4.35632 0.555423189872
-4.35183 0.555421658463
-4.34734 0.5554201096
-4.34285 0.555418543086
-4.33836 0.555416958725
-4.33387 0.555415356316
-4.32938 0.555413735658
-4.32489 0.555412096547
-4.3204 0.555410438777
-4.31591 0.555408762139
-4.31142 0.555407066422
-4.30693 0.555405351413
-4.30244 0.555403616897
-4.29795 0.555401862656
-4.29346 0.555400088471
-4.28897 0.555398294117
-4.28448 0.555396479372
-4.27999 0.555394644006
-4.2755 0.55539278779
-4.27101 0.555390910493
-4.26652 0.555389011878
-4.26203 0.555387091709
-4.25754 0.555385149745
-4.25305 0.555383185745
-4.24856 0.555381199461
-4.24407 0.555379190648
-4.23958 0.555377159053
-4.23509 0.555375104424
-4.2306 0.555373026504
-4.22611 0.555370925035
-4.22162 0.555368799755
-4.21713 0.555366650399
-4.21264 0.5553644767
-4.20815 0.555362278388
-4.20366 0.55536005519
-4.19917 0.555357806828
-4.19468 0.555355533025
-4.19019 0.555353233498
-4.1857 0.555350907962
-4.18121 0.555348556128
-4.17672 0.555346177705
-4.17223 0.555343772398
-4.16774 0.55534133991
-4.16325 0.55533887994
-4.15876 0.555336392183
-4.15427 0.555333876332
-4.14978 0.555331332077
-4.14529 0.555328759102
-4.1408 0.555326157091
-4.13631 0.555323525723
-4.13182 0.555320864672
-4.12733 0.555318173612
-4.12284 0.55531545221
-4.11835 0.555312700132
-4.11386 0.555309917039
-4.10937 0.555307102589
-4.10488 0.555304256436
-4.10039 0.555301378231
-4.0959 0.555298467619
-4.09141 0.555295524244
-4.08692 0.555292547745
-4.08243 0.555289537757
-4.07794 0.55528649391
-4.07345 0.555283415834
-4.06896 0.555280303149
-4.06447 0.555277155477
-4.05998 0.555273972432
-4.05549 0.555270753625
-4.051 0.555267498663
-4.04651 0.555264207148
-4.04202 0.55526087868
-4.03753 0.555257512852
-4.03304 0.555254109254
-4.02855 0.555250667471
-4.02406 0.555247187086
-4.01957 0.555243667673
-4.01508 0.555240108806
-4.01059 0.555236510051
-4.0061 0.555232870972
-4.00161 0.555229191127
-3.99712 0.555225470069
-3.99263 0.555221707347
-3.98814 0.555217902505
-3.98365 0.555214055083
-3.97916 0.555210164614
-3.97467 0.555206230628
-3.97018 0.555202252649
-3.96569 0.555198230197
-3.9612 0.555194162785
-3.95671 0.555190049922
-3.95222 0.555185891113
-3.94773 0.555181685856
-3.94324 0.555177433644
-3.93875 0.555173133965
-3.93426 0.555168786302
-3.92977 0.555164390131
-3.92528 0.555159944924
-3.92079 0.555155450147
-3.9163 0.55515090526
-3.91181 0.555146309718
-3.90732 0.555141662969
-3.90283 0.555136964456
-3.89834 0.555132213617
-3.89385 0.555127409883
-3.88936 0.555122552679
-3.88487 0.555117641424
-3.88038 0.55511267553
-3.87589 0.555107654406
-3.8714 0.555102577451
-3.86691 0.55509744406
-3.86242 0.555092253621
-3.85793 0.555087005515
-3.85344 0.555081699118
-3.84895 0.555076333797
-3.84446 0.555070908915
-3.83997 0.555065423827
-3.83548 0.555059877882
-3.83099 0.55505427042
-3.8265 0.555048600777
-3.82201 0.55504286828
-3.81752 0.55503707225
-3.81303 0.555031212002
-3.80854 0.55502528684
-3.80405 0.555019296065
-3.79956 0.555013238968
-3.79507 0.555007114834
-3.79058 0.55500092294
-3.78609 0.554994662555
-3.7816 0.554988332942
-3.77711 0.554981933355
-3.77262 0.554975463039
-3.76813 0.554968921234
-3.76364 0.554962307171
-3.75915 0.554955620072
-3.75466 0.554948859152
-3.75017 0.554942023618
-3.74568 0.554935112667
-3.74119 0.554928125489
-3.7367 0.554921061268
-3.73221 0.554913919174
-3.72772 0.554906698373
-3.72323 0.554899398022
-3.71874 0.554892017266
-3.71425 0.554884555244
-3.70976 0.554877011087
-3.70527 0.554869383914
-3.70078 0.554861672836
-3.69629 0.554853876956
-3.6918 0.554845995367
-3.68731 0.554838027153
-3.68282 0.554829971387
-3.67833 0.554821827135
-3.67384 0.554813593451
-3.66935 0.554805269381
-3.66486 0.554796853959
-3.66037 0.554788346213
-3.65588 0.554779745157
-3.65139 0.554771049797
-3.6469 0.554762259128
-3.64241 0.554753372135
-3.63792 0.554744387793
-3.63343 0.554735305066
-3.62894 0.554726122907
-3.62445 0.554716840259
-3.61996 0.554707456054
-3.61547 0.554697969214
-3.61098 0.554688378648
-3.60649 0.554678683255
-3.602 0.554668881924
-3.59751 0.554658973529
-3.59302 0.554648956938
-3.58853 0.554638831001
-3.58404 0.554628594563
-3.57955 0.554618246451
-3.57506 0.554607785485
-3.57057 0.554597210471
-3.56608 0.554586520202
-3.56159 0.55457571346
-3.5571 0.554564789015
-3.55261 0.554553745623
-3.54812 0.554542582029
-3.54363 0.554531296964
-3.53914 0.554519889146
-3.53465 0.554508357283
-3.53016 0.554496700066
-3.52567 0.554484916176
-3.52118 0.554473004277
-3.51669 0.554460963023
-3.5122 0.554448791054
-3.50771 0.554436486994
-3.50322 0.554424049456
-3.49873 0.554411477037
-3.49424 0.55439876832
-3.48975 0.554385921875
-3.48526 0.554372936257
-3.48077 0.554359810006
-3.47628 0.554346541648
-3.47179 0.554333129695
-3.4673 0.554319572642
-3.46281 0.554305868971
-3.45832 0.554292017148
-3.45383 0.554278015622
-3.44934 0.55426386283
-3.44485 0.554249557191
-3.44036 0.554235097108
-3.43587 0.55422048097
-3.43138 0.554205707148
-3.42689 0.554190773997
-3.4224 0.554175679858
-3.41791 0.554160423052
-3.41342 0.554145001885
-3.40893 0.554129414648
-3.40444 0.554113659612
-3.39995 0.554097735032
-3.39546 0.554081639146
-3.39097 0.554065370175
-3.38648 0.55404892632
-3.38199 0.554032305768
-3.3775 0.554015506686
-3.37301 0.553998527222
-3.36852 0.553981365506
-3.36403 0.553964019653
-3.35954 0.553946487754
-3.35505 0.553928767885
-3.35056 0.553910858102
-3.34607 0.553892756442
-3.34158 0.553874460923
-3.33709 0.553855969542
-3.3326 0.553837280278
-3.32811 0.55381839109
-3.32362 0.553799299917
-3.31913 0.553780004677
-3.31464 0.553760503268
-3.31015 0.553740793568
-3.30566 0.553720873433
-3.30117 0.553700740701
-3.29668 0.553680393185
-3.29219 0.55365982868
-3.2877 0.553639044957
-3.28321 0.553618039767
-3.27872 0.553596810839
-3.27423 0.553575355878
-3.26974 0.553553672571
-3.26525 0.553531758577
-3.26076 0.553509611538
-3.25627 0.553487229068
-3.25178 0.553464608761
-3.24729 0.553441748187
-3.2428 0.553418644893
-3.23831 0.553395296401
-3.23382 0.553371700211
-3.22933 0.553347853798
-3.22484 0.553323754611
-3.22035 0.553299400078
-3.21586 0.553274787599
-3.21137 0.553249914551
-3.20688 0.553224778285
-3.20239 0.553199376127
-3.1979 0.553173705377
-3.19341 0.55314776331
-3.18892 0.553121547174
-3.18443 0.55309505419
-3.17994 0.553068281555
-3.17545 0.553041226437
-3.17096 0.553013885978
-3.16647 0.552986257293
-3.16198 0.552958337468
-3.15749 0.552930123564
-3.153 0.552901612612
-3.14851 0.552872801615
-3.14402 0.552843687548
-3.13953 0.552814267358
-3.13504 0.552784537962
-3.13055 0.552754496248
-3.12606 0.552724139076
-3.12157 0.552693463275
-3.11708 0.552662465644
-3.11259 0.552631142952
-3.1081 0.55259949194
-3.10361 0.552567509314
-3.09912 0.552535191752
-3.09463 0.552502535901
-3.09014 0.552469538375
-3.08565 0.552436195758
-3.08116 0.5524025046
-3.07667 0.552368461421
-3.07218 0.552334062707
-3.06769 0.552299304911
-3.0632 0.552264184455
-3.05871 0.552228697725
-3.05422 0.552192841076
-3.04973 0.552156610827
-3.04524 0.552120003264
-3.04075 0.552083014638
-3.03626 0.552045641167
-3.03177 0.552007879031
-3.02728 0.551969724376
-3.02279 0.551931173315
-3.0183 0.551892221921
-3.01381 0.551852866233
-3.00932 0.551813102254
-3.00483 0.551772925949
-3.00034 0.551732333247
-2.99585 0.551691320039
-2.99136 0.551649882179
-2.98687 0.551608015481
-2.98238 0.551565715724
-2.97789 0.551522978646
-2.9734 0.551479799947
-2.96891 0.551436175288
-2.96442 0.55139210029
-2.95993 0.551347570535
-2.95544 0.551302581564
-2.95095 0.551257128878
-2.94646 0.551211207936
-2.94197 0.551164814159
-2.93748 0.551117942924
-2.93299 0.551070589566
-2.9285 0.55102274938
-2.92401 0.550974417617
-2.91952 0.550925589486
-2.91503 0.550876260152
-2.91054 0.550826424739
-2.90605 0.550776078324
-2.90156 0.550725215943
-2.89707 0.550673832584
-2.89258 0.550621923195
-2.88809 0.550569482676
-2.8836 0.55051650588
-2.87911 0.550462987618
-2.87462 0.550408922653
-2.87013 0.550354305701
-2.86564 0.550299131431
-2.86115 0.550243394468
-2.85666 0.550187089385
-2.85217 0.550130210709
-2.84768 0.550072752921
-2.84319 0.55001471045
-2.8387 0.549956077677
-2.83421 0.549896848935
-2.82972 0.549837018505
-2.82523 0.54977658062
-2.82074 0.549715529463
-2.81625 0.549653859163
-2.81176 0.549591563801
-2.80727 0.549528637404
-2.80278 0.54946507395
-2.79829 0.549400867362
-2.7938 0.549336011512
-2.78931 0.549270500217
-2.78482 0.549204327243
-2.78033 0.5491374863
-2.77584 0.549069971045
-2.77135 0.549001775081
-2.76686 0.548932891953
-2.76237 0.548863315155
-2.75788 0.548793038122
-2.75339 0.548722054233
-2.7489 0.548650356812
-2.74441 0.548577939126
-2.73992 0.548504794381
-2.73543 0.548430915731
-2.73094 0.548356296267
-2.72645 0.548280929025
-2.72196 0.548204806978
-2.71747 0.548127923044
-2.71298 0.548050270078
-2.70849 0.547971840876
-2.704 0.547892628175
-2.69951 0.547812624647
-2.69502 0.547731822906
-2.69053 0.547650215503
-2.68604 0.547567794927
-2.68155 0.547484553604
-2.67706 0.547400483897
-2.67257 0.547315578105
-2.66808 0.547229828465
-2.66359 0.547143227148
-2.6591 0.547055766259
-2.65461 0.546967437841
-2.65012 0.54687823387
-2.64563 0.546788146254
-2.64114 0.546697166838
-2.63665 0.546605287398
-2.63216 0.546512499643
-2.62767 0.546418795213
-2.62318 0.546324165684
-2.61869 0.546228602558
-2.6142 0.546132097273
-2.60971 0.546034641193
-2.60522 0.545936225616
-2.60073 0.545836841767
-2.59624 0.545736480802
-2.59175 0.545635133805
-2.58726 0.545532791788
-2.58277 0.545429445692
-2.57828 0.545325086384
-2.57379 0.545219704661
-2.5693 0.545113291243
-2.56481 0.545005836779
-2.56032 0.544897331843
-2.55583 0.544787766933
-2.55134 0.544677132474
-2.54685 0.544565418815
-2.54236 0.544452616228
-2.53787 0.544338714909
-2.53338 0.544223704978
-2.52889 0.544107576477
-2.5244 0.543990319371
-2.51991 0.543871923546
-2.51542 0.54375237881
-2.51093 0.543631674892
-2.50644 0.543509801441
-2.50195 0.543386748027
-2.49746 0.54326250414
-2.49297 0.543137059188
-2.48848 0.543010402499
-2.48399 0.542882523318
-2.4795 0.54275341081
-2.47501 0.542623054057
-2.47052 0.542491442056
-2.46603 0.542358563723
-2.46154 0.54222440789
-2.45705 0.542088963306
-2.45256 0.541952218631
-2.44807 0.541814162446
-2.44358 0.541674783241
-2.43909 0.541534069425
-2.4346 0.541392009318
-2.43011 0.541248591154
-2.42562 0.54110380308
-2.42113 0.540957633155
-2.41664 0.54081006935
-2.41215 0.540661099551
-2.40766 0.54051071155
-2.40317 0.540358893053
-2.39868 0.540205631676
-2.39419 0.540050914947
-2.3897 0.539894730299
-2.38521 0.539737065079
-2.38072 0.539577906541
-2.37623 0.539417241847
-2.37174 0.539255058067
-2.36725 0.539091342181
-2.36276 0.538926081075
-2.35827 0.53875926154
-2.35378 0.538590870277
-2.34929 0.538420893891
-2.3448 0.538249318894
-2.34031 0.538076131704
-2.33582 0.537901318642
-2.33133 0.537724865935
-2.32684 0.537546759716
-2.32235 0.537366986019
-2.31786 0.537185530785
-2.31337 0.537002379855
-2.30888 0.536817518977
-2.30439 0.536630933798
-2.2999 0.536442609869
-2.29541 0.536252532645
-2.29092 0.536060687479
-2.28643 0.535867059628
-2.28194 0.535671634251
-2.27745 0.535474396404
-2.27296 0.535275331047
-2.26847 0.535074423039
-2.26398 0.534871657139
-2.25949 0.534667018007
-2.255 0.5344604902
-2.25051 0.534252058176
-2.24602 0.53404170629
-2.24153 0.533829418799
-2.23704 0.533615179855
-2.23255 0.53339897351
-2.22806 0.533180783712
-2.22357 0.532960594309
-2.21908 0.532738389046
-2.21459 0.532514151563
-2.2101 0.532287865399
-2.20561 0.53205951399
-2.20112 0.531829080667
-2.19663 0.53159654866
-2.19214 0.531361901092
-2.18765 0.531125120985
-2.18316 0.530886191255
-2.17867 0.530645094715
-2.17418 0.530401814072
-2.16969 0.53015633193
-2.1652 0.529908630789
-2.16071 0.529658693041
-2.15622 0.529406500977
-2.15173 0.52915203678
-2.14724 0.528895282531
-2.14275 0.528636220202
-2.13826 0.528374831663
-2.13377 0.528111098678
-2.12928 0.527845002905
-2.12479 0.527576525896
-2.1203 0.5273056491
-2.11581 0.527032353859
-2.11132 0.526756621409
-2.10683 0.526478432882
-2.10234 0.526197769305
-2.09785 0.525914611597
-2.09336 0.525628940575
-2.08887 0.525340736948
-2.08438 0.525049981322
-2.07989 0.524756654198
-2.0754 0.524460735969
-2.07091 0.524162206927
-2.06642 0.523861047257
-2.06193 0.523557237039
-2.05744 0.52325075625
-2.05295 0.522941584763
-2.04846 0.522629702345
-2.04397 0.522315088661
-2.03948 0.521997723271
-2.03499 0.521677585631
-2.0305 0.521354655096
-2.02601 0.521028910916
-2.02152 0.520700332239
-2.01703 0.520368898111
-2.01254 0.520034587475
-2.00805 0.519697379173
-2.00356 0.519357251946
-1.99907 0.519014184431
-1.99458 0.518668155167
-1.99009 0.518319142593
-1.9856 0.517967125046
-1.98111 0.517612080764
-1.97662 0.517253987888
-1.97213 0.516892824458
-1.96764 0.516528568417
-1.96315 0.516161197609
-1.95866 0.515790689783
-1.95417 0.51541702259
-1.94968 0.515040173586
-1.94519 0.51466012023
-1.9407 0.514276839888
-1.93621 0.513890309831
-1.93172 0.513500507235
-1.92723 0.513107409186
-1.92274 0.512710992676
-1.91825 0.512311234606
-1.91376 0.511908111787
-1.90927 0.511501600937
-1.90478 0.511091678688
-1.90029 0.510678321584
-1.8958 0.510261506078
-1.89131 0.509841208539
-1.88682 0.509417405249
-1.88233 0.508990072407
-1.87784 0.508559186124
-1.87335 0.508124722433
-1.86886 0.50768665728
-1.86437 0.507244966534
-1.85988 0.506799625981
-1.85539 0.506350611329
-1.8509 0.505897898209
-1.84641 0.505441462174
-1.84192 0.504981278702
-1.83743 0.504517323196
-1.83294 0.504049570985
-1.82845 0.503577997328
-1.82396 0.503102577411
-1.81947 0.502623286352
-1.81498 0.5021400992
-1.81049 0.501652990936
-1.806 0.501161936478
-1.80151 0.500666910678
-1.79702 0.500167888326
-1.79253 0.49966484415
-1.78804 0.499157752818
-1.78355 0.498646588942
-1.77906 0.498131327074
-1.77457 0.497611941714
-1.77008 0.497088407307
-1.76559 0.496560698246
-1.7611 0.496028788874
-1.75661 0.495492653486
-1.75212 0.494952266331
-1.74763 0.494407601611
-1.74314 0.493858633488
-1.73865 0.493305336079
-1.73416 0.492747683465
-1.72967 0.492185649689
-1.72518 0.491619208758
-1.72069 0.491048334645
-1.7162 0.490473001293
-1.71171 0.489893182615
-1.70722 0.489308852499
-1.70273 0.488719984804
-1.69824 0.488126553369
-1.69375 0.487528532014
-1.68926 0.486925894536
-1.68477 0.48631861472
-1.68028 0.485706666337
-1.67579 0.485090023145
-1.6713 0.484468658895
-1.66681 0.483842547332
-1.66232 0.483211662194
-1.65783 0.482575977222
-1.65334 0.481935466156
-1.64885 0.481290102741
-1.64436 0.480639860727
-1.63987 0.479984713877
-1.63538 0.479324635962
-1.63089 0.478659600771
-1.6264 0.477989582111
-1.62191 0.477314553807
-1.61742 0.47663448971
-1.61293 0.475949363698
-1.60844 0.475259149677
-1.60395 0.474563821588
-1.59946 0.473863353406
-1.59497 0.473157719147
-1.59048 0.472446892868
-1.58599 0.471730848671
-1.5815 0.471009560709
-1.57701 0.470283003187
-1.57252 0.469551150363
-1.56803 0.468813976558
-1.56354 0.468071456153
-1.55905 0.467323563597
-1.55456 0.466570273406
-1.55007 0.465811560174
-1.54558 0.465047398567
-1.54109 0.464277763336
-1.5366 0.463502629315
-1.53211 0.462721971426
-1.52762 0.461935764684
-1.52313 0.461143984202
-1.51864 0.460346605191
-1.51415 0.459543602968
-1.50966 0.458734952957
-1.50517 0.457920630696
-1.50068 0.457100611839
-1.49619 0.456274872163
-1.4917 0.455443387568
-1.48721 0.454606134086
-1.48272 0.453763087881
-1.47823 0.452914225256
-1.47374 0.45205952266
-1.46925 0.451198956687
-1.46476 0.450332504084
-1.46027 0.449460141755
-1.45578 0.448581846766
-1.45129 0.447697596349
-1.4468 0.446807367908
-1.44231 0.445911139024
-1.43782 0.445008887458
-1.43333 0.444100591157
-1.42884 0.44318622826
-1.42435 0.442265777102
-1.41986 0.44133921622
-1.41537 0.440406524357
-1.41088 0.439467680468
-1.40639 0.438522663726
-1.4019 0.437571453527
-1.39741 0.436614029493
-1.39292 0.435650371482
-1.38843 0.434680459589
-1.38394 0.433704274156
-1.37945 0.432721795773
-1.37496 0.431733005288
-1.37047 0.430737883809
-1.36598 0.429736412714
-1.36149 0.428728573651
-1.357 0.42771434855
-1.35251 0.426693719627
-1.34802 0.425666669386
-1.34353 0.424633180632
-1.33904 0.423593236471
-1.33455 0.422546820321
-1.33006 0.421493915914
-1.32557 0.420434507304
-1.32108 0.419368578877
-1.31659 0.41829611535
-1.3121 0.417217101783
-1.30761 0.416131523585
-1.30312 0.415039366519
-1.29863 0.413940616707
-1.29414 0.412835260642
-1.28965 0.41172328519
-1.28516 0.410604677598
-1.28067 0.4094794255
-1.27618 0.408347516929
-1.27169 0.407208940314
-1.2672 0.406063684498
-1.26271 0.404911738737
-1.25822 0.403753092711
-1.25373 0.402587736529
-1.24924 0.401415660737
-1.24475 0.400236856327
-1.24026 0.399051314742
-1.23577 0.397859027882
-1.23128 0.396659988116
-1.22679 0.395454188285
-1.2223 0.394241621711
-1.21781 0.393022282205
-1.21332 0.391796164075
-1.20883 0.390563262131
-1.20434 0.389323571695
-1.19985 0.388077088608
-1.19536 0.386823809237
-1.19087 0.385563730486
-1.18638 0.384296849797
-1.18189 0.383023165165
-1.1774 0.381742675142
-1.17291 0.380455378846
-1.16842 0.379161275968
-1.16393 0.377860366781
-1.15944 0.376552652149
-1.15495 0.375238133531
-1.15046 0.373916812996
-1.14597 0.372588693222
-1.14148 0.371253777512
-1.13699 0.3699120698
-1.1325 0.368563574657
-1.12801 0.367208297301
-1.12352 0.365846243606
-1.11903 0.364477420107
-1.11454 0.363101834015
-1.11005 0.361719493216
-1.10556 0.360330406289
-1.10107 0.358934582507
-1.09658 0.357532031849
-1.09209 0.356122765009
-1.0876 0.354706793402
-1.08311 0.353284129174
-1.07862 0.351854785211
-1.07413 0.350418775146
-1.06964 0.34897611337
-1.06515 0.347526815038
-1.06066 0.346070896077
-1.05617 0.3446083732
-1.05168 0.343139263908
-1.04719 0.341663586502
-1.0427 0.340181360093
-1.03821 0.338692604606
-1.03372 0.337197340794
-1.02923 0.335695590242
-1.02474 0.33418737538
-1.02025 0.332672719489
-1.01576 0.331151646709
-1.01127 0.32962418205
-1.00678 0.328090351399
-1.00229 0.326550181531
-0.9978 0.325003700113
-0.99331 0.323450935719
-0.98882 0.321891917832
-0.98433 0.320326676859
-0.97984 0.318755244134
-0.97535 0.317177651932
-0.97086 0.315593933473
-0.96637 0.314004122934
-0.96188 0.312408255454
-0.95739 0.310806367146
-0.9529 0.309198495106
-0.94841 0.307584677417
-0.94392 0.305964953162
-0.93943 0.304339362431
-0.93494 0.302707946328
-0.93045 0.301070746983
-0.92596 0.299427807556
-0.92147 0.297779172249
-0.91698 0.296124886314
-0.91249 0.294464996058
-0.908 0.292799548855
-0.90351 0.291128593153
-0.89902 0.289452178482
-0.89453 0.287770355462
-0.89004 0.286083175811
-0.88555 0.284390692356
-0.88106 0.282692959035
-0.87657 0.280990030911
-0.87208 0.279281964177
-0.86759 0.277568816164
-0.8631 0.275850645349
-0.85861 0.274127511366
-0.85412 0.272399475006
-0.84963 0.270666598233
-0.84514 0.268928944187
-0.84065 0.267186577192
-0.83616 0.265439562765
-0.83167 0.263687967622
-0.82718 0.261931859687
-0.82269 0.260171308096
-0.8182 0.258406383207
-0.81371 0.256637156608
-0.80922 0.254863701121
-0.80473 0.253086090811
-0.80024 0.251304400993
-0.79575 0.249518708235
-0.79126 0.247729090373
-0.78677 0.245935626508
-0.78228 0.24413839702
-0.77779 0.24233748357
-0.7733 0.240532969108
-0.76881 0.23872493788
-0.76432 0.236913475432
-0.75983 0.235098668619
-0.75534 0.233280605608
-0.75085 0.231459375887
-0.74636 0.229635070266
-0.74187 0.227807780889
-0.73738 0.225977601235
-0.73289 0.224144626123
-0.7284 0.222308951721
-0.72391 0.22047067555
-0.71942 0.218629896486
-0.71493 0.216786714768
-0.71044 0.214941232004
-0.70595 0.213093551171
-0.70146 0.211243776624
-0.69697 0.209392014101
-0.69248 0.207538370721
-0.68799 0.205682954996
-0.6835 0.203825876832
-0.67901 0.20196724753
-0.67452 0.200107179795
-0.67003 0.198245787736
-0.66554 0.196383186872
-0.66105 0.194519494132
-0.65656 0.192654827864
-0.65207 0.190789307831
-0.64758 0.18892305522
-0.64309 0.187056192642
-0.6386 0.185188844135
-0.63411 0.183321135168
-0.62962 0.18145319264
-0.62513 0.179585144885
-0.62064 0.177717121676
-0.61615 0.175849254222
-0.61166 0.173981675172
-0.60717 0.172114518618
-0.60268 0.170247920096
-0.59819 0.168382016585
-0.5937 0.16651694651
-0.58921 0.164652849745
-0.58472 0.162789867608
-0.58023 0.160928142869
-0.57574 0.159067819743
-0.57125 0.157209043896
-0.56676 0.155351962444
-0.56227 0.15349672395
-0.55778 0.151643478426
-0.55329 0.149792377335
-0.5488 0.147943573586
-0.54431 0.146097221534
-0.53982 0.144253476982
-0.53533 0.142412497178
-0.53084 0.140574440814
-0.52635 0.138739468025
-0.52186 0.136907740384
-0.51737 0.135079420906
-0.51288 0.133254674041
-0.50839 0.131433665676
-0.5039 0.129616563129
-0.49941 0.127803535148
-0.49492 0.125994751909
-0.49043 0.12419038501
-0.48594 0.122390607473
-0.48145 0.120595593736
-0.47696 0.118805519653
-0.47247 0.117020562486
-0.46798 0.115240900908
-0.46349 0.11346671499
-0.459 0.111698186206
-0.45451 0.109935497421
-0.45002 0.108178832892
-0.44553 0.106428378259
-0.44104 0.104684320542
-0.43655 0.102946848137
-0.43206 0.101216150808
-0.42757 0.0994924196831
-0.42308 0.0977758472487
-0.41859 0.096066627343
-0.4141 0.0943649551501
-0.40961 0.0926710271938
-0.40512 0.0909850413314
-0.40063 0.0893071967462
-0.39614 0.0876376939416
-0.39165 0.0859767347334
-0.38716 0.0843245222427
-0.38267 0.0826812608889
-0.37818 0.0810471563812
-0.37369 0.079422415712
-0.3692 0.0778072471478
-0.36471 0.0762018602219
-0.36022 0.0746064657255
-0.35573 0.0730212756996
-0.35124 0.071446503426
-0.34675 0.0698823634185
-0.34226 0.0683290714142
-0.33777 0.0667868443638
-0.33328 0.0652559004222
-0.32879 0.0637364589396
-0.3243 0.0622287404508
-0.31981 0.0607329666661
-0.31532 0.0592493604607
-0.31083 0.0577781458646
-0.30634 0.0563195480525
-0.30185 0.0548737933324
-0.29736 0.0534411091358
-0.29287 0.0520217240062
-0.28838 0.050615867588
-0.28389 0.0492237706157
-0.2794 0.047845664902
-0.27491 0.0464817833265
-0.27042 0.0451323598242
-0.26593 0.043797629373
-0.26144 0.0424778279826
-0.25695 0.0411731926814
-0.25246 0.0398839615048
-0.24797 0.0386103734827
-0.24348 0.0373526686265
-0.23899 0.0361110879169
-0.2345 0.0348858732907
-0.23001 0.0336772676279
-0.22552 0.0324855147383
-0.22103 0.0313108593487
-0.21654 0.0301535470892
-0.21205 0.0290138244795
-0.20756 0.0278919389157
-0.20307 0.0267881386559
-0.19858 0.0257026728071
-0.19409 0.0246357913103
-0.1896 0.023587744927
-0.18511 0.0225587852247
-0.18062 0.0215491645626
-0.17613 0.020559136077
-0.17164 0.0195889536669
-0.16715 0.0186388719792
-0.16266 0.017709146394
-0.15817 0.0168000330096
-0.15368 0.0159117886279
-0.14919 0.0150446707386
-0.1447 0.0141989375048
-0.14021 0.0133748477476
-0.13572 0.0125726609302
-0.13123 0.0117926371433
-0.12674 0.0110350370892
-0.12225 0.0103001220662
-0.11776 0.00958815395302
-0.11327 0.00889939519339
-0.10878 0.00823410877986
-0.10429 0.00759255823822
-0.0998 0.00697500761153
-0.09531 0.00638172144422
-0.09082 0.00581296476607
-0.08633 0.00526900307614
-0.08184 0.0047501023267
-0.07735 0.00425652890705
-0.07286 0.00378854962737
-0.06837 0.00334643170247
-0.06388 0.00293044273552
-0.05939 0.00254085070176
-0.0549 0.00217792393218
-0.05041 0.00184193109715
-0.04592 0.00153314119005
-0.04143 0.00125182351088
-0.03694 0.000998247649787
-0.03245 0.000772683470709
-0.02796 0.000575401094871
-0.02347 0.00040667088435
-0.01898 0.000266763425611
-0.01449 0.000155949513046


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceMeanZero.tex <==
-4.5 0.157771599304
-4.49551 0.157688354544
-4.49102 0.15760515424
-4.48653 0.157813152836
-4.48204 0.157729587149
-4.47755 0.157646066144
-4.47306 0.157852950183
-4.46857 0.157769064199
-4.46408 0.157685223122
-4.45959 0.15760142699
-4.4551 0.157806783657
-4.45061 0.157722623139
-4.44612 0.157638507792
-4.44163 0.157842743529
-4.43714 0.157758264202
-4.43265 0.157673830271
-4.42816 0.157589441773
-4.42367 0.157792144362
-4.41918 0.157707392479
-4.41469 0.157622686254
-4.4102 0.157824261706
-4.40571 0.157739192506
-4.40122 0.157654169187
-4.39673 0.157854614364
-4.39224 0.157769228481
-4.38775 0.157683888701
-4.38326 0.157598595062
-4.37877 0.157797498572
-4.37428 0.157711842966
-4.36979 0.157626233722
-4.3653 0.157824000984
-4.36081 0.157738030186
-4.35632 0.157652105971
-4.35183 0.15784873396
-4.34734 0.157762448604
-4.34285 0.157676210052
-4.33836 0.157590018337
-4.33387 0.157785096497
-4.32938 0.15769854424
-4.32489 0.157612039039
-4.3204 0.157805972176
-4.31591 0.157719106846
-4.31142 0.157632288791
-4.30693 0.157825073984
-4.30244 0.157737896215
-4.29795 0.157650765936
-4.29346 0.1578424003
-4.28897 0.15775491072
-4.28448 0.157667468847
-4.27999 0.157580074712
-4.2755 0.157770148769
-4.27101 0.157682395929
-4.26652 0.15759469104
-4.26203 0.157783608795
-4.25754 0.157695545615
-4.25305 0.157607530598
-4.24856 0.157795289265
-4.24407 0.157706916368
-4.23958 0.157618591845
-4.23509 0.157805188668
-4.2306 0.157716506677
-4.22611 0.157627873268
-4.22162 0.157813305521
-4.21713 0.157724315055
-4.21264 0.157635373379
-4.20815 0.157819638368
-4.20366 0.157730340043
-4.19917 0.157641090713
-4.19468 0.157824185773
-4.19019 0.157734580203
-4.1857 0.157645023829
-4.18121 0.157826946325
-4.17672 0.157737034118
-4.17223 0.157647171309
-4.16774 0.157827918632
-4.16325 0.157737700394
-4.15876 0.157647531752
-4.15427 0.157827101322
-4.14978 0.157736577654
-4.14529 0.157646103779
-4.1408 0.157824493043
-4.13631 0.157733664542
-4.13182 0.157642886026
-4.12733 0.157820092458
-4.12284 0.157728959714
-4.11835 0.157637877147
-4.11386 0.157813898246
-4.10937 0.157722461845
-4.10488 0.15763107581
-4.10039 0.157805909099
-4.0959 0.157714169622
-4.09141 0.157622480694
-4.08692 0.157796123724
-4.08243 0.157704081742
-4.07794 0.157612090492
-4.07345 0.157784540835
-4.06896 0.157692196916
-4.06447 0.157599903907
-4.05998 0.157771159159
-4.05549 0.15767851386
-4.051 0.157585919648
-4.04651 0.157755977427
-4.04202 0.157663031301
-4.03753 0.157570136432
-4.03304 0.157738994378
-4.02855 0.157645747967
-4.02406 0.157552552982
-4.01957 0.157720208755
-4.01508 0.157626662594
-4.01059 0.15779351643
-4.0061 0.157699619304
-4.00161 0.157605773915
-3.99712 0.157771420764
-3.99263 0.157677224768
-3.98814 0.157583080668
-3.98365 0.15774751825
-3.97916 0.157653023893
-3.97467 0.157558581585
-3.97018 0.157721807639
-3.96569 0.157627015419
-3.9612 0.157789429612
-3.95671 0.15769428768
-3.95222 0.157599198082
-3.94773 0.157760396086
-3.94324 0.15766495711
-3.93875 0.15756957061
-3.93426 0.157729550216
-3.92977 0.157633814664
-3.92528 0.157792975153
-3.92079 0.157696890736
-3.9163 0.157600859059
-3.91181 0.157758796594
-3.90732 0.157662416367
-3.90283 0.157566089005
-3.89834 0.157722801422
-3.89385 0.157626125815
-3.88936 0.15778201202
-3.88487 0.157684988342
-3.88038 0.15758801777
-3.87589 0.157742674393
-3.8714 0.15764535604
-3.86691 0.157548090902
-3.86242 0.157701515819
-3.85793 0.15760390318
-3.85344 0.157756494938
-3.84895 0.157658534957
-3.84446 0.157560628404
-3.83997 0.157711984072
-3.83548 0.15761373044
-3.83099 0.157764248376
-3.8265 0.157665647814
-3.82201 0.157567100872
-3.81752 0.157716378384
-3.81303 0.157617484757
-3.80854 0.157765920022
-3.80405 0.157666679845
-3.79956 0.157567493463
-3.79507 0.157714684013
-3.79058 0.157615151306
-3.78609 0.157515672459
-3.7816 0.157661616238
-3.77711 0.157561791276
-3.77262 0.157706886149
-3.76813 0.157606715188
-3.76364 0.157750958939
-3.75915 0.157650442089
-3.75466 0.157549979314
-3.75017 0.15769296988
-3.74568 0.157592161394
-3.74119 0.157734296468
-3.7367 0.157633142367
-3.73221 0.157532042445
-3.72772 0.157672920143
-3.72323 0.157571474758
-3.71874 0.157711492638
-3.71425 0.157609701868
-3.70976 0.157507965356
-3.70527 0.15764672169
-3.70078 0.157544639917
-3.69629 0.157682532142
-3.6918 0.157580105171
-3.68731 0.157717131148
-3.68282 0.157614359033
-3.67833 0.157511641267
-3.67384 0.157647399423
-3.66935 0.157544336595
-3.66486 0.157679224262
-3.66037 0.157575816407
-3.65588 0.157709831474
-3.65139 0.157606078619
-3.6469 0.157502380144
-3.64241 0.15763512115
-3.63792 0.157531077711
-3.63343 0.157662941916
-3.62894 0.157558553519
-3.62445 0.157689538837
-3.61996 0.157584805477
-3.61547 0.157480126465
-3.61098 0.157609831494
-3.60649 0.157504807505
-3.602 0.157633629477
-3.59751 0.157528260484
-3.59302 0.15765619733
-3.58853 0.157550483295
-3.58404 0.157677532955
-3.57955 0.15757147383
-3.57506 0.157465468928
-3.57057 0.157591229978
-3.56608 0.1574848799
-3.56159 0.157609749622
-3.5571 0.157503054294
-3.55261 0.15762703064
-3.54812 0.157519989975
-3.54363 0.157643070905
-3.53914 0.157535684805
-3.53465 0.157657868281
-3.53016 0.157550136637
-3.52567 0.157442458906
-3.52118 0.157563343319
-3.51669 0.157455319859
-3.5122 0.157575302687
-3.50771 0.157466933357
-3.50322 0.15758601257
-3.49873 0.157477297217
-3.49424 0.157595470787
-3.48975 0.157486409243
-3.48526 0.157603675144
-3.48077 0.157494267231
-3.47628 0.157610623438
-3.47179 0.157500868962
-3.4673 0.157616313453
-3.46281 0.157506212205
-3.45832 0.157620742959
-3.45383 0.157510294717
-3.44934 0.157399899513
-3.44485 0.157513114239
-3.44036 0.157402371671
-3.43587 0.157514668497
-3.43138 0.157403578303
-3.42689 0.1575149552
-3.4224 0.157403517105
-3.41791 0.157513972044
-3.41342 0.157402185751
-3.40893 0.157511716701
-3.40444 0.157399581902
-3.39995 0.157508186829
-3.39546 0.157395703196
-3.39097 0.157503380065
-3.38648 0.157390547253
-3.38199 0.157497294025
-3.3775 0.157384111671
-3.37301 0.157489926302
-3.36852 0.157376394025
-3.36403 0.15748127447
-3.35954 0.15736739187
-3.35505 0.157471336077
-3.35056 0.157357102734
-3.34607 0.157460108647
-3.34158 0.157345524122
-3.33709 0.157447589678
-3.3326 0.157332653513
-3.32811 0.157433776644
-3.32362 0.157318488357
-3.31913 0.157418666988
-3.31464 0.157518301923
-3.31015 0.157402258126
-3.30566 0.157500944633
-3.30117 0.157384547446
-3.29668 0.157482283436
-3.29219 0.157365532303
-3.2877 0.157462315677
-3.28321 0.157345210021
-3.27872 0.157441038673
-3.27423 0.157323577892
-3.26974 0.157418449704
-3.26525 0.157300633173
-3.26076 0.157394546016
-3.25627 0.157276373085
-3.25178 0.157369324821
-3.24729 0.157461718344
-3.2428 0.157342783292
-3.23831 0.157434211721
-3.23382 0.157314918565
-3.22933 0.157405379735
-3.22484 0.157285727736
-3.22035 0.157375219469
-3.21586 0.157255207862
-3.21137 0.157343727966
-3.20688 0.157223355957
-3.20239 0.157310902224
-3.1979 0.157397879488
-3.19341 0.157276739199
-3.18892 0.157362738563
-3.18443 0.157241235801
-3.17994 0.157326255025
-3.17545 0.157204388895
-3.17096 0.157288425719
-3.16647 0.157371886426
-3.16198 0.157249247445
-3.15749 0.157331721626
-3.153 0.157208716951
-3.14851 0.157290202308
-3.14402 0.157166830936
-3.13953 0.15724732515
-3.13504 0.157327236117
-3.13055 0.157203086775
-3.12606 0.157282002399
-3.12157 0.157157483755
-3.11708 0.157235401668
-3.11259 0.157312731044
-3.1081 0.157187430417
-3.10361 0.157263757821
-3.09912 0.157138085079
-3.09463 0.157213408093
-3.09014 0.157087362029
-3.08565 0.157161678209
-3.08116 0.157235398661
-3.07667 0.157108564456
-3.07218 0.157181273713
-3.06769 0.157253383796
-3.0632 0.157125758617
-3.05871 0.157196853101
-3.05422 0.157068849504
-3.04973 0.157138925851
-3.04524 0.157208397661
-3.04075 0.15707959808
-3.03626 0.157148047265
-3.03177 0.157018865753
-3.02728 0.157086289706
-3.02279 0.157153103722
-3.0183 0.157023120847
-3.01381 0.157088905051
-3.00932 0.157154075827
-3.00483 0.157023288187
-3.00034 0.157087424515
-2.99585 0.156956248809
-2.99136 0.157019347964
-2.98687 0.157081828217
-2.98238 0.15694984174
-2.97789 0.157011280078
-2.9734 0.157072095981
-2.96891 0.156939294943
-2.96442 0.156999064123
-2.95993 0.157058207317
-2.95544 0.156924587775
-2.95095 0.156982679371
-2.94646 0.15704014141
-2.94197 0.156905699264
-2.93748 0.156962104759
-2.93299 0.157017877104
-2.9285 0.156882608092
-2.92401 0.156937318872
-2.91952 0.156991392887
-2.91503 0.156855292577
-2.91054 0.156908299927
-2.90605 0.156960666871
-2.90156 0.156823730663
-2.89707 0.15687502576
-2.89258 0.156925676782
-2.88809 0.156787899897
-2.8836 0.156837473804
-2.87911 0.15688639994
-2.87462 0.156747777418
-2.87013 0.156795621081
-2.86564 0.156842813244
-2.86115 0.156703339935
-2.85666 0.156749444175
-2.85217 0.156794893153
-2.84768 0.156654563717
-2.84319 0.156698919223
-2.8387 0.15674261567
-2.83421 0.156785651463
-2.82972 0.156644021895
-2.82523 0.156685956328
-2.82074 0.156727226262
-2.81625 0.156584727375
-2.81176 0.156624890165
-2.80727 0.156664384572
-2.80278 0.156703208981
-2.79829 0.156559391713
-2.7938 0.156597100771
-2.78931 0.156634135893
-2.78482 0.15667049545
-2.78033 0.156525348703
-2.77584 0.156560584511
-2.77135 0.15659514076
-2.76686 0.156449101662
-2.76237 0.156482527961
-2.75788 0.156515270658
-2.75339 0.156547328097
-2.7489 0.15639993879
-2.74441 0.156430857514
-2.73992 0.156461086872
-2.73543 0.156490625193
-2.73094 0.156341873095
-2.72645 0.156370263715
-2.72196 0.15639795912
-2.71747 0.156424957622
-2.71298 0.156451257526
-2.70849 0.15630067116
-2.704 0.15632581159
-2.69951 0.156350249156
-2.69502 0.156373982146
-2.69053 0.156222002601
-2.68604 0.156244566599
-2.68155 0.156266421676
-2.67706 0.156287566098
-2.67257 0.156307998124
-2.66808 0.15615414451
-2.66359 0.156173395083
-2.6591 0.156191928816
-2.65461 0.156209743945
-2.65012 0.156226838702
-2.64563 0.156071087209
-2.64114 0.156086987642
-2.63665 0.156102163149
-2.63216 0.156116611937
-2.62767 0.156130332207
-2.62318 0.155972657734
-2.61869 0.155985170376
-2.6142 0.155996949829
-2.60971 0.156007994268
-2.60522 0.15601830186
-2.60073 0.156027870767
-2.59624 0.155867764163
-2.59175 0.155876108726
-2.58726 0.155883709788
-2.58277 0.155890565479
-2.57828 0.155896673925
-2.57379 0.155902033243
-2.5693 0.155739454137
-2.56481 0.155743571712
-2.56032 0.155746935186
-2.55583 0.155749542645
-2.55134 0.155751392166
-2.54685 0.155752481822
-2.54236 0.155752809675
-2.53787 0.155752373781
-2.53338 0.155586281882
-2.52889 0.155584579687
-2.5244 0.155582108549
-2.51991 0.155578866487
-2.51542 0.155574851513
-2.51093 0.15557006163
-2.50644 0.155564494835
-2.50195 0.155558149113
-2.49746 0.155388462197
-2.49297 0.155380824252
-2.48848 0.155372401939
-2.48399 0.155363193207
-2.4795 0.155353195994
-2.47501 0.155342408229
-2.47052 0.155330827833
-2.46603 0.155318452717
-2.46154 0.15530528078
-2.45705 0.155291309915
-2.45256 0.155276538004
-2.44807 0.155260962919
-2.44358 0.15508549194
-2.43909 0.155068582681
-2.4346 0.155050864409
-2.43011 0.155032334954
-2.42562 0.155012992131
-2.42113 0.154992833747
-2.41664 0.1549718576
-2.41215 0.154950061473
-2.40766 0.154927443143
-2.40317 0.154904000372
-2.39868 0.154879730913
-2.39419 0.154854632508
-2.3897 0.154828702887
-2.38521 0.154801939769
-2.38072 0.154774340861
-2.37623 0.15474590386
-2.37174 0.154716626448
-2.36725 0.154686506299
-2.36276 0.154655541073
-2.35827 0.154623728418
-2.35378 0.154591065971
-2.34929 0.154557551355
-2.3448 0.154523182182
-2.34031 0.154487956052
-2.33582 0.15445187055
-2.33133 0.154414923252
-2.32684 0.154377111718
-2.32235 0.154338433497
-2.31786 0.154298886123
-2.31337 0.15425846712
-2.30888 0.154217173996
-2.30439 0.154175004248
-2.2999 0.154131955357
-2.29541 0.154088024794
-2.29092 0.154043210012
-2.28643 0.153997508455
-2.28194 0.153950917549
-2.27745 0.15390343471
-2.27296 0.153855057336
-2.26847 0.153953592603
-2.26398 0.15390311877
-2.25949 0.153851742052
-2.255 0.153799459795
-2.25051 0.153746269331
-2.24602 0.153692167978
-2.24153 0.153637153037
-2.23704 0.153581221799
-2.23255 0.153524371535
-2.22806 0.153466599504
-2.22357 0.15340790295
-2.21908 0.153492906165
-2.21459 0.153432047197
-2.2101 0.153370254915
-2.20561 0.153307526504
-2.20112 0.153243859136
-2.19663 0.153179249964
-2.19214 0.153113696127
-2.18765 0.15304719475
-2.18316 0.153122050618
-2.17867 0.153053336555
-2.17418 0.152983665823
-2.16969 0.152913035486
-2.1652 0.152841442589
-2.16071 0.152768884165
-2.15622 0.15283593483
-2.15173 0.152761124582
-2.14724 0.152685339417
-2.14275 0.152608576304
-2.13826 0.152530832195
-2.13377 0.152452104026
-2.12928 0.15251121593
-2.12479 0.152430195831
-2.1203 0.152348182015
-2.11581 0.152265171352
-2.11132 0.152181160697
-2.10683 0.152233521087
-2.10234 0.152147184119
-2.09785 0.152059837275
-2.09336 0.151971477344
-2.08887 0.152018327047
-2.08438 0.151927612562
-2.07989 0.151835874923
-2.0754 0.151743110853
-2.07091 0.151784385254
-2.06642 0.151689237948
-2.06193 0.151593053958
-2.05744 0.151495829941
-2.05295 0.151531463751
-2.04846 0.151431827369
-2.04397 0.151331140519
-2.03948 0.151229399792
-2.03499 0.151259327029
-2.0305 0.151155144355
-2.02601 0.151049897173
-2.02152 0.151075447863
-2.01703 0.150967735988
-2.01254 0.150858948835
-2.00805 0.150880083761
-2.00356 0.150768808923
-1.99907 0.150656447897
-1.99458 0.150673127577
-1.99009 0.150558255626
-1.9856 0.150442286437
-1.98111 0.150454471121
-1.97662 0.150335967519
-1.97213 0.150216355488
-1.96764 0.150224005159
-1.96315 0.150101834979
-1.95866 0.14997854504
-1.95417 0.149981619406
-1.94968 0.149855747336
-1.94519 0.149855673166
-1.9407 0.149727202538
-1.93621 0.149597592879
-1.93172 0.149592874788
-1.92723 0.149460642188
-1.92274 0.149452728077
-1.91825 0.149317855856
-1.91376 0.149181824962
-1.90927 0.149169197622
-1.90478 0.149030502329
-1.90029 0.149014631074
-1.8958 0.148873254455
-1.89131 0.148854119651
-1.88682 0.148710044684
-1.88233 0.148687626644
-1.87784 0.148540836214
-1.87335 0.148515115197
-1.86886 0.148365592098
-1.86437 0.148336548312
-1.85988 0.148184275248
-1.85539 0.148151888848
-1.8509 0.147996848435
-1.84641 0.14796109953
-1.84192 0.147803274295
-1.83743 0.147764142944
-1.83294 0.147603515333
-1.82845 0.14756098155
-1.82396 0.147397533925
-1.81947 0.14735157768
-1.81498 0.147185292324
-1.81049 0.147135893543
-1.806 0.146966752662
-1.80151 0.146913891233
-1.79702 0.146859162923
-1.79253 0.146685532734
-1.78804 0.146627310763
-1.78355 0.146450779921
-1.77906 0.146389044101
-1.77457 0.146325413723
-1.77008 0.146144324685
-1.76559 0.146077149371
-1.7611 0.145893114175
-1.75661 0.145822373678
-1.75212 0.145749710961
-1.74763 0.145561048198
-1.74314 0.145484789167
-1.73865 0.145406591144
-1.73416 0.145213258792
-1.72967 0.145131433321
-1.72518 0.145047652112
-1.72069 0.144849608042
-1.7162 0.144762168263
-1.71171 0.144672756037
-1.70722 0.14446995804
-1.70273 0.144376856146
-1.69824 0.144281765138
-1.69375 0.144074170948
-1.68926 0.143975359219
-1.68477 0.143874541758
-1.68028 0.143771712747
-1.67579 0.143557539912
-1.6713 0.143450948449
-1.66681 0.143342328907
-1.66232 0.143231675507
-1.65783 0.143010848056
-1.65334 0.142896390656
-1.64885 0.142779882975
-1.64436 0.142661319281
-1.63987 0.142540693859
-1.63538 0.142311352418
-1.63089 0.1421868711
-1.6264 0.142060311792
-1.62191 0.141931668833
-1.61742 0.141800936576
-1.61293 0.141668109393
-1.60844 0.141428323068
-1.60395 0.141291578165
-1.59946 0.141152722322
-1.59497 0.141011749976
-1.59048 0.140868655585
-1.58599 0.140723433625
-1.5815 0.140576078594
-1.57701 0.140426585012
-1.57252 0.140274947417
-1.56803 0.140018995936
-1.56354 0.139863349255
-1.55905 0.139705543035
-1.55456 0.139545571903
-1.55007 0.139383430511
-1.54558 0.139219113538
-1.54109 0.139052615687
-1.5366 0.13888393169
-1.53211 0.138713056303
-1.52762 0.138539984315
-1.52313 0.138364710541
-1.51864 0.138187229826
-1.51415 0.138007537046
-1.50966 0.137825627108
-1.50517 0.13764149495
-1.50068 0.137455135546
-1.49619 0.1372665439
-1.4917 0.137075715052
-1.48721 0.136882644079
-1.48272 0.136687326091
-1.47823 0.136489756237
-1.47374 0.136385751839
-1.46925 0.136183354788
-1.46476 0.135978690947
-1.46027 0.135771755628
-1.45578 0.135562544184
-1.45129 0.13535105201
-1.4468 0.135137274546
-1.44231 0.134921207274
-1.43782 0.134702845725
-1.43333 0.134575260225
-1.42884 0.134351982261
-1.42435 0.134126396339
-1.41986 0.133898498184
-1.41537 0.133668283577
-1.41088 0.133527298054
-1.40639 0.13329212039
-1.4019 0.133054613396
-1.39741 0.132814773073
-1.39292 0.132572595476
-1.38843 0.132418084609
-1.38394 0.13217090024
-1.37945 0.131921366613
-1.37496 0.131669480029
-1.37047 0.131504009791
-1.36598 0.131247083509
-1.36149 0.130987793068
-1.357 0.130813987261
-1.35251 0.130549633571
-1.34802 0.130282905156
-1.34353 0.130100724078
-1.33904 0.129828910214
-1.33455 0.129554711724
-1.33006 0.129364117895
-1.32557 0.129084813182
-1.32108 0.128803114652
-1.31659 0.12860407292
-1.3121 0.128317248894
-1.30761 0.12802802261
-1.30312 0.127820500273
-1.29863 0.127526130805
-1.29414 0.127312842244
-1.28965 0.127013318352
-1.28516 0.126794249846
-1.28067 0.12648956107
-1.27618 0.126264699742
-1.27169 0.125954836433
-1.2672 0.125724170282
-1.26271 0.125409123627
-1.25822 0.125172641552
-1.25373 0.124852403601
-1.24924 0.12461009543
-1.24475 0.124284659128
-1.24026 0.124036515645
-1.23577 0.12370587486
-1.23128 0.123451887837
-1.22679 0.123116037388
-1.2223 0.122856199614
-1.21781 0.122515135305
-1.21332 0.122249440616
-1.20883 0.12198066437
-1.20434 0.121631602579
-1.19985 0.121356961471
-1.19536 0.121079234292
-1.19087 0.12072217004
-1.18638 0.120438572631
-1.18189 0.120151885988
-1.1774 0.119786818104
-1.17291 0.119494258559
-1.16842 0.119198608022
-1.16393 0.11882553932
-1.15944 0.118524016021
-1.15495 0.118145732806
-1.15046 0.117618482846
-1.14597 0.11709033482
-1.14148 0.116561289455
-1.13699 0.116031347613
-1.1325 0.11550051029
-1.12801 0.114968778623
-1.12352 0.114436153892
-1.11903 0.113902637518
-1.11454 0.113368231071
-1.11005 0.112832936269
-1.10556 0.112296754982
-1.10107 0.111759689233
-1.09658 0.111221741202
-1.09209 0.110682913229
-1.0876 0.110143207815
-1.08311 0.109602627624
-1.07862 0.109061175489
-1.07413 0.10851885441
-1.06964 0.107975667562
-1.06515 0.107431618292
-1.06066 0.106886710127
-1.05617 0.10634094677
-1.05168 0.105794332112
-1.04719 0.105246870225
-1.0427 0.104698565371
-1.03821 0.104149422004
-1.03372 0.103599444769
-1.02923 0.10304863851
-1.02474 0.102497008269
-1.02025 0.10194455929
-1.01576 0.101391297022
-1.01127 0.10083722712
-1.00678 0.100282355453
-1.00229 0.0997266881
-0.9978 0.0991702313575
-0.99331 0.0986129917408
-0.98882 0.0980549759867
-0.98433 0.0974961910571
-0.97984 0.0969366441412
-0.97535 0.0963763426586
-0.97086 0.0958152942625
-0.96637 0.095253506842
-0.96188 0.0946909885258
-0.95739 0.0941277476841
-0.9529 0.0935637929325
-0.94841 0.0929991331344
-0.94392 0.0924337774038
-0.93943 0.0918677351088
-0.93494 0.0913010158737
-0.93045 0.0907336295827
-0.92596 0.0901655863826
-0.92147 0.0895968966852
-0.91698 0.0890275711711
-0.91249 0.088457620792
-0.908 0.0878870567738
-0.90351 0.0873158906195
-0.89902 0.0867441341122
-0.89453 0.0861717993179
-0.89004 0.0855988985883
-0.88555 0.0850254445641
-0.88106 0.0844514501774
-0.87657 0.0838769286549
-0.87208 0.0833018935205
-0.86759 0.0827263585985
-0.8631 0.0821503380161
-0.85861 0.0815738462064
-0.85412 0.0809968979114
-0.84963 0.0804195081842
-0.84514 0.0798416923925
-0.84065 0.0792634662209
-0.83616 0.078684845674
-0.83167 0.0781058470786
-0.82718 0.0775264870869
-0.82269 0.0769467826792
-0.8182 0.0763667511661
-0.81371 0.0757864101917
-0.80922 0.0752057777356
-0.80473 0.0746248721163
-0.80024 0.0740437119929
-0.79575 0.0734623163684
-0.79126 0.0728807045915
-0.78677 0.0722988963597
-0.78228 0.0717169117213
-0.77779 0.0711347710781
-0.7733 0.0705524951876
-0.76881 0.0699701051652
-0.76432 0.0693876224871
-0.75983 0.0688050689917
-0.75534 0.0682224668825
-0.75085 0.06763983873
-0.74636 0.067057207474
-0.74187 0.0664745964252
-0.73738 0.0658920292679
-0.73289 0.0653095300617
-0.7284 0.0647271232433
-0.72391 0.0641448336286
-0.71942 0.0635626864145
-0.71493 0.0629807071808
-0.71044 0.0623989218914
-0.70595 0.0618173568969
-0.70146 0.0612360389352
-0.69697 0.060654995134
-0.69248 0.0600742530116
-0.68799 0.0594938404786
-0.6835 0.0589137858393
-0.67901 0.058334117793
-0.67452 0.0577548654351
-0.67003 0.0571760582584
-0.66554 0.0565977261542
-0.66105 0.0560198994133
-0.65656 0.0554426087268
-0.65207 0.0548658851871
-0.64758 0.0542897602887
-0.64309 0.0537142659291
-0.6386 0.0531394344088
-0.63411 0.0525652984326
-0.62962 0.0519918911098
-0.62513 0.0514192459541
-0.62064 0.0508473968847
-0.61615 0.0502763782259
-0.61166 0.0497062247074
-0.60717 0.0491369714645
-0.60268 0.0485686540377
-0.59819 0.0480013083725
-0.5937 0.0474349708196
-0.58921 0.046869678134
-0.58472 0.0463054674747
-0.58023 0.0457423764044
-0.57574 0.0451804428882
-0.57125 0.0446197052934
-0.56676 0.0440602023884
-0.56227 0.0435019733414
-0.55778 0.0429450577198
-0.55329 0.0423894954884
-0.5488 0.0418353270086
-0.54431 0.0412825930366
-0.53982 0.0407313347216
-0.53533 0.0401815936048
-0.53084 0.0396334116168
-0.52635 0.0390868310761
-0.52186 0.0385418946868
-0.51737 0.0379986455367
-0.51288 0.0374571270945
-0.50839 0.0369173832077
-0.5039 0.0363794581
-0.49941 0.0358433963684
-0.49492 0.0353092429803
-0.49043 0.0347770432708
-0.48594 0.0342468429392
-0.48145 0.0337186880461
-0.47696 0.0331926250097
-0.47247 0.0326687006022
-0.46798 0.0321469619466
-0.46349 0.0316274565123
-0.459 0.0311102321114
-0.45451 0.0305953368944
-0.45002 0.0300828193463
-0.44553 0.0295727282816
-0.44104 0.0290651128404
-0.43655 0.028560022483
-0.43206 0.0280575069857
-0.42757 0.0275576164351
-0.42308 0.0270604012234
-0.41859 0.0265659120431
-0.4141 0.0260741998812
-0.40961 0.0255853160136
-0.40512 0.0250993119996
-0.40063 0.0246162396757
-0.39614 0.0241361511496
-0.39165 0.0236590987938
-0.38716 0.0231851352393
-0.38267 0.022714313369
-0.37818 0.0222466863109
-0.37369 0.0217823074312
-0.3692 0.0213212303275
-0.36471 0.0208635088209
-0.36022 0.0204091969494
-0.35573 0.01995834896
-0.35124 0.0195110193008
-0.34675 0.0190672626136
-0.34226 0.0186271337254
-0.33777 0.0181906876405
-0.33328 0.0177579795321
-0.32879 0.0173290647338
-0.3243 0.0169039987308
-0.31981 0.0164828371513
-0.31532 0.0160656357575
-0.31083 0.015652450436
-0.30634 0.0152433371893
-0.30185 0.0148383521255
-0.29736 0.0144375514495
-0.29287 0.0140409914525
-0.28838 0.0136487285025
-0.28389 0.0132608190344
-0.2794 0.0128773195392
-0.27491 0.012498286554
-0.27042 0.0121237766516
-0.26593 0.0117538464295
-0.26144 0.0113885524993
-0.25695 0.0110279514756
-0.25246 0.0106720999652
-0.24797 0.0103210545553
-0.24348 0.00997487180261
-0.23899 0.00963360822175
-0.2345 0.00929732027336
-0.23001 0.00896606435251
-0.22552 0.00863989677669
-0.22103 0.00831887377382
-0.21654 0.00800305146999
-0.21205 0.00769248587724
-0.20756 0.00738723288106
-0.20307 0.00708734822789
-0.19858 0.00679288751246
-0.19409 0.00650390616499
-0.1896 0.00622045943831
-0.18511 0.00594260239488
-0.18062 0.00567038989367
-0.17613 0.00540387657697
-0.17164 0.00514311685711
-0.16715 0.00488816490301
-0.16266 0.00463907462676
-0.15817 0.00439589967
-0.15368 0.00415869339026
-0.14919 0.00392750884726
-0.1447 0.00370239878904
-0.14021 0.00348341563811
-0.13572 0.00327061147746
-0.13123 0.00306403803655
-0.12674 0.00286374667724
-0.12225 0.0026697883796
-0.11776 0.00248221372774
-0.11327 0.00230107289557
-0.10878 0.00212641563251
-0.10429 0.00195829124914
-0.0998 0.00179674860285
-0.09531 0.00164183608345
-0.09082 0.00149360159874
-0.08633 0.00135209256008
-0.08184 0.00121735586792
-0.07735 0.00108943789733
-0.07286 0.000968384483564
-0.06837 0.000854240907531
-0.06388 0.000747051881364
-0.05939 0.000646861533944
-0.0549 0.00055371339646
-0.05041 0.000467650387979
-0.04592 0.00038871480105
-0.04143 0.000316948287335
-0.03694 0.000252391843272
-0.03245 0.000195085795791
-0.02796 0.000145069788068
-0.02347 0.000102382765331
-0.01898 6.70629607416e-05
-0.01449 3.91478813146e-05


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceProb0pt2.tex <==
-13.5 0.111111111111
-13.4736108605 0.111111111111
-13.447221721 0.111111111111
-13.4208325815 0.111111111111
-13.394443442 0.111111111111
-13.3680543024 0.111111111111
-13.3416651629 0.111111111111
-13.3152760234 0.111111111111
-13.2888868839 0.111111111111
-13.2624977444 0.111111111111
-13.2361086049 0.111111111111
-13.2097194654 0.111111111111
-13.1833303259 0.111111111111
-13.1569411863 0.111111111111
-13.1305520468 0.111111111111
-13.1041629073 0.111111111111
-13.0777737678 0.111111111111
-13.0513846283 0.111111111111
-13.0249954888 0.111111111111
-12.9986063493 0.111111111111
-12.9722172098 0.111111111111
-12.9458280702 0.111111111111
-12.9194389307 0.111111111111
-12.8930497912 0.111111111111
-12.8666606517 0.111111111111
-12.8402715122 0.111111111111
-12.8138823727 0.111111111111
-12.7874932332 0.111111111111
-12.7611040937 0.111111111111
-12.7347149541 0.111111111111
-12.7083258146 0.111111111111
-12.6819366751 0.111111111111
-12.6555475356 0.111111111111
-12.6291583961 0.111111111111
-12.6027692566 0.111111111111
-12.5763801171 0.111111111111
-12.5499909776 0.111111111111
-12.5236018381 0.111111111111
-12.4972126985 0.111111111111
-12.470823559 0.111111111111
-12.4444344195 0.111111111111
-12.41804528 0.111111111111
-12.3916561405 0.111111111111
-12.365267001 0.111111111111
-12.3388778615 0.111111111111
-12.312488722 0.111111111111
-12.2860995824 0.111111111111
-12.2597104429 0.111111111111
-12.2333213034 0.111111111111
-12.2069321639 0.111111111111
-12.1805430244 0.111111111111
-12.1541538849 0.111111111111
-12.1277647454 0.111111111111
-12.1013756059 0.111111111111
-12.0749864663 0.111111111111
-12.0485973268 0.111111111111
-12.0222081873 0.111111111111
-11.9958190478 0.111111111111
-11.9694299083 0.111111111111
-11.9430407688 0.111111111111
-11.9166516293 0.111111111111
-11.8902624898 0.111111111111
-11.8638733503 0.111111111111
-11.8374842107 0.111111111111
-11.8110950712 0.111111111111
-11.7847059317 0.111111111111
-11.7583167922 0.111111111111
-11.7319276527 0.111111111111
-11.7055385132 0.111111111111
-11.6791493737 0.111111111111
-11.6527602342 0.111111111111
-11.6263710946 0.111111111111
-11.5999819551 0.111111111111
-11.5735928156 0.111111111111
-11.5472036761 0.111111111111
-11.5208145366 0.111111111111
-11.4944253971 0.111111111111
-11.4680362576 0.111111111111
-11.4416471181 0.111111111111
-11.4152579785 0.111111111111
-11.388868839 0.111111111111
-11.3624796995 0.111111111111
-11.33609056 0.111111111111
-11.3097014205 0.111111111111
-11.283312281 0.111111111111
-11.2569231415 0.111111111111
-11.230534002 0.111111111111
-11.2041448624 0.111111111111
-11.1777557229 0.111111111111
-11.1513665834 0.111111111111
-11.1249774439 0.11111111111
-11.0985883044 0.11111111111
-11.0721991649 0.11111111111
-11.0458100254 0.11111111111
-11.0194208859 0.11111111111
-10.9930317464 0.11111111111
-10.9666426068 0.11111111111
-10.9402534673 0.11111111111
-10.9138643278 0.11111111111
-10.8874751883 0.11111111111
-10.8610860488 0.11111111111
-10.8346969093 0.11111111111
-10.8083077698 0.11111111111
-10.7819186303 0.111111111109
-10.7555294907 0.111111111109
-10.7291403512 0.111111111109
-10.7027512117 0.111111111109
-10.6763620722 0.111111111109
-10.6499729327 0.111111111109
-10.6235837932 0.111111111108
-10.5971946537 0.111111111108
-10.5708055142 0.111111111108
-10.5444163746 0.111111111108
-10.5180272351 0.111111111108
-10.4916380956 0.111111111107
-10.4652489561 0.111111111107
-10.4388598166 0.111111111107
-10.4124706771 0.111111111106
-10.3860815376 0.111111111106
-10.3596923981 0.111111111106
-10.3333032585 0.111111111105
-10.306914119 0.111111111105
-10.2805249795 0.111111111104
-10.25413584 0.111111111104
-10.2277467005 0.111111111103
-10.201357561 0.111111111103
-10.1749684215 0.111111111102
-10.148579282 0.111111111101
-10.1221901425 0.1111111111
-10.0958010029 0.1111111111
-10.0694118634 0.111111111099
-10.0430227239 0.111111111098
-10.0166335844 0.111111111097
-9.99024444489 0.111111111096
-9.96385530538 0.111111111094
-9.93746616587 0.111111111093
-9.91107702636 0.111111111092
-9.88468788684 0.11111111109
-9.85829874733 0.111111111089
-9.83190960782 0.111111111087
-9.80552046831 0.111111111085
-9.7791313288 0.111111111083
-9.75274218928 0.111111111081
-9.72635304977 0.111111111079
-9.69996391026 0.111111111076
-9.67357477075 0.111111111074
-9.64718563124 0.111111111071
-9.62079649172 0.111111111068
-9.59440735221 0.111111111064
-9.5680182127 0.111111111061
-9.54162907319 0.111111111057
-9.51523993368 0.111111111053
-9.48885079416 0.111111111048
-9.46246165465 0.111111111044
-9.43607251514 0.111111111038
-9.40968337563 0.111111111033
-9.38329423611 0.111111111027
-9.3569050966 0.11111111102
-9.33051595709 0.111111111014
-9.30412681758 0.111111111006
-9.27773767807 0.111111110998
-9.25134853855 0.11111111099
-9.22495939904 0.11111111098
-9.19857025953 0.11111111097
-9.17218112002 0.11111111096
-9.14579198051 0.111111110948
-9.11940284099 0.111111110936
-9.09301370148 0.111111110922
-9.06662456197 0.111111110908
-9.04023542246 0.111111110893
-9.01384628295 0.111111110876
-8.98745714343 0.111111110858
-8.96106800392 0.111111110839
-8.93467886441 0.111111110818
-8.9082897249 0.111111110796
-8.88190058539 0.111111110772
-8.85551144587 0.111111110747
-8.82912230636 0.111111110719
-8.80273316685 0.111111110689
-8.77634402734 0.111111110657
-8.74995488782 0.111111110623
-8.72356574831 0.111111110586
-8.6971766088 0.111111110546
-8.67078746929 0.111111110503
-8.64439832978 0.111111110457
-8.61800919026 0.111111110408
-8.59162005075 0.111111110355
-8.56523091124 0.111111110298
-8.53884177173 0.111111110236
-8.51245263222 0.11111111017
-8.4860634927 0.111111110099
-8.45967435319 0.111111110022
-8.43328521368 0.11111110994
-8.40689607417 0.111111109852
-8.38050693466 0.111111109757
-8.35411779514 0.111111109655
-8.32772865563 0.111111109545
-8.30133951612 0.111111109427
-8.27495037661 0.1111111093
-8.2485612371 0.111111109163
-8.22217209758 0.111111109016
-8.19578295807 0.111111108859
-8.16939381856 0.111111108689
-8.14300467905 0.111111108507
-8.11661553953 0.111111108311
-8.09022640002 0.1111111081
-8.06383726051 0.111111107874
-8.037448121 0.111111107631
-8.01105898149 0.111111107369
-7.98466984197 0.111111107088
-7.95828070246 0.111111106786
-7.93189156295 0.111111106461
-7.90550242344 0.111111106113
-7.87911328393 0.111111105738
-7.85272414441 0.111111105335
-7.8263350049 0.111111104902
-7.79994586539 0.111111104436
-7.77355672588 0.111111103936
-7.74716758637 0.111111103399
-7.72077844685 0.111111102822
-7.69438930734 0.111111102201
-7.66800016783 0.111111101535
-7.64161102832 0.111111100819
-7.61522188881 0.111111100049
-7.58883274929 0.111111099223
-7.56244360978 0.111111098335
-7.53605447027 0.111111097381
-7.50966533076 0.111111096356
-7.48327619124 0.111111095255
-7.45688705173 0.111111094072
-7.43049791222 0.111111092802
-7.40410877271 0.111111091437
-7.3777196332 0.111111089971
-7.35133049368 0.111111088397
-7.32494135417 0.111111086706
-7.29855221466 0.11111108489
-7.27216307515 0.111111082939
-7.24577393564 0.111111080844
-7.21938479612 0.111111078595
-7.19299565661 0.111111076179
-7.1666065171 0.111111073585
-7.14021737759 0.111111070799
-7.11382823808 0.111111067808
-7.08743909856 0.111111064596
-7.06104995905 0.111111061147
-7.03466081954 0.111111057444
-7.00827168003 0.111111053468
-6.98188254052 0.1111110492
-6.955493401 0.111111044618
-6.92910426149 0.111111039698
-6.90271512198 0.111111034417
-6.87632598247 0.111111028748
-6.84993684295 0.111111022663
-6.82354770344 0.111111016131
-6.79715856393 0.11111100912
-6.77076942442 0.111111001595
-6.74438028491 0.111110993518
-6.71799114539 0.11111098485
-6.69160200588 0.111110975547
-6.66521286637 0.111110965564
-6.63882372686 0.111110954851
-6.61243458735 0.111110943354
-6.58604544783 0.111110931018
-6.55965630832 0.111110917781
-6.53326716881 0.111110903579
-6.5068780293 0.11111088834
-6.48048888979 0.111110871992
-6.45409975027 0.111110854452
-6.42771061076 0.111110835635
-6.40132147125 0.11111081545
-6.37493233174 0.111110793796
-6.34854319223 0.111110770569
-6.32215405271 0.111110745656
-6.2957649132 0.111110718934
-6.26937577369 0.111110690274
-6.24298663418 0.111110659536
-6.21659749466 0.111110626571
-6.19020835515 0.11111059122
-6.16381921564 0.111110553312
-6.13743007613 0.111110512662
-6.11104093662 0.111110469075
-6.0846517971 0.111110422341
-6.05826265759 0.111110372234
-6.03187351808 0.111110318514
-6.00548437857 0.111110260922
-5.97909523906 0.111110199183
-5.95270609954 0.111110133002
-5.92631696003 0.111110062061
-5.89992782052 0.111109986022
-5.87353868101 0.111109904522
-5.8471495415 0.111109817175
-5.82076040198 0.111109723564
-5.79437126247 0.111109623245
-5.76798212296 0.111109515744
-5.74159298345 0.111109400552
-5.71520384394 0.111109277124
-5.68881470442 0.11110914488
-5.66242556491 0.111109003196
-5.6360364254 0.111108851407
-5.60964728589 0.111108688801
-5.58325814637 0.111108514616
-5.55686900686 0.111108328038
-5.53047986735 0.111108128196
-5.50409072784 0.111107914159
-5.47770158833 0.111107684932
-5.45131244881 0.111107439451
-5.4249233093 0.111107176577
-5.39853416979 0.111106895096
-5.37214503028 0.111106593707
-5.34575589077 0.111106271022
-5.31936675125 0.111105925557
-5.29297761174 0.111105555726
-5.26658847223 0.111105159834
-5.24019933272 0.111104736072
-5.21381019321 0.111104282506
-5.18742105369 0.111103797071
-5.16103191418 0.11110327756
-5.13464277467 0.111102721618
-5.10825363516 0.111102126729
-5.08186449565 0.111101490207
-5.05547535613 0.111100809183
-5.02908621662 0.111100080595
-5.00269707711 0.111099301177
-4.9763079376 0.111098467439
-4.94991879808 0.111097575658
-4.92352965857 0.111096621861
-4.89714051906 0.11109560181
-4.87075137955 0.111094510981
-4.84436224004 0.11109334455
-4.81797310052 0.11109209737
-4.79158396101 0.111090763952
-4.7651948215 0.111089338443
-4.73880568199 0.1110878146
-4.71241654248 0.111086185769
-4.68602740296 0.111084444853
-4.65963826345 0.111082584292
-4.63324912394 0.111080596023
-4.60685998443 0.111078471458
-4.58047084492 0.111076201443
-4.5540817054 0.111073776227
-4.52769256589 0.111071185421
-4.50130342638 0.111068417961
-4.47491428687 0.111065462063
-4.44852514736 0.111062305178
-4.42213600784 0.111058933946
-4.39574686833 0.111055334146
-4.36935772882 0.111051490638
-4.34296858931 0.111047387312
-4.31657944979 0.111043007025
-4.29019031028 0.111038331537
-4.26380117077 0.111033341446
-4.23741203126 0.111028016116
-4.21102289175 0.111022333603
-4.18463375223 0.111016270574
-4.15824461272 0.111009802224
-4.13185547321 0.111002902189
-4.1054663337 0.110995542451
-4.07907719419 0.110987693241
-4.05268805467 0.110979322934
-4.02629891516 0.110970397938
-3.99990977565 0.110960882584
-3.97352063614 0.110950738997
-3.94713149663 0.110939926975
-3.92074235711 0.110928403848
-3.8943532176 0.110916124339
-3.86796407809 0.110903040417
-3.84157493858 0.110889101133
-3.81518579907 0.110874252462
-3.78879665955 0.110858437126
-3.76240752004 0.110841594411
-3.73601838053 0.11082365998
-3.70962924102 0.110804565669
-3.6832401015 0.110784239277
-3.65685096199 0.110762604348
-3.63046182248 0.11073957994
-3.60407268297 0.110715080382
-3.57768354346 0.110689015024
-3.55129440394 0.110661287973
-3.52490526443 0.110631797819
-3.49851612492 0.110600437346
-3.47212698541 0.110567093235
-3.4457378459 0.11053164575
-3.41934870638 0.110493968417
-3.39295956687 0.110453927684
-3.36657042736 0.110411382573
-3.34018128785 0.110366184316
-3.31379214834 0.110318175978
-3.28740300882 0.110267192066
-3.26101386931 0.110213058129
-3.2346247298 0.110155590339
-3.20823559029 0.11009459506
-3.18184645078 0.110029868411
-3.15545731126 0.109961195804
-3.12906817175 0.109888351483
-3.10267903224 0.10981109804
-3.07628989273 0.109729185932
-3.04990075321 0.109642352973
-3.0235116137 0.109550323831
-2.99712247419 0.109452809508
-2.97073333468 0.109349506818
-2.94434419517 0.109240097855
-2.91795505565 0.109124249459
-2.89156591614 0.109001612685
-2.86517677663 0.108871822263
-2.83878763712 0.108734496069
-2.81239849761 0.108589234594
-2.78600935809 0.108435620431
-2.75962021858 0.108273217762
-2.73323107907 0.108101571868
-2.70684193956 0.107920208657
-2.68045280005 0.107728634215
-2.65406366053 0.107526334383
-2.62767452102 0.107312774374
-2.60128538151 0.107087398424
-2.574896242 0.10684962949
-2.54850710249 0.106598869003
-2.52211796297 0.10633449668
-2.49572882346 0.1060558704
-2.46933968395 0.105762326166
-2.44295054444 0.105453178137
-2.41656140492 0.105127718773
-2.39017226541 0.104785219071
-2.3637831259 0.104424928922
-2.33739398639 0.104046077599
-2.31100484688 0.103647874378
-2.28461570736 0.103229509319
-2.25822656785 0.102790154207
-2.23183742834 0.102328963673
-2.20544828883 0.101845076512
-2.17905914932 0.101337617211
-2.1526700098 0.100805697692
-2.12628087029 0.100248419306
-2.09989173078 0.0996648750716
-2.07350259127 0.0990541521936
-2.04711345176 0.0984153348587
-2.02072431224 0.0977475073393
-1.99433517273 0.0970497574098
-1.96794603322 0.0963211800947
-1.94155689371 0.0955608817598
-1.9151677542 0.0947679845585
-1.88877861468 0.0939416312436
-1.86238947517 0.0930809903537
-1.83600033566 0.0921852617788
-1.80961119615 0.0912536827099
-1.78322205663 0.0902855339711
-1.75683291712 0.0892801467322
-1.73044377761 0.0882369095917
-1.7040546381 0.0871552760194
-1.67766549859 0.0860347721382
-1.65127635907 0.0848750048226
-1.62488721956 0.08367567008
-1.59849808005 0.0824365616795
-1.57210894054 0.0811575799773
-1.54571980103 0.0798387408871
-1.51933066151 0.0784801849277
-1.492941522 0.0770821862753
-1.46655238249 0.0756451617335
-1.44016324298 0.0741696795271
-1.41377410347 0.0726564678123
-1.38738496395 0.0711064227862
-1.36099582444 0.0695206162667
-1.33460668493 0.0679003026051
-1.30821754542 0.0662469247823
-1.28182840591 0.0645621195324
-1.25543926639 0.0628477213284
-1.22905012688 0.0611057650608
-1.20266098737 0.059338487236
-1.17627184786 0.0575483255204
-1.14988270834 0.0557379164603
-1.12349356883 0.0539100912109
-1.09710442932 0.0520678691238
-1.07071528981 0.0502144490511
-1.0443261503 0.0483531982515
-1.01793701078 0.0464876388047
-0.991547871272 0.0446214314753
-0.96515873176 0.0427583570056
-0.938769592248 0.0409022948578
-0.912380452736 0.0390571994798
-0.885991313224 0.037227074219
-0.859602173712 0.0354159430708
-0.8332130342 0.0336278205095
-0.806823894688 0.0318666797123
-0.780434755176 0.0301364195523
-0.754045615663 0.0284408307975
-0.727656476151 0.0267835620099
-0.701267336639 0.0251680856903
-0.674878197127 0.0235976652522
-0.648489057615 0.0220753234405
-0.622099918103 0.0206038128186
-0.595710778591 0.0191855889493
-0.569321639079 0.0178227868657
-0.542932499567 0.0165172013899
-0.516543360055 0.0152702717899
-0.490154220543 0.0140830711832
-0.463765081031 0.0129563009921
-0.437375941518 0.0118902906386
-0.410986802006 0.010885002537
-0.384597662494 0.00994004230422
-0.358208522982 0.00905467397152
-0.33181938347 0.0082278398436
-0.305430243958 0.00745818452858
-0.30481938347 0.00744103304743
-0.304208522982 0.00742391140817
-0.303597662494 0.00740681967467
-0.302986802006 0.0073897579111
-0.302375941518 0.00737272618196
-0.301765081031 0.00735572455202
-0.301154220543 0.00733875308639
-0.300543360055 0.00732181185047
-0.299932499567 0.00730490091
-0.299321639079 0.00728802033098
-0.298710778591 0.00727117017977
-0.298099918103 0.00725435052301
-0.297489057615 0.00723756142766
-0.296878197127 0.007220802961
-0.296267336639 0.00720407519062
-0.295656476151 0.0071873781844
-0.295045615663 0.00717071201057
-0.294434755176 0.00715407673764
-0.293823894688 0.00713747243446
-0.2932130342 0.00712089917018
-0.292602173712 0.00710435701426
-0.291991313224 0.0070878460365
-0.291380452736 0.00707136630699
-0.290769592248 0.00705491789614
-0.29015873176 0.00703850087469
-0.289547871272 0.00702211531369
-0.288937010784 0.00700576128451
-0.288326150296 0.00698943885882
-0.287715289808 0.00697314810863
-0.287104429321 0.00695688910626
-0.286493568833 0.00694066192435
-0.285882708345 0.00692446663587
-0.285271847857 0.00690830331408
-0.284660987369 0.00689217203259
-0.284050126881 0.00687607286532
-0.283439266393 0.0068600058865
-0.282828405905 0.00684397117071
-0.282217545417 0.00682796879282
-0.281606684929 0.00681199882803
-0.280995824441 0.00679606135189
-0.280384963953 0.00678015644023
-0.279774103466 0.00676428416923
-0.279163242978 0.00674844461539
-0.27855238249 0.00673263785553
-0.277941522002 0.00671686396679
-0.277330661514 0.00670112302664
-0.276719801026 0.00668541511289
-0.276108940538 0.00666974030364
-0.27549808005 0.00665409867735
-0.274887219562 0.00663849031279
-0.274276359074 0.00662291528905
-0.273665498586 0.00660737368555
-0.273054638098 0.00659186558206
-0.272443777611 0.00657639105865
-0.271832917123 0.00656095019572
-0.271222056635 0.00654554307402
-0.270611196147 0.0065301697746
-0.270000335659 0.00651483037885
-0.269389475171 0.00649952496849
-0.268778614683 0.00648425362559
-0.268167754195 0.0064690164325
-0.267556893707 0.00645381347195
-0.266946033219 0.00643864482697
-0.266335172731 0.00642351058094
-0.265724312244 0.00640841081755
-0.265113451756 0.00639334562083
-0.264502591268 0.00637831507515
-0.26389173078 0.00636331926521
-0.263280870292 0.00634835827602
-0.262670009804 0.00633343219296
-0.262059149316 0.00631854110171
-0.261448288828 0.00630368508829
-0.26083742834 0.00628886423908
-0.260226567852 0.00627407864075
-0.259615707364 0.00625932838033
-0.259004846876 0.00624461354518
-0.258393986389 0.006229934223
-0.257783125901 0.00621529050181
-0.257172265413 0.00620068246999
-0.256561404925 0.00618611021621
-0.255950544437 0.00617157382953
-0.255339683949 0.0061570733993
-0.254728823461 0.00614260901524
-0.254117962973 0.00612818076739
-0.253507102485 0.00611378874612
-0.252896241997 0.00609943304215
-0.252285381509 0.00608511374652
-0.251674521021 0.00607083095064
-0.251063660534 0.00605658474622
-0.250452800046 0.00604237522533
-0.249841939558 0.00602820248037
-0.24923107907 0.00601406660408
-0.248620218582 0.00599996768954
-0.248009358094 0.00598590583017
-0.247398497606 0.00597188111972
-0.246787637118 0.00595789365228
-0.24617677663 0.0059439435223
-0.245565916142 0.00593003082454
-0.244955055654 0.00591615565411
-0.244344195166 0.00590231810648
-0.243733334679 0.00588851827744
-0.243122474191 0.00587475626311
-0.242511613703 0.00586103215998
-0.241900753215 0.00584734606486
-0.241289892727 0.0058336980749
-0.240679032239 0.00582008828761
-0.240068171751 0.00580651680081
-0.239457311263 0.0057929837127
-0.238846450775 0.0057794891218
-0.238235590287 0.00576603312696
-0.237624729799 0.0057526158274
-0.237013869311 0.00573923732267
-0.236403008824 0.00572589771265
-0.235792148336 0.00571259709758
-0.235181287848 0.00569933557803
-0.23457042736 0.00568611325494
-0.233959566872 0.00567293022955
-0.233348706384 0.00565978660347
-0.232737845896 0.00564668247867
-0.232126985408 0.00563361795742
-0.23151612492 0.00562059314236
-0.230905264432 0.00560760813648
-0.230294403944 0.00559466304311
-0.229683543456 0.0055817579659
-0.229072682969 0.00556889300888
-0.228461822481 0.0055560682764
-0.227850961993 0.00554328387317
-0.227240101505 0.00553053990423
-0.226629241017 0.00551783647498
-0.226018380529 0.00550517369115
-0.225407520041 0.00549255165883
-0.224796659553 0.00547997048444
-0.224185799065 0.00546743027475
-0.223574938577 0.00545493113689
-0.222964078089 0.00544247317832
-0.222353217601 0.00543005650684
-0.221742357114 0.00541768123061
-0.221131496626 0.00540534745814
-0.220520636138 0.00539305529826
-0.21990977565 0.00538080486017
-0.219298915162 0.00536859625341
-0.218688054674 0.00535642958786
-0.218077194186 0.00534430497375
-0.217466333698 0.00533222252166
-0.21685547321 0.00532018234251
-0.216244612722 0.00530818454757
-0.215633752234 0.00529622924844
-0.215022891746 0.0052843165571
-0.214412031259 0.00527244658585
-0.213801170771 0.00526061944733
-0.213190310283 0.00524883525455
-0.212579449795 0.00523709412086
-0.211968589307 0.00522539615994
-0.211357728819 0.00521374148584
-0.210746868331 0.00520213021293
-0.210136007843 0.00519056245594
-0.209525147355 0.00517903832995
-0.208914286867 0.00516755795039
-0.208303426379 0.00515612143301
-0.207692565891 0.00514472889393
-0.207081705404 0.00513338044961
-0.206470844916 0.00512207621685
-0.205859984428 0.00511081631281
-0.20524912394 0.00509960085498
-0.204638263452 0.0050884299612
-0.204027402964 0.00507730374965
-0.203416542476 0.00506622233887
-0.202805681988 0.00505518584773
-0.2021948215 0.00504419439546
-0.201583961012 0.00503324810162
-0.200973100524 0.00502234708611
-0.200362240036 0.0050114914692
-0.199751379549 0.00500068137148
-0.199140519061 0.00498991691389
-0.198529658573 0.00497919821772
-0.197918798085 0.00496852540461
-0.197307937597 0.00495789859651
-0.196697077109 0.00494731791575
-0.196086216621 0.00493678348499
-0.195475356133 0.00492629542722
-0.194864495645 0.00491585386579
-0.194253635157 0.00490545892439
-0.193642774669 0.00489511072703
-0.193031914181 0.00488480939809
-0.192421053694 0.00487455506228
-0.191810193206 0.00486434784464
-0.191199332718 0.00485418787055
-0.19058847223 0.00484407526576
-0.189977611742 0.00483401015633
-0.189366751254 0.00482399266865
-0.188755890766 0.00481402292949
-0.188145030278 0.00480410106591
-0.18753416979 0.00479422720534
-0.186923309302 0.00478440147554
-0.186312448814 0.0047746240046
-0.185701588326 0.00476489492094
-0.185090727839 0.00475521435334
-0.184479867351 0.00474558243088
-0.183869006863 0.00473599928301
-0.183258146375 0.00472646503949
-0.182647285887 0.00471697983042
-0.182036425399 0.00470754378623
-0.181425564911 0.00469815703768
-0.180814704423 0.00468881971587
-0.180203843935 0.00467953195221
-0.179592983447 0.00467029387848
-0.178982122959 0.00466110562673
-0.178371262472 0.0046519673294
-0.177760401984 0.0046428791192
-0.177149541496 0.0046338411292
-0.176538681008 0.00462485349279
-0.17592782052 0.00461591634369
-0.175316960032 0.00460702981591
-0.174706099544 0.00459819404383
-0.174095239056 0.00458940916212
-0.173484378568 0.00458067530578
-0.17287351808 0.00457199261012
-0.172262657592 0.00456336121079
-0.171651797104 0.00455478124372
-0.171040936617 0.0045462528452
-0.170430076129 0.0045377761518
-0.169819215641 0.00452935130043
-0.169208355153 0.00452097842828
-0.168597494665 0.00451265767287
-0.167986634177 0.00450438917204
-0.167375773689 0.00449617306393
-0.166764913201 0.00448800948696
-0.166154052713 0.0044798985799
-0.165543192225 0.00447184048179
-0.164932331737 0.00446383533199
-0.164321471249 0.00445588327015
-0.163710610762 0.00444798443623
-0.163099750274 0.00444013897047
-0.162488889786 0.00443234701343
-0.161878029298 0.00442460870593
-0.16126716881 0.00441692418912
-0.160656308322 0.00440929360441
-0.160045447834 0.00440171709352
-0.159434587346 0.00439419479844
-0.158823726858 0.00438672686144
-0.15821286637 0.0043793134251
-0.157602005882 0.00437195463226
-0.156991145394 0.00436465062603
-0.156380284907 0.00435740154981
-0.155769424419 0.00435020754728
-0.155158563931 0.00434306876236
-0.154547703443 0.00433598533927
-0.153936842955 0.00432895742249
-0.153325982467 0.00432198515675
-0.152715121979 0.00431506868705
-0.152104261491 0.00430820815865
-0.151493401003 0.00430140371707
-0.150882540515 0.00429465550806
-0.150271680027 0.00428796367765
-0.149660819539 0.00428132837209
-0.149049959052 0.00427474973791
-0.148439098564 0.00426822792183
-0.147828238076 0.00426176307085
-0.147217377588 0.00425535533219
-0.1466065171 0.00424900485331
-0.145995656612 0.00424271178187
-0.145384796124 0.00423647626579
-0.144773935636 0.00423029845318
-0.144163075148 0.0042241784924
-0.14355221466 0.00421811653199
-0.142941354172 0.00421211272072
-0.142330493684 0.00420616720756
-0.141719633197 0.00420028014169
-0.141108772709 0.00419445167247
-0.140497912221 0.00418868194947
-0.139887051733 0.00418297112243
-0.139276191245 0.00417731934131
-0.138665330757 0.00417172675621
-0.138054470269 0.00416619351742
-0.137443609781 0.00416071977542
-0.136832749293 0.00415530568084
-0.136221888805 0.00414995138446
-0.135611028317 0.00414465703723
-0.135000167829 0.00413942279026
-0.134389307342 0.00413424879479
-0.133778446854 0.0041291352022
-0.133167586366 0.00412408216402
-0.132556725878 0.00411908983189
-0.13194586539 0.00411415835759
-0.131335004902 0.00410928789302
-0.130724144414 0.00410447859017
-0.130113283926 0.00409973060115
-0.129502423438 0.00409504407818
-0.12889156295 0.00409041917355
-0.128280702462 0.00408585603964
-0.127669841974 0.00408135482894
-0.127058981487 0.00407691569397
-0.126448120999 0.00407253878734
-0.125837260511 0.00406822426172
-0.125226400023 0.00406397226983
-0.124615539535 0.00405978296441
-0.124004679047 0.00405565649827
-0.123393818559 0.00405159302423
-0.122782958071 0.00404759269513
-0.122172097583 0.00404365566384
-0.121561237095 0.0040397820832
-0.120950376607 0.00403597210608
-0.120339516119 0.00403222588532
-0.119728655632 0.00402854357373
-0.119117795144 0.00402492532412
-0.118506934656 0.00402137128922
-0.117896074168 0.00401788162173
-0.11728521368 0.0040144564743
-0.116674353192 0.0040110959995
-0.116063492704 0.00400780034981
-0.115452632216 0.00400456967763
-0.114841771728 0.00400140413527
-0.11423091124 0.00399830387492
-0.113620050752 0.00399526904864
-0.113009190264 0.00399229980837
-0.112398329777 0.00398939630591
-0.111787469289 0.00398655869288
-0.111176608801 0.00398378712075
-0.110565748313 0.00398108174081
-0.109954887825 0.00397844270416
-0.109344027337 0.00397587016169
-0.108733166849 0.00397336426407
-0.108122306361 0.00397092516174
-0.107511445873 0.00396855300489
-0.106900585385 0.00396624794348
-0.106289724897 0.00396401012717
-0.105678864409 0.00396183970534
-0.105068003922 0.00395973682707
-0.104457143434 0.00395770164113
-0.103846282946 0.00395573429596
-0.103235422458 0.00395383493964
-0.10262456197 0.00395200371991
-0.102013701482 0.00395024078412
-0.101402840994 0.00394854627922
-0.100791980506 0.00394692035176
-0.100181120018 0.00394536314787
-0.0995702595303 0.00394387481321
-0.0989593990424 0.00394245549299
-0.0983485385545 0.00394110533196
-0.0977376780666 0.00393982447433
-0.0971268175787 0.00393861306383
-0.0965159570907 0.00393747124363
-0.0959050966028 0.00393639915636
-0.0952942361149 0.00393539694405
-0.094683375627 0.00393446474816
-0.0940725151391 0.00393360270952
-0.0934616546512 0.00393281096832
-0.0928507941632 0.00393208966409
-0.0922399336753 0.00393143893568
-0.0916290731874 0.00393085892124
-0.0910182126995 0.00393034975819
-0.0904073522116 0.0039299115832
-0.0897964917237 0.00392954453217
-0.0891856312358 0.00392924874019
-0.0885747707478 0.00392902434154
-0.0879639102599 0.00392887146966
-0.087353049772 0.00392879025708
-0.0867421892841 0.00392878083548
-0.0861313287962 0.00392884333559
-0.0855204683083 0.00392897788717
-0.0849096078203 0.00392918461904
-0.0842987473324 0.00392946365899
-0.0836878868445 0.00392981513376
-0.0830770263566 0.00393023916904
-0.0824661658687 0.00393073588944
-0.0818553053808 0.00393130541842
-0.0812444448928 0.00393194787828
-0.0806335844049 0.00393266339016
-0.080022723917 0.00393345207395
-0.0794118634291 0.00393431404832
-0.0788010029412 0.00393524943062
-0.0781901424533 0.0039362583369
-0.0775792819653 0.00393734088186
-0.0769684214774 0.00393849717879
-0.0763575609895 0.00393972733959
-0.0757467005016 0.00394103147466
-0.0751358400137 0.00394240969294
-0.0745249795258 0.00394386210179
-0.0739141190378 0.00394538880705
-0.0733032585499 0.00394698991289
-0.072692398062 0.00394866552187
-0.0720815375741 0.00395041573484
-0.0714706770862 0.00395224065091
-0.0708598165983 0.00395414036743
-0.0702489561104 0.0039561149799
-0.0696380956224 0.00395816458198
-0.0690272351345 0.00396028926542
-0.0684163746466 0.00396248912001
-0.0678055141587 0.00396476423355
-0.0671946536708 0.00396711469176
-0.0665837931829 0.00396954057832
-0.0659729326949 0.00397204197472
-0.065362072207 0.00397461896027
-0.0647512117191 0.00397727161206
-0.0641403512312 0.00398000000485
-0.0635294907433 0.00398280421108
-0.0629186302554 0.00398568430078
-0.0623077697674 0.00398864034151
-0.0616969092795 0.00399167239834
-0.0610860487916 0.00399478053378
-0.0604751883037 0.0039979648077
-0.0598643278158 0.0040012252773
-0.0592534673279 0.00400456199703
-0.0586426068399 0.00400797501854
-0.058031746352 0.00401146439062
-0.0574208858641 0.00401503015915
-0.0568100253762 0.00401867236701
-0.0561991648883 0.00402239105401
-0.0555883044004 0.00402618625687
-0.0549774439124 0.00403005800911
-0.0543665834245 0.00403400634099
-0.0537557229366 0.00403803127947
-0.0531448624487 0.00404213284808
-0.0525340019608 0.00404631106692
-0.0519231414729 0.00405056595253
-0.051312280985 0.00405489751784
-0.050701420497 0.0040593057721
-0.0500905600091 0.00406379072077
-0.0494796995212 0.00406835236549
-0.0488688390333 0.00407299070396
-0.0482579785454 0.00407770572989
-0.0476471180575 0.00408249743288
-0.0470362575695 0.00408736579838
-0.0464253970816 0.00409231080755
-0.0458145365937 0.00409733243724
-0.0452036761058 0.00410243065985
-0.0445928156179 0.00410760544325
-0.04398195513 0.00411285675069
-0.043371094642 0.00411818454074
-0.0427602341541 0.00412358876714
-0.0421493736662 0.00412906937874
-0.0415385131783 0.00413462631937
-0.0409276526904 0.0041402595278
-0.0403167922025 0.00414596893757
-0.0397059317145 0.00415175447693
-0.0390950712266 0.00415761606871
-0.0384842107387 0.00416355363024
-0.0378733502508 0.0041695670732
-0.0372624897629 0.00417565630357
-0.036651629275 0.00418182122145
-0.0360407687871 0.004188061721
-0.0354299082991 0.00419437769028
-0.0348190478112 0.00420076901118
-0.0342081873233 0.00420723555925
-0.0335973268354 0.00421377720361
-0.0329864663475 0.0042203938068
-0.0323756058596 0.0042270852247
-0.0317647453716 0.00423385130634
-0.0311538848837 0.0042406918938
-0.0305430243958 0.0042476068221
-0.0299321639079 0.00425459591901
-0.02932130342 0.00426165900497
-0.0287104429321 0.00426879589288
-0.0280995824441 0.00427600638805
-0.0274887219562 0.00428329028797
-0.0268778614683 0.00429064738219
-0.0262670009804 0.00429807745221
-0.0256561404925 0.00430558027127
-0.0250452800046 0.00431315560421
-0.0244344195166 0.00432080320734
-0.0238235590287 0.00432852282826
-0.0232126985408 0.00433631420569
-0.0226018380529 0.0043441770693
-0.021990977565 0.00435211113959
-0.0213801170771 0.00436011612764
-0.0207692565891 0.004368191735
-0.0201583961012 0.00437633765348
-0.0195475356133 0.00438455356501
-0.0189366751254 0.00439283914138
-0.0183258146375 0.00440119404413
-0.0177149541496 0.00440961792433
-0.0171040936617 0.00441811042238
-0.0164932331737 0.00442667116784
-0.0158823726858 0.00443529977919
-0.0152715121979 0.00444399586367
-0.01466065171 0.00445275901705
-0.0140497912221 0.00446158882342
-0.0134389307342 0.00447048485502
-0.0128280702462 0.00447944667193
-0.0122172097583 0.00448847382196
-0.0116063492704 0.00449756584036
-0.0109954887825 0.0045067222496
-0.0103846282946 0.00451594255915
-0.00977376780666 0.00452522626525
-0.00916290731874 0.00453457285068
-0.00855204683083 0.00454398178446
-0.00794118634291 0.00455345252169
-0.00733032585499 0.00456298450324
-0.00671946536708 0.0045725771555
-0.00610860487916 0.00458222989015
-0.00549774439124 0.00459194210387
-0.00488688390333 0.00460171317809
-0.00427602341541 0.00461154247869
-0.0036651629275 0.00462142935578
-0.00305430243958 0.00463137314335
-0.00244344195166 0.00464137315904
-0.00183258146375 0.00465142870382
-0.00122172097583 0.0046615390617
-0.000610860487916 0.00467170349944
0.0 0.00468192126623
0.00160529707243 0.00470892667676
0.00321059414487 0.00473610179344
0.0048158912173 0.00476344781115
0.00642118828974 0.00479096593441
0.00802648536217 0.00481865737752
0.00963178243461 0.0048465233646
0.011237079507 0.00487456512972
0.0128423765795 0.00490278391694
0.0144476736519 0.00493118098049
0.0160529707243 0.00495975758477
0.0176582677968 0.00498851500453
0.0192635648692 0.00501745452492
0.0208688619416 0.00504657744159
0.0224741590141 0.00507588506082
0.0240794560865 0.00510537869959
0.025684753159 0.00513505968569
0.0272900502314 0.00516492935786
0.0288953473038 0.00519498906582
0.0305006443763 0.00522524017046
0.0321059414487 0.00525568404387
0.0337112385211 0.00528632206952
0.0353165355936 0.00531715564231
0.036921832666 0.00534818616872
0.0385271297384 0.0053794150669
0.0401324268109 0.00541084376678
0.0417377238833 0.00544247371023
0.0433430209557 0.00547430635111
0.0449483180282 0.00550634315543
0.0465536151006 0.00553858560145
0.048158912173 0.00557103517982
0.0497642092455 0.00560369339369
0.0513695063179 0.0056365617588
0.0529748033903 0.00566964180368
0.0545801004628 0.00570293506971
0.0561853975352 0.00573644311125
0.0577906946076 0.00577016749582
0.0593959916801 0.00580410980417
0.0610012887525 0.00583827163045
0.0626065858249 0.00587265458233
0.0642118828974 0.00590726028114
0.0658171799698 0.00594209036198
0.0674224770423 0.00597714647391
0.0690277741147 0.00601243028002
0.0706330711871 0.00604794345765
0.0722383682596 0.00608368769847
0.073843665332 0.00611966470863
0.0754489624044 0.00615587620896
0.0770542594769 0.00619232393505
0.0786595565493 0.00622900963743
0.0802648536217 0.00626593508174
0.0818701506942 0.00630310204885
0.0834754477666 0.00634051233502
0.085080744839 0.00637816775207
0.0866860419115 0.00641607012754
0.0882913389839 0.00645422130483
0.0898966360563 0.0064926231434
0.0915019331288 0.00653127751887
0.0931072302012 0.00657018632327
0.0947125272736 0.00660935146513
0.0963178243461 0.0066487748697
0.0979231214185 0.0066884584791
0.0995284184909 0.00672840425251
0.101133715563 0.00676861416633
0.102739012636 0.00680909021437
0.104344309708 0.00684983440802
0.105949606781 0.00689084877645
0.107554903853 0.00693213536677
0.109160200926 0.00697369624427
0.110765497998 0.00701553349252
0.11237079507 0.00705764921366
0.113976092143 0.00710004552852
0.115581389215 0.00714272457686
0.117186686288 0.00718568851756
0.11879198336 0.00722893952882
0.120397280433 0.00727247980833
0.122002577505 0.00731631157356
0.123607874577 0.00736043706188
0.12521317165 0.00740485853082
0.126818468722 0.00744957825829
0.128423765795 0.00749459854278
0.130029062867 0.00753992170356
0.13163435994 0.00758555008095
0.133239657012 0.00763148603652
0.134844954085 0.00767773195331
0.136450251157 0.00772429023609
0.138055548229 0.00777116331157
0.139660845302 0.00781835362863
0.141266142374 0.00786586365859
0.142871439447 0.00791369589545
0.144476736519 0.00796185285611
0.146082033592 0.00801033708063
0.147687330664 0.0080591511325
0.149292627736 0.0081082975989
0.150897924809 0.00815777909091
0.152503221881 0.00820759824383
0.154108518954 0.00825775771743
0.155713816026 0.00830826019621
0.157319113099 0.00835910838967
0.158924410171 0.00841030503259
0.160529707243 0.00846185288535
0.162135004316 0.00851375473415
0.163740301388 0.00856601339132
0.165345598461 0.00861863169566
0.166950895533 0.00867161251266
0.168556192606 0.00872495873485
0.170161489678 0.0087786732821
0.171766786751 0.0088327591019
0.173372083823 0.00888721916969
0.174977380895 0.0089420564892
0.176582677968 0.0089972740927
0.17818797504 0.00905287504142
0.179793272113 0.0091088624258
0.181398569185 0.00916523936585
0.183003866258 0.00922200901151
0.18460916333 0.00927917454295
0.186214460402 0.00933673917095
0.187819757475 0.00939470613725
0.189425054547 0.00945307871488
0.19103035162 0.00951186020855
0.192635648692 0.00957105395499
0.194240945765 0.00963066332337
0.195846242837 0.0096906917156
0.197451539909 0.00975114256679
0.199056836982 0.00981201934558
0.200662134054 0.00987332555457
0.202267431127 0.00993506473067
0.203872728199 0.00999724044558
0.205478025272 0.0100598563061
0.207083322344 0.0101229159547
0.208688619416 0.0101864230697
0.210293916489 0.0102503813659
0.211899213561 0.010314794595
0.213504510634 0.0103796665458
0.215109807706 0.0104450010451
0.216715104779 0.0105108019578
0.218320401851 0.0105770731872
0.219925698924 0.0106438186759
0.221530995996 0.0107110424062
0.223136293068 0.0107787484003
0.224741590141 0.0108469407207
0.226346887213 0.0109156234714
0.227952184286 0.0109848007976
0.229557481358 0.0110544768866
0.231162778431 0.0111246559682
0.232768075503 0.0111953423154
0.234373372575 0.0112665402447
0.235978669648 0.0113382541166
0.23758396672 0.0114104883364
0.239189263793 0.0114832473547
0.240794560865 0.0115565356677
0.242399857938 0.011630357818
0.24400515501 0.0117047183951
0.245610452082 0.0117796220362
0.247215749155 0.0118550734262
0.248821046227 0.011931077299
0.2504263433 0.0120076384378
0.252031640372 0.0120847616755
0.253636937445 0.0121624518959
0.255242234517 0.0122407140337
0.25684753159 0.0123195530755
0.258452828662 0.0123989740605
0.260058125734 0.012478982081
0.261663422807 0.0125595822831
0.263268719879 0.0126407798676
0.264874016952 0.0127225800903
0.266479314024 0.0128049882632
0.268084611097 0.0128880097547
0.269689908169 0.0129716499908
0.271295205241 0.0130559144555
0.272900502314 0.0131408086918
0.274505799386 0.0132263383022
0.276111096459 0.0133125089499
0.277716393531 0.013399326359
0.279321690604 0.0134867963159
0.280926987676 0.0135749246697
0.282532284748 0.0136637173332
0.284137581821 0.0137531802837
0.285742878893 0.0138433195638
0.287348175966 0.0139341412825
0.288953473038 0.0140256516158
0.290558770111 0.0141178568077
0.292164067183 0.0142107631711
0.293769364256 0.0143043770889
0.295374661328 0.0143987050145
0.2969799584 0.0144937534734
0.298585255473 0.0145895290634
0.300190552545 0.0146860384563
0.301795849618 0.0147832883984
0.30340114669 0.0148812857119
0.305006443763 0.0149800372956
0.306611740835 0.0150795501261
0.308217037907 0.0151798312588
0.30982233498 0.0152808878293
0.311427632052 0.015382727054
0.313032929125 0.0154853562315
0.314638226197 0.0155887827438
0.31624352327 0.0156930140575
0.317848820342 0.0157980577245
0.319454117414 0.0159039213838
0.321059414487 0.0160106127626
0.322664711559 0.016118139677
0.324270008632 0.016226510034
0.325875305704 0.0163357318323
0.327480602777 0.016445813164
0.329085899849 0.0165567622153
0.330691196922 0.0166685872686
0.332296493994 0.0167812967033
0.333901791066 0.0168948989973
0.335507088139 0.0170094027288
0.337112385211 0.0171248165774
0.338717682284 0.0172411493254
0.340322979356 0.0173584098597
0.341928276429 0.0174766071732
0.343533573501 0.0175957503662
0.345138870573 0.0177158486482
0.346744167646 0.0178369113391
0.348349464718 0.0179589478714
0.349954761791 0.0180819677915
0.351560058863 0.0182059807613
0.353165355936 0.0183309965602
0.354770653008 0.0184570250867
0.35637595008 0.0185840763603
0.357981247153 0.018712160523
0.359586544225 0.0188412878416
0.361191841298 0.0189714687092
0.36279713837 0.0191027136474
0.364402435443 0.0192350333079
0.366007732515 0.0193684384749
0.367613029588 0.0195029400668
0.36921832666 0.0196385491385
0.370823623732 0.0197752768833
0.372428920805 0.019913134635
0.374034217877 0.0200521338705
0.37563951495 0.0201922862114
0.377244812022 0.0203336034267
0.378850109095 0.0204760974349
0.380455406167 0.0206197803065
0.382060703239 0.0207646642663
0.383666000312 0.0209107616957
0.385271297384 0.0210580851355
0.386876594457 0.0212066472881
0.388481891529 0.0213564610203
0.390087188602 0.0215075393657
0.391692485674 0.0216598955278
0.393297782746 0.0218135428821
0.394903079819 0.0219684949796
0.396508376891 0.0221247655489
0.398113673964 0.0222823684999
0.399718971036 0.0224413179258
0.401324268109 0.022601628107
0.402929565181 0.0227633135137
0.404534862254 0.022926388809
0.406140159326 0.0230908688524
0.407745456398 0.0232567687026
0.409350753471 0.0234241036213
0.410956050543 0.0235928890763
0.412561347616 0.023763140745
0.414166644688 0.023934874518
0.415771941761 0.0241081065025
0.417377238833 0.0242828530263
0.418982535905 0.0244591306413
0.420587832978 0.0246369561273
0.42219313005 0.0248163464961
0.423798427123 0.0249973189954
0.425403724195 0.0251798911128
0.427009021268 0.0253640805798
0.42861431834 0.0255499053766
0.430219615412 0.0257373837359
0.431824912485 0.0259265341474
0.433430209557 0.0261173753626
0.43503550663 0.0263099263989
0.436640803702 0.0265042065451
0.438246100775 0.0267002353653
0.439851397847 0.0268980327045
0.44145669492 0.0270976186934
0.443061991992 0.0272990137534
0.444667289064 0.027502238602
0.446272586137 0.0277073142582
0.447877883209 0.0279142620477
0.449483180282 0.028123103609
0.451088477354 0.0283338608986
0.452693774427 0.0285465561972
0.454299071499 0.0287612121156
0.455904368571 0.0289778516005
0.457509665644 0.0291964979414
0.459114962716 0.0294171747764
0.460720259789 0.0296399060992
0.462325556861 0.0298647162654
0.463930853934 0.0300916299996
0.465536151006 0.0303206724023
0.467141448078 0.0305518689571
0.468746745151 0.0307852455382
0.470352042223 0.0310208284175
0.471957339296 0.0312586442728
0.473562636368 0.0314987201952
0.475167933441 0.0317410836974
0.476773230513 0.031985762722
0.478378527586 0.0322327856497
0.479983824658 0.0324821813083
0.48158912173 0.032733978981
0.483194418803 0.0329882084161
0.484799715875 0.0332448998359
0.486405012948 0.0335040839464
0.48801031002 0.0337657919467
0.489615607093 0.0340300555396
0.491220904165 0.0342969069412
0.492826201237 0.0345663788919
0.49443149831 0.0348385046668
0.496036795382 0.0351133180868
0.497642092455 0.0353908535303
0.499247389527 0.0356711459441
0.5008526866 0.0359542308558
0.502457983672 0.036240144386
0.504063280744 0.0365289232604
0.505668577817 0.0368206048229
0.507273874889 0.0371152270491
0.508879171962 0.037412828559
0.510484469034 0.0377134486317
0.512089766107 0.038017127219
0.513695063179 0.0383239049604
0.515300360252 0.0386338231981
0.516905657324 0.0389469239919
0.518510954396 0.0392632501358
0.520116251469 0.0395828451735
0.521721548541 0.0399057534157
0.523326845614 0.0402320199568
0.524932142686 0.0405616906928
0.526537439759 0.040894812339
0.528142736831 0.0412314324494
0.529748033903 0.0415715994349
0.531353330976 0.0419153625836
0.532958628048 0.0422627720807
0.534563925121 0.0426138790296
0.536169222193 0.0429687354728
0.537774519266 0.0433273944146
0.539379816338 0.043689909843
0.54098511341 0.0440563367535
0.542590410483 0.0444267311731
0.544195707555 0.0448011501846
0.545801004628 0.0451796519523
0.5474063017 0.0455622957481
0.549011598773 0.0459491419786
0.550616895845 0.0463402522126
0.552222192917 0.0467356892098
0.55382748999 0.0471355169504
0.555432787062 0.0475398006655
0.557038084135 0.0479486068681
0.558643381207 0.0483620033857
0.56024867828 0.0487800593934
0.561853975352 0.0492028454484
0.563459272425 0.0496304335253
0.565064569497 0.0500628970527
0.566669866569 0.0505003109507
0.568275163642 0.0509427516702
0.569880460714 0.0513902972329
0.571485757787 0.0518430272725
0.573091054859 0.052301023078
0.574696351932 0.0527643676379
0.576301649004 0.0532331456855
0.577906946076 0.0537074437465
0.579512243149 0.0541873501881
0.581117540221 0.0546729552688
0.582722837294 0.0551643511912
0.584328134366 0.0556616321558
0.585933431439 0.0561648944169
0.587538728511 0.0566742363405
0.589144025583 0.0571897584637
0.590749322656 0.0577115635575
0.592354619728 0.0582397566901
0.593959916801 0.0587744452939
0.595565213873 0.0593157392341
0.597170510946 0.0598637508801
0.598775808018 0.0604185951793
0.600381105091 0.0609803897342
0.601986402163 0.0615492548814
0.603591699235 0.0621253137742
0.605196996308 0.0627086924686
0.60680229338 0.0632995200116
0.608407590453 0.0638979285337
0.610012887525 0.0645040533445
0.611618184598 0.0651180330324
0.61322348167 0.065740009568
0.614828778742 0.0663701284112
0.616434075815 0.0670085386234
0.618039372887 0.0676553929833
0.61964466996 0.068310848108
0.621249967032 0.0689750645791
0.622855264105 0.0696482070728
0.624460561177 0.0703304444973
0.626065858249 0.0710219501344
0.627671155322 0.0717229017874
0.629276452394 0.0724334819361
0.630881749467 0.0731538778969
0.632487046539 0.0738842819914
0.634092343612 0.0746248917216
0.635697640684 0.0753759099524
0.637302937757 0.076137545103
0.638908234829 0.0769100113464
0.640513531901 0.0776935288183
0.642118828974 0.0784883238346
0.643724126046 0.0792946291204
0.645329423119 0.0801126840482
0.646934720191 0.0809427348879
0.648540017264 0.081785035069
0.650145314336 0.0826398454548
0.651750611408 0.0835074346296
0.653355908481 0.0843880792009
0.654961205553 0.0852820641156
0.656566502626 0.0861896829924
0.658171799698 0.0871112384703
0.659777096771 0.088047042576
0.661382393843 0.0889974171089
0.662987690915 0.0899626940469
0.664592987988 0.0909432159731
0.66619828506 0.0919393365251
0.667803582133 0.0929514208691
0.669408879205 0.0939798461988
0.671014176278 0.0950250022619
0.67261947335 0.0960872919164
0.674224770423 0.0971671317176
0.675830067495 0.0982649525382
0.677435364567 0.099381200225
0.67904066164 0.100516336293
0.680645958712 0.10167083866
0.682251255785 0.102845202427
0.683856552857 0.104039940703
0.68546184993 0.105255585482
0.687067147002 0.106492688576
0.688672444074 0.1077518226
0.690277741147 0.109033582029
0.691883038219 0.110338584316
0.693488335292 0.111667471086
0.695093632364 0.113020909408
0.696698929437 0.114399593155
0.698304226509 0.115804244453
0.699909523581 0.117235615234
0.701514820654 0.118694488894
0.703120117726 0.120181682076
0.704725414799 0.121698046572
0.706330711871 0.123244471376
0.707936008944 0.124821884881
0.709541306016 0.126431257249
0.711146603089 0.128073602962
0.712751900161 0.129749983574
0.714357197233 0.131461510675
0.715962494306 0.133209349114
0.717567791378 0.134994720467
0.719173088451 0.13681890681
0.720778385523 0.138683254814
0.722383682596 0.140589180194
0.723988979668 0.142538172555
0.72559427674 0.144531800682
0.727199573813 0.146571718313
0.728804870885 0.14865967046
0.730410167958 0.150797500347
0.73201546503 0.152987157016
0.733620762103 0.155230703715
0.735226059175 0.157530327141
0.736831356247 0.159888347655
0.73843665332 0.162307230604
0.740041950392 0.164789598891
0.741647247465 0.167338246963
0.743252544537 0.16995615643
0.74485784161 0.172646513536
0.746463138682 0.175412728772
0.748068435755 0.178258458955
0.749673732827 0.181187632153
0.751279029899 0.184204475936
0.752884326972 0.187313549501
0.754489624044 0.19051978033
0.756094921117 0.19382850622
0.757700218189 0.197245523639
0.759305515262 0.200777143649
0.760910812334 0.204430256878
0.762516109406 0.2082124094
0.764121406479 0.212131891873
0.765726703551 0.216197844856
0.767332000624 0.220420384089
0.768937297696 0.224810750559
0.770542594769 0.229381491653
0.772147891841 0.234146681693
0.773753188913 0.239122192889
0.775358485986 0.244326031642
0.776963783058 0.249778760683
0.778569080131 0.255504035607
0.780174377203 0.261529296448
0.781779674276 0.267886673258
0.783384971348 0.274614193415
0.784990268421 0.281757424669
0.786595565493 0.289371765201
0.788200862565 0.297525726167
0.789806159638 0.306305796458
0.79141145671 0.315823949899
0.793016753783 0.326229825915
0.794622050855 0.337731798116
0.796227347928 0.350636638072
0.797832645 0.365433578851
0.799437942072 0.383007696634
0.801043239145 0.405387867449


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceProb0pt4.tex <==
-13.5 0.111453299026
-13.473 0.111453299026
-13.446 0.111453299026
-13.419 0.111453299026
-13.392 0.111453299026
-13.365 0.111453299026
-13.338 0.111453299026
-13.311 0.111453299026
-13.284 0.111453299026
-13.257 0.111453299026
-13.23 0.111453299026
-13.203 0.111453299026
-13.176 0.111453299026
-13.149 0.111453299026
-13.122 0.111453299026
-13.095 0.111453299026
-13.068 0.111453299026
-13.041 0.111453299026
-13.014 0.111453299026
-12.987 0.111453299026
-12.96 0.111453299026
-12.933 0.111453299026
-12.906 0.111453299026
-12.879 0.111453299026
-12.852 0.111453299026
-12.825 0.111453299026
-12.798 0.111453299026
-12.771 0.111453299026
-12.744 0.111453299026
-12.717 0.111453299026
-12.69 0.111453299026
-12.663 0.111453299026
-12.636 0.111453299026
-12.609 0.111453299026
-12.582 0.111453299026
-12.555 0.111453299026
-12.528 0.111453299026
-12.501 0.111453299026
-12.474 0.111453299026
-12.447 0.111453299026
-12.42 0.111453299026
-12.393 0.111453299026
-12.366 0.111453299026
-12.339 0.111453299026
-12.312 0.111453299026
-12.285 0.111453299026
-12.258 0.111453299026
-12.231 0.111453299026
-12.204 0.111453299026
-12.177 0.111453299026
-12.15 0.111453299026
-12.123 0.111453299026
-12.096 0.111453299026
-12.069 0.111453299026
-12.042 0.111453299026
-12.015 0.111453299026
-11.988 0.111453299026
-11.961 0.111453299026
-11.934 0.111453299026
-11.907 0.111453299026
-11.88 0.111453299026
-11.853 0.111453299026
-11.826 0.111453299026
-11.799 0.111453299026
-11.772 0.111453299026
-11.745 0.111453299026
-11.718 0.111453299026
-11.691 0.111453299026
-11.664 0.111453299026
-11.637 0.111453299026
-11.61 0.111453299026
-11.583 0.111453299026
-11.556 0.111453299026
-11.529 0.111453299026
-11.502 0.111453299026
-11.475 0.111453299026
-11.448 0.111453299026
-11.421 0.111453299026
-11.394 0.111453299026
-11.367 0.111453299026
-11.34 0.111453299026
-11.313 0.111453299026
-11.286 0.111453299026
-11.259 0.111453299026
-11.232 0.111453299026
-11.205 0.111453299026
-11.178 0.111453299026
-11.151 0.111453299026
-11.124 0.111453299026
-11.097 0.111453299026
-11.07 0.111453299026
-11.043 0.111453299026
-11.016 0.111453299026
-10.989 0.111453299026
-10.962 0.111453299026
-10.935 0.111453299026
-10.908 0.111453299026
-10.881 0.111453299026
-10.854 0.111453299026
-10.827 0.111453299026
-10.8 0.111453299026
-10.773 0.111453299025
-10.746 0.111453299025
-10.719 0.111453299025
-10.692 0.111453299025
-10.665 0.111453299025
-10.638 0.111453299025
-10.611 0.111453299025
-10.584 0.111453299025
-10.557 0.111453299025
-10.53 0.111453299025
-10.503 0.111453299024
-10.476 0.111453299024
-10.449 0.111453299024
-10.422 0.111453299024
-10.395 0.111453299024
-10.368 0.111453299024
-10.341 0.111453299023
-10.314 0.111453299023
-10.287 0.111453299023
-10.26 0.111453299023
-10.233 0.111453299022
-10.206 0.111453299022
-10.179 0.111453299022
-10.152 0.111453299021
-10.125 0.111453299021
-10.098 0.11145329902
-10.071 0.11145329902
-10.044 0.111453299019
-10.017 0.111453299019
-9.99 0.111453299018
-9.963 0.111453299018
-9.936 0.111453299017
-9.909 0.111453299016
-9.882 0.111453299015
-9.855 0.111453299015
-9.828 0.111453299014
-9.801 0.111453299013
-9.774 0.111453299012
-9.747 0.11145329901
-9.72 0.111453299009
-9.693 0.111453299008
-9.666 0.111453299006
-9.639 0.111453299005
-9.612 0.111453299003
-9.585 0.111453299001
-9.558 0.111453298999
-9.531 0.111453298997
-9.504 0.111453298995
-9.477 0.111453298992
-9.45 0.11145329899
-9.423 0.111453298987
-9.396 0.111453298984
-9.369 0.11145329898
-9.342 0.111453298977
-9.315 0.111453298973
-9.288 0.111453298969
-9.261 0.111453298964
-9.234 0.111453298959
-9.207 0.111453298954
-9.18 0.111453298948
-9.153 0.111453298942
-9.126 0.111453298936
-9.099 0.111453298929
-9.072 0.111453298921
-9.045 0.111453298913
-9.018 0.111453298904
-8.991 0.111453298895
-8.964 0.111453298884
-8.937 0.111453298873
-8.91 0.111453298861
-8.883 0.111453298848
-8.856 0.111453298835
-8.829 0.11145329882
-8.802 0.111453298804
-8.775 0.111453298786
-8.748 0.111453298768
-8.721 0.111453298747
-8.694 0.111453298726
-8.667 0.111453298702
-8.64 0.111453298677
-8.613 0.11145329865
-8.586 0.111453298621
-8.559 0.111453298589
-8.532 0.111453298556
-8.505 0.111453298519
-8.478 0.11145329848
-8.451 0.111453298437
-8.424 0.111453298392
-8.397 0.111453298342
-8.37 0.111453298289
-8.343 0.111453298232
-8.316 0.111453298171
-8.289 0.111453298105
-8.262 0.111453298033
-8.235 0.111453297957
-8.208 0.111453297874
-8.181 0.111453297785
-8.154 0.111453297689
-8.127 0.111453297585
-8.1 0.111453297474
-8.073 0.111453297354
-8.046 0.111453297225
-8.019 0.111453297086
-7.992 0.111453296937
-7.965 0.111453296776
-7.938 0.111453296602
-7.911 0.111453296415
-7.884 0.111453296214
-7.857 0.111453295997
-7.83 0.111453295764
-7.803 0.111453295513
-7.776 0.111453295243
-7.749 0.111453294952
-7.722 0.111453294639
-7.695 0.111453294301
-7.668 0.111453293938
-7.641 0.111453293548
-7.614 0.111453293127
-7.587 0.111453292674
-7.56 0.111453292187
-7.533 0.111453291662
-7.506 0.111453291097
-7.479 0.11145329049
-7.452 0.111453289836
-7.425 0.111453289132
-7.398 0.111453288374
-7.371 0.111453287559
-7.344 0.111453286682
-7.317 0.111453285738
-7.29 0.111453284722
-7.263 0.111453283629
-7.236 0.111453282452
-7.209 0.111453281187
-7.182 0.111453279825
-7.155 0.11145327836
-7.128 0.111453276784
-7.101 0.111453275088
-7.074 0.111453273263
-7.047 0.111453271301
-7.02 0.11145326919
-6.993 0.111453266919
-6.966 0.111453264476
-6.939 0.111453261848
-6.912 0.111453259022
-6.885 0.111453255982
-6.858 0.111453252712
-6.831 0.111453249196
-6.804 0.111453245414
-6.777 0.111453241347
-6.75 0.111453236974
-6.723 0.111453232271
-6.696 0.111453227214
-6.669 0.111453221776
-6.642 0.111453215929
-6.615 0.111453209643
-6.588 0.111453202884
-6.561 0.111453195617
-6.534 0.111453187805
-6.507 0.111453179407
-6.48 0.111453170379
-6.453 0.111453160674
-6.426 0.111453150242
-6.399 0.11145313903
-6.372 0.111453126978
-6.345 0.111453114025
-6.318 0.111453100104
-6.291 0.111453085143
-6.264 0.111453069065
-6.237 0.111453051788
-6.21 0.111453033222
-6.183 0.111453013273
-6.156 0.111452991838
-6.129 0.111452968807
-6.102 0.111452944064
-6.075 0.111452917481
-6.048 0.111452888923
-6.021 0.111452858245
-5.994 0.111452825291
-5.967 0.111452789893
-5.94 0.111452751872
-5.913 0.111452711036
-5.886 0.111452667177
-5.859 0.111452620076
-5.832 0.111452569493
-5.805 0.111452515175
-5.778 0.111452456849
-5.751 0.11145239422
-5.724 0.111452326977
-5.697 0.111452254782
-5.67 0.111452177274
-5.643 0.111452094067
-5.616 0.111452004745
-5.589 0.111451908866
-5.562 0.111451805951
-5.535 0.111451695493
-5.508 0.111451576942
-5.481 0.111451449714
-5.454 0.111451313181
-5.427 0.111451166669
-5.4 0.11145100946
-5.373 0.11145084078
-5.346 0.111450659803
-5.319 0.111450465644
-5.292 0.111450257355
-5.265 0.11145003392
-5.238 0.111449794253
-5.211 0.111449537188
-5.184 0.111449261481
-5.157 0.111448965796
-5.13 0.111448648707
-5.103 0.111448308685
-5.076 0.111447944093
-5.049 0.111447553183
-5.022 0.11144713408
-4.995 0.111446684782
-4.968 0.111446203144
-4.941 0.111445686872
-4.914 0.111445133515
-4.887 0.111444540449
-4.86 0.111443904867
-4.833 0.11144322377
-4.806 0.111442493951
-4.779 0.111441711979
-4.752 0.111440874189
-4.725 0.111439976663
-4.698 0.111439015213
-4.671 0.111437985362
-4.644 0.11143688233
-4.617 0.111435701008
-4.59 0.111434435936
-4.563 0.111433081286
-4.536 0.11143163083
-4.509 0.111430077919
-4.482 0.111428415453
-4.455 0.111426635851
-4.428 0.111424731021
-4.401 0.111422692324
-4.374 0.111420510543
-4.347 0.11141817584
-4.32 0.11141567772
-4.293 0.111413004985
-4.266 0.111410145691
-4.239 0.111407087101
-4.212 0.111403815632
-4.185 0.111400316799
-4.158 0.111396575164
-4.131 0.111392574269
-4.104 0.111388296577
-4.077 0.111383723398
-4.05 0.111378834822
-4.023 0.111373609641
-3.996 0.111368025265
-3.969 0.111362057641
-3.942 0.111355681159
-3.915 0.111348868558
-3.888 0.111341590824
-3.861 0.111333817082
-3.834 0.111325514486
-3.807 0.111316648094
-3.78 0.111307180749
-3.753 0.111297072938
-3.726 0.11128628266
-3.699 0.11127476527
-3.672 0.111262473328
-3.645 0.111249356436
-3.618 0.111235361058
-3.591 0.111220430347
-3.564 0.111204503945
-3.537 0.111187517788
-3.51 0.111169403893
-3.483 0.111150090133
-3.456 0.111129500009
-3.429 0.1111075524
-3.402 0.111084161311
-3.375 0.111059235604
-3.348 0.111032678716
-3.321 0.111004388366
-3.294 0.110974256248
-3.267 0.110942167709
-3.24 0.110908001417
-3.213 0.110871629012
-3.186 0.11083291474
-3.159 0.110791715077
-3.132 0.110747878338
-3.105 0.110701244266
-3.078 0.110651643609
-3.051 0.110598897686
-3.024 0.110542817926
-2.997 0.110483205408
-2.97 0.110419850372
-2.943 0.110352531722
-2.916 0.110281016515
-2.889 0.110205059437
-2.862 0.110124402259
-2.835 0.110038773294
-2.808 0.109947886827
-2.781 0.10985144255
-2.754 0.109749124977
-2.727 0.109640602861
-2.7 0.109525528597
-2.673 0.109403537628
-2.646 0.109274247852
-2.619 0.109137259022
-2.592 0.108992152161
-2.565 0.10883848898
-2.538 0.108675811307
-2.511 0.108503640539
-2.484 0.108321477105
-2.457 0.108128799964
-2.43 0.107925066132
-2.403 0.10770971024
-2.376 0.107482144148
-2.349 0.107241756601
-2.322 0.106987912949
-2.295 0.106719954935
-2.268 0.106437200556
-2.241 0.106138944021
-2.214 0.10582445579
-2.187 0.105492982744
-2.16 0.105143748456
-2.133 0.104775953606
-2.106 0.104388776548
-2.079 0.103981374027
-2.052 0.103552882084
-2.025 0.103102417152
-1.998 0.102629077354
-1.971 0.102131944044
-1.944 0.101610083573
-1.917 0.101062549337
-1.89 0.100488384095
-1.863 0.0998866225905
-1.836 0.0992562944944
-1.809 0.0985964276852
-1.782 0.097906051887
-1.755 0.0971842026833
-1.728 0.0964299259234
-1.701 0.095642282538
-1.674 0.0948203537802
-1.647 0.0939632469024
-1.62 0.0930701012828
-1.593 0.0921400950074
-1.566 0.0911724519146
-1.539 0.0901664491018
-1.512 0.0891214248925
-1.485 0.088036787255
-1.458 0.0869120226602
-1.431 0.0857467053582
-1.404 0.0845405070473
-1.377 0.0832932069024
-1.35 0.0820047019197
-1.323 0.0806750175283
-1.296 0.0793043184073
-1.269 0.0778929194418
-1.242 0.0764412967367
-1.215 0.0749500986006
-1.188 0.0734201564017
-1.161 0.0718524951887
-1.134 0.0702483439608
-1.107 0.0686091454651
-1.08 0.0669365653943
-1.053 0.0652325008541
-1.026 0.063499087972
-0.999 0.061738708521
-0.972 0.0599539954435
-0.945 0.0581478371743
-0.918 0.0563233806823
-0.891 0.0544840331839
-0.864 0.0526334625165
-0.837 0.0507755962162
-0.81 0.0489146194017
-0.783 0.0470549716521
-0.756 0.0452013431555
-0.729 0.043358670526
-0.702 0.0415321328245
-0.675 0.0397271484865
-0.648 0.0379493740597
-0.621 0.0362047058994
-0.594 0.0344992862608
-0.567 0.0328395155916
-0.54 0.031232073274
-0.513 0.0296839496355
-0.486 0.02820249277
-0.459 0.0267954746583
-0.432 0.0254711823185
-0.405 0.0242385413806
-0.378 0.0231072817196
-0.351 0.0220881578227
-0.324 0.0211932407326
-0.297 0.0204363041312
-0.27 0.0198333350529
-0.243 0.019403210767
-0.216 0.0191685989761
-0.189 0.0191571609483
-0.162 0.0194031705657
-0.135 0.0199497140962
-0.108 0.0208517211697
-0.081 0.0221802304607
-0.054 0.0240285916123
-0.027 0.026521938745
0.0 0.0298327381143
0.000681100831688 0.0299286288128
0.00136220166338 0.0300248994533
0.00204330249506 0.0301215519528
0.00272440332675 0.0302185882405
0.00340550415844 0.0303160102581
0.00408660499013 0.03041381996
0.00476770582182 0.030512019313
0.0054488066535 0.0306106102967
0.00612990748519 0.0307095949037
0.00681100831688 0.0308089751394
0.00749210914857 0.0309087530223
0.00817320998026 0.0310089305842
0.00885431081194 0.03110950987
0.00953541164363 0.031210492938
0.0102165124753 0.0313118818602
0.010897613307 0.031413678722
0.0115787141387 0.0315158856225
0.0122598149704 0.0316185046748
0.0129409158021 0.0317215380059
0.0136220166338 0.0318249877567
0.0143031174654 0.0319288560825
0.0149842182971 0.0320331451527
0.0156653191288 0.0321378571513
0.0163464199605 0.0322429942767
0.0170275207922 0.032348558742
0.0177086216239 0.0324545527751
0.0183897224556 0.0325609786188
0.0190708232873 0.0326678385308
0.019751924119 0.0327751347843
0.0204330249506 0.0328828696674
0.0211141257823 0.0329910454838
0.021795226614 0.0330996645526
0.0224763274457 0.0332087292089
0.0231574282774 0.0333182418032
0.0238385291091 0.0334282047022
0.0245196299408 0.0335386202886
0.0252007307725 0.0336494909614
0.0258818316041 0.0337608191358
0.0265629324358 0.0338726072436
0.0272440332675 0.0339848577332
0.0279251340992 0.0340975730697
0.0286062349309 0.0342107557354
0.0292873357626 0.0343244082294
0.0299684365943 0.034438533068
0.030649537426 0.0345531327851
0.0313306382576 0.0346682099319
0.0320117390893 0.0347837670774
0.032692839921 0.0348998068084
0.0333739407527 0.0350163317296
0.0340550415844 0.0351333444639
0.0347361424161 0.0352508476526
0.0354172432478 0.0353688439552
0.0360983440795 0.0354873360501
0.0367794449112 0.0356063266342
0.0374605457428 0.0357258184237
0.0381416465745 0.0358458141536
0.0388227474062 0.0359663165784
0.0395038482379 0.0360873284718
0.0401849490696 0.0362088526276
0.0408660499013 0.0363308918588
0.041547150733 0.0364534489989
0.0422282515647 0.0365765269013
0.0429093523963 0.0367001284398
0.043590453228 0.0368242565088
0.0442715540597 0.0369489140234
0.0449526548914 0.0370741039193
0.0456337557231 0.0371998291539
0.0463148565548 0.0373260927052
0.0469959573865 0.0374528975732
0.0476770582182 0.0375802467794
0.0483581590498 0.037708143367
0.0490392598815 0.0378365904015
0.0497203607132 0.0379655909706
0.0504014615449 0.0380951481844
0.0510825623766 0.0382252651758
0.0517636632083 0.0383559451005
0.05244476404 0.0384871911374
0.0531258648717 0.0386190064885
0.0538069657034 0.0387513943797
0.054488066535 0.0388843580603
0.0551691673667 0.0390179008037
0.0558502681984 0.0391520259076
0.0565313690301 0.039286736694
0.0572124698618 0.0394220365096
0.0578935706935 0.039557928726
0.0585746715252 0.0396944167398
0.0592557723569 0.0398315039732
0.0599368731885 0.0399691938737
0.0606179740202 0.0401074899149
0.0612990748519 0.0402463955962
0.0619801756836 0.0403859144437
0.0626612765153 0.0405260500098
0.063342377347 0.0406668058738
0.0640234781787 0.0408081856422
0.0647045790104 0.0409501929487
0.065385679842 0.0410928314546
0.0660667806737 0.0412361048494
0.0667478815054 0.0413800168504
0.0674289823371 0.0415245712034
0.0681100831688 0.0416697716831
0.0687911840005 0.0418156220929
0.0694722848322 0.0419621262656
0.0701533856639 0.0421092880637
0.0708344864956 0.0422571113793
0.0715155873272 0.0424056001346
0.0721966881589 0.0425547582826
0.0728777889906 0.0427045898066
0.0735588898223 0.0428550987212
0.074239990654 0.0430062890721
0.0749210914857 0.043158164937
0.0756021923174 0.0433107304253
0.0762832931491 0.0434639896786
0.0769643939807 0.0436179468715
0.0776454948124 0.0437726062111
0.0783265956441 0.043927971938
0.0790076964758 0.0440840483263
0.0796887973075 0.0442408396842
0.0803698981392 0.0443983503539
0.0810509989709 0.0445565847126
0.0817320998026 0.0447155471721
0.0824132006342 0.0448752421797
0.0830943014659 0.0450356742185
0.0837754022976 0.0451968478075
0.0844565031293 0.0453587675022
0.085137603961 0.0455214378948
0.0858187047927 0.0456848636149
0.0864998056244 0.0458490493294
0.0871809064561 0.0460139997434
0.0878620072878 0.0461797196002
0.0885431081194 0.0463462136819
0.0892242089511 0.0465134868097
0.0899053097828 0.0466815438444
0.0905864106145 0.0468503896868
0.0912675114462 0.047020029278
0.0919486122779 0.0471904676
0.0926297131096 0.047361709676
0.0933108139413 0.047533760571
0.0939919147729 0.047706625392
0.0946730156046 0.0478803092886
0.0953541164363 0.0480548174534
0.096035217268 0.0482301551226
0.0967163180997 0.0484063275762
0.0973974189314 0.0485833401387
0.0980785197631 0.0487611981796
0.0987596205948 0.0489399071135
0.0994407214264 0.0491194724013
0.100121822258 0.0492998995499
0.10080292309 0.0494811941132
0.101484023922 0.0496633616925
0.102165124753 0.049846407937
0.102846225585 0.0500303385444
0.103527326417 0.0502151592613
0.104208427248 0.0504008758837
0.10488952808 0.0505874942577
0.105570628912 0.0507750202802
0.106251729743 0.0509634598989
0.106932830575 0.0511528191136
0.107613931407 0.0513431039761
0.108295032238 0.0515343205913
0.10897613307 0.0517264751174
0.109657233902 0.0519195737668
0.110338334733 0.0521136228067
0.111019435565 0.0523086285593
0.111700536397 0.052504597403
0.112381637229 0.0527015357726
0.11306273806 0.0528994501603
0.113743838892 0.0530983471161
0.114424939724 0.0532982332483
0.115106040555 0.0534991152247
0.115787141387 0.0537009997729
0.116468242219 0.053903893681
0.11714934305 0.0541078037983
0.117830443882 0.0543127370364
0.118511544714 0.0545187003693
0.119192645545 0.0547257008345
0.119873746377 0.0549337455337
0.120554847209 0.0551428416337
0.12123594804 0.0553529963666
0.121917048872 0.0555642170313
0.122598149704 0.0557765109938
0.123279250536 0.0559898856883
0.123960351367 0.0562043486176
0.124641452199 0.0564199073545
0.125322553031 0.056636569542
0.126003653862 0.0568543428947
0.126684754694 0.0570732351993
0.127365855526 0.0572932543156
0.128046956357 0.0575144081773
0.128728057189 0.0577367047932
0.129409158021 0.0579601522476
0.130090258852 0.0581847587016
0.130771359684 0.0584105323941
0.131452460516 0.0586374816423
0.132133561347 0.0588656148433
0.132814662179 0.0590949404744
0.133495763011 0.0593254670947
0.134176863843 0.0595572033457
0.134857964674 0.0597901579525
0.135539065506 0.0600243397249
0.136220166338 0.0602597575583
0.136901267169 0.0604964204349
0.137582368001 0.0607343374248
0.138263468833 0.0609735176869
0.138944569664 0.0612139704703
0.139625670496 0.0614557051154
0.140306771328 0.0616987310549
0.140987872159 0.061943057815
0.141668972991 0.062188695017
0.142350073823 0.0624356523777
0.143031174654 0.0626839397117
0.143712275486 0.0629335669316
0.144393376318 0.06318454405
0.14507447715 0.0634368811807
0.145755577981 0.0636905885398
0.146436678813 0.0639456764469
0.147117779645 0.0642021553271
0.147798880476 0.0644600357118
0.148479981308 0.0647193282402
0.14916108214 0.0649800436611
0.149842182971 0.0652421928338
0.150523283803 0.0655057867301
0.151204384635 0.0657708364355
0.151885485466 0.0660373531507
0.152566586298 0.0663053481934
0.15324768713 0.0665748329998
0.153928787961 0.066845819126
0.154609888793 0.0671183182499
0.155290989625 0.0673923421727
0.155972090457 0.0676679028206
0.156653191288 0.0679450122467
0.15733429212 0.0682236826325
0.158015392952 0.06850392629
0.158696493783 0.0687857556629
0.159377594615 0.0690691833294
0.160058695447 0.0693542220031
0.160739796278 0.0696408845355
0.16142089711 0.0699291839178
0.162101997942 0.0702191332828
0.162783098773 0.070510745907
0.163464199605 0.0708040352126
0.164145300437 0.0710990147697
0.164826401268 0.071395698298
0.1655075021 0.0716940996697
0.166188602932 0.0719942329109
0.166869703764 0.0722961122043
0.167550804595 0.0725997518916
0.168231905427 0.0729051664753
0.168913006259 0.0732123706215
0.16959410709 0.0735213791621
0.170275207922 0.0738322070973
0.170956308754 0.0741448695983
0.171637409585 0.0744593820093
0.172318510417 0.0747757598506
0.172999611249 0.0750940188211
0.17368071208 0.0754141748008
0.174361812912 0.0757362438537
0.175042913744 0.0760602422308
0.175724014576 0.0763861863722
0.176405115407 0.076714092911
0.177086216239 0.0770439786753
0.177767317071 0.077375860692
0.178448417902 0.0777097561891
0.179129518734 0.0780456825997
0.179810619566 0.0783836575642
0.180491720397 0.0787236989343
0.181172821229 0.0790658247759
0.181853922061 0.0794100533729
0.182535022892 0.07975640323
0.183216123724 0.0801048930768
0.183897224556 0.0804555418708
0.184578325387 0.0808083688018
0.185259426219 0.0811633932949
0.185940527051 0.0815206350146
0.186621627883 0.0818801138687
0.187302728714 0.0822418500123
0.187983829546 0.0826058638515
0.188664930378 0.0829721760479
0.189346031209 0.0833408075225
0.190027132041 0.0837117794604
0.190708232873 0.0840851133145
0.191389333704 0.0844608308107
0.192070434536 0.0848389539517
0.192751535368 0.0852195050224
0.193432636199 0.0856025065941
0.194113737031 0.0859879815296
0.194794837863 0.0863759529882
0.195475938694 0.0867664444304
0.196157039526 0.0871594796234
0.196838140358 0.0875550826465
0.19751924119 0.087953277896
0.198200342021 0.0883540900912
0.198881442853 0.0887575442795
0.199562543685 0.0891636658428
0.200243644516 0.0895724805028
0.200924745348 0.0899840143274
0.20160584618 0.0903982937367
0.202286947011 0.090815345509
0.202968047843 0.0912351967877
0.203649148675 0.0916578750877
0.204330249506 0.0920834083017
0.205011350338 0.0925118247079
0.20569245117 0.0929431529762
0.206373552001 0.0933774221757
0.207054652833 0.0938146617823
0.207735753665 0.0942549016857
0.208416854497 0.0946981721975
0.209097955328 0.095144504059
0.20977905616 0.0955939284491
0.210460156992 0.0960464769928
0.211141257823 0.0965021817691
0.211822358655 0.0969610753206
0.212503459487 0.0974231906612
0.213184560318 0.0978885612863
0.21386566115 0.0983572211811
0.214546761982 0.0988292048307
0.215227862813 0.0993045472299
0.215908963645 0.0997832838925
0.216590064477 0.100265450863
0.217271165308 0.100751084724
0.21795226614 0.101240222611
0.218633366972 0.101732902222
0.219314467804 0.102229161826
0.219995568635 0.102729040278
0.220676669467 0.10323257703
0.221357770299 0.103739812142
0.22203887113 0.104250786297
0.222719971962 0.104765540809
0.223401072794 0.105284117644
0.224082173625 0.105806559425
0.224763274457 0.106332909452
0.225444375289 0.106863211712
0.22612547612 0.107397510897
0.226806576952 0.107935852417
0.227487677784 0.108478282416
0.228168778615 0.109024847788
0.228849879447 0.109575596192
0.229530980279 0.110130576072
0.230212081111 0.110689836669
0.230893181942 0.111253428044
0.231574282774 0.111821401091
0.232255383606 0.112393807561
0.232936484437 0.112970700076
0.233617585269 0.113552132153
0.234298686101 0.114138158221
0.234979786932 0.114728833643
0.235660887764 0.11532421474
0.236341988596 0.115924358809
0.237023089427 0.116529324146
0.237704190259 0.117139170074
0.238385291091 0.117753956961
0.239066391922 0.118373746251
0.239747492754 0.118998600483
0.240428593586 0.119628583323
0.241109694418 0.120263759588
0.241790795249 0.120904195274
0.242471896081 0.121549957587
0.243152996913 0.12220111497
0.243834097744 0.122857737136
0.244515198576 0.123519895098
0.245196299408 0.124187661203
0.245877400239 0.124861109163
0.246558501071 0.125540314093
0.247239601903 0.126225352545
0.247920702734 0.126916302546
0.248601803566 0.127613243636
0.249282904398 0.128316256904
0.249964005229 0.129025425038
0.250645106061 0.129740832355
0.251326206893 0.130462564855
0.252007307725 0.13119071026
0.252688408556 0.131925358064
0.253369509388 0.132666599579
0.25405061022 0.133414527985
0.254731711051 0.134169238384
0.255412811883 0.134930827851
0.256093912715 0.135699395491
0.256775013546 0.136475042495
0.257456114378 0.1372578722
0.25813721521 0.138047990152
0.258818316041 0.138845504169
0.259499416873 0.139650524404
0.260180517705 0.140463163421
0.260861618536 0.141283536259
0.261542719368 0.142111760509
0.2622238202 0.142947956392
0.262904921032 0.143792246839
0.263586021863 0.144644757568
0.264267122695 0.14550561718
0.264948223527 0.146374957238
0.265629324358 0.147252912371
0.26631042519 0.14813962036
0.266991526022 0.149035222247
0.267672626853 0.149939862435
0.268353727685 0.150853688801
0.269034828517 0.151776852807
0.269715929348 0.152709509618
0.27039703018 0.15365181823
0.271078131012 0.154603941594
0.271759231844 0.155566046753
0.272440332675 0.156538304982
0.273121433507 0.157520891932
0.273802534339 0.15851398779
0.27448363517 0.15951777743
0.275164736002 0.160532450587
0.275845836834 0.161558202028
0.276526937665 0.162595231738
0.277208038497 0.163643745106
0.277889139329 0.164703953135
0.27857024016 0.165776072641
0.279251340992 0.166860326483
0.279932441824 0.167956943786
0.280613542655 0.169066160191
0.281294643487 0.170188218104
0.281975744319 0.171323366963
0.282656845151 0.172471863526
0.283337945982 0.173633972156
0.284019046814 0.174809965142
0.284700147646 0.176000123018
0.285381248477 0.177204734914
0.286062349309 0.178424098915
0.286743450141 0.179658522449
0.287424550972 0.180908322684
0.288105651804 0.182173826963
0.288786752636 0.183455373251
0.289467853467 0.184753310614
0.290148954299 0.186067999721
0.290830055131 0.187399813385
0.291511155962 0.188749137123
0.292192256794 0.190116369761
0.292873357626 0.191501924073
0.293554458458 0.192906227455
0.294235559289 0.19432972265
0.294916660121 0.195772868511
0.295597760953 0.197236140819
0.296278861784 0.198720033156
0.296959962616 0.200225057829
0.297641063448 0.201751746864
0.298322164279 0.203300653066
0.299003265111 0.204872351155
0.299684365943 0.206467438977
0.300365466774 0.208086538813
0.301046567606 0.20973029877
0.301727668438 0.211399394291
0.302408769269 0.213094529773
0.303089870101 0.214816440302
0.303770970933 0.216565893542
0.304452071765 0.218343691762
0.305133172596 0.220150674033
0.305814273428 0.221987718608
0.30649537426 0.2238557455
0.307176475091 0.225755719292
0.307857575923 0.227688652184
0.308538676755 0.22965560732
0.309219777586 0.23165770242
0.309900878418 0.233696113752
0.31058197925 0.235772080485
0.311263080081 0.237886909465
0.311944180913 0.240041980478
0.312625281745 0.242238752042
0.313306382576 0.244478767817
0.313987483408 0.246763663697
0.31466858424 0.249095175687
0.315349685072 0.251475148676
0.316030785903 0.253905546216
0.316711886735 0.256388461485
0.317392987567 0.258926129579
0.318074088398 0.261520941366
0.31875518923 0.264175459136
0.319436290062 0.266892434349
0.320117390893 0.269674827838
0.320798491725 0.272525832895
0.321479592557 0.275448901766
0.322160693388 0.278447776202
0.32284179422 0.281526522837
0.323522895052 0.284689574405
0.324203995883 0.287941777989
0.324885096715 0.291288451868
0.325566197547 0.29473545292
0.326247298379 0.298289257113
0.32692839921 0.301957056348
0.327609500042 0.305746875975
0.328290600874 0.309667718687
0.328971701705 0.313729742516
0.329652802537 0.31794448347
0.330333903369 0.322325137504
0.3310150042 0.326886922627
0.331696105032 0.331647551286
0.332377205864 0.336627857701
0.333058306695 0.341852648195
0.333739407527 0.347351881479
0.334420508359 0.353162353155
0.33510160919 0.359330180941
0.335782710022 0.365914621695
0.336463810854 0.372994233639
0.337144911686 0.380677477901
0.337826012517 0.389122560895
0.338507113349 0.39857921643
0.339188214181 0.409493969698
0.339869315012 0.422875621575


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceProb0pt5.tex <==
-13.5 0.115161735767
-13.473 0.115161735767
-13.446 0.115161735767
-13.419 0.115161735767
-13.392 0.115161735767
-13.365 0.115161735767
-13.338 0.115161735767
-13.311 0.115161735767
-13.284 0.115161735767
-13.257 0.115161735767
-13.23 0.115161735767
-13.203 0.115161735767
-13.176 0.115161735767
-13.149 0.115161735767
-13.122 0.115161735767
-13.095 0.115161735767
-13.068 0.115161735767
-13.041 0.115161735767
-13.014 0.115161735767
-12.987 0.115161735767
-12.96 0.115161735767
-12.933 0.115161735767
-12.906 0.115161735767
-12.879 0.115161735767
-12.852 0.115161735767
-12.825 0.115161735767
-12.798 0.115161735767
-12.771 0.115161735767
-12.744 0.115161735767
-12.717 0.115161735767
-12.69 0.115161735767
-12.663 0.115161735767
-12.636 0.115161735767
-12.609 0.115161735767
-12.582 0.115161735767
-12.555 0.115161735767
-12.528 0.115161735767
-12.501 0.115161735767
-12.474 0.115161735767
-12.447 0.115161735767
-12.42 0.115161735767
-12.393 0.115161735767
-12.366 0.115161735767
-12.339 0.115161735767
-12.312 0.115161735767
-12.285 0.115161735767
-12.258 0.115161735767
-12.231 0.115161735767
-12.204 0.115161735767
-12.177 0.115161735767
-12.15 0.115161735767
-12.123 0.115161735767
-12.096 0.115161735767
-12.069 0.115161735767
-12.042 0.115161735767
-12.015 0.115161735767
-11.988 0.115161735767
-11.961 0.115161735767
-11.934 0.115161735767
-11.907 0.115161735767
-11.88 0.115161735767
-11.853 0.115161735767
-11.826 0.115161735767
-11.799 0.115161735767
-11.772 0.115161735767
-11.745 0.115161735767
-11.718 0.115161735767
-11.691 0.115161735767
-11.664 0.115161735767
-11.637 0.115161735767
-11.61 0.115161735767
-11.583 0.115161735767
-11.556 0.115161735767
-11.529 0.115161735767
-11.502 0.115161735767
-11.475 0.115161735767
-11.448 0.115161735767
-11.421 0.115161735767
-11.394 0.115161735767
-11.367 0.115161735767
-11.34 0.115161735767
-11.313 0.115161735767
-11.286 0.115161735767
-11.259 0.115161735767
-11.232 0.115161735767
-11.205 0.115161735767
-11.178 0.115161735767
-11.151 0.115161735767
-11.124 0.115161735767
-11.097 0.115161735767
-11.07 0.115161735767
-11.043 0.115161735767
-11.016 0.115161735767
-10.989 0.115161735767
-10.962 0.115161735767
-10.935 0.115161735767
-10.908 0.115161735767
-10.881 0.115161735767
-10.854 0.115161735767
-10.827 0.115161735767
-10.8 0.115161735766
-10.773 0.115161735766
-10.746 0.115161735766
-10.719 0.115161735766
-10.692 0.115161735766
-10.665 0.115161735766
-10.638 0.115161735766
-10.611 0.115161735766
-10.584 0.115161735766
-10.557 0.115161735766
-10.53 0.115161735766
-10.503 0.115161735766
-10.476 0.115161735765
-10.449 0.115161735765
-10.422 0.115161735765
-10.395 0.115161735765
-10.368 0.115161735765
-10.341 0.115161735765
-10.314 0.115161735765
-10.287 0.115161735764
-10.26 0.115161735764
-10.233 0.115161735764
-10.206 0.115161735764
-10.179 0.115161735763
-10.152 0.115161735763
-10.125 0.115161735763
-10.098 0.115161735762
-10.071 0.115161735762
-10.044 0.115161735762
-10.017 0.115161735761
-9.99 0.115161735761
-9.963 0.11516173576
-9.936 0.115161735759
-9.909 0.115161735759
-9.882 0.115161735758
-9.855 0.115161735758
-9.828 0.115161735757
-9.801 0.115161735756
-9.774 0.115161735755
-9.747 0.115161735754
-9.72 0.115161735753
-9.693 0.115161735752
-9.666 0.115161735751
-9.639 0.11516173575
-9.612 0.115161735748
-9.585 0.115161735747
-9.558 0.115161735745
-9.531 0.115161735743
-9.504 0.115161735741
-9.477 0.115161735739
-9.45 0.115161735737
-9.423 0.115161735735
-9.396 0.115161735732
-9.369 0.11516173573
-9.342 0.115161735727
-9.315 0.115161735724
-9.288 0.11516173572
-9.261 0.115161735717
-9.234 0.115161735713
-9.207 0.115161735708
-9.18 0.115161735704
-9.153 0.115161735699
-9.126 0.115161735693
-9.099 0.115161735688
-9.072 0.115161735682
-9.045 0.115161735675
-9.018 0.115161735668
-8.991 0.11516173566
-8.964 0.115161735651
-8.937 0.115161735642
-8.91 0.115161735633
-8.883 0.115161735622
-8.856 0.115161735611
-8.829 0.115161735599
-8.802 0.115161735586
-8.775 0.115161735572
-8.748 0.115161735556
-8.721 0.11516173554
-8.694 0.115161735522
-8.667 0.115161735503
-8.64 0.115161735483
-8.613 0.115161735461
-8.586 0.115161735437
-8.559 0.115161735411
-8.532 0.115161735384
-8.505 0.115161735354
-8.478 0.115161735322
-8.451 0.115161735287
-8.424 0.11516173525
-8.397 0.11516173521
-8.37 0.115161735167
-8.343 0.11516173512
-8.316 0.11516173507
-8.289 0.115161735016
-8.262 0.115161734958
-8.235 0.115161734895
-8.208 0.115161734828
-8.181 0.115161734755
-8.154 0.115161734677
-8.127 0.115161734592
-8.1 0.115161734501
-8.073 0.115161734404
-8.046 0.115161734298
-8.019 0.115161734185
-7.992 0.115161734063
-7.965 0.115161733931
-7.938 0.115161733789
-7.911 0.115161733637
-7.884 0.115161733473
-7.857 0.115161733296
-7.83 0.115161733105
-7.803 0.1151617329
-7.776 0.11516173268
-7.749 0.115161732442
-7.722 0.115161732186
-7.695 0.11516173191
-7.668 0.115161731614
-7.641 0.115161731295
-7.614 0.115161730951
-7.587 0.115161730581
-7.56 0.115161730182
-7.533 0.115161729754
-7.506 0.115161729292
-7.479 0.115161728795
-7.452 0.115161728261
-7.425 0.115161727685
-7.398 0.115161727066
-7.371 0.115161726399
-7.344 0.115161725682
-7.317 0.115161724909
-7.29 0.115161724079
-7.263 0.115161723184
-7.236 0.115161722222
-7.209 0.115161721187
-7.182 0.115161720073
-7.155 0.115161718874
-7.128 0.115161717584
-7.101 0.115161716196
-7.074 0.115161714703
-7.047 0.115161713096
-7.02 0.115161711368
-6.993 0.115161709509
-6.966 0.115161707508
-6.939 0.115161705357
-6.912 0.115161703042
-6.885 0.115161700553
-6.858 0.115161697875
-6.831 0.115161694994
-6.804 0.115161691896
-6.777 0.115161688564
-6.75 0.115161684981
-6.723 0.115161681127
-6.696 0.115161676982
-6.669 0.115161672525
-6.642 0.115161667733
-6.615 0.115161662579
-6.588 0.115161657037
-6.561 0.115161651079
-6.534 0.115161644673
-6.507 0.115161637785
-6.48 0.11516163038
-6.453 0.11516162242
-6.426 0.115161613862
-6.399 0.115161604662
-6.372 0.115161594773
-6.345 0.115161584143
-6.318 0.115161572717
-6.291 0.115161560437
-6.264 0.115161547238
-6.237 0.115161533053
-6.21 0.115161517809
-6.183 0.115161501426
-6.156 0.115161483822
-6.129 0.115161464905
-6.102 0.115161444578
-6.075 0.115161422738
-6.048 0.115161399272
-6.021 0.115161374061
-5.994 0.115161346976
-5.967 0.11516131788
-5.94 0.115161286623
-5.913 0.115161253047
-5.886 0.115161216983
-5.859 0.115161178246
-5.832 0.115161136641
-5.805 0.115161091958
-5.778 0.115161043971
-5.751 0.115160992438
-5.724 0.1151609371
-5.697 0.115160877679
-5.67 0.115160813876
-5.643 0.115160745373
-5.616 0.115160671825
-5.589 0.115160592867
-5.562 0.115160508103
-5.535 0.115160417112
-5.508 0.115160319441
-5.481 0.115160214605
-5.454 0.115160102086
-5.427 0.115159981325
-5.4 0.115159851727
-5.373 0.115159712651
-5.346 0.115159563415
-5.319 0.115159403282
-5.292 0.115159231469
-5.265 0.115159047133
-5.238 0.115158849374
-5.211 0.115158637224
-5.184 0.115158409652
-5.157 0.11515816555
-5.13 0.115157903733
-5.103 0.115157622933
-5.076 0.115157321792
-5.049 0.115156998856
-5.022 0.115156652569
-4.995 0.115156281267
-4.968 0.115155883168
-4.941 0.115155456365
-4.914 0.11515499882
-4.887 0.11515450835
-4.86 0.115153982621
-4.833 0.115153419137
-4.806 0.115152815228
-4.779 0.115152168039
-4.752 0.115151474516
-4.725 0.115150731396
-4.698 0.11514993519
-4.671 0.115149082166
-4.644 0.115148168337
-4.617 0.115147189444
-4.59 0.115146140933
-4.563 0.115145017937
-4.536 0.11514381526
-4.509 0.115142527349
-4.482 0.115141148274
-4.455 0.115139671699
-4.428 0.115138090862
-4.401 0.11513639854
-4.374 0.115134587022
-4.347 0.115132648078
-4.32 0.115130572924
-4.293 0.115128352183
-4.266 0.115125975853
-4.239 0.115123433259
-4.212 0.115120713017
-4.185 0.115117802981
-4.158 0.115114690201
-4.131 0.115111360866
-4.104 0.115107800252
-4.077 0.115103992664
-4.05 0.115099921372
-4.023 0.115095568549
-3.996 0.115090915199
-3.969 0.115085941087
-3.942 0.115080624657
-3.915 0.115074942955
-3.888 0.115068871537
-3.861 0.115062384383
-3.834 0.115055453793
-3.807 0.115048050291
-3.78 0.115040142511
-3.753 0.115031697087
-3.726 0.115022678528
-3.699 0.115013049095
-3.672 0.11500276866
-3.645 0.11499179457
-3.618 0.114980081494
-3.591 0.114967581265
-3.564 0.114954242716
-3.537 0.114940011503
-3.51 0.114924829923
-3.483 0.114908636718
-3.456 0.114891366874
-3.429 0.114872951406
-3.402 0.114853317135
-3.375 0.11483238645
-3.348 0.114810077067
-3.321 0.114786301764
-3.294 0.114760968114
-3.267 0.114733978204
-3.24 0.114705228333
-3.213 0.114674608709
-3.186 0.114642003122
-3.159 0.114607288612
-3.132 0.114570335113
-3.105 0.114531005092
-3.078 0.114489153166
-3.051 0.114444625714
-3.024 0.114397260459
-2.997 0.114346886051
-2.97 0.114293321626
-2.943 0.114236376351
-2.916 0.114175848956
-2.889 0.114111527253
-2.862 0.114043187638
-2.835 0.113970594581
-2.808 0.113893500102
-2.781 0.113811643236
-2.754 0.113724749489
-2.727 0.113632530276
-2.7 0.113534682362
-2.673 0.113430887284
-2.646 0.113320810775
-2.619 0.113204102182
-2.592 0.113080393883
-2.565 0.112949300703
-2.538 0.112810419337
-2.511 0.112663327781
-2.484 0.11250758477
-2.457 0.112342729235
-2.43 0.112168279776
-2.403 0.111983734163
-2.376 0.111788568865
-2.349 0.11158223861
-2.322 0.111364176
-2.295 0.11113379116
-2.268 0.110890471453
-2.241 0.11063358126
-2.214 0.110362461832
-2.187 0.110076431228
-2.16 0.109774784343
-2.133 0.109456793053
-2.106 0.109121706463
-2.079 0.108768751301
-2.052 0.108397132442
-2.025 0.108006033608
-1.998 0.107594618224
-1.971 0.10716203048
-1.944 0.106707396591
-1.917 0.106229826287
-1.89 0.105728414544
-1.863 0.105202243582
-1.836 0.104650385136
-1.809 0.104071903041
-1.782 0.103465856132
-1.755 0.10283130149
-1.728 0.102167298051
-1.701 0.101472910603
-1.674 0.100747214185
-1.647 0.0999892989079
-1.62 0.0991982752305
-1.593 0.0983732796825
-1.566 0.0975134810731
-1.539 0.0966180871888
-1.512 0.0956863519942
-1.485 0.0947175833449
-1.458 0.093711151218
-1.431 0.0926664964633
-1.404 0.0915831400716
-1.377 0.0904606929544
-1.35 0.0892988662222
-1.323 0.0880974819448
-1.296 0.0868564843683
-1.269 0.0855759515604
-1.242 0.0842561074465
-1.215 0.0828973341933
-1.188 0.0815001848911
-1.161 0.0800653964774
-1.134 0.078593902843
-1.107 0.0770868480531
-1.08 0.0755455996175
-1.053 0.0739717617398
-1.026 0.0723671884829
-0.999 0.0707339967896
-0.972 0.0690745793138
-0.945 0.0673916170328
-0.918 0.0656880916384
-0.891 0.0639672977425
-0.864 0.0622328549797
-0.837 0.0604887201559
-0.81 0.0587391996745
-0.783 0.0569889625817
-0.756 0.0552430547076
-0.729 0.0535069145595
-0.702 0.0517863918421
-0.675 0.0500877697673
-0.648 0.0484177926749
-0.621 0.0467837009482
-0.594 0.0451932758061
-0.567 0.0436548973207
-0.54 0.042177620025
-0.513 0.0407712718078
-0.486 0.0394465835744
-0.459 0.0382153595682
-0.432 0.0370907015455
-0.405 0.0360873045771
-0.378 0.0352218487023
-0.351 0.0345135198864
-0.324 0.0339847071651
-0.297 0.0336619427996
-0.27 0.0335771825306
-0.243 0.0337695701258
-0.216 0.0342879058873
-0.189 0.0351941637479
-0.162 0.0365686164231
-0.135 0.038517513503
-0.108 0.0411849830142
-0.081 0.0447722703979
-0.054 0.04957048755
-0.027 0.0560200272119
0.0 0.0648272482622
0.000383576096602 0.0649742333259
0.000767152193205 0.0651216730413
0.00115072828981 0.0652695693632
0.00153430438641 0.065417924258
0.00191788048301 0.0655667397032
0.00230145657961 0.0657160176881
0.00268503267622 0.0658657602136
0.00306860877282 0.0660159692922
0.00345218486942 0.0661666469484
0.00383576096602 0.0663177952185
0.00421933706263 0.0664694161507
0.00460291315923 0.0666215118055
0.00498648925583 0.0667740842553
0.00537006535243 0.0669271355851
0.00575364144904 0.067080667892
0.00613721754564 0.0672346832857
0.00652079364224 0.0673891838884
0.00690436973884 0.0675441718348
0.00728794583545 0.0676996492727
0.00767152193205 0.0678556183625
0.00805509802865 0.0680120812775
0.00843867412525 0.0681690402043
0.00882225022185 0.0683264973425
0.00920582631846 0.0684844549048
0.00958940241506 0.0686429151175
0.00997297851166 0.0688018802202
0.0103565546083 0.0689613524663
0.0107401307049 0.0691213341226
0.0111237068015 0.0692818274698
0.0115072828981 0.0694428348025
0.0118908589947 0.0696043584293
0.0122744350913 0.0697664006729
0.0126580111879 0.0699289638701
0.0130415872845 0.0700920503723
0.0134251633811 0.0702556625452
0.0138087394777 0.070419802769
0.0141923155743 0.0705844734388
0.0145758916709 0.0707496769641
0.0149594677675 0.0709154157698
0.0153430438641 0.0710816922956
0.0157266199607 0.0712485089962
0.0161101960573 0.071415868342
0.0164937721539 0.0715837728184
0.0168773482505 0.0717522249266
0.0172609243471 0.0719212271832
0.0176445004437 0.072090782121
0.0180280765403 0.0722608922882
0.0184116526369 0.0724315602495
0.0187952287335 0.0726027885856
0.0191788048301 0.0727745798933
0.0195623809267 0.0729469367862
0.0199459570233 0.0731198618942
0.0203295331199 0.0732933578641
0.0207131092165 0.0734674273596
0.0210966853131 0.0736420730611
0.0214802614097 0.0738172976663
0.0218638375063 0.0739931038904
0.0222474136029 0.0741694944657
0.0226309896995 0.0743464721422
0.0230145657961 0.0745240396876
0.0233981418927 0.0747021998875
0.0237817179893 0.0748809555455
0.0241652940859 0.0750603094832
0.0245488701826 0.0752402645409
0.0249324462792 0.075420823577
0.0253160223758 0.0756019894687
0.0256995984724 0.0757837651121
0.026083174569 0.0759661534219
0.0264667506656 0.0761491573323
0.0268503267622 0.0763327797966
0.0272339028588 0.0765170237875
0.0276174789554 0.0767018922975
0.028001055052 0.0768873883385
0.0283846311486 0.0770735149428
0.0287682072452 0.0772602751625
0.0291517833418 0.0774476720702
0.0295353594384 0.0776357087588
0.029918935535 0.0778243883419
0.0303025116316 0.0780137139541
0.0306860877282 0.0782036887507
0.0310696638248 0.0783943159085
0.0314532399214 0.0785855986255
0.031836816018 0.0787775401213
0.0322203921146 0.0789701436373
0.0326039682112 0.0791634124368
0.0329875443078 0.0793573498054
0.0333711204044 0.0795519590507
0.033754696501 0.0797472435033
0.0341382725976 0.0799432065162
0.0345218486942 0.0801398514655
0.0349054247908 0.0803371817503
0.0352890008874 0.0805352007933
0.035672576984 0.0807339120406
0.0360561530806 0.0809333189621
0.0364397291772 0.0811334250518
0.0368233052738 0.0813342338277
0.0372068813704 0.0815357488325
0.037590457467 0.0817379736333
0.0379740335636 0.0819409118223
0.0383576096602 0.0821445670167
0.0387411857568 0.0823489428591
0.0391247618534 0.0825540430176
0.03950833795 0.082759871186
0.0398919140466 0.0829664310845
0.0402754901432 0.0831737264593
0.0406590662399 0.0833817610832
0.0410426423365 0.0835905387556
0.0414262184331 0.0838000633034
0.0418097945297 0.0840103385802
0.0421933706263 0.0842213684676
0.0425769467229 0.0844331568747
0.0429605228195 0.0846457077388
0.0433440989161 0.0848590250255
0.0437276750127 0.0850731127288
0.0441112511093 0.0852879748718
0.0444948272059 0.0855036155066
0.0448784033025 0.0857200387147
0.0452619793991 0.0859372486075
0.0456455554957 0.0861552493259
0.0460291315923 0.0863740450415
0.0464127076889 0.0865936399563
0.0467962837855 0.0868140383031
0.0471798598821 0.0870352443457
0.0475634359787 0.0872572623797
0.0479470120753 0.0874800967322
0.0483305881719 0.0877037517623
0.0487141642685 0.0879282318616
0.0490977403651 0.0881535414543
0.0494813164617 0.0883796849976
0.0498648925583 0.0886066669821
0.0502484686549 0.0888344919319
0.0506320447515 0.0890631644053
0.0510156208481 0.0892926889948
0.0513991969447 0.0895230703274
0.0517827730413 0.0897543130653
0.0521663491379 0.089986421906
0.0525499252345 0.0902194015828
0.0529335013311 0.0904532568648
0.0533170774277 0.0906879925578
0.0537006535243 0.0909236135043
0.0540842296209 0.0911601245838
0.0544678057175 0.0913975307135
0.0548513818141 0.0916358368486
0.0552349579107 0.0918750479823
0.0556185340073 0.0921151691468
0.0560021101039 0.0923562054132
0.0563856862005 0.0925981618922
0.0567692622972 0.0928410437343
0.0571528383938 0.0930848561303
0.0575364144904 0.0933296043118
0.057919990587 0.0935752935514
0.0583035666836 0.0938219291635
0.0586871427802 0.0940695165044
0.0590707188768 0.0943180609726
0.0594542949734 0.0945675680098
0.05983787107 0.0948180431009
0.0602214471666 0.0950694917746
0.0606050232632 0.0953219196038
0.0609885993598 0.0955753322062
0.0613721754564 0.0958297352447
0.061755751553 0.0960851344277
0.0621393276496 0.0963415355099
0.0625229037462 0.0965989442927
0.0629064798428 0.0968573666246
0.0632900559394 0.0971168084016
0.063673632036 0.097377275568
0.0640572081326 0.0976387741169
0.0644407842292 0.0979013100905
0.0648243603258 0.0981648895807
0.0652079364224 0.0984295187298
0.065591512519 0.0986952037308
0.0659750886156 0.0989619508283
0.0663586647122 0.0992297663188
0.0667422408088 0.0994986565511
0.0671258169054 0.0997686279275
0.067509393002 0.100039686904
0.0678929690986 0.10031183999
0.0682765451952 0.100585093751
0.0686601212918 0.100859454808
0.0690436973884 0.101134929837
0.069427273485 0.101411525572
0.0698108495816 0.101689248804
0.0701944256782 0.101968106381
0.0705780017748 0.102248105211
0.0709615778714 0.102529252262
0.071345153968 0.10281155456
0.0717287300646 0.103095019194
0.0721123061612 0.103379653312
0.0724958822578 0.103665464126
0.0728794583545 0.103952458911
0.0732630344511 0.104240645004
0.0736466105477 0.104530029808
0.0740301866443 0.10482062079
0.0744137627409 0.105112425484
0.0747973388375 0.105405451489
0.0751809149341 0.105699706472
0.0755644910307 0.105995198169
0.0759480671273 0.106291934385
0.0763316432239 0.106589922994
0.0767152193205 0.10688917194
0.0770987954171 0.10718968924
0.0774823715137 0.107491482983
0.0778659476103 0.107794561331
0.0782495237069 0.108098932519
0.0786330998035 0.10840460486
0.0790166759001 0.10871158674
0.0794002519967 0.109019886623
0.0797838280933 0.109329513049
0.0801674041899 0.109640474641
0.0805509802865 0.109952780097
0.0809345563831 0.110266438198
0.0813181324797 0.110581457807
0.0817017085763 0.110897847868
0.0820852846729 0.11121561741
0.0824688607695 0.111534775547
0.0828524368661 0.111855331477
0.0832360129627 0.112177294487
0.0836195890593 0.11250067395
0.0840031651559 0.11282547933
0.0843867412525 0.11315172018
0.0847703173491 0.113479406144
0.0851538934457 0.11380854696
0.0855374695423 0.114139152459
0.0859210456389 0.114471232566
0.0863046217355 0.114804797303
0.0866881978321 0.115139856789
0.0870717739287 0.115476421243
0.0874553500253 0.115814500982
0.0878389261219 0.116154106426
0.0882225022185 0.116495248095
0.0886060783151 0.116837936615
0.0889896544118 0.117182182717
0.0893732305084 0.117527997239
0.089756806605 0.117875391125
0.0901403827016 0.118224375431
0.0905239587982 0.118574961324
0.0909075348948 0.11892716008
0.0912911109914 0.119280983094
0.091674687088 0.119636441872
0.0920582631846 0.119993548041
0.0924418392812 0.120352313343
0.0928254153778 0.120712749643
0.0932089914744 0.121074868928
0.093592567571 0.121438683306
0.0939761436676 0.121804205012
0.0943597197642 0.12217144641
0.0947432958608 0.122540419991
0.0951268719574 0.122911138375
0.095510448054 0.123283614317
0.0958940241506 0.123657860706
0.0962776002472 0.124033890567
0.0966611763438 0.124411717062
0.0970447524404 0.124791353496
0.097428328537 0.125172813313
0.0978119046336 0.125556110102
0.0981954807302 0.125941257601
0.0985790568268 0.126328269693
0.0989626329234 0.126717160412
0.09934620902 0.127107943947
0.0997297851166 0.12750063464
0.100113361213 0.127895246991
0.10049693731 0.128291795658
0.100880513406 0.128690295464
0.101264089503 0.129090761394
0.1016476656 0.1294932086
0.102031241696 0.129897652404
0.102414817793 0.130304108299
0.102798393889 0.130712591954
0.103181969986 0.131123119212
0.103565546083 0.131535706099
0.103949122179 0.131950368821
0.104332698276 0.132367123772
0.104716274372 0.132785987531
0.105099850469 0.13320697687
0.105483426566 0.133630108756
0.105867002662 0.134055400349
0.106250578759 0.134482869014
0.106634154855 0.134912532316
0.107017730952 0.135344408027
0.107401307049 0.13577851413
0.107784883145 0.136214868821
0.108168459242 0.13665349051
0.108552035338 0.13709439783
0.108935611435 0.137537609636
0.109319187532 0.13798314501
0.109702763628 0.138431023265
0.110086339725 0.13888126395
0.110469915821 0.139333886851
0.110853491918 0.139788911996
0.111237068015 0.14024635966
0.111620644111 0.140706250369
0.112004220208 0.141168604903
0.112387796304 0.141633444302
0.112771372401 0.142100789867
0.113154948498 0.142570663168
0.113538524594 0.14304308605
0.113922100691 0.14351808063
0.114305676788 0.14399566931
0.114689252884 0.144475874778
0.115072828981 0.144958720014
0.115456405077 0.145444228293
0.115839981174 0.145932423193
0.116223557271 0.1464233286
0.116607133367 0.14691696871
0.116990709464 0.147413368039
0.11737428556 0.147912551427
0.117757861657 0.148414544043
0.118141437754 0.14891937139
0.11852501385 0.149427059315
0.118908589947 0.149937634012
0.119292166043 0.150451122028
0.11967574214 0.150967550272
0.120059318237 0.15148694602
0.120442894333 0.152009336921
0.12082647043 0.152534751007
0.121210046526 0.153063216696
0.121593622623 0.153594762804
0.12197719872 0.154129418547
0.122360774816 0.154667213554
0.122744350913 0.155208177873
0.123127927009 0.155752341975
0.123511503106 0.15629973677
0.123895079203 0.156850393609
0.124278655299 0.157404344296
0.124662231396 0.157961621093
0.125045807492 0.158522256737
0.125429383589 0.159086284439
0.125812959686 0.159653737901
0.126196535782 0.160224651325
0.126580111879 0.16079905942
0.126963687975 0.161376997413
0.127347264072 0.161958501063
0.127730840169 0.162543606668
0.128114416265 0.163132351077
0.128497992362 0.163724771704
0.128881568458 0.164320906536
0.129265144555 0.164920794146
0.129648720652 0.16552447371
0.130032296748 0.166131985013
0.130415872845 0.166743368464
0.130799448941 0.167358665114
0.131183025038 0.167977916663
0.131566601135 0.16860116548
0.131950177231 0.169228454612
0.132333753328 0.169859827806
0.132717329424 0.170495329517
0.133100905521 0.171135004929
0.133484481618 0.171778899968
0.133868057714 0.172427061323
0.134251633811 0.173079536459
0.134635209907 0.173736373635
0.135018786004 0.174397621927
0.135402362101 0.175063331241
0.135785938197 0.175733552335
0.136169514294 0.17640833684
0.13655309039 0.177087737279
0.136936666487 0.177771807089
0.137320242584 0.17846060064
0.13770381868 0.179154173265
0.138087394777 0.179852581272
0.138470970873 0.18055588198
0.13885454697 0.181264133734
0.139238123067 0.181977395935
0.139621699163 0.182695729066
0.14000527526 0.18341919472
0.140388851356 0.184147855624
0.140772427453 0.184881775672
0.14115600355 0.185621019954
0.141539579646 0.186365654785
0.141923155743 0.18711574774
0.142306731839 0.187871367683
0.142690307936 0.188632584804
0.143073884033 0.189399470655
0.143457460129 0.190172098181
0.143841036226 0.190950541766
0.144224612322 0.191734877263
0.144608188419 0.192525182042
0.144991764516 0.193321535028
0.145375340612 0.194124016743
0.145758916709 0.194932709355
0.146142492806 0.195747696721
0.146526068902 0.196569064435
0.146909644999 0.197396899882
0.147293221095 0.198231292285
0.147676797192 0.19907233276
0.148060373289 0.199920114374
0.148443949385 0.200774732201
0.148827525482 0.201636283381
0.149211101578 0.202504867186
0.149594677675 0.203380585079
0.149978253772 0.204263540788
0.150361829868 0.205153840372
0.150745405965 0.206051592295
0.151128982061 0.206956907502
0.151512558158 0.207869899496
0.151896134255 0.208790684424
0.152279710351 0.20971938116
0.152663286448 0.210656111394
0.153046862544 0.211600999727
0.153430438641 0.212554173764
0.153814014738 0.213515764222
0.154197590834 0.214485905027
0.154581166931 0.215464733433
0.154964743027 0.21645239013
0.155348319124 0.217449019369
0.155731895221 0.218454769084
0.156115471317 0.219469791028
0.156499047414 0.220494240907
0.15688262351 0.221528278527
0.157266199607 0.222572067943
0.157649775704 0.223625777618
0.1580333518 0.224689580588
0.158416927897 0.225763654638
0.158800503993 0.226848182484
0.15918408009 0.227943351963
0.159567656187 0.229049356238
0.159951232283 0.230166394006
0.16033480838 0.231294669725
0.160718384476 0.232434393844
0.161101960573 0.233585783056
0.16148553667 0.234749060552
0.161869112766 0.235924456299
0.162252688863 0.237112207331
0.162636264959 0.238312558052
0.163019841056 0.239525760559
0.163403417153 0.240752074988
0.163786993249 0.24199176987
0.164170569346 0.243245122517
0.164554145442 0.244512419427
0.164937721539 0.245793956715
0.165321297636 0.247090040567
0.165704873732 0.248400987728
0.166088449829 0.249727126015
0.166472025925 0.251068794867
0.166855602022 0.25242634593
0.167239178119 0.253800143677
0.167622754215 0.255190566073
0.168006330312 0.256598005287
0.168389906408 0.258022868447
0.168773482505 0.259465578455
0.169157058602 0.260926574855
0.169540634698 0.262406314764
0.169924210795 0.263905273878
0.170307786891 0.265423947542
0.170691362988 0.266962851917
0.171074939085 0.268522525222
0.171458515181 0.270103529083
0.171842091278 0.271706449994
0.172225667374 0.273331900886
0.172609243471 0.274980522839
0.172992819568 0.276652986935
0.173376395664 0.278349996269
0.173759971761 0.28007228815
0.174143547857 0.281820636487
0.174527123954 0.283595854406
0.174910700051 0.285398797115
0.175294276147 0.287230365038
0.175677852244 0.289091507267
0.17606142834 0.290983225364
0.176445004437 0.292906577552
0.176828580534 0.294862683357
0.17721215663 0.296852728753
0.177595732727 0.298877971887
0.177979308824 0.300939749453
0.17836288492 0.303039483831
0.178746461017 0.30517869108
0.179130037113 0.307358989937
0.17951361321 0.309582111973
0.179897189307 0.311849913094
0.180280765403 0.314164386616
0.1806643415 0.31652767819
0.181047917596 0.31894210291
0.181431493693 0.321410165012
0.18181506979 0.323934580661
0.182198645886 0.326518304458
0.182582221983 0.329164560433
0.182965798079 0.331876878511
0.183349374176 0.334659137689
0.183732950273 0.337515617527
0.184116526369 0.340451060007
0.184500102466 0.343470744495
0.184883678562 0.346580579382
0.185267254659 0.349787215284
0.185650830756 0.353098186399
0.186034406852 0.356522089255
0.186417982949 0.360068811882
0.186801559045 0.363749832255
0.187185135142 0.367578613951
0.187568711239 0.371571141449
0.187952287335 0.375746661743
0.188335863432 0.380128740651
0.188719439528 0.384746817987
0.189103015625 0.389638590818
0.189486591722 0.394853851923
0.189870167818 0.40046107662
0.190253743915 0.406559716451
0.190637320011 0.41330600435
0.191020896108 0.420977726304
0.191404472205 0.430198038241


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceProb0pt6.tex <==
-13.5 0.125052621402
-13.473 0.125052621402
-13.446 0.125052621402
-13.419 0.125052621402
-13.392 0.125052621402
-13.365 0.125052621402
-13.338 0.125052621402
-13.311 0.125052621402
-13.284 0.125052621402
-13.257 0.125052621402
-13.23 0.125052621402
-13.203 0.125052621402
-13.176 0.125052621402
-13.149 0.125052621402
-13.122 0.125052621402
-13.095 0.125052621402
-13.068 0.125052621402
-13.041 0.125052621402
-13.014 0.125052621402
-12.987 0.125052621402
-12.96 0.125052621402
-12.933 0.125052621402
-12.906 0.125052621402
-12.879 0.125052621402
-12.852 0.125052621402
-12.825 0.125052621402
-12.798 0.125052621402
-12.771 0.125052621402
-12.744 0.125052621402
-12.717 0.125052621402
-12.69 0.125052621402
-12.663 0.125052621402
-12.636 0.125052621402
-12.609 0.125052621402
-12.582 0.125052621402
-12.555 0.125052621402
-12.528 0.125052621402
-12.501 0.125052621402
-12.474 0.125052621402
-12.447 0.125052621402
-12.42 0.125052621402
-12.393 0.125052621402
-12.366 0.125052621402
-12.339 0.125052621402
-12.312 0.125052621402
-12.285 0.125052621402
-12.258 0.125052621402
-12.231 0.125052621402
-12.204 0.125052621402
-12.177 0.125052621402
-12.15 0.125052621402
-12.123 0.125052621402
-12.096 0.125052621402
-12.069 0.125052621402
-12.042 0.125052621402
-12.015 0.125052621402
-11.988 0.125052621402
-11.961 0.125052621402
-11.934 0.125052621402
-11.907 0.125052621402
-11.88 0.125052621402
-11.853 0.125052621401
-11.826 0.125052621401
-11.799 0.125052621401
-11.772 0.125052621401
-11.745 0.125052621401
-11.718 0.125052621401
-11.691 0.125052621401
-11.664 0.125052621401
-11.637 0.125052621401
-11.61 0.125052621401
-11.583 0.125052621401
-11.556 0.125052621401
-11.529 0.125052621401
-11.502 0.125052621401
-11.475 0.125052621401
-11.448 0.125052621401
-11.421 0.125052621401
-11.394 0.125052621401
-11.367 0.125052621401
-11.34 0.125052621401
-11.313 0.125052621401
-11.286 0.125052621401
-11.259 0.125052621401
-11.232 0.125052621401
-11.205 0.125052621401
-11.178 0.125052621401
-11.151 0.125052621401
-11.124 0.125052621401
-11.097 0.125052621401
-11.07 0.125052621401
-11.043 0.125052621401
-11.016 0.125052621401
-10.989 0.125052621401
-10.962 0.125052621401
-10.935 0.125052621401
-10.908 0.125052621401
-10.881 0.125052621401
-10.854 0.125052621401
-10.827 0.125052621401
-10.8 0.125052621401
-10.773 0.125052621401
-10.746 0.125052621401
-10.719 0.125052621401
-10.692 0.125052621401
-10.665 0.125052621401
-10.638 0.125052621401
-10.611 0.125052621401
-10.584 0.1250526214
-10.557 0.1250526214
-10.53 0.1250526214
-10.503 0.1250526214
-10.476 0.1250526214
-10.449 0.1250526214
-10.422 0.1250526214
-10.395 0.1250526214
-10.368 0.1250526214
-10.341 0.125052621399
-10.314 0.125052621399
-10.287 0.125052621399
-10.26 0.125052621399
-10.233 0.125052621399
-10.206 0.125052621398
-10.179 0.125052621398
-10.152 0.125052621398
-10.125 0.125052621398
-10.098 0.125052621397
-10.071 0.125052621397
-10.044 0.125052621397
-10.017 0.125052621396
-9.99 0.125052621396
-9.963 0.125052621396
-9.936 0.125052621395
-9.909 0.125052621395
-9.882 0.125052621394
-9.855 0.125052621393
-9.828 0.125052621393
-9.801 0.125052621392
-9.774 0.125052621391
-9.747 0.125052621391
-9.72 0.12505262139
-9.693 0.125052621389
-9.666 0.125052621388
-9.639 0.125052621387
-9.612 0.125052621385
-9.585 0.125052621384
-9.558 0.125052621383
-9.531 0.125052621381
-9.504 0.12505262138
-9.477 0.125052621378
-9.45 0.125052621376
-9.423 0.125052621374
-9.396 0.125052621372
-9.369 0.12505262137
-9.342 0.125052621367
-9.315 0.125052621365
-9.288 0.125052621362
-9.261 0.125052621359
-9.234 0.125052621355
-9.207 0.125052621352
-9.18 0.125052621348
-9.153 0.125052621344
-9.126 0.125052621339
-9.099 0.125052621334
-9.072 0.125052621329
-9.045 0.125052621323
-9.018 0.125052621317
-8.991 0.125052621311
-8.964 0.125052621304
-8.937 0.125052621296
-8.91 0.125052621288
-8.883 0.125052621279
-8.856 0.125052621269
-8.829 0.125052621259
-8.802 0.125052621248
-8.775 0.125052621236
-8.748 0.125052621223
-8.721 0.125052621209
-8.694 0.125052621194
-8.667 0.125052621178
-8.64 0.125052621161
-8.613 0.125052621142
-8.586 0.125052621122
-8.559 0.1250526211
-8.532 0.125052621076
-8.505 0.125052621051
-8.478 0.125052621024
-8.451 0.125052620995
-8.424 0.125052620963
-8.397 0.125052620929
-8.37 0.125052620892
-8.343 0.125052620853
-8.316 0.12505262081
-8.289 0.125052620765
-8.262 0.125052620715
-8.235 0.125052620662
-8.208 0.125052620605
-8.181 0.125052620543
-8.154 0.125052620477
-8.127 0.125052620405
-8.1 0.125052620328
-8.073 0.125052620245
-8.046 0.125052620156
-8.019 0.12505262006
-7.992 0.125052619956
-7.965 0.125052619844
-7.938 0.125052619724
-7.911 0.125052619594
-7.884 0.125052619455
-7.857 0.125052619305
-7.83 0.125052619143
-7.803 0.125052618969
-7.776 0.125052618781
-7.749 0.12505261858
-7.722 0.125052618362
-7.695 0.125052618128
-7.668 0.125052617876
-7.641 0.125052617605
-7.614 0.125052617313
-7.587 0.125052616999
-7.56 0.12505261666
-7.533 0.125052616296
-7.506 0.125052615904
-7.479 0.125052615481
-7.452 0.125052615027
-7.425 0.125052614538
-7.398 0.125052614011
-7.371 0.125052613445
-7.344 0.125052612835
-7.317 0.125052612178
-7.29 0.125052611472
-7.263 0.125052610711
-7.236 0.125052609893
-7.209 0.125052609013
-7.182 0.125052608065
-7.155 0.125052607045
-7.128 0.125052605948
-7.101 0.125052604768
-7.074 0.125052603497
-7.047 0.12505260213
-7.02 0.12505260066
-6.993 0.125052599078
-6.966 0.125052597375
-6.939 0.125052595544
-6.912 0.125052593574
-6.885 0.125052591455
-6.858 0.125052589175
-6.831 0.125052586723
-6.804 0.125052584085
-6.777 0.125052581248
-6.75 0.125052578196
-6.723 0.125052574914
-6.696 0.125052571384
-6.669 0.125052567588
-6.642 0.125052563505
-6.615 0.125052559115
-6.588 0.125052554393
-6.561 0.125052549317
-6.534 0.125052543857
-6.507 0.125052537988
-6.48 0.125052531676
-6.453 0.125052524891
-6.426 0.125052517595
-6.399 0.125052509752
-6.372 0.125052501321
-6.345 0.125052492257
-6.318 0.125052482513
-6.291 0.12505247204
-6.264 0.125052460782
-6.237 0.125052448682
-6.21 0.125052435677
-6.183 0.125052421699
-6.156 0.125052406678
-6.129 0.125052390535
-6.102 0.125052373187
-6.075 0.125052354546
-6.048 0.125052334515
-6.021 0.125052312992
-5.994 0.125052289867
-5.967 0.125052265022
-5.94 0.125052238329
-5.913 0.125052209654
-5.886 0.125052178848
-5.859 0.125052145757
-5.832 0.125052110212
-5.805 0.125052072033
-5.778 0.125052031026
-5.751 0.125051986984
-5.724 0.125051939685
-5.697 0.12505188889
-5.67 0.125051834343
-5.643 0.125051775771
-5.616 0.125051712878
-5.589 0.12505164535
-5.562 0.125051572848
-5.535 0.125051495011
-5.508 0.125051411449
-5.481 0.125051321746
-5.454 0.125051225457
-5.427 0.125051122102
-5.4 0.125051011169
-5.373 0.125050892108
-5.346 0.125050764332
-5.319 0.12505062721
-5.292 0.125050480065
-5.265 0.125050322175
-5.238 0.125050152763
-5.211 0.125049971001
-5.184 0.125049775997
-5.157 0.1250495668
-5.13 0.12504934239
-5.103 0.125049101675
-5.076 0.125048843485
-5.049 0.125048566569
-5.022 0.125048269586
-4.995 0.125047951103
-4.968 0.125047609584
-4.941 0.125047243385
-4.914 0.12504685075
-4.887 0.125046429795
-4.86 0.125045978509
-4.833 0.125045494738
-4.806 0.125044976178
-4.779 0.125044420366
-4.752 0.125043824665
-4.725 0.125043186258
-4.698 0.12504250213
-4.671 0.125041769061
-4.644 0.125040983605
-4.617 0.125040142079
-4.59 0.125039240548
-4.563 0.125038274806
-4.536 0.125037240356
-4.509 0.125036132396
-4.482 0.125034945794
-4.455 0.125033675068
-4.428 0.125032314361
-4.401 0.12503085742
-4.374 0.125029297567
-4.347 0.125027627669
-4.32 0.125025840113
-4.293 0.125023926772
-4.266 0.125021878971
-4.239 0.125019687451
-4.212 0.125017342334
-4.185 0.125014833078
-4.158 0.12501214844
-4.131 0.125009276425
-4.104 0.125006204242
-4.077 0.125002918252
-4.05 0.124999403912
-4.023 0.124995645719
-3.996 0.124991627149
-3.969 0.124987330594
-3.942 0.124982737291
-3.915 0.124977827251
-3.888 0.124972579183
-3.861 0.124966970409
-3.834 0.124960976786
-3.807 0.124954572608
-3.78 0.124947730511
-3.753 0.124940421376
-3.726 0.124932614218
-3.699 0.124924276073
-3.672 0.124915371878
-3.645 0.124905864349
-3.618 0.124895713842
-3.591 0.124884878217
-3.564 0.124873312688
-3.537 0.124860969666
-3.51 0.1248477986
-3.483 0.124833745797
-3.456 0.124818754247
-3.429 0.124802763426
-3.402 0.1247857091
-3.375 0.124767523113
-3.348 0.124748133162
-3.321 0.124727462569
-3.294 0.124705430036
-3.267 0.124681949392
-3.24 0.12465692932
-3.213 0.124630273087
-3.186 0.124601878242
-3.159 0.12457163632
-3.132 0.124539432518
-3.105 0.124505145367
-3.078 0.124468646381
-3.051 0.124429799706
-3.024 0.124388461738
-2.997 0.124344480738
-2.97 0.124297696432
-2.943 0.124247939589
-2.916 0.124195031593
-2.889 0.124138783995
-2.862 0.124078998055
-2.835 0.124015464267
-2.808 0.123947961871
-2.781 0.123876258356
-2.754 0.123800108944
-2.727 0.12371925607
-2.7 0.123633428845
-2.673 0.123542342515
-2.646 0.12344569791
-2.619 0.123343180886
-2.592 0.123234461763
-2.565 0.123119194765
-2.538 0.122997017449
-2.511 0.122867550151
-2.484 0.12273039543
-2.457 0.122585137519
-2.43 0.122431341794
-2.403 0.122268554258
-2.376 0.12209630105
-2.349 0.121914087977
-2.322 0.121721400079
-2.295 0.121517701236
-2.268 0.121302433822
-2.241 0.121075018405
-2.214 0.120834853519
-2.187 0.120581315495
-2.16 0.120313758386
-2.133 0.120031513966
-2.106 0.119733891846
-2.079 0.119420179693
-2.052 0.11908964358
-2.025 0.118741528476
-1.998 0.118375058892
-1.971 0.117989439692
-1.944 0.1175838571
-1.917 0.117157479905
-1.89 0.116709460893
-1.863 0.11623893852
-1.836 0.115745038847
-1.809 0.115226877766
-1.782 0.114683563521
-1.755 0.11411419957
-1.728 0.113517887794
-1.701 0.112893732082
-1.674 0.112240842322
-1.647 0.111558338815
-1.62 0.110845357143
-1.593 0.110101053513
-1.566 0.109324610602
-1.539 0.108515243934
-1.512 0.107672208801
-1.485 0.106794807758
-1.458 0.105882398725
-1.431 0.104934403689
-1.404 0.103950318056
-1.377 0.102929720651
-1.35 0.101872284384
-1.323 0.100777787604
-1.296 0.0996461261415
-1.269 0.0984773260582
-1.242 0.097271557104
-1.215 0.0960291468928
-1.188 0.0947505958002
-1.161 0.0934365925926
-1.134 0.0920880307944
-1.107 0.0907060258091
-1.08 0.0892919328151
-1.053 0.0878473654707
-1.026 0.086374215477
-0.999 0.0848746730746
-0.972 0.08335124858
-0.945 0.0818067951111
-0.918 0.080244532711
-0.891 0.0786680741527
-0.864 0.0770814528086
-0.837 0.0754891530951
-0.81 0.0738961441721
-0.783 0.0723079177898
-0.756 0.0707305314565
-0.729 0.0691706584604
-0.702 0.0676356467504
-0.675 0.066133589291
-0.648 0.0646734093118
-0.621 0.0632649649349
-0.594 0.0619191790746
-0.567 0.0606482024067
-0.54 0.0594656197779
-0.513 0.0583867139691
-0.486 0.0574288056384
-0.459 0.0566116952071
-0.432 0.0559582423655
-0.405 0.0554951333096
-0.378 0.055253907206
-0.351 0.0552723457264
-0.324 0.0555963795239
-0.297 0.0562827448643
-0.27 0.0574027530526
-0.243 0.0590477531894
-0.216 0.0613372490757
-0.189 0.0644313226617
-0.162 0.068550335656
-0.135 0.0740075428477
-0.108 0.081265997037
-0.081 0.0910446065426
-0.054 0.10453338002
-0.027 0.123883728994
0.0 0.153530967875
0.000140480687544 0.153726280949
0.000280961375088 0.153922012094
0.000421442062631 0.154118162763
0.000561922750175 0.154314734417
0.000702403437719 0.154511728526
0.000842884125263 0.154709146566
0.000983364812806 0.154906990021
0.00112384550035 0.155105260383
0.00126432618789 0.155303959153
0.00140480687544 0.155503087836
0.00154528756298 0.155702647949
0.00168576825053 0.155902641015
0.00182624893807 0.156103068565
0.00196672962561 0.156303932138
0.00210721031316 0.156505233281
0.0022476910007 0.156706973549
0.00238817168824 0.156909154507
0.00252865237579 0.157111777725
0.00266913306333 0.157314844785
0.00280961375088 0.157518357274
0.00295009443842 0.15772231679
0.00309057512596 0.157926724937
0.00323105581351 0.15813158333
0.00337153650105 0.158336893591
0.00351201718859 0.158542657352
0.00365249787614 0.158748876252
0.00379297856368 0.15895555194
0.00393345925123 0.159162686074
0.00407393993877 0.15937028032
0.00421442062631 0.159578336354
0.00435490131386 0.15978685586
0.0044953820014 0.159995840532
0.00463586268894 0.160205292074
0.00477634337649 0.160415212197
0.00491682406403 0.160625602622
0.00505730475158 0.160836465081
0.00519778543912 0.161047801314
0.00533826612666 0.161259613071
0.00547874681421 0.161471902111
0.00561922750175 0.161684670204
0.00575970818929 0.161897919129
0.00590018887684 0.162111650673
0.00604066956438 0.162325866637
0.00618115025193 0.162540568829
0.00632163093947 0.162755759067
0.00646211162701 0.16297143918
0.00660259231456 0.163187611007
0.0067430730021 0.163404276399
0.00688355368964 0.163621437213
0.00702403437719 0.163839095321
0.00716451506473 0.164057252603
0.00730499575228 0.16427591095
0.00744547643982 0.164495072265
0.00758595712736 0.164714738459
0.00772643781491 0.164934911457
0.00786691850245 0.165155593193
0.00800739918999 0.165376785612
0.00814787987754 0.165598490671
0.00828836056508 0.165820710339
0.00842884125263 0.166043446592
0.00856932194017 0.166266701423
0.00870980262771 0.166490476833
0.00885028331526 0.166714774836
0.0089907640028 0.166939597456
0.00913124469034 0.16716494673
0.00927172537789 0.167390824707
0.00941220606543 0.167617233447
0.00955268675298 0.167844175023
0.00969316744052 0.168071651519
0.00983364812806 0.168299665032
0.00997412881561 0.168528217671
0.0101146095032 0.168757311558
0.0102550901907 0.168986948826
0.0103955708782 0.169217131622
0.0105360515658 0.169447862105
0.0106765322533 0.169679142448
0.0108170129409 0.169910974834
0.0109574936284 0.170143361463
0.011097974316 0.170376304544
0.0112384550035 0.170609806303
0.011378935691 0.170843868976
0.0115194163786 0.171078494815
0.0116598970661 0.171313686084
0.0118003777537 0.171549445062
0.0119408584412 0.17178577404
0.0120813391288 0.172022675324
0.0122218198163 0.172260151235
0.0123623005039 0.172498204105
0.0125027811914 0.172736836283
0.0126432618789 0.172976050131
0.0127837425665 0.173215848027
0.012924223254 0.173456232362
0.0130647039416 0.173697205542
0.0132051846291 0.173938769988
0.0133456653167 0.174180928137
0.0134861460042 0.174423682439
0.0136266266917 0.174667035361
0.0137671073793 0.174910989384
0.0139075880668 0.175155547005
0.0140480687544 0.175400710738
0.0141885494419 0.17564648311
0.0143290301295 0.175892866666
0.014469510817 0.176139863967
0.0146099915046 0.176387477589
0.0147504721921 0.176635710124
0.0148909528796 0.176884564181
0.0150314335672 0.177134042388
0.0151719142547 0.177384147385
0.0153123949423 0.177634881832
0.0154528756298 0.177886248407
0.0155933563174 0.178138249801
0.0157338370049 0.178390888726
0.0158743176924 0.17864416791
0.01601479838 0.178898090099
0.0161552790675 0.179152658056
0.0162957597551 0.179407874564
0.0164362404426 0.179663742421
0.0165767211302 0.179920264446
0.0167172018177 0.180177443474
0.0168576825053 0.180435282361
0.0169981631928 0.18069378398
0.0171386438803 0.180952951224
0.0172791245679 0.181212787003
0.0174196052554 0.18147329425
0.017560085943 0.181734475914
0.0177005666305 0.181996334964
0.0178410473181 0.182258874391
0.0179815280056 0.182522097204
0.0181220086931 0.182786006433
0.0182624893807 0.183050605127
0.0184029700682 0.183315896357
0.0185434507558 0.183581883215
0.0186839314433 0.183848568813
0.0188244121309 0.184115956283
0.0189648928184 0.18438404878
0.019105373506 0.18465284948
0.0192458541935 0.184922361581
0.019386334881 0.185192588303
0.0195268155686 0.185463532886
0.0196672962561 0.185735198595
0.0198077769437 0.186007588716
0.0199482576312 0.186280706559
0.0200887383188 0.186554555455
0.0202292190063 0.18682913876
0.0203696996938 0.187104459853
0.0205101803814 0.187380522134
0.0206506610689 0.187657329032
0.0207911417565 0.187934883995
0.020931622444 0.188213190499
0.0210721031316 0.188492252041
0.0212125838191 0.188772072146
0.0213530645067 0.189052654363
0.0214935451942 0.189334002265
0.0216340258817 0.189616119452
0.0217745065693 0.189899009549
0.0219149872568 0.190182676207
0.0220554679444 0.190467123104
0.0221959486319 0.190752353943
0.0223364293195 0.191038372456
0.022476910007 0.1913251824
0.0226173906945 0.19161278756
0.0227578713821 0.191901191749
0.0228983520696 0.192190398807
0.0230388327572 0.192480412604
0.0231793134447 0.192771237036
0.0233197941323 0.193062876028
0.0234602748198 0.193355333537
0.0236007555074 0.193648613545
0.0237412361949 0.193942720068
0.0238817168824 0.194237657148
0.02402219757 0.194533428859
0.0241626782575 0.194830039306
0.0243031589451 0.195127492623
0.0244436396326 0.195425792978
0.0245841203202 0.195724944568
0.0247246010077 0.196024951623
0.0248650816952 0.196325818404
0.0250055623828 0.196627549206
0.0251460430703 0.196930148356
0.0252865237579 0.197233620215
0.0254270044454 0.197537969175
0.025567485133 0.197843199665
0.0257079658205 0.198149316147
0.0258484465081 0.198456323117
0.0259889271956 0.198764225106
0.0261294078831 0.199073026681
0.0262698885707 0.199382732445
0.0264103692582 0.199693347037
0.0265508499458 0.200004875131
0.0266913306333 0.20031732144
0.0268318113209 0.200630690712
0.0269722920084 0.200944987735
0.0271127726959 0.201260217335
0.0272532533835 0.201576384373
0.027393734071 0.201893493755
0.0275342147586 0.20221155042
0.0276746954461 0.202530559351
0.0278151761337 0.202850525571
0.0279556568212 0.203171454142
0.0280961375088 0.203493350168
0.0282366181963 0.203816218795
0.0283770988838 0.20414006521
0.0285175795714 0.204464894645
0.0286580602589 0.204790712371
0.0287985409465 0.205117523708
0.028939021634 0.205445334014
0.0290795023216 0.205774148697
0.0292199830091 0.206103973207
0.0293604636966 0.20643481304
0.0295009443842 0.206766673739
0.0296414250717 0.207099560892
0.0297819057593 0.207433480137
0.0299223864468 0.207768437156
0.0300628671344 0.208104437684
0.0302033478219 0.2084414875
0.0303438285095 0.208779592436
0.030484309197 0.209118758372
0.0306247898845 0.20945899124
0.0307652705721 0.209800297023
0.0309057512596 0.210142681755
0.0310462319472 0.210486151523
0.0311867126347 0.210830712468
0.0313271933223 0.211176370782
0.0314676740098 0.211523132716
0.0316081546973 0.211871004572
0.0317486353849 0.212219992709
0.0318891160724 0.212570103542
0.03202959676 0.212921343546
0.0321700774475 0.21327371925
0.0323105581351 0.213627237243
0.0324510388226 0.213981904174
0.0325915195102 0.214337726751
0.0327320001977 0.214694711744
0.0328724808852 0.215052865982
0.0330129615728 0.21541219636
0.0331534422603 0.215772709834
0.0332939229479 0.216134413423
0.0334344036354 0.216497314212
0.033574884323 0.216861419351
0.0337153650105 0.217226736058
0.033855845698 0.217593271616
0.0339963263856 0.217961033378
0.0341368070731 0.218330028763
0.0342772877607 0.218700265265
0.0344177684482 0.219071750443
0.0345582491358 0.219444491932
0.0346987298233 0.219818497438
0.0348392105109 0.220193774741
0.0349796911984 0.220570331695
0.0351201718859 0.220948176231
0.0352606525735 0.221327316355
0.035401133261 0.221707760152
0.0355416139486 0.222089515785
0.0356820946361 0.222472591497
0.0358225753237 0.222856995612
0.0359630560112 0.223242736536
0.0361035366987 0.223629822757
0.0362440173863 0.22401826285
0.0363844980738 0.224408065471
0.0365249787614 0.224799239368
0.0366654594489 0.225191793372
0.0368059401365 0.225585736406
0.036946420824 0.225981077483
0.0370869015116 0.226377825705
0.0372273821991 0.226775990269
0.0373678628866 0.227175580468
0.0375083435742 0.227576605686
0.0376488242617 0.227979075408
0.0377893049493 0.228382999215
0.0379297856368 0.228788386787
0.0380702663244 0.229195247909
0.0382107470119 0.229603592463
0.0383512276994 0.230013430441
0.038491708387 0.230424771936
0.0386321890745 0.230837627151
0.0387726697621 0.231252006396
0.0389131504496 0.231667920092
0.0390536311372 0.232085378774
0.0391941118247 0.232504393087
0.0393345925123 0.232924973795
0.0394750731998 0.233347131777
0.0396155538873 0.233770878032
0.0397560345749 0.23419622368
0.0398965152624 0.234623179963
0.04003699595 0.235051758247
0.0401774766375 0.235481970025
0.0403179573251 0.235913826921
0.0404584380126 0.236347340685
0.0405989187001 0.236782523203
0.0407393993877 0.237219386494
0.0408798800752 0.237657942714
0.0410203607628 0.238098204159
0.0411608414503 0.238540183263
0.0413013221379 0.238983892608
0.0414418028254 0.239429344918
0.041582283513 0.239876553066
0.0417227642005 0.240325530076
0.041863244888 0.240776289126
0.0420037255756 0.241228843548
0.0421442062631 0.241683206832
0.0422846869507 0.242139392628
0.0424251676382 0.242597414752
0.0425656483258 0.243057287184
0.0427061290133 0.243519024074
0.0428466097008 0.243982639742
0.0429870903884 0.244448148684
0.0431275710759 0.244915565574
0.0432680517635 0.245384905266
0.043408532451 0.245856182798
0.0435490131386 0.246329413395
0.0436894938261 0.246804612472
0.0438299745137 0.24728179564
0.0439704552012 0.247760978702
0.0441109358887 0.248242177667
0.0442514165763 0.248725408745
0.0443918972638 0.249210688355
0.0445323779514 0.249698033126
0.0446728586389 0.250187459903
0.0448133393265 0.250678985753
0.044953820014 0.251172627961
0.0450943007015 0.251668404044
0.0452347813891 0.252166331749
0.0453752620766 0.252666429058
0.0455157427642 0.253168714194
0.0456562234517 0.253673205625
0.0457967041393 0.254179922068
0.0459371848268 0.254688882495
0.0460776655144 0.255200106137
0.0462181462019 0.255713612487
0.0463586268894 0.25622942131
0.046499107577 0.256747552643
0.0466395882645 0.257268026805
0.0467800689521 0.257790864397
0.0469205496396 0.258316086315
0.0470610303272 0.258843713747
0.0472015110147 0.259373768188
0.0473419917022 0.259906271439
0.0474824723898 0.260441245616
0.0476229530773 0.260978713158
0.0477634337649 0.261518696829
0.0479039144524 0.262061219732
0.04804439514 0.262606305307
0.0481848758275 0.263153977346
0.0483253565151 0.263704259996
0.0484658372026 0.264257177766
0.0486063178901 0.26481275554
0.0487467985777 0.265371018578
0.0488872792652 0.265931992528
0.0490277599528 0.266495703436
0.0491682406403 0.267062177749
0.0493087213279 0.267631442331
0.0494492020154 0.268203524465
0.049589682703 0.268778451869
0.0497301633905 0.269356252701
0.049870644078 0.269936955569
0.0500111247656 0.270520589546
0.0501516054531 0.271107184175
0.0502920861407 0.271696769482
0.0504325668282 0.272289375989
0.0505730475158 0.272885034723
0.0507135282033 0.273483777228
0.0508540088908 0.274085635578
0.0509944895784 0.274690642392
0.0511349702659 0.275298830841
0.0512754509535 0.275910234668
0.051415931641 0.276524888196
0.0515564123286 0.277142826348
0.0516968930161 0.277764084656
0.0518373737037 0.278388699283
0.0519778543912 0.27901670703
0.0521183350787 0.27964814536
0.0522588157663 0.280283052411
0.0523992964538 0.280921467014
0.0525397771414 0.281563428711
0.0526802578289 0.282208977773
0.0528207385165 0.28285815522
0.052961219204 0.283511002841
0.0531016998915 0.284167563212
0.0532421805791 0.28482787972
0.0533826612666 0.285491996583
0.0535231419542 0.286159958876
0.0536636226417 0.286831812549
0.0538041033293 0.287507604455
0.0539445840168 0.288187382377
0.0540850647044 0.288871195049
0.0542255453919 0.289559092188
0.0543660260794 0.290251124517
0.054506506767 0.290947343801
0.0546469874545 0.29164780287
0.0547874681421 0.292352555657
0.0549279488296 0.293061657226
0.0550684295172 0.293775163807
0.0552089102047 0.294493132834
0.0553493908922 0.295215622976
0.0554898715798 0.295942694183
0.0556303522673 0.296674407717
0.0557708329549 0.2974108262
0.0559113136424 0.298152013655
0.05605179433 0.298898035548
0.0561922750175 0.29964895884
0.0563327557051 0.30040485203
0.0564732363926 0.30116578521
0.0566137170801 0.301931830115
0.0567541977677 0.302703060181
0.0568946784552 0.303479550599
0.0570351591428 0.30426137838
0.0571756398303 0.305048622413
0.0573161205179 0.305841363534
0.0574566012054 0.306639684593
0.0575970818929 0.307443670529
0.0577375625805 0.308253408442
0.057878043268 0.309068987673
0.0580185239556 0.309890499887
0.0581590046431 0.310718039161
0.0582994853307 0.311551702074
0.0584399660182 0.312391587801
0.0585804467058 0.313237798217
0.0587209273933 0.314090438
0.0588614080808 0.314949614742
0.0590018887684 0.315815439067
0.0591423694559 0.316688024754
0.0592828501435 0.317567488865
0.059423330831 0.318453951883
0.0595638115186 0.319347537855
0.0597042922061 0.320248374544
0.0598447728936 0.321156593592
0.0599852535812 0.322072330686
0.0601257342687 0.32299572574
0.0602662149563 0.323926923085
0.0604066956438 0.32486607167
0.0605471763314 0.325813325274
0.0606876570189 0.326768842736
0.0608281377065 0.327732788194
0.060968618394 0.328705331337
0.0611090990815 0.329686647684
0.0612495797691 0.330676918871
0.0613900604566 0.331676332955
0.0615305411442 0.332685084754
0.0616710218317 0.333703376187
0.0618115025193 0.334731416659
0.0619519832068 0.335769423462
0.0620924638943 0.336817622202
0.0622329445819 0.337876247266
0.0623734252694 0.338945542319
0.062513905957 0.340025760837
0.0626543866445 0.341117166681
0.0627948673321 0.342220034718
0.0629353480196 0.343334651493
0.0630758287072 0.344461315948
0.0632163093947 0.345600340207
0.0633567900822 0.346752050425
0.0634972707698 0.347916787712
0.0636377514573 0.349094909129
0.0637782321449 0.350286788788
0.0639187128324 0.35149281904
0.06405919352 0.352713411777
0.0641996742075 0.353948999863
0.064340154895 0.355200038701
0.0644806355826 0.356467007954
0.0646211162701 0.357750413449
0.0647615969577 0.359050789277
0.0649020776452 0.360368700116
0.0650425583328 0.36170474382
0.0651830390203 0.363059554289
0.0653235197079 0.364433804687
0.0654640003954 0.365828211034
0.0656044810829 0.36724353625
0.0657449617705 0.368680594708
0.065885442458 0.370140257383
0.0660259231456 0.371623457707
0.0661664038331 0.373131198227
0.0663068845207 0.374664558237
0.0664473652082 0.376224702554
0.0665878458957 0.377812891643
0.0667283265833 0.379430493391
0.0668688072708 0.381078996845
0.0670092879584 0.382760028346
0.0671497686459 0.384475370613
0.0672902493335 0.386226985455
0.067430730021 0.38801704101
0.0675712107086 0.389847944703
0.0677116913961 0.391722383459
0.0678521720836 0.393643373287
0.0679926527712 0.395614321087
0.0681331334587 0.397639102642
0.0682736141463 0.399722162418
0.0684140948338 0.401868643264
0.0685545755214 0.404084557976
0.0686950562089 0.406377020899
0.0688355368964 0.408754568029
0.068976017584 0.411227611819
0.0691164982715 0.413809109004
0.0692569789591 0.416515581171
0.0693974596466 0.419368753508
0.0695379403342 0.422398357697
0.0696784210217 0.425647344198
0.0698189017093 0.429182777899
0.0699593823968 0.433123051956
0.0700998630843 0.437731317613


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForConditionalVarianceLaplaceProb0pt8.tex <==
-13.5 0.18006620585
-13.4733405504 0.18006620585
-13.4466811008 0.18006620585
-13.4200216512 0.18006620585
-13.3933622017 0.18006620585
-13.3667027521 0.18006620585
-13.3400433025 0.18006620585
-13.3133838529 0.18006620585
-13.2867244033 0.18006620585
-13.2600649537 0.18006620585
-13.2334055042 0.18006620585
-13.2067460546 0.18006620585
-13.180086605 0.18006620585
-13.1534271554 0.18006620585
-13.1267677058 0.18006620585
-13.1001082562 0.18006620585
-13.0734488067 0.18006620585
-13.0467893571 0.18006620585
-13.0201299075 0.18006620585
-12.9934704579 0.18006620585
-12.9668110083 0.18006620585
-12.9401515587 0.18006620585
-12.9134921091 0.18006620585
-12.8868326596 0.18006620585
-12.86017321 0.18006620585
-12.8335137604 0.18006620585
-12.8068543108 0.18006620585
-12.7801948612 0.18006620585
-12.7535354116 0.18006620585
-12.7268759621 0.18006620585
-12.7002165125 0.18006620585
-12.6735570629 0.18006620585
-12.6468976133 0.18006620585
-12.6202381637 0.18006620585
-12.5935787141 0.18006620585
-12.5669192646 0.18006620585
-12.540259815 0.18006620585
-12.5136003654 0.18006620585
-12.4869409158 0.18006620585
-12.4602814662 0.18006620585
-12.4336220166 0.18006620585
-12.406962567 0.18006620585
-12.3803031175 0.18006620585
-12.3536436679 0.18006620585
-12.3269842183 0.18006620585
-12.3003247687 0.18006620585
-12.2736653191 0.18006620585
-12.2470058695 0.18006620585
-12.22034642 0.18006620585
-12.1936869704 0.18006620585
-12.1670275208 0.18006620585
-12.1403680712 0.18006620585
-12.1137086216 0.18006620585
-12.087049172 0.18006620585
-12.0603897225 0.18006620585
-12.0337302729 0.18006620585
-12.0070708233 0.18006620585
-11.9804113737 0.18006620585
-11.9537519241 0.18006620585
-11.9270924745 0.18006620585
-11.900433025 0.18006620585
-11.8737735754 0.18006620585
-11.8471141258 0.18006620585
-11.8204546762 0.18006620585
-11.7937952266 0.18006620585
-11.767135777 0.18006620585
-11.7404763274 0.18006620585
-11.7138168779 0.18006620585
-11.6871574283 0.18006620585
-11.6604979787 0.18006620585
-11.6338385291 0.18006620585
-11.6071790795 0.18006620585
-11.5805196299 0.18006620585
-11.5538601804 0.18006620585
-11.5272007308 0.18006620585
-11.5005412812 0.18006620585
-11.4738818316 0.18006620585
-11.447222382 0.18006620585
-11.4205629324 0.18006620585
-11.3939034829 0.18006620585
-11.3672440333 0.18006620585
-11.3405845837 0.18006620585
-11.3139251341 0.18006620585
-11.2872656845 0.18006620585
-11.2606062349 0.18006620585
-11.2339467853 0.18006620585
-11.2072873358 0.18006620585
-11.1806278862 0.18006620585
-11.1539684366 0.18006620585
-11.127308987 0.180066205849
-11.1006495374 0.180066205849
-11.0739900878 0.180066205849
-11.0473306383 0.180066205849
-11.0206711887 0.180066205849
-10.9940117391 0.180066205849
-10.9673522895 0.180066205849
-10.9406928399 0.180066205849
-10.9140333903 0.180066205849
-10.8873739408 0.180066205849
-10.8607144912 0.180066205849
-10.8340550416 0.180066205849
-10.807395592 0.180066205849
-10.7807361424 0.180066205849
-10.7540766928 0.180066205849
-10.7274172432 0.180066205849
-10.7007577937 0.180066205849
-10.6740983441 0.180066205849
-10.6474388945 0.180066205849
-10.6207794449 0.180066205849
-10.5941199953 0.180066205849
-10.5674605457 0.180066205849
-10.5408010962 0.180066205849
-10.5141416466 0.180066205849
-10.487482197 0.180066205849
-10.4608227474 0.180066205849
-10.4341632978 0.180066205848
-10.4075038482 0.180066205848
-10.3808443987 0.180066205848
-10.3541849491 0.180066205848
-10.3275254995 0.180066205848
-10.3008660499 0.180066205848
-10.2742066003 0.180066205848
-10.2475471507 0.180066205848
-10.2208877011 0.180066205847
-10.1942282516 0.180066205847
-10.167568802 0.180066205847
-10.1409093524 0.180066205847
-10.1142499028 0.180066205847
-10.0875904532 0.180066205846
-10.0609310036 0.180066205846
-10.0342715541 0.180066205846
-10.0076121045 0.180066205846
-9.98095265489 0.180066205845
-9.95429320531 0.180066205845
-9.92763375572 0.180066205845
-9.90097430614 0.180066205844
-9.87431485655 0.180066205844
-9.84765540697 0.180066205843
-9.82099595739 0.180066205843
-9.7943365078 0.180066205842
-9.76767705822 0.180066205842
-9.74101760863 0.180066205841
-9.71435815905 0.18006620584
-9.68769870947 0.18006620584
-9.66103925988 0.180066205839
-9.6343798103 0.180066205838
-9.60772036071 0.180066205837
-9.58106091113 0.180066205836
-9.55440146154 0.180066205835
-9.52774201196 0.180066205834
-9.50108256238 0.180066205833
-9.47442311279 0.180066205831
-9.44776366321 0.18006620583
-9.42110421362 0.180066205828
-9.39444476404 0.180066205827
-9.36778531446 0.180066205825
-9.34112586487 0.180066205823
-9.31446641529 0.180066205821
-9.2878069657 0.180066205819
-9.26114751612 0.180066205817
-9.23448806654 0.180066205814
-9.20782861695 0.180066205811
-9.18116916737 0.180066205808
-9.15450971778 0.180066205805
-9.1278502682 0.180066205802
-9.10119081861 0.180066205798
-9.07453136903 0.180066205794
-9.04787191945 0.18006620579
-9.02121246986 0.180066205785
-8.99455302028 0.18006620578
-8.96789357069 0.180066205775
-8.94123412111 0.180066205769
-8.91457467153 0.180066205763
-8.88791522194 0.180066205756
-8.86125577236 0.180066205749
-8.83459632277 0.180066205741
-8.80793687319 0.180066205733
-8.7812774236 0.180066205724
-8.75461797402 0.180066205714
-8.72795852444 0.180066205703
-8.70129907485 0.180066205692
-8.67463962527 0.18006620568
-8.64798017568 0.180066205667
-8.6213207261 0.180066205653
-8.59466127652 0.180066205638
-8.56800182693 0.180066205622
-8.54134237735 0.180066205604
-8.51468292776 0.180066205585
-8.48802347818 0.180066205565
-8.46136402859 0.180066205543
-8.43470457901 0.18006620552
-8.40804512943 0.180066205494
-8.38138567984 0.180066205467
-8.35472623026 0.180066205438
-8.32806678067 0.180066205406
-8.30140733109 0.180066205372
-8.27474788151 0.180066205336
-8.24808843192 0.180066205296
-8.22142898234 0.180066205254
-8.19476953275 0.180066205208
-8.16811008317 0.180066205159
-8.14145063358 0.180066205107
-8.114791184 0.18006620505
-8.08813173442 0.180066204989
-8.06147228483 0.180066204923
-8.03481283525 0.180066204852
-8.00815338566 0.180066204776
-7.98149393608 0.180066204694
-7.9548344865 0.180066204606
-7.92817503691 0.180066204511
-7.90151558733 0.180066204409
-7.87485613774 0.180066204299
-7.84819668816 0.180066204181
-7.82153723857 0.180066204053
-7.79487778899 0.180066203917
-7.76821833941 0.180066203769
-7.74155888982 0.180066203611
-7.71489944024 0.180066203441
-7.68823999065 0.180066203257
-7.66158054107 0.18006620306
-7.63492109149 0.180066202848
-7.6082616419 0.18006620262
-7.58160219232 0.180066202374
-7.55494274273 0.18006620211
-7.52828329315 0.180066201826
-7.50162384356 0.180066201521
-7.47496439398 0.180066201192
-7.4483049444 0.180066200839
-7.42164549481 0.180066200459
-7.39498604523 0.18006620005
-7.36832659564 0.180066199611
-7.34166714606 0.180066199138
-7.31500769648 0.180066198629
-7.28834824689 0.180066198083
-7.26168879731 0.180066197495
-7.23502934772 0.180066196863
-7.20836989814 0.180066196183
-7.18171044856 0.180066195452
-7.15505099897 0.180066194666
-7.12839154939 0.180066193821
-7.1017320998 0.180066192913
-7.07507265022 0.180066191936
-7.04841320063 0.180066190886
-7.02175375105 0.180066189758
-6.99509430147 0.180066188544
-6.96843485188 0.180066187239
-6.9417754023 0.180066185837
-6.91511595271 0.18006618433
-6.88845650313 0.180066182709
-6.86179705355 0.180066180968
-6.83513760396 0.180066179096
-6.80847815438 0.180066177083
-6.78181870479 0.180066174921
-6.75515925521 0.180066172597
-6.72849980562 0.180066170099
-6.70184035604 0.180066167415
-6.67518090646 0.18006616453
-6.64852145687 0.18006616143
-6.62186200729 0.1800661581
-6.5952025577 0.18006615452
-6.56854310812 0.180066150675
-6.54188365854 0.180066146542
-6.51522420895 0.180066142103
-6.48856475937 0.180066137333
-6.46190530978 0.180066132208
-6.4352458602 0.180066126703
-6.40858641061 0.180066120789
-6.38192696103 0.180066114436
-6.35526751145 0.180066107611
-6.32860806186 0.18006610028
-6.30194861228 0.180066092406
-6.27528916269 0.180066083949
-6.24862971311 0.180066074865
-6.22197026353 0.18006606511
-6.19531081394 0.180066054632
-6.16865136436 0.180066043381
-6.14199191477 0.180066031298
-6.11533246519 0.180066018323
-6.0886730156 0.18006600439
-6.06201356602 0.18006598943
-6.03535411644 0.180065973367
-6.00869466685 0.180065956121
-5.98203521727 0.180065937605
-5.95537576768 0.180065917727
-5.9287163181 0.180065896387
-5.90205686852 0.180065873479
-5.87539741893 0.180065848889
-5.84873796935 0.180065822493
-5.82207851976 0.180065794161
-5.79541907018 0.180065763752
-5.76875962059 0.180065731116
-5.74210017101 0.18006569609
-5.71544072143 0.180065658501
-5.68878127184 0.180065618164
-5.66212182226 0.18006557488
-5.63546237267 0.180065528435
-5.60880292309 0.180065478601
-5.58214347351 0.180065425133
-5.55548402392 0.180065367768
-5.52882457434 0.180065306227
-5.50216512475 0.180065240207
-5.47550567517 0.180065169386
-5.44884622558 0.18006509342
-5.422186776 0.180065011937
-5.39552732642 0.180064924542
-5.36886787683 0.180064830812
-5.34220842725 0.18006473029
-5.31554897766 0.180064622492
-5.28888952808 0.180064506896
-5.2622300785 0.180064382944
-5.23557062891 0.180064250041
-5.20891117933 0.180064107546
-5.18225172974 0.180063954777
-5.15559228016 0.180063791001
-5.12893283058 0.180063615435
-5.10227338099 0.180063427242
-5.07561393141 0.180063225523
-5.04895448182 0.18006300932
-5.02229503224 0.180062777605
-4.99563558265 0.180062529282
-4.96897613307 0.180062263174
-4.94231668349 0.180061978026
-4.9156572339 0.180061672493
-4.88899778432 0.180061345139
-4.86233833473 0.180060994426
-4.83567888515 0.180060618713
-4.80901943557 0.180060216241
-4.78235998598 0.180059785133
-4.7557005364 0.180059323382
-4.72904108681 0.180058828843
-4.70238163723 0.180058299221
-4.67572218764 0.180057732068
-4.64906273806 0.180057124763
-4.62240328848 0.180056474511
-4.59574383889 0.180055778323
-4.56908438931 0.180055033006
-4.54242493972 0.180054235151
-4.51576549014 0.180053381116
-4.48910604056 0.180052467013
-4.46244659097 0.18005148869
-4.43578714139 0.180050441713
-4.4091276918 0.180049321352
-4.38246824222 0.180048122555
-4.35580879263 0.180046839931
-4.32914934305 0.180045467727
-4.30248989347 0.180043999807
-4.27583044388 0.180042429621
-4.2491709943 0.180040750183
-4.22251154471 0.180038954043
-4.19585209513 0.180037033254
-4.16919264555 0.180034979343
-4.14253319596 0.180032783275
-4.11587374638 0.180030435419
-4.08921429679 0.18002792551
-4.06255484721 0.180025242605
-4.03589539762 0.180022375046
-4.00923594804 0.180019310412
-3.98257649846 0.18001603547
-3.95591704887 0.180012536124
-3.92925759929 0.180008797363
-3.9025981497 0.180004803205
-3.87593870012 0.180000536633
-3.84927925054 0.179995979534
-3.82261980095 0.179991112629
-3.79596035137 0.179985915406
-3.76930090178 0.179980366038
-3.7426414522 0.179974441312
-3.71598200261 0.179968116535
-3.68932255303 0.179961365452
-3.66266310345 0.179954160151
-3.63600365386 0.179946470962
-3.60934420428 0.179938266353
-3.58268475469 0.179929512822
-3.55602530511 0.179920174778
-3.52936585553 0.179910214422
-3.50270640594 0.179899591617
-3.47604695636 0.179888263751
-3.44938750677 0.179876185598
-3.42272805719 0.179863309165
-3.3960686076 0.179849583539
-3.36940915802 0.179834954718
-3.34274970844 0.17981936544
-3.31609025885 0.179802755002
-3.28943080927 0.179785059069
-3.26277135968 0.179766209475
-3.2361119101 0.179746134012
-3.20945246052 0.179724756219
-3.18279301093 0.179701995146
-3.15613356135 0.179677765124
-3.12947411176 0.179651975509
-3.10281466218 0.179624530432
-3.0761552126 0.179595328523
-3.04949576301 0.179564262635
-3.02283631343 0.179531219553
-2.99617686384 0.17949607969
-2.96951741426 0.179458716776
-2.94285796467 0.179418997537
-2.91619851509 0.179376781353
-2.88953906551 0.179331919921
-2.86287961592 0.179284256893
-2.83622016634 0.179233627512
-2.80956071675 0.179179858237
-2.78290126717 0.179122766355
-2.75624181759 0.179062159589
-2.729582368 0.178997835693
-2.70292291842 0.178929582048
-2.67626346883 0.178857175241
-2.64960401925 0.178780380648
-2.62294456966 0.178698952009
-2.59628512008 0.178612631007
-2.5696256705 0.178521146838
-2.54296622091 0.178424215791
-2.51630677133 0.178321540833
-2.48964732174 0.178212811193
-2.46298787216 0.178097701971
-2.43632842258 0.177975873746
-2.40966897299 0.177846972214
-2.38300952341 0.177710627842
-2.35635007382 0.177566455552
-2.32969062424 0.177414054436
-2.30303117465 0.177253007512
-2.27637172507 0.177082881523
-2.24971227549 0.176903226788
-2.2230528259 0.176713577118
-2.19639337632 0.176513449793
-2.16973392673 0.176302345627
-2.14307447715 0.176079749112
-2.11641502757 0.175845128671
-2.08975557798 0.17559793702
-2.0630961284 0.175337611652
-2.03643667881 0.175063575474
-2.00977722923 0.174775237587
-1.98311777964 0.174471994251
-1.95645833006 0.174153230035
-1.92979888048 0.173818319191
-1.90313943089 0.17346662725
-1.87647998131 0.17309751289
-1.84982053172 0.17271033008
-1.82316108214 0.172304430546
-1.79650163256 0.171879166567
-1.76984218297 0.171433894163
-1.74318273339 0.170967976678
-1.7165232838 0.17048078882
-1.68986383422 0.169971721186
-1.66320438463 0.169440185324
-1.63654493505 0.168885619368
-1.60988548547 0.168307494311
-1.58322603588 0.167705320966
-1.5565665863 0.167078657671
-1.52990713671 0.16642711881
-1.50324768713 0.165750384224
-1.47658823755 0.165048209592
-1.44992878796 0.164320437852
-1.42326933838 0.163567011796
-1.39660988879 0.162787987905
-1.36995043921 0.161983551579
-1.34329098962 0.161154033884
-1.31663154004 0.160299929963
-1.28997209046 0.159421919319
-1.26331264087 0.158520888136
-1.23665319129 0.157597953909
-1.2099937417 0.156654492644
-1.18333429212 0.155692168961
-1.15667484254 0.154712969489
-1.13001539295 0.153719240024
-1.10335594337 0.152713727004
-1.07669649378 0.151699623988
-1.0500370442 0.150680623968
-1.02337759461 0.149660978534
-0.996718145031 0.148645565156
-0.970058695447 0.147639964151
-0.943399245863 0.146650547295
-0.916739796278 0.145684580559
-0.890080346694 0.144750344086
-0.86342089711 0.143857273416
-0.836761447526 0.143016127072
-0.810101997942 0.142239187137
-0.783442548358 0.141540501462
-0.756783098773 0.140936178848
-0.730123649189 0.140444752269
-0.703464199605 0.140087630298
-0.676804750021 0.139889664056
-0.650145300437 0.139879867132
-0.623485850853 0.14009234051
-0.596826401268 0.140567475868
-0.570166951684 0.141353542451
-0.5435075021 0.142508811166
-0.516848052516 0.144104445094
-0.490188602932 0.146228506482
-0.463529153348 0.148991629637
-0.436869703764 0.15253524941
-0.410210254179 0.157043879486
-0.383550804595 0.162764060506
-0.356891355011 0.170034816141
-0.330231905427 0.179339137067
-0.303572455843 0.191396786496
-0.276913006259 0.207346459256
-0.250253556674 0.229148590088
-0.22359410709 0.260653857373
-0.196934657506 0.311535299056


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForGaussianSigma1.tex <==
0.998404231942 2.1954407823e-09
0.996808470268 1.71569571284e-08
0.995212721359 5.76503182146e-08
0.993616991599 1.36440680462e-07
0.992021287371 2.66292281172e-07
0.990425615056 4.59968132197e-07
0.988829981037 7.30229713657e-07
0.987234391695 1.08983666768e-06
0.985638853412 1.55154649222e-06
0.984043372566 2.12811423492e-06
0.982447955539 2.83229218707e-06
0.980852608708 3.67682957764e-06
0.979257338452 4.67447226737e-06
0.977662151148 5.83796244303e-06
0.976067053172 7.18003831172e-06
0.974472050899 8.71343379536e-06
0.972877150702 1.04508782252e-05
0.971282358956 1.24050960367e-05
0.96968768203 1.45888064641e-05
0.968093126294 1.70147232357e-05
0.966498698118 1.96955542691e-05
0.964904403869 2.26440013662e-05
0.963310249911 2.5872759909e-05
0.961716242608 2.93945185555e-05
0.960122388323 3.32219589353e-05
0.958528693415 3.73677553459e-05
0.956935164243 4.1844574449e-05
0.955341807163 4.66650749672e-05
0.953748628528 5.18419073808e-05
0.952155634692 5.73877136249e-05
0.950562832003 6.33151267866e-05
0.948970226809 6.96367708028e-05
0.947377825456 7.6365260158e-05
0.945785634286 8.35131995824e-05
0.944193659639 9.10931837503e-05
0.942601907853 9.91177969792e-05
0.941010385262 0.000107599612928
0.939419098199 0.000116551194299
0.937828052994 0.000125985092532
0.936237255972 0.000135913847511
0.934646713457 0.000146349987261
0.93305643177 0.000157306027649
0.931466417227 0.000168794472084
0.929876676144 0.000180827811223
0.92828721483 0.000193418522667
0.926698039593 0.000206579070666
0.925109156737 0.000220321905825
0.923520572564 0.0002346594648
0.921932293369 0.000249604170008
0.920344325446 0.000265168429326
0.918756675085 0.000281364635798
0.917169348571 0.00029820516734
0.915582352187 0.000315702386445
0.913995692211 0.000333868639887
0.912409374915 0.000352716258429
0.910823406571 0.000372257556528
0.909237793445 0.000392504832046
0.907652541796 0.000413470365951
0.906067657883 0.000435166422033
0.904483147959 0.000457605246605
0.902899018271 0.000480799068219
0.901315275063 0.000504760097369
0.899731924575 0.000529500526208
0.898148973041 0.000555032528254
0.896566426691 0.000581368258103
0.894984291749 0.000608519851141
0.893402574435 0.000636499423257
0.891821280965 0.000665319070553
0.890240417547 0.000694990869063
0.888659990388 0.000725526874463
0.887080005686 0.000756939121787
0.885500469636 0.000789239625142
0.883921388427 0.000822440377426
0.882342768242 0.000856553350043
0.88076461526 0.000891590492622
0.879186935652 0.000927563732731
0.877609735585 0.000964484975601
0.876033021221 0.00100236610384
0.874456798715 0.00104121897717
0.872881074217 0.0010810554321
0.87130585387 0.00112188728172
0.869731143811 0.00116372631537
0.868156950172 0.00120658429836
0.866583279079 0.00125047297173
0.86501013665 0.00129540405195
0.863437528998 0.00134138923065
0.861865462231 0.00138844017435
0.860293942447 0.00143656852416
0.85872297574 0.00148578589556
0.857152568198 0.00153610387808
0.855582725901 0.00158753403504
0.854013454922 0.0016400879033
0.852444761329 0.00169377699297
0.85087665118 0.00174861278714
0.84930913053 0.00180460674162
0.847742205425 0.00186177028469
0.846175881903 0.0019201148168
0.844610165997 0.0019796517103
0.84304506373 0.00204039230923
0.841480581122 0.002102347929
0.839916724181 0.00216552985615
0.83835349891 0.00222994934809
0.836790911305 0.00229561763283
0.835228967353 0.00236254590872
0.833667673035 0.0024307453442
0.832107034322 0.00250022707753
0.83054705718 0.00257100221653
0.828987747565 0.00264308183836
0.827429111426 0.00271647698919
0.825871154704 0.00279119868402
0.824313883331 0.00286725790638
0.822757303234 0.0029446656081
0.821201420328 0.00302343270904
0.819646240522 0.00310357009686
0.818091769716 0.00318508862675
0.816538013802 0.00326799912117
0.814984978663 0.00335231236965
0.813432670175 0.00343803912848
0.811881094202 0.00352519012053
0.810330256604 0.00361377603493
0.80878016323 0.0037038075269
0.807230819918 0.00379529521745
0.805682232502 0.00388824969316
0.804134406802 0.00398268150593
0.802587348634 0.00407860117278
0.801041063801 0.00417601917552
0.799495558099 0.00427494596063
0.797950837315 0.00437539193891
0.796406907225 0.00447736748533
0.794863773596 0.00458088293872
0.793321442189 0.00468594860162
0.791779918751 0.00479257473997
0.790239209023 0.00490077158292
0.788699318733 0.00501054932257
0.787160253604 0.0051219181138
0.785622019345 0.00523488807395
0.784084621658 0.00534946928268
0.782548066233 0.00546567178168
0.781012358753 0.00558350557448
0.779477504888 0.0057029806262
0.777943510301 0.00582410686337
0.776410380643 0.00594689417366
0.774878121554 0.00607135240567
0.773346738667 0.00619749136873
0.771816237602 0.00632532083267
0.77028662397 0.00645485052759
0.768757903372 0.00658609014368
0.767230081396 0.00671904933095
0.765703163623 0.00685373769907
0.764177155622 0.0069901648171
0.762652062951 0.00712834021336
0.761127891157 0.00726827337512
0.759604645777 0.00740997374848
0.758082332339 0.00755345073809
0.756560956356 0.00769871370701
0.755040523334 0.00784577197644
0.753521038765 0.00799463482556
0.752002508133 0.00814531149131
0.750484936909 0.0082978111682
0.748968330553 0.00845214300807
0.747452694515 0.00860831611996
0.745938034231 0.00876633956983
0.744424355129 0.00892622238044
0.742911662623 0.00908797353109
0.741399962119 0.00925160195748
0.739889259007 0.00941711655147
0.738379558668 0.00958452616091
0.736870866473 0.00975383958945
0.735363187777 0.00992506559636
0.733856527928 0.0100982128963
0.732350892259 0.0102732901592
0.730846286092 0.01045030601
0.729342714737 0.0106292690286
0.727840183494 0.0108101877494
0.726338697649 0.0109930706614
0.724838262475 0.011177926208
0.723338883236 0.0113647627866
0.721840565181 0.0115535887487
0.720343313548 0.0117444123993
0.718847133564 0.0119372419974
0.717352030441 0.0121320857551
0.715858009381 0.0123289518381
0.714365075572 0.0125278483648
0.71287323419 0.0127287834068
0.711382490399 0.0129317649884
0.70989284935 0.0131368010864
0.708404316181 0.0133438996301
0.706916896019 0.0135530685011
0.705430593976 0.0137643155329
0.703945415152 0.0139776485112
0.702461364634 0.0141930751733
0.700978447498 0.0144106032081
0.699496668805 0.014630240256
0.698016033603 0.0148519939087
0.696536546928 0.0150758717091
0.695058213802 0.015301881151
0.693581039235 0.015530029679
0.692105028222 0.0157603246886
0.690630185747 0.0159927735257
0.689156516779 0.0162273834865
0.687684026275 0.0164641618175
0.686212719176 0.0167031157155
0.684742600413 0.0169442523271
0.683273674902 0.0171875787486
0.681805947545 0.0174331020261
0.68033942323 0.0176808291553
0.678874106833 0.0179307670812
0.677410003216 0.0181829226981
0.675947117225 0.0184373028494
0.674485453696 0.0186939143275
0.673025017449 0.0189527638737
0.671565813289 0.0192138581781
0.67010784601 0.0194772038791
0.668651120389 0.0197428075639
0.667195641191 0.0200106757679
0.665741413167 0.0202808149748
0.664288441053 0.0205532316164
0.662836729571 0.0208279320723
0.661386283429 0.0211049226702
0.659937107321 0.0213842096854
0.658489205927 0.0216657993408
0.657042583912 0.021949697807
0.655597245926 0.0222359112018
0.654153196607 0.0225244455903
0.652710440576 0.0228153069848
0.651268982441 0.0231085013448
0.649828826794 0.0234040345764
0.648389978215 0.0237019125329
0.646952441268 0.0240021410142
0.645516220501 0.0243047257668
0.644081320449 0.0246096724837
0.642647745631 0.0249169868045
0.641215500554 0.025226674315
0.639784589707 0.0255387405472
0.638355017565 0.0258531909793
0.636926788589 0.0261700310355
0.635499907225 0.0264892660861
0.634074377903 0.026810901447
0.632650205039 0.0271349423801
0.631227393032 0.0274613940928
0.62980594627 0.0277902617382
0.628385869121 0.0281215504148
0.626967165942 0.0284552651667
0.625549841071 0.0287914109831
0.624133898835 0.0291299927987
0.622719343541 0.0294710154932
0.621306179485 0.0298144838913
0.619894410945 0.030160402763
0.618484042185 0.0305087768232
0.617075077452 0.0308596107313
0.615667520979 0.031212909092
0.614261376983 0.0315686764544
0.612856649666 0.0319269173123
0.611453343213 0.0322876361043
0.610051461795 0.0326508372132
0.608651009567 0.0330165249665
0.607251990667 0.033384703636
0.605854409219 0.0337553774378
0.604458269331 0.0341285505324
0.603063575094 0.0345042270245
0.601670330585 0.0348824109627
0.600278539863 0.03526310634
0.598888206974 0.0356463170933
0.597499335945 0.0360320471037
0.59611193079 0.0364203001958
0.594725995504 0.0368110801386
0.593341534069 0.0372043906447
0.591958550449 0.0376002353704
0.590577048592 0.0379986179159
0.589197032431 0.0383995418252
0.587818505883 0.0388030105858
0.586441472848 0.0392090276288
0.585065937209 0.0396175963291
0.583691902835 0.040028720005
0.582319373577 0.0404424019183
0.58094835327 0.0408586452744
0.579578845735 0.0412774532221
0.578210854772 0.0416988288535
0.57684438417 0.0421227752042
0.575479437698 0.0425492952532
0.57411601911 0.0429783919229
0.572754132142 0.0434100680787
0.571393780517 0.0438443265296
0.570034967938 0.0442811700277
0.568677698093 0.0447206012685
0.567321974653 0.0451626228904
0.565967801274 0.0456072374755
0.564615181593 0.0460544475486
0.563264119233 0.046504255578
0.561914617797 0.046956663975
0.560566680875 0.0474116750942
0.559220312039 0.0478692912331
0.557875514842 0.0483295146326
0.556532292825 0.0487923474766
0.555190649507 0.0492577918922
0.553850588394 0.0497258499494
0.552512112974 0.0501965236615
0.551175226719 0.0506698149849
0.549839933081 0.0511457258192
0.5485062355 0.0516242580069
0.547174137396 0.0521054133337
0.545843642172 0.0525891935286
0.544514753215 0.0530756002634
0.543187473895 0.0535646351534
0.541861807566 0.0540562997568
0.540537757563 0.0545505955751
0.539215327205 0.0550475240528
0.537894519795 0.0555470865777
0.536575338616 0.056049284481
0.535257786938 0.0565541190367
0.533941868011 0.0570615914623
0.532627585068 0.0575717029186
0.531314941328 0.0580844545096
0.530003939988 0.0585998472825
0.528694584231 0.059117882228
0.527386877224 0.05963856028
0.526080822113 0.0601618823159
0.52477642203 0.0606878491566
0.523473680089 0.061216461566
0.522172599386 0.0617477202521
0.520873183 0.0622816258658
0.519575433993 0.062818179002
0.518279355411 0.0633573801989
0.51698495028 0.0638992299384
0.515692221612 0.0644437286461
0.514401172398 0.0649908766911
0.513111805614 0.0655406743866
0.51182412422 0.0660931219891
0.510538131155 0.0666482196993
0.509253829343 0.0672059676616
0.50797122169 0.0677663659643
0.506690311086 0.0683294146397
0.505411100402 0.0688951136642
0.504133592491 0.0694634629581
0.502857790191 0.070034462386
0.50158369632 0.0706081117564
0.500311313681 0.0711844108223
0.499040645057 0.0717633592809
0.497771693216 0.0723449567737
0.496504460907 0.0729292028865
0.495238950862 0.0735160971499
0.493975165796 0.0741056390387
0.492713108404 0.0746978279724
0.491452781368 0.0752926633152
0.490194187349 0.075890144376
0.48893732899 0.0764902704085
0.48768220892 0.0770930406112
0.486428829748 0.0776984541276
0.485177194065 0.0783065100462
0.483927304446 0.0789172074006
0.482679163448 0.0795305451695
0.481432773609 0.0801465222769
0.480188137452 0.0807651375921
0.47894525748 0.0813863899296
0.47770413618 0.0820102780497
0.476464776021 0.082636800658
0.475227179455 0.0832659564059
0.473991348914 0.0838977438903
0.472757286816 0.0845321616542
0.471524995559 0.0851692081863
0.470294477523 0.0858088819212
0.469065735072 0.0864511812399
0.467838770553 0.0870961044692
0.466613586293 0.0877436498824
0.465390184602 0.088393815699
0.464168567774 0.0890466000851
0.462948738083 0.0897020011531
0.461730697789 0.0903600169624
0.46051444913 0.0910206455187
0.45929999433 0.0916838847749
0.458087335592 0.0923497326307
0.456876475105 0.0930181869327
0.455667415038 0.093689245475
0.454460157543 0.0943629059986
0.453254704754 0.0950391661921
0.452051058788 0.0957180236913
0.450849221745 0.0963994760799
0.449649195705 0.097083520889
0.448450982733 0.0977701555977
0.447254584875 0.0984593776329
0.44606000416 0.0991511843695
0.444867242599 0.0998455731307
0.443676302185 0.100542541188
0.442487184894 0.10124208576
0.441299892685 0.101944204017
0.440114427498 0.102648893074
0.438930791257 0.103356149997
0.437748985866 0.1040659718
0.436569013214 0.104778355448
0.435390875171 0.105493297851
0.434214573591 0.106210795873
0.433040110307 0.106930846324
0.431867487138 0.107653445965
0.430696705884 0.108378591505
0.429527768327 0.109106279605
0.428360676233 0.109836506874
0.427195431349 0.110569269873
0.426032035404 0.11130456511
0.424870490112 0.112042389047
0.423710797167 0.112782738094
0.422552958246 0.113525608612
0.42139697501 0.114270996912
0.4202428491 0.115018899258
0.419090582142 0.115769311863
0.417940175743 0.116522230892
0.416791631493 0.11727765246
0.415644950965 0.118035572636
0.414500135713 0.118795987438
0.413357187275 0.119558892836
0.412216107172 0.120324284753
0.411076896905 0.121092159064
0.409939557961 0.121862511595
0.408804091808 0.122635338124
0.407670499895 0.123410634384
0.406538783656 0.124188396057
0.405408944507 0.124968618781
0.404280983847 0.125751298144
0.403154903056 0.12653642969
0.402030703499 0.127324008914
0.400908386521 0.128114031265
0.399787953452 0.128906492145
0.398669405604 0.129701386911
0.397552744272 0.130498710874
0.396437970732 0.131298459296
0.395325086245 0.132100627396
0.394214092054 0.132905210347
0.393104989385 0.133712203276
0.391997779445 0.134521601264
0.390892463427 0.135333399348
0.389789042504 0.13614759252
0.388687517832 0.136964175725
0.387587890553 0.137783143867
0.386490161788 0.138604491802
0.385394332644 0.139428214344
0.384300404207 0.140254306261
0.383208377551 0.141082762278
0.382118253729 0.141913577078
0.381030033778 0.142746745296
0.379943718718 0.143582261527
0.378859309553 0.144420120322
0.37777680727 0.145260316188
0.376696212836 0.14610284359
0.375617527205 0.146947696949
0.374540751312 0.147794870646
0.373465886074 0.148644359017
0.372392932395 0.149496156356
0.371321891158 0.150350256916
0.370252763231 0.151206654909
0.369185549464 0.152065344502
0.368120250694 0.152926319824
0.367056867735 0.15378957496
0.365995401389 0.154655103957
0.36493585244 0.155522900818
0.363878221655 0.156392959506
0.362822509784 0.157265273945
0.36176871756 0.158139838017
0.3607168457 0.159016645564
0.359666894906 0.159895690389
0.35861886586 0.160776966255
0.357572759229 0.161660466884
0.356528575664 0.16254618596
0.355486315798 0.163434117127
0.35444598025 0.16432425399
0.353407569619 0.165216590116
0.352371084491 0.166111119033
0.351336525432 0.16700783423
0.350303892994 0.167906729159
0.349273187713 0.168807797232
0.348244410107 0.169711031824
0.347217560677 0.170616426274
0.346192639911 0.171523973881
0.345169648276 0.172433667908
0.344148586227 0.173345501582
0.343129454201 0.17425946809
0.342112252617 0.175175560586
0.341096981881 0.176093772185
0.340083642381 0.177014095968
0.339072234488 0.177936524977
0.338062758559 0.178861052221
0.337055214934 0.179787670671
0.336049603935 0.180716373265
0.335045925872 0.181647152904
0.334044181035 0.182580002455
0.3330443697 0.183514914749
0.332046492127 0.184451882584
0.331050548559 0.185390898722
0.330056539224 0.186331955892
0.329064464334 0.187275046788
0.328074324084 0.188220164073
0.327086118655 0.189167300372
0.326099848212 0.19011644828
0.325115512902 0.191067600357
0.324133112858 0.192020749133
0.323152648197 0.192975887102
0.322174119022 0.193933006727
0.321197525416 0.194892100439
0.320222867451 0.195853160635
0.31925014518 0.196816179684
0.318279358643 0.197781149919
0.317310507863 0.198748063645
0.316343592847 0.199716913135
0.315378613588 0.200687690628
0.314415570063 0.201660388337
0.313454462232 0.202634998442
0.312495290043 0.203611513091
0.311538053425 0.204589924407
0.310582752293 0.205570224477
0.309629386549 0.206552405362
0.308677956077 0.207536459094
0.307728460745 0.208522377673
0.30678090041 0.209510153073
0.305835274908 0.210499777237
0.304891584066 0.21149124208
0.30394982769 0.212484539489
0.303010005577 0.213479661324
0.302072117503 0.214476599414
0.301136163233 0.215475345563
0.300202142517 0.216475891547
0.299270055086 0.217478229114
0.298339900662 0.218482349986
0.297411678947 0.219488245857
0.296485389632 0.220495908397
0.29556103239 0.221505329245
0.294638606882 0.222516500019
0.293718112752 0.223529412307
0.292799549631 0.224544057675
0.291882917134 0.225560427661
0.290968214863 0.226578513778
0.290055442403 0.227598307516
0.289144599328 0.228619800337
0.288235685194 0.229642983681
0.287328699544 0.230667848963
0.286423641906 0.231694387574
0.285520511796 0.23272259088
0.284619308712 0.233752450226
0.28372003214 0.234783956931
0.28282268155 0.235817102292
0.281927256401 0.236851877583
0.281033756134 0.237888274056
0.280142180178 0.238926282937
0.279252527946 0.239965895436
0.27836479884 0.241007102734
0.277478992245 0.242049895996
0.276595107534 0.243094266362
0.275713144064 0.244140204952
0.27483310118 0.245187702865
0.273954978211 0.246236751177
0.273078774474 0.247287340947
0.272204489272 0.248339463211
0.271332121893 0.249393108984
0.270461671612 0.250448269264
0.26959313769 0.251504935028
0.268726519374 0.252563097231
0.2678618159 0.253622746813
0.266999026485 0.254683874692
0.266138150339 0.255746471769
0.265279186652 0.256810528924
0.264422134606 0.25787603702
0.263566993366 0.258942986904
0.262713762085 0.260011369401
0.261862439903 0.26108117532
0.261013025945 0.262152395455
0.260165519324 0.26322502058
0.259319919141 0.264299041452
0.25847622448 0.265374448812
0.257634434416 0.266451233386
0.256794548008 0.26752938588
0.255956564303 0.268608896987
0.255120482335 0.269689757384
0.254286301126 0.270771957732
0.253454019682 0.271855488674
0.252623636999 0.272940340842
0.25179515206 0.274026504851
0.250968563833 0.275113971302
0.250143871274 0.27620273078
0.249321073329 0.277292773857
0.248500168927 0.278384091092
0.247681156987 0.279476673028
0.246864036414 0.280570510197
0.246048806103 0.281665593115
0.245235464933 0.282761912286
0.244424011772 0.283859458203
0.243614445477 0.284958221343
0.24280676489 0.286058192173
0.242000968842 0.287159361148
0.241197056152 0.288261718709
0.240395025626 0.289365255288
0.239594876058 0.290469961303
0.238796606229 0.291575827162
0.23800021491 0.292682843261
0.237205700858 0.293790999988
0.236413062818 0.294900287717
0.235622299524 0.296010696814
0.234833409697 0.297122217633
0.234046392046 0.29823484052
0.23326124527 0.29934855581
0.232477968053 0.300463353829
0.231696559071 0.301579224894
0.230917016984 0.302696159312
0.230139340443 0.303814147384
0.229363528088 0.304933179399
0.228589578545 0.306053245639
0.22781749043 0.30717433638
0.227047262347 0.308296441886
0.226278892888 0.309419552418
0.225512380634 0.310543658226
0.224747724156 0.311668749553
0.22398492201 0.312794816639
0.223223972745 0.313921849712
0.222464874896 0.315049838996
0.221707626987 0.31617877471
0.220952227531 0.317308647065
0.220198675031 0.318439446267
0.219446967978 0.319571162515
0.218697104851 0.320703786004
0.21794908412 0.321837306924
0.217202904243 0.32297171546
0.216458563666 0.324107001791
0.215716060827 0.325243156092
0.214975394149 0.326380168534
0.214236562049 0.327518029285
0.213499562929 0.328656728508
0.212764395183 0.329796256361
0.212031057194 0.330936603001
0.211299547334 0.33207775858
0.210569863963 0.333219713249
0.209842005434 0.334362457155
0.209115970085 0.335505980441
0.208391756248 0.336650273251
0.207669362243 0.337795325723
0.206948786377 0.338941127997
0.206230026952 0.340087670209
0.205513082254 0.341234942493
0.204797950564 0.342382934983
0.20408463015 0.343531637813
0.203373119269 0.344681041113
0.202663416172 0.345831135015
0.201955519095 0.34698190965
0.201249426268 0.348133355149
0.200545135909 0.349285461642
0.199842646227 0.35043821926
0.19914195542 0.351591618134
0.198443061679 0.352745648396
0.197745963182 0.35390030018
0.197050658099 0.355055563618
0.196357144591 0.356211428846
0.195665420808 0.357367886002
0.194975484891 0.358524925222
0.194287334971 0.359682536648
0.193600969171 0.360840710421
0.192916385604 0.361999436688
0.192233582373 0.363158705593
0.191552557572 0.364318507289
0.190873309286 0.365478831926
0.19019583559 0.366639669663
0.189520134553 0.367801010657
0.188846204229 0.368962845071
0.188174042669 0.370125163073
0.187503647912 0.371287954834
0.186835017987 0.372451210526
0.186168150917 0.373614920331
0.185503044714 0.374779074431
0.184839697381 0.375943663014
0.184178106915 0.377108676275
0.183518271301 0.378274104412
0.182860188516 0.379439937628
0.182203856531 0.380606166133
0.181549273304 0.381772780142
0.180896436789 0.382939769876
0.180245344929 0.384107125563
0.179595995658 0.385274837435
0.178948386903 0.386442895734
0.178302516582 0.387611290705
0.177658382606 0.388780012602
0.177015982875 0.389949051687
0.176375315283 0.391118398228
0.175736377716 0.392288042499
0.175099168051 0.393457974784
0.174463684157 0.394628185375
0.173829923894 0.395798664571
0.173197885117 0.396969402678
0.17256756567 0.398140390014
0.17193896339 0.399311616902
0.171312076108 0.400483073676
0.170686901644 0.401654750678
0.170063437813 0.402826638259
0.169441682421 0.403998726781
0.168821633268 0.405171006615
0.168203288143 0.406343468139
0.16758664483 0.407516101745
0.166971701106 0.408688897832
0.166358454739 0.409861846811
0.16574690349 0.411034939103
0.165137045113 0.41220816514
0.164528877355 0.413381515364
0.163922397955 0.414554980228
0.163317604645 0.415728550197
0.16271449515 0.416902215747
0.162113067187 0.418075967366
0.161513318468 0.419249795552
0.160915246695 0.420423690817
0.160318849567 0.421597643684
0.159724124772 0.422771644689
0.159131069993 0.423945684378
0.158539682907 0.425119753314
0.157949961182 0.426293842068
0.157361902482 0.427467941227
0.156775504462 0.428642041391
0.156190764772 0.42981613317
0.155607681053 0.430990207193
0.155026250942 0.432164254097
0.154446472069 0.433338264536
0.153868342057 0.434512229178
0.153291858521 0.435686138703
0.152717019073 0.436859983807
0.152143821317 0.438033755201
0.15157226285 0.439207443608
0.151002341264 0.440381039769
0.150434054144 0.441554534436
0.149867399069 0.442727918381
0.149302373612 0.443901182387
0.148738975341 0.445074317254
0.148177201816 0.446247313798
0.147617050592 0.447420162849
0.147058519219 0.448592855257
0.146501605241 0.449765381882
0.145946306194 0.450937733605
0.14539261961 0.452109901322
0.144840543016 0.453281875944
0.144290073932 0.4544536484
0.143741209872 0.455625209637
0.143193948347 0.456796550616
0.142648286859 0.457967662317
0.142104222907 0.459138535738
0.141561753983 0.460309161892
0.141020877576 0.461479531812
0.140481591166 0.462649636547
0.139943892231 0.463819467165
0.139407778243 0.46498901475
0.138873246667 0.466158270407
0.138340294964 0.467327225258
0.137808920591 0.468495870443
0.137279120998 0.46966419712
0.136750893632 0.470832196467
0.136224235933 0.471999859681
0.135699145338 0.473167177977
0.135175619277 0.474334142589
0.134653655176 0.475500744772
0.134133250457 0.476666975799
0.133614402538 0.477832826961
0.133097108829 0.478998289573
0.132581366738 0.480163354966
0.132067173668 0.481328014492
0.131554527016 0.482492259523
0.131043424178 0.483656081453
0.130533862541 0.484819471694
0.13002583949 0.485982421679
0.129519352406 0.487144922862
0.129014398665 0.488306966718
0.128510975638 0.489468544743
0.128009080692 0.490629648452
0.127508711192 0.491790269385
0.127009864495 0.492950399099
0.126512537957 0.494110029175
0.126016728928 0.495269151215
0.125522434755 0.496427756842
0.125029652782 0.497585837702
0.124538380346 0.49874338546
0.124048614783 0.499900391808
0.123560353424 0.501056848454
0.123073593595 0.502212747134
0.122588332621 0.503368079601
0.122104567821 0.504522837636
0.121622296511 0.505677013038
0.121141516004 0.50683059763
0.120662223608 0.50798358326
0.120184416629 0.509135961795
0.119708092368 0.510287725129
0.119233248123 0.511438865177
0.11875988119 0.512589373876
0.118287988859 0.51373924319
0.117817568419 0.514888465103
0.117348617155 0.516037031624
0.116881132348 0.517184934787
0.116415111277 0.518332166647
0.115950551216 0.519478719285
0.115487449439 0.520624584806
0.115025803212 0.521769755337
0.114565609804 0.522914223032
0.114106866476 0.524057980068
0.113649570488 0.525201018645
0.113193719097 0.526343330991
0.112739309559 0.527484909355
0.112286339123 0.528625746014
0.111834805039 0.529765833267
0.111384704552 0.530905163438
0.110936034905 0.53204372888
0.11048879334 0.533181521965
0.110042977093 0.534318535096
0.109598583399 0.535454760697
0.109155609492 0.536590191219
0.108714052602 0.53772481914
0.108273909956 0.53885863696
0.10783517878 0.539991637209
0.107397856296 0.541123812439
0.106961939726 0.54225515523
0.106527426287 0.543385658187
0.106094313196 0.544515313942
0.105662597665 0.545644115151
0.105232276909 0.546772054499
0.104803348134 0.547899124694
0.10437580855 0.549025318474
0.103949655361 0.550150628601
0.10352488577 0.551275047864
0.10310149698 0.552398569079
0.10267948619 0.553521185088
0.102258850596 0.55464288876
0.101839587396 0.555763672992
0.101421693783 0.556883530705
0.101005166948 0.558002454851
0.100590004083 0.559120438405
0.100176202376 0.560237474372
0.0997637590147 0.561353555784
0.0993526711837 0.562468675697
0.0989429360673 0.5635828272
0.0985345508477 0.564696003404
0.0981275127059 0.56580819745
0.0977218188212 0.566919402507
0.0973174663715 0.568029611771
0.0969144525334 0.569138818465
0.0965127744823 0.570247015841
0.0961124293919 0.571354197177
0.0957134144349 0.572460355782
0.0953157267829 0.573565484989
0.0949193636059 0.574669578163
0.0945243220731 0.575772628694
0.0941305993525 0.576874630001
0.093738192611 0.577975575532
0.0933470990143 0.579075458762
0.0929573157274 0.580174273197
0.0925688399142 0.581272012367
0.0921816687375 0.582368669834
0.0917957993594 0.583464239187
0.0914112289411 0.584558714044
0.0910279546431 0.585652088051
0.0906459736249 0.586744354884
0.0902652830454 0.587835508246
0.0898858800627 0.58892554187
0.0895077618343 0.590014449517
0.0891309255171 0.591102224978
0.0887553682673 0.592188862071
0.0883810872406 0.593274354644
0.0880080795921 0.594358696574
0.0876363424765 0.595441881768
0.0872658730481 0.596523904161
0.0868966684605 0.597604757716
0.0865287258673 0.598684436428
0.0861620424215 0.599762934319
0.0857966152758 0.600840245441
0.0854324415827 0.601916363876
0.0850695184944 0.602991283732
0.0847078431629 0.604064999152
0.0843474127401 0.605137504304
0.0839882243776 0.606208793387
0.0836302752272 0.607278860629
0.0832735624402 0.608347700288
0.0829180831683 0.609415306651
0.0825638345628 0.610481674037
0.0822108137754 0.61154679679
0.0818590179576 0.612610669288
0.0815084442611 0.613673285937
0.0811590898378 0.614734641172
0.0808109518396 0.615794729459
0.0804640274187 0.616853545294
0.0801183137276 0.6179110832
0.079773807919 0.618967337734
0.079430507146 0.620022303481
0.0790884085617 0.621075975054
0.07874750932 0.622128347099
0.078407806575 0.62317941429
0.0780692974811 0.624229171333
0.0777319791935 0.625277612961
0.0773958488676 0.626324733939
0.0770609036595 0.627370529062
0.0767271407257 0.628414993155
0.0763945572236 0.629458121073
0.0760631503108 0.6304999077
0.0757329171458 0.631540347951
0.075403854888 0.632579436772
0.075075960697 0.633617169139
0.0747492317337 0.634653540056
0.0744236651594 0.63568854456
0.0740992581364 0.636722177715
0.0737760078277 0.63775443462
0.0734539113975 0.638785310399
0.0731329660104 0.63981480021
0.0728131688324 0.640842899239
0.0724945170303 0.641869602703
0.0721770077718 0.64289490585
0.0718606382259 0.643918803958
0.0715454055622 0.644941292334
0.071231306952 0.645962366317
0.0709183395672 0.646982021276
0.0706065005811 0.648000252609
0.0702957871681 0.649017055745
0.0699861965039 0.650032426144
0.0696777257654 0.651046359296
0.0693703721306 0.652058850721
0.0690641327792 0.653069895969
0.0687590048918 0.654079490621
0.0684549856506 0.655087630289
0.068152072239 0.656094310614
0.0678502618421 0.657099527268
0.0675495516463 0.658103275953
0.0672499388393 0.659105552401
0.0669514206105 0.660106352375
0.0666539941507 0.661105671668
0.0663576566525 0.662103506105
0.0660624053098 0.663099851537
0.0657682373183 0.66409470385
0.0654751498752 0.665088058958
0.0651831401795 0.666079912806
0.0648922054317 0.667070261368
0.0646023428343 0.668059100649
0.0643135495912 0.669046426685
0.0640258229085 0.670032235543
0.0637391599937 0.671016523317
0.0634535580564 0.671999286133
0.0631690143079 0.672980520149
0.0628855259615 0.673960221551
0.0626030902323 0.674938386556
0.0623217043374 0.67591501141
0.0620413654959 0.676890092391
0.0617620709287 0.677863625806
0.0614838178589 0.678835607993
0.0612066035117 0.679806035319
0.0609304251141 0.680774904181
0.0606552798955 0.681742211008
0.0603811650871 0.682707952257
0.0601080779224 0.683672124416
0.0598360156372 0.684634724003
0.0595649754692 0.685595747565
0.0592949546586 0.686555191681
0.0590259504476 0.687513052958
0.0587579600808 0.688469328035
0.0584909808051 0.689424013577
0.0582250098697 0.690377106284
0.0579600445261 0.691328602882
0.0576960820281 0.692278500128
0.057433119632 0.69322679481
0.0571711545965 0.694173483745
0.0569101841827 0.695118563778
0.0566502056542 0.696062031786
0.0563912162769 0.697003884675
0.0561332133195 0.697944119381
0.0558761940531 0.698882732869
0.0556201557512 0.699819722133
0.05536509569 0.700755084198
0.0551110111484 0.701688816119
0.0548578994077 0.702620914978
0.054605757752 0.703551377888
0.054354583468 0.704480201993
0.0541043738452 0.705407384463
0.0538551261756 0.7063329225
0.0536068377541 0.707256813334
0.0533595058783 0.708179054226
0.0531131278484 0.709099642464
0.0528677009678 0.710018575367
0.0526232225424 0.710935850282
0.0523796898809 0.711851464585
0.0521371002951 0.712765415684
0.0518954510995 0.713677701012
0.0516547396116 0.714588318033
0.0514149631518 0.71549726424
0.0511761190433 0.716404537156
0.0509382046125 0.717310134331
0.0507012171886 0.718214053344
0.0504651541039 0.719116291804
0.0502300126937 0.720016847348
0.0499957902964 0.720915717643
0.0497624842534 0.721812900382
0.0495300919091 0.72270839329
0.0492986106112 0.723602194118
0.0490680377103 0.724494300646
0.0488383705604 0.725384710684
0.0486096065185 0.726273422069
0.0483817429448 0.727160432667
0.0481547772027 0.728045740373
0.0479287066588 0.728929343108
0.047703528683 0.729811238824
0.0474792406485 0.730691425499
0.0472558399316 0.731569901142
0.0470333239121 0.732446663787
0.0468116899729 0.733321711498
0.0465909355004 0.734195042366
0.0463710578844 0.73506665451
0.0461520545178 0.735936546079
0.0459339227971 0.736804715247
0.0457166601222 0.737671160217
0.0455002638964 0.73853587922
0.0452847315263 0.739398870514
0.0450700604221 0.740260132386
0.0448562479974 0.74111966315
0.0446432916695 0.741977461145
0.0444311888589 0.742833524742
0.0442199369897 0.743687852336
0.0440095334897 0.74454044235
0.0437999757902 0.745391293236
0.0435912613259 0.746240403472
0.0433833875353 0.747087771562
0.0431763518604 0.747933396039
0.0429701517468 0.748777275463
0.0427647846439 0.749619408419
0.0425602480045 0.750459793522
0.0423565392853 0.751298429411
0.0421536559466 0.752135314754
0.0419515954524 0.752970448243
0.0417503552703 0.753803828601
0.0415499328718 0.754635454574
0.0413503257321 0.755465324935
0.0411515313302 0.756293438486
0.0409535471488 0.757119794052
0.0407563706743 0.757944390487
0.0405599993971 0.75876722667
0.0403644308114 0.759588301507
0.0401696624151 0.76040761393
0.0399756917101 0.761225162897
0.039782516202 0.762040947391
0.0395901334004 0.762854966423
0.0393985408188 0.763667219028
0.0392077359744 0.764477704269
0.0390177163887 0.765286421233
0.0388284795868 0.766093369034
0.0386400230979 0.76689854681
0.038452344455 0.767701953725
0.0382654411954 0.768503588971
0.0380793108599 0.769303451762
0.0378939509938 0.770101541339
0.0377093591461 0.770897856969
0.0375255328699 0.771692397943
0.0373424697223 0.772485163577
0.0371601672646 0.773276153213
0.0369786230619 0.774065366218
0.0367978346837 0.774852801983
0.0366177997033 0.775638459925
0.0364385156983 0.776422339486
0.0362599802501 0.77720444013
0.0360821909447 0.77798476135
0.0359051453719 0.77876330266
0.0357288411256 0.7795400636
0.0355532758041 0.780315043734
0.0353784470097 0.781088242651
0.035204352349 0.781859659963
0.0350309894325 0.782629295309
0.0348583558753 0.783397148348
0.0346864492965 0.784163218767
0.0345152673194 0.784927506274
0.0343448075715 0.785690010603
0.0341750676848 0.786450731511
0.0340060452953 0.787209668777
0.0338377380433 0.787966822208
0.0336701435734 0.788722191631
0.0335032595346 0.789475776897
0.03333708358 0.790227577881
0.0331716133672 0.790977594483
0.0330068465579 0.791725826622
0.0328427808184 0.792472274245
0.032679413819 0.793216937319
0.0325167432346 0.793959815836
0.0323547667443 0.794700909808
0.0321934820318 0.795440219274
0.0320328867848 0.796177744293
0.0318729786957 0.796913484947
0.0317137554611 0.797647441342
0.0315552147822 0.798379613604
0.0313973543643 0.799110001885
0.0312401719174 0.799838606356
0.0310836651558 0.800565427213
0.0309278317982 0.801290464673
0.0307726695679 0.802013718975
0.0306181761923 0.80273519038
0.0304643494037 0.803454879172
0.0303111869386 0.804172785656
0.030158686538 0.804888910159
0.0300068459475 0.80560325303
0.0298556629169 0.80631581464
0.0297051352008 0.80702659538
0.0295552605582 0.807735595665
0.0294060367526 0.808442815929
0.029257461552 0.809148256628
0.0291095327289 0.809851918241
0.0289622480604 0.810553801267
0.0288156053281 0.811253906224
0.0286696023182 0.811952233654
0.0285242368213 0.812648784118
0.0283795066328 0.8133435582
0.0282354095524 0.814036556503
0.0280919433846 0.81472777965
0.0279491059383 0.815417228286
0.027806895027 0.816104903077
0.027665308469 0.816790804707
0.0275243440869 0.817474933882
0.0273839997081 0.818157291329
0.0272442731646 0.818837877794
0.0271051622928 0.819516694043
0.0269666649341 0.820193740861
0.0268287789341 0.820869019056
0.0266915021434 0.821542529453
0.026554832417 0.822214272897
0.0264187676145 0.822884250254
0.0262833056004 0.823552462408
0.0261484442436 0.824218910264
0.0260141814179 0.824883594745
0.0258805150014 0.825546516793
0.0257474428772 0.826207677372
0.025614962933 0.826867077462
0.025483073061 0.827524718063
0.0253517711582 0.828180600195
0.0252210551264 0.828834724894
0.0250909228719 0.829487093219
0.0249613723057 0.830137706243
0.0248324013437 0.830786565061
0.0247040079062 0.831433670785
0.0245761899183 0.832079024546
0.0244489453101 0.832722627493
0.024322272016 0.833364480794
0.0241961679752 0.834004585633
0.0240706311319 0.834642943214
0.0239456594347 0.835279554759
0.0238212508371 0.835914421506
0.0236974032972 0.836547544713
0.0235741147779 0.837178925655
0.0234513832469 0.837808565623
0.0233292066765 0.838436465928
0.0232075830438 0.839062627897
0.0230865103307 0.839687052874
0.0229659865238 0.840309742222
0.0228460096143 0.840930697318
0.0227265775985 0.84154991956
0.0226076884771 0.84216741036
0.0224893402557 0.842783171148
0.0223715309447 0.843397203371
0.0222542585592 0.844009508492
0.022137521119 0.844620087991
0.0220213166488 0.845228943365
0.021905643178 0.845836076126
0.0217904987407 0.846441487805
0.0216758813759 0.847045179946
0.0215617891273 0.847647154111
0.0214482200434 0.848247411878
0.0213351721773 0.84884595484
0.0212226435871 0.849442784609
0.0211106323356 0.850037902808
0.0209991364905 0.85063131108
0.0208881541239 0.851223011081
0.0207776833131 0.851813004483
0.02066772214 0.852401292974
0.0205582686912 0.852987878258
0.0204493210583 0.853572762054
0.0203408773374 0.854155946093
0.0202329356297 0.854737432127
0.0201254940409 0.855317221917
0.0200185506817 0.855895317244
0.0199121036675 0.8564717199
0.0198061511183 0.857046431693
0.0197006911593 0.857619454447
0.0195957219201 0.858190789998
0.0194912415352 0.8587604402
0.0193872481441 0.859328406918
0.0192837398907 0.859894692032
0.0191807149241 0.860459297438
0.0190781713978 0.861022225044
0.0189761074703 0.861583476773
0.0188745213049 0.862143054562
0.0187734110697 0.862700960361
0.0186727749374 0.863257196136
0.0185726110856 0.863811763863
0.0184729176967 0.864364665536
0.0183736929579 0.864915903158
0.0182749350611 0.865465478749
0.0181766422032 0.86601339434
0.0180788125854 0.866559651976
0.0179814444143 0.867104253715
0.0178845359007 0.867647201629
0.0177880852607 0.868188497802
0.0176920907147 0.868728144331
0.0175965504882 0.869266143326
0.0175014628113 0.869802496909
0.017406825919 0.870337207214
0.017312638051 0.870870276391
0.0172188974518 0.871401706599
0.0171256023705 0.87193150001
0.0170327510613 0.872459658809
0.0169403417828 0.872986185192
0.0168483727987 0.873511081369
0.0167568423771 0.874034349561
0.0166657487912 0.874555991999
0.0165750903188 0.875076010929
0.0164848652423 0.875594408606
0.0163950718492 0.876111187299
0.0163057084314 0.876626349288
0.0162167732859 0.877139896862
0.016128264714 0.877651832324
0.0160401810222 0.878162157989
0.0159525205215 0.878670876179
0.0158652815275 0.879177989232
0.0157784623609 0.879683499494
0.0156920613469 0.880187409324
0.0156060768154 0.880689721089
0.0155205071011 0.881190437169
0.0154353505435 0.881689559954
0.0153506054866 0.882187091845
0.0152662702793 0.882683035253
0.0151823432752 0.8831773926
0.0150988228326 0.883670166318
0.0150157073145 0.884161358848
0.0149329950884 0.884650972644
0.014850684527 0.885139010168
0.0147687740071 0.885625473892
0.0146872619107 0.886110366299
0.0146061466242 0.88659368988
0.0145254265387 0.887075447138
0.0144451000501 0.887555640585
0.014365165559 0.88803427274
0.0142856214705 0.888511346137
0.0142064661946 0.888986863313
0.0141276981458 0.889460826819
0.0140493157432 0.889933239213
0.0139713174109 0.890404103063
0.0138937015772 0.890873420946
0.0138164666755 0.891341195447
0.0137396111436 0.891807429162
0.0136631334238 0.892272124694
0.0135870319635 0.892735284655
0.0135113052143 0.893196911666
0.0134359516326 0.893657008356
0.0133609696795 0.894115577365
0.0132863578206 0.894572621337
0.0132121145261 0.895028142928
0.0131382382711 0.8954821448
0.0130647275349 0.895934629626
0.0129915808017 0.896385600083
0.0129187965601 0.89683505886
0.0128463733036 0.89728300865
0.0127743095299 0.897729452159
0.0127026037415 0.898174392095
0.0126312544456 0.898617831178
0.0125602601537 0.899059772133
0.0124896193821 0.899500217694
0.0124193306516 0.899939170602
0.0123493924874 0.900376633605
0.0122798034195 0.900812609458
0.0122105619823 0.901247100925
0.0121416667149 0.901680110775
0.0120731161608 0.902111641786
0.0120049088681 0.902541696741
0.0119370433893 0.90297027843
0.0118695182816 0.903397389652
0.0118023321067 0.90382303321
0.0117354834307 0.904247211916
0.0116689708243 0.904669928587
0.0116027928627 0.905091186047
0.0115369481256 0.905510987126
0.0114714351971 0.905929334661
0.0114062526659 0.906346231495
0.0113413991252 0.906761680478
0.0112768731725 0.907175684463
0.01121267341 0.907588246314
0.0111487984442 0.907999368896
0.0110852468862 0.908409055083
0.0110220173513 0.908817307754
0.0109591084595 0.909224129793
0.0108965188351 0.909629524091
0.0108342471069 0.910033493544
0.0107722919081 0.910436041052
0.0107106518764 0.910837169522
0.0106493256538 0.911236881868
0.0105883118868 0.911635181005
0.0105276092261 0.912032069857
0.0104672163271 0.91242755135
0.0104071318494 0.912821628419
0.0103473544571 0.913214304
0.0102878828185 0.913605581037
0.0102287156064 0.913995462476
0.010169851498 0.914383951269
0.0101112891747 0.914771050375
0.0100530273225 0.915156762753
0.00999506463147 0.91554109137
0.0099373997962 0.915924039197
0.00988003151554 0.916305609209
0.00982295849269 0.916685804384
0.00976617943517 0.917064627706
0.00970969305479 0.917442082162
0.00965349806767 0.917818170745
0.00959759319425 0.918192896451
0.00954197715924 0.918566262278
0.00948664869165 0.918938271231
0.00943160652474 0.919308926317
0.00937684939606 0.919678230547
0.00932237604744 0.920046186936
0.00926818522493 0.920412798503
0.00921427567884 0.92077806827
0.00916064616375 0.921141999262
0.00910729543844 0.921504594509
0.00905422226593 0.921865857042
0.00900142541347 0.922225789898
0.00894890365251 0.922584396115
0.00889665575872 0.922941678734
0.00884468051194 0.923297640802
0.00879297669624 0.923652285367
0.00874154309985 0.924005615478
0.00869037851519 0.92435763419
0.00863948173883 0.92470834456
0.00858885157153 0.925057749647
0.00853848681818 0.925405852514
0.00848838628783 0.925752656224
0.00843854879366 0.926098163845
0.00838897315299 0.926442378447
0.00833965818728 0.926785303102
0.00829060272207 0.927126940885
0.00824180558704 0.927467294872
0.00819326561596 0.927806368142
0.0081449816467 0.928144163777
0.00809695252121 0.928480684859
0.00804917708552 0.928815934475
0.00800165418973 0.92914991571
0.00795438268801 0.929482631655
0.00790736143858 0.929814085401
0.00786058930371 0.930144280039
0.00781406514971 0.930473218666
0.00776778784692 0.930800904376
0.0077217562697 0.931127340268
0.00767596929645 0.93145252944
0.00763042580954 0.931776474995
0.00758512469537 0.932099180033
0.00754006484433 0.932420647659
0.00749524515077 0.932740880977
0.00745066451306 0.933059883093
0.00740632183349 0.933377657115
0.00736221601835 0.933694206151
0.00731834597786 0.93400953331
0.00727471062619 0.934323641702
0.00723130888144 0.93463653444
0.00718813966566 0.934948214635
0.0071452019048 0.9352586854
0.00710249452872 0.935567949849
0.0070600164712 0.935876011097
0.00701776666991 0.936182872258
0.00697574406639 0.936488536449
0.00693394760608 0.936793006785
0.00689237623829 0.937096286384
0.00685102891617 0.937398378362
0.00680990459676 0.937699285838
0.00676900224091 0.937999011928
0.00672832081334 0.938297559751
0.00668785928257 0.938594932425
0.00664761662096 0.938891133069
0.00660759180468 0.939186164802
0.0065677838137 0.939480030741
0.00652819163178 0.939772734005
0.00648881424649 0.940064277712
0.00644965064915 0.940354664982
0.00641069983487 0.940643898932
0.00637196080252 0.94093198268
0.00633343255472 0.941218919343
0.00629511409782 0.941504712039
0.00625700444195 0.941789363885
0.00621910260092 0.942072877997
0.00618140759228 0.942355257491
0.0061439184373 0.942636505483
0.00610663416094 0.942916625086
0.00606955379186 0.943195619416
0.00603267636241 0.943473491586
0.00599600090859 0.943750244708
0.00595952647011 0.944025881895
0.0059232520903 0.944300406256
0.00588717681618 0.944573820903
0.00585129969837 0.944846128945
0.00581561979116 0.945117333489
0.00578013615245 0.945387437643
0.00574484784375 0.945656444512
0.00570975393019 0.945924357202
0.0056748534805 0.946191178817
0.00564014556698 0.946456912458
0.00560562926553 0.946721561227
0.00557130365563 0.946985128223
0.0055371678203 0.947247616546
0.00550322084614 0.947509029291
0.00546946182328 0.947769369554
0.0054358898454 0.94802864043
0.0054025040097 0.948286845011
0.00536930341691 0.948543986387
0.00533628717125 0.948800067648
0.00530345438047 0.949055091881
0.00527080415581 0.949309062171
0.00523833561198 0.949561981603
0.00520604786718 0.949813853258
0.00517394004306 0.950064680217
0.00514201126477 0.950314465558
0.00511026066086 0.950563212356
0.00507868736335 0.950810923687
0.00504729050769 0.951057602622
0.00501606923275 0.951303252231
0.00498502268081 0.951547875583
0.00495414999757 0.951791475742
0.00492345033212 0.952034055773
0.00489292283693 0.952275618736
0.00486256666787 0.952516167691
0.00483238098415 0.952755705693
0.00480236494838 0.952994235798
0.00477251772649 0.953231761056
0.00474283848776 0.953468284518
0.00471332640483 0.953703809229
0.00468398065364 0.953938338233
0.00465480041346 0.954171874573
0.00462578486686 0.954404421287
0.00459693319972 0.954635981412
0.0045682446012 0.95486655798
0.00453971826375 0.955096154024
0.00451135338308 0.95532477257
0.0044831491582 0.955552416643
0.00445510479132 0.955779089267
0.00442721948795 0.95600479346
0.0043994924568 0.956229532239
0.00437192290983 0.956453308617
0.0043445100622 0.956676125605
0.00431725313231 0.956897986209
0.00429015134173 0.957118893436
0.00426320391524 0.957338850284
0.00423641008081 0.957557859753
0.00420976906957 0.957775924837
0.00418328011582 0.957993048528
0.00415694245703 0.958209233814
0.0041307553338 0.95842448368
0.00410471798988 0.958638801108
0.00407882967215 0.958852189075
0.00405308963061 0.959064650557
0.00402749711838 0.959276188526
0.00400205139167 0.959486805949
0.00397675170979 0.95969650579
0.00395159733514 0.959905291011
0.00392658753321 0.960113164568
0.00390172157252 0.960320129417
0.00387699872469 0.960526188506
0.00385241826438 0.960731344781
0.00382797946926 0.960935601187
0.00380368162009 0.961138960661
0.0037795240006 0.96134142614
0.00375550589757 0.961543000554
0.00373162660077 0.96174368683
0.00370788540297 0.961943487894
0.00368428159993 0.962142406664
0.00366081449039 0.962340446056
0.00363748337606 0.962537608983
0.00361428756161 0.962733898353
0.00359122635467 0.962929317068
0.00356829906581 0.963123868031
0.00354550500853 0.963317554135
0.00352284349926 0.963510378274
0.00350031385735 0.963702343335
0.00347791540506 0.9638934522
0.00345564746755 0.964083707751
0.00343350937286 0.964273112861
0.00341150045193 0.964461670402
0.00338962003855 0.964649383241
0.00336786746941 0.964836254239
0.00334624208403 0.965022286255
0.00332474322477 0.965207482143
0.00330337023685 0.965391844752
0.00328212246831 0.965575376926
0.00326099927002 0.965758081507
0.00323999999564 0.96593996133
0.00321912400165 0.966121019227
0.00319837064733 0.966301258025
0.00317773929473 0.966480680547
0.00315722930869 0.966659289611
0.0031368400568 0.966837088031
0.00311657090944 0.967014078614
0.00309642123971 0.967190264167
0.00307639042348 0.967365647487
0.00305647783932 0.96754023137
0.00303668286856 0.967714018607
0.00301700489522 0.967887011983
0.00299744330605 0.968059214279
0.00297799749047 0.96823062827
0.00295866684063 0.968401256729
0.00293945075131 0.968571102422
0.00292034862001 0.96874016811
0.00290135984686 0.968908456551
0.00288248383468 0.969075970495
0.0028637199889 0.969242712691
0.00284506771762 0.969408685881
0.00282652643155 0.969573892802
0.00280809554402 0.969738336185
0.00278977447098 0.96990201876
0.002771562631 0.970064943246
0.00275345944521 0.970227112364
0.00273546433735 0.970388528823
0.00271757673374 0.970549195333
0.00269979606326 0.970709114594
0.00268212175735 0.970868289305
0.00266455325002 0.971026722156
0.0026470899778 0.971184415836
0.00262973137977 0.971341373025
0.00261247689754 0.9714975964
0.00259532597523 0.971653088633
0.00257827805947 0.97180785239
0.0025613325994 0.971961890332
0.00254448904666 0.972115205115
0.00252774685534 0.972267799388
0.00251110548206 0.972419675798
0.00249456438585 0.972570836985
0.00247812302825 0.972721285582
0.00246178087323 0.97287102422
0.00244553738718 0.973020055522
0.00242939203898 0.973168382107
0.00241334429988 0.973316006589
0.00239739364359 0.973462931574
0.00238153954619 0.973609159667
0.00236578148621 0.973754693464
0.00235011894453 0.973899535556
0.00233455140443 0.97404368853
0.00231907835157 0.974187154967
0.00230369927398 0.974329937442
0.00228841366205 0.974472038525
0.0022732210085 0.974613460781
0.00225812080843 0.974754206768
0.00224311255924 0.974894279039
0.00222819576068 0.975033680142
0.00221336991482 0.97517241262
0.00219863452602 0.97531047901
0.00218398910096 0.975447881842
0.00216943314862 0.975584623642
0.00215496618024 0.97572070693
0.00214058770936 0.97585613422
0.00212629725178 0.975990908021
0.00211209432558 0.976125030836
0.00209797845106 0.976258505163
0.00208394915081 0.976391333492
0.00207000594961 0.976523518312
0.0020561483745 0.976655062101
0.00204237595474 0.976785967334
0.00202868822179 0.976916236481
0.00201508470933 0.977045872005
0.00200156495323 0.977174876363
0.00198812849155 0.977303252008
0.00197477486453 0.977431001385
0.00196150361459 0.977558126934
0.00194831428631 0.977684631092
0.00193520642644 0.977810516285
0.00192217958385 0.977935784938
0.00190923330959 0.978060439467
0.00189636715682 0.978184482285
0.00188358068083 0.978307915796
0.00187087343903 0.9784307424
0.00185824499095 0.978552964493
0.0018456948982 0.978674584461
0.00183322272452 0.978795604687
0.00182082803571 0.978916027548
0.00180851039964 0.979035855415
0.00179626938629 0.979155090651
0.00178410456768 0.979273735617
0.00177201551788 0.979391792665
0.00176000181302 0.979509264142
0.00174806303126 0.97962615239
0.00173619875282 0.979742459743
0.00172440855992 0.979858188532
0.00171269203679 0.979973341081
0.00170104876971 0.980087919706
0.00168947834692 0.980201926719
0.00167798035868 0.980315364427
0.00166655439722 0.980428235128
0.00165520005678 0.980540541118
0.00164391693354 0.980652284684
0.00163270462566 0.980763468108
0.00162156273325 0.980874093666
0.00161049085838 0.980984163629
0.00159948860506 0.98109368026
0.00158855557923 0.981202645818
0.00157769138875 0.981311062555
0.00156689564342 0.981418932717
0.00155616795494 0.981526258544
0.00154550793691 0.981633042271
0.00153491520485 0.981739286127
0.00152438937613 0.981844992333
0.00151393007005 0.981950163106
0.00150353690776 0.982054800655
0.00149320951227 0.982158907186
0.00148294750848 0.982262484897
0.00147275052311 0.98236553598
0.00146261818475 0.982468062622
0.00145255012382 0.982570067002
0.00144254597258 0.982671551295
0.00143260536511 0.982772517669
0.00142272793729 0.982872968286
0.00141291332684 0.982972905303
0.00140316117328 0.983072330871
0.00139347111789 0.983171247132
0.00138384280378 0.983269656225
0.00137427587583 0.983367560283
0.00136476998068 0.983464961431
0.00135532476676 0.983561861789
0.00134593988424 0.983658263472
0.00133661498505 0.983754168588
0.00132734972288 0.983849579238
0.00131814375314 0.983944497518
0.00130899673298 0.984038925519
0.00129990832127 0.984132865324
0.00129087817862 0.984226319011
0.00128190596732 0.984319288652
0.00127299135139 0.984411776313
0.00126413399653 0.984503784053
0.00125533357014 0.984595313926
0.0012465897413 0.98468636798
0.00123790218077 0.984776948256
0.00122927056099 0.984867056791
0.00122069455603 0.984956695613
0.00121217384165 0.985045866746
0.00120370809525 0.985134572207
0.00119529699587 0.985222814009
0.00118694022418 0.985310594157
0.00117863746249 0.98539791465
0.00117038839473 0.985484777481
0.00116219270644 0.985571184638
0.00115405008478 0.985657138103
0.0011459602185 0.98574263985
0.00113792279796 0.985827691849
0.00112993751509 0.985912296064
0.00112200406342 0.985996454451
0.00111412213805 0.986080168963
0.00110629143565 0.986163441543
0.00109851165444 0.986246274133
0.00109078249423 0.986328668664
0.00108310365634 0.986410627065
0.00107547484366 0.986492151256
0.0010678957606 0.986573243154
0.00106036611312 0.986653904666
0.00105288560868 0.986734137698
0.00104545395628 0.986813944145
0.00103807086641 0.9868933259
0.00103073605109 0.986972284847
0.0010234492238 0.987050822868
0.00101621009955 0.987128941833
0.00100901839482 0.987206643613
0.00100187382757 0.987283930067
0.000994776117227 0.987360803052
0.000987724984689 0.987437264416
0.000980720152318 0.987513316005
0.000973761343923 0.987588959656
0.000966848284768 0.9876641972
0.000959980701551 0.987739030464
0.000953158322411 0.987813461267
0.000946380876913 0.987887491424
0.000939648096046 0.987961122742
0.000932959712215 0.988034357024
0.000926315459236 0.988107196067
0.000919715072329 0.98817964166
0.000913158288113 0.988251695588
0.000906644844599 0.988323359631
0.000900174481184 0.988394635559
0.000893746938645 0.988465525142
0.000887361959134 0.988536030139
0.000881019286169 0.988606152305
0.000874718664633 0.98867589339
0.000868459840763 0.988745255138
0.000862242562147 0.988814239286
0.000856066577717 0.988882847565
0.000849931637743 0.988951081701
0.000843837493828 0.989018943416
0.000837783898901 0.989086434422
0.000831770607212 0.989153556428
0.000825797374325 0.989220311137
0.000819863957115 0.989286700246
0.000813970113758 0.989352725445
0.000808115603728 0.98941838842
0.000802300187791 0.98948369085
0.000796523627998 0.98954863441
0.00079078568768 0.989613220766
0.000785086131444 0.98967745158
0.000779424725164 0.989741328511
0.000773801235978 0.989804853207
0.000768215432279 0.989868027314
0.000762667083715 0.98993085247
0.000757155961178 0.98999333031
0.0007516818368 0.990055462461
0.000746244483949 0.990117250545
0.000740843677221 0.990178696179
0.000735479192438 0.990239800972
0.000730150806635 0.99030056653
0.000724858298066 0.990360994452
0.000719601446187 0.990421086331
0.000714380031659 0.990480843756
0.000709193836336 0.990540268309
0.000704042643264 0.990599361566
0.000698926236676 0.990658125098
0.000693844401982 0.990716560471
0.000688796925766 0.990774669244
0.000683783595785 0.990832452972
0.000678804200955 0.990889913202
0.000673858531354 0.990947051479
0.000668946378209 0.991003869338
0.000664067533898 0.991060368313
0.00065922179194 0.991116549928
0.00065440894699 0.991172415705
0.000649628794838 0.991227967159
0.000644881132396 0.991283205799
0.000640165757701 0.991338133129
0.000635482469904 0.991392750648
0.000630831069269 0.991447059849
0.000626211357162 0.991501062219
0.000621623136054 0.99155475924
0.000617066209509 0.991608152389
0.000612540382181 0.991661243136
0.000608045459811 0.991714032947
0.000603581249217 0.991766523283
0.000599147558296 0.991818715597
0.000594744196013 0.99187061134
0.000590370972396 0.991922211954
0.000586027698538 0.991973518879
0.000581714186581 0.992024533547
0.000577430249723 0.992075257386
0.000573175702201 0.992125691817
0.000568950359297 0.992175838258
0.000564754037326 0.992225698121
0.000560586553632 0.99227527281
0.000556447726588 0.992324563728
0.000552337375583 0.992373572269
0.000548255321026 0.992422299823
0.000544201384332 0.992470747776
0.000540175387927 0.992518917506
0.000536177155234 0.992566810387
0.000532206510675 0.99261442779
0.000528263279662 0.992661771077
0.000524347288595 0.992708841606
0.000520458364855 0.992755640731
0.0005165963368 0.992802169799
0.000512761033763 0.992848430154
0.000508952286043 0.992894423132
0.000505169924902 0.992940150065
0.000501413782561 0.992985612282
0.000497683692196 0.993030811103
0.000493979487933 0.993075747845
0.000490301004839 0.993120423819
0.000486648078925 0.993164840333
0.000483020547136 0.993208998686
0.000479418247348 0.993252900175
0.000475841018365 0.993296546092
0.00047228869991 0.993339937721
0.000468761132627 0.993383076344
0.000465258158071 0.993425963236
0.000461779618706 0.993468599668
0.000458325357899 0.993510986904
0.000454895219919 0.993553126206
0.000451489049929 0.99359501883
0.000448106693982 0.993636666024
0.000444747999019 0.993678069035
0.000441412812862 0.993719229103
0.00043810098421 0.993760147464
0.000434812362639 0.993800825347
0.000431546798589 0.993841263978
0.00042830414337 0.993881464577
0.000425084249147 0.993921428361
0.000421886968946 0.993961156538
0.000418712156643 0.994000650316
0.000415559666961 0.994039910895
0.000412429355468 0.99407893947
0.00040932107857 0.994117737233
0.000406234693509 0.994156305369
0.000403170058357 0.994194645059
0.000400127032015 0.994232757481
0.000397105474203 0.994270643804
0.000394105245463 0.994308305197
0.00039112620715 0.994345742821
0.000388168221429 0.994382957832
0.000385231151271 0.994419951383
0.000382314860451 0.994456724622
0.00037941921354 0.994493278691
0.000376544075903 0.994529614727
0.000373689313698 0.994565733865
0.000370854793867 0.994601637232
0.000368040384132 0.994637325952
0.000365245952998 0.994672801145
0.000362471369741 0.994708063924
0.000359716504407 0.994743115399
0.00035698122781 0.994777956675
0.000354265411525 0.994812588852
0.000351568927887 0.994847013026
0.000348891649984 0.994881230287
0.000346233451657 0.994915241723
0.000343594207492 0.994949048415
0.000340973792819 0.994982651439
0.000338372083706 0.995016051869
0.00033578895696 0.995049250773
0.000333224290117 0.995082249213
0.00033067796144 0.99511504825
0.00032814984992 0.995147648936
0.000325639835265 0.995180052322
0.000323147797901 0.995212259453
0.000320673618968 0.995244271371
0.000318217180315 0.99527608911
0.000315778364496 0.995307713703
0.000313357054768 0.995339146178
0.000310953135085 0.995370387557
0.000308566490098 0.995401438859
0.000306197005148 0.995432301097
0.000303844566262 0.995462975282
0.000301509060155 0.995493462419
0.000299190374219 0.995523763508
0.000296888396525 0.995553879545
0.000294603015815 0.995583811524
0.000292334121503 0.995613560432
0.000290081603669 0.995643127251
0.000287845353055 0.995672512962
0.000285625261064 0.995701718539
0.000283421219752 0.995730744952
0.00028123312183 0.995759593167
0.000279060860657 0.995788264147
0.000276904330239 0.99581675885
0.000274763425222 0.995845078227
0.000272638040892 0.99587322323
0.00027052807317 0.995901194802
0.000268433418609 0.995928993884
0.000266353974392 0.995956621413
0.000264289638326 0.995984078321
0.000262240308841 0.996011365537
0.000260205884984 0.996038483983
0.000258186266419 0.996065434581
0.000256181353422 0.996092218246
0.000254191046878 0.996118835889
0.000252215248277 0.996145288418
0.000250253859712 0.996171576736
0.000248306783874 0.996197701742
0.000246373924053 0.996223664333
0.000244455184128 0.996249465398
0.000242550468571 0.996275105825
0.000240659682437 0.996300586497
0.000238782731368 0.996325908294
0.000236919521583 0.996351072089
0.00023506995988 0.996376078755
0.000233233953631 0.996400929158
0.000231411410777 0.996425624161
0.000229602239828 0.996450164624
0.000227806349859 0.996474551401
0.000226023650506 0.996498785344
0.000224254051964 0.996522867301
0.000222497464984 0.996546798114
0.000220753800867 0.996570578623
0.000219022971467 0.996594209664
0.000217304889182 0.996617692068
0.000215599466955 0.996641026664
0.000213906618268 0.996664214276
0.000212226257144 0.996687255723
0.000210558298136 0.996710151823
0.000208902656332 0.996732903387
0.000207259247348 0.996755511224
0.000205627987327 0.996777976141
0.000204008792932 0.996800298937
0.000202401581351 0.99682248041
0.000200806270285 0.996844521355
0.000199222777952 0.996866422561
0.00019765102308 0.996888184814
0.000196090924908 0.996909808897
0.000194542403178 0.996931295589
0.000193005378139 0.996952645666
0.000191479770538 0.996973859898
0.00018996550162 0.996994939053
0.000188462493125 0.997015883897
0.000186970667285 0.997036695189
0.000185489946824 0.997057373686
0.000184020254948 0.997077920142
0.000182561515352 0.997098335307
0.000181113652208 0.997118619927
0.000179676590171 0.997138774744
0.000178250254368 0.997158800498
0.000176834570402 0.997178697924
0.000175429464345 0.997198467754
0.000174034862738 0.997218110717
0.000172650692589 0.997237627537
0.000171276881365 0.997257018937
0.000169913356996 0.997276285634
0.00016856004787 0.997295428342
0.000167216882828 0.997314447773
0.000165883791166 0.997333344634
0.000164560702627 0.99735211963
0.000163247547405 0.997370773461
0.000161944256136 0.997389306825
0.0001606507599 0.997407720416
0.000159366990216 0.997426014924
0.000158092879041 0.997444191036
0.000156828358767 0.997462249437
0.000155573362218 0.997480190806
0.000154327822648 0.997498015822
0.00015309167374 0.997515725157
0.0001518648496 0.997533319483
0.000150647284757 0.997550799466
0.000149438914163 0.997568165771
0.000148239673186 0.997585419058
0.000147049497608 0.997602559985
0.000145868323627 0.997619589205
0.00014469608785 0.99763650737
0.000143532727294 0.997653315128
0.00014237817938 0.997670013123
0.000141232381935 0.997686601995
0.000140095273186 0.997703082384
0.00013896679176 0.997719454924
0.00013784687668 0.997735720247
0.000136735467365 0.997751878982
0.000135632503624 0.997767931753
0.00013453792566 0.997783879184
0.000133451674059 0.997799721893
0.000132373689797 0.997815460497
0.00013130391423 0.997831095608
0.000130242289097 0.997846627837
0.000129188756514 0.99786205779
0.000128143258978 0.997877386071
0.000127105739355 0.99789261328
0.000126076140888 0.997907740016
0.000125054407186 0.997922766873
0.000124040482231 0.997937694443
0.000123034310367 0.997952523315
0.000122035836302 0.997967254073
0.000121045005108 0.997981887301
0.000120061762215 0.997996423579
0.000119086053411 0.998010863482
0.000118117824838 0.998025207586
0.000117157022993 0.998039456461
0.000116203594724 0.998053610675
0.000115257487226 0.998067670792
0.000114318648045 0.998081637376
0.000113387025068 0.998095510985
0.000112462566529 0.998109292176
0.000111545220998 0.998122981502
0.00011063493739 0.998136579514
0.000109731664951 0.99815008676
0.000108835353267 0.998163503784
0.000107945952255 0.99817683113
0.000107063412161 0.998190069336
0.000106187683565 0.99820321894
0.000105318717369 0.998216280474
0.000104456464804 0.998229254469
0.000103600877422 0.998242141456
0.000102751907097 0.998254941957
0.000101909506024 0.998267656498
0.000101073626713 0.998280285596
0.000100244221992 0.998292829771
9.94212450016e-05 0.998305289536
9.86046491939e-05 0.998317665404
9.77943883318e-05 0.998329957883
9.69904164865e-05 0.998342167481
9.61926880352e-05 0.998354294701
9.54011576598e-05 0.998366340044
9.46157803451e-05 0.99837830401
9.38365113763e-05 0.998390187094
9.30633063381e-05 0.998401989789
9.22961211124e-05 0.998413712587
9.15349118766e-05 0.998425355976
9.07796351018e-05 0.99843692044
9.00302475513e-05 0.998448406464
8.92867062781e-05 0.998459814527
8.85489686241e-05 0.998471145108
8.78169922178e-05 0.998482398682
8.70907349727e-05 0.998493575722
8.63701550855e-05 0.998504676698
8.56552110343e-05 0.998515702078
8.49458615775e-05 0.998526652327
8.42420657512e-05 0.998537527908
8.35437828681e-05 0.998548329282
8.28509725157e-05 0.998559056906
8.21635945547e-05 0.998569711236
8.14816091171e-05 0.998580292724
8.08049766047e-05 0.998590801822
8.01336576876e-05 0.998601238977
7.94676133021e-05 0.998611604636
7.880680465e-05 0.99862189924
7.81511931955e-05 0.998632123232
7.75007406654e-05 0.99864227705
7.68554090458e-05 0.99865236113
7.62151605816e-05 0.998662375906
7.55799577747e-05 0.998672321808
7.49497633822e-05 0.998682199268
7.43245404147e-05 0.99869200871
7.37042521353e-05 0.998701750559
7.30888620575e-05 0.998711425239
7.24783339443e-05 0.998721033167
7.18726318057e-05 0.998730574763
7.12717198982e-05 0.998740050441
7.06755627224e-05 0.998749460614
7.00841250223e-05 0.998758805693
6.94973717831e-05 0.998768086086
6.89152682301e-05 0.9987773022
6.83377798272e-05 0.998786454438
6.77648722753e-05 0.998795543203
6.71965115108e-05 0.998804568894
6.66326637042e-05 0.998813531907
6.60732952588e-05 0.99882243264
6.5518372809e-05 0.998831271483
6.4967863219e-05 0.998840048829
6.44217335813e-05 0.998848765066
6.38799512154e-05 0.99885742058
6.33424836662e-05 0.998866015756
6.28092987028e-05 0.998874550975
6.2280364317e-05 0.998883026619
6.17556487217e-05 0.998891443064
6.12351203499e-05 0.998899800688
6.07187478532e-05 0.998908099863
6.02065001002e-05 0.998916340961
5.96983461755e-05 0.998924524352
5.91942553778e-05 0.998932650403
5.86941972194e-05 0.998940719481
5.81981414238e-05 0.998948731947
5.77060579257e-05 0.998956688165
5.7217916868e-05 0.998964588493
5.6733688602e-05 0.998972433288
5.62533436855e-05 0.998980222906
5.57768528812e-05 0.9989879577
5.53041871556e-05 0.998995638022
5.48353176781e-05 0.99900326422
5.43702158193e-05 0.999010836643
5.39088531498e-05 0.999018355636
5.3451201439e-05 0.999025821541
5.29972326537e-05 0.999033234702
5.25469189571e-05 0.999040595456
5.21002327072e-05 0.999047904143
5.16571464561e-05 0.999055161097
5.12176329481e-05 0.999062366653
5.0781665119e-05 0.999069521142
5.03492160944e-05 0.999076624895
4.99202591893e-05 0.999083678239
4.94947679058e-05 0.999090681501
4.90727159328e-05 0.999097635006
4.86540771445e-05 0.999104539075
4.82388255989e-05 0.99911139403
4.78269355372e-05 0.999118200189
4.74183813821e-05 0.99912495787
4.70131377371e-05 0.999131667388
4.66111793851e-05 0.999138329055
4.6212481287e-05 0.999144943185
4.58170185811e-05 0.999151510086
4.54247665814e-05 0.999158030066
4.50357007771e-05 0.999164503432
4.46497968306e-05 0.999170930489
4.42670305776e-05 0.999177311538
4.38873780245e-05 0.999183646881
4.35108153486e-05 0.999189936818
4.31373188964e-05 0.999196181644
4.27668651823e-05 0.999202381658
4.23994308881e-05 0.999208537151
4.20349928615e-05 0.999214648417
4.1673528115e-05 0.999220715747
4.13150138251e-05 0.999226739428
4.09594273311e-05 0.999232719749
4.06067461337e-05 0.999238656995
4.0256947895e-05 0.99924455145
3.99100104359e-05 0.999250403396
3.95659117365e-05 0.999256213114
3.92246299341e-05 0.999261980882
3.88861433227e-05 0.999267706978
3.85504303519e-05 0.999273391677
3.82174696255e-05 0.999279035254
3.78872399011e-05 0.999284637981
3.75597200886e-05 0.999290200128
3.72348892492e-05 0.999295721966
3.69127265951e-05 0.999301203761
3.65932114874e-05 0.99930664578
3.62763234363e-05 0.999312048287
3.5962042099e-05 0.999317411545
3.56503472796e-05 0.999322735815
3.53412189277e-05 0.999328021357
3.50346371376e-05 0.99933326843
3.47305821472e-05 0.99933847729
3.44290343373e-05 0.999343648193
3.41299742302e-05 0.999348781391
3.38333824895e-05 0.999353877138
3.35392399184e-05 0.999358935683
3.32475274593e-05 0.999363957277
3.29582261924e-05 0.999368942166
3.26713173355e-05 0.999373890597
3.23867822423e-05 0.999378802814
3.21046024019e-05 0.999383679062
3.18247594382e-05 0.999388519581
3.15472351082e-05 0.999393324612
3.12720113019e-05 0.999398094394
3.09990700411e-05 0.999402829164
3.07283934782e-05 0.999407529158
3.04599638959e-05 0.999412194612
3.01937637062e-05 0.999416825758
2.99297754491e-05 0.999421422827
2.96679817922e-05 0.999425986051
2.94083655298e-05 0.999430515658
2.91509095818e-05 0.999435011877
2.88955969929e-05 0.999439474932
2.86424109325e-05 0.999443905049
2.83913346925e-05 0.999448302452
2.81423516875e-05 0.999452667362
2.78954454538e-05 0.999457000001
2.76505996484e-05 0.999461300587
2.74077980482e-05 0.99946556934
2.71670245495e-05 0.999469806475
2.69282631667e-05 0.999474012208
2.66914980318e-05 0.999478186754
2.64567133936e-05 0.999482330324
2.62238936171e-05 0.999486443132
2.5993023182e-05 0.999490525386
2.57640866828e-05 0.999494577295
2.55370688275e-05 0.999498599068
2.53119544371e-05 0.999502590911
2.50887284446e-05 0.999506553029
2.48673758945e-05 0.999510485626
2.46478819415e-05 0.999514388904
2.44302318505e-05 0.999518263064
2.42144109954e-05 0.999522108307
2.40004048586e-05 0.999525924832
2.37881990298e-05 0.999529712836
2.35777792058e-05 0.999533472516
2.33691311894e-05 0.999537204066
2.31622408891e-05 0.999540907682
2.29570943178e-05 0.999544583555
2.27536775925e-05 0.999548231877
2.25519769338e-05 0.999551852839
2.23519786643e-05 0.999555446629
2.21536692088e-05 0.999559013437
2.19570350933e-05 0.999562553448
2.17620629445e-05 0.999566066849
2.15687394881e-05 0.999569553823
2.13770515499e-05 0.999573014555
2.11869860534e-05 0.999576449226
2.09985300202e-05 0.999579858019
2.0811670569e-05 0.999583241111
2.06263949146e-05 0.999586598683
2.04426903679e-05 0.999589930913
2.02605443348e-05 0.999593237976
2.00799443155e-05 0.999596520048
1.9900877904e-05 0.999599777304
1.97233327875e-05 0.999603009917
1.95472967458e-05 0.99960621806
1.93727576503e-05 0.999609401902
1.91997034639e-05 0.999612561615
1.90281222396e-05 0.999615697367
1.8858002121e-05 0.999618809326
1.86893313404e-05 0.999621897659
1.85220982193e-05 0.999624962532
1.83562911671e-05 0.999628004109
1.81918986805e-05 0.999631022554
1.80289093433e-05 0.99963401803
1.78673118256e-05 0.999636990699
1.7707094883e-05 0.99963994072
1.75482473563e-05 0.999642868254
1.73907581706e-05 0.999645773459
1.72346163351e-05 0.999648656493
1.7079810942e-05 0.999651517511
1.69263311666e-05 0.99965435667
1.67741662659e-05 0.999657174125
1.66233055789e-05 0.999659970028
1.64737385254e-05 0.999662744532
1.63254546055e-05 0.999665497789
1.61784433993e-05 0.999668229949
1.60326945662e-05 0.999670941162
1.58881978441e-05 0.999673631578
1.57449430495e-05 0.999676301342
1.56029200762e-05 0.999678950603
1.54621188952e-05 0.999681579506
1.53225295542e-05 0.999684188196
1.51841421766e-05 0.999686776816
1.50469469614e-05 0.999689345511
1.49109341827e-05 0.999691894421
1.47760941888e-05 0.999694423689
1.46424174019e-05 0.999696933454
1.45098943176e-05 0.999699423856
1.43785155043e-05 0.999701895033
1.4248271603e-05 0.999704347123
1.41191533261e-05 0.999706780262
1.39911514574e-05 0.999709194587
1.38642568517e-05 0.999711590232
1.37384604338e-05 0.999713967331
1.36137531986e-05 0.999716326017
1.34901262102e-05 0.999718666423
1.33675706013e-05 0.999720988679
1.3246077573e-05 0.999723292918
1.31256383945e-05 0.999725579267
1.3006244402e-05 0.999727847856
1.28878869986e-05 0.999730098814
1.27705576539e-05 0.999732332267
1.26542479035e-05 0.999734548341
1.25389493482e-05 0.999736747162
1.24246536538e-05 0.999738928856
1.23113525508e-05 0.999741093544
1.21990378334e-05 0.999743241352
1.208770136e-05 0.9997453724
1.19773350513e-05 0.99974748681
1.18679308913e-05 0.999749584704
1.17594809259e-05 0.9997516662
1.16519772629e-05 0.999753731418
1.15454120715e-05 0.999755780476
1.14397775816e-05 0.999757813492
1.13350660836e-05 0.999759830581
1.12312699281e-05 0.999761831861
1.11283815251e-05 0.999763817447
1.10263933436e-05 0.999765787452
1.09252979117e-05 0.99976774199
1.08250878154e-05 0.999769681174
1.07257556989e-05 0.999771605117
1.06272942638e-05 0.999773513929
1.05296962685e-05 0.999775407722
1.04329545283e-05 0.999777286605
1.03370619144e-05 0.999779150687
1.02420113544e-05 0.999781000077
1.01477958304e-05 0.999782834882
1.00544083804e-05 0.99978465521
9.96184209656e-06 0.999786461167
9.8700901251e-06 0.999788252858
9.77914566636e-06 0.999790030388
9.68900197384e-06 0.999791793861
9.59965235448e-06 0.999793543382
9.51109016722e-06 0.999795279051
9.42330882381e-06 0.999797000972
9.33630178757e-06 0.999798709247
9.25006257346e-06 0.999800403974
9.16458474742e-06 0.999802085256
9.07986192633e-06 0.99980375319
8.99588777714e-06 0.999805407876
8.9126560171e-06 0.999807049412
8.83016041286e-06 0.999808677895
8.7483947806e-06 0.999810293421
8.6673529851e-06 0.999811896087
8.58702893991e-06 0.999813485988
8.50741660674e-06 0.999815063219
8.42850999494e-06 0.999816627873
8.35030316149e-06 0.999818180045
8.27279021065e-06 0.999819719827
8.19596529322e-06 0.999821247311
8.11982260662e-06 0.99982276259
8.04435639412e-06 0.999824265752
7.96956094506e-06 0.99982575689
7.89543059398e-06 0.999827236093
7.8219597206e-06 0.999828703449
7.74914274926e-06 0.999830159048
7.67697414883e-06 0.999831602977
7.60544843226e-06 0.999833035323
7.53456015634e-06 0.999834456173
7.46430392107e-06 0.999835865614
7.39467436972e-06 0.999837263729
7.32566618822e-06 0.999838650606
7.25727410533e-06 0.999840026327
7.18949289147e-06 0.999841390977
7.12231735922e-06 0.999842744638
7.05574236259e-06 0.999844087394
6.98976279689e-06 0.999845419325
6.92437359817e-06 0.999846740515
6.85956974333e-06 0.999848051043
6.79534624948e-06 0.99984935099
6.73169817356e-06 0.999850640435
6.66862061238e-06 0.999851919459
6.60610870218e-06 0.999853188139
6.54415761825e-06 0.999854446553
6.48276257476e-06 0.99985569478
6.42191882416e-06 0.999856932896
6.36162165768e-06 0.999858160978
6.30186640382e-06 0.999859379101
6.2426484293e-06 0.999860587342
6.1839631379e-06 0.999861785774
6.1258059707e-06 0.999862974474
6.06817240534e-06 0.999864153513
6.01105795639e-06 0.999865322966
5.95445817431e-06 0.999866482906
5.89836864573e-06 0.999867633405
5.84278499316e-06 0.999868774534
5.78770287418e-06 0.999869906366
5.7331179818e-06 0.99987102897
5.67902604409e-06 0.999872142418
5.62542282345e-06 0.999873246779
5.57230411691e-06 0.999874342122
5.51966575546e-06 0.999875428516
5.46750360408e-06 0.99987650603
5.41581356139e-06 0.999877574732
5.36459155931e-06 0.999878634689
5.31383356284e-06 0.999879685967
5.26353556984e-06 0.999880728634
5.21369361106e-06 0.999881762756
5.16430374897e-06 0.999882788397
5.11536207892e-06 0.999883805624
5.06686472745e-06 0.9998848145
5.01880785331e-06 0.99988581509
4.97118764609e-06 0.999886807458
4.92400032681e-06 0.999887791666
4.87724214759e-06 0.999888767778
4.83090939074e-06 0.999889735856
4.78499836942e-06 0.999890695961
4.73950542679e-06 0.999891648156
4.69442693596e-06 0.999892592502
4.64975929992e-06 0.999893529058
4.60549895098e-06 0.999894457886
4.56164235108e-06 0.999895379044
4.51818599079e-06 0.999896292593
4.47512638968e-06 0.999897198591
4.43246009618e-06 0.999898097097
4.39018368692e-06 0.999898988168
4.3482937665e-06 0.999899871862
4.30678696772e-06 0.999900748237
4.26565995126e-06 0.999901617349
4.22490940499e-06 0.999902479256
4.18453204443e-06 0.999903334011
4.14452461184e-06 0.999904181673
4.1048838767e-06 0.999905022295
4.06560663513e-06 0.999905855932
4.02668970967e-06 0.999906682639
3.98812994895e-06 0.99990750247
3.94992422803e-06 0.999908315478
3.91206944772e-06 0.999909121717
3.87456253437e-06 0.99990992124
3.83740043997e-06 0.999910714098
3.8005801416e-06 0.999911500345
3.76409864167e-06 0.999912280032
3.72795296733e-06 0.99991305321
3.69214017026e-06 0.99991381993
3.65665732704e-06 0.999914580244
3.62150153821e-06 0.9999153342
3.58666992861e-06 0.999916081849
3.55215964698e-06 0.999916823241
3.51796786557e-06 0.999917558424
3.48409178064e-06 0.999918287448
3.4505286115e-06 0.99991901036
3.41727560083e-06 0.99991972721
3.38433001401e-06 0.999920438044
3.35168913967e-06 0.99992114291
3.31935028874e-06 0.999921841856
3.28731079491e-06 0.999922534928
3.25556801395e-06 0.999923222171
3.22411932385e-06 0.999923903633
3.1929621247e-06 0.999924579359
3.16209383799e-06 0.999925249394
3.13151190712e-06 0.999925913784
3.10121379676e-06 0.999926572573
3.07119699317e-06 0.999927225805
3.04145900332e-06 0.999927873524
3.0119973552e-06 0.999928515774
2.98280959776e-06 0.9999291526
2.95389330041e-06 0.999929784042
2.92524605294e-06 0.999930410145
2.89686546573e-06 0.999931030951
2.86874916888e-06 0.999931646502
2.84089481262e-06 0.99993225684
2.81330006713e-06 0.999932862005
2.78596262204e-06 0.999933462041
2.75888018653e-06 0.999934056986
2.73205048917e-06 0.999934646883
2.70547127779e-06 0.999935231771
2.67914031893e-06 0.99993581169
2.65305539826e-06 0.99993638668
2.62721432032e-06 0.999936956781
2.60161490784e-06 0.999937522031
2.57625500233e-06 0.999938082469
2.5511324635e-06 0.999938638134
2.52624516905e-06 0.999939189065
2.50159101489e-06 0.999939735298
2.47716791468e-06 0.999940276872
2.45297379975e-06 0.999940813824
2.42900661918e-06 0.999941346192
2.40526433914e-06 0.999941874011
2.38174494349e-06 0.99994239732
2.35844643304e-06 0.999942916153
2.33536682559e-06 0.999943430547
2.31250415583e-06 0.999943940538
2.28985647532e-06 0.999944446162
2.26742185216e-06 0.999944947452
2.24519837089e-06 0.999945444446
2.22318413234e-06 0.999945937176
2.20137725371e-06 0.999946425678
2.17977586825e-06 0.999946909985
2.15837812501e-06 0.999947390132
2.13718218911e-06 0.999947866153
2.11618624113e-06 0.99994833808
2.0953884774e-06 0.999948805948
2.07478710956e-06 0.999949269788
2.05438036471e-06 0.999949729633
2.03416648514e-06 0.999950185516
2.01414372802e-06 0.99995063747
1.99431036574e-06 0.999951085525
1.97466468532e-06 0.999951529714
1.95520498869e-06 0.999951970068
1.93592959208e-06 0.999952406619
1.91683682649e-06 0.999952839396
1.89792503724e-06 0.999953268432
1.87919258365e-06 0.999953693756
1.86063783947e-06 0.999954115399
1.84225919231e-06 0.999954533391
1.82405504379e-06 0.999954947762
1.80602380906e-06 0.999955358541
1.78816391716e-06 0.999955765757
1.77047381078e-06 0.99995616944
1.75295194582e-06 0.999956569619
1.73559679173e-06 0.999956966322
1.71840683105e-06 0.999957359578
1.70138055955e-06 0.999957749415
1.68451648597e-06 0.999958135862
1.66781313182e-06 0.999958518945
1.65126903184e-06 0.999958898692
1.63488273297e-06 0.999959275132
1.61865279513e-06 0.999959648291
1.60257779058e-06 0.999960018196
1.5866563039e-06 0.999960384874
1.5708869322e-06 0.999960748352
1.55526828449e-06 0.999961108655
1.53979898221e-06 0.99996146581
1.52447765833e-06 0.999961819844
1.50930295828e-06 0.999962170781
1.49427353879e-06 0.999962518647
1.47938806871e-06 0.999962863469
1.4646452281e-06 0.99996320527
1.45004370877e-06 0.999963544076
1.43558221388e-06 0.999963879911
1.42125945801e-06 0.999964212801
1.40707416685e-06 0.99996454277
1.39302507718e-06 0.999964869841
1.37911093701e-06 0.999965194039
1.3653305051e-06 0.999965515388
1.35168255133e-06 0.999965833912
1.3381658559e-06 0.999966149633
1.32477921033e-06 0.999966462575
1.31152141614e-06 0.999966772762
1.29839128571e-06 0.999967080216
1.28538764177e-06 0.99996738496
1.27250931725e-06 0.999967687016
1.25975515541e-06 0.999967986407
1.24712400984e-06 0.999968283156
1.23461474399e-06 0.999968577283
1.22222623145e-06 0.999968868812
1.20995735542e-06 0.999969157764
1.19780700947e-06 0.99996944416
1.18577409636e-06 0.999969728021
1.17385752896e-06 0.99997000937
1.16205622935e-06 0.999970288226
1.15036912951e-06 0.999970564612
1.13879517039e-06 0.999970838547
1.12733330282e-06 0.999971110052
1.11598248642e-06 0.999971379147
1.10474169024e-06 0.999971645853
1.09360989253e-06 0.99997191019
1.08258608034e-06 0.999972172178
1.07166924979e-06 0.999972431836
1.0608584059e-06 0.999972689184
1.05015256269e-06 0.999972944241
1.0395507426e-06 0.999973197028
1.02905197696e-06 0.999973447562
1.01865530555e-06 0.999973695863
1.00835977668e-06 0.99997394195
9.9816444743e-07 0.999974185841
9.88068382779e-07 0.999974427555
9.78070656243e-07 0.999974667111
9.6817034978e-07 0.999974904526
9.58366553228e-07 0.999975139819
9.4865836453e-07 0.999975373008
9.39044889847e-07 0.99997560411
9.29525243221e-07 0.999975833143
9.20098546575e-07 0.999976060125
9.10763929718e-07 0.999976285073
9.01520530117e-07 0.999976508005
8.92367493011e-07 0.999976728936
8.83303971411e-07 0.999976947886
8.74329125655e-07 0.99997716487
8.65442123743e-07 0.999977379904
8.56642141001e-07 0.999977593007
8.47928360304e-07 0.999977804193
8.39299971744e-07 0.99997801348
8.30756172743e-07 0.999978220883
8.22296167713e-07 0.999978426419
8.13919168396e-07 0.999978630104
8.05624393529e-07 0.999978831953
7.97411069065e-07 0.999979031982
7.89278427504e-07 0.999979230206
7.81225708679e-07 0.999979426642
7.73252158859e-07 0.999979621304
7.65357031418e-07 0.999979814208
7.57539586282e-07 0.999980005368
7.49799090038e-07 0.999980194799
7.42134815934e-07 0.999980382517
7.34546043768e-07 0.999980568536
7.27032059888e-07 0.99998075287
7.19592156861e-07 0.999980935535
7.12225633914e-07 0.999981116544
7.0493179638e-07 0.999981295912
6.97709955921e-07 0.999981473652
6.90559430638e-07 0.999981649779
6.83479544517e-07 0.999981824307
6.76469627758e-07 0.999981997249
6.69529016561e-07 0.999982168619
6.62657053341e-07 0.999982338431
6.55853086173e-07 0.999982506698
6.49116469353e-07 0.999982673433
6.42446562837e-07 0.99998283865
6.35842732355e-07 0.999983002362
6.29304349631e-07 0.999983164582
6.22830791719e-07 0.999983325322
6.16421441779e-07 0.999983484596
6.1007568819e-07 0.999983642415
6.03792924991e-07 0.999983798794
5.97572552108e-07 0.999983953744
5.91413974238e-07 0.999984107277
5.85316602186e-07 0.999984259407
5.79279851531e-07 0.999984410145
5.73303143736e-07 0.999984559502
5.67385905148e-07 0.999984707492
5.61527567444e-07 0.999984854127
5.5572756763e-07 0.999984999417
5.49985347598e-07 0.999985143374
5.44300354566e-07 0.999985286011
5.38672040751e-07 0.999985427339
5.33099863254e-07 0.999985567368
5.27583284282e-07 0.999985706111
5.2212177104e-07 0.999985843579
5.16714795284e-07 0.999985979783
5.11361833988e-07 0.999986114733
5.06062368677e-07 0.999986248441
5.00815885762e-07 0.999986380918
4.95621876317e-07 0.999986512175
4.90479836079e-07 0.999986642221
4.85389265448e-07 0.999986771068
4.80349669374e-07 0.999986898726
4.75360557362e-07 0.999987025206
4.70421443466e-07 0.999987150518
4.65531846072e-07 0.999987274673
4.6069128834e-07 0.999987397679
4.55899297425e-07 0.999987519548
4.51155405146e-07 0.99998764029
4.4645914743e-07 0.999987759914
4.41810064533e-07 0.99998787843
4.37207701043e-07 0.999987995848
4.32651605653e-07 0.999988112178
4.28141331388e-07 0.999988227429
4.23676435157e-07 0.999988341611
4.1925647809e-07 0.999988454733
4.14881025312e-07 0.999988566805
4.10549646279e-07 0.999988677835
4.06261913888e-07 0.999988787833
4.02017405587e-07 0.999988896809
3.97815702158e-07 0.999989004771
3.9365638882e-07 0.999989111727
3.89539054235e-07 0.999989217688
3.85463291064e-07 0.999989322662
3.81428695739e-07 0.999989426657
3.77434868359e-07 0.999989529683
3.73481412796e-07 0.999989631748
3.69567936587e-07 0.99998973286
3.65694051041e-07 0.999989833028
3.61859370801e-07 0.99998993226
3.58063514505e-07 0.999990030564
3.543061039e-07 0.99999012795
3.50586764619e-07 0.999990224424
3.46905125626e-07 0.999990319996
3.43260819213e-07 0.999990414673
3.39653481451e-07 0.999990508463
3.36082751407e-07 0.999990601374
3.3254827192e-07 0.999990693414
3.29049688719e-07 0.999990784591
3.25586651417e-07 0.999990874912
3.22158812294e-07 0.999990964385
3.18765827179e-07 0.999991053017
3.15407355345e-07 0.999991140817
3.1208305884e-07 0.999991227791
3.08792603043e-07 0.999991313947
3.05535656553e-07 0.999991399293
3.02311891076e-07 0.999991483835
2.99120981206e-07 0.999991567581
2.95962604868e-07 0.999991650537
2.9283644265e-07 0.999991732712
2.89742178583e-07 0.999991814112
2.86679499362e-07 0.999991894743
2.83648094679e-07 0.999991974614
2.80647657114e-07 0.99999205373
2.77677882354e-07 0.999992132098
2.74738468753e-07 0.999992209726
2.71829117438e-07 0.99999228662
2.68949532645e-07 0.999992362786
2.66099421053e-07 0.999992438232
2.63278492452e-07 0.999992512963
2.60486459069e-07 0.999992586985
2.57723036023e-07 0.999992660307
2.54987941095e-07 0.999992732933
2.5228089473e-07 0.99999280487
2.49601619928e-07 0.999992876124
2.46949842464e-07 0.999992946702
2.44325290666e-07 0.999993016609
2.41727695194e-07 0.999993085852
2.39156789705e-07 0.999993154437
2.36612310078e-07 0.999993222369
2.34093994744e-07 0.999993289655
2.31601584577e-07 0.9999933563
2.29134823004e-07 0.99999342231
2.26693455896e-07 0.999993487691
2.24277231453e-07 0.999993552449
2.21885900209e-07 0.99999361659
2.19519215361e-07 0.999993680118
2.17176932105e-07 0.99999374304
2.1485880819e-07 0.999993805361
2.12564603586e-07 0.999993867086
2.10294080594e-07 0.999993928222
2.08047003736e-07 0.999993988772
2.05823139754e-07 0.999994048744
2.03622257722e-07 0.999994108141
2.01444128711e-07 0.99999416697
1.99288526348e-07 0.999994225235
1.97155226034e-07 0.999994282942
1.95044005502e-07 0.999994340095
1.92954644596e-07 0.9999943967
1.90886925266e-07 0.999994452761
1.88840631465e-07 0.999994508285
1.86815549363e-07 0.999994563275
1.84811467019e-07 0.999994617737
1.82828174711e-07 0.999994671675
1.80865464605e-07 0.999994725094
1.78923130756e-07 0.999994777999
1.77000969326e-07 0.999994830395
1.75098778588e-07 0.999994882286
1.73216358368e-07 0.999994933677
1.71353510825e-07 0.999994984573
1.69510039671e-07 0.999995034978
1.6768575084e-07 0.999995084897
1.65880451708e-07 0.999995134334
1.64093951871e-07 0.999995183293
1.62326062703e-07 0.999995231779
1.60576597241e-07 0.999995279797
1.58845370413e-07 0.999995327351
1.57132198919e-07 0.999995374444
1.5543690135e-07 0.999995421082
1.5375929785e-07 0.999995467268
1.52099210338e-07 0.999995513006
1.50456462511e-07 0.999995558302
1.48830879843e-07 0.999995603158
1.47222289359e-07 0.999995647579
1.45630519865e-07 0.99999569157
1.44055401607e-07 0.999995735133
1.42496766831e-07 0.999995778273
1.40954449002e-07 0.999995820994
1.39428283585e-07 0.999995863299
1.37918107379e-07 0.999995905194
1.36423758845e-07 0.99999594668
1.34945078001e-07 0.999995987763
1.33481906528e-07 0.999996028446
1.32034087441e-07 0.999996068732
1.30601465309e-07 0.999996108626
1.29183886477e-07 0.999996148131
1.27781198511e-07 0.99999618725
1.26393250643e-07 0.999996225988
1.25019893216e-07 0.999996264348
1.23660978568e-07 0.999996302332
1.2231635993e-07 0.999996339946
1.20985892416e-07 0.999996377192
1.19669432364e-07 0.999996414074
1.18366837443e-07 0.999996450595
1.17077966766e-07 0.999996486758
1.15802680778e-07 0.999996522567
1.14540841478e-07 0.999996558026
1.13292312087e-07 0.999996593137
1.12056957047e-07 0.999996627903
1.10834642242e-07 0.999996662329
1.09625235001e-07 0.999996696416
1.0842860354e-07 0.999996730169
1.07244617964e-07 0.999996763591
1.06073149042e-07 0.999996796684
1.0491406921e-07 0.999996829452
1.03767252013e-07 0.999996861897
1.0263257233e-07 0.999996894023
1.01509906036e-07 0.999996925833
1.00399130565e-07 0.99999695733
9.93001241234e-08 0.999996988517
9.82127666971e-08 0.999997019396
9.71369388258e-08 0.99999704997
9.6072522604e-08 0.999997080243
9.50194013472e-08 0.999997110217
9.3977459148e-08 0.999997139895
9.29465815425e-08 0.99999716928
9.19266550659e-08 0.999997198375
9.09175675856e-08 0.999997227182
8.99192077464e-08 0.999997255704
8.8931465525e-08 0.999997283944
8.79542318977e-08 0.999997311905
8.69873988396e-08 0.999997339588
8.60308596584e-08 0.999997366997
8.50845084388e-08 0.999997394135
8.41482404867e-08 0.999997421003
8.32219518854e-08 0.999997447605
8.23055401611e-08 0.999997473943
8.13989035064e-08 0.99999750002
8.05019412242e-08 0.999997525837
7.96145536164e-08 0.999997551398
7.87366420951e-08 0.999997576705
7.78681089608e-08 0.99999760176
7.7008857291e-08 0.999997626566
7.61587914955e-08 0.999997651125
7.53178165391e-08 0.999997675439
7.44858387192e-08 0.999997699511
7.36627649989e-08 0.999997723344
7.28485032297e-08 0.999997746938
7.20429624845e-08 0.999997770297
7.12460523911e-08 0.999997793423
7.04576836874e-08 0.999997816319
6.96777679998e-08 0.999997838985
6.89062177317e-08 0.999997861425
6.81429461746e-08 0.999997883641
6.73878676194e-08 0.999997905635
6.66408970229e-08 0.999997927408
6.59019502303e-08 0.999997948964
6.51709440858e-08 0.999997970304
6.44477960998e-08 0.99999799143
6.37324246711e-08 0.999998012344
6.30247490863e-08 0.999998033049
6.23246891873e-08 0.999998053546
6.16321658153e-08 0.999998073837
6.09471006996e-08 0.999998093925
6.02694162355e-08 0.999998113811
5.95990353736e-08 0.999998133497
5.89358822856e-08 0.999998152985
5.82798815874e-08 0.999998172277
5.7630958672e-08 0.999998191375
5.69890398205e-08 0.999998210281
5.63540519805e-08 0.999998228997
5.57259227651e-08 0.999998247524
5.51045805652e-08 0.999998265865
5.44899545485e-08 0.99999828402
5.38819746598e-08 0.999998301993
5.32805711773e-08 0.999998319784
5.26856756e-08 0.999998337395
5.20972197604e-08 0.999998354829
5.15151362679e-08 0.999998372087
5.09393583981e-08 0.99999838917
5.03698200927e-08 0.99999840608
4.98064560706e-08 0.99999842282
4.92492017168e-08 0.99999843939
4.86979927494e-08 0.999998455792
4.81527658858e-08 0.999998472029
4.76134582872e-08 0.9999984881
4.70800080032e-08 0.999998504009
4.65523533055e-08 0.999998519757
4.60304335759e-08 0.999998535344
4.55141883071e-08 0.999998550774
4.50035578803e-08 0.999998566047
4.44984833425e-08 0.999998581165
4.39989062961e-08 0.999998596129
4.35047686764e-08 0.999998610941
4.30160133069e-08 0.999998625602
4.25325835662e-08 0.999998640115
4.20544232771e-08 0.999998654479
4.15814769283e-08 0.999998668698
4.11136894529e-08 0.999998682771
4.06510065609e-08 0.999998696701
4.01933742955e-08 0.999998710489
3.97407392549e-08 0.999998724137
3.92930488147e-08 0.999998737645
3.88502506832e-08 0.999998751015
3.84122931241e-08 0.999998764249
3.79791249561e-08 0.999998777347
3.7550695553e-08 0.999998790312
3.71269546218e-08 0.999998803144
3.67078527574e-08 0.999998815845
3.62933406661e-08 0.999998828416
3.58833698311e-08 0.999998840858
3.54778920686e-08 0.999998853173
3.50768597501e-08 0.999998865362
3.46802256912e-08 0.999998877425
3.42879432624e-08 0.999998889365
3.38999662786e-08 0.999998901183
3.35162489984e-08 0.999998912879
3.31367461248e-08 0.999998924455
3.27614129159e-08 0.999998935913
3.23902051846e-08 0.999998947252
3.20230787443e-08 0.999998958475
3.16599904071e-08 0.999998969583
3.13008972075e-08 0.999998980576
3.09457565129e-08 0.999998991456
3.05945262458e-08 0.999999002224
3.02471646618e-08 0.999999012881
2.99036306828e-08 0.999999023429
2.95638833414e-08 0.999999033868
2.92278823366e-08 0.999999044199
2.88955877004e-08 0.999999054423
2.85669597977e-08 0.999999064542
2.82419594377e-08 0.999999074556
2.79205479847e-08 0.999999084467
2.7602687025e-08 0.999999094276
2.72883385888e-08 0.999999103983
2.69774650397e-08 0.99999911359
2.66700292961e-08 0.999999123097
2.63659944988e-08 0.999999132506
2.60653242323e-08 0.999999141818
2.57679824145e-08 0.999999151033
2.54739335181e-08 0.999999160152
2.51831421272e-08 0.999999169177
2.48955733806e-08 0.999999178109
2.46111925284e-08 0.999999186947
2.43299654867e-08 0.999999195694
2.40518585048e-08 0.999999204351
2.37768378319e-08 0.999999212917
2.35048703834e-08 0.999999221394
2.32359234076e-08 0.999999229783
2.2969964486e-08 0.999999238085
2.27069612002e-08 0.9999992463
2.24468820198e-08 0.99999925443
2.21896953034e-08 0.999999262475
2.19353700759e-08 0.999999270437
2.16838752509e-08 0.999999278315
2.14351805194e-08 0.999999286111
2.11892555724e-08 0.999999293826
2.09460706557e-08 0.999999301461
2.07055961265e-08 0.999999309016
2.0467802675e-08 0.999999316491
2.02326615462e-08 0.999999323889
2.00001438744e-08 0.99999933121
1.97702213489e-08 0.999999338453
1.95428659922e-08 0.999999345622
1.93180500485e-08 0.999999352715
1.90957458734e-08 0.999999359733
1.88759264885e-08 0.999999366679
1.86585649153e-08 0.999999373551
1.84436345085e-08 0.999999380352
1.82311089558e-08 0.999999387081
1.8020962167e-08 0.99999939374
1.78131683848e-08 0.999999400328
1.76077019631e-08 0.999999406848
1.7404537811e-08 0.999999413299
1.72036509483e-08 0.999999419682
1.7005016395e-08 0.999999425999
1.68086099483e-08 0.999999432249
1.66144072944e-08 0.999999438433
1.64223844523e-08 0.999999444552
1.62325177744e-08 0.999999450606
1.60447837239e-08 0.999999456597
1.58591590971e-08 0.999999462525
1.56756210234e-08 0.99999946839
1.54941466324e-08 0.999999474193
1.53147136084e-08 0.999999479935
1.5137299525e-08 0.999999485617
1.49618823997e-08 0.999999491239
1.47884405832e-08 0.999999496801
1.46169524262e-08 0.999999502304
1.44473966124e-08 0.999999507749
1.42797519365e-08 0.999999513137
1.41139977483e-08 0.999999518468
1.39501130647e-08 0.999999523742
1.37880777906e-08 0.999999528961
1.36278714979e-08 0.999999534124
1.34694742027e-08 0.999999539232
1.33128661428e-08 0.999999544287
1.31580276674e-08 0.999999549287
1.30049394587e-08 0.999999554235
1.28535823096e-08 0.99999955913
1.27039372355e-08 0.999999563973
1.25559853625e-08 0.999999568765
1.2409708372e-08 0.999999573506
1.22650877232e-08 0.999999578197
1.21221050975e-08 0.999999582837
1.19807428423e-08 0.999999587428
1.18409828609e-08 0.999999591971
1.17028076119e-08 0.999999596465
1.15661997757e-08 0.999999600911
1.14311420329e-08 0.99999960531
1.12976173972e-08 0.999999609662
1.11656088819e-08 0.999999613967
1.10350998339e-08 0.999999618227
1.09060737108e-08 0.999999622441
1.07785143033e-08 0.99999962661
1.06524052912e-08 0.999999630735
1.05277307982e-08 0.999999634815
1.04044749483e-08 0.999999638852
1.02826220871e-08 0.999999642846
1.01621566717e-08 0.999999646797
1.00430634919e-08 0.999999650706
9.92532722677e-09 0.999999654573
9.8089331102e-09 0.999999658399
9.69386604321e-09 0.999999662183
9.58011159291e-09 0.999999665927
9.46765510434e-09 0.999999669631
9.35648225564e-09 0.999999673295
9.24657872492e-09 0.99999967692
9.1379306344e-09 0.999999680506
9.03052388423e-09 0.999999684053
8.92434492972e-09 0.999999687563
8.81938000408e-09 0.999999691034
8.71561556259e-09 0.999999694469
8.61303850463e-09 0.999999697866
8.51163550752e-09 0.999999701227
8.41139358165e-09 0.999999704551
8.31229984843e-09 0.99999970784
8.21434142928e-09 0.999999711094
8.11750588969e-09 0.999999714312
8.02178057313e-09 0.999999717496
7.92715326714e-09 0.999999720645
7.83361164824e-09 0.99999972376
7.74114361501e-09 0.999999726842
7.64973728806e-09 0.99999972989
7.55938089902e-09 0.999999732906
7.47006256852e-09 0.999999735889
7.38177075021e-09 0.99999973884
7.29449423087e-09 0.999999741758
7.20822135314e-09 0.999999744646
7.12294112581e-09 0.999999747502
7.03864244667e-09 0.999999750327
6.95531421346e-09 0.999999753121
6.87294576807e-09 0.999999755885
6.79152634131e-09 0.99999975862
6.71104516403e-09 0.999999761324
6.63149191116e-09 0.999999763999
6.55285614659e-09 0.999999766646
6.47512765628e-09 0.999999769263
6.39829611515e-09 0.999999771852
6.32235164222e-09 0.999999774413
6.24728424548e-09 0.999999776946
6.17308404394e-09 0.999999779452
6.09974137866e-09 0.99999978193
6.02724659071e-09 0.999999784382
5.95559024319e-09 0.999999786806
5.88476278818e-09 0.999999789204
5.8147548998e-09 0.999999791577
5.74555758526e-09 0.999999793923
5.67716151867e-09 0.999999796244
5.60955781825e-09 0.999999798539
5.54273760223e-09 0.999999800809
5.47669187778e-09 0.999999803055
5.4114120962e-09 0.999999805276
5.34688959775e-09 0.999999807473
5.28311572268e-09 0.999999809646
5.22008225534e-09 0.999999811795
5.15778064702e-09 0.99999981392
5.0962027931e-09 0.999999816023
5.03534047791e-09 0.999999818102
4.97518548581e-09 0.999999820158
4.91573015626e-09 0.999999822192
4.85696627361e-09 0.999999824204
4.79888617733e-09 0.999999826194
4.74148220686e-09 0.999999828162
4.68474647963e-09 0.999999830108
4.62867166817e-09 0.999999832033
4.57325022296e-09 0.999999833937
4.51847481653e-09 0.99999983582
4.46433789936e-09 0.999999837682
4.41083247704e-09 0.999999839524
4.35795144416e-09 0.999999841345
4.30568747323e-09 0.999999843147
4.25403368087e-09 0.999999844928
4.20298318371e-09 0.99999984669
4.15252920938e-09 0.999999848433
4.10266487449e-09 0.999999850156
4.0533834067e-09 0.999999851861
4.0046783667e-09 0.999999853546
3.95654309315e-09 0.999999855214
3.90897114677e-09 0.999999856862
3.86195619928e-09 0.999999858493
3.81549181139e-09 0.999999860105
3.76957165482e-09 0.9999998617
3.72418973438e-09 0.999999863277
3.67933972178e-09 0.999999864837
3.63501573286e-09 0.999999866379
3.59121166138e-09 0.999999867904
3.54792162316e-09 0.999999869413
3.50513973402e-09 0.999999870905
3.46286022079e-09 0.99999987238
3.42107731033e-09 0.999999873839
3.37978534048e-09 0.999999875281
3.33897887117e-09 0.999999876708
3.29865212922e-09 0.999999878119
3.25879967455e-09 0.999999879514
3.21941617809e-09 0.999999880894
3.18049619974e-09 0.999999882259
3.14203452145e-09 0.999999883608
3.10402581416e-09 0.999999884942
3.06646497084e-09 0.999999886262
3.02934677343e-09 0.999999887567
2.99266622594e-09 0.999999888857
2.95641833237e-09 0.999999890133
2.92059798568e-09 0.999999891395
2.88520041192e-09 0.999999892642
2.8502207261e-09 0.999999893876
2.81565415428e-09 0.999999895096
2.7814960335e-09 0.999999896302
2.74774147879e-09 0.999999897495
2.71438593824e-09 0.999999898675
2.68142485993e-09 0.999999899842
2.64885369194e-09 0.999999900995
2.61666799339e-09 0.999999902136
2.58486332338e-09 0.999999903264
2.55343513e-09 0.999999904379
2.52237930543e-09 0.999999905482
2.49169151978e-09 0.999999906572
2.46136733217e-09 0.99999990765
2.43140285683e-09 0.999999908717
2.40179365285e-09 0.999999909771
2.37253583446e-09 0.999999910813
2.34362529383e-09 0.999999911844
2.31505803416e-09 0.999999912863
2.28682994763e-09 0.999999913871
2.25893737049e-09 0.999999914867
2.23137619493e-09 0.999999915853
2.2041427572e-09 0.999999916827
2.17723317153e-09 0.99999991779
2.15064366316e-09 0.999999918742
2.12437067937e-09 0.999999919684
2.09841033438e-09 0.999999920615
2.07275929753e-09 0.999999921536
2.04741368304e-09 0.999999922446
2.02237016023e-09 0.999999923346
1.99762517639e-09 0.999999924236
1.97317528983e-09 0.999999925116
1.94901705886e-09 0.999999925986
1.92514704178e-09 0.999999926846
1.90156190794e-09 0.999999927697
1.87825843767e-09 0.999999928538
1.85523330032e-09 0.999999929369
1.83248327623e-09 0.999999930191
1.81000514576e-09 0.999999931004
1.78779568927e-09 0.999999931807
1.76585190914e-09 0.999999932602
1.74417069676e-09 0.999999933387
1.7227489435e-09 0.999999934164
1.70158365176e-09 0.999999934932
1.68067182393e-09 0.999999935691
1.66001046242e-09 0.999999936441
1.63959679167e-09 0.999999937183
1.61942781407e-09 0.999999937917
1.59950064305e-09 0.999999938642
1.57981250304e-09 0.999999939359
1.56036061849e-09 0.999999940068
1.54114232487e-09 0.999999940769
1.52215462457e-09 0.999999941462
1.5033950751e-09 0.999999942147
1.4848609009e-09 0.999999942824
1.46654954847e-09 0.999999943494
1.44845835326e-09 0.999999944156
1.43058465074e-09 0.99999994481
1.41292610945e-09 0.999999945457
1.39548006484e-09 0.999999946097
1.3782439634e-09 0.999999946729
1.36121547367e-09 0.999999947355
1.34439215316e-09 0.999999947973
1.32777155937e-09 0.999999948583
1.31135124981e-09 0.999999949188
1.29512900404e-09 0.999999949785
1.27910249059e-09 0.999999950375
1.26326937799e-09 0.999999950958
1.24762722375e-09 0.999999951535
1.2321741405e-09 0.999999952106
1.21690757471e-09 0.999999952669
1.20182552799e-09 0.999999953227
1.18692566886e-09 0.999999953778
1.17220599893e-09 0.999999954322
1.15766440878e-09 0.999999954861
1.14329867795e-09 0.999999955393
1.12910691907e-09 0.999999955919
1.11508680067e-09 0.999999956439
1.1012365464e-09 0.999999956954
1.08755415784e-09 0.999999957462
1.07403741456e-09 0.999999957964
1.06068465122e-09 0.999999958461
1.0474937584e-09 0.999999958952
1.03446284871e-09 0.999999959437
1.02159003479e-09 0.999999959917
1.00887354026e-09 0.999999960392
9.96311366741e-10 0.99999996086
9.83901848883e-10 0.999999961324
9.71643099312e-10 0.999999961782
9.59533230649e-10 0.999999962235
9.47570688581e-10 0.999999962682
9.35753585729e-10 0.999999963125
9.24080256759e-10 0.999999963562
9.12548925314e-10 0.999999963994
9.01158037081e-10 0.999999964422
8.89905815704e-10 0.999999964844
8.78790706871e-10 0.999999965262
8.67811045246e-10 0.999999965674
8.56965165497e-10 0.999999966082
8.46251513309e-10 0.999999966486
8.35668645394e-10 0.999999966884
8.25214785394e-10 0.999999967278
8.14888601042e-10 0.999999967668
8.04688427003e-10 0.999999968053
7.94612819988e-10 0.999999968433
7.84660336706e-10 0.999999968809
7.74829422845e-10 0.999999969181
7.65118746138e-10 0.999999969548
7.55526863294e-10 0.999999969911
7.46052220002e-10 0.99999997027
7.36693595016e-10 0.999999970625
7.27449434024e-10 0.999999970976
7.1831851578e-10 0.999999971322
7.09299396995e-10 0.999999971665
7.00390856423e-10 0.999999972003
6.91591450774e-10 0.999999972338
6.82899958804e-10 0.999999972669
6.74315048244e-10 0.999999972996
6.65835386826e-10 0.999999973319
6.57459864328e-10 0.999999973638
6.49187148483e-10 0.999999973954
6.41016018044e-10 0.999999974266
6.32945251766e-10 0.999999974574
6.24973628405e-10 0.999999974879
6.17100037736e-10 0.99999997518
6.09323258516e-10 0.999999975478
6.0164218052e-10 0.999999975772
5.94055471481e-10 0.999999976063
5.86562243221e-10 0.99999997635
5.79161274494e-10 0.999999976634
5.71851455078e-10 0.999999976915
5.64631563726e-10 0.999999977192
5.57500823284e-10 0.999999977467
5.50457901483e-10 0.999999977738
5.43501799122e-10 0.999999978005
5.36631517001e-10 0.99999997827
5.29846055919e-10 0.999999978532
5.23144305653e-10 0.99999997879
5.16525267003e-10 0.999999979046
5.09988051789e-10 0.999999979298
5.03531549789e-10 0.999999979548
4.97154872825e-10 0.999999979794
4.90857021695e-10 0.999999980038
4.84637108222e-10 0.999999980279
4.78494022182e-10 0.999999980517
4.72427097442e-10 0.999999980752
4.66435223778e-10 0.999999980985
4.60517513012e-10 0.999999981215
4.54673076966e-10 0.999999981442
4.48901138483e-10 0.999999981666
4.43200698363e-10 0.999999981888
4.37570868428e-10 0.999999982107
4.32010982543e-10 0.999999982323
4.26520041508e-10 0.999999982538
4.21097157144e-10 0.999999982749
4.15741663318e-10 0.999999982958
4.10452671851e-10 0.999999983165
4.05229405587e-10 0.999999983369
4.00070976347e-10 0.99999998357
3.94976717999e-10 0.99999998377
3.89945853385e-10 0.999999983967
3.84977494328e-10 0.999999984161
3.80070974693e-10 0.999999984354
3.75225517324e-10 0.999999984544
3.70440345066e-10 0.999999984731
3.65714791783e-10 0.999999984917
3.61048080322e-10 0.9999999851
3.56439544547e-10 0.999999985282
3.51888518324e-10 0.999999985461
3.47394224498e-10 0.999999985638
3.42955885912e-10 0.999999985813
3.38573058478e-10 0.999999985985
3.34244854017e-10 0.999999986156
3.29970717416e-10 0.999999986325
3.25749982544e-10 0.999999986492
3.21581872242e-10 0.999999986656
3.17465942423e-10 0.999999986819
3.13401526952e-10 0.99999998698
3.09387848674e-10 0.999999987139
3.05424352476e-10 0.999999987296
3.01510483247e-10 0.999999987451
2.97645685876e-10 0.999999987605
2.93829183207e-10 0.999999987756
2.9006053115e-10 0.999999987906
2.86339063571e-10 0.999999988054
2.82664225359e-10 0.9999999882
2.79035461404e-10 0.999999988344
2.75452216592e-10 0.999999988487
2.71913935812e-10 0.999999988628
2.68420063954e-10 0.999999988767
2.64970045905e-10 0.999999988905
2.61563326553e-10 0.999999989041
2.58199350789e-10 0.999999989176
2.54877674521e-10 0.999999989308
2.51597853662e-10 0.99999998944
2.48359111055e-10 0.999999989569
2.45161224655e-10 0.999999989697
2.42003528328e-10 0.999999989824
2.38885466963e-10 0.999999989949
2.35806818516e-10 0.999999990072
2.3276680583e-10 0.999999990195
2.29765206861e-10 0.999999990315
2.26801355474e-10 0.999999990434
2.23874807581e-10 0.999999990552
2.20985230115e-10 0.999999990668
2.18132067964e-10 0.999999990783
2.15314877039e-10 0.999999990897
2.12533324273e-10 0.999999991009
2.09786854555e-10 0.99999999112
2.07075023795e-10 0.999999991229
2.04397498926e-10 0.999999991338
2.01753724838e-10 0.999999991445
1.99143479485e-10 0.99999999155
1.96566096733e-10 0.999999991655
1.9402146556e-10 0.999999991758
1.91508919833e-10 0.999999991859
1.89028237507e-10 0.99999999196
1.8657886347e-10 0.99999999206
1.84160575678e-10 0.999999992158
1.81772930041e-10 0.999999992255
1.79415482471e-10 0.999999992351
1.77088010922e-10 0.999999992445
1.74789960283e-10 0.999999992539
1.7252110851e-10 0.999999992631
1.70281011513e-10 0.999999992723
1.68069336226e-10 0.999999992813
1.65885749581e-10 0.999999992902
1.63729918512e-10 0.99999999299
1.61601398929e-10 0.999999993077
1.59499968788e-10 0.999999993163
1.57425295022e-10 0.999999993248
1.55376933542e-10 0.999999993332
1.53354662302e-10 0.999999993415
1.51358148237e-10 0.999999993497
1.49386947257e-10 0.999999993577
1.47440948339e-10 0.999999993657
1.45519596373e-10 0.999999993736
1.43622891358e-10 0.999999993814
1.4175016716e-10 0.999999993891
1.39901423779e-10 0.999999993967
1.38076217127e-10 0.999999994042
1.36274325158e-10 0.999999994117
1.34495414805e-10 0.99999999419
1.32739153003e-10 0.999999994262
1.31005428727e-10 0.999999994334
1.29293686868e-10 0.999999994405
1.27603927425e-10 0.999999994475
1.25935706308e-10 0.999999994544
1.24288912495e-10 0.999999994612
1.22662990876e-10 0.999999994679
1.21058052471e-10 0.999999994746
1.19473542171e-10 0.999999994811
1.17909237929e-10 0.999999994876
1.16365139746e-10 0.99999999494
1.14840692511e-10 0.999999995004
1.13335785201e-10 0.999999995066
1.11850195772e-10 0.999999995128
1.10383591156e-10 0.999999995189
1.08935860332e-10 0.999999995249
1.0750655921e-10 0.999999995309
1.06095687791e-10 0.999999995368
1.04703024029e-10 0.999999995426
1.03328123835e-10 0.999999995483
1.01970876187e-10 0.99999999554
1.00631059041e-10 0.999999995596
9.9308450352e-11 0.999999995651
9.80029390973e-11 0.999999995706
9.67140811881e-11 0.99999999576
9.54418766241e-11 0.999999995813
9.41859923387e-11 0.999999995866
9.29463173094e-11 0.999999995918
9.17226294916e-11 0.999999995969
9.05145958185e-11 0.99999999602
8.93222162901e-11 0.99999999607
8.81451578394e-11 0.999999996119
8.69833094441e-11 0.999999996168
8.58363380374e-11 0.999999996217
8.47042436192e-11 0.999999996264
8.35866931226e-11 0.999999996311
8.24836865476e-11 0.999999996358
8.13947798051e-11 0.999999996404
8.03199728949e-11 0.999999996449
7.92591547949e-11 0.999999996494
7.82118814158e-11 0.999999996538
7.71782637798e-11 0.999999996582
7.61579688202e-11 0.999999996625
7.51507744923e-11 0.999999996668
7.4156680796e-11 0.99999999671
7.31754656869e-11 0.999999996752
7.22070181425e-11 0.999999996793
7.1251005096e-11 0.999999996833
7.03074265473e-11 0.999999996874
6.9376060452e-11 0.999999996913
6.84566847653e-11 0.999999996952
6.75492994873e-11 0.999999996991
6.66536825733e-11 0.999999997029
6.57697230011e-11 0.999999997067
6.4897198726e-11 0.999999997104
6.40359987258e-11 0.999999997141
6.31859009559e-11 0.999999997177
6.23469054162e-11 0.999999997213
6.15187900621e-11 0.999999997248
6.07015548937e-11 0.999999997283
5.98947558217e-11 0.999999997318
5.90986148907e-11 0.999999997352
5.83126880116e-11 0.999999997386
5.75370862066e-11 0.999999997419
5.67715874311e-11 0.999999997452
5.60159696406e-11 0.999999997484
5.52702328349e-11 0.999999997516
5.45341549696e-11 0.999999997548
5.38077360446e-11 0.999999997579
5.30908650376e-11 0.99999999761
5.23832088817e-11 0.99999999764
5.16847675769e-11 0.999999997671
5.09955411232e-11 0.9999999977
5.0315307476e-11 0.99999999773
4.96438445907e-11 0.999999997759
4.89812634896e-11 0.999999997787
4.83272311058e-11 0.999999997816
4.76818584616e-11 0.999999997843
4.70448124901e-11 0.999999997871
4.64162042135e-11 0.999999997898
4.57957005651e-11 0.999999997925
4.5183412567e-11 0.999999997952
4.45791181747e-11 0.999999997978
4.39827063659e-11 0.999999998004
4.33940661182e-11 0.999999998029
4.28131974317e-11 0.999999998055
4.22398782618e-11 0.99999999808
4.16741086084e-11 0.999999998104
4.11157774494e-11 0.999999998128
4.05647737622e-11 0.999999998152
4.00209865248e-11 0.999999998176
3.94843047147e-11 0.9999999982
3.89546173096e-11 0.999999998223
3.84320353319e-11 0.999999998246
3.79162257147e-11 0.999999998268
3.74071884579e-11 0.99999999829
3.69048125393e-11 0.999999998312
3.64090979588e-11 0.999999998334
3.59199336941e-11 0.999999998355
3.54370977007e-11 0.999999998377
3.49607010008e-11 0.999999998398
3.44905215499e-11 0.999999998418
3.40265593479e-11 0.999999998439
3.35687033726e-11 0.999999998459
3.31168426015e-11 0.999999998479
3.26709770349e-11 0.999999998498
3.22309956502e-11 0.999999998518
3.17967874253e-11 0.999999998537
3.13683523601e-11 0.999999998556
3.094546841e-11 0.999999998574
3.05282465973e-11 0.999999998593
3.01165758998e-11 0.999999998611
2.97102342728e-11 0.999999998629
2.93093327386e-11 0.999999998646
2.89136492526e-11 0.999999998664
2.85232948372e-11 0.999999998681
2.81380474476e-11 0.999999998698
2.7757907084e-11 0.999999998715
2.7382762724e-11 0.999999998732
2.70126143675e-11 0.999999998748
2.66473509924e-11 0.999999998764
2.62869725987e-11 0.99999999878
2.59312571416e-11 0.999999998796
2.55803156435e-11 0.999999998812
2.52340370821e-11 0.999999998827
2.48923104351e-11 0.999999998842
2.45552467248e-11 0.999999998857
2.42225128844e-11 0.999999998872
2.3894219936e-11 0.999999998887
2.35702568574e-11 0.999999998901
2.32507346709e-11 0.999999998916
2.29353203096e-11 0.99999999893
2.26241247958e-11 0.999999998944
2.23170371072e-11 0.999999998957
2.20140572438e-11 0.999999998971
2.17151852056e-11 0.999999998984
2.14201989479e-11 0.999999998998
2.11290984709e-11 0.999999999011
2.08419947967e-11 0.999999999024
2.05585548585e-11 0.999999999036
2.02790007009e-11 0.999999999049
2.00032213016e-11 0.999999999061
1.97309946159e-11 0.999999999073
1.94624316663e-11 0.999999999086
1.91974214303e-11 0.999999999098
1.89360749303e-11 0.999999999109
1.86780590994e-11 0.999999999121
1.84235959821e-11 0.999999999132
1.8172463534e-11 0.999999999144
1.79246617549e-11 0.999999999155
1.76801906449e-11 0.999999999166
1.74390502039e-11 0.999999999177
1.72011294097e-11 0.999999999188
1.696631724e-11 0.999999999198
1.67346136948e-11 0.999999999209
1.65061297963e-11 0.999999999219
1.62806435e-11 0.999999999229
1.60581548059e-11 0.999999999239
1.58386637139e-11 0.999999999249
1.56220592018e-11 0.999999999259
1.54084522919e-11 0.999999999269
1.51976209395e-11 0.999999999279
1.4989676167e-11 0.999999999288
1.4784506952e-11 0.999999999297
1.45821132946e-11 0.999999999307
1.43823841725e-11 0.999999999316
1.41853195856e-11 0.999999999325
1.3990919534e-11 0.999999999334
1.37991840177e-11 0.999999999342
1.36100020143e-11 0.999999999351
1.34232625015e-11 0.99999999936
1.32391875241e-11 0.999999999368
1.30574440149e-11 0.999999999376
1.28782540187e-11 0.999999999385
1.27013954909e-11 0.999999999393
1.25269794538e-11 0.999999999401
1.23548948849e-11 0.999999999409
1.21850307622e-11 0.999999999416
1.20176091301e-11 0.999999999424
1.18522969217e-11 0.999999999432
1.16893161817e-11 0.999999999439
1.15285558877e-11 0.999999999447
1.13699050175e-11 0.999999999454
1.1213363571e-11 0.999999999461
1.10589315483e-11 0.999999999468
1.09066089493e-11 0.999999999475
1.07563957741e-11 0.999999999482
1.06081810003e-11 0.999999999489
1.0461964628e-11 0.999999999496
1.03176356347e-11 0.999999999502
1.0175305043e-11 0.999999999509
1.00349728527e-11 0.999999999515
9.89652804151e-12 0.999999999522
9.75985958718e-12 0.999999999528
9.62507851199e-12 0.999999999534
9.49218481594e-12 0.999999999541
9.36106747673e-12 0.999999999547
9.23161547206e-12 0.999999999553
9.10405084653e-12 0.999999999559
8.97815155554e-12 0.999999999565
8.85402862139e-12 0.99999999957
8.73145999947e-12 0.999999999576
8.61066773439e-12 0.999999999582
8.49142978154e-12 0.999999999587
8.37385716324e-12 0.999999999593
8.25794987946e-12 0.999999999598
8.14348588563e-12 0.999999999603
8.03068722632e-12 0.999999999609
7.91933185695e-12 0.999999999614
7.80953079982e-12 0.999999999619
7.70117303261e-12 0.999999999624
7.59436957765e-12 0.999999999629
7.48900941261e-12 0.999999999634
7.3849815152e-12 0.999999999639
7.28250793003e-12 0.999999999644
7.18125559018e-12 0.999999999649
7.08155756257e-12 0.999999999653
6.98308078029e-12 0.999999999658
6.88604728794e-12 0.999999999662
6.79034606321e-12 0.999999999667
6.69586608382e-12 0.999999999671
6.60271837205e-12 0.999999999676
6.51079190561e-12 0.99999999968
6.4201977068e-12 0.999999999684
6.33082475332e-12 0.999999999689
6.24267304516e-12 0.999999999693
6.15563156003e-12 0.999999999697
6.06992234253e-12 0.999999999701
5.98521232575e-12 0.999999999705
5.9018345766e-12 0.999999999709
5.81945602818e-12 0.999999999713
5.73829872508e-12 0.999999999717
5.658251645e-12 0.99999999972
5.57920376565e-12 0.999999999724
5.50137713162e-12 0.999999999728
5.42454969832e-12 0.999999999732
5.34872146574e-12 0.999999999735
5.27400345618e-12 0.999999999739
5.20028464734e-12 0.999999999742
5.12756503923e-12 0.999999999746
5.05584463184e-12 0.999999999749
4.98512342517e-12 0.999999999752
4.91529039692e-12 0.999999999756
4.8465675917e-12 0.999999999759
4.77873296489e-12 0.999999999762
4.71178651651e-12 0.999999999766
4.64572824654e-12 0.999999999769
4.5806691773e-12 0.999999999772
4.51638726418e-12 0.999999999775
4.45310455177e-12 0.999999999778
4.39071001779e-12 0.999999999781
4.32909263992e-12 0.999999999784
4.26836344047e-12 0.999999999787
4.20841139714e-12 0.99999999979
4.14934753223e-12 0.999999999792
4.09106082344e-12 0.999999999795
4.03355127077e-12 0.999999999798
3.97692989651e-12 0.999999999801
3.92097465607e-12 0.999999999803
3.86590759405e-12 0.999999999806
3.81150666584e-12 0.999999999809
3.75788289375e-12 0.999999999811
3.70503627778e-12 0.999999999814
3.65285579562e-12 0.999999999816
3.60145246958e-12 0.999999999819
3.55071527736e-12 0.999999999821
3.50064421895e-12 0.999999999824
3.45135031665e-12 0.999999999826
3.40272254817e-12 0.999999999828
3.35476091351e-12 0.999999999831
3.30746541266e-12 0.999999999833
3.26083604563e-12 0.999999999835
3.2147617901e-12 0.999999999838
3.1694646907e-12 0.99999999984
3.12461168051e-12 0.999999999842
3.08053582643e-12 0.999999999844
3.03701508386e-12 0.999999999846
2.99416047511e-12 0.999999999848
2.95174995557e-12 0.99999999985
2.91011659215e-12 0.999999999852
2.86892731793e-12 0.999999999854
2.82829315523e-12 0.999999999856
2.78832512635e-12 0.999999999858
2.74891220897e-12 0.99999999986
2.70994338081e-12 0.999999999862
2.67152966416e-12 0.999999999864
2.63378208132e-12 0.999999999866
2.59636756539e-12 0.999999999868
2.55961918327e-12 0.99999999987
2.52331489037e-12 0.999999999871
2.48756570898e-12 0.999999999873
2.45226061679e-12 0.999999999875
2.41751063612e-12 0.999999999877
2.38320474466e-12 0.999999999878
2.34934294241e-12 0.99999999988
2.31603625167e-12 0.999999999882
2.28306262784e-12 0.999999999883
2.25064411552e-12 0.999999999885
2.21866969241e-12 0.999999999886
2.18713935851e-12 0.999999999888
2.15605311382e-12 0.999999999889
2.12541095834e-12 0.999999999891
2.09510186977e-12 0.999999999892
2.06534789271e-12 0.999999999894
2.03592698256e-12 0.999999999895
2.00695016161e-12 0.999999999897
1.97841742988e-12 0.999999999898
1.95021776506e-12 0.9999999999
1.92235116714e-12 0.999999999901
1.89503968073e-12 0.999999999902
1.86795023893e-12 0.999999999904
1.84130488634e-12 0.999999999905
1.81510362296e-12 0.999999999906
1.78912440418e-12 0.999999999908
1.76358927462e-12 0.999999999909
1.73849823426e-12 0.99999999991
1.71362923851e-12 0.999999999911
1.68920433197e-12 0.999999999913
1.66500147003e-12 0.999999999914
1.6412426973e-12 0.999999999915
1.61781699148e-12 0.999999999916
1.59461333027e-12 0.999999999917
1.57185375826e-12 0.999999999918
1.54931623086e-12 0.99999999992
1.52711177037e-12 0.999999999921
1.50535139909e-12 0.999999999922
1.48370205011e-12 0.999999999923
1.46249679034e-12 0.999999999924
1.44151357517e-12 0.999999999925
1.42086342692e-12 0.999999999926
1.40054634556e-12 0.999999999927
1.38045130882e-12 0.999999999928
1.36068933898e-12 0.999999999929
1.34114941375e-12 0.99999999993
1.32183153312e-12 0.999999999931
1.3028467194e-12 0.999999999932
1.28419497258e-12 0.999999999933
1.26576527038e-12 0.999999999934
1.24755761277e-12 0.999999999935
1.22968302207e-12 0.999999999936
1.21191945368e-12 0.999999999936
1.19448895219e-12 0.999999999937
1.17739151761e-12 0.999999999938
1.16040510534e-12 0.999999999939
1.14375175997e-12 0.99999999994
1.1273204592e-12 0.999999999941
1.11100018074e-12 0.999999999942
1.09501296919e-12 0.999999999942
1.07924780224e-12 0.999999999943
1.06370467989e-12 0.999999999944
1.04838360215e-12 0.999999999945
1.03328456902e-12 0.999999999946
1.01840758049e-12 0.999999999946
1.00364161426e-12 0.999999999947
9.89208714941e-13 0.999999999948
9.74886837923e-13 0.999999999948
9.60898027813e-13 0.999999999949
9.47020240005e-13 0.99999999995
9.33364496802e-13 0.999999999951
9.19819775902e-13 0.999999999951
9.06497099606e-13 0.999999999952
8.93396467916e-13 0.999999999953
8.8051788083e-13 0.999999999953
8.67750316047e-13 0.999999999954
8.55204795869e-13 0.999999999955
8.42881320295e-13 0.999999999955
8.30668867025e-13 0.999999999956
8.18678458359e-13 0.999999999956
8.06799071995e-13 0.999999999957
7.95030707934e-13 0.999999999958
7.8359541078e-13 0.999999999958
7.72160113627e-13 0.999999999959
7.61057883381e-13 0.999999999959
7.49955653134e-13 0.99999999996
7.39075467493e-13 0.999999999961
7.28417326457e-13 0.999999999961
7.1775918542e-13 0.999999999962
7.07434111291e-13 0.999999999962
6.97109037162e-13 0.999999999963
6.87006007638e-13 0.999999999963
6.77014000416e-13 0.999999999964
6.67133015497e-13 0.999999999964
6.57474075183e-13 0.999999999965
6.47926157171e-13 0.999999999965
6.38489261462e-13 0.999999999966
6.29163388055e-13 0.999999999966
6.20059559253e-13 0.999999999967
6.11066752754e-13 0.999999999967
6.02073946254e-13 0.999999999968
5.9330318436e-13 0.999999999968
5.8475446707e-13 0.999999999969
5.7620574978e-13 0.999999999969
5.67768054793e-13 0.999999999969
5.59552404411e-13 0.99999999997
5.51336754029e-13 0.99999999997
5.43343148252e-13 0.999999999971
5.35349542474e-13 0.999999999971
5.27577981302e-13 0.999999999971
5.19917442432e-13 0.999999999972
5.12256903562e-13 0.999999999972
5.04818409297e-13 0.999999999973
4.97379915032e-13 0.999999999973
4.90163465372e-13 0.999999999973
4.82947015712e-13 0.999999999974
4.75952610657e-13 0.999999999974
4.68958205602e-13 0.999999999975
4.62074822849e-13 0.999999999975
4.55302462399e-13 0.999999999975
4.48641124251e-13 0.999999999976
4.42090808406e-13 0.999999999976
4.35651514863e-13 0.999999999976
4.2921222132e-13 0.999999999977
4.22994972382e-13 0.999999999977
4.16777723444e-13 0.999999999977
4.10671496809e-13 0.999999999978
4.04676292476e-13 0.999999999978
3.98681088143e-13 0.999999999978
3.92907928415e-13 0.999999999979
3.87134768687e-13 0.999999999979
3.81361608959e-13 0.999999999979
3.75810493836e-13 0.999999999979
3.70259378712e-13 0.99999999998
3.64819285892e-13 0.99999999998
3.59490215374e-13 0.99999999998
3.54161144855e-13 0.999999999981
3.4894309664e-13 0.999999999981
3.43836070726e-13 0.999999999981
3.38840067116e-13 0.999999999981
3.33844063505e-13 0.999999999982
3.28959082196e-13 0.999999999982
3.24074100888e-13 0.999999999982
3.19300141882e-13 0.999999999982
3.14637205179e-13 0.999999999983
3.09974268475e-13 0.999999999983
3.05422354074e-13 0.999999999983
3.00870439673e-13 0.999999999983
2.96429547575e-13 0.999999999984
2.92099677779e-13 0.999999999984
2.87769807983e-13 0.999999999984
2.83550960489e-13 0.999999999984
2.79332112996e-13 0.999999999985
2.75224287805e-13 0.999999999985
2.71116462613e-13 0.999999999985
2.67119659725e-13 0.999999999985
2.63233879139e-13 0.999999999985
2.59348098552e-13 0.999999999986
2.55462317966e-13 0.999999999986
2.51687559683e-13 0.999999999986
2.48023823701e-13 0.999999999986
2.44249065418e-13 0.999999999986
2.40696351739e-13 0.999999999987
2.3714363806e-13 0.999999999987
2.33590924381e-13 0.999999999987
2.30149233005e-13 0.999999999987
2.26707541628e-13 0.999999999987
2.23376872555e-13 0.999999999988
2.20046203481e-13 0.999999999988
2.16826556709e-13 0.999999999988
2.13606909938e-13 0.999999999988
2.10387263166e-13 0.999999999988
2.07278638698e-13 0.999999999988
2.04281036531e-13 0.999999999989
2.01172412062e-13 0.999999999989
1.98174809896e-13 0.999999999989
1.95288230032e-13 0.999999999989
1.92401650168e-13 0.999999999989
1.89515070304e-13 0.999999999989
1.86739512742e-13 0.99999999999
1.8396395518e-13 0.99999999999
1.81188397619e-13 0.99999999999
1.7852386236e-13 0.99999999999
1.75859327101e-13 0.99999999999
1.73194791842e-13 0.99999999999
1.70641278885e-13 0.99999999999
1.68087765928e-13 0.999999999991
1.65534252972e-13 0.999999999991
1.63091762317e-13 0.999999999991
1.60649271663e-13 0.999999999991
1.58317803312e-13 0.999999999991
1.55875312657e-13 0.999999999991
1.53654866608e-13 0.999999999991
1.51323398256e-13 0.999999999991
1.49102952207e-13 0.999999999992
1.46882506158e-13 0.999999999992
1.44662060109e-13 0.999999999992
1.42441614059e-13 0.999999999992
1.40332190313e-13 0.999999999992
1.38222766566e-13 0.999999999992
1.36224365122e-13 0.999999999992
1.34114941375e-13 0.999999999992
1.3211653993e-13 0.999999999992
1.30118138486e-13 0.999999999993
1.28230759344e-13 0.999999999993
1.26343380202e-13 0.999999999993
1.2445600106e-13 0.999999999993
1.22568621919e-13 0.999999999993
1.20681242777e-13 0.999999999993
1.18904885937e-13 0.999999999993
1.17128529098e-13 0.999999999993
1.15352172259e-13 0.999999999993
1.13686837722e-13 0.999999999994
1.11910480882e-13 0.999999999994
1.10245146345e-13 0.999999999994
1.08579811808e-13 0.999999999994
1.06914477271e-13 0.999999999994
1.05360165037e-13 0.999999999994
1.03805852802e-13 0.999999999994
1.02251540568e-13 0.999999999994
1.00697228334e-13 0.999999999994
9.9142916099e-14 0.999999999994
9.7699626167e-14 0.999999999994
9.6256336235e-14 0.999999999994
9.4813046303e-14 0.999999999995
9.3369756371e-14 0.999999999995
9.1926466439e-14 0.999999999995
9.05941988094e-14 0.999999999995
8.91509088774e-14 0.999999999995
8.78186412478e-14 0.999999999995
8.64863736183e-14 0.999999999995
8.52651282912e-14 0.999999999995
8.39328606617e-14 0.999999999995
8.27116153346e-14 0.999999999995
8.1379347705e-14 0.999999999995
8.01581023779e-14 0.999999999995
7.89368570508e-14 0.999999999995
7.78266340262e-14 0.999999999996
7.66053886991e-14 0.999999999996
7.54951656745e-14 0.999999999996
7.42739203474e-14 0.999999999996
7.31636973228e-14 0.999999999996
7.20534742982e-14 0.999999999996
7.1054273576e-14 0.999999999996
6.99440505514e-14 0.999999999996
6.88338275268e-14 0.999999999996
6.78346268046e-14 0.999999999996
6.68354260824e-14 0.999999999996
6.58362253603e-14 0.999999999996
6.48370246381e-14 0.999999999996
6.38378239159e-14 0.999999999996
6.28386231938e-14 0.999999999996
6.19504447741e-14 0.999999999996
6.09512440519e-14 0.999999999996
6.00630656322e-14 0.999999999996
5.91748872125e-14 0.999999999997
5.81756864904e-14 0.999999999997
5.73985303731e-14 0.999999999997
5.65103519534e-14 0.999999999997
5.56221735337e-14 0.999999999997
5.4733995114e-14 0.999999999997
5.39568389968e-14 0.999999999997
5.31796828795e-14 0.999999999997
5.22915044598e-14 0.999999999997
5.15143483426e-14 0.999999999997
5.07371922254e-14 0.999999999997
4.99600361081e-14 0.999999999997
4.91828799909e-14 0.999999999997
4.84057238737e-14 0.999999999997
4.77395900589e-14 0.999999999997
4.69624339416e-14 0.999999999997
4.62963001269e-14 0.999999999997
4.56301663121e-14 0.999999999997
4.48530101949e-14 0.999999999997
4.41868763801e-14 0.999999999997
4.35207425653e-14 0.999999999997
4.28546087505e-14 0.999999999997
4.21884749358e-14 0.999999999998
4.1522341121e-14 0.999999999998
4.09672296087e-14 0.999999999998
4.03010957939e-14 0.999999999998
3.97459842816e-14 0.999999999998
3.90798504668e-14 0.999999999998
3.85247389545e-14 0.999999999998
3.78586051397e-14 0.999999999998
3.73034936274e-14 0.999999999998
3.67483821151e-14 0.999999999998
3.61932706028e-14 0.999999999998
3.56381590905e-14 0.999999999998
3.50830475782e-14 0.999999999998
3.45279360658e-14 0.999999999998
3.39728245535e-14 0.999999999998
3.35287353437e-14 0.999999999998
3.29736238314e-14 0.999999999998
3.25295346215e-14 0.999999999998
3.19744231092e-14 0.999999999998
3.15303338994e-14 0.999999999998
3.0975222387e-14 0.999999999998
3.05311331772e-14 0.999999999998
3.00870439673e-14 0.999999999998
2.96429547575e-14 0.999999999998
2.91988655476e-14 0.999999999998
2.87547763378e-14 0.999999999998
2.83106871279e-14 0.999999999998
2.78665979181e-14 0.999999999998
2.74225087082e-14 0.999999999998
2.69784194984e-14 0.999999999998
2.65343302885e-14 0.999999999998
2.62012633812e-14 0.999999999998
2.57571741713e-14 0.999999999998
2.53130849615e-14 0.999999999998
2.49800180541e-14 0.999999999998
2.46469511467e-14 0.999999999999
2.42028619368e-14 0.999999999999
2.38697950294e-14 0.999999999999
2.34257058196e-14 0.999999999999
2.30926389122e-14 0.999999999999
2.27595720048e-14 0.999999999999
2.24265050974e-14 0.999999999999
2.209343819e-14 0.999999999999
2.17603712827e-14 0.999999999999
2.14273043753e-14 0.999999999999
2.10942374679e-14 0.999999999999
2.07611705605e-14 0.999999999999
2.04281036531e-14 0.999999999999
2.00950367457e-14 0.999999999999
1.97619698383e-14 0.999999999999
1.94289029309e-14 0.999999999999
1.9206858326e-14 0.999999999999
1.88737914186e-14 0.999999999999
1.85407245112e-14 0.999999999999
1.83186799063e-14 0.999999999999
1.79856129989e-14 0.999999999999
1.7763568394e-14 0.999999999999
1.74305014866e-14 0.999999999999
1.72084568817e-14 0.999999999999
1.69864122768e-14 0.999999999999
1.66533453694e-14 0.999999999999
1.64313007645e-14 0.999999999999
1.62092561595e-14 0.999999999999
1.58761892521e-14 0.999999999999
1.56541446472e-14 0.999999999999
1.54321000423e-14 0.999999999999
1.52100554374e-14 0.999999999999
1.49880108324e-14 0.999999999999
1.47659662275e-14 0.999999999999
1.44328993201e-14 0.999999999999
1.42108547152e-14 0.999999999999
1.39888101103e-14 0.999999999999
1.37667655054e-14 0.999999999999
1.36557432029e-14 0.999999999999
1.3433698598e-14 0.999999999999
1.3211653993e-14 0.999999999999
1.29896093881e-14 0.999999999999
1.27675647832e-14 0.999999999999
1.25455201783e-14 0.999999999999
1.24344978758e-14 0.999999999999
1.22124532709e-14 0.999999999999
1.1990408666e-14 0.999999999999
1.1768364061e-14 0.999999999999
1.16573417586e-14 0.999999999999
1.14352971536e-14 0.999999999999
1.13242748512e-14 0.999999999999
1.11022302463e-14 0.999999999999
1.08801856413e-14 0.999999999999
1.07691633389e-14 0.999999999999
1.05471187339e-14 0.999999999999
1.04360964315e-14 0.999999999999
1.02140518266e-14 0.999999999999
1.01030295241e-14 0.999999999999
9.99200722163e-15 0.999999999999
9.7699626167e-15 0.999999999999
9.65894031424e-15 0.999999999999
9.43689570931e-15 0.999999999999
9.32587340685e-15 0.999999999999
9.21485110439e-15 0.999999999999
8.99280649946e-15 0.999999999999
8.881784197e-15 0.999999999999
8.77076189454e-15 0.999999999999
8.65973959208e-15 0.999999999999
8.43769498715e-15 0.999999999999
8.32667268469e-15 0.999999999999
8.21565038223e-15 0.999999999999
8.10462807976e-15 0.999999999999
7.9936057773e-15 1.0
7.88258347484e-15 1.0
7.77156117238e-15 1.0
7.54951656745e-15 1.0
7.43849426499e-15 1.0
7.32747196253e-15 1.0
7.21644966006e-15 1.0
7.1054273576e-15 1.0
6.99440505514e-15 1.0
6.88338275268e-15 1.0
6.77236045021e-15 1.0
6.66133814775e-15 1.0
6.55031584529e-15 1.0
6.43929354283e-15 1.0
6.43929354283e-15 1.0
6.32827124036e-15 1.0
6.2172489379e-15 1.0
6.10622663544e-15 1.0
5.99520433298e-15 1.0
5.88418203051e-15 1.0
5.77315972805e-15 1.0
5.77315972805e-15 1.0
5.66213742559e-15 1.0
5.55111512313e-15 1.0
5.44009282066e-15 1.0
5.3290705182e-15 1.0
5.3290705182e-15 1.0
5.21804821574e-15 1.0
5.10702591328e-15 1.0
4.99600361081e-15 1.0
4.99600361081e-15 1.0
4.88498130835e-15 1.0
4.77395900589e-15 1.0
4.77395900589e-15 1.0
4.66293670343e-15 1.0
4.55191440096e-15 1.0
4.55191440096e-15 1.0
4.4408920985e-15 1.0
4.32986979604e-15 1.0
4.32986979604e-15 1.0
4.21884749358e-15 1.0
4.10782519111e-15 1.0
4.10782519111e-15 1.0
3.99680288865e-15 1.0
3.99680288865e-15 1.0
3.88578058619e-15 1.0
3.88578058619e-15 1.0
3.77475828373e-15 1.0
3.77475828373e-15 1.0
3.66373598126e-15 1.0
3.5527136788e-15 1.0
3.5527136788e-15 1.0
3.44169137634e-15 1.0
3.44169137634e-15 1.0
3.33066907388e-15 1.0
3.33066907388e-15 1.0
3.21964677141e-15 1.0
3.21964677141e-15 1.0
3.21964677141e-15 1.0
3.10862446895e-15 1.0
3.10862446895e-15 1.0
2.99760216649e-15 1.0
2.99760216649e-15 1.0
2.88657986403e-15 1.0
2.88657986403e-15 1.0
2.88657986403e-15 1.0
2.77555756156e-15 1.0
2.77555756156e-15 1.0
2.6645352591e-15 1.0
2.6645352591e-15 1.0
2.6645352591e-15 1.0
2.55351295664e-15 1.0
2.55351295664e-15 1.0
2.44249065418e-15 1.0
2.44249065418e-15 1.0
2.44249065418e-15 1.0
2.33146835171e-15 1.0
2.33146835171e-15 1.0
2.33146835171e-15 1.0
2.22044604925e-15 1.0
2.22044604925e-15 1.0
2.22044604925e-15 1.0
2.10942374679e-15 1.0
2.10942374679e-15 1.0
2.10942374679e-15 1.0
2.10942374679e-15 1.0
1.99840144433e-15 1.0
1.99840144433e-15 1.0
1.99840144433e-15 1.0
1.88737914186e-15 1.0
1.88737914186e-15 1.0
1.88737914186e-15 1.0
1.88737914186e-15 1.0
1.7763568394e-15 1.0
1.7763568394e-15 1.0
1.7763568394e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.55431223448e-15 1.0
1.55431223448e-15 1.0
1.55431223448e-15 1.0
1.55431223448e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForPeriodicSigma1initialPart.tex <==
2.0 -1.0
1.0 0.0
0.666666666667 0.333333333333
0.5 0.5
0.4 0.6
0.333333333333 0.666666666667
0.285714285714 0.714285714286
0.25 0.75
0.222222222222 0.777777777778
0.2 0.8
0.181818181818 0.818181818182
0.166666666667 0.833333333333
0.153846153846 0.846153846154
0.142857142857 0.857142857143
0.133333333333 0.866666666667
0.125 0.875
0.117647058824 0.882352941176
0.111111111111 0.888888888889
0.105263157895 0.894736842105
0.1 0.9
0.0952380952381 0.904761904762
0.0909090909091 0.909090909091
0.0869565217391 0.913043478261
0.0833333333333 0.916666666667
0.08 0.92
0.0769230769231 0.923076923077
0.0740740740741 0.925925925926
0.0714285714286 0.928571428571
0.0689655172414 0.931034482759
0.0666666666667 0.933333333333
0.0645161290323 0.935483870968
0.0625 0.9375
0.0606060606061 0.939393939394
0.0588235294118 0.941176470588
0.0571428571429 0.942857142857
0.0555555555556 0.944444444444
0.0540540540541 0.945945945946
0.0526315789474 0.947368421053
0.0512820512821 0.948717948718
0.05 0.95
0.0487804878049 0.951219512195
0.047619047619 0.952380952381
0.046511627907 0.953488372093
0.0454545454545 0.954545454545
0.0444444444444 0.955555555556
0.0434782608696 0.95652173913
0.0425531914894 0.957446808511
0.0416666666667 0.958333333333
0.0408163265306 0.959183673469
0.04 0.96
0.0392156862745 0.960784313725
0.0384615384615 0.961538461538
0.0377358490566 0.962264150943
0.037037037037 0.962962962963
0.0363636363636 0.963636363636
0.0357142857143 0.964285714286
0.0350877192982 0.964912280702
0.0344827586207 0.965517241379
0.0338983050847 0.966101694915
0.0333333333333 0.966666666667
0.0327868852459 0.967213114754
0.0322580645161 0.967741935484
0.031746031746 0.968253968254
0.03125 0.96875
0.0307692307692 0.969230769231
0.030303030303 0.969696969697
0.0298507462687 0.970149253731
0.0294117647059 0.970588235294
0.0289855072464 0.971014492754
0.0285714285714 0.971428571429
0.0281690140845 0.971830985915
0.0277777777778 0.972222222222
0.027397260274 0.972602739726
0.027027027027 0.972972972973
0.0266666666667 0.973333333333
0.0263157894737 0.973684210526
0.025974025974 0.974025974026
0.025641025641 0.974358974359
0.0253164556962 0.974683544304
0.025 0.975
0.0246913580247 0.975308641975
0.0243902439024 0.975609756098
0.0240963855422 0.975903614458
0.0238095238095 0.97619047619
0.0235294117647 0.976470588235
0.0232558139535 0.976744186047
0.0229885057471 0.977011494253
0.0227272727273 0.977272727273
0.0224719101124 0.977528089888
0.0222222222222 0.977777777778
0.021978021978 0.978021978022
0.0217391304348 0.978260869565
0.0215053763441 0.978494623656
0.0212765957447 0.978723404255
0.0210526315789 0.978947368421
0.0208333333333 0.979166666667
0.020618556701 0.979381443299
0.0204081632653 0.979591836735
0.020202020202 0.979797979798
0.02 0.98
0.019801980198 0.980198019802
0.0196078431373 0.980392156863
0.0194174757282 0.980582524272
0.0192307692308 0.980769230769
0.0190476190476 0.980952380952
0.0188679245283 0.981132075472
0.018691588785 0.981308411215
0.0185185185185 0.981481481481
0.0183486238532 0.981651376147
0.0181818181818 0.981818181818
0.018018018018 0.981981981982
0.0178571428571 0.982142857143
0.0176991150442 0.982300884956
0.0175438596491 0.982456140351
0.0173913043478 0.982608695652
0.0172413793103 0.98275862069
0.017094017094 0.982905982906
0.0169491525424 0.983050847458
0.0168067226891 0.983193277311
0.0166666666667 0.983333333333
0.0165289256198 0.98347107438
0.016393442623 0.983606557377
0.0162601626016 0.983739837398
0.0161290322581 0.983870967742
0.016 0.984
0.015873015873 0.984126984127
0.0157480314961 0.984251968504
0.015625 0.984375
0.015503875969 0.984496124031
0.0153846153846 0.984615384615
0.0152671755725 0.984732824427
0.0151515151515 0.984848484848
0.015037593985 0.984962406015
0.0149253731343 0.985074626866
0.0148148148148 0.985185185185
0.0147058823529 0.985294117647
0.014598540146 0.985401459854
0.0144927536232 0.985507246377
0.0143884892086 0.985611510791
0.0142857142857 0.985714285714
0.0141843971631 0.985815602837
0.0140845070423 0.985915492958
0.013986013986 0.986013986014
0.0138888888889 0.986111111111
0.0137931034483 0.986206896552
0.013698630137 0.986301369863
0.0136054421769 0.986394557823
0.0135135135135 0.986486486486
0.0134228187919 0.986577181208
0.0133333333333 0.986666666667
0.0132450331126 0.986754966887
0.0131578947368 0.986842105263
0.0130718954248 0.986928104575
0.012987012987 0.987012987013
0.0129032258065 0.987096774194
0.0128205128205 0.987179487179
0.0127388535032 0.987261146497
0.0126582278481 0.987341772152
0.0125786163522 0.987421383648
0.0125 0.9875
0.0124223602484 0.987577639752
0.0123456790123 0.987654320988
0.0122699386503 0.98773006135
0.0121951219512 0.987804878049
0.0121212121212 0.987878787879
0.0120481927711 0.987951807229
0.0119760479042 0.988023952096
0.0119047619048 0.988095238095
0.0118343195266 0.988165680473
0.0117647058824 0.988235294118
0.0116959064327 0.988304093567
0.0116279069767 0.988372093023
0.0115606936416 0.988439306358
0.0114942528736 0.988505747126
0.0114285714286 0.988571428571
0.0113636363636 0.988636363636
0.0112994350282 0.988700564972
0.0112359550562 0.988764044944
0.0111731843575 0.988826815642
0.0111111111111 0.988888888889
0.0110497237569 0.988950276243
0.010989010989 0.989010989011
0.0109289617486 0.989071038251
0.0108695652174 0.989130434783
0.0108108108108 0.989189189189
0.010752688172 0.989247311828
0.0106951871658 0.989304812834
0.0106382978723 0.989361702128
0.010582010582 0.989417989418
0.0105263157895 0.989473684211
0.0104712041885 0.989528795812
0.0104166666667 0.989583333333
0.0103626943005 0.989637305699
0.0103092783505 0.989690721649
0.0102564102564 0.989743589744
0.0102040816327 0.989795918367
0.010152284264 0.989847715736
0.010101010101 0.989898989899
0.0100502512563 0.989949748744
0.01 0.99
0.00995024875622 0.990049751244
0.00990099009901 0.990099009901
0.00985221674877 0.990147783251
0.00980392156863 0.990196078431
0.00975609756098 0.990243902439
0.00970873786408 0.990291262136
0.00966183574879 0.990338164251
0.00961538461538 0.990384615385
0.00956937799043 0.99043062201
0.00952380952381 0.990476190476
0.00947867298578 0.990521327014
0.00943396226415 0.990566037736
0.0093896713615 0.990610328638
0.00934579439252 0.990654205607
0.0093023255814 0.990697674419
0.00925925925926 0.990740740741
0.00921658986175 0.990783410138
0.00917431192661 0.990825688073
0.00913242009132 0.990867579909
0.00909090909091 0.990909090909
0.00904977375566 0.990950226244
0.00900900900901 0.990990990991
0.00896860986547 0.991031390135
0.00892857142857 0.991071428571
0.00888888888889 0.991111111111
0.00884955752212 0.991150442478
0.00881057268722 0.991189427313
0.00877192982456 0.991228070175
0.00873362445415 0.991266375546
0.00869565217391 0.991304347826
0.00865800865801 0.991341991342
0.00862068965517 0.991379310345
0.00858369098712 0.991416309013
0.00854700854701 0.991452991453
0.00851063829787 0.991489361702
0.00847457627119 0.991525423729
0.0084388185654 0.991561181435
0.00840336134454 0.991596638655
0.00836820083682 0.991631799163
0.00833333333333 0.991666666667
0.00829875518672 0.991701244813
0.00826446280992 0.99173553719
0.0082304526749 0.991769547325
0.00819672131148 0.991803278689
0.00816326530612 0.991836734694
0.00813008130081 0.991869918699
0.0080971659919 0.991902834008
0.00806451612903 0.991935483871
0.00803212851406 0.991967871486
0.008 0.992
0.00796812749004 0.99203187251
0.00793650793651 0.992063492063
0.00790513833992 0.99209486166
0.00787401574803 0.992125984252
0.0078431372549 0.992156862745
0.0078125 0.9921875
0.00778210116732 0.992217898833
0.0077519379845 0.992248062016
0.00772200772201 0.992277992278
0.00769230769231 0.992307692308
0.00766283524904 0.992337164751
0.00763358778626 0.992366412214
0.00760456273764 0.992395437262
0.00757575757576 0.992424242424
0.00754716981132 0.992452830189
0.00751879699248 0.992481203008
0.00749063670412 0.992509363296
0.00746268656716 0.992537313433
0.00743494423792 0.992565055762
0.00740740740741 0.992592592593
0.00738007380074 0.992619926199
0.00735294117647 0.992647058824
0.00732600732601 0.992673992674
0.00729927007299 0.992700729927
0.00727272727273 0.992727272727
0.00724637681159 0.992753623188
0.0072202166065 0.992779783394
0.00719424460432 0.992805755396
0.00716845878136 0.992831541219
0.00714285714286 0.992857142857
0.00711743772242 0.992882562278
0.00709219858156 0.992907801418
0.00706713780919 0.992932862191
0.00704225352113 0.992957746479
0.00701754385965 0.99298245614
0.00699300699301 0.993006993007
0.00696864111498 0.993031358885
0.00694444444444 0.993055555556
0.00692041522491 0.993079584775
0.00689655172414 0.993103448276
0.00687285223368 0.993127147766
0.00684931506849 0.993150684932
0.00682593856655 0.993174061433
0.00680272108844 0.993197278912
0.00677966101695 0.993220338983
0.00675675675676 0.993243243243
0.00673400673401 0.993265993266
0.00671140939597 0.993288590604
0.0066889632107 0.993311036789
0.00666666666667 0.993333333333
0.00664451827243 0.993355481728
0.00662251655629 0.993377483444
0.00660066006601 0.993399339934
0.00657894736842 0.993421052632
0.00655737704918 0.993442622951
0.00653594771242 0.993464052288
0.00651465798046 0.99348534202
0.00649350649351 0.993506493506
0.00647249190939 0.993527508091
0.00645161290323 0.993548387097
0.0064308681672 0.993569131833
0.00641025641026 0.99358974359
0.00638977635783 0.993610223642
0.00636942675159 0.993630573248
0.00634920634921 0.993650793651
0.00632911392405 0.993670886076
0.00630914826498 0.993690851735
0.0062893081761 0.993710691824
0.00626959247649 0.993730407524
0.00625 0.99375
0.00623052959502 0.993769470405
0.00621118012422 0.993788819876
0.0061919504644 0.993808049536
0.00617283950617 0.993827160494
0.00615384615385 0.993846153846
0.00613496932515 0.993865030675
0.00611620795107 0.993883792049
0.00609756097561 0.993902439024
0.00607902735562 0.993920972644
0.00606060606061 0.993939393939
0.00604229607251 0.993957703927
0.00602409638554 0.993975903614
0.00600600600601 0.993993993994
0.0059880239521 0.994011976048
0.00597014925373 0.994029850746
0.00595238095238 0.994047619048
0.00593471810089 0.994065281899
0.00591715976331 0.994082840237
0.00589970501475 0.994100294985
0.00588235294118 0.994117647059
0.0058651026393 0.994134897361
0.00584795321637 0.994152046784
0.00583090379009 0.99416909621
0.00581395348837 0.994186046512
0.00579710144928 0.994202898551
0.00578034682081 0.994219653179
0.00576368876081 0.994236311239
0.00574712643678 0.994252873563
0.00573065902579 0.994269340974
0.00571428571429 0.994285714286
0.00569800569801 0.994301994302
0.00568181818182 0.994318181818
0.0056657223796 0.99433427762
0.00564971751412 0.994350282486
0.0056338028169 0.994366197183
0.00561797752809 0.994382022472
0.00560224089636 0.994397759104
0.00558659217877 0.994413407821
0.00557103064067 0.994428969359
0.00555555555556 0.994444444444
0.00554016620499 0.994459833795
0.00552486187845 0.994475138122
0.00550964187328 0.994490358127
0.00549450549451 0.994505494505
0.00547945205479 0.994520547945
0.00546448087432 0.994535519126
0.00544959128065 0.994550408719
0.0054347826087 0.994565217391
0.00542005420054 0.994579945799
0.00540540540541 0.994594594595
0.00539083557951 0.99460916442
0.00537634408602 0.994623655914
0.00536193029491 0.994638069705
0.00534759358289 0.994652406417
0.00533333333333 0.994666666667
0.00531914893617 0.994680851064
0.0053050397878 0.994694960212
0.00529100529101 0.994708994709
0.00527704485488 0.994722955145
0.00526315789474 0.994736842105
0.00524934383202 0.994750656168
0.00523560209424 0.994764397906
0.00522193211488 0.994778067885
0.00520833333333 0.994791666667
0.00519480519481 0.994805194805
0.00518134715026 0.99481865285
0.00516795865633 0.994832041344
0.00515463917526 0.994845360825
0.00514138817481 0.994858611825
0.00512820512821 0.994871794872
0.00511508951407 0.994884910486
0.00510204081633 0.994897959184
0.00508905852417 0.994910941476
0.00507614213198 0.994923857868
0.00506329113924 0.994936708861
0.00505050505051 0.994949494949
0.00503778337531 0.994962216625
0.00502512562814 0.994974874372
0.00501253132832 0.994987468672
0.005 0.995
0.00498753117207 0.995012468828
0.00497512437811 0.995024875622
0.00496277915633 0.995037220844
0.0049504950495 0.99504950495
0.00493827160494 0.995061728395
0.00492610837438 0.995073891626
0.004914004914 0.995085995086
0.00490196078431 0.995098039216
0.00488997555012 0.99511002445
0.00487804878049 0.99512195122
0.00486618004866 0.995133819951
0.00485436893204 0.995145631068
0.00484261501211 0.995157384988
0.0048309178744 0.995169082126
0.00481927710843 0.995180722892
0.00480769230769 0.995192307692
0.00479616306954 0.99520383693
0.00478468899522 0.995215311005
0.00477326968974 0.99522673031
0.0047619047619 0.995238095238
0.00475059382423 0.995249406176
0.00473933649289 0.995260663507
0.00472813238771 0.995271867612
0.00471698113208 0.995283018868
0.00470588235294 0.995294117647
0.00469483568075 0.995305164319
0.00468384074941 0.995316159251
0.00467289719626 0.995327102804
0.004662004662 0.995337995338
0.0046511627907 0.995348837209
0.0046403712297 0.99535962877
0.00462962962963 0.99537037037
0.00461893764434 0.995381062356
0.00460829493088 0.995391705069
0.00459770114943 0.995402298851
0.0045871559633 0.995412844037
0.0045766590389 0.995423340961
0.00456621004566 0.995433789954
0.00455580865604 0.995444191344
0.00454545454545 0.995454545455
0.00453514739229 0.995464852608
0.00452488687783 0.995475113122
0.00451467268623 0.995485327314
0.0045045045045 0.995495495495
0.00449438202247 0.995505617978
0.00448430493274 0.995515695067
0.00447427293065 0.995525727069
0.00446428571429 0.995535714286
0.00445434298441 0.995545657016
0.00444444444444 0.995555555556
0.00443458980044 0.9955654102
0.00442477876106 0.995575221239
0.00441501103753 0.995584988962
0.00440528634361 0.995594713656
0.0043956043956 0.995604395604
0.00438596491228 0.995614035088
0.00437636761488 0.995623632385
0.00436681222707 0.995633187773
0.00435729847495 0.995642701525
0.00434782608696 0.995652173913
0.00433839479393 0.995661605206
0.004329004329 0.995670995671
0.00431965442765 0.995680345572
0.00431034482759 0.995689655172
0.00430107526882 0.995698924731
0.00429184549356 0.995708154506
0.00428265524625 0.995717344754
0.0042735042735 0.995726495726
0.00426439232409 0.995735607676
0.00425531914894 0.995744680851
0.00424628450106 0.995753715499
0.00423728813559 0.995762711864
0.00422832980973 0.99577167019
0.0042194092827 0.995780590717
0.00421052631579 0.995789473684
0.00420168067227 0.995798319328
0.0041928721174 0.995807127883
0.00418410041841 0.995815899582
0.00417536534447 0.995824634656
0.00416666666667 0.995833333333
0.004158004158 0.995841995842
0.00414937759336 0.995850622407
0.00414078674948 0.995859213251
0.00413223140496 0.995867768595
0.00412371134021 0.99587628866
0.00411522633745 0.995884773663
0.0041067761807 0.995893223819
0.00409836065574 0.995901639344
0.0040899795501 0.99591002045
0.00408163265306 0.995918367347
0.0040733197556 0.995926680244
0.00406504065041 0.99593495935
0.00405679513185 0.995943204868
0.00404858299595 0.995951417004
0.0040404040404 0.99595959596
0.00403225806452 0.995967741935
0.00402414486922 0.995975855131
0.00401606425703 0.995983935743
0.00400801603206 0.995991983968
0.004 0.996
0.00399201596806 0.996007984032
0.00398406374502 0.996015936255
0.00397614314115 0.996023856859
0.00396825396825 0.996031746032
0.0039603960396 0.99603960396
0.00395256916996 0.99604743083
0.00394477317554 0.996055226824
0.00393700787402 0.996062992126
0.00392927308448 0.996070726916
0.00392156862745 0.996078431373
0.00391389432485 0.996086105675
0.00390625 0.99609375
0.00389863547758 0.996101364522
0.00389105058366 0.996108949416
0.00388349514563 0.996116504854
0.00387596899225 0.996124031008
0.00386847195358 0.996131528046
0.003861003861 0.996138996139
0.00385356454721 0.996146435453
0.00384615384615 0.996153846154
0.00383877159309 0.996161228407
0.00383141762452 0.996168582375
0.0038240917782 0.996175908222
0.00381679389313 0.996183206107
0.00380952380952 0.99619047619
0.00380228136882 0.996197718631
0.00379506641366 0.996204933586
0.00378787878788 0.996212121212
0.00378071833648 0.996219281664
0.00377358490566 0.996226415094
0.00376647834275 0.996233521657
0.00375939849624 0.996240601504
0.00375234521576 0.996247654784
0.00374531835206 0.996254681648
0.00373831775701 0.996261682243
0.00373134328358 0.996268656716
0.00372439478585 0.996275605214
0.00371747211896 0.996282527881
0.00371057513915 0.996289424861
0.0037037037037 0.996296296296
0.00369685767098 0.996303142329
0.00369003690037 0.9963099631
0.0036832412523 0.996316758748
0.00367647058824 0.996323529412
0.00366972477064 0.996330275229
0.003663003663 0.996336996337
0.0036563071298 0.99634369287
0.0036496350365 0.996350364964
0.00364298724954 0.99635701275
0.00363636363636 0.996363636364
0.00362976406534 0.996370235935
0.0036231884058 0.996376811594
0.00361663652803 0.996383363472
0.00361010830325 0.996389891697
0.0036036036036 0.996396396396
0.00359712230216 0.996402877698
0.00359066427289 0.996409335727
0.00358422939068 0.996415770609
0.00357781753131 0.996422182469
0.00357142857143 0.996428571429
0.00356506238859 0.996434937611
0.00355871886121 0.996441281139
0.00355239786856 0.996447602131
0.00354609929078 0.996453900709
0.00353982300885 0.996460176991
0.00353356890459 0.996466431095
0.00352733686067 0.996472663139
0.00352112676056 0.996478873239
0.00351493848858 0.996485061511
0.00350877192982 0.99649122807
0.00350262697023 0.99649737303
0.0034965034965 0.996503496503
0.00349040139616 0.996509598604
0.00348432055749 0.996515679443
0.00347826086957 0.99652173913
0.00347222222222 0.996527777778
0.00346620450607 0.996533795494
0.00346020761246 0.996539792388
0.00345423143351 0.996545768566
0.00344827586207 0.996551724138
0.00344234079174 0.996557659208
0.00343642611684 0.996563573883
0.00343053173242 0.996569468268
0.00342465753425 0.996575342466
0.0034188034188 0.996581196581
0.00341296928328 0.996587030717
0.00340715502555 0.996592844974
0.00340136054422 0.996598639456
0.00339558573854 0.996604414261
0.00338983050847 0.996610169492
0.00338409475465 0.996615905245
0.00337837837838 0.996621621622
0.00337268128162 0.996627318718
0.003367003367 0.996632996633
0.00336134453782 0.996638655462
0.00335570469799 0.996644295302
0.00335008375209 0.996649916248
0.00334448160535 0.996655518395
0.00333889816361 0.996661101836
0.00333333333333 0.996666666667
0.00332778702163 0.996672212978
0.00332225913621 0.996677740864
0.00331674958541 0.996683250415
0.00331125827815 0.996688741722
0.00330578512397 0.996694214876
0.003300330033 0.996699669967
0.00329489291598 0.996705107084
0.00328947368421 0.996710526316
0.00328407224959 0.99671592775
0.00327868852459 0.996721311475
0.00327332242226 0.996726677578
0.00326797385621 0.996732026144
0.00326264274062 0.996737357259
0.00325732899023 0.99674267101
0.00325203252033 0.99674796748
0.00324675324675 0.996753246753
0.0032414910859 0.996758508914
0.00323624595469 0.996763754045
0.0032310177706 0.996768982229
0.00322580645161 0.996774193548
0.00322061191626 0.996779388084
0.0032154340836 0.996784565916
0.00321027287319 0.996789727127
0.00320512820513 0.996794871795
0.0032 0.9968
0.00319488817891 0.996805111821
0.00318979266348 0.996810207337
0.0031847133758 0.996815286624
0.00317965023847 0.996820349762
0.0031746031746 0.996825396825
0.00316957210777 0.996830427892
0.00316455696203 0.996835443038
0.00315955766193 0.996840442338
0.00315457413249 0.996845425868
0.00314960629921 0.996850393701
0.00314465408805 0.996855345912
0.00313971742543 0.996860282575
0.00313479623824 0.996865203762
0.00312989045383 0.996870109546
0.003125 0.996875
0.00312012480499 0.996879875195
0.00311526479751 0.996884735202
0.00311041990669 0.996889580093
0.00310559006211 0.996894409938
0.0031007751938 0.996899224806
0.0030959752322 0.996904024768
0.00309119010819 0.996908809892
0.00308641975309 0.996913580247
0.00308166409861 0.996918335901
0.00307692307692 0.996923076923
0.00307219662058 0.996927803379
0.00306748466258 0.996932515337
0.00306278713629 0.996937212864
0.00305810397554 0.996941896024
0.0030534351145 0.996946564885
0.0030487804878 0.996951219512
0.00304414003044 0.99695585997
0.00303951367781 0.996960486322
0.00303490136571 0.996965098634
0.0030303030303 0.99696969697
0.00302571860817 0.996974281392
0.00302114803625 0.996978851964
0.00301659125189 0.996983408748
0.00301204819277 0.996987951807
0.00300751879699 0.996992481203
0.003003003003 0.996996996997
0.00299850074963 0.99700149925
0.00299401197605 0.997005988024
0.00298953662182 0.997010463378
0.00298507462687 0.997014925373
0.00298062593145 0.997019374069
0.00297619047619 0.997023809524
0.00297176820208 0.997028231798
0.00296735905045 0.99703264095
0.00296296296296 0.997037037037
0.00295857988166 0.997041420118
0.00295420974889 0.997045790251
0.00294985250737 0.997050147493
0.00294550810015 0.9970544919
0.00294117647059 0.997058823529
0.00293685756241 0.997063142438
0.00293255131965 0.99706744868
0.00292825768668 0.997071742313
0.00292397660819 0.997076023392
0.0029197080292 0.997080291971
0.00291545189504 0.997084548105
0.00291120815138 0.997088791849
0.00290697674419 0.997093023256
0.00290275761974 0.99709724238
0.00289855072464 0.997101449275
0.00289435600579 0.997105643994
0.0028901734104 0.99710982659
0.002886002886 0.997113997114
0.0028818443804 0.99711815562
0.00287769784173 0.997122302158
0.00287356321839 0.997126436782
0.00286944045911 0.997130559541
0.00286532951289 0.997134670487
0.00286123032904 0.997138769671
0.00285714285714 0.997142857143
0.00285306704708 0.997146932953
0.002849002849 0.997150997151
0.00284495021337 0.997155049787
0.00284090909091 0.997159090909
0.00283687943262 0.997163120567
0.0028328611898 0.99716713881
0.002828854314 0.997171145686
0.00282485875706 0.997175141243
0.00282087447109 0.997179125529
0.00281690140845 0.997183098592
0.0028129395218 0.997187060478
0.00280898876404 0.997191011236
0.00280504908836 0.997194950912
0.00280112044818 0.997198879552
0.0027972027972 0.997202797203
0.00279329608939 0.997206703911
0.00278940027894 0.997210599721
0.00278551532033 0.99721448468
0.00278164116829 0.997218358832
0.00277777777778 0.997222222222
0.00277392510402 0.997226074896
0.00277008310249 0.997229916898
0.00276625172891 0.997233748271
0.00276243093923 0.997237569061
0.00275862068966 0.99724137931
0.00275482093664 0.997245179063
0.00275103163686 0.997248968363
0.00274725274725 0.997252747253
0.00274348422497 0.997256515775
0.0027397260274 0.997260273973
0.00273597811218 0.997264021888
0.00273224043716 0.997267759563
0.00272851296044 0.99727148704
0.00272479564033 0.99727520436
0.00272108843537 0.997278911565
0.00271739130435 0.997282608696
0.00271370420624 0.997286295794
0.00271002710027 0.9972899729
0.00270635994587 0.997293640054
0.0027027027027 0.997297297297
0.00269905533063 0.997300944669
0.00269541778976 0.99730458221
0.00269179004038 0.99730820996
0.00268817204301 0.997311827957
0.00268456375839 0.997315436242
0.00268096514745 0.997319034853
0.00267737617135 0.997322623829
0.00267379679144 0.997326203209
0.00267022696929 0.997329773031
0.00266666666667 0.997333333333
0.00266311584554 0.997336884154
0.00265957446809 0.997340425532
0.00265604249668 0.997343957503
0.0026525198939 0.997347480106
0.00264900662252 0.997350993377
0.0026455026455 0.997354497354
0.00264200792602 0.997357992074
0.00263852242744 0.997361477573
0.00263504611331 0.997364953887
0.00263157894737 0.997368421053
0.00262812089356 0.997371879106
0.00262467191601 0.997375328084
0.00262123197903 0.997378768021
0.00261780104712 0.997382198953
0.00261437908497 0.997385620915
0.00261096605744 0.997389033943
0.0026075619296 0.99739243807
0.00260416666667 0.997395833333
0.00260078023407 0.997399219766
0.0025974025974 0.997402597403
0.00259403372244 0.997405966278
0.00259067357513 0.997409326425
0.0025873221216 0.997412677878
0.00258397932817 0.997416020672
0.00258064516129 0.997419354839
0.00257731958763 0.997422680412
0.002574002574 0.997425997426
0.0025706940874 0.997429305913
0.00256739409499 0.997432605905
0.0025641025641 0.997435897436
0.00256081946223 0.997439180538
0.00255754475703 0.997442455243
0.00255427841635 0.997445721584
0.00255102040816 0.997448979592
0.00254777070064 0.997452229299
0.00254452926209 0.997455470738
0.00254129606099 0.997458703939
0.00253807106599 0.997461928934
0.00253485424588 0.997465145754
0.00253164556962 0.99746835443
0.00252844500632 0.997471554994
0.00252525252525 0.997474747475
0.00252206809584 0.997477931904
0.00251889168766 0.997481108312
0.00251572327044 0.99748427673
0.00251256281407 0.997487437186
0.00250941028858 0.997490589711
0.00250626566416 0.997493734336
0.00250312891114 0.997496871089
0.0025 0.9975
0.00249687890137 0.997503121099
0.00249376558603 0.997506234414
0.00249066002491 0.997509339975
0.00248756218905 0.997512437811
0.00248447204969 0.99751552795
0.00248138957816 0.997518610422
0.00247831474597 0.997521685254
0.00247524752475 0.997524752475
0.00247218788628 0.997527812114
0.00246913580247 0.997530864198
0.00246609124538 0.997533908755
0.00246305418719 0.997536945813
0.00246002460025 0.9975399754
0.002457002457 0.997542997543
0.00245398773006 0.99754601227
0.00245098039216 0.997549019608
0.00244798041616 0.997552019584
0.00244498777506 0.997555012225
0.002442002442 0.997557997558
0.00243902439024 0.99756097561
0.00243605359318 0.997563946407
0.00243309002433 0.997566909976
0.00243013365735 0.997569866343
0.00242718446602 0.997572815534
0.00242424242424 0.997575757576
0.00242130750605 0.997578692494
0.00241837968561 0.997581620314
0.0024154589372 0.997584541063
0.00241254523522 0.997587454765
0.00240963855422 0.997590361446
0.00240673886883 0.997593261131
0.00240384615385 0.997596153846
0.00240096038415 0.997599039616
0.00239808153477 0.997601918465
0.00239520958084 0.997604790419
0.00239234449761 0.997607655502
0.00238948626045 0.99761051374
0.00238663484487 0.997613365155
0.00238379022646 0.997616209774
0.00238095238095 0.997619047619
0.00237812128419 0.997621878716
0.00237529691211 0.997624703088
0.00237247924081 0.997627520759
0.00236966824645 0.997630331754
0.00236686390533 0.997633136095
0.00236406619385 0.997635933806
0.00236127508855 0.997638724911
0.00235849056604 0.997641509434
0.00235571260306 0.997644287397
0.00235294117647 0.997647058824
0.00235017626322 0.997649823737
0.00234741784038 0.99765258216
0.00234466588511 0.997655334115
0.00234192037471 0.997658079625
0.00233918128655 0.997660818713
0.00233644859813 0.997663551402
0.00233372228705 0.997666277713
0.002331002331 0.997668997669
0.0023282887078 0.997671711292
0.00232558139535 0.997674418605
0.00232288037166 0.997677119628
0.00232018561485 0.997679814385
0.00231749710313 0.997682502897
0.00231481481481 0.997685185185
0.00231213872832 0.997687861272
0.00230946882217 0.997690531178
0.00230680507497 0.997693194925
0.00230414746544 0.997695852535
0.00230149597238 0.997698504028
0.00229885057471 0.997701149425
0.00229621125144 0.997703788749
0.00229357798165 0.997706422018
0.00229095074456 0.997709049255
0.00228832951945 0.997711670481
0.00228571428571 0.997714285714
0.00228310502283 0.997716894977
0.00228050171038 0.99771949829
0.00227790432802 0.997722095672
0.00227531285552 0.997724687144
0.00227272727273 0.997727272727
0.00227014755959 0.99772985244
0.00226757369615 0.997732426304
0.00226500566251 0.997734994337
0.00226244343891 0.997737556561
0.00225988700565 0.997740112994
0.00225733634312 0.997742663657
0.00225479143179 0.997745208568
0.00225225225225 0.997747747748
0.00224971878515 0.997750281215
0.00224719101124 0.997752808989
0.00224466891134 0.997755331089
0.00224215246637 0.997757847534
0.00223964165733 0.997760358343
0.00223713646532 0.997762863535
0.00223463687151 0.997765363128
0.00223214285714 0.997767857143
0.00222965440357 0.997770345596
0.0022271714922 0.997772828508
0.00222469410456 0.997775305895
0.00222222222222 0.997777777778
0.00221975582686 0.997780244173
0.00221729490022 0.9977827051
0.00221483942414 0.997785160576
0.00221238938053 0.997787610619
0.00220994475138 0.997790055249
0.00220750551876 0.997792494481
0.00220507166483 0.997794928335
0.00220264317181 0.997797356828
0.002200220022 0.997799779978
0.0021978021978 0.997802197802
0.00219538968167 0.997804610318
0.00219298245614 0.997807017544
0.00219058050383 0.997809419496
0.00218818380744 0.997811816193
0.00218579234973 0.99781420765
0.00218340611354 0.997816593886
0.00218102508179 0.997818974918
0.00217864923747 0.997821350763
0.00217627856366 0.997823721436
0.00217391304348 0.997826086957
0.00217155266015 0.99782844734
0.00216919739696 0.997830802603
0.00216684723727 0.997833152763
0.0021645021645 0.997835497835
0.00216216216216 0.997837837838
0.00215982721382 0.997840172786
0.00215749730313 0.997842502697
0.00215517241379 0.997844827586
0.0021528525296 0.99784714747
0.00215053763441 0.997849462366
0.00214822771214 0.997851772288
0.00214592274678 0.997854077253
0.0021436227224 0.997856377278
0.00214132762313 0.997858672377
0.00213903743316 0.997860962567
0.00213675213675 0.997863247863
0.00213447171825 0.997865528282
0.00213219616205 0.997867803838
0.00212992545261 0.997870074547
0.00212765957447 0.997872340426
0.00212539851222 0.997874601488
0.00212314225053 0.997876857749
0.00212089077413 0.997879109226
0.0021186440678 0.997881355932
0.0021164021164 0.997883597884
0.00211416490486 0.997885835095
0.00211193241816 0.997888067582
0.00210970464135 0.997890295359
0.00210748155954 0.99789251844
0.00210526315789 0.997894736842
0.00210304942166 0.997896950578
0.00210084033613 0.997899159664
0.00209863588667 0.997901364113
0.0020964360587 0.997903563941
0.0020942408377 0.997905759162
0.00209205020921 0.997907949791
0.00208986415883 0.997910135841
0.00208768267223 0.997912317328
0.00208550573514 0.997914494265
0.00208333333333 0.997916666667
0.00208116545265 0.997918834547
0.002079002079 0.997920997921
0.00207684319834 0.997923156802
0.00207468879668 0.997925311203
0.0020725388601 0.99792746114
0.00207039337474 0.997929606625
0.00206825232678 0.997931747673
0.00206611570248 0.997933884298
0.00206398348813 0.997936016512
0.0020618556701 0.99793814433
0.00205973223481 0.997940267765
0.00205761316872 0.997942386831
0.00205549845838 0.997944501542
0.00205338809035 0.99794661191
0.00205128205128 0.997948717949
0.00204918032787 0.997950819672
0.00204708290686 0.997952917093
0.00204498977505 0.997955010225
0.00204290091931 0.997957099081
0.00204081632653 0.997959183673
0.00203873598369 0.997961264016
0.0020366598778 0.997963340122
0.00203458799593 0.997965412004
0.0020325203252 0.997967479675
0.00203045685279 0.997969543147
0.00202839756592 0.997971602434
0.00202634245187 0.997973657548
0.00202429149798 0.997975708502
0.00202224469161 0.997977755308
0.0020202020202 0.99797979798
0.00201816347124 0.997981836529
0.00201612903226 0.997983870968
0.00201409869084 0.997985901309
0.00201207243461 0.997987927565
0.00201005025126 0.997989949749
0.00200803212851 0.997991967871
0.00200601805416 0.997993981946
0.00200400801603 0.997995991984
0.002002002002 0.997997997998


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma1.tex <==
0.0 0.212431330344
0.00488 0.212506831159
0.00976 0.212730293452
0.01464 0.213097220759
0.01952 0.213603218529
0.0244 0.214243994385
0.02928 0.21501535823
0.03416 0.215913222196
0.03904 0.216933600442
0.04392 0.218072608804
0.0488 0.219326464296
0.05368 0.220691484482
0.05856 0.222164086705
0.06344 0.223740787195
0.06832 0.225418200055
0.0732 0.227193036133
0.07808 0.229062101789
0.08296 0.231022297557
0.08784 0.233070616729
0.09272 0.235204143837
0.0976 0.237420053077
0.10248 0.239715606649
0.10736 0.24208815305
0.11224 0.244535125302
0.11712 0.247054039144
0.122 0.249642491178
0.12688 0.252298156987
0.13176 0.25501878923
0.13664 0.257802215712
0.14152 0.260646337451
0.1464 0.263549126729
0.15128 0.266508625145
0.15616 0.269522941677
0.16104 0.272590250747
0.16592 0.275708790297
0.1708 0.278876859891
0.17568 0.282092818826
0.18056 0.285355084278
0.18544 0.288662129468
0.19032 0.292012481858
0.1952 0.295404721382
0.20008 0.298837478708
0.20496 0.302309433541
0.20984 0.305819312952
0.21472 0.309365889759
0.2196 0.312947980939
0.22448 0.316564446082
0.22936 0.320214185885
0.23424 0.32389614069
0.23912 0.327609289061
0.244 0.331352646404
0.24888 0.335125263625
0.25376 0.338926225833
0.25864 0.342754651083
0.26352 0.346609689156
0.2684 0.350490520387
0.27328 0.354396354519
0.27816 0.358326429611
0.28304 0.362280010969
0.28792 0.366256390127
0.2928 0.370254883858
0.29768 0.374274833214
0.30256 0.378315602616
0.30744 0.382376578964
0.31232 0.386457170785
0.3172 0.390556807413
0.32208 0.394674938199
0.32696 0.398811031749
0.33184 0.402964575194
0.33672 0.407135073489
0.3416 0.411322048731
0.34648 0.415525039513
0.35136 0.4197436003
0.35624 0.423977300823
0.36112 0.428225725508
0.366 0.432488472918
0.37088 0.436765155221
0.37576 0.441055397678
0.38064 0.445358838153
0.38552 0.449675126639
0.3904 0.454003924805
0.39528 0.458344905565
0.40016 0.462697752652
0.40504 0.467062160224
0.40992 0.471437832475
0.4148 0.475824483265
0.41968 0.480221835765
0.42456 0.484629622118
0.42944 0.489047583107
0.43432 0.493475467844
0.4392 0.497913033467
0.44408 0.502360044849
0.44896 0.50681627432
0.45384 0.511281501399
0.45872 0.515755512537
0.4636 0.520238100872
0.46848 0.524729065987
0.47336 0.529228213688
0.47824 0.533735355781
0.48312 0.538250309863
0.488 0.542772899122
0.49288 0.547302952137
0.49776 0.551840302698
0.50264 0.556384789623
0.50752 0.560936256584
0.5124 0.565494551946
0.51728 0.570059528604
0.52216 0.574631043831
0.52704 0.579208959127
0.53192 0.583793140085
0.5368 0.588383456247
0.54168 0.592979780976
0.54656 0.59758199133
0.55144 0.60218996794
0.55632 0.606803594893
0.5612 0.611422759619
0.56608 0.616047352783
0.57096 0.620677268183
0.57584 0.625312402645
0.58072 0.62995265593
0.5856 0.634597930639
0.59048 0.639248132126
0.59536 0.643903168408
0.60024 0.648562950084
0.60512 0.653227390253
0.61 0.65789640444
0.61488 0.662569910517
0.61976 0.667247828637
0.62464 0.671930081157
0.62952 0.676616592579
0.6344 0.681307289482
0.63928 0.686002100458
0.64416 0.690700956056
0.64904 0.695403788723
0.65392 0.700110532747
0.6588 0.704821124203
0.66368 0.709535500905
0.66856 0.71425360235
0.67344 0.718975369675
0.67832 0.723700745607
0.6832 0.728429674419
0.68808 0.733162101888
0.69296 0.737897975249
0.69784 0.742637243159
0.70272 0.747379855656
0.7076 0.752125764119
0.71248 0.756874921234
0.71736 0.76162728096
0.72224 0.76638279849
0.72712 0.771141430222
0.732 0.775903133727
0.73688 0.780667867716
0.74176 0.785435592012
0.74664 0.790206267519
0.75152 0.794979856197
0.7564 0.799756321034
0.76128 0.804535626019
0.76616 0.809317736118
0.77104 0.814102617247
0.77592 0.818890236254
0.7808 0.82368056089
0.78568 0.828473559792
0.79056 0.833269202456
0.79544 0.838067459223
0.80032 0.842868301255
0.8052 0.847671700514
0.81008 0.852477629749
0.81496 0.857286062472
0.81984 0.862096972945
0.82472 0.86691033616
0.8296 0.871726127824
0.83448 0.876544324343
0.83936 0.881364902806
0.84424 0.88618784097
0.84912 0.891013117249
0.854 0.895840710694
0.85888 0.900670600984
0.86376 0.905502768412
0.86864 0.910337193872
0.87352 0.915173858846
0.8784 0.920012745395
0.88328 0.924853836144
0.88816 0.929697114271
0.89304 0.934542563501
0.89792 0.939390168091
0.9028 0.944239912821
0.90768 0.949091782984
0.91256 0.953945764378
0.91744 0.958801843297
0.92232 0.963660006521
0.9272 0.968520241305
0.93208 0.973382535378
0.93696 0.978246876928
0.94184 0.983113254598
0.94672 0.987981657476
0.9516 0.992852075092
0.95648 0.997724497406
0.96136 1.00259891481
0.96624 1.0074753181
0.97112 1.0123536985
0.976 1.01723404764
0.98088 1.02211635754
0.98576 1.02700062064
0.99064 1.03188682974
0.99552 1.03677497804
1.0004 1.04166505912
1.00528 1.04655706694
1.01016 1.05145099581
1.01504 1.05634684045
1.01992 1.06124459588
1.0248 1.06614425754
1.02968 1.07104582118
1.03456 1.07594928292
1.03944 1.08085463923
1.04432 1.0857618869
1.0492 1.09067102309
1.05408 1.09558204527
1.05896 1.10049495126
1.06384 1.10540973922
1.06872 1.1103264076
1.0736 1.11524495523
1.07848 1.12016538121
1.08336 1.125087685
1.08824 1.13001186635
1.09312 1.13493792535
1.098 1.13986586239
1.10288 1.14479567819
1.10776 1.14972737375
1.11264 1.1546609504
1.11752 1.15959640979
1.1224 1.16453375386
1.12728 1.16947298485
1.13216 1.17441410533
1.13704 1.17935711814
1.14192 1.18430202645
1.1468 1.18924883372
1.15168 1.19419754372
1.15656 1.1991481605
1.16144 1.20410068844
1.16632 1.2090551322
1.1712 1.21401149675
1.17608 1.21896978734
1.18096 1.22393000955
1.18584 1.22889216924
1.19072 1.23385627258
1.1956 1.23882232602
1.20048 1.24379033634
1.20536 1.24876031061
1.21024 1.25373225618
1.21512 1.25870618074
1.22 1.26368209226
1.22488 1.26865999902
1.22976 1.2736399096
1.23464 1.27862183289
1.23952 1.2836057781
1.2444 1.28859175473
1.24928 1.2935797726
1.25416 1.29856984184
1.25904 1.30356197289
1.26392 1.30855617652
1.2688 1.31355246379
1.27368 1.31855084611
1.27856 1.32355133518
1.28344 1.32855394305
1.28832 1.33355868207
1.2932 1.33856556496
1.29808 1.34357460471
1.30296 1.34858581469
1.30784 1.35359920859
1.31272 1.35861480044
1.3176 1.3636326046
1.32248 1.36865263578
1.32736 1.37367490905
1.33224 1.37869943981
1.33712 1.38372624383
1.342 1.38875533723
1.34688 1.39378673649
1.35176 1.39882045845
1.35664 1.40385652032
1.36152 1.40889493969
1.3664 1.41393573453
1.37128 1.41897892317
1.37616 1.42402452433
1.38104 1.42907255713
1.38592 1.43412304108
1.3908 1.43917599609
1.39568 1.44423144246
1.40056 1.44928940091
1.40544 1.45434989256
1.41032 1.45941293898
1.4152 1.46447856212
1.42008 1.46954678439
1.42496 1.47461762863
1.42984 1.47969111811
1.43472 1.48476727657
1.4396 1.48984612816
1.44448 1.49492769754
1.44936 1.5000120098
1.45424 1.50509909053
1.45912 1.51018896577
1.464 1.51528166207
1.46888 1.52037720647
1.47376 1.52547562649
1.47864 1.5305769502
1.48352 1.53568120615
1.4884 1.54078842343
1.49328 1.54589863166
1.49816 1.55101186101
1.50304 1.55612814219
1.50792 1.56124750647
1.5128 1.5663699857
1.51768 1.57149561229
1.52256 1.57662441924
1.52744 1.58175644017
1.53232 1.58689170929
1.5372 1.59203026141
1.54208 1.597172132
1.54696 1.60231735716
1.55184 1.60746597362
1.55672 1.6126180188
1.5616 1.61777353078
1.56648 1.62293254833
1.57136 1.6280951109
1.57624 1.63326125869
1.58112 1.63843103257
1.586 1.6436044742
1.59088 1.64878162597
1.59576 1.65396253101
1.60064 1.65914723327
1.60552 1.66433577747
1.6104 1.66952820914
1.61528 1.67472457465
1.62016 1.6799249212
1.62504 1.68512929685
1.62992 1.69033775053
1.6348 1.69555033207
1.63968 1.7007670922
1.64456 1.70598808258
1.64944 1.71121335583
1.65432 1.71644296553
1.6592 1.72167696623
1.66408 1.7269154135
1.66896 1.73215836394
1.67384 1.7374058752
1.67872 1.74265800598
1.6836 1.7479148161
1.68848 1.7531763665
1.69336 1.75844271922
1.69824 1.76371393751
1.70312 1.7689900858
1.708 1.77427122973
1.71288 1.77955743617
1.71776 1.78484877331
1.72264 1.79014531058
1.72752 1.79544711879
1.7324 1.80075427009
1.73728 1.80606683802
1.74216 1.81138489754
1.74704 1.81670852507
1.75192 1.82203779854
1.7568 1.82737279737
1.76168 1.83271360258
1.76656 1.83806029675
1.77144 1.84341296412
1.77632 1.84877169061
1.7812 1.85413656385
1.78608 1.85950767322
1.79096 1.86488510992
1.79584 1.87026896699
1.80072 1.87565933937
1.8056 1.88105632392
1.81048 1.88646001953
1.81536 1.89187052708
1.82024 1.8972879496
1.82512 1.90271239223
1.83 1.90814396233
1.83488 1.91358276952
1.83976 1.91902892573
1.84464 1.92448254531
1.84952 1.92994374501
1.8544 1.93541264414
1.85928 1.94088936456
1.86416 1.94637403082
1.86904 1.95186677016
1.87392 1.95736771265
1.8788 1.96287699124
1.88368 1.96839474184
1.88856 1.97392110342
1.89344 1.97945621808
1.89832 1.98500023115
1.9032 1.99055329129
1.90808 1.99611555058
1.91296 2.00168716463
1.91784 2.00726829267
1.92272 2.01285909769
1.9276 2.01845974652
1.93248 2.02407040997
1.93736 2.02969126294
1.94224 2.03532248457
1.94712 2.04096425836
1.952 2.0466167723
1.95688 2.05228021902
1.96176 2.05795479598
1.96664 2.06364070555
1.97152 2.06933815525
1.9764 2.07504735788
1.98128 2.0807685317
1.98616 2.08650190063
1.99104 2.09224769445
1.99592 2.09800614897
2.0008 2.1037775063
2.00568 2.109562015
2.01056 2.11535993038
2.01544 2.1211715147
2.02032 2.12699703744
2.0252 2.13283677557
2.03008 2.13869101382
2.03496 2.14456004499
2.03984 2.15044417023
2.04472 2.15634369941
2.0496 2.16225895141
2.05448 2.1681902545
2.05936 2.1741379467
2.06424 2.18010237622
2.06912 2.18608390182
2.074 2.19208289327
2.07888 2.19809973184
2.08376 2.20413481072
2.08864 2.2101885356
2.09352 2.21626132519
2.0984 2.22235361177
2.10328 2.22846584185
2.10816 2.23459847675
2.11304 2.24075199333
2.11792 2.24692688468
2.1228 2.25312366092
2.12768 2.25934284997
2.13256 2.26558499845
2.13744 2.27185067259
2.14232 2.27814045918
2.1472 2.28445496668
2.15208 2.29079482625
2.15696 2.29716069301
2.16184 2.30355324727
2.16672 2.3099731959
2.1716 2.31642127378
2.17648 2.3228982454
2.18136 2.32940490647
2.18624 2.33594208578
2.19112 2.34251064712
2.196 2.34911149136
2.20088 2.35574555873
2.20576 2.36241383127
2.21064 2.36911733542
2.21552 2.37585714493
2.2204 2.38263438396
2.22528 2.38945023045
2.23016 2.39630591981
2.23504 2.40320274894
2.23992 2.41014208063
2.2448 2.41712534835
2.24968 2.42415406158
2.25456 2.43122981158
2.25944 2.43835427782
2.26432 2.44552923508
2.2692 2.45275656128
2.27408 2.46003824619
2.27896 2.46737640117
2.28384 2.47477327001
2.28872 2.48223124107
2.2936 2.48975286094
2.29848 2.49734084987
2.30336 2.50499811922
2.30824 2.51272779125
2.31312 2.52053322174
2.318 2.52841802595
2.32288 2.53638610843
2.32776 2.54444169758
2.33264 2.55258938583
2.33752 2.56083417668
2.3424 2.56918154012
2.34728 2.57763747832
2.35216 2.58620860414
2.35704 2.59490223572
2.36192 2.60372651143
2.3668 2.61269053105
2.37168 2.62180453092
2.37656 2.63108010418
2.38144 2.64053048126
2.38632 2.65017089296
2.3912 2.66001904882
2.39608 2.67009578041
2.40096 2.68042592752
2.40584 2.69103959377
2.41072 2.70197398722
2.4156 2.71327623281
2.42048 2.72500789892
2.42536 2.73725278996
2.43024 2.75013163718
2.43512 2.76383366104


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma1prob0pt1.tex <==
0.0 0.302797401727
0.004276 0.3028391063
0.008552 0.302963191086
0.012828 0.303168122132
0.017104 0.303452385467
0.02138 0.303814487236
0.025656 0.304252953814
0.029932 0.304766331913
0.034208 0.305353188661
0.038484 0.306012111684
0.04276 0.306741709154
0.047036 0.307540609837
0.051312 0.308407463115
0.055588 0.309340939005
0.059864 0.310339728154
0.06414 0.311402541828
0.068416 0.312528111878
0.072692 0.313715190706
0.076968 0.314962551204
0.081244 0.316268986691
0.08552 0.317633310834
0.089796 0.319054357556
0.094072 0.320530980936
0.098348 0.322062055093
0.102624 0.323646474065
0.1069 0.325283151674
0.111176 0.326971021384
0.115452 0.328709036148
0.119728 0.330496168244
0.124004 0.332331409111
0.12828 0.334213769164
0.132556 0.336142277616
0.136832 0.338115982279
0.141108 0.34013394937
0.145384 0.342195263306
0.14966 0.344299026489
0.153936 0.346444359093
0.158212 0.348630398845
0.162488 0.350856300796
0.166764 0.353121237093
0.17104 0.355424396746
0.175316 0.357764985393
0.179592 0.360142225058
0.183868 0.362555353913
0.188144 0.365003626031
0.19242 0.367486311142
0.196696 0.370002694386
0.200972 0.372552076065
0.205248 0.375133771393
0.209524 0.377747110248
0.2138 0.380391436921
0.218076 0.383066109868
0.222352 0.385770501458
0.226628 0.388503997729
0.230904 0.391265998135
0.23518 0.394055915301
0.239456 0.39687317478
0.243732 0.399717214805
0.248008 0.402587486048
0.252284 0.40548345138
0.25656 0.408404585631
0.260836 0.411350375356
0.265112 0.414320318595
0.269388 0.417313924648
0.273664 0.420330713843
0.27794 0.423370217305
0.282216 0.42643197674
0.286492 0.429515544206
0.290768 0.432620481903
0.295044 0.435746361948
0.29932 0.438892766172
0.303596 0.442059285905
0.307872 0.445245521774
0.312148 0.448451083498
0.316424 0.451675589687
0.3207 0.454918667653
0.324976 0.458179953207
0.329252 0.461459090479
0.333528 0.464755731727
0.337804 0.468069537153
0.34208 0.471400174729
0.346356 0.474747320016
0.350632 0.478110655993
0.354908 0.481489872887
0.359184 0.484884668009
0.36346 0.488294745589
0.367736 0.491719816618
0.372012 0.495159598689
0.376288 0.498613815849
0.380564 0.502082198444
0.38484 0.505564482975
0.389116 0.509060411955
0.393392 0.512569733766
0.397668 0.516092202526
0.401944 0.519627577948
0.40622 0.523175625215
0.410496 0.526736114849
0.414772 0.530308822585
0.419048 0.533893529247
0.423324 0.537490020633
0.4276 0.541098087392
0.431876 0.544717524913
0.436152 0.548348133212
0.440428 0.551989716823
0.444704 0.555642084693
0.44898 0.559305050074
0.453256 0.562978430424
0.457532 0.56666204731
0.461808 0.570355726305
0.466084 0.5740592969
0.47036 0.577772592406
0.474636 0.581495449871
0.478912 0.585227709984
0.483188 0.588969216994
0.487464 0.592719818629
0.49174 0.596479366007
0.496016 0.600247713563
0.500292 0.60402471897
0.504568 0.60781024306
0.508844 0.611604149755
0.51312 0.615406305991
0.517396 0.619216581651
0.521672 0.623034849495
0.525948 0.626860985094
0.530224 0.630694866764
0.5345 0.634536375503
0.538776 0.63838539493
0.543052 0.642241811225
0.547328 0.646105513067
0.551604 0.649976391582
0.55588 0.653854340283
0.560156 0.657739255017
0.564432 0.661631033912
0.568708 0.665529577325
0.572984 0.669434787795
0.57726 0.673346569986
0.581536 0.677264830648
0.585812 0.681189478565
0.590088 0.68512042451
0.594364 0.689057581204
0.59864 0.693000863268
0.602916 0.696950187185
0.607192 0.700905471257
0.611468 0.704866635566
0.615744 0.708833601933
0.62002 0.712806293883
0.624296 0.716784636607
0.628572 0.720768556923
0.632848 0.724757983245
0.637124 0.728752845548
0.6414 0.732753075333
0.645676 0.736758605595
0.649952 0.74076937079
0.654228 0.74478530681
0.658504 0.748806350944
0.66278 0.752832441855
0.667056 0.75686351955
0.671332 0.760899525353
0.675608 0.764940401872
0.679884 0.768986092983
0.68416 0.773036543794
0.688436 0.777091700627
0.692712 0.781151510988
0.696988 0.785215923549
0.701264 0.789284888119
0.70554 0.793358355625
0.709816 0.797436278089
0.714092 0.801518608606
0.718368 0.805605301323
0.722644 0.809696311421
0.72692 0.813791595089
0.731196 0.817891109513
0.735472 0.821994812849
0.739748 0.826102664211
0.744024 0.830214623648
0.7483 0.834330652129
0.752576 0.838450711529
0.756852 0.842574764605
0.761128 0.846702774985
0.765404 0.850834707152
0.76968 0.854970526427
0.773956 0.859110198956
0.778232 0.863253691693
0.782508 0.867400972387
0.786784 0.871552009569
0.79106 0.875706772536
0.795336 0.879865231343
0.799612 0.884027356783
0.803888 0.88819312038
0.808164 0.892362494376
0.81244 0.896535451717
0.816716 0.900711966044
0.820992 0.904892011681
0.825268 0.909075563622
0.829544 0.913262597524
0.83382 0.917453089695
0.838096 0.921647017083
0.842372 0.925844357268
0.846648 0.930045088451
0.850924 0.934249189446
0.8552 0.93845663967
0.859476 0.942667419136
0.863752 0.946881508441
0.868028 0.951098888762
0.872304 0.955319541845
0.87658 0.959543449999
0.880856 0.963770596086
0.885132 0.968000963517
0.889408 0.972234536242
0.893684 0.976471298745
0.89796 0.980711236036
0.902236 0.984954333644
0.906512 0.989200577614
0.910788 0.993449954496
0.915064 0.997702451343
0.91934 1.0019580557
0.923616 1.00621675562
0.927892 1.0104785396
0.932168 1.01474339667
0.936444 1.01901131629
0.94072 1.02328228842
0.944996 1.02755630346
0.949272 1.03183335229
0.953548 1.03611342623
0.957824 1.04039651707
0.9621 1.04468261704
0.966376 1.0489717188
0.970652 1.05326381547
0.974928 1.05755890059
0.979204 1.06185696816
0.98348 1.06615801257
0.987756 1.07046202867
0.992032 1.07476901171
0.996308 1.07907895739
1.000584 1.08339186178
1.00486 1.08770772142
1.009136 1.09202653323
1.013412 1.09634829453
1.017688 1.10067300308
1.021964 1.10500065703
1.02624 1.10933125493
1.030516 1.11366479574
1.034792 1.11800127881
1.039068 1.1223407039
1.043344 1.12668307116
1.04762 1.13102838114
1.051896 1.13537663477
1.056172 1.1397278334
1.060448 1.14408197875
1.064724 1.14843907295
1.069 1.1527991185
1.073276 1.1571621183
1.077552 1.16152807564
1.081828 1.16589699421
1.086104 1.17026887806
1.09038 1.17464373166
1.094656 1.17902155985
1.098932 1.18340236786
1.103208 1.18778616131
1.107484 1.19217294622
1.11176 1.19656272899
1.116036 1.2009555164
1.120312 1.20535131563
1.124588 1.20975013427
1.128864 1.21415198026
1.13314 1.21855686197
1.137416 1.22296478814
1.141692 1.22737576793
1.145968 1.23178981088
1.150244 1.23620692692
1.15452 1.24062712639
1.158796 1.24505042004
1.163072 1.24947681901
1.167348 1.25390633484
1.171624 1.25833897949
1.1759 1.26277476533
1.180176 1.26721370513
1.184452 1.27165581207
1.188728 1.27610109977
1.193004 1.28054958223
1.19728 1.28500127392
1.201556 1.28945618969
1.205832 1.29391434485
1.210108 1.29837575511
1.214384 1.30284043664
1.21866 1.30730840603
1.222936 1.31177968032
1.227212 1.316254277
1.231488 1.32073221398
1.235764 1.32521350966
1.24004 1.32969818286
1.244316 1.33418625289
1.248592 1.33867773951
1.252868 1.34317266295
1.257144 1.34767104392
1.26142 1.3521729036
1.265696 1.35667826366
1.269972 1.36118714626
1.274248 1.36569957404
1.278524 1.37021557017
1.2828 1.37473515829
1.287076 1.37925836258
1.291352 1.38378520771
1.295628 1.38831571892
1.299904 1.39284992192
1.30418 1.39738784299
1.308456 1.40192950897
1.312732 1.40647494721
1.317008 1.41102418564
1.321284 1.41557725276
1.32556 1.42013417763
1.329836 1.4246949899
1.334112 1.42925971979
1.338388 1.43382839814
1.342664 1.43840105639
1.34694 1.44297772657
1.351216 1.44755844137
1.355492 1.45214323408
1.359768 1.45673213864
1.364044 1.46132518966
1.36832 1.46592242239
1.372596 1.47052387275
1.376872 1.47512957736
1.381148 1.47973957351
1.385424 1.48435389921
1.3897 1.48897259318
1.393976 1.49359569486
1.398252 1.49822324445
1.402528 1.50285528287
1.406804 1.50749185182
1.41108 1.51213299379
1.415356 1.51677875204
1.419632 1.52142917064
1.423908 1.52608429447
1.428184 1.53074416927
1.43246 1.5354088416
1.436736 1.54007835889
1.441012 1.54475276946
1.445288 1.5494321225
1.449564 1.55411646814
1.45384 1.55880585742
1.458116 1.56350034234
1.462392 1.56819997584
1.466668 1.57290481188
1.470944 1.57761490539
1.47522 1.58233031233
1.479496 1.58705108971
1.483772 1.59177729559
1.488048 1.59650898913
1.492324 1.60124623058
1.4966 1.60598908133
1.500876 1.61073760392
1.505152 1.61549186205
1.509428 1.62025192064
1.513704 1.62501784584
1.51798 1.62978970503
1.522256 1.63456756687
1.526532 1.63935150135
1.530808 1.64414157978
1.535084 1.64893787483
1.53936 1.65374046057
1.543636 1.6585494125
1.547912 1.66336480756
1.552188 1.6681867242
1.556464 1.67301524239
1.56074 1.67785044366
1.565016 1.68269241113
1.569292 1.68754122955
1.573568 1.69239698537
1.577844 1.69725976672
1.58212 1.7021296635
1.586396 1.7070067674
1.590672 1.71189117196
1.594948 1.71678297258
1.599224 1.72168226662
1.6035 1.7265891534
1.607776 1.73150373428
1.612052 1.73642611271
1.616328 1.74135639424
1.620604 1.74629468665
1.62488 1.75124109994
1.629156 1.75619574643
1.633432 1.7611587408
1.637708 1.76613020016
1.641984 1.77111024411
1.64626 1.77609899483
1.650536 1.78109657711
1.654812 1.78610311846
1.659088 1.79111874917
1.663364 1.79614360239
1.66764 1.80117781421
1.671916 1.80622152373
1.676192 1.81127487318
1.680468 1.81633800798
1.684744 1.82141107684
1.68902 1.8264942319
1.693296 1.83158762874
1.697572 1.83669142657
1.701848 1.84180578832
1.706124 1.84693088073
1.7104 1.85206687446
1.714676 1.85721394427
1.718952 1.86237226911
1.723228 1.86754203223
1.727504 1.87272342136
1.73178 1.87791662887
1.736056 1.88312185185
1.740332 1.88833929233
1.744608 1.89356915743
1.748884 1.89881165952
1.75316 1.90406701643
1.757436 1.90933545157
1.761712 1.91461719422
1.765988 1.91991247967
1.770264 1.92522154944
1.77454 1.93054465153
1.778816 1.93588204065
1.783092 1.94123397844
1.787368 1.94660073377
1.791644 1.95198258298
1.79592 1.95737981018
1.800196 1.96279270754
1.804472 1.96822157561
1.808748 1.97366672365
1.813024 1.97912847
1.8173 1.98460714239
1.821576 1.99010307838
1.825852 1.99561662575
1.830128 2.00114814293
1.834404 2.00669799942
1.83868 2.01226657633
1.842956 2.01785426685
1.847232 2.02346147675
1.851508 2.02908862503
1.855784 2.03473614445
1.86006 2.04040448217
1.864336 2.04609410047
1.868612 2.05180547743
1.872888 2.05753910767
1.877164 2.06329550321
1.88144 2.06907519431
1.885716 2.07487873038
1.889992 2.08070668094
1.894268 2.08655963674
1.898544 2.09243821077
1.90282 2.09834303957
1.907096 2.10427478443
1.911372 2.11023413277
1.915648 2.11622179969
1.919924 2.12223852946
1.9242 2.12828509729
1.928476 2.13436231118
1.932752 2.14047101386
1.937028 2.14661208497
1.941304 2.1527864434
1.94558 2.1589950498
1.949856 2.16523890931
1.954132 2.17151907457
1.958408 2.17783664898
1.962684 2.18419279019
1.96696 2.19058871406
1.971236 2.19702569889
1.975512 2.20350509007
1.979788 2.21002830528
1.984064 2.21659684015
1.98834 2.22321227454
1.992616 2.22987627953
1.996892 2.23659062517
2.001168 2.2433571891
2.005444 2.25017796628
2.00972 2.25705507977
2.013996 2.26399079301
2.018272 2.27098752358
2.022548 2.27804785886
2.026824 2.28517457385
2.0311 2.29237065156
2.035376 2.29963930642
2.039652 2.3069840113
2.043928 2.31440852888
2.048204 2.32191694828
2.05248 2.32951372804
2.056756 2.33720374702
2.061032 2.34499236493
2.065308 2.35288549506
2.069584 2.36088969236
2.07386 2.36901226114
2.078136 2.37726138819
2.082412 2.38564630931
2.086688 2.3941775204
2.090964 2.40286704906
2.09524 2.41172881024
2.099516 2.42077908106
2.103792 2.43003714953
2.108068 2.43952622495
2.112344 2.44927475749
2.11662 2.45931842697
2.120896 2.46970328991
2.125172 2.48049107966
2.129448 2.49176890652
2.133724 2.50366921695


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma1prob0pt1pt5prob0pt5.tex <==
0.0 0.212431330344
0.004276 0.212457201831
0.008552 0.212534209276
0.012828 0.212661443745
0.017104 0.212838008132
0.02138 0.21306301719
0.025656 0.213335597555
0.029932 0.213654887758
0.034208 0.214020038238
0.038484 0.214430211347
0.04276 0.214884581346
0.047036 0.215382334397
0.051312 0.21592266855
0.055588 0.21650479372
0.059864 0.217127931664
0.06414 0.217791315947
0.068416 0.218494191906
0.072692 0.219235816606
0.076968 0.220015458792
0.081244 0.220832398836
0.08552 0.22168592868
0.089796 0.222575351769
0.094072 0.223499982986
0.098348 0.224459148576
0.102624 0.225452186074
0.1069 0.226478444217
0.111176 0.227537282865
0.115452 0.228628072905
0.119728 0.229750196164
0.124004 0.230903045305
0.12828 0.232086023735
0.132556 0.233298545496
0.136832 0.234540035158
0.141108 0.235809927713
0.145384 0.237107668461
0.14966 0.238432712897
0.153936 0.239784526592
0.158212 0.241162585074
0.162488 0.242566373709
0.166764 0.243995387576
0.17104 0.245449131347
0.175316 0.246927119152
0.179592 0.248428874463
0.183868 0.249953929955
0.188144 0.251501827387
0.19242 0.253072117461
0.196696 0.2546643597
0.200972 0.256278122312
0.205248 0.257912982058
0.209524 0.259568524122
0.2138 0.261244341975
0.218076 0.262940037249
0.222352 0.264655219595
0.226628 0.266389506562
0.230904 0.268142523455
0.23518 0.269913903211
0.239456 0.271703286264
0.243732 0.273510320416
0.248008 0.275334660707
0.252284 0.277175969286
0.25656 0.279033915284
0.260836 0.280908174687
0.265112 0.282798430209
0.269388 0.284704371166
0.273664 0.286625693355
0.27794 0.288562098929
0.282216 0.290513296279
0.286492 0.292478999908
0.290768 0.294458930319
0.295044 0.296452813892
0.29932 0.298460382772
0.303596 0.300481374753
0.307872 0.302515533167
0.312148 0.304562606767
0.316424 0.306622349624
0.3207 0.308694521015
0.324976 0.310778885317
0.329252 0.312875211903
0.333528 0.314983275035
0.337804 0.317102853767
0.34208 0.319233731842
0.346356 0.321375697593
0.350632 0.323528543847
0.354908 0.325692067831
0.359184 0.327866071076
0.36346 0.330050359326
0.367736 0.332244742448
0.372012 0.334449034343
0.376288 0.336663052859
0.380564 0.338886619705
0.38484 0.341119560369
0.389116 0.343361704033
0.393392 0.345612883494
0.397668 0.347872935085
0.401944 0.350141698596
0.40622 0.352419017201
0.410496 0.354704737379
0.414772 0.356998708846
0.419048 0.359300784479
0.423324 0.36161082025
0.4276 0.363928675153
0.431876 0.366254211143
0.436152 0.368587293062
0.440428 0.370927788583
0.444704 0.373275568142
0.44898 0.375630504878
0.453256 0.377992474571
0.457532 0.380361355586
0.461808 0.382737028813
0.466084 0.385119377611
0.47036 0.387508287755
0.474636 0.389903647377
0.478912 0.392305346918
0.483188 0.394713279075
0.487464 0.39712733875
0.49174 0.399547423001
0.496016 0.401973430992
0.500292 0.404405263951
0.504568 0.406842825117
0.508844 0.409286019701
0.51312 0.411734754838
0.517396 0.414188939547
0.521672 0.416648484687
0.525948 0.419113302917
0.530224 0.421583308654
0.5345 0.424058418036
0.538776 0.426538548885
0.543052 0.429023620666
0.547328 0.431513554451
0.551604 0.434008272888
0.55588 0.436507700159
0.560156 0.439011761953
0.564432 0.441520385427
0.568708 0.444033499177
0.572984 0.446551033207
0.57726 0.449072918893
0.581536 0.451599088959
0.585812 0.454129477444
0.590088 0.456664019674
0.594364 0.459202652232
0.59864 0.461745312935
0.602916 0.464291940802
0.607192 0.466842476032
0.611468 0.469396859974
0.615744 0.471955035108
0.62002 0.474516945014
0.624296 0.477082534352
0.628572 0.47965174884
0.632848 0.482224535227
0.637124 0.484800841274
0.6414 0.487380615731
0.645676 0.489963808315
0.649952 0.492550369693
0.654228 0.495140251457
0.658504 0.497733406109
0.66278 0.500329787036
0.667056 0.502929348496
0.671332 0.5055320456
0.675608 0.508137834288
0.679884 0.51074667132
0.68416 0.51335851425
0.688436 0.515973321418
0.692712 0.518591051926
0.696988 0.521211665627
0.701264 0.523835123108
0.70554 0.526461385673
0.709816 0.529090415331
0.714092 0.531722174781
0.718368 0.534356627395
0.722644 0.536993737206
0.72692 0.539633468897
0.731196 0.542275787783
0.735472 0.544920659801
0.739748 0.547568051496
0.744024 0.550217930011
0.7483 0.552870263071
0.752576 0.555525018976
0.756852 0.558182166585
0.761128 0.560841675308
0.765404 0.563503515091
0.76968 0.566167656412
0.773956 0.568834070263
0.778232 0.571502728144
0.782508 0.574173602052
0.786784 0.576846664473
0.79106 0.579521888367
0.795336 0.582199247166
0.799612 0.584878714758
0.803888 0.587560265483
0.808164 0.590243874122
0.81244 0.592929515888
0.816716 0.595617166418
0.820992 0.598306801767
0.825268 0.600998398396
0.829544 0.603691933167
0.83382 0.606387383336
0.838096 0.609084726543
0.842372 0.611783940804
0.846648 0.614485004509
0.850924 0.617187896409
0.8552 0.619892595614
0.859476 0.62259908158
0.863752 0.625307334112
0.868028 0.628017333347
0.872304 0.630729059756
0.87658 0.633442494134
0.880856 0.636157617593
0.885132 0.638874411558
0.889408 0.641592857764
0.893684 0.644312938244
0.89796 0.647034635327
0.902236 0.649757931634
0.906512 0.652482810071
0.910788 0.655209253822
0.915064 0.657937246348
0.91934 0.660666771379
0.923616 0.66339781291
0.927892 0.666130355197
0.932168 0.668864382751
0.936444 0.671599880335
0.94072 0.674336832958
0.944996 0.677075225871
0.949272 0.679815044564
0.953548 0.682556274762
0.957824 0.685298902416
0.9621 0.688042913707
0.966376 0.690788295036
0.970652 0.693535033023
0.974928 0.6962831145
0.979204 0.699032526512
0.98348 0.70178325631
0.987756 0.70453529135
0.992032 0.707288619286
0.996308 0.710043227969
1.000584 0.712799105445
1.00486 0.715556239948
1.009136 0.718314619901
1.013412 0.721074233908
1.017688 0.723835070757
1.021964 0.72659711941
1.02624 0.729360369008
1.030516 0.732124808861
1.034792 0.734890428449
1.039068 0.737657217418
1.043344 0.740425165578
1.04762 0.7431942629
1.051896 0.745964499513
1.056172 0.748735865703
1.060448 0.751508351907
1.064724 0.754281948715
1.069 0.757056646866
1.073276 0.759832437243
1.077552 0.762609310873
1.081828 0.765387258928
1.086104 0.768166272714
1.09038 0.77094634368
1.094656 0.773727463405
1.098932 0.776509623604
1.103208 0.779292816122
1.107484 0.782077032934
1.11176 0.78486226614
1.116036 0.787648507966
1.120312 0.790435750763
1.124588 0.793223987
1.128864 0.796013209269
1.13314 0.798803410276
1.137416 0.801594582846
1.141692 0.804386719917
1.145968 0.807179814539
1.150244 0.809973859875
1.15452 0.812768849196
1.158796 0.815564775879
1.163072 0.818361633411
1.167348 0.821159415381
1.171624 0.823958115482
1.1759 0.826757727507
1.180176 0.829558245353
1.184452 0.832359663012
1.188728 0.835161974575
1.193004 0.837965174231
1.19728 0.84076925626
1.201556 0.843574215038
1.205832 0.846380045033
1.210108 0.849186740803
1.214384 0.851994296997
1.21866 0.854802708352
1.222936 0.85761196969
1.227212 0.860422075923
1.231488 0.863233022046
1.235764 0.866044803138
1.24004 0.86885741436
1.244316 0.871670850957
1.248592 0.874485108251
1.252868 0.877300181648
1.257144 0.880116066629
1.26142 0.882932758754
1.265696 0.885750253659
1.269972 0.888568547058
1.274248 0.891387634736
1.278524 0.894207512554
1.2828 0.897028176446
1.287076 0.899849622417
1.291352 0.902671846544
1.295628 0.905494844973
1.299904 0.90831861392
1.30418 0.911143149671
1.308456 0.913968448577
1.312732 0.916794507057
1.317008 0.919621321599
1.321284 0.922448888751
1.32556 0.925277205131
1.329836 0.928106267418
1.334112 0.930936072353
1.338388 0.933766616744
1.342664 0.936597897456
1.34694 0.939429911419
1.351216 0.942262655619
1.355492 0.945096127107
1.359768 0.947930322989
1.364044 0.950765240432
1.36832 0.953600876659
1.372596 0.956437228953
1.376872 0.95927429465
1.381148 0.962112071145
1.385424 0.964950555888
1.3897 0.967789746383
1.393976 0.970629640189
1.398252 0.97347023492
1.402528 0.976311528241
1.406804 0.979153517871
1.41108 0.981996201583
1.415356 0.984839577199
1.419632 0.987683642594
1.423908 0.990528395694
1.428184 0.993373834475
1.43246 0.996219956962
1.436736 0.999066761231
1.441012 1.00191424541
1.445288 1.00476240766
1.449564 1.00761124622
1.45384 1.01046075934
1.458116 1.01331094536
1.462392 1.01616180262
1.466668 1.01901332954
1.470944 1.02186552458
1.47522 1.02471838623
1.479496 1.02757191305
1.483772 1.03042610363
1.488048 1.03328095661
1.492324 1.03613647066
1.4966 1.03899264452
1.500876 1.04184947695
1.505152 1.04470696677
1.509428 1.04756511284
1.513704 1.05042391404
1.51798 1.05328336933
1.522256 1.05614347769
1.526532 1.05900423814
1.530808 1.06186564975
1.535084 1.06472771164
1.53936 1.06759042295
1.543636 1.07045378287
1.547912 1.07331779064
1.552188 1.07618244552
1.556464 1.07904774683
1.56074 1.08191369393
1.565016 1.0847802862
1.569292 1.08764752307
1.573568 1.09051540402
1.577844 1.09338392856
1.58212 1.09625309624
1.586396 1.09912290663
1.590672 1.10199335938
1.594948 1.10486445414
1.599224 1.10773619061
1.6035 1.11060856854
1.607776 1.11348158771
1.612052 1.11635524792
1.616328 1.11922954904
1.620604 1.12210449095
1.62488 1.12498007359
1.629156 1.1278562969
1.633432 1.13073316091
1.637708 1.13361066564
1.641984 1.13648881117
1.64626 1.13936759762
1.650536 1.14224702512
1.654812 1.14512709387
1.659088 1.14800780408
1.663364 1.15088915601
1.66764 1.15377114995
1.671916 1.15665378623
1.676192 1.15953706521
1.680468 1.1624209873
1.684744 1.16530555293
1.68902 1.16819076256
1.693296 1.17107661671
1.697572 1.17396311591
1.701848 1.17685026075
1.706124 1.17973805183
1.7104 1.1826264898
1.714676 1.18551557535
1.718952 1.18840530919
1.723228 1.19129569207
1.727504 1.19418672479
1.73178 1.19707840815
1.736056 1.19997074303
1.740332 1.20286373032
1.744608 1.20575737093
1.748884 1.20865166584
1.75316 1.21154661604
1.757436 1.21444222256
1.761712 1.21733848648
1.765988 1.22023540888
1.770264 1.22313299092
1.77454 1.22603123376
1.778816 1.2289301386
1.783092 1.2318297067
1.787368 1.23472993932
1.791644 1.23763083778
1.79592 1.24053240343
1.800196 1.24343463764
1.804472 1.24633754184
1.808748 1.24924111747
1.813024 1.25214536603
1.8173 1.25505028903
1.821576 1.25795588803
1.825852 1.26086216463
1.830128 1.26376912046
1.834404 1.26667675718
1.83868 1.26958507648
1.842956 1.27249408011
1.847232 1.27540376984
1.851508 1.27831414746
1.855784 1.28122521483
1.86006 1.28413697383
1.864336 1.28704942636
1.868612 1.28996257438
1.872888 1.29287641987
1.877164 1.29579096487
1.88144 1.29870621142
1.885716 1.30162216163
1.889992 1.30453881762
1.894268 1.30745618158
1.898544 1.3103742557
1.90282 1.31329304223
1.907096 1.31621254345
1.911372 1.31913276168
1.915648 1.32205369927
1.919924 1.32497535863
1.9242 1.32789774217
1.928476 1.33082085238
1.932752 1.33374469175
1.937028 1.33666926284
1.941304 1.33959456822
1.94558 1.34252061053
1.949856 1.34544739242
1.954132 1.34837491659
1.958408 1.35130318578
1.962684 1.35423220278
1.96696 1.3571619704
1.971236 1.36009249149
1.975512 1.36302376897
1.979788 1.36595580576
1.984064 1.36888860485
1.98834 1.37182216926
1.992616 1.37475650204
1.996892 1.37769160629
2.001168 1.38062748517
2.005444 1.38356414184
2.00972 1.38650157955
2.013996 1.38943980156
2.018272 1.39237881117
2.022548 1.39531861174
2.026824 1.39825920666
2.0311 1.40120059938
2.035376 1.40414279337
2.039652 1.40708579216
2.043928 1.41002959932
2.048204 1.41297421846
2.05248 1.41591965323
2.056756 1.41886590734
2.061032 1.42181298454
2.065308 1.42476088862
2.069584 1.42770962342
2.07386 1.43065919281
2.078136 1.43360960073
2.082412 1.43656085116
2.086688 1.43951294811
2.090964 1.44246589567
2.09524 1.44541969794
2.099516 1.44837435909
2.103792 1.45132988334
2.108068 1.45428627495
2.112344 1.45724353823
2.11662 1.46020167754
2.120896 1.46316069729
2.125172 1.46612060195
2.129448 1.46908139602
2.133724 1.47204308406


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma1pt5.tex <==
0.0 0.302797401727
0.0064 0.302838924999
0.0128 0.302962472597
0.0192 0.303166520526
0.0256 0.3034495646
0.032 0.30381012057
0.0384 0.304246724243
0.0448 0.304757931581
0.0512 0.305342318789
0.0576 0.305998482385
0.064 0.306725039257
0.0704 0.307520626704
0.0768 0.308383902466
0.0832 0.309313544735
0.0896 0.310308252153
0.096 0.311366743803
0.1024 0.312487759176
0.1088 0.313670058135
0.1152 0.314912420859
0.1216 0.316213647777
0.128 0.317572559492
0.1344 0.318987996693
0.1408 0.320458820051
0.1472 0.321983910111
0.1536 0.323562167168
0.16 0.325192511137
0.1664 0.32687388141
0.1728 0.328605236709
0.1792 0.33038555492
0.1856 0.332213832934
0.192 0.334089086466
0.1984 0.336010349874
0.2048 0.337976675968
0.2112 0.339987135816
0.2176 0.34204081854
0.224 0.344136831109
0.2304 0.346274298125
0.2368 0.348452361604
0.2432 0.350670180755
0.2496 0.352926931753
0.256 0.35522180751
0.2624 0.357554017437
0.2688 0.359922787213
0.2752 0.362327358544
0.2816 0.364766988923
0.288 0.367240951384
0.2944 0.369748534262
0.3008 0.372289040947
0.3072 0.374861789634
0.3136 0.37746611308
0.32 0.380101358359
0.3264 0.382766886607
0.3328 0.385462072786
0.3392 0.388186305429
0.3456 0.3909389864
0.352 0.393719530648
0.3584 0.396527365962
0.3648 0.399361932733
0.3712 0.402222683713
0.3776 0.405109083773
0.384 0.408020609671
0.3904 0.410956749817
0.3968 0.413917004039
0.4032 0.416900883354
0.4096 0.419907909741
0.416 0.422937615919
0.4224 0.425989545119
0.4288 0.429063250871
0.4352 0.432158296784
0.4416 0.435274256335
0.448 0.438410712657
0.4544 0.441567258333
0.4608 0.444743495189
0.4672 0.447939034099
0.4736 0.45115349478
0.48 0.454386505606
0.4864 0.457637703407
0.4928 0.46090673329
0.4992 0.464193248447
0.5056 0.467496909982
0.512 0.470817386723
0.5184 0.474154355056
0.5248 0.477507498748
0.5312 0.480876508784
0.5376 0.484261083195
0.544 0.487660926904
0.5504 0.491075751563
0.5568 0.494505275398
0.5632 0.49794922306
0.5696 0.501407325472
0.576 0.504879319689
0.5824 0.508364948749
0.5888 0.511863961539
0.5952 0.515376112654
0.6016 0.518901162266
0.608 0.522438875996
0.6144 0.525989024779
0.6208 0.529551384746
0.6272 0.5331257371
0.6336 0.536711867997
0.64 0.540309568425
0.6464 0.543918634099
0.6528 0.547538865342
0.6592 0.551170066981
0.6656 0.554812048237
0.672 0.558464622628
0.6784 0.562127607859
0.6848 0.565800825731
0.6912 0.56948410204
0.6976 0.573177266488
0.704 0.576880152583
0.7104 0.580592597559
0.7168 0.58431444228
0.7232 0.588045531162
0.7296 0.591785712086
0.736 0.595534836315
0.7424 0.59929275842
0.7488 0.603059336198
0.7552 0.606834430602
0.7616 0.610617905662
0.768 0.614409628415
0.7744 0.618209468838
0.7808 0.622017299776
0.7872 0.62583299688
0.7936 0.629656438538
0.8 0.633487505813
0.8064 0.637326082383
0.8128 0.64117205448
0.8192 0.645025310832
0.8256 0.648885742604
0.832 0.652753243346
0.8384 0.656627708935
0.8448 0.660509037525
0.8512 0.664397129495
0.8576 0.668291887396
0.864 0.672193215907
0.8704 0.676101021783
0.8768 0.68001521381
0.8832 0.683935702762
0.8896 0.687862401353
0.896 0.691795224195
0.9024 0.69573408776
0.9088 0.699678910332
0.9152 0.703629611973
0.9216 0.707586114483
0.928 0.711548341359
0.9344 0.715516217764
0.9408 0.719489670484
0.9472 0.723468627897
0.9536 0.727453019942
0.96 0.731442778077
0.9664 0.735437835255
0.9728 0.739438125889
0.9792 0.743443585818
0.9856 0.747454152284
0.992 0.751469763896
0.9984 0.755490360607
1.0048 0.759515883682
1.0112 0.763546275672
1.0176 0.76758148039
1.024 0.771621442881
1.0304 0.7756661094
1.0368 0.779715427389
1.0432 0.783769345448
1.0496 0.787827813317
1.056 0.791890781848
1.0624 0.795958202991
1.0688 0.800030029763
1.0752 0.804106216234
1.0816 0.808186717503
1.088 0.812271489682
1.0944 0.81636048987
1.1008 0.820453676141
1.1072 0.824551007522
1.1136 0.828652443975
1.12 0.832757946381
1.1264 0.836867476522
1.1328 0.840980997064
1.1392 0.845098471543
1.1456 0.849219864347
1.152 0.853345140699
1.1584 0.857474266649
1.1648 0.86160720905
1.1712 0.865743935552
1.1776 0.869884414584
1.184 0.87402861534
1.1904 0.878176507769
1.1968 0.882328062559
1.2032 0.886483251126
1.2096 0.890642045604
1.216 0.894804418828
1.2224 0.898970344328
1.2288 0.903139796314
1.2352 0.907312749667
1.2416 0.911489179928
1.248 0.915669063287
1.2544 0.919852376575
1.2608 0.924039097251
1.2672 0.928229203395
1.2736 0.932422673698
1.28 0.936619487453
1.2864 0.940819624547
1.2928 0.945023065451
1.2992 0.949229791212
1.3056 0.953439783447
1.312 0.957653024333
1.3184 0.961869496599
1.3248 0.966089183521
1.3312 0.970312068914
1.3376 0.974538137124
1.344 0.97876737302
1.3504 0.982999761993
1.3568 0.987235289944
1.3632 0.991473943278
1.3696 0.995715708904
1.376 0.999960574222
1.3824 1.00420852712
1.3888 1.00845955597
1.3952 1.01271364963
1.4016 1.01697079742
1.408 1.02123098912
1.4144 1.025494215
1.4208 1.02976046576
1.4272 1.03402973257
1.4336 1.03830200705
1.44 1.04257728126
1.4464 1.0468555477
1.4528 1.05113679933
1.4592 1.0554210295
1.4656 1.05970823204
1.472 1.06399840117
1.4784 1.06829153156
1.4848 1.07258761828
1.4912 1.07688665683
1.4976 1.08118864313
1.504 1.08549357351
1.5104 1.0898014447
1.5168 1.09411225384
1.5232 1.09842599849
1.5296 1.1027426766
1.536 1.10706228652
1.5424 1.11138482701
1.5488 1.11571029722
1.5552 1.1200386967
1.5616 1.12437002539
1.568 1.12870428362
1.5744 1.13304147213
1.5808 1.13738159203
1.5872 1.14172464482
1.5936 1.14607063241
1.6 1.15041955707
1.6064 1.15477142148
1.6128 1.1591262287
1.6192 1.16348398216
1.6256 1.16784468569
1.632 1.17220834351
1.6384 1.17657496021
1.6448 1.18094454079
1.6512 1.1853170906
1.6576 1.1896926154
1.664 1.19407112134
1.6704 1.19845261493
1.6768 1.2028371031
1.6832 1.20722459314
1.6896 1.21161509273
1.696 1.21600860997
1.7024 1.2204051533
1.7088 1.2248047316
1.7152 1.22920735412
1.7216 1.23361303048
1.728 1.23802177075
1.7344 1.24243358534
1.7408 1.24684848511
1.7472 1.25126648127
1.7536 1.25568758546
1.76 1.26011180973
1.7664 1.26453916653
1.7728 1.26896966869
1.7792 1.27340332951
1.7856 1.27784016264
1.792 1.28228018218
1.7984 1.28672340266
1.8048 1.291169839
1.8112 1.29561950656
1.8176 1.30007242114
1.824 1.30452859895
1.8304 1.30898805664
1.8368 1.31345081131
1.8432 1.31791688049
1.8496 1.32238628216
1.856 1.32685903474
1.8624 1.33133515712
1.8688 1.33581466864
1.8752 1.3402975891
1.8816 1.34478393877
1.888 1.34927373839
1.8944 1.35376700919
1.9008 1.35826377284
1.9072 1.36276405155
1.9136 1.36726786799
1.92 1.37177524534
1.9264 1.37628620726
1.9328 1.38080077795
1.9392 1.38531898212
1.9456 1.38984084498
1.952 1.39436639228
1.9584 1.39889565031
1.9648 1.40342864589
1.9712 1.4079654064
1.9776 1.41250595977
1.984 1.41705033449
1.9904 1.42159855961
1.9968 1.42615066478
2.0032 1.43070668022
2.0096 1.43526663675
2.016 1.43983056579
2.0224 1.44439849937
2.0288 1.44897047015
2.0352 1.4535465114
2.0416 1.45812665704
2.048 1.46271094165
2.0544 1.46729940044
2.0608 1.47189206932
2.0672 1.47648898485
2.0736 1.48109018429
2.08 1.48569570563
2.0864 1.49030558752
2.0928 1.49491986936
2.0992 1.49953859131
2.1056 1.50416179422
2.112 1.50878951977
2.1184 1.51342181035
2.1248 1.51805870917
2.1312 1.52270026025
2.1376 1.5273465084
2.144 1.53199749927
2.1504 1.53665327937
2.1568 1.54131389603
2.1632 1.5459793975
2.1696 1.55064983288
2.176 1.55532525222
2.1824 1.56000570647
2.1888 1.56469124752
2.1952 1.56938192823
2.2016 1.57407780243
2.208 1.57877892497
2.2144 1.58348535169
2.2208 1.58819713948
2.2272 1.59291434628
2.2336 1.59763703114
2.24 1.60236525417
2.2464 1.60709907664
2.2528 1.61183856093
2.2592 1.61658377063
2.2656 1.6213347705
2.272 1.62609162652
2.2784 1.63085440595
2.2848 1.63562317727
2.2912 1.64039801031
2.2976 1.6451789762
2.304 1.64996614745
2.3104 1.65475959793
2.3168 1.65955940296
2.3232 1.66436563929
2.3296 1.66917838518
2.336 1.67399772038
2.3424 1.6788237262
2.3488 1.68365648557
2.3552 1.688496083
2.3616 1.6933426047
2.368 1.69819613857
2.3744 1.70305677427
2.3808 1.70792460323
2.3872 1.71279971873
2.3936 1.71768221591
2.4 1.72257219183
2.4064 1.72746974556
2.4128 1.73237497815
2.4192 1.73728799273
2.4256 1.74220889457
2.432 1.74713779111
2.4384 1.75207479203
2.4448 1.7570200093
2.4512 1.76197355725
2.4576 1.76693555265
2.464 1.77190611471
2.4704 1.77688536522
2.4768 1.7818734286
2.4832 1.78687043195
2.4896 1.79187650512
2.496 1.79689178085
2.5024 1.80191639476
2.5088 1.80695048552
2.5152 1.81199419487
2.5216 1.81704766776
2.528 1.82211105239
2.5344 1.82718450037
2.5408 1.83226816675
2.5472 1.83736221022
2.5536 1.8424667931
2.56 1.84758208155
2.5664 1.85270824565
2.5728 1.85784545952
2.5792 1.86299390145
2.5856 1.86815375405
2.592 1.87332520435
2.5984 1.87850844401
2.6048 1.88370366938
2.6112 1.88891108174
2.6176 1.89413088743
2.624 1.899363298
2.6304 1.90460853043
2.6368 1.90986680729
2.6432 1.91513835694
2.6496 1.92042341375
2.656 1.92572221827
2.6624 1.93103501752
2.6688 1.93636206515
2.6752 1.94170362176
2.6816 1.9470599551
2.688 1.95243134035
2.6944 1.95781806044
2.7008 1.9632204063
2.7072 1.96863867719
2.7136 1.97407318106
2.72 1.97952423483
2.7264 1.98499216481
2.7328 1.99047730707
2.7392 1.99598000782
2.7456 2.00150062387
2.752 2.00703952305
2.7584 2.01259708471
2.7648 2.0181737002
2.7712 2.0237697734
2.7776 2.02938572131
2.784 2.03502197462
2.7904 2.04067897833
2.7968 2.04635719246
2.8032 2.0520570927
2.8096 2.05777917123
2.816 2.06352393747
2.8224 2.06929191897
2.8288 2.0750836623
2.8352 2.08089973402
2.8416 2.08674072173
2.848 2.09260723517
2.8544 2.09849990741
2.8608 2.10441939612
2.8672 2.11036638493
2.8736 2.11634158489
2.88 2.12234573606
2.8864 2.12837960918
2.8928 2.13444400751
2.8992 2.14053976879
2.9056 2.1466677674
2.912 2.15282891661
2.9184 2.15902417114
2.9248 2.16525452983
2.9312 2.17152103862
2.9376 2.17782479374
2.944 2.18416694526
2.9504 2.19054870092
2.9568 2.19697133031
2.9632 2.20343616953
2.9696 2.2099446263
2.976 2.21649818551
2.9824 2.22309841551
2.9888 2.22974697492
2.9952 2.23644562037
3.0016 2.24319621495
3.008 2.25000073781
3.0144 2.25686129487
3.0208 2.26378013081
3.0272 2.27075964275
3.0336 2.27780239559
3.04 2.28491113965
3.0464 2.29208883067
3.0528 2.29933865288
3.0592 2.3066640456
3.0656 2.31406873402
3.072 2.32155676528
3.0784 2.32913255059
3.0848 2.33680091521
3.0912 2.34456715779
3.0976 2.35243712167
3.104 2.36041728101
3.1104 2.3685148462
3.1168 2.37673789383
3.1232 2.38509552917
3.1296 2.39359809182
3.136 2.40225741992
3.1424 2.41108719547
3.1488 2.42010340443
3.1552 2.42932496378
3.1616 2.43877459912
3.168 2.44848011221
3.1744 2.45847628348
3.1808 2.46880786649
3.1872 2.47953459676
3.1936 2.49074027328


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma1pt5prob0pt05.tex <==
0.0 0.212431330344
0.004276 0.212457201831
0.008552 0.212534209276
0.012828 0.212661443745
0.017104 0.212838008132
0.02138 0.21306301719
0.025656 0.213335597555
0.029932 0.213654887758
0.034208 0.214020038238
0.038484 0.214430211347
0.04276 0.214884581346
0.047036 0.215382334397
0.051312 0.21592266855
0.055588 0.21650479372
0.059864 0.217127931664
0.06414 0.217791315947
0.068416 0.218494191906
0.072692 0.219235816606
0.076968 0.220015458792
0.081244 0.220832398836
0.08552 0.22168592868
0.089796 0.222575351769
0.094072 0.223499982986
0.098348 0.224459148576
0.102624 0.225452186074
0.1069 0.226478444217
0.111176 0.227537282865
0.115452 0.228628072905
0.119728 0.229750196164
0.124004 0.230903045305
0.12828 0.232086023735
0.132556 0.233298545496
0.136832 0.234540035158
0.141108 0.235809927713
0.145384 0.237107668461
0.14966 0.238432712897
0.153936 0.239784526592
0.158212 0.241162585074
0.162488 0.242566373709
0.166764 0.243995387576
0.17104 0.245449131347
0.175316 0.246927119152
0.179592 0.248428874463
0.183868 0.249953929955
0.188144 0.251501827387
0.19242 0.253072117461
0.196696 0.2546643597
0.200972 0.256278122312
0.205248 0.257912982058
0.209524 0.259568524122
0.2138 0.261244341975
0.218076 0.262940037249
0.222352 0.264655219595
0.226628 0.266389506562
0.230904 0.268142523455
0.23518 0.269913903211
0.239456 0.271703286264
0.243732 0.273510320416
0.248008 0.275334660707
0.252284 0.277175969286
0.25656 0.279033915284
0.260836 0.280908174687
0.265112 0.282798430209
0.269388 0.284704371166
0.273664 0.286625693355
0.27794 0.288562098929
0.282216 0.290513296279
0.286492 0.292478999908
0.290768 0.294458930319
0.295044 0.296452813892
0.29932 0.298460382772
0.303596 0.300481374753
0.307872 0.302515533167
0.312148 0.304562606767
0.316424 0.306622349624
0.3207 0.308694521015
0.324976 0.310778885317
0.329252 0.312875211903
0.333528 0.314983275035
0.337804 0.317102853767
0.34208 0.319233731842
0.346356 0.321375697593
0.350632 0.323528543847
0.354908 0.325692067831
0.359184 0.327866071076
0.36346 0.330050359326
0.367736 0.332244742448
0.372012 0.334449034343
0.376288 0.336663052859
0.380564 0.338886619705
0.38484 0.341119560369
0.389116 0.343361704033
0.393392 0.345612883494
0.397668 0.347872935085
0.401944 0.350141698596
0.40622 0.352419017201
0.410496 0.354704737379
0.414772 0.356998708846
0.419048 0.359300784479
0.423324 0.36161082025
0.4276 0.363928675153
0.431876 0.366254211143
0.436152 0.368587293062
0.440428 0.370927788583
0.444704 0.373275568142
0.44898 0.375630504878
0.453256 0.377992474571
0.457532 0.380361355586
0.461808 0.382737028813
0.466084 0.385119377611
0.47036 0.387508287755
0.474636 0.389903647377
0.478912 0.392305346918
0.483188 0.394713279075
0.487464 0.39712733875
0.49174 0.399547423001
0.496016 0.401973430992
0.500292 0.404405263951
0.504568 0.406842825117
0.508844 0.409286019701
0.51312 0.411734754838
0.517396 0.414188939547
0.521672 0.416648484687
0.525948 0.419113302917
0.530224 0.421583308654
0.5345 0.424058418036
0.538776 0.426538548885
0.543052 0.429023620666
0.547328 0.431513554451
0.551604 0.434008272888
0.55588 0.436507700159
0.560156 0.439011761953
0.564432 0.441520385427
0.568708 0.444033499177
0.572984 0.446551033207
0.57726 0.449072918893
0.581536 0.451599088959
0.585812 0.454129477444
0.590088 0.456664019674
0.594364 0.459202652232
0.59864 0.461745312935
0.602916 0.464291940802
0.607192 0.466842476032
0.611468 0.469396859974
0.615744 0.471955035108
0.62002 0.474516945014
0.624296 0.477082534352
0.628572 0.47965174884
0.632848 0.482224535227
0.637124 0.484800841274
0.6414 0.487380615731
0.645676 0.489963808315
0.649952 0.492550369693
0.654228 0.495140251457
0.658504 0.497733406109
0.66278 0.500329787036
0.667056 0.502929348496
0.671332 0.5055320456
0.675608 0.508137834288
0.679884 0.51074667132
0.68416 0.51335851425
0.688436 0.515973321418
0.692712 0.518591051926
0.696988 0.521211665627
0.701264 0.523835123108
0.70554 0.526461385673
0.709816 0.529090415331
0.714092 0.531722174781
0.718368 0.534356627395
0.722644 0.536993737206
0.72692 0.539633468897
0.731196 0.542275787783
0.735472 0.544920659801
0.739748 0.547568051496
0.744024 0.550217930011
0.7483 0.552870263071
0.752576 0.555525018976
0.756852 0.558182166585
0.761128 0.560841675308
0.765404 0.563503515091
0.76968 0.566167656412
0.773956 0.568834070263
0.778232 0.571502728144
0.782508 0.574173602052
0.786784 0.576846664473
0.79106 0.579521888367
0.795336 0.582199247166
0.799612 0.584878714758
0.803888 0.587560265483
0.808164 0.590243874122
0.81244 0.592929515888
0.816716 0.595617166418
0.820992 0.598306801767
0.825268 0.600998398396
0.829544 0.603691933167
0.83382 0.606387383336
0.838096 0.609084726543
0.842372 0.611783940804
0.846648 0.614485004509
0.850924 0.617187896409
0.8552 0.619892595614
0.859476 0.62259908158
0.863752 0.625307334112
0.868028 0.628017333347
0.872304 0.630729059756
0.87658 0.633442494134
0.880856 0.636157617593
0.885132 0.638874411558
0.889408 0.641592857764
0.893684 0.644312938244
0.89796 0.647034635327
0.902236 0.649757931634
0.906512 0.652482810071
0.910788 0.655209253822
0.915064 0.657937246348
0.91934 0.660666771379
0.923616 0.66339781291
0.927892 0.666130355197
0.932168 0.668864382751
0.936444 0.671599880335
0.94072 0.674336832958
0.944996 0.677075225871
0.949272 0.679815044564
0.953548 0.682556274762
0.957824 0.685298902416
0.9621 0.688042913707
0.966376 0.690788295036
0.970652 0.693535033023
0.974928 0.6962831145
0.979204 0.699032526512
0.98348 0.70178325631
0.987756 0.70453529135
0.992032 0.707288619286
0.996308 0.710043227969
1.000584 0.712799105445
1.00486 0.715556239948
1.009136 0.718314619901
1.013412 0.721074233908
1.017688 0.723835070757
1.021964 0.72659711941
1.02624 0.729360369008
1.030516 0.732124808861
1.034792 0.734890428449
1.039068 0.737657217418
1.043344 0.740425165578
1.04762 0.7431942629
1.051896 0.745964499513
1.056172 0.748735865703
1.060448 0.751508351907
1.064724 0.754281948715
1.069 0.757056646866
1.073276 0.759832437243
1.077552 0.762609310873
1.081828 0.765387258928
1.086104 0.768166272714
1.09038 0.77094634368
1.094656 0.773727463405
1.098932 0.776509623604
1.103208 0.779292816122
1.107484 0.782077032934
1.11176 0.78486226614
1.116036 0.787648507966
1.120312 0.790435750763
1.124588 0.793223987
1.128864 0.796013209269
1.13314 0.798803410276
1.137416 0.801594582846
1.141692 0.804386719917
1.145968 0.807179814539
1.150244 0.809973859875
1.15452 0.812768849196
1.158796 0.815564775879
1.163072 0.818361633411
1.167348 0.821159415381
1.171624 0.823958115482
1.1759 0.826757727507
1.180176 0.829558245353
1.184452 0.832359663012
1.188728 0.835161974575
1.193004 0.837965174231
1.19728 0.84076925626
1.201556 0.843574215038
1.205832 0.846380045033
1.210108 0.849186740803
1.214384 0.851994296997
1.21866 0.854802708352
1.222936 0.85761196969
1.227212 0.860422075923
1.231488 0.863233022046
1.235764 0.866044803138
1.24004 0.86885741436
1.244316 0.871670850957
1.248592 0.874485108251
1.252868 0.877300181648
1.257144 0.880116066629
1.26142 0.882932758754
1.265696 0.885750253659
1.269972 0.888568547058
1.274248 0.891387634736
1.278524 0.894207512554
1.2828 0.897028176446
1.287076 0.899849622417
1.291352 0.902671846544
1.295628 0.905494844973
1.299904 0.90831861392
1.30418 0.911143149671
1.308456 0.913968448577
1.312732 0.916794507057
1.317008 0.919621321599
1.321284 0.922448888751
1.32556 0.925277205131
1.329836 0.928106267418
1.334112 0.930936072353
1.338388 0.933766616744
1.342664 0.936597897456
1.34694 0.939429911419
1.351216 0.942262655619
1.355492 0.945096127107
1.359768 0.947930322989
1.364044 0.950765240432
1.36832 0.953600876659
1.372596 0.956437228953
1.376872 0.95927429465
1.381148 0.962112071145
1.385424 0.964950555888
1.3897 0.967789746383
1.393976 0.970629640189
1.398252 0.97347023492
1.402528 0.976311528241
1.406804 0.979153517871
1.41108 0.981996201583
1.415356 0.984839577199
1.419632 0.987683642594
1.423908 0.990528395694
1.428184 0.993373834475
1.43246 0.996219956962
1.436736 0.999066761231
1.441012 1.00191424541
1.445288 1.00476240766
1.449564 1.00761124622
1.45384 1.01046075934
1.458116 1.01331094536
1.462392 1.01616180262
1.466668 1.01901332954
1.470944 1.02186552458
1.47522 1.02471838623
1.479496 1.02757191305
1.483772 1.03042610363
1.488048 1.03328095661
1.492324 1.03613647066
1.4966 1.03899264452
1.500876 1.04184947695
1.505152 1.04470696677
1.509428 1.04756511284
1.513704 1.05042391404
1.51798 1.05328336933
1.522256 1.05614347769
1.526532 1.05900423814
1.530808 1.06186564975
1.535084 1.06472771164
1.53936 1.06759042295
1.543636 1.07045378287
1.547912 1.07331779064
1.552188 1.07618244552
1.556464 1.07904774683
1.56074 1.08191369393
1.565016 1.0847802862
1.569292 1.08764752307
1.573568 1.09051540402
1.577844 1.09338392856
1.58212 1.09625309624
1.586396 1.09912290663
1.590672 1.10199335938
1.594948 1.10486445414
1.599224 1.10773619061
1.6035 1.11060856854
1.607776 1.11348158771
1.612052 1.11635524792
1.616328 1.11922954904
1.620604 1.12210449095
1.62488 1.12498007359
1.629156 1.1278562969
1.633432 1.13073316091
1.637708 1.13361066564
1.641984 1.13648881117
1.64626 1.13936759762
1.650536 1.14224702512
1.654812 1.14512709387
1.659088 1.14800780408
1.663364 1.15088915601
1.66764 1.15377114995
1.671916 1.15665378623
1.676192 1.15953706521
1.680468 1.1624209873
1.684744 1.16530555293
1.68902 1.16819076256
1.693296 1.17107661671
1.697572 1.17396311591
1.701848 1.17685026075
1.706124 1.17973805183
1.7104 1.1826264898
1.714676 1.18551557535
1.718952 1.18840530919
1.723228 1.19129569207
1.727504 1.19418672479
1.73178 1.19707840815
1.736056 1.19997074303
1.740332 1.20286373032
1.744608 1.20575737093
1.748884 1.20865166584
1.75316 1.21154661604
1.757436 1.21444222256
1.761712 1.21733848648
1.765988 1.22023540888
1.770264 1.22313299092
1.77454 1.22603123376
1.778816 1.2289301386
1.783092 1.2318297067
1.787368 1.23472993932
1.791644 1.23763083778
1.79592 1.24053240343
1.800196 1.24343463764
1.804472 1.24633754184
1.808748 1.24924111747
1.813024 1.25214536603
1.8173 1.25505028903
1.821576 1.25795588803
1.825852 1.26086216463
1.830128 1.26376912046
1.834404 1.26667675718
1.83868 1.26958507648
1.842956 1.27249408011
1.847232 1.27540376984
1.851508 1.27831414746
1.855784 1.28122521483
1.86006 1.28413697383
1.864336 1.28704942636
1.868612 1.28996257438
1.872888 1.29287641987
1.877164 1.29579096487
1.88144 1.29870621142
1.885716 1.30162216163
1.889992 1.30453881762
1.894268 1.30745618158
1.898544 1.3103742557
1.90282 1.31329304223
1.907096 1.31621254345
1.911372 1.31913276168
1.915648 1.32205369927
1.919924 1.32497535863
1.9242 1.32789774217
1.928476 1.33082085238
1.932752 1.33374469175
1.937028 1.33666926284
1.941304 1.33959456822
1.94558 1.34252061053
1.949856 1.34544739242
1.954132 1.34837491659
1.958408 1.35130318578
1.962684 1.35423220278
1.96696 1.3571619704
1.971236 1.36009249149
1.975512 1.36302376897
1.979788 1.36595580576
1.984064 1.36888860485
1.98834 1.37182216926
1.992616 1.37475650204
1.996892 1.37769160629
2.001168 1.38062748517
2.005444 1.38356414184
2.00972 1.38650157955
2.013996 1.38943980156
2.018272 1.39237881117
2.022548 1.39531861174
2.026824 1.39825920666
2.0311 1.40120059938
2.035376 1.40414279337
2.039652 1.40708579216
2.043928 1.41002959932
2.048204 1.41297421846
2.05248 1.41591965323
2.056756 1.41886590734
2.061032 1.42181298454
2.065308 1.42476088862
2.069584 1.42770962342
2.07386 1.43065919281
2.078136 1.43360960073
2.082412 1.43656085116
2.086688 1.43951294811
2.090964 1.44246589567
2.09524 1.44541969794
2.099516 1.44837435909
2.103792 1.45132988334
2.108068 1.45428627495
2.112344 1.45724353823
2.11662 1.46020167754
2.120896 1.46316069729
2.125172 1.46612060195
2.129448 1.46908139602
2.133724 1.47204308406


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma2.tex <==
0.0 0.302797401727
0.00853 0.302838892665
0.01706 0.302962344457
0.02559 0.303166234883
0.03412 0.303449061498
0.04265 0.303809341765
0.05118 0.304245613172
0.05971 0.304756433327
0.06824 0.305340380053
0.07677 0.305996051452
0.0853 0.306722065965
0.09383 0.307517062411
0.10236 0.308379700019
0.11089 0.309308658437
0.11942 0.310302637733
0.12795 0.311360358381
0.13648 0.312480561235
0.14501 0.313662007486
0.15354 0.314903478613
0.16207 0.316203776311
0.1706 0.31756172242
0.17913 0.318976158834
0.18766 0.3204459474
0.19619 0.321969969808
0.20472 0.323547127468
0.21325 0.32517634138
0.22178 0.326856551995
0.23031 0.328586719061
0.23884 0.330365821467
0.24737 0.332192857074
0.2559 0.334066842541
0.26443 0.335986813145
0.27296 0.337951822587
0.28149 0.339960942801
0.29002 0.342013263746
0.29855 0.344107893207
0.30708 0.346243956575
0.31561 0.348420596631
0.32414 0.350636973327
0.33267 0.352892263555
0.3412 0.355185660923
0.34973 0.357516375516
0.35826 0.359883633666
0.36679 0.362286677708
0.37532 0.364724765745
0.38385 0.367197171403
0.39238 0.369703183585
0.40091 0.372242106231
0.40944 0.374813258071
0.41797 0.377415972375
0.4265 0.380049596712
0.43503 0.382713492699
0.44356 0.385407035759
0.45209 0.388129614872
0.46062 0.390880632331
0.46915 0.3936595035
0.47768 0.396465656568
0.48621 0.399298532312
0.49474 0.402157583853
0.50327 0.405042276422
0.5118 0.40795208712
0.52033 0.410886504689
0.52886 0.413845029275
0.53739 0.416827172203
0.54592 0.419832455748
0.55445 0.42286041291
0.56298 0.425910587197
0.57151 0.4289825324
0.58004 0.43207581238
0.58857 0.435190000857
0.5971 0.438324681197
0.60563 0.441479446205
0.61416 0.444653897924
0.62269 0.447847647434
0.63122 0.45106031465
0.63975 0.454291528134
0.64828 0.457540924901
0.65681 0.46080815023
0.66534 0.464092857483
0.67387 0.467394707922
0.6824 0.470713370531
0.69093 0.474048521842
0.69946 0.477399845765
0.70799 0.480767033417
0.71652 0.484149782962
0.72505 0.487547799444
0.73358 0.490960794633
0.74211 0.494388486871
0.75064 0.497830600915
0.75917 0.501286867793
0.7677 0.504757024657
0.77623 0.508240814641
0.78476 0.51173798672
0.79329 0.515248295577
0.80182 0.518771501466
0.81035 0.522307370085
0.81888 0.525855672444
0.82741 0.529416184745
0.83594 0.532988688259
0.84447 0.536572969204
0.853 0.540168818633
0.86153 0.543776032315
0.87006 0.547394410631
0.87859 0.551023758459
0.88712 0.554663885071
0.89565 0.558314604029
0.90418 0.561975733087
0.91271 0.565647094085
0.92124 0.56932851286
0.92977 0.573019819151
0.9383 0.576720846503
0.94683 0.580431432182
0.95536 0.584151417085
0.96389 0.587880645656
0.97242 0.591618965803
0.98095 0.595366228818
0.98948 0.599122289295
0.99801 0.602887005054
1.00654 0.606660237069
1.01507 0.610441849388
1.0236 0.614231709069
1.03213 0.618029686104
1.04066 0.621835653355
1.04919 0.625649486486
1.05772 0.629471063898
1.06625 0.633300266666
1.07478 0.63713697848
1.08331 0.64098108558
1.09184 0.644832476703
1.10037 0.648691043022
1.1089 0.652556678093
1.11743 0.656429277798
1.12596 0.660308740298
1.13449 0.664194965972
1.14302 0.668087857378
1.15155 0.671987319194
1.16008 0.675893258178
1.16861 0.679805583117
1.17714 0.683724204784
1.18567 0.687649035892
1.1942 0.691579991052
1.20273 0.695516986733
1.21126 0.699459941218
1.21979 0.703408774564
1.22832 0.707363408568
1.23685 0.711323766722
1.24538 0.715289774183
1.25391 0.719261357733
1.26244 0.723238445744
1.27097 0.727220968146
1.2795 0.731208856392
1.28803 0.735202043427
1.29656 0.739200463655
1.30509 0.743204052908
1.31362 0.747212748418
1.32215 0.751226488786
1.33068 0.755245213954
1.33921 0.759268865177
1.34774 0.763297384996
1.35627 0.767330717212
1.3648 0.77136880686
1.37333 0.775411600184
1.38186 0.779459044613
1.39039 0.783511088734
1.39892 0.787567682275
1.40745 0.791628776078
1.41598 0.795694322075
1.42451 0.799764273272
1.43304 0.803838583725
1.44157 0.807917208519
1.4501 0.812000103751
1.45863 0.816087226506
1.46716 0.820178534843
1.47569 0.824273987773
1.48422 0.828373545243
1.49275 0.832477168118
1.50128 0.836584818164
1.50981 0.840696458032
1.51834 0.844812051239
1.52687 0.848931562157
1.5354 0.853054955993
1.54393 0.857182198778
1.55246 0.861313257349
1.56099 0.865448099338
1.56952 0.869586693155
1.57805 0.873729007976
1.58658 0.877875013731
1.59511 0.882024681089
1.60364 0.886177981449
1.61217 0.890334886924
1.6207 0.89449537033
1.62923 0.898659405176
1.63776 0.902826965653
1.64629 0.906998026622
1.65482 0.911172563602
1.66335 0.915350552765
1.67188 0.919531970917
1.68041 0.923716795498
1.68894 0.927905004567
1.69747 0.932096576793
1.706 0.936291491446
1.71453 0.940489728391
1.72306 0.944691268076
1.73159 0.948896091526
1.74012 0.953104180335
1.74865 0.957315516656
1.75718 0.961530083195
1.76571 0.965747863204
1.77424 0.969968840473
1.78277 0.974192999323
1.7913 0.978420324601
1.79983 0.982650801671
1.80836 0.986884416408
1.81689 0.991121155195
1.82542 0.99536100491
1.83395 0.999603952931
1.84248 1.00384998712
1.85101 1.00809909582
1.85954 1.01235126786
1.86807 1.01660649253
1.8766 1.02086475959
1.88513 1.02512605928
1.89366 1.02939038227
1.90219 1.0336577197
1.91072 1.03792806316
1.91925 1.04220140469
1.92778 1.04647773676
1.93631 1.05075705228
1.94484 1.05503934459
1.95337 1.05932460748
1.9619 1.06361283514
1.97043 1.0679040222
1.97896 1.07219816372
1.98749 1.07649525516
1.99602 1.08079529239
2.00455 1.08509827172
2.01308 1.08940418985
2.02161 1.09371304388
2.03014 1.09802483133
2.03867 1.10233955013
2.0472 1.10665719858
2.05573 1.11097777542
2.06426 1.11530127975
2.07279 1.11962771108
2.08132 1.12395706933
2.08985 1.12828935478
2.09838 1.13262456813
2.10691 1.13696271046
2.11544 1.14130378323
2.12397 1.14564778831
2.1325 1.14999472792
2.14103 1.15434460471
2.14956 1.15869742169
2.15809 1.16305318225
2.16662 1.16741189019
2.17515 1.17177354967
2.18368 1.17613816525
2.19221 1.18050574187
2.20074 1.18487628486
2.20927 1.18924979991
2.2178 1.19362629313
2.22633 1.198005771
2.23486 1.20238824037
2.24339 1.20677370851
2.25192 1.21116218305
2.26045 1.21555367202
2.26898 1.21994818384
2.27751 1.2243457273
2.28604 1.22874631163
2.29457 1.23314994639
2.3031 1.23755664158
2.31163 1.24196640759
2.32016 1.24637925519
2.32869 1.25079519555
2.33722 1.25521424027
2.34575 1.25963640131
2.35428 1.26406169108
2.36281 1.26849012236
2.37134 1.27292170836
2.37987 1.2773564627
2.3884 1.28179439941
2.39693 1.28623553294
2.40546 1.29067987816
2.41399 1.29512745038
2.42252 1.2995782653
2.43105 1.30403233909
2.43958 1.30848968833
2.44811 1.31295033004
2.45664 1.31741428168
2.46517 1.32188156116
2.4737 1.32635218684
2.48223 1.33082617753
2.49076 1.33530355249
2.49929 1.33978433145
2.50782 1.3442685346
2.51635 1.3487561826
2.52488 1.35324729658
2.53341 1.35774189818
2.54194 1.36224000949
2.55047 1.36674165309
2.559 1.37124685209
2.56753 1.37575563008
2.57606 1.38026801114
2.58459 1.3847840199
2.59312 1.38930368148
2.60165 1.39382702155
2.61018 1.39835406629
2.61871 1.40288484243
2.62724 1.40741937725
2.63577 1.41195769857
2.6443 1.4164998348
2.65283 1.42104581487
2.66136 1.42559566833
2.66989 1.4301494253
2.67842 1.43470711648
2.68695 1.43926877318
2.69548 1.44383442733
2.70401 1.44840411145
2.71254 1.45297785872
2.72107 1.45755570293
2.7296 1.46213767852
2.73813 1.46672382061
2.74666 1.47131416496
2.75519 1.47590874802
2.76372 1.4805076069
2.77225 1.48511077946
2.78078 1.48971830422
2.78931 1.49433022045
2.79784 1.49894656814
2.80637 1.50356738803
2.8149 1.50819272162
2.82343 1.51282261118
2.83196 1.51745709975
2.84049 1.5220962312
2.84902 1.52674005017
2.85755 1.53138860217
2.86608 1.53604193351
2.87461 1.54070009139
2.88314 1.54536312386
2.89167 1.55003107987
2.9002 1.55470400927
2.90873 1.55938196282
2.91726 1.56406499224
2.92579 1.56875315019
2.93432 1.57344649032
2.94285 1.57814506725
2.95138 1.58284893664
2.95991 1.58755815518
2.96844 1.59227278059
2.97697 1.59699287168
2.9855 1.60171848837
2.99403 1.60644969168
3.00256 1.61118654378
3.01109 1.61592910801
3.01962 1.62067744889
3.02815 1.62543163217
3.03668 1.63019172482
3.04521 1.63495779509
3.05374 1.63972991254
3.06227 1.64450814803
3.0708 1.64929257378
3.07933 1.6540832634
3.08786 1.6588802919
3.09639 1.66368373575
3.10492 1.66849367289
3.11345 1.67331018277
3.12198 1.67813334638
3.13051 1.68296324632
3.13904 1.68779996677
3.14757 1.69264359359
3.1561 1.69749421435
3.16463 1.70235191832
3.17316 1.70721679659
3.18169 1.71208894204
3.19022 1.71696844943
3.19875 1.72185541544
3.20728 1.72674993871
3.21581 1.73165211988
3.22434 1.73656206166
3.23287 1.74147986886
3.2414 1.74640564849
3.24993 1.75133950976
3.25846 1.75628156416
3.26699 1.76123192555
3.27552 1.76619071015
3.28405 1.77115803671
3.29258 1.77613402647
3.30111 1.78111880329
3.30964 1.78611249371
3.31817 1.79111522704
3.3267 1.79612713539
3.33523 1.80114835379
3.34376 1.80617902028
3.35229 1.81121927596
3.36082 1.8162692651
3.36935 1.82132913523
3.37788 1.82639903725
3.38641 1.8314791255
3.39494 1.83656955789
3.40347 1.841670496
3.412 1.84678210519
3.42053 1.85190455472
3.42906 1.85703801786
3.43759 1.86218267203
3.44612 1.86733869895
3.45465 1.87250628471
3.46318 1.87768562001
3.47171 1.88287690023
3.48024 1.8880803256
3.48877 1.89329610142
3.4973 1.89852443814
3.50583 1.90376555162
3.51436 1.90901966324
3.52289 1.91428700016
3.53142 1.9195677955
3.53995 1.92486228851
3.54848 1.93017072485
3.55701 1.9354933568
3.56554 1.9408304435
3.57407 1.9461822512
3.5826 1.95154905353
3.59113 1.95693113179
3.59966 1.96232877525
3.60819 1.96774228142
3.61672 1.97317195643
3.62525 1.97861811533
3.63378 1.98408108247
3.64231 1.98956119186
3.65084 1.99505878761
3.65937 2.0005742243
3.6679 2.00610786746
3.67643 2.01166009402
3.68496 2.01723129283
3.69349 2.02282186515
3.70202 2.02843222524
3.71055 2.03406280091
3.71908 2.03971403418
3.72761 2.04538638192
3.73614 2.05108031656
3.74467 2.05679632682
3.7532 2.06253491852
3.76173 2.06829661541
3.77026 2.07408196009
3.77879 2.07989151494
3.78732 2.08572586317
3.79585 2.09158560988
3.80438 2.09747138327
3.81291 2.10338383586
3.82144 2.10932364587
3.82997 2.1152915186
3.8385 2.12128818807
3.84703 2.12731441858
3.85556 2.13337100662
3.86409 2.13945878272
3.87262 2.1455786136
3.88115 2.1517314044
3.88968 2.15791810118
3.89821 2.16413969356
3.90674 2.17039721764
3.91527 2.17669175914
3.9238 2.18302445688
3.93233 2.18939650654
3.94086 2.19580916479
3.94939 2.20226375383
3.95792 2.2087616664
3.96645 2.21530437125
3.97498 2.22189341928
3.98351 2.22853045023
3.99204 2.23521720022
4.00057 2.24195551005
4.0091 2.2487473346
4.01763 2.25559475321
4.02616 2.26249998151
4.03469 2.26946538464
4.04322 2.27649349234
4.05175 2.28358701601
4.06028 2.29074886824
4.06881 2.29798218527
4.07734 2.30529035274
4.08587 2.31267703569
4.0944 2.32014621337
4.10293 2.32770222018
4.11146 2.3353497939
4.11999 2.34309413299
4.12852 2.3509409653
4.13705 2.358896631
4.14558 2.36696818371
4.15411 2.37516351512
4.16264 2.38349151024
4.17117 2.39196224345
4.1797 2.40058722963
4.18823 2.40937975111
4.19676 2.41835529169
4.20529 2.42753212527
4.21382 2.43693213509
4.22235 2.44658198918
4.23088 2.45651489019
4.23941 2.46677330155
4.24794 2.47741344742
4.25647 2.48851332698


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt05.tex <==
0.0 0.212431330344
0.008276 0.212485700302
0.016552 0.212646953884
0.024828 0.212912335474
0.033104 0.213279142092
0.04138 0.213744723529
0.049656 0.214306482438
0.057932 0.214961874351
0.066208 0.215708407653
0.074484 0.216543643486
0.08276 0.217465195606
0.091036 0.218470730187
0.099312 0.219557965566
0.107588 0.220724671943
0.115864 0.221968671031
0.12414 0.223287835657
0.132416 0.224680089321
0.140692 0.226143405712
0.148968 0.227675808182
0.157244 0.229275369184
0.16552 0.23094020967
0.173796 0.232668498465
0.182072 0.234458451601
0.190348 0.236308331623
0.198624 0.23821644688
0.2069 0.240181150775
0.215176 0.242200841011
0.223452 0.244273958806
0.231728 0.246398988098
0.240004 0.248574454734
0.24828 0.250798925645
0.256556 0.253071008015
0.264832 0.255389348438
0.273108 0.257752632076
0.281384 0.260159581802
0.28966 0.262608957351
0.297936 0.265099554466
0.306212 0.267630204046
0.314488 0.270199771296
0.322764 0.272807154881
0.33104 0.275451286088
0.339316 0.278131127991
0.347592 0.280845674625
0.355868 0.28359395017
0.364144 0.286375008146
0.37242 0.289187930611
0.380696 0.292031827382
0.388972 0.294905835259
0.397248 0.297809117266
0.405524 0.300740861901
0.4138 0.303700282409
0.422076 0.306686616059
0.430352 0.309699123438
0.438628 0.312737087766
0.446904 0.315799814217
0.45518 0.318886629264
0.463456 0.32199688003
0.471732 0.325129933663
0.480008 0.328285176721
0.488284 0.331462014574
0.49656 0.334659870822
0.504836 0.337878186728
0.513112 0.341116420663
0.521388 0.344374047574
0.529664 0.347650558456
0.53794 0.350945459849
0.546216 0.354258273343
0.554492 0.357588535098
0.562768 0.360935795382
0.571044 0.364299618117
0.57932 0.367679580443
0.587596 0.371075272296
0.595872 0.37448629599
0.604148 0.377912265826
0.612424 0.381352807703
0.6207 0.384807558741
0.628976 0.388276166924
0.637252 0.391758290743
0.645528 0.395253598865
0.653804 0.398761769796
0.66208 0.402282491568
0.670356 0.40581546143
0.678632 0.40936038555
0.686908 0.412916978729
0.695184 0.416484964121
0.70346 0.420064072965
0.711736 0.423654044325
0.720012 0.427254624837
0.728288 0.430865568467
0.736564 0.434486636278
0.74484 0.438117596198
0.753116 0.441758222807
0.761392 0.445408297118
0.769668 0.449067606379
0.777944 0.452735943869
0.78622 0.456413108712
0.794496 0.460098905687
0.802772 0.463793145053
0.811048 0.467495642377
0.819324 0.471206218362
0.8276 0.474924698694
0.835876 0.478650913878
0.844152 0.482384699095
0.852428 0.486125894051
0.860704 0.48987434284
0.86898 0.493629893808
0.877256 0.497392399421
0.885532 0.501161716137
0.893808 0.504937704289
0.902084 0.50872022796
0.91036 0.512509154874
0.918636 0.516304356283
0.926912 0.520105706859
0.935188 0.523913084596
0.943464 0.527726370705
0.95174 0.531545449519
0.960016 0.535370208403
0.968292 0.539200537658
0.976568 0.543036330442
0.984844 0.546877482676
0.99312 0.550723892971
1.001396 0.554575462547
1.009672 0.558432095152
1.017948 0.562293696997
1.026224 0.566160176676
1.0345 0.570031445105
1.042776 0.573907415449
1.051052 0.577788003062
1.059328 0.581673125421
1.067604 0.58556270207
1.07588 0.589456654558
1.084156 0.593354906382
1.092432 0.597257382937
1.100708 0.601164011459
1.108984 0.605074720973
1.11726 0.608989442247
1.125536 0.612908107743
1.133812 0.616830651568
1.142088 0.620757009431
1.150364 0.624687118599
1.15864 0.628620917857
1.166916 0.632558347461
1.175192 0.636499349106
1.183468 0.640443865881
1.191744 0.644391842238
1.20002 0.648343223949
1.208296 0.652297958077
1.216572 0.65625599294
1.224848 0.660217278078
1.233124 0.66418176422
1.2414 0.668149403255
1.249676 0.672120148204
1.257952 0.676093953185
1.266228 0.680070773391
1.274504 0.68405056506
1.28278 0.688033285447
1.291056 0.692018892803
1.299332 0.696007346345
1.307608 0.699998606236
1.315884 0.703992633559
1.32416 0.707989390296
1.332436 0.711988839304
1.340712 0.715990944295
1.348988 0.719995669816
1.357264 0.724002981226
1.36554 0.72801284468
1.373816 0.732025227109
1.382092 0.736040096198
1.390368 0.740057420375
1.398644 0.744077168785
1.40692 0.748099311282
1.415196 0.752123818406
1.423472 0.75615066137
1.431748 0.760179812046
1.440024 0.764211242944
1.4483 0.768244927206
1.456576 0.772280838585
1.464852 0.776318951433
1.473128 0.780359240689
1.481404 0.784401681866
1.48968 0.788446251036
1.497956 0.79249292482
1.506232 0.796541680376
1.514508 0.800592495386
1.522784 0.804645348047
1.53106 0.808700217055
1.539336 0.812757081602
1.547612 0.81681592136
1.555888 0.820876716471
1.564164 0.824939447542
1.57244 0.829004095628
1.580716 0.833070642231
1.588992 0.837139069285
1.597268 0.84120935915
1.605544 0.8452814946
1.61382 0.849355458822
1.622096 0.8534312354
1.630372 0.857508808313
1.638648 0.861588161921
1.646924 0.865669280966
1.6552 0.869752150559
1.663476 0.873836756173
1.671752 0.877923083638
1.680028 0.882011119136
1.688304 0.886100849189
1.69658 0.89019226066
1.704856 0.894285340739
1.713132 0.898380076946
1.721408 0.902476457116
1.729684 0.906574469401
1.73796 0.910674102258
1.746236 0.914775344451
1.754512 0.91887818504
1.762788 0.922982613376
1.771064 0.927088619101
1.77934 0.931196192139
1.787616 0.935305322692
1.795892 0.939416001238
1.804168 0.943528218522
1.812444 0.947641965556
1.82072 0.951757233614
1.828996 0.955874014227
1.837272 0.959992299179
1.845548 0.964112080503
1.853824 0.968233350479
1.8621 0.97235610163
1.870376 0.976480326716
1.878652 0.980606018735
1.886928 0.984733170915
1.895204 0.988861776713
1.90348 0.992991829815
1.911756 0.997123324126
1.920032 1.00125625377
1.928308 1.0053906131
1.936584 1.00952639667
1.94486 1.01366359925
1.953136 1.01780221582
1.961412 1.02194224156
1.969688 1.02608367187
1.977964 1.03022650234
1.98624 1.03437072875
1.994516 1.03851634711
2.002792 1.04266335359
2.011068 1.04681174458
2.019344 1.05096151663
2.02762 1.05511266652
2.035896 1.05926519118
2.044172 1.06341908775
2.052448 1.06757435354
2.060724 1.07173098604
2.069 1.07588898295
2.077276 1.08004834211
2.085552 1.08420906155
2.093828 1.0883711395
2.102104 1.09253457432
2.11038 1.09669936459
2.118656 1.10086550903
2.126932 1.10503300654
2.135208 1.10920185619
2.143484 1.11337205722
2.15176 1.11754360903
2.160036 1.12171651121
2.168312 1.12589076348
2.176588 1.13006636575
2.184864 1.13424331808
2.19314 1.1384216207
2.201416 1.14260127401
2.209692 1.14678227855
2.217968 1.15096463503
2.226244 1.15514834433
2.23452 1.15933340748
2.242796 1.16351982566
2.251072 1.16770760023
2.259348 1.17189673268
2.267624 1.17608722469
2.2759 1.18027907807
2.284176 1.18447229479
2.292452 1.18866687699
2.300728 1.19286282695
2.309004 1.19706014712
2.31728 1.20125884009
2.325556 1.20545890862
2.333832 1.20966035562
2.342108 1.21386318415
2.350384 1.21806739742
2.35866 1.22227299882
2.366936 1.22647999187
2.375212 1.23068838025
2.383488 1.2348981678
2.391764 1.23910935853
2.40004 1.24332195656
2.408316 1.24753596622
2.416592 1.25175139197
2.424868 1.25596823841
2.433144 1.26018651033
2.44142 1.26440621266
2.449696 1.26862735049
2.457972 1.27284992906
2.466248 1.27707395378
2.474524 1.28129943021
2.4828 1.28552636408
2.491076 1.28975476128
2.499352 1.29398462783
2.507628 1.29821596997
2.515904 1.30244879404
2.52418 1.30668310658
2.532456 1.3109189143
2.540732 1.31515622403
2.549008 1.31939504282
2.557284 1.32363537786
2.56556 1.32787723649
2.573836 1.33212062625
2.582112 1.33636555483
2.590388 1.34061203009
2.598664 1.34486006009
2.60694 1.34910965302
2.615216 1.35336081727
2.623492 1.35761356139
2.631768 1.36186789413
2.640044 1.36612382438
2.64832 1.37038136126
2.656596 1.37464051402
2.664872 1.37890129211
2.673148 1.38316370518
2.681424 1.38742776305
2.6897 1.39169347571
2.697976 1.39596085337
2.706252 1.40022990641
2.714528 1.4045006454
2.722804 1.40877308111
2.73108 1.4130472245
2.739356 1.41732308674
2.747632 1.42160067918
2.755908 1.42588001337
2.764184 1.43016110108
2.77246 1.43444395427
2.780736 1.43872858511
2.789012 1.44301500598
2.797288 1.44730322947
2.805564 1.45159326838
2.81384 1.45588513573
2.822116 1.46017884475
2.830392 1.46447440891
2.838668 1.46877184187
2.846944 1.47307115754
2.85522 1.47737237005
2.863496 1.48167549377
2.871772 1.48598054327
2.880048 1.4902875334
2.888324 1.49459647922
2.8966 1.49890739603
2.904876 1.50322029939
2.913152 1.5075352051
2.921428 1.51185212921
2.929704 1.51617108802
2.93798 1.52049209809
2.946256 1.52481517624
2.954532 1.52914033955
2.962808 1.53346760538
2.971084 1.53779699134
2.97936 1.54212851533
2.987636 1.54646219552
2.995912 1.55079805035
3.004188 1.55513609858
3.012464 1.55947635922
3.02074 1.56381885159
3.029016 1.56816359532
3.037292 1.5725106103
3.045568 1.57685991678
3.053844 1.58121153528
3.06212 1.58556548665
3.070396 1.58992179205
3.078672 1.59428047297
3.086948 1.59864155123
3.095224 1.60300504898
3.1035 1.60737098871
3.111776 1.61173939324
3.120052 1.61611028576
3.128328 1.62048368979
3.136604 1.62485962924
3.14488 1.62923812834
3.153156 1.63361921174
3.161432 1.63800290442
3.169708 1.64238923177
3.177984 1.64677821957
3.18626 1.65116989397
3.194536 1.65556428153
3.202812 1.65996140924
3.211088 1.66436130447
3.219364 1.66876399502
3.22764 1.67316950912
3.235916 1.67757787544
3.244192 1.68198912308
3.252468 1.68640328159
3.260744 1.69082038098
3.26902 1.69524045173
3.277296 1.69966352476
3.285572 1.70408963151
3.293848 1.70851880388
3.302124 1.71295107427
3.3104 1.7173864756
3.318676 1.72182504129
3.326952 1.72626680528
3.335228 1.73071180204
3.343504 1.7351600666
3.35178 1.73961163452
3.360056 1.74406654192
3.368332 1.74852482551
3.376608 1.75298652256
3.384884 1.75745167095
3.39316 1.76192030914
3.401436 1.76639247623
3.409712 1.77086821191
3.417988 1.77534755655
3.426264 1.77983055113
3.43454 1.78431723731
3.442816 1.78880765743
3.451092 1.79330185449
3.459368 1.79779987221
3.467644 1.80230175502
3.47592 1.80680754808
3.484196 1.81131729727
3.492472 1.81583104925
3.500748 1.82034885144
3.509024 1.82487075205
3.5173 1.82939680008
3.525576 1.83392704536
3.533852 1.83846153855
3.542128 1.84300033116
3.550404 1.84754347556
3.55868 1.85209102503
3.566956 1.85664303373
3.575232 1.86119955675
3.583508 1.86576065013
3.591784 1.87032637087
3.60006 1.87489677695
3.608336 1.87947192736
3.616612 1.8840518821
3.624888 1.88863670224
3.633164 1.89322644991
3.64144 1.89782118832
3.649716 1.90242098182
3.657992 1.90702589589
3.666268 1.91163599719
3.674544 1.91625135356
3.68282 1.92087203407
3.691096 1.92549810904
3.699372 1.93012965005
3.707648 1.93476673002
3.715924 1.93940942317
3.7242 1.94405780512
3.732476 1.94871195287
3.740752 1.95337194486
3.749028 1.95803786099
3.757304 1.96270978268
3.76558 1.96738779288
3.773856 1.9720719761
3.782132 1.97676241849
3.790408 1.98145920783
3.798684 1.98616243362
3.80696 1.99087218708
3.815236 1.9955885612
3.823512 2.00031165083
3.831788 2.00504155265
3.840064 2.0097783653
3.84834 2.01452218936
3.856616 2.01927312745
3.864892 2.02403128424
3.873168 2.02879676655
3.881444 2.03356968338
3.88972 2.03835014597
3.897996 2.04313826787
3.906272 2.04793416497
3.914548 2.05273795563
3.922824 2.05754976069
3.9311 2.06236970354
3.939376 2.06719791025
3.947652 2.07203450957
3.955928 2.07687963305
3.964204 2.08173341512
3.97248 2.08659599316
3.980756 2.09146750759
3.989032 2.09634810196
3.997308 2.10123792306
4.005584 2.10613712096
4.01386 2.11104584921
4.022136 2.11596426482
4.030412 2.12089252849
4.038688 2.12583080463
4.046964 2.13077926153
4.05524 2.13573807146
4.063516 2.1407074108
4.071792 2.14568746018
4.080068 2.15067840461
4.088344 2.15568043361
4.09662 2.16069374141
4.104896 2.16571852704
4.113172 2.17075499455
4.121448 2.17580335312
4.129724 2.18086381732


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt1.tex <==
0.0 0.605594803453
0.0841218682305 0.613235310435
0.168243736461 0.634361835277
0.252365604692 0.666569449344
0.336487472922 0.707827951057
0.420609341153 0.756455185036
0.504731209383 0.811077930808
0.588853077614 0.87058740455
0.672974945844 0.934094898218
0.757096814075 1.00089109379
0.841218682305 1.07041079889
0.925340550536 1.14220355546
1.00946241877 1.2159097971
1.093584287 1.29124185818
1.17770615523 1.36796902637
1.26182802346 1.44590586331
1.34594989169 1.52490311557
1.43007175992 1.60484065494
1.51419362815 1.68562199873
1.59831549638 1.76717005797
1.68243736461 1.84942384149
1.76655923284 1.93233590749
1.85068110107 2.01587040448
1.9348029693 2.10000158212
2.01892483753 2.18471268268
2.10304670576 2.26999514747
2.18716857399 2.35584809115
2.27129044222 2.44227801205
2.35541231046 2.52929871959
2.43953417869 2.61693147127
2.52365604692 2.70520532317
2.60777791515 2.79415770932
2.69189978338 2.88383527882
2.77602165161 2.97429503606
2.86014351984 3.06560585041
2.94426538807 3.15785043081
3.0283872563 3.25112790156
3.11250912453 3.34555717486
3.19663099276 3.44128140503
3.28075286099 3.5384739467
3.36487472922 3.63734645869
3.44899659745 3.73816015646
3.53311846568 3.8412418354
3.61724033391 3.94700739859
3.70136220214 4.05599772794
3.78548407037 4.16893600065
3.8696059386 4.28682492682
3.95372780684 4.41112533599
4.03784967507 4.54412255633
4.1219715433 4.6898152272


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt3.tex <==
0.0 1.08570849158
0.0608288216233 1.08825086988
0.121657643247 1.0956356355
0.18248646487 1.10751169183
0.243315286493 1.12354569781
0.304144108116 1.14342311879
0.36497292974 1.1668488905
0.425801751363 1.19354772739
0.486630572986 1.22326411521
0.54745939461 1.25576203277
0.608288216233 1.2908244506
0.669117037856 1.32825265423
0.72994585948 1.36786543744
0.790774681103 1.40949820728
0.851603502726 1.45300203818
0.912432324349 1.49824270655
0.973261145973 1.54509973272
1.0340899676 1.59346545139
1.09491878922 1.64324412736
1.15574761084 1.69435112928
1.21657643247 1.74671217083
1.27740525409 1.80026262613
1.33823407571 1.85494692423
1.39906289734 1.91071802632
1.45989171896 1.96753698869
1.52072054058 2.02537261429
1.58154936221 2.08420119664
1.64237818383 2.14400636048
1.70320700545 2.20477900588
1.76403582708 2.2665173648
1.8248646487 2.32922718281
1.88569347032 2.39292204339
1.94652229195 2.45762385887
2.00735111357 2.5233635609
2.06817993519 2.59018203573
2.12900875682 2.65813136692
2.18983757844 2.72727647306
2.25066640006 2.79769726443
2.31149522169 2.86949149729
2.37232404331 2.9427785886
2.43315286493 3.01770478695
2.49398168656 3.09445031383
2.55481050818 3.17323946063
2.6156393298 3.25435528802
2.67646815143 3.33816181825
2.73729697305 3.42513910868
2.79812579467 3.51594204339
2.85895461629 3.61150690545
2.91978343792 3.71326691868
2.98061225954 3.82366697785


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt6.tex <==
0.0 1.63820438154
0.0396220919817 1.63908128563
0.0792441839634 1.64167785387
0.118866275945 1.64594353725
0.158488367927 1.65182877612
0.198110459909 1.65928510572
0.23773255189 1.66826525469
0.277354643872 1.67872323684
0.316976735854 1.69061443623
0.356598827835 1.7038956858
0.396220919817 1.71852533991
0.435843011799 1.73446334133
0.475465103781 1.75167128304
0.515087195762 1.77011246577
0.554709287744 1.78975195175
0.594331379726 1.81055661574
0.633953471707 1.83249519419
0.673575563689 1.85553833357
0.713197655671 1.87965863919
0.752819747653 1.90483072568
0.792441839634 1.93103127066
0.832063931616 1.95823907341
0.871686023598 1.98643512017
0.911308115579 2.01560265855
0.950930207561 2.04572728332
0.990552299543 2.07679703678
1.03017439152 2.10880252714
1.06979648351 2.14173706919
1.10941857549 2.17559685262
1.14904066747 2.21038114423
1.18866275945 2.2460925324
1.22828485143 2.28273722394
1.26790694341 2.32032540663
1.3075290354 2.35887169484
1.34715112738 2.39839568097
1.38677321936 2.43892262372
1.42639531134 2.48048431521
1.46601740332 2.5231201858
1.50563949531 2.56687873004
1.54526158729 2.61181937537
1.58488367927 2.65801497506
1.62450577125 2.70555520467
1.66412786323 2.75455130708
1.70374995521 2.80514292455
1.7433720472 2.85750830585
1.78299413918 2.91188027362
1.82261623116 2.96857271847
1.86223832314 3.02802813457
1.90186041512 3.09091275886
1.9414825071 3.15834132813


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma2pt01.tex <==
0.0 0.605594803453
0.0841218682305 0.613235310435
0.168243736461 0.634361835277
0.252365604692 0.666569449344
0.336487472922 0.707827951057
0.420609341153 0.756455185036
0.504731209383 0.811077930808
0.588853077614 0.87058740455
0.672974945844 0.934094898218
0.757096814075 1.00089109379
0.841218682305 1.07041079889
0.925340550536 1.14220355546
1.00946241877 1.2159097971
1.093584287 1.29124185818
1.17770615523 1.36796902637
1.26182802346 1.44590586331
1.34594989169 1.52490311557
1.43007175992 1.60484065494
1.51419362815 1.68562199873
1.59831549638 1.76717005797
1.68243736461 1.84942384149
1.76655923284 1.93233590749
1.85068110107 2.01587040448
1.9348029693 2.10000158212
2.01892483753 2.18471268268
2.10304670576 2.26999514747
2.18716857399 2.35584809115
2.27129044222 2.44227801205
2.35541231046 2.52929871959
2.43953417869 2.61693147127
2.52365604692 2.70520532317
2.60777791515 2.79415770932
2.69189978338 2.88383527882
2.77602165161 2.97429503606
2.86014351984 3.06560585041
2.94426538807 3.15785043081
3.0283872563 3.25112790156
3.11250912453 3.34555717486
3.19663099276 3.44128140503
3.28075286099 3.5384739467
3.36487472922 3.63734645869
3.44899659745 3.73816015646
3.53311846568 3.8412418354
3.61724033391 3.94700739859
3.70136220214 4.05599772794
3.78548407037 4.16893600065
3.8696059386 4.28682492682
3.95372780684 4.41112533599
4.03784967507 4.54412255633
4.1219715433 4.6898152272


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma4prob0pt3.tex <==
0.0 2.17141698317
0.121657643247 2.17650173976
0.243315286493 2.19127127099
0.36497292974 2.21502338366
0.486630572986 2.24709139562
0.608288216233 2.28684623758
0.72994585948 2.33369778099
0.851603502726 2.38709545478
0.973261145973 2.44652823043
1.09491878922 2.51152406553
1.21657643247 2.58164890119
1.33823407571 2.65650530847
1.45989171896 2.73573087487
1.58154936221 2.81899641457
1.70320700545 2.90600407636
1.8248646487 2.9964854131
1.94652229195 3.09019946544
2.06817993519 3.18693090279
2.18983757844 3.28648825473
2.31149522169 3.38870225856
2.43315286493 3.49342434165
2.55481050818 3.60052525225
2.67646815143 3.70989384846
2.79812579467 3.82143605265
2.91978343792 3.93507397737
3.04144108116 4.05074522858
3.16309872441 4.16840239329
3.28475636766 4.28801272096
3.4064140109 4.40955801176
3.52807165415 4.5330347296
3.6497292974 4.65845436562
3.77138694064 4.78584408678
3.89304458389 4.91524771775
4.01470222714 5.0467271218
4.13635987038 5.18036407146
4.25801751363 5.31626273384
4.37967515688 5.45455294613
4.50133280012 5.59539452886
4.62299044337 5.73898299459
4.74464808662 5.88555717721
4.86630572986 6.0354095739
4.98796337311 6.18890062767
5.10962101636 6.34647892127
5.2312786596 6.50871057604
5.35293630285 6.6763236365
5.4745939461 6.85027821737
5.59625158934 7.03188408677
5.71790923259 7.2230138109
5.83956687584 7.42653383736
5.96122451908 7.6473339557


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt3.tex <==
0.0 4.34283396634
0.243315286493 4.35300347952
0.486630572986 4.38254254198
0.72994585948 4.43004676732
0.973261145973 4.49418279124
1.21657643247 4.57369247516
1.45989171896 4.66739556198
1.70320700545 4.77419090956
1.94652229195 4.89305646085
2.18983757844 5.02304813106
2.43315286493 5.16329780239
2.67646815143 5.31301061694
2.91978343792 5.47146174974
3.16309872441 5.63799282914
3.4064140109 5.81200815273
3.6497292974 5.9929708262
3.89304458389 6.18039893089
4.13635987038 6.37386180558
4.37967515688 6.57297650946
4.62299044337 6.77740451712
4.86630572986 6.98684868331
5.10962101636 7.20105050451
5.35293630285 7.41978769691
5.59625158934 7.6428721053
5.83956687584 7.87014795475
6.08288216233 8.10149045717
6.32619744882 8.33680478657
6.56951273532 8.57602544193
6.81282802181 8.81911602352
7.0561433083 9.0660694592
7.2994585948 9.31690873124
7.54277388129 9.57168817357
7.78608916778 9.83049543549
8.02940445428 10.0934542436
8.27271974077 10.3607281429
8.51603502726 10.6325254677
8.75935031375 10.9091058923
9.00266560025 11.1907890577
9.24598088674 11.4779659892
9.48929617323 11.7711143544
9.73261145973 12.0708191478
9.97592674622 12.3778012553
10.2192420327 12.6929578425
10.4625573192 13.0174211521
10.7058726057 13.352647273
10.9491878922 13.7005564347
11.1925031787 14.0637681735
11.4358184652 14.4460276218
11.6791337517 14.8530676747
11.9224490382 15.2946679114


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt6.tex <==
0.0 6.55281752616
0.158488367927 6.55632514251
0.316976735854 6.5667114155
0.475465103781 6.58377414899
0.633953471707 6.60731510449
0.792441839634 6.63714042289
0.950930207561 6.67306101876
1.10941857549 6.71489294736
1.26790694341 6.76245774493
1.42639531134 6.81558274319
1.58488367927 6.87410135965
1.7433720472 6.93785336531
1.90186041512 7.00668513216
2.06034878305 7.08044986307
2.21883715098 7.15900780699
2.3773255189 7.24222646296
2.53581388683 7.32998077675
2.69430225476 7.42215333429
2.85279062268 7.51863455678
3.01127899061 7.6193229027
3.16976735854 7.72412508263
3.32825572646 7.83295629362
3.48674409439 7.94574048069
3.64523246232 8.06241063421
3.80372083024 8.18290913329
3.96220919817 8.30718814714
4.1206975661 8.43521010855
4.27918593403 8.56694827678
4.43767430195 8.70238741049
4.59616266988 8.84152457693
4.75465103781 8.98437012961
4.91313940573 9.13094889574
5.07162777366 9.28130162652
5.23011614159 9.43548677935
5.38860450951 9.59358272387
5.54709287744 9.75569049486
5.70558124537 9.92193726084
5.86406961329 10.0924807432
6.02255798122 10.2675149202
6.18104634915 10.4472775015
6.33953471707 10.6320599002
6.498023085 10.8222208187
6.65651145293 11.0182052283
6.81499982086 11.2205716982
6.97348818878 11.4300332234
7.13197655671 11.6475210945
7.29046492464 11.8742908739
7.44895329256 12.1121125383
7.60744166049 12.3636510354
7.76593002842 12.6333653125


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt7.tex <==
0.0 7.2741317407
0.132433347565 7.27654448121
0.26486669513 7.28371439829
0.397300042696 7.29554031459
0.529733390261 7.31192292338
0.662166737826 7.33276495201
0.794600085391 7.35797132256
0.927033432956 7.38744930949
1.05946678052 7.42110869487
1.19190012809 7.45886192129
1.32433347565 7.50062424321
1.45676682322 7.54631387722
1.58920017078 7.59585215231
1.72163351835 7.64916366101
1.85406686591 7.70617641277
1.98650021348 7.76682199095
2.11893356104 7.83103571529
2.25136690861 7.89875681174
2.38380025617 7.96992859213
2.51623360374 8.04449864641
2.6486669513 8.12241905066
2.78110029887 8.20364659477
2.91353364643 8.28814303423
3.045966994 8.37587537146
3.17840034157 8.46681617308
3.31083368913 8.56094393085
3.4432670367 8.65824347582
3.57570038426 8.75870645713
3.70813373183 8.8623318999
3.84056707939 8.96912685998
3.97300042696 9.07910719826
4.10543377452 9.19229850326
4.23786712209 9.30873719923
4.37030046965 9.42847188842
4.50273381722 9.55156499178
4.63516716478 9.67809477499
4.76760051235 9.80815787798
4.90003385991 9.94187251297
5.03246720748 10.0793825651
5.16490055504 10.2208629362
5.29733390261 10.3665266386
5.42976725017 10.5166344194
5.56220059774 10.6715081561
5.6946339453 10.8315500793
5.82706729287 10.9972714042
5.95950064043 11.169336996
6.091933988 11.3486392867
6.22436733556 11.5364305719
6.35680068313 11.7345871752
6.4892340307 11.9462321295


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt8.tex <==
0.0 8.03256415469
0.104749805795 8.03409467573
0.20949961159 8.03865676714
0.314249417386 8.04620690425
0.418999223181 8.0567025351
0.523749028976 8.07010213233
0.628498834771 8.08636524743
0.733248640566 8.10545256746
0.837998446361 8.12732597447
0.942748252157 8.1519486077
1.04749805795 8.17928492919
1.15224786375 8.20930079279
1.25699766954 8.24196351731
1.36174747534 8.27724196437
1.46649728113 8.31510662138
1.57124708693 8.35552969073
1.67599689272 8.398485186
1.78074669852 8.44394903626
1.88549650431 8.49189919989
1.99024631011 8.54231578942
2.0949961159 8.5951812092
2.1997459217 8.65048030826
2.30449572749 8.70820055087
2.40924553329 8.768332208
2.51399533908 8.83086857362
2.61874514488 8.89580621048
2.72349495067 8.963145231
2.82824475647 9.0328896206
2.93299456226 9.10504761195
3.03774436806 9.17963212148
3.14249417386 9.2566612618
3.24724397965 9.33615894817
3.35199378545 9.41815562178
3.45674359124 9.5026891202
3.56149339704 9.58980573483
3.66624320283 9.67956150906
3.77099300863 9.77202385052
3.87574281442 9.86727355948
3.98049262022 9.96540741822
4.08524242601 10.0665415516
4.18999223181 10.1708158721
4.2947420376 10.2784000905
4.3994918434 10.3895020555
4.50424164919 10.5043796894
4.60899145499 10.62335872
4.71374126078 10.7468602778
4.81849106658 10.8754464697
4.92324087237 11.0099017872
5.02799067817 11.1513953717
5.13274048396 11.3018629034


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMean.tex <==
0.0 0.302797401727
0.00853 0.302838892665
0.01706 0.302962344457
0.02559 0.303166234883
0.03412 0.303449061498
0.04265 0.303809341765
0.05118 0.304245613172
0.05971 0.304756433327
0.06824 0.305340380053
0.07677 0.305996051452
0.0853 0.306722065965
0.09383 0.307517062411
0.10236 0.308379700019
0.11089 0.309308658437
0.11942 0.310302637733
0.12795 0.311360358381
0.13648 0.312480561235
0.14501 0.313662007486
0.15354 0.314903478613
0.16207 0.316203776311
0.1706 0.31756172242
0.17913 0.318976158834
0.18766 0.3204459474
0.19619 0.321969969808
0.20472 0.323547127468
0.21325 0.32517634138
0.22178 0.326856551995
0.23031 0.328586719061
0.23884 0.330365821467
0.24737 0.332192857074
0.2559 0.334066842541
0.26443 0.335986813145
0.27296 0.337951822587
0.28149 0.339960942801
0.29002 0.342013263746
0.29855 0.344107893207
0.30708 0.346243956575
0.31561 0.348420596631
0.32414 0.350636973327
0.33267 0.352892263555
0.3412 0.355185660923
0.34973 0.357516375516
0.35826 0.359883633666
0.36679 0.362286677708
0.37532 0.364724765745
0.38385 0.367197171403
0.39238 0.369703183585
0.40091 0.372242106231
0.40944 0.374813258071
0.41797 0.377415972375
0.4265 0.380049596712
0.43503 0.382713492699
0.44356 0.385407035759
0.45209 0.388129614872
0.46062 0.390880632331
0.46915 0.3936595035
0.47768 0.396465656568
0.48621 0.399298532312
0.49474 0.402157583853
0.50327 0.405042276422
0.5118 0.40795208712
0.52033 0.410886504689
0.52886 0.413845029275
0.53739 0.416827172203
0.54592 0.419832455748
0.55445 0.42286041291
0.56298 0.425910587197
0.57151 0.4289825324
0.58004 0.43207581238
0.58857 0.435190000857
0.5971 0.438324681197
0.60563 0.441479446205
0.61416 0.444653897924
0.62269 0.447847647434
0.63122 0.45106031465
0.63975 0.454291528134
0.64828 0.457540924901
0.65681 0.46080815023
0.66534 0.464092857483
0.67387 0.467394707922
0.6824 0.470713370531
0.69093 0.474048521842
0.69946 0.477399845765
0.70799 0.480767033417
0.71652 0.484149782962
0.72505 0.487547799444
0.73358 0.490960794633
0.74211 0.494388486871
0.75064 0.497830600915
0.75917 0.501286867793
0.7677 0.504757024657
0.77623 0.508240814641
0.78476 0.51173798672
0.79329 0.515248295577
0.80182 0.518771501466
0.81035 0.522307370085
0.81888 0.525855672444
0.82741 0.529416184745
0.83594 0.532988688259
0.84447 0.536572969204
0.853 0.540168818633
0.86153 0.543776032315
0.87006 0.547394410631
0.87859 0.551023758459
0.88712 0.554663885071
0.89565 0.558314604029
0.90418 0.561975733087
0.91271 0.565647094085
0.92124 0.56932851286
0.92977 0.573019819151
0.9383 0.576720846503
0.94683 0.580431432182
0.95536 0.584151417085
0.96389 0.587880645656
0.97242 0.591618965803
0.98095 0.595366228818
0.98948 0.599122289295
0.99801 0.602887005054
1.00654 0.606660237069
1.01507 0.610441849388
1.0236 0.614231709069
1.03213 0.618029686104
1.04066 0.621835653355
1.04919 0.625649486486
1.05772 0.629471063898
1.06625 0.633300266666
1.07478 0.63713697848
1.08331 0.64098108558
1.09184 0.644832476703
1.10037 0.648691043022
1.1089 0.652556678093
1.11743 0.656429277798
1.12596 0.660308740298
1.13449 0.664194965972
1.14302 0.668087857378
1.15155 0.671987319194
1.16008 0.675893258178
1.16861 0.679805583117
1.17714 0.683724204784
1.18567 0.687649035892
1.1942 0.691579991052
1.20273 0.695516986733
1.21126 0.699459941218
1.21979 0.703408774564
1.22832 0.707363408568
1.23685 0.711323766722
1.24538 0.715289774183
1.25391 0.719261357733
1.26244 0.723238445744
1.27097 0.727220968146
1.2795 0.731208856392
1.28803 0.735202043427
1.29656 0.739200463655
1.30509 0.743204052908
1.31362 0.747212748418
1.32215 0.751226488786
1.33068 0.755245213954
1.33921 0.759268865177
1.34774 0.763297384996
1.35627 0.767330717212
1.3648 0.77136880686
1.37333 0.775411600184
1.38186 0.779459044613
1.39039 0.783511088734
1.39892 0.787567682275
1.40745 0.791628776078
1.41598 0.795694322075
1.42451 0.799764273272
1.43304 0.803838583725
1.44157 0.807917208519
1.4501 0.812000103751
1.45863 0.816087226506
1.46716 0.820178534843
1.47569 0.824273987773
1.48422 0.828373545243
1.49275 0.832477168118
1.50128 0.836584818164
1.50981 0.840696458032
1.51834 0.844812051239
1.52687 0.848931562157
1.5354 0.853054955993
1.54393 0.857182198778
1.55246 0.861313257349
1.56099 0.865448099338
1.56952 0.869586693155
1.57805 0.873729007976
1.58658 0.877875013731
1.59511 0.882024681089
1.60364 0.886177981449
1.61217 0.890334886924
1.6207 0.89449537033
1.62923 0.898659405176
1.63776 0.902826965653
1.64629 0.906998026622
1.65482 0.911172563602
1.66335 0.915350552765
1.67188 0.919531970917
1.68041 0.923716795498
1.68894 0.927905004567
1.69747 0.932096576793
1.706 0.936291491446
1.71453 0.940489728391
1.72306 0.944691268076
1.73159 0.948896091526
1.74012 0.953104180335
1.74865 0.957315516656
1.75718 0.961530083195
1.76571 0.965747863204
1.77424 0.969968840473
1.78277 0.974192999323
1.7913 0.978420324601
1.79983 0.982650801671
1.80836 0.986884416408
1.81689 0.991121155195
1.82542 0.99536100491
1.83395 0.999603952931
1.84248 1.00384998712
1.85101 1.00809909582
1.85954 1.01235126786
1.86807 1.01660649253
1.8766 1.02086475959
1.88513 1.02512605928
1.89366 1.02939038227
1.90219 1.0336577197
1.91072 1.03792806316
1.91925 1.04220140469
1.92778 1.04647773676
1.93631 1.05075705228
1.94484 1.05503934459
1.95337 1.05932460748
1.9619 1.06361283514
1.97043 1.0679040222
1.97896 1.07219816372
1.98749 1.07649525516
1.99602 1.08079529239
2.00455 1.08509827172
2.01308 1.08940418985
2.02161 1.09371304388
2.03014 1.09802483133
2.03867 1.10233955013
2.0472 1.10665719858
2.05573 1.11097777542
2.06426 1.11530127975
2.07279 1.11962771108
2.08132 1.12395706933
2.08985 1.12828935478
2.09838 1.13262456813
2.10691 1.13696271046
2.11544 1.14130378323
2.12397 1.14564778831
2.1325 1.14999472792
2.14103 1.15434460471
2.14956 1.15869742169
2.15809 1.16305318225
2.16662 1.16741189019
2.17515 1.17177354967
2.18368 1.17613816525
2.19221 1.18050574187
2.20074 1.18487628486
2.20927 1.18924979991
2.2178 1.19362629313
2.22633 1.198005771
2.23486 1.20238824037
2.24339 1.20677370851
2.25192 1.21116218305
2.26045 1.21555367202
2.26898 1.21994818384
2.27751 1.2243457273
2.28604 1.22874631163
2.29457 1.23314994639
2.3031 1.23755664158
2.31163 1.24196640759
2.32016 1.24637925519
2.32869 1.25079519555
2.33722 1.25521424027
2.34575 1.25963640131
2.35428 1.26406169108
2.36281 1.26849012236
2.37134 1.27292170836
2.37987 1.2773564627
2.3884 1.28179439941
2.39693 1.28623553294
2.40546 1.29067987816
2.41399 1.29512745038
2.42252 1.2995782653
2.43105 1.30403233909
2.43958 1.30848968833
2.44811 1.31295033004
2.45664 1.31741428168
2.46517 1.32188156116
2.4737 1.32635218684
2.48223 1.33082617753
2.49076 1.33530355249
2.49929 1.33978433145
2.50782 1.3442685346
2.51635 1.3487561826
2.52488 1.35324729658
2.53341 1.35774189818
2.54194 1.36224000949
2.55047 1.36674165309
2.559 1.37124685209
2.56753 1.37575563008
2.57606 1.38026801114
2.58459 1.3847840199
2.59312 1.38930368148
2.60165 1.39382702155
2.61018 1.39835406629
2.61871 1.40288484243
2.62724 1.40741937725
2.63577 1.41195769857
2.6443 1.4164998348
2.65283 1.42104581487
2.66136 1.42559566833
2.66989 1.4301494253
2.67842 1.43470711648
2.68695 1.43926877318
2.69548 1.44383442733
2.70401 1.44840411145
2.71254 1.45297785872
2.72107 1.45755570293
2.7296 1.46213767852
2.73813 1.46672382061
2.74666 1.47131416496
2.75519 1.47590874802
2.76372 1.4805076069
2.77225 1.48511077946
2.78078 1.48971830422
2.78931 1.49433022045
2.79784 1.49894656814
2.80637 1.50356738803
2.8149 1.50819272162
2.82343 1.51282261118
2.83196 1.51745709975
2.84049 1.5220962312
2.84902 1.52674005017
2.85755 1.53138860217
2.86608 1.53604193351
2.87461 1.54070009139
2.88314 1.54536312386
2.89167 1.55003107987
2.9002 1.55470400927
2.90873 1.55938196282
2.91726 1.56406499224
2.92579 1.56875315019
2.93432 1.57344649032
2.94285 1.57814506725
2.95138 1.58284893664
2.95991 1.58755815518
2.96844 1.59227278059
2.97697 1.59699287168
2.9855 1.60171848837
2.99403 1.60644969168
3.00256 1.61118654378
3.01109 1.61592910801
3.01962 1.62067744889
3.02815 1.62543163217
3.03668 1.63019172482
3.04521 1.63495779509
3.05374 1.63972991254
3.06227 1.64450814803
3.0708 1.64929257378
3.07933 1.6540832634
3.08786 1.6588802919
3.09639 1.66368373575
3.10492 1.66849367289
3.11345 1.67331018277
3.12198 1.67813334638
3.13051 1.68296324632
3.13904 1.68779996677
3.14757 1.69264359359
3.1561 1.69749421435
3.16463 1.70235191832
3.17316 1.70721679659
3.18169 1.71208894204
3.19022 1.71696844943
3.19875 1.72185541544
3.20728 1.72674993871
3.21581 1.73165211988
3.22434 1.73656206166
3.23287 1.74147986886
3.2414 1.74640564849
3.24993 1.75133950976
3.25846 1.75628156416
3.26699 1.76123192555
3.27552 1.76619071015
3.28405 1.77115803671
3.29258 1.77613402647
3.30111 1.78111880329
3.30964 1.78611249371
3.31817 1.79111522704
3.3267 1.79612713539
3.33523 1.80114835379
3.34376 1.80617902028
3.35229 1.81121927596
3.36082 1.8162692651
3.36935 1.82132913523
3.37788 1.82639903725
3.38641 1.8314791255
3.39494 1.83656955789
3.40347 1.841670496
3.412 1.84678210519
3.42053 1.85190455472
3.42906 1.85703801786
3.43759 1.86218267203
3.44612 1.86733869895
3.45465 1.87250628471
3.46318 1.87768562001
3.47171 1.88287690023
3.48024 1.8880803256
3.48877 1.89329610142
3.4973 1.89852443814
3.50583 1.90376555162
3.51436 1.90901966324
3.52289 1.91428700016
3.53142 1.9195677955
3.53995 1.92486228851
3.54848 1.93017072485
3.55701 1.9354933568
3.56554 1.9408304435
3.57407 1.9461822512
3.5826 1.95154905353
3.59113 1.95693113179
3.59966 1.96232877525
3.60819 1.96774228142
3.61672 1.97317195643
3.62525 1.97861811533
3.63378 1.98408108247
3.64231 1.98956119186
3.65084 1.99505878761
3.65937 2.0005742243
3.6679 2.00610786746
3.67643 2.01166009402
3.68496 2.01723129283
3.69349 2.02282186515
3.70202 2.02843222524
3.71055 2.03406280091
3.71908 2.03971403418
3.72761 2.04538638192
3.73614 2.05108031656
3.74467 2.05679632682
3.7532 2.06253491852
3.76173 2.06829661541
3.77026 2.07408196009
3.77879 2.07989151494
3.78732 2.08572586317
3.79585 2.09158560988
3.80438 2.09747138327
3.81291 2.10338383586
3.82144 2.10932364587
3.82997 2.1152915186
3.8385 2.12128818807
3.84703 2.12731441858
3.85556 2.13337100662
3.86409 2.13945878272
3.87262 2.1455786136
3.88115 2.1517314044
3.88968 2.15791810118
3.89821 2.16413969356
3.90674 2.17039721764
3.91527 2.17669175914
3.9238 2.18302445688
3.93233 2.18939650654
3.94086 2.19580916479
3.94939 2.20226375383
3.95792 2.2087616664
3.96645 2.21530437125
3.97498 2.22189341928
3.98351 2.22853045023
3.99204 2.23521720022
4.00057 2.24195551005
4.0091 2.2487473346
4.01763 2.25559475321
4.02616 2.26249998151
4.03469 2.26946538464
4.04322 2.27649349234
4.05175 2.28358701601
4.06028 2.29074886824
4.06881 2.29798218527
4.07734 2.30529035274
4.08587 2.31267703569
4.0944 2.32014621337
4.10293 2.32770222018
4.11146 2.3353497939
4.11999 2.34309413299
4.12852 2.3509409653
4.13705 2.358896631
4.14558 2.36696818371
4.15411 2.37516351512
4.16264 2.38349151024
4.17117 2.39196224345
4.1797 2.40058722963
4.18823 2.40937975111
4.19676 2.41835529169
4.20529 2.42753212527
4.21382 2.43693213509
4.22235 2.44658198918
4.23088 2.45651489019
4.23941 2.46677330155
4.24794 2.47741344742
4.25647 2.48851332698


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1.tex <==
0.0 0.23451626127
0.00488 0.234567541235
0.00976 0.23474276739
0.01464 0.234992242008
0.01952 0.235329247628
0.0244 0.235766127298
0.02928 0.236314681523
0.03416 0.236953280993
0.03904 0.237659176776
0.04392 0.238476341162
0.0488 0.239382015299
0.05368 0.240352571364
0.05856 0.24143406032
0.06344 0.242604062975
0.06832 0.243875958703
0.0732 0.245190726867
0.07808 0.24663709355
0.08296 0.248157560755
0.08784 0.249730573232
0.09272 0.251414128952
0.0976 0.253190590188
0.10248 0.25504213292
0.10736 0.256950674281
0.11224 0.258941668008
0.11712 0.261044483212
0.122 0.263200737445
0.12688 0.26539470928
0.13176 0.267707469761
0.13664 0.270080809563
0.14152 0.272502642126
0.1464 0.27501350327
0.15128 0.277605783396
0.15616 0.280272228613
0.16104 0.282948682417
0.16592 0.285741412103
0.1708 0.288527891352
0.17568 0.291421800181
0.18056 0.294358701078
0.18544 0.297399780254
0.19032 0.300409630976
0.1952 0.303518697528
0.20008 0.306656879739
0.20496 0.309895701567
0.20984 0.313162013977
0.21472 0.316453576915
0.2196 0.319768623142
0.22448 0.323190531462
0.22936 0.326551874631
0.23424 0.330024541029
0.23912 0.333524453525
0.244 0.337052771289
0.24888 0.340709973832
0.25376 0.344304092779
0.25864 0.347933907554
0.26352 0.351603140091
0.2684 0.355316212204
0.27328 0.359078269757
0.27816 0.362895206912
0.28304 0.366651595407
0.28792 0.370469571743
0.2928 0.374357131213
0.29768 0.378189596996
0.30256 0.382102179952
0.30744 0.386105170073
0.31232 0.39006395455
0.3172 0.393977763149
0.32208 0.398000675967
0.32696 0.402146129151
0.33184 0.406101319441
0.33672 0.410190073439
0.3416 0.414255092519
0.34648 0.418476554819
0.35136 0.422505932574
0.35624 0.426707562517
0.36112 0.430907159969
0.366 0.435108959141
0.37088 0.439317672055
0.37576 0.443538499571
0.38064 0.447777142149
0.38552 0.451818536679
0.3904 0.456106064359
0.39528 0.460431497823
0.40016 0.464802637604
0.40504 0.468982299762
0.40992 0.473464111836
0.4148 0.477759907302
0.41968 0.482124926906
0.42456 0.486297855331
0.42944 0.49082597386
0.43432 0.495170515425
0.4392 0.499614814985
0.44408 0.503871702436
0.44896 0.508239111879
0.45384 0.512730271282
0.45872 0.517359035462
0.4636 0.521810619015
0.46848 0.526076949851
0.47336 0.530494747333
0.47824 0.535079718674
0.48312 0.539487322303
0.488 0.544079066469
0.49288 0.548494851529
0.49776 0.553113196393
0.50264 0.557557987725
0.50752 0.562225234235
0.5124 0.566722351744
0.51728 0.571042570112
0.52216 0.575608851565
0.52704 0.580002872981
0.53192 0.58466627477
0.5368 0.589163118325
0.54168 0.593954193188
0.54656 0.598585486469
0.55144 0.603051111163
0.55632 0.607841283009
0.5612 0.612473848343
0.56608 0.616943224632
0.57096 0.621243820215
0.57584 0.625906588551
0.58072 0.630957098724
0.5856 0.635306695126
0.59048 0.640054716618
0.59536 0.644649277237
0.60024 0.649085433683
0.60512 0.65395880838
0.61 0.65868600366
0.61488 0.663262409231
0.61976 0.667683418623
0.62464 0.672589855656
0.62952 0.677354665742
0.6344 0.681973580121
0.63928 0.686442337605
0.64416 0.691448666492
0.64904 0.695616262957
0.65392 0.700336960451
0.6588 0.70564284535
0.66368 0.710086261359
0.66856 0.714379198432
0.67344 0.719282660988
0.67832 0.724052904995
0.6832 0.728686379476
0.68808 0.733982197413
0.69296 0.73834432057
0.69784 0.743387509917
0.70272 0.747464640695
0.7076 0.752241997747
0.71248 0.756888102661
0.71736 0.762280497125
0.72224 0.766667961567
0.72712 0.771822267259
0.732 0.775938953407
0.73688 0.780843450101
0.74176 0.785625522444
0.74664 0.790282380315
0.75152 0.794811253342
0.7564 0.800198983842
0.76128 0.804477631474
0.76616 0.809637794845
0.77104 0.814687422476
0.77592 0.819624073641
0.7808 0.824445327159
0.78568 0.829148782182
0.79056 0.833732058974
0.79544 0.838192799682
0.80032 0.842528669105
0.8052 0.847869863037
0.81008 0.853110900814
0.81496 0.857087823293
0.81984 0.862107551696
0.82472 0.867020883691
0.8296 0.87182580042
0.83448 0.876520304328
0.83936 0.881102419774
0.84424 0.886821551699
0.84912 0.891188149622
0.854 0.895436617409
0.85888 0.900861852294
0.86376 0.906195676119
0.86864 0.910109103926
0.87352 0.915239696268
0.8784 0.920273778917
0.88328 0.925209706558
0.88816 0.930045854436
0.89304 0.934780618816
0.89792 0.939412417439
0.9028 0.943939689971
0.90768 0.949811657019
0.91256 0.954140859346
0.91744 0.958361015202
0.92232 0.963968197045
0.9272 0.967981515209
0.93208 0.973410305399
0.93696 0.978755679868
0.94184 0.982456118863
0.94672 0.987614999415
0.9516 0.992686525476
0.95648 0.99766942699
0.96136 1.00256245303
0.96624 1.00736437211
0.97112 1.01207397249
0.976 1.01669006249
0.98088 1.02289746833
0.98576 1.02733878195
0.99064 1.0316831297
0.99552 1.03592940104
1.0004 1.04182541591
1.00528 1.04588800055
1.01016 1.051629606
1.01504 1.05550427342
1.01992 1.06108726659
1.0248 1.06659724353
1.02968 1.07019026193
1.03456 1.07553556965
1.03944 1.08080488156
1.04432 1.08599723009
1.0492 1.09111166374
1.05408 1.09614724726
1.05896 1.10110306181
1.06384 1.1059782052
1.06872 1.11077179203
1.0736 1.11548295389
1.07848 1.12011083951
1.08336 1.12465461491
1.08824 1.12911346362
1.09312 1.13552999819
1.098 1.13983176766
1.10288 1.14404621937
1.10776 1.1502613166
1.11264 1.15431391345
1.11752 1.16039560144
1.1224 1.16428328356
1.12728 1.17022834649
1.13216 1.17394817972
1.13704 1.17975351368
1.14192 1.18330269158
1.1468 1.18896530661
1.15168 1.19456273033
1.15656 1.19785817431
1.16144 1.20330854258
1.16632 1.20869151072
1.1712 1.21400634461
1.17608 1.21925232254
1.18096 1.22442873532
1.18584 1.22953488636
1.19072 1.23457009181
1.1956 1.23953368062
1.20048 1.24442499466
1.20536 1.24924338881
1.21024 1.25398823103
1.21512 1.25865890245
1.22 1.26325479749
1.22488 1.26777532387
1.22976 1.27221990272
1.23464 1.27904423004
1.23952 1.28334823694
1.2444 1.2875745416
1.24928 1.29421757647
1.25416 1.29829961489
1.25904 1.30230230988
1.26392 1.3087579081
1.2688 1.31261285736
1.27368 1.31894431282
1.27856 1.32264924494
1.28344 1.32885389522
1.28832 1.33240663297
1.2932 1.3384818985
1.29808 1.34188035982
1.30296 1.3478237451
1.30784 1.35370600761
1.31272 1.35687503873
1.3176 1.36262171677
1.32248 1.36830528486
1.32736 1.37392505866
1.33224 1.37948036285
1.33712 1.38226430073
1.342 1.38767809401
1.34688 1.39302557636
1.35176 1.39830611063
1.35664 1.40351906912
1.36152 1.40866383358
1.3664 1.41373979536
1.37128 1.4187463554
1.37616 1.42368292438
1.38104 1.42854892272
1.38592 1.43334378068
1.3908 1.43806693841
1.39568 1.44271784597
1.40056 1.44729596347
1.40544 1.45464291764
1.41032 1.4590825376
1.4152 1.46344766307
1.42008 1.46773779368
1.42496 1.47482834214
1.42984 1.47897509842
1.43472 1.48304527147
1.4396 1.48993805531
1.44448 1.49386131826
1.44936 1.50062122421
1.45424 1.50439521278
1.45912 1.5080901164
1.464 1.5146417296
1.46888 1.51818410652
1.47376 1.5245957872
1.47864 1.53093972186
1.48352 1.5342524502
1.4884 1.54045218121
1.49328 1.54360693152
1.49816 1.54965980503
1.50304 1.55564114145
1.50792 1.56155014471
1.5128 1.56438850538
1.51768 1.57014524247
1.52256 1.5758274713
1.52744 1.58143443081
1.53232 1.58696536878
1.5372 1.59241954192
1.54208 1.59476962755
1.54696 1.60006380982
1.55184 1.60527921644
1.55672 1.61041514108
1.5616 1.61547088677
1.56648 1.62044576591
1.57136 1.62838881878
1.57624 1.63320321513
1.58112 1.63793457281
1.586 1.64258224228
1.59088 1.64714558376
1.59576 1.65162396728
1.60064 1.65908360889
1.60552 1.66339249888
1.6104 1.6676144327
1.61528 1.67482194055
1.62016 1.67886997047
1.62504 1.68282913547
1.62992 1.68977676915
1.6348 1.69355779946
1.63968 1.7003283721
1.64456 1.70392843663
1.64944 1.71051848559
1.65432 1.71393483554
1.6592 1.7203409811
1.66408 1.72665404668
1.66896 1.72978989753
1.67384 1.73591398041
1.67872 1.74194224014
1.6836 1.74479137617
1.68848 1.75062576757
1.69336 1.75636169101
1.69824 1.76199823145
1.70312 1.76753448519
1.708 1.77296955994
1.71288 1.77830257492
1.71776 1.78353266086
1.72264 1.78865896012
1.72752 1.79368062673
1.7324 1.7985968264
1.73728 1.80340673662
1.74216 1.80810954667
1.74704 1.81576589128
1.75192 1.82024935316
1.7568 1.82462319076
1.76168 1.83193926864
1.76656 1.83608833054
1.77144 1.84012535382
1.77632 1.84709197483
1.7812 1.85089901921
1.78608 1.85762642788
1.79096 1.86120004327
1.79584 1.86768420139
1.80072 1.87404305395
1.8056 1.87725801518
1.81048 1.88336760171
1.81536 1.88934869963
1.82024 1.8952002236
1.82512 1.90092110251
1.83 1.9065102795
1.83488 1.91196671191
1.83976 1.91728937129
1.84464 1.92247724338
1.84952 1.92752932809
1.8544 1.93244463942
1.85928 1.93722220548
1.86416 1.94186106836
1.86904 1.94930446067
1.87392 1.95365640462
1.8788 1.95786670762
1.88368 1.96485809801
1.88856 1.96877529286
1.89344 1.97545723312
1.89832 1.98197899543
1.9032 1.98544513529
1.90808 1.99165045527
1.91296 1.99769195701
1.91784 2.0035684116
1.92272 2.00927860603
1.9276 2.0148213431
1.93248 2.02019544117
1.93736 2.02539973402
1.94224 2.03043307062
1.94712 2.03529431489
1.952 2.0427929975
1.95688 2.04729760891
1.96176 2.05162667484
1.96664 2.05856206601
1.97152 2.06252732855
1.9764 2.06907754725
1.98128 2.07542835128
1.98616 2.08157833454
1.99104 2.08752610675
1.99592 2.09054625936
2.0008 2.0960957587
2.00568 2.10414248208
2.01056 2.10926780783
2.01544 2.11418419238
2.02032 2.11889033047
2.0252 2.12604558528
2.03008 2.13031638257
2.03496 2.13701155017
2.03984 2.14346882582
2.04472 2.14968661659
2.0496 2.15305873647
2.05448 2.15880437618
2.05936 2.16688733101
2.06424 2.17213148742
2.06912 2.17712836193
2.074 2.1818764218
2.07888 2.18890782239
2.08376 2.19566297622
2.08864 2.19963084742
2.09352 2.20584041532
2.0984 2.21176836413
2.10328 2.21741287616
2.10816 2.22277213478
2.11304 2.23029056762
2.11792 2.23506097554
2.1228 2.24196096245
2.12768 2.24854216679
2.13256 2.25240828247
2.13744 2.25835878717
2.14232 2.26635181014
2.1472 2.27163655492
2.15208 2.27659178721
2.15696 2.28354240797
2.16184 2.29013175245
2.16672 2.29405761295
2.1716 2.30221654903
2.17648 2.30770688935
2.18136 2.31282572037
2.18624 2.31981432431
2.19112 2.32639778594
2.196 2.33257309937
2.20088 2.33833719669
2.20576 2.34368694062
2.21064 2.3507917756
2.21552 2.35528858469
2.2204 2.36150469479
2.22528 2.36939283111
2.23016 2.37467626297
2.23504 2.38159449555
2.23992 2.38801408563
2.2448 2.39393054271
2.24968 2.39933920021
2.25456 2.40627566841
2.25944 2.41266443782
2.26432 2.41849998612
2.2692 2.42577204866
2.27408 2.43244881504
2.27896 2.43852367264
2.28384 2.44398964132
2.28872 2.45077431726
2.2936 2.45690431872
2.29848 2.46427564874
2.30336 2.47094400127
2.30824 2.4768994043
2.31312 2.48398984376
2.318 2.49031430009
2.32288 2.49768814524
2.32776 2.50423876814
2.33264 2.50995102537
2.33752 2.51659020614
2.3424 2.52409177889
2.34728 2.53063809822
2.35216 2.53794226553
2.35704 2.54421244118
2.36192 2.55112513375
2.3668 2.5569125185
2.37168 2.56488618666
2.37656 2.57159454881
2.38144 2.57863257329
2.38632 2.58589780136
2.3912 2.5932778437
2.39608 2.5990505007
2.40096 2.60628417714
2.40584 2.61476983995
2.41072 2.62116702131
2.4156 2.62835977495
2.42048 2.63600809181
2.42536 2.6436786068
2.43024 2.65227116445
2.43512 2.66086021886


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1prob0pt1.tex <==
0.0 0.333808418527
0.004276 0.333806678676
0.008552 0.333886857632
0.012828 0.334043537963
0.017104 0.334226406958
0.02138 0.334473912959
0.025656 0.334779752126
0.029932 0.335137345056
0.034208 0.335539832531
0.038484 0.336025459752
0.04276 0.336541843354
0.047036 0.337081315517
0.051312 0.337682021462
0.055588 0.338336533252
0.059864 0.339083948193
0.06414 0.339823337986
0.068416 0.340640477
0.072692 0.341480446707
0.076968 0.34238299242
0.081244 0.343340691854
0.08552 0.344395050862
0.089796 0.345440733852
0.094072 0.346518504612
0.098348 0.347670887348
0.102624 0.348891311484
0.1069 0.350121512903
0.111176 0.351405276125
0.115452 0.352788622628
0.119728 0.354159585116
0.124004 0.355563392688
0.12828 0.357047773541
0.132556 0.358607644528
0.136832 0.360181653109
0.141108 0.361762460796
0.145384 0.36345829857
0.14966 0.36514909003
0.153936 0.366886714552
0.158212 0.36866597531
0.162488 0.370542963661
0.166764 0.372390757816
0.17104 0.374327689303
0.175316 0.376287229849
0.179592 0.378264116912
0.183868 0.380319295195
0.188144 0.382450637498
0.19242 0.384519259691
0.196696 0.386725187302
0.200972 0.388928489748
0.205248 0.391123835336
0.209524 0.393379003871
0.2138 0.395692312682
0.218076 0.398062196736
0.222352 0.40041014042
0.226628 0.402887588014
0.230904 0.405337764213
0.23518 0.407836544425
0.239456 0.410300140501
0.243732 0.412891531401
0.248008 0.415442892394
0.252284 0.418036125005
0.25656 0.420670540151
0.260836 0.423345574535
0.265112 0.426060792632
0.269388 0.428815888806
0.273664 0.431610689534
0.27794 0.434347711495
0.282216 0.437220122758
0.286492 0.440031381176
0.290768 0.442879197187
0.295044 0.445763980508
0.29932 0.448686287122
0.303596 0.451646822065
0.307872 0.454646442258
0.312148 0.457686159386
0.316424 0.460651984436
0.3207 0.463656082832
0.324976 0.466819347652
0.329252 0.469906520713
0.333528 0.472912589153
0.337804 0.476085191451
0.34208 0.479304622242
0.346356 0.482441988965
0.350632 0.485625940973
0.354908 0.48885894896
0.359184 0.492005095884
0.36346 0.495341805022
0.367736 0.498592316258
0.372012 0.501898305167
0.376288 0.505263070175
0.380564 0.508538286851
0.38484 0.511873922448
0.389116 0.515273750637
0.393392 0.518581476023
0.397668 0.52195575413
0.401944 0.525400853933
0.40622 0.528752144975
0.410496 0.532177371435
0.414772 0.535681316592
0.419048 0.53909064598
0.423324 0.542582595744
0.4276 0.546162481176
0.431876 0.549647890465
0.436152 0.553225957083
0.440428 0.556707965081
0.444704 0.560287827695
0.44898 0.563770356753
0.453256 0.567356424976
0.457532 0.571052560431
0.461808 0.574653614559
0.466084 0.578155793539
0.47036 0.5817744302
0.474636 0.585516738665
0.478912 0.589163606635
0.483188 0.592711409916
0.487464 0.596390660545
0.49174 0.600209276521
0.496016 0.603933497432
0.500292 0.607559884935
0.504568 0.61133484649
0.508844 0.615013119928
0.51312 0.618591350794
0.517396 0.622328268836
0.521672 0.626232989271
0.525948 0.630044402407
0.530224 0.633759362886
0.5345 0.637374714965
0.538776 0.641170650077
0.543052 0.645157135647
0.547328 0.648760065587
0.551604 0.652556361856
0.55588 0.656556480575
0.560156 0.66046544082
0.564432 0.664280416513
0.568708 0.667998576602
0.572984 0.671936672853
0.57726 0.675781714333
0.581536 0.679530983919
0.585812 0.683515624747
0.590088 0.687408734217
0.594364 0.691207712431
0.59864 0.695258464819
0.602916 0.698866339968
0.607192 0.703089262164
0.611468 0.706864347077
0.615744 0.710911176871
0.62002 0.714868922806
0.624296 0.71873522774
0.628572 0.722507736641
0.632848 0.726573403904
0.637124 0.730551123556
0.6414 0.734438665099
0.645676 0.738233801645
0.649952 0.742344940045
0.654228 0.746370081052
0.658504 0.750307122928
0.66278 0.75415396878
0.667056 0.758341067984
0.671332 0.762444929897
0.675608 0.766463582171
0.679884 0.770395058266
0.68416 0.774237397969
0.688436 0.778449372666
0.692712 0.782579791127
0.696988 0.786626816374
0.701264 0.79058861841
0.70554 0.794463374701
0.709816 0.798739018335
0.714092 0.802440150762
0.718368 0.806550433736
0.722644 0.810578425531
0.72692 0.815035976827
0.731196 0.818900361801
0.735472 0.823203066275
0.739748 0.826897291998
0.744024 0.831038751673
0.7483 0.835100281176
0.752576 0.839080337025
0.756852 0.843533683279
0.761128 0.847352420376
0.765404 0.85165390068
0.76968 0.855880401459
0.773956 0.860030507213
0.778232 0.864102811958
0.782508 0.868095919574
0.786784 0.87200844415
0.79106 0.876445758956
0.795336 0.880199418108
0.799612 0.884488021844
0.803888 0.888703546132
0.808164 0.892844725435
0.81244 0.896910304383
0.816716 0.900899038074
0.820992 0.905461771485
0.825268 0.909299680785
0.829544 0.913722301706
0.83382 0.918076409595
0.838096 0.922360868679
0.842372 0.925889528974
0.846648 0.930716347692
0.850924 0.934785147215
0.8552 0.938779857625
0.859476 0.942699395818
0.863752 0.947261056639
0.868028 0.951033759288
0.872304 0.955459920115
0.87658 0.95982017286
0.880856 0.964113527841
0.885132 0.968339005509
0.889408 0.972495636659
0.893684 0.976582462643
0.89796 0.980598535573
0.902236 0.985322045301
0.906512 0.989200611623
0.910788 0.993798378977
0.915064 0.997535809558
0.91934 1.00200427575
0.923616 1.00641019031
0.927892 1.01075269937
0.932168 1.01503095893
0.936444 1.01924413498
0.94072 1.02339140366
0.944996 1.02747195148
0.949272 1.0314849754
0.953548 1.03629064041
0.957824 1.04017308539
0.9621 1.04486027831
0.966376 1.04860905915
0.970652 1.05317473198
0.974928 1.05768193524
0.979204 1.06122802798
0.98348 1.06560928238
0.987756 1.06992989173
0.992032 1.07418914857
0.996308 1.07838635496
1.000584 1.08345673237
1.00486 1.08753456476
1.009136 1.09154830333
1.013412 1.09549728872
1.017688 1.100343848
1.021964 1.10416813635
1.02624 1.10890219094
1.030516 1.11358238352
1.034792 1.11721821086
1.039068 1.121782068
1.043344 1.12629016872
1.04762 1.13074189408
1.051896 1.13513663348
1.056172 1.13947378474
1.060448 1.14375275418
1.064724 1.14797295673
1.069 1.15213381601
1.073276 1.15623476443
1.077552 1.16133129973
1.081828 1.16531728412
1.086104 1.16924168852
1.09038 1.17417953635
1.094656 1.1779856564
1.098932 1.18281705029
1.103208 1.18650274206
1.107484 1.19122548255
1.11176 1.19589626895
1.116036 1.20051455038
1.120312 1.20395954632
1.124588 1.20846491346
1.128864 1.21291619209
1.13314 1.21731286058
1.137416 1.22165440461
1.141692 1.22594031724
1.145968 1.23017009899
1.150244 1.23550687471
1.15452 1.23962900727
1.158796 1.24369352484
1.163072 1.24888170556
1.167348 1.25283557792
1.171624 1.25673041655
1.1759 1.26176536326
1.180176 1.26554668743
1.184452 1.27047893298
1.188728 1.275361982
1.193004 1.27897244688
1.19728 1.28374981416
1.201556 1.28847646882
1.205832 1.29191196147
1.210108 1.29653006928
1.214384 1.30109600415
1.21866 1.30560927877
1.222936 1.31006941181
1.227212 1.314475928
1.231488 1.31882835818
1.235764 1.32312623931
1.24004 1.32865281973
1.244316 1.33284552146
1.248592 1.33698227894
1.252868 1.34106265357
1.257144 1.34639076491
1.26142 1.35036218943
1.265696 1.35427590806
1.269972 1.3594512163
1.274248 1.36325325655
1.278524 1.3683258961
1.2828 1.37334888858
1.287076 1.37698247858
1.291352 1.38189983173
1.295628 1.38676600279
1.299904 1.39022712104
1.30418 1.39498477588
1.308456 1.39968975882
1.312732 1.40434156635
1.317008 1.40893969983
1.321284 1.41348366551
1.32556 1.41797297462
1.329836 1.42240714333
1.334112 1.42678569286
1.338388 1.43110814947
1.342664 1.4353740445
1.34694 1.44098400958
1.351216 1.4451394125
1.355492 1.44923682289
1.359768 1.45468874255
1.364044 1.45867267543
1.36832 1.46401779072
1.372596 1.46788626524
1.376872 1.47312238438
1.381148 1.47687345738
1.385424 1.48199842341
1.3897 1.48563018994
1.393976 1.49064188129
1.398252 1.49559782675
1.402528 1.5004974491
1.406804 1.50388830162
1.41108 1.50867039277
1.415356 1.51339451495
1.419632 1.51806010765
1.423908 1.52266661458
1.428184 1.52721348364
1.43246 1.531700167
1.436736 1.53612612113
1.441012 1.54196629753
1.445288 1.54627184878
1.449564 1.55051500221
1.45384 1.55469523143
1.458116 1.56029776675
1.462392 1.56435299736
1.466668 1.56983416647
1.470944 1.57376208535
1.47522 1.57911933029
1.479496 1.58291765714
1.483772 1.588148451
1.488048 1.59181493879
1.492324 1.59691678614
1.4966 1.60195416103
1.500876 1.60692638446
1.505152 1.61183278116
1.509428 1.61516258415
1.513704 1.61993373331
1.51798 1.62463712057
1.522256 1.62927208605
1.526532 1.63535399405
1.530808 1.63985146213
1.535084 1.64427848328
1.53936 1.64863441298
1.543636 1.6529186106
1.547912 1.6586522925
1.552188 1.6627920852
1.556464 1.66838186166
1.56074 1.67237445612
1.565016 1.67781727064
1.569292 1.68165990348
1.573568 1.6869527286
1.577844 1.69216969078
1.58212 1.69578250386
1.586396 1.70084491986
1.590672 1.7058291055
1.594948 1.71073425529
1.599224 1.71555956724
1.6035 1.72030424287
1.607776 1.7249674872
1.612052 1.7295485087
1.616328 1.73404651931
1.620604 1.73998904596
1.62488 1.74431842436
1.629156 1.74856237731
1.633432 1.75424741891
1.637708 1.75831772797
1.641984 1.76382646912
1.64626 1.7692453762
1.650536 1.77304859242
1.654812 1.7782856974
1.659088 1.78343012508
1.663364 1.78848091008
1.66764 1.79343708991
1.671916 1.79829770491
1.676192 1.80306179818
1.680468 1.80772841543
1.684744 1.81229660498
1.68902 1.8182806777
1.693296 1.82264774403
1.697572 1.82691347137
1.701848 1.8325876701
1.706124 1.83664626019
1.7104 1.84210800639
1.714676 1.8474610084
1.718952 1.85270412061
1.723228 1.85783619903
1.727504 1.86285610106
1.73178 1.86776268534
1.736056 1.87255481151
1.740332 1.87723134001
1.744608 1.88179113183
1.748884 1.88772168666
1.75316 1.89204216222
1.757436 1.89772610658
1.761712 1.90180243426
1.765988 1.90723466036
1.770264 1.91253774737
1.77454 1.91771034749
1.778816 1.92275111137
1.783092 1.92765868763
1.787368 1.93243172251
1.791644 1.93852993764
1.79592 1.9430266859
1.800196 1.94883947392
1.804472 1.9530542111
1.808748 1.95857556387
1.813024 1.963947225
1.8173 1.96916761048
1.821576 1.97423512963
1.825852 1.97914818428
1.830128 1.98390516799
1.834404 1.98993107684
1.83868 1.99436725342
1.842956 2.00006132985
1.847232 2.00558485297
1.851508 2.01093596856
1.855784 2.01611280826
1.86006 2.0211134883
1.864336 2.02593610801
1.868612 2.03197298321
1.872888 2.03642937472
1.877164 2.04208732419
1.88144 2.04755042705
1.885716 2.05281648841
1.889992 2.05788328601
1.894268 2.06411583069
1.898544 2.06877260461
1.90282 2.07458097786
1.907096 2.08017115168
1.911372 2.08554054943
1.915648 2.09068655031
1.919924 2.09560648559
1.9242 2.10163065048
1.928476 2.10608510971
1.932752 2.11162781176
1.937028 2.11692266412
1.941304 2.12327867738
1.94558 2.12806295158
1.949856 2.13389102683
1.954132 2.13944717426
1.958408 2.14472772386
1.962684 2.1510137344
1.96696 2.15572600366
1.971236 2.16142444793
1.975512 2.16681989823
1.979788 2.17316989575
1.984064 2.17793989366
1.98834 2.1836431729
1.992616 2.19025689664
1.996892 2.19528086342
2.001168 2.20119211435
2.005444 2.20674014816
2.00972 2.21191855544
2.013996 2.21793463839
2.018272 2.22355480219
2.022548 2.22997296756
2.026824 2.23477145769
2.0311 2.24152742277
2.035376 2.24664547236
2.039652 2.25248705645
2.043928 2.25902197308
2.048204 2.26389235249
2.05248 2.27057509015
2.056756 2.27671646142
2.061032 2.28230094997
2.065308 2.28844850795
2.069584 2.29399002153
2.07386 2.30002809822
2.078136 2.30651905869
2.082412 2.31230595665
2.086688 2.31846187642
2.090964 2.32383527885
2.09524 2.33056519702
2.099516 2.33639799407
2.103792 2.34342927054
2.108068 2.34941252619
2.112344 2.35532684997
2.11662 2.36210188614
2.120896 2.36851338587
2.125172 2.37539981457
2.129448 2.38246312906
2.133724 2.38927212064


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1prob0pt1pt5prob0pt5.tex <==
0.0 0.147880225764
0.004276 0.147933398943
0.008552 0.148091744473
0.012828 0.14835361007
0.017104 0.148717501834
0.02138 0.14918207647
0.025656 0.149746133931
0.029932 0.150408610421
0.034208 0.151168571768
0.038484 0.152025207133
0.04276 0.152977823035
0.047036 0.154025837684
0.051312 0.155168775599
0.055588 0.156406262492
0.059864 0.157738020408
0.06414 0.159163863114
0.068416 0.160683691702
0.072692 0.162297490416
0.076968 0.164005322678
0.081244 0.16580732731
0.08552 0.167703714927
0.089796 0.16969476451
0.094072 0.171780820137
0.098348 0.173962287865
0.102624 0.176239632754
0.1069 0.178613376036
0.111176 0.181084092396
0.115452 0.183652407393
0.119728 0.186318994981
0.124004 0.189084575146
0.12828 0.191949911643
0.132556 0.194915809832
0.136832 0.197983114604
0.141108 0.201152708394
0.145384 0.20442550928
0.14966 0.207802469156
0.153936 0.211284571979
0.158212 0.21244039093
0.162488 0.212459953312
0.166764 0.212501794379
0.17104 0.21258452889
0.175316 0.212684522909
0.179592 0.212799190165
0.183868 0.212925972056
0.188144 0.213106094685
0.19242 0.213293934288
0.196696 0.213509239194
0.200972 0.21375008214
0.205248 0.214014580467
0.209524 0.214300893259
0.2138 0.214607218638
0.218076 0.214954949576
0.222352 0.215319611636
0.226628 0.215699523974
0.230904 0.216116838727
0.23518 0.216570617695
0.239456 0.21701145167
0.243732 0.217510612176
0.248008 0.218018542443
0.252284 0.218558790594
0.25656 0.219105414672
0.260836 0.219682558692
0.265112 0.220289666053
0.269388 0.220926241637
0.273664 0.221565430759
0.27794 0.222259397286
0.282216 0.222927631937
0.286492 0.223650031223
0.290768 0.224399656059
0.295044 0.225148332353
0.29932 0.225923298292
0.303596 0.226724497897
0.307872 0.227551937678
0.312148 0.22837623714
0.316424 0.229256049891
0.3207 0.230132276763
0.324976 0.231034604056
0.329252 0.231932313125
0.333528 0.23288739952
0.337804 0.233837825313
0.34208 0.234782795814
0.346356 0.235787004774
0.350632 0.236786021911
0.354908 0.237812805301
0.359184 0.238833968081
0.36346 0.239883483645
0.367736 0.240962211118
0.372012 0.242035488503
0.376288 0.243138907168
0.380564 0.244236901212
0.38484 0.245366185888
0.389116 0.246527961009
0.393392 0.24768525271
0.397668 0.248837742344
0.401944 0.250024530151
0.40622 0.251207121128
0.410496 0.252425877131
0.414772 0.253641252975
0.419048 0.254894920396
0.423324 0.256103823545
0.4276 0.257395197639
0.431876 0.258641777749
0.436152 0.259930389275
0.440428 0.261218071663
0.444704 0.262504959116
0.44898 0.263837641175
0.453256 0.265171315834
0.457532 0.266506260237
0.461808 0.267842790089
0.466084 0.269181260529
0.47036 0.27052206701
0.474636 0.271916479306
0.478912 0.273315696843
0.483188 0.274667876407
0.487464 0.27607761962
0.49174 0.277493962606
0.496016 0.278917598671
0.500292 0.280349268257
0.504568 0.281733229047
0.508844 0.283182516445
0.51312 0.284642338158
0.517396 0.286113632446
0.521672 0.287537328656
0.525948 0.289033675875
0.530224 0.29048270959
0.5345 0.292008444415
0.538776 0.293487315626
0.543052 0.294982448845
0.547328 0.296495124266
0.551604 0.297959944212
0.55588 0.299510770301
0.560156 0.301014554569
0.564432 0.30253950927
0.568708 0.304087172184
0.572984 0.305659143529
0.57726 0.307184107086
0.581536 0.308734591792
0.585812 0.310312347371
0.590088 0.311842902903
0.594364 0.313402164915
0.59864 0.314992039012
0.602916 0.316614499026
0.607192 0.318190694241
0.611468 0.319719174695
0.615744 0.321365034611
0.62002 0.3229650943
0.624296 0.324517942203
0.628572 0.326196095491
0.632848 0.327740975171
0.637124 0.329415907985
0.6414 0.331045611232
0.645676 0.33262873202
0.649952 0.334257322531
0.654228 0.335934004328
0.658504 0.337565374455
0.66278 0.339150116886
0.667056 0.340785746628
0.671332 0.342475104785
0.675608 0.344119464351
0.679884 0.34582062381
0.68416 0.347477104442
0.688436 0.349087654887
0.692712 0.350758452978
0.696988 0.352383758369
0.701264 0.354072762142
0.70554 0.355828770778
0.709816 0.357428209675
0.714092 0.359095318408
0.718368 0.360833560981
0.722644 0.362528308725
0.72692 0.364178404844
0.731196 0.365904073461
0.735472 0.367586008507
0.739748 0.369347739857
0.744024 0.371066780503
0.7483 0.372742025076
0.752576 0.374372360601
0.756852 0.376088076787
0.761128 0.377893225778
0.765404 0.379522183285
0.76968 0.381241908283
0.773956 0.383056626901
0.778232 0.384690228388
0.782508 0.386420311166
0.786784 0.388251278758
0.79106 0.389896236922
0.795336 0.391643725068
0.799612 0.393348893822
0.803888 0.395162065905
0.808164 0.396934725642
0.81244 0.398665906119
0.816716 0.400354634734
0.820992 0.402159007229
0.825268 0.403922922849
0.829544 0.405645441955
0.83382 0.407325619616
0.838096 0.409129600041
0.842372 0.4108934282
0.846648 0.412616193952
0.850924 0.414470274532
0.8552 0.41611026446
0.859476 0.417883958573
0.863752 0.419796832544
0.868028 0.421490862529
0.872304 0.423326642275
0.87658 0.424937526637
0.880856 0.426881145325
0.885132 0.42859817498
0.889408 0.430273920743
0.893684 0.432102611442
0.89796 0.433892851484
0.902236 0.435643827932
0.906512 0.437556694554
0.910788 0.439229019008
0.915064 0.441066284237
0.91934 0.442865744651
0.923616 0.444626621693
0.927892 0.446348133419
0.932168 0.44824571479
0.936444 0.45010723228
0.94072 0.451710831803
0.944996 0.453495528126
0.949272 0.45546799886
0.953548 0.457177842986
0.957824 0.459079020023
0.9621 0.460711080099
0.966376 0.462538091545
0.970652 0.464328227933
0.974928 0.466322199267
0.979204 0.468039077314
0.98348 0.469963642457
0.987756 0.471604480282
0.992032 0.473456919425
0.996308 0.475273616296
1.000584 0.47705390183
1.00486 0.478797104673
1.009136 0.480765443523
1.013412 0.482435224045
1.017688 0.484334357313
1.021964 0.486199325567
1.02624 0.488029501342
1.030516 0.489824255191
1.034792 0.491582955721
1.039068 0.493587621232
1.043344 0.495275209255
1.04762 0.497213320446
1.051896 0.498827321341
1.056172 0.500696469887
1.060448 0.502531715308
1.064724 0.504332468844
1.069 0.506401459971
1.073276 0.508134483555
1.077552 0.509831257938
1.081828 0.511803644548
1.086104 0.513744756016
1.09038 0.515335407893
1.094656 0.517209219896
1.098932 0.51905010693
1.103208 0.520857522571
1.107484 0.522630919133
1.11176 0.524704177303
1.116036 0.526411100791
1.120312 0.528423249258
1.124588 0.530061568628
1.128864 0.532010545909
1.13314 0.533928806202
1.137416 0.535815849458
1.141692 0.537671174623
1.145968 0.539494279669
1.150244 0.541284661619
1.15452 0.543041816577
1.158796 0.544765239752
1.163072 0.546828652395
1.167348 0.548486531282
1.171624 0.550490298502
1.1759 0.552465274655
1.180176 0.554022915879
1.184452 0.55593543684
1.188728 0.557817786292
1.193004 0.559669508856
1.19728 0.5614901485
1.201556 0.563685086915
1.205832 0.56544579513
1.210108 0.567174067107
1.214384 0.56886944443
1.21866 0.570951838608
1.222936 0.572583728121
1.227212 0.574609110864
1.231488 0.576607211229
1.235764 0.57857762359
1.24004 0.58008098837
1.244316 0.581991034106
1.248592 0.583872154015
1.252868 0.585723940823
1.257144 0.587545986898
1.26142 0.589795880951
1.265696 0.591561084891
1.269972 0.593295341539
1.274248 0.594998242033
1.278524 0.597142938652
1.2828 0.598785835802
1.287076 0.600877620517
1.291352 0.602458948943
1.295628 0.60449632821
1.299904 0.606507949146
1.30418 0.608493455877
1.308456 0.609950990036
1.312732 0.611879135934
1.317008 0.613780081012
1.321284 0.615653468823
1.32556 0.617498942822
1.329836 0.619316146381
1.334112 0.621630879348
1.338388 0.62339464368
1.342664 0.625129085253
1.34694 0.626833847286
1.351216 0.629051524059
1.355492 0.630700099705
1.359768 0.632869398519
1.364044 0.634460431945
1.36832 0.636580067847
1.372596 0.63811220352
1.376872 0.640180891752
1.381148 0.642225799062
1.385424 0.644246621954
1.3897 0.645661281986
1.393976 0.647628624304
1.398252 0.649570954714
1.402528 0.651487970061
1.406804 0.653379367311
1.41108 0.655244843561
1.415356 0.657084096057
1.419632 0.658896822216
1.423908 0.660682719634
1.428184 0.663063496922
1.43246 0.664799386991
1.436736 0.666507559398
1.441012 0.668823443951
1.445288 0.670479884105
1.449564 0.67210771965
1.45384 0.674356254047
1.458116 0.675930636416
1.462392 0.678134466368
1.466668 0.679654262051
1.470944 0.681812322002
1.47522 0.683949460178
1.479496 0.685387626143
1.483772 0.687477416323
1.488048 0.689545521682
1.492324 0.691591693854
1.4966 0.692918755024
1.500876 0.694915493961
1.505152 0.696889539972
1.509428 0.698840645835
1.513704 0.700768564635
1.51798 0.702673049774
1.522256 0.704553854987
1.526532 0.706410734352
1.530808 0.708243442306
1.535084 0.710051733653
1.53936 0.711835363582
1.543636 0.714344951477
1.547912 0.716083523997
1.552188 0.717796718707
1.556464 0.719484292394
1.56074 0.721916951589
1.565016 0.723557615747
1.569292 0.725171947356
1.573568 0.727545880288
1.577844 0.729111929339
1.58212 0.731447340118
1.586396 0.732964205628
1.590672 0.735260255505
1.594948 0.736727039952
1.599224 0.738982893234
1.6035 0.740398702742
1.607776 0.742613526961
1.612052 0.744810137753
1.616328 0.746150437567
1.620604 0.74830479162
1.62488 0.750440342212
1.629156 0.752556898286
1.633432 0.753795261029
1.637708 0.755867945272
1.641984 0.75792104995
1.64626 0.759954385658
1.650536 0.761967763408
1.654812 0.763960994644
1.659088 0.765933891246
1.663364 0.767886265542
1.66764 0.769817930316
1.671916 0.77172869882
1.676192 0.773618384779
1.680468 0.775486802403
1.684744 0.777333766395
1.68902 0.779159091963
1.693296 0.780962594824
1.697572 0.782744091218
1.701848 0.784503397913
1.706124 0.787191513487
1.7104 0.788911436104
1.714676 0.790608635555
1.718952 0.792282930742
1.723228 0.794907568551
1.727504 0.79654110837
1.73178 0.79815121675
1.736056 0.800727959771
1.740332 0.802296301186
1.744608 0.803840688915
1.748884 0.806368120347
1.75316 0.807869738868
1.757436 0.81036540756
1.761712 0.811823602182
1.765988 0.813256988253
1.770264 0.815701024106
1.77454 0.817090000416
1.778816 0.819500757918
1.783092 0.821897527225
1.787368 0.823221565161
1.791644 0.825584176838
1.79592 0.826862215875
1.800196 0.829190080899
1.804472 0.831503255558
1.808748 0.832714022284
1.813024 0.834991585505
1.8173 0.837254044728
1.821576 0.838396165994
1.825852 0.840622158071
1.830128 0.842832636746
1.834404 0.845027470023
1.83868 0.846077920539
1.842956 0.848235167395
1.847232 0.850376365266
1.851508 0.852501384024
1.855784 0.854610093998
1.86006 0.856702365983
1.864336 0.858778071244
1.868612 0.859666950062
1.872888 0.861703166475
1.877164 0.863722423259
1.88144 0.865724593714
1.885716 0.867709551638
1.889992 0.869677171334
1.894268 0.871627327615
1.898544 0.873559895811
1.90282 0.875474751774
1.907096 0.87737177188
1.911372 0.87925083304
1.915648 0.881111812702
1.919924 0.882954588857
1.9242 0.886027516068
1.928476 0.887839609598
1.932752 0.889633145236
1.937028 0.891408003098
1.941304 0.893164063873
1.94558 0.894901208822
1.949856 0.896619319785
1.954132 0.899609538652
1.958408 0.901295373891
1.962684 0.902961831829
1.96696 0.904608796573
1.971236 0.906236152838
1.975512 0.909165836778
1.979788 0.910759814133
1.984064 0.91233384795
1.98834 0.915228435788
1.992616 0.916768446862
1.996892 0.918288184342
2.001168 0.921146769127
2.005444 0.92263184923
2.00972 0.924096330803
2.013996 0.926918017236
2.018272 0.928347216232
2.022548 0.929755497007
2.026824 0.932539401764
2.0311 0.933911784423
2.035376 0.936672103064
2.039652 0.938008186586
2.043928 0.940744543207
2.048204 0.942043930748
2.05248 0.943321678796
2.056756 0.946018251755
2.061032 0.947258711266
2.065308 0.94993039217
2.069584 0.952592641158
2.07386 0.953779602384
2.078136 0.956416419877
2.082412 0.957565140742
2.086688 0.960176168189
2.090964 0.961286273645
2.09524 0.963871156134
2.099516 0.964942275672
2.103792 0.967500661983
2.108068 0.970048840076
2.112344 0.971063972343
2.11662 0.973585138242
2.120896 0.976095845534
2.125172 0.977054193987
2.129448 0.979537381004
2.133724 0.982009862537


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1pt5.tex <==
0.0 0.208916205288
0.0064 0.208999387658
0.0128 0.209247010917
0.0192 0.209656385231
0.0256 0.210225085186
0.032 0.210950936208
0.0384 0.211832001658
0.0448 0.212866570567
0.0512 0.21405314599
0.0576 0.215390433933
0.064 0.216877332828
0.0704 0.21851292353
0.0768 0.220296459801
0.0832 0.222227359258
0.0896 0.224305194765
0.096 0.226529686229
0.1024 0.228900692799
0.1088 0.231418205427
0.1152 0.234082339783
0.1216 0.236893329496
0.128 0.239851519712
0.1344 0.242957360941
0.1408 0.246211403185
0.1472 0.249614290334
0.1536 0.253166754798
0.16 0.256869612389
0.1664 0.26072375741
0.1728 0.264730157969
0.1792 0.268889851482
0.1856 0.273203940364
0.192 0.277673587907
0.1984 0.282300014318
0.2048 0.287084492921
0.2112 0.29202834651
0.2176 0.297132943849
0.224 0.302399696305
0.2304 0.302813240164
0.2368 0.302855187534
0.2432 0.302956564474
0.2496 0.303083782785
0.256 0.303262496441
0.2624 0.303458848998
0.2688 0.303729523719
0.2752 0.304010357504
0.2816 0.304359135701
0.288 0.304710867717
0.2944 0.305124492757
0.3008 0.305597655568
0.3072 0.306096042896
0.3136 0.306616616677
0.32 0.307189078981
0.3264 0.307811455643
0.3328 0.308481875518
0.3392 0.309198567639
0.3456 0.309925795644
0.352 0.310695303563
0.3584 0.311540386167
0.3648 0.312390380738
0.3712 0.313278382573
0.3776 0.314203143322
0.384 0.315199962954
0.3904 0.316195289946
0.3968 0.317261527081
0.4032 0.318323527981
0.4096 0.319455688748
0.416 0.320581168662
0.4224 0.321776458494
0.4288 0.323002744711
0.4352 0.32425960717
0.4416 0.32554671595
0.448 0.32686383239
0.4544 0.328210810253
0.4608 0.329587597038
0.4672 0.330994235413
0.4736 0.332430864767
0.48 0.333897722882
0.4864 0.335350034936
0.4928 0.336877807234
0.4992 0.338437115365
0.5056 0.340028609256
0.512 0.341605209376
0.5184 0.343262739882
0.5248 0.344905757812
0.5312 0.346583150076
0.5376 0.348296082741
0.544 0.349994257064
0.5504 0.351729071688
0.5568 0.353502008997
0.5632 0.355314677786
0.5696 0.357113953078
0.576 0.358954845097
0.5824 0.360782708548
0.5888 0.362654443916
0.5952 0.364572227568
0.6016 0.366479051604
0.608 0.368434815577
0.6144 0.370380846958
0.6208 0.37231691916
0.6272 0.374306049009
0.6336 0.376351138155
0.64 0.378324773531
0.6464 0.380356456318
0.6528 0.382449453557
0.6592 0.384538772117
0.6656 0.386555189919
0.672 0.388707625473
0.6784 0.390787937857
0.6848 0.39293904952
0.6912 0.395090924443
0.6976 0.397244227996
0.704 0.399399693027
0.7104 0.401558121245
0.7168 0.403799335822
0.7232 0.405967638212
0.7296 0.408223246934
0.736 0.410488357576
0.7424 0.412680082614
0.7488 0.414966606659
0.7552 0.417266517029
0.7616 0.419493096188
0.768 0.421822845698
0.7744 0.424079604028
0.7808 0.426445614026
0.7872 0.428739231555
0.7936 0.43105326239
0.8 0.433389616122
0.8064 0.435750291314
0.8128 0.438137376748
0.8192 0.440451633867
0.8256 0.442896602384
0.832 0.445270202126
0.8384 0.447676252491
0.8448 0.450117249947
0.8512 0.452486321262
0.8576 0.454892284217
0.864 0.457337867381
0.8704 0.459825899369
0.8768 0.462243043061
0.8832 0.464705093421
0.8896 0.467095334477
0.896 0.469654724421
0.9024 0.472145134644
0.9088 0.474564450271
0.9152 0.47703761753
0.9216 0.479568108943
0.928 0.482028657503
0.9344 0.484549967088
0.9408 0.487135772718
0.9472 0.489653261272
0.9536 0.492100452326
0.96 0.494756621176
0.9664 0.49720391332
0.9728 0.499723702066
0.9792 0.502320200683
0.9856 0.504848893454
0.992 0.507458855317
0.9984 0.510001505036
1.0048 0.512630230354
1.0112 0.515192301673
1.0176 0.517845506249
1.024 0.520432882843
1.0304 0.522952681702
1.0368 0.52556941946
1.0432 0.528119599838
1.0496 0.530772354965
1.056 0.533359748517
1.0624 0.536055615589
1.0688 0.538687495214
1.0752 0.541253765612
1.0816 0.54393544734
1.088 0.546553102346
1.0944 0.549105150248
1.1008 0.5517799919
1.1072 0.554583500633
1.1136 0.557131693168
1.12 0.559810536575
1.1264 0.56242606721
1.1328 0.565179443555
1.1392 0.567871711998
1.1456 0.570501434274
1.152 0.573277671108
1.1584 0.575780626591
1.1648 0.578648406518
1.1712 0.581240122138
1.1776 0.583988816571
1.184 0.586677303935
1.1904 0.589304241705
1.1968 0.592097863643
1.2032 0.594832860643
1.2096 0.597507942787
1.216 0.60012181693
1.2224 0.602914137466
1.2288 0.605648445649
1.2352 0.608323502672
1.2416 0.611187769394
1.248 0.613743556212
1.2544 0.616492023136
1.2608 0.619182282235
1.2672 0.622074812624
1.2736 0.624912845283
1.28 0.627427475436
1.2864 0.630150038348
1.2928 0.633088658953
1.2992 0.635697394466
1.3056 0.638526215392
1.312 0.641300079294
1.3184 0.644017910701
1.3248 0.646968447208
1.3312 0.649574214135
1.3376 0.652417033955
1.344 0.655206075
1.3504 0.65794031903
1.3568 0.660618747202
1.3632 0.663549849752
1.3696 0.666429805378
1.376 0.669257654921
1.3824 0.672032438922
1.3888 0.674753197732
1.3952 0.677418971613
1.4016 0.680358736678
1.408 0.683248546591
1.4144 0.685750597298
1.4208 0.68887470281
1.4272 0.691609250519
1.4336 0.694290246086
1.44 0.697267869878
1.4464 0.69984265944
1.4528 0.702719506369
1.4592 0.705546493875
1.4656 0.708322784515
1.472 0.711416775359
1.4784 0.714092851757
1.4848 0.717092372542
1.4912 0.719664971025
1.4976 0.722566837846
1.504 0.725420567975
1.5104 0.728225387174
1.5168 0.730980522268
1.5232 0.734084469614
1.5296 0.736741760047
1.536 0.739754034779
1.5424 0.742721312305
1.5488 0.745228152802
1.5552 0.748099391288
1.5616 0.750923482481
1.568 0.754126230222
1.5744 0.756857868298
1.5808 0.759540257569
1.5872 0.762611148952
1.5936 0.765639417876
1.6 0.768177915664
1.6064 0.77111494889
1.6128 0.774007404041
1.6192 0.776854638199
1.6256 0.77965601013
1.632 0.782877798327
1.6384 0.785589663229
1.6448 0.788728969866
1.6512 0.791348851048
1.6576 0.79440327273
1.664 0.797416453676
1.6704 0.799895855849
1.6768 0.802820590013
1.6832 0.805702335112
1.6896 0.80904521128
1.696 0.811843535691
1.7024 0.814597171567
1.7088 0.817305551225
1.7152 0.820489997883
1.7216 0.823110508365
1.728 0.826214663415
1.7344 0.82928006003
1.7408 0.832306185844
1.7472 0.835292530428
1.7536 0.838238585343
1.76 0.841143844185
1.7664 0.844007802645
1.7728 0.846829958554
1.7792 0.849609811937
1.7856 0.852917228932
1.792 0.855615477371
1.7984 0.858269950475
1.8048 0.861464030169
1.8112 0.864622412615
1.8176 0.867151712308
1.824 0.870232809149
1.8304 0.873276861081
1.8368 0.876283427298
1.8432 0.879252069107
1.8496 0.882182349966
1.856 0.885073835528
1.8624 0.88792609368
1.8688 0.891368394048
1.8752 0.89414555896
1.8816 0.896882225387
1.888 0.900221644767
1.8944 0.902880730443
1.9008 0.90615111185
1.9072 0.908730988361
1.9136 0.911930755742
1.92 0.91509699017
1.9264 0.918229314431
1.9328 0.920650707422
1.9392 0.923709338615
1.9456 0.926732930701
1.952 0.929721114994
1.9584 0.932673524985
1.9648 0.935589796373
1.9712 0.93917485078
1.9776 0.942022565999
1.984 0.944833071982
1.9904 0.948325730828
1.9968 0.951065585207
2.0032 0.953767179727
2.0096 0.957164391932
2.016 0.959793278737
2.0224 0.963126810721
2.0288 0.966430443446
2.0352 0.968950194442
2.0416 0.972188204318
2.048 0.97539536357
2.0544 0.978571361337
2.0608 0.981715888711
2.0672 0.984050518777
2.0736 0.987126278318
2.08 0.99016964679
2.0864 0.993180323507
2.0928 0.996955797483
2.0992 0.999905127699
2.1056 1.00282088179
2.112 1.00570276731
2.1184 1.00855049396
2.1248 1.0121862557
2.1312 1.01496975714
2.1376 1.01855063247
2.144 1.02126879049
2.1504 1.02395137901
2.1568 1.02744539735
2.1632 1.03091323172
2.1696 1.03349741155
2.176 1.0369071205
2.1824 1.03942269798
2.1888 1.0427732314
2.1952 1.04609627685
2.2016 1.0493915797
2.208 1.05265888697
2.2144 1.05500587845
2.2208 1.05821145722
2.2272 1.06138829017
2.2336 1.06453613125
2.24 1.06765473615
2.2464 1.07074386226
2.2528 1.07380326876
2.2592 1.07775970251
2.2656 1.08076394468
2.272 1.08373775523
2.2784 1.08668090022
2.2848 1.08959314746
2.2912 1.09342619004
2.2976 1.0962809407
2.304 1.09910410698
2.3104 1.10286233564
2.3168 1.10562664404
2.3232 1.10933552255
2.3296 1.1120400804
2.336 1.11569871479
2.3424 1.11834264182
2.3488 1.12195014893
2.3552 1.1255342433
2.3616 1.12808808494
2.368 1.13161974455
2.3744 1.13512733874
2.3808 1.13758917493
2.3872 1.14104305032
2.3936 1.14447221839
2.4 1.14787646612
2.4064 1.15125558155
2.4128 1.15460935378
2.4192 1.15793757295
2.4256 1.16124003027
2.432 1.16451651801
2.4384 1.16776682947
2.4448 1.17099075899
2.4512 1.17418810196
2.4576 1.17735865481
2.464 1.18050221497
2.4704 1.1836185809
2.4768 1.18670755208
2.4832 1.19086881911
2.4896 1.19390725023
2.496 1.19691768334
2.5024 1.19989992164
2.5088 1.20397298399
2.5152 1.20690306105
2.5216 1.21093316912
2.528 1.21381027432
2.5344 1.21665819683
2.5408 1.22061991192
2.5472 1.2234136645
2.5536 1.22733033121
2.56 1.23122652574
2.5664 1.23393989576
2.5728 1.23778977648
2.5792 1.24044697467
2.5856 1.24424970643
2.592 1.2480308899
2.5984 1.25060469044
2.6048 1.25433746248
2.6112 1.25804803745
2.6176 1.2617361946
2.624 1.26540171279
2.6304 1.26904437039
2.6368 1.27145056906
2.6432 1.27504225984
2.6496 1.27861043553
2.656 1.28215487246
2.6624 1.28567534628
2.6688 1.28917163188
2.6752 1.2926435033
2.6816 1.29609073375
2.688 1.30076270941
2.6944 1.30416443719
2.7008 1.30754082203
2.7072 1.31089163265
2.7136 1.31421663651
2.72 1.31751559975
2.7264 1.32206442254
2.7328 1.32531496338
2.7392 1.32853873597
2.7456 1.33302466019
2.752 1.33619848708
2.7584 1.34064254844
2.7648 1.34376538028
2.7712 1.34686018548
2.7776 1.35123721343
2.784 1.35427942971
2.7904 1.358611738
2.7968 1.36292331886
2.8032 1.36588665413
2.8096 1.37015168995
2.816 1.37439503733
2.8224 1.37727685294
2.8288 1.38147175632
2.8352 1.38564396923
2.8416 1.38979314006
2.848 1.39256329939
2.8544 1.39666134409
2.8608 1.40073527941
2.8672 1.40478472929
2.8736 1.4088093106
2.88 1.41280863286
2.8864 1.4167822978
2.8928 1.42072989894
2.8992 1.42465102119
2.9056 1.42854524031
2.912 1.43241212244
2.9184 1.43764909541
2.9248 1.44146364756
2.9312 1.44524947008
2.9376 1.44900608424
2.944 1.45414542406
2.9504 1.45784570691
2.9568 1.46151523573
2.9632 1.46657650559
2.9696 1.47018638725
2.976 1.47519376682
2.9824 1.47874159802
2.9888 1.48369248047
2.9952 1.48861574678
3.0016 1.4920672993
3.008 1.49692978615
3.0144 1.50176234922
3.0208 1.5065641491
3.0272 1.5113343131
3.0336 1.51607193261
3.04 1.52077606033
3.0464 1.52544570707
3.0528 1.53007983822
3.0592 1.53467736989
3.0656 1.53923716445
3.072 1.54375802566
3.0784 1.54971869907
3.0848 1.55416063212
3.0912 1.56004509856
3.0976 1.56440227684
3.104 1.57020417327
3.1104 1.57447002782
3.1168 1.58018215587
3.1232 1.58584761826
3.1296 1.59146414989
3.136 1.59702930747
3.1424 1.60254044488
3.1488 1.60950238493
3.1552 1.61489875621
3.1616 1.62174352207
3.168 1.62701099224
3.1744 1.63372272175
3.1808 1.64036181697
3.1872 1.64844236018
3.1936 1.65492088809


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1pt5prob0pt05.tex <==
0.0 0.147880225764
0.004276 0.147933398943
0.008552 0.148091744473
0.012828 0.14835361007
0.017104 0.148717501834
0.02138 0.14918207647
0.025656 0.149746133931
0.029932 0.150408610421
0.034208 0.151168571768
0.038484 0.152025207133
0.04276 0.152977823035
0.047036 0.154025837684
0.051312 0.155168775599
0.055588 0.156406262492
0.059864 0.157738020408
0.06414 0.159163863114
0.068416 0.160683691702
0.072692 0.162297490416
0.076968 0.164005322678
0.081244 0.16580732731
0.08552 0.167703714927
0.089796 0.16969476451
0.094072 0.171780820137
0.098348 0.173962287865
0.102624 0.176239632754
0.1069 0.178613376036
0.111176 0.181084092396
0.115452 0.183652407393
0.119728 0.186318994981
0.124004 0.189084575146
0.12828 0.191949911643
0.132556 0.194915809832
0.136832 0.197983114604
0.141108 0.201152708394
0.145384 0.20442550928
0.14966 0.207802469156
0.153936 0.211284571979
0.158212 0.21244039093
0.162488 0.212459953312
0.166764 0.212501794379
0.17104 0.21258452889
0.175316 0.212684522909
0.179592 0.212799190165
0.183868 0.212925972056
0.188144 0.213106094685
0.19242 0.213293934288
0.196696 0.213509239194
0.200972 0.21375008214
0.205248 0.214014580467
0.209524 0.214300893259
0.2138 0.214607218638
0.218076 0.214954949576
0.222352 0.215319611636
0.226628 0.215699523974
0.230904 0.216116838727
0.23518 0.216570617695
0.239456 0.21701145167
0.243732 0.217510612176
0.248008 0.218018542443
0.252284 0.218558790594
0.25656 0.219105414672
0.260836 0.219682558692
0.265112 0.220289666053
0.269388 0.220926241637
0.273664 0.221565430759
0.27794 0.222259397286
0.282216 0.222927631937
0.286492 0.223650031223
0.290768 0.224399656059
0.295044 0.225148332353
0.29932 0.225923298292
0.303596 0.226724497897
0.307872 0.227551937678
0.312148 0.22837623714
0.316424 0.229256049891
0.3207 0.230132276763
0.324976 0.231034604056
0.329252 0.231932313125
0.333528 0.23288739952
0.337804 0.233837825313
0.34208 0.234782795814
0.346356 0.235787004774
0.350632 0.236786021911
0.354908 0.237812805301
0.359184 0.238833968081
0.36346 0.239883483645
0.367736 0.240962211118
0.372012 0.242035488503
0.376288 0.243138907168
0.380564 0.244236901212
0.38484 0.245366185888
0.389116 0.246527961009
0.393392 0.24768525271
0.397668 0.248837742344
0.401944 0.250024530151
0.40622 0.251207121128
0.410496 0.252425877131
0.414772 0.253641252975
0.419048 0.254894920396
0.423324 0.256103823545
0.4276 0.257395197639
0.431876 0.258641777749
0.436152 0.259930389275
0.440428 0.261218071663
0.444704 0.262504959116
0.44898 0.263837641175
0.453256 0.265171315834
0.457532 0.266506260237
0.461808 0.267842790089
0.466084 0.269181260529
0.47036 0.27052206701
0.474636 0.271916479306
0.478912 0.273315696843
0.483188 0.274667876407
0.487464 0.27607761962
0.49174 0.277493962606
0.496016 0.278917598671
0.500292 0.280349268257
0.504568 0.281733229047
0.508844 0.283182516445
0.51312 0.284642338158
0.517396 0.286113632446
0.521672 0.287537328656
0.525948 0.289033675875
0.530224 0.29048270959
0.5345 0.292008444415
0.538776 0.293487315626
0.543052 0.294982448845
0.547328 0.296495124266
0.551604 0.297959944212
0.55588 0.299510770301
0.560156 0.301014554569
0.564432 0.30253950927
0.568708 0.304087172184
0.572984 0.305659143529
0.57726 0.307184107086
0.581536 0.308734591792
0.585812 0.310312347371
0.590088 0.311842902903
0.594364 0.313402164915
0.59864 0.314992039012
0.602916 0.316614499026
0.607192 0.318190694241
0.611468 0.319719174695
0.615744 0.321365034611
0.62002 0.3229650943
0.624296 0.324517942203
0.628572 0.326196095491
0.632848 0.327740975171
0.637124 0.329415907985
0.6414 0.331045611232
0.645676 0.33262873202
0.649952 0.334257322531
0.654228 0.335934004328
0.658504 0.337565374455
0.66278 0.339150116886
0.667056 0.340785746628
0.671332 0.342475104785
0.675608 0.344119464351
0.679884 0.34582062381
0.68416 0.347477104442
0.688436 0.349087654887
0.692712 0.350758452978
0.696988 0.352383758369
0.701264 0.354072762142
0.70554 0.355828770778
0.709816 0.357428209675
0.714092 0.359095318408
0.718368 0.360833560981
0.722644 0.362528308725
0.72692 0.364178404844
0.731196 0.365904073461
0.735472 0.367586008507
0.739748 0.369347739857
0.744024 0.371066780503
0.7483 0.372742025076
0.752576 0.374372360601
0.756852 0.376088076787
0.761128 0.377893225778
0.765404 0.379522183285
0.76968 0.381241908283
0.773956 0.383056626901
0.778232 0.384690228388
0.782508 0.386420311166
0.786784 0.388251278758
0.79106 0.389896236922
0.795336 0.391643725068
0.799612 0.393348893822
0.803888 0.395162065905
0.808164 0.396934725642
0.81244 0.398665906119
0.816716 0.400354634734
0.820992 0.402159007229
0.825268 0.403922922849
0.829544 0.405645441955
0.83382 0.407325619616
0.838096 0.409129600041
0.842372 0.4108934282
0.846648 0.412616193952
0.850924 0.414470274532
0.8552 0.41611026446
0.859476 0.417883958573
0.863752 0.419796832544
0.868028 0.421490862529
0.872304 0.423326642275
0.87658 0.424937526637
0.880856 0.426881145325
0.885132 0.42859817498
0.889408 0.430273920743
0.893684 0.432102611442
0.89796 0.433892851484
0.902236 0.435643827932
0.906512 0.437556694554
0.910788 0.439229019008
0.915064 0.441066284237
0.91934 0.442865744651
0.923616 0.444626621693
0.927892 0.446348133419
0.932168 0.44824571479
0.936444 0.45010723228
0.94072 0.451710831803
0.944996 0.453495528126
0.949272 0.45546799886
0.953548 0.457177842986
0.957824 0.459079020023
0.9621 0.460711080099
0.966376 0.462538091545
0.970652 0.464328227933
0.974928 0.466322199267
0.979204 0.468039077314
0.98348 0.469963642457
0.987756 0.471604480282
0.992032 0.473456919425
0.996308 0.475273616296
1.000584 0.47705390183
1.00486 0.478797104673
1.009136 0.480765443523
1.013412 0.482435224045
1.017688 0.484334357313
1.021964 0.486199325567
1.02624 0.488029501342
1.030516 0.489824255191
1.034792 0.491582955721
1.039068 0.493587621232
1.043344 0.495275209255
1.04762 0.497213320446
1.051896 0.498827321341
1.056172 0.500696469887
1.060448 0.502531715308
1.064724 0.504332468844
1.069 0.506401459971
1.073276 0.508134483555
1.077552 0.509831257938
1.081828 0.511803644548
1.086104 0.513744756016
1.09038 0.515335407893
1.094656 0.517209219896
1.098932 0.51905010693
1.103208 0.520857522571
1.107484 0.522630919133
1.11176 0.524704177303
1.116036 0.526411100791
1.120312 0.528423249258
1.124588 0.530061568628
1.128864 0.532010545909
1.13314 0.533928806202
1.137416 0.535815849458
1.141692 0.537671174623
1.145968 0.539494279669
1.150244 0.541284661619
1.15452 0.543041816577
1.158796 0.544765239752
1.163072 0.546828652395
1.167348 0.548486531282
1.171624 0.550490298502
1.1759 0.552465274655
1.180176 0.554022915879
1.184452 0.55593543684
1.188728 0.557817786292
1.193004 0.559669508856
1.19728 0.5614901485
1.201556 0.563685086915
1.205832 0.56544579513
1.210108 0.567174067107
1.214384 0.56886944443
1.21866 0.570951838608
1.222936 0.572583728121
1.227212 0.574609110864
1.231488 0.576607211229
1.235764 0.57857762359
1.24004 0.58008098837
1.244316 0.581991034106
1.248592 0.583872154015
1.252868 0.585723940823
1.257144 0.587545986898
1.26142 0.589795880951
1.265696 0.591561084891
1.269972 0.593295341539
1.274248 0.594998242033
1.278524 0.597142938652
1.2828 0.598785835802
1.287076 0.600877620517
1.291352 0.602458948943
1.295628 0.60449632821
1.299904 0.606507949146
1.30418 0.608493455877
1.308456 0.609950990036
1.312732 0.611879135934
1.317008 0.613780081012
1.321284 0.615653468823
1.32556 0.617498942822
1.329836 0.619316146381
1.334112 0.621630879348
1.338388 0.62339464368
1.342664 0.625129085253
1.34694 0.626833847286
1.351216 0.629051524059
1.355492 0.630700099705
1.359768 0.632869398519
1.364044 0.634460431945
1.36832 0.636580067847
1.372596 0.63811220352
1.376872 0.640180891752
1.381148 0.642225799062
1.385424 0.644246621954
1.3897 0.645661281986
1.393976 0.647628624304
1.398252 0.649570954714
1.402528 0.651487970061
1.406804 0.653379367311
1.41108 0.655244843561
1.415356 0.657084096057
1.419632 0.658896822216
1.423908 0.660682719634
1.428184 0.663063496922
1.43246 0.664799386991
1.436736 0.666507559398
1.441012 0.668823443951
1.445288 0.670479884105
1.449564 0.67210771965
1.45384 0.674356254047
1.458116 0.675930636416
1.462392 0.678134466368
1.466668 0.679654262051
1.470944 0.681812322002
1.47522 0.683949460178
1.479496 0.685387626143
1.483772 0.687477416323
1.488048 0.689545521682
1.492324 0.691591693854
1.4966 0.692918755024
1.500876 0.694915493961
1.505152 0.696889539972
1.509428 0.698840645835
1.513704 0.700768564635
1.51798 0.702673049774
1.522256 0.704553854987
1.526532 0.706410734352
1.530808 0.708243442306
1.535084 0.710051733653
1.53936 0.711835363582
1.543636 0.714344951477
1.547912 0.716083523997
1.552188 0.717796718707
1.556464 0.719484292394
1.56074 0.721916951589
1.565016 0.723557615747
1.569292 0.725171947356
1.573568 0.727545880288
1.577844 0.729111929339
1.58212 0.731447340118
1.586396 0.732964205628
1.590672 0.735260255505
1.594948 0.736727039952
1.599224 0.738982893234
1.6035 0.740398702742
1.607776 0.742613526961
1.612052 0.744810137753
1.616328 0.746150437567
1.620604 0.74830479162
1.62488 0.750440342212
1.629156 0.752556898286
1.633432 0.753795261029
1.637708 0.755867945272
1.641984 0.75792104995
1.64626 0.759954385658
1.650536 0.761967763408
1.654812 0.763960994644
1.659088 0.765933891246
1.663364 0.767886265542
1.66764 0.769817930316
1.671916 0.77172869882
1.676192 0.773618384779
1.680468 0.775486802403
1.684744 0.777333766395
1.68902 0.779159091963
1.693296 0.780962594824
1.697572 0.782744091218
1.701848 0.784503397913
1.706124 0.787191513487
1.7104 0.788911436104
1.714676 0.790608635555
1.718952 0.792282930742
1.723228 0.794907568551
1.727504 0.79654110837
1.73178 0.79815121675
1.736056 0.800727959771
1.740332 0.802296301186
1.744608 0.803840688915
1.748884 0.806368120347
1.75316 0.807869738868
1.757436 0.81036540756
1.761712 0.811823602182
1.765988 0.813256988253
1.770264 0.815701024106
1.77454 0.817090000416
1.778816 0.819500757918
1.783092 0.821897527225
1.787368 0.823221565161
1.791644 0.825584176838
1.79592 0.826862215875
1.800196 0.829190080899
1.804472 0.831503255558
1.808748 0.832714022284
1.813024 0.834991585505
1.8173 0.837254044728
1.821576 0.838396165994
1.825852 0.840622158071
1.830128 0.842832636746
1.834404 0.845027470023
1.83868 0.846077920539
1.842956 0.848235167395
1.847232 0.850376365266
1.851508 0.852501384024
1.855784 0.854610093998
1.86006 0.856702365983
1.864336 0.858778071244
1.868612 0.859666950062
1.872888 0.861703166475
1.877164 0.863722423259
1.88144 0.865724593714
1.885716 0.867709551638
1.889992 0.869677171334
1.894268 0.871627327615
1.898544 0.873559895811
1.90282 0.875474751774
1.907096 0.87737177188
1.911372 0.87925083304
1.915648 0.881111812702
1.919924 0.882954588857
1.9242 0.886027516068
1.928476 0.887839609598
1.932752 0.889633145236
1.937028 0.891408003098
1.941304 0.893164063873
1.94558 0.894901208822
1.949856 0.896619319785
1.954132 0.899609538652
1.958408 0.901295373891
1.962684 0.902961831829
1.96696 0.904608796573
1.971236 0.906236152838
1.975512 0.909165836778
1.979788 0.910759814133
1.984064 0.91233384795
1.98834 0.915228435788
1.992616 0.916768446862
1.996892 0.918288184342
2.001168 0.921146769127
2.005444 0.92263184923
2.00972 0.924096330803
2.013996 0.926918017236
2.018272 0.928347216232
2.022548 0.929755497007
2.026824 0.932539401764
2.0311 0.933911784423
2.035376 0.936672103064
2.039652 0.938008186586
2.043928 0.940744543207
2.048204 0.942043930748
2.05248 0.943321678796
2.056756 0.946018251755
2.061032 0.947258711266
2.065308 0.94993039217
2.069584 0.952592641158
2.07386 0.953779602384
2.078136 0.956416419877
2.082412 0.957565140742
2.086688 0.960176168189
2.090964 0.961286273645
2.09524 0.963871156134
2.099516 0.964942275672
2.103792 0.967500661983
2.108068 0.970048840076
2.112344 0.971063972343
2.11662 0.973585138242
2.120896 0.976095845534
2.125172 0.977054193987
2.129448 0.979537381004
2.133724 0.982009862537


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2.tex <==
0.0 0.0900282553096
0.00853 0.0900645934754
0.01706 0.090172769951
0.02559 0.0903516162454
0.03412 0.0906000831503
0.04265 0.0909172346294
0.05118 0.0913022420318
0.05971 0.0917543786124
0.06824 0.0922730143419
0.07677 0.0928576109899
0.0853 0.0935077174666
0.09383 0.0942229654065
0.10236 0.0950030649831
0.11089 0.0958478009388
0.11942 0.0967570288196
0.12795 0.0977306714007
0.13648 0.0987687152947
0.14501 0.0998712077291
0.15354 0.101038253486
0.16207 0.10227001199
0.1706 0.103566694546
0.17913 0.104928561701
0.18766 0.106355920743
0.19619 0.107849123312
0.20472 0.10940856313
0.21325 0.111034673827
0.22178 0.112727926882
0.23031 0.114488829646
0.23884 0.116317923459
0.24737 0.118215781851
0.2559 0.120183008826
0.26443 0.122220237213
0.27296 0.124328127098
0.28149 0.126507364313
0.29002 0.128758659001
0.29855 0.131082744228
0.30708 0.133480374663
0.31561 0.135952325305
0.32414 0.138499390266
0.33267 0.141122381601
0.3412 0.143822128183
0.34973 0.146599474623
0.35826 0.149455280234
0.36679 0.152390418031
0.37532 0.155405773772
0.38385 0.15850224503
0.39238 0.16168074031
0.40091 0.164942178185
0.40944 0.168287486473
0.41797 0.171717601441
0.4265 0.175233467038
0.43503 0.178836034151
0.44356 0.182526259894
0.45209 0.186305106917
0.46062 0.19017354274
0.46915 0.194132539111
0.47768 0.198183071385
0.48621 0.202326117922
0.49474 0.206562659507
0.50327 0.210893678792
0.5118 0.215320159751
0.52033 0.219843087155
0.52886 0.224463446067
0.53739 0.229182221348
0.54592 0.234000397183
0.55445 0.238918956622
0.56298 0.243938881131
0.57151 0.249061150164
0.58004 0.25428674074
0.58857 0.259616627045
0.5971 0.265051780033
0.60563 0.270593167048
0.61416 0.276241751458
0.62269 0.281998492292
0.63122 0.287864343897
0.63975 0.293840255602
0.64828 0.299927171391
0.65681 0.302793805764
0.66534 0.302867249126
0.67387 0.302943870435
0.6824 0.303082513628
0.69093 0.303283863577
0.69946 0.303518435722
0.70799 0.303786374453
0.71652 0.304118675545
0.72505 0.304485358715
0.73358 0.304886786418
0.74211 0.305323389329
0.75064 0.305795667791
0.75917 0.306304193363
0.7677 0.306849610486
0.77623 0.307465462797
0.78476 0.30808721985
0.79329 0.308748265715
0.80182 0.30941573574
0.81035 0.310157957034
0.81888 0.310908048022
0.82741 0.31170101014
0.83594 0.312502852185
0.84447 0.313349432856
0.853 0.314242179531
0.86153 0.315109748203
0.87006 0.316061831095
0.87859 0.317026828498
0.88712 0.318005254452
0.89565 0.318997673104
0.90418 0.320043258637
0.91271 0.321105023458
0.92124 0.322183716334
0.92977 0.323280142323
0.9383 0.324395164275
0.94683 0.32552970436
0.95536 0.32672615208
0.96389 0.327903246131
0.97242 0.329103005827
0.98095 0.330369561773
0.98948 0.3316187809
0.99801 0.332850370544
1.00654 0.334153227805
1.01507 0.335440165747
1.0236 0.336802441393
1.03213 0.338104455861
1.04066 0.339485032081
1.04919 0.340852673113
1.05772 0.342255463845
1.06625 0.343646528556
1.07478 0.34507527979
1.08331 0.346493705084
1.09184 0.347952588316
1.10037 0.349402745653
1.1089 0.350896376893
1.11743 0.352383091386
1.12596 0.353863186144
1.13449 0.355391053536
1.14302 0.3569144106
1.15155 0.358489178331
1.16008 0.360005543477
1.16861 0.361575747675
1.17714 0.363202574707
1.18567 0.364771919269
1.1942 0.366341384827
1.20273 0.367971687713
1.21126 0.369605069437
1.21979 0.371242303489
1.22832 0.372884203547
1.23685 0.374531624208
1.24538 0.376185461728
1.25391 0.377846654753
1.26244 0.379516185053
1.27097 0.381261795291
1.2795 0.38295200306
1.28803 0.384653770518
1.29656 0.386368259304
1.30509 0.388096677812
1.31362 0.389840281909
1.32215 0.391528202453
1.33068 0.393305189835
1.33921 0.395027330408
1.34774 0.396843265784
1.35627 0.398605345667
1.3648 0.400389170778
1.37333 0.402118283342
1.38186 0.40394935187
1.39039 0.405726956068
1.39892 0.407530822786
1.40745 0.409362703245
1.41598 0.41122440384
1.42451 0.41303348801
1.43304 0.414874000845
1.44157 0.416661402076
1.4501 0.418569536551
1.45863 0.420337661201
1.46716 0.422230612001
1.47569 0.424071954753
1.48422 0.425952553077
1.49275 0.427874623891
1.50128 0.429745960098
1.50981 0.431565326085
1.51834 0.433525227979
1.52687 0.435337422978
1.5354 0.437294988334
1.54393 0.439203001405
1.55246 0.441060282097
1.56099 0.442968710898
1.56952 0.444930913435
1.57805 0.446843946998
1.58658 0.448813598483
1.59511 0.450734405483
1.60364 0.452605242848
1.61217 0.454535879203
1.6207 0.456529216761
1.62923 0.458474612723
1.63776 0.460370982809
1.64629 0.462333603904
1.65482 0.464365569453
1.66335 0.466350862999
1.67188 0.468288444407
1.68041 0.47017726768
1.68894 0.47226324202
1.69747 0.474179242026
1.706 0.476172686977
1.71453 0.478119097078
1.72306 0.480146864358
1.73159 0.482128602448
1.74012 0.484195762467
1.74865 0.486084035892
1.75718 0.488194366069
1.76571 0.490123900012
1.77424 0.492144287468
1.78277 0.494119085034
1.7913 0.496189189709
1.79983 0.498215052136
1.80836 0.500195765124
1.81689 0.502277123142
1.82542 0.504314803555
1.83395 0.506307923509
1.84248 0.508407291608
1.85101 0.510463697951
1.85954 0.512476285089
1.86807 0.514444191897
1.8766 0.516525080936
1.88513 0.518563035441
1.89366 0.520557220936
1.90219 0.522670586997
1.91072 0.5247420623
1.91925 0.526770839993
1.92778 0.528925275337
1.93631 0.530868041936
1.94484 0.53293849824
1.95337 0.535141357402
1.9619 0.537128372788
1.97043 0.53924996047
1.97896 0.541330709201
1.98749 0.543369864729
1.99602 0.545550748515
2.00455 0.547506366432
2.01308 0.549606062215
2.02161 0.551665031498
2.03014 0.55387439482
2.03867 0.555851698284
2.0472 0.55798190862
2.05573 0.560072480245
2.06426 0.562322545037
2.07279 0.564333768483
2.08132 0.566507163787
2.08985 0.568642234158
2.09838 0.570738311538
2.10691 0.572794725995
2.11544 0.574810805744
2.12397 0.577000182416
2.1325 0.579152116071
2.14103 0.581265968658
2.14956 0.583341100487
2.15809 0.585599738402
2.16662 0.587597676265
2.17515 0.589782206204
2.18368 0.591929853342
2.19221 0.594040009535
2.20074 0.596112065244
2.20927 0.598381518332
2.2178 0.600377791632
2.22633 0.602574768891
2.23486 0.604735765909
2.24339 0.606860206057
2.25192 0.608947511547
2.26045 0.611246929877
2.26898 0.613260560418
2.27751 0.615489834213
2.28604 0.617684382144
2.29457 0.619843660537
2.3031 0.62196712477
2.31163 0.624054229295
2.32016 0.626370860873
2.32869 0.62838603081
2.33722 0.630634509298
2.34575 0.632849353658
2.35428 0.635030053662
2.36281 0.637176098343
2.37134 0.639286976028
2.37987 0.641645862772
2.3884 0.643687386414
2.39693 0.645980954504
2.40546 0.648242403844
2.41399 0.650177420011
2.42252 0.652370634669
2.43105 0.654829283217
2.43958 0.656957498789
2.44811 0.659051213685
2.45664 0.661416773773
2.46517 0.663442689754
2.4737 0.665744793064
2.48223 0.668015820371
2.49076 0.670255331691
2.49929 0.67246288671
2.50782 0.674638044804
2.51635 0.676780365061
2.52488 0.678889406299
2.53341 0.681295750283
2.54194 0.683339663378
2.55047 0.685685530436
2.559 0.688001925464
2.56753 0.689946327139
2.57606 0.692199762729
2.58459 0.694422503934
2.59312 0.696614147408
2.60165 0.699127711737
2.61018 0.701258807902
2.61871 0.703357608877
2.62724 0.705785747113
2.63577 0.707821644521
2.6443 0.710191892503
2.65283 0.71253409041
2.66136 0.714847873668
2.66989 0.717132877749
2.67842 0.719388738191
2.68695 0.721615090608
2.69548 0.723811570714
2.70401 0.725977814333
2.71254 0.728113457422
2.72107 0.730612750004
2.7296 0.732689139762
2.73813 0.735134554811
2.74666 0.737150288682
2.75519 0.739540475913
2.76372 0.741904088098
2.77225 0.744240801145
2.78078 0.746550291202
2.78931 0.748832234677
2.79784 0.751086308251
2.80637 0.753312188894
2.8149 0.755509553882
2.82343 0.757678080807
2.83196 0.760252557327
2.84049 0.762365646815
2.84902 0.764890475546
2.85755 0.766946893219
2.86608 0.769420892155
2.87461 0.771870660618
2.88314 0.773841396923
2.89167 0.776238581174
2.9002 0.778610678633
2.90873 0.780957408954
2.91726 0.783278492255
2.92579 0.785573649132
2.93432 0.787842600671
2.94285 0.790085068467
2.95138 0.792781878241
2.95991 0.794973925165
2.96844 0.797138668916
2.97697 0.799767111132
2.9855 0.801879837884
2.99403 0.804462569668
3.00256 0.806522229481
3.01109 0.809058253449
3.01962 0.811572283373
3.02815 0.813552125005
3.03668 0.816017972931
3.04521 0.818461111389
3.05374 0.820881307413
3.06227 0.82327832874
3.0708 0.825651943822
3.07933 0.82800192185
3.08786 0.830328032761
3.09639 0.832630047262
3.10492 0.834907736839
3.11345 0.837708289782
3.12198 0.839940261364
3.13051 0.842147239804
3.13904 0.844887291864
3.14757 0.847047260732
3.1561 0.849747179259
3.16463 0.851859294516
3.17316 0.854518288701
3.18169 0.856581713633
3.19022 0.859199000176
3.19875 0.861797002462
3.20728 0.863787709118
3.21581 0.866342855977
3.22434 0.86887816788
3.23287 0.871393467515
3.2414 0.873888578679
3.24993 0.876363326299
3.25846 0.878817536457
3.26699 0.881251036418
3.27552 0.883663654649
3.28405 0.88605522085
3.29258 0.88842556598
3.30111 0.891404246883
3.30964 0.893735531148
3.31817 0.896045107559
3.3267 0.898332812402
3.33523 0.901243810574
3.34376 0.903491220151
3.35229 0.906369489014
3.36082 0.908576016104
3.36935 0.911421024746
3.37788 0.913586094553
3.38641 0.916397324994
3.39494 0.91852037575
3.40347 0.921297323583
3.412 0.924058959593
3.42053 0.926119982273
3.42906 0.928846618783
3.43759 0.931557612656
3.44612 0.934252861885
3.45465 0.936230774285
3.46318 0.938890131513
3.47171 0.941533438087
3.48024 0.944160600788
3.48877 0.946771528766
3.4973 0.949366133608
3.50583 0.951944329411
3.51436 0.954506032858
3.52289 0.957051163298
3.53142 0.960318552287
3.53995 0.962834529465
3.54848 0.965333721987
3.55701 0.9678160608
3.56554 0.970281479972
3.57407 0.973490071976
3.5826 0.975925758746
3.59113 0.978344361742
3.59966 0.981518892426
3.60819 0.983907508256
3.61672 0.986278908904
3.62525 0.989419152014
3.63378 0.991760380633
3.64231 0.994879155629
3.65084 0.997190141451
3.65937 1.00028745388
3.6679 1.00337626243
3.67643 1.00564405955
3.68496 1.00871150529
3.69349 1.0117705443
3.70202 1.01399526577
3.71055 1.01703314505
3.71908 1.02006277048
3.72761 1.02224469124
3.73614 1.02525347755
3.74467 1.02825422648
3.7532 1.03124703131
3.76173 1.03423199398
3.77026 1.03720922551
3.77879 1.04017884642
3.78732 1.04226927026
3.79585 1.04521940623
3.80438 1.04816233782
3.81291 1.05109822878
3.82144 1.05402725522
3.82997 1.05694960635
3.8385 1.06076546944
3.84703 1.06367987045
3.85556 1.06658826987
3.86409 1.06949091793
3.87262 1.07238808249
3.88115 1.07528005012
3.88968 1.07816712737
3.89821 1.08198347476
3.90674 1.08486669947
3.91527 1.08774611
3.9238 1.0915707619
3.93233 1.09444876839
3.94086 1.09732427673
3.94939 1.10116146736
3.95792 1.10403856002
3.96645 1.10691476936
3.97498 1.11076965344
3.98351 1.11365111315
3.99204 1.11752293959
4.00057 1.12041257964
4.0091 1.12430461315
4.01763 1.12720582218
4.02616 1.13112183731
4.03469 1.1340385552
4.04322 1.13798294219
4.05175 1.14091977883
4.06028 1.14489768012
4.06881 1.14786006996
4.07734 1.15187755938
4.08587 1.15592024976
4.0944 1.15893628831
4.10293 1.16303001667
4.11146 1.16715560562
4.11999 1.17131577345
4.12852 1.17443677378
4.13705 1.17866966537
4.14558 1.18294726742
4.15411 1.18727386008
4.16264 1.19055369793
4.17117 1.19498743649
4.1797 1.19948694816
4.18823 1.20405971805
4.19676 1.20871456253
4.20529 1.21232977173
4.21382 1.21717588683
4.22235 1.2221428803
4.23088 1.22725050413
4.23941 1.23252433471
4.24794 1.23799868254
4.25647 1.24372181311


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt05.tex <==
0.0 0.063045006828
0.008276 0.0630929904667
0.016552 0.0632354443447
0.024828 0.0634703466344
0.033104 0.0637959686838
0.04138 0.0642108544897
0.049656 0.0647138017242
0.057932 0.0653038441889
0.066208 0.0659802355847
0.074484 0.0667424344872
0.08276 0.0675900904331
0.091036 0.068523031026
0.099312 0.0695412499786
0.107588 0.070644896016
0.115864 0.0718342625686
0.12414 0.0731097781919
0.132416 0.0744719976537
0.140692 0.0759215936348
0.148968 0.0774593489937
0.157244 0.0790861495514
0.16552 0.0808029773532
0.173796 0.082610904371
0.182072 0.0845110866125
0.190348 0.086504758603
0.198624 0.0885932282147
0.2069 0.0907778718145
0.215176 0.0930601297069
0.223452 0.0954415018518
0.231728 0.0979235438341
0.240004 0.10050786307
0.24828 0.103196115229
0.256556 0.105990000863
0.264832 0.108891262221
0.273108 0.111901680239
0.281384 0.115023071697
0.28966 0.118257286525
0.297936 0.121606205258
0.306212 0.125071736616
0.314488 0.128655815218
0.322764 0.132360399404
0.33104 0.136187469179
0.339316 0.140139024244
0.347592 0.14421708214
0.355868 0.148423676473
0.364144 0.152760855224
0.37242 0.157230679148
0.380696 0.161835220241
0.388972 0.166576560278
0.397248 0.171456789427
0.405524 0.176478004915
0.4138 0.181642309765
0.422076 0.186951811581
0.430352 0.192408621392
0.438628 0.198014852543
0.446904 0.203772619636
0.45518 0.209684037519
0.463456 0.212450042882
0.471732 0.212503564887
0.480008 0.212630779006
0.488284 0.212811034847
0.49656 0.213044783834
0.504836 0.213332660738
0.513112 0.213675487716
0.521388 0.214074279036
0.529664 0.214507348379
0.53794 0.215021612386
0.546216 0.21554908769
0.554492 0.216137343875
0.562768 0.216764238301
0.571044 0.217430981572
0.57932 0.218138951783
0.587596 0.218889700516
0.595872 0.219684959207
0.604148 0.220500712929
0.612424 0.221364217278
0.6207 0.222251015722
0.628976 0.223189484925
0.637252 0.224154704804
0.645528 0.225148227731
0.653804 0.226171759
0.66208 0.227227162512
0.670356 0.228316466643
0.678632 0.229411966324
0.686908 0.230544934876
0.695184 0.23171789067
0.70346 0.232902090903
0.711736 0.234098812578
0.720012 0.235341996185
0.728288 0.236601756286
0.736564 0.237879786547
0.74484 0.239177916262
0.753116 0.240498114867
0.761392 0.24184249652
0.769668 0.243213324746
0.777944 0.244576227336
0.78622 0.245969247312
0.794496 0.247395080919
0.802772 0.248817777757
0.811048 0.250277779646
0.819324 0.251738019879
0.8276 0.253199650545
0.835876 0.254705630565
0.844152 0.256217119382
0.852428 0.257735613111
0.860704 0.259262714822
0.86898 0.260844976112
0.877256 0.262395363996
0.885532 0.263959855129
0.893808 0.265540509932
0.902084 0.267139510515
0.91036 0.268759163664
0.918636 0.270401903818
0.926912 0.272019404457
0.935188 0.273663401841
0.943464 0.275283923996
0.95174 0.276988453438
0.960016 0.278618861217
0.968292 0.280339454001
0.976568 0.281986455602
0.984844 0.283730305565
0.99312 0.285401396874
1.001396 0.287116707356
1.009672 0.288880002702
1.017948 0.29057129733
1.026224 0.292314167418
1.0345 0.294048579085
1.042776 0.295840743362
1.051052 0.297562145337
1.059328 0.299345629734
1.067604 0.301127027398
1.07588 0.302907553069
1.084156 0.30468849215
1.092432 0.306471202
1.100708 0.308257113241
1.108984 0.310122758727
1.11726 0.311920956153
1.125536 0.313727117031
1.133812 0.31554297801
1.142088 0.317370355395
1.150364 0.319211146416
1.15864 0.321067330481
1.166916 0.322856520378
1.175192 0.324748344446
1.183468 0.326574681506
1.191744 0.328422245704
1.20002 0.330293388971
1.208296 0.33219055228
1.216572 0.334023031535
1.224848 0.335883624852
1.233124 0.337774989293
1.2414 0.339699875218
1.249676 0.341561662142
1.257952 0.343459543802
1.266228 0.34529380503
1.274504 0.347271261847
1.28278 0.349082021642
1.291056 0.351042303168
1.299332 0.352941702541
1.307608 0.354889571106
1.315884 0.356776522111
1.32416 0.358715434065
1.332436 0.360593526915
1.340712 0.36252728625
1.348988 0.364400462824
1.357264 0.366333229971
1.36554 0.368329487321
1.373816 0.370267666713
1.382092 0.372146184502
1.390368 0.374092836674
1.398644 0.376111832535
1.40692 0.37807419884
1.415196 0.379978423605
1.423472 0.38196025655
1.431748 0.383884932117
1.440024 0.385750966511
1.4483 0.387843658356
1.456576 0.389737558686
1.464852 0.391720132543
1.473128 0.39364658018
1.481404 0.395667343491
1.48968 0.397633479437
1.497956 0.39954361974
1.506232 0.401554802777
1.514508 0.403511685064
1.522784 0.405412934829
1.53106 0.407422378634
1.539336 0.409378086537
1.547612 0.411448539983
1.555888 0.413467334395
1.564164 0.415433224369
1.57244 0.417344957619
1.580716 0.419380521543
1.588992 0.421364245196
1.597268 0.423294919054
1.605544 0.425357904267
1.61382 0.427370373694
1.622096 0.429331162511
1.630372 0.431433203979
1.638648 0.433289664363
1.646924 0.435290164918
1.6552 0.437441304649
1.663476 0.439340917908
1.671752 0.441394185959
1.680028 0.443398206916
1.688304 0.445351900688
1.69658 0.447469320637
1.704856 0.449321827395
1.713132 0.451341375893
1.721408 0.453535185442
1.729684 0.455458229026
1.73796 0.457559087677
1.746236 0.459613388369
1.754512 0.461620145632
1.762788 0.463578369951
1.771064 0.465487067831
1.77934 0.467588672162
1.787616 0.469644655206
1.795892 0.471654078437
1.804168 0.47361599975
1.812444 0.475784850693
1.82072 0.477651969672
1.828996 0.47973024701
1.837272 0.481763416749
1.845548 0.483750586957
1.853824 0.48596168237
1.8621 0.487857321129
1.870376 0.489981444314
1.878652 0.492062395686
1.886928 0.494099336018
1.895204 0.496091423372
1.90348 0.498037813153
1.911756 0.500231054373
1.920032 0.50208682042
1.928308 0.50419441417
1.936584 0.50625965276
1.94486 0.508281747241
1.953136 0.510570116236
1.961412 0.512506977542
1.969688 0.514398337317
1.977964 0.516563970378
1.98624 0.518689504665
1.994516 0.520774206886
2.002792 0.522817341852
2.011068 0.524818172528
2.019344 0.526775960071
2.02762 0.529031885852
2.035896 0.530905001577
2.044172 0.533082092541
2.052448 0.535220559842
2.060724 0.537319725017
2.069 0.539378908108
2.077276 0.541397427707
2.085552 0.543374600995
2.093828 0.545309743782
2.102104 0.547577672693
2.11038 0.549430542375
2.118656 0.551622562113
2.126932 0.553777609315
2.135208 0.555895062384
2.143484 0.557974298612
2.15176 0.560014694215
2.160036 0.562015624375
2.168312 0.563976463274
2.176588 0.566307535958
2.184864 0.568190364552
2.19314 0.570450324681
2.201416 0.572252720311
2.209692 0.574439233415
2.217968 0.576590218687
2.226244 0.578705113008
2.23452 0.580783352532
2.242796 0.582824372719
2.251072 0.584827608368
2.259348 0.58679249365
2.267624 0.589175272764
2.2759 0.591066063639
2.284176 0.593382272741
2.292452 0.595196790359
2.300728 0.597444339637
2.309004 0.599658973174
2.31728 0.601357196984
2.325556 0.603500051658
2.333832 0.605608463244
2.342108 0.607681929427
2.350384 0.609719947556
2.35866 0.611722014672
2.366936 0.614197621159
2.375212 0.616130855536
2.383488 0.618026651022
2.391764 0.620408303323
2.40004 0.622232355915
2.408316 0.624550596175
2.416592 0.62683878745
2.424868 0.628553969339
2.433144 0.630776013884
2.44142 0.63296667507
2.449696 0.635125515339
2.457972 0.637252097055
2.466248 0.639345982533
2.474524 0.64140673406
2.4828 0.643433913924
2.491076 0.645427084436
2.499352 0.647385807954
2.507628 0.649900540968
2.515904 0.65179401676
2.52418 0.654252589128
2.532456 0.656079155769
2.540732 0.658479994285
2.549008 0.660237991196
2.557284 0.662579523393
2.56556 0.664267291206
2.573836 0.666547945714
2.582112 0.668800139401
2.590388 0.671023501647
2.598664 0.673217662006
2.60694 0.675382250225
2.615216 0.677516896271
2.623492 0.679621230343
2.631768 0.6816948829
2.640044 0.683737484676
2.64832 0.685748666703
2.656596 0.687728060329
2.664872 0.68967529724
2.673148 0.692284211456
2.681424 0.694171421949
2.6897 0.696025394114
2.697976 0.698556197271
2.706252 0.700348046404
2.714528 0.702826942706
2.722804 0.70455528882
2.73108 0.706980983435
2.739356 0.709382360691
2.747632 0.711015650899
2.755908 0.713361910587
2.764184 0.715682927732
2.77246 0.717978401564
2.780736 0.719482129617
2.789012 0.721719956606
2.797288 0.723931320026
2.805564 0.726115920811
2.81384 0.728273460343
2.822116 0.730403640471
2.830392 0.732506163529
2.838668 0.734580732347
2.846944 0.736627050268
2.85522 0.739462385777
2.863496 0.741457154465
2.871772 0.743422805326
2.880048 0.74535904385
2.888324 0.747265576117
2.8966 0.749989071161
2.904876 0.75184125032
2.913152 0.75452172221
2.921428 0.7563184578
2.929704 0.758084065613
2.93798 0.760695101949
2.946256 0.762403619724
2.954532 0.764969094913
2.962808 0.767514450069
2.971084 0.769138358018
2.97936 0.771636672744
2.987636 0.773200822194
2.995912 0.77565110337
3.004188 0.778080079698
3.012464 0.780487523345
3.02074 0.781935168693
3.029016 0.784292644427
3.037292 0.786627888876
3.045568 0.788940676496
3.053844 0.791230782328
3.06212 0.793497982008
3.070396 0.794766409404
3.078672 0.796980795718
3.086948 0.799171588536
3.095224 0.801338566063
3.1035 0.803481507154
3.111776 0.806607664391
3.120052 0.808708291199
3.128328 0.810784239726
3.136604 0.812835291468
3.14488 0.814861228627
3.153156 0.816861834122
3.161432 0.818836891598
3.169708 0.821838956966
3.177984 0.82376881299
3.18626 0.825672493432
3.194536 0.827549784871
3.202812 0.830479507309
3.211088 0.832309991924
3.219364 0.83411346871
3.22764 0.836988631315
3.235916 0.838744120502
3.244192 0.841584222878
3.252468 0.843290955519
3.260744 0.846095297186
3.26902 0.847752510132
3.277296 0.850520395853
3.285572 0.852127331898
3.293848 0.854858071822
3.302124 0.856413979851
3.3104 0.85910688966
3.318676 0.860611024793
3.326952 0.863265425838
3.335228 0.865903742849
3.343504 0.86733226902
3.35178 0.869931085654
3.360056 0.872513348789
3.368332 0.873864672576
3.376608 0.876406456787
3.384884 0.878931224325
3.39316 0.881438827216
3.401436 0.883929118165
3.409712 0.885152947892
3.417988 0.887601178988
3.426264 0.890031645796
3.43454 0.8924442039
3.442816 0.894838709609
3.451092 0.897215019959
3.459368 0.899572992723
3.467644 0.901912486421
3.47592 0.902927972114
3.484196 0.905222974558
3.492472 0.907499064057
3.500748 0.909756102274
3.509024 0.911993951657
3.5173 0.91421247545
3.525576 0.9164115377
3.533852 0.919946464518
3.542128 0.922113407093
3.550404 0.924260498615
3.55868 0.926387606347
3.566956 0.928494598399
3.575232 0.930581343729
3.583508 0.93264771216
3.591784 0.934693574382
3.60006 0.938132292941
3.608336 0.94014407175
3.616612 0.942134974564
3.624888 0.944104875558
3.633164 0.946053649818
3.64144 0.949431352051
3.649716 0.951344878641
3.657992 0.953236921789
3.666268 0.956579699541
3.674544 0.958435827014
3.68282 0.960270122421
3.691096 0.962082467322
3.699372 0.965374805371
3.707648 0.967150360513
3.715924 0.970420618321
3.7242 0.972158969633
3.732476 0.973874816873
3.740752 0.977107525041
3.749028 0.978785549361
3.757304 0.981995271442
3.76558 0.983635077487
3.773856 0.986821468246
3.782132 0.9884226684
3.790408 0.990000633021
3.798684 0.993147604516
3.80696 0.994686385436
3.815236 0.99780918391
3.823512 1.00092358371
3.831788 1.00240672073
3.840064 1.00549648373
3.84834 1.00693954561
3.856616 1.01000436539
3.864892 1.01140700613
3.873168 1.01444658471
3.881444 1.01747727948
3.88972 1.01882251539
3.897996 1.02182754903
3.906272 1.02313154927
3.914548 1.02611064596
3.922824 1.02908054594
3.9311 1.03032599018
3.939376 1.03326956762
3.947652 1.03620377664
3.955928 1.03912856588
3.964204 1.04029754708
3.97248 1.04319554092
3.980756 1.0460839582
3.989032 1.0489627527
3.997308 1.05005424237
4.005584 1.05290581041
4.01386 1.05574761503
4.022136 1.05857961558
4.030412 1.05959267326
4.038688 1.06239706141
4.046964 1.06519152239
4.05524 1.06797602163
4.063516 1.07075052617
4.071792 1.0735150047
4.080068 1.07441283562
4.088344 1.07714922614
4.09662 1.07987549691
4.104896 1.08259162364
4.113172 1.08529758388
4.121448 1.0879933571
4.129724 1.09067892476


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt1.tex <==
0.0 0.667616837054
0.0841218682305 0.672852075515
0.168243736461 0.688044582385
0.252365604692 0.712701125396
0.336487472922 0.746158671838
0.420609341153 0.787679970271
0.504731209383 0.836219008942
0.588853077614 0.890833907482
0.672974945844 0.950212032527
0.757096814075 1.01377162623
0.841218682305 1.0810332708
0.925340550536 1.15075696393
1.00946241877 1.22293118237
1.093584287 1.29677003707
1.17770615523 1.37245400874
1.26182802346 1.44965750716
1.34594989169 1.5279938986
1.43007175992 1.60713440563
1.51419362815 1.68703332162
1.59831549638 1.76825759909
1.68243736461 1.84967668353
1.76655923284 1.93213604894
1.85068110107 2.01636548398
1.9348029693 2.09934671387
2.01892483753 2.18428424866
2.10304670576 2.26898060596
2.18716857399 2.3546113305
2.27129044222 2.44011892237
2.35541231046 2.52636666536
2.43953417869 2.6141897773
2.52365604692 2.70172631064
2.60777791515 2.78932522965
2.69189978338 2.88002720961
2.77602165161 2.96840581225
2.86014351984 3.06004366061
2.94426538807 3.14885446937
3.0283872563 3.24328274545
3.11250912453 3.33362000864
3.19663099276 3.42797363904
3.28075286099 3.52506993351
3.36487472922 3.62016798946
3.44899659745 3.7172212282
3.53311846568 3.81648788735
3.61724033391 3.91743145217
3.70136220214 4.01855051764
3.78548407037 4.12265104793
3.8696059386 4.23030852394
3.95372780684 4.33917717162
4.03784967507 4.45010006914
4.1219715433 4.56498180311


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt3.tex <==
0.0 1.18705533876
0.0608288216233 1.18878960072
0.121657643247 1.1938197879
0.18248646487 1.20219676905
0.243315286493 1.21354510197
0.304144108116 1.22801966935
0.36497292974 1.24571095471
0.425801751363 1.26638778559
0.486630572986 1.28999358549
0.54745939461 1.31635415887
0.608288216233 1.34554259515
0.669117037856 1.3775324817
0.72994585948 1.41169043461
0.790774681103 1.44843553006
0.851603502726 1.48728824882
0.912432324349 1.52839953683
0.973261145973 1.57128270743
1.0340899676 1.61578679094
1.09491878922 1.6621974226
1.15574761084 1.70991858466
1.21657643247 1.75942198422
1.27740525409 1.81015198404
1.33823407571 1.86188038039
1.39906289734 1.91528329884
1.45989171896 1.96926658294
1.52072054058 2.02506503537
1.58154936221 2.08146756031
1.64237818383 2.13869973711
1.70320700545 2.19702944566
1.76403582708 2.25612387324
1.8248646487 2.31622107609
1.88569347032 2.3768818732
1.94652229195 2.43899619488
2.00735111357 2.5013203355
2.06817993519 2.5654661761
2.12900875682 2.62924282069
2.18983757844 2.69422500026
2.25066640006 2.76044309863
2.31149522169 2.82700014782
2.37232404331 2.8954761347
2.43315286493 2.96391994636
2.49398168656 3.03286217469
2.55481050818 3.10366991147
2.6156393298 3.17484528048
2.67646815143 3.24743244809
2.73729697305 3.32038373172
2.79812579467 3.39508464724
2.85895461629 3.47055376252
2.91978343792 3.54777289321
2.98061225954 3.62714100814


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt6.tex <==
0.0 1.74826716143
0.0396220919817 1.74879512228
0.0792441839634 1.75029653747
0.118866275945 1.75306628167
0.158488367927 1.75666139316
0.198110459909 1.76149461
0.23773255189 1.76724158239
0.277354643872 1.77400758023
0.316976735854 1.78189769123
0.356598827835 1.79071424281
0.396220919817 1.80071656853
0.435843011799 1.81170894849
0.475465103781 1.82381040736
0.515087195762 1.83682846183
0.554709287744 1.85106610502
0.594331379726 1.86617998573
0.633953471707 1.88250574517
0.673575563689 1.89971017531
0.713197655671 1.91817054003
0.752819747653 1.93738344301
0.792441839634 1.95776346673
0.832063931616 1.97899997229
0.871686023598 2.00136470466
0.911308115579 2.02455641797
0.950930207561 2.04867602809
0.990552299543 2.0736325817
1.03017439152 2.09955819706
1.06979648351 2.126383822
1.10941857549 2.15381230109
1.14904066747 2.18223725718
1.18866275945 2.21137227531
1.22828485143 2.2414068084
1.26790694341 2.27204696169
1.3075290354 2.3034962295
1.34715112738 2.33571596055
1.38677321936 2.36839627566
1.42639531134 2.40203254425
1.46601740332 2.43603507492
1.50563949531 2.47091510746
1.54526158729 2.5063451711
1.58488367927 2.54226795163
1.62450577125 2.57891958918
1.66412786323 2.61623906891
1.70374995521 2.65415296521
1.7433720472 2.69257345162
1.78299413918 2.7317116917
1.82261623116 2.77113496945
1.86223832314 2.81166060198
1.90186041512 2.85314223671
1.9414825071 2.89574201706


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2pt01.tex <==
0.0 0.667616837054
0.0841218682305 0.672852075515
0.168243736461 0.688044582385
0.252365604692 0.712701125396
0.336487472922 0.746158671838
0.420609341153 0.787679970271
0.504731209383 0.836219008942
0.588853077614 0.890833907482
0.672974945844 0.950212032527
0.757096814075 1.01377162623
0.841218682305 1.0810332708
0.925340550536 1.15075696393
1.00946241877 1.22293118237
1.093584287 1.29677003707
1.17770615523 1.37245400874
1.26182802346 1.44965750716
1.34594989169 1.5279938986
1.43007175992 1.60713440563
1.51419362815 1.68703332162
1.59831549638 1.76825759909
1.68243736461 1.84967668353
1.76655923284 1.93213604894
1.85068110107 2.01636548398
1.9348029693 2.09934671387
2.01892483753 2.18428424866
2.10304670576 2.26898060596
2.18716857399 2.3546113305
2.27129044222 2.44011892237
2.35541231046 2.52636666536
2.43953417869 2.6141897773
2.52365604692 2.70172631064
2.60777791515 2.78932522965
2.69189978338 2.88002720961
2.77602165161 2.96840581225
2.86014351984 3.06004366061
2.94426538807 3.14885446937
3.0283872563 3.24328274545
3.11250912453 3.33362000864
3.19663099276 3.42797363904
3.28075286099 3.52506993351
3.36487472922 3.62016798946
3.44899659745 3.7172212282
3.53311846568 3.81648788735
3.61724033391 3.91743145217
3.70136220214 4.01855051764
3.78548407037 4.12265104793
3.8696059386 4.23030852394
3.95372780684 4.33917717162
4.03784967507 4.45010006914
4.1219715433 4.56498180311


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma4prob0pt3.tex <==
0.0 2.37411067752
0.121657643247 2.37757920143
0.243315286493 2.3876395758
0.36497292974 2.40439353809
0.486630572986 2.42709020395
0.608288216233 2.4560393387
0.72994585948 2.49142190942
0.851603502726 2.53277557117
0.973261145973 2.57998717097
1.09491878922 2.63270831774
1.21657643247 2.69108519031
1.33823407571 2.7550649634
1.45989171896 2.82338086923
1.58154936221 2.89687106012
1.70320700545 2.97457649765
1.8248646487 3.05679907367
1.94652229195 3.14256541486
2.06817993519 3.23157358187
2.18983757844 3.32439484521
2.31149522169 3.41983716933
2.43315286493 3.51884396844
2.55481050818 3.62030396808
2.67646815143 3.72376076078
2.79812579467 3.83056659767
2.91978343792 3.93853316587
3.04144108116 4.05013007075
3.16309872441 4.16293512062
3.28475636766 4.27739947422
3.4064140109 4.39405889132
3.52807165415 4.51224774648
3.6497292974 4.63244215218
3.77138694064 4.7537637464
3.89304458389 4.87799238976
4.01470222714 5.002640671
4.13635987038 5.13093235221
4.25801751363 5.25848564139
4.37967515688 5.38845000052
4.50133280012 5.52088619727
4.62299044337 5.65400029565
4.74464808662 5.7909522694
4.86630572986 5.92783989273
4.98796337311 6.06572434938
5.10962101636 6.20733982293
5.2312786596 6.34969056096
5.35293630285 6.49486489618
5.4745939461 6.64076746344
5.59625158934 6.79016929448
5.71790923259 6.94110752504
5.83956687584 7.09554578643
5.96122451908 7.25428201627


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt3.tex <==
0.0 4.74822135504
0.243315286493 4.75515840287
0.486630572986 4.77527915161
0.72994585948 4.80878707619
0.973261145973 4.85418040789
1.21657643247 4.91207867741
1.45989171896 4.98284381883
1.70320700545 5.06555114234
1.94652229195 5.15997434194
2.18983757844 5.26541663549
2.43315286493 5.38217038061
2.67646815143 5.5101299268
2.91978343792 5.64676173845
3.16309872441 5.79374212024
3.4064140109 5.9491529953
3.6497292974 6.11359814733
3.89304458389 6.28513082972
4.13635987038 6.46314716375
4.37967515688 6.64878969041
4.62299044337 6.83967433865
4.86630572986 7.03768793689
5.10962101636 7.24060793616
5.35293630285 7.44752152156
5.59625158934 7.66113319534
5.83956687584 7.87706633174
6.08288216233 8.10026014149
6.32619744882 8.32587024124
6.56951273532 8.55479894844
6.81282802181 8.78811778265
7.0561433083 9.02449549295
7.2994585948 9.26488430437
7.54277388129 9.50752749281
7.78608916778 9.75598477952
8.02940445428 10.005281342
8.27271974077 10.2618647044
8.51603502726 10.5169712828
8.75935031375 10.776900001
9.00266560025 11.0417723945
9.24598088674 11.3080005913
9.48929617323 11.5819045388
9.73261145973 11.8556797855
9.97592674622 12.1314486988
10.2192420327 12.4146796459
10.4625573192 12.6993811219
10.7058726057 12.9897297924
10.9491878922 13.2815349269
11.1925031787 13.580338589
11.4358184652 13.8822150501
11.6791337517 14.1910915729
11.9224490382 14.5085640325


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt6.tex <==
0.0 6.9930686457
0.158488367927 6.99518048911
0.316976735854 7.00118614987
0.475465103781 7.01226512668
0.633953471707 7.02664557265
0.792441839634 7.04597843998
0.950930207561 7.06896632957
1.10941857549 7.09603032094
1.26790694341 7.12759076492
1.42639531134 7.16285697123
1.58488367927 7.20286627411
1.7433720472 7.24683579396
1.90186041512 7.29524162945
2.06034878305 7.34731384731
2.21883715098 7.40426442008
2.3773255189 7.4647199429
2.53581388683 7.53002298067
2.69430225476 7.59884070123
2.85279062268 7.67268216014
3.01127899061 7.74953377203
3.16976735854 7.83105386691
3.32825572646 7.91599988915
3.48674409439 8.00545881862
3.64523246232 8.09822567189
3.80372083024 8.19470411235
3.96220919817 8.29453032679
4.1206975661 8.39823278822
4.27918593403 8.505535288
4.43767430195 8.61524920438
4.59616266988 8.72894902873
4.75465103781 8.84548910123
4.91313940573 8.9656272336
5.07162777366 9.08818784677
5.23011614159 9.21398491799
5.38860450951 9.34286384218
5.54709287744 9.47358510264
5.70558124537 9.60813017699
5.86406961329 9.74414029969
6.02255798122 9.88366042983
6.18104634915 10.0253806844
6.33953471707 10.1690718065
6.498023085 10.3156783567
6.65651145293 10.4649562757
6.81499982086 10.6166118608
6.97348818878 10.7702938065
7.13197655671 10.9268467668
7.29046492464 11.0845398778
7.44895329256 11.2466424079
7.60744166049 11.4125689468
7.76593002842 11.5829680682


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt7.tex <==
0.0 7.65201087312
0.132433347565 7.6531464162
0.26486669513 7.65746418317
0.397300042696 7.66421160717
0.529733390261 7.67365991293
0.662166737826 7.68553077287
0.794600085391 7.70005456047
0.927033432956 7.71745018199
1.05946678052 7.73792988816
1.19190012809 7.76061554826
1.32433347565 7.78569238657
1.45676682322 7.81390069692
1.58920017078 7.84488971493
1.72163351835 7.8788625844
1.85406686591 7.91546472808
1.98650021348 7.95491058722
2.11893356104 7.99743383461
2.25136690861 8.04269816381
2.38380025617 8.09036218181
2.51623360374 8.14129831812
2.6486669513 8.19520719663
2.78110029887 8.25178841964
2.91353364643 8.31074040403
3.045966994 8.3730538349
3.17840034157 8.4378284088
3.31083368913 8.50545905448
3.4432670367 8.57570586206
3.57570038426 8.64833087311
3.70813373183 8.72379768971
3.84056707939 8.80190553544
3.97300042696 8.88245615199
4.10543377452 8.96598704051
4.23786712209 9.05084844584
4.37030046965 9.1390827778
4.50273381722 9.22903176285
4.63516716478 9.32128407036
4.76760051235 9.41647353208
4.90003385991 9.51287430377
5.03246720748 9.61191908506
5.16490055504 9.71347967087
5.29733390261 9.81659239816
5.42976725017 9.92109275674
5.56220059774 10.0285157813
5.6946339453 10.1378890822
5.82706729287 10.2490729826
5.95950064043 10.3628089042
6.091933988 10.4790052959
6.22436733556 10.5976164282
6.35680068313 10.718708677
6.4892340307 10.8444235348


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt8.tex <==
0.0 8.28210551064
0.104749805795 8.28296816209
0.20949961159 8.28507141802
0.314249417386 8.28877666826
0.418999223181 8.29356066033
0.523749028976 8.30020983205
0.628498834771 8.30774580214
0.733248640566 8.3173868775
0.837998446361 8.32814082025
0.942748252157 8.34033459756
1.04749805795 8.35384829079
1.15224786375 8.36900579755
1.25699766954 8.3856825972
1.36174747534 8.4042036063
1.46649728113 8.42398657421
1.57124708693 8.4458122949
1.67599689272 8.46909425076
1.78074669852 8.4936964547
1.88549650431 8.52041542574
1.99024631011 8.54865703801
2.0949961159 8.57876123772
2.1997459217 8.61012365507
2.30449572749 8.64356915539
2.40924553329 8.67849414828
2.51399533908 8.71574723229
2.61874514488 8.75423408987
2.72349495067 8.79432037374
2.82824475647 8.83638751247
2.93299456226 8.88032775262
3.03774436806 8.92552351195
3.14249417386 8.97288370583
3.24724397965 9.0217959509
3.35199378545 9.07215443656
3.45674359124 9.12438179951
3.56149339704 9.17838739751
3.66624320283 9.23354581606
3.77099300863 9.29083762914
3.87574281442 9.34964560116
3.98049262022 9.40988718076
4.08524242601 9.47148347587
4.18999223181 9.53491704005
4.2947420376 9.60013171097
4.3994918434 9.66651598546
4.50424164919 9.73515817835
4.60899145499 9.80491061376
4.71374126078 9.87634834087
4.81849106658 9.9501039022
4.92324087237 10.0257428669
5.02799067817 10.1041289961
5.13274048396 10.1852940748


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-conditionalMeanCentered.tex <==
0.0 0.0900282553096
0.00853 0.0900645934754
0.01706 0.090172769951
0.02559 0.0903516162454
0.03412 0.0906000831503
0.04265 0.0909172346294
0.05118 0.0913022420318
0.05971 0.0917543786124
0.06824 0.0922730143419
0.07677 0.0928576109899
0.0853 0.0935077174666
0.09383 0.0942229654065
0.10236 0.0950030649831
0.11089 0.0958478009388
0.11942 0.0967570288196
0.12795 0.0977306714007
0.13648 0.0987687152947
0.14501 0.0998712077291
0.15354 0.101038253486
0.16207 0.10227001199
0.1706 0.103566694546
0.17913 0.104928561701
0.18766 0.106355920743
0.19619 0.107849123312
0.20472 0.10940856313
0.21325 0.111034673827
0.22178 0.112727926882
0.23031 0.114488829646
0.23884 0.116317923459
0.24737 0.118215781851
0.2559 0.120183008826
0.26443 0.122220237213
0.27296 0.124328127098
0.28149 0.126507364313
0.29002 0.128758659001
0.29855 0.131082744228
0.30708 0.133480374663
0.31561 0.135952325305
0.32414 0.138499390266
0.33267 0.141122381601
0.3412 0.143822128183
0.34973 0.146599474623
0.35826 0.149455280234
0.36679 0.152390418031
0.37532 0.155405773772
0.38385 0.15850224503
0.39238 0.16168074031
0.40091 0.164942178185
0.40944 0.168287486473
0.41797 0.171717601441
0.4265 0.175233467038
0.43503 0.178836034151
0.44356 0.182526259894
0.45209 0.186305106917
0.46062 0.19017354274
0.46915 0.194132539111
0.47768 0.198183071385
0.48621 0.202326117922
0.49474 0.206562659507
0.50327 0.210893678792
0.5118 0.215320159751
0.52033 0.219843087155
0.52886 0.224463446067
0.53739 0.229182221348
0.54592 0.234000397183
0.55445 0.238918956622
0.56298 0.243938881131
0.57151 0.249061150164
0.58004 0.25428674074
0.58857 0.259616627045
0.5971 0.265051780033
0.60563 0.270593167048
0.61416 0.276241751458
0.62269 0.281998492292
0.63122 0.287864343897
0.63975 0.293840255602
0.64828 0.299927171391
0.65681 0.302793805764
0.66534 0.302867249126
0.67387 0.302943870435
0.6824 0.303082513628
0.69093 0.303283863577
0.69946 0.303518435722
0.70799 0.303786374453
0.71652 0.304118675545
0.72505 0.304485358715
0.73358 0.304886786418
0.74211 0.305323389329
0.75064 0.305795667791
0.75917 0.306304193363
0.7677 0.306849610486
0.77623 0.307465462797
0.78476 0.30808721985
0.79329 0.308748265715
0.80182 0.30941573574
0.81035 0.310157957034
0.81888 0.310908048022
0.82741 0.31170101014
0.83594 0.312502852185
0.84447 0.313349432856
0.853 0.314242179531
0.86153 0.315109748203
0.87006 0.316061831095
0.87859 0.317026828498
0.88712 0.318005254452
0.89565 0.318997673104
0.90418 0.320043258637
0.91271 0.321105023458
0.92124 0.322183716334
0.92977 0.323280142323
0.9383 0.324395164275
0.94683 0.32552970436
0.95536 0.32672615208
0.96389 0.327903246131
0.97242 0.329103005827
0.98095 0.330369561773
0.98948 0.3316187809
0.99801 0.332850370544
1.00654 0.334153227805
1.01507 0.335440165747
1.0236 0.336802441393
1.03213 0.338104455861
1.04066 0.339485032081
1.04919 0.340852673113
1.05772 0.342255463845
1.06625 0.343646528556
1.07478 0.34507527979
1.08331 0.346493705084
1.09184 0.347952588316
1.10037 0.349402745653
1.1089 0.350896376893
1.11743 0.352383091386
1.12596 0.353863186144
1.13449 0.355391053536
1.14302 0.3569144106
1.15155 0.358489178331
1.16008 0.360005543477
1.16861 0.361575747675
1.17714 0.363202574707
1.18567 0.364771919269
1.1942 0.366341384827
1.20273 0.367971687713
1.21126 0.369605069437
1.21979 0.371242303489
1.22832 0.372884203547
1.23685 0.374531624208
1.24538 0.376185461728
1.25391 0.377846654753
1.26244 0.379516185053
1.27097 0.381261795291
1.2795 0.38295200306
1.28803 0.384653770518
1.29656 0.386368259304
1.30509 0.388096677812
1.31362 0.389840281909
1.32215 0.391528202453
1.33068 0.393305189835
1.33921 0.395027330408
1.34774 0.396843265784
1.35627 0.398605345667
1.3648 0.400389170778
1.37333 0.402118283342
1.38186 0.40394935187
1.39039 0.405726956068
1.39892 0.407530822786
1.40745 0.409362703245
1.41598 0.41122440384
1.42451 0.41303348801
1.43304 0.414874000845
1.44157 0.416661402076
1.4501 0.418569536551
1.45863 0.420337661201
1.46716 0.422230612001
1.47569 0.424071954753
1.48422 0.425952553077
1.49275 0.427874623891
1.50128 0.429745960098
1.50981 0.431565326085
1.51834 0.433525227979
1.52687 0.435337422978
1.5354 0.437294988334
1.54393 0.439203001405
1.55246 0.441060282097
1.56099 0.442968710898
1.56952 0.444930913435
1.57805 0.446843946998
1.58658 0.448813598483
1.59511 0.450734405483
1.60364 0.452605242848
1.61217 0.454535879203
1.6207 0.456529216761
1.62923 0.458474612723
1.63776 0.460370982809
1.64629 0.462333603904
1.65482 0.464365569453
1.66335 0.466350862999
1.67188 0.468288444407
1.68041 0.47017726768
1.68894 0.47226324202
1.69747 0.474179242026
1.706 0.476172686977
1.71453 0.478119097078
1.72306 0.480146864358
1.73159 0.482128602448
1.74012 0.484195762467
1.74865 0.486084035892
1.75718 0.488194366069
1.76571 0.490123900012
1.77424 0.492144287468
1.78277 0.494119085034
1.7913 0.496189189709
1.79983 0.498215052136
1.80836 0.500195765124
1.81689 0.502277123142
1.82542 0.504314803555
1.83395 0.506307923509
1.84248 0.508407291608
1.85101 0.510463697951
1.85954 0.512476285089
1.86807 0.514444191897
1.8766 0.516525080936
1.88513 0.518563035441
1.89366 0.520557220936
1.90219 0.522670586997
1.91072 0.5247420623
1.91925 0.526770839993
1.92778 0.528925275337
1.93631 0.530868041936
1.94484 0.53293849824
1.95337 0.535141357402
1.9619 0.537128372788
1.97043 0.53924996047
1.97896 0.541330709201
1.98749 0.543369864729
1.99602 0.545550748515
2.00455 0.547506366432
2.01308 0.549606062215
2.02161 0.551665031498
2.03014 0.55387439482
2.03867 0.555851698284
2.0472 0.55798190862
2.05573 0.560072480245
2.06426 0.562322545037
2.07279 0.564333768483
2.08132 0.566507163787
2.08985 0.568642234158
2.09838 0.570738311538
2.10691 0.572794725995
2.11544 0.574810805744
2.12397 0.577000182416
2.1325 0.579152116071
2.14103 0.581265968658
2.14956 0.583341100487
2.15809 0.585599738402
2.16662 0.587597676265
2.17515 0.589782206204
2.18368 0.591929853342
2.19221 0.594040009535
2.20074 0.596112065244
2.20927 0.598381518332
2.2178 0.600377791632
2.22633 0.602574768891
2.23486 0.604735765909
2.24339 0.606860206057
2.25192 0.608947511547
2.26045 0.611246929877
2.26898 0.613260560418
2.27751 0.615489834213
2.28604 0.617684382144
2.29457 0.619843660537
2.3031 0.62196712477
2.31163 0.624054229295
2.32016 0.626370860873
2.32869 0.62838603081
2.33722 0.630634509298
2.34575 0.632849353658
2.35428 0.635030053662
2.36281 0.637176098343
2.37134 0.639286976028
2.37987 0.641645862772
2.3884 0.643687386414
2.39693 0.645980954504
2.40546 0.648242403844
2.41399 0.650177420011
2.42252 0.652370634669
2.43105 0.654829283217
2.43958 0.656957498789
2.44811 0.659051213685
2.45664 0.661416773773
2.46517 0.663442689754
2.4737 0.665744793064
2.48223 0.668015820371
2.49076 0.670255331691
2.49929 0.67246288671
2.50782 0.674638044804
2.51635 0.676780365061
2.52488 0.678889406299
2.53341 0.681295750283
2.54194 0.683339663378
2.55047 0.685685530436
2.559 0.688001925464
2.56753 0.689946327139
2.57606 0.692199762729
2.58459 0.694422503934
2.59312 0.696614147408
2.60165 0.699127711737
2.61018 0.701258807902
2.61871 0.703357608877
2.62724 0.705785747113
2.63577 0.707821644521
2.6443 0.710191892503
2.65283 0.71253409041
2.66136 0.714847873668
2.66989 0.717132877749
2.67842 0.719388738191
2.68695 0.721615090608
2.69548 0.723811570714
2.70401 0.725977814333
2.71254 0.728113457422
2.72107 0.730612750004
2.7296 0.732689139762
2.73813 0.735134554811
2.74666 0.737150288682
2.75519 0.739540475913
2.76372 0.741904088098
2.77225 0.744240801145
2.78078 0.746550291202
2.78931 0.748832234677
2.79784 0.751086308251
2.80637 0.753312188894
2.8149 0.755509553882
2.82343 0.757678080807
2.83196 0.760252557327
2.84049 0.762365646815
2.84902 0.764890475546
2.85755 0.766946893219
2.86608 0.769420892155
2.87461 0.771870660618
2.88314 0.773841396923
2.89167 0.776238581174
2.9002 0.778610678633
2.90873 0.780957408954
2.91726 0.783278492255
2.92579 0.785573649132
2.93432 0.787842600671
2.94285 0.790085068467
2.95138 0.792781878241
2.95991 0.794973925165
2.96844 0.797138668916
2.97697 0.799767111132
2.9855 0.801879837884
2.99403 0.804462569668
3.00256 0.806522229481
3.01109 0.809058253449
3.01962 0.811572283373
3.02815 0.813552125005
3.03668 0.816017972931
3.04521 0.818461111389
3.05374 0.820881307413
3.06227 0.82327832874
3.0708 0.825651943822
3.07933 0.82800192185
3.08786 0.830328032761
3.09639 0.832630047262
3.10492 0.834907736839
3.11345 0.837708289782
3.12198 0.839940261364
3.13051 0.842147239804
3.13904 0.844887291864
3.14757 0.847047260732
3.1561 0.849747179259
3.16463 0.851859294516
3.17316 0.854518288701
3.18169 0.856581713633
3.19022 0.859199000176
3.19875 0.861797002462
3.20728 0.863787709118
3.21581 0.866342855977
3.22434 0.86887816788
3.23287 0.871393467515
3.2414 0.873888578679
3.24993 0.876363326299
3.25846 0.878817536457
3.26699 0.881251036418
3.27552 0.883663654649
3.28405 0.88605522085
3.29258 0.88842556598
3.30111 0.891404246883
3.30964 0.893735531148
3.31817 0.896045107559
3.3267 0.898332812402
3.33523 0.901243810574
3.34376 0.903491220151
3.35229 0.906369489014
3.36082 0.908576016104
3.36935 0.911421024746
3.37788 0.913586094553
3.38641 0.916397324994
3.39494 0.91852037575
3.40347 0.921297323583
3.412 0.924058959593
3.42053 0.926119982273
3.42906 0.928846618783
3.43759 0.931557612656
3.44612 0.934252861885
3.45465 0.936230774285
3.46318 0.938890131513
3.47171 0.941533438087
3.48024 0.944160600788
3.48877 0.946771528766
3.4973 0.949366133608
3.50583 0.951944329411
3.51436 0.954506032858
3.52289 0.957051163298
3.53142 0.960318552287
3.53995 0.962834529465
3.54848 0.965333721987
3.55701 0.9678160608
3.56554 0.970281479972
3.57407 0.973490071976
3.5826 0.975925758746
3.59113 0.978344361742
3.59966 0.981518892426
3.60819 0.983907508256
3.61672 0.986278908904
3.62525 0.989419152014
3.63378 0.991760380633
3.64231 0.994879155629
3.65084 0.997190141451
3.65937 1.00028745388
3.6679 1.00337626243
3.67643 1.00564405955
3.68496 1.00871150529
3.69349 1.0117705443
3.70202 1.01399526577
3.71055 1.01703314505
3.71908 1.02006277048
3.72761 1.02224469124
3.73614 1.02525347755
3.74467 1.02825422648
3.7532 1.03124703131
3.76173 1.03423199398
3.77026 1.03720922551
3.77879 1.04017884642
3.78732 1.04226927026
3.79585 1.04521940623
3.80438 1.04816233782
3.81291 1.05109822878
3.82144 1.05402725522
3.82997 1.05694960635
3.8385 1.06076546944
3.84703 1.06367987045
3.85556 1.06658826987
3.86409 1.06949091793
3.87262 1.07238808249
3.88115 1.07528005012
3.88968 1.07816712737
3.89821 1.08198347476
3.90674 1.08486669947
3.91527 1.08774611
3.9238 1.0915707619
3.93233 1.09444876839
3.94086 1.09732427673
3.94939 1.10116146736
3.95792 1.10403856002
3.96645 1.10691476936
3.97498 1.11076965344
3.98351 1.11365111315
3.99204 1.11752293959
4.00057 1.12041257964
4.0091 1.12430461315
4.01763 1.12720582218
4.02616 1.13112183731
4.03469 1.1340385552
4.04322 1.13798294219
4.05175 1.14091977883
4.06028 1.14489768012
4.06881 1.14786006996
4.07734 1.15187755938
4.08587 1.15592024976
4.0944 1.15893628831
4.10293 1.16303001667
4.11146 1.16715560562
4.11999 1.17131577345
4.12852 1.17443677378
4.13705 1.17866966537
4.14558 1.18294726742
4.15411 1.18727386008
4.16264 1.19055369793
4.17117 1.19498743649
4.1797 1.19948694816
4.18823 1.20405971805
4.19676 1.20871456253
4.20529 1.21232977173
4.21382 1.21717588683
4.22235 1.2221428803
4.23088 1.22725050413
4.23941 1.23252433471
4.24794 1.23799868254
4.25647 1.24372181311


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-leftEnd-sigma2prob0pt1.tex <==
0.0 0.0
0.0841218682305 0.0841218682305
0.168243736461 0.168243736461
0.252365604692 0.252365604692
0.336487472922 0.336487472922
0.420609341153 0.420609341153
0.504731209383 0.504731209383
0.588853077614 0.588853077614
0.672974945844 0.672974945844
0.757096814075 0.757096814075
0.841218682305 0.841218682305
0.925340550536 0.925340550536
1.00946241877 1.00946241877
1.093584287 1.093584287
1.17770615523 1.17770615523
1.26182802346 1.26182802346
1.34594989169 1.34594989169
1.43007175992 1.43007175992
1.51419362815 1.51419362815
1.59831549638 1.59831549638
1.68243736461 1.68243736461
1.76655923284 1.76655923284
1.85068110107 1.85068110107
1.9348029693 1.9348029693
2.01892483753 2.01892483753
2.10304670576 2.10304670576
2.18716857399 2.18716857399
2.27129044222 2.27129044222
2.35541231046 2.35541231046
2.43953417869 2.43953417869
2.52365604692 2.52365604692
2.60777791515 2.60777791515
2.69189978338 2.69189978338
2.77602165161 2.77602165161
2.86014351984 2.86014351984
2.94426538807 2.94426538807
3.0283872563 3.0283872563
3.11250912453 3.11250912453
3.19663099276 3.19663099276
3.28075286099 3.28075286099
3.36487472922 3.36487472922
3.44899659745 3.44899659745
3.53311846568 3.53311846568
3.61724033391 3.61724033391
3.70136220214 3.70136220214
3.78548407037 3.78548407037
3.8696059386 3.8696059386
3.95372780684 3.95372780684
4.03784967507 4.03784967507
4.1219715433 4.1219715433


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-leftEnd-sigma2prob0pt3.tex <==
0.0 0.0
0.0608288216233 0.0608288216233
0.121657643247 0.121657643247
0.18248646487 0.18248646487
0.243315286493 0.243315286493
0.304144108116 0.304144108116
0.36497292974 0.36497292974
0.425801751363 0.425801751363
0.486630572986 0.486630572986
0.54745939461 0.54745939461
0.608288216233 0.608288216233
0.669117037856 0.669117037856
0.72994585948 0.72994585948
0.790774681103 0.790774681103
0.851603502726 0.851603502726
0.912432324349 0.912432324349
0.973261145973 0.973261145973
1.0340899676 1.0340899676
1.09491878922 1.09491878922
1.15574761084 1.15574761084
1.21657643247 1.21657643247
1.27740525409 1.27740525409
1.33823407571 1.33823407571
1.39906289734 1.39906289734
1.45989171896 1.45989171896
1.52072054058 1.52072054058
1.58154936221 1.58154936221
1.64237818383 1.64237818383
1.70320700545 1.70320700545
1.76403582708 1.76403582708
1.8248646487 1.8248646487
1.88569347032 1.88569347032
1.94652229195 1.94652229195
2.00735111357 2.00735111357
2.06817993519 2.06817993519
2.12900875682 2.12900875682
2.18983757844 2.18983757844
2.25066640006 2.25066640006
2.31149522169 2.31149522169
2.37232404331 2.37232404331
2.43315286493 2.43315286493
2.49398168656 2.49398168656
2.55481050818 2.55481050818
2.6156393298 2.6156393298
2.67646815143 2.67646815143
2.73729697305 2.73729697305
2.79812579467 2.79812579467
2.85895461629 2.85895461629
2.91978343792 2.91978343792
2.98061225954 2.98061225954


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt3.tex <==
0.0 0.0
0.243315286493 0.243315286493
0.486630572986 0.486630572986
0.72994585948 0.72994585948
0.973261145973 0.973261145973
1.21657643247 1.21657643247
1.45989171896 1.45989171896
1.70320700545 1.70320700545
1.94652229195 1.94652229195
2.18983757844 2.18983757844
2.43315286493 2.43315286493
2.67646815143 2.67646815143
2.91978343792 2.91978343792
3.16309872441 3.16309872441
3.4064140109 3.4064140109
3.6497292974 3.6497292974
3.89304458389 3.89304458389
4.13635987038 4.13635987038
4.37967515688 4.37967515688
4.62299044337 4.62299044337
4.86630572986 4.86630572986
5.10962101636 5.10962101636
5.35293630285 5.35293630285
5.59625158934 5.59625158934
5.83956687584 5.83956687584
6.08288216233 6.08288216233
6.32619744882 6.32619744882
6.56951273532 6.56951273532
6.81282802181 6.81282802181
7.0561433083 7.0561433083
7.2994585948 7.2994585948
7.54277388129 7.54277388129
7.78608916778 7.78608916778
8.02940445428 8.02940445428
8.27271974077 8.27271974077
8.51603502726 8.51603502726
8.75935031375 8.75935031375
9.00266560025 9.00266560025
9.24598088674 9.24598088674
9.48929617323 9.48929617323
9.73261145973 9.73261145973
9.97592674622 9.97592674622
10.2192420327 10.2192420327
10.4625573192 10.4625573192
10.7058726057 10.7058726057
10.9491878922 10.9491878922
11.1925031787 11.1925031787
11.4358184652 11.4358184652
11.6791337517 11.6791337517
11.9224490382 11.9224490382


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt6.tex <==
0.0 0.0
0.158488367927 0.158488367927
0.316976735854 0.316976735854
0.475465103781 0.475465103781
0.633953471707 0.633953471707
0.792441839634 0.792441839634
0.950930207561 0.950930207561
1.10941857549 1.10941857549
1.26790694341 1.26790694341
1.42639531134 1.42639531134
1.58488367927 1.58488367927
1.7433720472 1.7433720472
1.90186041512 1.90186041512
2.06034878305 2.06034878305
2.21883715098 2.21883715098
2.3773255189 2.3773255189
2.53581388683 2.53581388683
2.69430225476 2.69430225476
2.85279062268 2.85279062268
3.01127899061 3.01127899061
3.16976735854 3.16976735854
3.32825572646 3.32825572646
3.48674409439 3.48674409439
3.64523246232 3.64523246232
3.80372083024 3.80372083024
3.96220919817 3.96220919817
4.1206975661 4.1206975661
4.27918593403 4.27918593403
4.43767430195 4.43767430195
4.59616266988 4.59616266988
4.75465103781 4.75465103781
4.91313940573 4.91313940573
5.07162777366 5.07162777366
5.23011614159 5.23011614159
5.38860450951 5.38860450951
5.54709287744 5.54709287744
5.70558124537 5.70558124537
5.86406961329 5.86406961329
6.02255798122 6.02255798122
6.18104634915 6.18104634915
6.33953471707 6.33953471707
6.498023085 6.498023085
6.65651145293 6.65651145293
6.81499982086 6.81499982086
6.97348818878 6.97348818878
7.13197655671 7.13197655671
7.29046492464 7.29046492464
7.44895329256 7.44895329256
7.60744166049 7.60744166049
7.76593002842 7.76593002842


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt7.tex <==
0.0 0.0
0.132433347565 0.132433347565
0.26486669513 0.26486669513
0.397300042696 0.397300042696
0.529733390261 0.529733390261
0.662166737826 0.662166737826
0.794600085391 0.794600085391
0.927033432956 0.927033432956
1.05946678052 1.05946678052
1.19190012809 1.19190012809
1.32433347565 1.32433347565
1.45676682322 1.45676682322
1.58920017078 1.58920017078
1.72163351835 1.72163351835
1.85406686591 1.85406686591
1.98650021348 1.98650021348
2.11893356104 2.11893356104
2.25136690861 2.25136690861
2.38380025617 2.38380025617
2.51623360374 2.51623360374
2.6486669513 2.6486669513
2.78110029887 2.78110029887
2.91353364643 2.91353364643
3.045966994 3.045966994
3.17840034157 3.17840034157
3.31083368913 3.31083368913
3.4432670367 3.4432670367
3.57570038426 3.57570038426
3.70813373183 3.70813373183
3.84056707939 3.84056707939
3.97300042696 3.97300042696
4.10543377452 4.10543377452
4.23786712209 4.23786712209
4.37030046965 4.37030046965
4.50273381722 4.50273381722
4.63516716478 4.63516716478
4.76760051235 4.76760051235
4.90003385991 4.90003385991
5.03246720748 5.03246720748
5.16490055504 5.16490055504
5.29733390261 5.29733390261
5.42976725017 5.42976725017
5.56220059774 5.56220059774
5.6946339453 5.6946339453
5.82706729287 5.82706729287
5.95950064043 5.95950064043
6.091933988 6.091933988
6.22436733556 6.22436733556
6.35680068313 6.35680068313
6.4892340307 6.4892340307


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt8.tex <==
0.0 0.0
0.104749805795 0.104749805795
0.20949961159 0.20949961159
0.314249417386 0.314249417386
0.418999223181 0.418999223181
0.523749028976 0.523749028976
0.628498834771 0.628498834771
0.733248640566 0.733248640566
0.837998446361 0.837998446361
0.942748252157 0.942748252157
1.04749805795 1.04749805795
1.15224786375 1.15224786375
1.25699766954 1.25699766954
1.36174747534 1.36174747534
1.46649728113 1.46649728113
1.57124708693 1.57124708693
1.67599689272 1.67599689272
1.78074669852 1.78074669852
1.88549650431 1.88549650431
1.99024631011 1.99024631011
2.0949961159 2.0949961159
2.1997459217 2.1997459217
2.30449572749 2.30449572749
2.40924553329 2.40924553329
2.51399533908 2.51399533908
2.61874514488 2.61874514488
2.72349495067 2.72349495067
2.82824475647 2.82824475647
2.93299456226 2.93299456226
3.03774436806 3.03774436806
3.14249417386 3.14249417386
3.24724397965 3.24724397965
3.35199378545 3.35199378545
3.45674359124 3.45674359124
3.56149339704 3.56149339704
3.66624320283 3.66624320283
3.77099300863 3.77099300863
3.87574281442 3.87574281442
3.98049262022 3.98049262022
4.08524242601 4.08524242601
4.18999223181 4.18999223181
4.2947420376 4.2947420376
4.3994918434 4.3994918434
4.50424164919 4.50424164919
4.60899145499 4.60899145499
4.71374126078 4.71374126078
4.81849106658 4.81849106658
4.92324087237 4.92324087237
5.02799067817 5.02799067817
5.13274048396 5.13274048396


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-lowerEnd-sigma2prob0pt1.tex <==
0.0 0.0
0.0841218682305 0.0841218682305
0.168243736461 0.168243736461
0.252365604692 0.252365604692
0.336487472922 0.336487472922
0.420609341153 0.420609341153
0.504731209383 0.504731209383
0.588853077614 0.588853077614
0.672974945844 0.672974945844
0.757096814075 0.757096814075
0.841218682305 0.841218682305
0.925340550536 0.925340550536
1.00946241877 1.00946241877
1.093584287 1.093584287
1.17770615523 1.17770615523
1.26182802346 1.26182802346
1.34594989169 1.34594989169
1.43007175992 1.43007175992
1.51419362815 1.51419362815
1.59831549638 1.59831549638
1.68243736461 1.68243736461
1.76655923284 1.76655923284
1.85068110107 1.85068110107
1.9348029693 1.9348029693
2.01892483753 2.01892483753
2.10304670576 2.10304670576
2.18716857399 2.18716857399
2.27129044222 2.27129044222
2.35541231046 2.35541231046
2.43953417869 2.43953417869
2.52365604692 2.52365604692
2.60777791515 2.60777791515
2.69189978338 2.69189978338
2.77602165161 2.77602165161
2.86014351984 2.86014351984
2.94426538807 2.94426538807
3.0283872563 3.0283872563
3.11250912453 3.11250912453
3.19663099276 3.19663099276
3.28075286099 3.28075286099
3.36487472922 3.36487472922
3.44899659745 3.44899659745
3.53311846568 3.53311846568
3.61724033391 3.61724033391
3.70136220214 3.70136220214
3.78548407037 3.78548407037
3.8696059386 3.8696059386
3.95372780684 3.95372780684
4.03784967507 4.03784967507
4.1219715433 4.1219715433


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma1.tex <==
0.0 0.160145706136
0.00488 0.162605271339
0.00976 0.165103952687
0.01464 0.167641707448
0.01952 0.170218464577
0.0244 0.172834124972
0.02928 0.175488561835
0.03416 0.17818162113
0.03904 0.180913122131
0.04392 0.18368285806
0.0488 0.186490596817
0.05368 0.189336081773
0.05856 0.192219032649
0.06344 0.195139146451
0.06832 0.19809609847
0.0732 0.201089543327
0.07808 0.204119116062
0.08296 0.207184433267
0.08784 0.210285094233
0.09272 0.213420682134
0.0976 0.216590765212
0.10248 0.219794897976
0.10736 0.223032622402
0.11224 0.226303469121
0.11712 0.229606958601
0.122 0.232942602311
0.12688 0.23630990386
0.13176 0.239708360111
0.13664 0.243137462266
0.14152 0.24659669691
0.1464 0.25008554703
0.15128 0.253603492981
0.15616 0.257150013416
0.16104 0.260724586172
0.16592 0.264326689114
0.1708 0.267955800923
0.17568 0.27161140185
0.18056 0.275292974415
0.18544 0.279000004064
0.19032 0.282731979776
0.1952 0.286488394628
0.20008 0.290268746315
0.20496 0.294072537626
0.20984 0.297899276879
0.21472 0.301748478312
0.2196 0.30561966244
0.22448 0.309512356371
0.22936 0.313426094085
0.23424 0.317360416684
0.23912 0.321314872604
0.244 0.325289017799
0.24888 0.329282415895
0.25376 0.333294638319
0.25864 0.337325264399
0.26352 0.341373881445
0.2684 0.3454400848
0.27328 0.349523477881
0.27816 0.353623672193
0.28304 0.357740287325
0.28792 0.36187295094
0.2928 0.366021298735
0.29768 0.370184974404
0.30256 0.374363629571
0.30744 0.378556923733
0.31232 0.38276452417
0.3172 0.386986105869
0.32208 0.39122135142
0.32696 0.395469950918
0.33184 0.399731601857
0.33672 0.404006009013
0.3416 0.408292884328
0.34648 0.412591946786
0.35136 0.416902922294
0.35624 0.421225543545
0.36112 0.425559549898
0.366 0.429904687242
0.37088 0.434260707861
0.37576 0.438627370306
0.38064 0.443004439258
0.38552 0.447391685399
0.3904 0.45178888527
0.39528 0.456195821149
0.40016 0.460612280909
0.40504 0.465038057897
0.40992 0.469472950797
0.4148 0.473916763505
0.41968 0.478369305001
0.42456 0.482830389227
0.42944 0.487299834963
0.43432 0.491777465702
0.4392 0.496263109538
0.44408 0.500756599045
0.44896 0.505257771161
0.45384 0.50976646708
0.45872 0.514282532139
0.4636 0.518805815709
0.46848 0.523336171093
0.47336 0.527873455421
0.47824 0.532417529546
0.48312 0.536968257952
0.488 0.541525508652
0.49288 0.546089153097
0.49776 0.550659066083
0.50264 0.555235125663
0.50752 0.559817213059
0.5124 0.564405212575
0.51728 0.568999011519
0.52216 0.57359850012
0.52704 0.578203571448
0.53192 0.58281412134
0.5368 0.587430048324
0.54168 0.59205125355
0.54656 0.596677640714
0.55144 0.601309115995
0.55632 0.605945587988
0.5612 0.610586967635
0.56608 0.615233168166
0.57096 0.619884105039
0.57584 0.624539695877
0.58072 0.629199860412
0.5856 0.63386452043
0.59048 0.638533599717
0.59536 0.643207024003
0.60024 0.647884720915
0.60512 0.652566619922
0.61 0.657252652292
0.61488 0.661942751043
0.61976 0.666636850895
0.62464 0.671334888231
0.62952 0.676036801047
0.6344 0.680742528918
0.63928 0.685452012951
0.64416 0.69016519575
0.64904 0.694882021376
0.65392 0.699602435309
0.6588 0.704326384416
0.66368 0.709053816911
0.66856 0.713784682325
0.67344 0.718518931471
0.67832 0.723256516414
0.6832 0.727997390439
0.68808 0.732741508019
0.69296 0.737488824791
0.69784 0.742239297523
0.70272 0.746992884087
0.7076 0.751749543437
0.71248 0.756509235575
0.71736 0.761271921536
0.72224 0.766037563354
0.72712 0.770806124046
0.732 0.775577567583
0.73688 0.780351858873
0.74176 0.785128963737
0.74664 0.789908848886
0.75152 0.794691481905
0.7564 0.79947683123
0.76128 0.804264866132
0.76616 0.809055556694
0.77104 0.813848873797
0.77592 0.8186447891
0.7808 0.823443275026
0.78568 0.828244304741
0.79056 0.833047852145
0.79544 0.837853891847
0.80032 0.842662399159
0.8052 0.847473350076
0.81008 0.852286721265
0.81496 0.857102490049
0.81984 0.861920634394
0.82472 0.866741132899
0.8296 0.871563964778
0.83448 0.876389109854
0.83936 0.881216548543
0.84424 0.886046261844
0.84912 0.890878231328
0.854 0.895712439127
0.85888 0.900548867926
0.86376 0.905387500948
0.86864 0.910228321947
0.87352 0.915071315202
0.8784 0.9199164655
0.88328 0.924763758135
0.88816 0.929613178894
0.89304 0.934464714053
0.89792 0.939318350364
0.9028 0.944174075051
0.90768 0.949031875801
0.91256 0.953891740759
0.91744 0.958753658516
0.92232 0.963617618107
0.9272 0.968483609002
0.93208 0.973351621101
0.93696 0.978221644726
0.94184 0.983093670616
0.94672 0.987967689924
0.9516 0.992843694205
0.95648 0.997721675417
0.96136 1.00260162591
0.96624 1.00748353844
0.97112 1.01236740612
0.976 1.01725322246
0.98088 1.02214098136
0.98576 1.02703067707
0.99064 1.03192230422
0.99552 1.03681585781
1.0004 1.04171133317
1.00528 1.04660872603
1.01016 1.05150803245
1.01504 1.05640924884
1.01992 1.06131237197
1.0248 1.06621739893
1.02968 1.07112432718
1.03456 1.0760331545
1.03944 1.08094387901
1.04432 1.08585649918
1.0492 1.09077101378
1.05408 1.09568742194
1.05896 1.1006057231
1.06384 1.10552591702
1.06872 1.11044800382
1.0736 1.11537198389
1.07848 1.12029785798
1.08336 1.12522562714
1.08824 1.13015529275
1.09312 1.1350868565
1.098 1.1400203204
1.10288 1.14495568676
1.10776 1.14989295823
1.11264 1.15483213775
1.11752 1.1597732286
1.1224 1.16471623433
1.12728 1.16966115885
1.13216 1.17460800635
1.13704 1.17955678135
1.14192 1.18450748866
1.1468 1.18946013343
1.15168 1.19441472111
1.15656 1.19937125745
1.16144 1.20432974853
1.16632 1.20929020074
1.1712 1.21425262079
1.17608 1.21921701569
1.18096 1.22418339277
1.18584 1.22915175969
1.19072 1.23412212442
1.1956 1.23909449525
1.20048 1.24406888079
1.20536 1.24904528998
1.21024 1.25402373206
1.21512 1.25900421663
1.22 1.26398675359
1.22488 1.26897135318
1.22976 1.27395802599
1.23464 1.2789467829
1.23952 1.28393763516
1.2444 1.28893059435
1.24928 1.29392567238
1.25416 1.29892288153
1.25904 1.3039222344
1.26392 1.30892374395
1.2688 1.31392742349
1.27368 1.31893328667
1.27856 1.32394134754
1.28344 1.32895162046
1.28832 1.33396412018
1.2932 1.33897886184
1.29808 1.34399586091
1.30296 1.34901513326
1.30784 1.35403669514
1.31272 1.35906056319
1.3176 1.36408675441
1.32248 1.36911528624
1.32736 1.37414617647
1.33224 1.37917944332
1.33712 1.38421510541
1.342 1.38925318178
1.34688 1.39429369188
1.35176 1.39933665559
1.35664 1.4043820932
1.36152 1.40943002546
1.3664 1.41448047355
1.37128 1.41953345908
1.37616 1.42458900415
1.38104 1.42964713128
1.38592 1.43470786348
1.3908 1.43977122422
1.39568 1.44483723745
1.40056 1.44990592763
1.40544 1.45497731967
1.41032 1.46005143903
1.4152 1.46512831164
1.42008 1.47020796396
1.42496 1.47529042299
1.42984 1.48037571625
1.43472 1.48546387181
1.4396 1.49055491827
1.44448 1.49564888483
1.44936 1.50074580123
1.45424 1.50584569779
1.45912 1.51094860545
1.464 1.51605455571
1.46888 1.52116358072
1.47376 1.52627571321
1.47864 1.53139098659
1.48352 1.53650943488
1.4884 1.54163109276
1.49328 1.5467559956
1.49816 1.55188417942
1.50304 1.55701568096
1.50792 1.56215053765
1.5128 1.56728878765
1.51768 1.57243046985
1.52256 1.57757562388
1.52744 1.58272429015
1.53232 1.58787650983
1.5372 1.5930323249
1.54208 1.59819177813
1.54696 1.60335491314
1.55184 1.60852177436
1.55672 1.61369240712
1.5616 1.61886685758
1.56648 1.62404517284
1.57136 1.62922740089
1.57624 1.63441359066
1.58112 1.63960379202
1.586 1.64479805583
1.59088 1.64999643395
1.59576 1.65519897924
1.60064 1.66040574561
1.60552 1.66561678802
1.6104 1.67083216253
1.61528 1.6760519263
1.62016 1.68127613762
1.62504 1.68650485597
1.62992 1.69173814197
1.6348 1.6969760575
1.63968 1.70221866565
1.64456 1.7074660308
1.64944 1.71271821863
1.65432 1.71797529613
1.6592 1.72323733169
1.66408 1.72850439507
1.66896 1.73377655748
1.67384 1.73905389157
1.67872 1.74433647152
1.6836 1.74962437304
1.68848 1.7549176734
1.69336 1.76021645151
1.69824 1.76552078792
1.70312 1.77083076489
1.708 1.77614646643
1.71288 1.78146797831
1.71776 1.78679538817
1.72264 1.7921287855
1.72752 1.79746826175
1.7324 1.80281391033
1.73728 1.80816582671
1.74216 1.81352410843
1.74704 1.81888885519
1.75192 1.82426016888
1.7568 1.82963815369
1.76168 1.8350229161
1.76656 1.84041456502
1.77144 1.8458132118
1.77632 1.85121897033
1.7812 1.8566319571
1.78608 1.8620522913
1.79096 1.86748009485
1.79584 1.87291549251
1.80072 1.87835861199
1.8056 1.88380958397
1.81048 1.88926854226
1.81536 1.89473562383
1.82024 1.90021096897
1.82512 1.90569472134
1.83 1.9111870281
1.83488 1.91668803999
1.83976 1.9221979115
1.84464 1.92771680094
1.84952 1.93324487055
1.8544 1.93878228668
1.85928 1.94432921988
1.86416 1.94988584506
1.86904 1.95545234161
1.87392 1.96102889359
1.8788 1.96661568982
1.88368 1.97221292411
1.88856 1.9778207954
1.89344 1.98343950792
1.89832 1.9890692714
1.9032 1.99471030126
1.90808 2.0003628188
1.91296 2.0060270514
1.91784 2.01170323277
1.92272 2.01739160316
1.9276 2.02309240959
1.93248 2.02880590613
1.93736 2.03453235412
1.94224 2.04027202249
1.94712 2.04602518803
1.952 2.05179213568
1.95688 2.05757315886
1.96176 2.0633685598
1.96664 2.06917864989
1.97152 2.07500375003
1.9764 2.08084419105
1.98128 2.08670031409
1.98616 2.09257247103
1.99104 2.09846102491
1.99592 2.10436635048
2.0008 2.1102888346
2.00568 2.11622887684
2.01056 2.12218688998
2.01544 2.12816330063
2.02032 2.13415854982
2.0252 2.14017309367
2.03008 2.14620740407
2.03496 2.15226196938
2.03984 2.15833729524
2.04472 2.16443390539
2.0496 2.17055234247
2.05448 2.17669316902
2.05936 2.18285696839
2.06424 2.1890443458
2.06912 2.19525592944
2.074 2.20149237163
2.07888 2.20775435006
2.08376 2.21404256915
2.08864 2.22035776141
2.09352 2.22670068898
2.0984 2.23307214526
2.10328 2.2394729566
2.10816 2.24590398415
2.11304 2.25236612585
2.11792 2.25886031856
2.1228 2.26538754031
2.12768 2.27194881274
2.13256 2.27854520375
2.13744 2.28517783035
2.14232 2.29184786164
2.1472 2.29855652219
2.15208 2.30530509553
2.15696 2.31209492806
2.16184 2.31892743317
2.16672 2.3258040958
2.1716 2.33272647733
2.17648 2.33969622096
2.18136 2.34671505751
2.18624 2.35378481178
2.19112 2.36090740948
2.196 2.36808488488
2.20088 2.37531938909
2.20576 2.38261319922
2.21064 2.3899687285
2.21552 2.39738853731
2.2204 2.40487534549
2.22528 2.4124320459
2.23016 2.42006171947
2.23504 2.42776765193
2.23992 2.43555335246
2.2448 2.44342257454
2.24968 2.45137933924
2.25456 2.45942796142
2.25944 2.46757307923
2.26432 2.4758196874
2.2692 2.48417317494
2.27408 2.49263936807
2.27896 2.501224579
2.28384 2.50993566199
2.28872 2.51878007752
2.2936 2.52776596647
2.29848 2.53690223601
2.30336 2.54619865948
2.30824 2.5556659933
2.31312 2.56531611425
2.318 2.57516218182
2.32288 2.58521883116
2.32776 2.59550240391
2.33264 2.60603122623
2.33752 2.6168259462
2.3424 2.62790994645
2.34728 2.63930985312
2.35216 2.65105616979
2.35704 2.66318407502
2.36192 2.6757344371
2.3668 2.68875512166
2.37168 2.70230269985
2.37656 2.71644471472
2.38144 2.7312627411
2.38632 2.74685659853
2.3912 2.76335028415
2.39608 2.78090054676
2.40096 2.79970965864
2.40584 2.82004513296
2.41072 2.84227150079
2.4156 2.86690429499
2.42048 2.8947080431
2.42536 2.92689014648
2.43024 2.96553216795
2.43512 3.01472789297


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma1prob0pt1.tex <==
0.0 0.229521802513
0.004276 0.231670866425
0.008552 0.233842055028
0.012828 0.236035358932
0.017104 0.238250762499
0.02138 0.24048824387
0.025656 0.242747774992
0.029932 0.245029321663
0.034208 0.247332843578
0.038484 0.249658294386
0.04276 0.252005621759
0.047036 0.254374767465
0.051312 0.256765667447
0.055588 0.259178251916
0.059864 0.261612445446
0.06414 0.26406816708
0.068416 0.266545330439
0.072692 0.269043843837
0.076968 0.271563610408
0.081244 0.274104528233
0.08552 0.276666490473
0.089796 0.279249385508
0.094072 0.281853097082
0.098348 0.284477504447
0.102624 0.287122482517
0.1069 0.28978790202
0.111176 0.292473629658
0.115452 0.295179528263
0.119728 0.297905456959
0.124004 0.300651271327
0.12828 0.30341682357
0.132556 0.306201962675
0.136832 0.30900653458
0.141108 0.311830382343
0.145384 0.314673346302
0.14966 0.317535264246
0.153936 0.320415971573
0.158212 0.323315301461
0.162488 0.326233085022
0.166764 0.329169151467
0.17104 0.332123328259
0.175316 0.335095441275
0.179592 0.338085314953
0.183868 0.341092772446
0.188144 0.344117635769
0.19242 0.347159725942
0.196696 0.350218863132
0.200972 0.353294866791
0.205248 0.35638755579
0.209524 0.35949674855
0.2138 0.36262226317
0.218076 0.365763917547
0.222352 0.368921529497
0.226628 0.372094916871
0.230904 0.375283897666
0.23518 0.378488290131
0.239456 0.381707912871
0.243732 0.384942584948
0.248008 0.388192125974
0.252284 0.3914563562
0.25656 0.39473509661
0.260836 0.398028168997
0.265112 0.401335396046
0.269388 0.404656601409
0.273664 0.407991609775
0.27794 0.411340246941
0.282216 0.414702339872
0.286492 0.418077716764
0.290768 0.421466207099
0.295044 0.424867641702
0.29932 0.428281852787
0.303596 0.431708674004
0.307872 0.435147940488
0.312148 0.438599488889
0.316424 0.442063157421
0.3207 0.445538785888
0.324976 0.449026215717
0.329252 0.452525289991
0.333528 0.456035853471
0.337804 0.459557752619
0.34208 0.463090835623
0.346356 0.466634952413
0.350632 0.470189954677
0.354908 0.473755695877
0.359184 0.47733203126
0.36346 0.48091881787
0.367736 0.484515914552
0.372012 0.488123181963
0.376288 0.491740482576
0.380564 0.495367680681
0.38484 0.499004642387
0.389116 0.502651235624
0.393392 0.506307330139
0.397668 0.509972797494
0.401944 0.513647511065
0.40622 0.517331346032
0.410496 0.521024179375
0.414772 0.524725889868
0.419048 0.528436358068
0.423324 0.532155466307
0.4276 0.535883098682
0.431876 0.539619141045
0.436152 0.543363480989
0.440428 0.547116007835
0.444704 0.550876612625
0.44898 0.5546451881
0.453256 0.558421628691
0.457532 0.562205830504
0.461808 0.565997691304
0.466084 0.569797110497
0.47036 0.573603989118
0.474636 0.577418229814
0.478912 0.581239736824
0.483188 0.585068415967
0.487464 0.58890417462
0.49174 0.592746921704
0.496016 0.596596567666
0.500292 0.60045302446
0.504568 0.60431620553
0.508844 0.608186025793
0.51312 0.612062401618
0.517396 0.615945250812
0.521672 0.619834492598
0.525948 0.623730047602
0.530224 0.627631837827
0.5345 0.631539786645
0.538776 0.635453818769
0.543052 0.639373860242
0.547328 0.643299838417
0.551604 0.647231681938
0.55588 0.651169320723
0.560156 0.655112685948
0.564432 0.659061710025
0.568708 0.663016326591
0.572984 0.666976470487
0.57726 0.670942077738
0.581536 0.674913085543
0.585812 0.678889432254
0.590088 0.682871057358
0.594364 0.686857901463
0.59864 0.690849906284
0.602916 0.694847014621
0.607192 0.698849170346
0.611468 0.70285631839
0.615744 0.706868404724
0.62002 0.710885376344
0.624296 0.714907181257
0.628572 0.718933768465
0.632848 0.722965087952
0.637124 0.727001090669
0.6414 0.731041728517
0.645676 0.735086954338
0.649952 0.739136721895
0.654228 0.743190985865
0.658504 0.74724970182
0.66278 0.751312826217
0.667056 0.755380316383
0.671332 0.759452130505
0.675608 0.763528227613
0.679884 0.767608567574
0.68416 0.771693111074
0.688436 0.775781819606
0.692712 0.779874655466
0.696988 0.783971581731
0.701264 0.788072562256
0.70554 0.792177561657
0.709816 0.796286545305
0.714092 0.800399479312
0.718368 0.804516330522
0.722644 0.8086370665
0.72692 0.812761655523
0.731196 0.816890066568
0.735472 0.821022269305
0.739748 0.825158234085
0.744024 0.829297931934
0.7483 0.83344133454
0.752576 0.837588414247
0.756852 0.841739144044
0.761128 0.845893497559
0.765404 0.850051449049
0.76968 0.854212973392
0.773956 0.858378046079
0.778232 0.862546643207
0.782508 0.866718741471
0.786784 0.870894318155
0.79106 0.875073351127
0.795336 0.879255818832
0.799612 0.883441700282
0.803888 0.887630975051
0.808164 0.891823623272
0.81244 0.896019625623
0.816716 0.900218963327
0.820992 0.904421618145
0.825268 0.908627572365
0.829544 0.912836808804
0.83382 0.917049310796
0.838096 0.921265062189
0.842372 0.92548404734
0.846648 0.92970625111
0.850924 0.933931658856
0.8552 0.93816025643
0.859476 0.942392030173
0.863752 0.946626966907
0.868028 0.950865053937
0.872304 0.95510627904
0.87658 0.959350630467
0.880856 0.963598096933
0.885132 0.967848667616
0.889408 0.972102332156
0.893684 0.976359080644
0.89796 0.980618903627
0.902236 0.984881792097
0.906512 0.989147737494
0.910788 0.993416731698
0.915064 0.997688767029
0.91934 1.00196383624
0.923616 1.00624193253
0.927892 1.01052304951
0.932168 1.01480718123
0.936444 1.01909432216
0.94072 1.0233844672
0.944996 1.02767761168
0.949272 1.03197375132
0.953548 1.03627288229
0.957824 1.04057500116
0.9621 1.0448801049
0.966376 1.04918819092
0.970652 1.05349925703
0.974928 1.05781330145
0.979204 1.0621303228
0.98348 1.06645032011
0.987756 1.07077329284
0.992032 1.07509924081
0.996308 1.0794281643
1.000584 1.08376006394
1.00486 1.0880949408
1.009136 1.09243279634
1.013412 1.09677363243
1.017688 1.10111745133
1.021964 1.10546425573
1.02624 1.10981404868
1.030516 1.11416683367
1.034792 1.11852261458
1.039068 1.12288139569
1.043344 1.1272431817
1.04762 1.13160797769
1.051896 1.13597578917
1.056172 1.14034662205
1.060448 1.14472048264
1.064724 1.14909737765
1.069 1.15347731424
1.073276 1.15786029994
1.077552 1.16224634272
1.081828 1.16663545094
1.086104 1.1710276334
1.09038 1.1754228993
1.094656 1.17982125828
1.098932 1.18422272038
1.103208 1.18862729609
1.107484 1.19303499631
1.11176 1.19744583237
1.116036 1.20185981604
1.120312 1.20627695952
1.124588 1.21069727545
1.128864 1.21512077692
1.13314 1.21954747745
1.137416 1.22397739101
1.141692 1.22841053203
1.145968 1.2328469154
1.150244 1.23728655645
1.15452 1.24172947098
1.158796 1.24617567527
1.163072 1.25062518607
1.167348 1.25507802058
1.171624 1.25953419651
1.1759 1.26399373204
1.180176 1.26845664585
1.184452 1.2729229571
1.188728 1.27739268547
1.193004 1.28186585114
1.19728 1.28634247479
1.201556 1.29082257763
1.205832 1.29530618139
1.210108 1.29979330834
1.214384 1.30428398127
1.21866 1.30877822351
1.222936 1.31327605897
1.227212 1.31777751208
1.231488 1.32228260787
1.235764 1.32679137191
1.24004 1.33130383037
1.244316 1.33582001
1.248592 1.34033993814
1.252868 1.34486364275
1.257144 1.34939115239
1.26142 1.35392249625
1.265696 1.35845770414
1.269972 1.36299680652
1.274248 1.3675398345
1.278524 1.37208681984
1.2828 1.37663779499
1.287076 1.38119279306
1.291352 1.38575184787
1.295628 1.39031499393
1.299904 1.39488226646
1.30418 1.39945370144
1.308456 1.40402933555
1.312732 1.40860920624
1.317008 1.41319335173
1.321284 1.417781811
1.32556 1.42237462384
1.329836 1.42697183084
1.334112 1.4315734734
1.338388 1.43617959377
1.342664 1.44079023504
1.34694 1.44540544117
1.351216 1.450025257
1.355492 1.45464972828
1.359768 1.45927890166
1.364044 1.46391282474
1.36832 1.46855154605
1.372596 1.47319511512
1.376872 1.47784358245
1.381148 1.48249699955
1.385424 1.48715541897
1.3897 1.4918188943
1.393976 1.49648748021
1.398252 1.50116123248
1.402528 1.50584020797
1.406804 1.51052446471
1.41108 1.5152140619
1.415356 1.51990905992
1.419632 1.52460952035
1.423908 1.52931550605
1.428184 1.53402708112
1.43246 1.53874431097
1.436736 1.54346726233
1.441012 1.54819600331
1.445288 1.55293060339
1.449564 1.55767113346
1.45384 1.56241766589
1.458116 1.56717027452
1.462392 1.57192903471
1.466668 1.57669402339
1.470944 1.58146531907
1.47522 1.58624300191
1.479496 1.59102715372
1.483772 1.59581785804
1.488048 1.60061520017
1.492324 1.6054192672
1.4966 1.61023014805
1.500876 1.61504793357
1.505152 1.6198727165
1.509428 1.62470459161
1.513704 1.62954365568
1.51798 1.6343900076
1.522256 1.63924374839
1.526532 1.6441049813
1.530808 1.64897381182
1.535084 1.65385034775
1.53936 1.65873469932
1.543636 1.66362697917
1.547912 1.66852730247
1.552188 1.67343578699
1.556464 1.67835255314
1.56074 1.68327772407
1.565016 1.68821142575
1.569292 1.69315378702
1.573568 1.69810493973
1.577844 1.70306501876
1.58212 1.70803416215
1.586396 1.71301251119
1.590672 1.71800021049
1.594948 1.72299740814
1.599224 1.72800425572
1.6035 1.73302090851
1.607776 1.73804752552
1.612052 1.74308426967
1.616328 1.74813130785
1.620604 1.7531888111
1.62488 1.7582569547
1.629156 1.76333591836
1.633432 1.76842588629
1.637708 1.77352704741
1.641984 1.77863959545
1.64626 1.78376372918
1.650536 1.7888996525
1.654812 1.79404757467
1.659088 1.79920771049
1.663364 1.80438028043
1.66764 1.8095655109
1.671916 1.81476363443
1.676192 1.81997488989
1.680468 1.82519952268
1.684744 1.83043778502
1.68902 1.83568993619
1.693296 1.84095624273
1.697572 1.84623697878
1.701848 1.85153242634
1.706124 1.85684287555
1.7104 1.86216862501
1.714676 1.86750998213
1.718952 1.87286726344
1.723228 1.87824079495
1.727504 1.88363091256
1.73178 1.88903796241
1.736056 1.89446230134
1.740332 1.8999042973
1.744608 1.90536432981
1.748884 1.91084279047
1.75316 1.91634008344
1.757436 1.92185662599
1.761712 1.92739284909
1.765988 1.93294919795
1.770264 1.93852613272
1.77454 1.94412412912
1.778816 1.94974367914
1.783092 1.95538529181
1.787368 1.96104949396
1.791644 1.96673683109
1.79592 1.97244786823
1.800196 1.97818319089
1.804472 1.98394340606
1.808748 1.98972914325
1.813024 1.99554105563
1.8173 2.00137982124
1.821576 2.00724614423
1.825852 2.01314075624
1.830128 2.01906441784
1.834404 2.02501792008
1.83868 2.03100208612
1.842956 2.03701777301
1.847232 2.04306587357
1.851508 2.04914731839
1.855784 2.05526307802
1.86006 2.06141416528
1.864336 2.06760163774
1.868612 2.07382660043
1.872888 2.08009020868
1.877164 2.08639367127
1.88144 2.09273825377
1.885716 2.09912528217
1.889992 2.10555614676
1.894268 2.11203230642
1.898544 2.11855529321
1.90282 2.12512671731
1.907096 2.13174827253
1.911372 2.13842174217
1.915648 2.14514900546
1.919924 2.15193204463
1.9242 2.1587729526
1.928476 2.16567394138
1.932752 2.17263735139
1.937028 2.17966566159
1.941304 2.18676150074
1.94558 2.19392765972
1.949856 2.20116710532
1.954132 2.20848299531
1.958408 2.21587869537
1.962684 2.22335779787
1.96696 2.23092414275
1.971236 2.23858184104
1.975512 2.24633530112
1.979788 2.25418925828
1.984064 2.26214880814
1.98834 2.2702194444
1.992616 2.27840710169
1.996892 2.28671820442
2.001168 2.29515972262
2.005444 2.30373923597
2.00972 2.31246500758
2.013996 2.32134606939
2.018272 2.33039232128
2.022548 2.33961464696
2.026824 2.34902504976
2.0311 2.358636813
2.035376 2.36846469019
2.039652 2.37852513216
2.043928 2.38883656004
2.048204 2.39941969572
2.05248 2.41029796508
2.056756 2.42149799404
2.061032 2.43305022454
2.065308 2.44498968708
2.069584 2.45735698037
2.07386 2.47019952875
2.078136 2.48357321802
2.082412 2.49754455559
2.086688 2.51219357155
2.090964 2.52761778937
2.09524 2.54393777949
2.099516 2.56130512271
2.103792 2.57991416411
2.108068 2.60001996329
2.112344 2.62196684798
2.11662 2.64623614777
2.120896 2.67353109548
2.125172 2.70494037594
2.129448 2.74228875552
2.133724 2.78901262453


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma1pt5.tex <==
0.0 0.302797401727
0.0064 0.302838924999
0.0128 0.302962472597
0.0192 0.303166520526
0.0256 0.3034495646
0.032 0.30381012057
0.0384 0.304246724243
0.0448 0.304757931581
0.0512 0.305342318789
0.0576 0.305998482385
0.064 0.306725039257
0.0704 0.307520626704
0.0768 0.308383902466
0.0832 0.309313544735
0.0896 0.310308252153
0.096 0.311366743803
0.1024 0.312487759176
0.1088 0.313670058135
0.1152 0.314912420859
0.1216 0.316213647777
0.128 0.317572559492
0.1344 0.318987996693
0.1408 0.320458820051
0.1472 0.321983910111
0.1536 0.323562167168
0.16 0.325192511137
0.1664 0.32687388141
0.1728 0.328605236709
0.1792 0.33038555492
0.1856 0.332213832934
0.192 0.334089086466
0.1984 0.336010349874
0.2048 0.337976675968
0.2112 0.339987135816
0.2176 0.34204081854
0.224 0.344136831109
0.2304 0.346274298125
0.2368 0.348452361604
0.2432 0.350670180755
0.2496 0.352926931753
0.256 0.35522180751
0.2624 0.357554017437
0.2688 0.359922787213
0.2752 0.362327358544
0.2816 0.364766988923
0.288 0.367240951384
0.2944 0.369748534262
0.3008 0.372289040947
0.3072 0.374861789634
0.3136 0.37746611308
0.32 0.380101358359
0.3264 0.382766886607
0.3328 0.385462072786
0.3392 0.388186305429
0.3456 0.3909389864
0.352 0.393719530648
0.3584 0.396527365962
0.3648 0.399361932733
0.3712 0.402222683713
0.3776 0.405109083773
0.384 0.408020609671
0.3904 0.410956749817
0.3968 0.413917004039
0.4032 0.416900883354
0.4096 0.419907909741
0.416 0.422937615919
0.4224 0.425989545119
0.4288 0.429063250871
0.4352 0.432158296784
0.4416 0.435274256335
0.448 0.438410712657
0.4544 0.441567258333
0.4608 0.444743495189
0.4672 0.447939034099
0.4736 0.45115349478
0.48 0.454386505606
0.4864 0.457637703407
0.4928 0.46090673329
0.4992 0.464193248447
0.5056 0.467496909982
0.512 0.470817386723
0.5184 0.474154355056
0.5248 0.477507498748
0.5312 0.480876508784
0.5376 0.484261083195
0.544 0.487660926904
0.5504 0.491075751563
0.5568 0.494505275398
0.5632 0.49794922306
0.5696 0.501407325472
0.576 0.504879319689
0.5824 0.508364948749
0.5888 0.511863961539
0.5952 0.515376112654
0.6016 0.518901162266
0.608 0.522438875996
0.6144 0.525989024779
0.6208 0.529551384746
0.6272 0.5331257371
0.6336 0.536711867997
0.64 0.540309568425
0.6464 0.543918634099
0.6528 0.547538865342
0.6592 0.551170066981
0.6656 0.554812048237
0.672 0.558464622628
0.6784 0.562127607859
0.6848 0.565800825731
0.6912 0.56948410204
0.6976 0.573177266488
0.704 0.576880152583
0.7104 0.580592597559
0.7168 0.58431444228
0.7232 0.588045531162
0.7296 0.591785712086
0.736 0.595534836315
0.7424 0.59929275842
0.7488 0.603059336198
0.7552 0.606834430602
0.7616 0.610617905662
0.768 0.614409628415
0.7744 0.618209468838
0.7808 0.622017299776
0.7872 0.62583299688
0.7936 0.629656438538
0.8 0.633487505813
0.8064 0.637326082383
0.8128 0.64117205448
0.8192 0.645025310832
0.8256 0.648885742604
0.832 0.652753243346
0.8384 0.656627708935
0.8448 0.660509037525
0.8512 0.664397129495
0.8576 0.668291887396
0.864 0.672193215907
0.8704 0.676101021783
0.8768 0.68001521381
0.8832 0.683935702762
0.8896 0.687862401353
0.896 0.691795224195
0.9024 0.69573408776
0.9088 0.699678910332
0.9152 0.703629611973
0.9216 0.707586114483
0.928 0.711548341359
0.9344 0.715516217764
0.9408 0.719489670484
0.9472 0.723468627897
0.9536 0.727453019942
0.96 0.731442778077
0.9664 0.735437835255
0.9728 0.739438125889
0.9792 0.743443585818
0.9856 0.747454152284
0.992 0.751469763896
0.9984 0.755490360607
1.0048 0.759515883682
1.0112 0.763546275672
1.0176 0.76758148039
1.024 0.771621442881
1.0304 0.7756661094
1.0368 0.779715427389
1.0432 0.783769345448
1.0496 0.787827813317
1.056 0.791890781848
1.0624 0.795958202991
1.0688 0.800030029763
1.0752 0.804106216234
1.0816 0.808186717503
1.088 0.812271489682
1.0944 0.81636048987
1.1008 0.820453676141
1.1072 0.824551007522
1.1136 0.828652443975
1.12 0.832757946381
1.1264 0.836867476522
1.1328 0.840980997064
1.1392 0.845098471543
1.1456 0.849219864347
1.152 0.853345140699
1.1584 0.857474266649
1.1648 0.86160720905
1.1712 0.865743935552
1.1776 0.869884414584
1.184 0.87402861534
1.1904 0.878176507769
1.1968 0.882328062559
1.2032 0.886483251126
1.2096 0.890642045604
1.216 0.894804418828
1.2224 0.898970344328
1.2288 0.903139796314
1.2352 0.907312749667
1.2416 0.911489179928
1.248 0.915669063287
1.2544 0.919852376575
1.2608 0.924039097251
1.2672 0.928229203395
1.2736 0.932422673698
1.28 0.936619487453
1.2864 0.940819624547
1.2928 0.945023065451
1.2992 0.949229791212
1.3056 0.953439783447
1.312 0.957653024333
1.3184 0.961869496599
1.3248 0.966089183521
1.3312 0.970312068914
1.3376 0.974538137124
1.344 0.97876737302
1.3504 0.982999761993
1.3568 0.987235289944
1.3632 0.991473943278
1.3696 0.995715708904
1.376 0.999960574222
1.3824 1.00420852712
1.3888 1.00845955597
1.3952 1.01271364963
1.4016 1.01697079742
1.408 1.02123098912
1.4144 1.025494215
1.4208 1.02976046576
1.4272 1.03402973257
1.4336 1.03830200705
1.44 1.04257728126
1.4464 1.0468555477
1.4528 1.05113679933
1.4592 1.0554210295
1.4656 1.05970823204
1.472 1.06399840117
1.4784 1.06829153156
1.4848 1.07258761828
1.4912 1.07688665683
1.4976 1.08118864313
1.504 1.08549357351
1.5104 1.0898014447
1.5168 1.09411225384
1.5232 1.09842599849
1.5296 1.1027426766
1.536 1.10706228652
1.5424 1.11138482701
1.5488 1.11571029722
1.5552 1.1200386967
1.5616 1.12437002539
1.568 1.12870428362
1.5744 1.13304147213
1.5808 1.13738159203
1.5872 1.14172464482
1.5936 1.14607063241
1.6 1.15041955707
1.6064 1.15477142148
1.6128 1.1591262287
1.6192 1.16348398216
1.6256 1.16784468569
1.632 1.17220834351
1.6384 1.17657496021
1.6448 1.18094454079
1.6512 1.1853170906
1.6576 1.1896926154
1.664 1.19407112134
1.6704 1.19845261493
1.6768 1.2028371031
1.6832 1.20722459314
1.6896 1.21161509273
1.696 1.21600860997
1.7024 1.2204051533
1.7088 1.2248047316
1.7152 1.22920735412
1.7216 1.23361303048
1.728 1.23802177075
1.7344 1.24243358534
1.7408 1.24684848511
1.7472 1.25126648127
1.7536 1.25568758546
1.76 1.26011180973
1.7664 1.26453916653
1.7728 1.26896966869
1.7792 1.27340332951
1.7856 1.27784016264
1.792 1.28228018218
1.7984 1.28672340266
1.8048 1.291169839
1.8112 1.29561950656
1.8176 1.30007242114
1.824 1.30452859895
1.8304 1.30898805664
1.8368 1.31345081131
1.8432 1.31791688049
1.8496 1.32238628216
1.856 1.32685903474
1.8624 1.33133515712
1.8688 1.33581466864
1.8752 1.3402975891
1.8816 1.34478393877
1.888 1.34927373839
1.8944 1.35376700919
1.9008 1.35826377284
1.9072 1.36276405155
1.9136 1.36726786799
1.92 1.37177524534
1.9264 1.37628620726
1.9328 1.38080077795
1.9392 1.38531898212
1.9456 1.38984084498
1.952 1.39436639228
1.9584 1.39889565031
1.9648 1.40342864589
1.9712 1.4079654064
1.9776 1.41250595977
1.984 1.41705033449
1.9904 1.42159855961
1.9968 1.42615066478
2.0032 1.43070668022
2.0096 1.43526663675
2.016 1.43983056579
2.0224 1.44439849937
2.0288 1.44897047015
2.0352 1.4535465114
2.0416 1.45812665704
2.048 1.46271094165
2.0544 1.46729940044
2.0608 1.47189206932
2.0672 1.47648898485
2.0736 1.48109018429
2.08 1.48569570563
2.0864 1.49030558752
2.0928 1.49491986936
2.0992 1.49953859131
2.1056 1.50416179422
2.112 1.50878951977
2.1184 1.51342181035
2.1248 1.51805870917
2.1312 1.52270026025
2.1376 1.5273465084
2.144 1.53199749927
2.1504 1.53665327937
2.1568 1.54131389603
2.1632 1.5459793975
2.1696 1.55064983288
2.176 1.55532525222
2.1824 1.56000570647
2.1888 1.56469124752
2.1952 1.56938192823
2.2016 1.57407780243
2.208 1.57877892497
2.2144 1.58348535169
2.2208 1.58819713948
2.2272 1.59291434628
2.2336 1.59763703114
2.24 1.60236525417
2.2464 1.60709907664
2.2528 1.61183856093
2.2592 1.61658377063
2.2656 1.6213347705
2.272 1.62609162652
2.2784 1.63085440595
2.2848 1.63562317727
2.2912 1.64039801031
2.2976 1.6451789762
2.304 1.64996614745
2.3104 1.65475959793
2.3168 1.65955940296
2.3232 1.66436563929
2.3296 1.66917838518
2.336 1.67399772038
2.3424 1.6788237262
2.3488 1.68365648557
2.3552 1.688496083
2.3616 1.6933426047
2.368 1.69819613857
2.3744 1.70305677427
2.3808 1.70792460323
2.3872 1.71279971873
2.3936 1.71768221591
2.4 1.72257219183
2.4064 1.72746974556
2.4128 1.73237497815
2.4192 1.73728799273
2.4256 1.74220889457
2.432 1.74713779111
2.4384 1.75207479203
2.4448 1.7570200093
2.4512 1.76197355725
2.4576 1.76693555265
2.464 1.77190611471
2.4704 1.77688536522
2.4768 1.7818734286
2.4832 1.78687043195
2.4896 1.79187650512
2.496 1.79689178085
2.5024 1.80191639476
2.5088 1.80695048552
2.5152 1.81199419487
2.5216 1.81704766776
2.528 1.82211105239
2.5344 1.82718450037
2.5408 1.83226816675
2.5472 1.83736221022
2.5536 1.8424667931
2.56 1.84758208155
2.5664 1.85270824565
2.5728 1.85784545952
2.5792 1.86299390145
2.5856 1.86815375405
2.592 1.87332520435
2.5984 1.87850844401
2.6048 1.88370366938
2.6112 1.88891108174
2.6176 1.89413088743
2.624 1.899363298
2.6304 1.90460853043
2.6368 1.90986680729
2.6432 1.91513835694
2.6496 1.92042341375
2.656 1.92572221827
2.6624 1.93103501752
2.6688 1.93636206515
2.6752 1.94170362176
2.6816 1.9470599551
2.688 1.95243134035
2.6944 1.95781806044
2.7008 1.9632204063
2.7072 1.96863867719
2.7136 1.97407318106
2.72 1.97952423483
2.7264 1.98499216481
2.7328 1.99047730707
2.7392 1.99598000782
2.7456 2.00150062387
2.752 2.00703952305
2.7584 2.01259708471
2.7648 2.0181737002
2.7712 2.0237697734
2.7776 2.02938572131
2.784 2.03502197462
2.7904 2.04067897833
2.7968 2.04635719246
2.8032 2.0520570927
2.8096 2.05777917123
2.816 2.06352393747
2.8224 2.06929191897
2.8288 2.0750836623
2.8352 2.08089973402
2.8416 2.08674072173
2.848 2.09260723517
2.8544 2.09849990741
2.8608 2.10441939612
2.8672 2.11036638493
2.8736 2.11634158489
2.88 2.12234573606
2.8864 2.12837960918
2.8928 2.13444400751
2.8992 2.14053976879
2.9056 2.1466677674
2.912 2.15282891661
2.9184 2.15902417114
2.9248 2.16525452983
2.9312 2.17152103862
2.9376 2.17782479374
2.944 2.18416694526
2.9504 2.19054870092
2.9568 2.19697133031
2.9632 2.20343616953
2.9696 2.2099446263
2.976 2.21649818551
2.9824 2.22309841551
2.9888 2.22974697492
2.9952 2.23644562037
3.0016 2.24319621495
3.008 2.25000073781
3.0144 2.25686129487
3.0208 2.26378013081
3.0272 2.27075964275
3.0336 2.27780239559
3.04 2.28491113965
3.0464 2.29208883067
3.0528 2.29933865288
3.0592 2.3066640456
3.0656 2.31406873402
3.072 2.32155676528
3.0784 2.32913255059
3.0848 2.33680091521
3.0912 2.34456715779
3.0976 2.35243712167
3.104 2.36041728101
3.1104 2.3685148462
3.1168 2.37673789383
3.1232 2.38509552917
3.1296 2.39359809182
3.136 2.40225741992
3.1424 2.41108719547
3.1488 2.42010340443
3.1552 2.42932496378
3.1616 2.43877459912
3.168 2.44848011221
3.1744 2.45847628348
3.1808 2.46880786649
3.1872 2.47953459676
3.1936 2.49074027328


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma1pt5prob0pt05.tex <==
0.0 0.240218559204
0.004276 0.242366574095
0.008552 0.244534616277
0.012828 0.246722678277
0.017104 0.24893074765
0.02138 0.251158806998
0.025656 0.253406833986
0.029932 0.255674801375
0.034208 0.25796267705
0.038484 0.260270424067
0.04276 0.262598000692
0.047036 0.264945360456
0.051312 0.26731245221
0.055588 0.269699220186
0.059864 0.272105604069
0.06414 0.274531539063
0.068416 0.276976955971
0.072692 0.279441781279
0.076968 0.281925937237
0.081244 0.284429341953
0.08552 0.286951909485
0.089796 0.28949354994
0.094072 0.292054169574
0.098348 0.294633670899
0.102624 0.297231952785
0.1069 0.299848910577
0.111176 0.3024844362
0.115452 0.305138418279
0.119728 0.307810742253
0.124004 0.310501290492
0.12828 0.313209942418
0.132556 0.315936574626
0.136832 0.318681061001
0.141108 0.321443272847
0.145384 0.324223079002
0.14966 0.327020345964
0.153936 0.329834938013
0.158212 0.332666717333
0.162488 0.335515544134
0.166764 0.338381276769
0.17104 0.341263771859
0.175316 0.344162884408
0.179592 0.347078467925
0.183868 0.350010374533
0.188144 0.35295845509
0.19242 0.355922559298
0.196696 0.358902535815
0.200972 0.361898232364
0.205248 0.364909495841
0.209524 0.367936172416
0.2138 0.370978107638
0.218076 0.374035146535
0.222352 0.377107133712
0.226628 0.38019391344
0.230904 0.383295329758
0.23518 0.386411226554
0.239456 0.389541447657
0.243732 0.392685836919
0.248008 0.395844238296
0.252284 0.399016495929
0.25656 0.402202454219
0.260836 0.405401957898
0.265112 0.408614852102
0.269388 0.411840982439
0.273664 0.41508019505
0.27794 0.418332336676
0.282216 0.421597254714
0.286492 0.424874797275
0.290768 0.428164813238
0.295044 0.4314671523
0.29932 0.434781665028
0.303596 0.438108202903
0.307872 0.441446618365
0.312148 0.444796764851
0.316424 0.448158496841
0.3207 0.451531669887
0.324976 0.454916140653
0.329252 0.458311766945
0.333528 0.461718407741
0.337804 0.46513592322
0.34208 0.468564174785
0.346356 0.472003025092
0.350632 0.475452338068
0.354908 0.478911978932
0.359184 0.482381814213
0.36346 0.48586171177
0.367736 0.489351540802
0.372012 0.492851171863
0.376288 0.496360476878
0.380564 0.499879329146
0.38484 0.503407603355
0.389116 0.506945175585
0.393392 0.510491923319
0.397668 0.514047725443
0.401944 0.517612462253
0.40622 0.521186015456
0.410496 0.524768268172
0.414772 0.528359104933
0.419048 0.531958411687
0.423324 0.535566075789
0.4276 0.539181986006
0.431876 0.542806032507
0.436152 0.546438106866
0.440428 0.55007810205
0.444704 0.553725912418
0.44898 0.557381433714
0.453256 0.561044563058
0.457532 0.56471519894
0.461808 0.568393241214
0.466084 0.572078591083
0.47036 0.575771151098
0.474636 0.579470825142
0.478912 0.583177518423
0.483188 0.586891137461
0.487464 0.590611590082
0.49174 0.594338785403
0.496016 0.598072633819
0.500292 0.601813046997
0.504568 0.605559937859
0.508844 0.60931322057
0.51312 0.61307281053
0.517396 0.616838624355
0.521672 0.620610579869
0.525948 0.62438859609
0.530224 0.628172593215
0.5345 0.631962492608
0.538776 0.635758216787
0.543052 0.63955968941
0.547328 0.643366835263
0.551604 0.647179580242
0.55588 0.650997851346
0.560156 0.654821576658
0.564432 0.658650685334
0.568708 0.662485107587
0.572984 0.666324774678
0.57726 0.670169618897
0.581536 0.674019573553
0.585812 0.677874572959
0.590088 0.681734552419
0.594364 0.685599448214
0.59864 0.689469197589
0.602916 0.693343738741
0.607192 0.697223010802
0.611468 0.701106953832
0.615744 0.704995508799
0.62002 0.708888617572
0.624296 0.712786222902
0.628572 0.716688268417
0.632848 0.720594698603
0.637124 0.724505458794
0.6414 0.728420495158
0.645676 0.732339754688
0.649952 0.736263185187
0.654228 0.740190735256
0.658504 0.744122354283
0.66278 0.748057992431
0.667056 0.751997600628
0.671332 0.755941130552
0.675608 0.759888534621
0.679884 0.763839765984
0.68416 0.767794778506
0.688436 0.771753526762
0.692712 0.775715966019
0.696988 0.779682052234
0.701264 0.783651742035
0.70554 0.787624992718
0.709816 0.79160176223
0.714092 0.795582009164
0.718368 0.799565692746
0.722644 0.803552772829
0.72692 0.807543209875
0.731196 0.811536964957
0.735472 0.815533999738
0.739748 0.819534276471
0.744024 0.823537757983
0.7483 0.827544407671
0.752576 0.831554189489
0.756852 0.835567067943
0.761128 0.839583008078
0.765404 0.843601975475
0.76968 0.847623936236
0.773956 0.851648856983
0.778232 0.855676704842
0.782508 0.859707447442
0.786784 0.863741052904
0.79106 0.867777489833
0.795336 0.871816727308
0.799612 0.875858734883
0.803888 0.879903482569
0.808164 0.883950940833
0.81244 0.888001080591
0.816716 0.892053873197
0.820992 0.89610929044
0.825268 0.900167304535
0.829544 0.904227888116
0.83382 0.908291014233
0.838096 0.91235665634
0.842372 0.916424788293
0.846648 0.920495384341
0.850924 0.924568419122
0.8552 0.928643867655
0.859476 0.932721705337
0.863752 0.936801907932
0.868028 0.940884451571
0.872304 0.944969312741
0.87658 0.949056468284
0.880856 0.95314589539
0.885132 0.957237571588
0.889408 0.961331474748
0.893684 0.965427583068
0.89796 0.969525875076
0.902236 0.973626329617
0.906512 0.977728925857
0.910788 0.981833643272
0.915064 0.985940461643
0.91934 0.990049361056
0.923616 0.994160321892
0.927892 0.998273324828
0.932168 1.00238835083
0.936444 1.00650538114
0.94072 1.01062439729
0.944996 1.01474538108
0.949272 1.01886831459
0.953548 1.02299318016
0.957824 1.0271199604
0.9621 1.03124863816
0.966376 1.03537919658
0.970652 1.03951161902
0.974928 1.04364588911
0.979204 1.0477819907
0.98348 1.05191990791
0.987756 1.05605962507
0.992032 1.06020112676
0.996308 1.06434439779
1.000584 1.06848942319
1.00486 1.07263618822
1.009136 1.07678467834
1.013412 1.08093487926
1.017688 1.08508677689
1.021964 1.08924035733
1.02624 1.09339560691
1.030516 1.09755251217
1.034792 1.10171105984
1.039068 1.10587123685
1.043344 1.11003303032
1.04762 1.11419642757
1.051896 1.11836141612
1.056172 1.12252798366
1.060448 1.12669611808
1.064724 1.13086580744
1.069 1.13503703999
1.073276 1.13920980416
1.077552 1.14338408853
1.081828 1.1475598819
1.086104 1.15173717318
1.09038 1.1559159515
1.094656 1.16009620613
1.098932 1.16427792651
1.103208 1.16846110224
1.107484 1.17264572308
1.11176 1.17683177895
1.116036 1.18101925991
1.120312 1.18520815618
1.124588 1.18939845815
1.128864 1.19359015634
1.13314 1.1977832414
1.137416 1.20197770417
1.141692 1.20617353559
1.145968 1.21037072677
1.150244 1.21456926894
1.15452 1.21876915347
1.158796 1.22297037188
1.163072 1.22717291581
1.167348 1.23137677703
1.171624 1.23558194746
1.1759 1.23978841913
1.180176 1.2439961842
1.184452 1.24820523497
1.188728 1.25241556383
1.193004 1.25662716334
1.19728 1.26084002615
1.201556 1.26505414503
1.205832 1.26926951288
1.210108 1.27348612272
1.214384 1.27770396765
1.21866 1.28192304094
1.222936 1.28614333593
1.227212 1.29036484608
1.231488 1.29458756497
1.235764 1.29881148629
1.24004 1.30303660383
1.244316 1.30726291147
1.248592 1.31149040323
1.252868 1.31571907321
1.257144 1.31994891562
1.26142 1.32417992477
1.265696 1.32841209507
1.269972 1.33264542104
1.274248 1.33687989726
1.278524 1.34111551847
1.2828 1.34535227944
1.287076 1.34959017509
1.291352 1.3538292004
1.295628 1.35806935045
1.299904 1.36231062042
1.30418 1.36655300558
1.308456 1.37079650129
1.312732 1.37504110298
1.317008 1.37928680619
1.321284 1.38353360655
1.32556 1.38778149976
1.329836 1.39203048162
1.334112 1.39628054801
1.338388 1.40053169489
1.342664 1.4047839183
1.34694 1.40903721437
1.351216 1.41329157932
1.355492 1.41754700943
1.359768 1.42180350108
1.364044 1.42606105072
1.36832 1.43031965488
1.372596 1.43457931016
1.376872 1.43884001325
1.381148 1.4431017609
1.385424 1.44736454997
1.3897 1.45162837736
1.393976 1.45589324006
1.398252 1.46015913513
1.402528 1.4644260597
1.406804 1.46869401098
1.41108 1.47296298626
1.415356 1.47723298288
1.419632 1.48150399827
1.423908 1.48577602992
1.428184 1.49004907539
1.43246 1.49432313232
1.436736 1.49859819841
1.441012 1.50287427142
1.445288 1.5071513492
1.449564 1.51142942966
1.45384 1.51570851076
1.458116 1.51998859054
1.462392 1.52426966711
1.466668 1.52855173864
1.470944 1.53283480337
1.47522 1.5371188596
1.479496 1.54140390569
1.483772 1.54568994007
1.488048 1.54997696123
1.492324 1.55426496774
1.4966 1.55855395821
1.500876 1.56284393131
1.505152 1.5671348858
1.509428 1.57142682048
1.513704 1.57571973422
1.51798 1.58001362594
1.522256 1.58430849463
1.526532 1.58860433935
1.530808 1.59290115919
1.535084 1.59719895333
1.53936 1.601497721
1.543636 1.60579746149
1.547912 1.61009817413
1.552188 1.61439985835
1.556464 1.6187025136
1.56074 1.6230061394
1.565016 1.62731073533
1.569292 1.63161630104
1.573568 1.63592283622
1.577844 1.64023034063
1.58212 1.64453881406
1.586396 1.6488482564
1.590672 1.65315866756
1.594948 1.65747004753
1.599224 1.66178239634
1.6035 1.66609571409
1.607776 1.67041000093
1.612052 1.67472525706
1.616328 1.67904148274
1.620604 1.6833586783
1.62488 1.68767684411
1.629156 1.69199598059
1.633432 1.69631608823
1.637708 1.70063716756
1.641984 1.70495921919
1.64626 1.70928224376
1.650536 1.71360624198
1.654812 1.7179312146
1.659088 1.72225716245
1.663364 1.72658408638
1.66764 1.73091198732
1.671916 1.73524086625
1.676192 1.73957072421
1.680468 1.74390156228
1.684744 1.7482333816
1.68902 1.75256618337
1.693296 1.75689996884
1.697572 1.76123473931
1.701848 1.76557049616
1.706124 1.76990724078
1.7104 1.77424497465
1.714676 1.7785836993
1.718952 1.78292341629
1.723228 1.78726412728
1.727504 1.79160583393
1.73178 1.79594853799
1.736056 1.80029224127
1.740332 1.80463694561
1.744608 1.80898265292
1.748884 1.81332936515
1.75316 1.81767708433
1.757436 1.82202581253
1.761712 1.82637555187
1.765988 1.83072630453
1.770264 1.83507807276
1.77454 1.83943085884
1.778816 1.84378466512
1.783092 1.84813949401
1.787368 1.85249534796
1.791644 1.85685222949
1.79592 1.86121014118
1.800196 1.86556908564
1.804472 1.86992906557
1.808748 1.87429008371
1.813024 1.87865214284
1.8173 1.88301524583
1.821576 1.8873793956
1.825852 1.89174459509
1.830128 1.89611084736
1.834404 1.90047815547
1.83868 1.90484652256
1.842956 1.90921595185
1.847232 1.91358644659
1.851508 1.91795801009
1.855784 1.92233064572
1.86006 1.92670435694
1.864336 1.93107914722
1.868612 1.93545502012
1.872888 1.93983197926
1.877164 1.94421002831
1.88144 1.948589171
1.885716 1.95296941112
1.889992 1.95735075254
1.894268 1.96173319917
1.898544 1.96611675498
1.90282 1.97050142402
1.907096 1.97488721039
1.911372 1.97927411825
1.915648 1.98366215184
1.919924 1.98805131544
1.9242 1.9924416134
1.928476 1.99683305015
1.932752 2.00122563017
1.937028 2.005619358
1.941304 2.01001423826
1.94558 2.01441027562
1.949856 2.01880747484
1.954132 2.02320584071
1.958408 2.02760537812
1.962684 2.03200609201
1.96696 2.03640798739
1.971236 2.04081106934
1.975512 2.04521534302
1.979788 2.04962081362
1.984064 2.05402748645
1.98834 2.05843536686
1.992616 2.06284446027
1.996892 2.06725477218
2.001168 2.07166630816
2.005444 2.07607907385
2.00972 2.08049307497
2.013996 2.0849083173
2.018272 2.08932480669
2.022548 2.09374254909
2.026824 2.0981615505
2.0311 2.102581817
2.035376 2.10700335475
2.039652 2.11142616999
2.043928 2.11585026904
2.048204 2.12027565827
2.05248 2.12470234416
2.056756 2.12913033325
2.061032 2.13355963218
2.065308 2.13799024765
2.069584 2.14242218644
2.07386 2.14685545542
2.078136 2.15129006155
2.082412 2.15572601186
2.086688 2.16016331346
2.090964 2.16460197357
2.09524 2.16904199946
2.099516 2.1734833985
2.103792 2.17792617817
2.108068 2.182370346
2.112344 2.18681590962
2.11662 2.19126287677
2.120896 2.19571125526
2.125172 2.20016105298
2.129448 2.20461227795
2.133724 2.20906493823


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma1pt5prob0pt5.tex <==
0.0 0.240218559204
0.004276 0.242366574095
0.008552 0.244534616277
0.012828 0.246722678277
0.017104 0.24893074765
0.02138 0.251158806998
0.025656 0.253406833986
0.029932 0.255674801375
0.034208 0.25796267705
0.038484 0.260270424067
0.04276 0.262598000692
0.047036 0.264945360456
0.051312 0.26731245221
0.055588 0.269699220186
0.059864 0.272105604069
0.06414 0.274531539063
0.068416 0.276976955971
0.072692 0.279441781279
0.076968 0.281925937237
0.081244 0.284429341953
0.08552 0.286951909485
0.089796 0.28949354994
0.094072 0.292054169574
0.098348 0.294633670899
0.102624 0.297231952785
0.1069 0.299848910577
0.111176 0.3024844362
0.115452 0.305138418279
0.119728 0.307810742253
0.124004 0.310501290492
0.12828 0.313209942418
0.132556 0.315936574626
0.136832 0.318681061001
0.141108 0.321443272847
0.145384 0.324223079002
0.14966 0.327020345964
0.153936 0.329834938013
0.158212 0.332666717333
0.162488 0.335515544134
0.166764 0.338381276769
0.17104 0.341263771859
0.175316 0.344162884408
0.179592 0.347078467925
0.183868 0.350010374533
0.188144 0.35295845509
0.19242 0.355922559298
0.196696 0.358902535815
0.200972 0.361898232364
0.205248 0.364909495841
0.209524 0.367936172416
0.2138 0.370978107638
0.218076 0.374035146535
0.222352 0.377107133712
0.226628 0.38019391344
0.230904 0.383295329758
0.23518 0.386411226554
0.239456 0.389541447657
0.243732 0.392685836919
0.248008 0.395844238296
0.252284 0.399016495929
0.25656 0.402202454219
0.260836 0.405401957898
0.265112 0.408614852102
0.269388 0.411840982439
0.273664 0.41508019505
0.27794 0.418332336676
0.282216 0.421597254714
0.286492 0.424874797275
0.290768 0.428164813238
0.295044 0.4314671523
0.29932 0.434781665028
0.303596 0.438108202903
0.307872 0.441446618365
0.312148 0.444796764851
0.316424 0.448158496841
0.3207 0.451531669887
0.324976 0.454916140653
0.329252 0.458311766945
0.333528 0.461718407741
0.337804 0.46513592322
0.34208 0.468564174785
0.346356 0.472003025092
0.350632 0.475452338068
0.354908 0.478911978932
0.359184 0.482381814213
0.36346 0.48586171177
0.367736 0.489351540802
0.372012 0.492851171863
0.376288 0.496360476878
0.380564 0.499879329146
0.38484 0.503407603355
0.389116 0.506945175585
0.393392 0.510491923319
0.397668 0.514047725443
0.401944 0.517612462253
0.40622 0.521186015456
0.410496 0.524768268172
0.414772 0.528359104933
0.419048 0.531958411687
0.423324 0.535566075789
0.4276 0.539181986006
0.431876 0.542806032507
0.436152 0.546438106866
0.440428 0.55007810205
0.444704 0.553725912418
0.44898 0.557381433714
0.453256 0.561044563058
0.457532 0.56471519894
0.461808 0.568393241214
0.466084 0.572078591083
0.47036 0.575771151098
0.474636 0.579470825142
0.478912 0.583177518423
0.483188 0.586891137461
0.487464 0.590611590082
0.49174 0.594338785403
0.496016 0.598072633819
0.500292 0.601813046997
0.504568 0.605559937859
0.508844 0.60931322057
0.51312 0.61307281053
0.517396 0.616838624355
0.521672 0.620610579869
0.525948 0.62438859609
0.530224 0.628172593215
0.5345 0.631962492608
0.538776 0.635758216787
0.543052 0.63955968941
0.547328 0.643366835263
0.551604 0.647179580242
0.55588 0.650997851346
0.560156 0.654821576658
0.564432 0.658650685334
0.568708 0.662485107587
0.572984 0.666324774678
0.57726 0.670169618897
0.581536 0.674019573553
0.585812 0.677874572959
0.590088 0.681734552419
0.594364 0.685599448214
0.59864 0.689469197589
0.602916 0.693343738741
0.607192 0.697223010802
0.611468 0.701106953832
0.615744 0.704995508799
0.62002 0.708888617572
0.624296 0.712786222902
0.628572 0.716688268417
0.632848 0.720594698603
0.637124 0.724505458794
0.6414 0.728420495158
0.645676 0.732339754688
0.649952 0.736263185187
0.654228 0.740190735256
0.658504 0.744122354283
0.66278 0.748057992431
0.667056 0.751997600628
0.671332 0.755941130552
0.675608 0.759888534621
0.679884 0.763839765984
0.68416 0.767794778506
0.688436 0.771753526762
0.692712 0.775715966019
0.696988 0.779682052234
0.701264 0.783651742035
0.70554 0.787624992718
0.709816 0.79160176223
0.714092 0.795582009164
0.718368 0.799565692746
0.722644 0.803552772829
0.72692 0.807543209875
0.731196 0.811536964957
0.735472 0.815533999738
0.739748 0.819534276471
0.744024 0.823537757983
0.7483 0.827544407671
0.752576 0.831554189489
0.756852 0.835567067943
0.761128 0.839583008078
0.765404 0.843601975475
0.76968 0.847623936236
0.773956 0.851648856983
0.778232 0.855676704842
0.782508 0.859707447442
0.786784 0.863741052904
0.79106 0.867777489833
0.795336 0.871816727308
0.799612 0.875858734883
0.803888 0.879903482569
0.808164 0.883950940833
0.81244 0.888001080591
0.816716 0.892053873197
0.820992 0.89610929044
0.825268 0.900167304535
0.829544 0.904227888116
0.83382 0.908291014233
0.838096 0.91235665634
0.842372 0.916424788293
0.846648 0.920495384341
0.850924 0.924568419122
0.8552 0.928643867655
0.859476 0.932721705337
0.863752 0.936801907932
0.868028 0.940884451571
0.872304 0.944969312741
0.87658 0.949056468284
0.880856 0.95314589539
0.885132 0.957237571588
0.889408 0.961331474748
0.893684 0.965427583068
0.89796 0.969525875076
0.902236 0.973626329617
0.906512 0.977728925857
0.910788 0.981833643272
0.915064 0.985940461643
0.91934 0.990049361056
0.923616 0.994160321892
0.927892 0.998273324828
0.932168 1.00238835083
0.936444 1.00650538114
0.94072 1.01062439729
0.944996 1.01474538108
0.949272 1.01886831459
0.953548 1.02299318016
0.957824 1.0271199604
0.9621 1.03124863816
0.966376 1.03537919658
0.970652 1.03951161902
0.974928 1.04364588911
0.979204 1.0477819907
0.98348 1.05191990791
0.987756 1.05605962507
0.992032 1.06020112676
0.996308 1.06434439779
1.000584 1.06848942319
1.00486 1.07263618822
1.009136 1.07678467834
1.013412 1.08093487926
1.017688 1.08508677689
1.021964 1.08924035733
1.02624 1.09339560691
1.030516 1.09755251217
1.034792 1.10171105984
1.039068 1.10587123685
1.043344 1.11003303032
1.04762 1.11419642757
1.051896 1.11836141612
1.056172 1.12252798366
1.060448 1.12669611808
1.064724 1.13086580744
1.069 1.13503703999
1.073276 1.13920980416
1.077552 1.14338408853
1.081828 1.1475598819
1.086104 1.15173717318
1.09038 1.1559159515
1.094656 1.16009620613
1.098932 1.16427792651
1.103208 1.16846110224
1.107484 1.17264572308
1.11176 1.17683177895
1.116036 1.18101925991
1.120312 1.18520815618
1.124588 1.18939845815
1.128864 1.19359015634
1.13314 1.1977832414
1.137416 1.20197770417
1.141692 1.20617353559
1.145968 1.21037072677
1.150244 1.21456926894
1.15452 1.21876915347
1.158796 1.22297037188
1.163072 1.22717291581
1.167348 1.23137677703
1.171624 1.23558194746
1.1759 1.23978841913
1.180176 1.2439961842
1.184452 1.24820523497
1.188728 1.25241556383
1.193004 1.25662716334
1.19728 1.26084002615
1.201556 1.26505414503
1.205832 1.26926951288
1.210108 1.27348612272
1.214384 1.27770396765
1.21866 1.28192304094
1.222936 1.28614333593
1.227212 1.29036484608
1.231488 1.29458756497
1.235764 1.29881148629
1.24004 1.30303660383
1.244316 1.30726291147
1.248592 1.31149040323
1.252868 1.31571907321
1.257144 1.31994891562
1.26142 1.32417992477
1.265696 1.32841209507
1.269972 1.33264542104
1.274248 1.33687989726
1.278524 1.34111551847
1.2828 1.34535227944
1.287076 1.34959017509
1.291352 1.3538292004
1.295628 1.35806935045
1.299904 1.36231062042
1.30418 1.36655300558
1.308456 1.37079650129
1.312732 1.37504110298
1.317008 1.37928680619
1.321284 1.38353360655
1.32556 1.38778149976
1.329836 1.39203048162
1.334112 1.39628054801
1.338388 1.40053169489
1.342664 1.4047839183
1.34694 1.40903721437
1.351216 1.41329157932
1.355492 1.41754700943
1.359768 1.42180350108
1.364044 1.42606105072
1.36832 1.43031965488
1.372596 1.43457931016
1.376872 1.43884001325
1.381148 1.4431017609
1.385424 1.44736454997
1.3897 1.45162837736
1.393976 1.45589324006
1.398252 1.46015913513
1.402528 1.4644260597
1.406804 1.46869401098
1.41108 1.47296298626
1.415356 1.47723298288
1.419632 1.48150399827
1.423908 1.48577602992
1.428184 1.49004907539
1.43246 1.49432313232
1.436736 1.49859819841
1.441012 1.50287427142
1.445288 1.5071513492
1.449564 1.51142942966
1.45384 1.51570851076
1.458116 1.51998859054
1.462392 1.52426966711
1.466668 1.52855173864
1.470944 1.53283480337
1.47522 1.5371188596
1.479496 1.54140390569
1.483772 1.54568994007
1.488048 1.54997696123
1.492324 1.55426496774
1.4966 1.55855395821
1.500876 1.56284393131
1.505152 1.5671348858
1.509428 1.57142682048
1.513704 1.57571973422
1.51798 1.58001362594
1.522256 1.58430849463
1.526532 1.58860433935
1.530808 1.59290115919
1.535084 1.59719895333
1.53936 1.601497721
1.543636 1.60579746149
1.547912 1.61009817413
1.552188 1.61439985835
1.556464 1.6187025136
1.56074 1.6230061394
1.565016 1.62731073533
1.569292 1.63161630104
1.573568 1.63592283622
1.577844 1.64023034063
1.58212 1.64453881406
1.586396 1.6488482564
1.590672 1.65315866756
1.594948 1.65747004753
1.599224 1.66178239634
1.6035 1.66609571409
1.607776 1.67041000093
1.612052 1.67472525706
1.616328 1.67904148274
1.620604 1.6833586783
1.62488 1.68767684411
1.629156 1.69199598059
1.633432 1.69631608823
1.637708 1.70063716756
1.641984 1.70495921919
1.64626 1.70928224376
1.650536 1.71360624198
1.654812 1.7179312146
1.659088 1.72225716245
1.663364 1.72658408638
1.66764 1.73091198732
1.671916 1.73524086625
1.676192 1.73957072421
1.680468 1.74390156228
1.684744 1.7482333816
1.68902 1.75256618337
1.693296 1.75689996884
1.697572 1.76123473931
1.701848 1.76557049616
1.706124 1.76990724078
1.7104 1.77424497465
1.714676 1.7785836993
1.718952 1.78292341629
1.723228 1.78726412728
1.727504 1.79160583393
1.73178 1.79594853799
1.736056 1.80029224127
1.740332 1.80463694561
1.744608 1.80898265292
1.748884 1.81332936515
1.75316 1.81767708433
1.757436 1.82202581253
1.761712 1.82637555187
1.765988 1.83072630453
1.770264 1.83507807276
1.77454 1.83943085884
1.778816 1.84378466512
1.783092 1.84813949401
1.787368 1.85249534796
1.791644 1.85685222949
1.79592 1.86121014118
1.800196 1.86556908564
1.804472 1.86992906557
1.808748 1.87429008371
1.813024 1.87865214284
1.8173 1.88301524583
1.821576 1.8873793956
1.825852 1.89174459509
1.830128 1.89611084736
1.834404 1.90047815547
1.83868 1.90484652256
1.842956 1.90921595185
1.847232 1.91358644659
1.851508 1.91795801009
1.855784 1.92233064572
1.86006 1.92670435694
1.864336 1.93107914722
1.868612 1.93545502012
1.872888 1.93983197926
1.877164 1.94421002831
1.88144 1.948589171
1.885716 1.95296941112
1.889992 1.95735075254
1.894268 1.96173319917
1.898544 1.96611675498
1.90282 1.97050142402
1.907096 1.97488721039
1.911372 1.97927411825
1.915648 1.98366215184
1.919924 1.98805131544
1.9242 1.9924416134
1.928476 1.99683305015
1.932752 2.00122563017
1.937028 2.005619358
1.941304 2.01001423826
1.94558 2.01441027562
1.949856 2.01880747484
1.954132 2.02320584071
1.958408 2.02760537812
1.962684 2.03200609201
1.96696 2.03640798739
1.971236 2.04081106934
1.975512 2.04521534302
1.979788 2.04962081362
1.984064 2.05402748645
1.98834 2.05843536686
1.992616 2.06284446027
1.996892 2.06725477218
2.001168 2.07166630816
2.005444 2.07607907385
2.00972 2.08049307497
2.013996 2.0849083173
2.018272 2.08932480669
2.022548 2.09374254909
2.026824 2.0981615505
2.0311 2.102581817
2.035376 2.10700335475
2.039652 2.11142616999
2.043928 2.11585026904
2.048204 2.12027565827
2.05248 2.12470234416
2.056756 2.12913033325
2.061032 2.13355963218
2.065308 2.13799024765
2.069584 2.14242218644
2.07386 2.14685545542
2.078136 2.15129006155
2.082412 2.15572601186
2.086688 2.16016331346
2.090964 2.16460197357
2.09524 2.16904199946
2.099516 2.1734833985
2.103792 2.17792617817
2.108068 2.182370346
2.112344 2.18681590962
2.11662 2.19126287677
2.120896 2.19571125526
2.125172 2.20016105298
2.129448 2.20461227795
2.133724 2.20906493823


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma2.tex <==
0.0 0.459043605026
0.00853 0.463330619152
0.01706 0.467661655327
0.02559 0.472036694963
0.03412 0.476455707107
0.04265 0.480918648484
0.05118 0.485425463566
0.05971 0.489976084645
0.06824 0.494570431933
0.07677 0.499208413674
0.0853 0.503889926274
0.09383 0.508614854449
0.10236 0.513383071382
0.11089 0.518194438903
0.11942 0.523048807679
0.12795 0.527946017418
0.13648 0.532885897088
0.14501 0.537868265146
0.15354 0.542892929783
0.16207 0.547959689173
0.1706 0.553068331743
0.17913 0.55821863644
0.18766 0.563410373019
0.19619 0.568643302329
0.20472 0.573917176614
0.21325 0.579231739813
0.22178 0.584586727875
0.23031 0.58998186907
0.23884 0.595416884306
0.24737 0.600891487458
0.2559 0.606405385684
0.26443 0.611958279756
0.27296 0.617549864385
0.28149 0.623179828554
0.29002 0.628847855835
0.29855 0.634553624726
0.30708 0.640296808968
0.31561 0.64607707787
0.32414 0.65189409663
0.33267 0.657747526646
0.3412 0.663637025834
0.34973 0.669562248931
0.35826 0.675522847802
0.36679 0.681518471732
0.37532 0.687548767724
0.38385 0.693613380779
0.39238 0.699711954181
0.40091 0.705844129765
0.40944 0.712009548187
0.41797 0.718207849178
0.4265 0.724438671802
0.43503 0.730701654695
0.44356 0.736996436301
0.45209 0.743322655105
0.46062 0.74967994985
0.46915 0.756067959751
0.47768 0.762486324701
0.48621 0.768934685467
0.49474 0.775412683879
0.50327 0.781919963009
0.5118 0.78845616735
0.52033 0.795020942976
0.52886 0.801613937701
0.53739 0.808234801231
0.54592 0.814883185304
0.55445 0.821558743824
0.56298 0.828261132995
0.57151 0.834990011431
0.58004 0.841745040281
0.58857 0.848525883327
0.5971 0.855332207087
0.60563 0.862163680908
0.61416 0.869019977053
0.62269 0.875900770784
0.63122 0.882805740431
0.63975 0.889734567467
0.64828 0.896686936569
0.65681 0.903662535672
0.66534 0.91066105603
0.67387 0.917682192256
0.6824 0.924725642366
0.69093 0.931791107821
0.69946 0.938878293556
0.70799 0.94598690801
0.71652 0.953116663153
0.72505 0.960267274504
0.73358 0.967438461151
0.74211 0.97462994576
0.75064 0.981841454591
0.75917 0.989072717501
0.7677 0.996323467948
0.77623 1.00359344299
0.78476 1.0108823833
0.79329 1.01819003311
0.80182 1.02551614029
0.81035 1.03286045624
0.81888 1.04022273596
0.82741 1.04760273799
0.83594 1.0550002244
0.84447 1.06241496079
0.853 1.06984671626
0.86153 1.07729526336
0.87006 1.08476037813
0.87859 1.09224184002
0.88712 1.0997394319
0.89565 1.10725293999
0.90418 1.1147821539
0.91271 1.12232686654
0.92124 1.1298868741
0.92977 1.13746197605
0.9383 1.14505197509
0.94683 1.1526566771
0.95536 1.16027589116
0.96389 1.16790942945
0.97242 1.17555710726
0.98095 1.18321874294
0.98948 1.19089415787
0.99801 1.19858317644
1.00654 1.20628562599
1.01507 1.21400133677
1.0236 1.22173014194
1.03213 1.2294718775
1.04066 1.23722638228
1.04919 1.24499349788
1.05772 1.25277306866
1.06625 1.26056494168
1.07478 1.26836896667
1.08331 1.27618499601
1.09184 1.28401288468
1.10037 1.29185249024
1.1089 1.29970367276
1.11743 1.30756629483
1.12596 1.3154402215
1.13449 1.32332532024
1.14302 1.33122146092
1.15155 1.33912851579
1.16008 1.34704635939
1.16861 1.3549748686
1.17714 1.36291392252
1.18567 1.37086340251
1.1942 1.37882319212
1.20273 1.38679317704
1.21126 1.39477324514
1.21979 1.40276328636
1.22832 1.41076319271
1.23685 1.41877285826
1.24538 1.42679217907
1.25391 1.43482105322
1.26244 1.44285938069
1.27097 1.45090706343
1.2795 1.45896400525
1.28803 1.46703011186
1.29656 1.47510529078
1.30509 1.48318945137
1.31362 1.49128250476
1.32215 1.49938436384
1.33068 1.50749494325
1.33921 1.51561415931
1.34774 1.52374193005
1.35627 1.53187817515
1.3648 1.54002281593
1.37333 1.54817577532
1.38186 1.55633697782
1.39039 1.56450634953
1.39892 1.57268381806
1.40745 1.58086931255
1.41598 1.58906276367
1.42451 1.59726410352
1.43304 1.60547326568
1.44157 1.61369018517
1.4501 1.62191479842
1.45863 1.63014704326
1.46716 1.6383868589
1.47569 1.6466341859
1.48422 1.65488896616
1.49275 1.66315114292
1.50128 1.6714206607
1.50981 1.67969746533
1.51834 1.68798150389
1.52687 1.69627272472
1.5354 1.70457107741
1.54393 1.71287651275
1.55246 1.72118898274
1.56099 1.72950844059
1.56952 1.73783484067
1.57805 1.7461681385
1.58658 1.75450829077
1.59511 1.76285525529
1.60364 1.77120899099
1.61217 1.7795694579
1.6207 1.78793661716
1.62923 1.79631043097
1.63776 1.80469086262
1.64629 1.81307787644
1.65482 1.82147143782
1.66335 1.82987151316
1.67188 1.8382780699
1.68041 1.8466910765
1.68894 1.8551105024
1.69747 1.86353631804
1.706 1.87196849484
1.71453 1.8804070052
1.72306 1.88885182248
1.73159 1.89730292098
1.74012 1.90576027596
1.74865 1.91422386361
1.75718 1.92269366105
1.76571 1.93116964632
1.77424 1.93965179837
1.78277 1.94814009707
1.7913 1.95663452316
1.79983 1.96513505829
1.80836 1.97364168499
1.81689 1.98215438668
1.82542 1.99067314764
1.83395 1.99919795301
1.84248 2.0077287888
1.85101 2.01626564189
1.85954 2.02480849998
1.86807 2.03335735163
1.8766 2.04191218625
1.88513 2.05047299408
1.89366 2.05903976618
1.90219 2.06761249446
1.91072 2.07619117163
1.91925 2.08477579125
1.92778 2.09336634767
1.93631 2.10196283608
1.94484 2.11056525246
1.95337 2.11917359361
1.9619 2.12778785715
1.97043 2.13640804149
1.97896 2.14503414585
1.98749 2.15366617024
1.99602 2.16230411548
2.00455 2.17094798321
2.01308 2.17959777583
2.02161 2.18825349656
2.03014 2.19691514942
2.03867 2.20558273923
2.0472 2.21425627159
2.05573 2.22293575291
2.06426 2.2316211904
2.07279 2.24031259206
2.08132 2.2490099667
2.08985 2.25771332392
2.09838 2.26642267414
2.10691 2.27513802857
2.11544 2.28385939922
2.12397 2.29258679892
2.1325 2.30132024132
2.14103 2.31005974086
2.14956 2.3188053128
2.15809 2.32755697324
2.16662 2.33631473909
2.17515 2.34507862806
2.18368 2.35384865874
2.19221 2.36262485052
2.20074 2.37140722363
2.20927 2.38019579915
2.2178 2.38899059901
2.22633 2.39779164598
2.23486 2.40659896371
2.24339 2.41541257669
2.25192 2.42423251029
2.26045 2.43305879077
2.26898 2.44189144523
2.27751 2.45073050172
2.28604 2.45957598913
2.29457 2.46842793729
2.3031 2.47728637692
2.31163 2.48615133967
2.32016 2.49502285812
2.32869 2.50390096578
2.33722 2.5127856971
2.34575 2.5216770875
2.35428 2.53057517334
2.36281 2.53947999197
2.37134 2.54839158173
2.37987 2.55730998194
2.3884 2.56623523293
2.39693 2.57516737605
2.40546 2.58410645368
2.41399 2.59305250922
2.42252 2.60200558716
2.43105 2.61096573301
2.43958 2.6199329934
2.44811 2.62890741604
2.45664 2.63788904973
2.46517 2.6468779444
2.4737 2.65587415113
2.48223 2.66487772214
2.49076 2.67388871081
2.49929 2.68290717171
2.50782 2.69193316062
2.51635 2.70096673452
2.52488 2.71000795164
2.53341 2.71905687146
2.54194 2.72811355472
2.55047 2.73717806346
2.559 2.74625046105
2.56753 2.75533081216
2.57606 2.76441918284
2.58459 2.7735156405
2.59312 2.78262025395
2.60165 2.79173309342
2.61018 2.8008542306
2.61871 2.80998373862
2.62724 2.81912169213
2.63577 2.82826816727
2.6443 2.83742324176
2.65283 2.84658699487
2.66136 2.85575950748
2.66989 2.86494086209
2.67842 2.87413114286
2.68695 2.88333043566
2.69548 2.89253882805
2.70401 2.90175640936
2.71254 2.91098327072
2.72107 2.92021950504
2.7296 2.92946520713
2.73813 2.93872047366
2.74666 2.94798540324
2.75519 2.95726009646
2.76372 2.96654465588
2.77225 2.97583918614
2.78078 2.98514379395
2.78931 2.99445858817
2.79784 3.00378367981
2.80637 3.01311918211
2.8149 3.02246521059
2.82343 3.03182188307
2.83196 3.04118931975
2.84049 3.05056764321
2.84902 3.05995697855
2.85755 3.06935745336
2.86608 3.0787691978
2.87461 3.08819234471
2.88314 3.09762702957
2.89167 3.10707339066
2.9002 3.11653156906
2.90873 3.12600170874
2.91726 3.13548395662
2.92579 3.14497846264
2.93432 3.15448537983
2.94285 3.16400486439
2.95138 3.17353707577
2.95991 3.18308217672
2.96844 3.1926403334
2.97697 3.20221171546
2.9855 3.21179649612
2.99403 3.22139485225
3.00256 3.23100696447
3.01109 3.24063301727
3.01962 3.25027319906
3.02815 3.2599277023
3.03668 3.26959672361
3.04521 3.27928046385
3.05374 3.28897912829
3.06227 3.29869292665
3.0708 3.30842207327
3.07933 3.31816678722
3.08786 3.32792729243
3.09639 3.33770381783
3.10492 3.34749659748
3.11345 3.3573058707
3.12198 3.36713188225
3.13051 3.37697488245
3.13904 3.38683512736
3.14757 3.39671287894
3.1561 3.4066084052
3.16463 3.41652198043
3.17316 3.42645388532
3.18169 3.4364044072
3.19022 3.44637384019
3.19875 3.45636248547
3.20728 3.46637065143
3.21581 3.47639865393
3.22434 3.48644681651
3.23287 3.49651547065
3.2414 3.506604956
3.24993 3.51671562065
3.25846 3.52684782139
3.26699 3.53700192401
3.27552 3.54717830358
3.28405 3.55737734473
3.29258 3.56759944201
3.30111 3.57784500021
3.30964 3.58811443468
3.31817 3.5984081717
3.3267 3.60872664889
3.33523 3.61907031553
3.34376 3.62943963305
3.35229 3.63983507539
3.36082 3.65025712949
3.36935 3.66070629572
3.37788 3.67118308841
3.38641 3.68168803632
3.39494 3.69222168319
3.40347 3.7027845883
3.412 3.71337732707
3.42053 3.72400049164
3.42906 3.73465469153
3.43759 3.74534055433
3.44612 3.75605872636
3.45465 3.76680987348
3.46318 3.77759468183
3.47171 3.78841385864
3.48024 3.79926813311
3.48877 3.81015825733
3.4973 3.82108500721
3.50583 3.83204918348
3.51436 3.8430516128
3.52289 3.85409314881
3.53142 3.86517467335
3.53995 3.87629709768
3.54848 3.88746136383
3.55701 3.89866844594
3.56554 3.90991935175
3.57407 3.92121512416
3.5826 3.93255684286
3.59113 3.94394562609
3.59966 3.95538263244
3.60819 3.96686906286
3.61672 3.97840616273
3.62525 3.98999522405
3.63378 4.00163758778
3.64231 4.01333464638
3.65084 4.02508784645
3.65937 4.03689869155
3.6679 4.04876874526
3.67643 4.06069963438
3.68496 4.07269305242
3.69349 4.08475076325
3.70202 4.0968746051
3.71055 4.10906649474
3.71908 4.12132843209
3.72761 4.13366250505
3.73614 4.14607089478
3.74467 4.15855588131
3.7532 4.17111984964
3.76173 4.18376529631
3.77026 4.19649483644
3.77879 4.20931121144
3.78732 4.22221729723
3.79585 4.23521611328
3.80438 4.24831083229
3.81291 4.26150479085
3.82144 4.27480150089
3.82997 4.28820466232
3.8385 4.30171817666
3.84703 4.3153461621
3.85556 4.32909296987
3.86409 4.34296320228
3.87262 4.35696173252
3.88115 4.37109372641
3.88968 4.38536466649
3.89821 4.3997803786
3.90674 4.41434706125
3.91527 4.4290713184
3.9238 4.44396019574
3.93233 4.45902122125
3.94086 4.4742624506
3.94939 4.48969251787
3.95792 4.50532069277
3.96645 4.52115694494
3.97498 4.53721201681
3.98351 4.5534975061
3.99204 4.57002595982
4.00057 4.5868109815
4.0091 4.60386735416
4.01763 4.62121118177
4.02616 4.63886005268
4.03469 4.6568332293
4.04322 4.6751518692
4.05175 4.69383928422
4.06028 4.71292124555
4.06881 4.73242634526
4.07734 4.75238642702
4.08587 4.77283710287
4.0944 4.79381837736
4.10293 4.81537540732
4.11146 4.83755943424
4.11999 4.86042893876
4.12852 4.88405108427
4.13705 4.90850354133
4.14558 4.93387682079
4.15411 4.96027729656
4.16264 4.9878311791
4.17117 5.01668982419
4.1797 5.0470369568
4.18823 5.07909870749
4.19676 5.1131578933
4.20529 5.1495749075
4.21382 5.18881928405
4.22235 5.23151926853
4.23088 5.27854339456
4.23941 5.33114273535
4.24794 5.39121795535
4.25647 5.46187206455


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt05.tex <==
0.0 0.320291412272
0.008276 0.32445754832
0.016552 0.328679941716
0.024828 0.332958548254
0.033104 0.337293294386
0.04138 0.341684077413
0.049656 0.34613076576
0.057932 0.35063319931
0.066208 0.355191189826
0.074484 0.359804521428
0.08276 0.364472951148
0.091036 0.369196209541
0.099312 0.37397400136
0.107588 0.378806006282
0.115864 0.383691879692
0.12414 0.388631253511
0.132416 0.393623737066
0.140692 0.398668918
0.148968 0.40376636322
0.157244 0.408915619862
0.16552 0.414116216299
0.173796 0.419367663149
0.182072 0.424669454312
0.190348 0.430021068012
0.198624 0.435421967844
0.2069 0.440871603831
0.215176 0.446369413464
0.223452 0.451914822753
0.231728 0.457507247255
0.240004 0.463146093099
0.24828 0.468830757985
0.256556 0.474560632173
0.264832 0.480335099444
0.273108 0.486153538042
0.281384 0.492015321584
0.28966 0.497919819947
0.297936 0.503866400123
0.306212 0.509854427041
0.314488 0.515883264364
0.322764 0.521952275241
0.33104 0.528060823038
0.339316 0.534208272026
0.347592 0.540393988038
0.355868 0.54661733909
0.364144 0.55287769597
0.37242 0.559174432788
0.380696 0.565506927497
0.388972 0.571874562375
0.397248 0.578276724483
0.405524 0.58471280608
0.4138 0.591182205014
0.422076 0.597684325079
0.430352 0.604218576344
0.438628 0.610784375454
0.446904 0.6173811459
0.45518 0.624008318268
0.463456 0.630665330454
0.471732 0.637351627864
0.480008 0.644066663586
0.488284 0.650809898538
0.49656 0.6575808016
0.504836 0.66437884972
0.513112 0.671203528008
0.521388 0.678054329804
0.529664 0.684930756739
0.53794 0.691832318769
0.546216 0.698758534206
0.554492 0.705708929725
0.562768 0.712683040363
0.571044 0.719680409508
0.57932 0.726700588871
0.587596 0.733743138454
0.595872 0.740807626504
0.604148 0.747893629459
0.612424 0.755000731889
0.6207 0.762128526425
0.628976 0.769276613686
0.637252 0.776444602197
0.645528 0.783632108303
0.653804 0.790838756077
0.66208 0.798064177223
0.670356 0.805308010979
0.678632 0.812569904011
0.686908 0.819849510311
0.695184 0.827146491083
0.70346 0.834460514639
0.711736 0.841791256279
0.720012 0.849138398183
0.728288 0.856501629293
0.736564 0.8638806452
0.74484 0.87127514802
0.753116 0.878684846288
0.761392 0.88610945483
0.769668 0.893548694655
0.777944 0.901002292831
0.78622 0.908469982374
0.794496 0.915951502128
0.802772 0.923446596653
0.811048 0.93095501611
0.819324 0.938476516147
0.8276 0.946010857789
0.835876 0.953557807322
0.844152 0.961117136192
0.852428 0.968688620888
0.860704 0.976272042841
0.86898 0.983867188316
0.877256 0.991473848309
0.885532 0.999091818444
0.893808 1.00672089887
0.902084 1.01436089418
0.91036 1.02201161328
0.918636 1.02967286932
0.926912 1.03734447959
0.935188 1.04502626544
0.943464 1.05271805217
0.95174 1.06041966895
0.960016 1.06813094874
0.968292 1.0758517282
0.976568 1.0835818476
0.984844 1.09132115075
0.99312 1.09906948491
1.001396 1.1068267007
1.009672 1.11459265208
1.017948 1.12236719619
1.026224 1.13015019334
1.0345 1.13794150692
1.042776 1.14574100332
1.051052 1.15354855188
1.059328 1.1613640248
1.067604 1.16918729709
1.07588 1.17701824652
1.084156 1.18485675351
1.092432 1.19270270113
1.100708 1.20055597498
1.108984 1.20841646318
1.11726 1.2162840563
1.125536 1.22415864728
1.133812 1.23204013141
1.142088 1.23992840625
1.150364 1.2478233716
1.15864 1.25572492944
1.166916 1.26363298387
1.175192 1.27154744109
1.183468 1.27946820931
1.191744 1.28739519875
1.20002 1.29532832158
1.208296 1.30326749185
1.216572 1.3112126255
1.224848 1.31916364026
1.233124 1.32712045565
1.2414 1.33508299294
1.249676 1.34305117509
1.257952 1.35102492671
1.266228 1.35900417407
1.274504 1.36698884499
1.28278 1.37497886889
1.291056 1.38297417668
1.299332 1.39097470077
1.307608 1.39898037505
1.315884 1.40699113479
1.32416 1.4150069167
1.332436 1.42302765884
1.340712 1.4310533006
1.348988 1.43908378268
1.357264 1.44711904709
1.36554 1.45515903705
1.373816 1.46320369704
1.382092 1.47125297273
1.390368 1.47930681098
1.398644 1.48736515978
1.40692 1.49542796828
1.415196 1.50349518672
1.423472 1.51156676643
1.431748 1.51964265979
1.440024 1.52772282023
1.4483 1.53580720221
1.456576 1.54389576118
1.464852 1.55198845357
1.473128 1.56008523677
1.481404 1.56818606912
1.48968 1.57629090988
1.497956 1.58439971921
1.506232 1.59251245816
1.514508 1.60062908866
1.522784 1.60874957349
1.53106 1.61687387627
1.539336 1.62500196144
1.547612 1.63313379425
1.555888 1.64126934074
1.564164 1.64940856773
1.57244 1.65755144281
1.580716 1.66569793432
1.588992 1.67384801133
1.597268 1.68200164362
1.605544 1.69015880172
1.61382 1.69831945681
1.622096 1.70648358081
1.630372 1.71465114626
1.638648 1.7228221264
1.646924 1.73099649511
1.6552 1.73917422691
1.663476 1.74735529695
1.671752 1.755539681
1.680028 1.76372735544
1.688304 1.77191829725
1.69658 1.78011248399
1.704856 1.78830989382
1.713132 1.79651050545
1.721408 1.80471429817
1.729684 1.81292125182
1.73796 1.82113134677
1.746236 1.82934456395
1.754512 1.83756088481
1.762788 1.84578029131
1.771064 1.85400276595
1.77934 1.8622282917
1.787616 1.87045685206
1.795892 1.87868843101
1.804168 1.88692301302
1.812444 1.89516058304
1.82072 1.90340112648
1.828996 1.91164462924
1.837272 1.91989107765
1.845548 1.92814045852
1.853824 1.9363927591
1.8621 1.94464796708
1.870376 1.95290607059
1.878652 1.96116705819
1.886928 1.96943091887
1.895204 1.97769764205
1.90348 1.98596721756
1.911756 1.99423963565
1.920032 2.00251488695
1.928308 2.01079296254
1.936584 2.01907385387
1.94486 2.02735755278
1.953136 2.03564405154
1.961412 2.04393334276
1.969688 2.05222541948
1.977964 2.06052027508
1.98624 2.06881790334
1.994516 2.07711829842
2.002792 2.08542145484
2.011068 2.09372736748
2.019344 2.10203603161
2.02762 2.11034744284
2.035896 2.11866159714
2.044172 2.12697849085
2.052448 2.13529812066
2.060724 2.14362048361
2.069 2.15194557708
2.077276 2.16027339882
2.085552 2.1686039469
2.093828 2.17693721974
2.102104 2.18527321613
2.11038 2.19361193515
2.118656 2.20195337626
2.126932 2.21029753923
2.135208 2.21864442419
2.143484 2.22699403156
2.15176 2.23534636215
2.160036 2.24370141705
2.168312 2.25205919771
2.176588 2.26041970589
2.184864 2.26878294369
2.19314 2.27714891354
2.201416 2.28551761818
2.209692 2.29388906068
2.217968 2.30226324445
2.226244 2.31064017321
2.23452 2.31901985099
2.242796 2.32740228218
2.251072 2.33578747146
2.259348 2.34417542384
2.267624 2.35256614467
2.2759 2.36095963961
2.284176 2.36935591463
2.292452 2.37775497605
2.300728 2.38615683049
2.309004 2.3945614849
2.31728 2.40296894655
2.325556 2.41137922306
2.333832 2.41979232234
2.342108 2.42820825264
2.350384 2.43662702254
2.35866 2.44504864095
2.366936 2.45347311708
2.375212 2.46190046051
2.383488 2.47033068112
2.391764 2.47876378913
2.40004 2.4871997951
2.408316 2.49563870991
2.416592 2.50408054478
2.424868 2.51252531127
2.433144 2.52097302127
2.44142 2.52942368702
2.449696 2.53787732109
2.457972 2.5463339364
2.466248 2.55479354622
2.474524 2.56325616416
2.4828 2.57172180417
2.491076 2.58019048056
2.499352 2.588662208
2.507628 2.59713700151
2.515904 2.60561487646
2.52418 2.6140958486
2.532456 2.62257993401
2.540732 2.63106714918
2.549008 2.63955751093
2.557284 2.64805103647
2.56556 2.65654774338
2.573836 2.66504764962
2.582112 2.67355077353
2.590388 2.68205713383
2.598664 2.69056674963
2.60694 2.69907964044
2.615216 2.70759582615
2.623492 2.71611532704
2.631768 2.72463816383
2.640044 2.73316435761
2.64832 2.74169392988
2.656596 2.75022690258
2.664872 2.75876329805
2.673148 2.76730313905
2.681424 2.77584644877
2.6897 2.78439325084
2.697976 2.79294356931
2.706252 2.8014974287
2.714528 2.81005485393
2.722804 2.81861587041
2.73108 2.827180504
2.739356 2.835748781
2.747632 2.8443207282
2.755908 2.85289637285
2.764184 2.86147574268
2.77246 2.87005886591
2.780736 2.87864577125
2.789012 2.88723648789
2.797288 2.89583104554
2.805564 2.90442947441
2.81384 2.91303180523
2.822116 2.92163806925
2.830392 2.93024829826
2.838668 2.93886252457
2.846944 2.94748078103
2.85522 2.95610310106
2.863496 2.96472951863
2.871772 2.97336006827
2.880048 2.9819947851
2.888324 2.9906337048
2.8966 2.99927686367
2.904876 3.00792429857
2.913152 3.016576047
2.921428 3.02523214708
2.929704 3.03389263752
2.93798 3.0425575577
2.946256 3.05122694764
2.954532 3.05990084801
2.962808 3.06857930012
2.971084 3.077262346
2.97936 3.08595002834
2.987636 3.09464239053
2.995912 3.10333947666
3.004188 3.11204133156
3.012464 3.12074800076
3.02074 3.12945953055
3.029016 3.13817596798
3.037292 3.14689736086
3.045568 3.15562375776
3.053844 3.16435520807
3.06212 3.17309176197
3.070396 3.18183347046
3.078672 3.19058038537
3.086948 3.19933255939
3.095224 3.20809004606
3.1035 3.21685289979
3.111776 3.22562117588
3.120052 3.23439493056
3.128328 3.24317422097
3.136604 3.25195910517
3.14488 3.2607496422
3.153156 3.26954589206
3.161432 3.27834791576
3.169708 3.28715577529
3.177984 3.29596953368
3.18626 3.30478925501
3.194536 3.31361500442
3.202812 3.32244684815
3.211088 3.33128485351
3.219364 3.34012908897
3.22764 3.34897962413
3.235916 3.35783652977
3.244192 3.36669987786
3.252468 3.37556974157
3.260744 3.38444619534
3.26902 3.39332931483
3.277296 3.40221917702
3.285572 3.41111586019
3.293848 3.42001944398
3.302124 3.42893000935
3.3104 3.43784763871
3.318676 3.44677241585
3.326952 3.45570442602
3.335228 3.46464375596
3.343504 3.47359049392
3.35178 3.48254472968
3.360056 3.49150655461
3.368332 3.50047606168
3.376608 3.50945334549
3.384884 3.51843850235
3.39316 3.52743163023
3.401436 3.53643282891
3.409712 3.5454421999
3.417988 3.55445984658
3.426264 3.56348587416
3.43454 3.57252038979
3.442816 3.58156350255
3.451092 3.59061532351
3.459368 3.59967596578
3.467644 3.60874554456
3.47592 3.61782417718
3.484196 3.62691198313
3.492472 3.63600908416
3.500748 3.64511560428
3.509024 3.65423166984
3.5173 3.66335740957
3.525576 3.67249295465
3.533852 3.68163843877
3.542128 3.69079399818
3.550404 3.69995977174
3.55868 3.709135901
3.566956 3.71832253029
3.575232 3.72751980672
3.583508 3.73672788032
3.591784 3.74594690407
3.60006 3.75517703397
3.608336 3.76441842916
3.616612 3.77367125194
3.624888 3.78293566791
3.633164 3.79221184599
3.64144 3.80149995858
3.649716 3.81080018158
3.657992 3.82011269453
3.666268 3.82943768066
3.674544 3.83877532707
3.68282 3.84812582471
3.691096 3.85748936862
3.699372 3.86686615792
3.707648 3.87625639599
3.715924 3.8856602906
3.7242 3.89507805395
3.732476 3.9045099029
3.740752 3.913956059
3.749028 3.92341674868
3.757304 3.93289220341
3.76558 3.94238265976
3.773856 3.95188835964
3.782132 3.96140955038
3.790408 3.97094648496
3.798684 3.9804994221
3.80696 3.99006862649
3.815236 3.99965436894
3.823512 4.0092569266
3.831788 4.01887658308
3.840064 4.02851362872
3.84834 4.03816836077
3.856616 4.04784108361
3.864892 4.05753210897
3.873168 4.06724175614
3.881444 4.07697035226
3.88972 4.08671823254
3.897996 4.09648574053
3.906272 4.10627322839
3.914548 4.11608105716
3.922824 4.12590959709
3.9311 4.13575922791
3.939376 4.1456303392
3.947652 4.15552333066
3.955928 4.16543861251
3.964204 4.17537660584
3.97248 4.18533774298
3.980756 4.19532246793
3.989032 4.20533123673
3.997308 4.21536451791
4.005584 4.22542279298
4.01386 4.23550655686
4.022136 4.24561631838
4.030412 4.25575260082
4.038688 4.26591594246
4.046964 4.27610689712
4.05524 4.28632603479
4.063516 4.29657394224
4.071792 4.30685122366
4.080068 4.31715850141
4.088344 4.32749641668
4.09662 4.3378656303
4.104896 4.3482668235
4.113172 4.35870069881
4.121448 4.36916798087
4.129724 4.37966941745


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt1.tex <==
0.0 0.459043605026
0.0841218682305 0.5032407464
0.168243736461 0.55165298416
0.252365604692 0.604115959843
0.336487472922 0.660378844751
0.420609341153 0.720132324207
0.504731209383 0.78303758718
0.588853077614 0.848751351875
0.672974945844 0.916944410345
0.757096814075 0.987313382263
0.841218682305 1.0595867203
0.925340550536 1.13352651328
1.00946241877 1.20892758045
1.093584287 1.28561504554
1.17770615523 1.36344122559
1.26182802346 1.44228236604
1.34594989169 1.52203552842
1.43007175992 1.60261578634
1.51419362815 1.68395379188
1.59831549638 1.76599372116
1.68243736461 1.84869158003
1.76655923284 1.93201383942
1.85068110107 2.01593636734
1.9348029693 2.10044362735
2.01892483753 2.18552811884
2.10304670576 2.27119004145
2.18716857399 2.35743717377
2.27129044222 2.44428496535
2.35541231046 2.53175685052
2.43953417869 2.61988480413
2.52365604692 2.70871017309
2.60777791515 2.79828483543
2.69189978338 2.88867276235
2.77602165161 2.97995209153
2.86014351984 3.07221786644
2.94426538807 3.16558566499
3.0283872563 3.26019644251
3.11250912453 3.35622307211
3.19663099276 3.45387931399
3.28075286099 3.55343235203
3.36487472922 3.65522072098
3.44899659745 3.75968064908
3.53311846568 3.86738604338
3.61724033391 3.97911159929
3.70136220214 4.09593726876
3.78548407037 4.21943176773
3.8696059386 4.35200039994
3.95372780684 4.49761463232
4.03784967507 4.66357732911
4.1219715433 4.86584665822


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt3.tex <==
0.0 0.844600430901
0.0608288216233 0.875796868305
0.121657643247 0.908553958713
0.18248646487 0.942861602995
0.243315286493 0.978703301404
0.304144108116 1.01605663158
0.36497292974 1.05489387958
0.425801751363 1.09518279066
0.486630572986 1.13688740278
0.54745939461 1.17996892581
0.608288216233 1.22438663168
0.669117037856 1.27009872561
0.72994585948 1.31706317466
0.790774681103 1.36523847652
0.851603502726 1.41458435838
0.912432324349 1.46506240175
0.973261145973 1.51663659452
1.0340899676 1.56927381589
1.09491878922 1.62294426299
1.15574761084 1.67762183088
1.21657643247 1.73328445899
1.27740525409 1.78991445859
1.33823407571 1.84749883713
1.39906289734 1.90602963609
1.45989171896 1.9655043007
1.52072054058 2.02592610158
1.58154936221 2.08730463114
1.64237818383 2.14965640171
1.70320700545 2.21300557768
1.76403582708 2.27738488225
1.8248646487 2.3428367303
1.88569347032 2.4094146551
1.94652229195 2.47718511908
2.00735111357 2.54622983154
2.06817993519 2.61664874379
2.12900875682 2.68856396273
2.18983757844 2.76212493044
2.25066640006 2.83751538225
2.31149522169 2.91496285684
2.37232404331 2.9947519584
2.43315286493 3.07724328967
2.49398168656 3.16290123453
2.55481050818 3.25233607653
2.6156393298 3.34637039366
2.67646815143 3.44614882434
2.73729697305 3.55333061841
2.79812579467 3.67045406284
2.85895461629 3.80169963955
2.91978343792 3.95473315531
2.98061225954 4.14625281077


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt6.tex <==
0.0 1.35372872606
0.0396220919817 1.37390218105
0.0792441839634 1.39480051277
0.118866275945 1.4164239019
0.158488367927 1.43877266481
0.198110459909 1.46184727641
0.23773255189 1.48564840232
0.277354643872 1.51017694034
0.316976735854 1.5354340715
0.356598827835 1.56142132095
0.396220919817 1.58814062891
0.435843011799 1.61559443227
0.475465103781 1.64378575747
0.515087195762 1.67271832529
0.554709287744 1.70239666892
0.594331379726 1.73282626632
0.633953471707 1.76401368885
0.673575563689 1.79596676813
0.713197655671 1.82869478404
0.752819747653 1.86220867702
0.792441839634 1.89652128914
0.832063931616 1.93164763903
0.871686023598 1.96760523743
0.911308115579 2.00441445163
0.950930207561 2.04209892927
0.990552299543 2.08068609481
1.03017439152 2.12020773549
1.06979648351 2.16070069871
1.10941857549 2.20220772872
1.14904066747 2.24477847966
1.18866275945 2.2884707533
1.22828485143 2.3333520265
1.26790694341 2.37950135629
1.3075290354 2.42701178276
1.34715112738 2.47599339794
1.38677321936 2.52657731819
1.42639531134 2.57892090366
1.46601740332 2.63321473114
1.50563949531 2.68969208476
1.54526158729 2.74864215034
1.58488367927 2.8104288091
1.62450577125 2.8755181705
1.66412786323 2.94452026243
1.70374995521 3.0182546941
1.7433720472 3.09785914402
1.78299413918 3.1849795823
1.82261623116 3.28213017087
1.86223832314 3.39344677598
1.90186041512 3.52650657882
1.9414825071 3.69780434443


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma2pt01.tex <==
0.0 0.459043605026
0.0841218682305 0.5032407464
0.168243736461 0.55165298416
0.252365604692 0.604115959843
0.336487472922 0.660378844751
0.420609341153 0.720132324207
0.504731209383 0.78303758718
0.588853077614 0.848751351875
0.672974945844 0.916944410345
0.757096814075 0.987313382263
0.841218682305 1.0595867203
0.925340550536 1.13352651328
1.00946241877 1.20892758045
1.093584287 1.28561504554
1.17770615523 1.36344122559
1.26182802346 1.44228236604
1.34594989169 1.52203552842
1.43007175992 1.60261578634
1.51419362815 1.68395379188
1.59831549638 1.76599372116
1.68243736461 1.84869158003
1.76655923284 1.93201383942
1.85068110107 2.01593636734
1.9348029693 2.10044362735
2.01892483753 2.18552811884
2.10304670576 2.27119004145
2.18716857399 2.35743717377
2.27129044222 2.44428496535
2.35541231046 2.53175685052
2.43953417869 2.61988480413
2.52365604692 2.70871017309
2.60777791515 2.79828483543
2.69189978338 2.88867276235
2.77602165161 2.97995209153
2.86014351984 3.07221786644
2.94426538807 3.16558566499
3.0283872563 3.26019644251
3.11250912453 3.35622307211
3.19663099276 3.45387931399
3.28075286099 3.55343235203
3.36487472922 3.65522072098
3.44899659745 3.75968064908
3.53311846568 3.86738604338
3.61724033391 3.97911159929
3.70136220214 4.09593726876
3.78548407037 4.21943176773
3.8696059386 4.35200039994
3.95372780684 4.49761463232
4.03784967507 4.66357732911
4.1219715433 4.86584665822


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma4prob0pt3.tex <==
0.0 1.6892008618
0.121657643247 1.75159373661
0.243315286493 1.81710791743
0.36497292974 1.88572320599
0.486630572986 1.95740660281
0.608288216233 2.03211326315
0.72994585948 2.10978775916
0.851603502726 2.19036558132
0.973261145973 2.27377480557
1.09491878922 2.35993785162
1.21657643247 2.44877326335
1.33823407571 2.54019745122
1.45989171896 2.63412634932
1.58154936221 2.73047695304
1.70320700545 2.82916871675
1.8248646487 2.93012480349
1.94652229195 3.03327318905
2.06817993519 3.13854763178
2.18983757844 3.24588852597
2.31149522169 3.35524366176
2.43315286493 3.46656891798
2.55481050818 3.57982891718
2.67646815143 3.69499767426
2.79812579467 3.81205927218
2.91978343792 3.93100860141
3.04144108116 4.05185220316
3.16309872441 4.17460926228
3.28475636766 4.29931280341
3.4064140109 4.42601115536
3.52807165415 4.5547697645
3.6497292974 4.6856734606
3.77138694064 4.81882931021
3.89304458389 4.95437023817
4.01470222714 5.09245966308
4.13635987038 5.23329748758
4.25801751363 5.37712792546
4.37967515688 5.52424986088
4.50133280012 5.6750307645
4.62299044337 5.82992571367
4.74464808662 5.9895039168
4.86630572986 6.15448657934
4.98796337311 6.32580246906
5.10962101636 6.50467215307
5.2312786596 6.69274078732
5.35293630285 6.89229764867
5.4745939461 7.10666123681
5.59625158934 7.34090812567
5.71790923259 7.60339927909
5.83956687584 7.90946631063
5.96122451908 8.29250562155


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt3.tex <==
0.0 3.3784017236
0.243315286493 3.50318747322
0.486630572986 3.63421583485
0.72994585948 3.77144641198
0.973261145973 3.91481320562
1.21657643247 4.0642265263
1.45989171896 4.21957551832
1.70320700545 4.38073116265
1.94652229195 4.54754961113
2.18983757844 4.71987570324
2.43315286493 4.89754652671
2.67646815143 5.08039490244
2.91978343792 5.26825269865
3.16309872441 5.46095390608
3.4064140109 5.65833743351
3.6497292974 5.86024960698
3.89304458389 6.0665463781
4.13635987038 6.27709526355
4.37967515688 6.49177705194
4.62299044337 6.71048732353
4.86630572986 6.93313783596
5.10962101636 7.15965783437
5.35293630285 7.38999534851
5.59625158934 7.62411854435
5.83956687584 7.86201720281
6.08288216233 8.10370440632
6.32619744882 8.34921852456
6.56951273532 8.59862560682
6.81282802181 8.85202231072
7.0561433083 9.109539529
7.2994585948 9.37134692121
7.54277388129 9.63765862042
7.78608916778 9.90874047634
8.02940445428 10.1849193262
8.27271974077 10.4665949752
8.51603502726 10.7542558509
8.75935031375 11.0484997218
9.00266560025 11.350061529
9.24598088674 11.6598514273
9.48929617323 11.9790078336
9.73261145973 12.3089731587
9.97592674622 12.6516049381
10.2192420327 13.0093443061
10.4625573192 13.3854815746
10.7058726057 13.7845952973
10.9491878922 14.2133224736
11.1925031787 14.6818162513
11.4358184652 15.2067985582
11.6791337517 15.8189326213
11.9224490382 16.5850112431


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt6.tex <==
0.0 5.41491490422
0.158488367927 5.49560872421
0.316976735854 5.5792020511
0.475465103781 5.66569560762
0.633953471707 5.75509065924
0.792441839634 5.84738910565
0.950930207561 5.94259360928
1.10941857549 6.04070776134
1.26790694341 6.141736286
1.42639531134 6.2456852838
1.58488367927 6.35256251563
1.7433720472 6.4623777291
1.90186041512 6.57514302986
2.06034878305 6.69087330115
2.21883715098 6.80958667567
2.3773255189 6.93130506529
2.53581388683 7.05605475538
2.69430225476 7.18386707252
2.85279062268 7.31477913614
3.01127899061 7.44883470809
3.16976735854 7.58608515657
3.32825572646 7.72659055612
3.48674409439 7.87042094971
3.64523246232 8.01765780651
3.80372083024 8.1683957171
3.96220919817 8.32274437924
4.1206975661 8.48083094197
4.27918593403 8.64280279482
4.43767430195 8.80883091488
4.59616266988 8.97911391865
4.75465103781 9.15388301318
4.91313940573 9.33340810602
5.07162777366 9.51800542516
5.23011614159 9.70804713105
5.38860450951 9.90397359176
5.54709287744 10.1063092728
5.70558124537 10.3156836147
5.86406961329 10.5328589246
6.02255798122 10.758768339
6.18104634915 10.9945686014
6.33953471707 11.2417152364
6.498023085 11.502072682
6.65651145293 11.7780810497
6.81499982086 12.0730187764
6.97348818878 12.3914365761
7.13197655671 12.7399183292
7.29046492464 13.1285206835
7.44895329256 13.5737871039
7.60744166049 14.1060263153
7.76593002842 14.7912173777


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt7.tex <==
0.0 6.20702261462
0.132433347565 6.27441670023
0.26486669513 6.34416653012
0.397300042696 6.41627487851
0.529733390261 6.49074641043
0.662166737826 6.56758774411
0.794600085391 6.64680753949
0.927033432956 6.72841661375
1.05946678052 6.81242808543
1.19190012809 6.89885754889
1.32433347565 6.98772328155
1.45676682322 7.07904648675
1.58920017078 7.17285157575
1.72163351835 7.26916649329
1.85406686591 7.36802309189
1.98650021348 7.46945756134
2.11893356104 7.57351092122
2.25136690861 7.68022958575
2.38380025617 7.78966601274
2.51623360374 7.90187945062
2.6486669513 8.01693680094
2.78110029887 8.13491361774
2.91353364643 8.25589527027
3.045966994 8.37997830215
3.17840034157 8.50727202824
3.31083368913 8.63790042156
3.4432670367 8.77200435681
3.57570038426 8.90974429553
3.70813373183 9.05130352339
3.84056707939 9.19689208359
3.97300042696 9.34675159675
4.10543377452 9.50116122153
4.23786712209 9.6604451001
4.37030046965 9.82498176054
4.50273381722 9.99521613404
4.63516716478 10.1716751194
4.76760051235 10.3549880411
4.90003385991 10.5459139873
5.03246720748 10.7453790262
5.16490055504 10.9545279528
5.29733390261 11.1747980055
5.42976725017 11.408026873
5.56220059774 11.6566162605
5.6946339453 11.9237895492
5.82706729287 12.2140175782
5.95950064043 12.5337653717
6.091933988 12.8929053239
6.22436733556 13.3076769061
6.35680068313 13.8078368023
6.4892340307 14.4581893519


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt8.tex <==
0.0 7.17649031198
0.104749805795 7.22982091121
0.20949961159 7.28506410738
0.314249417386 7.34222352366
0.418999223181 7.40130523353
0.523749028976 7.46231781353
0.628498834771 7.52527241828
0.733248640566 7.59018287889
0.837998446361 7.6570658262
0.942748252157 7.72594084094
1.04749805795 7.79683063308
1.15224786375 7.86976125357
1.25699766954 7.94476234184
1.36174747534 8.02186741382
1.46649728113 8.10111419545
1.57124708693 8.18254500831
1.67599689272 8.26620721522
1.78074669852 8.3521537349
1.88549650431 8.44044363742
1.99024631011 8.53114283418
2.0949961159 8.62432487933
2.1997459217 8.72007190376
2.30449572749 8.81847570725
2.40924553329 8.91963904095
2.51399533908 9.02367712055
2.61874514488 9.13071942058
2.72349495067 9.24091181447
2.82824475647 9.35441914283
2.93299456226 9.47142831679
3.03774436806 9.59215209587
3.14249417386 9.71683372475
3.24724397965 9.84575267483
3.35199378545 9.97923182392
3.45674359124 10.117646531
3.56149339704 10.2614362433
3.66624320283 10.411119538
3.77099300863 10.5673139043
3.87574281442 10.7307621881
3.98049262022 10.9023686074
4.08524242601 11.0832488462
4.18999223181 11.2748014405
4.2947420376 11.4788124068
4.3994918434 11.6976137473
4.50424164919 11.9343332306
4.60899145499 12.1933073222
4.71374126078 12.480805707
4.81849106658 12.8064031607
4.92324087237 13.1858544743
5.02799067817 13.6480448071
5.13274048396 14.2559377466


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-midPoint.tex <==
0.0 0.459043605026
0.00853 0.463330619152
0.01706 0.467661655327
0.02559 0.472036694963
0.03412 0.476455707107
0.04265 0.480918648484
0.05118 0.485425463566
0.05971 0.489976084645
0.06824 0.494570431933
0.07677 0.499208413674
0.0853 0.503889926274
0.09383 0.508614854449
0.10236 0.513383071382
0.11089 0.518194438903
0.11942 0.523048807679
0.12795 0.527946017418
0.13648 0.532885897088
0.14501 0.537868265146
0.15354 0.542892929783
0.16207 0.547959689173
0.1706 0.553068331743
0.17913 0.55821863644
0.18766 0.563410373019
0.19619 0.568643302329
0.20472 0.573917176614
0.21325 0.579231739813
0.22178 0.584586727875
0.23031 0.58998186907
0.23884 0.595416884306
0.24737 0.600891487458
0.2559 0.606405385684
0.26443 0.611958279756
0.27296 0.617549864385
0.28149 0.623179828554
0.29002 0.628847855835
0.29855 0.634553624726
0.30708 0.640296808968
0.31561 0.64607707787
0.32414 0.65189409663
0.33267 0.657747526646
0.3412 0.663637025834
0.34973 0.669562248931
0.35826 0.675522847802
0.36679 0.681518471732
0.37532 0.687548767724
0.38385 0.693613380779
0.39238 0.699711954181
0.40091 0.705844129765
0.40944 0.712009548187
0.41797 0.718207849178
0.4265 0.724438671802
0.43503 0.730701654695
0.44356 0.736996436301
0.45209 0.743322655105
0.46062 0.74967994985
0.46915 0.756067959751
0.47768 0.762486324701
0.48621 0.768934685467
0.49474 0.775412683879
0.50327 0.781919963009
0.5118 0.78845616735
0.52033 0.795020942976
0.52886 0.801613937701
0.53739 0.808234801231
0.54592 0.814883185304
0.55445 0.821558743824
0.56298 0.828261132995
0.57151 0.834990011431
0.58004 0.841745040281
0.58857 0.848525883327
0.5971 0.855332207087
0.60563 0.862163680908
0.61416 0.869019977053
0.62269 0.875900770784
0.63122 0.882805740431
0.63975 0.889734567467
0.64828 0.896686936569
0.65681 0.903662535672
0.66534 0.91066105603
0.67387 0.917682192256
0.6824 0.924725642366
0.69093 0.931791107821
0.69946 0.938878293556
0.70799 0.94598690801
0.71652 0.953116663153
0.72505 0.960267274504
0.73358 0.967438461151
0.74211 0.97462994576
0.75064 0.981841454591
0.75917 0.989072717501
0.7677 0.996323467948
0.77623 1.00359344299
0.78476 1.0108823833
0.79329 1.01819003311
0.80182 1.02551614029
0.81035 1.03286045624
0.81888 1.04022273596
0.82741 1.04760273799
0.83594 1.0550002244
0.84447 1.06241496079
0.853 1.06984671626
0.86153 1.07729526336
0.87006 1.08476037813
0.87859 1.09224184002
0.88712 1.0997394319
0.89565 1.10725293999
0.90418 1.1147821539
0.91271 1.12232686654
0.92124 1.1298868741
0.92977 1.13746197605
0.9383 1.14505197509
0.94683 1.1526566771
0.95536 1.16027589116
0.96389 1.16790942945
0.97242 1.17555710726
0.98095 1.18321874294
0.98948 1.19089415787
0.99801 1.19858317644
1.00654 1.20628562599
1.01507 1.21400133677
1.0236 1.22173014194
1.03213 1.2294718775
1.04066 1.23722638228
1.04919 1.24499349788
1.05772 1.25277306866
1.06625 1.26056494168
1.07478 1.26836896667
1.08331 1.27618499601
1.09184 1.28401288468
1.10037 1.29185249024
1.1089 1.29970367276
1.11743 1.30756629483
1.12596 1.3154402215
1.13449 1.32332532024
1.14302 1.33122146092
1.15155 1.33912851579
1.16008 1.34704635939
1.16861 1.3549748686
1.17714 1.36291392252
1.18567 1.37086340251
1.1942 1.37882319212
1.20273 1.38679317704
1.21126 1.39477324514
1.21979 1.40276328636
1.22832 1.41076319271
1.23685 1.41877285826
1.24538 1.42679217907
1.25391 1.43482105322
1.26244 1.44285938069
1.27097 1.45090706343
1.2795 1.45896400525
1.28803 1.46703011186
1.29656 1.47510529078
1.30509 1.48318945137
1.31362 1.49128250476
1.32215 1.49938436384
1.33068 1.50749494325
1.33921 1.51561415931
1.34774 1.52374193005
1.35627 1.53187817515
1.3648 1.54002281593
1.37333 1.54817577532
1.38186 1.55633697782
1.39039 1.56450634953
1.39892 1.57268381806
1.40745 1.58086931255
1.41598 1.58906276367
1.42451 1.59726410352
1.43304 1.60547326568
1.44157 1.61369018517
1.4501 1.62191479842
1.45863 1.63014704326
1.46716 1.6383868589
1.47569 1.6466341859
1.48422 1.65488896616
1.49275 1.66315114292
1.50128 1.6714206607
1.50981 1.67969746533
1.51834 1.68798150389
1.52687 1.69627272472
1.5354 1.70457107741
1.54393 1.71287651275
1.55246 1.72118898274
1.56099 1.72950844059
1.56952 1.73783484067
1.57805 1.7461681385
1.58658 1.75450829077
1.59511 1.76285525529
1.60364 1.77120899099
1.61217 1.7795694579
1.6207 1.78793661716
1.62923 1.79631043097
1.63776 1.80469086262
1.64629 1.81307787644
1.65482 1.82147143782
1.66335 1.82987151316
1.67188 1.8382780699
1.68041 1.8466910765
1.68894 1.8551105024
1.69747 1.86353631804
1.706 1.87196849484
1.71453 1.8804070052
1.72306 1.88885182248
1.73159 1.89730292098
1.74012 1.90576027596
1.74865 1.91422386361
1.75718 1.92269366105
1.76571 1.93116964632
1.77424 1.93965179837
1.78277 1.94814009707
1.7913 1.95663452316
1.79983 1.96513505829
1.80836 1.97364168499
1.81689 1.98215438668
1.82542 1.99067314764
1.83395 1.99919795301
1.84248 2.0077287888
1.85101 2.01626564189
1.85954 2.02480849998
1.86807 2.03335735163
1.8766 2.04191218625
1.88513 2.05047299408
1.89366 2.05903976618
1.90219 2.06761249446
1.91072 2.07619117163
1.91925 2.08477579125
1.92778 2.09336634767
1.93631 2.10196283608
1.94484 2.11056525246
1.95337 2.11917359361
1.9619 2.12778785715
1.97043 2.13640804149
1.97896 2.14503414585
1.98749 2.15366617024
1.99602 2.16230411548
2.00455 2.17094798321
2.01308 2.17959777583
2.02161 2.18825349656
2.03014 2.19691514942
2.03867 2.20558273923
2.0472 2.21425627159
2.05573 2.22293575291
2.06426 2.2316211904
2.07279 2.24031259206
2.08132 2.2490099667
2.08985 2.25771332392
2.09838 2.26642267414
2.10691 2.27513802857
2.11544 2.28385939922
2.12397 2.29258679892
2.1325 2.30132024132
2.14103 2.31005974086
2.14956 2.3188053128
2.15809 2.32755697324
2.16662 2.33631473909
2.17515 2.34507862806
2.18368 2.35384865874
2.19221 2.36262485052
2.20074 2.37140722363
2.20927 2.38019579915
2.2178 2.38899059901
2.22633 2.39779164598
2.23486 2.40659896371
2.24339 2.41541257669
2.25192 2.42423251029
2.26045 2.43305879077
2.26898 2.44189144523
2.27751 2.45073050172
2.28604 2.45957598913
2.29457 2.46842793729
2.3031 2.47728637692
2.31163 2.48615133967
2.32016 2.49502285812
2.32869 2.50390096578
2.33722 2.5127856971
2.34575 2.5216770875
2.35428 2.53057517334
2.36281 2.53947999197
2.37134 2.54839158173
2.37987 2.55730998194
2.3884 2.56623523293
2.39693 2.57516737605
2.40546 2.58410645368
2.41399 2.59305250922
2.42252 2.60200558716
2.43105 2.61096573301
2.43958 2.6199329934
2.44811 2.62890741604
2.45664 2.63788904973
2.46517 2.6468779444
2.4737 2.65587415113
2.48223 2.66487772214
2.49076 2.67388871081
2.49929 2.68290717171
2.50782 2.69193316062
2.51635 2.70096673452
2.52488 2.71000795164
2.53341 2.71905687146
2.54194 2.72811355472
2.55047 2.73717806346
2.559 2.74625046105
2.56753 2.75533081216
2.57606 2.76441918284
2.58459 2.7735156405
2.59312 2.78262025395
2.60165 2.79173309342
2.61018 2.8008542306
2.61871 2.80998373862
2.62724 2.81912169213
2.63577 2.82826816727
2.6443 2.83742324176
2.65283 2.84658699487
2.66136 2.85575950748
2.66989 2.86494086209
2.67842 2.87413114286
2.68695 2.88333043566
2.69548 2.89253882805
2.70401 2.90175640936
2.71254 2.91098327072
2.72107 2.92021950504
2.7296 2.92946520713
2.73813 2.93872047366
2.74666 2.94798540324
2.75519 2.95726009646
2.76372 2.96654465588
2.77225 2.97583918614
2.78078 2.98514379395
2.78931 2.99445858817
2.79784 3.00378367981
2.80637 3.01311918211
2.8149 3.02246521059
2.82343 3.03182188307
2.83196 3.04118931975
2.84049 3.05056764321
2.84902 3.05995697855
2.85755 3.06935745336
2.86608 3.0787691978
2.87461 3.08819234471
2.88314 3.09762702957
2.89167 3.10707339066
2.9002 3.11653156906
2.90873 3.12600170874
2.91726 3.13548395662
2.92579 3.14497846264
2.93432 3.15448537983
2.94285 3.16400486439
2.95138 3.17353707577
2.95991 3.18308217672
2.96844 3.1926403334
2.97697 3.20221171546
2.9855 3.21179649612
2.99403 3.22139485225
3.00256 3.23100696447
3.01109 3.24063301727
3.01962 3.25027319906
3.02815 3.2599277023
3.03668 3.26959672361
3.04521 3.27928046385
3.05374 3.28897912829
3.06227 3.29869292665
3.0708 3.30842207327
3.07933 3.31816678722
3.08786 3.32792729243
3.09639 3.33770381783
3.10492 3.34749659748
3.11345 3.3573058707
3.12198 3.36713188225
3.13051 3.37697488245
3.13904 3.38683512736
3.14757 3.39671287894
3.1561 3.4066084052
3.16463 3.41652198043
3.17316 3.42645388532
3.18169 3.4364044072
3.19022 3.44637384019
3.19875 3.45636248547
3.20728 3.46637065143
3.21581 3.47639865393
3.22434 3.48644681651
3.23287 3.49651547065
3.2414 3.506604956
3.24993 3.51671562065
3.25846 3.52684782139
3.26699 3.53700192401
3.27552 3.54717830358
3.28405 3.55737734473
3.29258 3.56759944201
3.30111 3.57784500021
3.30964 3.58811443468
3.31817 3.5984081717
3.3267 3.60872664889
3.33523 3.61907031553
3.34376 3.62943963305
3.35229 3.63983507539
3.36082 3.65025712949
3.36935 3.66070629572
3.37788 3.67118308841
3.38641 3.68168803632
3.39494 3.69222168319
3.40347 3.7027845883
3.412 3.71337732707
3.42053 3.72400049164
3.42906 3.73465469153
3.43759 3.74534055433
3.44612 3.75605872636
3.45465 3.76680987348
3.46318 3.77759468183
3.47171 3.78841385864
3.48024 3.79926813311
3.48877 3.81015825733
3.4973 3.82108500721
3.50583 3.83204918348
3.51436 3.8430516128
3.52289 3.85409314881
3.53142 3.86517467335
3.53995 3.87629709768
3.54848 3.88746136383
3.55701 3.89866844594
3.56554 3.90991935175
3.57407 3.92121512416
3.5826 3.93255684286
3.59113 3.94394562609
3.59966 3.95538263244
3.60819 3.96686906286
3.61672 3.97840616273
3.62525 3.98999522405
3.63378 4.00163758778
3.64231 4.01333464638
3.65084 4.02508784645
3.65937 4.03689869155
3.6679 4.04876874526
3.67643 4.06069963438
3.68496 4.07269305242
3.69349 4.08475076325
3.70202 4.0968746051
3.71055 4.10906649474
3.71908 4.12132843209
3.72761 4.13366250505
3.73614 4.14607089478
3.74467 4.15855588131
3.7532 4.17111984964
3.76173 4.18376529631
3.77026 4.19649483644
3.77879 4.20931121144
3.78732 4.22221729723
3.79585 4.23521611328
3.80438 4.24831083229
3.81291 4.26150479085
3.82144 4.27480150089
3.82997 4.28820466232
3.8385 4.30171817666
3.84703 4.3153461621
3.85556 4.32909296987
3.86409 4.34296320228
3.87262 4.35696173252
3.88115 4.37109372641
3.88968 4.38536466649
3.89821 4.3997803786
3.90674 4.41434706125
3.91527 4.4290713184
3.9238 4.44396019574
3.93233 4.45902122125
3.94086 4.4742624506
3.94939 4.48969251787
3.95792 4.50532069277
3.96645 4.52115694494
3.97498 4.53721201681
3.98351 4.5534975061
3.99204 4.57002595982
4.00057 4.5868109815
4.0091 4.60386735416
4.01763 4.62121118177
4.02616 4.63886005268
4.03469 4.6568332293
4.04322 4.6751518692
4.05175 4.69383928422
4.06028 4.71292124555
4.06881 4.73242634526
4.07734 4.75238642702
4.08587 4.77283710287
4.0944 4.79381837736
4.10293 4.81537540732
4.11146 4.83755943424
4.11999 4.86042893876
4.12852 4.88405108427
4.13705 4.90850354133
4.14558 4.93387682079
4.15411 4.96027729656
4.16264 4.9878311791
4.17117 5.01668982419
4.1797 5.0470369568
4.18823 5.07909870749
4.19676 5.1131578933
4.20529 5.1495749075
4.21382 5.18881928405
4.22235 5.23151926853
4.23088 5.27854339456
4.23941 5.33114273535
4.24794 5.39121795535
4.25647 5.46187206455


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma2prob0pt1.tex <==
0.0 0.918087210053
0.0841218682305 0.922359624569
0.168243736461 0.935062231858
0.252365604692 0.955866314995
0.336487472922 0.98427021658
0.420609341153 1.01965530726
0.504731209383 1.06134396498
0.588853077614 1.10864962614
0.672974945844 1.16091387485
0.757096814075 1.21752995045
0.841218682305 1.2779547583
0.925340550536 1.34171247602
1.00946241877 1.40839274214
1.093584287 1.47764580409
1.17770615523 1.54917629596
1.26182802346 1.62273670863
1.34594989169 1.69812116516
1.43007175992 1.77515981275
1.51419362815 1.8537139556
1.59831549638 1.93367194593
1.68243736461 2.01494579545
1.76655923284 2.097468446
1.85068110107 2.18119163361
1.9348029693 2.26608428539
2.01892483753 2.35213140015
2.10304670576 2.43933337714
2.18716857399 2.52770577355
2.27129044222 2.61727948848
2.35541231046 2.70810139059
2.43953417869 2.80023542958
2.52365604692 2.89376429926
2.60777791515 2.98879175571
2.69189978338 3.08544574133
2.77602165161 3.18388253145
2.86014351984 3.28429221304
2.94426538807 3.3869059419
3.0283872563 3.49200562872
3.11250912453 3.59993701969
3.19663099276 3.71112763521
3.28075286099 3.82611184307
3.36487472922 3.94556671273
3.44899659745 4.07036470071
3.53311846568 4.20165362107
3.61724033391 4.34098286467
3.70136220214 4.49051233537
3.78548407037 4.65337946509
3.8696059386 4.83439486127
3.95372780684 5.04150145781
4.03784967507 5.28930498316
4.1219715433 5.60972177315


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma2prob0pt3.tex <==
0.0 1.6892008618
0.0608288216233 1.69076491499
0.121657643247 1.69545027418
0.18248646487 1.70323674112
0.243315286493 1.71409131631
0.304144108116 1.72796915503
0.36497292974 1.74481482942
0.425801751363 1.76456382996
0.486630572986 1.78714423258
0.54745939461 1.81247845701
0.608288216233 1.84048504712
0.669117037856 1.87108041337
0.72994585948 1.90418048984
0.790774681103 1.93970227194
0.851603502726 1.97756521403
0.912432324349 2.01769247914
0.973261145973 2.06001204308
1.0340899676 2.10445766418
1.09491878922 2.15096973675
1.15574761084 2.19949605092
1.21657643247 2.24999248551
1.27740525409 2.3024236631
1.33823407571 2.35676359854
1.39906289734 2.41299637484
1.45989171896 2.47111688245
1.52072054058 2.53113166258
1.58154936221 2.59305990008
1.64237818383 2.65693461958
1.70320700545 2.72280414991
1.76403582708 2.79073393743
1.8248646487 2.86080881191
1.88569347032 2.93313583989
1.94652229195 3.00784794622
2.00735111357 3.08510854951
2.06817993519 3.16511755239
2.12900875682 3.24811916864
2.18983757844 3.33441228245
2.25066640006 3.42436436443
2.31149522169 3.51843049199
2.37232404331 3.61717987349
2.43315286493 3.72133371441
2.49398168656 3.83182078251
2.55481050818 3.94986164489
2.6156393298 4.07710145752
2.67646815143 4.21582949725
2.73729697305 4.36936426376
2.79812579467 4.542782331
2.85895461629 4.7444446628
2.91978343792 4.98968287271
2.98061225954 5.311893362


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma2prob0pt6.tex <==
0.0 2.70745745211
0.0396220919817 2.70818227013
0.0792441839634 2.71035684158
0.118866275945 2.71398152786
0.158488367927 2.71905696169
0.198110459909 2.72558409292
0.23773255189 2.73356425275
0.277354643872 2.7429992368
0.316976735854 2.75389140715
0.356598827835 2.76624381407
0.396220919817 2.780060338
0.435843011799 2.79534585275
0.475465103781 2.81210641115
0.515087195762 2.83034945482
0.554709287744 2.85008405009
0.594331379726 2.87132115292
0.633953471707 2.89407390598
0.673575563689 2.91835797257
0.713197655671 2.9441919124
0.752819747653 2.97159760639
0.792441839634 3.00060073865
0.832063931616 3.03123134644
0.871686023598 3.06352445126
0.911308115579 3.09752078768
0.950930207561 3.13326765099
0.990552299543 3.17081989008
1.03017439152 3.21024107946
1.06979648351 3.2516049139
1.10941857549 3.29499688195
1.14904066747 3.34051629185
1.18866275945 3.38827874714
1.22828485143 3.43841920158
1.26790694341 3.49109576917
1.3075290354 3.54649453013
1.34715112738 3.6048356685
1.38677321936 3.66638141702
1.42639531134 3.73144649599
1.46601740332 3.80041205896
1.50563949531 3.87374467422
1.54526158729 3.95202271339
1.58488367927 4.03597393892
1.62450577125 4.12653056974
1.66412786323 4.22491266162
1.70374995521 4.33275943298
1.7433720472 4.45234624085
1.78299413918 4.58696502543
1.82261623116 4.74164411059
1.86223832314 4.92465522882
1.90186041512 5.15115274251
1.9414825071 5.45412618175


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma2pt01.tex <==
0.0 0.918087210053
0.0841218682305 0.922359624569
0.168243736461 0.935062231858
0.252365604692 0.955866314995
0.336487472922 0.98427021658
0.420609341153 1.01965530726
0.504731209383 1.06134396498
0.588853077614 1.10864962614
0.672974945844 1.16091387485
0.757096814075 1.21752995045
0.841218682305 1.2779547583
0.925340550536 1.34171247602
1.00946241877 1.40839274214
1.093584287 1.47764580409
1.17770615523 1.54917629596
1.26182802346 1.62273670863
1.34594989169 1.69812116516
1.43007175992 1.77515981275
1.51419362815 1.8537139556
1.59831549638 1.93367194593
1.68243736461 2.01494579545
1.76655923284 2.097468446
1.85068110107 2.18119163361
1.9348029693 2.26608428539
2.01892483753 2.35213140015
2.10304670576 2.43933337714
2.18716857399 2.52770577355
2.27129044222 2.61727948848
2.35541231046 2.70810139059
2.43953417869 2.80023542958
2.52365604692 2.89376429926
2.60777791515 2.98879175571
2.69189978338 3.08544574133
2.77602165161 3.18388253145
2.86014351984 3.28429221304
2.94426538807 3.3869059419
3.0283872563 3.49200562872
3.11250912453 3.59993701969
3.19663099276 3.71112763521
3.28075286099 3.82611184307
3.36487472922 3.94556671273
3.44899659745 4.07036470071
3.53311846568 4.20165362107
3.61724033391 4.34098286467
3.70136220214 4.49051233537
3.78548407037 4.65337946509
3.8696059386 4.83439486127
3.95372780684 5.04150145781
4.03784967507 5.28930498316
4.1219715433 5.60972177315


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma4prob0pt3.tex <==
0.0 3.3784017236
0.121657643247 3.38152982998
0.243315286493 3.39090054836
0.36497292974 3.40647348224
0.486630572986 3.42818263263
0.608288216233 3.45593831007
0.72994585948 3.48962965884
0.851603502726 3.52912765992
0.973261145973 3.57428846516
1.09491878922 3.62495691402
1.21657643247 3.68097009424
1.33823407571 3.74216082673
1.45989171896 3.80836097969
1.58154936221 3.87940454387
1.70320700545 3.95513042805
1.8248646487 4.03538495828
1.94652229195 4.12002408615
2.06817993519 4.20891532836
2.18983757844 4.3019394735
2.31149522169 4.39899210184
2.43315286493 4.49998497103
2.55481050818 4.60484732619
2.67646815143 4.71352719709
2.79812579467 4.82599274968
2.91978343792 4.94223376489
3.04144108116 5.06226332516
3.16309872441 5.18611980015
3.28475636766 5.31386923917
3.4064140109 5.44560829981
3.52807165415 5.58146787485
3.6497292974 5.72161762381
3.77138694064 5.86627167978
3.89304458389 6.01569589245
4.01470222714 6.17021709903
4.13635987038 6.33023510478
4.25801751363 6.49623833729
4.37967515688 6.66882456489
4.50133280012 6.84872872887
4.62299044337 7.03686098397
4.74464808662 7.23435974698
4.86630572986 7.44266742881
4.98796337311 7.66364156502
5.10962101636 7.89972328978
5.2312786596 8.15420291504
5.35293630285 8.43165899449
5.4745939461 8.73872852753
5.59625158934 9.085564662
5.71790923259 9.48888932559
5.83956687584 9.97936574542
5.96122451908 10.623786724


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt3.tex <==
0.0 6.7568034472
0.243315286493 6.76305965995
0.486630572986 6.78180109672
0.72994585948 6.81294696448
0.973261145973 6.85636526526
1.21657643247 6.91187662014
1.45989171896 6.97925931769
1.70320700545 7.05825531985
1.94652229195 7.14857693032
2.18983757844 7.24991382805
2.43315286493 7.36194018848
2.67646815143 7.48432165346
2.91978343792 7.61672195937
3.16309872441 7.75880908775
3.4064140109 7.91026085611
3.6497292974 8.07076991657
3.89304458389 8.2400481723
4.13635987038 8.41783065672
4.37967515688 8.60387894701
4.62299044337 8.79798420368
4.86630572986 8.99996994206
5.10962101636 9.20969465238
5.35293630285 9.42705439418
5.59625158934 9.65198549936
5.83956687584 9.88446752979
6.08288216233 10.1245266503
6.32619744882 10.3722396003
6.56951273532 10.6277384783
6.81282802181 10.8912165996
7.0561433083 11.1629357497
7.2994585948 11.4432352476
7.54277388129 11.7325433596
7.78608916778 12.0313917849
8.02940445428 12.3404341981
8.27271974077 12.6604702096
8.51603502726 12.9924766746
8.75935031375 13.3376491298
9.00266560025 13.6974574577
9.24598088674 14.0737219679
9.48929617323 14.468719494
9.73261145973 14.8853348576
9.97592674622 15.32728313
10.2192420327 15.7994465796
10.4625573192 16.3084058301
10.7058726057 16.863317989
10.9491878922 17.4774570551
11.1925031787 18.171129324
11.4358184652 18.9777786512
11.6791337517 19.9587314908
11.9224490382 21.247573448


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt6.tex <==
0.0 10.8298298084
0.158488367927 10.8327290805
0.316976735854 10.8414273663
0.475465103781 10.8559261115
0.633953471707 10.8762278468
0.792441839634 10.9023363717
0.950930207561 10.934257011
1.10941857549 10.9719969472
1.26790694341 11.0155656286
1.42639531134 11.0649752563
1.58488367927 11.120241352
1.7433720472 11.181383411
1.90186041512 11.2484256446
2.06034878305 11.3213978193
2.21883715098 11.4003362004
2.3773255189 11.4852846117
2.53581388683 11.5762956239
2.69430225476 11.6734318903
2.85279062268 11.7767676496
3.01127899061 11.8863904256
3.16976735854 12.0024029546
3.32825572646 12.1249253858
3.48674409439 12.254097805
3.64523246232 12.3900831507
3.80372083024 12.5330706039
3.96220919817 12.6832795603
4.1206975661 12.8409643178
4.27918593403 13.0064196556
4.43767430195 13.1799875278
4.59616266988 13.3620651674
4.75465103781 13.5531149886
4.91313940573 13.7536768063
5.07162777366 13.9643830767
5.23011614159 14.1859781205
5.38860450951 14.419342674
5.54709287744 14.6655256681
5.70558124537 14.9257859839
5.86406961329 15.2016482359
6.02255798122 15.4949786969
6.18104634915 15.8080908536
6.33953471707 16.1438957557
6.498023085 16.506122279
6.65651145293 16.8996506465
6.81499982086 17.3310377319
6.97348818878 17.8093849634
7.13197655671 18.3478601017
7.29046492464 18.9665764423
7.44895329256 19.6986209153
7.60744166049 20.60461097
7.76593002842 21.816504727


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt7.tex <==
0.0 12.4140452292
0.132433347565 12.4164000529
0.26486669513 12.4234663651
0.397300042696 12.4352497143
0.529733390261 12.4517594306
0.662166737826 12.4730087504
0.794600085391 12.4990149936
0.927033432956 12.5297997945
1.05946678052 12.5653893903
1.19190012809 12.6058149697
1.32433347565 12.6511130874
1.45676682322 12.7013261503
1.58920017078 12.7565029807
1.72163351835 12.8166994682
1.85406686591 12.8819793179
1.98650021348 12.9524149092
2.11893356104 13.0280882814
2.25136690861 13.1090922629
2.38380025617 13.1955317693
2.51623360374 13.2875252975
2.6486669513 13.3852066506
2.78110029887 13.4887269366
2.91353364643 13.5982568941
3.045966994 13.7139896103
3.17840034157 13.8361437149
3.31083368913 13.964967154
3.4432670367 14.1007416769
3.57570038426 14.2437882068
3.70813373183 14.394473315
3.84056707939 14.5532170878
3.97300042696 14.7205027665
4.10543377452 14.8968886685
4.23786712209 15.0830230781
4.37030046965 15.2796630514
4.50273381722 15.4876984509
4.63516716478 15.708183074
4.76760051235 15.9423755699
4.90003385991 16.1917941147
5.03246720748 16.4582908448
5.16490055504 16.7441553506
5.29733390261 17.0522621084
5.42976725017 17.3862864957
5.56220059774 17.7510319232
5.6946339453 18.1529451532
5.82706729287 18.6009678635
5.95950064043 19.1080301031
6.091933988 19.6938766597
6.22436733556 20.3909864766
6.35680068313 21.2588729216
6.4892340307 22.4271446731


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt8.tex <==
0.0 14.352980624
0.104749805795 14.3548920166
0.20949961159 14.3606286032
0.314249417386 14.3701976299
0.418999223181 14.3836112439
0.523749028976 14.4008865981
0.628498834771 14.4220460018
0.733248640566 14.4471171172
0.837998446361 14.476133206
0.942748252157 14.5091334297
1.04749805795 14.5461632082
1.15224786375 14.5872746434
1.25699766954 14.6325270141
1.36174747534 14.6819873523
1.46649728113 14.7357311098
1.57124708693 14.7938429297
1.67599689272 14.8564175377
1.78074669852 14.9235607713
1.88549650431 14.9953907705
1.99024631011 15.0720393582
2.0949961159 15.1536536428
2.1997459217 15.2403978858
2.30449572749 15.332455687
2.40924553329 15.4300325486
2.51399533908 15.533358902
2.61874514488 15.6426936963
2.72349495067 15.7583286783
2.82824475647 15.8805935292
2.93299456226 16.0098620713
3.03774436806 16.1465598237
3.14249417386 16.2911732756
3.24724397965 16.44426137
3.35199378545 16.6064698624
3.45674359124 16.7785494708
3.56149339704 16.9613790895
3.66624320283 17.1559958731
3.77099300863 17.3636347999
3.87574281442 17.5857815618
3.98049262022 17.8242445946
4.08524242601 18.0812552664
4.18999223181 18.3596106492
4.2947420376 18.662882776
4.3994918434 18.9957356513
4.50424164919 19.3644248119
4.60899145499 19.7776231894
4.71374126078 20.2478701531
4.81849106658 20.7943152547
4.92324087237 21.4484680762
5.02799067817 22.2680989361
5.13274048396 23.3791350092


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-upperEnd-sigma1prob0pt1.tex <==
0.0 0.459043605026
0.004276 0.45906573285
0.008552 0.459132110057
0.012828 0.459242717864
0.017104 0.459397524999
0.02138 0.45959648774
0.025656 0.459839549984
0.029932 0.460126643326
0.034208 0.460457687155
0.038484 0.460832588772
0.04276 0.461251243519
0.047036 0.46171353493
0.051312 0.462219334894
0.055588 0.462768503831
0.059864 0.463360890892
0.06414 0.463996334161
0.068416 0.464674660878
0.072692 0.465395687674
0.076968 0.466159220816
0.081244 0.466965056466
0.08552 0.467812980946
0.089796 0.468702771017
0.094072 0.469634194164
0.098348 0.470607008894
0.102624 0.471620965034
0.1069 0.472675804041
0.111176 0.473771259317
0.115452 0.474907056525
0.119728 0.476082913917
0.124004 0.477298542654
0.12828 0.47855364714
0.132556 0.47984792535
0.136832 0.481181069161
0.141108 0.482552764686
0.145384 0.483962692604
0.14966 0.485410528491
0.153936 0.486895943147
0.158212 0.488418602923
0.162488 0.489978170045
0.166764 0.491574302933
0.17104 0.493206656518
0.175316 0.49487488255
0.179592 0.496578629906
0.183868 0.498317544893
0.188144 0.500091271538
0.19242 0.501899451884
0.196696 0.503741726263
0.200972 0.505617733581
0.205248 0.50752711158
0.209524 0.509469497101
0.2138 0.511444526341
0.218076 0.513451835094
0.222352 0.515491058994
0.226628 0.517561833742
0.230904 0.519663795331
0.23518 0.521796580261
0.239456 0.523959825742
0.243732 0.526153169897
0.248008 0.528376251948
0.252284 0.530628712401
0.25656 0.53291019322
0.260836 0.535220337994
0.265112 0.537558792092
0.269388 0.539925202818
0.273664 0.542319219551
0.27794 0.544740493883
0.282216 0.547188679744
0.286492 0.549663433527
0.290768 0.552164414198
0.295044 0.554691283404
0.29932 0.557243705573
0.303596 0.559821348009
0.307872 0.562423880975
0.312148 0.565050977779
0.316424 0.567702314842
0.3207 0.570377571775
0.324976 0.573076431434
0.329252 0.575798579982
0.333528 0.578543706942
0.337804 0.581311505238
0.34208 0.584101671247
0.346356 0.586913904826
0.350632 0.589747909354
0.354908 0.592603391754
0.359184 0.595480062521
0.36346 0.59837763574
0.367736 0.601295829103
0.372012 0.604234363927
0.376288 0.607192965153
0.380564 0.610171361363
0.38484 0.613169284775
0.389116 0.616186471248
0.393392 0.619222660278
0.397668 0.622277594989
0.401944 0.625351022131
0.40622 0.628442692064
0.410496 0.631552358751
0.414772 0.634679779736
0.419048 0.637824716136
0.423324 0.640986932614
0.4276 0.644166197365
0.431876 0.647362282091
0.436152 0.650574961977
0.440428 0.653804015671
0.444704 0.65704922525
0.44898 0.6603103762
0.453256 0.663587257382
0.457532 0.666879661009
0.461808 0.670187382607
0.466084 0.673510220993
0.47036 0.676847978236
0.474636 0.680200459627
0.478912 0.683567473648
0.483188 0.686948831933
0.487464 0.690344349239
0.49174 0.693753843408
0.496016 0.697177135332
0.500292 0.70061404892
0.504568 0.704064411061
0.508844 0.707528051586
0.51312 0.711004803236
0.517396 0.714494501623
0.521672 0.717996985196
0.525948 0.721512095203
0.530224 0.725039675655
0.5345 0.72857957329
0.538776 0.732131637538
0.543052 0.735695720485
0.547328 0.739271676835
0.551604 0.742859363877
0.55588 0.746458641447
0.560156 0.750069371895
0.564432 0.75369142005
0.568708 0.757324653183
0.572984 0.760968940973
0.57726 0.764624155476
0.581536 0.768290171087
0.585812 0.771966864507
0.590088 0.775654114715
0.594364 0.779351802927
0.59864 0.783059812568
0.602916 0.786778029241
0.607192 0.790506340692
0.611468 0.794244636781
0.615744 0.797992809449
0.62002 0.801750752688
0.624296 0.805518362513
0.628572 0.80929553693
0.632848 0.813082175904
0.637124 0.816878181338
0.6414 0.820683457034
0.645676 0.824497908676
0.649952 0.82832144379
0.654228 0.83215397173
0.658504 0.83599540364
0.66278 0.839845652433
0.667056 0.843704632766
0.671332 0.847572261009
0.675608 0.851448455227
0.679884 0.855333135149
0.68416 0.859226222147
0.688436 0.863127639213
0.692712 0.867037310932
0.696988 0.870955163462
0.701264 0.874881124511
0.70554 0.878815123314
0.709816 0.88275709061
0.714092 0.886706958624
0.718368 0.890664661044
0.722644 0.894630133
0.72692 0.898603311046
0.731196 0.902584133136
0.735472 0.906572538609
0.739748 0.91056846817
0.744024 0.914571863868
0.7483 0.91858266908
0.752576 0.922600828493
0.756852 0.926626288087
0.761128 0.930658995118
0.765404 0.934698898097
0.76968 0.938745946783
0.773956 0.942800092157
0.778232 0.946861286414
0.782508 0.950929482941
0.786784 0.95500463631
0.79106 0.959086702255
0.795336 0.963175637664
0.799612 0.967271400563
0.803888 0.971373950103
0.808164 0.975483246544
0.81244 0.979599251246
0.816716 0.983721926655
0.820992 0.98785123629
0.825268 0.99198714473
0.829544 0.996129617608
0.83382 1.00027862159
0.838096 1.00443412438
0.842372 1.00859609468
0.846648 1.01276450222
0.850924 1.01693931771
0.8552 1.02112051286
0.859476 1.02530806035
0.863752 1.02950193381
0.868028 1.03370210787
0.872304 1.03790855808
0.87658 1.04212126093
0.880856 1.04634019387
0.885132 1.05056533523
0.889408 1.05479666431
0.893684 1.05903416129
0.89796 1.06327780725
0.902236 1.06752758419
0.906512 1.07178347499
0.910788 1.0760454634
0.915064 1.08031353406
0.91934 1.08458767249
0.923616 1.08886786506
0.927892 1.09315409902
0.932168 1.09744636245
0.936444 1.10174464432
0.94072 1.10604893441
0.944996 1.11035922336
0.949272 1.11467550265
0.953548 1.11899776458
0.957824 1.12332600231
0.9621 1.1276602098
0.966376 1.13200038185
0.970652 1.13634651407
0.974928 1.1406986029
0.979204 1.1450566456
0.98348 1.14942064023
0.987756 1.15379058568
0.992032 1.15816648163
0.996308 1.16254832859
1.000584 1.16693612788
1.00486 1.1713298816
1.009136 1.17572959268
1.013412 1.18013526486
1.017688 1.18454690267
1.021964 1.18896451145
1.02624 1.19338809736
1.030516 1.19781766734
1.034792 1.20225322916
1.039068 1.20669479138
1.043344 1.21114236339
1.04762 1.21559595538
1.051896 1.22005557835
1.056172 1.2245212441
1.060448 1.22899296527
1.064724 1.23347075531
1.069 1.23795462849
1.073276 1.24244459989
1.077552 1.24694068544
1.081828 1.25144290188
1.086104 1.25595126679
1.09038 1.2604657986
1.094656 1.26498651655
1.098932 1.26951344076
1.103208 1.27404659218
1.107484 1.27858599262
1.11176 1.28313166474
1.116036 1.28768363208
1.120312 1.29224191904
1.124588 1.29680655091
1.128864 1.30137755384
1.13314 1.30595495489
1.137416 1.31053878202
1.141692 1.31512906406
1.145968 1.31972583079
1.150244 1.32432911289
1.15452 1.32893894196
1.158796 1.33355535055
1.163072 1.33817837213
1.167348 1.34280804116
1.171624 1.34744439301
1.1759 1.35208746408
1.180176 1.35673729169
1.184452 1.3613939142
1.188728 1.36605737094
1.193004 1.37072770228
1.19728 1.37540494958
1.201556 1.38008915526
1.205832 1.38478036279
1.210108 1.38947861668
1.214384 1.39418396253
1.21866 1.39889644702
1.222936 1.40361611794
1.227212 1.40834302417
1.231488 1.41307721574
1.235764 1.41781874382
1.24004 1.42256766074
1.244316 1.42732402
1.248592 1.43208787629
1.252868 1.43685928551
1.257144 1.44163830479
1.26142 1.4464249925
1.265696 1.45121940828
1.269972 1.45602161305
1.274248 1.460831669
1.278524 1.46564963969
1.2828 1.47047558998
1.287076 1.47530958612
1.291352 1.48015169574
1.295628 1.48500198785
1.299904 1.48986053293
1.30418 1.49472740288
1.308456 1.4996026711
1.312732 1.50448641248
1.317008 1.50937870346
1.321284 1.51427962201
1.32556 1.51918924769
1.329836 1.52410766168
1.334112 1.5290349468
1.338388 1.53397118754
1.342664 1.53891647008
1.34694 1.54387088234
1.351216 1.54883451401
1.355492 1.55380745656
1.359768 1.55878980333
1.364044 1.56378164948
1.36832 1.56878309211
1.372596 1.57379423024
1.376872 1.5788151649
1.381148 1.5838459991
1.385424 1.58888683793
1.3897 1.59393778859
1.393976 1.59899896042
1.398252 1.60407046495
1.402528 1.60915241594
1.406804 1.61424492943
1.41108 1.61934812381
1.415356 1.62446211984
1.419632 1.62958704071
1.423908 1.6347230121
1.428184 1.63987016223
1.43246 1.64502862193
1.436736 1.65019852467
1.441012 1.65538000663
1.445288 1.66057320678
1.449564 1.66577826693
1.45384 1.67099533179
1.458116 1.67622454904
1.462392 1.68146606943
1.466668 1.68672004678
1.470944 1.69198663815
1.47522 1.69726600381
1.479496 1.70255830744
1.483772 1.70786371608
1.488048 1.71318240034
1.492324 1.71851453439
1.4966 1.7238602961
1.500876 1.72921986713
1.505152 1.734593433
1.509428 1.73998118322
1.513704 1.74538331136
1.51798 1.7508000152
1.522256 1.75623149679
1.526532 1.7616779626
1.530808 1.76713962363
1.535084 1.77261669551
1.53936 1.77810939864
1.543636 1.78361795834
1.547912 1.78914260495
1.552188 1.79468357398
1.556464 1.80024110628
1.56074 1.80581544814
1.565016 1.81140685149
1.569292 1.81701557405
1.573568 1.82264187946
1.577844 1.82828603752
1.58212 1.8339483243
1.586396 1.83962902237
1.590672 1.84532842099
1.594948 1.85104681627
1.599224 1.85678451145
1.6035 1.86254181702
1.607776 1.86831905105
1.612052 1.87411653934
1.616328 1.87993461569
1.620604 1.88577362219
1.62488 1.89163390941
1.629156 1.89751583673
1.633432 1.90341977259
1.637708 1.90934609481
1.641984 1.9152951909
1.64626 1.92126745835
1.650536 1.927263305
1.654812 1.93328314935
1.659088 1.93932742097
1.663364 1.94539656085
1.66764 1.9514910218
1.671916 1.95761126887
1.676192 1.96375777977
1.680468 1.96993104536
1.684744 1.97613157005
1.68902 1.98235987237
1.693296 1.98861648545
1.697572 1.99490195756
1.701848 2.00121685268
1.706124 2.00756175109
1.7104 2.01393725003
1.714676 2.02034396427
1.718952 2.02678252688
1.723228 2.0332535899
1.727504 2.03975782512
1.73178 2.04629592482
1.736056 2.05286860268
1.740332 2.05947659459
1.744608 2.06612065962
1.748884 2.07280158094
1.75316 2.07952016688
1.757436 2.08627725199
1.761712 2.09307369818
1.765988 2.0999103959
1.770264 2.10678826545
1.77454 2.11370825825
1.778816 2.12067135828
1.783092 2.12767858361
1.787368 2.13473098792
1.791644 2.14182966218
1.79592 2.14897573646
1.800196 2.15617038179
1.804472 2.16341481212
1.808748 2.1707102865
1.813024 2.17805811126
1.8173 2.18545964248
1.821576 2.19291628846
1.825852 2.20042951247
1.830128 2.20800083568
1.834404 2.21563184016
1.83868 2.22332417224
1.842956 2.23107954603
1.847232 2.23889974714
1.851508 2.24678663678
1.855784 2.25474215604
1.86006 2.26276833056
1.864336 2.27086727549
1.868612 2.27904120085
1.872888 2.28729241735
1.877164 2.29562334254
1.88144 2.30403650755
1.885716 2.31253456434
1.889992 2.32112029352
1.894268 2.32979661285
1.898544 2.33856658641
1.90282 2.34743343462
1.907096 2.35640054506
1.911372 2.36547148433
1.915648 2.37465001092
1.919924 2.38394008927
1.9242 2.3933459052
1.928476 2.40287188277
1.932752 2.41252270278
1.937028 2.42230332319
1.941304 2.43221900147
1.94558 2.44227531945
1.949856 2.45247821063
1.954132 2.46283399061
1.958408 2.47334939075
1.962684 2.48403159574
1.96696 2.49488828551
1.971236 2.50592768209
1.975512 2.51715860223
1.979788 2.52859051656
1.984064 2.54023361628
1.98834 2.5520988888
1.992616 2.56419820337
1.996892 2.57654440884
2.001168 2.58915144524
2.005444 2.60203447193
2.00972 2.61521001517
2.013996 2.62869613877
2.018272 2.64251264257
2.022548 2.65668129391
2.026824 2.67122609951
2.0311 2.68617362599
2.035376 2.70155338038
2.039652 2.71739826433
2.043928 2.73374512008
2.048204 2.75063539144
2.05248 2.76811593016
2.056756 2.78623998808
2.061032 2.80506844908
2.065308 2.82467137416
2.069584 2.84512996074
2.07386 2.86653905751
2.078136 2.88901043604
2.082412 2.91267711118
2.086688 2.9376991431
2.090964 2.96427157874
2.09524 2.99263555898
2.099516 3.02309424542
2.103792 3.05603632821
2.108068 3.09197192658
2.112344 3.13158969596
2.11662 3.17585229553
2.120896 3.22616619096
2.125172 3.28470875188
2.129448 3.35512951105
2.133724 3.44430124906


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-upperEnd-sigma1pt5prob0pt05.tex <==
0.0 0.480437118408
0.004276 0.48045714819
0.008552 0.480517232554
0.012828 0.480617356553
0.017104 0.480757495301
0.02138 0.480937613996
0.025656 0.481157667973
0.029932 0.481417602749
0.034208 0.4817173541
0.038484 0.482056848134
0.04276 0.482436001384
0.047036 0.482854720912
0.051312 0.483312904419
0.055588 0.483810440372
0.059864 0.484347208138
0.06414 0.484923078126
0.068416 0.485537911943
0.072692 0.486191562559
0.076968 0.486883874475
0.081244 0.487614683906
0.08552 0.48838381897
0.089796 0.489191099879
0.094072 0.490036339148
0.098348 0.490919341798
0.102624 0.491839905571
0.1069 0.492797821154
0.111176 0.493792872401
0.115452 0.494824836559
0.119728 0.495893484506
0.124004 0.496998580984
0.12828 0.498139884836
0.132556 0.499317149251
0.136832 0.500530122003
0.141108 0.501778545694
0.145384 0.503062158004
0.14966 0.504380691928
0.153936 0.505733876026
0.158212 0.507121434667
0.162488 0.508543088267
0.166764 0.509998553537
0.17104 0.511487543717
0.175316 0.513009768817
0.179592 0.51456493585
0.183868 0.516152749067
0.188144 0.51777291018
0.19242 0.519425118596
0.196696 0.52110907163
0.200972 0.522824464729
0.205248 0.524570991682
0.209524 0.526348344831
0.2138 0.528156215276
0.218076 0.529994293071
0.222352 0.531862267423
0.226628 0.533759826881
0.230904 0.535686659516
0.23518 0.537642453109
0.239456 0.539626895315
0.243732 0.541639673838
0.248008 0.543680476592
0.252284 0.545748991858
0.25656 0.547844908438
0.260836 0.549967915795
0.265112 0.552117704204
0.269388 0.554293964878
0.273664 0.5564963901
0.27794 0.558724673352
0.282216 0.560978509428
0.286492 0.56325759455
0.290768 0.565561626475
0.295044 0.5678903046
0.29932 0.570243330056
0.303596 0.572620405807
0.307872 0.575021236729
0.312148 0.577445529702
0.316424 0.579892993681
0.3207 0.582363339774
0.324976 0.584856281306
0.329252 0.58737153389
0.333528 0.589908815483
0.337804 0.59246784644
0.34208 0.59504834957
0.346356 0.597650050185
0.350632 0.600272676136
0.354908 0.602915957864
0.359184 0.605579628427
0.36346 0.60826342354
0.367736 0.610967081603
0.372012 0.613690343726
0.376288 0.616432953756
0.380564 0.619194658292
0.38484 0.621975206709
0.389116 0.62477435117
0.393392 0.627591846638
0.397668 0.630427450887
0.401944 0.633280924507
0.40622 0.636152030912
0.410496 0.639040536344
0.414772 0.641946209867
0.419048 0.644868823374
0.423324 0.647808151578
0.4276 0.650763972011
0.431876 0.653736065014
0.436152 0.656724213731
0.440428 0.659728204099
0.444704 0.662747824836
0.44898 0.665782867427
0.453256 0.668833126115
0.457532 0.671898397881
0.461808 0.674978482428
0.466084 0.678073182167
0.47036 0.681182302197
0.474636 0.684305650284
0.478912 0.687443036845
0.483188 0.690594274922
0.487464 0.693759180165
0.49174 0.696937570806
0.496016 0.700129267639
0.500292 0.703334093995
0.504568 0.706551875718
0.508844 0.70978244114
0.51312 0.713025621059
0.517396 0.716281248709
0.521672 0.719549159738
0.525948 0.72282919218
0.530224 0.72612118643
0.5345 0.729424985216
0.538776 0.732740433574
0.543052 0.736067378821
0.547328 0.739405670526
0.551604 0.742755160485
0.55588 0.746115702693
0.560156 0.749487153317
0.564432 0.752869370668
0.568708 0.756262215175
0.572984 0.759665549357
0.57726 0.763079237795
0.581536 0.766503147107
0.585812 0.769937145919
0.590088 0.773381104838
0.594364 0.776834896428
0.59864 0.780298395178
0.602916 0.783771477481
0.607192 0.787254021605
0.611468 0.790745907664
0.615744 0.794247017599
0.62002 0.797757235143
0.624296 0.801276445804
0.628572 0.804804536835
0.632848 0.808341397207
0.637124 0.811886917588
0.6414 0.815440990316
0.645676 0.819003509377
0.649952 0.822574370374
0.654228 0.826153470511
0.658504 0.829740708565
0.66278 0.833335984863
0.667056 0.836939201257
0.671332 0.840550261104
0.675608 0.844169069242
0.679884 0.847795531968
0.68416 0.851429557013
0.688436 0.855071053524
0.692712 0.858719932039
0.696988 0.862376104468
0.701264 0.866039484071
0.70554 0.869709985435
0.709816 0.873387524459
0.714092 0.877072018327
0.718368 0.880763385493
0.722644 0.884461545657
0.72692 0.888166419751
0.731196 0.891877929913
0.735472 0.895595999476
0.739748 0.899320552941
0.744024 0.903051515966
0.7483 0.906788815341
0.752576 0.910532378978
0.756852 0.914282135885
0.761128 0.918038016156
0.765404 0.92179995095
0.76968 0.925567872473
0.773956 0.929341713965
0.778232 0.933121409684
0.782508 0.936906894885
0.786784 0.940698105809
0.79106 0.944494979665
0.795336 0.948297454617
0.799612 0.952105469766
0.803888 0.955918965138
0.808164 0.959737881667
0.81244 0.963562161182
0.816716 0.967391746394
0.820992 0.97122658088
0.825268 0.975066609069
0.829544 0.978911776233
0.83382 0.982762028466
0.838096 0.98661731268
0.842372 0.990477576585
0.846648 0.994342768681
0.850924 0.998212838243
0.8552 1.00208773531
0.859476 1.00596741067
0.863752 1.00985181586
0.868028 1.01374090314
0.872304 1.01763462548
0.87658 1.02153293657
0.880856 1.02543579078
0.885132 1.02934314318
0.889408 1.0332549495
0.893684 1.03717116614
0.89796 1.04109175015
0.902236 1.04501665923
0.906512 1.04894585171
0.910788 1.05287928654
0.915064 1.05681692329
0.91934 1.06075872211
0.923616 1.06470464378
0.927892 1.06865464966
0.932168 1.07260870166
0.936444 1.07656676228
0.94072 1.08052879458
0.944996 1.08449476216
0.949272 1.08846462918
0.953548 1.09243836032
0.957824 1.09641592079
0.9621 1.10039727633
0.966376 1.10438239316
0.970652 1.10837123805
0.974928 1.11236377822
0.979204 1.1163599814
0.98348 1.12035981582
0.987756 1.12436325014
0.992032 1.12837025353
0.996308 1.13238079559
1.000584 1.13639484638
1.00486 1.14041237643
1.009136 1.14443335668
1.013412 1.14845775853
1.017688 1.15248555377
1.021964 1.15651671465
1.02624 1.16055121383
1.030516 1.16458902435
1.034792 1.16863011968
1.039068 1.1726744737
1.043344 1.17672206063
1.04762 1.18077285514
1.051896 1.18482683224
1.056172 1.18888396732
1.060448 1.19294423616
1.064724 1.19700761488
1.069 1.20107407999
1.073276 1.20514360832
1.077552 1.20921617707
1.081828 1.21329176379
1.086104 1.21737034636
1.09038 1.221451903
1.094656 1.22553641227
1.098932 1.22962385303
1.103208 1.23371420449
1.107484 1.23780744617
1.11176 1.24190355789
1.116036 1.24600251981
1.120312 1.25010431236
1.124588 1.2542089163
1.128864 1.25831631267
1.13314 1.26242648281
1.137416 1.26653940834
1.141692 1.27065507119
1.145968 1.27477345354
1.150244 1.27889453787
1.15452 1.28301830694
1.158796 1.28714474375
1.163072 1.29127383161
1.167348 1.29540555406
1.171624 1.29953989492
1.1759 1.30367683826
1.180176 1.3078163684
1.184452 1.31195846993
1.188728 1.31610312767
1.193004 1.32025032669
1.19728 1.3244000523
1.201556 1.32855229007
1.205832 1.33270702577
1.210108 1.33686424543
1.214384 1.34102393531
1.21866 1.34518608188
1.222936 1.34935067185
1.227212 1.35351769216
1.231488 1.35768712995
1.235764 1.36185897258
1.24004 1.36603320765
1.244316 1.37020982294
1.248592 1.37438880646
1.252868 1.37857014643
1.257144 1.38275383125
1.26142 1.38693984955
1.265696 1.39112819015
1.269972 1.39531884207
1.274248 1.39951179453
1.278524 1.40370703693
1.2828 1.40790455888
1.287076 1.41210435018
1.291352 1.4163064008
1.295628 1.4205107009
1.299904 1.42471724085
1.30418 1.42892601117
1.308456 1.43313700257
1.312732 1.43735020595
1.317008 1.44156561238
1.321284 1.4457832131
1.32556 1.45000299953
1.329836 1.45422496325
1.334112 1.45844909602
1.338388 1.46267538977
1.342664 1.46690383659
1.34694 1.47113442874
1.351216 1.47536715864
1.355492 1.47960201887
1.359768 1.48383900217
1.364044 1.48807810144
1.36832 1.49231930975
1.372596 1.49656262031
1.376872 1.50080802649
1.381148 1.50505552181
1.385424 1.50930509995
1.3897 1.51355675472
1.393976 1.51781048012
1.398252 1.52206627025
1.402528 1.5263241194
1.406804 1.53058402197
1.41108 1.53484597252
1.415356 1.53910996576
1.419632 1.54337599654
1.423908 1.54764405984
1.428184 1.55191415078
1.43246 1.55618626464
1.436736 1.56046039681
1.441012 1.56473654284
1.445288 1.56901469841
1.449564 1.57329485931
1.45384 1.57757702151
1.458116 1.58186118108
1.462392 1.58614733422
1.466668 1.59043547729
1.470944 1.59472560674
1.47522 1.5990177192
1.479496 1.60331181138
1.483772 1.60760788014
1.488048 1.61190592247
1.492324 1.61620593548
1.4966 1.62050791641
1.500876 1.62481186263
1.505152 1.62911777161
1.509428 1.63342564097
1.513704 1.63773546844
1.51798 1.64204725188
1.522256 1.64636098927
1.526532 1.65067667869
1.530808 1.65499431838
1.535084 1.65931390666
1.53936 1.663635442
1.543636 1.66795892297
1.547912 1.67228434827
1.552188 1.6766117167
1.556464 1.68094102719
1.56074 1.6852722788
1.565016 1.68960547067
1.569292 1.69394060209
1.573568 1.69827767245
1.577844 1.70261668125
1.58212 1.70695762812
1.586396 1.71130051279
1.590672 1.71564533512
1.594948 1.71999209505
1.599224 1.72434079268
1.6035 1.72869142818
1.607776 1.73304400185
1.612052 1.73739851411
1.616328 1.74175496549
1.620604 1.7461133566
1.62488 1.75047368822
1.629156 1.75483596118
1.633432 1.75920017645
1.637708 1.76356633513
1.641984 1.76793443839
1.64626 1.77230448753
1.650536 1.77667648396
1.654812 1.78105042921
1.659088 1.78542632489
1.663364 1.78980417275
1.66764 1.79418397464
1.671916 1.79856573251
1.676192 1.80294944842
1.680468 1.80733512455
1.684744 1.81172276319
1.68902 1.81611236673
1.693296 1.82050393767
1.697572 1.82489747863
1.701848 1.82929299231
1.706124 1.83369048156
1.7104 1.8380899493
1.714676 1.84249139859
1.718952 1.84689483259
1.723228 1.85130025455
1.727504 1.85570766786
1.73178 1.86011707599
1.736056 1.86452848254
1.740332 1.86894189122
1.744608 1.87335730583
1.748884 1.8777747303
1.75316 1.88219416866
1.757436 1.88661562506
1.761712 1.89103910373
1.765988 1.89546460906
1.770264 1.89989214552
1.77454 1.90432171768
1.778816 1.90875333024
1.783092 1.91318698801
1.787368 1.91762269592
1.791644 1.92206045898
1.79592 1.92650028235
1.800196 1.93094217128
1.804472 1.93538613114
1.808748 1.93983216741
1.813024 1.94428028568
1.8173 1.94873049167
1.821576 1.95318279119
1.825852 1.95763719019
1.830128 1.96209369471
1.834404 1.96655231093
1.83868 1.97101304513
1.842956 1.9754759037
1.847232 1.97994089317
1.851508 1.98440802017
1.855784 1.98887729145
1.86006 1.99334871388
1.864336 1.99782229444
1.868612 2.00229804025
1.872888 2.00677595852
1.877164 2.01125605662
1.88144 2.01573834199
1.885716 2.02022282225
1.889992 2.02470950508
1.894268 2.02919839834
1.898544 2.03368950996
1.90282 2.03818284804
1.907096 2.04267842078
1.911372 2.04717623651
1.915648 2.05167630368
1.919924 2.05617863087
1.9242 2.0606832268
1.928476 2.0651901003
1.932752 2.06969926033
1.937028 2.07421071599
1.941304 2.07872447651
1.94558 2.08324055124
1.949856 2.08775894967
1.954132 2.09227968142
1.958408 2.09680275624
1.962684 2.10132818402
1.96696 2.10585597478
1.971236 2.11038613869
1.975512 2.11491868603
1.979788 2.11945362724
1.984064 2.1239909729
1.98834 2.12853073371
1.992616 2.13307292053
1.996892 2.13761754436
2.001168 2.14216461632
2.005444 2.14671414771
2.00972 2.15126614994
2.013996 2.15582063459
2.018272 2.16037761338
2.022548 2.16493709818
2.026824 2.16949910099
2.0311 2.174063634
2.035376 2.1786307095
2.039652 2.18320033999
2.043928 2.18777253807
2.048204 2.19234731654
2.05248 2.19692468832
2.056756 2.20150466651
2.061032 2.20608726436
2.065308 2.21067249529
2.069584 2.21526037287
2.07386 2.21985091084
2.078136 2.2244441231
2.082412 2.22904002372
2.086688 2.23363862693
2.090964 2.23823994713
2.09524 2.24284399891
2.099516 2.24745079701
2.103792 2.25206035633
2.108068 2.25667269199
2.112344 2.26128781924
2.11662 2.26590575354
2.120896 2.27052651052
2.125172 2.27515010597
2.129448 2.27977655589
2.133724 2.28440587647


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-upperEnd-sigma1pt5prob0pt5.tex <==
0.0 0.480437118408
0.004276 0.48045714819
0.008552 0.480517232554
0.012828 0.480617356553
0.017104 0.480757495301
0.02138 0.480937613996
0.025656 0.481157667973
0.029932 0.481417602749
0.034208 0.4817173541
0.038484 0.482056848134
0.04276 0.482436001384
0.047036 0.482854720912
0.051312 0.483312904419
0.055588 0.483810440372
0.059864 0.484347208138
0.06414 0.484923078126
0.068416 0.485537911943
0.072692 0.486191562559
0.076968 0.486883874475
0.081244 0.487614683906
0.08552 0.48838381897
0.089796 0.489191099879
0.094072 0.490036339148
0.098348 0.490919341798
0.102624 0.491839905571
0.1069 0.492797821154
0.111176 0.493792872401
0.115452 0.494824836559
0.119728 0.495893484506
0.124004 0.496998580984
0.12828 0.498139884836
0.132556 0.499317149251
0.136832 0.500530122003
0.141108 0.501778545694
0.145384 0.503062158004
0.14966 0.504380691928
0.153936 0.505733876026
0.158212 0.507121434667
0.162488 0.508543088267
0.166764 0.509998553537
0.17104 0.511487543717
0.175316 0.513009768817
0.179592 0.51456493585
0.183868 0.516152749067
0.188144 0.51777291018
0.19242 0.519425118596
0.196696 0.52110907163
0.200972 0.522824464729
0.205248 0.524570991682
0.209524 0.526348344831
0.2138 0.528156215276
0.218076 0.529994293071
0.222352 0.531862267423
0.226628 0.533759826881
0.230904 0.535686659516
0.23518 0.537642453109
0.239456 0.539626895315
0.243732 0.541639673838
0.248008 0.543680476592
0.252284 0.545748991858
0.25656 0.547844908438
0.260836 0.549967915795
0.265112 0.552117704204
0.269388 0.554293964878
0.273664 0.5564963901
0.27794 0.558724673352
0.282216 0.560978509428
0.286492 0.56325759455
0.290768 0.565561626475
0.295044 0.5678903046
0.29932 0.570243330056
0.303596 0.572620405807
0.307872 0.575021236729
0.312148 0.577445529702
0.316424 0.579892993681
0.3207 0.582363339774
0.324976 0.584856281306
0.329252 0.58737153389
0.333528 0.589908815483
0.337804 0.59246784644
0.34208 0.59504834957
0.346356 0.597650050185
0.350632 0.600272676136
0.354908 0.602915957864
0.359184 0.605579628427
0.36346 0.60826342354
0.367736 0.610967081603
0.372012 0.613690343726
0.376288 0.616432953756
0.380564 0.619194658292
0.38484 0.621975206709
0.389116 0.62477435117
0.393392 0.627591846638
0.397668 0.630427450887
0.401944 0.633280924507
0.40622 0.636152030912
0.410496 0.639040536344
0.414772 0.641946209867
0.419048 0.644868823374
0.423324 0.647808151578
0.4276 0.650763972011
0.431876 0.653736065014
0.436152 0.656724213731
0.440428 0.659728204099
0.444704 0.662747824836
0.44898 0.665782867427
0.453256 0.668833126115
0.457532 0.671898397881
0.461808 0.674978482428
0.466084 0.678073182167
0.47036 0.681182302197
0.474636 0.684305650284
0.478912 0.687443036845
0.483188 0.690594274922
0.487464 0.693759180165
0.49174 0.696937570806
0.496016 0.700129267639
0.500292 0.703334093995
0.504568 0.706551875718
0.508844 0.70978244114
0.51312 0.713025621059
0.517396 0.716281248709
0.521672 0.719549159738
0.525948 0.72282919218
0.530224 0.72612118643
0.5345 0.729424985216
0.538776 0.732740433574
0.543052 0.736067378821
0.547328 0.739405670526
0.551604 0.742755160485
0.55588 0.746115702693
0.560156 0.749487153317
0.564432 0.752869370668
0.568708 0.756262215175
0.572984 0.759665549357
0.57726 0.763079237795
0.581536 0.766503147107
0.585812 0.769937145919
0.590088 0.773381104838
0.594364 0.776834896428
0.59864 0.780298395178
0.602916 0.783771477481
0.607192 0.787254021605
0.611468 0.790745907664
0.615744 0.794247017599
0.62002 0.797757235143
0.624296 0.801276445804
0.628572 0.804804536835
0.632848 0.808341397207
0.637124 0.811886917588
0.6414 0.815440990316
0.645676 0.819003509377
0.649952 0.822574370374
0.654228 0.826153470511
0.658504 0.829740708565
0.66278 0.833335984863
0.667056 0.836939201257
0.671332 0.840550261104
0.675608 0.844169069242
0.679884 0.847795531968
0.68416 0.851429557013
0.688436 0.855071053524
0.692712 0.858719932039
0.696988 0.862376104468
0.701264 0.866039484071
0.70554 0.869709985435
0.709816 0.873387524459
0.714092 0.877072018327
0.718368 0.880763385493
0.722644 0.884461545657
0.72692 0.888166419751
0.731196 0.891877929913
0.735472 0.895595999476
0.739748 0.899320552941
0.744024 0.903051515966
0.7483 0.906788815341
0.752576 0.910532378978
0.756852 0.914282135885
0.761128 0.918038016156
0.765404 0.92179995095
0.76968 0.925567872473
0.773956 0.929341713965
0.778232 0.933121409684
0.782508 0.936906894885
0.786784 0.940698105809
0.79106 0.944494979665
0.795336 0.948297454617
0.799612 0.952105469766
0.803888 0.955918965138
0.808164 0.959737881667
0.81244 0.963562161182
0.816716 0.967391746394
0.820992 0.97122658088
0.825268 0.975066609069
0.829544 0.978911776233
0.83382 0.982762028466
0.838096 0.98661731268
0.842372 0.990477576585
0.846648 0.994342768681
0.850924 0.998212838243
0.8552 1.00208773531
0.859476 1.00596741067
0.863752 1.00985181586
0.868028 1.01374090314
0.872304 1.01763462548
0.87658 1.02153293657
0.880856 1.02543579078
0.885132 1.02934314318
0.889408 1.0332549495
0.893684 1.03717116614
0.89796 1.04109175015
0.902236 1.04501665923
0.906512 1.04894585171
0.910788 1.05287928654
0.915064 1.05681692329
0.91934 1.06075872211
0.923616 1.06470464378
0.927892 1.06865464966
0.932168 1.07260870166
0.936444 1.07656676228
0.94072 1.08052879458
0.944996 1.08449476216
0.949272 1.08846462918
0.953548 1.09243836032
0.957824 1.09641592079
0.9621 1.10039727633
0.966376 1.10438239316
0.970652 1.10837123805
0.974928 1.11236377822
0.979204 1.1163599814
0.98348 1.12035981582
0.987756 1.12436325014
0.992032 1.12837025353
0.996308 1.13238079559
1.000584 1.13639484638
1.00486 1.14041237643
1.009136 1.14443335668
1.013412 1.14845775853
1.017688 1.15248555377
1.021964 1.15651671465
1.02624 1.16055121383
1.030516 1.16458902435
1.034792 1.16863011968
1.039068 1.1726744737
1.043344 1.17672206063
1.04762 1.18077285514
1.051896 1.18482683224
1.056172 1.18888396732
1.060448 1.19294423616
1.064724 1.19700761488
1.069 1.20107407999
1.073276 1.20514360832
1.077552 1.20921617707
1.081828 1.21329176379
1.086104 1.21737034636
1.09038 1.221451903
1.094656 1.22553641227
1.098932 1.22962385303
1.103208 1.23371420449
1.107484 1.23780744617
1.11176 1.24190355789
1.116036 1.24600251981
1.120312 1.25010431236
1.124588 1.2542089163
1.128864 1.25831631267
1.13314 1.26242648281
1.137416 1.26653940834
1.141692 1.27065507119
1.145968 1.27477345354
1.150244 1.27889453787
1.15452 1.28301830694
1.158796 1.28714474375
1.163072 1.29127383161
1.167348 1.29540555406
1.171624 1.29953989492
1.1759 1.30367683826
1.180176 1.3078163684
1.184452 1.31195846993
1.188728 1.31610312767
1.193004 1.32025032669
1.19728 1.3244000523
1.201556 1.32855229007
1.205832 1.33270702577
1.210108 1.33686424543
1.214384 1.34102393531
1.21866 1.34518608188
1.222936 1.34935067185
1.227212 1.35351769216
1.231488 1.35768712995
1.235764 1.36185897258
1.24004 1.36603320765
1.244316 1.37020982294
1.248592 1.37438880646
1.252868 1.37857014643
1.257144 1.38275383125
1.26142 1.38693984955
1.265696 1.39112819015
1.269972 1.39531884207
1.274248 1.39951179453
1.278524 1.40370703693
1.2828 1.40790455888
1.287076 1.41210435018
1.291352 1.4163064008
1.295628 1.4205107009
1.299904 1.42471724085
1.30418 1.42892601117
1.308456 1.43313700257
1.312732 1.43735020595
1.317008 1.44156561238
1.321284 1.4457832131
1.32556 1.45000299953
1.329836 1.45422496325
1.334112 1.45844909602
1.338388 1.46267538977
1.342664 1.46690383659
1.34694 1.47113442874
1.351216 1.47536715864
1.355492 1.47960201887
1.359768 1.48383900217
1.364044 1.48807810144
1.36832 1.49231930975
1.372596 1.49656262031
1.376872 1.50080802649
1.381148 1.50505552181
1.385424 1.50930509995
1.3897 1.51355675472
1.393976 1.51781048012
1.398252 1.52206627025
1.402528 1.5263241194
1.406804 1.53058402197
1.41108 1.53484597252
1.415356 1.53910996576
1.419632 1.54337599654
1.423908 1.54764405984
1.428184 1.55191415078
1.43246 1.55618626464
1.436736 1.56046039681
1.441012 1.56473654284
1.445288 1.56901469841
1.449564 1.57329485931
1.45384 1.57757702151
1.458116 1.58186118108
1.462392 1.58614733422
1.466668 1.59043547729
1.470944 1.59472560674
1.47522 1.5990177192
1.479496 1.60331181138
1.483772 1.60760788014
1.488048 1.61190592247
1.492324 1.61620593548
1.4966 1.62050791641
1.500876 1.62481186263
1.505152 1.62911777161
1.509428 1.63342564097
1.513704 1.63773546844
1.51798 1.64204725188
1.522256 1.64636098927
1.526532 1.65067667869
1.530808 1.65499431838
1.535084 1.65931390666
1.53936 1.663635442
1.543636 1.66795892297
1.547912 1.67228434827
1.552188 1.6766117167
1.556464 1.68094102719
1.56074 1.6852722788
1.565016 1.68960547067
1.569292 1.69394060209
1.573568 1.69827767245
1.577844 1.70261668125
1.58212 1.70695762812
1.586396 1.71130051279
1.590672 1.71564533512
1.594948 1.71999209505
1.599224 1.72434079268
1.6035 1.72869142818
1.607776 1.73304400185
1.612052 1.73739851411
1.616328 1.74175496549
1.620604 1.7461133566
1.62488 1.75047368822
1.629156 1.75483596118
1.633432 1.75920017645
1.637708 1.76356633513
1.641984 1.76793443839
1.64626 1.77230448753
1.650536 1.77667648396
1.654812 1.78105042921
1.659088 1.78542632489
1.663364 1.78980417275
1.66764 1.79418397464
1.671916 1.79856573251
1.676192 1.80294944842
1.680468 1.80733512455
1.684744 1.81172276319
1.68902 1.81611236673
1.693296 1.82050393767
1.697572 1.82489747863
1.701848 1.82929299231
1.706124 1.83369048156
1.7104 1.8380899493
1.714676 1.84249139859
1.718952 1.84689483259
1.723228 1.85130025455
1.727504 1.85570766786
1.73178 1.86011707599
1.736056 1.86452848254
1.740332 1.86894189122
1.744608 1.87335730583
1.748884 1.8777747303
1.75316 1.88219416866
1.757436 1.88661562506
1.761712 1.89103910373
1.765988 1.89546460906
1.770264 1.89989214552
1.77454 1.90432171768
1.778816 1.90875333024
1.783092 1.91318698801
1.787368 1.91762269592
1.791644 1.92206045898
1.79592 1.92650028235
1.800196 1.93094217128
1.804472 1.93538613114
1.808748 1.93983216741
1.813024 1.94428028568
1.8173 1.94873049167
1.821576 1.95318279119
1.825852 1.95763719019
1.830128 1.96209369471
1.834404 1.96655231093
1.83868 1.97101304513
1.842956 1.9754759037
1.847232 1.97994089317
1.851508 1.98440802017
1.855784 1.98887729145
1.86006 1.99334871388
1.864336 1.99782229444
1.868612 2.00229804025
1.872888 2.00677595852
1.877164 2.01125605662
1.88144 2.01573834199
1.885716 2.02022282225
1.889992 2.02470950508
1.894268 2.02919839834
1.898544 2.03368950996
1.90282 2.03818284804
1.907096 2.04267842078
1.911372 2.04717623651
1.915648 2.05167630368
1.919924 2.05617863087
1.9242 2.0606832268
1.928476 2.0651901003
1.932752 2.06969926033
1.937028 2.07421071599
1.941304 2.07872447651
1.94558 2.08324055124
1.949856 2.08775894967
1.954132 2.09227968142
1.958408 2.09680275624
1.962684 2.10132818402
1.96696 2.10585597478
1.971236 2.11038613869
1.975512 2.11491868603
1.979788 2.11945362724
1.984064 2.1239909729
1.98834 2.12853073371
1.992616 2.13307292053
1.996892 2.13761754436
2.001168 2.14216461632
2.005444 2.14671414771
2.00972 2.15126614994
2.013996 2.15582063459
2.018272 2.16037761338
2.022548 2.16493709818
2.026824 2.16949910099
2.0311 2.174063634
2.035376 2.1786307095
2.039652 2.18320033999
2.043928 2.18777253807
2.048204 2.19234731654
2.05248 2.19692468832
2.056756 2.20150466651
2.061032 2.20608726436
2.065308 2.21067249529
2.069584 2.21526037287
2.07386 2.21985091084
2.078136 2.2244441231
2.082412 2.22904002372
2.086688 2.23363862693
2.090964 2.23823994713
2.09524 2.24284399891
2.099516 2.24745079701
2.103792 2.25206035633
2.108068 2.25667269199
2.112344 2.26128781924
2.11662 2.26590575354
2.120896 2.27052651052
2.125172 2.27515010597
2.129448 2.27977655589
2.133724 2.28440587647


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-upperEnd-sigma2prob0pt05.tex <==
0.0 0.640582824544
0.008276 0.64063909664
0.016552 0.640807883433
0.024828 0.641089096509
0.033104 0.641482588771
0.04138 0.641988154827
0.049656 0.64260553152
0.057932 0.643334398621
0.066208 0.644174379652
0.074484 0.645125042856
0.08276 0.646185902295
0.091036 0.647356419082
0.099312 0.648636002719
0.107588 0.650024012564
0.115864 0.651519759384
0.12414 0.653122507022
0.132416 0.654831474132
0.140692 0.656645836001
0.148968 0.658564726439
0.157244 0.660587239725
0.16552 0.662712432599
0.173796 0.664939326299
0.182072 0.667266908625
0.190348 0.669694136024
0.198624 0.672219935689
0.2069 0.674843207662
0.215176 0.677562826928
0.223452 0.680377645505
0.231728 0.68328649451
0.240004 0.686288186198
0.24828 0.68938151597
0.256556 0.692565264345
0.264832 0.695838198888
0.273108 0.699199076084
0.281384 0.702646643168
0.28966 0.706179639895
0.297936 0.709796800246
0.306212 0.713496854083
0.314488 0.717278528728
0.322764 0.721140550481
0.33104 0.725081646075
0.339316 0.729100544052
0.347592 0.733195976076
0.355868 0.737366678181
0.364144 0.741611391941
0.37242 0.745928865576
0.380696 0.750317854993
0.388972 0.75477712475
0.397248 0.759305448966
0.405524 0.76390161216
0.4138 0.768564410028
0.422076 0.773292650157
0.430352 0.778085152687
0.438628 0.782940750907
0.446904 0.7878582918
0.45518 0.792836636535
0.463456 0.797874660907
0.471732 0.802971255728
0.480008 0.808125327172
0.488284 0.813335797076
0.49656 0.8186016032
0.504836 0.82392169944
0.513112 0.829295056015
0.521388 0.834720659608
0.529664 0.840197513477
0.53794 0.845724637538
0.546216 0.851301068412
0.554492 0.856925859449
0.562768 0.862598080725
0.571044 0.868316819015
0.57932 0.874081177742
0.587596 0.879890276909
0.595872 0.885743253009
0.604148 0.891639258919
0.612424 0.897577463778
0.6207 0.90355705285
0.628976 0.909577227372
0.637252 0.915637204395
0.645528 0.921736216607
0.653804 0.927873512154
0.66208 0.934048354446
0.670356 0.940260021957
0.678632 0.946507808022
0.686908 0.952791020622
0.695184 0.959108982167
0.70346 0.965461029278
0.711736 0.971846512558
0.720012 0.978264796366
0.728288 0.984715258587
0.736564 0.991197290399
0.74484 0.997710296041
0.753116 1.00425369258
0.761392 1.01082690966
0.769668 1.01742938931
0.777944 1.02406058566
0.78622 1.03071996475
0.794496 1.03740700426
0.802772 1.04412119331
0.811048 1.05086203222
0.819324 1.05762903229
0.8276 1.06442171558
0.835876 1.07123961464
0.844152 1.07808227238
0.852428 1.08494924178
0.860704 1.09184008568
0.86898 1.09875437663
0.877256 1.10569169662
0.885532 1.11265163689
0.893808 1.11963379775
0.902084 1.12663778837
0.91036 1.13366322656
0.918636 1.14070973864
0.926912 1.14777695919
0.935188 1.15486453089
0.943464 1.16197210434
0.95174 1.1690993379
0.960016 1.17624589749
0.968292 1.18341145641
0.976568 1.19059569521
0.984844 1.1977983015
0.99312 1.20501896981
1.001396 1.21225740141
1.009672 1.21951330416
1.017948 1.22678639238
1.026224 1.23407638668
1.0345 1.24138301384
1.042776 1.24870600664
1.051052 1.25604510376
1.059328 1.2634000496
1.067604 1.27077059419
1.07588 1.27815649304
1.084156 1.28555750702
1.092432 1.29297340225
1.100708 1.30040394995
1.108984 1.30784892636
1.11726 1.3153081126
1.125536 1.32278129456
1.133812 1.33026826282
1.142088 1.33776881251
1.150364 1.34528274321
1.15864 1.35280985889
1.166916 1.36034996775
1.175192 1.36790288217
1.183468 1.37546841861
1.191744 1.3830463975
1.20002 1.39063664315
1.208296 1.3982389837
1.216572 1.405853251
1.224848 1.41347928052
1.233124 1.42111691131
1.2414 1.42876598589
1.249676 1.43642635018
1.257952 1.44409785342
1.266228 1.45178034813
1.274504 1.45947368998
1.28278 1.46717773778
1.291056 1.47489235336
1.299332 1.48261740155
1.307608 1.49035275009
1.315884 1.49809826958
1.32416 1.5058538334
1.332436 1.51361931768
1.340712 1.52139460119
1.348988 1.52917956537
1.357264 1.53697409417
1.36554 1.5447780741
1.373816 1.55259139407
1.382092 1.56041394546
1.390368 1.56824562195
1.398644 1.57608631957
1.40692 1.58393593657
1.415196 1.59179437345
1.423472 1.59966153286
1.431748 1.60753731957
1.440024 1.61542164046
1.4483 1.62331440443
1.456576 1.63121552236
1.464852 1.63912490714
1.473128 1.64704247355
1.481404 1.65496813825
1.48968 1.66290181976
1.497956 1.67084343841
1.506232 1.67879291632
1.514508 1.68675017732
1.522784 1.69471514698
1.53106 1.70268775254
1.539336 1.71066792287
1.547612 1.71865558849
1.555888 1.72665068147
1.564164 1.73465313546
1.57244 1.74266288563
1.580716 1.75067986864
1.588992 1.75870402265
1.597268 1.76673528724
1.605544 1.77477360343
1.61382 1.78281891363
1.622096 1.79087116161
1.630372 1.79893029252
1.638648 1.8069962528
1.646924 1.81506899022
1.6552 1.82314845382
1.663476 1.8312345939
1.671752 1.839327362
1.680028 1.84742671088
1.688304 1.85553259449
1.69658 1.86364496797
1.704856 1.87176378763
1.713132 1.8798890109
1.721408 1.88802059634
1.729684 1.89615850364
1.73796 1.90430269355
1.746236 1.91245312791
1.754512 1.92060976962
1.762788 1.92877258263
1.771064 1.93694153189
1.77934 1.9451165834
1.787616 1.95329770412
1.795892 1.96148486202
1.804168 1.96967802605
1.812444 1.97787716608
1.82072 1.98608225297
1.828996 1.99429325848
1.837272 2.0025101553
1.845548 2.01073291704
1.853824 2.0189615182
1.8621 2.02719593415
1.870376 2.03543614117
1.878652 2.04368211637
1.886928 2.05193383774
1.895204 2.06019128411
1.90348 2.06845443513
1.911756 2.07672327129
1.920032 2.0849977739
1.928308 2.09327792508
1.936584 2.10156370773
1.94486 2.10985510557
1.953136 2.11815210308
1.961412 2.12645468553
1.969688 2.13476283895
1.977964 2.14307655015
1.98624 2.15139580668
1.994516 2.15972059684
2.002792 2.16805090968
2.011068 2.17638673497
2.019344 2.18472806322
2.02762 2.19307488568
2.035896 2.20142719428
2.044172 2.20978498171
2.052448 2.21814824133
2.060724 2.22651696722
2.069 2.23489115417
2.077276 2.24327079764
2.085552 2.25165589379
2.093828 2.26004643949
2.102104 2.26844243226
2.11038 2.2768438703
2.118656 2.28525075252
2.126932 2.29366307847
2.135208 2.30208084837
2.143484 2.31050406313
2.15176 2.3189327243
2.160036 2.3273668341
2.168312 2.33580639541
2.176588 2.34425141178
2.184864 2.35270188739
2.19314 2.36115782708
2.201416 2.36961923636
2.209692 2.37808612137
2.217968 2.3865584889
2.226244 2.39503634641
2.23452 2.40351970198
2.242796 2.41200856436
2.251072 2.42050294291
2.259348 2.42900284769
2.267624 2.43750828935
2.2759 2.44601927922
2.284176 2.45453582927
2.292452 2.4630579521
2.300728 2.47158566097
2.309004 2.48011896979
2.31728 2.48865789311
2.325556 2.49720244612
2.333832 2.50575264468
2.342108 2.51430850528
2.350384 2.52287004509
2.35866 2.53143728189
2.366936 2.54001023417
2.375212 2.54858892102
2.383488 2.55717336224
2.391764 2.56576357827
2.40004 2.5743595902
2.408316 2.58296141982
2.416592 2.59156908956
2.424868 2.60018262253
2.433144 2.60880204254
2.44142 2.61742737403
2.449696 2.62605864218
2.457972 2.63469587281
2.466248 2.64333909245
2.474524 2.65198832832
2.4828 2.66064360833
2.491076 2.66930496112
2.499352 2.67797241601
2.507628 2.68664600302
2.515904 2.69532575293
2.52418 2.7040116972
2.532456 2.71270386803
2.540732 2.72140229836
2.549008 2.73010702186
2.557284 2.73881807294
2.56556 2.74753548676
2.573836 2.75625929924
2.582112 2.76498954706
2.590388 2.77372626766
2.598664 2.78246949927
2.60694 2.79121928088
2.615216 2.79997565229
2.623492 2.80873865409
2.631768 2.81750832766
2.640044 2.82628471521
2.64832 2.83506785976
2.656596 2.84385780516
2.664872 2.85265459609
2.673148 2.86145827809
2.681424 2.87026889754
2.6897 2.87908650168
2.697976 2.88791113863
2.706252 2.89674285739
2.714528 2.90558170786
2.722804 2.91442774083
2.73108 2.923281008
2.739356 2.932141562
2.747632 2.9410094564
2.755908 2.9498847457
2.764184 2.95876748537
2.77246 2.96765773183
2.780736 2.97655554249
2.789012 2.98546097577
2.797288 2.99437409107
2.805564 3.00329494881
2.81384 3.01222361046
2.822116 3.02116013851
2.830392 3.03010459652
2.838668 3.03905704913
2.846944 3.04801756206
2.85522 3.05698620212
2.863496 3.06596303726
2.871772 3.07494813655
2.880048 3.0839415702
2.888324 3.09294340961
2.8966 3.10195372733
2.904876 3.11097259714
2.913152 3.12000009401
2.921428 3.12903629415
2.929704 3.13808127504
2.93798 3.14713511541
2.946256 3.15619789529
2.954532 3.16526969601
2.962808 3.17435060025
2.971084 3.18344069201
2.97936 3.19254005669
2.987636 3.20164878106
2.995912 3.21076695333
3.004188 3.21989466312
3.012464 3.22903200152
3.02074 3.23817906111
3.029016 3.24733593597
3.037292 3.25650272171
3.045568 3.26567951552
3.053844 3.27486641614
3.06212 3.28406352394
3.070396 3.29327094092
3.078672 3.30248877075
3.086948 3.31171711879
3.095224 3.32095609212
3.1035 3.33020579957
3.111776 3.33946635177
3.120052 3.34873786113
3.128328 3.35802044194
3.136604 3.36731421034
3.14488 3.3766192844
3.153156 3.38593578413
3.161432 3.39526383152
3.169708 3.40460355057
3.177984 3.41395506736
3.18626 3.42331851002
3.194536 3.43269400885
3.202812 3.44208169629
3.211088 3.45148170702
3.219364 3.46089417794
3.22764 3.47031924826
3.235916 3.47975705955
3.244192 3.48920775572
3.252468 3.49867148315
3.260744 3.50814839067
3.26902 3.51763862965
3.277296 3.52714235404
3.285572 3.53665972039
3.293848 3.54619088795
3.302124 3.55573601871
3.3104 3.56529527742
3.318676 3.57486883169
3.326952 3.58445685204
3.335228 3.59405951192
3.343504 3.60367698784
3.35178 3.61330945936
3.360056 3.62295710922
3.368332 3.63262012336
3.376608 3.64229869099
3.384884 3.65199300469
3.39316 3.66170326047
3.401436 3.67142965781
3.409712 3.6811723998
3.417988 3.69093169315
3.426264 3.70070774833
3.43454 3.71050077958
3.442816 3.7203110051
3.451092 3.73013864701
3.459368 3.73998393156
3.467644 3.74984708912
3.47592 3.75972835435
3.484196 3.76962796627
3.492472 3.77954616833
3.500748 3.78948320857
3.509024 3.79943933968
3.5173 3.80941481914
3.525576 3.8194099093
3.533852 3.82942487755
3.542128 3.83945999635
3.550404 3.84951554347
3.55868 3.85959180201
3.566956 3.86968906058
3.575232 3.87980761345
3.583508 3.88994776065
3.591784 3.90010980814
3.60006 3.91029406794
3.608336 3.92050085832
3.616612 3.93073050388
3.624888 3.94098333581
3.633164 3.95125969199
3.64144 3.96155991716
3.649716 3.97188436316
3.657992 3.98223338905
3.666268 3.99260736133
3.674544 4.00300665413
3.68282 4.01343164943
3.691096 4.02388273723
3.699372 4.03436031583
3.707648 4.04486479199
3.715924 4.0553965812
3.7242 4.06595610791
3.732476 4.0765438058
3.740752 4.08716011799
3.749028 4.09780549737
3.757304 4.10848040682
3.76558 4.11918531952
3.773856 4.12992071927
3.782132 4.14068710077
3.790408 4.15148496991
3.798684 4.16231484419
3.80696 4.17317725297
3.815236 4.18407273789
3.823512 4.19500185319
3.831788 4.20596516615
3.840064 4.21696325744
3.84834 4.22799672154
3.856616 4.23906616723
3.864892 4.25017221793
3.873168 4.26131551228
3.881444 4.27249670452
3.88972 4.28371646509
3.897996 4.29497548107
3.906272 4.30627445678
3.914548 4.31761411432
3.922824 4.32899519417
3.9311 4.34041845583
3.939376 4.35188467839
3.947652 4.36339466131
3.955928 4.37494922501
3.964204 4.38654921167
3.97248 4.39819548597
3.980756 4.40988893586
3.989032 4.42163047345
3.997308 4.43342103583
4.005584 4.44526158597
4.01386 4.45715311372
4.022136 4.46909663675
4.030412 4.48109320164
4.038688 4.49314388492
4.046964 4.50524979424
4.05524 4.51741206958
4.063516 4.52963188447
4.071792 4.54191044732
4.080068 4.55424900282
4.088344 4.56664883337
4.09662 4.5791112606
4.104896 4.59163764701
4.113172 4.60422939761
4.121448 4.61688796174
4.129724 4.62961483489


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForRayleigh-upperEnd-sigma2prob0pt1.tex <==
0.0 0.918087210053
0.00856 0.918131548535
0.01712 0.918264551407
0.02568 0.918486180962
0.03424 0.91879637442
0.0428 0.919195044011
0.05136 0.919682077111
0.05992 0.920257336397
0.06848 0.920920660047
0.07704 0.921671861972
0.0856 0.922510732081
0.09416 0.923437036577
0.10272 0.924450518291
0.11128 0.925550897035
0.11984 0.926737869998
0.1284 0.928011112163
0.13696 0.929370276749
0.14552 0.930814995681
0.15408 0.932344880091
0.16264 0.933959520828
0.1712 0.935658488998
0.17976 0.937441336525
0.18832 0.939307596725
0.19688 0.941256784896
0.20544 0.943288398928
0.214 0.945401919922
0.22256 0.947596812819
0.23112 0.949872527045
0.23968 0.952228497157
0.24824 0.954664143501
0.2568 0.957178872869
0.26536 0.959772079169
0.27392 0.962443144087
0.28248 0.965191437754
0.29104 0.968016319412
0.2996 0.970917138082
0.30816 0.973893233214
0.31672 0.976943935355
0.32528 0.980068566785
0.33384 0.983266442172
0.3424 0.986536869194
0.35096 0.989879149175
0.35952 0.993292577689
0.36808 0.996776445175
0.37664 1.00033003752
0.3852 1.00395263664
0.39376 1.00764352106
0.40232 1.01140196645
0.41088 1.01522724617
0.41944 1.01911863178
0.428 1.02307539361
0.43656 1.02709680115
0.44512 1.03118212363
0.45368 1.03533063043
0.46224 1.03954159152
0.4708 1.04381427792
0.47936 1.0481479621
0.48792 1.05254191837
0.49648 1.05699542329
0.50504 1.06150775599
0.5136 1.06607819856
0.52216 1.07070603636
0.53072 1.07539055836
0.53928 1.0801310574
0.54784 1.08492683054
0.5564 1.08977717927
0.56496 1.0946814098
0.57352 1.09963883328
0.58208 1.10464876608
0.59064 1.10971052992
0.5992 1.11482345214
0.60776 1.11998686586
0.61632 1.12520011015
0.62488 1.13046253021
0.63344 1.1357734775
0.642 1.14113230986
0.65056 1.1465383917
0.65912 1.15199109405
0.66768 1.1574897947
0.67624 1.16303387827
0.6848 1.16862273631
0.69336 1.17425576739
0.70192 1.17993237712
0.71048 1.18565197824
0.71904 1.19141399068
0.7276 1.19721784156
0.73616 1.20306296526
0.74472 1.20894880342
0.75328 1.21487480498
0.76184 1.22084042616
0.7704 1.2268451305
0.77896 1.23288838886
0.78752 1.23896967937
0.79608 1.24508848746
0.80464 1.25124430583
0.8132 1.25743663444
0.82176 1.26366498047
0.83032 1.26992885829
0.83888 1.27622778942
0.84744 1.28256130252
0.856 1.28892893334
0.86456 1.29533022464
0.87312 1.30176472618
0.88168 1.30823199468
0.89024 1.31473159371
0.8988 1.32126309371
0.90736 1.32782607188
0.91592 1.33442011211
0.92448 1.341044805
0.93304 1.34769974768
0.9416 1.35438454386
0.95016 1.36109880367
0.95872 1.36784214366
0.96728 1.3746141867
0.97584 1.38141456191
0.9844 1.38824290461
0.99296 1.39509885623
1.00152 1.40198206424
1.01008 1.4088921821
1.01864 1.41582886916
1.0272 1.4227917906
1.03576 1.42978061737
1.04432 1.43679502608
1.05288 1.44383469898
1.06144 1.45089932384
1.07 1.45798859391
1.07856 1.46510220782
1.08712 1.47223986954
1.09568 1.47940128827
1.10424 1.4865861784
1.1128 1.49379425944
1.12136 1.5010252559
1.12992 1.50827889729
1.13848 1.515554918
1.14704 1.52285305726
1.1556 1.53017305905
1.16416 1.53751467203
1.17272 1.54487764951
1.18128 1.55226174933
1.18984 1.55966673383
1.1984 1.56709236978
1.20696 1.5745384283
1.21552 1.58200468482
1.22408 1.589490919
1.23264 1.59699691465
1.2412 1.60452245972
1.24976 1.6120673462
1.25832 1.61963137007
1.26688 1.62721433122
1.27544 1.63481603344
1.284 1.64243628433
1.29256 1.65007489523
1.30112 1.65773168122
1.30968 1.66540646098
1.31824 1.67309905682
1.3268 1.6808092946
1.33536 1.68853700362
1.34392 1.69628201668
1.35248 1.70404416992
1.36104 1.71182330284
1.3696 1.71961925824
1.37816 1.72743188213
1.38672 1.73526102375
1.39528 1.74310653547
1.40384 1.75096827276
1.4124 1.75884609417
1.42096 1.76673986124
1.42952 1.77464943849
1.43808 1.7825746934
1.44664 1.79051549629
1.4552 1.79847172037
1.46376 1.80644324164
1.47232 1.81442993889
1.48088 1.8224316936
1.48944 1.83044839001
1.498 1.83847991496
1.50656 1.84652615794
1.51512 1.85458701105
1.52368 1.8626623689
1.53224 1.87075212866
1.5408 1.87885618996
1.54936 1.8869744549
1.55792 1.89510682802
1.56648 1.90325321623
1.57504 1.91141352882
1.5836 1.9195876774
1.59216 1.92777557592
1.60072 1.93597714057
1.60928 1.94419228981
1.61784 1.95242094435
1.6264 1.96066302705
1.63496 1.968918463
1.64352 1.97718717939
1.65208 1.98546910558
1.66064 1.99376417301
1.6692 2.0020723152
1.67776 2.01039346773
1.68632 2.01872756824
1.69488 2.02707455635
1.70344 2.03543437371
1.712 2.04380696393
1.72056 2.05219227257
1.72912 2.06059024715
1.73768 2.0690008371
1.74624 2.07742399375
1.7548 2.08585967033
1.76336 2.09430782193
1.77192 2.1027684055
1.78048 2.11124137982
1.78904 2.11972670552
1.7976 2.12822434502
1.80616 2.13673426253
1.81472 2.14525642408
1.82328 2.15379079745
1.83184 2.16233735217
1.8404 2.17089605953
1.84896 2.17946689256
1.85752 2.18804982603
1.86608 2.19664483639
1.87464 2.20525190183
1.8832 2.21387100223
1.89176 2.22250211916
1.90032 2.23114523586
1.90888 2.23980033728
1.91744 2.24846740998
1.926 2.25714644224
1.93456 2.26583742395
1.94312 2.27454034669
1.95168 2.28325520363
1.96024 2.29198198964
1.9688 2.30072070118
1.97736 2.30947133635
1.98592 2.31823389489
1.99448 2.32700837817
2.00304 2.33579478915
2.0116 2.34459313245
2.02016 2.35340341428
2.02872 2.36222564249
2.03728 2.37105982652
2.04584 2.37990597745
2.0544 2.38876410798
2.06296 2.39763423241
2.07152 2.40651636669
2.08008 2.41541052835
2.08864 2.42431673658
2.0972 2.43323501219
2.10576 2.4421653776
2.11432 2.4511078569
2.12288 2.46006247578
2.13144 2.4690292616
2.14 2.47800824337
2.14856 2.48699945172
2.15712 2.49600291899
2.16568 2.50501867915
2.17424 2.51404676786
2.1828 2.52308722245
2.19136 2.53214008196
2.19992 2.5412053871
2.20848 2.55028318033
2.21704 2.55937350579
2.2256 2.56847640936
2.23416 2.57759193867
2.24272 2.58672014308
2.25128 2.59586107374
2.25984 2.60501478356
2.2684 2.61418132723
2.27696 2.62336076127
2.28552 2.63255314398
2.29408 2.64175853551
2.30264 2.65097699788
2.3112 2.66020859493
2.31976 2.66945339241
2.32832 2.67871145796
2.33688 2.68798286113
2.34544 2.69726767342
2.354 2.70656596826
2.36256 2.71587782107
2.37112 2.72520330927
2.37968 2.73454251228
2.38824 2.74389551157
2.3968 2.75326239066
2.40536 2.76264323518
2.41392 2.77203813283
2.42248 2.78144717349
2.43104 2.79087044916
2.4396 2.80030805406
2.44816 2.80976008461
2.45672 2.81922663947
2.46528 2.82870781959
2.47384 2.83820372821
2.4824 2.84771447091
2.49096 2.85724015565
2.49952 2.86678089276
2.50808 2.87633679503
2.51664 2.88590797773
2.5252 2.8954945586
2.53376 2.90509665797
2.54232 2.91471439871
2.55088 2.92434790633
2.55944 2.93399730901
2.568 2.94366273763
2.57656 2.95334432581
2.58512 2.96304220996
2.59368 2.97275652934
2.60224 2.98248742608
2.6108 2.99223504526
2.61936 3.00199953493
2.62792 3.01178104616
2.63648 3.02157973314
2.64504 3.03139575316
2.6536 3.04122926673
2.66216 3.0510804376
2.67072 3.06094943284
2.67928 3.07083642289
2.68784 3.08074158161
2.6964 3.09066508637
2.70496 3.10060711809
2.71352 3.11056786134
2.72208 3.12054750437
2.73064 3.1305462392
2.7392 3.14056426172
2.74776 3.15060177172
2.75632 3.16065897299
2.76488 3.17073607339
2.77344 3.18083328498
2.782 3.19095082402
2.79056 3.20108891113
2.79912 3.21124777135
2.80768 3.22142763424
2.81624 3.23162873397
2.8248 3.24185130941
2.83336 3.25209560426
2.84192 3.26236186713
2.85048 3.27265035166
2.85904 3.28296131661
2.8676 3.29329502602
2.87616 3.30365174926
2.88472 3.31403176121
2.89328 3.32443534238
2.90184 3.33486277898
2.9104 3.34531436314
2.91896 3.35579039298
2.92752 3.36629117278
2.93608 3.37681701313
2.94464 3.38736823104
2.9532 3.39794515018
2.96176 3.40854810093
2.97032 3.41917742066
2.97888 3.42983345379
2.98744 3.44051655207
2.996 3.45122707468
3.00456 3.46196538846
3.01312 3.47273186811
3.02168 3.48352689636
3.03024 3.49435086421
3.0388 3.50520417113
3.04736 3.51608722527
3.05592 3.52700044373
3.06448 3.53794425275
3.07304 3.54891908799
3.0816 3.55992539476
3.09016 3.57096362832
3.09872 3.58203425412
3.10728 3.59313774807
3.11584 3.60427459691
3.1244 3.6154452984
3.13296 3.62665036175
3.14152 3.63789030786
3.15008 3.6491656697
3.15864 3.66047699265
3.1672 3.67182483487
3.17576 3.68320976766
3.18432 3.6946323759
3.19288 3.70609325839
3.20144 3.71759302832
3.21 3.72913231369
3.21856 3.74071175779
3.22712 3.75233201965
3.23568 3.76399377453
3.24424 3.77569771446
3.2528 3.78744454876
3.26136 3.79923500459
3.26992 3.81106982754
3.27848 3.82294978223
3.28704 3.83487565293
3.2956 3.84684824422
3.30416 3.8588683817
3.31272 3.87093691263
3.32128 3.88305470676
3.32984 3.89522265703
3.3384 3.90744168045
3.34696 3.91971271888
3.35552 3.93203673994
3.36408 3.94441473794
3.37264 3.95684773484
3.3812 3.96933678126
3.38976 3.98188295752
3.39832 3.99448737477
3.40688 4.00715117613
3.41544 4.01987553791
3.424 4.03266167089
3.43256 4.04551082163
3.44112 4.05842427392
3.44968 4.07140335016
3.45824 4.08444941301
3.4668 4.09756386693
3.47536 4.11074815992
3.48392 4.12400378531
3.49248 4.13733228365
3.50104 4.15073524467
3.5096 4.1642143094
3.51816 4.17777117238
3.52672 4.19140758397
3.53528 4.20512535281
3.54384 4.2189263484
3.5524 4.23281250387
3.56096 4.24678581887
3.56952 4.26084836259
3.57808 4.27500227706
3.58664 4.28924978055
3.5952 4.30359317125
3.60376 4.31803483108
3.61232 4.33257722983
3.62088 4.34722292949
3.62944 4.36197458894
3.638 4.37683496878
3.64656 4.39180693667
3.65512 4.40689347286
3.66368 4.4220976762
3.67224 4.43742277045
3.6808 4.45287211113
3.68936 4.46844919278
3.69792 4.48415765671
3.70648 4.50000129938
3.71504 4.51598408132
3.7236 4.53211013675
3.73216 4.54838378386
3.74072 4.56480953593
3.74928 4.58139211329
3.75784 4.59813645618
3.7664 4.61504773867
3.77496 4.63213138369
3.78352 4.64939307928
3.79208 4.66683879624
3.80064 4.68447480722
3.8092 4.70230770751
3.81776 4.72034443759
3.82632 4.73859230782
3.83488 4.75705902524
3.84344 4.77575272297
3.852 4.79468199233
3.86056 4.8138559181
3.86912 4.83328411724
3.87768 4.8529767815
3.88624 4.87294472437
3.8948 4.89319943308
3.90336 4.91375312598
3.91192 4.93461881636
3.92048 4.95581038338
3.92904 4.97734265103
3.9376 4.99923147653
3.94616 5.02149384921
3.95472 5.04414800166
3.96328 5.0672135349
3.97184 5.09071155981
3.9804 5.11466485736
3.98896 5.1390980609
3.99752 5.164037864
4.00608 5.18951325857
4.01464 5.21555580849
4.0232 5.24219996552
4.03176 5.2694834354
4.04032 5.29744760431
4.04888 5.3261380378
4.05744 5.35560506781
4.066 5.38590448698
4.07456 5.41709837495
4.08312 5.44925608791
4.09168 5.48245545192
4.10024 5.51678421269
4.1088 5.55234181129
4.11736 5.58924157799
4.12592 5.62761346892
4.13448 5.66760751571
4.14304 5.70939822411
4.1516 5.75319025456
4.16016 5.79922586283
4.16872 5.84779480106
4.17728 5.89924772954
4.18584 5.95401475412
4.1944 6.01263164623
4.20296 6.07577793231
4.21152 6.14433397835
4.22008 6.21946976626
4.22864 6.30278925457
4.2372 6.39657838242
4.24576 6.50426177906
4.25432 6.63132393347
4.26288 6.78741494
4.27144 6.99214594989


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMean-lambda1.tex <==
0.0 0.484011655289
0.0069908289012 0.496075388345
0.0139816578024 0.508220129963
0.0209724867036 0.520448129349
0.0279633156048 0.532761738418
0.034954144506 0.545163418632
0.0419449734072 0.557655748446
0.0489358023084 0.570241431442
0.0559266312096 0.582923305208
0.0629174601108 0.595704351067
0.069908289012 0.608587704758
0.0768991179132 0.621576668172
0.0838899468144 0.634674722298
0.0908807757156 0.64788554152
0.0978716046168 0.661213009451
0.104862433518 0.674661236511
0.111853262419 0.688234579511
0.11884409132 0.701937663498
0.125834920222 0.715775406241
0.132825749123 0.729753045728
0.139816578024 0.74387617117
0.146807406925 0.758150758074
0.153798235826 0.772583208081
0.160789064728 0.787180394386
0.167779893629 0.801949713767
0.17477072253 0.816899146436
0.181761551431 0.832037325257
0.188752380332 0.847373616207
0.195743209234 0.862918212453
0.202734038135 0.878682245028
0.209724867036 0.894677913932
0.216715695937 0.910918644547
0.223706524838 0.927419275766
0.23069735374 0.944196288265
0.237688182641 0.961268084154
0.244679011542 0.978655333278
0.251669840443 0.996381407176
0.258660669344 1.01447293019
0.265651498246 1.03296048993
0.272642327147 1.05187956905
0.279633156048 1.07127179135
0.286623984949 1.09118662668
0.29361481385 1.11168378656
0.300605642752 1.13283669912
0.307596471653 1.15473774764
0.314587300554 1.17750655365
0.321578129455 1.20130389618
0.328568958356 1.22635706317
0.335559787258 1.25301151686
0.342550616159 1.28185574633


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMean-lambda1prob0pt5.tex <==
0.0 0.30685281944
0.013585684739 0.325743799658
0.0271713694779 0.344751622427
0.0407570542169 0.363880012679
0.0543427389559 0.383132874209
0.0679284236949 0.402514301906
0.0815141084338 0.422028595084
0.0950997931728 0.441680272047
0.108685477912 0.461474086033
0.122271162651 0.481415042708
0.13585684739 0.501508419375
0.149442532129 0.521759786148
0.163028216868 0.542175029313
0.176613901607 0.562760377176
0.190199586346 0.583522428734
0.203785271085 0.604468185558
0.217370955824 0.625605087344
0.230956640563 0.646941051661
0.244542325302 0.668484518548
0.258128010041 0.690244500687
0.271713694779 0.71223064005
0.285299379518 0.734453272104
0.298885064257 0.756923498825
0.312470748996 0.779653272107
0.326056433735 0.802655489433
0.339642118474 0.825944104133
0.353227803213 0.849534253094
0.366813487952 0.873442405463
0.380399172691 0.897686536804
0.39398485743 0.922286334343
0.407570542169 0.947263440483
0.421156226908 0.972641743855
0.434741911647 0.998447729991
0.448327596386 1.02471090755
0.461913281125 1.05146433145
0.475498965864 1.07874525177
0.489084650603 1.10659592845
0.502670335342 1.13506466776
0.516256020081 1.16420716097
0.52984170482 1.1940882433
0.543427389559 1.22478425063
0.557013074298 1.25638625014
0.570598759037 1.28900458861
0.584184443776 1.32277550276
0.597770128515 1.35787110428
0.611355813254 1.39451520002
0.624941497993 1.43300993132
0.638527182732 1.47378439486
0.652112867471 1.51749394376
0.66569855221 1.56526069445


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMean-lambda1prob0pt75.tex <==
0.0 0.537901879627
0.00563856862005 0.548358668405
0.0112771372401 0.558885674637
0.0169157058602 0.569484782273
0.0225542744802 0.580157960215
0.0281928431003 0.590907267935
0.0338314117203 0.6017348616
0.0394699803404 0.612643000739
0.0451085489604 0.62363405554
0.0507471175805 0.634710514833
0.0563856862005 0.645874994845
0.0620242548206 0.657130248832
0.0676628234407 0.66847917769
0.0733013920607 0.679924841663
0.0789399606808 0.691470473325
0.0845785293008 0.70311949197
0.0902170979209 0.714875519639
0.0958556665409 0.726742399005
0.101494235161 0.738724213399
0.107132803781 0.750825309292
0.112771372401 0.763050321646
0.118409941021 0.775404202571
0.124048509641 0.787892253862
0.129687078261 0.8005201641
0.135325646881 0.813294051105
0.140964215501 0.826220510785
0.146602784121 0.839306673589
0.152241352741 0.852560270109
0.157879921362 0.865989707757
0.163518489982 0.879604160944
0.169157058602 0.893413677841
0.174795627222 0.907429307724
0.180434195842 0.921663254074
0.186072764462 0.936129060267
0.191711333082 0.950841836979
0.197349901702 0.965818543673
0.202988470322 0.981078341196
0.208627038942 0.996643039388
0.214265607562 1.01253767389
0.219904176182 1.0287912623
0.225542744802 1.04543781503
0.231181313422 1.06251771773
0.236819882042 1.08007967307
0.242458450662 1.09818351603
0.248097019282 1.11690445637
0.253735587902 1.13633978374
0.259374156523 1.15662013038
0.265012725143 1.17792997499
0.270651293763 1.20054941002
0.276289862383 1.2249550274


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMean-lambda1prob0pt85.tex <==
0.0 0.665214120314
0.00318537101816 0.672346248907
0.00637074203631 0.679524479528
0.00955611305447 0.686749960165
0.0127414840726 0.694023889198
0.0159268550908 0.701347518684
0.0191122261089 0.708722157943
0.0222975971271 0.716149177451
0.0254829681453 0.723630013102
0.0286683391634 0.731166170867
0.0318537101816 0.738759231901
0.0350390811997 0.746410858159
0.0382244522179 0.75412279857
0.041409823236 0.761896895859
0.0445951942542 0.769735094096
0.0477805652723 0.777639447057
0.0509659362905 0.78561212754
0.0541513073087 0.793655437743
0.0573366783268 0.801771820881
0.060522049345 0.809963874222
0.0637074203631 0.818234363767
0.0668927913813 0.826586240846
0.0700781623994 0.835022660936
0.0732635334176 0.843547005107
0.0764489044358 0.852162904551
0.0796342754539 0.860874268776
0.0828196464721 0.869685318174
0.0860050174902 0.878600621835
0.0891903885084 0.887625141716
0.0923757595265 0.896764284551
0.0955611305447 0.906023963255
0.0987465015628 0.915410670123
0.101931872581 0.924931564762
0.105117243599 0.934594580664
0.108302614617 0.94440855563
0.111487985635 0.954383393077
0.114673356654 0.964530263962
0.117858727672 0.974861862909
0.12104409869 0.98539273803
0.124229469708 0.996139722952
0.127414840726 1.00712251394
0.130600211744 1.01836445855
0.133785582763 1.0298936625
0.136970953781 1.04174459327
0.140156324799 1.05396049464
0.143341695817 1.06659719987
0.146527066835 1.07972953153
0.149712437853 1.09346294299
0.152897808872 1.10795721286
0.15608317989 1.12348362781


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1.tex <==
0.0 0.484011655289
0.0069908289012 0.484011655289
0.0139816578024 0.484011655289
0.0209724867036 0.484011655289
0.0279633156048 0.484011655289
0.034954144506 0.484011655289
0.0419449734072 0.484011655289
0.0489358023084 0.484011655289
0.0559266312096 0.484011655289
0.0629174601108 0.484011655289
0.069908289012 0.489245099459
0.0768991179132 0.499502303469
0.0838899468144 0.509790905262
0.0908807757156 0.520111639781
0.0978716046168 0.530465293538
0.104862433518 0.540852709976
0.111853262419 0.551274795506
0.11884409132 0.561732526334
0.125834920222 0.572226956189
0.132825749123 0.58275922511
0.139816578024 0.593330569459
0.146807406925 0.603942333372
0.153798235826 0.614595981909
0.160789064728 0.625293116215
0.167779893629 0.636035491056
0.17477072253 0.646825035216
0.181761551431 0.657663875329
0.188752380332 0.668554363866
0.195743209234 0.679499112197
0.202734038135 0.690501029879
0.209724867036 0.701563371678
0.216715695937 0.712689794231
0.223706524838 0.723884424899
0.23069735374 0.735151946161
0.237688182641 0.746497700063
0.244679011542 0.757927818902
0.251669840443 0.769449390687
0.258660669344 0.781070671494
0.265651498246 0.792801362146
0.272642327147 0.80465297501
0.279633156048 0.816639329978
0.286623984949 0.828777240724
0.29361481385 0.841087490197
0.300605642752 0.85359626249
0.307596471653 0.866337328008
0.314587300554 0.879355542931
0.321578129455 0.892712808453
0.328568958356 0.906499077532
0.335559787258 0.920855123724
0.342550616159 0.936028467717


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1prob0pt5.tex <==
0.0 0.30685281944
0.013585684739 0.30685281944
0.0271713694779 0.30685281944
0.0407570542169 0.322826487276
0.0543427389559 0.340546682936
0.0679284236949 0.358330362932
0.0815141084338 0.376178593432
0.0950997931728 0.394092467349
0.108685477912 0.412073106348
0.122271162651 0.430121663125
0.13585684739 0.448239324032
0.149442532129 0.466427312083
0.163028216868 0.484686890418
0.176613901607 0.503019366299
0.190199586346 0.521426095727
0.203785271085 0.539908488785
0.217370955824 0.558468015845
0.230956640563 0.577106214781
0.244542325302 0.595824699386
0.258128010041 0.614625169198
0.271713694779 0.633509421015
0.285299379518 0.652479362425
0.298885064257 0.671537027735
0.312470748996 0.690684596808
0.326056433735 0.709924417382
0.339642118474 0.72925903164
0.353227803213 0.748691207952
0.366813487952 0.768223978954
0.380399172691 0.78786068747
0.39398485743 0.807605042155
0.407570542169 0.827461185327
0.421156226908 0.84743377618
0.434741911647 0.8675280936
0.448327596386 0.887750164196
0.461913281125 0.908106923179
0.475498965864 0.928606418501
0.489084650603 0.949258072849
0.502670335342 0.970073024171
0.516256020081 0.991064574785
0.52984170482 1.01224879363
0.543427389559 1.03364533969
0.557013074298 1.05527861339
0.570598759037 1.07717941024
0.584184443776 1.09938737266
0.597770128515 1.12195476909
0.611355813254 1.14495260686
0.624941497993 1.16848114782
0.638527182732 1.19268953575
0.652112867471 1.21781685047
0.66569855221 1.2442941738


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1prob0pt75.tex <==
0.0 0.537901879627
0.00563856862005 0.537901879627
0.0112771372401 0.537901879627
0.0169157058602 0.537901879627
0.0225542744802 0.537901879627
0.0281928431003 0.537901879627
0.0338314117203 0.537901879627
0.0394699803404 0.537901879627
0.0451085489604 0.537901879627
0.0507471175805 0.537901879627
0.0563856862005 0.537901879627
0.0620242548206 0.537901879627
0.0676628234407 0.537901879627
0.0733013920607 0.537901879627
0.0789399606808 0.537901879627
0.0845785293008 0.545256752409
0.0902170979209 0.553880075434
0.0958556665409 0.562532559225
0.101494235161 0.571215184589
0.107132803781 0.579929011551
0.112771372401 0.588675188118
0.118409941021 0.597454960273
0.124048509641 0.606269683424
0.129687078261 0.615120835553
0.135325646881 0.624010032395
0.140964215501 0.632939045046
0.146602784121 0.641909820472
0.152241352741 0.650924505546
0.157879921362 0.659985475369
0.163518489982 0.66909536685
0.169157058602 0.678257118798
0.174795627222 0.687474020133
0.180434195842 0.696749768345
0.186072764462 0.706088540988
0.191711333082 0.715495083989
0.197349901702 0.724974821912
0.202988470322 0.734533997285
0.208627038942 0.744179849052
0.214265607562 0.753920844631
0.219904176182 0.763766986937
0.225542744802 0.773730228715
0.231181313422 0.783825044678
0.236819882042 0.794069243112
0.242458450662 0.804485154723
0.248097019282 0.815101443038
0.253735587902 0.825955997306
0.259374156523 0.837100847465
0.265012725143 0.848611220123
0.270651293763 0.860604223466
0.276289862383 0.873284612311


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1prob0pt85.tex <==
0.0 0.665214120314
0.00318537101816 0.665214120314
0.00637074203631 0.665214120314
0.00955611305447 0.665214120314
0.0127414840726 0.665214120314
0.0159268550908 0.665214120314
0.0191122261089 0.665214120314
0.0222975971271 0.665214120314
0.0254829681453 0.665214120314
0.0286683391634 0.665214120314
0.0318537101816 0.665214120314
0.0350390811997 0.665214120314
0.0382244522179 0.665214120314
0.041409823236 0.665214120314
0.0445951942542 0.665214120314
0.0477805652723 0.665214120314
0.0509659362905 0.665214120314
0.0541513073087 0.665214120314
0.0573366783268 0.665214120314
0.060522049345 0.665214120314
0.0637074203631 0.665214120314
0.0668927913813 0.665214120314
0.0700781623994 0.665214120314
0.0732635334176 0.665214120314
0.0764489044358 0.665214120314
0.0796342754539 0.665214120314
0.0828196464721 0.665214120314
0.0860050174902 0.665214120314
0.0891903885084 0.665214120314
0.0923757595265 0.665214120314
0.0955611305447 0.665214120314
0.0987465015628 0.665214120314
0.101931872581 0.665214120314
0.105117243599 0.665214120314
0.108302614617 0.665214120314
0.111487985635 0.668597139454
0.114673356654 0.674455573811
0.117858727672 0.680373266856
0.12104409869 0.686355795245
0.124229469708 0.692409690705
0.127414840726 0.698542691075
0.130600211744 0.704764085607
0.133785582763 0.711085202796
0.136970953781 0.717520121989
0.140156324799 0.724086752371
0.143341695817 0.730808549421
0.146527066835 0.737717417545
0.149712437853 0.744859032021
0.152897808872 0.752303762103
0.15608317989 0.7601732722


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-leftEnd-lambda1.tex <==
0.0 0.0
0.0069908289012 0.0069908289012
0.0139816578024 0.0139816578024
0.0209724867036 0.0209724867036
0.0279633156048 0.0279633156048
0.034954144506 0.034954144506
0.0419449734072 0.0419449734072
0.0489358023084 0.0489358023084
0.0559266312096 0.0559266312096
0.0629174601108 0.0629174601108
0.069908289012 0.069908289012
0.0768991179132 0.0768991179132
0.0838899468144 0.0838899468144
0.0908807757156 0.0908807757156
0.0978716046168 0.0978716046168
0.104862433518 0.104862433518
0.111853262419 0.111853262419
0.11884409132 0.11884409132
0.125834920222 0.125834920222
0.132825749123 0.132825749123
0.139816578024 0.139816578024
0.146807406925 0.146807406925
0.153798235826 0.153798235826
0.160789064728 0.160789064728
0.167779893629 0.167779893629
0.17477072253 0.17477072253
0.181761551431 0.181761551431
0.188752380332 0.188752380332
0.195743209234 0.195743209234
0.202734038135 0.202734038135
0.209724867036 0.209724867036
0.216715695937 0.216715695937
0.223706524838 0.223706524838
0.23069735374 0.23069735374
0.237688182641 0.237688182641
0.244679011542 0.244679011542
0.251669840443 0.251669840443
0.258660669344 0.258660669344
0.265651498246 0.265651498246
0.272642327147 0.272642327147
0.279633156048 0.279633156048
0.286623984949 0.286623984949
0.29361481385 0.29361481385
0.300605642752 0.300605642752
0.307596471653 0.307596471653
0.314587300554 0.314587300554
0.321578129455 0.321578129455
0.328568958356 0.328568958356
0.335559787258 0.335559787258
0.342550616159 0.342550616159


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-leftEnd-lambda1prob0pt5.tex <==
0.0 0.0
0.013585684739 0.013585684739
0.0271713694779 0.0271713694779
0.0407570542169 0.0407570542169
0.0543427389559 0.0543427389559
0.0679284236949 0.0679284236949
0.0815141084338 0.0815141084338
0.0950997931728 0.0950997931728
0.108685477912 0.108685477912
0.122271162651 0.122271162651
0.13585684739 0.13585684739
0.149442532129 0.149442532129
0.163028216868 0.163028216868
0.176613901607 0.176613901607
0.190199586346 0.190199586346
0.203785271085 0.203785271085
0.217370955824 0.217370955824
0.230956640563 0.230956640563
0.244542325302 0.244542325302
0.258128010041 0.258128010041
0.271713694779 0.271713694779
0.285299379518 0.285299379518
0.298885064257 0.298885064257
0.312470748996 0.312470748996
0.326056433735 0.326056433735
0.339642118474 0.339642118474
0.353227803213 0.353227803213
0.366813487952 0.366813487952
0.380399172691 0.380399172691
0.39398485743 0.39398485743
0.407570542169 0.407570542169
0.421156226908 0.421156226908
0.434741911647 0.434741911647
0.448327596386 0.448327596386
0.461913281125 0.461913281125
0.475498965864 0.475498965864
0.489084650603 0.489084650603
0.502670335342 0.502670335342
0.516256020081 0.516256020081
0.52984170482 0.52984170482
0.543427389559 0.543427389559
0.557013074298 0.557013074298
0.570598759037 0.570598759037
0.584184443776 0.584184443776
0.597770128515 0.597770128515
0.611355813254 0.611355813254
0.624941497993 0.624941497993
0.638527182732 0.638527182732
0.652112867471 0.652112867471
0.66569855221 0.66569855221


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-leftEnd-lambda1prob0pt75.tex <==
0.0 0.0
0.00563856862005 0.00563856862005
0.0112771372401 0.0112771372401
0.0169157058602 0.0169157058602
0.0225542744802 0.0225542744802
0.0281928431003 0.0281928431003
0.0338314117203 0.0338314117203
0.0394699803404 0.0394699803404
0.0451085489604 0.0451085489604
0.0507471175805 0.0507471175805
0.0563856862005 0.0563856862005
0.0620242548206 0.0620242548206
0.0676628234407 0.0676628234407
0.0733013920607 0.0733013920607
0.0789399606808 0.0789399606808
0.0845785293008 0.0845785293008
0.0902170979209 0.0902170979209
0.0958556665409 0.0958556665409
0.101494235161 0.101494235161
0.107132803781 0.107132803781
0.112771372401 0.112771372401
0.118409941021 0.118409941021
0.124048509641 0.124048509641
0.129687078261 0.129687078261
0.135325646881 0.135325646881
0.140964215501 0.140964215501
0.146602784121 0.146602784121
0.152241352741 0.152241352741
0.157879921362 0.157879921362
0.163518489982 0.163518489982
0.169157058602 0.169157058602
0.174795627222 0.174795627222
0.180434195842 0.180434195842
0.186072764462 0.186072764462
0.191711333082 0.191711333082
0.197349901702 0.197349901702
0.202988470322 0.202988470322
0.208627038942 0.208627038942
0.214265607562 0.214265607562
0.219904176182 0.219904176182
0.225542744802 0.225542744802
0.231181313422 0.231181313422
0.236819882042 0.236819882042
0.242458450662 0.242458450662
0.248097019282 0.248097019282
0.253735587902 0.253735587902
0.259374156523 0.259374156523
0.265012725143 0.265012725143
0.270651293763 0.270651293763
0.276289862383 0.276289862383


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-leftEnd-lambda1prob0pt85.tex <==
0.0 0.0
0.00318537101816 0.00318537101816
0.00637074203631 0.00637074203631
0.00955611305447 0.00955611305447
0.0127414840726 0.0127414840726
0.0159268550908 0.0159268550908
0.0191122261089 0.0191122261089
0.0222975971271 0.0222975971271
0.0254829681453 0.0254829681453
0.0286683391634 0.0286683391634
0.0318537101816 0.0318537101816
0.0350390811997 0.0350390811997
0.0382244522179 0.0382244522179
0.041409823236 0.041409823236
0.0445951942542 0.0445951942542
0.0477805652723 0.0477805652723
0.0509659362905 0.0509659362905
0.0541513073087 0.0541513073087
0.0573366783268 0.0573366783268
0.060522049345 0.060522049345
0.0637074203631 0.0637074203631
0.0668927913813 0.0668927913813
0.0700781623994 0.0700781623994
0.0732635334176 0.0732635334176
0.0764489044358 0.0764489044358
0.0796342754539 0.0796342754539
0.0828196464721 0.0828196464721
0.0860050174902 0.0860050174902
0.0891903885084 0.0891903885084
0.0923757595265 0.0923757595265
0.0955611305447 0.0955611305447
0.0987465015628 0.0987465015628
0.101931872581 0.101931872581
0.105117243599 0.105117243599
0.108302614617 0.108302614617
0.111487985635 0.111487985635
0.114673356654 0.114673356654
0.117858727672 0.117858727672
0.12104409869 0.12104409869
0.124229469708 0.124229469708
0.127414840726 0.127414840726
0.130600211744 0.130600211744
0.133785582763 0.133785582763
0.136970953781 0.136970953781
0.140156324799 0.140156324799
0.143341695817 0.143341695817
0.146527066835 0.146527066835
0.149712437853 0.149712437853
0.152897808872 0.152897808872
0.15608317989 0.15608317989


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-midPoint-lambda1.tex <==
0.0 0.601986402163
0.0069908289012 0.61722949998
0.0139816578024 0.632670450647
0.0209724867036 0.648317493409
0.0279633156048 0.664179387773
0.034954144506 0.680265458256
0.0419449734072 0.696585644037
0.0489358023084 0.713150554195
0.0559266312096 0.729971529291
0.0629174601108 0.747060710197
0.069908289012 0.76443111521
0.0768991179132 0.78209672669
0.0838899468144 0.800072588659
0.0908807757156 0.818374917075
0.0978716046168 0.837021224803
0.104862433518 0.856030463704
0.111853262419 0.87542318673
0.11884409132 0.895221733515
0.125834920222 0.915450443643
0.132825749123 0.936135902742
0.139816578024 0.957307227617
0.146807406925 0.978996398125
0.153798235826 1.00123864529
0.160789064728 1.0240729075
0.167779893629 1.04754236962
0.17477072253 1.07169510388
0.181761551431 1.09658483627
0.188752380332 1.12227186952
0.195743209234 1.14882420231
0.202734038135 1.17631889721
0.209724867036 1.20484376681
0.216715695937 1.23449947111
0.223706524838 1.26540215269
0.23069735374 1.29768678435
0.237688182641 1.33151147339
0.244679011542 1.36706307071
0.251669840443 1.40456459023
0.258660669344 1.44428518828
0.265651498246 1.48655384218
0.272642327147 1.531778506
0.279633156048 1.58047360643
0.286623984949 1.63330065497
0.29361481385 1.69113028467
0.300605642752 1.7551408907
0.307596471653 1.82698330288
0.314587300554 1.90907285225
0.321578129455 2.00514912516
0.328568958356 2.12146535528
0.335559787258 2.26971137305
0.342550616159 2.47600583887


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-midPoint-lambda1prob0pt5.tex <==
0.0 0.34657359028
0.013585684739 0.367045675311
0.0271713694779 0.387710121052
0.0407570542169 0.408575160455
0.0543427389559 0.42964954685
0.0679284236949 0.450942598697
0.0815141084338 0.472464249234
0.0950997931728 0.494225101721
0.108685477912 0.516236491021
0.122271162651 0.538510552425
0.13585684739 0.561060298772
0.149442532129 0.583899707086
0.163028216868 0.607043816175
0.176613901607 0.630508836904
0.190199586346 0.654312277168
0.203785271085 0.678473083982
0.217370955824 0.703011805578
0.230956640563 0.727950776988
0.244542325302 0.753314333327
0.258128010041 0.779129055872
0.271713694779 0.805424057206
0.285299379518 0.832231313088
0.298885064257 0.859586050572
0.312470748996 0.887527204199
0.326056433735 0.916097955128
0.339642118474 0.945346371975
0.353227803213 0.975326177293
0.366813487952 1.00609767047
0.380399172691 1.03772884696
0.39398485743 1.07029676628
0.407570542169 1.10388923807
0.421156226908 1.13860691949
0.434741911647 1.17456595044
0.448327596386 1.21190130117
0.461913281125 1.25077107653
0.475498965864 1.29136212513
0.489084650603 1.33389745871
0.502670335342 1.37864623156
0.516256020081 1.42593741909
0.52984170482 1.4761789736
0.543427389559 1.52988532012
0.557013074298 1.58771796865
0.570598759037 1.65054755084
0.584184443776 1.7195524606
0.597770128515 1.79638352663
0.611355813254 1.88345607899
0.624941497993 1.98450970316
0.638527182732 2.10579763208
0.652112867471 2.2590096956
0.66569855221 2.47026455365


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-midPoint-lambda1prob0pt75.tex <==
0.0 0.69314718056
0.00563856862005 0.707340256107
0.0112771372401 0.72173188896
0.0169157058602 0.736330318642
0.0225542744802 0.75114430494
0.0281928431003 0.766183172637
0.0338314117203 0.781456861177
0.0394699803404 0.796975979898
0.0451085489604 0.812751869615
0.0507471175805 0.828796671446
0.0563856862005 0.845123403931
0.0620242548206 0.861746049666
0.0676628234407 0.878679652904
0.0733013920607 0.895940429827
0.0789399606808 0.913545893521
0.0845785293008 0.931514996059
0.0902170979209 0.949868290605
0.0958556665409 0.96862811699
0.101494235161 0.987818815
0.107132803781 1.00746697045
0.112771372401 1.02760170034
0.118409941021 1.04825498469
0.124048509641 1.06946205472
0.129687078261 1.09126184897
0.135325646881 1.11369755248
0.140964215501 1.13681723761
0.146602784121 1.16067463054
0.152241352741 1.18533003413
0.157879921362 1.21085144719
0.163518489982 1.23731593244
0.169157058602 1.26481130259
0.174795627222 1.29343821777
0.180434195842 1.32331282067
0.186072764462 1.3545700842
0.191711333082 1.38736811578
0.197349901702 1.4218937664
0.202988470322 1.45837005007
0.208627038942 1.49706612322
0.214265607562 1.53831096324
0.219904176182 1.5825125243
0.225542744802 1.63018523314
0.231181313422 1.68199060134
0.236819882042 1.738799262
0.242458450662 1.80178961035
0.248097019282 1.87261247625
0.253735587902 1.9536831908
0.259374156523 2.04874134039
0.265012725143 2.16404015869
0.270651293763 2.31126947619
0.276289862383 2.51654795332


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-midPoint-lambda1prob0pt85.tex <==
0.0 0.948559992443
0.00318537101816 0.960867683898
0.00637074203631 0.973374829895
0.00955611305447 0.986089670144
0.0127414840726 0.999020964612
0.0159268550908 1.01217803826
0.0191122261089 1.02557083072
0.0222975971271 1.03920995148
0.0254829681453 1.05310674154
0.0286683391634 1.06727334217
0.0318537101816 1.08172277207
0.0350390811997 1.09646901401
0.0382244522179 1.11152711237
0.041409823236 1.1269132835
0.0445951942542 1.14264504062
0.0477805652723 1.15874133596
0.0509659362905 1.1752227228
0.0541513073087 1.19211154112
0.0573366783268 1.20943213083
0.060522049345 1.22721107788
0.0637074203631 1.24547749938
0.0668927913813 1.26426337548
0.0700781623994 1.2836039375
0.0732635334176 1.3035381241
0.0764489044358 1.32410912044
0.0796342754539 1.34536499897
0.0828196464721 1.36735948598
0.0860050174902 1.39015288441
0.0891903885084 1.41381319317
0.0923757595265 1.43841747507
0.0955611305447 1.46405354292
0.0987465015628 1.4908220569
0.101931872581 1.5188391598
0.105117243599 1.54823982461
0.108302614617 1.57918215879
0.111487985635 1.61185301343
0.114673356654 1.64647540259
0.117858727672 1.68331848274
0.12104409869 1.72271123135
0.124229469708 1.76506160263
0.127414840726 1.81088402337
0.130600211744 1.86084000519
0.133785582763 1.91580018124
0.136970953781 1.97694294677
0.140156324799 2.04591913169
0.143341695817 2.12514406711
0.146527066835 2.21835733945
0.149712437853 2.33181218242
0.152897808872 2.47719842651
0.15608317989 2.68063473215


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-rightEnd-lambda1.tex <==
0.0 1.20397280433
0.0069908289012 1.22746817106
0.0139816578024 1.25135924349
0.0209724867036 1.27566250011
0.0279633156048 1.30039545994
0.034954144506 1.32557677201
0.0419449734072 1.35122631467
0.0489358023084 1.37736530608
0.0559266312096 1.40401642737
0.0629174601108 1.43120396028
0.069908289012 1.45895394141
0.0768991179132 1.48729433547
0.0838899468144 1.5162552305
0.0908807757156 1.54586905844
0.0978716046168 1.57617084499
0.104862433518 1.60719849389
0.111853262419 1.63899311104
0.11884409132 1.67159937571
0.125834920222 1.70506596706
0.132825749123 1.73944605636
0.139816578024 1.77479787721
0.146807406925 1.81118538933
0.153798235826 1.84867905475
0.160789064728 1.88735675027
0.167779893629 1.92730484562
0.17477072253 1.96861948522
0.181761551431 2.01140812111
0.188752380332 2.05579135871
0.195743209234 2.10190519538
0.202734038135 2.14990375628
0.209724867036 2.19996266659
0.216715695937 2.25228324628
0.223706524838 2.30709778054
0.23069735374 2.36467621496
0.237688182641 2.42533476414
0.244679011542 2.48944712989
0.251669840443 2.55745934003
0.258660669344 2.62990970722
0.265651498246 2.70745618611
0.272642327147 2.79091468486
0.279633156048 2.8813140568
0.286623984949 2.97997732499
0.29361481385 3.08864575549
0.300605642752 3.20967613865
0.307596471653 3.3463701341
0.314587300554 3.50355840394
0.321578129455 3.68872012087
0.328568958356 3.91436175221
0.335559787258 4.20386295884
0.342550616159 4.60946106158


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-rightEnd-lambda1prob0pt5.tex <==
0.0 0.69314718056
0.013585684739 0.720505665882
0.0271713694779 0.748248872626
0.0407570542169 0.776393266692
0.0543427389559 0.804956354745
0.0679284236949 0.833956773698
0.0815141084338 0.863414390034
0.0950997931728 0.893350410269
0.108685477912 0.92378750413
0.122271162651 0.954749942198
0.13585684739 0.986263750154
0.149442532129 1.01835688204
0.163028216868 1.05105941548
0.176613901607 1.0844037722
0.190199586346 1.11842496799
0.203785271085 1.15316089688
0.217370955824 1.18865265533
0.230956640563 1.22494491341
0.244542325302 1.26208634135
0.258128010041 1.3001301017
0.271713694779 1.33913441963
0.285299379518 1.37916324666
0.298885064257 1.42028703689
0.312470748996 1.4625836594
0.326056433735 1.50613947652
0.339642118474 1.55105062548
0.353227803213 1.59742455137
0.366813487952 1.64538185298
0.380399172691 1.69505852123
0.39398485743 1.74660867513
0.407570542169 1.80020793397
0.421156226908 1.85605761207
0.434741911647 1.91438998924
0.448327596386 1.97547500595
0.461913281125 2.03962887193
0.475498965864 2.10722528439
0.489084650603 2.17871026681
0.502670335342 2.25462212778
0.516256020081 2.3356188181
0.52984170482 2.42251624239
0.543427389559 2.51634325069
0.557013074298 2.618422863
0.570598759037 2.73049634264
0.584184443776 2.85492047742
0.597770128515 2.99499692475
0.611355813254 3.15555634472
0.624941497993 3.34407790833
0.638527182732 3.57306808143
0.652112867471 3.86590652372
0.66569855221 4.27483055509


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-rightEnd-lambda1prob0pt75.tex <==
0.0 1.38629436112
0.00563856862005 1.40904194359
0.0112771372401 1.43218664068
0.0169157058602 1.45574493142
0.0225542744802 1.4797343354
0.0281928431003 1.50417350217
0.0338314117203 1.52908231063
0.0394699803404 1.55448197946
0.0451085489604 1.58039519027
0.0507471175805 1.60684622531
0.0563856862005 1.63386112166
0.0620242548206 1.66146784451
0.0676628234407 1.68969648237
0.0733013920607 1.71857946759
0.0789399606808 1.74815182636
0.0845785293008 1.77845146282
0.0902170979209 1.80951948329
0.0958556665409 1.84140056744
0.101494235161 1.87414339484
0.107132803781 1.90780113712
0.112771372401 1.94243202828
0.118409941021 1.97810002837
0.124048509641 2.0148755998
0.129687078261 2.05283661967
0.135325646881 2.09206945807
0.140964215501 2.13267025972
0.146602784121 2.17474647696
0.152241352741 2.21841871552
0.157879921362 2.26382297302
0.163518489982 2.31111337489
0.169157058602 2.36046554659
0.174795627222 2.41208080831
0.180434195842 2.46619144549
0.186072764462 2.52306740394
0.191711333082 2.58302489847
0.197349901702 2.6464376311
0.202988470322 2.71375162982
0.208627038942 2.7855052075
0.214265607562 2.86235631892
0.219904176182 2.94512087242
0.225542744802 3.03482772147
0.231181313422 3.13279988925
0.236819882042 3.24077864196
0.242458450662 3.36112077004
0.248097019282 3.49712793323
0.253735587902 3.6536307937
0.259374156523 3.83810852425
0.265012725143 4.06306759224
0.270651293763 4.35188765863
0.276289862383 4.75680604425


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForSingleLaplace-rightEnd-lambda1prob0pt85.tex <==
0.0 1.89711998489
0.00318537101816 1.91854999678
0.00637074203631 1.94037891775
0.00955611305447 1.96262322723
0.0127414840726 1.98530044515
0.0159268550908 2.00842922144
0.0191122261089 2.03202943532
0.0222975971271 2.05612230583
0.0254829681453 2.08073051493
0.0286683391634 2.10587834517
0.0318537101816 2.13159183396
0.0350390811997 2.15789894681
0.0382244522179 2.18482977252
0.041409823236 2.21241674377
0.0445951942542 2.24069488699
0.0477805652723 2.26970210664
0.0509659362905 2.29947950931
0.0541513073087 2.33007177493
0.0573366783268 2.36152758334
0.060522049345 2.39390010642
0.0637074203631 2.42724757839
0.0668927913813 2.46163395958
0.0700781623994 2.4971297126
0.0732635334176 2.53381271479
0.0764489044358 2.57176933644
0.0796342754539 2.61109572249
0.0828196464721 2.65189932548
0.0860050174902 2.69430075132
0.0891903885084 2.73843599783
0.0923757595265 2.78445919062
0.0955611305447 2.83254595529
0.0987465015628 2.88289761224
0.101931872581 2.93574644702
0.105117243599 2.99136240562
0.108302614617 3.05006170297
0.111487985635 3.11221804122
0.114673356654 3.17827744852
0.117858727672 3.24877823781
0.12104409869 3.32437836401
0.124229469708 3.40589373555
0.127414840726 3.49435320601
0.130600211744 3.59107979863
0.133785582763 3.69781477971
0.136970953781 3.81691493976
0.140156324799 3.95168193858
0.143341695817 4.1069464384
0.146527066835 4.29018761207
0.149712437853 4.51391192699
0.152897808872 4.80149904414
0.15608317989 5.20518628441


==> centered-silence-sets scalar-log-concave/figuresAndData/dataForUniformSigma1.tex <==
0.998 4e-06
0.996 1.6e-05
0.994 3.6e-05
0.992 6.4e-05
0.99 0.0001
0.988 0.000144
0.986 0.000196
0.984 0.000256
0.982 0.000324
0.98 0.0004
0.978 0.000484
0.976 0.000576
0.974 0.000676
0.972 0.000784
0.97 0.0009
0.968 0.001024
0.966 0.001156
0.964 0.001296
0.962 0.001444
0.96 0.0016
0.958 0.001764
0.956 0.001936
0.954 0.002116
0.952 0.002304
0.95 0.0025
0.948 0.002704
0.946 0.002916
0.944 0.003136
0.942 0.003364
0.94 0.0036
0.938 0.003844
0.936 0.004096
0.934 0.004356
0.932 0.004624
0.93 0.0049
0.928 0.005184
0.926 0.005476
0.924 0.005776
0.922 0.006084
0.92 0.0064
0.918 0.006724
0.916 0.007056
0.914 0.007396
0.912 0.007744
0.91 0.0081
0.908 0.008464
0.906 0.008836
0.904 0.009216
0.902 0.009604
0.9 0.01
0.898 0.010404
0.896 0.010816
0.894 0.011236
0.892 0.011664
0.89 0.0121
0.888 0.012544
0.886 0.012996
0.884 0.013456
0.882 0.013924
0.88 0.0144
0.878 0.014884
0.876 0.015376
0.874 0.015876
0.872 0.016384
0.87 0.0169
0.868 0.017424
0.866 0.017956
0.864 0.018496
0.862 0.019044
0.86 0.0196
0.858 0.020164
0.856 0.020736
0.854 0.021316
0.852 0.021904
0.85 0.0225
0.848 0.023104
0.846 0.023716
0.844 0.024336
0.842 0.024964
0.84 0.0256
0.838 0.026244
0.836 0.026896
0.834 0.027556
0.832 0.028224
0.83 0.0289
0.828 0.029584
0.826 0.030276
0.824 0.030976
0.822 0.031684
0.82 0.0324
0.818 0.033124
0.816 0.033856
0.814 0.034596
0.812 0.035344
0.81 0.0361
0.808 0.036864
0.806 0.037636
0.804 0.038416
0.802 0.039204
0.8 0.04
0.798 0.040804
0.796 0.041616
0.794 0.042436
0.792 0.043264
0.79 0.0441
0.788 0.044944
0.786 0.045796
0.784 0.046656
0.782 0.047524
0.78 0.0484
0.778 0.049284
0.776 0.050176
0.774 0.051076
0.772 0.051984
0.77 0.0529
0.768 0.053824
0.766 0.054756
0.764 0.055696
0.762 0.056644
0.76 0.0576
0.758 0.058564
0.756 0.059536
0.754 0.060516
0.752 0.061504
0.75 0.0625
0.748 0.063504
0.746 0.064516
0.744 0.065536
0.742 0.066564
0.74 0.0676
0.738 0.068644
0.736 0.069696
0.734 0.070756
0.732 0.071824
0.73 0.0729
0.728 0.073984
0.726 0.075076
0.724 0.076176
0.722 0.077284
0.72 0.0784
0.718 0.079524
0.716 0.080656
0.714 0.081796
0.712 0.082944
0.71 0.0841
0.708 0.085264
0.706 0.086436
0.704 0.087616
0.702 0.088804
0.7 0.09
0.698 0.091204
0.696 0.092416
0.694 0.093636
0.692 0.094864
0.69 0.0961
0.688 0.097344
0.686 0.098596
0.684 0.099856
0.682 0.101124
0.68 0.1024
0.678 0.103684
0.676 0.104976
0.674 0.106276
0.672 0.107584
0.67 0.1089
0.668 0.110224
0.666 0.111556
0.664 0.112896
0.662 0.114244
0.66 0.1156
0.658 0.116964
0.656 0.118336
0.654 0.119716
0.652 0.121104
0.65 0.1225
0.648 0.123904
0.646 0.125316
0.644 0.126736
0.642 0.128164
0.64 0.1296
0.638 0.131044
0.636 0.132496
0.634 0.133956
0.632 0.135424
0.63 0.1369
0.628 0.138384
0.626 0.139876
0.624 0.141376
0.622 0.142884
0.62 0.1444
0.618 0.145924
0.616 0.147456
0.614 0.148996
0.612 0.150544
0.61 0.1521
0.608 0.153664
0.606 0.155236
0.604 0.156816
0.602 0.158404
0.6 0.16
0.598 0.161604
0.596 0.163216
0.594 0.164836
0.592 0.166464
0.59 0.1681
0.588 0.169744
0.586 0.171396
0.584 0.173056
0.582 0.174724
0.58 0.1764
0.578 0.178084
0.576 0.179776
0.574 0.181476
0.572 0.183184
0.57 0.1849
0.568 0.186624
0.566 0.188356
0.564 0.190096
0.562 0.191844
0.56 0.1936
0.558 0.195364
0.556 0.197136
0.554 0.198916
0.552 0.200704
0.55 0.2025
0.548 0.204304
0.546 0.206116
0.544 0.207936
0.542 0.209764
0.54 0.2116
0.538 0.213444
0.536 0.215296
0.534 0.217156
0.532 0.219024
0.53 0.2209
0.528 0.222784
0.526 0.224676
0.524 0.226576
0.522 0.228484
0.52 0.2304
0.518 0.232324
0.516 0.234256
0.514 0.236196
0.512 0.238144
0.51 0.2401
0.508 0.242064
0.506 0.244036
0.504 0.246016
0.502 0.248004
0.5 0.25
0.498 0.252004
0.496 0.254016
0.494 0.256036
0.492 0.258064
0.49 0.2601
0.488 0.262144
0.486 0.264196
0.484 0.266256
0.482 0.268324
0.48 0.2704
0.478 0.272484
0.476 0.274576
0.474 0.276676
0.472 0.278784
0.47 0.2809
0.468 0.283024
0.466 0.285156
0.464 0.287296
0.462 0.289444
0.46 0.2916
0.458 0.293764
0.456 0.295936
0.454 0.298116
0.452 0.300304
0.45 0.3025
0.448 0.304704
0.446 0.306916
0.444 0.309136
0.442 0.311364
0.44 0.3136
0.438 0.315844
0.436 0.318096
0.434 0.320356
0.432 0.322624
0.43 0.3249
0.428 0.327184
0.426 0.329476
0.424 0.331776
0.422 0.334084
0.42 0.3364
0.418 0.338724
0.416 0.341056
0.414 0.343396
0.412 0.345744
0.41 0.3481
0.408 0.350464
0.406 0.352836
0.404 0.355216
0.402 0.357604
0.4 0.36
0.398 0.362404
0.396 0.364816
0.394 0.367236
0.392 0.369664
0.39 0.3721
0.388 0.374544
0.386 0.376996
0.384 0.379456
0.382 0.381924
0.38 0.3844
0.378 0.386884
0.376 0.389376
0.374 0.391876
0.372 0.394384
0.37 0.3969
0.368 0.399424
0.366 0.401956
0.364 0.404496
0.362 0.407044
0.36 0.4096
0.358 0.412164
0.356 0.414736
0.354 0.417316
0.352 0.419904
0.35 0.4225
0.348 0.425104
0.346 0.427716
0.344 0.430336
0.342 0.432964
0.34 0.4356
0.338 0.438244
0.336 0.440896
0.334 0.443556
0.332 0.446224
0.33 0.4489
0.328 0.451584
0.326 0.454276
0.324 0.456976
0.322 0.459684
0.32 0.4624
0.318 0.465124
0.316 0.467856
0.314 0.470596
0.312 0.473344
0.31 0.4761
0.308 0.478864
0.306 0.481636
0.304 0.484416
0.302 0.487204
0.3 0.49
0.298 0.492804
0.296 0.495616
0.294 0.498436
0.292 0.501264
0.29 0.5041
0.288 0.506944
0.286 0.509796
0.284 0.512656
0.282 0.515524
0.28 0.5184
0.278 0.521284
0.276 0.524176
0.274 0.527076
0.272 0.529984
0.27 0.5329
0.268 0.535824
0.266 0.538756
0.264 0.541696
0.262 0.544644
0.26 0.5476
0.258 0.550564
0.256 0.553536
0.254 0.556516
0.252 0.559504
0.25 0.5625
0.248 0.565504
0.246 0.568516
0.244 0.571536
0.242 0.574564
0.24 0.5776
0.238 0.580644
0.236 0.583696
0.234 0.586756
0.232 0.589824
0.23 0.5929
0.228 0.595984
0.226 0.599076
0.224 0.602176
0.222 0.605284
0.22 0.6084
0.218 0.611524
0.216 0.614656
0.214 0.617796
0.212 0.620944
0.21 0.6241
0.208 0.627264
0.206 0.630436
0.204 0.633616
0.202 0.636804
0.2 0.64
0.198 0.643204
0.196 0.646416
0.194 0.649636
0.192 0.652864
0.19 0.6561
0.188 0.659344
0.186 0.662596
0.184 0.665856
0.182 0.669124
0.18 0.6724
0.178 0.675684
0.176 0.678976
0.174 0.682276
0.172 0.685584
0.17 0.6889
0.168 0.692224
0.166 0.695556
0.164 0.698896
0.162 0.702244
0.16 0.7056
0.158 0.708964
0.156 0.712336
0.154 0.715716
0.152 0.719104
0.15 0.7225
0.148 0.725904
0.146 0.729316
0.144 0.732736
0.142 0.736164
0.14 0.7396
0.138 0.743044
0.136 0.746496
0.134 0.749956
0.132 0.753424
0.13 0.7569
0.128 0.760384
0.126 0.763876
0.124 0.767376
0.122 0.770884
0.12 0.7744
0.118 0.777924
0.116 0.781456
0.114 0.784996
0.112 0.788544
0.11 0.7921
0.108 0.795664
0.106 0.799236
0.104 0.802816
0.102 0.806404
0.1 0.81
0.098 0.813604
0.096 0.817216
0.094 0.820836
0.092 0.824464
0.09 0.8281
0.088 0.831744
0.086 0.835396
0.084 0.839056
0.082 0.842724
0.08 0.8464
0.078 0.850084
0.076 0.853776
0.074 0.857476
0.072 0.861184
0.07 0.8649
0.068 0.868624
0.066 0.872356
0.064 0.876096
0.062 0.879844
0.06 0.8836
0.058 0.887364
0.056 0.891136
0.054 0.894916
0.052 0.898704
0.05 0.9025
0.048 0.906304
0.046 0.910116
0.044 0.913936
0.042 0.917764
0.04 0.9216
0.038 0.925444
0.036 0.929296
0.034 0.933156
0.032 0.937024
0.03 0.9409
0.028 0.944784
0.026 0.948676
0.024 0.952576
0.022 0.956484
0.02 0.9604
0.018 0.964324
0.016 0.968256
0.014 0.972196
0.012 0.976144
0.01 0.9801
0.008 0.984064
0.006 0.988036
0.004 0.992016
0.002 0.996004


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5MeanZero.tex <==
-0.5 0.0357096718032
-0.49501 0.0356957014811
-0.49002 0.035654141861
-0.48503 0.0355833107285
-0.48004 0.0354868727149
-0.47505 0.0353657503028
-0.47006 0.0352208407726
-0.46507 0.035050480076
-0.46008 0.0348606258829
-0.45509 0.0346470654179
-0.4501 0.0344131475513
-0.44511 0.0341596645629
-0.44012 0.0338873907074
-0.43513 0.0335970831281
-0.43014 0.0332894827051
-0.42515 0.0329653148425
-0.42016 0.0326252901998
-0.41517 0.0322701053713
-0.41018 0.0319004435171
-0.40519 0.0315191081323
-0.4002 0.0311224550134
-0.39521 0.0307132991706
-0.39022 0.0302943005252
-0.38523 0.0298619965793
-0.38024 0.0294210141005
-0.37525 0.0289699310506
-0.37026 0.0285093407334
-0.36527 0.0280398271148
-0.36028 0.027561965127
-0.35529 0.0270780877172
-0.3503 0.0265851817304
-0.34531 0.026087292803
-0.34032 0.0255831955046
-0.33533 0.0250750409994
-0.33034 0.0245600828864
-0.32535 0.0240420377708
-0.32036 0.0235197997076
-0.31537 0.0229953420706
-0.31038 0.0224676198838
-0.30539 0.0219371245321
-0.3004 0.0214043408729
-0.29541 0.0208710688198
-0.29042 0.0203363860774
-0.28543 0.019800759024
-0.28044 0.0192646479418
-0.27545 0.0187296839708
-0.27046 0.0181962086045
-0.26547 0.0176623469261
-0.26048 0.0171307841004
-0.25549 0.016601847343
-0.2505 0.0160748582496
-0.24551 0.0155502388288
-0.24052 0.0150293393468
-0.23553 0.0145115700257
-0.23054 0.013997337362
-0.22555 0.0134878770113
-0.22056 0.0129826853741
-0.21557 0.0124829243033
-0.21058 0.0119881464314
-0.20559 0.0114994417478
-0.2006 0.0110164176686
-0.19561 0.0105400943439
-0.19062 0.0100701323706
-0.18563 0.00960689513739
-0.18064 0.00915186176945
-0.17565 0.00870361946153
-0.17066 0.0082636113945
-0.16567 0.0078321006529
-0.16068 0.0074088962756
-0.15569 0.00699433455055
-0.1507 0.00658914782242
-0.14571 0.00619358832894
-0.14072 0.00580755339879
-0.13573 0.0054316915739
-0.13074 0.0050659407226
-0.12575 0.00471089622214
-0.12076 0.00436653390563
-0.11577 0.00403339873151
-0.11078 0.0037117266427
-0.10579 0.00340154641113
-0.1008 0.00310314608086
-0.09581 0.00281714874658
-0.09082 0.00254342382787
-0.08583 0.00228224692999
-0.08084 0.0020340107241
-0.07585 0.00179893652876
-0.07086 0.0015771495973
-0.06587 0.0013689897389
-0.06088 0.00117460230049
-0.05589 0.000994295151312
-0.0509 0.000828280214379
-0.04591 0.000676727912836
-0.04092 0.000539905899612
-0.03593 0.000418021213985
-0.03094 0.000311261505507
-0.02595 0.00021986221305
-0.02096 0.000144017004764
-0.01597 8.39485205566e-05
-0.01098 3.98423138112e-05
-0.00599 1.1904058059e-05


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt2.tex <==
-0.5 0.0111111111111
-0.497763932023 0.0111094665008
-0.495527864045 0.011104619582
-0.493291796068 0.0110966978116
-0.49105572809 0.011085824842
-0.488819660113 0.0110721206167
-0.486583592135 0.011055701463
-0.484347524158 0.0110366801833
-0.48211145618 0.011015166145
-0.479875388203 0.0109912653673
-0.477639320225 0.0109650806076
-0.475403252248 0.0109367114452
-0.47316718427 0.0109062543632
-0.470931116293 0.0108738028296
-0.468695048315 0.0108394473754
-0.466458980338 0.010803275672
-0.46422291236 0.0107653726066
-0.461986844383 0.0107258203555
-0.459750776405 0.0106846984571
-0.457514708428 0.0106420838814
-0.45527864045 0.0105980511
-0.453042572473 0.0105526721529
-0.450806504495 0.0105060167145
-0.448570436518 0.0104581521585
-0.44633436854 0.0104091436204
-0.444098300563 0.0103590540593
-0.441862232585 0.0103079443181
-0.439626164608 0.0102558731822
-0.43739009663 0.0102028974369
-0.435154028653 0.0101490719235
-0.432917960675 0.0100944495938
-0.430681892698 0.010039081564
-0.42844582472 0.0099830171667
-0.426209756743 0.00992630400159
-0.423973688765 0.0098689879855
-0.421737620788 0.00981111340076
-0.41950155281 0.00975272294256
-0.417265484833 0.00969385776513
-0.415029416855 0.0096345575268
-0.412793348878 0.00957486043391
-0.4105572809 0.00951480328367
-0.408321212923 0.00945442150592
-0.406085144945 0.00939374920388
-0.403849076968 0.00933281919382
-0.40161300899 0.00927166304374
-0.399376941013 0.00921031111111
-0.397140873035 0.0091487925796
-0.394904805058 0.00908713549483
-0.39266873708 0.00902536679928
-0.390432669103 0.00896351236622
-0.388196601125 0.00890159703279
-0.385960533148 0.00883964463219
-0.38372446517 0.00877767802503
-0.381488397193 0.00871571912982
-0.379252329215 0.00865378895273
-0.377016261238 0.00859190761641
-0.37478019326 0.00853009438819
-0.372544125283 0.00846836770737
-0.370308057305 0.00840674521192
-0.368071989328 0.00834524376427
-0.36583592135 0.00828387947657
-0.363599853373 0.00822266773514
-0.361363785395 0.00816162322424
-0.359127717418 0.00810075994926
-0.35689164944 0.00804009125921
-0.354655581463 0.00797962986851
-0.352419513485 0.0079193878783
-0.350183445508 0.00785937679707
-0.34794737753 0.00779960756066
-0.345711309553 0.00774009055178
-0.343475241575 0.0076808356189
-0.341239173598 0.00762185209462
-0.33900310562 0.00756314881351
-0.336767037643 0.0075047341294
-0.334530969665 0.00744661593221
-0.332294901688 0.00738880166424
-0.33005883371 0.00733129833601
-0.327822765733 0.00727411254161
-0.325586697755 0.00721725047359
-0.323350629778 0.00716071793744
-0.3211145618 0.00710452036557
-0.318878493823 0.00704866283093
-0.316642425845 0.00699315006018
-0.314406357868 0.00693798644648
-0.31217028989 0.00688317606185
-0.309934221913 0.00682872266922
-0.307698153935 0.00677462973403
-0.305462085958 0.0067209004355
-0.30322601798 0.00666753767759
-0.300989950003 0.00661454409956
-0.298753882025 0.00656192208619
-0.296517814048 0.00650967377777
-0.29428174607 0.00645780107966
-0.292045678093 0.00640630567159
-0.289809610115 0.00635518901673
-0.287573542138 0.00630445237032
-0.28533747416 0.00625409678818
-0.283101406183 0.00620412313482
-0.280865338205 0.00615453209139
-0.278629270228 0.00610532416327
-0.27639320225 0.0060564996875
-0.273629270228 0.00599668050619
-0.270865338205 0.00593745368025
-0.268101406183 0.00587882534014
-0.26533747416 0.00582080154918
-0.262573542138 0.00576338831695
-0.259809610115 0.00570659161176
-0.257045678093 0.00565041737206
-0.25428174607 0.00559487151696
-0.251517814048 0.0055399599558
-0.248753882025 0.0054856885968
-0.245989950003 0.00543206335492
-0.24322601798 0.00537909015881
-0.240462085958 0.00532677495699
-0.237698153935 0.00527512372325
-0.234934221913 0.00522414246127
-0.23217028989 0.00517383720853
-0.229406357868 0.0051242140395
-0.226642425845 0.00507527906813
-0.223878493823 0.0050270384497
-0.2211145618 0.00497949838199
-0.218350629778 0.00493266510588
-0.215586697755 0.00488654490525
-0.212822765733 0.00484114410638
-0.21005883371 0.00479646907672
-0.207294901688 0.00475252622311
-0.204530969665 0.00470932198941
-0.201767037643 0.00466686285373
-0.19900310562 0.00462515532492
-0.196239173598 0.00458420593875
-0.193475241575 0.00454402125347
-0.190711309553 0.00450460784488
-0.18794737753 0.00446597230091
-0.185183445508 0.0044281212158
-0.182419513485 0.00439106118361
-0.179655581463 0.00435479879143
-0.17689164944 0.00431934061204
-0.174127717418 0.00428469319601
-0.171363785395 0.00425086306345
-0.168599853373 0.0042178566952
-0.16583592135 0.00418568052351
-0.163071989328 0.00415434092226
-0.160308057305 0.00412384419666
-0.157544125283 0.00409419657242
-0.15478019326 0.00406540418441
-0.152016261238 0.00403747306476
-0.149252329215 0.00401040913042
-0.146488397193 0.00398421817016
-0.14372446517 0.00395890583091
-0.140960533148 0.00393447760356
-0.138196601125 0.00391093880813
-0.135432669103 0.00388829457823
-0.13266873708 0.00386654984485
-0.129904805058 0.0038457093195
-0.127140873035 0.00382577747652
-0.124376941013 0.00380675853468
-0.12161300899 0.00378865643795
-0.118849076968 0.00377147483545
-0.116085144945 0.00375521706045
-0.113321212923 0.00373988610856
-0.1105572809 0.00372548461483
-0.107793348878 0.00371201482994
-0.105029416855 0.00369947859528
-0.102265484833 0.00368787731692
-0.09950155281 0.00367721193841
-0.0967376207875 0.00366748291238
-0.093973688765 0.00365869017089
-0.0912097567425 0.0036508330943
-0.08844582472 0.00364391047894
-0.0856818926975 0.0036379205031
-0.082917960675 0.00363286069162
-0.0801540286525 0.00362872787879
-0.07739009663 0.00362551816955
-0.0746261646075 0.00362322689894
-0.071862232585 0.00362184858964
-0.0690983005625 0.00362137690761
-0.06633436854 0.00362180461564
-0.0635704365175 0.00362312352478
-0.060806504495 0.00362532444348
-0.0580425724725 0.00362839712448
-0.05527864045 0.00363233020915
-0.0525147084275 0.00363711116929
-0.049750776405 0.00364272624627
-0.0469868443825 0.00364916038733
-0.04422291236 0.00365639717898
-0.0414589803375 0.00366441877727
-0.038695048315 0.00367320583493
-0.0359311162925 0.00368273742514
-0.03316718427 0.00369299096179
-0.0304032522475 0.00370394211608
-0.027639320225 0.0037155647294
-0.0248753882025 0.00372783072212
-0.02211145618 0.00374070999836
-0.0193475241575 0.00375417034632
-0.016583592135 0.00376817733423
-0.0138196601125 0.00378269420152
-0.01105572809 0.00379768174511
-0.0082917960675 0.00381309820066
-0.005527864045 0.00382889911843
-0.0027639320225 0.00384503723367
0.0 0.00386146233122
0.00725403330759 0.00390529001642
0.0145080666152 0.00394990838629
0.0217620999228 0.0039953375494
0.0290161332303 0.00404159828771
0.0362701665379 0.00408871208499
0.0435241998455 0.00413670115661
0.0507782331531 0.00418558848097
0.0580322664607 0.00423539783252
0.0652862997683 0.00428615381651
0.0725403330759 0.00433788190567
0.0797943663834 0.00439060847876
0.087048399691 0.00444436086129
0.0943024329986 0.00449916736844
0.101556466306 0.0045550573504
0.108810499614 0.00461206124017
0.116064532921 0.00467021060414
0.123318566229 0.00472953819553
0.130572599537 0.00479007801091
0.137826632844 0.00485186535003
0.145080666152 0.00491493687917
0.152334699459 0.00497933069825
0.159588732767 0.00504508641202
0.166842766074 0.00511224520559
0.174096799382 0.00518084992455
0.18135083269 0.00525094516014
0.188604865997 0.0053225773398
0.195858899305 0.00539579482345
0.203112932612 0.005470648006
0.21036696592 0.00554718942659
0.217620999228 0.005625473885
0.224875032535 0.00570555856586
0.232129065843 0.00578750317135
0.23938309915 0.0058713700629
0.246637132458 0.00595722441281
0.253891165765 0.00604513436656
0.261145199073 0.00613517121669
0.268399232381 0.00622740958923
0.275653265688 0.00632192764383
0.282907298996 0.00641880728886
0.290161332303 0.00651813441257
0.297415365611 0.00661999913212
0.304669398919 0.0067244960618
0.311923432226 0.00683172460258
0.319177465534 0.0069417892546
0.326431498841 0.00705479995532
0.333685532149 0.00717087244539
0.340939565457 0.00729012866535
0.348193598764 0.00741269718613
0.355447632072 0.00753871367684
0.362701665379 0.00766832141393
0.369955698687 0.00780167183599
0.377209731994 0.00793892514921
0.384463765302 0.00808025098922
0.39171779861 0.00822582914566
0.398971831917 0.00837585035663
0.406225865225 0.00853051718143
0.413479898532 0.00869004496092
0.42073393184 0.00885466287622
0.427987965148 0.00902461511819
0.435241998455 0.00920016218181
0.442496031763 0.00938158230199
0.44975006507 0.00956917304951
0.457004098378 0.0097632531094
0.464258131685 0.00996416426728
0.471512164993 0.0101722736337
0.478766198301 0.0103879761414
0.486020231608 0.0106116973583
0.493274264916 0.010843896663
0.500528298223 0.0110850708437
0.507782331531 0.0113357581892
0.515036364839 0.0115965431559
0.522290398146 0.0118680617121
0.529544431454 0.012151007483
0.536798464761 0.0124461388459
0.544052498069 0.0127542871612
0.551306531376 0.0130763663671
0.558560564684 0.0134133842236
0.565814597992 0.0137664555655
0.573068631299 0.0141368180177
0.580322664607 0.0145258507579
0.587576697914 0.0149350970807
0.594830731222 0.0153662917494
0.60208476453 0.0158213944447
0.609338797837 0.0163026310673
0.616592831145 0.0168125452882
0.623846864452 0.0173540636692
0.63110089776 0.0179305790438
0.638354931067 0.0185460589298
0.645608964375 0.0192051889847
0.652862997683 0.0199135667241
0.66011703099 0.0206779694095
0.667371064298 0.0215067351164
0.674625097605 0.0224103236415
0.681879130913 0.0234021777335
0.689133164221 0.0245001183598
0.696387197528 0.0257287709573
0.703641230836 0.0271242204071
0.710895264143 0.0287443665483
0.718149297451 0.0306987457151


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt4.tex <==
-0.5 0.0234601434715
-0.495 0.0234524350944
-0.49 0.0234299939278
-0.485 0.0233938105277
-0.48 0.0233448298184
-0.475 0.0232839529822
-0.47 0.0232120392859
-0.465 0.0231299078452
-0.46 0.0230383393279
-0.455 0.0229380775985
-0.45 0.022829831306
-0.445 0.0227142754148
-0.44 0.0225920526825
-0.435 0.0224637750844
-0.43 0.0223300251868
-0.425 0.0221913574706
-0.42 0.0220482996065
-0.415 0.0219013536829
-0.41 0.0217509973887
-0.405 0.0215976851513
-0.4 0.0214418492312
-0.395 0.0212839007757
-0.39 0.0211242308312
-0.385 0.0209632113168
-0.38 0.0208011959588
-0.375 0.0206385211892
-0.37 0.0204755070073
-0.365 0.0203124578073
-0.36 0.0201496631716
-0.355 0.0199873986314
-0.35 0.0198259263959
-0.345 0.0196654960505
-0.34 0.019506345225
-0.335 0.0193487002338
-0.33 0.0191927766873
-0.325 0.0190387800764
-0.32 0.0188869063312
-0.315 0.0187373423541
-0.31 0.0185902665282
-0.305 0.0184458492019
-0.3 0.0183042531506
-0.295 0.018165634016
-0.29 0.0180301407236
-0.285 0.0178979158792
-0.28 0.0177690961451
-0.275 0.0176438125967
-0.27 0.0175221910593
-0.265 0.0174043524269
-0.26 0.0172904129624
-0.255 0.0171804845802
-0.25 0.0170746751114
-0.245 0.0169730885529
-0.24 0.0168758252987
-0.235 0.0167829823565
-0.23 0.0166946535478
-0.225 0.0166109296921
-0.22 0.0165318987767
-0.215 0.016457646111
-0.21 0.0163882544655
-0.205 0.0163238041968
-0.2 0.0162643733572
-0.195 0.01621003779
-0.19 0.0161608712102
-0.185 0.0161169452701
-0.18 0.0160783296103
-0.175 0.0160450918962
-0.17 0.0160172978388
-0.165 0.0159950112001
-0.16 0.0159782937835
-0.155 0.0159672054079
-0.15 0.0159618038648
-0.145 0.0159621448602
-0.14 0.015968281937
-0.135 0.0159802663819
-0.13 0.0159981471116
-0.125 0.0160219705413
-0.12 0.0160517804326
-0.115 0.0160876177208
-0.11 0.0161295203203
-0.105 0.0161775229075
-0.1 0.01623165668
-0.095 0.0162919490909
-0.09 0.0163584235571
-0.085 0.0164310991403
-0.08 0.0165099901989
-0.075 0.0165951060106
-0.07 0.0166864503624
-0.065 0.0167840211078
-0.06 0.0168878096887
-0.055 0.0169978006206
-0.05 0.0171139709389
-0.045 0.0172362896046
-0.04 0.0173647168667
-0.035 0.0174992035799
-0.03 0.0176396904754
-0.025 0.0177861073809
-0.02 0.0179383723899
-0.015 0.0180963909751
-0.01 0.0182600550461
-0.005 0.018429241946
0.0 0.018603813387
0.0040455488499 0.0187481435215
0.00809109769979 0.0188943885223
0.0121366465497 0.0190425865365
0.0161821953996 0.0191927767638
0.0202277442495 0.0193449994945
0.0242732930994 0.019499296149
0.0283188419493 0.0196557093197
0.0323643907992 0.0198142828141
0.0364099396491 0.0199750617006
0.040455488499 0.0201380923557
0.0445010373489 0.0203034225145
0.0485465861988 0.0204711013224
0.0525921350487 0.0206411793904
0.0566376838986 0.020813708852
0.0606832327485 0.0209887434244
0.0647287815983 0.0211663384708
0.0687743304482 0.0213465510681
0.0728198792981 0.0215294400759
0.076865428148 0.0217150662107
0.0809109769979 0.0219034921229
0.0849565258478 0.0220947824786
0.0890020746977 0.0222890040454
0.0930476235476 0.0224862257824
0.0970931723975 0.0226865189364
0.101138721247 0.022889957142
0.105184270097 0.023096616528
0.109229818947 0.0233065758296
0.113275367797 0.0235199165076
0.117320916647 0.0237367228734
0.121366465497 0.0239570822223
0.125412014347 0.0241810849743
0.129457563197 0.0244088248233
0.133503112047 0.0246403988958
0.137548660896 0.0248759079189
0.141594209746 0.0251154563989
0.145639758596 0.025359152812
0.149685307446 0.0256071098057
0.153730856296 0.0258594444151
0.157776405146 0.0261162782923
0.161821953996 0.0263777379515
0.165867502846 0.0266439550314
0.169913051696 0.0269150665746
0.173958600546 0.0271912153276
0.178004149395 0.0274725500622
0.182049698245 0.0277592259193
0.186095247095 0.028051404779
0.190140795945 0.0283492556581
0.194186344795 0.0286529551378
0.198231893645 0.0289626878244
0.202277442495 0.0292786468468
0.206322991345 0.0296010343939
0.210368540195 0.0299300622952
0.214414089045 0.0302659526509
0.218459637894 0.0306089385147
0.222505186744 0.0309592646361
0.226550735594 0.0313171882682
0.230596284444 0.0316829800486
0.234641833294 0.0320569249608
0.238687382144 0.0324393233866
0.242732930994 0.0328304922597
0.246778479844 0.0332307663326
0.250824028694 0.033640499571
0.254869577543 0.034060066692
0.258915126393 0.0344898648651
0.262960675243 0.0349303155969
0.267006224093 0.0353818668261
0.271051772943 0.0358449952565
0.275097321793 0.0363202089651
0.279142870643 0.0368080503243
0.283188419493 0.0373090992876
0.287233968343 0.0378239770961
0.291279517193 0.0383533504753
0.295325066042 0.0388979364055
0.299370614892 0.0394585075654
0.303416163742 0.0400358985726
0.307461712592 0.0406310131717
0.311507261442 0.0412448325549
0.315552810292 0.0418784250481
0.319598359142 0.0425329574528
0.323643907992 0.0432097084149
0.327689456842 0.0439100842927
0.331735005692 0.0446356381388
0.335780554541 0.0453880926021
0.339826103391 0.0461693678204
0.343871652241 0.04698161575
0.347917201091 0.0478272629181
0.351962749941 0.0487090643735
0.356008298791 0.0496301728009
0.360053847641 0.050594228603
0.364099396491 0.0516054796788
0.368144945341 0.0526689444661
0.37219049419 0.0537906401498
0.37623604304 0.0549779130514
0.38028159189 0.056239937365
0.38432714074 0.0575885091384
0.38837268959 0.0590394022105
0.39241823844 0.0606149212715
0.39646378729 0.0623494701753
0.40050933614 0.0643052457837


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt5.tex <==
-0.5 0.0325395998849
-0.495 0.032532352819
-0.49 0.032511236032
-0.485 0.0324771572588
-0.48 0.0324309869027
-0.475 0.0323735594678
-0.47 0.032305674947
-0.465 0.0322281001658
-0.46 0.0321415700832
-0.455 0.032046789051
-0.45 0.0319444320333
-0.445 0.0318351457856
-0.44 0.0317195499965
-0.435 0.0315982383917
-0.43 0.0314717798016
-0.425 0.0313407191939
-0.42 0.031205578672
-0.415 0.0310668584398
-0.41 0.0309250377344
-0.405 0.0307805757267
-0.4 0.0306339123923
-0.395 0.0304854693521
-0.39 0.0303356506841
-0.385 0.0301848437072
-0.38 0.0300334197375
-0.375 0.0298817348192
-0.37 0.0297301304283
-0.365 0.0295789341523
-0.36 0.029428460346
-0.355 0.0292790107633
-0.35 0.0291308751659
-0.345 0.0289843319115
-0.34 0.0288396485183
-0.335 0.0286970822113
-0.33 0.0285568804464
-0.325 0.0284192814159
-0.32 0.0282845145357
-0.315 0.0281528009128
-0.31 0.0280243537964
-0.305 0.0278993790109
-0.3 0.0277780753729
-0.295 0.0276606350916
-0.29 0.0275472441539
-0.285 0.0274380826941
-0.28 0.0273333253492
-0.275 0.0272331415999
-0.27 0.0271376960978
-0.265 0.027047148979
-0.26 0.0269616561656
-0.255 0.0268813696537
-0.25 0.0268064377897
-0.245 0.0267370055353
-0.24 0.0266732147199
-0.235 0.0266152042831
-0.23 0.0265631105057
-0.225 0.0265170672309
-0.22 0.0264772060747
-0.215 0.0264436566266
-0.21 0.0264165466414
-0.205 0.0263960022211
-0.2 0.0263821479876
-0.195 0.0263751072474
-0.19 0.0263750021472
-0.185 0.0263819538213
-0.18 0.0263960825313
-0.175 0.0264175077977
-0.17 0.0264463485244
-0.165 0.0264827231151
-0.16 0.0265267495837
-0.155 0.0265785456575
-0.15 0.0266382288735
-0.145 0.0267059166693
-0.14 0.0267817264679
-0.135 0.0268657757565
-0.13 0.0269581821611
-0.125 0.027059063516
-0.12 0.027168537929
-0.115 0.0272867238432
-0.11 0.0274137400961
-0.105 0.027549705976
-0.1 0.0276947412777
-0.095 0.0278489663569
-0.09 0.0280125021861
-0.085 0.0281854704122
-0.08 0.0283679934177
-0.075 0.0285601943864
-0.07 0.0287621973778
-0.065 0.0289741274093
-0.06 0.0291961105519
-0.055 0.0294282740403
-0.05 0.0296707464022
-0.045 0.0299236576114
-0.04 0.0301871392673
-0.035 0.0304613248093
-0.03 0.0307463497711
-0.025 0.0310423520822
-0.02 0.0313494724273
-0.015 0.0316678546718
-0.01 0.0319976463671
-0.005 0.03233899935
0.0 0.0326920704511
0.00275255128608 0.0328907757948
0.00550510257217 0.0330916680619
0.00825765385825 0.0332947851691
0.0110102051443 0.0335001659774
0.0137627564304 0.0337078503237
0.0165153077165 0.0339178790536
0.0192678590026 0.0341302940561
0.0220204102887 0.0343451382994
0.0247729615748 0.0345624558681
0.0275255128608 0.0347822920026
0.0302780641469 0.0350046931398
0.033030615433 0.0352297069562
0.0357831667191 0.0354573824121
0.0385357180052 0.0356877697987
0.0412882692913 0.0359209207868
0.0440408205773 0.0361568884786
0.0467933718634 0.0363957274609
0.0495459231495 0.0366374938615
0.0522984744356 0.0368822454086
0.0550510257217 0.0371300414926
0.0578035770078 0.037380943231
0.0605561282939 0.0376350135373
0.0633086795799 0.0378923171924
0.066061230866 0.0381529209205
0.0688137821521 0.0384168934685
0.0715663334382 0.0386843056901
0.0743188847243 0.0389552306336
0.0770714360104 0.0392297436353
0.0798239872964 0.0395079224179
0.0825765385825 0.0397898471935
0.0853290898686 0.0400756007739
0.0880816411547 0.0403652686859
0.0908341924408 0.0406589392939
0.0935867437269 0.0409567039295
0.0963392950129 0.0412586570292
0.099091846299 0.0415648962799
0.101844397585 0.0418755227733
0.104596948871 0.0421906411708
0.107349500157 0.0425103598773
0.110102051443 0.0428347912275
0.112854602729 0.0431640516835
0.115607154016 0.0434982620459
0.118359705302 0.0438375476785
0.121112256588 0.0441820387491
0.123864807874 0.0445318704858
0.12661735916 0.044887183453
0.129369910446 0.0452481238452
0.132122461732 0.0456148438041
0.134875013018 0.0459875017575
0.137627564304 0.0463662627854
0.14038011559 0.0467512990127
0.143132666876 0.0471427900336
0.145885218162 0.04754092337
0.148637769449 0.0479458949663
0.151390320735 0.0483579097264
0.154142872021 0.0487771820951
0.156895423307 0.0492039366907
0.159647974593 0.0496384089931
0.162400525879 0.0500808460943
0.165153077165 0.0505315075179
0.167905628451 0.0509906661164
0.170658179737 0.0514586090557
0.173410731023 0.051935638896
0.176163282309 0.0524220747847
0.178915833595 0.0529182537717
0.181668384882 0.0534245322673
0.184420936168 0.0539412876595
0.187173487454 0.0544689201151
0.18992603874 0.0550078545907
0.192678590026 0.0555585430852
0.195431141312 0.0561214671712
0.198183692598 0.0566971408504
0.200936243884 0.0572861137867
0.20368879517 0.0578889749817
0.206441346456 0.0585063569716
0.209193897742 0.0591389406419
0.211946449028 0.0597874607793
0.214699000315 0.0604527125079
0.217451551601 0.0611355587962
0.220204102887 0.0618369392681
0.222956654173 0.0625578806189
0.225709205459 0.0632995090227
0.228461756745 0.0640630650385
0.231214308031 0.0648499216881
0.233966859317 0.0656616066088
0.236719410603 0.0664998295211
0.239471961889 0.0673665167387
0.242224513175 0.0682638551795
0.244977064461 0.0691943494693
0.247729615748 0.0701608975228
0.250482167034 0.0711668929459
0.25323471832 0.0722163676928
0.255987269606 0.0733141976103
0.258739820892 0.0744664112086
0.261492372178 0.0756806787875
0.264244923464 0.0769671435293
0.26699747475 0.0783399782161
0.269750026036 0.0798207621553
0.272502577322 0.0814479436577


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt6.tex <==
-0.5 0.0449051370549
-0.495 0.0448984914013
-0.49 0.0448791403218
-0.485 0.0448479380993
-0.48 0.0448057072552
-0.475 0.0447532397166
-0.47 0.0446912979491
-0.465 0.0446206160563
-0.46 0.044541900848
-0.455 0.0444558328756
-0.45 0.0443630674383
-0.445 0.0442642355583
-0.44 0.0441599449284
-0.435 0.0440507808307
-0.43 0.0439373070284
-0.425 0.0438200666312
-0.42 0.0436995829346
-0.415 0.043576360235
-0.41 0.0434508846199
-0.405 0.0433236247347
-0.4 0.0431950325274
-0.395 0.0430655439703
-0.39 0.0429355797609
-0.385 0.0428055460021
-0.38 0.0426758348622
-0.375 0.0425468252152
-0.37 0.0424188832631
-0.365 0.0422923631396
-0.36 0.0421676074963
-0.355 0.0420449480723
-0.35 0.0419247062471
-0.345 0.0418071935785
-0.34 0.041692712325
-0.335 0.0415815559537
-0.33 0.0414740096346
-0.325 0.0413703507216
-0.32 0.0412708492204
-0.315 0.0411757682449
-0.31 0.0410853644617
-0.305 0.0409998885234
-0.3 0.0409195854922
-0.295 0.0408446952531
-0.29 0.0407754529183
-0.285 0.0407120892226
-0.28 0.0406548309113
-0.275 0.0406039011203
-0.27 0.04055951975
-0.265 0.040521903832
-0.26 0.040491267892
-0.255 0.0404678243065
-0.25 0.0404517836559
-0.245 0.0404433550749
-0.24 0.0404427465996
-0.235 0.040450165513
-0.23 0.0404658186899
-0.225 0.0404899129414
-0.22 0.0405226553611
-0.215 0.0405642536722
-0.21 0.0406149165783
-0.205 0.0406748541187
-0.2 0.0407442780279
-0.195 0.0408234021036
-0.19 0.0409124425814
-0.185 0.0410116185201
-0.18 0.0411211521986
-0.175 0.0412412695261
-0.17 0.0413722004674
-0.165 0.0415141794869
-0.16 0.0416674460122
-0.155 0.0418322449213
-0.15 0.0420088270558
-0.145 0.0421974497636
-0.14 0.0423983774758
-0.135 0.0426118823208
-0.13 0.0428382447809
-0.125 0.0430777543979
-0.12 0.0433307105312
-0.115 0.0435974231786
-0.11 0.0438782138638
-0.105 0.044173416603
-0.1 0.0444833789571
-0.095 0.0448084631836
-0.09 0.0451490474991
-0.085 0.0455055274674
-0.08 0.045878317531
-0.075 0.0462678527038
-0.07 0.0466745904476
-0.065 0.0470990127582
-0.06 0.0475416284904
-0.055 0.0480029759558
-0.05 0.0484836258333
-0.045 0.0489841844389
-0.04 0.0495052974093
-0.035 0.0500476538631
-0.03 0.0506119911142
-0.025 0.0511991000293
-0.02 0.0518098311322
-0.015 0.0524451015857
-0.01 0.0531059032017
-0.005 0.0537933116638
0.0 0.0545084971875
0.001583592135 0.0547405136537
0.00316718427 0.0549744957342
0.004750776405 0.0552104718459
0.00633436854001 0.0554484710314
0.00791796067501 0.0556885229783
0.00950155281001 0.0559306580392
0.011085144945 0.0561749072525
0.01266873708 0.0564213023644
0.014252329215 0.0566698758509
0.01583592135 0.0569206609422
0.017419513485 0.0571736916467
0.01900310562 0.0574290027765
0.020586697755 0.0576866299748
0.02217028989 0.0579466097434
0.023753882025 0.0582089794715
0.02533747416 0.058473777467
0.026921066295 0.0587410429876
0.02850465843 0.0590108162746
0.030088250565 0.0592831385871
0.0316718427 0.0595580522394
0.033255434835 0.0598356006384
0.03483902697 0.0601158283238
0.036422619105 0.0603987810105
0.03800621124 0.0606845056321
0.039589803375 0.0609730503875
0.04117339551 0.0612644647891
0.042756987645 0.0615587997144
0.04434057978 0.061856107459
0.045924171915 0.0621564417936
0.04750776405 0.0624598580231
0.049091356185 0.0627664130496
0.05067494832 0.0630761654383
0.052258540455 0.063389175487
0.05384213259 0.0637055053004
0.055425724725 0.064025218867
0.05700931686 0.0643483821423
0.058592908995 0.0646750631353
0.06017650113 0.0650053320008
0.061760093265 0.0653392611375
0.0633436854001 0.0656769252918
0.0649272775351 0.0660184016678
0.0665108696701 0.0663637700446
0.0680944618051 0.066713112901
0.0696780539401 0.0670665155487
0.0712616460751 0.0674240662735
0.0728452382101 0.0677858564867
0.0744288303451 0.0681519808868
0.0760124224801 0.0685225376321
0.0775960146151 0.0688976285264
0.0791796067501 0.069277359217
0.0807631988851 0.0696618394082
0.0823467910201 0.0700511830908
0.0839303831551 0.0704455087886
0.0855139752901 0.070844939825
0.0870975674251 0.0712496046101
0.0886811595601 0.0716596369521
0.0902647516951 0.0720751763937
0.0918483438301 0.072496368578
0.0934319359651 0.0729233656459
0.0950155281001 0.0733563266689
0.0965991202351 0.0737954181214
0.0981827123701 0.0742408143976
0.0997663045051 0.0746926983773
0.10134989664 0.075151262048
0.102933488775 0.0756167071894
0.10451708091 0.0760892461289
0.106100673045 0.0765691025783
0.10768426518 0.0770565125619
0.109267857315 0.0775517254489
0.11085144945 0.078055005108
0.112435041585 0.078566631199
0.11401863372 0.0790869006261
0.115602225855 0.079616129178
0.11718581799 0.080154653386
0.118769410125 0.0807028326394
0.12035300226 0.0812610516041
0.121936594395 0.081829723002
0.12352018653 0.0824092908234
0.125103778665 0.0830002340601
0.1266873708 0.0836030710735
0.128270962935 0.08421836474
0.12985455507 0.0848467285599
0.131438147205 0.0854888339714
0.13302173934 0.0861454191898
0.134605331475 0.086817300002
0.13618892361 0.0875053831043
0.137772515745 0.0882106827994
0.13935610788 0.0889343422161
0.140939700015 0.0896776607422
0.14252329215 0.0904421302023
0.144106884285 0.0912294836963
0.14569047642 0.0920417633837
0.147274068555 0.0928814177883
0.14885766069 0.0937514474165
0.150441252825 0.0946556345539
0.15202484496 0.0955989322035
0.153608437095 0.0965881897149
0.15519202923 0.0976337204033
0.156775621365 0.0987536749614


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5Prob0pt8.tex <==
-0.5 0.0852206031035
-0.495527864045 0.0852171448302
-0.49105572809 0.0852071622872
-0.486583592135 0.0851912326502
-0.48211145618 0.0851699185346
-0.477639320225 0.0851437685197
-0.47316718427 0.0851133176647
-0.468695048315 0.0850790880155
-0.46422291236 0.0850415891041
-0.459750776405 0.0850013184403
-0.45527864045 0.0849587619956
-0.450806504495 0.0849143946809
-0.44633436854 0.0848686808174
-0.441862232585 0.0848220746014
-0.43739009663 0.084775020564
-0.432917960675 0.0847279540248
-0.42844582472 0.0846813015418
-0.423973688765 0.0846354813565
-0.41950155281 0.0845909038357
-0.415029416855 0.0845479719095
-0.4105572809 0.0845070815069
-0.406085144945 0.0844686219895
-0.40161300899 0.0844329765832
-0.397140873035 0.0844005228091
-0.39266873708 0.0843716329138
-0.388196601125 0.0843466743002
-0.38372446517 0.0843260099596
-0.379252329215 0.0843099989043
-0.37478019326 0.0842989966043
-0.370308057305 0.0842933554259
-0.36583592135 0.0842934250754
-0.361363785395 0.0842995530471
-0.35689164944 0.0843120850781
-0.352419513485 0.0843313656099
-0.34794737753 0.084357738258
-0.343475241575 0.0843915462916
-0.33900310562 0.0844331331239
-0.334530969665 0.0844828428139
-0.33005883371 0.0845410205837
-0.325586697755 0.084608013349
-0.3211145618 0.0846841702691
-0.316642425845 0.0847698433146
-0.31217028989 0.0848653878571
-0.307698153935 0.0849711632828
-0.30322601798 0.0850875336319
-0.298753882025 0.0852148682683
-0.29428174607 0.0853535425801
-0.289809610115 0.0855039387171
-0.28533747416 0.0856664463677
-0.280865338205 0.0858414635787
-0.27639320225 0.086029397625
-0.271921066295 0.0862306659316
-0.26744893034 0.0864456970559
-0.262976794385 0.0866749317358
-0.25850465843 0.0869188240107
-0.254032522475 0.0871778424241
-0.24956038652 0.0874524713162
-0.245088250565 0.0877432122181
-0.24061611461 0.0880505853575
-0.236143978655 0.0883751312909
-0.2316718427 0.0887174126755
-0.227199706745 0.0890780162001
-0.22272757079 0.0894575546926
-0.218255434835 0.0898566694279
-0.21378329888 0.0902760326619
-0.209311162925 0.0907163504207
-0.20483902697 0.0911783655817
-0.200366891015 0.0916628612847
-0.19589475506 0.0921706647222
-0.191422619105 0.092702651364
-0.18695048315 0.093259749681
-0.182478347195 0.0938429464471
-0.17800621124 0.094453292711
-0.173534075285 0.0950919105499
-0.16906193933 0.0957600007376
-0.164589803375 0.0964588514916
-0.16011766742 0.0971898484954
-0.155645531465 0.0979544864418
-0.15117339551 0.0987543823992
-0.146701259555 0.0995912913802
-0.1422291236 0.10046712459
-0.137756987645 0.101383970963
-0.13328485169 0.102344122778
-0.128812715735 0.103350106374
-0.12434057978 0.104404719318
-0.119868443825 0.105511075859
-0.11539630787 0.106672663141
-0.110924171915 0.107893411635
-0.10645203596 0.109177784693
-0.101979900005 0.11053089436
-0.09750776405 0.11195865411
-0.093035628095 0.113467984976
-0.08856349214 0.11506710148
-0.084091356185 0.11676592172
-0.07961922023 0.118576680323
-0.075147084275 0.120514894188
-0.07067494832 0.122600993828
-0.066202812365 0.124863359653
-0.06173067641 0.12734486272
-0.057258540455 0.130121048943


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5equalAreas.tex <==
-0.5 0.0325395998849
-0.49501 0.0325271248953
-0.49002 0.0324903225052
-0.48503 0.0324301010943
-0.48004 0.0323473366933
-0.47505 0.0322428749138
-0.47006 0.0321175327517
-0.46507 0.031972100273
-0.46008 0.0318073421887
-0.45509 0.0316239993296
-0.4501 0.031422790025
-0.44511 0.0312044113946
-0.44012 0.0309695405575
-0.43513 0.030718835765
-0.43014 0.0304529374632
-0.42515 0.0301724692875
-0.42016 0.0298780389965
-0.41517 0.0295702393477
-0.41018 0.0292496489185
-0.40519 0.0289168328772
-0.4002 0.0285723437066
-0.39521 0.0282167218831
-0.39022 0.0278504965145
-0.38523 0.0274741859386
-0.38024 0.0270882982858
-0.37525 0.0266933320074
-0.37026 0.0262897763715
-0.36527 0.025878111929
-0.36028 0.0254588109518
-0.35529 0.0250323378435
-0.3503 0.0245991495261
-0.34531 0.0241596958027
-0.34032 0.0237144196983
-0.33533 0.0232637577799
-0.33034 0.0228081404572
-0.32535 0.0223479922645
-0.32036 0.0218837321263
-0.31537 0.0214157736053
-0.31038 0.0209445251365
-0.30539 0.0204703902457
-0.3004 0.0199937677556
-0.29541 0.0195150519777
-0.29042 0.0190346328938
-0.28543 0.0185528963248
-0.28044 0.0180702240898
-0.27545 0.0175869941547
-0.27046 0.017103580771
-0.26547 0.0166203546067
-0.26048 0.0161376828682
-0.25549 0.0156559294138
-0.2505 0.015175454861
-0.24551 0.0146966166857
-0.24052 0.0142197693157
-0.23553 0.013745264217
-0.23054 0.0132734499757
-0.22555 0.0128046723728
-0.22056 0.0123392744555
-0.21557 0.0118775966022
-0.21058 0.0114199765841
-0.20559 0.0109667496221
-0.2006 0.0105182484395
-0.19561 0.0100748033114
-0.19062 0.00963674211043
-0.18563 0.00920439034909
-0.18064 0.00877807121919
-0.17565 0.00835810562837
-0.17066 0.00794481223393
-0.16567 0.0075385074742
-0.16068 0.00713950559753
-0.15569 0.00674811868916
-0.1507 0.00636465669606
-0.14571 0.00598942744987
-0.14072 0.00562273668813
-0.13573 0.00526488807386
-0.13074 0.00491618321367
-0.12575 0.00457692167447
-0.12076 0.00424740099893
-0.11577 0.00392791671971
-0.11078 0.00361876237264
-0.10579 0.00332022950894
-0.1008 0.00303260770644
-0.09581 0.00275618458005
-0.09082 0.00249124579142
-0.08583 0.00223807505797
-0.08084 0.00199695416121
-0.07585 0.00176816295455
-0.07086 0.00155197937066
-0.06587 0.00134867942823
-0.06088 0.00115853723848
-0.05589 0.000981825011233
-0.0509 0.000818813060701
-0.04591 0.000669769810997
-0.04092 0.000534961801418
-0.03593 0.000414653691538
-0.03094 0.000309108266132
-0.02595 0.000218586439968
-0.02096 0.000143347262501
-0.01597 8.36479224892e-05
-0.01098 3.97437525512e-05
-0.00599 1.18882337026e-05


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5equalSides.tex <==
-0.5 0.0555555555556
-0.49501 0.0549576285556
-0.49002 0.0543426805787
-0.48503 0.053711649361
-0.48004 0.0530654464779
-0.47505 0.0524049581703
-0.47006 0.0517310461405
-0.46507 0.0510445483209
-0.46008 0.0503462796151
-0.45509 0.0496370326124
-0.4501 0.0489175782782
-0.44511 0.0481886666193
-0.44012 0.0474510273267
-0.43513 0.0467053703962
-0.43014 0.0459523867271
-0.42515 0.0451927487009
-0.42016 0.0444271107396
-0.41517 0.0436561098458
-0.41018 0.0428803661238
-0.40519 0.0421004832835
-0.4002 0.0413170491272
-0.39521 0.0405306360201
-0.39022 0.0397418013453
-0.38523 0.0389510879435
-0.38024 0.0381590245382
-0.37525 0.037366126147
-0.37026 0.0365728944793
-0.36527 0.035779818321
-0.36028 0.034987373907
-0.35529 0.0341960252809
-0.3503 0.0334062246439
-0.34531 0.0326184126924
-0.34032 0.0318330189437
-0.33533 0.031050462053
-0.33034 0.0302711501189
-0.32535 0.0294954809801
-0.32036 0.0287238425023
-0.31537 0.0279566128564
-0.31038 0.0271941607874
-0.30539 0.0264368458759
-0.3004 0.0256850187905
-0.29541 0.024939021533
-0.29042 0.0241991876756
-0.28543 0.0234658425916
-0.28044 0.0227393036777
-0.27545 0.0220198805712
-0.27046 0.0213078753588
-0.26547 0.0206035827809
-0.26048 0.0199072904282
-0.25549 0.0192192789331
-0.2505 0.0185398221558
-0.24551 0.0178691873636
-0.24052 0.0172076354063
-0.23553 0.0165554208851
-0.23054 0.0159127923176
-0.22555 0.0152799922973
-0.22056 0.0146572576485
-0.21557 0.0140448195769
-0.21058 0.0134429038156
-0.20559 0.0128517307671
-0.2006 0.0122715156407
-0.19561 0.0117024685867
-0.19062 0.011144794826
-0.18563 0.0105986947764
-0.18064 0.0100643641752
-0.17565 0.0095419941985
-0.17066 0.0090317715766
-0.16567 0.00853387870672
-0.16068 0.0080484937622
-0.15569 0.00757579079878
-0.1507 0.00711593985783
-0.14571 0.00666910706674
-0.14072 0.00623545473651
-0.13573 0.00581514145661
-0.13074 0.00540832218731
-0.12575 0.00501514834931
-0.12076 0.00463576791108
-0.11577 0.00427032547368
-0.11078 0.00391896235333
-0.10579 0.00358181666174
-0.1008 0.00325902338422
-0.09581 0.0029507144557
-0.09082 0.00265701883471
-0.08583 0.00237806257538
-0.08084 0.00211396889746
-0.07585 0.00186485825455
-0.07086 0.00163084840043
-0.06587 0.00141205445371
-0.06088 0.00120858896069
-0.05589 0.00102056195663
-0.0509 0.000848081025347
-0.04591 0.000691251357327
-0.04092 0.000550175806224
-0.03593 0.000424954943955
-0.03094 0.000315687114333
-0.02595 0.000222468485315
-0.02096 0.000145393099901
-0.01597 8.45529257169e-05
-0.01098 4.00379033271e-05
-0.00599 1.19359933043e-05


==> figuresAndData/dataForConditionalVarianceA0pt5B1pt5levelSets.tex <==
-0.5 0.180555555556
-0.49501 0.18045642652
-0.49002 0.180166279471
-0.48503 0.179695586175
-0.48004 0.179054324186
-0.47505 0.178252004682
-0.47006 0.177297698473
-0.46507 0.176200060344
-0.46008 0.174967351824
-0.45509 0.173607462522
-0.4501 0.172127930113
-0.44511 0.170535959091
-0.44012 0.168838438348
-0.43513 0.167041957692
-0.43014 0.165152823357
-0.42515 0.163177072579
-0.42016 0.161120487306
-0.41517 0.158988607095
-0.41018 0.15678674126
-0.40519 0.154519980304
-0.4002 0.1521932067
-0.39521 0.149811105053
-0.39022 0.147378171687
-0.38523 0.144898723693
-0.38024 0.142376907472
-0.37525 0.139816706805
-0.37026 0.137221950481
-0.36527 0.13459631951
-0.36028 0.131943353948
-0.35529 0.12926645935
-0.3503 0.126568912888
-0.34531 0.123853869138
-0.34032 0.121124365573
-0.33533 0.118383327762
-0.33034 0.115633574306
-0.32535 0.11287782152
-0.32036 0.110118687873
-0.31537 0.107358698212
-0.31038 0.104600287767
-0.30539 0.101845805964
-0.3004 0.0990975200379
-0.29541 0.0963576184836
-0.29042 0.0936282143268
-0.28543 0.0909113482433
-0.28044 0.0882089915256
-0.27545 0.0855230489096
-0.27046 0.0828553612665
-0.26547 0.0802077081692
-0.26048 0.0775818103375
-0.25549 0.074979331971
-0.2505 0.0724018829742
-0.24551 0.0698510210792
-0.24052 0.067328253873
-0.23553 0.0648350407321
-0.23054 0.0623727946708
-0.22555 0.0599428841075
-0.22056 0.0575466345518
-0.21557 0.0551853302184
-0.21058 0.0528602155693
-0.20559 0.0505724967901
-0.2006 0.0483233432017
-0.19561 0.0461138886121
-0.19062 0.0439452326098
-0.18563 0.0418184418027
-0.18064 0.0397345510055
-0.17565 0.0376945643761
-0.17066 0.0356994565056
-0.16567 0.0337501734631
-0.16068 0.0318476337972
-0.15569 0.0299927294968
-0.1507 0.0281863269131
-0.14571 0.0264292676437
-0.14072 0.0247223693819
-0.13573 0.0230664267314
-0.13074 0.0214622119895
-0.12575 0.0199104758988
-0.12076 0.018411948369
-0.11577 0.016967339172
-0.11078 0.0155773386083
-0.10579 0.0142426181489
-0.1008 0.0129638310518
-0.09581 0.0117416129558
-0.09082 0.0105765824512
-0.08583 0.0094693416285
-0.08084 0.00842047660799
-0.07585 0.007430558048
-0.07086 0.0065001416352
-0.06587 0.00562976855655
-0.06088 0.00481996595385
-0.05589 0.00407124736181
-0.0509 0.00338411313013
-0.04591 0.00275905083033
-0.04092 0.002196535648
-0.03593 0.00169703076093
-0.03094 0.0012609877039
-0.02595 0.000888846720458
-0.02096 0.00058103710238
-0.01597 0.000337977517188
-0.01098 0.00016007632428
-0.00599 4.77318800925e-05


==> figuresAndData/dataForConditionalVarianceCircularEqualAreas.tex <==
-0.450442616461 0.0582998243664
-0.449561731229 0.0579839015579
-0.448680845996 0.0579005571713
-0.447799960763 0.0578157053666
-0.44691907553 0.0577296835335
-0.446038190297 0.0574087522934
-0.445157305064 0.0573210582147
-0.444276419831 0.0572326209376
-0.443395534598 0.0569104249306
-0.442514649365 0.0568208619054
-0.441633764132 0.0567307436728
-0.440752878899 0.0564078801507
-0.439871993666 0.0563169260519
-0.438991108433 0.0562255291476
-0.438110223201 0.0559023557026
-0.437229337968 0.0558103107638
-0.436348452735 0.0557178999941
-0.435467567502 0.0553946637433
-0.434586682269 0.0553017397487
-0.433705797036 0.0552085069128
-0.432824911803 0.0548853929078
-0.43194402657 0.0547917498667
-0.431063141337 0.0546978423782
-0.430182256104 0.0543749965519
-0.429301370871 0.0542807610059
-0.428420485638 0.0539583552082
-0.427539600405 0.0538638385338
-0.426658715173 0.0537691138772
-0.42577782994 0.0534471654643
-0.424896944707 0.0533522197334
-0.424016059474 0.0532570925427
-0.423135174241 0.0529356917285
-0.422254289008 0.0528403946525
-0.421373403775 0.0527449388171
-0.420492518542 0.0524241638191
-0.419611633309 0.052328582423
-0.418730748076 0.0520084616255
-0.417849862843 0.0519127815757
-0.41696897761 0.0518169744425
-0.416088092377 0.0514975909307
-0.415207207145 0.0514017209627
-0.414326321912 0.0513057398645
-0.413445436679 0.0509871505309
-0.412564551446 0.0508911385476
-0.411683666213 0.0505733088942
-0.41080278098 0.0504772859115
-0.409921895747 0.0503811748732
-0.409041010514 0.0500642235227
-0.408160125281 0.0499681283426
-0.407279240048 0.0498719570545
-0.406398354815 0.0495559280912
-0.405517469582 0.0494597970825
-0.404636584349 0.0491446100388
-0.403755699117 0.0490485347832
-0.402874813884 0.0489524011253
-0.401993928651 0.0486382033149
-0.401113043418 0.048542146493
-0.400232158185 0.0482288341786
-0.399351272952 0.0481328676714
-0.398470387719 0.0480368580525
-0.397589502486 0.0477245939588
-0.396708617253 0.0476286930869
-0.39582773202 0.0473173533155
-0.394946846787 0.0472215730668
-0.394065961554 0.0471257630643
-0.393185076321 0.0468155241593
-0.392304191089 0.0467198510649
-0.391423305856 0.0464105714312
-0.390542420623 0.04631504581
-0.38966153539 0.0462195022176
-0.388780650157 0.0459113708818
-0.387899764924 0.045815989278
-0.387018879691 0.0455088489429
-0.386137994458 0.0454136388033
-0.385257109225 0.0453184211709
-0.384376223992 0.0450124722094
-0.383495338759 0.0449174390774
-0.382614453526 0.0446125101335
-0.381733568293 0.0445176700599
-0.380852683061 0.0444228318776
-0.379971797828 0.0441191336951
-0.379090912595 0.0440245003557
-0.378210027362 0.0437218488928
-0.377329142129 0.0436274281726
-0.376448256896 0.0435330177991
-0.375567371663 0.0432316333262
-0.37468648643 0.0431374462855
-0.373805601197 0.042837133237
-0.372924715964 0.042743176633
-0.372043830731 0.0424439447799
-0.371162945498 0.0423502254707
-0.370282060265 0.0422565270983
-0.369401175033 0.0419586089236
-0.3685202898 0.0418651572966
-0.367639404567 0.0415683426384
-0.366758519334 0.0414751440622
-0.365877634101 0.0411794418073
-0.364996748868 0.0410865023836
-0.364115863635 0.0409935932011
-0.363234978402 0.0406992468269
-0.362354093169 0.0406066052028
-0.361473207936 0.0403133915556
-0.360592322703 0.0402210231305
-0.35971143747 0.0401286908864
-0.358830552237 0.0398368605929
-0.357949667005 0.0397448093149
-0.357068781772 0.0394541308395
-0.356187896539 0.03936236576
-0.355307011306 0.0390728467772
-0.354426126073 0.038981372976
-0.35354524084 0.0388899429399
-0.352664355607 0.0386018433957
-0.351783470374 0.038510711627
-0.350902585141 0.0382237891437
-0.350021699908 0.0381329603744
-0.349140814675 0.0378472220488
-0.348259929442 0.0377567008806
-0.347379044209 0.0376662302649
-0.346498158977 0.0373819445656
-0.345617273744 0.0372917878748
-0.344736388511 0.0370087025815
-0.343855503278 0.0369188641184
-0.342974618045 0.0366369858234
-0.342093732812 0.0365474697776
-0.341212847579 0.0364580103897
-0.340331962346 0.0361776153913
-0.339451077113 0.0360884841709
-0.33857019188 0.0358093112638
-0.337689306647 0.0357205121411
-0.336808421414 0.0354425674735
-0.335927536181 0.0353541042803
-0.335046650949 0.0350773938804
-0.334165765716 0.034989270354
-0.333284880483 0.0349012105167
-0.33240399525 0.0346260199208
-0.331523110017 0.034538304869
-0.330642224784 0.0342643623391
-0.329761339551 0.0341769955914
-0.328880454318 0.0339043067739
-0.327999569085 0.0338172917655
-0.327118683852 0.033730345317
-0.326237798619 0.0334592022891
-0.325356913386 0.0333726122771
-0.324476028153 0.0331027358813
-0.323595142921 0.0330165055482
-0.322714257688 0.0327479010889
-0.321833372455 0.0326620336032
-0.320952487222 0.0323947062911
-0.320071601989 0.0323092047499
-0.319190716756 0.032223777436
-0.318309831523 0.0319580271366
-0.31742894629 0.0318729699922
-0.316548061057 0.031608508756
-0.315667175824 0.0315238247127
-0.314786290591 0.0312606574507
-0.313905405358 0.0311763493763
-0.313024520125 0.0309144809168
-0.312143634893 0.0308305516174
-0.31126274966 0.0307467016017
-0.310381864427 0.0304864389304
-0.309500979194 0.0304029715083
-0.308620093961 0.0301440186735
-0.307739208728 0.0300609365076
-0.306858323495 0.0298032980724
-0.305977438262 0.0297206037699
-0.305096553029 0.0294642842237
-0.304215667796 0.0293819803383
-0.303334782563 0.029126984099
-0.30245389733 0.0290450731317
-0.301573012097 0.0289632469441
-0.300692126865 0.0287098889489
-0.299811241632 0.0286284590721
-0.298930356399 0.0283764344707
-0.298049471166 0.0282954032845
-0.297168585933 0.0280447162638
-0.2962877007 0.0279640861006
-0.295406815467 0.0277147407831
-0.294525930234 0.0276345139292
-0.293645045001 0.0275543758383
-0.292764159768 0.0273066930718
-0.291883274535 0.0272269613832
-0.291002389302 0.0269806297249
-0.290121504069 0.026901306618
-0.289240618837 0.0266563299823
-0.288359733604 0.0265774175948
-0.287478848371 0.0263337998382
-0.286597963138 0.0262553002669
-0.285717077905 0.0260130451887
-0.284836192672 0.0259349604909
-0.283955307439 0.0258569689265
-0.283074422206 0.0256164040292
-0.282193536973 0.0255388301117
-0.28131265174 0.0252996365516
-0.280431766507 0.0252224822461
-0.279550881274 0.0249846636381
-0.278669996041 0.0249079308732
-0.277789110809 0.0246714907804
-0.276908225576 0.0245951814493
-0.276027340343 0.0243601233838
-0.27514645511 0.0242842393453
-0.274265569877 0.0240505667693
-0.273384684644 0.0239751098486
-0.272503799411 0.0238997506106
-0.271622914178 0.0236677981647
-0.270742028945 0.023592868495
-0.269861143712 0.0233623094192
-0.268980258479 0.0232878110644
-0.268099373246 0.0230586486592
-0.267218488013 0.022984583335
-0.266337602781 0.0227568208548
-0.265456717548 0.0226831902468
-0.264575832315 0.0224568309012
-0.263694947082 0.0223836366653
-0.262814061849 0.0221586836196
-0.261933176616 0.0220859273828
-0.261052291383 0.0220132727989
-0.26017140615 0.0217900671202
-0.259290520917 0.0217178527108
-0.258409635684 0.0214960605279
-0.257528750451 0.0214242878529
-0.256647865218 0.0212039121876
-0.255766979985 0.0211325827798
-0.254886094753 0.0209136266131
-0.25400520952 0.0208427419795
-0.253124324287 0.0206252082522
-0.252243439054 0.0205547698742
-0.251362553821 0.0203386614874
-0.250481668588 0.0202686708212
-0.249600783355 0.0201987852877
-0.248719898122 0.0199844491148
-0.247839012889 0.0199150132321
-0.246958127656 0.0197021089869
-0.246077242423 0.0196331241529
-0.24519635719 0.0194216546082
-0.244315471957 0.0193531221977
-0.243434586725 0.0191430900895
-0.242553701492 0.0190750114545
-0.241672816259 0.0188664194826
-0.240791931026 0.0187987959525
-0.239911045793 0.018591646781
-0.23903016056 0.0185244796638
-0.238149275327 0.0183187759217
-0.237268390094 0.0182520665035
-0.236387504861 0.0181854657271
-0.235506619628 0.0179815603313
-0.234625734395 0.0179154189583
-0.233744849162 0.0177129649523
-0.232863963929 0.0176472842191
-0.231983078697 0.0174462841175
-0.231102193464 0.0173810652404
-0.230221308231 0.0171815215253
-0.229340422998 0.017116765701
-0.228459537765 0.0169186808217
-0.227578652532 0.0168543892277
-0.226697767299 0.0166577656017
-0.225816882066 0.0165939393964
-0.224935996833 0.0163987794098
-0.2240551116 0.016335419733
-0.223174226367 0.0161417257406
-0.222293341134 0.0160788337142
-0.221412455901 0.0160160537504
-0.220531570669 0.0158241847679
-0.219650685436 0.0157618739327
-0.218769800203 0.0155714762742
-0.21788891497 0.0155096356468
-0.217008029737 0.0153207115661
-0.216127144504 0.0152593422088
-0.215246259271 0.0150718939302
-0.214365374038 0.0150109968884
-0.213484488805 0.0148250266073
-0.212603603572 0.0147646029099
-0.211722718339 0.0145801127932
-0.210841833106 0.0145201634528
-0.209960947873 0.0143371556391
-0.209080062641 0.0142776816524
-0.208199177408 0.0140961582524
-0.207318292175 0.0140371606005
-0.206437406942 0.0138571236975
-0.205556521709 0.0137986033458
-0.204675636476 0.0137401982947
-0.203794751243 0.013562012895
-0.20291386601 0.013504086409
-0.202032980777 0.0133273922126
-0.201152095544 0.0132699452216
-0.200271210311 0.0130947442222
-0.199390325078 0.0130377776414
-0.198509439846 0.0128640718065
-0.197628554613 0.0128075865368
-0.19674766938 0.0126353778083
-0.195866784147 0.0125793747365
-0.194985898914 0.0124086650306
-0.194105013681 0.0123531450297
-0.193224128448 0.0121839362374
-0.192343243215 0.0121289001666
-0.191462357982 0.011961194154
-0.190581472749 0.0119066428592
-0.189700587516 0.0117404414677
-0.188819702283 0.0116863757816
-0.18793881705 0.0115216808281
-0.187057931818 0.0114681015702
-0.186177046585 0.011414640597
-0.185296161352 0.0112518228248
-0.184415276119 0.0111988493465
-0.183534390886 0.0110375421083
-0.182653505653 0.0109850569143
-0.18177262042 0.0108252619477
-0.180891735187 0.010773265815
-0.180010849954 0.0106149848343
-0.179129964721 0.0105634785279
-0.178249079488 0.0104067132242
-0.177368194255 0.0103556974968
-0.176487309022 0.0102004495386
-0.17560642379 0.0101499251312
-0.174725538557 0.00999619616413
-0.173844653324 0.00994616380614
-0.172963768091 0.0097939554536
-0.172082882858 0.0097444158628
-0.171201997625 0.00959372972599
-0.170321112392 0.00954468360885
-0.169440227159 0.00939552126703
-0.168559341926 0.00934696931883
-0.167678456693 0.00919933232949
-0.16679757146 0.00915127523446
-0.165916686227 0.00910333910415
-0.165035800994 0.00895760356506
-0.164154915762 0.00891016317228
-0.163274030529 0.00876595648782
-0.162393145296 0.00871901249133
-0.161512260063 0.00857633614819
-0.16063137483 0.0085298891962
-0.159750489597 0.0083887446602
-0.158869604364 0.00834279539052
-0.157988719131 0.00820318410677
-0.157107833898 0.00815773314693
-0.156226948665 0.00801965654001
-0.155346063432 0.00797470450742
-0.154465178199 0.00783816398157
-0.153584292966 0.00779371148363
-0.152703407734 0.0076587084229
-0.151822522501 0.00761475605711
-0.150941637268 0.00748129182556
-0.150060752035 0.00743784017968
-0.149179866802 0.00730591612152
-0.148298981569 0.00726296577364
-0.147418096336 0.0071325832134
-0.146537211103 0.0070901347321
-0.14565632587 0.0069612949748
-0.144775440637 0.00691934891924
-0.143894555404 0.00687752617066
-0.143013670171 0.00675061017056
-0.142132784938 0.00670929056516
-0.141251899706 0.00658392029317
-0.140371014473 0.00654310436846
-0.13949012924 0.006419281066
-0.138609244007 0.00637896935045
-0.137728358774 0.00625669424009
-0.136847473541 0.00621688725324
-0.135966588308 0.00609616153882
-0.135085703075 0.00605685979136
-0.134204817842 0.00593768465814
-0.133323932609 0.00589888865202
-0.132443047376 0.00578126526681
-0.131562162143 0.00574297549535
-0.13068127691 0.00562690500664
-0.129800391678 0.00558912195459
-0.128919506445 0.00547460549267
-0.128038621212 0.00543732963634
-0.127157735979 0.00532436831344
-0.126276850746 0.00528760012075
-0.125395965513 0.00517619503118
-0.12451508028 0.00513993496177
-0.123634195047 0.005030087182
-0.122753309814 0.00499433568732
-0.121872424581 0.00488604627612
-0.120991539348 0.0048508037995
-0.120110654115 0.00474407379807
-0.119229768882 0.0047093407748
-0.11834888365 0.00460417120686
-0.117467998417 0.00456994806428
-0.116587113184 0.00453585046721
-0.115706227951 0.00443262709375
-0.114825342718 0.00439903992077
-0.113944457485 0.00429737926399
-0.113063572252 0.0042643029242
-0.112182687019 0.00416420595089
-0.111301801786 0.00413164084572
-0.110420916553 0.00403310850564
-0.10954003132 0.00400105502889
-0.108659146087 0.00390408825489
-0.107778260854 0.00387254679282
-0.106897375622 0.00377714650097
-0.106016490389 0.00374611743231
-0.105135605156 0.00365228452197
-0.104254719923 0.00362176821808
-0.10337383469 0.00352950357197
-0.102492949457 0.00349950039681
-0.101612064224 0.00340880488116
-0.100731178991 0.00337931519143
-0.0998502937581 0.00329018965601
-0.0989694085252 0.00326121380116
-0.0980885232923 0.00317365907941
-0.0972076380594 0.00314519740171
-0.0963267528264 0.00305921431081
-0.0954458675935 0.00303126714543
-0.0945649823606 0.00294685648638
-0.0936840971277 0.00291942416144
-0.0928032118948 0.00283658671913
-0.0919223266618 0.00280966955573
-0.0910414414289 0.00272840609907
-0.090160556196 0.00270200441137
-0.0892796709631 0.00262231569329
-0.0883987857301 0.00259642978856
-0.0875179004972 0.00251831654617
-0.0866370152643 0.00249294672483
-0.0857561300314 0.00246770425496
-0.0848752447984 0.00239155623511
-0.0839943595655 0.00236683022643
-0.0831134743326 0.00229225931186
-0.0822325890997 0.00226805004921
-0.0813517038668 0.00219505692522
-0.0804708186338 0.00217136468674
-0.0795899334009 0.00209995002309
-0.078709048168 0.0020767750803
-0.0778281629351 0.00200693953126
-0.0769472777021 0.00198428214909
-0.0760663924692 0.0019160263535
-0.0751855072363 0.00189388679035
-0.0743046220034 0.0018272113717
-0.0734237367704 0.00180558987946
-0.0725428515375 0.00174049544593
-0.0716619663046 0.00171939227004
-0.0707810810717 0.00165587941458
-0.0699001958388 0.00163529479405
-0.0690193106058 0.00157336409443
-0.0681384253729 0.00155329826189
-0.06725754014 0.00149295028074
-0.0663766549071 0.00147340346249
-0.0654957696741 0.00141463874737
-0.0646148844412 0.0013956111634
-0.0637339992083 0.00133843024686
-0.0628531139754 0.00131992211088
-0.0619722287425 0.00126432551049
-0.0610913435095 0.00124633702999
-0.0602104582766 0.00119232524841
-0.0593295730437 0.00117485662464
-0.0584486878108 0.00112243014966
-0.0575678025778 0.00110548157773
-0.0566869173449 0.0010546408823
-0.055806032112 0.00103821255118
-0.0549251468791 0.000988958093485
-0.0540442616461 0.000973050186007
-0.0531633764132 0.000925382409497
-0.0522824911803 0.000909995102428
-0.0514016059474 0.000894736423917
-0.0505207207145 0.000849047899899
-0.0496398354815 0.00083431004002
-0.0487589502486 0.000790209157196
-0.0478780650157 0.000775992278877
-0.0469971797828 0.000733479432477
-0.0461162945498 0.000719783692655
-0.0452354093169 0.000678859263346
-0.044354524084 0.000665684812992
-0.0434736388511 0.000626349166911
-0.0425927536181 0.00061369615105
-0.0417118683852 0.000575949639841
-0.0408309831523 0.00056381819758
-0.0399500979194 0.000527661158425
-0.0390692126865 0.00051605142297
-0.0381883274535 0.000481484178621
-0.0373074422206 0.000470396277297
-0.0364265569877 0.000437419136107
-0.0355456717548 0.000426853190383
-0.0346647865218 0.000395466446333
-0.0337839012889 0.000385422571835
-0.032903016056 0.000355626504561
-0.0320221308231 0.000346104811092
-0.0311412455901 0.000317899685913
-0.0302603603572 0.000308900277471
-0.0293794751243 0.000282286345411
-0.0284985898914 0.000273809320202
-0.0276177046585 0.000248786818016
-0.0267368194255 0.000240832268473
-0.0258559341926 0.000217401418666
-0.0249750489597 0.000209969431459
-0.0240941637268 0.000188130442307
-0.0232132784938 0.000181221098359
-0.0223323932609 0.000160974163931
-0.021451508028 0.000154587538429
-0.0205706227951 0.000135932838603
-0.0196897375622 0.00013006900101
-0.0188088523292 0.000113006701486
-0.0179279670963 0.000107665715554
-0.0170470818634 9.2195967874e-05
-0.0161661966305 8.73778916484e-05
-0.0152853113975 7.35008332104e-05
-0.0144044261646 6.92057190432e-05
-0.0135235409317 6.50398791563e-05
-0.0126426556988 5.31493676672e-05
-0.0117617704658 4.95065486174e-05
-0.0108808852329 3.9208987648e-05


==> figuresAndData/dataForConditionalVarianceCircularEqualSides.tex <==
-0.450442616461 0.062598021111
-0.449561731229 0.0623963165375
-0.448680845996 0.0621923022804
-0.447799960763 0.0619869529256
-0.44691907553 0.0617806193854
-0.446038190297 0.06157350596
-0.445157305064 0.0613657514445
-0.444276419831 0.0611574584025
-0.443395534598 0.0609487068038
-0.442514649365 0.0607395613814
-0.441633764132 0.0605300760049
-0.440752878899 0.0603202964691
-0.439871993666 0.0601102623689
-0.438991108433 0.0599000084128
-0.438110223201 0.0596895653757
-0.437229337968 0.0594789608085
-0.436348452735 0.0592682195794
-0.435467567502 0.0590573642953
-0.434586682269 0.0588464156351
-0.433705797036 0.0586353926179
-0.432824911803 0.0584243128209
-0.43194402657 0.0582131925588
-0.431063141337 0.0580020470342
-0.430182256104 0.057790890462
-0.429301370871 0.057579736177
-0.428420485638 0.0573685967238
-0.427539600405 0.0571574839357
-0.426658715173 0.0569464090016
-0.42577782994 0.0567353825253
-0.424896944707 0.0565244145769
-0.424016059474 0.0563135147378
-0.423135174241 0.056102692141
-0.422254289008 0.0558919555065
-0.421373403775 0.055681313173
-0.420492518542 0.055470773126
-0.419611633309 0.0552603430233
-0.418730748076 0.0550500302181
-0.417849862843 0.0548398417793
-0.41696897761 0.0546297845104
-0.416088092377 0.0544198649666
-0.415207207145 0.05421008947
-0.414326321912 0.0540004641242
-0.413445436679 0.0537909948267
-0.412564551446 0.0535816872813
-0.411683666213 0.0533725470088
-0.41080278098 0.0531635793571
-0.409921895747 0.0529547895103
-0.409041010514 0.0527461824977
-0.408160125281 0.0525377632015
-0.407279240048 0.0523295363641
-0.406398354815 0.0521215065953
-0.405517469582 0.0519136783785
-0.404636584349 0.0517060560764
-0.403755699117 0.0514986439372
-0.402874813884 0.0512914460993
-0.401993928651 0.0510844665962
-0.401113043418 0.0508777093614
-0.400232158185 0.0506711782323
-0.399351272952 0.0504648769546
-0.398470387719 0.0502588091857
-0.397589502486 0.0500529784986
-0.396708617253 0.0498473883852
-0.39582773202 0.0496420422592
-0.394946846787 0.0494369434594
-0.394065961554 0.0492320952526
-0.393185076321 0.049027500836
-0.392304191089 0.0488231633399
-0.391423305856 0.04861908583
-0.390542420623 0.04841527131
-0.38966153539 0.0482117227233
-0.388780650157 0.0480084429555
-0.387899764924 0.047805434836
-0.387018879691 0.0476027011403
-0.386137994458 0.0474002445913
-0.385257109225 0.0471980678613
-0.384376223992 0.0469961735736
-0.383495338759 0.046794564304
-0.382614453526 0.046593242582
-0.381733568293 0.0463922108929
-0.380852683061 0.0461914716784
-0.379971797828 0.0459910273383
-0.379090912595 0.0457908802317
-0.378210027362 0.045591032678
-0.377329142129 0.0453914869584
-0.376448256896 0.0451922453166
-0.375567371663 0.0449933099599
-0.37468648643 0.0447946830605
-0.373805601197 0.0445963667561
-0.372924715964 0.0443983631511
-0.372043830731 0.0442006743173
-0.371162945498 0.0440033022949
-0.370282060265 0.0438062490931
-0.369401175033 0.0436095166911
-0.3685202898 0.043413107039
-0.367639404567 0.0432170220581
-0.366758519334 0.043021263642
-0.365877634101 0.0428258336569
-0.364996748868 0.0426307339427
-0.364115863635 0.0424359663133
-0.363234978402 0.0422415325576
-0.362354093169 0.0420474344395
-0.361473207936 0.0418536736988
-0.360592322703 0.0416602520521
-0.35971143747 0.0414671711927
-0.358830552237 0.0412744327914
-0.357949667005 0.0410820384972
-0.357068781772 0.0408899899374
-0.356187896539 0.0406982887183
-0.355307011306 0.0405069364258
-0.354426126073 0.0403159346253
-0.35354524084 0.0401252848628
-0.352664355607 0.0399349886649
-0.351783470374 0.0397450475392
-0.350902585141 0.0395554629748
-0.350021699908 0.0393662364429
-0.349140814675 0.0391773693966
-0.348259929442 0.0389888632717
-0.347379044209 0.038800719487
-0.346498158977 0.0386129394444
-0.345617273744 0.0384255245296
-0.344736388511 0.0382384761121
-0.343855503278 0.0380517955454
-0.342974618045 0.0378654841678
-0.342093732812 0.0376795433023
-0.341212847579 0.037493974257
-0.340331962346 0.0373087783252
-0.339451077113 0.0371239567859
-0.33857019188 0.0369395109042
-0.337689306647 0.036755441931
-0.336808421414 0.0365717511037
-0.335927536181 0.0363884396465
-0.335046650949 0.0362055087701
-0.334165765716 0.0360229596726
-0.333284880483 0.0358407935392
-0.33240399525 0.0356590115427
-0.331523110017 0.0354776148436
-0.330642224784 0.0352966045905
-0.329761339551 0.0351159819198
-0.328880454318 0.0349357479565
-0.327999569085 0.0347559038141
-0.327118683852 0.0345764505946
-0.326237798619 0.0343973893892
-0.325356913386 0.034218721278
-0.324476028153 0.0340404473303
-0.323595142921 0.0338625686048
-0.322714257688 0.03368508615
-0.321833372455 0.0335080010039
-0.320952487222 0.0333313141944
-0.320071601989 0.0331550267396
-0.319190716756 0.0329791396477
-0.318309831523 0.0328036539173
-0.31742894629 0.0326285705374
-0.316548061057 0.0324538904878
-0.315667175824 0.0322796147388
-0.314786290591 0.032105744252
-0.313905405358 0.0319322799796
-0.313024520125 0.0317592228652
-0.312143634893 0.0315865738437
-0.31126274966 0.0314143338415
-0.310381864427 0.0312425037762
-0.309500979194 0.0310710845573
-0.308620093961 0.0309000770862
-0.307739208728 0.0307294822558
-0.306858323495 0.0305593009514
-0.305977438262 0.0303895340501
-0.305096553029 0.0302201824214
-0.304215667796 0.030051246927
-0.303334782563 0.0298827284211
-0.30245389733 0.0297146277503
-0.301573012097 0.0295469457539
-0.300692126865 0.029379683264
-0.299811241632 0.0292128411052
-0.298930356399 0.0290464200955
-0.298049471166 0.0288804210453
-0.297168585933 0.0287148447585
-0.2962877007 0.0285496920321
-0.295406815467 0.0283849636562
-0.294525930234 0.0282206604143
-0.293645045001 0.0280567830834
-0.292764159768 0.0278933324339
-0.291883274535 0.0277303092298
-0.291002389302 0.0275677142288
-0.290121504069 0.0274055481823
-0.289240618837 0.0272438118356
-0.288359733604 0.0270825059276
-0.287478848371 0.0269216311914
-0.286597963138 0.0267611883542
-0.285717077905 0.026601178137
-0.284836192672 0.0264416012552
-0.283955307439 0.0262824584184
-0.283074422206 0.0261237503303
-0.282193536973 0.0259654776893
-0.28131265174 0.0258076411878
-0.280431766507 0.0256502415131
-0.279550881274 0.0254932793468
-0.278669996041 0.0253367553652
-0.277789110809 0.0251806702393
-0.276908225576 0.0250250246346
-0.276027340343 0.0248698192118
-0.27514645511 0.024715054626
-0.274265569877 0.0245607315274
-0.273384684644 0.0244068505613
-0.272503799411 0.0242534123678
-0.271622914178 0.024100417582
-0.270742028945 0.0239478668344
-0.269861143712 0.0237957607503
-0.268980258479 0.0236440999505
-0.268099373246 0.023492885051
-0.267218488013 0.0233421166629
-0.266337602781 0.023191795393
-0.265456717548 0.0230419218433
-0.264575832315 0.0228924966112
-0.263694947082 0.0227435202897
-0.262814061849 0.0225949934674
-0.261933176616 0.0224469167283
-0.261052291383 0.0222992906521
-0.26017140615 0.0221521158144
-0.259290520917 0.0220053927862
-0.258409635684 0.0218591221343
-0.257528750451 0.0217133044215
-0.256647865218 0.0215679402063
-0.255766979985 0.021423030043
-0.254886094753 0.021278574482
-0.25400520952 0.0211345740695
-0.253124324287 0.0209910293478
-0.252243439054 0.0208479408551
-0.251362553821 0.0207053091259
-0.250481668588 0.0205631346905
-0.249600783355 0.0204214180756
-0.248719898122 0.0202801598039
-0.247839012889 0.0201393603943
-0.246958127656 0.0199990203622
-0.246077242423 0.0198591402189
-0.24519635719 0.0197197204724
-0.244315471957 0.0195807616267
-0.243434586725 0.0194422641823
-0.242553701492 0.0193042286362
-0.241672816259 0.0191666554817
-0.240791931026 0.0190295452087
-0.239911045793 0.0188928983034
-0.23903016056 0.0187567152488
-0.238149275327 0.0186209965243
-0.237268390094 0.0184857426058
-0.236387504861 0.018350953966
-0.235506619628 0.0182166310741
-0.234625734395 0.018082774396
-0.233744849162 0.0179493843945
-0.232863963929 0.0178164615288
-0.231983078697 0.017684006255
-0.231102193464 0.0175520190261
-0.230221308231 0.0174205002918
-0.229340422998 0.0172894504986
-0.228459537765 0.0171588700898
-0.227578652532 0.0170287595058
-0.226697767299 0.0168991191837
-0.225816882066 0.0167699495577
-0.224935996833 0.0166412510588
-0.2240551116 0.0165130241151
-0.223174226367 0.0163852691515
-0.222293341134 0.0162579865903
-0.221412455901 0.0161311768505
-0.220531570669 0.0160048403483
-0.219650685436 0.015878977497
-0.218769800203 0.015753588707
-0.21788891497 0.0156286743858
-0.217008029737 0.0155042349383
-0.216127144504 0.0153802707662
-0.215246259271 0.0152567822686
-0.214365374038 0.0151337698418
-0.213484488805 0.0150112338795
-0.212603603572 0.0148891747723
-0.211722718339 0.0147675929084
-0.210841833106 0.0146464886732
-0.209960947873 0.0145258624494
-0.209080062641 0.0144057146171
-0.208199177408 0.0142860455535
-0.207318292175 0.0141668556337
-0.206437406942 0.0140481452296
-0.205556521709 0.013929914711
-0.204675636476 0.0138121644449
-0.203794751243 0.0136948947956
-0.20291386601 0.0135781061252
-0.202032980777 0.0134617987931
-0.201152095544 0.0133459731563
-0.200271210311 0.0132306295691
-0.199390325078 0.0131157683835
-0.198509439846 0.0130013899492
-0.197628554613 0.0128874946131
-0.19674766938 0.0127740827199
-0.195866784147 0.012661154612
-0.194985898914 0.0125487106292
-0.194105013681 0.012436751109
-0.193224128448 0.0123252763867
-0.192343243215 0.012214286795
-0.191462357982 0.0121037826644
-0.190581472749 0.0119937643232
-0.189700587516 0.0118842320972
-0.188819702283 0.01177518631
-0.18793881705 0.011666627283
-0.187057931818 0.0115585553354
-0.186177046585 0.0114509707839
-0.185296161352 0.0113438739431
-0.184415276119 0.0112372651256
-0.183534390886 0.0111311446415
-0.182653505653 0.0110255127988
-0.18177262042 0.0109203699035
-0.180891735187 0.0108157162592
-0.180010849954 0.0107115521675
-0.179129964721 0.0106078779278
-0.178249079488 0.0105046938375
-0.177368194255 0.0104020001916
-0.176487309022 0.0102997972834
-0.17560642379 0.0101980854037
-0.174725538557 0.0100968648417
-0.173844653324 0.0099961358841
-0.172963768091 0.0098958988158
-0.172082882858 0.00979615391957
-0.171201997625 0.00969690147619
-0.170321112392 0.00959814176441
-0.169440227159 0.00949987506099
-0.168559341926 0.00940210164068
-0.167678456693 0.00930482177625
-0.16679757146 0.0092080357385
-0.165916686227 0.0091117437963
-0.165035800994 0.00901594621652
-0.164154915762 0.00892064326412
-0.163274030529 0.00882583520213
-0.162393145296 0.00873152229165
-0.161512260063 0.00863770479189
-0.16063137483 0.00854438296013
-0.159750489597 0.0084515570518
-0.158869604364 0.00835922732041
-0.157988719131 0.00826739401763
-0.157107833898 0.00817605739325
-0.156226948665 0.00808521769524
-0.155346063432 0.00799487516968
-0.154465178199 0.00790503006086
-0.153584292966 0.00781568261123
-0.152703407734 0.00772683306143
-0.151822522501 0.00763848165028
-0.150941637268 0.00755062861482
-0.150060752035 0.0074632741903
-0.149179866802 0.00737641861018
-0.148298981569 0.00729006210616
-0.147418096336 0.00720420490817
-0.146537211103 0.0071188472444
-0.14565632587 0.00703398934127
-0.144775440637 0.00694963142348
-0.143894555404 0.006865773714
-0.143013670171 0.00678241643407
-0.142132784938 0.00669955980323
-0.141251899706 0.00661720403928
-0.140371014473 0.00653534935837
-0.13949012924 0.00645399597492
-0.138609244007 0.00637314410169
-0.137728358774 0.00629279394974
-0.136847473541 0.0062129457285
-0.135966588308 0.00613359964569
-0.135085703075 0.00605475590741
-0.134204817842 0.00597641471811
-0.133323932609 0.00589857628059
-0.132443047376 0.00582124079602
-0.131562162143 0.00574440846394
-0.13068127691 0.00566807948229
-0.129800391678 0.00559225404736
-0.128919506445 0.00551693235387
-0.128038621212 0.00544211459493
-0.127157735979 0.00536780096204
-0.126276850746 0.00529399164515
-0.125395965513 0.00522068683258
-0.12451508028 0.00514788671113
-0.123634195047 0.00507559146598
-0.122753309814 0.0050038012808
-0.121872424581 0.00493251633766
-0.120991539348 0.0048617368171
-0.120110654115 0.00479146289813
-0.119229768882 0.0047216947582
-0.11834888365 0.00465243257324
-0.117467998417 0.00458367651765
-0.116587113184 0.0045154267643
-0.115706227951 0.00444768348456
-0.114825342718 0.0043804468483
-0.113944457485 0.00431371702386
-0.113063572252 0.00424749417809
-0.112182687019 0.00418177847636
-0.111301801786 0.00411657008255
-0.110420916553 0.00405186915903
-0.10954003132 0.00398767586673
-0.108659146087 0.00392399036509
-0.107778260854 0.00386081281208
-0.106897375622 0.00379814336421
-0.106016490389 0.00373598217654
-0.105135605156 0.00367432940268
-0.104254719923 0.00361318519477
-0.10337383469 0.00355254970354
-0.102492949457 0.00349242307825
-0.101612064224 0.00343280546675
-0.100731178991 0.00337369701545
-0.0998502937581 0.00331509786934
-0.0989694085252 0.00325700817199
-0.0980885232923 0.00319942806555
-0.0972076380594 0.00314235769076
-0.0963267528264 0.00308579718697
-0.0954458675935 0.00302974669211
-0.0945649823606 0.0029742063427
-0.0936840971277 0.00291917627391
-0.0928032118948 0.00286465661947
-0.0919223266618 0.00281064751175
-0.0910414414289 0.00275714908174
-0.090160556196 0.00270416145906
-0.0892796709631 0.00265168477192
-0.0883987857301 0.0025997191472
-0.0875179004972 0.00254826471039
-0.0866370152643 0.00249732158563
-0.0857561300314 0.00244688989569
-0.0848752447984 0.002396969762
-0.0839943595655 0.00234756130464
-0.0831134743326 0.00229866464231
-0.0822325890997 0.00225027989241
-0.0813517038668 0.00220240717097
-0.0804708186338 0.00215504659269
-0.0795899334009 0.00210819827093
-0.078709048168 0.00206186231775
-0.0778281629351 0.00201603884384
-0.0769472777021 0.00197072795859
-0.0760663924692 0.00192592977007
-0.0751855072363 0.00188164438503
-0.0743046220034 0.0018378719089
-0.0734237367704 0.0017946124458
-0.0725428515375 0.00175186609854
-0.0716619663046 0.00170963296864
-0.0707810810717 0.0016679131563
-0.0699001958388 0.00162670676043
-0.0690193106058 0.00158601387864
-0.0681384253729 0.00154583460725
-0.06725754014 0.00150616904128
-0.0663766549071 0.00146701727447
-0.0654957696741 0.00142837939927
-0.0646148844412 0.00139025550686
-0.0637339992083 0.00135264568712
-0.0628531139754 0.00131555002867
-0.0619722287425 0.00127896861884
-0.0610913435095 0.0012429015437
-0.0602104582766 0.00120734888804
-0.0593295730437 0.00117231073539
-0.0584486878108 0.00113778716802
-0.0575678025778 0.00110377826691
-0.0566869173449 0.00107028411182
-0.055806032112 0.00103730478121
-0.0549251468791 0.00100484035232
-0.0540442616461 0.000972890901111
-0.0531633764132 0.000941456502304
-0.0522824911803 0.000910537229369
-0.0514016059474 0.000880133154526
-0.0505207207145 0.000850244348751
-0.0496398354815 0.000820870881777
-0.0487589502486 0.000792012822093
-0.0478780650157 0.000763670236951
-0.0469971797828 0.000735843192365
-0.0461162945498 0.000708531753111
-0.0452354093169 0.000681735982734
-0.044354524084 0.000655455943544
-0.0434736388511 0.000629691696622
-0.0425927536181 0.00060444330182
-0.0417118683852 0.000579710817761
-0.0408309831523 0.000555494301847
-0.0399500979194 0.00053179381025
-0.0390692126865 0.000508609397925
-0.0381883274535 0.000485941118604
-0.0373074422206 0.000463789024798
-0.0364265569877 0.000442153167803
-0.0355456717548 0.000421033597697
-0.0346647865218 0.000400430363344
-0.0337839012889 0.000380343512392
-0.032903016056 0.00036077309128
-0.0320221308231 0.000341719145232
-0.0311412455901 0.000323181718267
-0.0302603603572 0.00030516085319
-0.0293794751243 0.000287656591603
-0.0284985898914 0.000270668973899
-0.0276177046585 0.000254198039267
-0.0267368194255 0.000238243825691
-0.0258559341926 0.000222806369953
-0.0249750489597 0.000207885707633
-0.0240941637268 0.000193481873109
-0.0232132784938 0.000179594899559
-0.0223323932609 0.000166224818963
-0.021451508028 0.0001533716621
-0.0205706227951 0.000141035458555
-0.0196897375622 0.000129216236715
-0.0188088523292 0.000117914023768
-0.0179279670963 0.000107128845713
-0.0170470818634 9.68607273482e-05
-0.0161661966305 8.71096922827e-05
-0.0152853113975 7.78757629304e-05
-0.0144044261646 6.9158960513e-05
-0.0135235409317 6.09593050604e-05
-0.0126426556988 5.32768154112e-05
-0.0117617704658 4.61115092129e-05
-0.0108808852329 3.94634029229e-05


==> figuresAndData/dataForConditionalVarianceCircularLevelSets.tex <==
-0.450442616461 0.12309389097
-0.450442616461 0.123093890969
-0.450442616461 0.123093890962
-0.450442616461 0.123093890945
-0.450442616461 0.123093890912
-0.450442616461 0.123093890857
-0.450442616461 0.123093890776
-0.450442616461 0.123093890662
-0.450442616461 0.12309389051
-0.450442616461 0.123093890315
-0.450442616461 0.123093890072
-0.450442616461 0.123093889775
-0.450442616461 0.123093889419
-0.450442616461 0.123093888998
-0.450442616461 0.123093888507
-0.450442616461 0.123093887941
-0.450442616461 0.123093887294
-0.450442616461 0.123093886561
-0.450442616461 0.123093885737
-0.450442616461 0.123093884815
-0.450442616461 0.123093883791
-0.450442616461 0.12309388266
-0.450442616461 0.123093881415
-0.450442616461 0.123093880052
-0.450442616461 0.123093878566
-0.450442616461 0.12309387695
-0.450442616461 0.123093875199
-0.450442616461 0.123093873309
-0.450442616461 0.123093871273
-0.450442616461 0.123093869086
-0.450442616461 0.123093866743
-0.450442616461 0.123093864239
-0.450442616461 0.123093861568
-0.450442616461 0.123093858725
-0.450442616461 0.123093855704
-0.450442616461 0.1230938525
-0.450442616461 0.123093849107
-0.450442616461 0.123093845521
-0.450442616461 0.123093841736
-0.450442616461 0.123093837746
-0.450442616461 0.123093833546
-0.450442616461 0.12309382913
-0.450442616461 0.123093824494
-0.450442616461 0.123093819632
-0.450442616461 0.123093814539
-0.450442616461 0.123093809209
-0.450442616461 0.123093803636
-0.450442616461 0.123093797816
-0.450442616461 0.123093791743
-0.450442616461 0.123093785411
-0.450442616461 0.123093778816
-0.450442616461 0.123093771952
-0.450442616461 0.123093764813
-0.450442616461 0.123093757394
-0.450442616461 0.12309374969
-0.450442616461 0.123093741695
-0.450442616461 0.123093733405
-0.450442616461 0.123093724813
-0.450442616461 0.123093715914
-0.450442616461 0.123093706703
-0.450442616461 0.123093697174
-0.450442616461 0.123093687322
-0.450442616461 0.123093677143
-0.450442616461 0.123093666629
-0.450442616461 0.123093655776
-0.450442616461 0.123093644579
-0.450442616461 0.123093633033
-0.450442616461 0.123093621131
-0.450442616461 0.123093608868
-0.450442616461 0.123093596239
-0.450442616461 0.12309358324
-0.450442616461 0.123093569863
-0.450442616461 0.123093556104
-0.450442616461 0.123093541958
-0.450442616461 0.123093527419
-0.450442616461 0.123093512482
-0.450442616461 0.123093497141
-0.450442616461 0.123093481392
-0.450442616461 0.123093465228
-0.450442616461 0.123093448644
-0.450442616461 0.123093431635
-0.450442616461 0.123093414196
-0.450442616461 0.123093396321
-0.450442616461 0.123093378005
-0.450442616461 0.123093359242
-0.450442616461 0.123093340027
-0.450442616461 0.123093320355
-0.450442616461 0.12309330022
-0.450442616461 0.123093279617
-0.450442616461 0.12309325854
-0.450442616461 0.123093236985
-0.450442616461 0.123093214945
-0.450442616461 0.123093192416
-0.450442616461 0.123093169392
-0.450442616461 0.123093145868
-0.450442616461 0.123093121838
-0.450442616461 0.123093097297
-0.450442616461 0.12309307224
-0.450442616461 0.12309304666
-0.450442616461 0.123093020554
-0.450442616461 0.123092993915
-0.450442616461 0.123092966738
-0.450442616461 0.123092939018
-0.450442616461 0.123092910749
-0.450442616461 0.123092881926
-0.450442616461 0.123092852544
-0.450442616461 0.123092822597
-0.450442616461 0.12309279208
-0.450442616461 0.123092760987
-0.450442616461 0.123092729313
-0.450442616461 0.123092697054
-0.450442616461 0.123092664202
-0.450442616461 0.123092630754
-0.450442616461 0.123092596703
-0.450442616461 0.123092562045
-0.450442616461 0.123092526773
-0.450442616461 0.123092490884
-0.450442616461 0.12309245437
-0.450442616461 0.123092417227
-0.450442616461 0.12309237945
-0.450442616461 0.123092341032
-0.450442616461 0.12309230197
-0.450442616461 0.123092262257
-0.450442616461 0.123092221888
-0.450442616461 0.123092180857
-0.450442616461 0.12309213916
-0.450442616461 0.123092096791
-0.450442616461 0.123092053744
-0.450442616461 0.123092010014
-0.450442616461 0.123091965597
-0.450442616461 0.123091920486
-0.450442616461 0.123091874676
-0.450442616461 0.123091828161
-0.450442616461 0.123091780937
-0.450442616461 0.123091732998
-0.450442616461 0.123091684339
-0.450442616461 0.123091634954
-0.450442616461 0.123091584838
-0.450442616461 0.123091533986
-0.450442616461 0.123091482392
-0.450442616461 0.12309143005
-0.450442616461 0.123091376957
-0.450442616461 0.123091323105
-0.450442616461 0.12309126849
-0.450442616461 0.123091213107
-0.450442616461 0.12309115695
-0.450442616461 0.123091100013
-0.450442616461 0.123091042292
-0.450442616461 0.123090983781
-0.450442616461 0.123090924475
-0.450442616461 0.123090864368
-0.450442616461 0.123090803455
-0.450442616461 0.12309074173
-0.450442616461 0.123090679189
-0.450442616461 0.123090615825
-0.450442616461 0.123090551635
-0.450442616461 0.123090486611
-0.450442616461 0.123090420749
-0.450442616461 0.123090354044
-0.450442616461 0.12309028649
-0.450442616461 0.123090218082
-0.450442616461 0.123090148814
-0.450442616461 0.123090078681
-0.450442616461 0.123090007678
-0.450442616461 0.123089935799
-0.450442616461 0.12308986304
-0.450442616461 0.123089789394
-0.450442616461 0.123089714857
-0.450442616461 0.123089639422
-0.450442616461 0.123089563085
-0.450442616461 0.123089485841
-0.450442616461 0.123089407683
-0.450442616461 0.123089328607
-0.450442616461 0.123089248608
-0.450442616461 0.123089167679
-0.450442616461 0.123089085816
-0.450442616461 0.123089003013
-0.450442616461 0.123088919265
-0.450442616461 0.123088834567
-0.450442616461 0.123088748913
-0.450442616461 0.123088662297
-0.450442616461 0.123088574716
-0.450442616461 0.123088486162
-0.450442616461 0.123088396631
-0.450442616461 0.123088306118
-0.450442616461 0.123088214617
-0.450442616461 0.123088122123
-0.450442616461 0.12308802863
-0.450442616461 0.123087934134
-0.450442616461 0.123087838628
-0.450442616461 0.123087742108
-0.450442616461 0.123087644568
-0.450442616461 0.123087546003
-0.450442616461 0.123087446407
-0.450442616461 0.123087345776
-0.450442616461 0.123087244103
-0.450442616461 0.123087141384
-0.450442616461 0.123087037612
-0.450442616461 0.123086932784
-0.450442616461 0.123086826893
-0.450442616461 0.123086719934
-0.450442616461 0.123086611903
-0.450442616461 0.123086502792
-0.450442616461 0.123086392598
-0.450442616461 0.123086281314
-0.450442616461 0.123086168936
-0.450442616461 0.123086055459
-0.450442616461 0.123085940876
-0.450442616461 0.123085825182
-0.450442616461 0.123085708373
-0.450442616461 0.123085590442
-0.450442616461 0.123085471386
-0.450442616461 0.123085351197
-0.450442616461 0.123085229871
-0.450442616461 0.123085107403
-0.450442616461 0.123084983787
-0.450442616461 0.123084859017
-0.450442616461 0.12308473309
-0.450442616461 0.123084605998
-0.450442616461 0.123084477738
-0.450442616461 0.123084348303
-0.450442616461 0.123084217689
-0.450442616461 0.123084085889
-0.450442616461 0.123083952899
-0.450442616461 0.123083818714
-0.450442616461 0.123083683327
-0.450442616461 0.123083546734
-0.450442616461 0.12308340893
-0.450442616461 0.123083269908
-0.450442616461 0.123083129665
-0.450442616461 0.123082988193
-0.450442616461 0.123082845489
-0.450442616461 0.123082701547
-0.450442616461 0.123082556361
-0.450442616461 0.123082409926
-0.450442616461 0.123082262237
-0.450442616461 0.123082113289
-0.450442616461 0.123081963075
-0.450442616461 0.123081811592
-0.450442616461 0.123081658834
-0.450442616461 0.123081504794
-0.450442616461 0.123081349469
-0.450442616461 0.123081192852
-0.450442616461 0.123081034939
-0.450442616461 0.123080875723
-0.450442616461 0.123080715201
-0.450442616461 0.123080553366
-0.450442616461 0.123080390213
-0.450442616461 0.123080225737
-0.450442616461 0.123080059932
-0.450442616461 0.123079892794
-0.450442616461 0.123079724316
-0.450442616461 0.123079554494
-0.450442616461 0.123079383323
-0.450442616461 0.123079210796
-0.450442616461 0.123079036909
-0.450442616461 0.123078861657
-0.450442616461 0.123078685033
-0.450442616461 0.123078507034
-0.450442616461 0.123078327653
-0.450442616461 0.123078146885
-0.450442616461 0.123077964725
-0.450442616461 0.123077781168
-0.450442616461 0.123077596208
-0.450442616461 0.12307740984
-0.450442616461 0.123077222059
-0.450442616461 0.123077032859
-0.450442616461 0.123076842235
-0.450442616461 0.123076650182
-0.450442616461 0.123076456695
-0.450442616461 0.123076261768
-0.450442616461 0.123076065396
-0.450442616461 0.123075867573
-0.450442616461 0.123075668295
-0.450442616461 0.123075467556
-0.450442616461 0.123075265351
-0.450442616461 0.123075061675
-0.450442616461 0.123074856521
-0.450442616461 0.123074649886
-0.450442616461 0.123074441763
-0.450442616461 0.123074232148
-0.450442616461 0.123074021034
-0.450442616461 0.123073808418
-0.450442616461 0.123073594293
-0.450442616461 0.123073378654
-0.450442616461 0.123073161496
-0.450442616461 0.123072942814
-0.450442616461 0.123072722602
-0.450442616461 0.123072500856
-0.450442616461 0.123072277569
-0.450442616461 0.123072052737
-0.450442616461 0.123071826354
-0.450442616461 0.123071598415
-0.450442616461 0.123071368915
-0.450442616461 0.123071137848
-0.450442616461 0.123070905209
-0.450442616461 0.123070670994
-0.450442616461 0.123070435196
-0.450442616461 0.12307019781
-0.450442616461 0.123069958831
-0.450442616461 0.123069718254
-0.450442616461 0.123069476074
-0.450442616461 0.123069232285
-0.450442616461 0.123068986882
-0.450442616461 0.12306873986
-0.450442616461 0.123068491213
-0.450442616461 0.123068240936
-0.450442616461 0.123067989025
-0.450442616461 0.123067735472
-0.450442616461 0.123067480275
-0.450442616461 0.123067223426
-0.450442616461 0.123066964922
-0.450442616461 0.123066704755
-0.450442616461 0.123066442923
-0.450442616461 0.123066179418
-0.450442616461 0.123065914236
-0.450442616461 0.123065647372
-0.450442616461 0.12306537882
-0.450442616461 0.123065108575
-0.450442616461 0.123064836632
-0.450442616461 0.123064562985
-0.450442616461 0.12306428763
-0.450442616461 0.12306401056
-0.450442616461 0.123063731772
-0.450442616461 0.123063451258
-0.450442616461 0.123063169016
-0.450442616461 0.123062885038
-0.450442616461 0.12306259932
-0.450442616461 0.123062311856
-0.450442616461 0.123062022641
-0.450442616461 0.123061731671
-0.450442616461 0.123061438939
-0.450442616461 0.123061144441
-0.450442616461 0.123060848171
-0.450442616461 0.123060550124
-0.450442616461 0.123060250295
-0.450442616461 0.123059948678
-0.450442616461 0.123059645269
-0.450442616461 0.123059340062
-0.450442616461 0.123059033051
-0.450442616461 0.123058724232
-0.450442616461 0.123058413599
-0.450442616461 0.123058101148
-0.450442616461 0.123057786872
-0.450442616461 0.123057470766
-0.450442616461 0.123057152826
-0.450442616461 0.123056833046
-0.450442616461 0.123056511421
-0.450442616461 0.123056187946
-0.450442616461 0.123055862615
-0.450442616461 0.123055535423
-0.450442616461 0.123055206365
-0.450442616461 0.123054875436
-0.450442616461 0.12305454263
-0.450442616461 0.123054207943
-0.450442616461 0.123053871368
-0.450442616461 0.123053532901
-0.450442616461 0.123053192537
-0.450442616461 0.12305285027
-0.450442616461 0.123052506095
-0.450442616461 0.123052160008
-0.450442616461 0.123051812001
-0.450442616461 0.123051462071
-0.450442616461 0.123051110213
-0.450442616461 0.12305075642
-0.450442616461 0.123050400688
-0.450442616461 0.123050043011
-0.450442616461 0.123049683385
-0.450442616461 0.123049321804
-0.450442616461 0.123048958263
-0.450442616461 0.123048592756
-0.450442616461 0.123048225279
-0.450442616461 0.123047855826
-0.450442616461 0.123047484392
-0.450442616461 0.123047110972
-0.450442616461 0.123046735561
-0.450442616461 0.123046358152
-0.450442616461 0.123045978742
-0.450442616461 0.123045597325
-0.450442616461 0.123045213896
-0.450442616461 0.123044828449
-0.450442616461 0.123044440979
-0.450442616461 0.123044051482
-0.450442616461 0.123043659951
-0.450442616461 0.123043266382
-0.450442616461 0.12304287077
-0.450442616461 0.123042473108
-0.450442616461 0.123042073393
-0.450442616461 0.123041671619
-0.450442616461 0.123041267781
-0.450442616461 0.123040861872
-0.450442616461 0.12304045389
-0.450442616461 0.123040043827
-0.450442616461 0.123039631679
-0.450442616461 0.123039217441
-0.450442616461 0.123038801107
-0.450442616461 0.123038382673
-0.450442616461 0.123037962132
-0.450442616461 0.123037539481
-0.450442616461 0.123037114713
-0.450442616461 0.123036687824
-0.450442616461 0.123036258808
-0.450442616461 0.12303582766
-0.450442616461 0.123035394375
-0.450442616461 0.123034958948
-0.450442616461 0.123034521373
-0.450442616461 0.123034081646
-0.450442616461 0.123033639761
-0.450442616461 0.123033195713
-0.450442616461 0.123032749497
-0.450442616461 0.123032301107
-0.450442616461 0.123031850539
-0.450442616461 0.123031397787
-0.450442616461 0.123030942846
-0.450442616461 0.123030485711
-0.450442616461 0.123030026377
-0.450442616461 0.123029564839
-0.450442616461 0.12302910109
-0.450442616461 0.123028635127
-0.450442616461 0.123028166944
-0.450442616461 0.123027696536
-0.450442616461 0.123027223898
-0.450442616461 0.123026749024
-0.450442616461 0.123026271909
-0.450442616461 0.123025792549
-0.450442616461 0.123025310938
-0.450442616461 0.12302482707
-0.450442616461 0.123024340941
-0.450442616461 0.123023852546
-0.450442616461 0.123023361878
-0.450442616461 0.123022868934
-0.450442616461 0.123022373708
-0.450442616461 0.123021876195
-0.450442616461 0.12302137639
-0.450442616461 0.123020874287
-0.450442616461 0.123020369881
-0.450442616461 0.123019863168
-0.450442616461 0.123019354142
-0.450442616461 0.123018842797
-0.450442616461 0.123018329129
-0.450442616461 0.123017813133
-0.450442616461 0.123017294803
-0.450442616461 0.123016774135
-0.450442616461 0.123016251122
-0.450442616461 0.123015725761
-0.450442616461 0.123015198045
-0.450442616461 0.12301466797
-0.450442616461 0.12301413553
-0.450442616461 0.123013600721
-0.450442616461 0.123013063537
-0.450442616461 0.123012523973
-0.450442616461 0.123011982024
-0.450442616461 0.123011437685
-0.450442616461 0.123010890951
-0.450442616461 0.123010341816
-0.450442616461 0.123009790275
-0.450442616461 0.123009236323
-0.450442616461 0.123008679956
-0.450442616461 0.123008121167
-0.450442616461 0.123007559952
-0.450442616461 0.123006996306
-0.450442616461 0.123006430224
-0.450442616461 0.123005861699
-0.450442616461 0.123005290729
-0.450442616461 0.123004717306
-0.450442616461 0.123004141426
-0.450442616461 0.123003563084
-0.450442616461 0.123002982275
-0.450442616461 0.123002398993
-0.450442616461 0.123001813234
-0.450442616461 0.123001224992
-0.450442616461 0.123000634262
-0.450442616461 0.12300004104
-0.450442616461 0.122999445319
-0.450442616461 0.122998847096
-0.450442616461 0.122998246364
-0.450442616461 0.122997643118
-0.450442616461 0.122997037354
-0.450442616461 0.122996429067
-0.450442616461 0.122995818251
-0.450442616461 0.122995204901
-0.450442616461 0.122994589011
-0.450442616461 0.122993970578
-0.450442616461 0.122993349596
-0.450442616461 0.122992726059
-0.450442616461 0.122992099963
-0.450442616461 0.122991471302
-0.450442616461 0.122990840072
-0.450442616461 0.122990206267
-0.450442616461 0.122989569882
-0.450442616461 0.122988930912
-0.450442616461 0.122988289352
-0.450442616461 0.122987645197
-0.450442616461 0.122986998441
-0.450442616461 0.122986349081
-0.450442616461 0.122985697109
-0.450442616461 0.122985042522
-0.450442616461 0.122984385315
-0.450442616461 0.122983725481
-0.450442616461 0.122983063017
-0.450442616461 0.122982397917
-0.450442616461 0.122981730175
-0.450442616461 0.122981059788
-0.450442616461 0.122980386749
-0.450442616461 0.122979711054
-0.450442616461 0.122979032698
-0.450442616461 0.122978351674
-0.450442616461 0.12297766798
-0.450442616461 0.122976981608
-0.450442616461 0.122976292555
-0.450442616461 0.122975600815
-0.450442616461 0.122974906383
-0.450442616461 0.122974209254
-0.450442616461 0.122973509423
-0.450442616461 0.122972806884
-0.450442616461 0.122972101633
-0.450442616461 0.122971393665
-0.450442616461 0.122970682975
-0.450442616461 0.122969969556
-0.450442616461 0.122969253406
-0.450442616461 0.122968534517
-0.450442616461 0.122967812886
-0.450442616461 0.122967088507
-0.450442616461 0.122966361375
-0.450442616461 0.122965631485
-0.450442616461 0.122964898833
-0.450442616461 0.122964163412
-0.450442616461 0.122963425217
-0.450442616461 0.122962684245
-0.450442616461 0.122961940489
-0.450442616461 0.122961193945
-0.450442616461 0.122960444608
-0.450442616461 0.122959692472
-0.450442616461 0.122958937532
-0.450442616461 0.122958179784
-0.450442616461 0.122957419222
-0.450442616461 0.122956655841
-0.450442616461 0.122955889637
-0.450442616461 0.122955120603
-0.450442616461 0.122954348736
-0.450442616461 0.12295357403
-0.450442616461 0.12295279648
-0.450442616461 0.122952016081
-0.450442616461 0.122951232827
-0.450442616461 0.122950446715
-0.450442616461 0.122949657738
-0.450442616461 0.122948865892
-0.450442616461 0.122948071172
-0.450442616461 0.122947273572
-0.450442616461 0.122946473088
-0.450442616461 0.122945669715
-0.450442616461 0.122944863447
-0.450442616461 0.122944054279
-0.450442616461 0.122943242207
-0.450442616461 0.122942427226
-0.450442616461 0.12294160933
-0.450442616461 0.122940788514
-0.450442616461 0.122939964773
-0.450442616461 0.122939138103
-0.450442616461 0.122938308498
-0.450442616461 0.122937475953
-0.450442616461 0.122936640463
-0.450442616461 0.122935802023
-0.450442616461 0.122934960629
-0.450442616461 0.122934116274
-0.450442616461 0.122933268955
-0.450442616461 0.122932418666
-0.450442616461 0.122931565402
-0.450442616461 0.122930709157
-0.450442616461 0.122929849928
-0.450442616461 0.122928987708
-0.450442616461 0.122928122494
-0.450442616461 0.122927254279
-0.450442616461 0.12292638306
-0.450442616461 0.12292550883
-0.450442616461 0.122924631585
-0.450442616461 0.12292375132
-0.450442616461 0.122922868029
-0.450442616461 0.122921981709
-0.450442616461 0.122921092353
-0.450442616461 0.122920199957
-0.450442616461 0.122919304516
-0.450442616461 0.122918406025
-0.450442616461 0.122917504479
-0.450442616461 0.122916599872
-0.450442616461 0.1229156922
-0.450442616461 0.122914781458
-0.450442616461 0.12291386764
-0.450442616461 0.122912950743
-0.450442616461 0.12291203076
-0.450442616461 0.122911107687
-0.450442616461 0.122910181518
-0.450442616461 0.12290925225
-0.450442616461 0.122908319876
-0.450442616461 0.122907384392
-0.450442616461 0.122906445793
-0.450442616461 0.122905504073
-0.450442616461 0.122904559229
-0.450442616461 0.122903611254
-0.450442616461 0.122902660144
-0.450442616461 0.122901705894
-0.450442616461 0.122900748499
-0.450442616461 0.122899787954
-0.450442616461 0.122898824253
-0.450442616461 0.122897857393
-0.450442616461 0.122896887368
-0.450442616461 0.122895914172
-0.450442616461 0.122894937801
-0.450442616461 0.122893958251
-0.450442616461 0.122892975515
-0.450442616461 0.12289198959
-0.450442616461 0.12289100047
-0.450442616461 0.122890008149
-0.450442616461 0.122889012624
-0.450442616461 0.122888013889
-0.450442616461 0.12288701194
-0.450442616461 0.12288600677
-0.450442616461 0.122884998376
-0.450442616461 0.122883986752
-0.450442616461 0.122882971893
-0.450442616461 0.122881953795
-0.450442616461 0.122880932452
-0.450442616461 0.12287990786
-0.450442616461 0.122878880013
-0.450442616461 0.122877848907
-0.450442616461 0.122876814536
-0.450442616461 0.122875776896
-0.450442616461 0.122874735982
-0.450442616461 0.122873691788
-0.450442616461 0.12287264431
-0.450442616461 0.122871593543
-0.450442616461 0.122870539482
-0.450442616461 0.122869482121
-0.450442616461 0.122868421457
-0.450442616461 0.122867357484
-0.450442616461 0.122866290196
-0.450442616461 0.12286521959
-0.450442616461 0.12286414566
-0.450442616461 0.122863068402
-0.450442616461 0.122861987809
-0.450442616461 0.122860903878
-0.450442616461 0.122859816603
-0.450442616461 0.12285872598
-0.450442616461 0.122857632004
-0.450442616461 0.122856534669
-0.450442616461 0.122855433971
-0.450442616461 0.122854329904
-0.450442616461 0.122853222465
-0.450442616461 0.122852111647
-0.450442616461 0.122850997446
-0.450442616461 0.122849879857
-0.450442616461 0.122848758876
-0.450442616461 0.122847634496
-0.450442616461 0.122846506714
-0.450442616461 0.122845375524
-0.450442616461 0.122844240922
-0.450442616461 0.122843102902
-0.450442616461 0.12284196146
-0.450442616461 0.12284081659
-0.450442616461 0.122839668289
-0.450442616461 0.12283851655
-0.450442616461 0.122837361369
-0.450442616461 0.122836202741
-0.450442616461 0.122835040661
-0.450442616461 0.122833875124
-0.450442616461 0.122832706125
-0.450442616461 0.12283153366
-0.450442616461 0.122830357724
-0.450442616461 0.122829178311
-0.450442616461 0.122827995416
-0.450442616461 0.122826809036
-0.450442616461 0.122825619164
-0.450442616461 0.122824425796
-0.450442616461 0.122823228928
-0.450442616461 0.122822028553
-0.450442616461 0.122820824668
-0.450442616461 0.122819617267
-0.450442616461 0.122818406345
-0.450442616461 0.122817191899
-0.450442616461 0.122815973921
-0.450442616461 0.122814752409
-0.450442616461 0.122813527357
-0.450442616461 0.122812298759
-0.450442616461 0.122811066612
-0.450442616461 0.12280983091
-0.450442616461 0.122808591648
-0.450442616461 0.122807348822
-0.450442616461 0.122806102427
-0.450442616461 0.122804852457
-0.450442616461 0.122803598908
-0.450442616461 0.122802341775
-0.450442616461 0.122801081053
-0.450442616461 0.122799816737
-0.450442616461 0.122798548823
-0.450442616461 0.122797277305
-0.450442616461 0.122796002179
-0.450442616461 0.122794723439
-0.450442616461 0.122793441082
-0.450442616461 0.122792155101
-0.450442616461 0.122790865493
-0.450442616461 0.122789572251
-0.450442616461 0.122788275372
-0.450442616461 0.122786974851
-0.450442616461 0.122785670682
-0.450442616461 0.122784362862
-0.450442616461 0.122783051384
-0.450442616461 0.122781736244
-0.450442616461 0.122780417437
-0.450442616461 0.122779094959
-0.450442616461 0.122777768805
-0.450442616461 0.122776438969
-0.450442616461 0.122775105447
-0.450442616461 0.122773768234
-0.450442616461 0.122772427325
-0.450442616461 0.122771082715
-0.450442616461 0.1227697344
-0.450442616461 0.122768382374
-0.450442616461 0.122767026633
-0.450442616461 0.122765667172
-0.450442616461 0.122764303986
-0.450442616461 0.12276293707
-0.450442616461 0.12276156642
-0.450442616461 0.12276019203
-0.450442616461 0.122758813896
-0.450442616461 0.122757432013
-0.450442616461 0.122756046376
-0.450442616461 0.12275465698
-0.450442616461 0.12275326382
-0.450442616461 0.122751866892
-0.450442616461 0.122750466191
-0.450442616461 0.122749061712
-0.450442616461 0.122747653449
-0.450442616461 0.122746241399
-0.450442616461 0.122744825557
-0.450442616461 0.122743405916
-0.450442616461 0.122741982474
-0.450442616461 0.122740555225
-0.450442616461 0.122739124164
-0.450442616461 0.122737689286
-0.450442616461 0.122736250587
-0.450442616461 0.122734808061
-0.450442616461 0.122733361704
-0.450442616461 0.122731911512
-0.450442616461 0.122730457478
-0.450442616461 0.122728999599
-0.450442616461 0.12272753787
-0.450442616461 0.122726072286
-0.450442616461 0.122724602841
-0.450442616461 0.122723129532
-0.450442616461 0.122721652354
-0.450442616461 0.1227201713
-0.450442616461 0.122718686368
-0.450442616461 0.122717197552
-0.450442616461 0.122715704847
-0.450442616461 0.122714208248
-0.450442616461 0.122712707751
-0.450442616461 0.122711203351
-0.450442616461 0.122709695043
-0.450442616461 0.122708182823
-0.450442616461 0.122706666684
-0.450442616461 0.122705146624
-0.450442616461 0.122703622636
-0.450442616461 0.122702094717
-0.450442616461 0.12270056286
-0.450442616461 0.122699027063
-0.450442616461 0.122697487319
-0.450442616461 0.122695943624
-0.450442616461 0.122694395973
-0.450442616461 0.122692844362
-0.450442616461 0.122691288785
-0.450442616461 0.122689729238
-0.450442616461 0.122688165717
-0.450442616461 0.122686598216
-0.450442616461 0.12268502673
-0.450442616461 0.122683451255
-0.450442616461 0.122681871786
-0.450442616461 0.122680288318
-0.450442616461 0.122678700847
-0.450442616461 0.122677109368
-0.450442616461 0.122675513875
-0.450442616461 0.122673914365
-0.450442616461 0.122672310832
-0.450442616461 0.122670703272
-0.450442616461 0.12266909168
-0.450442616461 0.122667476051
-0.450442616461 0.12266585638
-0.450442616461 0.122664232663
-0.450442616461 0.122662604895
-0.450442616461 0.122660973071
-0.450442616461 0.122659337187
-0.450442616461 0.122657697237
-0.450442616461 0.122656053217
-0.450442616461 0.122654405122
-0.450442616461 0.122652752948
-0.450442616461 0.122651096689
-0.450442616461 0.122649436342
-0.450442616461 0.1226477719
-0.450442616461 0.12264610336
-0.450442616461 0.122644430717
-0.450442616461 0.122642753965
-0.450442616461 0.122641073101
-0.450442616461 0.12263938812
-0.450442616461 0.122637699016
-0.450442616461 0.122636005785
-0.450442616461 0.122634308423
-0.450442616461 0.122632606924
-0.450442616461 0.122630901284
-0.450442616461 0.122629191498
-0.450442616461 0.122627477562
-0.450442616461 0.12262575947
-0.450442616461 0.122624037218
-0.450442616461 0.122622310802
-0.450442616461 0.122620580216
-0.450442616461 0.122618845455
-0.450442616461 0.122617106516
-0.450442616461 0.122615363394
-0.450442616461 0.122613616082
-0.450442616461 0.122611864578
-0.450442616461 0.122610108877
-0.450442616461 0.122608348972
-0.450442616461 0.122606584861
-0.450442616461 0.122604816537
-0.450442616461 0.122603043997
-0.450442616461 0.122601267236
-0.450442616461 0.122599486249
-0.450442616461 0.122597701031
-0.450442616461 0.122595911578
-0.450442616461 0.122594117884
-0.450442616461 0.122592319946
-0.450442616461 0.122590517758
-0.450442616461 0.122588711316
-0.450442616461 0.122586900616
-0.450442616461 0.122585085651
-0.450442616461 0.122583266419
-0.450442616461 0.122581442913
-0.450442616461 0.12257961513
-0.450442616461 0.122577783065
-0.450442616461 0.122575946712
-0.450442616461 0.122574106068
-0.450442616461 0.122572261127
-0.450442616461 0.122570411886
-0.450442616461 0.122568558338
-0.450442616461 0.12256670048
-0.450442616461 0.122564838308
-0.450442616461 0.122562971815
-0.450442616461 0.122561100998
-0.450442616461 0.122559225852
-0.450442616461 0.122557346372
-0.450442616461 0.122555462553
-0.450442616461 0.122553574392
-0.450442616461 0.122551681882
-0.450442616461 0.122549785021
-0.450442616461 0.122547883802
-0.450442616461 0.122545978221
-0.450442616461 0.122544068274
-0.450442616461 0.122542153955
-0.450442616461 0.122540235261
-0.450442616461 0.122538312187
-0.450442616461 0.122536384727
-0.450442616461 0.122534452878
-0.450442616461 0.122532516634
-0.450442616461 0.122530575992
-0.450442616461 0.122528630945
-0.450442616461 0.12252668149
-0.450442616461 0.122524727623
-0.450442616461 0.122522769337
-0.450442616461 0.122520806629
-0.450442616461 0.122518839495
-0.450442616461 0.122516867929
-0.450442616461 0.122514891926
-0.450442616461 0.122512911483
-0.450442616461 0.122510926594
-0.450442616461 0.122508937255
-0.450442616461 0.122506943461
-0.450442616461 0.122504945208
-0.450442616461 0.122502942491
-0.450442616461 0.122500935305
-0.450442616461 0.122498923646
-0.450442616461 0.122496907509
-0.450442616461 0.12249488689
-0.450442616461 0.122492861783
-0.450442616461 0.122490832185
-0.450442616461 0.12248879809
-0.450442616461 0.122486759494
-0.450442616461 0.122484716392
-0.450442616461 0.12248266878
-0.450442616461 0.122480616653
-0.450442616461 0.122478560007
-0.450442616461 0.122476498836
-0.450442616461 0.122474433137
-0.450442616461 0.122472362904
-0.450442616461 0.122470288133
-0.450442616461 0.12246820882
-0.450442616461 0.12246612496
-0.450442616461 0.122464036547
-0.450442616461 0.122461943579
-0.450442616461 0.122459846049
-0.450442616461 0.122457743954
-0.450442616461 0.122455637288
-0.450442616461 0.122453526048
-0.450442616461 0.122451410228
-0.450442616461 0.122449289824
-0.450442616461 0.122447164832
-0.450442616461 0.122445035247
-0.450442616461 0.122442901063
-0.450442616461 0.122440762278
-0.450442616461 0.122438618885
-0.450442616461 0.122436470881
-0.450442616461 0.12243431826
-0.450442616461 0.122432161019
-0.450442616461 0.122429999152
-0.450442616461 0.122427832656
-0.450442616461 0.122425661525
-0.450442616461 0.122423485755
-0.450442616461 0.122421305342
-0.450442616461 0.12241912028
-0.450442616461 0.122416930565
-0.450442616461 0.122414736193
-0.450442616461 0.122412537159
-0.450442616461 0.122410333459
-0.450442616461 0.122408125087
-0.450442616461 0.12240591204
-0.450442616461 0.122403694313
-0.450442616461 0.1224014719
-0.450442616461 0.122399244799
-0.450442616461 0.122397013003
-0.450442616461 0.122394776509
-0.450442616461 0.122392535312
-0.450442616461 0.122390289408
-0.450442616461 0.122388038791
-0.450442616461 0.122385783457
-0.450442616461 0.122383523402
-0.450442616461 0.122381258622
-0.450442616461 0.122378989111
-0.450442616461 0.122376714865
-0.450442616461 0.122374435879
-0.450442616461 0.12237215215
-0.450442616461 0.122369863672
-0.450442616461 0.122367570441
-0.450442616461 0.122365272452
-0.450442616461 0.122362969701
-0.450442616461 0.122360662183
-0.450442616461 0.122358349894
-0.450442616461 0.122356032829
-0.450442616461 0.122353710984
-0.450442616461 0.122351384354
-0.450442616461 0.122349052934
-0.450442616461 0.122346716721
-0.450442616461 0.122344375709
-0.450442616461 0.122342029894
-0.450442616461 0.122339679271
-0.450442616461 0.122337323836
-0.450442616461 0.122334963585
-0.450442616461 0.122332598512
-0.450442616461 0.122330228614
-0.450442616461 0.122327853886
-0.450442616461 0.122325474323
-0.450442616461 0.122323089921
-0.450442616461 0.122320700675
-0.450442616461 0.122318306581
-0.450442616461 0.122315907634
-0.450442616461 0.12231350383
-0.450442616461 0.122311095164
-0.450442616461 0.122308681632
-0.450442616461 0.122306263228
-0.450442616461 0.12230383995
-0.450442616461 0.122301411792
-0.450442616461 0.122298978749
-0.450442616461 0.122296540818
-0.450442616461 0.122294097993
-0.450442616461 0.122291650271
-0.450442616461 0.122289197646
-0.450442616461 0.122286740115
-0.450442616461 0.122284277672
-0.450442616461 0.122281810313
-0.450442616461 0.122279338034
-0.450442616461 0.12227686083
-0.450442616461 0.122274378697
-0.450442616461 0.12227189163
-0.450442616461 0.122269399625
-0.450442616461 0.122266902677
-0.450442616461 0.122264400782
-0.450442616461 0.122261893935
-0.450442616461 0.122259382132
-0.450442616461 0.122256865368
-0.450442616461 0.12225434364
-0.450442616461 0.122251816941
-0.450442616461 0.122249285269
-0.450442616461 0.122246748617
-0.450442616461 0.122244206983
-0.450442616461 0.122241660361
-0.450442616461 0.122239108748
-0.450442616461 0.122236552138
-0.450442616461 0.122233990526
-0.450442616461 0.12223142391
-0.450442616461 0.122228852284
-0.450442616461 0.122226275643
-0.450442616461 0.122223693983
-0.450442616461 0.122221107301
-0.450442616461 0.12221851559
-0.450442616461 0.122215918848
-0.450442616461 0.122213317068
-0.450442616461 0.122210710248
-0.450442616461 0.122208098382
-0.450442616461 0.122205481467
-0.450442616461 0.122202859496
-0.450442616461 0.122200232467
-0.450442616461 0.122197600375
-0.450442616461 0.122194963215
-0.450442616461 0.122192320982
-0.450442616461 0.122189673673
-0.450442616461 0.122187021283
-0.450442616461 0.122184363807
-0.450442616461 0.122181701242
-0.450442616461 0.122179033582
-0.450442616461 0.122176360823
-0.450442616461 0.122173682961
-0.450442616461 0.122170999991
-0.450442616461 0.122168311909
-0.450442616461 0.12216561871
-0.450442616461 0.122162920391
-0.450442616461 0.122160216945
-0.450442616461 0.122157508371
-0.450442616461 0.122154794661
-0.450442616461 0.122152075813
-0.450442616461 0.122149351822
-0.450442616461 0.122146622684
-0.450442616461 0.122143888393
-0.450442616461 0.122141148946
-0.450442616461 0.122138404339
-0.450442616461 0.122135654566
-0.450442616461 0.122132899623
-0.450442616461 0.122130139507
-0.450442616461 0.122127374212
-0.450442616461 0.122124603734
-0.450442616461 0.122121828069
-0.450442616461 0.122119047212
-0.450442616461 0.122116261159
-0.450442616461 0.122113469905
-0.450442616461 0.122110673447
-0.450442616461 0.12210787178
-0.450442616461 0.122105064898
-0.450442616461 0.122102252799
-0.450442616461 0.122099435477
-0.450442616461 0.122096612929
-0.450442616461 0.122093785149
-0.450442616461 0.122090952134
-0.450442616461 0.122088113878
-0.450442616461 0.122085270378
-0.450442616461 0.122082421629
-0.450442616461 0.122079567627
-0.450442616461 0.122076708368
-0.450442616461 0.122073843846
-0.450442616461 0.122070974058
-0.450442616461 0.122068099
-0.450442616461 0.122065218666
-0.450442616461 0.122062333053
-0.450442616461 0.122059442156
-0.450442616461 0.122056545971
-0.450442616461 0.122053644493
-0.450442616461 0.122050737718
-0.450442616461 0.122047825642
-0.450442616461 0.12204490826
-0.450442616461 0.122041985568
-0.450442616461 0.122039057562
-0.450442616461 0.122036124237
-0.450442616461 0.122033185588
-0.450442616461 0.122030241612
-0.450442616461 0.122027292305
-0.450442616461 0.122024337661
-0.450442616461 0.122021377676
-0.450442616461 0.122018412346
-0.450442616461 0.122015441667
-0.450442616461 0.122012465635
-0.450442616461 0.122009484244
-0.450442616461 0.122006497491
-0.450442616461 0.122003505372
-0.450442616461 0.122000507881
-0.450442616461 0.121997505015
-0.450442616461 0.121994496769
-0.450442616461 0.121991483139
-0.450442616461 0.121988464121
-0.450442616461 0.121985439709
-0.450442616461 0.121982409901
-0.450442616461 0.121979374691
-0.450442616461 0.121976334076
-0.450442616461 0.12197328805
-0.450442616461 0.12197023661
-0.450442616461 0.121967179751
-0.450442616461 0.121964117469
-0.450442616461 0.12196104976
-0.450442616461 0.121957976619
-0.450442616461 0.121954898042
-0.450442616461 0.121951814024
-0.450442616461 0.121948724562
-0.450442616461 0.12194562965
-0.450442616461 0.121942529285
-0.450442616461 0.121939423463
-0.450442616461 0.121936312178
-0.450442616461 0.121933195428
-0.450442616461 0.121930073206
-0.450442616461 0.12192694551
-0.450442616461 0.121923812334
-0.450442616461 0.121920673675
-0.450442616461 0.121917529528
-0.450442616461 0.121914379888
-0.450442616461 0.121911224753
-0.450442616461 0.121908064116
-0.450442616461 0.121904897974
-0.450442616461 0.121901726323
-0.450442616461 0.121898549159
-0.450442616461 0.121895366476
-0.450442616461 0.121892178271
-0.450442616461 0.12188898454
-0.450442616461 0.121885785277
-0.450442616461 0.12188258048
-0.450442616461 0.121879370142
-0.450442616461 0.121876154262
-0.450442616461 0.121872932833
-0.450442616461 0.121869705852
-0.450442616461 0.121866473314
-0.450442616461 0.121863235215
-0.450442616461 0.121859991552
-0.450442616461 0.121856742318
-0.450442616461 0.121853487512
-0.450442616461 0.121850227127
-0.450442616461 0.121846961159
-0.450442616461 0.121843689606
-0.450442616461 0.121840412461
-0.450442616461 0.121837129721
-0.450442616461 0.121833841382
-0.450442616461 0.12183054744
-0.450442616461 0.121827247889
-0.450442616461 0.121823942726
-0.450442616461 0.121820631947
-0.450442616461 0.121817315547
-0.450442616461 0.121813993523
-0.450442616461 0.121810665869
-0.450442616461 0.121807332581
-0.450442616461 0.121803993656
-0.450442616461 0.121800649089
-0.450442616461 0.121797298875
-0.450442616461 0.121793943011
-0.450442616461 0.121790581493
-0.450442616461 0.121787214315
-0.450442616461 0.121783841474
-0.450442616461 0.121780462966
-0.450442616461 0.121777078786
-0.450442616461 0.12177368893
-0.450442616461 0.121770293393
-0.450442616461 0.121766892173
-0.450442616461 0.121763485263
-0.450442616461 0.121760072661
-0.450442616461 0.121756654361
-0.450442616461 0.12175323036
-0.450442616461 0.121749800654
-0.450442616461 0.121746365237
-0.450442616461 0.121742924106
-0.450442616461 0.121739477257
-0.450442616461 0.121736024686
-0.450442616461 0.121732566388
-0.450442616461 0.121729102358
-0.450442616461 0.121725632594
-0.450442616461 0.12172215709
-0.450442616461 0.121718675842
-0.450442616461 0.121715188846
-0.450442616461 0.121711696099
-0.450442616461 0.121708197595
-0.450442616461 0.12170469333
-0.450442616461 0.121701183301
-0.450442616461 0.121697667502
-0.450442616461 0.121694145931
-0.450442616461 0.121690618582
-0.450442616461 0.121687085451
-0.450442616461 0.121683546535
-0.450442616461 0.121680001829
-0.450442616461 0.121676451328
-0.450442616461 0.121672895029
-0.450442616461 0.121669332927
-0.450442616461 0.121665765019
-0.450442616461 0.121662191299
-0.450442616461 0.121658611765
-0.450442616461 0.121655026411
-0.450442616461 0.121651435233
-0.450442616461 0.121647838227
-0.450442616461 0.12164423539
-0.450442616461 0.121640626716
-0.450442616461 0.121637012202
-0.450442616461 0.121633391844
-0.450442616461 0.121629765636
-0.450442616461 0.121626133576
-0.450442616461 0.121622495659
-0.450442616461 0.12161885188
-0.450442616461 0.121615202236
-0.450442616461 0.121611546722
-0.450442616461 0.121607885335
-0.450442616461 0.121604218069
-0.450442616461 0.121600544922
-0.450442616461 0.121596865888
-0.450442616461 0.121593180963
-0.450442616461 0.121589490144
-0.450442616461 0.121585793426
-0.450442616461 0.121582090805
-0.450442616461 0.121578382277
-0.450442616461 0.121574667838
-0.450442616461 0.121570947483
-0.450442616461 0.121567221208
-0.450442616461 0.12156348901
-0.450442616461 0.121559750883
-0.450442616461 0.121556006825
-0.450442616461 0.12155225683
-0.450442616461 0.121548500895
-0.450442616461 0.121544739015
-0.450442616461 0.121540971186
-0.450442616461 0.121537197405
-0.450442616461 0.121533417666
-0.450442616461 0.121529631967
-0.450442616461 0.121525840302
-0.450442616461 0.121522042667
-0.450442616461 0.121518239059
-0.450442616461 0.121514429473
-0.450442616461 0.121510613906
-0.450442616461 0.121506792352
-0.450442616461 0.121502964808
-0.450442616461 0.12149913127
-0.450442616461 0.121495291734
-0.450442616461 0.121491446195
-0.450442616461 0.121487594649
-0.450442616461 0.121483737092
-0.450442616461 0.121479873521
-0.450442616461 0.12147600393
-0.450442616461 0.121472128316
-0.450442616461 0.121468246675
-0.450442616461 0.121464359003
-0.450442616461 0.121460465295
-0.450442616461 0.121456565547
-0.450442616461 0.121452659756
-0.450442616461 0.121448747916
-0.450442616461 0.121444830025
-0.450442616461 0.121440906077
-0.450442616461 0.12143697607
-0.450442616461 0.121433039997
-0.450442616461 0.121429097857
-0.450442616461 0.121425149644
-0.450442616461 0.121421195354
-0.450442616461 0.121417234983
-0.450442616461 0.121413268528
-0.450442616461 0.121409295983
-0.450442616461 0.121405317346
-0.450442616461 0.121401332611
-0.450442616461 0.121397341775
-0.450442616461 0.121393344834
-0.450442616461 0.121389341783
-0.450442616461 0.121385332619
-0.450442616461 0.121381317337
-0.450442616461 0.121377295933
-0.450442616461 0.121373268403
-0.450442616461 0.121369234744
-0.450442616461 0.12136519495
-0.450442616461 0.121361149019
-0.450442616461 0.121357096945
-0.450442616461 0.121353038725
-0.450442616461 0.121348974355
-0.450442616461 0.12134490383
-0.450442616461 0.121340827147
-0.450442616461 0.121336744301
-0.450442616461 0.121332655289
-0.450442616461 0.121328560106
-0.450442616461 0.121324458748
-0.450442616461 0.121320351212
-0.450442616461 0.121316237492
-0.450442616461 0.121312117586
-0.450442616461 0.121307991488
-0.450442616461 0.121303859196
-0.450442616461 0.121299720704
-0.450442616461 0.121295576009
-0.450442616461 0.121291425106
-0.450442616461 0.121287267993
-0.450442616461 0.121283104664
-0.450442616461 0.121278935115
-0.450442616461 0.121274759343
-0.450442616461 0.121270577344
-0.450442616461 0.121266389112
-0.450442616461 0.121262194646
-0.450442616461 0.121257993939
-0.450442616461 0.121253786989
-0.450442616461 0.121249573791
-0.450442616461 0.121245354341
-0.450442616461 0.121241128635
-0.450442616461 0.121236896669
-0.450442616461 0.121232658439
-0.450442616461 0.121228413942
-0.450442616461 0.121224163172
-0.450442616461 0.121219906126
-0.450442616461 0.1212156428
-0.450442616461 0.12121137319
-0.450442616461 0.121207097292
-0.450442616461 0.121202815101
-0.450442616461 0.121198526614
-0.450442616461 0.121194231827
-0.450442616461 0.121189930736
-0.450442616461 0.121185623336
-0.450442616461 0.121181309625
-0.450442616461 0.121176989596
-0.450442616461 0.121172663248
-0.450442616461 0.121168330575
-0.450442616461 0.121163991573
-0.450442616461 0.121159646239
-0.450442616461 0.121155294569
-0.450442616461 0.121150936558
-0.450442616461 0.121146572203
-0.450442616461 0.121142201499
-0.450442616461 0.121137824443
-0.450442616461 0.121133441031
-0.450442616461 0.121129051258
-0.450442616461 0.12112465512
-0.450442616461 0.121120252614
-0.450442616461 0.121115843735
-0.450442616461 0.12111142848
-0.450442616461 0.121107006845
-0.450442616461 0.121102578825
-0.450442616461 0.121098144416
-0.450442616461 0.121093703615
-0.450442616461 0.121089256417
-0.450442616461 0.121084802819
-0.450442616461 0.121080342817
-0.450442616461 0.121075876406
-0.450442616461 0.121071403583
-0.450442616461 0.121066924343
-0.450442616461 0.121062438683
-0.450442616461 0.121057946599
-0.450442616461 0.121053448086
-0.450442616461 0.12104894314
-0.450442616461 0.121044431759
-0.450442616461 0.121039913937
-0.450442616461 0.121035389671
-0.450442616461 0.121030858957
-0.450442616461 0.12102632179
-0.450442616461 0.121021778167
-0.450442616461 0.121017228085
-0.450442616461 0.121012671538
-0.450442616461 0.121008108522
-0.450442616461 0.121003539035
-0.450442616461 0.120998963072
-0.450442616461 0.120994380629
-0.450442616461 0.120989791702
-0.450442616461 0.120985196287
-0.450442616461 0.12098059438
-0.450442616461 0.120975985977
-0.450442616461 0.120971371074
-0.450442616461 0.120966749668
-0.450442616461 0.120962121754
-0.450442616461 0.120957487328
-0.450442616461 0.120952846387
-0.450442616461 0.120948198926
-0.450442616461 0.120943544942
-0.450442616461 0.120938884431
-0.450442616461 0.120934217387
-0.450442616461 0.120929543809
-0.450442616461 0.120924863691
-0.450442616461 0.120920177031
-0.450442616461 0.120915483823
-0.450442616461 0.120910784064
-0.450442616461 0.12090607775
-0.450442616461 0.120901364877
-0.450442616461 0.120896645441
-0.450442616461 0.120891919438
-0.450442616461 0.120887186864
-0.450442616461 0.120882447716
-0.450442616461 0.120877701989
-0.450442616461 0.12087294968
-0.450442616461 0.120868190784
-0.450442616461 0.120863425298
-0.450442616461 0.120858653218
-0.450442616461 0.120853874539
-0.450442616461 0.120849089259
-0.450442616461 0.120844297372
-0.450442616461 0.120839498875
-0.450442616461 0.120834693764
-0.450442616461 0.120829882036
-0.450442616461 0.120825063686
-0.450442616461 0.12082023871
-0.450442616461 0.120815407104
-0.450442616461 0.120810568865
-0.450442616461 0.120805723989
-0.450442616461 0.120800872472
-0.450442616461 0.120796014309
-0.450442616461 0.120791149498
-0.450442616461 0.120786278033
-0.450442616461 0.120781399912
-0.450442616461 0.120776515129
-0.450442616461 0.120771623682
-0.450442616461 0.120766725567
-0.450442616461 0.120761820779
-0.450442616461 0.120756909315
-0.450442616461 0.12075199117
-0.450442616461 0.120747066342
-0.450442616461 0.120742134825
-0.450442616461 0.120737196617
-0.450442616461 0.120732251712
-0.450442616461 0.120727300108
-0.450442616461 0.120722341801
-0.450442616461 0.120717376786
-0.450442616461 0.12071240506
-0.450442616461 0.120707426618
-0.450442616461 0.120702441458
-0.450442616461 0.120697449574
-0.450442616461 0.120692450964
-0.450442616461 0.120687445623
-0.450442616461 0.120682433547
-0.450442616461 0.120677414733
-0.450442616461 0.120672389177
-0.450442616461 0.120667356875
-0.450442616461 0.120662317822
-0.450442616461 0.120657272016
-0.450442616461 0.120652219452
-0.450442616461 0.120647160126
-0.450442616461 0.120642094035
-0.450442616461 0.120637021174
-0.450442616461 0.12063194154
-0.450442616461 0.120626855129
-0.450442616461 0.120621761937
-0.450442616461 0.120616661961
-0.450442616461 0.120611555195
-0.450442616461 0.120606441638
-0.450442616461 0.120601321284
-0.450442616461 0.120596194129
-0.450442616461 0.120591060171
-0.450442616461 0.120585919405
-0.450442616461 0.120580771827
-0.450442616461 0.120575617434
-0.450442616461 0.120570456221
-0.450442616461 0.120565288185
-0.450442616461 0.120560113322
-0.450442616461 0.120554931628
-0.450442616461 0.120549743099
-0.450442616461 0.120544547731
-0.450442616461 0.120539345522
-0.450442616461 0.120534136466
-0.450442616461 0.120528920559
-0.450442616461 0.120523697799
-0.450442616461 0.120518468182
-0.450442616461 0.120513231702
-0.450442616461 0.120507988358
-0.450442616461 0.120502738144
-0.450442616461 0.120497481057
-0.450442616461 0.120492217093
-0.450442616461 0.120486946248
-0.450442616461 0.120481668519
-0.450442616461 0.120476383902
-0.450442616461 0.120471092392
-0.450442616461 0.120465793987
-0.450442616461 0.120460488682
-0.450442616461 0.120455176473
-0.450442616461 0.120449857357
-0.450442616461 0.12044453133
-0.450442616461 0.120439198387
-0.450442616461 0.120433858526
-0.450442616461 0.120428511742
-0.450442616461 0.120423158032
-0.450442616461 0.120417797392
-0.450442616461 0.120412429818
-0.450442616461 0.120407055306
-0.450442616461 0.120401673852
-0.450442616461 0.120396285453
-0.450442616461 0.120390890104
-0.450442616461 0.120385487803
-0.450442616461 0.120380078545
-0.450442616461 0.120374662326
-0.450442616461 0.120369239143
-0.450442616461 0.120363808992
-0.450442616461 0.120358371869
-0.450442616461 0.12035292777
-0.450442616461 0.120347476691
-0.450442616461 0.12034201863
-0.450442616461 0.120336553581
-0.450442616461 0.120331081541
-0.450442616461 0.120325602507
-0.450442616461 0.120320116474
-0.450442616461 0.120314623439
-0.450442616461 0.120309123398
-0.450442616461 0.120303616348
-0.450442616461 0.120298102284
-0.450442616461 0.120292581202
-0.450442616461 0.1202870531
-0.450442616461 0.120281517973
-0.450442616461 0.120275975817
-0.450442616461 0.120270426629
-0.450442616461 0.120264870404
-0.450442616461 0.12025930714
-0.450442616461 0.120253736832
-0.450442616461 0.120248159477
-0.450442616461 0.120242575071
-0.450442616461 0.12023698361
-0.450442616461 0.12023138509
-0.450442616461 0.120225779507
-0.450442616461 0.120220166859
-0.450442616461 0.12021454714
-0.450442616461 0.120208920348
-0.450442616461 0.120203286479
-0.450442616461 0.120197645528
-0.450442616461 0.120191997492
-0.450442616461 0.120186342368
-0.450442616461 0.120180680151
-0.450442616461 0.120175010838
-0.450442616461 0.120169334425
-0.450442616461 0.120163650909
-0.450442616461 0.120157960285
-0.450442616461 0.12015226255
-0.450442616461 0.1201465577
-0.450442616461 0.120140845732
-0.450442616461 0.120135126641
-0.450442616461 0.120129400424
-0.450442616461 0.120123667078
-0.450442616461 0.120117926598
-0.450442616461 0.12011217898
-0.450442616461 0.120106424222
-0.450442616461 0.120100662319
-0.450442616461 0.120094893268
-0.450442616461 0.120089117064
-0.450442616461 0.120083333705
-0.450442616461 0.120077543186
-0.450442616461 0.120071745504
-0.450442616461 0.120065940654
-0.450442616461 0.120060128634
-0.450442616461 0.12005430944
-0.450442616461 0.120048483067
-0.450442616461 0.120042649513
-0.450442616461 0.120036808773
-0.450442616461 0.120030960844
-0.450442616461 0.120025105721
-0.450442616461 0.120019243402
-0.450442616461 0.120013373883
-0.450442616461 0.120007497159
-0.450442616461 0.120001613228
-0.450442616461 0.119995722085
-0.450442616461 0.119989823727
-0.450442616461 0.11998391815
-0.450442616461 0.11997800535
-0.450442616461 0.119972085324
-0.450442616461 0.119966158068
-0.450442616461 0.119960223578
-0.450442616461 0.119954281851
-0.450442616461 0.119948332883
-0.450442616461 0.11994237667
-0.450442616461 0.119936413209
-0.450442616461 0.119930442495
-0.450442616461 0.119924464526
-0.450442616461 0.119918479297
-0.450442616461 0.119912486805
-0.450442616461 0.119906487046
-0.450442616461 0.119900480016
-0.450442616461 0.119894465713
-0.450442616461 0.119888444131
-0.450442616461 0.119882415267
-0.450442616461 0.119876379119
-0.450442616461 0.119870335681
-0.450442616461 0.119864284951
-0.450442616461 0.119858226925
-0.450442616461 0.119852161598
-0.450442616461 0.119846088968
-0.450442616461 0.119840009031
-0.450442616461 0.119833921782
-0.450442616461 0.119827827219
-0.450442616461 0.119821725338
-0.450442616461 0.119815616135
-0.450442616461 0.119809499606
-0.450442616461 0.119803375748
-0.450442616461 0.119797244557
-0.450442616461 0.119791106029
-0.450442616461 0.119784960161
-0.450442616461 0.119778806949
-0.450442616461 0.11977264639
-0.450442616461 0.11976647848
-0.450442616461 0.119760303214
-0.450442616461 0.11975412059
-0.450442616461 0.119747930604
-0.450442616461 0.119741733252
-0.450442616461 0.119735528531
-0.450442616461 0.119729316436
-0.450442616461 0.119723096965
-0.450442616461 0.119716870113
-0.450442616461 0.119710635878
-0.450442616461 0.119704394255
-0.450442616461 0.11969814524
-0.450442616461 0.119691888831
-0.450442616461 0.119685625022
-0.450442616461 0.119679353812
-0.450442616461 0.119673075196
-0.450442616461 0.11966678917
-0.450442616461 0.119660495732
-0.450442616461 0.119654194876
-0.450442616461 0.119647886601
-0.450442616461 0.119641570901
-0.450442616461 0.119635247773
-0.450442616461 0.119628917215
-0.450442616461 0.119622579221
-0.450442616461 0.11961623379
-0.450442616461 0.119609880916
-0.450442616461 0.119603520596
-0.450442616461 0.119597152827
-0.450442616461 0.119590777605
-0.450442616461 0.119584394926
-0.450442616461 0.119578004787
-0.450442616461 0.119571607185
-0.450442616461 0.119565202115
-0.450442616461 0.119558789574
-0.450442616461 0.119552369559
-0.450442616461 0.119545942065
-0.450442616461 0.119539507089
-0.450442616461 0.119533064628
-0.450442616461 0.119526614678
-0.450442616461 0.119520157235
-0.450442616461 0.119513692296
-0.450442616461 0.119507219857
-0.450442616461 0.119500739915
-0.450442616461 0.119494252466
-0.450442616461 0.119487757506
-0.450442616461 0.119481255032
-0.450442616461 0.11947474504
-0.450442616461 0.119468227526
-0.450442616461 0.119461702488
-0.450442616461 0.119455169921
-0.450442616461 0.119448629822
-0.450442616461 0.119442082187
-0.450442616461 0.119435527013
-0.450442616461 0.119428964295
-0.450442616461 0.119422394032
-0.450442616461 0.119415816218
-0.450442616461 0.11940923085
-0.450442616461 0.119402637925
-0.450442616461 0.11939603744
-0.450442616461 0.119389429389
-0.450442616461 0.119382813771
-0.450442616461 0.119376190582
-0.450442616461 0.119369559817
-0.450442616461 0.119362921473
-0.450442616461 0.119356275547
-0.450442616461 0.119349622036
-0.450442616461 0.119342960935
-0.450442616461 0.11933629224
-0.450442616461 0.11932961595
-0.450442616461 0.119322932059
-0.450442616461 0.119316240564
-0.450442616461 0.119309541463
-0.450442616461 0.11930283475
-0.450442616461 0.119296120423
-0.450442616461 0.119289398478
-0.450442616461 0.119282668912
-0.450442616461 0.11927593172
-0.450442616461 0.1192691869
-0.450442616461 0.119262434448
-0.450442616461 0.11925567436
-0.450442616461 0.119248906633
-0.450442616461 0.119242131263
-0.450442616461 0.119235348247
-0.450442616461 0.11922855758
-0.450442616461 0.119221759261
-0.450442616461 0.119214953284
-0.450442616461 0.119208139647
-0.450442616461 0.119201318345
-0.450442616461 0.119194489376
-0.450442616461 0.119187652736
-0.450442616461 0.119180808421
-0.450442616461 0.119173956428
-0.450442616461 0.119167096754
-0.450442616461 0.119160229393
-0.450442616461 0.119153354344
-0.450442616461 0.119146471603
-0.450442616461 0.119139581166
-0.450442616461 0.119132683029
-0.450442616461 0.119125777189
-0.450442616461 0.119118863643
-0.450442616461 0.119111942387
-0.450442616461 0.119105013417
-0.450442616461 0.11909807673
-0.450442616461 0.119091132322
-0.450442616461 0.119084180191
-0.450442616461 0.119077220332
-0.450442616461 0.119070252741
-0.450442616461 0.119063277416
-0.450442616461 0.119056294353
-0.450442616461 0.119049303548
-0.450442616461 0.119042304997
-0.450442616461 0.119035298698
-0.450442616461 0.119028284647
-0.450442616461 0.11902126284
-0.450442616461 0.119014233274
-0.450442616461 0.119007195945
-0.450442616461 0.119000150849
-0.450442616461 0.118993097984
-0.450442616461 0.118986037346
-0.450442616461 0.11897896893
-0.450442616461 0.118971892735
-0.450442616461 0.118964808755
-0.450442616461 0.118957716988
-0.450442616461 0.118950617431
-0.450442616461 0.118943510079
-0.450442616461 0.118936394929
-0.450442616461 0.118929271978
-0.450442616461 0.118922141222
-0.450442616461 0.118915002658
-0.450442616461 0.118907856282
-0.450442616461 0.118900702091
-0.450442616461 0.118893540081
-0.450442616461 0.118886370249
-0.450442616461 0.118879192591
-0.450442616461 0.118872007104
-0.450442616461 0.118864813784
-0.450442616461 0.118857612628
-0.450442616461 0.118850403632
-0.450442616461 0.118843186794
-0.450442616461 0.118835962108
-0.450442616461 0.118828729572
-0.450442616461 0.118821489183
-0.450442616461 0.118814240937
-0.450442616461 0.11880698483
-0.450442616461 0.118799720859
-0.450442616461 0.11879244902
-0.450442616461 0.118785169311
-0.450442616461 0.118777881727
-0.450442616461 0.118770586265
-0.450442616461 0.118763282922
-0.450442616461 0.118755971694
-0.450442616461 0.118748652578
-0.450442616461 0.11874132557
-0.450442616461 0.118733990667
-0.450442616461 0.118726647865
-0.450442616461 0.11871929716
-0.450442616461 0.118711938551
-0.450442616461 0.118704572032
-0.450442616461 0.1186971976
-0.450442616461 0.118689815253
-0.450442616461 0.118682424986
-0.450442616461 0.118675026796
-0.450442616461 0.11866762068
-0.450442616461 0.118660206634
-0.450442616461 0.118652784655
-0.450442616461 0.118645354739
-0.450442616461 0.118637916882
-0.450442616461 0.118630471083
-0.450442616461 0.118623017336
-0.450442616461 0.118615555638
-0.450442616461 0.118608085987
-0.450442616461 0.118600608378
-0.450442616461 0.118593122809
-0.450442616461 0.118585629275
-0.450442616461 0.118578127773
-0.450442616461 0.118570618301
-0.450442616461 0.118563100853
-0.450442616461 0.118555575428
-0.450442616461 0.118548042021
-0.450442616461 0.118540500629
-0.450442616461 0.118532951249
-0.450442616461 0.118525393878
-0.450442616461 0.118517828511
-0.450442616461 0.118510255145
-0.450442616461 0.118502673777
-0.450442616461 0.118495084404
-0.450442616461 0.118487487022
-0.450442616461 0.118479881628
-0.450442616461 0.118472268217
-0.450442616461 0.118464646788
-0.450442616461 0.118457017336
-0.450442616461 0.118449379858
-0.450442616461 0.118441734351
-0.450442616461 0.11843408081
-0.450442616461 0.118426419234
-0.450442616461 0.118418749618
-0.450442616461 0.118411071958
-0.450442616461 0.118403386252
-0.450442616461 0.118395692497
-0.450442616461 0.118387990687
-0.450442616461 0.118380280822
-0.450442616461 0.118372562895
-0.450442616461 0.118364836906
-0.450442616461 0.118357102849
-0.450442616461 0.118349360722
-0.450442616461 0.118341610521
-0.450442616461 0.118333852243
-0.450442616461 0.118326085885
-0.450442616461 0.118318311442
-0.450442616461 0.118310528912
-0.450442616461 0.118302738291
-0.450442616461 0.118294939576
-0.450442616461 0.118287132764
-0.450442616461 0.11827931785
-0.450442616461 0.118271494832
-0.450442616461 0.118263663707
-0.450442616461 0.11825582447
-0.450442616461 0.118247977118
-0.450442616461 0.118240121649
-0.450442616461 0.118232258058
-0.450442616461 0.118224386343
-0.450442616461 0.118216506499
-0.450442616461 0.118208618524
-0.450442616461 0.118200722414
-0.450442616461 0.118192818166
-0.450442616461 0.118184905776
-0.450442616461 0.118176985241
-0.450442616461 0.118169056557
-0.450442616461 0.118161119722
-0.450442616461 0.118153174732
-0.450442616461 0.118145221583
-0.450442616461 0.118137260272
-0.450442616461 0.118129290796
-0.450442616461 0.118121313151
-0.450442616461 0.118113327334
-0.450442616461 0.118105333342
-0.450442616461 0.118097331171
-0.450442616461 0.118089320817
-0.450442616461 0.118081302279
-0.450442616461 0.118073275551
-0.450442616461 0.118065240631
-0.450442616461 0.118057197515
-0.450442616461 0.118049146201
-0.450442616461 0.118041086684
-0.450442616461 0.118033018961
-0.450442616461 0.118024943029
-0.450442616461 0.118016858885
-0.450442616461 0.118008766525
-0.450442616461 0.118000665946
-0.450442616461 0.117992557144
-0.450442616461 0.117984440117
-0.450442616461 0.11797631486
-0.450442616461 0.117968181371
-0.450442616461 0.117960039645
-0.450442616461 0.117951889681
-0.450442616461 0.117943731474
-0.450442616461 0.11793556502
-0.450442616461 0.117927390318
-0.450442616461 0.117919207362
-0.450442616461 0.117911016151
-0.450442616461 0.117902816681
-0.450442616461 0.117894608947
-0.450442616461 0.117886392948
-0.450442616461 0.117878168679
-0.450442616461 0.117869936137
-0.450442616461 0.11786169532
-0.450442616461 0.117853446223
-0.450442616461 0.117845188843
-0.450442616461 0.117836923177
-0.450442616461 0.117828649221
-0.450442616461 0.117820366973
-0.450442616461 0.117812076429
-0.450442616461 0.117803777585
-0.450442616461 0.117795470439
-0.450442616461 0.117787154986
-0.450442616461 0.117778831224
-0.450442616461 0.11777049915
-0.450442616461 0.117762158759
-0.450442616461 0.117753810048
-0.450442616461 0.117745453015
-0.450442616461 0.117737087656
-0.450442616461 0.117728713968
-0.450442616461 0.117720331947
-0.450442616461 0.11771194159
-0.450442616461 0.117703542893
-0.450442616461 0.117695135854
-0.450442616461 0.117686720469
-0.450442616461 0.117678296734
-0.450442616461 0.117669864647
-0.450442616461 0.117661424204
-0.450442616461 0.117652975402
-0.450442616461 0.117644518237
-0.450442616461 0.117636052706
-0.450442616461 0.117627578806
-0.450442616461 0.117619096534
-0.450442616461 0.117610605886
-0.450442616461 0.117602106858
-0.450442616461 0.117593599449
-0.450442616461 0.117585083653
-0.450442616461 0.117576559469
-0.450442616461 0.117568026892
-0.450442616461 0.117559485919
-0.450442616461 0.117550936548
-0.450442616461 0.117542378774
-0.450442616461 0.117533812595
-0.450442616461 0.117525238007
-0.450442616461 0.117516655006
-0.450442616461 0.117508063591
-0.450442616461 0.117499463756
-0.450442616461 0.1174908555
-0.450442616461 0.117482238818
-0.450442616461 0.117473613708
-0.450442616461 0.117464980166
-0.450442616461 0.117456338188
-0.450442616461 0.117447687772
-0.450442616461 0.117439028914
-0.450442616461 0.117430361612
-0.450442616461 0.11742168586
-0.450442616461 0.117413001658
-0.450442616461 0.117404309
-0.450442616461 0.117395607884
-0.450442616461 0.117386898306
-0.450442616461 0.117378180264
-0.450442616461 0.117369453754
-0.450442616461 0.117360718772
-0.450442616461 0.117351975316
-0.450442616461 0.117343223382
-0.450442616461 0.117334462967
-0.450442616461 0.117325694067
-0.450442616461 0.117316916679
-0.450442616461 0.117308130801
-0.450442616461 0.117299336428
-0.450442616461 0.117290533558
-0.450442616461 0.117281722186
-0.450442616461 0.117272902311
-0.450442616461 0.117264073929
-0.450442616461 0.117255237035
-0.450442616461 0.117246391628
-0.450442616461 0.117237537704
-0.450442616461 0.117228675259
-0.450442616461 0.117219804291
-0.450442616461 0.117210924796
-0.450442616461 0.11720203677
-0.450442616461 0.117193140211
-0.450442616461 0.117184235115
-0.450442616461 0.117175321479
-0.450442616461 0.1171663993
-0.450442616461 0.117157468575
-0.450442616461 0.117148529299
-0.450442616461 0.117139581471
-0.450442616461 0.117130625086
-0.450442616461 0.117121660142
-0.450442616461 0.117112686635
-0.450442616461 0.117103704562
-0.450442616461 0.117094713919
-0.450442616461 0.117085714704
-0.450442616461 0.117076706914
-0.450442616461 0.117067690544
-0.450442616461 0.117058665592
-0.450442616461 0.117049632054
-0.450442616461 0.117040589928
-0.450442616461 0.117031539209
-0.450442616461 0.117022479895
-0.450442616461 0.117013411983
-0.450442616461 0.117004335469
-0.450442616461 0.11699525035
-0.450442616461 0.116986156623
-0.450442616461 0.116977054284
-0.450442616461 0.11696794333
-0.450442616461 0.116958823759
-0.450442616461 0.116949695566
-0.450442616461 0.116940558749
-0.450442616461 0.116931413304
-0.450442616461 0.116922259228
-0.450442616461 0.116913096518
-0.450442616461 0.116903925171
-0.450442616461 0.116894745183
-0.450442616461 0.116885556552
-0.450442616461 0.116876359273
-0.450442616461 0.116867153344
-0.450442616461 0.116857938761
-0.450442616461 0.116848715522
-0.450442616461 0.116839483623
-0.450442616461 0.11683024306
-0.450442616461 0.116820993831
-0.450442616461 0.116811735933
-0.450442616461 0.116802469361
-0.450442616461 0.116793194114
-0.450442616461 0.116783910187
-0.450442616461 0.116774617578
-0.450442616461 0.116765316283
-0.450442616461 0.116756006299
-0.450442616461 0.116746687622
-0.450442616461 0.116737360251
-0.450442616461 0.11672802418
-0.450442616461 0.116718679408
-0.450442616461 0.116709325931
-0.450442616461 0.116699963746
-0.450442616461 0.116690592849
-0.450442616461 0.116681213237
-0.450442616461 0.116671824908
-0.450442616461 0.116662427857
-0.450442616461 0.116653022083
-0.450442616461 0.11664360758
-0.450442616461 0.116634184347
-0.450442616461 0.11662475238
-0.450442616461 0.116615311676
-0.450442616461 0.116605862232
-0.450442616461 0.116596404044
-0.450442616461 0.116586937109
-0.450442616461 0.116577461424
-0.450442616461 0.116567976987
-0.450442616461 0.116558483792
-0.450442616461 0.116548981839
-0.450442616461 0.116539471122
-0.450442616461 0.11652995164
-0.450442616461 0.116520423389
-0.450442616461 0.116510886365
-0.450442616461 0.116501340566
-0.450442616461 0.116491785988
-0.450442616461 0.116482222628
-0.450442616461 0.116472650483
-0.450442616461 0.116463069549
-0.450442616461 0.116453479825
-0.450442616461 0.116443881305
-0.450442616461 0.116434273988
-0.450442616461 0.11642465787
-0.450442616461 0.116415032947
-0.450442616461 0.116405399217
-0.450442616461 0.116395756677
-0.450442616461 0.116386105322
-0.450442616461 0.116376445151
-0.450442616461 0.116366776159
-0.450442616461 0.116357098345
-0.450442616461 0.116347411703
-0.450442616461 0.116337716232
-0.450442616461 0.116328011928
-0.450442616461 0.116318298789
-0.450442616461 0.116308576809
-0.450442616461 0.116298845988
-0.450442616461 0.116289106321
-0.450442616461 0.116279357805
-0.450442616461 0.116269600437
-0.450442616461 0.116259834214
-0.450442616461 0.116250059133
-0.450442616461 0.11624027519
-0.450442616461 0.116230482383
-0.450442616461 0.116220680708
-0.450442616461 0.116210870162
-0.450442616461 0.116201050742
-0.450442616461 0.116191222445
-0.450442616461 0.116181385267
-0.450442616461 0.116171539205
-0.450442616461 0.116161684257
-0.450442616461 0.116151820419
-0.450442616461 0.116141947687
-0.450442616461 0.11613206606
-0.450442616461 0.116122175533
-0.450442616461 0.116112276103
-0.450442616461 0.116102367767
-0.450442616461 0.116092450523
-0.450442616461 0.116082524367
-0.450442616461 0.116072589295
-0.450442616461 0.116062645305
-0.450442616461 0.116052692393
-0.450442616461 0.116042730557
-0.450442616461 0.116032759792
-0.450442616461 0.116022780097
-0.450442616461 0.116012791468
-0.450442616461 0.116002793901
-0.450442616461 0.115992787394
-0.450442616461 0.115982771943
-0.450442616461 0.115972747545
-0.450442616461 0.115962714197
-0.450442616461 0.115952671897
-0.450442616461 0.11594262064
-0.450442616461 0.115932560423
-0.450442616461 0.115922491244
-0.450442616461 0.1159124131
-0.450442616461 0.115902325987
-0.450442616461 0.115892229901
-0.450442616461 0.115882124841
-0.450442616461 0.115872010802
-0.450442616461 0.115861887782
-0.450442616461 0.115851755778
-0.450442616461 0.115841614785
-0.450442616461 0.115831464802
-0.450442616461 0.115821305825
-0.450442616461 0.115811137851
-0.450442616461 0.115800960877
-0.450442616461 0.115790774899
-0.450442616461 0.115780579915
-0.450442616461 0.115770375921
-0.450442616461 0.115760162915
-0.450442616461 0.115749940892
-0.450442616461 0.115739709851
-0.450442616461 0.115729469787
-0.450442616461 0.115719220698
-0.450442616461 0.115708962581
-0.450442616461 0.115698695432
-0.450442616461 0.115688419248
-0.450442616461 0.115678134027
-0.450442616461 0.115667839765
-0.450442616461 0.115657536458
-0.450442616461 0.115647224105
-0.450442616461 0.115636902701
-0.450442616461 0.115626572243
-0.450442616461 0.115616232729
-0.450442616461 0.115605884155
-0.450442616461 0.115595526519
-0.450442616461 0.115585159816
-0.450442616461 0.115574784045
-0.450442616461 0.115564399201
-0.450442616461 0.115554005282
-0.450442616461 0.115543602285
-0.450442616461 0.115533190206
-0.450442616461 0.115522769042
-0.450442616461 0.115512338791
-0.450442616461 0.115501899449
-0.450442616461 0.115491451012
-0.450442616461 0.115480993479
-0.450442616461 0.115470526845
-0.450442616461 0.115460051108
-0.450442616461 0.115449566265
-0.450442616461 0.115439072312
-0.450442616461 0.115428569246
-0.450442616461 0.115418057064
-0.450442616461 0.115407535764
-0.450442616461 0.115397005341
-0.450442616461 0.115386465794
-0.450442616461 0.115375917118
-0.450442616461 0.115365359311
-0.450442616461 0.115354792369
-0.450442616461 0.11534421629
-0.450442616461 0.11533363107
-0.450442616461 0.115323036707
-0.450442616461 0.115312433196
-0.450442616461 0.115301820536
-0.450442616461 0.115291198722
-0.450442616461 0.115280567752
-0.450442616461 0.115269927623
-0.450442616461 0.115259278332
-0.450442616461 0.115248619875
-0.450442616461 0.11523795225
-0.450442616461 0.115227275453
-0.450442616461 0.115216589481
-0.450442616461 0.115205894331
-0.450442616461 0.11519519
-0.450442616461 0.115184476485
-0.450442616461 0.115173753783
-0.450442616461 0.115163021891
-0.450442616461 0.115152280806
-0.450442616461 0.115141530524
-0.450442616461 0.115130771042
-0.450442616461 0.115120002358
-0.450442616461 0.115109224468
-0.450442616461 0.115098437369
-0.450442616461 0.115087641058
-0.450442616461 0.115076835533
-0.450442616461 0.115066020789
-0.450442616461 0.115055196824
-0.450442616461 0.115044363635
-0.450442616461 0.115033521219
-0.450442616461 0.115022669572
-0.450442616461 0.115011808691
-0.450442616461 0.115000938574
-0.450442616461 0.114990059217
-0.450442616461 0.114979170618
-0.450442616461 0.114968272773
-0.450442616461 0.114957365678
-0.450442616461 0.114946449332
-0.450442616461 0.11493552373
-0.450442616461 0.114924588871
-0.450442616461 0.11491364475
-0.450442616461 0.114902691365
-0.450442616461 0.114891728712
-0.450442616461 0.114880756789
-0.450442616461 0.114869775592
-0.450442616461 0.114858785119
-0.450442616461 0.114847785366
-0.450442616461 0.11483677633
-0.450442616461 0.114825758008
-0.450442616461 0.114814730397
-0.450442616461 0.114803693494
-0.450442616461 0.114792647296
-0.450442616461 0.1147815918
-0.450442616461 0.114770527003
-0.450442616461 0.114759452901
-0.450442616461 0.114748369492
-0.450442616461 0.114737276773
-0.450442616461 0.114726174739
-0.450442616461 0.11471506339
-0.450442616461 0.11470394272
-0.450442616461 0.114692812728
-0.450442616461 0.11468167341
-0.450442616461 0.114670524764
-0.450442616461 0.114659366785
-0.450442616461 0.114648199471
-0.450442616461 0.114637022819
-0.450442616461 0.114625836826
-0.450442616461 0.114614641489
-0.450442616461 0.114603436804
-0.450442616461 0.11459222277
-0.450442616461 0.114580999381
-0.450442616461 0.114569766637
-0.450442616461 0.114558524532
-0.450442616461 0.114547273066
-0.450442616461 0.114536012233
-0.450442616461 0.114524742032
-0.450442616461 0.114513462459
-0.450442616461 0.114502173511
-0.450442616461 0.114490875186
-0.450442616461 0.114479567479
-0.450442616461 0.114468250389
-0.450442616461 0.114456923911
-0.450442616461 0.114445588043
-0.450442616461 0.114434242782
-0.450442616461 0.114422888125
-0.450442616461 0.114411524069
-0.450442616461 0.11440015061
-0.450442616461 0.114388767746
-0.450442616461 0.114377375474
-0.450442616461 0.11436597379
-0.450442616461 0.114354562691
-0.450442616461 0.114343142175
-0.450442616461 0.114331712238
-0.450442616461 0.114320272878
-0.450442616461 0.11430882409
-0.450442616461 0.114297365873
-0.450442616461 0.114285898223
-0.450442616461 0.114274421138
-0.450442616461 0.114262934613
-0.450442616461 0.114251438646
-0.450442616461 0.114239933234
-0.450442616461 0.114228418375
-0.450442616461 0.114216894064
-0.450442616461 0.114205360299
-0.450442616461 0.114193817076
-0.450442616461 0.114182264394
-0.450442616461 0.114170702248
-0.450442616461 0.114159130635
-0.450442616461 0.114147549554
-0.450442616461 0.114135959
-0.450442616461 0.11412435897
-0.450442616461 0.114112749462
-0.450442616461 0.114101130472
-0.450442616461 0.114089501998
-0.450442616461 0.114077864036
-0.450442616461 0.114066216584
-0.450442616461 0.114054559637
-0.450442616461 0.114042893194
-0.450442616461 0.114031217252
-0.450442616461 0.114019531806
-0.450442616461 0.114007836854
-0.450442616461 0.113996132394
-0.450442616461 0.113984418422
-0.450442616461 0.113972694934
-0.450442616461 0.113960961929
-0.450442616461 0.113949219402
-0.450442616461 0.113937467352
-0.450442616461 0.113925705774
-0.450442616461 0.113913934667
-0.450442616461 0.113902154026
-0.450442616461 0.113890363848
-0.450442616461 0.113878564132
-0.450442616461 0.113866754873
-0.450442616461 0.113854936069
-0.450442616461 0.113843107717
-0.450442616461 0.113831269813
-0.450442616461 0.113819422355
-0.450442616461 0.113807565339
-0.450442616461 0.113795698763
-0.450442616461 0.113783822624
-0.450442616461 0.113771936918
-0.450442616461 0.113760041642
-0.450442616461 0.113748136794
-0.450442616461 0.11373622237
-0.450442616461 0.113724298368
-0.450442616461 0.113712364784
-0.450442616461 0.113700421615
-0.450442616461 0.113688468859
-0.450442616461 0.113676506511
-0.450442616461 0.11366453457
-0.450442616461 0.113652553033
-0.450442616461 0.113640561895
-0.450442616461 0.113628561155
-0.450442616461 0.113616550809
-0.450442616461 0.113604530853
-0.450442616461 0.113592501286
-0.450442616461 0.113580462105
-0.450442616461 0.113568413305
-0.450442616461 0.113556354884
-0.450442616461 0.113544286839
-0.450442616461 0.113532209167
-0.450442616461 0.113520121866
-0.450442616461 0.113508024931
-0.450442616461 0.11349591836
-0.450442616461 0.11348380215
-0.450442616461 0.113471676298
-0.450442616461 0.113459540801
-0.450442616461 0.113447395655
-0.450442616461 0.113435240859
-0.450442616461 0.113423076408
-0.450442616461 0.1134109023
-0.450442616461 0.113398718532
-0.450442616461 0.113386525101
-0.450442616461 0.113374322003
-0.450442616461 0.113362109237
-0.450442616461 0.113349886798
-0.450442616461 0.113337654684
-0.450442616461 0.113325412891
-0.450442616461 0.113313161417
-0.450442616461 0.113300900259
-0.450442616461 0.113288629414
-0.450442616461 0.113276348878
-0.450442616461 0.113264058649
-0.450442616461 0.113251758723
-0.450442616461 0.113239449098
-0.450442616461 0.113227129771
-0.450442616461 0.113214800738
-0.450442616461 0.113202461997
-0.450442616461 0.113190113544
-0.450442616461 0.113177755378
-0.450442616461 0.113165387493
-0.450442616461 0.113153009888
-0.450442616461 0.11314062256
-0.450442616461 0.113128225505
-0.450442616461 0.113115818721
-0.450442616461 0.113103402204
-0.450442616461 0.113090975952
-0.450442616461 0.113078539961
-0.450442616461 0.113066094229
-0.450442616461 0.113053638752
-0.450442616461 0.113041173528
-0.450442616461 0.113028698553
-0.450442616461 0.113016213825
-0.450442616461 0.11300371934
-0.450442616461 0.112991215096
-0.450442616461 0.112978701089
-0.450442616461 0.112966177317
-0.450442616461 0.112953643776
-0.450442616461 0.112941100463
-0.450442616461 0.112928547376
-0.450442616461 0.112915984511
-0.450442616461 0.112903411866
-0.450442616461 0.112890829437
-0.450442616461 0.112878237222
-0.450442616461 0.112865635217
-0.450442616461 0.112853023419
-0.450442616461 0.112840401826
-0.450442616461 0.112827770434
-0.450442616461 0.112815129241
-0.450442616461 0.112802478243
-0.450442616461 0.112789817438
-0.450442616461 0.112777146822
-0.450442616461 0.112764466392
-0.450442616461 0.112751776146
-0.450442616461 0.11273907608
-0.450442616461 0.112726366192
-0.450442616461 0.112713646478
-0.450442616461 0.112700916935
-0.450442616461 0.112688177561
-0.450442616461 0.112675428352
-0.450442616461 0.112662669306
-0.450442616461 0.112649900419
-0.450442616461 0.112637121689
-0.450442616461 0.112624333111
-0.450442616461 0.112611534685
-0.450442616461 0.112598726406
-0.450442616461 0.112585908271
-0.450442616461 0.112573080278
-0.450442616461 0.112560242423
-0.450442616461 0.112547394703
-0.450442616461 0.112534537117
-0.450442616461 0.112521669659
-0.450442616461 0.112508792328
-0.450442616461 0.11249590512
-0.450442616461 0.112483008033
-0.450442616461 0.112470101064
-0.450442616461 0.112457184209
-0.450442616461 0.112444257465
-0.450442616461 0.11243132083
-0.450442616461 0.1124183743
-0.450442616461 0.112405417873
-0.450442616461 0.112392451545
-0.450442616461 0.112379475314
-0.450442616461 0.112366489176
-0.450442616461 0.112353493129
-0.450442616461 0.11234048717
-0.450442616461 0.112327471295
-0.450442616461 0.112314445501
-0.450442616461 0.112301409786
-0.450442616461 0.112288364147
-0.450442616461 0.11227530858
-0.450442616461 0.112262243083
-0.450442616461 0.112249167652
-0.450442616461 0.112236082285
-0.450442616461 0.112222986979
-0.450442616461 0.11220988173
-0.450442616461 0.112196766536
-0.450442616461 0.112183641393
-0.450442616461 0.112170506299
-0.450442616461 0.112157361251
-0.450442616461 0.112144206245
-0.450442616461 0.112131041279
-0.450442616461 0.11211786635
-0.450442616461 0.112104681455
-0.450442616461 0.11209148659
-0.450442616461 0.112078281752
-0.450442616461 0.11206506694
-0.450442616461 0.112051842149
-0.450442616461 0.112038607377
-0.450442616461 0.112025362621
-0.450442616461 0.112012107878
-0.450442616461 0.111998843144
-0.450442616461 0.111985568417
-0.450442616461 0.111972283694
-0.450442616461 0.111958988971
-0.450442616461 0.111945684247
-0.450442616461 0.111932369517
-0.450442616461 0.111919044779
-0.450442616461 0.11190571003
-0.450442616461 0.111892365267
-0.450442616461 0.111879010487
-0.450442616461 0.111865645687
-0.450442616461 0.111852270863
-0.450442616461 0.111838886014
-0.450442616461 0.111825491135
-0.450442616461 0.111812086224
-0.450442616461 0.111798671278
-0.450442616461 0.111785246295
-0.450442616461 0.11177181127
-0.450442616461 0.111758366201
-0.450442616461 0.111744911085
-0.450442616461 0.111731445919
-0.450442616461 0.1117179707
-0.450442616461 0.111704485426
-0.450442616461 0.111690990092
-0.450442616461 0.111677484696
-0.450442616461 0.111663969236
-0.450442616461 0.111650443707
-0.450442616461 0.111636908108
-0.450442616461 0.111623362434
-0.450442616461 0.111609806684
-0.450442616461 0.111596240854
-0.450442616461 0.111582664941
-0.450442616461 0.111569078943
-0.450442616461 0.111555482855
-0.450442616461 0.111541876676
-0.450442616461 0.111528260402
-0.450442616461 0.11151463403
-0.450442616461 0.111500997557
-0.450442616461 0.111487350981
-0.450442616461 0.111473694298
-0.450442616461 0.111460027505
-0.450442616461 0.111446350599
-0.450442616461 0.111432663578
-0.450442616461 0.111418966438
-0.450442616461 0.111405259176
-0.450442616461 0.11139154179
-0.450442616461 0.111377814276
-0.450442616461 0.111364076632
-0.450442616461 0.111350328853
-0.450442616461 0.111336570939
-0.450442616461 0.111322802884
-0.450442616461 0.111309024687
-0.450442616461 0.111295236345
-0.450442616461 0.111281437854
-0.450442616461 0.111267629211
-0.450442616461 0.111253810414
-0.450442616461 0.11123998146
-0.450442616461 0.111226142345
-0.450442616461 0.111212293066
-0.450442616461 0.111198433621
-0.450442616461 0.111184564007
-0.450442616461 0.11117068422
-0.450442616461 0.111156794258
-0.450442616461 0.111142894117
-0.450442616461 0.111128983795
-0.450442616461 0.111115063289
-0.450442616461 0.111101132595
-0.450442616461 0.111087191711
-0.450442616461 0.111073240633
-0.450442616461 0.11105927936
-0.450442616461 0.111045307886
-0.450442616461 0.111031326211
-0.450442616461 0.11101733433
-0.450442616461 0.111003332241
-0.450442616461 0.110989319941
-0.450442616461 0.110975297427
-0.450442616461 0.110961264695
-0.450442616461 0.110947221743
-0.450442616461 0.110933168568
-0.450442616461 0.110919105167
-0.450442616461 0.110905031536
-0.450442616461 0.110890947673
-0.450442616461 0.110876853575
-0.450442616461 0.11086274924
-0.450442616461 0.110848634662
-0.450442616461 0.110834509841
-0.450442616461 0.110820374773
-0.450442616461 0.110806229454
-0.450442616461 0.110792073883
-0.450442616461 0.110777908055
-0.450442616461 0.110763731969
-0.450442616461 0.11074954562
-0.450442616461 0.110735349006
-0.450442616461 0.110721142124
-0.450442616461 0.110706924972
-0.450442616461 0.110692697545
-0.450442616461 0.110678459841
-0.450442616461 0.110664211857
-0.450442616461 0.110649953591
-0.450442616461 0.110635685038
-0.450442616461 0.110621406196
-0.450442616461 0.110607117063
-0.450442616461 0.110592817634
-0.450442616461 0.110578507908
-0.450442616461 0.11056418788
-0.450442616461 0.110549857549
-0.450442616461 0.110535516911
-0.450442616461 0.110521165963
-0.450442616461 0.110506804702
-0.450442616461 0.110492433125
-0.450442616461 0.11047805123
-0.450442616461 0.110463659012
-0.450442616461 0.11044925647
-0.450442616461 0.1104348436
-0.450442597657 0.110420418279
-0.450442509572 0.11040597481
-0.450442349433 0.110391512871
-0.450442117239 0.110377032455
-0.450441812989 0.110362533553
-0.450441436685 0.110348016156
-0.450440988325 0.110333480257
-0.450440467909 0.110318925846
-0.450439875438 0.110304352915
-0.45043921091 0.110289761457
-0.450438474326 0.110275151462
-0.450437665686 0.110260522923
-0.450436784988 0.11024587583
-0.450435832232 0.110231210176
-0.450434807418 0.110216525952
-0.450433710546 0.110201823149
-0.450432541615 0.11018710176
-0.450431300624 0.110172361776
-0.450429987572 0.110157603189
-0.45042860246 0.11014282599
-0.450427145286 0.110128030172
-0.45042561605 0.110113215725
-0.450424014751 0.110098382641
-0.450422341389 0.110083530912
-0.450420595962 0.11006866053
-0.450418778469 0.110053771486
-0.45041688891 0.110038863773
-0.450414927284 0.110023937381
-0.45041289359 0.110008992302
-0.450410787826 0.109994028528
-0.450408609993 0.109979046052
-0.450406360089 0.109964044864
-0.450404038112 0.109949024956
-0.450401644062 0.109933986319
-0.450399177937 0.109918928947
-0.450396639737 0.10990385283
-0.45039402946 0.109888757959
-0.450391347105 0.109873644328
-0.45038859267 0.109858511927
-0.450385766154 0.109843360748
-0.450382867557 0.109828190783
-0.450379896876 0.109813002024
-0.45037685411 0.109797794462
-0.450373739257 0.109782568089
-0.450370552317 0.109767322898
-0.450367293287 0.109752058878
-0.450363962167 0.109736776023
-0.450360558954 0.109721474325
-0.450357083646 0.109706153774
-0.450353536243 0.109690814363
-0.450349916742 0.109675456083
-0.450346225141 0.109660078926
-0.45034246144 0.109644682885
-0.450338625636 0.10962926795
-0.450334717727 0.109613834114
-0.450330737711 0.109598381367
-0.450326685587 0.109582909704
-0.450322561352 0.109567419113
-0.450318365005 0.109551909589
-0.450314096543 0.109536381122
-0.450309755965 0.109520833704
-0.450305343269 0.109505267328
-0.450300858451 0.109489681984
-0.450296301511 0.109474077665
-0.450291672445 0.109458454363
-0.450286971252 0.109442812069
-0.45028219793 0.109427150775
-0.450277352476 0.109411470473
-0.450272434887 0.109395771154
-0.450267445162 0.109380052812
-0.450262383298 0.109364315437
-0.450257249293 0.109348559021
-0.450252043144 0.109332783557
-0.450246764848 0.109316989035
-0.450241414404 0.109301175449
-0.450235991808 0.109285342789
-0.450230497058 0.109269491048
-0.450224930151 0.109253620217
-0.450219291085 0.109237730289
-0.450213579857 0.109221821254
-0.450207796464 0.109205893106
-0.450201940904 0.109189945836
-0.450196013172 0.109173979436
-0.450190013268 0.109157993897
-0.450183941188 0.109141989212
-0.450177796928 0.109125965372
-0.450171580486 0.10910992237
-0.450165291859 0.109093860197
-0.450158931045 0.109077778846
-0.450152498039 0.109061678307
-0.450145992838 0.109045558574
-0.450139415441 0.109029419637
-0.450132765843 0.10901326149
-0.450126044041 0.108997084123
-0.450119250032 0.108980887528
-0.450112383813 0.108964671699
-0.450105445381 0.108948436626
-0.450098434731 0.108932182301
-0.450091351862 0.108915908717
-0.450084196769 0.108899615865
-0.450076969448 0.108883303738
-0.450069669897 0.108866972326
-0.450062298112 0.108850621623
-0.450054854089 0.108834251621
-0.450047337825 0.10881786231
-0.450039749317 0.108801453683
-0.450032088559 0.108785025733
-0.45002435555 0.10876857845
-0.450016550285 0.108752111828
-0.45000867276 0.108735625857
-0.450000722971 0.108719120531
-0.449992700915 0.10870259584
-0.449984606588 0.108686051778
-0.449976439986 0.108669488335
-0.449968201105 0.108652905505
-0.449959889941 0.108636303278
-0.44995150649 0.108619681647
-0.449943050748 0.108603040604
-0.449934522711 0.108586380141
-0.449925922375 0.108569700251
-0.449917249735 0.108553000924
-0.449908504788 0.108536282153
-0.449899687529 0.10851954393
-0.449890797954 0.108502786247
-0.449881836058 0.108486009096
-0.449872801839 0.10846921247
-0.44986369529 0.10845239636
-0.449854516408 0.108435560757
-0.449845265188 0.108418705655
-0.449835941625 0.108401831046
-0.449826545716 0.108384936921
-0.449817077456 0.108368023272
-0.44980753684 0.108351090092
-0.449797923864 0.108334137372
-0.449788238522 0.108317165105
-0.44977848081 0.108300173282
-0.449768650725 0.108283161897
-0.449758748259 0.10826613094
-0.44974877341 0.108249080404
-0.449738726172 0.108232010281
-0.449728606541 0.108214920563
-0.449718414511 0.108197811243
-0.449708150077 0.108180682311
-0.449697813235 0.108163533762
-0.449687403979 0.108146365585
-0.449676922305 0.108129177774
-0.449666368208 0.108111970321
-0.449655741682 0.108094743218
-0.449645042722 0.108077496457
-0.449634271323 0.108060230029
-0.44962342748 0.108042943928
-0.449612511188 0.108025638145
-0.449601522441 0.108008312673
-0.449590461234 0.107990967503
-0.449579327561 0.107973602628
-0.449568121418 0.10795621804
-0.449556842799 0.107938813731
-0.449545491698 0.107921389693
-0.449534068111 0.107903945918
-0.44952257203 0.107886482399
-0.449511003452 0.107868999128
-0.449499362369 0.107851496096
-0.449487648778 0.107833973296
-0.449475862671 0.10781643072
-0.449464004044 0.107798868361
-0.44945207289 0.10778128621
-0.449440069203 0.10776368426
-0.449427992979 0.107746062502
-0.449415844211 0.10772842093
-0.449403622893 0.107710759535
-0.449391329019 0.107693078309
-0.449378962583 0.107675377245
-0.44936652358 0.107657656335
-0.449354012003 0.107639915571
-0.449341427846 0.107622154945
-0.449328771104 0.107604374449
-0.449316041769 0.107586574077
-0.449303239837 0.107568753819
-0.449290365299 0.107550913668
-0.449277418152 0.107533053616
-0.449264398387 0.107515173656
-0.449251305999 0.10749727378
-0.449238140982 0.10747935398
-0.449224903328 0.107461414249
-0.449211593033 0.107443454578
-0.449198210088 0.107425474959
-0.449184754488 0.107407475386
-0.449171226226 0.10738945585
-0.449157625296 0.107371416343
-0.449143951691 0.107353356859
-0.449130205404 0.107335277388
-0.449116386429 0.107317177924
-0.449102494759 0.107299058458
-0.449088530387 0.107280918983
-0.449074493307 0.107262759492
-0.449060383511 0.107244579976
-0.449046200992 0.107226380427
-0.449031945745 0.107208160839
-0.449017617762 0.107189921203
-0.449003217035 0.107171661512
-0.448988743559 0.107153381758
-0.448974197326 0.107135081932
-0.448959578328 0.107116762029
-0.448944886559 0.107098422039
-0.448930122012 0.107080061956
-0.448915284679 0.107061681771
-0.448900374554 0.107043281476
-0.448885391628 0.107024861065
-0.448870335895 0.10700642053
-0.448855207348 0.106987959862
-0.448840005978 0.106969479054
-0.448824731779 0.106950978099
-0.448809384744 0.106932456989
-0.448793964864 0.106913915716
-0.448778472132 0.106895354272
-0.44876290654 0.106876772651
-0.448747268082 0.106858170843
-0.448731556749 0.106839548842
-0.448715772534 0.10682090664
-0.448699915429 0.10680224423
-0.448683985427 0.106783561603
-0.448667982519 0.106764858752
-0.448651906697 0.10674613567
-0.448635757955 0.106727392348
-0.448619536284 0.10670862878
-0.448603241676 0.106689844957
-0.448586874123 0.106671040873
-0.448570433617 0.106652216519
-0.448553920151 0.106633371887
-0.448537333716 0.106614506971
-0.448520674304 0.106595621762
-0.448503941906 0.106576716254
-0.448487136516 0.106557790438
-0.448470258124 0.106538844306
-0.448453306722 0.106519877852
-0.448436282303 0.106500891068
-0.448419184857 0.106481883946
-0.448402014376 0.106462856478
-0.448384770852 0.106443808657
-0.448367454277 0.106424740476
-0.448350064642 0.106405651927
-0.448332601939 0.106386543002
-0.448315066159 0.106367413694
-0.448297457293 0.106348263995
-0.448279775333 0.106329093897
-0.44826202027 0.106309903394
-0.448244192095 0.106290692477
-0.448226290801 0.10627146114
-0.448208316377 0.106252209374
-0.448190268816 0.106232937172
-0.448172148108 0.106213644526
-0.448153954244 0.106194331429
-0.448135687217 0.106174997874
-0.448117347015 0.106155643853
-0.448098933632 0.106136269358
-0.448080447057 0.106116874382
-0.448061887282 0.106097458918
-0.448043254297 0.106078022957
-0.448024548094 0.106058566493
-0.448005768663 0.106039089517
-0.447986915994 0.106019592024
-0.44796799008 0.106000074004
-0.44794899091 0.10598053545
-0.447929918475 0.105960976356
-0.447910772766 0.105941396713
-0.447891553773 0.105921796514
-0.447872261487 0.105902175751
-0.447852895899 0.105882534418
-0.447833456999 0.105862872507
-0.447813944777 0.105843190009
-0.447794359223 0.105823486918
-0.447774700329 0.105803763227
-0.447754968085 0.105784018927
-0.447735162481 0.105764254012
-0.447715283506 0.105744468474
-0.447695331152 0.105724662305
-0.447675305408 0.105704835498
-0.447655206266 0.105684988046
-0.447635033713 0.105665119942
-0.447614787742 0.105645231177
-0.447594468342 0.105625321744
-0.447574075502 0.105605391636
-0.447553609214 0.105585440846
-0.447533069466 0.105565469366
-0.447512456249 0.105545477189
-0.447491769552 0.105525464307
-0.447471009366 0.105505430713
-0.44745017568 0.105485376399
-0.447429268484 0.105465301359
-0.447408287767 0.105445205584
-0.447387233519 0.105425089068
-0.44736610573 0.105404951803
-0.44734490439 0.105384793781
-0.447323629487 0.105364614996
-0.447302281012 0.105344415439
-0.447280858954 0.105324195104
-0.447259363302 0.105303953983
-0.447237794046 0.105283692069
-0.447216151175 0.105263409354
-0.447194434678 0.105243105831
-0.447172644545 0.105222781493
-0.447150780765 0.105202436333
-0.447128843326 0.105182070342
-0.44710683222 0.105161683514
-0.447084747433 0.105141275841
-0.447062588956 0.105120847316
-0.447040356777 0.105100397932
-0.447018050886 0.105079927682
-0.446995671271 0.105059436557
-0.446973217922 0.105038924551
-0.446950690827 0.105018391656
-0.446928089974 0.104997837866
-0.446905415354 0.104977263172
-0.446882666955 0.104956667568
-0.446859844765 0.104936051045
-0.446836948773 0.104915413598
-0.446813978968 0.104894755218
-0.446790935338 0.104874075899
-0.446767817872 0.104853375632
-0.446744626559 0.104832654411
-0.446721361387 0.104811912228
-0.446698022344 0.104791149077
-0.446674609419 0.104770364949
-0.4466511226 0.104749559838
-0.446627561876 0.104728733737
-0.446603927235 0.104707886637
-0.446580218665 0.104687018532
-0.446556436154 0.104666129415
-0.446532579691 0.104645219277
-0.446508649263 0.104624288113
-0.44648464486 0.104603335915
-0.446460566468 0.104582362675
-0.446436414076 0.104561368386
-0.446412187673 0.104540353042
-0.446387887245 0.104519316634
-0.44636351278 0.104498259156
-0.446339064268 0.1044771806
-0.446314541695 0.104456080959
-0.446289945049 0.104434960226
-0.446265274318 0.104413818394
-0.44624052949 0.104392655455
-0.446215710553 0.104371471403
-0.446190817493 0.104350266229
-0.446165850299 0.104329039927
-0.446140808958 0.10430779249
-0.446115693458 0.104286523911
-0.446090503786 0.104265234181
-0.44606523993 0.104243923295
-0.446039901877 0.104222591245
-0.446014489614 0.104201238023
-0.445989003129 0.104179863623
-0.445963442408 0.104158468037
-0.44593780744 0.104137051258
-0.445912098212 0.104115613279
-0.445886314709 0.104094154093
-0.445860456921 0.104072673693
-0.445834524833 0.104051172071
-0.445808518433 0.10402964922
-0.445782437707 0.104008105134
-0.445756282644 0.103986539804
-0.445730053229 0.103964953225
-0.445703749449 0.103943345388
-0.445677371292 0.103921716287
-0.445650918744 0.103900065914
-0.445624391792 0.103878394263
-0.445597790422 0.103856701325
-0.445571114622 0.103834987095
-0.445544364377 0.103813251565
-0.445517539675 0.103791494728
-0.445490640502 0.103769716576
-0.445463666845 0.103747917103
-0.445436618689 0.103726096301
-0.445409496022 0.103704254164
-0.44538229883 0.103682390684
-0.445355027099 0.103660505854
-0.445327680815 0.103638599668
-0.445300259965 0.103616672117
-0.445272764535 0.103594723195
-0.445245194512 0.103572752895
-0.44521754988 0.10355076121
-0.445189830627 0.103528748132
-0.445162036738 0.103506713655
-0.4451341682 0.103484657771
-0.445106224998 0.103462580474
-0.445078207119 0.103440481756
-0.445050114548 0.103418361611
-0.445021947271 0.10339622003
-0.444993705274 0.103374057008
-0.444965388543 0.103351872537
-0.444936997063 0.10332966661
-0.44490853082 0.103307439221
-0.4448799898 0.103285190361
-0.444851373989 0.103262920024
-0.444822683371 0.103240628203
-0.444793917933 0.103218314891
-0.44476507766 0.10319598008
-0.444736162537 0.103173623765
-0.44470717255 0.103151245937
-0.444678107685 0.10312884659
-0.444648967925 0.103106425717
-0.444619753258 0.103083983311
-0.444590463667 0.103061519364
-0.444561099139 0.10303903387
-0.444531659658 0.103016526822
-0.444502145209 0.102993998213
-0.444472555778 0.102971448035
-0.44444289135 0.102948876282
-0.444413151909 0.102926282947
-0.44438333744 0.102903668023
-0.444353447929 0.102881031502
-0.44432348336 0.102858373379
-0.444293443718 0.102835693645
-0.444263328988 0.102812992294
-0.444233139154 0.102790269319
-0.444202874202 0.102767524712
-0.444172534115 0.102744758468
-0.444142118879 0.102721970579
-0.444111628478 0.102699161038
-0.444081062896 0.102676329838
-0.444050422119 0.102653476972
-0.444019706129 0.102630602433
-0.443988914913 0.102607706214
-0.443958048454 0.102584788309
-0.443927106736 0.102561848711
-0.443896089744 0.102538887411
-0.443864997462 0.102515904404
-0.443833829874 0.102492899683
-0.443802586965 0.102469873241
-0.443771268717 0.10244682507
-0.443739875117 0.102423755164
-0.443708406146 0.102400663516
-0.44367686179 0.102377550119
-0.443645242032 0.102354414966
-0.443613546857 0.10233125805
-0.443581776247 0.102308079365
-0.443549930188 0.102284878903
-0.443518008662 0.102261656658
-0.443486011653 0.102238412622
-0.443453939145 0.102215146789
-0.443421791121 0.102191859152
-0.443389567566 0.102168549703
-0.443357268462 0.102145218437
-0.443324893793 0.102121865346
-0.443292443543 0.102098490424
-0.443259917695 0.102075093663
-0.443227316233 0.102051675056
-0.443194639138 0.102028234598
-0.443161886396 0.10200477228
-0.443129057989 0.101981288096
-0.4430961539 0.10195778204
-0.443063174113 0.101934254104
-0.44303011861 0.101910704281
-0.442996987375 0.101887132565
-0.442963780391 0.101863538949
-0.44293049764 0.101839923426
-0.442897139105 0.101816285989
-0.44286370477 0.101792626632
-0.442830194617 0.101768945346
-0.442796608629 0.101745242127
-0.442762946789 0.101721516967
-0.442729209079 0.101697769858
-0.442695395483 0.101674000795
-0.442661505982 0.101650209771
-0.442627540559 0.101626396778
-0.442593499197 0.101602561809
-0.442559381878 0.101578704859
-0.442525188585 0.10155482592
-0.4424909193 0.101530924986
-0.442456574005 0.101507002049
-0.442422152683 0.101483057104
-0.442387655317 0.101459090142
-0.442353081887 0.101435101157
-0.442318432376 0.101411090144
-0.442283706767 0.101387057094
-0.442248905042 0.101363002001
-0.442214027182 0.101338924858
-0.44217907317 0.101314825659
-0.442144042987 0.101290704396
-0.442108936615 0.101266561063
-0.442073754037 0.101242395654
-0.442038495234 0.101218208161
-0.442003160187 0.101193998578
-0.441967748879 0.101169766898
-0.441932261292 0.101145513114
-0.441896697406 0.10112123722
-0.441861057203 0.101096939208
-0.441825340665 0.101072619073
-0.441789547774 0.101048276807
-0.44175367851 0.101023912403
-0.441717732856 0.100999525855
-0.441681710792 0.100975117157
-0.441645612301 0.100950686301
-0.441609437362 0.10092623328
-0.441573185957 0.100901758089
-0.441536858069 0.10087726072
-0.441500453676 0.100852741167
-0.441463972762 0.100828199422
-0.441427415306 0.10080363548
-0.44139078129 0.100779049334
-0.441354070694 0.100754440976
-0.4413172835 0.1007298104
-0.441280419689 0.1007051576
-0.44124347924 0.100680482569
-0.441206462136 0.1006557853
-0.441169368356 0.100631065787
-0.441132197882 0.100606324022
-0.441094950693 0.100581559999
-0.441057626771 0.100556773712
-0.441020226096 0.100531965154
-0.440982748648 0.100507134318
-0.440945194408 0.100482281198
-0.440907563356 0.100457405786
-0.440869855473 0.100432508076
-0.440832070739 0.100407588063
-0.440794209134 0.100382645738
-0.440756270638 0.100357681095
-0.440718255232 0.100332694128
-0.440680162895 0.100307684831
-0.440641993608 0.100282653195
-0.44060374735 0.100257599216
-0.440565424102 0.100232522885
-0.440527023844 0.100207424197
-0.440488546554 0.100182303146
-0.440449992214 0.100157159723
-0.440411360803 0.100131993923
-0.4403726523 0.10010680574
-0.440333866686 0.100081595166
-0.440295003939 0.100056362195
-0.44025606404 0.10003110682
-0.440217046968 0.100005829035
-0.440177952702 0.0999805288331
-0.440138781223 0.0999552062079
-0.440099532508 0.0999298611527
-0.440060206538 0.0999044936609
-0.440020803292 0.099879103726
-0.43998132275 0.0998536913414
-0.439941764889 0.0998282565005
-0.43990212969 0.0998027991968
-0.439862417132 0.0997773194236
-0.439822627193 0.0997518171745
-0.439782759853 0.0997262924429
-0.43974281509 0.0997007452222
-0.439702792884 0.0996751755059
-0.439662693213 0.0996495832874
-0.439622516056 0.0996239685603
-0.439582261392 0.0995983313179
-0.4395419292 0.0995726715537
-0.439501519458 0.0995469892612
-0.439461032145 0.0995212844338
-0.439420467239 0.0994955570651
-0.439379824719 0.0994698071485
-0.439339104563 0.0994440346775
-0.43929830675 0.0994182396455
-0.439257431259 0.0993924220461
-0.439216478066 0.0993665818728
-0.439175447152 0.099340719119
-0.439134338493 0.0993148337782
-0.439093152069 0.099288925844
-0.439051887856 0.0992629953098
-0.439010545834 0.0992370421692
-0.43896912598 0.0992110664156
-0.438927628273 0.0991850680426
-0.438886052689 0.0991590470436
-0.438844399208 0.0991330034123
-0.438802667806 0.0991069371421
-0.438760858462 0.0990808482265
-0.438718971154 0.0990547366591
-0.438677005858 0.0990286024334
-0.438634962553 0.099002445543
-0.438592841216 0.0989762659813
-0.438550641825 0.0989500637419
-0.438508364357 0.0989238388184
-0.43846600879 0.0988975912043
-0.438423575101 0.0988713208932
-0.438381063267 0.0988450278785
-0.438338473265 0.098818712154
-0.438295805073 0.098792373713
-0.438253058668 0.0987660125493
-0.438210234027 0.0987396286563
-0.438167331127 0.0987132220276
-0.438124349945 0.0986867926568
-0.438081290458 0.0986603405375
-0.438038152643 0.0986338656632
-0.437994936477 0.0986073680276
-0.437951641937 0.0985808476242
-0.437908268999 0.0985543044466
-0.43786481764 0.0985277384883
-0.437821287836 0.0985011497431
-0.437777679565 0.0984745382045
-0.437733992803 0.098447903866
-0.437690227526 0.0984212467213
-0.437646383711 0.0983945667641
-0.437602461334 0.0983678639878
-0.437558460372 0.0983411383861
-0.4375143808 0.0983143899527
-0.437470222596 0.0982876186812
-0.437425985735 0.0982608245651
-0.437381670193 0.0982340075981
-0.437337275947 0.0982071677739
-0.437292802972 0.098180305086
-0.437248251245 0.0981534195281
-0.437203620741 0.0981265110939
-0.437158911436 0.0980995797769
-0.437114123307 0.0980726255708
-0.437069256328 0.0980456484694
-0.437024310476 0.0980186484661
-0.436979285726 0.0979916255547
-0.436934182054 0.0979645797289
-0.436888999435 0.0979375109822
-0.436843737846 0.0979104193084
-0.43679839726 0.0978833047011
-0.436752977655 0.097856167154
-0.436707479004 0.0978290066608
-0.436661901284 0.0978018232151
-0.436616244469 0.0977746168107
-0.436570508536 0.0977473874411
-0.436524693458 0.0977201351001
-0.436478799211 0.0976928597814
-0.436432825771 0.0976655614786
-0.436386773111 0.0976382401855
-0.436340641207 0.0976108958958
-0.436294430034 0.0975835286031
-0.436248139567 0.0975561383012
-0.43620176978 0.0975287249838
-0.436155320648 0.0975012886445
-0.436108792146 0.0974738292771
-0.436062184248 0.0974463468753
-0.436015496929 0.0974188414329
-0.435968730164 0.0973913129435
-0.435921883926 0.0973637614008
-0.43587495819 0.0973361867987
-0.435827952931 0.0973085891308
-0.435780868122 0.0972809683909
-0.435733703738 0.0972533245727
-0.435686459754 0.0972256576699
-0.435639136142 0.0971979676763
-0.435591732878 0.0971702545857
-0.435544249935 0.0971425183918
-0.435496687288 0.0971147590882
-0.435449044909 0.0970869766689
-0.435401322773 0.0970591711276
-0.435353520854 0.097031342458
-0.435305639125 0.0970034906538
-0.435257677561 0.0969756157089
-0.435209636134 0.0969477176171
-0.435161514818 0.096919796372
-0.435113313586 0.0968918519676
-0.435065032413 0.0968638843974
-0.435016671272 0.0968358936555
-0.434968230135 0.0968078797354
-0.434919708976 0.0967798426311
-0.434871107769 0.0967517823364
-0.434822426486 0.0967236988449
-0.434773665101 0.0966955921505
-0.434724823586 0.0966674622471
-0.434675901915 0.0966393091284
-0.43462690006 0.0966111327882
-0.434577817995 0.0965829332203
-0.434528655692 0.0965547104186
-0.434479413125 0.0965264643769
-0.434430090264 0.096498195089
-0.434380687085 0.0964699025487
-0.434331203558 0.0964415867499
-0.434281639656 0.0964132476864
-0.434231995353 0.0963848853519
-0.43418227062 0.0963564997404
-0.434132465429 0.0963280908457
-0.434082579754 0.0962996586616
-0.434032613566 0.0962712031821
-0.433982566838 0.0962427244008
-0.433932439541 0.0962142223117
-0.433882231648 0.0961856969086
-0.43383194313 0.0961571481855
-0.43378157396 0.0961285761361
-0.43373112411 0.0960999807543
-0.433680593551 0.096071362034
-0.433629982256 0.096042719969
-0.433579290195 0.0960140545533
-0.433528517341 0.0959853657807
-0.433477663665 0.0959566536451
-0.433426729139 0.0959279181403
-0.433375713734 0.0958991592603
-0.433324617422 0.0958703769989
-0.433273440174 0.09584157135
-0.433222181961 0.0958127423076
-0.433170842755 0.0957838898655
-0.433119422527 0.0957550140176
-0.433067921248 0.0957261147579
-0.433016338889 0.0956971920802
-0.432964675421 0.0956682459784
-0.432912930815 0.0956392764465
-0.432861105041 0.0956102834784
-0.432809198072 0.0955812670679
-0.432757209877 0.0955522272091
-0.432705140428 0.0955231638958
-0.432652989694 0.095494077122
-0.432600757647 0.0954649668815
-0.432548444257 0.0954358331685
-0.432496049495 0.0954066759766
-0.432443573331 0.0953774953
-0.432391015735 0.0953482911326
-0.432338376678 0.0953190634682
-0.432285656129 0.0952898123009
-0.43223285406 0.0952605376246
-0.43217997044 0.0952312394332
-0.432127005239 0.0952019177208
-0.432073958428 0.0951725724812
-0.432020829976 0.0951432037085
-0.431967619852 0.0951138113965
-0.431914328028 0.0950843955394
-0.431860954473 0.095054956131
-0.431807499155 0.0950254931653
-0.431753962046 0.0949960066364
-0.431700343114 0.0949664965381
-0.43164664233 0.0949369628645
-0.431592859661 0.0949074056096
-0.431538995079 0.0948778247673
-0.431485048552 0.0948482203317
-0.431431020049 0.0948185922967
-0.43137690954 0.0947889406564
-0.431322716994 0.0947592654047
-0.43126844238 0.0947295665357
-0.431214085667 0.0946998440433
-0.431159646823 0.0946700979217
-0.431105125818 0.0946403281647
-0.431050522621 0.0946105347664
-0.4309958372 0.0945807177209
-0.430941069524 0.0945508770221
-0.430886219562 0.0945210126641
-0.430831287282 0.0944911246409
-0.430776272652 0.0944612129466
-0.430721175642 0.0944312775752
-0.43066599622 0.0944013185207
-0.430610734353 0.0943713357772
-0.43055539001 0.0943413293386
-0.43049996316 0.0943112991992
-0.43044445377 0.0942812453529
-0.430388861809 0.0942511677937
-0.430333187244 0.0942210665157
-0.430277430043 0.0941909415131
-0.430221590175 0.0941607927798
-0.430165667607 0.0941306203099
-0.430109662307 0.0941004240975
-0.430053574243 0.0940702041367
-0.429997403381 0.0940399604215
-0.429941149691 0.094009692946
-0.429884813138 0.0939794017043
-0.429828393691 0.0939490866905
-0.429771891317 0.0939187478986
-0.429715305983 0.0938883853228
-0.429658637657 0.0938579989572
-0.429601886306 0.0938275887958
-0.429545051896 0.0937971548327
-0.429488134395 0.0937666970621
-0.429431133769 0.093736215478
-0.429374049986 0.0937057100746
-0.429316883013 0.093675180846
-0.429259632816 0.0936446277862
-0.429202299361 0.0936140508895
-0.429144882616 0.0935834501499
-0.429087382548 0.0935528255615
-0.429029799122 0.0935221771185
-0.428972132304 0.093491504815
-0.428914382063 0.0934608086451
-0.428856548363 0.093430088603
-0.42879863117 0.0933993446828
-0.428740630452 0.0933685768786
-0.428682546174 0.0933377851847
-0.428624378303 0.093306969595
-0.428566126803 0.0932761301039
-0.428507791642 0.0932452667054
-0.428449372784 0.0932143793936
-0.428390870196 0.0931834681628
-0.428332283843 0.0931525330072
-0.428273613692 0.0931215739208
-0.428214859706 0.0930905908978
-0.428156021853 0.0930595839325
-0.428097100097 0.093028553019
-0.428038094404 0.0929974981514
-0.427979004739 0.0929664193239
-0.427919831068 0.0929353165308
-0.427860573355 0.0929041897662
-0.427801231565 0.0928730390243
-0.427741805663 0.0928418642992
-0.427682295616 0.0928106655853
-0.427622701386 0.0927794428766
-0.42756302294 0.0927481961674
-0.427503260241 0.0927169254519
-0.427443413255 0.0926856307242
-0.427383481946 0.0926543119787
-0.427323466279 0.0926229692094
-0.427263366217 0.0925916024107
-0.427203181726 0.0925602115767
-0.42714291277 0.0925287967017
-0.427082559313 0.0924973577798
-0.427022121319 0.0924658948054
-0.426961598752 0.0924344077726
-0.426900991577 0.0924028966756
-0.426840299757 0.0923713615087
-0.426779523256 0.0923398022662
-0.426718662038 0.0923082189423
-0.426657716067 0.0922766115312
-0.426596685306 0.0922449800271
-0.426535569719 0.0922133244244
-0.426474369269 0.0921816447172
-0.426413083921 0.0921499408998
-0.426351713637 0.0921182129666
-0.42629025838 0.0920864609116
-0.426228718115 0.0920546847293
-0.426167092803 0.0920228844139
-0.426105382409 0.0919910599596
-0.426043586895 0.0919592113607
-0.425981706225 0.0919273386115
-0.42591974036 0.0918954417063
-0.425857689264 0.0918635206393
-0.4257955529 0.0918315754048
-0.42573333123 0.0917996059972
-0.425671024217 0.0917676124107
-0.425608631823 0.0917355946396
-0.425546154012 0.0917035526782
-0.425483590744 0.0916714865208
-0.425420941983 0.0916393961616
-0.425358207691 0.0916072815951
-0.425295387829 0.0915751428155
-0.425232482361 0.0915429798172
-0.425169491248 0.0915107925943
-0.425106414451 0.0914785811413
-0.425043251933 0.0914463454525
-0.424980003656 0.0914140855222
-0.424916669581 0.0913818013447
-0.424853249669 0.0913494929143
-0.424789743884 0.0913171602254
-0.424726152185 0.0912848032724
-0.424662474534 0.0912524220494
-0.424598710893 0.091220016551
-0.424534861223 0.0911875867713
-0.424470925485 0.0911551327049
-0.42440690364 0.0911226543459
-0.424342795649 0.0910901516889
-0.424278601474 0.091057624728
-0.424214321074 0.0910250734577
-0.424149954412 0.0909924978724
-0.424085501446 0.0909598979664
-0.424020962139 0.090927273734
-0.423956336451 0.0908946251696
-0.423891624342 0.0908619522677
-0.423826825773 0.0908292550225
-0.423761940703 0.0907965334285
-0.423696969094 0.0907637874801
-0.423631910906 0.0907310171715
-0.423566766097 0.0906982224972
-0.42350153463 0.0906654034517
-0.423436216463 0.0906325600292
-0.423370811556 0.0905996922241
-0.423305319869 0.090566800031
-0.423239741363 0.0905338834441
-0.423174075996 0.0905009424579
-0.423108323728 0.0904679770667
-0.423042484518 0.0904349872651
-0.422976558327 0.0904019730473
-0.422910545113 0.0903689344078
-0.422844444835 0.0903358713411
-0.422778257453 0.0903027838415
-0.422711982926 0.0902696719035
-0.422645621213 0.0902365355214
-0.422579172272 0.0902033746898
-0.422512636063 0.090170189403
-0.422446012544 0.0901369796555
-0.422379301674 0.0901037454418
-0.422312503412 0.0900704867562
-0.422245617716 0.0900372035931
-0.422178644545 0.0900038959472
-0.422111583856 0.0899705638127
-0.422044435609 0.0899372071842
-0.421977199761 0.089903826056
-0.421909876271 0.0898704204228
-0.421842465096 0.0898369902788
-0.421774966195 0.0898035356186
-0.421707379525 0.0897700564366
-0.421639705045 0.0897365527274
-0.421571942711 0.0897030244853
-0.421504092482 0.0896694717049
-0.421436154315 0.0896358943806
-0.421368128168 0.0896022925069
-0.421300013997 0.0895686660783
-0.421231811761 0.0895350150893
-0.421163521416 0.0895013395343
-0.42109514292 0.0894676394079
-0.42102667623 0.0894339147045
-0.420958121302 0.0894001654186
-0.420889478093 0.0893663915448
-0.420820746561 0.0893325930776
-0.420751926662 0.0892987700113
-0.420683018353 0.0892649223406
-0.420614021589 0.08923105006
-0.420544936329 0.089197153164
-0.420475762527 0.089163231647
-0.420406500141 0.0891292855037
-0.420337149126 0.0890953147285
-0.420267709439 0.0890613193159
-0.420198181036 0.0890272992605
-0.420128563872 0.0889932545568
-0.420058857904 0.0889591851994
-0.419989063087 0.0889250911827
-0.419919179377 0.0888909725014
-0.41984920673 0.0888568291499
-0.419779145101 0.0888226611228
-0.419708994445 0.0887884684146
-0.419638754719 0.0887542510199
-0.419568425876 0.0887200089333
-0.419498007873 0.0886857421493
-0.419427500665 0.0886514506625
-0.419356904206 0.0886171344673
-0.419286218451 0.0885827935585
-0.419215443356 0.0885484279305
-0.419144578874 0.0885140375779
-0.419073624961 0.0884796224953
-0.419002581571 0.0884451826773
-0.418931448659 0.0884107181184
-0.418860226179 0.0883762288132
-0.418788914086 0.0883417147563
-0.418717512333 0.0883071759423
-0.418646020875 0.0882726123658
-0.418574439665 0.0882380240214
-0.418502768658 0.0882034109036
-0.418431007808 0.0881687730071
-0.418359157068 0.0881341103265
-0.418287216391 0.0880994228563
-0.418215185733 0.0880647105911
-0.418143065045 0.0880299735257
-0.418070854283 0.0879952116545
-0.417998553397 0.0879604249722
-0.417926162343 0.0879256134735
-0.417853681073 0.0878907771528
-0.41778110954 0.0878559160049
-0.417708447698 0.0878210300245
-0.417635695498 0.087786119206
-0.417562852894 0.0877511835441
-0.417489919839 0.0877162230335
-0.417416896285 0.0876812376688
-0.417343782184 0.0876462274447
-0.417270577489 0.0876111923557
-0.417197282153 0.0875761323966
-0.417123896126 0.0875410475619
-0.417050419363 0.0875059378464
-0.416976851814 0.0874708032446
-0.416903193432 0.0874356437513
-0.416829444168 0.087400459361
-0.416755603975 0.0873652500686
-0.416681672803 0.0873300158685
-0.416607650605 0.0872947567555
-0.416533537331 0.0872594727242
-0.416459332934 0.0872241637693
-0.416385037364 0.0871888298856
-0.416310650573 0.0871534710676
-0.416236172512 0.08711808731
-0.416161603132 0.0870826786076
-0.416086942383 0.087047244955
-0.416012190217 0.0870117863469
-0.415937346584 0.086976302778
-0.415862411435 0.086940794243
-0.415787384721 0.0869052607366
-0.415712266391 0.0868697022534
-0.415637056396 0.0868341187882
-0.415561754687 0.0867985103357
-0.415486361213 0.0867628768906
-0.415410875924 0.0867272184476
-0.415335298771 0.0866915350015
-0.415259629704 0.0866558265468
-0.415183868671 0.0866200930784
-0.415108015623 0.086584334591
-0.41503207051 0.0865485510793
-0.41495603328 0.086512742538
-0.414879903883 0.0864769089618
-0.414803682268 0.0864410503455
-0.414727368385 0.0864051666838
-0.414650962183 0.0863692579715
-0.414574463609 0.0863333242033
-0.414497872615 0.0862973653739
-0.414421189147 0.0862613814781
-0.414344413155 0.0862253725106
-0.414267544587 0.0861893384662
-0.414190583392 0.0861532793396
-0.414113529518 0.0861171951256
-0.414036382914 0.086081085819
-0.413959143527 0.0860449514144
-0.413881811305 0.0860087919067
-0.413804386198 0.0859726072907
-0.413726868151 0.0859363975611
-0.413649257114 0.0859001627126
-0.413571553033 0.0858639027402
-0.413493755857 0.0858276176384
-0.413415865532 0.0857913074022
-0.413337882007 0.0857549720262
-0.413259805228 0.0857186115053
-0.413181635142 0.0856822258344
-0.413103371697 0.085645815008
-0.41302501484 0.0856093790212
-0.412946564516 0.0855729178685
-0.412868020674 0.085536431545
-0.412789383259 0.0854999200453
-0.412710652219 0.0854633833642
-0.412631827498 0.0854268214966
-0.412552909045 0.0853902344373
-0.412473896805 0.0853536221811
-0.412394790724 0.0853169847228
-0.412315590748 0.0852803220572
-0.412236296823 0.0852436341792
-0.412156908894 0.0852069210835
-0.412077426908 0.085170182765
-0.411997850811 0.0851334192186
-0.411918180546 0.085096630439
-0.41183841606 0.085059816421
-0.411758557299 0.0850229771597
-0.411678604207 0.0849861126496
-0.411598556728 0.0849492228858
-0.411518414809 0.0849123078631
-0.411438178394 0.0848753675762
-0.411357847428 0.0848384020202
-0.411277421855 0.0848014111897
-0.411196901619 0.0847643950796
-0.411116286666 0.0847273536849
-0.411035576939 0.0846902870004
-0.410954772382 0.0846531950209
-0.410873872941 0.0846160777414
-0.410792878557 0.0845789351566
-0.410711789176 0.0845417672614
-0.410630604742 0.0845045740508
-0.410549325197 0.0844673555196
-0.410467950485 0.0844301116627
-0.410386480549 0.084392842475
-0.410304915334 0.0843555479513
-0.410223254781 0.0843182280865
-0.410141498835 0.0842808828756
-0.410059647438 0.0842435123134
-0.409977700532 0.0842061163948
-0.409895658061 0.0841686951147
-0.409813519968 0.0841312484681
-0.409731286194 0.0840937764498
-0.409648956682 0.0840562790547
-0.409566531374 0.0840187562777
-0.409484010213 0.0839812081138
-0.40940139314 0.0839436345579
-0.409318680098 0.0839060356048
-0.409235871028 0.0838684112496
-0.409152965872 0.0838307614871
-0.409069964571 0.0837930863122
-0.408986867068 0.0837553857199
-0.408903673302 0.0837176597051
-0.408820383217 0.0836799082627
-0.408736996752 0.0836421313878
-0.408653513848 0.0836043290751
-0.408569934448 0.0835665013197
-0.40848625849 0.0835286481165
-0.408402485917 0.0834907694604
-0.408318616668 0.0834528653464
-0.408234650684 0.0834149357695
-0.408150587905 0.0833769807246
-0.408066428271 0.0833390002066
-0.407982171724 0.0833009942106
-0.407897818201 0.0832629627314
-0.407813367644 0.083224905764
-0.407728819991 0.0831868233035
-0.407644175184 0.0831487153448
-0.40755943316 0.0831105818828
-0.407474593859 0.0830724229125
-0.407389657221 0.0830342384289
-0.407304623185 0.0829960284271
-0.40721949169 0.0829577929018
-0.407134262674 0.0829195318483
-0.407048936076 0.0828812452614
-0.406963511835 0.0828429331361
-0.406877989889 0.0828045954674
-0.406792370178 0.0827662322504
-0.406706652638 0.08272784348
-0.406620837208 0.0826894291512
-0.406534923827 0.082650989259
-0.406448912431 0.0826125237985
-0.40636280296 0.0825740327646
-0.40627659535 0.0825355161523
-0.406190289539 0.0824969739567
-0.406103885464 0.0824584061729
-0.406017383063 0.0824198127957
-0.405930782272 0.0823811938202
-0.405844083029 0.0823425492415
-0.405757285271 0.0823038790546
-0.405670388935 0.0822651832545
-0.405583393956 0.0822264618362
-0.405496300272 0.0821877147948
-0.405409107819 0.0821489421253
-0.405321816534 0.0821101438228
-0.405234426351 0.0820713198822
-0.405146937208 0.0820324702988
-0.40505934904 0.0819935950674
-0.404971661784 0.0819546941831
-0.404883875373 0.0819157676411
-0.404795989745 0.0818768154363
-0.404708004835 0.0818378375638
-0.404619920577 0.0817988340186
-0.404531736906 0.081759804796
-0.404443453759 0.0817207498908
-0.404355071069 0.0816816692982
-0.404266588772 0.0816425630132
-0.404178006801 0.0816034310309
-0.404089325092 0.0815642733465
-0.404000543578 0.0815250899549
-0.403911662195 0.0814858808513
-0.403822680875 0.0814466460307
-0.403733599553 0.0814073854882
-0.403644418163 0.081368099219
-0.403555136638 0.081328787218
-0.403465754911 0.0812894494805
-0.403376272917 0.0812500860015
-0.403286690589 0.081210696776
-0.403197007859 0.0811712817993
-0.403107224661 0.0811318410664
-0.403017340927 0.0810923745724
-0.40292735659 0.0810528823124
-0.402837271583 0.0810133642815
-0.402747085838 0.080973820475
-0.402656799288 0.0809342508877
-0.402566411864 0.080894655515
-0.402475923499 0.0808550343519
-0.402385334124 0.0808153873935
-0.402294643672 0.080775714635
-0.402203852074 0.0807360160715
-0.402112959262 0.0806962916981
-0.402021965166 0.08065654151
-0.401930869718 0.0806167655024
-0.401839672849 0.0805769636702
-0.401748374491 0.0805371360088
-0.401656974573 0.0804972825131
-0.401565473027 0.0804574031785
-0.401473869783 0.080417498
-0.401382164771 0.0803775669728
-0.401290357921 0.0803376100921
-0.401198449165 0.0802976273529
-0.401106438431 0.0802576187505
-0.401014325649 0.0802175842801
-0.40092211075 0.0801775239368
-0.400829793662 0.0801374377157
-0.400737374315 0.080097325612
-0.400644852639 0.080057187621
-0.400552228562 0.0800170237378
-0.400459502013 0.0799768339575
-0.400366672921 0.0799366182754
-0.400273741215 0.0798963766866
-0.400180706823 0.0798561091863
-0.400087569674 0.0798158157698
-0.399994329695 0.0797754964321
-0.399900986816 0.0797351511686
-0.399807540963 0.0796947799743
-0.399713992065 0.0796543828445
-0.399620340049 0.0796139597745
-0.399526584843 0.0795735107593
-0.399432726374 0.0795330357942
-0.399338764569 0.0794925348745
-0.399244699356 0.0794520079953
-0.399150530661 0.0794114551518
-0.39905625841 0.0793708763393
-0.398961882531 0.079330271553
-0.39886740295 0.079289640788
-0.398772819594 0.0792489840397
-0.398678132388 0.0792083013033
-0.398583341258 0.0791675925739
-0.39848844613 0.0791268578469
-0.39839344693 0.0790860971174
-0.398298343584 0.0790453103807
-0.398203136017 0.079004497632
-0.398107824153 0.0789636588666
-0.398012407919 0.0789227940797
-0.397916887239 0.0788819032666
-0.397821262037 0.0788409864225
-0.397725532239 0.0788000435426
-0.397629697769 0.0787590746223
-0.397533758551 0.0787180796567
-0.397437714509 0.0786770586412
-0.397341565568 0.078636011571
-0.39724531165 0.0785949384413
-0.397148952681 0.0785538392475
-0.397052488582 0.0785127139848
-0.396955919279 0.0784715626485
-0.396859244693 0.0784303852338
-0.396762464748 0.078389181736
-0.396665579367 0.0783479521505
-0.396568588473 0.0783066964724
-0.396471491988 0.0782654146971
-0.396374289834 0.0782241068199
-0.396276981934 0.078182772836
-0.396179568209 0.0781414127408
-0.396082048583 0.0781000265295
-0.395984422975 0.0780586141974
-0.395886691309 0.0780171757399
-0.395788853506 0.0779757111522
-0.395690909486 0.0779342204296
-0.395592859171 0.0778927035675
-0.395494702482 0.0778511605612
-0.39539643934 0.077809591406
-0.395298069664 0.0777679960971
-0.395199593377 0.0777263746299
-0.395101010397 0.0776847269998
-0.395002320646 0.077643053202
-0.394903524042 0.0776013532319
-0.394804620506 0.0775596270847
-0.394705609958 0.0775178747559
-0.394606492317 0.0774760962408
-0.394507267501 0.0774342915346
-0.394407935431 0.0773924606328
-0.394308496026 0.0773506035307
-0.394208949203 0.0773087202236
-0.394109294882 0.0772668107068
-0.39400953298 0.0772248749757
-0.393909663418 0.0771829130257
-0.393809686111 0.0771409248521
-0.393709600979 0.0770989104503
-0.393609407938 0.0770568698155
-0.393509106908 0.0770148029433
-0.393408697804 0.0769727098289
-0.393308180545 0.0769305904677
-0.393207555047 0.076888444855
-0.393106821227 0.0768462729863
-0.393005979002 0.0768040748569
-0.392905028288 0.0767618504622
-0.392803969002 0.0767195997976
-0.392702801061 0.0766773228583
-0.392601524379 0.07663501964
-0.392500138873 0.0765926901378
-0.392398644458 0.0765503343472
-0.39229704105 0.0765079522636
-0.392195328564 0.0764655438823
-0.392093506916 0.0764231091988
-0.39199157602 0.0763806482085
-0.391889535791 0.0763381609067
-0.391787386143 0.0762956472889
-0.391685126992 0.0762531073505
-0.39158275825 0.0762105410868
-0.391480279833 0.0761679484933
-0.391377691654 0.0761253295654
-0.391274993627 0.0760826842985
-0.391172185664 0.076040012688
-0.39106926768 0.0759973147294
-0.390966239588 0.075954590418
-0.390863101301 0.0759118397492
-0.39075985273 0.0758690627186
-0.39065649379 0.0758262593215
-0.390553024391 0.0757834295534
-0.390449444447 0.0757405734097
-0.39034575387 0.0756976908858
-0.39024195257 0.0756547819771
-0.390138040461 0.0756118466792
-0.390034017453 0.0755688849874
-0.389929883457 0.0755258968972
-0.389825638385 0.0754828824041
-0.389721282147 0.0754398415034
-0.389616814654 0.0753967741907
-0.389512235817 0.0753536804614
-0.389407545546 0.0753105603109
-0.389302743751 0.0752674137348
-0.389197830341 0.0752242407284
-0.389092805227 0.0751810412873
-0.388987668319 0.0751378154068
-0.388882419525 0.0750945630826
-0.388777058754 0.07505128431
-0.388671585916 0.0750079790845
-0.388566000919 0.0749646474016
-0.388460303672 0.0749212892568
-0.388354494083 0.0748779046455
-0.38824857206 0.0748344935633
-0.388142537512 0.0747910560056
-0.388036390346 0.0747475919679
-0.387930130469 0.0747041014457
-0.387823757789 0.0746605844345
-0.387717272213 0.0746170409298
-0.387610673648 0.0745734709271
-0.387503962001 0.0745298744219
-0.387397137179 0.0744862514097
-0.387290199087 0.074442601886
-0.387183147632 0.0743989258463
-0.387075982719 0.0743552232861
-0.386968704255 0.0743114942009
-0.386861312145 0.0742677385863
-0.386753806295 0.0742239564377
-0.386646186609 0.0741801477507
-0.386538452992 0.0741363125208
-0.38643060535 0.0740924507435
-0.386322643586 0.0740485624144
-0.386214567605 0.074004647529
-0.386106377311 0.0739607060828
-0.385998072608 0.0739167380713
-0.3858896534 0.0738727434901
-0.38578111959 0.0738287223347
-0.385672471081 0.0737846746007
-0.385563707776 0.0737406002836
-0.385454829578 0.073696499379
-0.38534583639 0.0736523718823
-0.385236728114 0.0736082177892
-0.385127504653 0.0735640370952
-0.385018165908 0.0735198297959
-0.384908711781 0.0734755958867
-0.384799142173 0.0734313353634
-0.384689456986 0.0733870482213
-0.384579656122 0.0733427344562
-0.38446973948 0.0732983940636
-0.384359706962 0.073254027039
-0.384249558468 0.0732096333779
-0.384139293898 0.0731652130761
-0.384028913153 0.0731207661291
-0.383918416132 0.0730762925323
-0.383807802734 0.0730317922815
-0.383697072859 0.0729872653722
-0.383586226407 0.0729427118
-0.383475263275 0.0728981315605
-0.383364183363 0.0728535246493
-0.38325298657 0.0728088910619
-0.383141672793 0.0727642307939
-0.38303024193 0.072719543841
-0.38291869388 0.0726748301988
-0.382807028539 0.0726300898628
-0.382695245805 0.0725853228287
-0.382583345576 0.0725405290921
-0.382471327748 0.0724957086486
-0.382359192217 0.0724508614937
-0.382246938881 0.0724059876231
-0.382134567634 0.0723610870325
-0.382022078375 0.0723161597174
-0.381909470997 0.0722712056735
-0.381796745396 0.0722262248963
-0.381683901469 0.0721812173816
-0.381570939109 0.0721361831249
-0.381457858211 0.0720911221219
-0.381344658671 0.0720460343682
-0.381231340382 0.0720009198594
-0.381117903238 0.0719557785912
-0.381004347134 0.0719106105592
-0.380890671963 0.0718654157591
-0.380776877618 0.0718201941865
-0.380662963993 0.0717749458371
-0.380548930979 0.0717296707064
-0.380434778471 0.0716843687902
-0.38032050636 0.0716390400841
-0.380206114538 0.0715936845838
-0.380091602898 0.0715483022848
-0.379976971331 0.071502893183
-0.379862219729 0.0714574572739
-0.379747347982 0.0714119945533
-0.379632355981 0.0713665050167
-0.379517243618 0.0713209886598
-0.379402010783 0.0712754454784
-0.379286657366 0.0712298754681
-0.379171183257 0.0711842786246
-0.379055588345 0.0711386549435
-0.37893987252 0.0710930044205
-0.378824035672 0.0710473270514
-0.378708077689 0.0710016228318
-0.378591998459 0.0709558917574
-0.378475797872 0.0709101338238
-0.378359475816 0.0708643490269
-0.378243032178 0.0708185373622
-0.378126466846 0.0707726988255
-0.378009779707 0.0707268334125
-0.37789297065 0.0706809411189
-0.37777603956 0.0706350219403
-0.377658986324 0.0705890758725
-0.377541810829 0.0705431029113
-0.377424512961 0.0704971030522
-0.377307092605 0.0704510762911
-0.377189549647 0.0704050226236
-0.377071883974 0.0703589420455
-0.376954095468 0.0703128345525
-0.376836184017 0.0702667001403
-0.376718149503 0.0702205388046
-0.376599991812 0.0701743505411
-0.376481710827 0.0701281353457
-0.376363306433 0.070081893214
-0.376244778512 0.0700356241418
-0.376126126947 0.0699893281247
-0.376007351623 0.0699430051586
-0.375888452421 0.0698966552392
-0.375769429224 0.0698502783621
-0.375650281914 0.0698038745233
-0.375531010373 0.0697574437184
-0.375411614482 0.0697109859431
-0.375292094123 0.0696645011933
-0.375172449177 0.0696179894647
-0.375052679525 0.0695714507529
-0.374932785046 0.0695248850539
-0.374812765622 0.0694782923634
-0.374692621133 0.069431672677
-0.374572351457 0.0693850259907
-0.374451956474 0.0693383523001
-0.374331436064 0.0692916516011
-0.374210790105 0.0692449238893
-0.374090018476 0.0691981691607
-0.373969121054 0.0691513874109
-0.373848097719 0.0691045786357
-0.373726948347 0.069057742831
-0.373605672816 0.0690108799924
-0.373484271003 0.0689639901159
-0.373362742785 0.0689170731972
-0.373241088039 0.068870129232
-0.37311930664 0.0688231582162
-0.372997398465 0.0687761601456
-0.372875363389 0.0687291350159
-0.372753201288 0.0686820828231
-0.372630912036 0.0686350035628
-0.372508495509 0.0685878972308
-0.372385951581 0.0685407638231
-0.372263280126 0.0684936033354
-0.372140481018 0.0684464157634
-0.37201755413 0.0683992011031
-0.371894499337 0.0683519593503
-0.37177131651 0.0683046905006
-0.371648005523 0.0682573945501
-0.371524566248 0.0682100714945
-0.371400998557 0.0681627213296
-0.371277302322 0.0681153440513
-0.371153477414 0.0680679396554
-0.371029523705 0.0680205081377
-0.370905441065 0.067973049494
-0.370781229365 0.0679255637202
-0.370656888475 0.0678780508122
-0.370532418266 0.0678305107658
-0.370407818606 0.0677829435768
-0.370283089365 0.067735349241
-0.370158230412 0.0676877277544
-0.370033241616 0.0676400791127
-0.369908122845 0.0675924033118
-0.369782873967 0.0675447003477
-0.369657494851 0.067496970216
-0.369531985362 0.0674492129128
-0.369406345369 0.0674014284338
-0.369280574739 0.0673536167749
-0.369154673337 0.067305777932
-0.36902864103 0.0672579119009
-0.368902477684 0.0672100186776
-0.368776183165 0.0671620982579
-0.368649757337 0.0671141506376
-0.368523200065 0.0670661758127
-0.368396511214 0.0670181737791
-0.368269690648 0.0669701445325
-0.368142738231 0.0669220880689
-0.368015653826 0.0668740043843
-0.367888437297 0.0668258934744
-0.367761088507 0.0667777553351
-0.367633607318 0.0667295899624
-0.367505993592 0.0666813973522
-0.367378247192 0.0666331775003
-0.367250367978 0.0665849304026
-0.367122355812 0.0665366560551
-0.366994210555 0.0664883544537
-0.366865932068 0.0664400255942
-0.36673752021 0.0663916694726
-0.366608974842 0.0663432860848
-0.366480295823 0.0662948754267
-0.366351483012 0.0662464374941
-0.366222536268 0.0661979722831
-0.366093455449 0.0661494797896
-0.365964240414 0.0661009600094
-0.36583489102 0.0660524129385
-0.365705407125 0.0660038385728
-0.365575788586 0.0659552369083
-0.36544603526 0.0659066079409
-0.365316147002 0.0658579516664
-0.36518612367 0.065809268081
-0.365055965118 0.0657605571804
-0.364925671202 0.0657118189606
-0.364795241777 0.0656630534176
-0.364664676698 0.0656142605473
-0.364533975818 0.0655654403456
-0.364403138992 0.0655165928086
-0.364272166074 0.0654677179321
-0.364141056915 0.0654188157121
-0.36400981137 0.0653698861446
-0.363878429291 0.0653209292255
-0.363746910528 0.0652719449508
-0.363615254936 0.0652229333164
-0.363483462363 0.0651738943183
-0.363351532663 0.0651248279525
-0.363219465684 0.0650757342149
-0.363087261278 0.0650266131016
-0.362954919294 0.0649774646084
-0.362822439581 0.0649282887314
-0.36268982199 0.0648790854665
-0.362557066367 0.0648298548097
-0.362424172562 0.064780596757
-0.362291140423 0.0647313113044
-0.362157969797 0.0646819984479
-0.362024660532 0.0646326581834
-0.361891212474 0.064583290507
-0.361757625469 0.0645338954146
-0.361623899363 0.0644844729022
-0.361490034003 0.0644350229658
-0.361356029234 0.0643855456015
-0.361221884899 0.0643360408051
-0.361087600845 0.0642865085728
-0.360953176914 0.0642369489006
-0.360818612951 0.0641873617844
-0.360683908798 0.0641377472202
-0.360549064299 0.0640881052041
-0.360414079296 0.064038435732
-0.360278953631 0.0639887388001
-0.360143687147 0.0639390144042
-0.360008279683 0.0638892625405
-0.359872731081 0.063839483205
-0.359737041181 0.0637896763936
-0.359601209824 0.0637398421024
-0.359465236849 0.0636899803274
-0.359329122096 0.0636400910647
-0.359192865403 0.0635901743104
-0.359056466608 0.0635402300603
-0.358919925549 0.0634902583106
-0.358783242065 0.0634402590573
-0.358646415993 0.0633902322965
-0.358509447168 0.0633401780242
-0.358372335427 0.0632900962364
-0.358235080607 0.0632399869292
-0.358097682543 0.0631898500986
-0.357960141069 0.0631396857407
-0.357822456021 0.0630894938516
-0.357684627232 0.0630392744273
-0.357546654537 0.0629890274639
-0.357408537769 0.0629387529573
-0.35727027676 0.0628884509038
-0.357131871343 0.0628381212993
-0.356993321351 0.06278776414
-0.356854626614 0.0627373794218
-0.356715786964 0.0626869671409
-0.356576802232 0.0626365272933
-0.356437672248 0.0625860598752
-0.356298396841 0.0625355648826
-0.356158975842 0.0624850423115
-0.356019409079 0.0624344921581
-0.35587969638 0.0623839144184
-0.355739837575 0.0623333090885
-0.355599832489 0.0622826761646
-0.355459680951 0.0622320156427
-0.355319382787 0.0621813275189
-0.355178937824 0.0621306117893
-0.355038345886 0.06207986845
-0.354897606801 0.062029097497
-0.354756720391 0.0619782989266
-0.354615686483 0.0619274727348
-0.354474504899 0.0618766189177
-0.354333175463 0.0618257374714
-0.354191697999 0.061774828392
-0.354050072328 0.0617238916757
-0.353908298273 0.0616729273185
-0.353766375656 0.0616219353166
-0.353624304297 0.061570915666
-0.353482084018 0.061519868363
-0.353339714638 0.0614687934037
-0.353197195977 0.0614176907841
-0.353054527854 0.0613665605003
-0.352911710088 0.0613154025486
-0.352768742498 0.061264216925
-0.352625624901 0.0612130036258
-0.352482357114 0.0611617626469
-0.352338938955 0.0611104939846
-0.352195370238 0.061059197635
-0.352051650781 0.0610078735942
-0.351907780399 0.0609565218584
-0.351763758906 0.0609051424237
-0.351619586117 0.0608537352863
-0.351475261845 0.0608023004423
-0.351330785904 0.060750837888
-0.351186158107 0.0606993476193
-0.351041378266 0.0606478296325
-0.350896446192 0.0605962839238
-0.350751361698 0.0605447104893
-0.350606124593 0.0604931093252
-0.350460734688 0.0604414804276
-0.350315191794 0.0603898237927
-0.350169495718 0.0603381394167
-0.35002364627 0.0602864272957
-0.349877643258 0.060234687426
-0.34973148649 0.0601829198037
-0.349585175773 0.0601311244249
-0.349438710913 0.0600793012859
-0.349292091717 0.0600274503828
-0.349145317989 0.0599755717119
-0.348998389536 0.0599236652692
-0.348851306162 0.0598717310511
-0.34870406767 0.0598197690536
-0.348556673864 0.059767779273
-0.348409124547 0.0597157617055
-0.348261419522 0.0596637163473
-0.348113558589 0.0596116431945
-0.347965541551 0.0595595422434
-0.347817368207 0.0595074134901
-0.347669038359 0.059455256931
-0.347520551806 0.0594030725621
-0.347371908346 0.0593508603797
-0.347223107779 0.05929862038
-0.347074149902 0.0592463525593
-0.346925034512 0.0591940569136
-0.346775761407 0.0591417334394
-0.346626330383 0.0590893821327
-0.346476741234 0.0590370029897
-0.346326993758 0.0589845960068
-0.346177087747 0.0589321611802
-0.346027022996 0.058879698506
-0.345876799298 0.0588272079805
-0.345726416447 0.0587746895999
-0.345575874234 0.0587221433605
-0.34542517245 0.0586695692585
-0.345274310888 0.0586169672901
-0.345123289338 0.0585643374516
-0.344972107588 0.0585116797392
-0.34482076543 0.0584589941492
-0.34466926265 0.0584062806778
-0.344517599038 0.0583535393213
-0.344365774382 0.0583007700758
-0.344213788467 0.0582479729377
-0.34406164108 0.0581951479033
-0.343909332007 0.0581422949687
-0.343756861033 0.0580894141302
-0.343604227942 0.0580365053842
-0.343451432519 0.0579835687268
-0.343298474546 0.0579306041543
-0.343145353806 0.057877611663
-0.342992070081 0.0578245912491
-0.342838623153 0.057771542909
-0.342685012803 0.0577184666388
-0.342531238809 0.057665362435
-0.342377300953 0.0576122302937
-0.342223199012 0.0575590702112
-0.342068932766 0.0575058821838
-0.341914501991 0.0574526662079
-0.341759906465 0.0573994222796
-0.341605145964 0.0573461503953
-0.341450220263 0.0572928505512
-0.341295129138 0.0572395227437
-0.341139872364 0.057186166969
-0.340984449713 0.0571327832234
-0.340828860958 0.0570793715033
-0.340673105873 0.0570259318049
-0.340517184229 0.0569724641246
-0.340361095798 0.0569189684586
-0.340204840348 0.0568654448032
-0.340048417651 0.0568118931548
-0.339891827476 0.0567583135096
-0.33973506959 0.0567047058641
-0.339578143762 0.0566510702144
-0.339421049758 0.0565974065569
-0.339263787346 0.0565437148879
-0.33910635629 0.0564899952038
-0.338948756356 0.0564362475008
-0.338790987308 0.0563824717753
-0.338633048909 0.0563286680236
-0.338474940923 0.0562748362421
-0.338316663112 0.056220976427
-0.338158215238 0.0561670885747
-0.33799959706 0.0561131726816
-0.33784080834 0.0560592287439
-0.337681848837 0.0560052567581
-0.337522718309 0.0559512567203
-0.337363416515 0.0558972286271
-0.337203943211 0.0558431724747
-0.337044298154 0.0557890882595
-0.336884481101 0.0557349759778
-0.336724491806 0.055680835626
-0.336564330023 0.0556266672004
-0.336403995507 0.0555724706975
-0.336243488009 0.0555182461134
-0.336082807283 0.0554639934446
-0.33592195308 0.0554097126876
-0.33576092515 0.0553554038385
-0.335599723243 0.0553010668938
-0.335438347108 0.0552467018498
-0.335276796495 0.055192308703
-0.33511507115 0.0551378874497
-0.33495317082 0.0550834380862
-0.334791095253 0.0550289606089
-0.334628844192 0.0549744550143
-0.334466417382 0.0549199212987
-0.334303814568 0.0548653594584
-0.334141035493 0.0548107694899
-0.333978079898 0.0547561513895
-0.333814947525 0.0547015051536
-0.333651638115 0.0546468307786
-0.333488151408 0.054592128261
-0.333324487143 0.054537397597
-0.333160645058 0.0544826387831
-0.332996624891 0.0544278518157
-0.332832426379 0.0543730366912
-0.332668049257 0.0543181934059
-0.33250349326 0.0542633219563
-0.332338758124 0.0542084223388
-0.33217384358 0.0541534945498
-0.332008749363 0.0540985385857
-0.331843475203 0.0540435544429
-0.331678020833 0.0539885421178
-0.331512385981 0.0539335016069
-0.331346570377 0.0538784329065
-0.331180573751 0.0538233360131
-0.331014395829 0.053768210923
-0.330848036338 0.0537130576328
-0.330681495004 0.0536578761388
-0.330514771553 0.0536026664374
-0.330347865708 0.0535474285252
-0.330180777194 0.0534921623984
-0.330013505732 0.0534368680536
-0.329846051044 0.0533815454872
-0.329678412852 0.0533261946956
-0.329510590874 0.0532708156753
-0.32934258483 0.0532154084226
-0.329174394439 0.0531599729341
-0.329006019417 0.0531045092061
-0.328837459481 0.0530490172352
-0.328668714347 0.0529934970177
-0.328499783728 0.0529379485502
-0.328330667339 0.052882371829
-0.328161364892 0.0528267668507
-0.3279918761 0.0527711336116
-0.327822200673 0.0527154721083
-0.327652338322 0.0526597823371
-0.327482288755 0.0526040642947
-0.32731205168 0.0525483179773
-0.327141626806 0.0524925433815
-0.326971013838 0.0524367405038
-0.326800212481 0.0523809093406
-0.326629222441 0.0523250498884
-0.326458043421 0.0522691621436
-0.326286675123 0.0522132461028
-0.326115117248 0.0521573017624
-0.325943369499 0.0521013291189
-0.325771431573 0.0520453281687
-0.32559930317 0.0519892989084
-0.325426983989 0.0519332413345
-0.325254473724 0.0518771554434
-0.325081772073 0.0518210412316
-0.32490887873 0.0517648986956
-0.324735793389 0.0517087278319
-0.324562515743 0.0516525286369
-0.324389045483 0.0515963011073
-0.324215382301 0.0515400452395
-0.324041525885 0.0514837610299
-0.323867475926 0.0514274484752
-0.323693232111 0.0513711075717
-0.323518794126 0.051314738316
-0.323344161658 0.0512583407046
-0.323169334391 0.0512019147341
-0.322994312008 0.0511454604009
-0.322819094193 0.0510889777015
-0.322643680627 0.0510324666324
-0.32246807099 0.0509759271903
-0.322292264963 0.0509193593715
-0.322116262223 0.0508627631726
-0.321940062447 0.0508061385902
-0.321763665313 0.0507494856207
-0.321587070496 0.0506928042607
-0.321410277669 0.0506360945068
-0.321233286505 0.0505793563554
-0.321056096677 0.050522589803
-0.320878707856 0.0504657948463
-0.320701119711 0.0504089714817
-0.320523331911 0.0503521197059
-0.320345344123 0.0502952395152
-0.320167156015 0.0502383309063
-0.319988767251 0.0501813938758
-0.319810177495 0.0501244284201
-0.319631386411 0.0500674345358
-0.319452393661 0.0500104122194
-0.319273198906 0.0499533614676
-0.319093801804 0.0498962822769
-0.318914202015 0.0498391746438
-0.318734399197 0.0497820385648
-0.318554393004 0.0497248740366
-0.318374183093 0.0496676810557
-0.318193769117 0.0496104596187
-0.318013150729 0.0495532097221
-0.317832327581 0.0494959313625
-0.317651299322 0.0494386245364
-0.317470065601 0.0493812892405
-0.317288626068 0.0493239254713
-0.317106980368 0.0492665332254
-0.316925128147 0.0492091124993
-0.31674306905 0.0491516632897
-0.316560802718 0.0490941855931
-0.316378328795 0.0490366794061
-0.316195646921 0.0489791447253
-0.316012756735 0.0489215815473
-0.315829657875 0.0488639898686
-0.315646349978 0.0488063696859
-0.315462832679 0.0487487209958
-0.315279105614 0.0486910437947
-0.315095168415 0.0486333380794
-0.314911020714 0.0485756038464
-0.314726662141 0.0485178410924
-0.314542092326 0.0484600498139
-0.314357310897 0.0484022300075
-0.314172317479 0.0483443816699
-0.313987111699 0.0482865047976
-0.313801693181 0.0482285993872
-0.313616061546 0.0481706654355
-0.313430216417 0.0481127029389
-0.313244157414 0.0480547118941
-0.313057884154 0.0479966922977
-0.312871396257 0.0479386441463
-0.312684693336 0.0478805674366
-0.312497775007 0.0478224621652
-0.312310640884 0.0477643283286
-0.312123290578 0.0477061659236
-0.311935723699 0.0476479749467
-0.311747939857 0.0475897553946
-0.31155993866 0.0475315072639
-0.311371719713 0.0474732305512
-0.311183282621 0.0474149252532
-0.310994626989 0.0473565913665
-0.310805752418 0.0472982288878
-0.310616658508 0.0472398378137
-0.310427344859 0.0471814181408
-0.310237811069 0.0471229698658
-0.310048056733 0.0470644929853
-0.309858081448 0.047005987496
-0.309667884805 0.0469474533945
-0.309477466397 0.0468888906775
-0.309286825815 0.0468302993416
-0.309095962646 0.0467716793835
-0.30890487648 0.0467130307999
-0.3087135669 0.0466543535874
-0.308522033493 0.0465956477426
-0.308330275841 0.0465369132622
-0.308138293525 0.046478150143
-0.307946086124 0.0464193583815
-0.307753653218 0.0463605379744
-0.307560994383 0.0463016889184
-0.307368109194 0.0462428112102
-0.307174997225 0.0461839048465
-0.306981658047 0.0461249698238
-0.306788091232 0.046066006139
-0.306594296348 0.0460070137886
-0.306400272962 0.0459479927694
-0.30620602064 0.0458889430781
-0.306011538946 0.0458298647113
-0.305816827442 0.0457707576657
-0.305621885689 0.045711621938
-0.305426713246 0.0456524575249
-0.305231309672 0.045593264423
-0.30503567452 0.0455340426292
-0.304839807347 0.0454747921401
-0.304643707703 0.0454155129523
-0.30444737514 0.0453562050626
-0.304250809208 0.0452968684677
-0.304054009452 0.0452375031643
-0.30385697542 0.045178109149
-0.303659706655 0.0451186864187
-0.303462202699 0.04505923497
-0.303264463093 0.0449997547995
-0.303066487375 0.0449402459042
-0.302868275083 0.0448807082805
-0.302669825752 0.0448211419254
-0.302471138915 0.0447615468354
-0.302272214103 0.0447019230073
-0.302073050847 0.0446422704378
-0.301873648675 0.0445825891237
-0.301674007113 0.0445228790616
-0.301474125685 0.0444631402484
-0.301274003914 0.0444033726807
-0.30107364132 0.0443435763552
-0.300873037424 0.0442837512687
-0.300672191741 0.044223897418
-0.300471103786 0.0441640147997
-0.300269773074 0.0441041034107
-0.300068199114 0.0440441632476
-0.299866381418 0.0439841943071
-0.299664319492 0.0439241965861
-0.299462012842 0.0438641700813
-0.299259460972 0.0438041147894
-0.299056663383 0.0437440307072
-0.298853619575 0.0436839178314
-0.298650329046 0.0436237761587
-0.298446791292 0.043563605686
-0.298243005806 0.04350340641
-0.298038972081 0.0434431783275
-0.297834689606 0.0433829214351
-0.29763015787 0.0433226357298
-0.297425376357 0.0432623212081
-0.297220344552 0.043201977867
-0.297015061936 0.0431416057031
-0.296809527989 0.0430812047133
-0.296603742188 0.0430207748942
-0.296397704009 0.0429603162428
-0.296191412925 0.0428998287557
-0.295984868408 0.0428393124298
-0.295778069925 0.0427787672617
-0.295571016946 0.0427181932484
-0.295363708933 0.0426575903865
-0.29515614535 0.0425969586728
-0.294948325657 0.0425362981043
-0.294740249312 0.0424756086775
-0.294531915772 0.0424148903894
-0.294323324491 0.0423541432367
-0.294114474919 0.0422933672161
-0.293905366506 0.0422325623246
-0.2936959987 0.0421717285589
-0.293486370945 0.0421108659157
-0.293276482684 0.042049974392
-0.293066333358 0.0419890539845
-0.292855922403 0.0419281046899
-0.292645249256 0.0418671265051
-0.29243431335 0.041806119427
-0.292223114117 0.0417450834523
-0.292011650984 0.0416840185778
-0.291799923379 0.0416229248003
-0.291587930724 0.0415618021167
-0.291375672442 0.0415006505238
-0.291163147951 0.0414394700184
-0.290950356668 0.0413782605972
-0.290737298008 0.0413170222572
-0.290523971382 0.0412557549952
-0.290310376199 0.0411944588079
-0.290096511866 0.0411331336923
-0.289882377788 0.041071779645
-0.289667973366 0.0410103966631
-0.289453298 0.0409489847432
-0.289238351085 0.0408875438823
-0.289023132017 0.0408260740771
-0.288807640187 0.0407645753245
-0.288591874984 0.0407030476214
-0.288375835795 0.0406414909645
-0.288159522002 0.0405799053508
-0.287942932987 0.0405182907771
-0.287726068129 0.0404566472401
-0.287508926804 0.0403949747368
-0.287291508384 0.0403332732641
-0.28707381224 0.0402715428187
-0.28685583774 0.0402097833975
-0.286637584248 0.0401479949974
-0.286419051128 0.0400861776152
-0.286200237737 0.0400243312479
-0.285981143434 0.0399624558921
-0.285761767571 0.0399005515449
-0.285542109501 0.039838618203
-0.28532216857 0.0397766558634
-0.285101944125 0.0397146645229
-0.284881435508 0.0396526441784
-0.284660642059 0.0395905948267
-0.284439563114 0.0395285164648
-0.284218198007 0.0394664090894
-0.283996546069 0.0394042726975
-0.283774606628 0.039342107286
-0.283552379008 0.0392799128517
-0.283329862533 0.0392176893914
-0.283107056519 0.0391554369022
-0.282883960284 0.0390931553809
-0.282660573141 0.0390308448243
-0.282436894398 0.0389685052294
-0.282212923363 0.038906136593
-0.281988659339 0.0388437389121
-0.281764101626 0.0387813121835
-0.281539249522 0.0387188564041
-0.281314102321 0.0386563715708
-0.281088659314 0.0385938576806
-0.280862919789 0.0385313147302
-0.280636883029 0.0384687427167
-0.280410548316 0.038406141637
-0.280183914928 0.0383435114878
-0.27995698214 0.0382808522662
-0.279729749223 0.038218163969
-0.279502215445 0.0381554465932
-0.279274380071 0.0380927001357
-0.279046242362 0.0380299245934
-0.278817801575 0.0379671199631
-0.278589056966 0.0379042862419
-0.278360007784 0.0378414234266
-0.278130653279 0.0377785315142
-0.277900992693 0.0377156105016
-0.277671025267 0.0376526603857
-0.277440750239 0.0375896811634
-0.277210166842 0.0375266728317
-0.276979274305 0.0374636353875
-0.276748071855 0.0374005688277
-0.276516558714 0.0373374731493
-0.276284734101 0.0372743483491
-0.276052597233 0.0372111944242
-0.27582014732 0.0371480113715
-0.275587383569 0.0370847991879
-0.275354305186 0.0370215578703
-0.275120911371 0.0369582874157
-0.27488720132 0.0368949878211
-0.274653174226 0.0368316590834
-0.274418829277 0.0367683011995
-0.27418416566 0.0367049141664
-0.273949182554 0.036641497981
-0.273713879137 0.0365780526404
-0.273478254582 0.0365145781414
-0.273242308059 0.036451074481
-0.273006038732 0.0363875416561
-0.272769445763 0.0363239796638
-0.272532528309 0.036260388501
-0.272295285523 0.0361967681647
-0.272057716554 0.0361331186518
-0.271819820546 0.0360694399592
-0.27158159664 0.0360057320841
-0.271343043973 0.0359419950232
-0.271104161677 0.0358782287737
-0.270864948879 0.0358144333324
-0.270625404704 0.0357506086964
-0.27038552827 0.0356867548627
-0.270145318692 0.0356228718281
-0.269904775081 0.0355589595898
-0.269663896543 0.0354950181446
-0.269422682179 0.0354310474896
-0.269181131087 0.0353670476217
-0.26893924236 0.035303018538
-0.268697015086 0.0352389602354
-0.268454448347 0.0351748727109
-0.268211541224 0.0351107559616
-0.267968292791 0.0350466099843
-0.267724702116 0.0349824347762
-0.267480768266 0.0349182303341
-0.267236490301 0.0348539966552
-0.266991867275 0.0347897337364
-0.26674689824 0.0347254415746
-0.266501582242 0.034661120167
-0.266255918321 0.0345967695105
-0.266009905513 0.0345323896022
-0.26576354285 0.0344679804389
-0.265516829358 0.0344035420179
-0.265269764058 0.034339074336
-0.265022345966 0.0342745773902
-0.264774574093 0.0342100511777
-0.264526447444 0.0341454956954
-0.264277965022 0.0340809109403
-0.26402912582 0.0340162969095
-0.26377992883 0.0339516536
-0.263530373036 0.0338869810087
-0.263280457419 0.0338222791329
-0.263030180952 0.0337575479693
-0.262779542604 0.0336927875152
-0.262528541339 0.0336279977675
-0.262277176116 0.0335631787232
-0.262025445886 0.0334983303795
-0.261773349596 0.0334334527333
-0.261520886189 0.0333685457816
-0.261268054599 0.0333036095216
-0.261014853757 0.0332386439502
-0.260761282587 0.0331736490645
-0.260507340008 0.0331086248615
-0.260253024933 0.0330435713384
-0.259998336268 0.0329784884921
-0.259743272914 0.0329133763196
-0.259487833767 0.0328482348181
-0.259232017716 0.0327830639847
-0.258975823644 0.0327178638162
-0.258719250428 0.0326526343099
-0.258462296938 0.0325873754627
-0.25820496204 0.0325220872718
-0.257947244592 0.0324567697341
-0.257689143446 0.0323914228468
-0.257430657448 0.0323260466069
-0.257171785437 0.0322606410115
-0.256912526247 0.0321952060577
-0.256652878705 0.0321297417425
-0.25639284163 0.032064248063
-0.256132413837 0.0319987250162
-0.255871594131 0.0319331725993
-0.255610381314 0.0318675908093
-0.255348774179 0.0318019796434
-0.255086771512 0.0317363390985
-0.254824372095 0.0316706691717
-0.254561574699 0.0316049698602
-0.254298378092 0.0315392411611
-0.254034781031 0.0314734830713
-0.25377078227 0.0314076955881
-0.253506380553 0.0313418787085
-0.253241574619 0.0312760324295
-0.252976363197 0.0312101567484
-0.252710745012 0.0311442516621
-0.252444718779 0.0310783171678
-0.252178283206 0.0310123532626
-0.251911436996 0.0309463599435
-0.251644178842 0.0308803372078
-0.251376507429 0.0308142850524
-0.251108421437 0.0307482034744
-0.250839919535 0.0306820924711
-0.250571000388 0.0306159520395
-0.25030166265 0.0305497821767
-0.250031904968 0.0304835828798
-0.249761725982 0.0304173541459
-0.249491124323 0.0303510959722
-0.249220098614 0.0302848083558
-0.248948647471 0.0302184912937
-0.248676769499 0.0301521447831
-0.248404463298 0.0300857688212
-0.248131727458 0.030019363405
-0.24785856056 0.0299529285317
-0.247584961178 0.0298864641984
-0.247310927877 0.0298199704022
-0.247036459211 0.0297534471402
-0.246761553729 0.0296868944097
-0.246486209969 0.0296203122076
-0.24621042646 0.0295537005312
-0.245934201724 0.0294870593777
-0.245657534272 0.029420388744
-0.245380422605 0.0293536886274
-0.245102865219 0.029286959025
-0.244824860596 0.029220199934
-0.244546407212 0.0291534113514
-0.244267503531 0.0290865932745
-0.24398814801 0.0290197457004
-0.243708339094 0.0289528686262
-0.243428075221 0.0288859620491
-0.243147354817 0.0288190259662
-0.242866176299 0.0287520603747
-0.242584538074 0.0286850652718
-0.242302438538 0.0286180406546
-0.24201987608 0.0285509865202
-0.241736849075 0.0284839028659
-0.24145335589 0.0284167896888
-0.241169394881 0.028349646986
-0.240884964394 0.0282824747547
-0.240600062763 0.0282152729921
-0.240314688313 0.0281480416953
-0.240028839358 0.0280807808616
-0.239742514199 0.028013490488
-0.239455711129 0.0279461705719
-0.239168428429 0.0278788211102
-0.238880664369 0.0278114421003
-0.238592417205 0.0277440335392
-0.238303685186 0.0276765954243
-0.238014466547 0.0276091277526
-0.237724759512 0.0275416305213
-0.237434562293 0.0274741037276
-0.23714387309 0.0274065473688
-0.236852690093 0.0273389614419
-0.236561011477 0.0272713459442
-0.236268835407 0.0272037008729
-0.235976160036 0.0271360262252
-0.235682983503 0.0270683219982
-0.235389303935 0.0270005881892
-0.235095119448 0.0269328247953
-0.234800428143 0.0268650318138
-0.234505228111 0.0267972092418
-0.234209517426 0.0267293570766
-0.233913294154 0.0266614753153
-0.233616556342 0.0265935639552
-0.23331930203 0.0265256229935
-0.233021529239 0.0264576524273
-0.232723235981 0.0263896522539
-0.23242442025 0.0263216224706
-0.232125080029 0.0262535630744
-0.231825213286 0.0261854740626
-0.231524817976 0.0261173554325
-0.231223892039 0.0260492071813
-0.230922433399 0.0259810293061
-0.230620439969 0.0259128218043
-0.230317909643 0.0258445846729
-0.230014840305 0.0257763179093
-0.22971122982 0.0257080215107
-0.229407076041 0.0256396954742
-0.229102376802 0.0255713397972
-0.228797129925 0.0255029544769
-0.228491333215 0.0254345395104
-0.228184984461 0.0253660948951
-0.227878081438 0.0252976206281
-0.227570621902 0.0252291167067
-0.227262603595 0.0251605831281
-0.226954024242 0.0250920198896
-0.226644881552 0.0250234269885
-0.226335173215 0.0249548044219
-0.226024896907 0.024886152187
-0.225714050285 0.0248174702813
-0.22540263099 0.0247487587018
-0.225090636646 0.0246800174459
-0.224778064856 0.0246112465107
-0.22446491321 0.0245424458936
-0.224151179277 0.0244736155918
-0.223836860608 0.0244047556026
-0.223521954737 0.0243358659232
-0.223206459178 0.0242669465508
-0.222890371427 0.0241979974828
-0.222573688962 0.0241290187164
-0.22225640924 0.0240600102488
-0.221938529699 0.0239909720774
-0.221620047759 0.0239219041993
-0.221300960819 0.0238528066119
-0.220981266258 0.0237836793124
-0.220660961435 0.0237145222981
-0.220340043689 0.0236453355663
-0.220018510337 0.0235761191142
-0.219696358677 0.0235068729392
-0.219373585985 0.0234375970384
-0.219050189515 0.0233682914092
-0.218726166501 0.0232989560489
-0.218401514154 0.0232295909547
-0.218076229664 0.0231601961239
-0.217750310196 0.0230907715538
-0.217423752897 0.0230213172418
-0.217096554887 0.022951833185
-0.216768713266 0.0228823193807
-0.216440225108 0.0228127758264
-0.216111087465 0.0227432025192
-0.215781297366 0.0226735994564
-0.215450851814 0.0226039666354
-0.215119747789 0.0225343040534
-0.214787982245 0.0224646117077
-0.214455552113 0.0223948895957
-0.214122454296 0.0223251377147
-0.213788685675 0.0222553560618
-0.213454243103 0.0221855446346
-0.213119123405 0.0221157034302
-0.212783323384 0.0220458324459
-0.212446839814 0.0219759316791
-0.21210966944 0.0219060011272
-0.211771808984 0.0218360407873
-0.211433255135 0.0217660506568
-0.21109400456 0.021696030733
-0.210754053892 0.0216259810133
-0.210413399738 0.021555901495
-0.210072038677 0.0214857921754
-0.209729967256 0.0214156530517
-0.209387181994 0.0213454841214
-0.20904367938 0.0212752853817
-0.20869945587 0.0212050568301
-0.208354507893 0.0211347984637
-0.208008831844 0.02106451028
-0.207662424087 0.0209941922762
-0.207315280955 0.0209238444498
-0.206967398746 0.020853466798
-0.206618773728 0.0207830593181
-0.206269402135 0.0207126220076
-0.205919280166 0.0206421548637
-0.205568403987 0.0205716578838
-0.205216769731 0.0205011310652
-0.204864373492 0.0204305744053
-0.204511211333 0.0203599879015
-0.204157279278 0.020289371551
-0.203802573317 0.0202187253512
-0.203447089401 0.0201480492994
-0.203090823445 0.0200773433931
-0.202733771327 0.0200066076296
-0.202375928886 0.0199358420061
-0.202017291921 0.0198650465202
-0.201657856193 0.019794221169
-0.201297617425 0.0197233659501
-0.200936571296 0.0196524808607
-0.200574713447 0.0195815658982
-0.200212039477 0.01951062106
-0.199848544942 0.0194396463435
-0.199484225357 0.0193686417459
-0.199119076193 0.0192976072647
-0.198753092878 0.0192265428972
-0.198386270795 0.0191554486409
-0.198018605283 0.019084324493
-0.197650091635 0.019013170451
-0.197280725098 0.0189419865123
-0.196910500874 0.0188707726741
-0.196539414114 0.0187995289339
-0.196167459923 0.0187282552891
-0.195794633359 0.018656951737
-0.195420929429 0.0185856182751
-0.195046343088 0.0185142549007
-0.194670869244 0.0184428616111
-0.194294502751 0.0183714384039
-0.193917238412 0.0182999852763
-0.193539070976 0.0182285022258
-0.193159995138 0.0181569892497
-0.192780005541 0.0180854463455
-0.19239909677 0.0180138735106
-0.192017263355 0.0179422707422
-0.191634499768 0.0178706380379
-0.191250800426 0.0177989753951
-0.190866159684 0.0177272828111
-0.19048057184 0.0176555602833
-0.19009403113 0.0175838078091
-0.189706531729 0.017512025386
-0.189318067752 0.0174402130113
-0.188928633247 0.0173683706825
-0.188538222201 0.017296498397
-0.188146828535 0.0172245961522
-0.187754446104 0.0171526639454
-0.187361068696 0.0170807017741
-0.186966690029 0.0170087096358
-0.186571303756 0.0169366875278
-0.186174903455 0.0168646354475
-0.185777482637 0.0167925533925
-0.185379034738 0.01672044136
-0.18497955312 0.0166482993475
-0.184579031072 0.0165761273525
-0.184177461806 0.0165039253723
-0.183774838457 0.0164316934045
-0.183371154083 0.0163594314463
-0.182966401659 0.0162871394953
-0.182560574083 0.0162148175489
-0.182153664168 0.0161424656046
-0.181745664644 0.0160700836596
-0.181336568157 0.0159976717116
-0.180926367265 0.0159252297579
-0.18051505444 0.0158527577959
-0.180102622064 0.0157802558232
-0.179689062427 0.015707723837
-0.179274367728 0.015635161835
-0.178858530072 0.0155625698145
-0.178441541469 0.015489947773
-0.17802339383 0.015417295708
-0.17760407897 0.0153446136168
-0.177183588601 0.0152719014969
-0.176761914334 0.0151991593458
-0.176339047677 0.0151263871609
-0.17591498003 0.0150535849397
-0.175489702687 0.0149807526797
-0.175063206833 0.0149078903783
-0.174635483538 0.0148349980329
-0.174206523763 0.0147620756411
-0.17377631835 0.0146891232002
-0.173344858026 0.0146161407078
-0.172912133396 0.0145431281613
-0.172478134945 0.0144700855581
-0.172042853032 0.0143970128958
-0.171606277891 0.0143239101719
-0.171168399626 0.0142507773837
-0.170729208212 0.0141776145288
-0.170288693487 0.0141044216046
-0.169846845155 0.0140311986086
-0.169403652781 0.0139579455383
-0.168959105789 0.0138846623912
-0.168513193458 0.0138113491647
-0.16806590492 0.0137380058564
-0.167617229158 0.0136646324636
-0.167167155003 0.013591228984
-0.166715671128 0.0135177954149
-0.166262766049 0.0134443317539
-0.165808428121 0.0133708379984
-0.165352645532 0.013297314146
-0.164895406303 0.0132237601941
-0.164436698282 0.0131501761402
-0.163976509144 0.0130765619819
-0.163514826383 0.0130029177166
-0.163051637311 0.0129292433417
-0.162586929055 0.0128555388549
-0.162120688551 0.0127818042536
-0.16165290254 0.0127080395353
-0.161183557567 0.0126342446976
-0.160712639974 0.0125604197378
-0.160240135894 0.0124865646536
-0.159766031253 0.0124126794424
-0.159290311759 0.0123387641017
-0.1588129629 0.0122648186291
-0.158333969939 0.0121908430221
-0.15785331791 0.0121168372781
-0.157370991611 0.0120428013947
-0.1568869756 0.0119687353694
-0.156401254189 0.0118946391998
-0.155913811441 0.0118205128832
-0.155424631159 0.0117463564174
-0.154933696886 0.0116721697997
-0.154440991895 0.0115979530277
-0.153946499184 0.0115237060989
-0.15345020147 0.0114494290109
-0.152952081184 0.0113751217612
-0.15245212046 0.0113007843473
-0.151950301131 0.0112264167667
-0.151446604722 0.011152019017
-0.15094101244 0.0110775910957
-0.150433505171 0.0110031330003
-0.149924063468 0.0109286447284
-0.149412667542 0.0108541262775
-0.14889929726 0.0107795776452
-0.148383932127 0.0107049988289
-0.147866551287 0.0106303898263
-0.147347133506 0.0105557506349
-0.146825657166 0.0104810812521
-0.146302100255 0.0104063816756
-0.145776440355 0.010331651903
-0.145248654634 0.0102568919316
-0.144718719834 0.0101821017592
-0.144186612258 0.0101072813833
-0.143652307763 0.0100324308013
-0.143115781742 0.00995755001092
-0.142577009116 0.00988263900965
-0.142035964319 0.00980769779506
-0.141492621287 0.00973272636469
-0.14094695344 0.00965772471612
-0.140398933673 0.00958269284691
-0.139848534335 0.00950763075461
-0.13929572722 0.00943253843679
-0.138740483546 0.00935741589101
-0.138182773943 0.00928226311485
-0.13762256843 0.00920708010586
-0.137059836403 0.00913186686163
-0.136494546614 0.00905662337971
-0.135926667151 0.00898134965769
-0.135356165419 0.00890604569313
-0.13478300812 0.00883071148361
-0.134207161232 0.00875534702671
-0.133628589983 0.00867995232001
-0.133047258831 0.00860452736107
-0.132463131441 0.0085290721475
-0.131876170655 0.00845358667686
-0.131286338471 0.00837807094674
-0.130693596011 0.00830252495472
-0.130097903497 0.00822694869839
-0.129499220219 0.00815134217535
-0.128897504504 0.00807570538317
-0.128292713682 0.00800003831945
-0.127684804059 0.00792434098177
-0.127073730874 0.00784861336774
-0.126459448265 0.00777285547495
-0.125841909235 0.00769706730099
-0.125221065604 0.00762124884346
-0.124596867974 0.00754540009996
-0.123969265682 0.00746952106809
-0.123338206755 0.00739361174545
-0.122703637861 0.00731767212965
-0.122065504258 0.00724170221828
-0.121423749745 0.00716570200895
-0.120778316603 0.00708967149928
-0.120129145538 0.00701361068686
-0.119476175619 0.00693751956931
-0.118819344219 0.00686139814424
-0.118158586939 0.00678524640926
-0.117493837545 0.00670906436199
-0.11682502789 0.00663285200004
-0.116152087837 0.00655660932103
-0.115474945175 0.00648033632257
-0.114793525533 0.00640403300229
-0.114107752289 0.00632769935781
-0.11341754647 0.00625133538674
-0.112722826655 0.00617494108672
-0.112023508862 0.00609851645536
-0.111319506437 0.00602206149029
-0.110610729931 0.00594557618915
-0.109897086973 0.00586906054955
-0.109178482135 0.00579251456914
-0.108454816787 0.00571593824553
-0.107725988946 0.00563933157637
-0.10699189311 0.00556269455929
-0.106252420089 0.00548602719193
-0.105507456824 0.00540932947191
-0.104756886184 0.00533260139689
-0.104000586764 0.0052558429645
-0.103238432662 0.00517905417238
-0.102470293239 0.00510223501818
-0.10169603287 0.00502538549954
-0.100915510668 0.0049485056141
-0.100128580196 0.00487159535951
-0.0993350891559 0.00479465473342
-0.0985348790534 0.00471768373348
-0.0977277848384 0.00464068235733
-0.0969136345188 0.00456365060265
-0.0960922487443 0.00448658846706
-0.0952634403573 0.00440949594824
-0.0944270139079 0.00433237304383
-0.0935827651296 0.0042552197515
-0.0927304803714 0.0041780360689
-0.0918699359823 0.00410082199369
-0.0910008976426 0.00402357752354
-0.0901231196364 0.00394630265611
-0.0892363440595 0.00386899738906
-0.0883402999548 0.00379166172006
-0.0874347023668 0.00371429564678
-0.086519251307 0.00363689916688
-0.0855936306179 0.00355947227803
-0.0846575067247 0.00348201497791
-0.0837105272605 0.00340452726419
-0.0827523195475 0.00332700913454
-0.081782488918 0.00324946058663
-0.0808006168518 0.00317188161815
-0.0798062589056 0.00309427222677
-0.0787989424058 0.00301663241017
-0.0777781638696 0.00293896216604
-0.0767433861153 0.00286126149204
-0.0756940350149 0.00278353038587
-0.0746294958318 0.00270576884521
-0.0735491090786 0.00262797686775
-0.072452165815 0.00255015445118
-0.0713379022904 0.00247230159317
-0.0702054938162 0.00239441829143
-0.0690540477281 0.00231650454365
-0.0678825952669 0.00223856034751
-0.0666900821681 0.00216058570071
-0.0654753576995 0.00208258060094
-0.0642371618227 0.00200454504591
-0.0629741100698 0.00192647903332
-0.0616846756173 0.00184838256085
-0.0603671678962 0.00177025562621
-0.0590197068824 0.00169209822711
-0.05764019195 0.00161391036124
-0.0562262638138 0.00153569202631
-0.0547752575874 0.00145744322003
-0.0532841442828 0.0013791639401
-0.0517494570698 0.00130085418424
-0.0501671971407 0.00122251395015
-0.048532711832 0.00114414323555
-0.0468405342995 0.00106574203814
-0.0450841687961 0.00098731035564
-0.0432557971315 0.000908848185769
-0.0413458677718 0.00083035552624
-0.0393425045594 0.000751832374772
-0.0372306276483 0.000673278729085
-0.0349905943368 0.000594694586898
-0.0325959941691 0.000516079945934
-0.0300098494929 0.000437434803916
-0.0271775345492 0.000358759158568
-0.0240120967147 0.000280053007616
-0.0203587396461 0.000201316348789
-0.0158842959616 0.000122549179813


==> figuresAndData/dataForConditionalVarianceCircularMeanZero.tex <==
-0.450442616461 0.0590073193873
-0.449561731229 0.05892590042
-0.448680845996 0.0586060482466
-0.447799960763 0.058520782129
-0.44691907553 0.0584343392036
-0.446038190297 0.0581117702745
-0.445157305064 0.0580236436336
-0.444276419831 0.0579347690681
-0.443395534598 0.0576109158272
-0.442514649365 0.0575209066343
-0.441633764132 0.0574303384114
-0.440752878899 0.0571058008867
-0.439871993666 0.0570143892828
-0.438991108433 0.0569225315914
-0.438110223201 0.0565976690237
-0.437229337968 0.0565051566626
-0.436348452735 0.0564122755598
-0.435467567502 0.0560873361998
-0.434586682269 0.0559939358661
-0.433705797036 0.0559002240555
-0.432824911803 0.0555753938021
-0.43194402657 0.0554812662598
-0.431063141337 0.0551567830968
-0.430182256104 0.0550622973043
-0.429301370871 0.0549675696923
-0.428420485638 0.054643425936
-0.427539600405 0.0545484122656
-0.426658715173 0.0544531884667
-0.42577782994 0.0541294904994
-0.424896944707 0.0540340409752
-0.424016059474 0.0537108860431
-0.423135174241 0.0536152464278
-0.422254289008 0.0535194391298
-0.421373403775 0.0531968753871
-0.420492518542 0.053100924622
-0.419611633309 0.0527789923738
-0.418730748076 0.0526829263319
-0.417849862843 0.0525867258664
-0.41696897761 0.0522655013098
-0.416088092377 0.0521692230084
-0.415207207145 0.0518487024015
-0.414326321912 0.0517523693038
-0.413445436679 0.0516559287175
-0.412564551446 0.0513362122703
-0.411683666213 0.0512397478125
-0.41080278098 0.0511431896421
-0.409921895747 0.0508243273187
-0.409041010514 0.0507277731537
-0.408160125281 0.0504097077145
-0.407279240048 0.0503131750713
-0.406398354815 0.0499959271471
-0.405517469582 0.0498994324947
-0.404636584349 0.0498028716275
-0.403755699117 0.0494865805185
-0.402874813884 0.0493900800425
-0.401993928651 0.0490746524154
-0.401113043418 0.0489782266017
-0.400232158185 0.048881750824
-0.399351272952 0.0485673421651
-0.398470387719 0.0484709605414
-0.397589502486 0.0481574561341
-0.396708617253 0.0480611811848
-0.39582773202 0.0479648704075
-0.394946846787 0.0476524402067
-0.394065961554 0.047556253257
-0.393185076321 0.0472447638685
-0.392304191089 0.0471487118442
-0.391423305856 0.0470526364158
-0.390542420623 0.0467422708274
-0.38966153539 0.0466463455629
-0.388780650157 0.0463369538752
-0.387899764924 0.0462411886977
-0.387018879691 0.0459327837345
-0.386137994458 0.0458371881496
-0.385257109225 0.0457415843165
-0.384376223992 0.0454343654149
-0.383495338759 0.0453389442539
-0.382614453526 0.0450327412089
-0.381733568293 0.0449375113056
-0.380852683061 0.0446323355141
-0.379971797828 0.0445373051232
-0.379090912595 0.0444422794714
-0.378210027362 0.0441383446896
-0.377329142129 0.0440435299211
-0.376448256896 0.0437406483572
-0.375567371663 0.0436460519895
-0.37468648643 0.0433442338833
-0.373805601197 0.0432498631662
-0.372924715964 0.0431555084476
-0.372043830731 0.0428549803928
-0.371162945498 0.0427608613156
-0.370282060265 0.0424614200925
-0.369401175033 0.0423675433047
-0.3685202898 0.0420691981961
-0.367639404567 0.0419755701249
-0.366758519334 0.0418819679092
-0.365877634101 0.0415849570307
-0.364996748868 0.0414916123885
-0.364115863635 0.0411957188425
-0.363234978402 0.0411026377022
-0.362354093169 0.0408078699675
-0.361473207936 0.0407150580731
-0.360592322703 0.040622280734
-0.35971143747 0.0403288873389
-0.358830552237 0.0402363871569
-0.357949667005 0.0399441389694
-0.357068781772 0.0398519212693
-0.356187896539 0.039560826083
-0.355307011306 0.0394688960334
-0.354426126073 0.0391789614615
-0.35354524084 0.0390873240819
-0.352664355607 0.0389957310839
-0.351783470374 0.0387072177321
-0.350902585141 0.0386159243097
-0.350021699908 0.0383285889986
-0.349140814675 0.0382375998305
-0.348259929442 0.0379514496058
-0.347379044209 0.0378607692426
-0.346498158977 0.0377701399636
-0.345617273744 0.0374854438689
-0.344736388511 0.0373951296481
-0.343855503278 0.0371116347689
-0.342974618045 0.0370216398636
-0.342093732812 0.0367393527494
-0.341212847579 0.036649681306
-0.340331962346 0.0363686083732
-0.339451077113 0.0362792644316
-0.33857019188 0.0359994119686
-0.337689306647 0.0359103994662
-0.336808421414 0.0358214473359
-0.335927536181 0.0355430964131
-0.335046650949 0.0354544811207
-0.334165765716 0.0351773650608
-0.333284880483 0.0350890903079
-0.33240399525 0.0348132149904
-0.331523110017 0.0347252843888
-0.330642224784 0.0344506555828
-0.329761339551 0.0343630726578
-0.328880454318 0.0342755566813
-0.327999569085 0.0340024642184
-0.327118683852 0.0339153007417
-0.326237798619 0.0336434679899
-0.325356913386 0.0335566603382
-0.324476028153 0.033286092713
-0.323595142921 0.0331996441349
-0.322714257688 0.0329303469553
-0.321833372455 0.0328442606257
-0.320952487222 0.0325762391171
-0.320071601989 0.0324905181391
-0.319190716756 0.032404871171
-0.318309831523 0.0321384248437
-0.31742894629 0.032053147461
-0.316548061057 0.0317879887527
-0.315667175824 0.0317030838928
-0.314786290591 0.0314392177285
-0.313905405358 0.031354688265
-0.313024520125 0.0310921194869
-0.312143634893 0.0310079682318
-0.31126274966 0.0307467016017
-0.310381864427 0.0306629313068
-0.309500979194 0.0305792411646
-0.308620093961 0.0303195848675
-0.307739208728 0.0302362794285
-0.306858323495 0.0299779361585
-0.305977438262 0.0298950180354
-0.305096553029 0.0296379922953
-0.304215667796 0.0295554640471
-0.303334782563 0.029299760268
-0.30245389733 0.029217624401
-0.301573012097 0.0289632469441
-0.300692126865 0.0288815059142
-0.299811241632 0.0287998504157
-0.298930356399 0.0285471152857
-0.298049471166 0.0284658579536
-0.297168585933 0.0282144590999
-0.2962877007 0.0281336022717
-0.295406815467 0.0278835438296
-0.294525930234 0.0278030897966
-0.293645045001 0.0275543758383
-0.292764159768 0.0274743268473
-0.291883274535 0.0272269613832
-0.291002389302 0.0271473196375
-0.290121504069 0.026901306618
-0.289240618837 0.0268220742783
-0.288359733604 0.0267429330225
-0.287478848371 0.0264985967806
-0.286597963138 0.0264198678485
-0.285717077905 0.0261768930574
-0.284836192672 0.0260985785112
-0.283955307439 0.0258569689265
-0.283074422206 0.0257790707893
-0.282193536973 0.0255388301117
-0.28131265174 0.0254613503693
-0.280431766507 0.0252224822461
-0.279550881274 0.0251454228474
-0.278669996041 0.0249079308732
-0.277789110809 0.0248312937313
-0.276908225576 0.0247547524827
-0.276027340343 0.0245189684423
-0.27514645511 0.0244428520233
-0.274265569877 0.0242084523174
-0.273384684644 0.0241327625576
-0.272503799411 0.0238997506106
-0.271622914178 0.0238244893067
-0.270742028945 0.023592868495
-0.269861143712 0.0235180374116
-0.268980258479 0.0232878110644
-0.268099373246 0.0232134119348
-0.267218488013 0.022984583335
-0.266337602781 0.0229106178617
-0.265456717548 0.0226831902468
-0.264575832315 0.0226096601026
-0.263694947082 0.0225362306486
-0.262814061849 0.0223105434937
-0.261933176616 0.0222375516076
-0.261052291383 0.0220132727989
-0.26017140615 0.0219407200836
-0.259290520917 0.0217178527108
-0.258409635684 0.0216457407417
-0.257528750451 0.0214242878529
-0.256647865218 0.0213526181783
-0.255766979985 0.0211325827798
-0.254886094753 0.0210613569216
-0.25400520952 0.0208427419795
-0.253124324287 0.0207719614338
-0.252243439054 0.0205547698742
-0.251362553821 0.0204844361115
-0.250481668588 0.0202686708212
-0.249600783355 0.0201987852877
-0.248719898122 0.0201290050728
-0.247839012889 0.0199150132321
-0.246958127656 0.019845683171
-0.246077242423 0.0196331241529
-0.24519635719 0.0195642456338
-0.244315471957 0.0193531221977
-0.243434586725 0.0192846965857
-0.242553701492 0.0190750114545
-0.241672816259 0.0190070400922
-0.240791931026 0.0187987959525
-0.239911045793 0.0187312801604
-0.23903016056 0.0185244796638
-0.238149275327 0.0184574207407
-0.237268390094 0.0182520665035
-0.236387504861 0.0181854657271
-0.235506619628 0.0179815603313
-0.234625734395 0.0179154189583
-0.233744849162 0.0177129649523
-0.232863963929 0.0176472842191
-0.231983078697 0.0175817131479
-0.231102193464 0.0173810652404
-0.230221308231 0.0173159564446
-0.229340422998 0.017116765701
-0.228459537765 0.0170521203693
-0.227578652532 0.0168543892277
-0.226697767299 0.0167902085299
-0.225816882066 0.0165939393964
-0.224935996833 0.0165302244834
-0.2240551116 0.016335419733
-0.223174226367 0.0162721717374
-0.222293341134 0.0160788337142
-0.221412455901 0.0160160537504
-0.220531570669 0.0158241847679
-0.219650685436 0.0157618739327
-0.218769800203 0.0155714762742
-0.21788891497 0.0155096356468
-0.217008029737 0.0153207115661
-0.216127144504 0.0152593422088
-0.215246259271 0.0151980861386
-0.214365374038 0.0150109968884
-0.213484488805 0.014950213485
-0.212603603572 0.0147646029099
-0.211722718339 0.0147042931957
-0.210841833106 0.0145201634528
-0.209960947873 0.0144603284341
-0.209080062641 0.0142776816524
-0.208199177408 0.0142183223198
-0.207318292175 0.0140371606005
-0.206437406942 0.0139782779288
-0.205556521709 0.0137986033458
-0.204675636476 0.0137401982947
-0.203794751243 0.013562012895
-0.20291386601 0.013504086409
-0.202032980777 0.0133273922126
-0.201152095544 0.0132699452216
-0.200271210311 0.0130947442222
-0.199390325078 0.0130377776414
-0.198509439846 0.0128640718065
-0.197628554613 0.0128075865368
-0.19674766938 0.0126353778083
-0.195866784147 0.0125793747365
-0.194985898914 0.0125234885762
-0.194105013681 0.0123531450297
-0.193224128448 0.012297742225
-0.192343243215 0.0121289001666
-0.191462357982 0.0120739815717
-0.190581472749 0.0119066428592
-0.189700587516 0.0118522093149
-0.188819702283 0.0116863757816
-0.18793881705 0.0116324281155
-0.187057931818 0.0114681015702
-0.186177046585 0.011414640597
-0.185296161352 0.0112518228248
-0.184415276119 0.0111988493465
-0.183534390886 0.0110375421083
-0.182653505653 0.0109850569143
-0.18177262042 0.0108252619477
-0.180891735187 0.010773265815
-0.180010849954 0.0106149848343
-0.179129964721 0.0105634785279
-0.178249079488 0.0104067132242
-0.177368194255 0.0103556974968
-0.176487309022 0.0102004495386
-0.17560642379 0.0101499251312
-0.174725538557 0.00999619616413
-0.173844653324 0.00994616380614
-0.172963768091 0.00989625152897
-0.172082882858 0.0097444158628
-0.171201997625 0.00969499657991
-0.170321112392 0.00954468360885
-0.169440227159 0.00949575802258
-0.168559341926 0.00934696931883
-0.167678456693 0.00929853812041
-0.16679757146 0.00915127523446
-0.165916686227 0.00910333910415
-0.165035800994 0.00895760356506
-0.164154915762 0.00891016317228
-0.163274030529 0.00876595648782
-0.162393145296 0.00871901249133
-0.161512260063 0.00857633614819
-0.16063137483 0.0085298891962
-0.159750489597 0.0083887446602
-0.158869604364 0.00834279539052
-0.157988719131 0.00820318410677
-0.157107833898 0.00815773314693
-0.156226948665 0.00801965654001
-0.155346063432 0.00797470450742
-0.154465178199 0.00783816398157
-0.153584292966 0.00779371148363
-0.152703407734 0.0076587084229
-0.151822522501 0.00761475605711
-0.150941637268 0.00748129182556
-0.150060752035 0.00743784017968
-0.149179866802 0.00730591612152
-0.148298981569 0.00726296577364
-0.147418096336 0.00722013838791
-0.146537211103 0.0070901347321
-0.14565632587 0.00704780938699
-0.144775440637 0.00691934891924
-0.143894555404 0.00687752617066
-0.143013670171 0.00675061017056
-0.142132784938 0.00670929056516
-0.141251899706 0.00658392029317
-0.140371014473 0.00654310436846
-0.13949012924 0.006419281066
-0.138609244007 0.00637896935045
-0.137728358774 0.00625669424009
-0.136847473541 0.00621688725324
-0.135966588308 0.00609616153882
-0.135085703075 0.00605685979136
-0.134204817842 0.00593768465814
-0.133323932609 0.00589888865202
-0.132443047376 0.00578126526681
-0.131562162143 0.00574297549535
-0.13068127691 0.00562690500664
-0.129800391678 0.00558912195459
-0.128919506445 0.00547460549267
-0.128038621212 0.00543732963634
-0.127157735979 0.00532436831344
-0.126276850746 0.00528760012075
-0.125395965513 0.00517619503118
-0.12451508028 0.00513993496177
-0.123634195047 0.005030087182
-0.122753309814 0.00499433568732
-0.121872424581 0.00488604627612
-0.120991539348 0.0048508037995
-0.120110654115 0.00481568661281
-0.119229768882 0.0047093407748
-0.11834888365 0.00467473317055
-0.117467998417 0.00456994806428
-0.116587113184 0.00453585046721
-0.115706227951 0.00443262709375
-0.114825342718 0.00439903992077
-0.113944457485 0.00429737926399
-0.113063572252 0.0042643029242
-0.112182687019 0.00416420595089
-0.111301801786 0.00413164084572
-0.110420916553 0.00403310850564
-0.10954003132 0.00400105502889
-0.108659146087 0.00390408825489
-0.107778260854 0.00387254679282
-0.106897375622 0.00377714650097
-0.106016490389 0.00374611743231
-0.105135605156 0.00365228452197
-0.104254719923 0.00362176821808
-0.10337383469 0.00352950357197
-0.102492949457 0.00349950039681
-0.101612064224 0.00340880488116
-0.100731178991 0.00337931519143
-0.0998502937581 0.00329018965601
-0.0989694085252 0.00326121380116
-0.0980885232923 0.00317365907941
-0.0972076380594 0.00314519740171
-0.0963267528264 0.00305921431081
-0.0954458675935 0.00303126714543
-0.0945649823606 0.00294685648638
-0.0936840971277 0.00291942416144
-0.0928032118948 0.00283658671913
-0.0919223266618 0.00280966955573
-0.0910414414289 0.00272840609907
-0.090160556196 0.00270200441137
-0.0892796709631 0.00262231569329
-0.0883987857301 0.00259642978856
-0.0875179004972 0.00257067114904
-0.0866370152643 0.00249294672483
-0.0857561300314 0.00246770425496
-0.0848752447984 0.00239155623511
-0.0839943595655 0.00236683022643
-0.0831134743326 0.00229225931186
-0.0822325890997 0.00226805004921
-0.0813517038668 0.00219505692522
-0.0804708186338 0.00217136468674
-0.0795899334009 0.00209995002309
-0.078709048168 0.0020767750803
-0.0778281629351 0.00200693953126
-0.0769472777021 0.00198428214909
-0.0760663924692 0.0019160263535
-0.0751855072363 0.00189388679035
-0.0743046220034 0.0018272113717
-0.0734237367704 0.00180558987946
-0.0725428515375 0.00174049544593
-0.0716619663046 0.00171939227004
-0.0707810810717 0.00165587941458
-0.0699001958388 0.00163529479405
-0.0690193106058 0.00157336409443
-0.0681384253729 0.00155329826189
-0.06725754014 0.00149295028074
-0.0663766549071 0.00147340346249
-0.0654957696741 0.00141463874737
-0.0646148844412 0.0013956111634
-0.0637339992083 0.00133843024686
-0.0628531139754 0.00131992211088
-0.0619722287425 0.00126432551049
-0.0610913435095 0.00124633702999
-0.0602104582766 0.00119232524841
-0.0593295730437 0.00117485662464
-0.0584486878108 0.00112243014966
-0.0575678025778 0.00110548157773
-0.0566869173449 0.0010546408823
-0.055806032112 0.00103821255118
-0.0549251468791 0.000988958093485
-0.0540442616461 0.000973050186007
-0.0531633764132 0.000925382409497
-0.0522824911803 0.000909995102428
-0.0514016059474 0.000894736423917
-0.0505207207145 0.000849047899899
-0.0496398354815 0.00083431004002
-0.0487589502486 0.000790209157196
-0.0478780650157 0.000775992278877
-0.0469971797828 0.000733479432477
-0.0461162945498 0.000719783692655
-0.0452354093169 0.000678859263346
-0.044354524084 0.000665684812992
-0.0434736388511 0.000626349166911
-0.0425927536181 0.00061369615105
-0.0417118683852 0.000575949639841
-0.0408309831523 0.00056381819758
-0.0399500979194 0.000527661158425
-0.0390692126865 0.00051605142297
-0.0381883274535 0.000481484178621
-0.0373074422206 0.000470396277297
-0.0364265569877 0.000437419136107
-0.0355456717548 0.000426853190383
-0.0346647865218 0.000395466446333
-0.0337839012889 0.000385422571835
-0.032903016056 0.000355626504561
-0.0320221308231 0.000346104811092
-0.0311412455901 0.000317899685913
-0.0302603603572 0.000308900277471
-0.0293794751243 0.000282286345411
-0.0284985898914 0.000273809320202
-0.0276177046585 0.000248786818016
-0.0267368194255 0.000240832268473
-0.0258559341926 0.000217401418666
-0.0249750489597 0.000209969431459
-0.0240941637268 0.000188130442307
-0.0232132784938 0.000181221098359
-0.0223323932609 0.000160974163931
-0.021451508028 0.000154587538429
-0.0205706227951 0.000135932838603
-0.0196897375622 0.00013006900101
-0.0188088523292 0.000113006701486
-0.0179279670963 0.000107665715554
-0.0170470818634 9.2195967874e-05
-0.0161661966305 8.73778916484e-05
-0.0152853113975 7.35008332104e-05
-0.0144044261646 6.92057190432e-05
-0.0135235409317 5.69214731108e-05
-0.0126426556988 5.31493676672e-05
-0.0117617704658 4.95065486174e-05
-0.0108808852329 3.9208987648e-05


==> figuresAndData/dataForConditionalVarianceCircularProb0pt2.tex <==
-0.450442616461 0.00571066117218
-0.449995759368 0.00570759889139
-0.449548902275 0.00570027636448
-0.449102045182 0.00569721866103
-0.448655188089 0.00569209411223
-0.448208330995 0.00568478374297
-0.447761473902 0.00568126593488
-0.447314616809 0.00567541097007
-0.446867759716 0.00567019710223
-0.446420902622 0.00566257191538
-0.445974045529 0.00565851988146
-0.445527188436 0.00565199993758
-0.445080331343 0.00564898038458
-0.444633474249 0.00564345338303
-0.444186617156 0.00563839185952
-0.443739760063 0.00563080727676
-0.44329290297 0.00562662576773
-0.442846045876 0.00562285553824
-0.442399188783 0.00561653250602
-0.44195233169 0.00561060485351
-0.441505474597 0.00560505957072
-0.441058617504 0.00559988449744
-0.44061176041 0.00559506822404
-0.440164903317 0.00559060000815
-0.439718046224 0.00558356098891
-0.439271189131 0.00557976575973
-0.438824332037 0.00557339455379
-0.438377474944 0.00557023583524
-0.437930617851 0.00556449779659
-0.437483760758 0.00555906773713
-0.437036903664 0.00555393811821
-0.436590046571 0.00554910170811
-0.436143189478 0.00554455155844
-0.435696332385 0.00553743366724
-0.435249475291 0.00553344311915
-0.434802618198 0.00552688597104
-0.434355761105 0.00552343019809
-0.433908904012 0.00551740986398
-0.433462046919 0.00551165291251
-0.433015189825 0.00550895975018
-0.432568332732 0.00550370653302
-0.432121475639 0.00549870092404
-0.431674618546 0.00549393796895
-0.431227761452 0.00548663490731
-0.430780904359 0.00548234992973
-0.430334047266 0.00547829354115
-0.429887190173 0.00547170434907
-0.429440333079 0.00546809891805
-0.428993475986 0.00546196615802
-0.428546618893 0.0054587947694
-0.4280997618 0.00545310196025
-0.427652904706 0.00544762670303
-0.427206047613 0.00544236515832
-0.42675919052 0.00543731356908
-0.426312333427 0.00543246825725
-0.425865476334 0.00542782562047
-0.42541861924 0.0054233821291
-0.424971762147 0.00541913432333
-0.424524905054 0.00541507881053
-0.424078047961 0.00540854710611
-0.423631190867 0.00540487336563
-0.423184333774 0.00540138212447
-0.422737476681 0.00539542641069
-0.422290619588 0.00538966119761
-0.421843762494 0.00538671304787
-0.421396905401 0.00538131269324
-0.420950048308 0.00537609391998
-0.420503191215 0.00537105385519
-0.420056334122 0.00536879071031
-0.419609477028 0.0053640924819
-0.419162619935 0.00535956461264
-0.418715762842 0.00535262482257
-0.418268905749 0.00534843678723
-0.417822048655 0.00534441115266
-0.417375191562 0.00534054534395
-0.416928334469 0.00533683682404
-0.416481477376 0.00533073933319
-0.416034620282 0.00532734510139
-0.415587763189 0.00532157135847
-0.415140906096 0.00531848170624
-0.414694049003 0.00531302214932
-0.414247191909 0.00530771977302
-0.413800334816 0.00530507295956
-0.413353477723 0.00530007090868
-0.41290662063 0.00529521924909
-0.412459763537 0.0052905157768
-0.412012906443 0.00528595831581
-0.41156604935 0.00528154471744
-0.411119192257 0.00527727285971
-0.410672335164 0.0052731406468
-0.41022547807 0.00526914600842
-0.409778620977 0.0052652868993
-0.409331763884 0.00526156129866
-0.408884906791 0.00525554571937
-0.408438049697 0.00525208837471
-0.407991192604 0.00524875861865
-0.407544335511 0.00524315465575
-0.407097478418 0.00524008152285
-0.406650621324 0.00523474481262
-0.406203764231 0.00523192076665
-0.405756907138 0.00522684385869
-0.405310050045 0.00522189771552
-0.404863192952 0.00521708053527
-0.404416335858 0.00521473992372
-0.403969478765 0.00521016812692
-0.403522621672 0.00520572000142
-0.403075764579 0.00520139382031
-0.402628907485 0.00519718787456
-0.402182050392 0.00519310047277
-0.401735193299 0.00518912994081
-0.401288336206 0.0051852746216
-0.400841479112 0.00518153287481
-0.400394622019 0.00517790307656
-0.399947764926 0.00517210633968
-0.399500907833 0.00516870283733
-0.399054050739 0.00516540650681
-0.398607193646 0.00515996013071
-0.398160336553 0.00515688067876
-0.39771347946 0.00515390376055
-0.397266622367 0.00514879381339
-0.396819765273 0.00514602462642
-0.39637290818 0.00514113382215
-0.395926051087 0.0051363539694
-0.395479193994 0.00513388884296
-0.3950323369 0.00512931931208
-0.394585479807 0.00512485638031
-0.394138622714 0.00512268227998
-0.393691765621 0.00511842108992
-0.393244908527 0.00511426226407
-0.392798051434 0.00511020441532
-0.392351194341 0.00510624616884
-0.391904337248 0.00510238616199
-0.391457480155 0.0050986230441
-0.391010623061 0.00509495547636
-0.390563765968 0.00509138213165
-0.390116908875 0.00508790169441
-0.389670051782 0.0050845128605
-0.389223194688 0.00507910967187
-0.388776337595 0.00507590734069
-0.388329480502 0.00507279276419
-0.387882623409 0.00506768151511
-0.387435766315 0.00506474583245
-0.386988909222 0.00506189415328
-0.386542052129 0.00505706354983
-0.386095195036 0.0050543833463
-0.385648337942 0.00504973608966
-0.385201480849 0.00504722251655
-0.384754623756 0.00504275378698
-0.384307766663 0.00504040207899
-0.38386090957 0.00503610713508
-0.383414052476 0.00503190089957
-0.382967195383 0.00502778221181
-0.38252033829 0.00502574735935
-0.382073481197 0.00502179319455
-0.381626624103 0.00501792315447
-0.38117976701 0.00501413611479
-0.380732909917 0.00501043096004
-0.380286052824 0.00500680658348
-0.37983919573 0.00500326188706
-0.379392338637 0.0049997957813
-0.378945481544 0.00499640718522
-0.378498624451 0.00499309502629
-0.378051767357 0.00498985824029
-0.377604910264 0.00498669577128
-0.377158053171 0.00498360657152
-0.376711196078 0.00497868447053
-0.376264338985 0.00497574576543
-0.375817481891 0.00497287722955
-0.375370624798 0.00497007784708
-0.374923767705 0.00496546974227
-0.374476910612 0.00496281269652
-0.374030053518 0.00495835904389
-0.373583196425 0.00495584034287
-0.373136339332 0.00495153715945
-0.372689482239 0.00494915287102
-0.372242625145 0.00494499623259
-0.371795768052 0.00494274248353
-0.371348910959 0.00493872852366
-0.370902053866 0.00493660149862
-0.370455196772 0.00493272640773
-0.370008339679 0.00492892284965
-0.369561482586 0.00492518988714
-0.369114625493 0.00492331206799
-0.3686677684 0.00491971051029
-0.368220911306 0.00491617678258
-0.367774054213 0.00491270997433
-0.36732719712 0.00490930918159
-0.366880340027 0.00490597350685
-0.366433482933 0.00490270205908
-0.36598662584 0.00489949395364
-0.365539768747 0.0048963483122
-0.365092911654 0.00489326426278
-0.36464605456 0.0048902409396
-0.364199197467 0.00488727748313
-0.363752340374 0.00488437303999
-0.363305483281 0.00488152676291
-0.362858626188 0.00487873781072
-0.362411769094 0.00487432424174
-0.361964912001 0.00487165434563
-0.361518054908 0.00486903927996
-0.361071197815 0.00486481785313
-0.360624340721 0.00486231688725
-0.360177483628 0.00485986831019
-0.359730626535 0.00485583161829
-0.359283769442 0.00485349228868
-0.358836912348 0.00484957701186
-0.358390055255 0.00484734374676
-0.357943198162 0.00484354669621
-0.357496341069 0.0048414163572
-0.357049483975 0.00483773438782
-0.356602626882 0.00483570388043
-0.356155769789 0.00483213389032
-0.355708912696 0.00482862216197
-0.355262055603 0.00482673909336
-0.354815198509 0.00482333476379
-0.354368341416 0.00481998641826
-0.353921484323 0.00481824404434
-0.35347462723 0.00481499861087
-0.353027770136 0.00481180692992
-0.352580913043 0.00480866826523
-0.35213405595 0.00480558188552
-0.351687198857 0.00480254706445
-0.351240341763 0.00479956308058
-0.35079348467 0.00479662921738
-0.350346627577 0.00479374476315
-0.349899770484 0.00479090901102
-0.34945291339 0.00478812125895
-0.349006056297 0.00478538080963
-0.348559199204 0.00478268697052
-0.348112342111 0.0047800390538
-0.347665485018 0.00477743637634
-0.347218627924 0.00477487825967
-0.346771770831 0.00477236402996
-0.346324913738 0.00476845693124
-0.345878056645 0.00476603514333
-0.345431199551 0.00476365524001
-0.344984342458 0.00475990051177
-0.344537485365 0.00475760906096
-0.344090628272 0.0047553575329
-0.343643771178 0.0047517491885
-0.343196914085 0.00474958220362
-0.342750056992 0.00474745321954
-0.342303199899 0.00474398539015
-0.341856342805 0.00474193711862
-0.341409485712 0.00473856197349
-0.340962628619 0.00473659189797
-0.340515771526 0.00473330690265
-0.340068914433 0.00473141254055
-0.339622057339 0.00472821519395
-0.339175200246 0.00472506403845
-0.338728343153 0.00472328193037
-0.33828148606 0.0047202147249
-0.337834628966 0.00471719186619
-0.337387771873 0.00471551658619
-0.33694091478 0.00471257405175
-0.336494057687 0.0047096740557
-0.336047200593 0.00470681600015
-0.3356003435 0.00470399929108
-0.335153486407 0.0047024946017
-0.334706629314 0.00469975232076
-0.334259772221 0.00469704963666
-0.333812915127 0.00469438597079
-0.333366058034 0.00469176074836
-0.332919200941 0.00468917339836
-0.332472343848 0.00468662335353
-0.332025486754 0.00468411005036
-0.331578629661 0.00468163292906
-0.331131772568 0.00467919143358
-0.330684915475 0.00467678501153
-0.330238058381 0.00467441311423
-0.329791201288 0.00467207519663
-0.329344344195 0.00466858319661
-0.328897487102 0.0046663179923
-0.328450630008 0.00466408514455
-0.328003772915 0.00466188412278
-0.327556915822 0.00465971439996
-0.327110058729 0.00465641976064
-0.326663201636 0.00465431739395
-0.326216344542 0.00465224475646
-0.325769487449 0.00464906464421
-0.325322630356 0.00464705622487
-0.324875773263 0.00464507599639
-0.324428916169 0.00464200567626
-0.323982059076 0.00464008659003
-0.323535201983 0.00463708898321
-0.32308834489 0.0046352290159
-0.322641487796 0.00463339474083
-0.322194630703 0.00463049922728
-0.32174777361 0.00462764092266
-0.321300916517 0.00462589323059
-0.320854059423 0.00462310156755
-0.32040720233 0.0046214070849
-0.319960345237 0.00461868009187
-0.319513488144 0.00461598781254
-0.319066631051 0.0046143726328
-0.318619773957 0.00461174210403
-0.318172916864 0.00460914482803
-0.317726059771 0.00460760469344
-0.317279202678 0.0046050663057
-0.316832345584 0.00460255973801
-0.316385488491 0.00460008451549
-0.315938631398 0.00459863999168
-0.315491774305 0.00459621992165
-0.315044917211 0.00459382980117
-0.314598060118 0.00459146916757
-0.314151203025 0.00458913756124
-0.313704345932 0.00458683452553
-0.313257488838 0.00458455960681
-0.312810631745 0.00458231235442
-0.312363774652 0.00458009232067
-0.311916917559 0.00457789906083
-0.311470060466 0.00457573213314
-0.311023203372 0.00457359109874
-0.310576346279 0.00457147552171
-0.310129489186 0.00456938496907
-0.309682632093 0.00456731901071
-0.309235774999 0.00456527721943
-0.308788917906 0.00456325917092
-0.308342060813 0.00456126444374
-0.30789520372 0.00455929261931
-0.307448346626 0.00455645798531
-0.307001489533 0.00455453663902
-0.30655463244 0.00455263694549
-0.306107775347 0.00455075849744
-0.305660918253 0.00454803925918
-0.30521406116 0.00454620796321
-0.304767204067 0.00454439669629
-0.304320346974 0.00454176107764
-0.303873489881 0.00453999452062
-0.303426632787 0.00453824680109
-0.302979775694 0.00453569109032
-0.302532918601 0.00453398568764
-0.302086061508 0.00453148317529
-0.301639204414 0.0045298185134
-0.301192347321 0.00452736758809
-0.300745490228 0.00452574211232
-0.300298633135 0.00452334118373
-0.299851776041 0.00452175336063
-0.299404918948 0.00451940085932
-0.298958061855 0.00451784917652
-0.298511204762 0.00451554355381
-0.298064347669 0.00451402651991
-0.297617490575 0.00451176624775
-0.297170633482 0.00450953094955
-0.296723776389 0.00450806596295
-0.296276919296 0.00450587374978
-0.295830062202 0.00450370537153
-0.295383205109 0.00450228915695
-0.294936348016 0.00450016164367
-0.294489490923 0.00449805684876
-0.294042633829 0.00449597440103
-0.293595776736 0.00449391393172
-0.293148919643 0.00449257561358
-0.29270206255 0.0044905523929
-0.292255205456 0.00448855007102
-0.291808348363 0.00448656828893
-0.29136149127 0.00448460669002
-0.290914634177 0.00448266492011
-0.290467777084 0.00448074262736
-0.29002091999 0.00447883946236
-0.289574062897 0.00447695507807
-0.289127205804 0.0044750891298
-0.288680348711 0.00447324127524
-0.288233491617 0.00447141117444
-0.287786634524 0.00446959848979
-0.287339777431 0.00446780288602
-0.286892920338 0.00446602403021
-0.286446063244 0.00446426159175
-0.285999206151 0.00446251524237
-0.285552349058 0.0044607846561
-0.285105491965 0.00445906950928
-0.284658634871 0.00445736948056
-0.284211777778 0.00445509362959
-0.283764920685 0.004453428248
-0.283318063592 0.00445177702158
-0.282871206499 0.00445013963808
-0.282424349405 0.00444851578751
-0.281977492312 0.00444634131808
-0.281530635219 0.00444474891526
-0.281083778126 0.00444316911622
-0.280636921032 0.00444105372059
-0.280190063939 0.00443950349306
-0.279743206846 0.00443796496019
-0.279296349753 0.0044359057588
-0.278849492659 0.00443439496078
-0.278402635566 0.0044323734143
-0.277955778473 0.00443088914001
-0.27750892138 0.00442941508486
-0.277062064286 0.00442744505054
-0.276615207193 0.0044259957477
-0.2761683501 0.00442406027925
-0.275721493007 0.00442263456067
-0.275274635914 0.00442073244707
-0.27482777882 0.00441932916176
-0.274380921727 0.00441745920878
-0.273934064634 0.00441560747372
-0.273487207541 0.00441423825283
-0.273040350447 0.00441241690539
-0.272593493354 0.00441106730115
-0.272146636261 0.00440927518867
-0.271699779168 0.00440749981429
-0.271252922074 0.00440618009527
-0.270806064981 0.00440443224466
-0.270359207888 0.00440270026615
-0.269912350795 0.00440098387073
-0.269465493702 0.00439970186216
-0.269018636608 0.00439801075711
-0.268571779515 0.00439633439328
-0.268124922422 0.00439467248967
-0.267678065329 0.00439302476721
-0.267231208235 0.00439178516526
-0.266784351142 0.00439016002521
-0.266337494049 0.00438854825428
-0.265890636956 0.00438694958128
-0.265443779862 0.004385363737
-0.264996922769 0.00438379045416
-0.264550065676 0.00438222946744
-0.264103208583 0.00438068051343
-0.263656351489 0.00437914333066
-0.263209494396 0.00437761765961
-0.262762637303 0.00437610324264
-0.26231578021 0.00437459982406
-0.261868923117 0.00437310715008
-0.261422066023 0.00437162496881
-0.26097520893 0.00437015303028
-0.260528351837 0.00436869108639
-0.260081494744 0.00436723889097
-0.25963463765 0.00436579619971
-0.259187780557 0.00436436277019
-0.258740923464 0.00436293836188
-0.258294066371 0.0043615227361
-0.257847209277 0.00435982258548
-0.257400352184 0.00435842848352
-0.256953495091 0.00435704244559
-0.256506637998 0.00435566424045
-0.256059780904 0.00435429363873
-0.255612923811 0.00435266062123
-0.255166066718 0.00435130914413
-0.254719209625 0.00434996457956
-0.254272352532 0.00434837074822
-0.253825495438 0.00434704390153
-0.253378638345 0.00434572329288
-0.252931781252 0.00434416645858
-0.252484924159 0.00434286219358
-0.252038067065 0.00434156350839
-0.251591209972 0.00434004153015
-0.251144352879 0.00433875784666
-0.250697495786 0.00433725945352
-0.250250638692 0.00433598988561
-0.249803781599 0.00433472483166
-0.249356924506 0.00433325781848
-0.248910067413 0.00433200559141
-0.248463210319 0.00433055986657
-0.248016353226 0.00432931961549
-0.247569496133 0.00432789427903
-0.24712263904 0.00432666516703
-0.246675781947 0.00432525933282
-0.246228924853 0.00432386512204
-0.24578206776 0.00432265333251
-0.245335210667 0.0043212773064
-0.244888353574 0.00432007461023
-0.24444149648 0.00431871591683
-0.243994639387 0.0043173677396
-0.243547782294 0.00431617932643
-0.243100925201 0.00431484721528
-0.242654068107 0.00431352497329
-0.242207211014 0.00431221238342
-0.241760353921 0.00431104166005
-0.241313496828 0.00430974348497
-0.240866639735 0.00430845433499
-0.240419782641 0.00430717399966
-0.239972925548 0.00430601788786
-0.239526068455 0.00430475036933
-0.239079211362 0.00430349105825
-0.238632354268 0.00430223975074
-0.238185497175 0.00430099624453
-0.237738640082 0.00429976033898
-0.237291782989 0.00429862262341
-0.236844925895 0.00429739722219
-0.236398068802 0.00429617884384
-0.235951211709 0.00429496729419
-0.235504354616 0.00429376238069
-0.235057497522 0.00429256391238
-0.234610640429 0.00429137169992
-0.234163783336 0.00429018555555
-0.233716926243 0.00428900529312
-0.23327006915 0.00428783072806
-0.232823212056 0.00428666167738
-0.232376354963 0.0042854979597
-0.23192949787 0.0042843393952
-0.231482640777 0.00428318580565
-0.231035783683 0.00428203701439
-0.23058892659 0.00428089284633
-0.230142069497 0.00427975312795
-0.229695212404 0.00427859465608
-0.22924835531 0.00427746717745
-0.228801498217 0.0042763436227
-0.228354641124 0.00427522382454
-0.227907784031 0.00427410761724
-0.227460926937 0.00427299483661
-0.227014069844 0.00427188527901
-0.226560041705 0.00427076215863
-0.226106013565 0.00426965167546
-0.225651985425 0.00426853077109
-0.225197957285 0.00426743745325
-0.224743929146 0.00426631812279
-0.224289901006 0.00426524121342
-0.223835872866 0.00426412282872
-0.223381844727 0.00426306158471
-0.222927816587 0.00426194353152
-0.222473788447 0.00426089722342
-0.222019760308 0.00425986189195
-0.221565732168 0.0042587468133
-0.221111704028 0.00425772531847
-0.220657675889 0.00425660906533
-0.220203647749 0.0042556007116
-0.219749619609 0.00425448271766
-0.21929559147 0.0042534868229
-0.21884156333 0.00425250057652
-0.21838753519 0.0042513824309
-0.21793350705 0.0042504076146
-0.217479478911 0.00424944189349
-0.217025450771 0.00424832230581
-0.216571422631 0.00424736701564
-0.216117394492 0.00424624349528
-0.215663366352 0.00424529800697
-0.215209338212 0.00424436073487
-0.214755310073 0.00424323375215
-0.214301281933 0.00424230533189
-0.213847253793 0.00424138461373
-0.213393225654 0.00424047141915
-0.212939197514 0.00423934021002
-0.212485169374 0.00423843462526
-0.212031141235 0.00423753606919
-0.211577113095 0.00423639870169
-0.211123084955 0.0042355068731
-0.210669056815 0.0042346215926
-0.210215028676 0.00423374269274
-0.209761000536 0.00423259759048
-0.209306972396 0.00423172426545
-0.208852944257 0.00423085685936
-0.208398916117 0.00422999521103
-0.207944887977 0.00422884049211
-0.207490859838 0.00422798331628
-0.207036831698 0.0042271314552
-0.206582803558 0.00422628475388
-0.206128775419 0.00422544305883
-0.205674747279 0.00422427535595
-0.205220719139 0.00422343680992
-0.204766691 0.00422260285028
-0.20431266286 0.00422177332966
-0.20385863472 0.00422094810223
-0.20340460658 0.00422012702363
-0.202950578441 0.0042189414243
-0.202496550301 0.00421812199533
-0.202042522161 0.00421730632267
-0.201588494022 0.004216494268
-0.201134465882 0.00421568569448
-0.200680437742 0.00421488046678
-0.200226409603 0.00421407845104
-0.199772381463 0.0042132795149
-0.199318353323 0.00421206643151
-0.198864325184 0.00421126729404
-0.198410297044 0.00421047087946
-0.197956268904 0.00420967706131
-0.197502240764 0.00420888571457
-0.197048212625 0.00420809671571
-0.196594184485 0.00420730994263
-0.196140156345 0.0042065252747
-0.195686128206 0.00420574259274
-0.195232100066 0.004204961779
-0.194778071926 0.00420418271719
-0.194324043787 0.00420340529244
-0.193870015647 0.00420262939134
-0.193415987507 0.00420185490189
-0.192961959368 0.00420108171353
-0.192507931228 0.00420030971713
-0.192053903088 0.00419953880496
-0.191599874949 0.00419876887073
-0.191145846809 0.00419799980955
-0.190691818669 0.00419723151794
-0.190237790529 0.00419646389386
-0.18978376239 0.00419569683662
-0.18932973425 0.00419493024698
-0.18887570611 0.00419416402706
-0.188421677971 0.0041933980804
-0.187967649831 0.00419263231191
-0.187513621691 0.0041918666279
-0.187059593552 0.00419110093606
-0.186605565412 0.00419033514545
-0.186151537272 0.00419014651998
-0.185697509133 0.00418938531456
-0.185243480993 0.004188623714
-0.184789452853 0.00418786163287
-0.184335424714 0.00418709898706
-0.183881396574 0.00418633569386
-0.183427368434 0.00418557167187
-0.182973340294 0.00418480684108
-0.182519312155 0.0041846582872
-0.182065284015 0.00418389639898
-0.181611255875 0.00418313343812
-0.181157227736 0.00418236932996
-0.180703199596 0.0041816040012
-0.180249171456 0.00418083737984
-0.179795143317 0.00418006939523
-0.179341115177 0.00417995033559
-0.178887087037 0.00417918398907
-0.178433058898 0.0041784160434
-0.177979030758 0.0041776464332
-0.177525002618 0.00417687509439
-0.177070974479 0.00417677515482
-0.176616946339 0.00417600458316
-0.176162918199 0.00417523206664
-0.175708890059 0.00417445754643
-0.17525486192 0.00417437190258
-0.17480083378 0.00417359748674
-0.17434680564 0.00417282086651
-0.173892777501 0.00417204198818
-0.173438749361 0.00417196896901
-0.172984721221 0.00417118957353
-0.172530693082 0.00417040773466
-0.172076664942 0.00416962340382
-0.171622636802 0.00416956142015
-0.171168608663 0.00416877599145
-0.170714580523 0.00416798790073
-0.170260552383 0.00416793426191
-0.169806524243 0.00416714464825
-0.169352496104 0.00416635221385
-0.168898467964 0.00416630605647
-0.168444439824 0.00416551169664
-0.167990411685 0.00416471436858
-0.167536383545 0.00416467486293
-0.167082355405 0.00416387522936
-0.166628327266 0.00416307249126
-0.166174299126 0.00416303884106
-0.165720270986 0.0041622334396
-0.165266242847 0.0041614248084
-0.164812214707 0.00416139625061
-0.164358186567 0.00416058462029
-0.163904158428 0.00416056031311
-0.163450130288 0.00415974545056
-0.162996102148 0.00415892716332
-0.162542074008 0.00415890671721
-0.162088045869 0.00415808489844
-0.161634017729 0.00415806785753
-0.161179989589 0.00415724229826
-0.16072596145 0.00415641314954
-0.16027193331 0.00415639882892
-0.15981790517 0.00415556567641
-0.159363877031 0.00415555397563
-0.158909848891 0.00415471663422
-0.158455820751 0.00415470724258
-0.158001792612 0.00415386553665
-0.157547764472 0.00415385815291
-0.157093736332 0.00415301191624
-0.156639708193 0.00415216185564
-0.156185680053 0.00415215532432
-0.155731651913 0.0041513005334
-0.155277623773 0.00415129533089
-0.154823595634 0.00415043566678
-0.154369567494 0.00415043152459
-0.153915539354 0.00414956685367
-0.153461511215 0.00414956351253
-0.153007483075 0.00414956197733
-0.152553454935 0.00414869092028
-0.152099426796 0.00414868978153
-0.151645398656 0.00414781339173
-0.151191370516 0.00414781241313
-0.150737342377 0.00414693058903
-0.150283314237 0.00414692954339
-0.149829286097 0.00414604219248
-0.149375257958 0.00414604086166
-0.148921229818 0.00414514790046
-0.148467201678 0.00414514607537
-0.148013173538 0.00414514524572
-0.147559145399 0.00414424490985
-0.147105117259 0.00414424325613
-0.146651089119 0.00414333710831
-0.14619706098 0.0041433344438
-0.14574303284 0.00414333244222
-0.1452890047 0.00414241857857
-0.144834976561 0.0041424152698
-0.144380948421 0.00414149544794
-0.143926920281 0.00414149066737
-0.143472892142 0.00414148624492
-0.143018864002 0.00414055844874
-0.142564835862 0.0041405522911
-0.142110807722 0.00414054631519
-0.141656779583 0.00413961040958
-0.141202751443 0.00413960245471
-0.140748723303 0.00413959451495
-0.140294695164 0.00413865039401
-0.139840667024 0.00413864025103
-0.139386638884 0.00413862996629
-0.138932610745 0.0041376775531
-0.138478582605 0.00413766486021
-0.138024554465 0.00413765187835
-0.137570526326 0.00413763854949
-0.137116498186 0.00413667554905
-0.136662470046 0.00413665954678
-0.136208441907 0.00413664306307
-0.135754413767 0.00413567167044
-0.135300385627 0.00413565235304
-0.134846357487 0.00413563242932
-0.134392329348 0.00413561184862
-0.133938301208 0.00413462976387
-0.133484273068 0.0041346061433
-0.133030244929 0.00413458175345
-0.132576216789 0.00413455654785
-0.132122188649 0.0041335637845
-0.13166816051 0.00413353536618
-0.13121413237 0.00413350603228
-0.13076010423 0.0041334757405
-0.130306076091 0.00413344444957
-0.129852047951 0.00413243873363
-0.129398019811 0.00413240404392
-0.128943991672 0.00413236827067
-0.128489963532 0.0041323313767
-0.128035935392 0.00413229332585
-0.127581907252 0.00413127482895
-0.127127879113 0.00413123324432
-0.126673850973 0.00413119043368
-0.126219822833 0.00413114636494
-0.125765794694 0.00413110100702
-0.125311766554 0.00413105432984
-0.124857738414 0.00413002105043
-0.124403710275 0.0041299707309
-0.123949682135 0.00412991904107
-0.123495653995 0.00412986595487
-0.123041625856 0.00412981144722
-0.122587597716 0.00412975549403
-0.122133569576 0.00412969807221
-0.121679541437 0.00412864836631
-0.121225513297 0.00412858725509
-0.120771485157 0.00412852464499
-0.120317457017 0.00412846051686
-0.119863428878 0.00412839485253
-0.119409400738 0.0041283276348
-0.118955372598 0.00412825884747
-0.118501344459 0.00412818847528
-0.118047316319 0.00412811650396
-0.117593288179 0.00412804292022
-0.11713926004 0.00412796771173
-0.1166852319 0.0041278908671
-0.11623120376 0.00412781237595
-0.115777175621 0.00412673525694
-0.115323147481 0.0041266531867
-0.114869119341 0.00412656947743
-0.114415091201 0.00412648412255
-0.113961063062 0.00412639711642
-0.113507034922 0.00412630845436
-0.113053006782 0.00412621813265
-0.112598978643 0.00412612614849
-0.112144950503 0.00412603250004
-0.111690922363 0.00412593718639
-0.111236894224 0.00412584020759
-0.110782866084 0.0041257415646
-0.110328837944 0.00412564125933
-0.109874809805 0.00412553929463
-0.109420781665 0.00412543567426
-0.108966753525 0.00412533040292
-0.108512725386 0.00412522348624
-0.108058697246 0.00412511493077
-0.107604669106 0.00412500474396
-0.107150640966 0.00412489293422
-0.106696612827 0.00412477951085
-0.106242584687 0.00412565998657
-0.105788556547 0.00412554293713
-0.105334528408 0.0041254242748
-0.104880500268 0.00412530401257
-0.104426472128 0.00412518216429
-0.103972443989 0.00412505874475
-0.103518415849 0.00412493376963
-0.103064387709 0.0041248072555
-0.10261035957 0.00412467921984
-0.10215633143 0.00412454968104
-0.10170230329 0.00412441865834
-0.101248275151 0.0041242861719
-0.100794247011 0.00412514055726
-0.100340218871 0.00412500438493
-0.0998861907315 0.00412486678221
-0.0994321625918 0.00412472777282
-0.0989781344521 0.00412458738135
-0.0985241063124 0.00412444563327
-0.0980700781727 0.00412430255493
-0.097616050033 0.00412415817355
-0.0971620218933 0.00412499346075
-0.0967079937536 0.00412484547551
-0.096253965614 0.00412469624183
-0.0957999374743 0.0041245457904
-0.0953459093346 0.0041243941528
-0.0948918811949 0.00412424136148
-0.0944378530552 0.00412506151877
-0.0939838249155 0.00412490524284
-0.0935297967758 0.00412474788344
-0.0930757686361 0.00412458947644
-0.0926217404965 0.00412443005858
-0.0921677123568 0.00412426966742
-0.0917136842171 0.004125074359
-0.0912596560774 0.00412491066519
-0.0908056279377 0.00412474608381
-0.090351599798 0.0041245806558
-0.0898975716583 0.00412537445175
-0.0894435435186 0.00412520585498
-0.0889895153789 0.0041250365075
-0.0885354872393 0.00412486645363
-0.0880814590996 0.00412469573852
-0.0876274309599 0.00412547619286
-0.0871734028202 0.00412530253106
-0.0867193746805 0.00412512831651
-0.0862653465408 0.00412495359768
-0.0858113184011 0.00412572304372
-0.0853572902614 0.00412554557316
-0.0849032621217 0.0041253677168
-0.0844492339821 0.00412612844872
-0.0839952058424 0.00412594798816
-0.0835411777027 0.00412576726772
-0.083087149563 0.00412558634156
-0.0826331214233 0.0041263361092
-0.0821790932836 0.0041261528205
-0.0817250651439 0.00412596946181
-0.0812710370042 0.00412671055151
-0.0808170088646 0.00412652501261
-0.0803629807249 0.00412633954673
-0.0799089525852 0.00412615421366
-0.0794549244455 0.00412688454837
-0.0790008963058 0.00412669732267
-0.0785468681661 0.00412651038243
-0.0780928400264 0.0041272321986
-0.0776388118867 0.00412704358227
-0.077184783747 0.00412685541123
-0.0767307556074 0.00412756880002
-0.0762767274677 0.00412737918395
-0.075822699328 0.00412808617533
-0.0753686711883 0.0041278952549
-0.0749146430486 0.0041277050515
-0.0744606149089 0.00412840378321
-0.0740065867692 0.00412821253049
-0.0735525586295 0.00412802217353
-0.0730985304898 0.00412871279564
-0.0726445023502 0.00412852165865
-0.0721904742105 0.00412920603838
-0.0717364460708 0.00412901428746
-0.0712824179311 0.00412882373527
-0.0708283897914 0.00412950027056
-0.0703743616517 0.00412930939725
-0.069920333512 0.00412997983132
-0.0694663053723 0.00412978881866
-0.0690122772326 0.00412959932692
-0.068558249093 0.00413026224178
-0.0681042209533 0.00413007292674
-0.0676501928136 0.00413072992152
-0.0671961646739 0.00413054098043
-0.0667421365342 0.00413119212534
-0.0662881083945 0.0041310037616
-0.0658340802548 0.0041308173955
-0.0653800521151 0.00413146155635
-0.0649260239755 0.00413127611572
-0.0644719958358 0.00413191466316
-0.0640179676961 0.00413173036662
-0.0635639395564 0.00413236339286
-0.0631099114167 0.00413218046508
-0.062655883277 0.00413280806859
-0.0622018551373 0.00413262674028
-0.0617478269976 0.00413324902571
-0.0612937988579 0.00413306953355
-0.0608397707183 0.00413368661177
-0.0603857425786 0.0041335091984
-0.0599317144389 0.00413412118642
-0.0594776862992 0.00413394610042
-0.0590236581595 0.00413455312138
-0.0585696300198 0.00413438061722
-0.0581156018801 0.00413498280036
-0.0576615737404 0.0041348131384
-0.0572075456007 0.00413541061903
-0.0567535174611 0.00413524406544
-0.0562994893214 0.00413583698492
-0.0558454611817 0.0041356738117
-0.055391433042 0.00413626231741
-0.0549374049023 0.00413684664824
-0.0544833767626 0.00413668704763
-0.0540293486229 0.00413726716426
-0.0535753204832 0.00413711161842
-0.0531212923436 0.0041376876832
-0.0526672642039 0.00413753648427
-0.0522132360642 0.00413810866548
-0.0517592079245 0.00413867682995
-0.0513051797848 0.00413853058306
-0.0508511516451 0.00413909509487
-0.0503971235054 0.00413895391941
-0.0499430953657 0.00413951496157
-0.049489067226 0.00414007211775
-0.0490350390864 0.0041399369308
-0.0485810109467 0.00414049087035
-0.048126982807 0.00414036151463
-0.0476729546673 0.00414091243513
-0.0472189265276 0.00414145961902
-0.0467648983879 0.00414133734122
-0.0463108702482 0.00414188178093
-0.0458568421085 0.00414176612899
-0.0454028139688 0.00414230803646
-0.0449487858292 0.00414284637512
-0.0444947576895 0.0041427389428
-0.0440407295498 0.00414327504569
-0.0435867014101 0.00414380768258
-0.0431326732704 0.00414370916147
-0.0426786451307 0.00414423987194
-0.042224616991 0.00414476722576
-0.0417705888513 0.00414467832598
-0.0413165607117 0.00414520407549
-0.040862532572 0.00414572658421
-0.0404085044323 0.00414564803428
-0.0399544762926 0.00414616927349
-0.0395004481529 0.00414668739421
-0.0390464200132 0.00414661994088
-0.0385923918735 0.00414713713949
-0.0381383637338 0.00414765134834
-0.0376843355941 0.00414816260085
-0.0372303074545 0.00414810940308
-0.0367762793148 0.00414862019502
-0.0363222511751 0.00414912816787
-0.0358682230354 0.00414908784937
-0.0354141948957 0.00414959573813
-0.034960166756 0.00415010095132
-0.0345061386163 0.00415060352736
-0.0340521104766 0.00415057983653
-0.0335980823369 0.00415108282863
-0.0331440541973 0.00415158333549
-0.0326900260576 0.00415208139835
-0.0322359979179 0.00415207573168
-0.0317819697782 0.00415257473254
-0.0313279416385 0.00415307144961
-0.0308739134988 0.00415356592692
-0.0304198853591 0.00415357972263
-0.0299658572194 0.00415407568145
-0.0295118290798 0.00415456956893
-0.0290578009401 0.00415506143187
-0.0286037728004 0.00415509616948
-0.0281497446607 0.00415559007881
-0.027695716521 0.00415608214016
-0.0272416883813 0.00415657240308
-0.0267876602416 0.0041570609178
-0.0263336321019 0.00415712249822
-0.0258796039622 0.00415761377973
-0.0254255758226 0.00415810349969
-0.0249715476829 0.00415859171104
-0.0245175195432 0.00415907846742
-0.0240634914035 0.00415956382314
-0.0236094632638 0.00415965954835
-0.0231554351241 0.00416014856633
-0.0227014069844 0.00416063638226
-0.0222473788447 0.00416112305311
-0.021793350705 0.00416160863655
-0.0213393225654 0.00416209319089
-0.0208852944257 0.00416222655556
-0.020431266286 0.0041627157143
-0.0199772381463 0.00416320405435
-0.0195232100066 0.00416369163667
-0.0190691818669 0.00416417852288
-0.0186151537272 0.00416466477527
-0.0181611255875 0.00416515045679
-0.0177070974479 0.00416533125242
-0.0172530693082 0.00416582268544
-0.0167990411685 0.00416631377152
-0.0163450130288 0.00416680457621
-0.0158909848891 0.0041672951657
-0.0154369567494 0.00416778560682
-0.0149829286097 0.00416827596706
-0.01452890047 0.00416876631457
-0.0140748723303 0.00416925671813
-0.0136208441907 0.00416950407061
-0.013166816051 0.00417000177371
-0.0127127879113 0.00417049977389
-0.0122587597716 0.00417099814246
-0.0118047316319 0.00417149695138
-0.0113507034922 0.00417199627322
-0.0108966753525 0.00417249618123
-0.0104426472128 0.00417299674926
-0.00998861907315 0.00417349805179
-0.00953459093346 0.00417400016395
-0.00908056279377 0.00417450316149
-0.00862653465408 0.00417500712078
-0.00817250651439 0.00417551211883
-0.0077184783747 0.00417601823325
-0.00726445023502 0.0041765255423
-0.00681042209533 0.00417689857732
-0.00635639395564 0.00417741594721
-0.00590236581595 0.00417793478042
-0.00544833767626 0.00417845515762
-0.00499430953657 0.00417897716011
-0.00454028139688 0.00417950086979
-0.0040862532572 0.00418002636918
-0.00363222511751 0.00418055374142
-0.00317819697782 0.00418108307022
-0.00272416883813 0.00418161443994
-0.00227014069844 0.00418214793551
-0.00181611255875 0.00418268364249
-0.00136208441907 0.00418322164701
-0.000908056279377 0.00418376203584
-0.000454028139689 0.0041843048963
0.0 0.00418485031635
0.00103039649401 0.00418609806914
0.00206079298802 0.00418736072153
0.00309118948202 0.00418860596906
0.00412158597603 0.00418988326625
0.00515198247004 0.00419117858488
0.00618237896405 0.00419249305621
0.00721277545806 0.00419382783151
0.00824317195206 0.00419518408205
0.00927356844607 0.00419641670052
0.0103039649401 0.00419780020699
0.0113343614341 0.0041992086753
0.0123647579281 0.00420064335749
0.0133951544221 0.00420188081545
0.0144255509161 0.0042033518812
0.0154559474101 0.00420485289236
0.0164863439041 0.00420610000208
0.0175167403981 0.00420764460294
0.0185471368921 0.0042092230655
0.0195775333862 0.00421048980254
0.0206079298802 0.00421211943599
0.0216383263742 0.00421378703268
0.0226687228682 0.0042150839487
0.0236991193622 0.0042168106737
0.0247295158562 0.00421812660131
0.0257599123502 0.00421991787403
0.0267903088442 0.00422125773491
0.0278207053382 0.00422260035708
0.0288511018322 0.00422448803479
0.0298814983262 0.00422586215399
0.0309118948202 0.0042278285312
0.0319422913142 0.0042292395075
0.0329726878083 0.00423065950703
0.0340030843023 0.00423274396929
0.0350334807963 0.00423420905236
0.0360638772903 0.00423568715562
0.0370942737843 0.00423790340573
0.0381246702783 0.00423943521932
0.0391550667723 0.00424098425347
0.0401854632663 0.00424255190605
0.0412158597603 0.00424495835471
0.0422462562543 0.00424659175289
0.0432766527483 0.00424824824291
0.0443070492423 0.0042499293148
0.0453374457363 0.00425163648184
0.0463678422304 0.00425337128063
0.0473982387244 0.00425513527109
0.0484286352184 0.00425693003655
0.0494590317124 0.0042587571837
0.0504894282064 0.00426061834271
0.0515198247004 0.00426251516719
0.0525502211944 0.00426444933424
0.0535806176884 0.00426642254452
0.0546110141824 0.00426843652223
0.0556414106764 0.00427049301517
0.0566718071704 0.00427259379474
0.0577022036644 0.00427474065601
0.0587326001585 0.00427693541772
0.0597629966525 0.00427790418202
0.0607933931465 0.00428017364511
0.0618237896405 0.00428249647916
0.0628541861345 0.00428487459868
0.0638845826285 0.00428730994198
0.0649149791225 0.00428839352674
0.0659453756165 0.00429092193841
0.0669757721105 0.00429351340784
0.0680061686045 0.00429467608688
0.0690365650985 0.00429737213347
0.0700669615925 0.00429858724406
0.0710973580865 0.00430139570606
0.0721277545806 0.00430427739853
0.0731581510746 0.00430559959316
0.0741885475686 0.00430860595929
0.0752189440626 0.00430999967318
0.0762493405566 0.00431313905523
0.0772797370506 0.00431461223662
0.0783101335446 0.00431789318004
0.0793405300386 0.0043194539872
0.0803709265326 0.00432104684668
0.0814013230266 0.00432454204311
0.0824317195206 0.00432623503886
0.0834621160146 0.00432796627747
0.0844925125086 0.00433169575796
0.0855229090027 0.00433354012457
0.0865533054967 0.00433542916957
0.0875837019907 0.00433736505252
0.0886140984847 0.00434142931752
0.0896444949787 0.00434349632572
0.0906748914727 0.00434561693676
0.0917052879667 0.00434779342153
0.0927356844607 0.00435002807907
0.0937660809547 0.00435232323663
0.0947964774487 0.0043546812497
0.0958268739427 0.00435710450209
0.0968572704367 0.00436192400503
0.0978876669308 0.00436451677181
0.0989180634248 0.0043647899584
0.0999484599188 0.00436749857342
0.100978856413 0.00437028477269
0.102009252907 0.00437315111069
0.103039649401 0.0043761001705
0.104070045895 0.00437913456384
0.105100442389 0.00438225693112
0.106130838883 0.00438546994145
0.107161235377 0.0043861241682
0.108191631871 0.00438949374555
0.109222028365 0.00439296204506
0.110252424859 0.00439653185212
0.111282821353 0.00439742091365
0.112313217847 0.00440116896171
0.113343614341 0.0044050269503
0.114374010835 0.00440611169133
0.115404407329 0.00441016475675
0.116434803823 0.00441138218955
0.117465200317 0.00441564179422
0.118495596811 0.00441700310416
0.119525993305 0.0044214809565
0.120556389799 0.00442299758383
0.121586786293 0.00442770563902
0.122617182787 0.00442938927968
0.123647579281 0.0044343397404
0.124677975775 0.00443620234688
0.125708372269 0.00443814123142
0.126738768763 0.00444346144611
0.127769165257 0.00444559761546
0.128799561751 0.00444781922885
0.129829958245 0.00445012937718
0.130860354739 0.00445597560455
0.131890751233 0.00445850832026
0.132921147727 0.00446113913839
0.133951544221 0.00446387128566
0.134981940715 0.00446670802316
0.136012337209 0.00446965264642
0.137042733703 0.00447270848549
0.138073130197 0.00447587890496
0.139103526691 0.00447916730404
0.140133923185 0.00448257711662
0.141164319679 0.0044861118113
0.142194716173 0.00448977489148
0.143225112667 0.00449356989537
0.144255509161 0.0044975003961
0.145285905655 0.00450157000172
0.146316302149 0.00450578235527
0.147346698643 0.00450610921598
0.148377095137 0.00451058075635
0.149407491631 0.00451520611413
0.150437888125 0.00451998907412
0.151468284619 0.00452075036998
0.152498681113 0.00452582237188
0.153529077607 0.00453106347712
0.154559474101 0.004532180101
0.155589870595 0.00453773337492
0.156620267089 0.00453909302378
0.157650663583 0.00454497421167
0.158681060077 0.00454659251288
0.159711456571 0.00455281766055
0.160741853065 0.00455471055325
0.161772249559 0.00455672705256
0.162802646053 0.0045634797441
0.163833042547 0.00456579526831
0.164863439041 0.00456824669962
0.165893835535 0.00457556457574
0.166924232029 0.00457834018098
0.167954628523 0.00458126435881
0.168985025017 0.00458434139327
0.170015421511 0.0045875756102
0.171045818005 0.00459097137728
0.172076214499 0.00459949798702
0.173106610993 0.00460327028799
0.174137007487 0.00460721754436
0.175167403981 0.00461134429046
0.176197800475 0.00461565510282
0.177228196969 0.00461498841532
0.178258593463 0.00461964085955
0.179288989957 0.0046244913107
0.180319386451 0.00462954451628
0.181349782945 0.00463480526632
0.182380179439 0.00464027839345
0.183410575933 0.00464055813847
0.184440972427 0.00464643004904
0.185471368921 0.00465252905729
0.186501765415 0.00465332605554
0.187532161909 0.00465985357632
0.188562558403 0.00466100621189
0.189592954897 0.00466798249155
0.190623351391 0.00467521127334
0.191653747885 0.00467695670433
0.192684144379 0.00467888186583
0.193714540873 0.00468681785826
0.194744937367 0.0046891606644
0.195775333862 0.00469760834141
0.196805730356 0.00470039021934
0.19783612685 0.00470337852828
0.198866523344 0.00470657874504
0.199896919838 0.00471607426204
0.200927316332 0.00471975751132
0.201957712826 0.00472366942079
0.20298810932 0.00472781566758
0.204018505814 0.00473220197956
0.205048902308 0.00473683413541
0.206079298802 0.00474171796471
0.207109695296 0.00474685934799
0.20814009179 0.00475226421683
0.209170488284 0.00475793855392
0.210200884778 0.00476388839317
0.211231281272 0.00476357275984
0.212261677766 0.00477004921311
0.21329207426 0.00477681957889
0.214322470754 0.00478389009846
0.215352867248 0.0047845475945
0.216383263742 0.00479219466335
0.217413660236 0.00479335444332
0.21844405673 0.00480160367764
0.219474453224 0.00480329159061
0.220504849718 0.00481216904403
0.221535246212 0.00481441139286
0.222565642706 0.00482394355769
0.2235960392 0.00482676710041
0.224626435694 0.00482986927841
0.225656832188 0.00484041285996
0.226687228682 0.00484413724197
0.227717625176 0.00484816104864
0.22874802167 0.00485249133431
0.229778418164 0.00485713521396
0.230808814658 0.00486209986329
0.231839211152 0.00486739251879
0.232869607646 0.00487302047788
0.23390000414 0.00487899109895
0.234930400634 0.00488531180146
0.235960797128 0.00489199006604
0.236991193622 0.00489903343452
0.238021590116 0.00490644951006
0.23905198661 0.00490651677806
0.240082383104 0.00491465746311
0.241112779598 0.00492319407844
0.242143176092 0.00492427207575
0.243173572586 0.00493358044475
0.24420396908 0.00493535695264
0.245234365574 0.0049454691817
0.246264762068 0.0049479767594
0.247295158562 0.00495892547715
0.248325555056 0.00496219722548
0.24935595155 0.00496584103777
0.250386348044 0.00497808514686
0.251416744538 0.00498254385917
0.252447141032 0.00498740039828
0.253477537526 0.00499266351332
0.25450793402 0.00499834202546
0.255538330514 0.00500444482795
0.256568727008 0.00501098088627
0.257599123502 0.00501795923816
0.258629519996 0.00502538899374
0.25965991649 0.0050332793356
0.260690312984 0.00504163951887
0.261720709478 0.00504176692197
0.262751105972 0.00505105055929
0.263781502466 0.00506083232809
0.26481189896 0.00506227535741
0.265842295454 0.00507303809281
0.266872691948 0.00507539167405
0.267903088442 0.0050871745415
0.268933484936 0.00509047852267
0.26996388143 0.00509425008208
0.270994277924 0.00510761617226
0.272024674418 0.00511239920453
0.273055070912 0.00511768086859
0.274085467406 0.0051234717165
0.2751158639 0.00512978238491
0.276146260394 0.00513662359513
0.277176656888 0.00514400615325
0.278207053382 0.00515194095022
0.279237449876 0.00516043896192
0.28026784637 0.00516951124927
0.281298242864 0.00517916895828
0.282328639358 0.00517981430306
0.283359035852 0.00519063261718
0.284389432346 0.00520207043906
0.28541982884 0.00520439664018
0.286450225334 0.00521706443198
0.287480621828 0.00522055495818
0.288511018322 0.0052246230205
0.289541414816 0.00523920296795
0.29057181131 0.00524450803394
0.291602207804 0.0052504276225
0.292632604298 0.00525697430651
0.293663000792 0.00526416075735
0.294693397286 0.00527199974501
0.29572379378 0.00528050413815
0.296754190274 0.00528968690418
0.297784586768 0.00529956110937
0.298814983262 0.00531013991888
0.299845379756 0.00531107185864
0.30087577625 0.0053230564452
0.301906172744 0.00533578591072
0.302936569238 0.00533877765713
0.303966965732 0.00535299491404
0.304997362226 0.00535741473065
0.30602775872 0.0053625477218
0.307058155214 0.00537908054078
0.308088551708 0.00538572768119
0.309118948202 0.00539313182831
0.310149344696 0.005401307885
0.31117974119 0.00541027086799
0.312210137684 0.00542003590794
0.313240534178 0.00543061824949
0.314270930672 0.00543105767048
0.315301327166 0.00544327832955
0.31633172366 0.00545636294005
0.317362120154 0.00545922285431
0.318392516648 0.00547404082498
0.319422913142 0.00547858074934
0.320453309636 0.00549519679207
0.32148370613 0.005501482893
0.322514102624 0.00550864579081
0.323544499118 0.00551670265635
0.324574895612 0.00552567079088
0.325605292106 0.00553556762617
0.326635688601 0.00554641072455
0.327666085095 0.0055582177789
0.328696481589 0.00557100661278
0.329726878083 0.00557318385005
0.330757274577 0.00558794957552
0.331787671071 0.00559205720748
0.332818067565 0.0056088738553
0.333848464059 0.00561498762881
0.334878860553 0.0056221124662
0.335909257047 0.0056302680364
0.336939653541 0.00565137415582
0.337970050035 0.00566169138924
0.339000446529 0.00567309893261
0.340030843023 0.00567359622408
0.341061239517 0.00568720569272
0.342091636011 0.00570196702825
0.343122032505 0.00570576021637
0.344152428999 0.00572284896296
0.345182825493 0.00572893287294
0.346213221987 0.00573617488976
0.347243618481 0.00575689656314
0.348274014975 0.0057665613474
0.349304411469 0.00577745153639
0.350334807963 0.00578959001773
0.351365204457 0.00580299984723
0.352395600951 0.00580521274351
0.353425997445 0.00582119779518
0.354456393939 0.00583852476816
0.355486790433 0.00584461310202
0.356517186927 0.0058520167401
0.357547583421 0.00587344116488
0.358577979915 0.00588358884803
0.359608376409 0.00589512791604
0.360638772903 0.00590808424506
0.361669169397 0.00590965709337
0.362699565891 0.00592549076875
0.363729962385 0.00594282091998
0.364760358879 0.00594874003045
0.365790755373 0.00596910904931
0.366821151867 0.00597805141308
0.367851548361 0.00598852991306
0.368881944855 0.00600057339764
0.369912341349 0.00601421092758
0.370942737843 0.00602947177589
0.371973134337 0.0060463854277
0.373003530831 0.00605177137455
0.374033927325 0.00607204769315
0.375064323819 0.00608079090916
0.376094720313 0.00609124316255
0.377125116807 0.00610343662505
0.378155513301 0.00611740370558
0.379185909795 0.00613317705002
0.380216306289 0.00615078954107
0.381246702783 0.00617027429799
0.382277099277 0.00617816606171
0.383307495771 0.00618793667457
0.384337892265 0.00621318208534
0.385368288759 0.00622684747002
0.386398685253 0.00624249874337
0.387429081747 0.00624652401516
0.388459478241 0.00626622847942
0.389489874735 0.00627432377152
0.390520271229 0.00629823173655
0.391550667723 0.0063105510552
0.392581064217 0.00632502716967
0.393611460711 0.00634170010664
0.394641857205 0.0063606101849
0.395672253699 0.0063679303792
0.396702650193 0.00639141230677
0.397733046687 0.0064033369006
0.398763443181 0.00641761547538
0.399793839675 0.00643429203351
0.400824236169 0.00645341090058
0.401854632663 0.00647501672487
0.402885029157 0.00648511749553
0.403915425651 0.00649775140931
0.404945822145 0.00651296648055
0.405976218639 0.00653081108053
0.407006615133 0.00655133393687
0.408037011627 0.00657458413309
0.409067408121 0.00658644699407
0.410097804615 0.00660109877815
0.411128201109 0.00661859225863
0.412158597603 0.0066389806013
0.413188994097 0.00666231736382
0.414219390591 0.0066744010826
0.415249787085 0.00670378175349
0.416280183579 0.00672198828358
0.417310580073 0.00672903090706
0.418340976567 0.00675356040678
0.419371373061 0.00676701563615
0.420401769555 0.00679810750046
0.421432166049 0.00681822054304
0.422462562543 0.00682738026062
0.423492959037 0.00685437899418
0.424523355531 0.00687053189821
0.425553752025 0.00689027647612
0.426584148519 0.00691368120023
0.427614545013 0.0069263961125
0.428644941507 0.00695732212498
0.429675338001 0.00697768565811
0.430705734495 0.00700197975484
0.431736130989 0.00701583515347
0.432766527483 0.00703376309651
0.433796923977 0.00705584314474
0.434827320471 0.0070821554776
0.435857716965 0.0071127808923
0.436888113459 0.00713334482037
0.437918509953 0.00715838750667
0.438948906447 0.00717354049923
0.439979302941 0.00719335140202
0.441009699435 0.00721791257323
0.442040095929 0.00724731710739
0.443070492423 0.00726721833805
0.444100888917 0.00729216544961
0.445131285411 0.00732225833068
0.446161681905 0.0073431797937
0.447192078399 0.00736947021267
0.448222474893 0.00738683903676
0.449252871387 0.00742420291997
0.450283267881 0.00743851871898
0.451313664375 0.00747305854846
0.452344060869 0.0074992121308
0.453374457363 0.00753147372833
0.454404853857 0.00755566271107
0.455435250351 0.00758624954105
0.456465646845 0.00760910342286
0.45749604334 0.00763866645821
0.458526439834 0.0076608640886
0.459556836328 0.00769010507885
0.460587232822 0.00772653761558
0.461617629316 0.00775618255752
0.46264802581 0.00777928738483
0.463678422304 0.00781017651108
0.464708818798 0.00784901729319
0.465739215292 0.00788198846684
0.466769611786 0.00790938060334
0.46780000828 0.00794540854728
0.468830404774 0.00797639573156
0.469860801268 0.00800267203447
0.470891197762 0.00803835567877
0.471921594256 0.00806993711825
0.47295199075 0.00811145832987
0.473982387244 0.00814953260391
0.475012783738 0.00818456408998
0.476043180232 0.00821697669488
0.477073576726 0.00824721510943
0.47810397322 0.00828910598323
0.479134369714 0.00832963763895
0.480164766208 0.0083693137655
0.481195162702 0.00840866274248
0.482225559196 0.00844823891473
0.48325595569 0.00848862393555
0.484286352184 0.00851754575139
0.485316748678 0.00856150322694
0.486347145172 0.00860819745036
0.487377541666 0.00864574603813
0.48840793816 0.00868769430285
0.489438334654 0.00873483674677
0.490468731148 0.00878800821208
0.491499127642 0.00883596165527
0.492529524136 0.00888001262669
0.49355992063 0.00892156511764
0.494590317124 0.00897382762246
0.495620713618 0.00902638664686
0.496651110112 0.00908093151749
0.497681506606 0.00912804994735
0.4987119031 0.00918126558648
0.499742299594 0.00923184691219
0.500772696088 0.00929332053098
0.501803092582 0.00934733499526
0.502833489076 0.00940816097262
0.50386388557 0.0094696183205
0.504894282064 0.00952698430899
0.505924678558 0.00959597042699
0.506955075052 0.00966469923528
0.507985471546 0.00972491524908
0.50901586804 0.00979766837394
0.510046264534 0.00987321451509
0.511076661028 0.00995056745588
0.512107057522 0.0100277116256
0.513137454016 0.0101097681891
0.51416785051 0.0102008222931


==> figuresAndData/dataForConditionalVarianceCircularProb0pt4.tex <==
-0.450442616461 0.0190678050482
-0.445938190297 0.0189785640243
-0.441433764132 0.0188953393677
-0.436929337968 0.018807677442
-0.432424911803 0.0187252000057
-0.427920485638 0.0186404308269
-0.423416059474 0.0185629538579
-0.418911633309 0.0184841282819
-0.414407207145 0.0184038922786
-0.40990278098 0.018332810222
-0.405398354815 0.0182608938879
-0.400893928651 0.0181880004089
-0.396389502486 0.0181139887751
-0.391885076321 0.0180509410584
-0.387380650157 0.017987248081
-0.382876223992 0.0179227552259
-0.378371797828 0.0178573186597
-0.373867371663 0.017790806084
-0.369362945498 0.0177371316154
-0.364858519334 0.0176828198446
-0.360354093169 0.0176277358775
-0.355849667005 0.0175717572359
-0.35134524084 0.0175301482533
-0.346840814675 0.0174723564609
-0.342336388511 0.0174293399039
-0.337831962346 0.0173856094984
-0.333327536181 0.0173410625235
-0.328823110017 0.017295608068
-0.324318683852 0.0172491668573
-0.319814257688 0.0172190028194
-0.315309831523 0.0171881996276
-0.310805405358 0.0171388543879
-0.306300979194 0.0171062988592
-0.301796553029 0.0170728857946
-0.297292126865 0.0170385589752
-0.2927877007 0.0170218752045
-0.288283274535 0.0169857543819
-0.283778848371 0.0169675299866
-0.279274422206 0.0169294549468
-0.274769996041 0.0169095100052
-0.270265569877 0.0168887232742
-0.265761143712 0.0168670639079
-0.261256717548 0.0168445105453
-0.256752291383 0.0168406719263
-0.252247865218 0.0168163659354
-0.247743439054 0.0168108910186
-0.243239012889 0.016784797353
-0.238734586725 0.0167776260908
-0.23423016056 0.016769615945
-0.229725734395 0.0167607631129
-0.225221308231 0.016751072514
-0.220716882066 0.0167405576576
-0.216212455901 0.0167292405098
-0.211708029737 0.016717151359
-0.207203603572 0.0167239715765
-0.202699177408 0.0167103753713
-0.198194751243 0.0167155988214
-0.193690325078 0.0167200166814
-0.189185898914 0.0167236549622
-0.184681472749 0.0167265479359
-0.180177046585 0.0167287380338
-0.17567262042 0.0167302757437
-0.171168194255 0.0167312195057
-0.166663768091 0.0167500551242
-0.162159341926 0.0167498080718
-0.157654915762 0.0167671663509
-0.153150489597 0.0167659989877
-0.148646063432 0.0167821237015
-0.144141637268 0.0167976115035
-0.139637211103 0.0168125328606
-0.135132784938 0.0168269663739
-0.130628358774 0.0168409987036
-0.126123932609 0.0168547244905
-0.121619506445 0.0168839610868
-0.11711508028 0.016897042801
-0.112610654115 0.0169101361748
-0.108106227951 0.0169380008851
-0.103601801786 0.0169653629736
-0.0990973756215 0.0169923256329
-0.0945929494569 0.0170190007826
-0.0900885232923 0.017045509021
-0.0855840971277 0.0170719795727
-0.0810796709631 0.0170985502349
-0.0765752447984 0.0171253673201
-0.0720708186338 0.0171637377618
-0.0675663924692 0.0171910327041
-0.0630619663046 0.0172292074234
-0.05855754014 0.0172576241905
-0.0540531139754 0.0172962383911
-0.0495486878108 0.0173350620572
-0.0450442616461 0.0173742714821
-0.0405398354815 0.0174140527652
-0.0360354093169 0.0174614662608
-0.0315309831523 0.0175024063356
-0.0270265569877 0.0175445266386
-0.0225221308231 0.017593126625
-0.0180177046585 0.0176421342619
-0.0135132784938 0.0176879586022
-0.00900885232923 0.0177391014801
-0.00450442616461 0.0177913600887
0.0 0.0178449909125
0.00267562914178 0.0178787479844
0.00535125828356 0.0179114524473
0.00802688742534 0.0179457036842
0.0107025165671 0.0179798247884
0.0133781457089 0.0180148068453
0.0160537748507 0.0180505961263
0.0187294039925 0.01808656076
0.0214050331342 0.0181229037686
0.024080662276 0.0181614979509
0.0267562914178 0.018199228449
0.0294319205596 0.0182375466046
0.0321075497014 0.0182765259373
0.0347831788432 0.01831624215
0.0374588079849 0.0183567731373
0.0401344371267 0.0183981989944
0.0428100662685 0.0184406020246
0.0454856954103 0.0184840667475
0.0481613245521 0.0185286799056
0.0508369536938 0.018574530471
0.0535125828356 0.0186151665795
0.0561882119774 0.0186633366223
0.0588638411192 0.018705589573
0.061539470261 0.0187564647881
0.0642150994027 0.0188007325183
0.0668907285445 0.0188547189767
0.0695663576863 0.0189014215159
0.0722419868281 0.0189492774295
0.0749176159699 0.0190085254045
0.0775932451116 0.0190594895895
0.0802688742534 0.0191119592648
0.0829445033952 0.0191660585202
0.085620132537 0.0192219146198
0.0882957616788 0.0192796580109
0.0909713908206 0.0193394223322
0.0936470199623 0.0193880928809
0.0963226491041 0.0194518775817
0.0989982782459 0.0195039548529
0.101673907388 0.0195723480208
0.104349536529 0.0196284493376
0.107025165671 0.0197020680074
0.109700794813 0.019762841984
0.112376423955 0.0198259835169
0.115052053097 0.0198916718231
0.117727682238 0.0199600905348
0.12040331138 0.0200314277071
0.123078940522 0.0201058758242
0.125754569664 0.0201651162611
0.128430198805 0.0202459744383
0.131105827947 0.020311198547
0.133781457089 0.0203993198833
0.136457086231 0.020471430912
0.139132715373 0.020547132923
0.141808344514 0.0206266768076
0.144483973656 0.0207103194199
0.147159602798 0.0207983235767
0.14983523194 0.0208909580541
0.152510861082 0.0209659885984
0.155186490223 0.0210454766871
0.157862119365 0.0211530020632
0.160537748507 0.0212427361327
0.163213377649 0.021337905955
0.16588900679 0.0214388572233
0.168564635932 0.0215213492733
0.171240265074 0.0216346337404
0.173915894216 0.0217295952652
0.176591523358 0.0218312549447
0.179267152499 0.0219400498131
0.181942781641 0.0220564269879
0.184618410783 0.0221545456112
0.187294039925 0.0222607088999
0.189969669066 0.0223754581775
0.192645298208 0.0224993475957
0.19532092735 0.0226329440808
0.197996556492 0.0227495167406
0.200672185634 0.0228766987807
0.203347814775 0.023015176913
0.206023443917 0.0231379733756
0.208699073059 0.0232733562881
0.211374702201 0.0234221577398
0.214050331342 0.0235852297753
0.216725960484 0.0237078594957
0.219401589626 0.0238745062025
0.222077218768 0.0240307328776
0.22475284791 0.0242055292342
0.227428477051 0.0243727744177
0.230104106193 0.0245344081784
0.232779735335 0.0247195615934
0.235455364477 0.0249034052279
0.238130993619 0.0250888874032
0.24080662276 0.0253050267927
0.243482251902 0.025504079742
0.246157881044 0.0257167568602
0.248833510186 0.0259484355994
0.251509139327 0.0261828273346
0.254184768469 0.0264305772979
0.256860397611 0.0266848099308
0.259536026753 0.0269486721568
0.262211655895 0.0272408403591
0.264887285036 0.0275684132642


==> figuresAndData/dataForConditionalVarianceCircularProb0pt6.tex <==
-0.450442616461 0.0401952228333
-0.445938190297 0.0400978410914
-0.441433764132 0.0400271957691
-0.436929337968 0.0399380533696
-0.432424911803 0.0398347561322
-0.427920485638 0.0397488820821
-0.423416059474 0.0396822236035
-0.418911633309 0.0396068878979
-0.414407207145 0.0395237558989
-0.40990278098 0.0394335316262
-0.405398354815 0.0393661252638
-0.400893928651 0.0392927450181
-0.396389502486 0.0392431880159
-0.391885076321 0.0391884485209
-0.387380650157 0.039128813551
-0.382876223992 0.039064542513
-0.378371797828 0.0389958734295
-0.373867371663 0.0389524820071
-0.369362945498 0.0389050980223
-0.364858519334 0.0388538924716
-0.360354093169 0.0388284554186
-0.355849667005 0.0387700607446
-0.35134524084 0.0387376782981
-0.346840814675 0.0387020076326
-0.342336388511 0.0386924650621
-0.337831962346 0.0386505357957
-0.333327536181 0.0386348654534
-0.328823110017 0.0386162623561
-0.324318683852 0.0385948288471
-0.319814257688 0.0385706703006
-0.315309831523 0.0385727748123
-0.310805405358 0.0385433950358
-0.306300979194 0.0385402970866
-0.301796553029 0.0385346949717
-0.297292126865 0.0385266869966
-0.2927877007 0.0385447075603
-0.288283274535 0.0385320663264
-0.283778848371 0.0385453927505
-0.279274422206 0.0385564484975
-0.274769996041 0.038565332429
-0.270265569877 0.0385997445358
-0.265761143712 0.0386044324747
-0.261256717548 0.0386345186519
-0.256752291383 0.0386625063205
-0.252247865218 0.0386885008164
-0.247743439054 0.0387126146571
-0.243239012889 0.0387614218678
-0.238734586725 0.0387819210293
-0.23423016056 0.0388269227565
-0.229725734395 0.0388700900209
-0.225221308231 0.0389115482526
-0.220716882066 0.0389767215609
-0.216212455901 0.0390149140068
-0.211708029737 0.0390765865988
-0.207203603572 0.0391365844085
-0.202699177408 0.0391950522452
-0.198194751243 0.0392760826008
-0.193690325078 0.0393316693912
-0.189185898914 0.0394095559272
-0.184681472749 0.0394859652653
-0.180177046585 0.0395610693601
-0.17567262042 0.0396350504938
-0.171168194255 0.0397301827392
-0.166663768091 0.039823923305
-0.162159341926 0.0399164689927
-0.157654915762 0.0400080283283
-0.153150489597 0.0401195325935
-0.148646063432 0.0402297898439
-0.144141637268 0.04033903037
-0.139637211103 0.0404474977766
-0.135132784938 0.0405554489275
-0.130628358774 0.0406820251048
-0.126123932609 0.0408078776796
-0.121619506445 0.0409513913518
-0.11711508028 0.0410762889609
-0.112610654115 0.0412186827868
-0.108106227951 0.0413777115803
-0.103601801786 0.0415195101206
-0.0990973756215 0.0416778452585
-0.0945929494569 0.0418361906776
-0.0900885232923 0.0420102221325
-0.0855840971277 0.04218426022
-0.0810796709631 0.0423587459317
-0.0765752447984 0.0425481752008
-0.0720708186338 0.0427381752188
-0.0675663924692 0.0429424596992
-0.0630619663046 0.0431475441213
-0.05855754014 0.0433540034369
-0.0540531139754 0.0435863530832
-0.0495486878108 0.043808139673
-0.0450442616461 0.0440546760936
-0.0405398354815 0.0443027940506
-0.0360354093169 0.044553272217
-0.0315309831523 0.0448168584293
-0.0270265569877 0.0451027886562
-0.0225221308231 0.0453913653913
-0.0180177046585 0.045683596779
-0.0135132784938 0.0459973736456
-0.00900885232923 0.0463316499462
-0.00450442616461 0.04667011909
0.0 0.0470288360191
0.00041620897761 0.0470657071424
0.000832417955221 0.0470952875379
0.00124862693283 0.0471322301157
0.00166483591044 0.0471619436269
0.00208104488805 0.0471989623856
0.00249725386566 0.0472360048196
0.00291346284327 0.0472659126493
0.00332967182088 0.0473030385093
0.00374588079849 0.0473401919533
0.0041620897761 0.0473773743465
0.00457829875371 0.0474075475645
0.00499450773132 0.0474448230751
0.00541071670893 0.0474821313936
0.00582692568655 0.0475194738655
0.00624313466416 0.0475568518301
0.00665934364177 0.0475873745463
0.00707555261938 0.047624857624
0.00749176159699 0.0476623799668
0.0079079705746 0.0476999428863
0.00832417955221 0.0477375476858
0.00874038852982 0.0477751956599
0.00915659750743 0.047812888094
0.00957280648504 0.0478506262635
0.00998901546265 0.0478884114336
0.0104052244403 0.0479262448587
0.0108214334179 0.0479641277815
0.0112376423955 0.0480020614331
0.0116538513731 0.0480400470316
0.0120700603507 0.0480780857821
0.0124862693283 0.0481161788757
0.0129024783059 0.0481607884204
0.0133186872835 0.0481989664964
0.0137348962611 0.0482372025774
0.0141511052388 0.0482754977897
0.0145673142164 0.0483138532418
0.014983523194 0.048358590975
0.0153997321716 0.048397043828
0.0158159411492 0.0484355602969
0.0162321501268 0.0484803782828
0.0166483591044 0.0485189992118
0.017064568082 0.0485576869233
0.0174807770596 0.0486025967012
0.0178969860372 0.0486413954468
0.0183131950149 0.0486863621698
0.0187294039925 0.048725276125
0.0191456129701 0.0487703044454
0.0195618219477 0.0488153500959
0.0199780309253 0.0488544317242
0.0203942399029 0.0488995454227
0.0208104488805 0.0489446796545
0.0212266578581 0.0489839369631
0.0216428668357 0.049029144746
0.0220590758134 0.0490743757165
0.022475284791 0.049119630653
0.0228914937686 0.0491649102522
0.0233077027462 0.049210215126
0.0237239117238 0.0492555457966
0.0241401207014 0.0493009026925
0.024556329679 0.0493462861438
0.0249725386566 0.0493916963774
0.0253887476342 0.0494371335118
0.0258049566118 0.0494825975517
0.0262211655895 0.0495336351528
0.0266373745671 0.0495791231495
0.0270535835447 0.0496246372264
0.0274697925223 0.0496756297334
0.0278860014999 0.0497211644466
0.0283022104775 0.0497721106855
0.0287184194551 0.0498230138481
0.0291346284327 0.0498685560129
0.0295508374103 0.0499194030205
0.0299670463879 0.0499702002616
0.0303832553656 0.0500209446947
0.0307994643432 0.0500716328809
0.0312156733208 0.0501222609578
0.0316318822984 0.0501728246107
0.032048091276 0.0502283689803
0.0324643002536 0.0502787482048
0.0328805092312 0.0503340074203
0.0332967182088 0.0503841748368
0.0337129271864 0.0504391142343
0.0341291361641 0.0504938523472
0.0345453451417 0.050548375902
0.0349615541193 0.0506026702129
0.0353777630969 0.050661360032
0.0357939720745 0.0507150850193
0.0362101810521 0.0507730332877
0.0366263900297 0.0508305321614
0.0370425990073 0.0508875461456
0.0374588079849 0.0509482964442
0.0378750169625 0.0510082873703
0.0382912259402 0.0510674484074
0.0387074349178 0.0511296230308
0.0391236438954 0.0511905251093
0.039539852873 0.0512536194591
0.0399560618506 0.0513181530808
0.0403722708282 0.0513831137158
0.0407884798058 0.0514470786388
0.0412046887834 0.0515147344064


==> figuresAndData/dataForConditionalVarianceCircularProb0pt8.tex <==
-0.450442616461 0.071606609885
-0.447766086434 0.0715901797583
-0.445089556407 0.0715535566331
-0.44241302638 0.0715413622323
-0.439736496353 0.0714823885228
-0.437059966326 0.0714888981808
-0.434383436299 0.0714513087249
-0.431706906272 0.071443997138
-0.429030376245 0.0714307550277
-0.426353846218 0.0714120795796
-0.423677316191 0.0713883846321
-0.421000786164 0.0713964194978
-0.418324256137 0.0713636136456
-0.41564772611 0.071362948301
-0.412971196083 0.0713582571657
-0.410294666056 0.0713497474672
-0.407618136029 0.0713376070236
-0.404941606002 0.0713579067179
-0.402265075975 0.0713389136791
-0.399588545948 0.0713524801149
-0.396912015921 0.0713628355122
-0.394235485894 0.0713701002784
-0.391558955867 0.0713743876034
-0.38888242584 0.0714111376365
-0.386205895813 0.0714096819345
-0.383529365786 0.0714406790073
-0.380852835759 0.0714338574125
-0.378176305732 0.0714594516513
-0.375499775705 0.0714824119645
-0.372823245678 0.0715028135809
-0.370146715651 0.0715553070736
-0.367470185624 0.0715706899911
-0.364793655597 0.0716180668335
-0.36211712557 0.0716286964429
-0.359440595543 0.0716712053928
-0.356764065516 0.071711307737
-0.354087535489 0.0717490594471
-0.351411005462 0.0718182325989
-0.348734475435 0.0718513149519
-0.346057945408 0.0718822074408
-0.343381415381 0.0719442763288
-0.340704885354 0.0720039825943
-0.338028355327 0.0720613713492
-0.3353518253 0.0721164875579
-0.332675295273 0.072169376094
-0.329998765246 0.0722526753259
-0.327322235219 0.0723010915547
-0.324645705192 0.0723797003813
-0.321969175165 0.0724559457962
-0.319292645138 0.0725298656082
-0.316616115111 0.072601497926
-0.313939585084 0.0726708811728
-0.311263055057 0.0727695321191
-0.30858652503 0.0728343643769
-0.305909995003 0.0729281976904
-0.303233464976 0.0730195861964
-0.300556934949 0.0731085625432
-0.297880404922 0.0732257568876
-0.295203874895 0.0733098245856
-0.292527344868 0.0734218019376
-0.289850814841 0.0735311181462
-0.287174284814 0.0736377999449
-0.284497754787 0.0737715100324
-0.28182122476 0.0738728040229
-0.279144694733 0.0740007707798
-0.276468164706 0.0741257939487
-0.273791634679 0.0742478929383
-0.271115104652 0.0743670873
-0.268438574625 0.0745117584623
-0.265762044597 0.0746531124782
-0.26308551457 0.074791158306
-0.260408984543 0.0749535658159
-0.257732454516 0.075084780674
-0.255055924489 0.0752670474639
-0.252379394462 0.0754181100286
-0.249702864435 0.0755920267792
-0.247026334408 0.0757616057021
-0.244349804381 0.0759268193272
-0.241673274354 0.0761134563914
-0.238996744327 0.0762950834994
-0.2363202143 0.076471642517
-0.233643684273 0.0766679814216
-0.230967154246 0.0768830611348
-0.228290624219 0.0770915244425
-0.225614094192 0.0772932273973
-0.222937564165 0.0775350445906
-0.220261034138 0.0777451147581
-0.217584504111 0.0779925171219
-0.214907974084 0.0782298595369
-0.212231444057 0.0784785505786
-0.20955491403 0.0787366712419
-0.206878384003 0.0790228020806
-0.204201853976 0.0792923625436
-0.201525323949 0.0795832638995
-0.198848793922 0.0798899201525
-0.196172263895 0.0802055173486
-0.193495733868 0.080521544501
-0.190819203841 0.0808738542822
-0.188142673814 0.0812334627178
-0.185466143787 0.0816232718214


==> figuresAndData/dataForConditionalVarianceLaplaceEqualAreas.tex <==
-4.5 0.13656204421
-4.49551 0.136561861464
-4.49102 0.136561676614
-4.48653 0.136561489637
-4.48204 0.136561300509
-4.47755 0.136561109205
-4.47306 0.136560915701
-4.46857 0.136560719972
-4.46408 0.136560521993
-4.45959 0.136560321738
-4.4551 0.136560119181
-4.45061 0.136559914297
-4.44612 0.136559707059
-4.44163 0.13655949744
-4.43714 0.136559285415
-4.43265 0.136559070954
-4.42816 0.136558854032
-4.42367 0.136558634619
-4.41918 0.136558412689
-4.41469 0.136558188213
-4.4102 0.136557961161
-4.40571 0.136557731505
-4.40122 0.136557499216
-4.39673 0.136557264263
-4.39224 0.136557026617
-4.38775 0.136556786248
-4.38326 0.136556543124
-4.37877 0.136556297215
-4.37428 0.136556048489
-4.36979 0.136555796915
-4.3653 0.136555542461
-4.36081 0.136555285093
-4.35632 0.13655502478
-4.35183 0.136554761488
-4.34734 0.136554495183
-4.34285 0.136554225833
-4.33836 0.136553953402
-4.33387 0.136553677856
-4.32938 0.136553399159
-4.32489 0.136553117278
-4.3204 0.136552832175
-4.31591 0.136552543815
-4.31142 0.13655225216
-4.30693 0.136551957175
-4.30244 0.136551658822
-4.29795 0.136551357062
-4.29346 0.136551051858
-4.28897 0.136550743171
-4.28448 0.136550430962
-4.27999 0.136550115192
-4.2755 0.13654979582
-4.27101 0.136549472807
-4.26652 0.136549146111
-4.26203 0.136548815692
-4.25754 0.136548481507
-4.25305 0.136548143515
-4.24856 0.136547801672
-4.24407 0.136547455936
-4.23958 0.136547106264
-4.23509 0.136546752611
-4.2306 0.136546394933
-4.22611 0.136546033184
-4.22162 0.13654566732
-4.21713 0.136545297294
-4.21264 0.136544923061
-4.20815 0.136544544572
-4.20366 0.13654416178
-4.19917 0.136543774639
-4.19468 0.136543383098
-4.19019 0.136542987109
-4.1857 0.136542586622
-4.18121 0.136542181587
-4.17672 0.136541771954
-4.17223 0.136541357671
-4.16774 0.136540938687
-4.16325 0.136540514949
-4.15876 0.136540086404
-4.15427 0.136539652999
-4.14978 0.13653921468
-4.14529 0.136538771391
-4.1408 0.136538323079
-4.13631 0.136537869686
-4.13182 0.136537411157
-4.12733 0.136536947434
-4.12284 0.13653647846
-4.11835 0.136536004177
-4.11386 0.136535524525
-4.10937 0.136535039445
-4.10488 0.136534548876
-4.10039 0.136534052759
-4.0959 0.13653355103
-4.09141 0.136533043629
-4.08692 0.136532530492
-4.08243 0.136532011556
-4.07794 0.136531486756
-4.07345 0.136530956028
-4.06896 0.136530419305
-4.06447 0.136529876522
-4.05998 0.136529327612
-4.05549 0.136528772506
-4.051 0.136528211137
-4.04651 0.136527643434
-4.04202 0.136527069329
-4.03753 0.136526488749
-4.03304 0.136525901625
-4.02855 0.136525307883
-4.02406 0.13652470745
-4.01957 0.136524100253
-4.01508 0.136523486217
-4.01059 0.136522865266
-4.0061 0.136522237324
-4.00161 0.136521602315
-3.99712 0.13652096016
-3.99263 0.136520310781
-3.98814 0.136519654097
-3.98365 0.13651899003
-3.97916 0.136518318496
-3.97467 0.136517639415
-3.97018 0.136516952703
-3.96569 0.136516258276
-3.9612 0.13651555605
-3.95671 0.136514845938
-3.95222 0.136514127854
-3.94773 0.136513401711
-3.94324 0.13651266742
-3.93875 0.136511924891
-3.93426 0.136511174035
-3.92977 0.136510414759
-3.92528 0.136509646972
-3.92079 0.136508870579
-3.9163 0.136508085488
-3.91181 0.136507291602
-3.90732 0.136506488825
-3.90283 0.13650567706
-3.89834 0.136504856208
-3.89385 0.136504026171
-3.88936 0.136503186846
-3.88487 0.136502338134
-3.88038 0.136501479931
-3.87589 0.136500612133
-3.8714 0.136499734636
-3.86691 0.136498847333
-3.86242 0.136497950119
-3.85793 0.136497042883
-3.85344 0.136496125518
-3.84895 0.136495197912
-3.84446 0.136494259954
-3.83997 0.136493311531
-3.83548 0.136492352529
-3.83099 0.136491382833
-3.8265 0.136490402326
-3.82201 0.13648941089
-3.81752 0.136488408407
-3.81303 0.136487394756
-3.80854 0.136486369816
-3.80405 0.136485333464
-3.79956 0.136484285576
-3.79507 0.136483226027
-3.79058 0.136482154689
-3.78609 0.136481071436
-3.7816 0.136479976137
-3.77711 0.136478868662
-3.77262 0.136477748879
-3.76813 0.136476616654
-3.76364 0.136475471852
-3.75915 0.136474314338
-3.75466 0.136473143973
-3.75017 0.136471960618
-3.74568 0.136470764133
-3.74119 0.136469554375
-3.7367 0.136468331201
-3.73221 0.136467094466
-3.72772 0.136465844022
-3.72323 0.136464579723
-3.71874 0.136463301418
-3.71425 0.136462008956
-3.70976 0.136460702184
-3.70527 0.136459380948
-3.70078 0.136458045091
-3.69629 0.136456694457
-3.6918 0.136455328885
-3.68731 0.136453948214
-3.68282 0.136452552283
-3.67833 0.136451140926
-3.67384 0.136449713977
-3.66935 0.13644827127
-3.66486 0.136446812633
-3.66037 0.136445337896
-3.65588 0.136443846886
-3.65139 0.136442339428
-3.6469 0.136440815346
-3.64241 0.13643927446
-3.63792 0.13643771659
-3.63343 0.136436141554
-3.62894 0.136434549168
-3.62445 0.136432939246
-3.61996 0.1364313116
-3.61547 0.13642966604
-3.61098 0.136428002374
-3.60649 0.136426320408
-3.602 0.136424619947
-3.59751 0.136422900792
-3.59302 0.136421162744
-3.58853 0.136419405601
-3.58404 0.136417629158
-3.57955 0.13641583321
-3.57506 0.136414017547
-3.57057 0.136412181961
-3.56608 0.136410326237
-3.56159 0.136408450162
-3.5571 0.136406553518
-3.55261 0.136404636087
-3.54812 0.136402697646
-3.54363 0.136400737972
-3.53914 0.136398756839
-3.53465 0.136396754018
-3.53016 0.13639472928
-3.52567 0.13639268239
-3.52118 0.136390613114
-3.51669 0.136388521214
-3.5122 0.136386406449
-3.50771 0.136384268577
-3.50322 0.136382107352
-3.49873 0.136379922527
-3.49424 0.136377713852
-3.48975 0.136375481073
-3.48526 0.136373223936
-3.48077 0.136370942183
-3.47628 0.136368635553
-3.47179 0.136366303782
-3.4673 0.136363946606
-3.46281 0.136361563755
-3.45832 0.136359154958
-3.45383 0.136356719941
-3.44934 0.136354258428
-3.44485 0.136351770138
-3.44036 0.136349254789
-3.43587 0.136346712096
-3.43138 0.13634414177
-3.42689 0.136341543521
-3.4224 0.136338917055
-3.41791 0.136336262074
-3.41342 0.136333578278
-3.40893 0.136330865364
-3.40444 0.136328123027
-3.39995 0.136325350957
-3.39546 0.136322548841
-3.39097 0.136319716365
-3.38648 0.13631685321
-3.38199 0.136313959053
-3.3775 0.13631103357
-3.37301 0.136308076433
-3.36852 0.13630508731
-3.36403 0.136302065866
-3.35954 0.136299011763
-3.35505 0.136295924658
-3.35056 0.136292804208
-3.34607 0.136289650064
-3.34158 0.136286461872
-3.33709 0.136283239279
-3.3326 0.136279981925
-3.32811 0.136276689448
-3.32362 0.13627336148
-3.31913 0.136269997653
-3.31464 0.136266597592
-3.31015 0.136263160921
-3.30566 0.136259687257
-3.30117 0.136256176218
-3.29668 0.136252627413
-3.29219 0.13624904045
-3.2877 0.136245414934
-3.28321 0.136241750463
-3.27872 0.136238046634
-3.27423 0.136234303037
-3.26974 0.136230519262
-3.26525 0.13622669489
-3.26076 0.136222829503
-3.25627 0.136218922675
-3.25178 0.136214973978
-3.24729 0.136210982978
-3.2428 0.136206949238
-3.23831 0.136202872317
-3.23382 0.136198751768
-3.22933 0.136194587142
-3.22484 0.136190377983
-3.22035 0.136186123833
-3.21586 0.136181824227
-3.21137 0.136177478698
-3.20688 0.136173086772
-3.20239 0.136168647972
-3.1979 0.136164161816
-3.19341 0.136159627818
-3.18892 0.136155045485
-3.18443 0.136150414322
-3.17994 0.136145733826
-3.17545 0.136141003493
-3.17096 0.136136222811
-3.16647 0.136131391263
-3.16198 0.13612650833
-3.15749 0.136121573485
-3.153 0.136116586197
-3.14851 0.136111545929
-3.14402 0.13610645214
-3.13953 0.136101304284
-3.13504 0.136096101809
-3.13055 0.136090844157
-3.12606 0.136085530765
-3.12157 0.136080161065
-3.11708 0.136074734484
-3.11259 0.136069250442
-3.1081 0.136063708356
-3.10361 0.136058107634
-3.09912 0.13605244768
-3.09463 0.136046727893
-3.09014 0.136040947666
-3.08565 0.136035106385
-3.08116 0.13602920343
-3.07667 0.136023238177
-3.07218 0.136017209995
-3.06769 0.136011118246
-3.0632 0.136004962288
-3.05871 0.13599874147
-3.05422 0.135992455139
-3.04973 0.135986102631
-3.04524 0.135979683278
-3.04075 0.135973196407
-3.03626 0.135966641337
-3.03177 0.13596001738
-3.02728 0.135953323843
-3.02279 0.135946560025
-3.0183 0.135939725219
-3.01381 0.135932818712
-3.00932 0.135925839783
-3.00483 0.135918787705
-3.00034 0.135911661744
-2.99585 0.13590446116
-2.99136 0.135897185204
-2.98687 0.135889833121
-2.98238 0.135882404149
-2.97789 0.13587489752
-2.9734 0.135867312456
-2.96891 0.135859648174
-2.96442 0.135851903884
-2.95993 0.135844078786
-2.95544 0.135836172075
-2.95095 0.135828182938
-2.94646 0.135820110553
-2.94197 0.135811954092
-2.93748 0.135803712718
-2.93299 0.135795385588
-2.9285 0.13578697185
-2.92401 0.135778470644
-2.91952 0.135769881102
-2.91503 0.135761202348
-2.91054 0.135752433498
-2.90605 0.135743573661
-2.90156 0.135734621935
-2.89707 0.135725577413
-2.89258 0.135716439177
-2.88809 0.135707206302
-2.8836 0.135697877854
-2.87911 0.135688452891
-2.87462 0.13567893046
-2.87013 0.135669309604
-2.86564 0.135659589352
-2.86115 0.135649768727
-2.85666 0.135639846743
-2.85217 0.135629822404
-2.84768 0.135619694706
-2.84319 0.135609462636
-2.8387 0.135599125169
-2.83421 0.135588681275
-2.82972 0.135578129911
-2.82523 0.135567470026
-2.82074 0.135556700561
-2.81625 0.135545820445
-2.81176 0.135534828597
-2.80727 0.135523723929
-2.80278 0.135512505342
-2.79829 0.135501171725
-2.7938 0.13548972196
-2.78931 0.135478154917
-2.78482 0.135466469458
-2.78033 0.135454664432
-2.77584 0.135442738679
-2.77135 0.13543069103
-2.76686 0.135418520303
-2.76237 0.135406225307
-2.75788 0.135393804841
-2.75339 0.135381257691
-2.7489 0.135368582634
-2.74441 0.135355778436
-2.73992 0.135342843853
-2.73543 0.135329777626
-2.73094 0.13531657849
-2.72645 0.135303245166
-2.72196 0.135289776364
-2.71747 0.135276170782
-2.71298 0.135262427109
-2.70849 0.13524854402
-2.704 0.135234520178
-2.69951 0.135220354238
-2.69502 0.135206044838
-2.69053 0.135191590609
-2.68604 0.135176990167
-2.68155 0.135162242117
-2.67706 0.135147345051
-2.67257 0.135132297549
-2.66808 0.13511709818
-2.66359 0.1351017455
-2.6591 0.135086238051
-2.65461 0.135070574364
-2.65012 0.135054752956
-2.64563 0.135038772334
-2.64114 0.135022630987
-2.63665 0.135006327397
-2.63216 0.134989860029
-2.62767 0.134973227336
-2.62318 0.134956427757
-2.61869 0.134939459718
-2.6142 0.134922321634
-2.60971 0.134905011902
-2.60522 0.134887528909
-2.60073 0.134869871027
-2.59624 0.134852036613
-2.59175 0.134834024012
-2.58726 0.134815831553
-2.58277 0.134797457554
-2.57828 0.134778900316
-2.57379 0.134760158125
-2.5693 0.134741229256
-2.56481 0.134722111967
-2.56032 0.134702804502
-2.55583 0.13468330509
-2.55134 0.134663611945
-2.54685 0.134643723267
-2.54236 0.134623637241
-2.53787 0.134603352035
-2.53338 0.134582865805
-2.52889 0.134562176688
-2.5244 0.134541282808
-2.51991 0.134520182273
-2.51542 0.134498873175
-2.51093 0.134477353591
-2.50644 0.134455621582
-2.50195 0.134433675192
-2.49746 0.13441151245
-2.49297 0.134389131368
-2.48848 0.134366529942
-2.48399 0.134343706154
-2.4795 0.134320657966
-2.47501 0.134297383325
-2.47052 0.134273880161
-2.46603 0.134250146388
-2.46154 0.134226179902
-2.45705 0.134201978583
-2.45256 0.134177540294
-2.44807 0.13415286288
-2.44358 0.134127944169
-2.43909 0.134102781971
-2.4346 0.13407737408
-2.43011 0.13405171827
-2.42562 0.134025812301
-2.42113 0.13399965391
-2.41664 0.133973240821
-2.41215 0.133946570738
-2.40766 0.133919641345
-2.40317 0.133892450311
-2.39868 0.133864995284
-2.39419 0.133837273895
-2.3897 0.133809283756
-2.38521 0.13378102246
-2.38072 0.133752487581
-2.37623 0.133723676676
-2.37174 0.133694587279
-2.36725 0.133665216909
-2.36276 0.133635563064
-2.35827 0.133605623222
-2.35378 0.133575394843
-2.34929 0.133544875366
-2.3448 0.133514062211
-2.34031 0.133482952778
-2.33582 0.133451544448
-2.33133 0.13341983458
-2.32684 0.133387820515
-2.32235 0.133355499573
-2.31786 0.133322869053
-2.31337 0.133289926234
-2.30888 0.133256668374
-2.30439 0.133223092712
-2.2999 0.133189196465
-2.29541 0.133154976829
-2.29092 0.133120430978
-2.28643 0.133085556068
-2.28194 0.13305034923
-2.27745 0.133014807578
-2.27296 0.132978928199
-2.26847 0.132942708164
-2.26398 0.13290614452
-2.25949 0.132869234291
-2.255 0.132831974481
-2.25051 0.132794362072
-2.24602 0.132756394022
-2.24153 0.13271806727
-2.23704 0.132679378729
-2.23255 0.132640325294
-2.22806 0.132600903833
-2.22357 0.132561111195
-2.21908 0.132520944205
-2.21459 0.132480399664
-2.2101 0.132439474351
-2.20561 0.132398165024
-2.20112 0.132356468415
-2.19663 0.132314381234
-2.19214 0.132271900168
-2.18765 0.13222902188
-2.18316 0.13218574301
-2.17867 0.132142060175
-2.17418 0.132097969966
-2.16969 0.132053468953
-2.1652 0.13200855368
-2.16071 0.131963220669
-2.15622 0.131917466416
-2.15173 0.131871287394
-2.14724 0.131824680052
-2.14275 0.131777640814
-2.13826 0.131730166079
-2.13377 0.131682252223
-2.12928 0.131633895596
-2.12479 0.131585092524
-2.1203 0.131535839308
-2.11581 0.131486132225
-2.11132 0.131435967525
-2.10683 0.131385341435
-2.10234 0.131334250155
-2.09785 0.131282689863
-2.09336 0.131230656707
-2.08887 0.131178146814
-2.08438 0.131125156282
-2.07989 0.131071681187
-2.0754 0.131017717576
-2.07091 0.130963261472
-2.06642 0.130908308873
-2.06193 0.13085285575
-2.05744 0.130796898047
-2.05295 0.130740431685
-2.04846 0.130683452556
-2.04397 0.130625956527
-2.03948 0.13056793944
-2.03499 0.130509397109
-2.0305 0.130450325322
-2.02601 0.130390719842
-2.02152 0.130330576403
-2.01703 0.130269890715
-2.01254 0.130208658459
-2.00805 0.130146875293
-2.00356 0.130084536844
-1.99907 0.130021638716
-1.99458 0.129958176483
-1.99009 0.129894145694
-1.9856 0.129829541872
-1.98111 0.12976436051
-1.97662 0.129698597078
-1.97213 0.129632247015
-1.96764 0.129565305736
-1.96315 0.129497768627
-1.95866 0.129429631048
-1.95417 0.129360888331
-1.94968 0.129291535781
-1.94519 0.129221568677
-1.9407 0.129150982269
-1.93621 0.12907977178
-1.93172 0.129007932406
-1.92723 0.128935459317
-1.92274 0.128862347653
-1.91825 0.128788592528
-1.91376 0.12871418903
-1.90927 0.128639132216
-1.90478 0.12856341712
-1.90029 0.128487038745
-1.8958 0.128409992068
-1.89131 0.128332272039
-1.88682 0.12825387358
-1.88233 0.128174791585
-1.87784 0.128095020922
-1.87335 0.12801455643
-1.86886 0.127933392921
-1.86437 0.127851525182
-1.85988 0.127768947969
-1.85539 0.127685656012
-1.8509 0.127601644015
-1.84641 0.127516906653
-1.84192 0.127431438575
-1.83743 0.127345234401
-1.83294 0.127258288725
-1.82845 0.127170596115
-1.82396 0.12708215111
-1.81947 0.126992948221
-1.81498 0.126902981936
-1.81049 0.126812246711
-1.806 0.126720736979
-1.80151 0.126628447144
-1.79702 0.126535371585
-1.79253 0.126441504651
-1.78804 0.126346840668
-1.78355 0.126251373933
-1.77906 0.126155098718
-1.77457 0.126058009267
-1.77008 0.125960099799
-1.76559 0.125861364505
-1.7611 0.125761797553
-1.75661 0.125661393081
-1.75212 0.125560145203
-1.74763 0.125458048008
-1.74314 0.125355095558
-1.73865 0.125251281888
-1.73416 0.125146601011
-1.72967 0.125041046911
-1.72518 0.124934613549
-1.72069 0.124827294859
-1.7162 0.124719084752
-1.71171 0.124609977113
-1.70722 0.124499965801
-1.70273 0.124389044653
-1.69824 0.12427720748
-1.69375 0.124164448068
-1.68926 0.124050760181
-1.68477 0.123936137556
-1.68028 0.123820573909
-1.67579 0.123704062932
-1.6713 0.123586598291
-1.66681 0.123468173632
-1.66232 0.123348782576
-1.65783 0.123228418721
-1.65334 0.123107075643
-1.64885 0.122984746897
-1.64436 0.122861426012
-1.63987 0.122737106499
-1.63538 0.122611781844
-1.63089 0.122485445513
-1.6264 0.12235809095
-1.62191 0.122229711579
-1.61742 0.122100300803
-1.61293 0.121969852002
-1.60844 0.121838358539
-1.60395 0.121705813754
-1.59946 0.121572210969
-1.59497 0.121437543487
-1.59048 0.12130180459
-1.58599 0.121164987541
-1.5815 0.121027085586
-1.57701 0.120888091951
-1.57252 0.120747999845
-1.56803 0.120606802459
-1.56354 0.120464492967
-1.55905 0.120321064524
-1.55456 0.120176510271
-1.55007 0.12003082333
-1.54558 0.119883996809
-1.54109 0.119736023799
-1.5366 0.119586897376
-1.53211 0.119436610601
-1.52762 0.11928515652
-1.52313 0.119132528166
-1.51864 0.118978718558
-1.51415 0.118823720699
-1.50966 0.118667527583
-1.50517 0.118510132188
-1.50068 0.118351527481
-1.49619 0.118191706419
-1.4917 0.118030661944
-1.48721 0.11786838699
-1.48272 0.117704874481
-1.47823 0.117540117328
-1.47374 0.117374108435
-1.46925 0.117206840696
-1.46476 0.117038306998
-1.46027 0.116868500218
-1.45578 0.116697413226
-1.45129 0.116525038885
-1.4468 0.116351370053
-1.44231 0.116176399579
-1.43782 0.11600012031
-1.43333 0.115822525087
-1.42884 0.115643606744
-1.42435 0.115463358115
-1.41986 0.115281772029
-1.41537 0.115098841313
-1.41088 0.114914558792
-1.40639 0.114728917288
-1.4019 0.114541909625
-1.39741 0.114353528625
-1.39292 0.114163767111
-1.38843 0.113972617908
-1.38394 0.11378007384
-1.37945 0.113586127737
-1.37496 0.11339077243
-1.37047 0.113194000755
-1.36598 0.112995805551
-1.36149 0.112796179663
-1.357 0.112595115943
-1.35251 0.112392607248
-1.34802 0.112188646445
-1.34353 0.111983226405
-1.33904 0.111776340011
-1.33455 0.111567980156
-1.33006 0.111358139742
-1.32557 0.111146811683
-1.32108 0.110933988906
-1.31659 0.110719664348
-1.3121 0.110503830963
-1.30761 0.110286481719
-1.30312 0.110067609598
-1.29863 0.1098472076
-1.29414 0.109625268741
-1.28965 0.109401786056
-1.28516 0.1091767526
-1.28067 0.108950161445
-1.27618 0.108722005688
-1.27169 0.108492278444
-1.2672 0.108260972854
-1.26271 0.108028082081
-1.25822 0.107793599314
-1.25373 0.107557517766
-1.24924 0.107319830681
-1.24475 0.107080531326
-1.24026 0.106839613
-1.23577 0.106597069032
-1.23128 0.106352892781
-1.22679 0.106107077639
-1.2223 0.105859617033
-1.21781 0.105610504422
-1.21332 0.105359733301
-1.20883 0.105107297204
-1.20434 0.104853189701
-1.19985 0.104597404403
-1.19536 0.104339934961
-1.19087 0.104080775066
-1.18638 0.103819918455
-1.18189 0.103557358908
-1.1774 0.10329309025
-1.17291 0.103027106354
-1.16842 0.102759401141
-1.16393 0.102489968582
-1.15944 0.102218802698
-1.15495 0.101945897563
-1.15046 0.101671247307
-1.14597 0.101394846112
-1.14148 0.101116688218
-1.13699 0.100836767924
-1.1325 0.100555079589
-1.12801 0.100271617632
-1.12352 0.099986376536
-1.11903 0.099699350848
-1.11454 0.0994105351814
-1.11005 0.099119924217
-1.10556 0.0988275127052
-1.10107 0.0985332954674
-1.09658 0.0982372673977
-1.09209 0.0979394234647
-1.0876 0.0976397587133
-1.08311 0.0973382682665
-1.07862 0.097034947327
-1.07413 0.0967297911791
-1.06964 0.096422795191
-1.06515 0.096113954816
-1.06066 0.0958032655949
-1.05617 0.0954907231578
-1.05168 0.0951763232262
-1.04719 0.0948600616149
-1.0427 0.0945419342341
-1.03821 0.0942219370913
-1.03372 0.0939000662937
-1.02923 0.0935763180504
-1.02474 0.0932506886742
-1.02025 0.092923174584
-1.01576 0.0925937723073
-1.01127 0.0922624784819
-1.00678 0.0919292898591
-1.00229 0.0915942033052
-0.9978 0.0912572158042
-0.99331 0.0909183244607
-0.98882 0.0905775265015
-0.98433 0.0902348192789
-0.97984 0.0898902002729
-0.97535 0.0895436670938
-0.97086 0.089195217485
-0.96637 0.0888448493254
-0.96188 0.0884925606325
-0.95739 0.088138349565
-0.9529 0.0877822144255
-0.94841 0.0874241536636
-0.94392 0.0870641658786
-0.93943 0.0867022498227
-0.93494 0.0863384044038
-0.93045 0.0859726286886
-0.92596 0.0856049219059
-0.92147 0.0852352834497
-0.91698 0.084863712882
-0.91249 0.0844902099368
-0.908 0.0841147745229
-0.90351 0.0837374067276
-0.89902 0.0833581068197
-0.89453 0.0829768752535
-0.89004 0.0825937126722
-0.88555 0.0822086199114
-0.88106 0.0818215980029
-0.87657 0.0814326481783
-0.87208 0.081041771873
-0.86759 0.0806489707301
-0.8631 0.080254246604
-0.85861 0.0798576015649
-0.85412 0.0794590379024
-0.84963 0.0790585581301
-0.84514 0.0786561649892
-0.84065 0.0782518614536
-0.83616 0.0778456507336
-0.83167 0.0774375362805
-0.82718 0.0770275217915
-0.82269 0.0766156112136
-0.8182 0.0762018087489
-0.81371 0.075786118859
-0.80922 0.0753685462699
-0.80473 0.074949095977
-0.80024 0.0745277732499
-0.79575 0.0741045836379
-0.79126 0.0736795329746
-0.78677 0.0732526273834
-0.78228 0.0728238732833
-0.77779 0.0723932773934
-0.7733 0.0719608467394
-0.76881 0.0715265886586
-0.76432 0.0710905108056
-0.75983 0.0706526211588
-0.75534 0.0702129280253
-0.75085 0.0697714400479
-0.74636 0.0693281662105
-0.74187 0.0688831158447
-0.73738 0.068436298636
-0.73289 0.0679877246302
-0.7284 0.06753740424
-0.72391 0.0670853482516
-0.71942 0.0666315678317
-0.71493 0.0661760745338
-0.71044 0.0657188803059
-0.70595 0.0652599974969
-0.70146 0.0647994388644
-0.69697 0.0643372175817
-0.69248 0.0638733472452
-0.68799 0.0634078418824
-0.6835 0.0629407159591
-0.67901 0.0624719843874
-0.67452 0.0620016625338
-0.67003 0.061529766227
-0.66554 0.0610563117664
-0.66105 0.0605813159301
-0.65656 0.0601047959836
-0.65207 0.0596267696884
-0.64758 0.0591472553105
-0.64309 0.0586662716296
-0.6386 0.0581838379478
-0.63411 0.0576999740987
-0.62962 0.0572147004572
-0.62513 0.0567280379482
-0.62064 0.0562400080566
-0.61615 0.055750632837
-0.61166 0.0552599349234
-0.60717 0.0547679375392
-0.60268 0.0542746645073
-0.59819 0.0537801402606
-0.5937 0.0532843898522
-0.58921 0.052787438966
-0.58472 0.0522893139277
-0.58023 0.0517900417153
-0.57574 0.0512896499703
-0.57125 0.0507881670089
-0.56676 0.0502856218334
-0.56227 0.0497820441435
-0.55778 0.0492774643481
-0.55329 0.0487719135771
-0.5488 0.0482654236931
-0.54431 0.047758027304
-0.53982 0.0472497577747
-0.53533 0.0467406492399
-0.53084 0.0462307366165
-0.52635 0.0457200556164
-0.52186 0.0452086427595
-0.51737 0.0446965353862
-0.51288 0.0441837716714
-0.50839 0.0436703906373
-0.5039 0.0431564321669
-0.49941 0.0426419370179
-0.49492 0.0421269468365
-0.49043 0.0416115041709
-0.48594 0.0410956524861
-0.48145 0.0405794361776
-0.47696 0.0400629005862
-0.47247 0.0395460920123
-0.46798 0.0390290577305
-0.46349 0.0385118460048
-0.459 0.0379945061034
-0.45451 0.0374770883138
-0.45002 0.0369596439581
-0.44553 0.0364422254084
-0.44104 0.0359248861023
-0.43655 0.0354076805588
-0.43206 0.0348906643937
-0.42757 0.034373894336
-0.42308 0.0338574282434
-0.41859 0.0333413251191
-0.4141 0.0328256451277
-0.40961 0.0323104496117
-0.40512 0.0317958011081
-0.40063 0.0312817633648
-0.39614 0.0307684013577
-0.39165 0.0302557813073
-0.38716 0.0297439706957
-0.38267 0.0292330382838
-0.37818 0.0287230541281
-0.37369 0.0282140895981
-0.3692 0.0277062173936
-0.36471 0.0271995115621
-0.36022 0.0266940475162
-0.35573 0.026189902051
-0.35124 0.0256871533617
-0.34675 0.0251858810614
-0.34226 0.0246861661986
-0.33777 0.0241880912749
-0.33328 0.0236917402628
-0.32879 0.0231971986235
-0.3243 0.0227045533247
-0.31981 0.0222138928582
-0.31532 0.0217253072582
-0.31083 0.0212388881186
-0.30634 0.0207547286113
-0.30185 0.0202729235037
-0.29736 0.0197935691766
-0.29287 0.019316763642
-0.28838 0.018842606561
-0.28389 0.0183711992613
-0.2794 0.0179026447547
-0.27491 0.0174370477553
-0.27042 0.0169745146964
-0.26593 0.0165151537484
-0.26144 0.016059074836
-0.25695 0.0156063896554
-0.25246 0.0151572116917
-0.24797 0.014711656236
-0.24348 0.0142698404023
-0.23899 0.0138318831442
-0.2345 0.0133979052717
-0.23001 0.0129680294682
-0.22552 0.012542380306
-0.22103 0.0121210842636
-0.21654 0.0117042697408
-0.21205 0.0112920670755
-0.20756 0.0108846085584
-0.20307 0.0104820284497
-0.19858 0.0100844629931
-0.19409 0.00969205043192
-0.1896 0.00930493102332
-0.18511 0.00892324705308
-0.18062 0.00854714284991
-0.17613 0.0081767647995
-0.17164 0.00781226135833
-0.16715 0.00745378306717
-0.16266 0.00710148256426
-0.15817 0.00675551459829
-0.15368 0.00641603604091
-0.14919 0.00608320589903
-0.1447 0.00575718532678
-0.14021 0.00543813763703
-0.13572 0.00512622831269
-0.13123 0.00482162501751
-0.12674 0.0045244976066
-0.12225 0.00423501813653
-0.11776 0.00395336087503
-0.11327 0.0036797023103
-0.10878 0.00341422115987
-0.10429 0.0031570983791
-0.0998 0.00290851716916
-0.09531 0.00266866298468
-0.09082 0.00243772354081
-0.08633 0.00221588881994
-0.08184 0.00200335107791
-0.07735 0.00180030484968
-0.07286 0.00160694695464
-0.06837 0.00142347650128
-0.06388 0.00125009489149
-0.05939 0.00108700582427
-0.0549 0.00093441529892
-0.05041 0.000792531617761
-0.04592 0.000661565388262
-0.04143 0.000541729524667
-0.03694 0.000433239249058
-0.03245 0.000336312091872
-0.02796 0.000251167891858
-0.02347 0.000178028795467
-0.01898 0.000117119255675
-0.01449 6.86660302318e-05


==> figuresAndData/dataForConditionalVarianceLaplaceEqualSides.tex <==
-4.5 0.537366491512
-4.49551 0.53727746771
-4.49102 0.537188038527
-4.48653 0.537098202323
-4.48204 0.537007957453
-4.47755 0.53691730227
-4.47306 0.536826235117
-4.46857 0.536734754335
-4.46408 0.53664285826
-4.45959 0.536550545219
-4.4551 0.536457813539
-4.45061 0.536364661538
-4.44612 0.536271087529
-4.44163 0.536177089823
-4.43714 0.536082666721
-4.43265 0.535987816523
-4.42816 0.535892537521
-4.42367 0.535796828002
-4.41918 0.53570068625
-4.41469 0.53560411054
-4.4102 0.535507099145
-4.40571 0.535409650331
-4.40122 0.535311762359
-4.39673 0.535213433485
-4.39224 0.53511466196
-4.38775 0.535015446028
-4.38326 0.53491578393
-4.37877 0.5348156739
-4.37428 0.534715114167
-4.36979 0.534614102955
-4.3653 0.534512638482
-4.36081 0.534410718963
-4.35632 0.534308342604
-4.35183 0.534205507608
-4.34734 0.534102212172
-4.34285 0.533998454488
-4.33836 0.533894232742
-4.33387 0.533789545116
-4.32938 0.533684389785
-4.32489 0.533578764918
-4.3204 0.533472668683
-4.31591 0.533366099236
-4.31142 0.533259054734
-4.30693 0.533151533324
-4.30244 0.53304353315
-4.29795 0.53293505235
-4.29346 0.532826089056
-4.28897 0.532716641396
-4.28448 0.532606707492
-4.27999 0.532496285459
-4.2755 0.53238537341
-4.27101 0.532273969448
-4.26652 0.532162071675
-4.26203 0.532049678186
-4.25754 0.531936787069
-4.25305 0.531823396409
-4.24856 0.531709504284
-4.24407 0.531595108767
-4.23958 0.531480207926
-4.23509 0.531364799824
-4.2306 0.531248882516
-4.22611 0.531132454055
-4.22162 0.531015512487
-4.21713 0.530898055851
-4.21264 0.530780082184
-4.20815 0.530661589515
-4.20366 0.530542575869
-4.19917 0.530423039263
-4.19468 0.530302977713
-4.19019 0.530182389225
-4.1857 0.530061271803
-4.18121 0.529939623444
-4.17672 0.529817442139
-4.17223 0.529694725875
-4.16774 0.529571472634
-4.16325 0.529447680389
-4.15876 0.529323347113
-4.15427 0.529198470768
-4.14978 0.529073049316
-4.14529 0.528947080709
-4.1408 0.528820562896
-4.13631 0.52869349382
-4.13182 0.528565871419
-4.12733 0.528437693625
-4.12284 0.528308958365
-4.11835 0.52817966356
-4.11386 0.528049807127
-4.10937 0.527919386977
-4.10488 0.527788401013
-4.10039 0.527656847137
-4.0959 0.527524723243
-4.09141 0.527392027221
-4.08692 0.527258756952
-4.08243 0.527124910317
-4.07794 0.526990485188
-4.07345 0.526855479433
-4.06896 0.526719890915
-4.06447 0.526583717489
-4.05998 0.526446957007
-4.05549 0.526309607317
-4.051 0.526171666258
-4.04651 0.526033131666
-4.04202 0.525894001372
-4.03753 0.5257542732
-4.03304 0.52561394497
-4.02855 0.525473014495
-4.02406 0.525331479586
-4.01957 0.525189338045
-4.01508 0.525046587671
-4.01059 0.524903226257
-4.0061 0.52475925159
-4.00161 0.524614661454
-3.99712 0.524469453624
-3.99263 0.524323625874
-3.98814 0.524177175969
-3.98365 0.524030101671
-3.97916 0.523882400736
-3.97467 0.523734070915
-3.97018 0.523585109954
-3.96569 0.523435515593
-3.9612 0.523285285568
-3.95671 0.523134417608
-3.95222 0.522982909437
-3.94773 0.522830758777
-3.94324 0.522677963341
-3.93875 0.522524520838
-3.93426 0.522370428973
-3.92977 0.522215685444
-3.92528 0.522060287946
-3.92079 0.521904234167
-3.9163 0.52174752179
-3.91181 0.521590148494
-3.90732 0.521432111953
-3.90283 0.521273409834
-3.89834 0.521114039801
-3.89385 0.520953999512
-3.88936 0.52079328662
-3.88487 0.520631898773
-3.88038 0.520469833613
-3.87589 0.520307088779
-3.8714 0.520143661904
-3.86691 0.519979550615
-3.86242 0.519814752536
-3.85793 0.519649265285
-3.85344 0.519483086473
-3.84895 0.519316213711
-3.84446 0.519148644599
-3.83997 0.518980376738
-3.83548 0.518811407719
-3.83099 0.518641735132
-3.8265 0.51847135656
-3.82201 0.518300269582
-3.81752 0.51812847177
-3.81303 0.517955960695
-3.80854 0.51778273392
-3.80405 0.517608789005
-3.79956 0.517434123504
-3.79507 0.517258734967
-3.79058 0.517082620939
-3.78609 0.516905778959
-3.7816 0.516728206565
-3.77711 0.516549901286
-3.77262 0.516370860648
-3.76813 0.516191082173
-3.76364 0.516010563378
-3.75915 0.515829301774
-3.75466 0.51564729487
-3.75017 0.515464540168
-3.74568 0.515281035167
-3.74119 0.515096777359
-3.7367 0.514911764235
-3.73221 0.514725993279
-3.72772 0.51453946197
-3.72323 0.514352167785
-3.71874 0.514164108195
-3.71425 0.513975280667
-3.70976 0.513785682662
-3.70527 0.513595311638
-3.70078 0.513404165049
-3.69629 0.513212240345
-3.6918 0.513019534968
-3.68731 0.512826046361
-3.68282 0.512631771959
-3.67833 0.512436709193
-3.67384 0.512240855491
-3.66935 0.512044208277
-3.66486 0.511846764969
-3.66037 0.511648522982
-3.65588 0.511449479727
-3.65139 0.51124963261
-3.6469 0.511048979034
-3.64241 0.510847516396
-3.63792 0.510645242091
-3.63343 0.510442153509
-3.62894 0.510238248036
-3.62445 0.510033523053
-3.61996 0.50982797594
-3.61547 0.509621604069
-3.61098 0.509414404811
-3.60649 0.509206375532
-3.602 0.508997513594
-3.59751 0.508787816357
-3.59302 0.508577281173
-3.58853 0.508365905395
-3.58404 0.508153686369
-3.57955 0.507940621438
-3.57506 0.507726707942
-3.57057 0.507511943217
-3.56608 0.507296324594
-3.56159 0.507079849403
-3.5571 0.506862514967
-3.55261 0.506644318609
-3.54812 0.506425257646
-3.54363 0.506205329392
-3.53914 0.505984531158
-3.53465 0.50576286025
-3.53016 0.505540313974
-3.52567 0.505316889628
-3.52118 0.505092584511
-3.51669 0.504867395915
-3.5122 0.50464132113
-3.50771 0.504414357445
-3.50322 0.504186502142
-3.49873 0.503957752502
-3.49424 0.503728105803
-3.48975 0.503497559317
-3.48526 0.503266110317
-3.48077 0.50303375607
-3.47628 0.502800493842
-3.47179 0.502566320893
-3.4673 0.502331234482
-3.46281 0.502095231866
-3.45832 0.501858310298
-3.45383 0.501620467026
-3.44934 0.501381699299
-3.44485 0.501142004361
-3.44036 0.500901379453
-3.43587 0.500659821814
-3.43138 0.500417328679
-3.42689 0.500173897283
-3.4224 0.499929524856
-3.41791 0.499684208626
-3.41342 0.499437945818
-3.40893 0.499190733655
-3.40444 0.498942569358
-3.39995 0.498693450145
-3.39546 0.498443373231
-3.39097 0.49819233583
-3.38648 0.497940335151
-3.38199 0.497687368405
-3.3775 0.497433432796
-3.37301 0.497178525529
-3.36852 0.496922643805
-3.36403 0.496665784825
-3.35954 0.496407945785
-3.35505 0.496149123881
-3.35056 0.495889316306
-3.34607 0.495628520252
-3.34158 0.495366732908
-3.33709 0.495103951462
-3.3326 0.494840173099
-3.32811 0.494575395002
-3.32362 0.494309614355
-3.31913 0.494042828337
-3.31464 0.493775034126
-3.31015 0.4935062289
-3.30566 0.493236409834
-3.30117 0.492965574101
-3.29668 0.492693718874
-3.29219 0.492420841323
-3.2877 0.492146938617
-3.28321 0.491872007924
-3.27872 0.491596046411
-3.27423 0.491319051243
-3.26974 0.491041019583
-3.26525 0.490761948594
-3.26076 0.490481835438
-3.25627 0.490200677274
-3.25178 0.489918471263
-3.24729 0.489635214562
-3.2428 0.489350904329
-3.23831 0.489065537719
-3.23382 0.488779111888
-3.22933 0.488491623991
-3.22484 0.488203071181
-3.22035 0.487913450611
-3.21586 0.487622759433
-3.21137 0.487330994799
-3.20688 0.487038153861
-3.20239 0.486744233767
-3.1979 0.486449231668
-3.19341 0.486153144714
-3.18892 0.485855970053
-3.18443 0.485557704835
-3.17994 0.485258346207
-3.17545 0.484957891317
-3.17096 0.484656337313
-3.16647 0.484353681344
-3.16198 0.484049920555
-3.15749 0.483745052096
-3.153 0.483439073113
-3.14851 0.483131980754
-3.14402 0.482823772166
-3.13953 0.482514444498
-3.13504 0.482203994897
-3.13055 0.481892420511
-3.12606 0.481579718489
-3.12157 0.48126588598
-3.11708 0.480950920133
-3.11259 0.480634818098
-3.1081 0.480317577024
-3.10361 0.479999194064
-3.09912 0.479679666367
-3.09463 0.479358991087
-3.09014 0.479037165376
-3.08565 0.478714186388
-3.08116 0.478390051277
-3.07667 0.478064757199
-3.07218 0.477738301309
-3.06769 0.477410680766
-3.0632 0.477081892728
-3.05871 0.476751934354
-3.05422 0.476420802805
-3.04973 0.476088495243
-3.04524 0.475755008831
-3.04075 0.475420340734
-3.03626 0.475084488117
-3.03177 0.474747448149
-3.02728 0.474409217998
-3.02279 0.474069794834
-3.0183 0.47372917583
-3.01381 0.47338735816
-3.00932 0.473044338999
-3.00483 0.472700115525
-3.00034 0.472354684917
-2.99585 0.472008044357
-2.99136 0.471660191027
-2.98687 0.471311122112
-2.98238 0.470960834801
-2.97789 0.470609326282
-2.9734 0.470256593748
-2.96891 0.469902634393
-2.96442 0.469547445412
-2.95993 0.469191024005
-2.95544 0.468833367373
-2.95095 0.468474472719
-2.94646 0.468114337251
-2.94197 0.467752958177
-2.93748 0.467390332708
-2.93299 0.46702645806
-2.9285 0.46666133145
-2.92401 0.466294950097
-2.91952 0.465927311226
-2.91503 0.465558412061
-2.91054 0.465188249834
-2.90605 0.464816821775
-2.90156 0.46444412512
-2.89707 0.464070157109
-2.89258 0.463694914984
-2.88809 0.46331839599
-2.8836 0.462940597375
-2.87911 0.462561516394
-2.87462 0.462181150302
-2.87013 0.461799496358
-2.86564 0.461416551827
-2.86115 0.461032313974
-2.85666 0.460646780073
-2.85217 0.460259947397
-2.84768 0.459871813225
-2.84319 0.45948237484
-2.8387 0.45909162953
-2.83421 0.458699574586
-2.82972 0.458306207302
-2.82523 0.45791152498
-2.82074 0.457515524922
-2.81625 0.457118204437
-2.81176 0.456719560838
-2.80727 0.456319591442
-2.80278 0.455918293573
-2.79829 0.455515664555
-2.7938 0.455111701721
-2.78931 0.454706402407
-2.78482 0.454299763954
-2.78033 0.453891783709
-2.77584 0.453482459021
-2.77135 0.453071787247
-2.76686 0.452659765749
-2.76237 0.452246391893
-2.75788 0.45183166305
-2.75339 0.451415576597
-2.7489 0.450998129917
-2.74441 0.450579320398
-2.73992 0.450159145432
-2.73543 0.449737602419
-2.73094 0.449314688763
-2.72645 0.448890401875
-2.72196 0.44846473917
-2.71747 0.44803769807
-2.71298 0.447609276004
-2.70849 0.447179470404
-2.704 0.446748278711
-2.69951 0.446315698371
-2.69502 0.445881726835
-2.69053 0.445446361562
-2.68604 0.445009600017
-2.68155 0.444571439671
-2.67706 0.444131878
-2.67257 0.443690912489
-2.66808 0.443248540629
-2.66359 0.442804759917
-2.6591 0.442359567856
-2.65461 0.441912961957
-2.65012 0.441464939738
-2.64563 0.441015498723
-2.64114 0.440564636443
-2.63665 0.440112350436
-2.63216 0.439658638249
-2.62767 0.439203497434
-2.62318 0.43874692555
-2.61869 0.438288920165
-2.6142 0.437829478853
-2.60971 0.437368599197
-2.60522 0.436906278786
-2.60073 0.436442515216
-2.59624 0.435977306093
-2.59175 0.435510649029
-2.58726 0.435042541644
-2.58277 0.434572981567
-2.57828 0.434101966432
-2.57379 0.433629493883
-2.5693 0.433155561574
-2.56481 0.432680167163
-2.56032 0.432203308318
-2.55583 0.431724982717
-2.55134 0.431245188044
-2.54685 0.430763921991
-2.54236 0.43028118226
-2.53787 0.429796966561
-2.53338 0.429311272613
-2.52889 0.428824098143
-2.5244 0.428335440885
-2.51991 0.427845298586
-2.51542 0.427353668999
-2.51093 0.426860549885
-2.50644 0.426365939016
-2.50195 0.425869834172
-2.49746 0.425372233142
-2.49297 0.424873133725
-2.48848 0.424372533729
-2.48399 0.423870430971
-2.4795 0.423366823277
-2.47501 0.422861708482
-2.47052 0.422355084432
-2.46603 0.421846948982
-2.46154 0.421337299996
-2.45705 0.420826135349
-2.45256 0.420313452923
-2.44807 0.419799250613
-2.44358 0.419283526323
-2.43909 0.418766277964
-2.4346 0.418247503462
-2.43011 0.41772720075
-2.42562 0.41720536777
-2.42113 0.416682002478
-2.41664 0.416157102837
-2.41215 0.415630666822
-2.40766 0.415102692418
-2.40317 0.414573177619
-2.39868 0.414042120432
-2.39419 0.413509518874
-2.3897 0.412975370971
-2.38521 0.412439674761
-2.38072 0.411902428294
-2.37623 0.411363629628
-2.37174 0.410823276833
-2.36725 0.410281367993
-2.36276 0.409737901198
-2.35827 0.409192874553
-2.35378 0.408646286172
-2.34929 0.408098134182
-2.3448 0.407548416719
-2.34031 0.406997131933
-2.33582 0.406444277985
-2.33133 0.405889853045
-2.32684 0.405333855297
-2.32235 0.404776282936
-2.31786 0.404217134169
-2.31337 0.403656407215
-2.30888 0.403094100304
-2.30439 0.402530211677
-2.2999 0.401964739591
-2.29541 0.40139768231
-2.29092 0.400829038113
-2.28643 0.400258805292
-2.28194 0.399686982149
-2.27745 0.399113566999
-2.27296 0.398538558171
-2.26847 0.397961954003
-2.26398 0.39738375285
-2.25949 0.396803953076
-2.255 0.39622255306
-2.25051 0.395639551191
-2.24602 0.395054945874
-2.24153 0.394468735525
-2.23704 0.393880918574
-2.23255 0.393291493462
-2.22806 0.392700458646
-2.22357 0.392107812594
-2.21908 0.391513553789
-2.21459 0.390917680724
-2.2101 0.390320191909
-2.20561 0.389721085866
-2.20112 0.389120361131
-2.19663 0.388518016253
-2.19214 0.387914049794
-2.18765 0.387308460332
-2.18316 0.386701246457
-2.17867 0.386092406773
-2.17418 0.385481939898
-2.16969 0.384869844466
-2.1652 0.384256119122
-2.16071 0.383640762527
-2.15622 0.383023773357
-2.15173 0.3824051503
-2.14724 0.381784892061
-2.14275 0.381162997358
-2.13826 0.380539464923
-2.13377 0.379914293506
-2.12928 0.379287481867
-2.12479 0.378659028784
-2.1203 0.37802893305
-2.11581 0.377397193472
-2.11132 0.376763808871
-2.10683 0.376128778086
-2.10234 0.375492099969
-2.09785 0.374853773389
-2.09336 0.374213797228
-2.08887 0.373572170387
-2.08438 0.372928891779
-2.07989 0.372283960335
-2.0754 0.371637375003
-2.07091 0.370989134742
-2.06642 0.370339238533
-2.06193 0.369687685369
-2.05744 0.36903447426
-2.05295 0.368379604233
-2.04846 0.367723074332
-2.04397 0.367064883616
-2.03948 0.366405031161
-2.03499 0.365743516059
-2.0305 0.365080337422
-2.02601 0.364415494374
-2.02152 0.36374898606
-2.01703 0.36308081164
-2.01254 0.362410970292
-2.00805 0.361739461212
-2.00356 0.361066283611
-1.99907 0.36039143672
-1.99458 0.359714919787
-1.99009 0.359036732077
-1.9856 0.358356872874
-1.98111 0.357675341479
-1.97662 0.356992137212
-1.97213 0.356307259411
-1.96764 0.355620707432
-1.96315 0.35493248065
-1.95866 0.354242578458
-1.95417 0.353551000268
-1.94968 0.352857745512
-1.94519 0.35216281364
-1.9407 0.351466204121
-1.93621 0.350767916444
-1.93172 0.350067950116
-1.92723 0.349366304666
-1.92274 0.348662979641
-1.91825 0.347957974608
-1.91376 0.347251289156
-1.90927 0.34654292289
-1.90478 0.34583287544
-1.90029 0.345121146454
-1.8958 0.3444077356
-1.89131 0.34369264257
-1.88682 0.342975867073
-1.88233 0.342257408842
-1.87784 0.341537267631
-1.87335 0.340815443215
-1.86886 0.340091935389
-1.86437 0.339366743974
-1.85988 0.338639868809
-1.85539 0.337911309758
-1.8509 0.337181066706
-1.84641 0.33644913956
-1.84192 0.335715528252
-1.83743 0.334980232735
-1.83294 0.334243252987
-1.82845 0.333504589008
-1.82396 0.332764240822
-1.81947 0.332022208477
-1.81498 0.331278492045
-1.81049 0.330533091623
-1.806 0.329786007332
-1.80151 0.329037239317
-1.79702 0.328286787749
-1.79253 0.327534652824
-1.78804 0.326780834763
-1.78355 0.326025333814
-1.77906 0.325268150249
-1.77457 0.324509284368
-1.77008 0.323748736497
-1.76559 0.322986506988
-1.7611 0.322222596221
-1.75661 0.321457004602
-1.75212 0.320689732567
-1.74763 0.319920780577
-1.74314 0.319150149123
-1.73865 0.318377838723
-1.73416 0.317603849926
-1.72967 0.316828183309
-1.72518 0.316050839476
-1.72069 0.315271819064
-1.7162 0.314491122738
-1.71171 0.313708751195
-1.70722 0.312924705161
-1.70273 0.312138985394
-1.69824 0.311351592683
-1.69375 0.310562527847
-1.68926 0.309771791741
-1.68477 0.308979385249
-1.68028 0.308185309288
-1.67579 0.307389564811
-1.6713 0.306592152801
-1.66681 0.305793074277
-1.66232 0.304992330291
-1.65783 0.304189921931
-1.65334 0.303385850319
-1.64885 0.302580116614
-1.64436 0.30177272201
-1.63987 0.300963667737
-1.63538 0.300152955061
-1.63089 0.299340585289
-1.6264 0.298526559762
-1.62191 0.29771087986
-1.61742 0.296893547002
-1.61293 0.296074562648
-1.60844 0.295253928294
-1.60395 0.294431645478
-1.59946 0.29360771578
-1.59497 0.292782140818
-1.59048 0.291954922255
-1.58599 0.291126061793
-1.5815 0.290295561178
-1.57701 0.289463422201
-1.57252 0.288629646695
-1.56803 0.287794236536
-1.56354 0.286957193648
-1.55905 0.286118519999
-1.55456 0.285278217603
-1.55007 0.28443628852
-1.54558 0.28359273486
-1.54109 0.282747558777
-1.5366 0.281900762478
-1.53211 0.281052348215
-1.52762 0.280202318293
-1.52313 0.279350675067
-1.51864 0.278497420941
-1.51415 0.277642558373
-1.50966 0.276786089874
-1.50517 0.275928018006
-1.50068 0.275068345388
-1.49619 0.27420707469
-1.4917 0.273344208642
-1.48721 0.272479750026
-1.48272 0.271613701684
-1.47823 0.270746066514
-1.47374 0.269876847474
-1.46925 0.26900604758
-1.46476 0.268133669908
-1.46027 0.267259717597
-1.45578 0.266384193846
-1.45129 0.265507101917
-1.4468 0.264628445136
-1.44231 0.263748226894
-1.43782 0.262866450645
-1.43333 0.261983119913
-1.42884 0.261098238285
-1.42435 0.260211809418
-1.41986 0.25932383704
-1.41537 0.258434324945
-1.41088 0.257543277
-1.40639 0.256650697145
-1.4019 0.255756589391
-1.39741 0.254860957825
-1.39292 0.253963806605
-1.38843 0.253065139971
-1.38394 0.252164962234
-1.37945 0.251263277787
-1.37496 0.250360091102
-1.37047 0.24945540673
-1.36598 0.248549229304
-1.36149 0.247641563539
-1.357 0.246732414235
-1.35251 0.245821786277
-1.34802 0.244909684635
-1.34353 0.243996114366
-1.33904 0.243081080617
-1.33455 0.242164588625
-1.33006 0.241246643716
-1.32557 0.240327251309
-1.32108 0.239406416919
-1.31659 0.238484146152
-1.3121 0.237560444713
-1.30761 0.236635318404
-1.30312 0.235708773124
-1.29863 0.234780814876
-1.29414 0.233851449762
-1.28965 0.232920683986
-1.28516 0.23198852386
-1.28067 0.231054975799
-1.27618 0.230120046327
-1.27169 0.229183742076
-1.2672 0.228246069789
-1.26271 0.227307036321
-1.25822 0.22636664864
-1.25373 0.225424913829
-1.24924 0.224481839088
-1.24475 0.223537431735
-1.24026 0.222591699208
-1.23577 0.221644649066
-1.23128 0.220696288991
-1.22679 0.219746626791
-1.2223 0.218795670399
-1.21781 0.217843427877
-1.21332 0.216889907417
-1.20883 0.215935117343
-1.20434 0.214979066112
-1.19985 0.214021762314
-1.19536 0.213063214681
-1.19087 0.212103432081
-1.18638 0.211142423521
-1.18189 0.210180198155
-1.1774 0.209216765278
-1.17291 0.208252134333
-1.16842 0.207286314911
-1.16393 0.206319316755
-1.15944 0.205351149758
-1.15495 0.204381823968
-1.15046 0.20341134959
-1.14597 0.202439736988
-1.14148 0.201466996686
-1.13699 0.200493139369
-1.1325 0.19951817589
-1.12801 0.198542117267
-1.12352 0.197564974686
-1.11903 0.196586759507
-1.11454 0.195607483261
-1.11005 0.194627157656
-1.10556 0.193645794578
-1.10107 0.192663406091
-1.09658 0.191680004445
-1.09209 0.190695602072
-1.0876 0.189710211592
-1.08311 0.188723845815
-1.07862 0.187736517743
-1.07413 0.18674824057
-1.06964 0.185759027689
-1.06515 0.184768892692
-1.06066 0.183777849372
-1.05617 0.182785911725
-1.05168 0.181793093956
-1.04719 0.180799410476
-1.0427 0.179804875911
-1.03821 0.178809505098
-1.03372 0.177813313095
-1.02923 0.176816315174
-1.02474 0.175818526833
-1.02025 0.174819963794
-1.01576 0.173820642006
-1.01127 0.172820577648
-1.00678 0.171819787132
-1.00229 0.170818287106
-0.9978 0.169816094454
-0.99331 0.168813226305
-0.98882 0.167809700029
-0.98433 0.166805533244
-0.97984 0.165800743816
-0.97535 0.164795349866
-0.97086 0.163789369769
-0.96637 0.162782822157
-0.96188 0.161775725925
-0.95739 0.160768100231
-0.9529 0.1597599645
-0.94841 0.158751338428
-0.94392 0.157742241984
-0.93943 0.156732695411
-0.93494 0.155722719233
-0.93045 0.154712334255
-0.92596 0.153701561569
-0.92147 0.152690422552
-0.91698 0.151678938876
-0.91249 0.150667132504
-0.908 0.149655025699
-0.90351 0.148642641024
-0.89902 0.147630001346
-0.89453 0.146617129837
-0.89004 0.145604049983
-0.88555 0.14459078558
-0.88106 0.143577360743
-0.87657 0.142563799906
-0.87208 0.141550127825
-0.86759 0.140536369584
-0.8631 0.139522550596
-0.85861 0.138508696607
-0.85412 0.1374948337
-0.84963 0.136480988295
-0.84514 0.135467187156
-0.84065 0.134453457396
-0.83616 0.133439826472
-0.83167 0.132426322199
-0.82718 0.131412972745
-0.82269 0.130399806637
-0.8182 0.129386852768
-0.81371 0.128374140394
-0.80922 0.127361699142
-0.80473 0.126349559011
-0.80024 0.125337750377
-0.79575 0.124326303997
-0.79126 0.123315251008
-0.78677 0.122304622935
-0.78228 0.121294451693
-0.77779 0.12028476959
-0.7733 0.119275609329
-0.76881 0.118267004017
-0.76432 0.117258987159
-0.75983 0.11625159267
-0.75534 0.115244854875
-0.75085 0.114238808511
-0.74636 0.113233488733
-0.74187 0.112228931114
-0.73738 0.111225171653
-0.73289 0.110222246776
-0.7284 0.109220193335
-0.72391 0.108219048621
-0.71942 0.107218850358
-0.71493 0.106219636711
-0.71044 0.105221446289
-0.70595 0.104224318147
-0.70146 0.103228291789
-0.69697 0.102233407174
-0.69248 0.101239704716
-0.68799 0.100247225289
-0.6835 0.0992560102288
-0.67901 0.0982661013386
-0.67452 0.0972775408896
-0.67003 0.0962903716253
-0.66554 0.0953046367645
-0.66105 0.0943203800042
-0.65656 0.0933376455228
-0.65207 0.092356477983
-0.64758 0.091376922535
-0.64309 0.0903990248191
-0.6386 0.0894228309689
-0.63411 0.0884483876142
-0.62962 0.0874757418838
-0.62513 0.086504941408
-0.62064 0.0855360343222
-0.61615 0.0845690692687
-0.61166 0.0836040954002
-0.60717 0.0826411623819
-0.60268 0.0816803203945
-0.59819 0.0807216201366
-0.5937 0.0797651128273
-0.58921 0.0788108502087
-0.58472 0.0778588845483
-0.58023 0.0769092686415
-0.57574 0.0759620558139
-0.57125 0.0750172999233
-0.56676 0.0740750553627
-0.56227 0.0731353770615
-0.55778 0.0721983204885
-0.55329 0.0712639416534
-0.5488 0.0703322971091
-0.54431 0.0694034439533
-0.53982 0.0684774398311
-0.53533 0.0675543429359
-0.53084 0.0666342120118
-0.52635 0.0657171063552
-0.52186 0.064803085816
-0.51737 0.0638922107996
-0.51288 0.0629845422683
-0.50839 0.0620801417423
-0.5039 0.0611790713017
-0.49941 0.0602813935869
-0.49492 0.0593871718006
-0.49043 0.0584964697081
-0.48594 0.0576093516388
-0.48145 0.0567258824871
-0.47696 0.0558461277128
-0.47247 0.0549701533423
-0.46798 0.0540980259688
-0.46349 0.0532298127531
-0.459 0.0523655814242
-0.45451 0.0515054002792
-0.45002 0.0506493381838
-0.44553 0.0497974645725
-0.44104 0.0489498494487
-0.43655 0.0481065633841
-0.43206 0.0472676775193
-0.42757 0.0464332635631
-0.42308 0.045603393792
-0.41859 0.0447781410499
-0.4141 0.0439575787477
-0.40961 0.0431417808621
-0.40512 0.0423308219349
-0.40063 0.0415247770723
-0.39614 0.0407237219435
-0.39165 0.0399277327796
-0.38716 0.0391368863723
-0.38267 0.0383512600723
-0.37818 0.0375709317879
-0.37369 0.0367959799832
-0.3692 0.0360264836761
-0.36471 0.0352625224363
-0.36022 0.0345041763835
-0.35573 0.0337515261847
-0.35124 0.0330046530522
-0.34675 0.0322636387407
-0.34226 0.0315285655448
-0.33777 0.0307995162958
-0.33328 0.0300765743594
-0.32879 0.0293598236319
-0.3243 0.0286493485373
-0.31981 0.0279452340234
-0.31532 0.0272475655589
-0.31083 0.026556429129
-0.30634 0.0258719112316
-0.30185 0.0251940988736
-0.29736 0.0245230795661
-0.29287 0.0238589413206
-0.28838 0.0232017726439
-0.28389 0.0225516625335
-0.2794 0.021908700473
-0.27491 0.0212729764265
-0.27042 0.0206445808338
-0.26593 0.0200236046047
-0.26144 0.0194101391137
-0.25695 0.0188042761937
-0.25246 0.0182061081307
-0.24797 0.017615727657
-0.24348 0.0170332279456
-0.23899 0.016458702603
-0.2345 0.015892245663
-0.23001 0.0153339515797
-0.22552 0.0147839152202
-0.22103 0.0142422318579
-0.21654 0.0137089971646
-0.21205 0.0131843072029
-0.20756 0.0126682584189
-0.20307 0.0121609476336
-0.19858 0.0116624720348
-0.19409 0.0111729291692
-0.1896 0.0106924169331
-0.18511 0.0102210335644
-0.18062 0.0097588776329
-0.17613 0.00930604803158
-0.17164 0.00886264396709
-0.16715 0.0084287649502
-0.16266 0.00800451078603
-0.15817 0.00758998156407
-0.15368 0.00718527764802
-0.14919 0.00679049966546
-0.1447 0.0064057484972
-0.14021 0.00603112526657
-0.13572 0.00566673132843
-0.13123 0.00531266825801
-0.12674 0.00496903783947
-0.12225 0.0046359420544
-0.11776 0.00431348306997
-0.11327 0.00400176322698
-0.10878 0.00370088502767
-0.10429 0.0034109511233
-0.0998 0.00313206430157
-0.09531 0.00286432747383
-0.09082 0.00260784366209
-0.08633 0.00236271598578
-0.08184 0.0021290476484
-0.07735 0.00190694192387
-0.07286 0.00169650214277
-0.06837 0.00149783167832
-0.06388 0.00131103393219
-0.05939 0.00113621232009
-0.0549 0.000973470257211
-0.05041 0.000822911143396
-0.04592 0.000684638348192
-0.04143 0.000558755195664
-0.03694 0.000445364949028
-0.03245 0.000344570795099
-0.02796 0.000256475828546
-0.02347 0.000181183035956
-0.01898 0.000118795279714
-0.01449 6.94152817088e-05


==> figuresAndData/dataForConditionalVarianceLaplaceLevelSets.tex <==
-4.5 0.555464043873
-4.49551 0.555462979559
-4.49102 0.555461903038
-4.48653 0.555460814172
-4.48204 0.555459712821
-4.47755 0.555458598844
-4.47306 0.555457472101
-4.46857 0.555456332446
-4.46408 0.555455179734
-4.45959 0.555454013818
-4.4551 0.55545283455
-4.45061 0.555451641779
-4.44612 0.555450435353
-4.44163 0.555449215119
-4.43714 0.555447980922
-4.43265 0.555446732603
-4.42816 0.555445470005
-4.42367 0.555444192967
-4.41918 0.555442901326
-4.41469 0.555441594919
-4.4102 0.55544027358
-4.40571 0.555438937141
-4.40122 0.555437585432
-4.39673 0.555436218283
-4.39224 0.555434835519
-4.38775 0.555433436966
-4.38326 0.555432022447
-4.37877 0.555430591782
-4.37428 0.555429144791
-4.36979 0.55542768129
-4.3653 0.555426201095
-4.36081 0.555424704019
-4.35632 0.555423189872
-4.35183 0.555421658463
-4.34734 0.5554201096
-4.34285 0.555418543086
-4.33836 0.555416958725
-4.33387 0.555415356316
-4.32938 0.555413735658
-4.32489 0.555412096547
-4.3204 0.555410438777
-4.31591 0.555408762139
-4.31142 0.555407066422
-4.30693 0.555405351413
-4.30244 0.555403616897
-4.29795 0.555401862656
-4.29346 0.555400088471
-4.28897 0.555398294117
-4.28448 0.555396479372
-4.27999 0.555394644006
-4.2755 0.55539278779
-4.27101 0.555390910493
-4.26652 0.555389011878
-4.26203 0.555387091709
-4.25754 0.555385149745
-4.25305 0.555383185745
-4.24856 0.555381199461
-4.24407 0.555379190648
-4.23958 0.555377159053
-4.23509 0.555375104424
-4.2306 0.555373026504
-4.22611 0.555370925035
-4.22162 0.555368799755
-4.21713 0.555366650399
-4.21264 0.5553644767
-4.20815 0.555362278388
-4.20366 0.55536005519
-4.19917 0.555357806828
-4.19468 0.555355533025
-4.19019 0.555353233498
-4.1857 0.555350907962
-4.18121 0.555348556128
-4.17672 0.555346177705
-4.17223 0.555343772398
-4.16774 0.55534133991
-4.16325 0.55533887994
-4.15876 0.555336392183
-4.15427 0.555333876332
-4.14978 0.555331332077
-4.14529 0.555328759102
-4.1408 0.555326157091
-4.13631 0.555323525723
-4.13182 0.555320864672
-4.12733 0.555318173612
-4.12284 0.55531545221
-4.11835 0.555312700132
-4.11386 0.555309917039
-4.10937 0.555307102589
-4.10488 0.555304256436
-4.10039 0.555301378231
-4.0959 0.555298467619
-4.09141 0.555295524244
-4.08692 0.555292547745
-4.08243 0.555289537757
-4.07794 0.55528649391
-4.07345 0.555283415834
-4.06896 0.555280303149
-4.06447 0.555277155477
-4.05998 0.555273972432
-4.05549 0.555270753625
-4.051 0.555267498663
-4.04651 0.555264207148
-4.04202 0.55526087868
-4.03753 0.555257512852
-4.03304 0.555254109254
-4.02855 0.555250667471
-4.02406 0.555247187086
-4.01957 0.555243667673
-4.01508 0.555240108806
-4.01059 0.555236510051
-4.0061 0.555232870972
-4.00161 0.555229191127
-3.99712 0.555225470069
-3.99263 0.555221707347
-3.98814 0.555217902505
-3.98365 0.555214055083
-3.97916 0.555210164614
-3.97467 0.555206230628
-3.97018 0.555202252649
-3.96569 0.555198230197
-3.9612 0.555194162785
-3.95671 0.555190049922
-3.95222 0.555185891113
-3.94773 0.555181685856
-3.94324 0.555177433644
-3.93875 0.555173133965
-3.93426 0.555168786302
-3.92977 0.555164390131
-3.92528 0.555159944924
-3.92079 0.555155450147
-3.9163 0.55515090526
-3.91181 0.555146309718
-3.90732 0.555141662969
-3.90283 0.555136964456
-3.89834 0.555132213617
-3.89385 0.555127409883
-3.88936 0.555122552679
-3.88487 0.555117641424
-3.88038 0.55511267553
-3.87589 0.555107654406
-3.8714 0.555102577451
-3.86691 0.55509744406
-3.86242 0.555092253621
-3.85793 0.555087005515
-3.85344 0.555081699118
-3.84895 0.555076333797
-3.84446 0.555070908915
-3.83997 0.555065423827
-3.83548 0.555059877882
-3.83099 0.55505427042
-3.8265 0.555048600777
-3.82201 0.55504286828
-3.81752 0.55503707225
-3.81303 0.555031212002
-3.80854 0.55502528684
-3.80405 0.555019296065
-3.79956 0.555013238968
-3.79507 0.555007114834
-3.79058 0.55500092294
-3.78609 0.554994662555
-3.7816 0.554988332942
-3.77711 0.554981933355
-3.77262 0.554975463039
-3.76813 0.554968921234
-3.76364 0.554962307171
-3.75915 0.554955620072
-3.75466 0.554948859152
-3.75017 0.554942023618
-3.74568 0.554935112667
-3.74119 0.554928125489
-3.7367 0.554921061268
-3.73221 0.554913919174
-3.72772 0.554906698373
-3.72323 0.554899398022
-3.71874 0.554892017266
-3.71425 0.554884555244
-3.70976 0.554877011087
-3.70527 0.554869383914
-3.70078 0.554861672836
-3.69629 0.554853876956
-3.6918 0.554845995367
-3.68731 0.554838027153
-3.68282 0.554829971387
-3.67833 0.554821827135
-3.67384 0.554813593451
-3.66935 0.554805269381
-3.66486 0.554796853959
-3.66037 0.554788346213
-3.65588 0.554779745157
-3.65139 0.554771049797
-3.6469 0.554762259128
-3.64241 0.554753372135
-3.63792 0.554744387793
-3.63343 0.554735305066
-3.62894 0.554726122907
-3.62445 0.554716840259
-3.61996 0.554707456054
-3.61547 0.554697969214
-3.61098 0.554688378648
-3.60649 0.554678683255
-3.602 0.554668881924
-3.59751 0.554658973529
-3.59302 0.554648956938
-3.58853 0.554638831001
-3.58404 0.554628594563
-3.57955 0.554618246451
-3.57506 0.554607785485
-3.57057 0.554597210471
-3.56608 0.554586520202
-3.56159 0.55457571346
-3.5571 0.554564789015
-3.55261 0.554553745623
-3.54812 0.554542582029
-3.54363 0.554531296964
-3.53914 0.554519889146
-3.53465 0.554508357283
-3.53016 0.554496700066
-3.52567 0.554484916176
-3.52118 0.554473004277
-3.51669 0.554460963023
-3.5122 0.554448791054
-3.50771 0.554436486994
-3.50322 0.554424049456
-3.49873 0.554411477037
-3.49424 0.55439876832
-3.48975 0.554385921875
-3.48526 0.554372936257
-3.48077 0.554359810006
-3.47628 0.554346541648
-3.47179 0.554333129695
-3.4673 0.554319572642
-3.46281 0.554305868971
-3.45832 0.554292017148
-3.45383 0.554278015622
-3.44934 0.55426386283
-3.44485 0.554249557191
-3.44036 0.554235097108
-3.43587 0.55422048097
-3.43138 0.554205707148
-3.42689 0.554190773997
-3.4224 0.554175679858
-3.41791 0.554160423052
-3.41342 0.554145001885
-3.40893 0.554129414648
-3.40444 0.554113659612
-3.39995 0.554097735032
-3.39546 0.554081639146
-3.39097 0.554065370175
-3.38648 0.55404892632
-3.38199 0.554032305768
-3.3775 0.554015506686
-3.37301 0.553998527222
-3.36852 0.553981365506
-3.36403 0.553964019653
-3.35954 0.553946487754
-3.35505 0.553928767885
-3.35056 0.553910858102
-3.34607 0.553892756442
-3.34158 0.553874460923
-3.33709 0.553855969542
-3.3326 0.553837280278
-3.32811 0.55381839109
-3.32362 0.553799299917
-3.31913 0.553780004677
-3.31464 0.553760503268
-3.31015 0.553740793568
-3.30566 0.553720873433
-3.30117 0.553700740701
-3.29668 0.553680393185
-3.29219 0.55365982868
-3.2877 0.553639044957
-3.28321 0.553618039767
-3.27872 0.553596810839
-3.27423 0.553575355878
-3.26974 0.553553672571
-3.26525 0.553531758577
-3.26076 0.553509611538
-3.25627 0.553487229068
-3.25178 0.553464608761
-3.24729 0.553441748187
-3.2428 0.553418644893
-3.23831 0.553395296401
-3.23382 0.553371700211
-3.22933 0.553347853798
-3.22484 0.553323754611
-3.22035 0.553299400078
-3.21586 0.553274787599
-3.21137 0.553249914551
-3.20688 0.553224778285
-3.20239 0.553199376127
-3.1979 0.553173705377
-3.19341 0.55314776331
-3.18892 0.553121547174
-3.18443 0.55309505419
-3.17994 0.553068281555
-3.17545 0.553041226437
-3.17096 0.553013885978
-3.16647 0.552986257293
-3.16198 0.552958337468
-3.15749 0.552930123564
-3.153 0.552901612612
-3.14851 0.552872801615
-3.14402 0.552843687548
-3.13953 0.552814267358
-3.13504 0.552784537962
-3.13055 0.552754496248
-3.12606 0.552724139076
-3.12157 0.552693463275
-3.11708 0.552662465644
-3.11259 0.552631142952
-3.1081 0.55259949194
-3.10361 0.552567509314
-3.09912 0.552535191752
-3.09463 0.552502535901
-3.09014 0.552469538375
-3.08565 0.552436195758
-3.08116 0.5524025046
-3.07667 0.552368461421
-3.07218 0.552334062707
-3.06769 0.552299304911
-3.0632 0.552264184455
-3.05871 0.552228697725
-3.05422 0.552192841076
-3.04973 0.552156610827
-3.04524 0.552120003264
-3.04075 0.552083014638
-3.03626 0.552045641167
-3.03177 0.552007879031
-3.02728 0.551969724376
-3.02279 0.551931173315
-3.0183 0.551892221921
-3.01381 0.551852866233
-3.00932 0.551813102254
-3.00483 0.551772925949
-3.00034 0.551732333247
-2.99585 0.551691320039
-2.99136 0.551649882179
-2.98687 0.551608015481
-2.98238 0.551565715724
-2.97789 0.551522978646
-2.9734 0.551479799947
-2.96891 0.551436175288
-2.96442 0.55139210029
-2.95993 0.551347570535
-2.95544 0.551302581564
-2.95095 0.551257128878
-2.94646 0.551211207936
-2.94197 0.551164814159
-2.93748 0.551117942924
-2.93299 0.551070589566
-2.9285 0.55102274938
-2.92401 0.550974417617
-2.91952 0.550925589486
-2.91503 0.550876260152
-2.91054 0.550826424739
-2.90605 0.550776078324
-2.90156 0.550725215943
-2.89707 0.550673832584
-2.89258 0.550621923195
-2.88809 0.550569482676
-2.8836 0.55051650588
-2.87911 0.550462987618
-2.87462 0.550408922653
-2.87013 0.550354305701
-2.86564 0.550299131431
-2.86115 0.550243394468
-2.85666 0.550187089385
-2.85217 0.550130210709
-2.84768 0.550072752921
-2.84319 0.55001471045
-2.8387 0.549956077677
-2.83421 0.549896848935
-2.82972 0.549837018505
-2.82523 0.54977658062
-2.82074 0.549715529463
-2.81625 0.549653859163
-2.81176 0.549591563801
-2.80727 0.549528637404
-2.80278 0.54946507395
-2.79829 0.549400867362
-2.7938 0.549336011512
-2.78931 0.549270500217
-2.78482 0.549204327243
-2.78033 0.5491374863
-2.77584 0.549069971045
-2.77135 0.549001775081
-2.76686 0.548932891953
-2.76237 0.548863315155
-2.75788 0.548793038122
-2.75339 0.548722054233
-2.7489 0.548650356812
-2.74441 0.548577939126
-2.73992 0.548504794381
-2.73543 0.548430915731
-2.73094 0.548356296267
-2.72645 0.548280929025
-2.72196 0.548204806978
-2.71747 0.548127923044
-2.71298 0.548050270078
-2.70849 0.547971840876
-2.704 0.547892628175
-2.69951 0.547812624647
-2.69502 0.547731822906
-2.69053 0.547650215503
-2.68604 0.547567794927
-2.68155 0.547484553604
-2.67706 0.547400483897
-2.67257 0.547315578105
-2.66808 0.547229828465
-2.66359 0.547143227148
-2.6591 0.547055766259
-2.65461 0.546967437841
-2.65012 0.54687823387
-2.64563 0.546788146254
-2.64114 0.546697166838
-2.63665 0.546605287398
-2.63216 0.546512499643
-2.62767 0.546418795213
-2.62318 0.546324165684
-2.61869 0.546228602558
-2.6142 0.546132097273
-2.60971 0.546034641193
-2.60522 0.545936225616
-2.60073 0.545836841767
-2.59624 0.545736480802
-2.59175 0.545635133805
-2.58726 0.545532791788
-2.58277 0.545429445692
-2.57828 0.545325086384
-2.57379 0.545219704661
-2.5693 0.545113291243
-2.56481 0.545005836779
-2.56032 0.544897331843
-2.55583 0.544787766933
-2.55134 0.544677132474
-2.54685 0.544565418815
-2.54236 0.544452616228
-2.53787 0.544338714909
-2.53338 0.544223704978
-2.52889 0.544107576477
-2.5244 0.543990319371
-2.51991 0.543871923546
-2.51542 0.54375237881
-2.51093 0.543631674892
-2.50644 0.543509801441
-2.50195 0.543386748027
-2.49746 0.54326250414
-2.49297 0.543137059188
-2.48848 0.543010402499
-2.48399 0.542882523318
-2.4795 0.54275341081
-2.47501 0.542623054057
-2.47052 0.542491442056
-2.46603 0.542358563723
-2.46154 0.54222440789
-2.45705 0.542088963306
-2.45256 0.541952218631
-2.44807 0.541814162446
-2.44358 0.541674783241
-2.43909 0.541534069425
-2.4346 0.541392009318
-2.43011 0.541248591154
-2.42562 0.54110380308
-2.42113 0.540957633155
-2.41664 0.54081006935
-2.41215 0.540661099551
-2.40766 0.54051071155
-2.40317 0.540358893053
-2.39868 0.540205631676
-2.39419 0.540050914947
-2.3897 0.539894730299
-2.38521 0.539737065079
-2.38072 0.539577906541
-2.37623 0.539417241847
-2.37174 0.539255058067
-2.36725 0.539091342181
-2.36276 0.538926081075
-2.35827 0.53875926154
-2.35378 0.538590870277
-2.34929 0.538420893891
-2.3448 0.538249318894
-2.34031 0.538076131704
-2.33582 0.537901318642
-2.33133 0.537724865935
-2.32684 0.537546759716
-2.32235 0.537366986019
-2.31786 0.537185530785
-2.31337 0.537002379855
-2.30888 0.536817518977
-2.30439 0.536630933798
-2.2999 0.536442609869
-2.29541 0.536252532645
-2.29092 0.536060687479
-2.28643 0.535867059628
-2.28194 0.535671634251
-2.27745 0.535474396404
-2.27296 0.535275331047
-2.26847 0.535074423039
-2.26398 0.534871657139
-2.25949 0.534667018007
-2.255 0.5344604902
-2.25051 0.534252058176
-2.24602 0.53404170629
-2.24153 0.533829418799
-2.23704 0.533615179855
-2.23255 0.53339897351
-2.22806 0.533180783712
-2.22357 0.532960594309
-2.21908 0.532738389046
-2.21459 0.532514151563
-2.2101 0.532287865399
-2.20561 0.53205951399
-2.20112 0.531829080667
-2.19663 0.53159654866
-2.19214 0.531361901092
-2.18765 0.531125120985
-2.18316 0.530886191255
-2.17867 0.530645094715
-2.17418 0.530401814072
-2.16969 0.53015633193
-2.1652 0.529908630789
-2.16071 0.529658693041
-2.15622 0.529406500977
-2.15173 0.52915203678
-2.14724 0.528895282531
-2.14275 0.528636220202
-2.13826 0.528374831663
-2.13377 0.528111098678
-2.12928 0.527845002905
-2.12479 0.527576525896
-2.1203 0.5273056491
-2.11581 0.527032353859
-2.11132 0.526756621409
-2.10683 0.526478432882
-2.10234 0.526197769305
-2.09785 0.525914611597
-2.09336 0.525628940575
-2.08887 0.525340736948
-2.08438 0.525049981322
-2.07989 0.524756654198
-2.0754 0.524460735969
-2.07091 0.524162206927
-2.06642 0.523861047257
-2.06193 0.523557237039
-2.05744 0.52325075625
-2.05295 0.522941584763
-2.04846 0.522629702345
-2.04397 0.522315088661
-2.03948 0.521997723271
-2.03499 0.521677585631
-2.0305 0.521354655096
-2.02601 0.521028910916
-2.02152 0.520700332239
-2.01703 0.520368898111
-2.01254 0.520034587475
-2.00805 0.519697379173
-2.00356 0.519357251946
-1.99907 0.519014184431
-1.99458 0.518668155167
-1.99009 0.518319142593
-1.9856 0.517967125046
-1.98111 0.517612080764
-1.97662 0.517253987888
-1.97213 0.516892824458
-1.96764 0.516528568417
-1.96315 0.516161197609
-1.95866 0.515790689783
-1.95417 0.51541702259
-1.94968 0.515040173586
-1.94519 0.51466012023
-1.9407 0.514276839888
-1.93621 0.513890309831
-1.93172 0.513500507235
-1.92723 0.513107409186
-1.92274 0.512710992676
-1.91825 0.512311234606
-1.91376 0.511908111787
-1.90927 0.511501600937
-1.90478 0.511091678688
-1.90029 0.510678321584
-1.8958 0.510261506078
-1.89131 0.509841208539
-1.88682 0.509417405249
-1.88233 0.508990072407
-1.87784 0.508559186124
-1.87335 0.508124722433
-1.86886 0.50768665728
-1.86437 0.507244966534
-1.85988 0.506799625981
-1.85539 0.506350611329
-1.8509 0.505897898209
-1.84641 0.505441462174
-1.84192 0.504981278702
-1.83743 0.504517323196
-1.83294 0.504049570985
-1.82845 0.503577997328
-1.82396 0.503102577411
-1.81947 0.502623286352
-1.81498 0.5021400992
-1.81049 0.501652990936
-1.806 0.501161936478
-1.80151 0.500666910678
-1.79702 0.500167888326
-1.79253 0.49966484415
-1.78804 0.499157752818
-1.78355 0.498646588942
-1.77906 0.498131327074
-1.77457 0.497611941714
-1.77008 0.497088407307
-1.76559 0.496560698246
-1.7611 0.496028788874
-1.75661 0.495492653486
-1.75212 0.494952266331
-1.74763 0.494407601611
-1.74314 0.493858633488
-1.73865 0.493305336079
-1.73416 0.492747683465
-1.72967 0.492185649689
-1.72518 0.491619208758
-1.72069 0.491048334645
-1.7162 0.490473001293
-1.71171 0.489893182615
-1.70722 0.489308852499
-1.70273 0.488719984804
-1.69824 0.488126553369
-1.69375 0.487528532014
-1.68926 0.486925894536
-1.68477 0.48631861472
-1.68028 0.485706666337
-1.67579 0.485090023145
-1.6713 0.484468658895
-1.66681 0.483842547332
-1.66232 0.483211662194
-1.65783 0.482575977222
-1.65334 0.481935466156
-1.64885 0.481290102741
-1.64436 0.480639860727
-1.63987 0.479984713877
-1.63538 0.479324635962
-1.63089 0.478659600771
-1.6264 0.477989582111
-1.62191 0.477314553807
-1.61742 0.47663448971
-1.61293 0.475949363698
-1.60844 0.475259149677
-1.60395 0.474563821588
-1.59946 0.473863353406
-1.59497 0.473157719147
-1.59048 0.472446892868
-1.58599 0.471730848671
-1.5815 0.471009560709
-1.57701 0.470283003187
-1.57252 0.469551150363
-1.56803 0.468813976558
-1.56354 0.468071456153
-1.55905 0.467323563597
-1.55456 0.466570273406
-1.55007 0.465811560174
-1.54558 0.465047398567
-1.54109 0.464277763336
-1.5366 0.463502629315
-1.53211 0.462721971426
-1.52762 0.461935764684
-1.52313 0.461143984202
-1.51864 0.460346605191
-1.51415 0.459543602968
-1.50966 0.458734952957
-1.50517 0.457920630696
-1.50068 0.457100611839
-1.49619 0.456274872163
-1.4917 0.455443387568
-1.48721 0.454606134086
-1.48272 0.453763087881
-1.47823 0.452914225256
-1.47374 0.45205952266
-1.46925 0.451198956687
-1.46476 0.450332504084
-1.46027 0.449460141755
-1.45578 0.448581846766
-1.45129 0.447697596349
-1.4468 0.446807367908
-1.44231 0.445911139024
-1.43782 0.445008887458
-1.43333 0.444100591157
-1.42884 0.44318622826
-1.42435 0.442265777102
-1.41986 0.44133921622
-1.41537 0.440406524357
-1.41088 0.439467680468
-1.40639 0.438522663726
-1.4019 0.437571453527
-1.39741 0.436614029493
-1.39292 0.435650371482
-1.38843 0.434680459589
-1.38394 0.433704274156
-1.37945 0.432721795773
-1.37496 0.431733005288
-1.37047 0.430737883809
-1.36598 0.429736412714
-1.36149 0.428728573651
-1.357 0.42771434855
-1.35251 0.426693719627
-1.34802 0.425666669386
-1.34353 0.424633180632
-1.33904 0.423593236471
-1.33455 0.422546820321
-1.33006 0.421493915914
-1.32557 0.420434507304
-1.32108 0.419368578877
-1.31659 0.41829611535
-1.3121 0.417217101783
-1.30761 0.416131523585
-1.30312 0.415039366519
-1.29863 0.413940616707
-1.29414 0.412835260642
-1.28965 0.41172328519
-1.28516 0.410604677598
-1.28067 0.4094794255
-1.27618 0.408347516929
-1.27169 0.407208940314
-1.2672 0.406063684498
-1.26271 0.404911738737
-1.25822 0.403753092711
-1.25373 0.402587736529
-1.24924 0.401415660737
-1.24475 0.400236856327
-1.24026 0.399051314742
-1.23577 0.397859027882
-1.23128 0.396659988116
-1.22679 0.395454188285
-1.2223 0.394241621711
-1.21781 0.393022282205
-1.21332 0.391796164075
-1.20883 0.390563262131
-1.20434 0.389323571695
-1.19985 0.388077088608
-1.19536 0.386823809237
-1.19087 0.385563730486
-1.18638 0.384296849797
-1.18189 0.383023165165
-1.1774 0.381742675142
-1.17291 0.380455378846
-1.16842 0.379161275968
-1.16393 0.377860366781
-1.15944 0.376552652149
-1.15495 0.375238133531
-1.15046 0.373916812996
-1.14597 0.372588693222
-1.14148 0.371253777512
-1.13699 0.3699120698
-1.1325 0.368563574657
-1.12801 0.367208297301
-1.12352 0.365846243606
-1.11903 0.364477420107
-1.11454 0.363101834015
-1.11005 0.361719493216
-1.10556 0.360330406289
-1.10107 0.358934582507
-1.09658 0.357532031849
-1.09209 0.356122765009
-1.0876 0.354706793402
-1.08311 0.353284129174
-1.07862 0.351854785211
-1.07413 0.350418775146
-1.06964 0.34897611337
-1.06515 0.347526815038
-1.06066 0.346070896077
-1.05617 0.3446083732
-1.05168 0.343139263908
-1.04719 0.341663586502
-1.0427 0.340181360093
-1.03821 0.338692604606
-1.03372 0.337197340794
-1.02923 0.335695590242
-1.02474 0.33418737538
-1.02025 0.332672719489
-1.01576 0.331151646709
-1.01127 0.32962418205
-1.00678 0.328090351399
-1.00229 0.326550181531
-0.9978 0.325003700113
-0.99331 0.323450935719
-0.98882 0.321891917832
-0.98433 0.320326676859
-0.97984 0.318755244134
-0.97535 0.317177651932
-0.97086 0.315593933473
-0.96637 0.314004122934
-0.96188 0.312408255454
-0.95739 0.310806367146
-0.9529 0.309198495106
-0.94841 0.307584677417
-0.94392 0.305964953162
-0.93943 0.304339362431
-0.93494 0.302707946328
-0.93045 0.301070746983
-0.92596 0.299427807556
-0.92147 0.297779172249
-0.91698 0.296124886314
-0.91249 0.294464996058
-0.908 0.292799548855
-0.90351 0.291128593153
-0.89902 0.289452178482
-0.89453 0.287770355462
-0.89004 0.286083175811
-0.88555 0.284390692356
-0.88106 0.282692959035
-0.87657 0.280990030911
-0.87208 0.279281964177
-0.86759 0.277568816164
-0.8631 0.275850645349
-0.85861 0.274127511366
-0.85412 0.272399475006
-0.84963 0.270666598233
-0.84514 0.268928944187
-0.84065 0.267186577192
-0.83616 0.265439562765
-0.83167 0.263687967622
-0.82718 0.261931859687
-0.82269 0.260171308096
-0.8182 0.258406383207
-0.81371 0.256637156608
-0.80922 0.254863701121
-0.80473 0.253086090811
-0.80024 0.251304400993
-0.79575 0.249518708235
-0.79126 0.247729090373
-0.78677 0.245935626508
-0.78228 0.24413839702
-0.77779 0.24233748357
-0.7733 0.240532969108
-0.76881 0.23872493788
-0.76432 0.236913475432
-0.75983 0.235098668619
-0.75534 0.233280605608
-0.75085 0.231459375887
-0.74636 0.229635070266
-0.74187 0.227807780889
-0.73738 0.225977601235
-0.73289 0.224144626123
-0.7284 0.222308951721
-0.72391 0.22047067555
-0.71942 0.218629896486
-0.71493 0.216786714768
-0.71044 0.214941232004
-0.70595 0.213093551171
-0.70146 0.211243776624
-0.69697 0.209392014101
-0.69248 0.207538370721
-0.68799 0.205682954996
-0.6835 0.203825876832
-0.67901 0.20196724753
-0.67452 0.200107179795
-0.67003 0.198245787736
-0.66554 0.196383186872
-0.66105 0.194519494132
-0.65656 0.192654827864
-0.65207 0.190789307831
-0.64758 0.18892305522
-0.64309 0.187056192642
-0.6386 0.185188844135
-0.63411 0.183321135168
-0.62962 0.18145319264
-0.62513 0.179585144885
-0.62064 0.177717121676
-0.61615 0.175849254222
-0.61166 0.173981675172
-0.60717 0.172114518618
-0.60268 0.170247920096
-0.59819 0.168382016585
-0.5937 0.16651694651
-0.58921 0.164652849745
-0.58472 0.162789867608
-0.58023 0.160928142869
-0.57574 0.159067819743
-0.57125 0.157209043896
-0.56676 0.155351962444
-0.56227 0.15349672395
-0.55778 0.151643478426
-0.55329 0.149792377335
-0.5488 0.147943573586
-0.54431 0.146097221534
-0.53982 0.144253476982
-0.53533 0.142412497178
-0.53084 0.140574440814
-0.52635 0.138739468025
-0.52186 0.136907740384
-0.51737 0.135079420906
-0.51288 0.133254674041
-0.50839 0.131433665676
-0.5039 0.129616563129
-0.49941 0.127803535148
-0.49492 0.125994751909
-0.49043 0.12419038501
-0.48594 0.122390607473
-0.48145 0.120595593736
-0.47696 0.118805519653
-0.47247 0.117020562486
-0.46798 0.115240900908
-0.46349 0.11346671499
-0.459 0.111698186206
-0.45451 0.109935497421
-0.45002 0.108178832892
-0.44553 0.106428378259
-0.44104 0.104684320542
-0.43655 0.102946848137
-0.43206 0.101216150808
-0.42757 0.0994924196831
-0.42308 0.0977758472487
-0.41859 0.096066627343
-0.4141 0.0943649551501
-0.40961 0.0926710271938
-0.40512 0.0909850413314
-0.40063 0.0893071967462
-0.39614 0.0876376939416
-0.39165 0.0859767347334
-0.38716 0.0843245222427
-0.38267 0.0826812608889
-0.37818 0.0810471563812
-0.37369 0.079422415712
-0.3692 0.0778072471478
-0.36471 0.0762018602219
-0.36022 0.0746064657255
-0.35573 0.0730212756996
-0.35124 0.071446503426
-0.34675 0.0698823634185
-0.34226 0.0683290714142
-0.33777 0.0667868443638
-0.33328 0.0652559004222
-0.32879 0.0637364589396
-0.3243 0.0622287404508
-0.31981 0.0607329666661
-0.31532 0.0592493604607
-0.31083 0.0577781458646
-0.30634 0.0563195480525
-0.30185 0.0548737933324
-0.29736 0.0534411091358
-0.29287 0.0520217240062
-0.28838 0.050615867588
-0.28389 0.0492237706157
-0.2794 0.047845664902
-0.27491 0.0464817833265
-0.27042 0.0451323598242
-0.26593 0.043797629373
-0.26144 0.0424778279826
-0.25695 0.0411731926814
-0.25246 0.0398839615048
-0.24797 0.0386103734827
-0.24348 0.0373526686265
-0.23899 0.0361110879169
-0.2345 0.0348858732907
-0.23001 0.0336772676279
-0.22552 0.0324855147383
-0.22103 0.0313108593487
-0.21654 0.0301535470892
-0.21205 0.0290138244795
-0.20756 0.0278919389157
-0.20307 0.0267881386559
-0.19858 0.0257026728071
-0.19409 0.0246357913103
-0.1896 0.023587744927
-0.18511 0.0225587852247
-0.18062 0.0215491645626
-0.17613 0.020559136077
-0.17164 0.0195889536669
-0.16715 0.0186388719792
-0.16266 0.017709146394
-0.15817 0.0168000330096
-0.15368 0.0159117886279
-0.14919 0.0150446707386
-0.1447 0.0141989375048
-0.14021 0.0133748477476
-0.13572 0.0125726609302
-0.13123 0.0117926371433
-0.12674 0.0110350370892
-0.12225 0.0103001220662
-0.11776 0.00958815395302
-0.11327 0.00889939519339
-0.10878 0.00823410877986
-0.10429 0.00759255823822
-0.0998 0.00697500761153
-0.09531 0.00638172144422
-0.09082 0.00581296476607
-0.08633 0.00526900307614
-0.08184 0.0047501023267
-0.07735 0.00425652890705
-0.07286 0.00378854962737
-0.06837 0.00334643170247
-0.06388 0.00293044273552
-0.05939 0.00254085070176
-0.0549 0.00217792393218
-0.05041 0.00184193109715
-0.04592 0.00153314119005
-0.04143 0.00125182351088
-0.03694 0.000998247649787
-0.03245 0.000772683470709
-0.02796 0.000575401094871
-0.02347 0.00040667088435
-0.01898 0.000266763425611
-0.01449 0.000155949513046


==> figuresAndData/dataForConditionalVarianceLaplaceMeanZero.tex <==
-4.5 0.157771599304
-4.49551 0.157688354544
-4.49102 0.15760515424
-4.48653 0.157813152836
-4.48204 0.157729587149
-4.47755 0.157646066144
-4.47306 0.157852950183
-4.46857 0.157769064199
-4.46408 0.157685223122
-4.45959 0.15760142699
-4.4551 0.157806783657
-4.45061 0.157722623139
-4.44612 0.157638507792
-4.44163 0.157842743529
-4.43714 0.157758264202
-4.43265 0.157673830271
-4.42816 0.157589441773
-4.42367 0.157792144362
-4.41918 0.157707392479
-4.41469 0.157622686254
-4.4102 0.157824261706
-4.40571 0.157739192506
-4.40122 0.157654169187
-4.39673 0.157854614364
-4.39224 0.157769228481
-4.38775 0.157683888701
-4.38326 0.157598595062
-4.37877 0.157797498572
-4.37428 0.157711842966
-4.36979 0.157626233722
-4.3653 0.157824000984
-4.36081 0.157738030186
-4.35632 0.157652105971
-4.35183 0.15784873396
-4.34734 0.157762448604
-4.34285 0.157676210052
-4.33836 0.157590018337
-4.33387 0.157785096497
-4.32938 0.15769854424
-4.32489 0.157612039039
-4.3204 0.157805972176
-4.31591 0.157719106846
-4.31142 0.157632288791
-4.30693 0.157825073984
-4.30244 0.157737896215
-4.29795 0.157650765936
-4.29346 0.1578424003
-4.28897 0.15775491072
-4.28448 0.157667468847
-4.27999 0.157580074712
-4.2755 0.157770148769
-4.27101 0.157682395929
-4.26652 0.15759469104
-4.26203 0.157783608795
-4.25754 0.157695545615
-4.25305 0.157607530598
-4.24856 0.157795289265
-4.24407 0.157706916368
-4.23958 0.157618591845
-4.23509 0.157805188668
-4.2306 0.157716506677
-4.22611 0.157627873268
-4.22162 0.157813305521
-4.21713 0.157724315055
-4.21264 0.157635373379
-4.20815 0.157819638368
-4.20366 0.157730340043
-4.19917 0.157641090713
-4.19468 0.157824185773
-4.19019 0.157734580203
-4.1857 0.157645023829
-4.18121 0.157826946325
-4.17672 0.157737034118
-4.17223 0.157647171309
-4.16774 0.157827918632
-4.16325 0.157737700394
-4.15876 0.157647531752
-4.15427 0.157827101322
-4.14978 0.157736577654
-4.14529 0.157646103779
-4.1408 0.157824493043
-4.13631 0.157733664542
-4.13182 0.157642886026
-4.12733 0.157820092458
-4.12284 0.157728959714
-4.11835 0.157637877147
-4.11386 0.157813898246
-4.10937 0.157722461845
-4.10488 0.15763107581
-4.10039 0.157805909099
-4.0959 0.157714169622
-4.09141 0.157622480694
-4.08692 0.157796123724
-4.08243 0.157704081742
-4.07794 0.157612090492
-4.07345 0.157784540835
-4.06896 0.157692196916
-4.06447 0.157599903907
-4.05998 0.157771159159
-4.05549 0.15767851386
-4.051 0.157585919648
-4.04651 0.157755977427
-4.04202 0.157663031301
-4.03753 0.157570136432
-4.03304 0.157738994378
-4.02855 0.157645747967
-4.02406 0.157552552982
-4.01957 0.157720208755
-4.01508 0.157626662594
-4.01059 0.15779351643
-4.0061 0.157699619304
-4.00161 0.157605773915
-3.99712 0.157771420764
-3.99263 0.157677224768
-3.98814 0.157583080668
-3.98365 0.15774751825
-3.97916 0.157653023893
-3.97467 0.157558581585
-3.97018 0.157721807639
-3.96569 0.157627015419
-3.9612 0.157789429612
-3.95671 0.15769428768
-3.95222 0.157599198082
-3.94773 0.157760396086
-3.94324 0.15766495711
-3.93875 0.15756957061
-3.93426 0.157729550216
-3.92977 0.157633814664
-3.92528 0.157792975153
-3.92079 0.157696890736
-3.9163 0.157600859059
-3.91181 0.157758796594
-3.90732 0.157662416367
-3.90283 0.157566089005
-3.89834 0.157722801422
-3.89385 0.157626125815
-3.88936 0.15778201202
-3.88487 0.157684988342
-3.88038 0.15758801777
-3.87589 0.157742674393
-3.8714 0.15764535604
-3.86691 0.157548090902
-3.86242 0.157701515819
-3.85793 0.15760390318
-3.85344 0.157756494938
-3.84895 0.157658534957
-3.84446 0.157560628404
-3.83997 0.157711984072
-3.83548 0.15761373044
-3.83099 0.157764248376
-3.8265 0.157665647814
-3.82201 0.157567100872
-3.81752 0.157716378384
-3.81303 0.157617484757
-3.80854 0.157765920022
-3.80405 0.157666679845
-3.79956 0.157567493463
-3.79507 0.157714684013
-3.79058 0.157615151306
-3.78609 0.157515672459
-3.7816 0.157661616238
-3.77711 0.157561791276
-3.77262 0.157706886149
-3.76813 0.157606715188
-3.76364 0.157750958939
-3.75915 0.157650442089
-3.75466 0.157549979314
-3.75017 0.15769296988
-3.74568 0.157592161394
-3.74119 0.157734296468
-3.7367 0.157633142367
-3.73221 0.157532042445
-3.72772 0.157672920143
-3.72323 0.157571474758
-3.71874 0.157711492638
-3.71425 0.157609701868
-3.70976 0.157507965356
-3.70527 0.15764672169
-3.70078 0.157544639917
-3.69629 0.157682532142
-3.6918 0.157580105171
-3.68731 0.157717131148
-3.68282 0.157614359033
-3.67833 0.157511641267
-3.67384 0.157647399423
-3.66935 0.157544336595
-3.66486 0.157679224262
-3.66037 0.157575816407
-3.65588 0.157709831474
-3.65139 0.157606078619
-3.6469 0.157502380144
-3.64241 0.15763512115
-3.63792 0.157531077711
-3.63343 0.157662941916
-3.62894 0.157558553519
-3.62445 0.157689538837
-3.61996 0.157584805477
-3.61547 0.157480126465
-3.61098 0.157609831494
-3.60649 0.157504807505
-3.602 0.157633629477
-3.59751 0.157528260484
-3.59302 0.15765619733
-3.58853 0.157550483295
-3.58404 0.157677532955
-3.57955 0.15757147383
-3.57506 0.157465468928
-3.57057 0.157591229978
-3.56608 0.1574848799
-3.56159 0.157609749622
-3.5571 0.157503054294
-3.55261 0.15762703064
-3.54812 0.157519989975
-3.54363 0.157643070905
-3.53914 0.157535684805
-3.53465 0.157657868281
-3.53016 0.157550136637
-3.52567 0.157442458906
-3.52118 0.157563343319
-3.51669 0.157455319859
-3.5122 0.157575302687
-3.50771 0.157466933357
-3.50322 0.15758601257
-3.49873 0.157477297217
-3.49424 0.157595470787
-3.48975 0.157486409243
-3.48526 0.157603675144
-3.48077 0.157494267231
-3.47628 0.157610623438
-3.47179 0.157500868962
-3.4673 0.157616313453
-3.46281 0.157506212205
-3.45832 0.157620742959
-3.45383 0.157510294717
-3.44934 0.157399899513
-3.44485 0.157513114239
-3.44036 0.157402371671
-3.43587 0.157514668497
-3.43138 0.157403578303
-3.42689 0.1575149552
-3.4224 0.157403517105
-3.41791 0.157513972044
-3.41342 0.157402185751
-3.40893 0.157511716701
-3.40444 0.157399581902
-3.39995 0.157508186829
-3.39546 0.157395703196
-3.39097 0.157503380065
-3.38648 0.157390547253
-3.38199 0.157497294025
-3.3775 0.157384111671
-3.37301 0.157489926302
-3.36852 0.157376394025
-3.36403 0.15748127447
-3.35954 0.15736739187
-3.35505 0.157471336077
-3.35056 0.157357102734
-3.34607 0.157460108647
-3.34158 0.157345524122
-3.33709 0.157447589678
-3.3326 0.157332653513
-3.32811 0.157433776644
-3.32362 0.157318488357
-3.31913 0.157418666988
-3.31464 0.157518301923
-3.31015 0.157402258126
-3.30566 0.157500944633
-3.30117 0.157384547446
-3.29668 0.157482283436
-3.29219 0.157365532303
-3.2877 0.157462315677
-3.28321 0.157345210021
-3.27872 0.157441038673
-3.27423 0.157323577892
-3.26974 0.157418449704
-3.26525 0.157300633173
-3.26076 0.157394546016
-3.25627 0.157276373085
-3.25178 0.157369324821
-3.24729 0.157461718344
-3.2428 0.157342783292
-3.23831 0.157434211721
-3.23382 0.157314918565
-3.22933 0.157405379735
-3.22484 0.157285727736
-3.22035 0.157375219469
-3.21586 0.157255207862
-3.21137 0.157343727966
-3.20688 0.157223355957
-3.20239 0.157310902224
-3.1979 0.157397879488
-3.19341 0.157276739199
-3.18892 0.157362738563
-3.18443 0.157241235801
-3.17994 0.157326255025
-3.17545 0.157204388895
-3.17096 0.157288425719
-3.16647 0.157371886426
-3.16198 0.157249247445
-3.15749 0.157331721626
-3.153 0.157208716951
-3.14851 0.157290202308
-3.14402 0.157166830936
-3.13953 0.15724732515
-3.13504 0.157327236117
-3.13055 0.157203086775
-3.12606 0.157282002399
-3.12157 0.157157483755
-3.11708 0.157235401668
-3.11259 0.157312731044
-3.1081 0.157187430417
-3.10361 0.157263757821
-3.09912 0.157138085079
-3.09463 0.157213408093
-3.09014 0.157087362029
-3.08565 0.157161678209
-3.08116 0.157235398661
-3.07667 0.157108564456
-3.07218 0.157181273713
-3.06769 0.157253383796
-3.0632 0.157125758617
-3.05871 0.157196853101
-3.05422 0.157068849504
-3.04973 0.157138925851
-3.04524 0.157208397661
-3.04075 0.15707959808
-3.03626 0.157148047265
-3.03177 0.157018865753
-3.02728 0.157086289706
-3.02279 0.157153103722
-3.0183 0.157023120847
-3.01381 0.157088905051
-3.00932 0.157154075827
-3.00483 0.157023288187
-3.00034 0.157087424515
-2.99585 0.156956248809
-2.99136 0.157019347964
-2.98687 0.157081828217
-2.98238 0.15694984174
-2.97789 0.157011280078
-2.9734 0.157072095981
-2.96891 0.156939294943
-2.96442 0.156999064123
-2.95993 0.157058207317
-2.95544 0.156924587775
-2.95095 0.156982679371
-2.94646 0.15704014141
-2.94197 0.156905699264
-2.93748 0.156962104759
-2.93299 0.157017877104
-2.9285 0.156882608092
-2.92401 0.156937318872
-2.91952 0.156991392887
-2.91503 0.156855292577
-2.91054 0.156908299927
-2.90605 0.156960666871
-2.90156 0.156823730663
-2.89707 0.15687502576
-2.89258 0.156925676782
-2.88809 0.156787899897
-2.8836 0.156837473804
-2.87911 0.15688639994
-2.87462 0.156747777418
-2.87013 0.156795621081
-2.86564 0.156842813244
-2.86115 0.156703339935
-2.85666 0.156749444175
-2.85217 0.156794893153
-2.84768 0.156654563717
-2.84319 0.156698919223
-2.8387 0.15674261567
-2.83421 0.156785651463
-2.82972 0.156644021895
-2.82523 0.156685956328
-2.82074 0.156727226262
-2.81625 0.156584727375
-2.81176 0.156624890165
-2.80727 0.156664384572
-2.80278 0.156703208981
-2.79829 0.156559391713
-2.7938 0.156597100771
-2.78931 0.156634135893
-2.78482 0.15667049545
-2.78033 0.156525348703
-2.77584 0.156560584511
-2.77135 0.15659514076
-2.76686 0.156449101662
-2.76237 0.156482527961
-2.75788 0.156515270658
-2.75339 0.156547328097
-2.7489 0.15639993879
-2.74441 0.156430857514
-2.73992 0.156461086872
-2.73543 0.156490625193
-2.73094 0.156341873095
-2.72645 0.156370263715
-2.72196 0.15639795912
-2.71747 0.156424957622
-2.71298 0.156451257526
-2.70849 0.15630067116
-2.704 0.15632581159
-2.69951 0.156350249156
-2.69502 0.156373982146
-2.69053 0.156222002601
-2.68604 0.156244566599
-2.68155 0.156266421676
-2.67706 0.156287566098
-2.67257 0.156307998124
-2.66808 0.15615414451
-2.66359 0.156173395083
-2.6591 0.156191928816
-2.65461 0.156209743945
-2.65012 0.156226838702
-2.64563 0.156071087209
-2.64114 0.156086987642
-2.63665 0.156102163149
-2.63216 0.156116611937
-2.62767 0.156130332207
-2.62318 0.155972657734
-2.61869 0.155985170376
-2.6142 0.155996949829
-2.60971 0.156007994268
-2.60522 0.15601830186
-2.60073 0.156027870767
-2.59624 0.155867764163
-2.59175 0.155876108726
-2.58726 0.155883709788
-2.58277 0.155890565479
-2.57828 0.155896673925
-2.57379 0.155902033243
-2.5693 0.155739454137
-2.56481 0.155743571712
-2.56032 0.155746935186
-2.55583 0.155749542645
-2.55134 0.155751392166
-2.54685 0.155752481822
-2.54236 0.155752809675
-2.53787 0.155752373781
-2.53338 0.155586281882
-2.52889 0.155584579687
-2.5244 0.155582108549
-2.51991 0.155578866487
-2.51542 0.155574851513
-2.51093 0.15557006163
-2.50644 0.155564494835
-2.50195 0.155558149113
-2.49746 0.155388462197
-2.49297 0.155380824252
-2.48848 0.155372401939
-2.48399 0.155363193207
-2.4795 0.155353195994
-2.47501 0.155342408229
-2.47052 0.155330827833
-2.46603 0.155318452717
-2.46154 0.15530528078
-2.45705 0.155291309915
-2.45256 0.155276538004
-2.44807 0.155260962919
-2.44358 0.15508549194
-2.43909 0.155068582681
-2.4346 0.155050864409
-2.43011 0.155032334954
-2.42562 0.155012992131
-2.42113 0.154992833747
-2.41664 0.1549718576
-2.41215 0.154950061473
-2.40766 0.154927443143
-2.40317 0.154904000372
-2.39868 0.154879730913
-2.39419 0.154854632508
-2.3897 0.154828702887
-2.38521 0.154801939769
-2.38072 0.154774340861
-2.37623 0.15474590386
-2.37174 0.154716626448
-2.36725 0.154686506299
-2.36276 0.154655541073
-2.35827 0.154623728418
-2.35378 0.154591065971
-2.34929 0.154557551355
-2.3448 0.154523182182
-2.34031 0.154487956052
-2.33582 0.15445187055
-2.33133 0.154414923252
-2.32684 0.154377111718
-2.32235 0.154338433497
-2.31786 0.154298886123
-2.31337 0.15425846712
-2.30888 0.154217173996
-2.30439 0.154175004248
-2.2999 0.154131955357
-2.29541 0.154088024794
-2.29092 0.154043210012
-2.28643 0.153997508455
-2.28194 0.153950917549
-2.27745 0.15390343471
-2.27296 0.153855057336
-2.26847 0.153953592603
-2.26398 0.15390311877
-2.25949 0.153851742052
-2.255 0.153799459795
-2.25051 0.153746269331
-2.24602 0.153692167978
-2.24153 0.153637153037
-2.23704 0.153581221799
-2.23255 0.153524371535
-2.22806 0.153466599504
-2.22357 0.15340790295
-2.21908 0.153492906165
-2.21459 0.153432047197
-2.2101 0.153370254915
-2.20561 0.153307526504
-2.20112 0.153243859136
-2.19663 0.153179249964
-2.19214 0.153113696127
-2.18765 0.15304719475
-2.18316 0.153122050618
-2.17867 0.153053336555
-2.17418 0.152983665823
-2.16969 0.152913035486
-2.1652 0.152841442589
-2.16071 0.152768884165
-2.15622 0.15283593483
-2.15173 0.152761124582
-2.14724 0.152685339417
-2.14275 0.152608576304
-2.13826 0.152530832195
-2.13377 0.152452104026
-2.12928 0.15251121593
-2.12479 0.152430195831
-2.1203 0.152348182015
-2.11581 0.152265171352
-2.11132 0.152181160697
-2.10683 0.152233521087
-2.10234 0.152147184119
-2.09785 0.152059837275
-2.09336 0.151971477344
-2.08887 0.152018327047
-2.08438 0.151927612562
-2.07989 0.151835874923
-2.0754 0.151743110853
-2.07091 0.151784385254
-2.06642 0.151689237948
-2.06193 0.151593053958
-2.05744 0.151495829941
-2.05295 0.151531463751
-2.04846 0.151431827369
-2.04397 0.151331140519
-2.03948 0.151229399792
-2.03499 0.151259327029
-2.0305 0.151155144355
-2.02601 0.151049897173
-2.02152 0.151075447863
-2.01703 0.150967735988
-2.01254 0.150858948835
-2.00805 0.150880083761
-2.00356 0.150768808923
-1.99907 0.150656447897
-1.99458 0.150673127577
-1.99009 0.150558255626
-1.9856 0.150442286437
-1.98111 0.150454471121
-1.97662 0.150335967519
-1.97213 0.150216355488
-1.96764 0.150224005159
-1.96315 0.150101834979
-1.95866 0.14997854504
-1.95417 0.149981619406
-1.94968 0.149855747336
-1.94519 0.149855673166
-1.9407 0.149727202538
-1.93621 0.149597592879
-1.93172 0.149592874788
-1.92723 0.149460642188
-1.92274 0.149452728077
-1.91825 0.149317855856
-1.91376 0.149181824962
-1.90927 0.149169197622
-1.90478 0.149030502329
-1.90029 0.149014631074
-1.8958 0.148873254455
-1.89131 0.148854119651
-1.88682 0.148710044684
-1.88233 0.148687626644
-1.87784 0.148540836214
-1.87335 0.148515115197
-1.86886 0.148365592098
-1.86437 0.148336548312
-1.85988 0.148184275248
-1.85539 0.148151888848
-1.8509 0.147996848435
-1.84641 0.14796109953
-1.84192 0.147803274295
-1.83743 0.147764142944
-1.83294 0.147603515333
-1.82845 0.14756098155
-1.82396 0.147397533925
-1.81947 0.14735157768
-1.81498 0.147185292324
-1.81049 0.147135893543
-1.806 0.146966752662
-1.80151 0.146913891233
-1.79702 0.146859162923
-1.79253 0.146685532734
-1.78804 0.146627310763
-1.78355 0.146450779921
-1.77906 0.146389044101
-1.77457 0.146325413723
-1.77008 0.146144324685
-1.76559 0.146077149371
-1.7611 0.145893114175
-1.75661 0.145822373678
-1.75212 0.145749710961
-1.74763 0.145561048198
-1.74314 0.145484789167
-1.73865 0.145406591144
-1.73416 0.145213258792
-1.72967 0.145131433321
-1.72518 0.145047652112
-1.72069 0.144849608042
-1.7162 0.144762168263
-1.71171 0.144672756037
-1.70722 0.14446995804
-1.70273 0.144376856146
-1.69824 0.144281765138
-1.69375 0.144074170948
-1.68926 0.143975359219
-1.68477 0.143874541758
-1.68028 0.143771712747
-1.67579 0.143557539912
-1.6713 0.143450948449
-1.66681 0.143342328907
-1.66232 0.143231675507
-1.65783 0.143010848056
-1.65334 0.142896390656
-1.64885 0.142779882975
-1.64436 0.142661319281
-1.63987 0.142540693859
-1.63538 0.142311352418
-1.63089 0.1421868711
-1.6264 0.142060311792
-1.62191 0.141931668833
-1.61742 0.141800936576
-1.61293 0.141668109393
-1.60844 0.141428323068
-1.60395 0.141291578165
-1.59946 0.141152722322
-1.59497 0.141011749976
-1.59048 0.140868655585
-1.58599 0.140723433625
-1.5815 0.140576078594
-1.57701 0.140426585012
-1.57252 0.140274947417
-1.56803 0.140018995936
-1.56354 0.139863349255
-1.55905 0.139705543035
-1.55456 0.139545571903
-1.55007 0.139383430511
-1.54558 0.139219113538
-1.54109 0.139052615687
-1.5366 0.13888393169
-1.53211 0.138713056303
-1.52762 0.138539984315
-1.52313 0.138364710541
-1.51864 0.138187229826
-1.51415 0.138007537046
-1.50966 0.137825627108
-1.50517 0.13764149495
-1.50068 0.137455135546
-1.49619 0.1372665439
-1.4917 0.137075715052
-1.48721 0.136882644079
-1.48272 0.136687326091
-1.47823 0.136489756237
-1.47374 0.136385751839
-1.46925 0.136183354788
-1.46476 0.135978690947
-1.46027 0.135771755628
-1.45578 0.135562544184
-1.45129 0.13535105201
-1.4468 0.135137274546
-1.44231 0.134921207274
-1.43782 0.134702845725
-1.43333 0.134575260225
-1.42884 0.134351982261
-1.42435 0.134126396339
-1.41986 0.133898498184
-1.41537 0.133668283577
-1.41088 0.133527298054
-1.40639 0.13329212039
-1.4019 0.133054613396
-1.39741 0.132814773073
-1.39292 0.132572595476
-1.38843 0.132418084609
-1.38394 0.13217090024
-1.37945 0.131921366613
-1.37496 0.131669480029
-1.37047 0.131504009791
-1.36598 0.131247083509
-1.36149 0.130987793068
-1.357 0.130813987261
-1.35251 0.130549633571
-1.34802 0.130282905156
-1.34353 0.130100724078
-1.33904 0.129828910214
-1.33455 0.129554711724
-1.33006 0.129364117895
-1.32557 0.129084813182
-1.32108 0.128803114652
-1.31659 0.12860407292
-1.3121 0.128317248894
-1.30761 0.12802802261
-1.30312 0.127820500273
-1.29863 0.127526130805
-1.29414 0.127312842244
-1.28965 0.127013318352
-1.28516 0.126794249846
-1.28067 0.12648956107
-1.27618 0.126264699742
-1.27169 0.125954836433
-1.2672 0.125724170282
-1.26271 0.125409123627
-1.25822 0.125172641552
-1.25373 0.124852403601
-1.24924 0.12461009543
-1.24475 0.124284659128
-1.24026 0.124036515645
-1.23577 0.12370587486
-1.23128 0.123451887837
-1.22679 0.123116037388
-1.2223 0.122856199614
-1.21781 0.122515135305
-1.21332 0.122249440616
-1.20883 0.12198066437
-1.20434 0.121631602579
-1.19985 0.121356961471
-1.19536 0.121079234292
-1.19087 0.12072217004
-1.18638 0.120438572631
-1.18189 0.120151885988
-1.1774 0.119786818104
-1.17291 0.119494258559
-1.16842 0.119198608022
-1.16393 0.11882553932
-1.15944 0.118524016021
-1.15495 0.118145732806
-1.15046 0.117618482846
-1.14597 0.11709033482
-1.14148 0.116561289455
-1.13699 0.116031347613
-1.1325 0.11550051029
-1.12801 0.114968778623
-1.12352 0.114436153892
-1.11903 0.113902637518
-1.11454 0.113368231071
-1.11005 0.112832936269
-1.10556 0.112296754982
-1.10107 0.111759689233
-1.09658 0.111221741202
-1.09209 0.110682913229
-1.0876 0.110143207815
-1.08311 0.109602627624
-1.07862 0.109061175489
-1.07413 0.10851885441
-1.06964 0.107975667562
-1.06515 0.107431618292
-1.06066 0.106886710127
-1.05617 0.10634094677
-1.05168 0.105794332112
-1.04719 0.105246870225
-1.0427 0.104698565371
-1.03821 0.104149422004
-1.03372 0.103599444769
-1.02923 0.10304863851
-1.02474 0.102497008269
-1.02025 0.10194455929
-1.01576 0.101391297022
-1.01127 0.10083722712
-1.00678 0.100282355453
-1.00229 0.0997266881
-0.9978 0.0991702313575
-0.99331 0.0986129917408
-0.98882 0.0980549759867
-0.98433 0.0974961910571
-0.97984 0.0969366441412
-0.97535 0.0963763426586
-0.97086 0.0958152942625
-0.96637 0.095253506842
-0.96188 0.0946909885258
-0.95739 0.0941277476841
-0.9529 0.0935637929325
-0.94841 0.0929991331344
-0.94392 0.0924337774038
-0.93943 0.0918677351088
-0.93494 0.0913010158737
-0.93045 0.0907336295827
-0.92596 0.0901655863826
-0.92147 0.0895968966852
-0.91698 0.0890275711711
-0.91249 0.088457620792
-0.908 0.0878870567738
-0.90351 0.0873158906195
-0.89902 0.0867441341122
-0.89453 0.0861717993179
-0.89004 0.0855988985883
-0.88555 0.0850254445641
-0.88106 0.0844514501774
-0.87657 0.0838769286549
-0.87208 0.0833018935205
-0.86759 0.0827263585985
-0.8631 0.0821503380161
-0.85861 0.0815738462064
-0.85412 0.0809968979114
-0.84963 0.0804195081842
-0.84514 0.0798416923925
-0.84065 0.0792634662209
-0.83616 0.078684845674
-0.83167 0.0781058470786
-0.82718 0.0775264870869
-0.82269 0.0769467826792
-0.8182 0.0763667511661
-0.81371 0.0757864101917
-0.80922 0.0752057777356
-0.80473 0.0746248721163
-0.80024 0.0740437119929
-0.79575 0.0734623163684
-0.79126 0.0728807045915
-0.78677 0.0722988963597
-0.78228 0.0717169117213
-0.77779 0.0711347710781
-0.7733 0.0705524951876
-0.76881 0.0699701051652
-0.76432 0.0693876224871
-0.75983 0.0688050689917
-0.75534 0.0682224668825
-0.75085 0.06763983873
-0.74636 0.067057207474
-0.74187 0.0664745964252
-0.73738 0.0658920292679
-0.73289 0.0653095300617
-0.7284 0.0647271232433
-0.72391 0.0641448336286
-0.71942 0.0635626864145
-0.71493 0.0629807071808
-0.71044 0.0623989218914
-0.70595 0.0618173568969
-0.70146 0.0612360389352
-0.69697 0.060654995134
-0.69248 0.0600742530116
-0.68799 0.0594938404786
-0.6835 0.0589137858393
-0.67901 0.058334117793
-0.67452 0.0577548654351
-0.67003 0.0571760582584
-0.66554 0.0565977261542
-0.66105 0.0560198994133
-0.65656 0.0554426087268
-0.65207 0.0548658851871
-0.64758 0.0542897602887
-0.64309 0.0537142659291
-0.6386 0.0531394344088
-0.63411 0.0525652984326
-0.62962 0.0519918911098
-0.62513 0.0514192459541
-0.62064 0.0508473968847
-0.61615 0.0502763782259
-0.61166 0.0497062247074
-0.60717 0.0491369714645
-0.60268 0.0485686540377
-0.59819 0.0480013083725
-0.5937 0.0474349708196
-0.58921 0.046869678134
-0.58472 0.0463054674747
-0.58023 0.0457423764044
-0.57574 0.0451804428882
-0.57125 0.0446197052934
-0.56676 0.0440602023884
-0.56227 0.0435019733414
-0.55778 0.0429450577198
-0.55329 0.0423894954884
-0.5488 0.0418353270086
-0.54431 0.0412825930366
-0.53982 0.0407313347216
-0.53533 0.0401815936048
-0.53084 0.0396334116168
-0.52635 0.0390868310761
-0.52186 0.0385418946868
-0.51737 0.0379986455367
-0.51288 0.0374571270945
-0.50839 0.0369173832077
-0.5039 0.0363794581
-0.49941 0.0358433963684
-0.49492 0.0353092429803
-0.49043 0.0347770432708
-0.48594 0.0342468429392
-0.48145 0.0337186880461
-0.47696 0.0331926250097
-0.47247 0.0326687006022
-0.46798 0.0321469619466
-0.46349 0.0316274565123
-0.459 0.0311102321114
-0.45451 0.0305953368944
-0.45002 0.0300828193463
-0.44553 0.0295727282816
-0.44104 0.0290651128404
-0.43655 0.028560022483
-0.43206 0.0280575069857
-0.42757 0.0275576164351
-0.42308 0.0270604012234
-0.41859 0.0265659120431
-0.4141 0.0260741998812
-0.40961 0.0255853160136
-0.40512 0.0250993119996
-0.40063 0.0246162396757
-0.39614 0.0241361511496
-0.39165 0.0236590987938
-0.38716 0.0231851352393
-0.38267 0.022714313369
-0.37818 0.0222466863109
-0.37369 0.0217823074312
-0.3692 0.0213212303275
-0.36471 0.0208635088209
-0.36022 0.0204091969494
-0.35573 0.01995834896
-0.35124 0.0195110193008
-0.34675 0.0190672626136
-0.34226 0.0186271337254
-0.33777 0.0181906876405
-0.33328 0.0177579795321
-0.32879 0.0173290647338
-0.3243 0.0169039987308
-0.31981 0.0164828371513
-0.31532 0.0160656357575
-0.31083 0.015652450436
-0.30634 0.0152433371893
-0.30185 0.0148383521255
-0.29736 0.0144375514495
-0.29287 0.0140409914525
-0.28838 0.0136487285025
-0.28389 0.0132608190344
-0.2794 0.0128773195392
-0.27491 0.012498286554
-0.27042 0.0121237766516
-0.26593 0.0117538464295
-0.26144 0.0113885524993
-0.25695 0.0110279514756
-0.25246 0.0106720999652
-0.24797 0.0103210545553
-0.24348 0.00997487180261
-0.23899 0.00963360822175
-0.2345 0.00929732027336
-0.23001 0.00896606435251
-0.22552 0.00863989677669
-0.22103 0.00831887377382
-0.21654 0.00800305146999
-0.21205 0.00769248587724
-0.20756 0.00738723288106
-0.20307 0.00708734822789
-0.19858 0.00679288751246
-0.19409 0.00650390616499
-0.1896 0.00622045943831
-0.18511 0.00594260239488
-0.18062 0.00567038989367
-0.17613 0.00540387657697
-0.17164 0.00514311685711
-0.16715 0.00488816490301
-0.16266 0.00463907462676
-0.15817 0.00439589967
-0.15368 0.00415869339026
-0.14919 0.00392750884726
-0.1447 0.00370239878904
-0.14021 0.00348341563811
-0.13572 0.00327061147746
-0.13123 0.00306403803655
-0.12674 0.00286374667724
-0.12225 0.0026697883796
-0.11776 0.00248221372774
-0.11327 0.00230107289557
-0.10878 0.00212641563251
-0.10429 0.00195829124914
-0.0998 0.00179674860285
-0.09531 0.00164183608345
-0.09082 0.00149360159874
-0.08633 0.00135209256008
-0.08184 0.00121735586792
-0.07735 0.00108943789733
-0.07286 0.000968384483564
-0.06837 0.000854240907531
-0.06388 0.000747051881364
-0.05939 0.000646861533944
-0.0549 0.00055371339646
-0.05041 0.000467650387979
-0.04592 0.00038871480105
-0.04143 0.000316948287335
-0.03694 0.000252391843272
-0.03245 0.000195085795791
-0.02796 0.000145069788068
-0.02347 0.000102382765331
-0.01898 6.70629607416e-05
-0.01449 3.91478813146e-05


==> figuresAndData/dataForConditionalVarianceLaplaceProb0pt2.tex <==
-13.5 0.111111111111
-13.4736108605 0.111111111111
-13.447221721 0.111111111111
-13.4208325815 0.111111111111
-13.394443442 0.111111111111
-13.3680543024 0.111111111111
-13.3416651629 0.111111111111
-13.3152760234 0.111111111111
-13.2888868839 0.111111111111
-13.2624977444 0.111111111111
-13.2361086049 0.111111111111
-13.2097194654 0.111111111111
-13.1833303259 0.111111111111
-13.1569411863 0.111111111111
-13.1305520468 0.111111111111
-13.1041629073 0.111111111111
-13.0777737678 0.111111111111
-13.0513846283 0.111111111111
-13.0249954888 0.111111111111
-12.9986063493 0.111111111111
-12.9722172098 0.111111111111
-12.9458280702 0.111111111111
-12.9194389307 0.111111111111
-12.8930497912 0.111111111111
-12.8666606517 0.111111111111
-12.8402715122 0.111111111111
-12.8138823727 0.111111111111
-12.7874932332 0.111111111111
-12.7611040937 0.111111111111
-12.7347149541 0.111111111111
-12.7083258146 0.111111111111
-12.6819366751 0.111111111111
-12.6555475356 0.111111111111
-12.6291583961 0.111111111111
-12.6027692566 0.111111111111
-12.5763801171 0.111111111111
-12.5499909776 0.111111111111
-12.5236018381 0.111111111111
-12.4972126985 0.111111111111
-12.470823559 0.111111111111
-12.4444344195 0.111111111111
-12.41804528 0.111111111111
-12.3916561405 0.111111111111
-12.365267001 0.111111111111
-12.3388778615 0.111111111111
-12.312488722 0.111111111111
-12.2860995824 0.111111111111
-12.2597104429 0.111111111111
-12.2333213034 0.111111111111
-12.2069321639 0.111111111111
-12.1805430244 0.111111111111
-12.1541538849 0.111111111111
-12.1277647454 0.111111111111
-12.1013756059 0.111111111111
-12.0749864663 0.111111111111
-12.0485973268 0.111111111111
-12.0222081873 0.111111111111
-11.9958190478 0.111111111111
-11.9694299083 0.111111111111
-11.9430407688 0.111111111111
-11.9166516293 0.111111111111
-11.8902624898 0.111111111111
-11.8638733503 0.111111111111
-11.8374842107 0.111111111111
-11.8110950712 0.111111111111
-11.7847059317 0.111111111111
-11.7583167922 0.111111111111
-11.7319276527 0.111111111111
-11.7055385132 0.111111111111
-11.6791493737 0.111111111111
-11.6527602342 0.111111111111
-11.6263710946 0.111111111111
-11.5999819551 0.111111111111
-11.5735928156 0.111111111111
-11.5472036761 0.111111111111
-11.5208145366 0.111111111111
-11.4944253971 0.111111111111
-11.4680362576 0.111111111111
-11.4416471181 0.111111111111
-11.4152579785 0.111111111111
-11.388868839 0.111111111111
-11.3624796995 0.111111111111
-11.33609056 0.111111111111
-11.3097014205 0.111111111111
-11.283312281 0.111111111111
-11.2569231415 0.111111111111
-11.230534002 0.111111111111
-11.2041448624 0.111111111111
-11.1777557229 0.111111111111
-11.1513665834 0.111111111111
-11.1249774439 0.11111111111
-11.0985883044 0.11111111111
-11.0721991649 0.11111111111
-11.0458100254 0.11111111111
-11.0194208859 0.11111111111
-10.9930317464 0.11111111111
-10.9666426068 0.11111111111
-10.9402534673 0.11111111111
-10.9138643278 0.11111111111
-10.8874751883 0.11111111111
-10.8610860488 0.11111111111
-10.8346969093 0.11111111111
-10.8083077698 0.11111111111
-10.7819186303 0.111111111109
-10.7555294907 0.111111111109
-10.7291403512 0.111111111109
-10.7027512117 0.111111111109
-10.6763620722 0.111111111109
-10.6499729327 0.111111111109
-10.6235837932 0.111111111108
-10.5971946537 0.111111111108
-10.5708055142 0.111111111108
-10.5444163746 0.111111111108
-10.5180272351 0.111111111108
-10.4916380956 0.111111111107
-10.4652489561 0.111111111107
-10.4388598166 0.111111111107
-10.4124706771 0.111111111106
-10.3860815376 0.111111111106
-10.3596923981 0.111111111106
-10.3333032585 0.111111111105
-10.306914119 0.111111111105
-10.2805249795 0.111111111104
-10.25413584 0.111111111104
-10.2277467005 0.111111111103
-10.201357561 0.111111111103
-10.1749684215 0.111111111102
-10.148579282 0.111111111101
-10.1221901425 0.1111111111
-10.0958010029 0.1111111111
-10.0694118634 0.111111111099
-10.0430227239 0.111111111098
-10.0166335844 0.111111111097
-9.99024444489 0.111111111096
-9.96385530538 0.111111111094
-9.93746616587 0.111111111093
-9.91107702636 0.111111111092
-9.88468788684 0.11111111109
-9.85829874733 0.111111111089
-9.83190960782 0.111111111087
-9.80552046831 0.111111111085
-9.7791313288 0.111111111083
-9.75274218928 0.111111111081
-9.72635304977 0.111111111079
-9.69996391026 0.111111111076
-9.67357477075 0.111111111074
-9.64718563124 0.111111111071
-9.62079649172 0.111111111068
-9.59440735221 0.111111111064
-9.5680182127 0.111111111061
-9.54162907319 0.111111111057
-9.51523993368 0.111111111053
-9.48885079416 0.111111111048
-9.46246165465 0.111111111044
-9.43607251514 0.111111111038
-9.40968337563 0.111111111033
-9.38329423611 0.111111111027
-9.3569050966 0.11111111102
-9.33051595709 0.111111111014
-9.30412681758 0.111111111006
-9.27773767807 0.111111110998
-9.25134853855 0.11111111099
-9.22495939904 0.11111111098
-9.19857025953 0.11111111097
-9.17218112002 0.11111111096
-9.14579198051 0.111111110948
-9.11940284099 0.111111110936
-9.09301370148 0.111111110922
-9.06662456197 0.111111110908
-9.04023542246 0.111111110893
-9.01384628295 0.111111110876
-8.98745714343 0.111111110858
-8.96106800392 0.111111110839
-8.93467886441 0.111111110818
-8.9082897249 0.111111110796
-8.88190058539 0.111111110772
-8.85551144587 0.111111110747
-8.82912230636 0.111111110719
-8.80273316685 0.111111110689
-8.77634402734 0.111111110657
-8.74995488782 0.111111110623
-8.72356574831 0.111111110586
-8.6971766088 0.111111110546
-8.67078746929 0.111111110503
-8.64439832978 0.111111110457
-8.61800919026 0.111111110408
-8.59162005075 0.111111110355
-8.56523091124 0.111111110298
-8.53884177173 0.111111110236
-8.51245263222 0.11111111017
-8.4860634927 0.111111110099
-8.45967435319 0.111111110022
-8.43328521368 0.11111110994
-8.40689607417 0.111111109852
-8.38050693466 0.111111109757
-8.35411779514 0.111111109655
-8.32772865563 0.111111109545
-8.30133951612 0.111111109427
-8.27495037661 0.1111111093
-8.2485612371 0.111111109163
-8.22217209758 0.111111109016
-8.19578295807 0.111111108859
-8.16939381856 0.111111108689
-8.14300467905 0.111111108507
-8.11661553953 0.111111108311
-8.09022640002 0.1111111081
-8.06383726051 0.111111107874
-8.037448121 0.111111107631
-8.01105898149 0.111111107369
-7.98466984197 0.111111107088
-7.95828070246 0.111111106786
-7.93189156295 0.111111106461
-7.90550242344 0.111111106113
-7.87911328393 0.111111105738
-7.85272414441 0.111111105335
-7.8263350049 0.111111104902
-7.79994586539 0.111111104436
-7.77355672588 0.111111103936
-7.74716758637 0.111111103399
-7.72077844685 0.111111102822
-7.69438930734 0.111111102201
-7.66800016783 0.111111101535
-7.64161102832 0.111111100819
-7.61522188881 0.111111100049
-7.58883274929 0.111111099223
-7.56244360978 0.111111098335
-7.53605447027 0.111111097381
-7.50966533076 0.111111096356
-7.48327619124 0.111111095255
-7.45688705173 0.111111094072
-7.43049791222 0.111111092802
-7.40410877271 0.111111091437
-7.3777196332 0.111111089971
-7.35133049368 0.111111088397
-7.32494135417 0.111111086706
-7.29855221466 0.11111108489
-7.27216307515 0.111111082939
-7.24577393564 0.111111080844
-7.21938479612 0.111111078595
-7.19299565661 0.111111076179
-7.1666065171 0.111111073585
-7.14021737759 0.111111070799
-7.11382823808 0.111111067808
-7.08743909856 0.111111064596
-7.06104995905 0.111111061147
-7.03466081954 0.111111057444
-7.00827168003 0.111111053468
-6.98188254052 0.1111110492
-6.955493401 0.111111044618
-6.92910426149 0.111111039698
-6.90271512198 0.111111034417
-6.87632598247 0.111111028748
-6.84993684295 0.111111022663
-6.82354770344 0.111111016131
-6.79715856393 0.11111100912
-6.77076942442 0.111111001595
-6.74438028491 0.111110993518
-6.71799114539 0.11111098485
-6.69160200588 0.111110975547
-6.66521286637 0.111110965564
-6.63882372686 0.111110954851
-6.61243458735 0.111110943354
-6.58604544783 0.111110931018
-6.55965630832 0.111110917781
-6.53326716881 0.111110903579
-6.5068780293 0.11111088834
-6.48048888979 0.111110871992
-6.45409975027 0.111110854452
-6.42771061076 0.111110835635
-6.40132147125 0.11111081545
-6.37493233174 0.111110793796
-6.34854319223 0.111110770569
-6.32215405271 0.111110745656
-6.2957649132 0.111110718934
-6.26937577369 0.111110690274
-6.24298663418 0.111110659536
-6.21659749466 0.111110626571
-6.19020835515 0.11111059122
-6.16381921564 0.111110553312
-6.13743007613 0.111110512662
-6.11104093662 0.111110469075
-6.0846517971 0.111110422341
-6.05826265759 0.111110372234
-6.03187351808 0.111110318514
-6.00548437857 0.111110260922
-5.97909523906 0.111110199183
-5.95270609954 0.111110133002
-5.92631696003 0.111110062061
-5.89992782052 0.111109986022
-5.87353868101 0.111109904522
-5.8471495415 0.111109817175
-5.82076040198 0.111109723564
-5.79437126247 0.111109623245
-5.76798212296 0.111109515744
-5.74159298345 0.111109400552
-5.71520384394 0.111109277124
-5.68881470442 0.11110914488
-5.66242556491 0.111109003196
-5.6360364254 0.111108851407
-5.60964728589 0.111108688801
-5.58325814637 0.111108514616
-5.55686900686 0.111108328038
-5.53047986735 0.111108128196
-5.50409072784 0.111107914159
-5.47770158833 0.111107684932
-5.45131244881 0.111107439451
-5.4249233093 0.111107176577
-5.39853416979 0.111106895096
-5.37214503028 0.111106593707
-5.34575589077 0.111106271022
-5.31936675125 0.111105925557
-5.29297761174 0.111105555726
-5.26658847223 0.111105159834
-5.24019933272 0.111104736072
-5.21381019321 0.111104282506
-5.18742105369 0.111103797071
-5.16103191418 0.11110327756
-5.13464277467 0.111102721618
-5.10825363516 0.111102126729
-5.08186449565 0.111101490207
-5.05547535613 0.111100809183
-5.02908621662 0.111100080595
-5.00269707711 0.111099301177
-4.9763079376 0.111098467439
-4.94991879808 0.111097575658
-4.92352965857 0.111096621861
-4.89714051906 0.11109560181
-4.87075137955 0.111094510981
-4.84436224004 0.11109334455
-4.81797310052 0.11109209737
-4.79158396101 0.111090763952
-4.7651948215 0.111089338443
-4.73880568199 0.1110878146
-4.71241654248 0.111086185769
-4.68602740296 0.111084444853
-4.65963826345 0.111082584292
-4.63324912394 0.111080596023
-4.60685998443 0.111078471458
-4.58047084492 0.111076201443
-4.5540817054 0.111073776227
-4.52769256589 0.111071185421
-4.50130342638 0.111068417961
-4.47491428687 0.111065462063
-4.44852514736 0.111062305178
-4.42213600784 0.111058933946
-4.39574686833 0.111055334146
-4.36935772882 0.111051490638
-4.34296858931 0.111047387312
-4.31657944979 0.111043007025
-4.29019031028 0.111038331537
-4.26380117077 0.111033341446
-4.23741203126 0.111028016116
-4.21102289175 0.111022333603
-4.18463375223 0.111016270574
-4.15824461272 0.111009802224
-4.13185547321 0.111002902189
-4.1054663337 0.110995542451
-4.07907719419 0.110987693241
-4.05268805467 0.110979322934
-4.02629891516 0.110970397938
-3.99990977565 0.110960882584
-3.97352063614 0.110950738997
-3.94713149663 0.110939926975
-3.92074235711 0.110928403848
-3.8943532176 0.110916124339
-3.86796407809 0.110903040417
-3.84157493858 0.110889101133
-3.81518579907 0.110874252462
-3.78879665955 0.110858437126
-3.76240752004 0.110841594411
-3.73601838053 0.11082365998
-3.70962924102 0.110804565669
-3.6832401015 0.110784239277
-3.65685096199 0.110762604348
-3.63046182248 0.11073957994
-3.60407268297 0.110715080382
-3.57768354346 0.110689015024
-3.55129440394 0.110661287973
-3.52490526443 0.110631797819
-3.49851612492 0.110600437346
-3.47212698541 0.110567093235
-3.4457378459 0.11053164575
-3.41934870638 0.110493968417
-3.39295956687 0.110453927684
-3.36657042736 0.110411382573
-3.34018128785 0.110366184316
-3.31379214834 0.110318175978
-3.28740300882 0.110267192066
-3.26101386931 0.110213058129
-3.2346247298 0.110155590339
-3.20823559029 0.11009459506
-3.18184645078 0.110029868411
-3.15545731126 0.109961195804
-3.12906817175 0.109888351483
-3.10267903224 0.10981109804
-3.07628989273 0.109729185932
-3.04990075321 0.109642352973
-3.0235116137 0.109550323831
-2.99712247419 0.109452809508
-2.97073333468 0.109349506818
-2.94434419517 0.109240097855
-2.91795505565 0.109124249459
-2.89156591614 0.109001612685
-2.86517677663 0.108871822263
-2.83878763712 0.108734496069
-2.81239849761 0.108589234594
-2.78600935809 0.108435620431
-2.75962021858 0.108273217762
-2.73323107907 0.108101571868
-2.70684193956 0.107920208657
-2.68045280005 0.107728634215
-2.65406366053 0.107526334383
-2.62767452102 0.107312774374
-2.60128538151 0.107087398424
-2.574896242 0.10684962949
-2.54850710249 0.106598869003
-2.52211796297 0.10633449668
-2.49572882346 0.1060558704
-2.46933968395 0.105762326166
-2.44295054444 0.105453178137
-2.41656140492 0.105127718773
-2.39017226541 0.104785219071
-2.3637831259 0.104424928922
-2.33739398639 0.104046077599
-2.31100484688 0.103647874378
-2.28461570736 0.103229509319
-2.25822656785 0.102790154207
-2.23183742834 0.102328963673
-2.20544828883 0.101845076512
-2.17905914932 0.101337617211
-2.1526700098 0.100805697692
-2.12628087029 0.100248419306
-2.09989173078 0.0996648750716
-2.07350259127 0.0990541521936
-2.04711345176 0.0984153348587
-2.02072431224 0.0977475073393
-1.99433517273 0.0970497574098
-1.96794603322 0.0963211800947
-1.94155689371 0.0955608817598
-1.9151677542 0.0947679845585
-1.88877861468 0.0939416312436
-1.86238947517 0.0930809903537
-1.83600033566 0.0921852617788
-1.80961119615 0.0912536827099
-1.78322205663 0.0902855339711
-1.75683291712 0.0892801467322
-1.73044377761 0.0882369095917
-1.7040546381 0.0871552760194
-1.67766549859 0.0860347721382
-1.65127635907 0.0848750048226
-1.62488721956 0.08367567008
-1.59849808005 0.0824365616795
-1.57210894054 0.0811575799773
-1.54571980103 0.0798387408871
-1.51933066151 0.0784801849277
-1.492941522 0.0770821862753
-1.46655238249 0.0756451617335
-1.44016324298 0.0741696795271
-1.41377410347 0.0726564678123
-1.38738496395 0.0711064227862
-1.36099582444 0.0695206162667
-1.33460668493 0.0679003026051
-1.30821754542 0.0662469247823
-1.28182840591 0.0645621195324
-1.25543926639 0.0628477213284
-1.22905012688 0.0611057650608
-1.20266098737 0.059338487236
-1.17627184786 0.0575483255204
-1.14988270834 0.0557379164603
-1.12349356883 0.0539100912109
-1.09710442932 0.0520678691238
-1.07071528981 0.0502144490511
-1.0443261503 0.0483531982515
-1.01793701078 0.0464876388047
-0.991547871272 0.0446214314753
-0.96515873176 0.0427583570056
-0.938769592248 0.0409022948578
-0.912380452736 0.0390571994798
-0.885991313224 0.037227074219
-0.859602173712 0.0354159430708
-0.8332130342 0.0336278205095
-0.806823894688 0.0318666797123
-0.780434755176 0.0301364195523
-0.754045615663 0.0284408307975
-0.727656476151 0.0267835620099
-0.701267336639 0.0251680856903
-0.674878197127 0.0235976652522
-0.648489057615 0.0220753234405
-0.622099918103 0.0206038128186
-0.595710778591 0.0191855889493
-0.569321639079 0.0178227868657
-0.542932499567 0.0165172013899
-0.516543360055 0.0152702717899
-0.490154220543 0.0140830711832
-0.463765081031 0.0129563009921
-0.437375941518 0.0118902906386
-0.410986802006 0.010885002537
-0.384597662494 0.00994004230422
-0.358208522982 0.00905467397152
-0.33181938347 0.0082278398436
-0.305430243958 0.00745818452858
-0.30481938347 0.00744103304743
-0.304208522982 0.00742391140817
-0.303597662494 0.00740681967467
-0.302986802006 0.0073897579111
-0.302375941518 0.00737272618196
-0.301765081031 0.00735572455202
-0.301154220543 0.00733875308639
-0.300543360055 0.00732181185047
-0.299932499567 0.00730490091
-0.299321639079 0.00728802033098
-0.298710778591 0.00727117017977
-0.298099918103 0.00725435052301
-0.297489057615 0.00723756142766
-0.296878197127 0.007220802961
-0.296267336639 0.00720407519062
-0.295656476151 0.0071873781844
-0.295045615663 0.00717071201057
-0.294434755176 0.00715407673764
-0.293823894688 0.00713747243446
-0.2932130342 0.00712089917018
-0.292602173712 0.00710435701426
-0.291991313224 0.0070878460365
-0.291380452736 0.00707136630699
-0.290769592248 0.00705491789614
-0.29015873176 0.00703850087469
-0.289547871272 0.00702211531369
-0.288937010784 0.00700576128451
-0.288326150296 0.00698943885882
-0.287715289808 0.00697314810863
-0.287104429321 0.00695688910626
-0.286493568833 0.00694066192435
-0.285882708345 0.00692446663587
-0.285271847857 0.00690830331408
-0.284660987369 0.00689217203259
-0.284050126881 0.00687607286532
-0.283439266393 0.0068600058865
-0.282828405905 0.00684397117071
-0.282217545417 0.00682796879282
-0.281606684929 0.00681199882803
-0.280995824441 0.00679606135189
-0.280384963953 0.00678015644023
-0.279774103466 0.00676428416923
-0.279163242978 0.00674844461539
-0.27855238249 0.00673263785553
-0.277941522002 0.00671686396679
-0.277330661514 0.00670112302664
-0.276719801026 0.00668541511289
-0.276108940538 0.00666974030364
-0.27549808005 0.00665409867735
-0.274887219562 0.00663849031279
-0.274276359074 0.00662291528905
-0.273665498586 0.00660737368555
-0.273054638098 0.00659186558206
-0.272443777611 0.00657639105865
-0.271832917123 0.00656095019572
-0.271222056635 0.00654554307402
-0.270611196147 0.0065301697746
-0.270000335659 0.00651483037885
-0.269389475171 0.00649952496849
-0.268778614683 0.00648425362559
-0.268167754195 0.0064690164325
-0.267556893707 0.00645381347195
-0.266946033219 0.00643864482697
-0.266335172731 0.00642351058094
-0.265724312244 0.00640841081755
-0.265113451756 0.00639334562083
-0.264502591268 0.00637831507515
-0.26389173078 0.00636331926521
-0.263280870292 0.00634835827602
-0.262670009804 0.00633343219296
-0.262059149316 0.00631854110171
-0.261448288828 0.00630368508829
-0.26083742834 0.00628886423908
-0.260226567852 0.00627407864075
-0.259615707364 0.00625932838033
-0.259004846876 0.00624461354518
-0.258393986389 0.006229934223
-0.257783125901 0.00621529050181
-0.257172265413 0.00620068246999
-0.256561404925 0.00618611021621
-0.255950544437 0.00617157382953
-0.255339683949 0.0061570733993
-0.254728823461 0.00614260901524
-0.254117962973 0.00612818076739
-0.253507102485 0.00611378874612
-0.252896241997 0.00609943304215
-0.252285381509 0.00608511374652
-0.251674521021 0.00607083095064
-0.251063660534 0.00605658474622
-0.250452800046 0.00604237522533
-0.249841939558 0.00602820248037
-0.24923107907 0.00601406660408
-0.248620218582 0.00599996768954
-0.248009358094 0.00598590583017
-0.247398497606 0.00597188111972
-0.246787637118 0.00595789365228
-0.24617677663 0.0059439435223
-0.245565916142 0.00593003082454
-0.244955055654 0.00591615565411
-0.244344195166 0.00590231810648
-0.243733334679 0.00588851827744
-0.243122474191 0.00587475626311
-0.242511613703 0.00586103215998
-0.241900753215 0.00584734606486
-0.241289892727 0.0058336980749
-0.240679032239 0.00582008828761
-0.240068171751 0.00580651680081
-0.239457311263 0.0057929837127
-0.238846450775 0.0057794891218
-0.238235590287 0.00576603312696
-0.237624729799 0.0057526158274
-0.237013869311 0.00573923732267
-0.236403008824 0.00572589771265
-0.235792148336 0.00571259709758
-0.235181287848 0.00569933557803
-0.23457042736 0.00568611325494
-0.233959566872 0.00567293022955
-0.233348706384 0.00565978660347
-0.232737845896 0.00564668247867
-0.232126985408 0.00563361795742
-0.23151612492 0.00562059314236
-0.230905264432 0.00560760813648
-0.230294403944 0.00559466304311
-0.229683543456 0.0055817579659
-0.229072682969 0.00556889300888
-0.228461822481 0.0055560682764
-0.227850961993 0.00554328387317
-0.227240101505 0.00553053990423
-0.226629241017 0.00551783647498
-0.226018380529 0.00550517369115
-0.225407520041 0.00549255165883
-0.224796659553 0.00547997048444
-0.224185799065 0.00546743027475
-0.223574938577 0.00545493113689
-0.222964078089 0.00544247317832
-0.222353217601 0.00543005650684
-0.221742357114 0.00541768123061
-0.221131496626 0.00540534745814
-0.220520636138 0.00539305529826
-0.21990977565 0.00538080486017
-0.219298915162 0.00536859625341
-0.218688054674 0.00535642958786
-0.218077194186 0.00534430497375
-0.217466333698 0.00533222252166
-0.21685547321 0.00532018234251
-0.216244612722 0.00530818454757
-0.215633752234 0.00529622924844
-0.215022891746 0.0052843165571
-0.214412031259 0.00527244658585
-0.213801170771 0.00526061944733
-0.213190310283 0.00524883525455
-0.212579449795 0.00523709412086
-0.211968589307 0.00522539615994
-0.211357728819 0.00521374148584
-0.210746868331 0.00520213021293
-0.210136007843 0.00519056245594
-0.209525147355 0.00517903832995
-0.208914286867 0.00516755795039
-0.208303426379 0.00515612143301
-0.207692565891 0.00514472889393
-0.207081705404 0.00513338044961
-0.206470844916 0.00512207621685
-0.205859984428 0.00511081631281
-0.20524912394 0.00509960085498
-0.204638263452 0.0050884299612
-0.204027402964 0.00507730374965
-0.203416542476 0.00506622233887
-0.202805681988 0.00505518584773
-0.2021948215 0.00504419439546
-0.201583961012 0.00503324810162
-0.200973100524 0.00502234708611
-0.200362240036 0.0050114914692
-0.199751379549 0.00500068137148
-0.199140519061 0.00498991691389
-0.198529658573 0.00497919821772
-0.197918798085 0.00496852540461
-0.197307937597 0.00495789859651
-0.196697077109 0.00494731791575
-0.196086216621 0.00493678348499
-0.195475356133 0.00492629542722
-0.194864495645 0.00491585386579
-0.194253635157 0.00490545892439
-0.193642774669 0.00489511072703
-0.193031914181 0.00488480939809
-0.192421053694 0.00487455506228
-0.191810193206 0.00486434784464
-0.191199332718 0.00485418787055
-0.19058847223 0.00484407526576
-0.189977611742 0.00483401015633
-0.189366751254 0.00482399266865
-0.188755890766 0.00481402292949
-0.188145030278 0.00480410106591
-0.18753416979 0.00479422720534
-0.186923309302 0.00478440147554
-0.186312448814 0.0047746240046
-0.185701588326 0.00476489492094
-0.185090727839 0.00475521435334
-0.184479867351 0.00474558243088
-0.183869006863 0.00473599928301
-0.183258146375 0.00472646503949
-0.182647285887 0.00471697983042
-0.182036425399 0.00470754378623
-0.181425564911 0.00469815703768
-0.180814704423 0.00468881971587
-0.180203843935 0.00467953195221
-0.179592983447 0.00467029387848
-0.178982122959 0.00466110562673
-0.178371262472 0.0046519673294
-0.177760401984 0.0046428791192
-0.177149541496 0.0046338411292
-0.176538681008 0.00462485349279
-0.17592782052 0.00461591634369
-0.175316960032 0.00460702981591
-0.174706099544 0.00459819404383
-0.174095239056 0.00458940916212
-0.173484378568 0.00458067530578
-0.17287351808 0.00457199261012
-0.172262657592 0.00456336121079
-0.171651797104 0.00455478124372
-0.171040936617 0.0045462528452
-0.170430076129 0.0045377761518
-0.169819215641 0.00452935130043
-0.169208355153 0.00452097842828
-0.168597494665 0.00451265767287
-0.167986634177 0.00450438917204
-0.167375773689 0.00449617306393
-0.166764913201 0.00448800948696
-0.166154052713 0.0044798985799
-0.165543192225 0.00447184048179
-0.164932331737 0.00446383533199
-0.164321471249 0.00445588327015
-0.163710610762 0.00444798443623
-0.163099750274 0.00444013897047
-0.162488889786 0.00443234701343
-0.161878029298 0.00442460870593
-0.16126716881 0.00441692418912
-0.160656308322 0.00440929360441
-0.160045447834 0.00440171709352
-0.159434587346 0.00439419479844
-0.158823726858 0.00438672686144
-0.15821286637 0.0043793134251
-0.157602005882 0.00437195463226
-0.156991145394 0.00436465062603
-0.156380284907 0.00435740154981
-0.155769424419 0.00435020754728
-0.155158563931 0.00434306876236
-0.154547703443 0.00433598533927
-0.153936842955 0.00432895742249
-0.153325982467 0.00432198515675
-0.152715121979 0.00431506868705
-0.152104261491 0.00430820815865
-0.151493401003 0.00430140371707
-0.150882540515 0.00429465550806
-0.150271680027 0.00428796367765
-0.149660819539 0.00428132837209
-0.149049959052 0.00427474973791
-0.148439098564 0.00426822792183
-0.147828238076 0.00426176307085
-0.147217377588 0.00425535533219
-0.1466065171 0.00424900485331
-0.145995656612 0.00424271178187
-0.145384796124 0.00423647626579
-0.144773935636 0.00423029845318
-0.144163075148 0.0042241784924
-0.14355221466 0.00421811653199
-0.142941354172 0.00421211272072
-0.142330493684 0.00420616720756
-0.141719633197 0.00420028014169
-0.141108772709 0.00419445167247
-0.140497912221 0.00418868194947
-0.139887051733 0.00418297112243
-0.139276191245 0.00417731934131
-0.138665330757 0.00417172675621
-0.138054470269 0.00416619351742
-0.137443609781 0.00416071977542
-0.136832749293 0.00415530568084
-0.136221888805 0.00414995138446
-0.135611028317 0.00414465703723
-0.135000167829 0.00413942279026
-0.134389307342 0.00413424879479
-0.133778446854 0.0041291352022
-0.133167586366 0.00412408216402
-0.132556725878 0.00411908983189
-0.13194586539 0.00411415835759
-0.131335004902 0.00410928789302
-0.130724144414 0.00410447859017
-0.130113283926 0.00409973060115
-0.129502423438 0.00409504407818
-0.12889156295 0.00409041917355
-0.128280702462 0.00408585603964
-0.127669841974 0.00408135482894
-0.127058981487 0.00407691569397
-0.126448120999 0.00407253878734
-0.125837260511 0.00406822426172
-0.125226400023 0.00406397226983
-0.124615539535 0.00405978296441
-0.124004679047 0.00405565649827
-0.123393818559 0.00405159302423
-0.122782958071 0.00404759269513
-0.122172097583 0.00404365566384
-0.121561237095 0.0040397820832
-0.120950376607 0.00403597210608
-0.120339516119 0.00403222588532
-0.119728655632 0.00402854357373
-0.119117795144 0.00402492532412
-0.118506934656 0.00402137128922
-0.117896074168 0.00401788162173
-0.11728521368 0.0040144564743
-0.116674353192 0.0040110959995
-0.116063492704 0.00400780034981
-0.115452632216 0.00400456967763
-0.114841771728 0.00400140413527
-0.11423091124 0.00399830387492
-0.113620050752 0.00399526904864
-0.113009190264 0.00399229980837
-0.112398329777 0.00398939630591
-0.111787469289 0.00398655869288
-0.111176608801 0.00398378712075
-0.110565748313 0.00398108174081
-0.109954887825 0.00397844270416
-0.109344027337 0.00397587016169
-0.108733166849 0.00397336426407
-0.108122306361 0.00397092516174
-0.107511445873 0.00396855300489
-0.106900585385 0.00396624794348
-0.106289724897 0.00396401012717
-0.105678864409 0.00396183970534
-0.105068003922 0.00395973682707
-0.104457143434 0.00395770164113
-0.103846282946 0.00395573429596
-0.103235422458 0.00395383493964
-0.10262456197 0.00395200371991
-0.102013701482 0.00395024078412
-0.101402840994 0.00394854627922
-0.100791980506 0.00394692035176
-0.100181120018 0.00394536314787
-0.0995702595303 0.00394387481321
-0.0989593990424 0.00394245549299
-0.0983485385545 0.00394110533196
-0.0977376780666 0.00393982447433
-0.0971268175787 0.00393861306383
-0.0965159570907 0.00393747124363
-0.0959050966028 0.00393639915636
-0.0952942361149 0.00393539694405
-0.094683375627 0.00393446474816
-0.0940725151391 0.00393360270952
-0.0934616546512 0.00393281096832
-0.0928507941632 0.00393208966409
-0.0922399336753 0.00393143893568
-0.0916290731874 0.00393085892124
-0.0910182126995 0.00393034975819
-0.0904073522116 0.0039299115832
-0.0897964917237 0.00392954453217
-0.0891856312358 0.00392924874019
-0.0885747707478 0.00392902434154
-0.0879639102599 0.00392887146966
-0.087353049772 0.00392879025708
-0.0867421892841 0.00392878083548
-0.0861313287962 0.00392884333559
-0.0855204683083 0.00392897788717
-0.0849096078203 0.00392918461904
-0.0842987473324 0.00392946365899
-0.0836878868445 0.00392981513376
-0.0830770263566 0.00393023916904
-0.0824661658687 0.00393073588944
-0.0818553053808 0.00393130541842
-0.0812444448928 0.00393194787828
-0.0806335844049 0.00393266339016
-0.080022723917 0.00393345207395
-0.0794118634291 0.00393431404832
-0.0788010029412 0.00393524943062
-0.0781901424533 0.0039362583369
-0.0775792819653 0.00393734088186
-0.0769684214774 0.00393849717879
-0.0763575609895 0.00393972733959
-0.0757467005016 0.00394103147466
-0.0751358400137 0.00394240969294
-0.0745249795258 0.00394386210179
-0.0739141190378 0.00394538880705
-0.0733032585499 0.00394698991289
-0.072692398062 0.00394866552187
-0.0720815375741 0.00395041573484
-0.0714706770862 0.00395224065091
-0.0708598165983 0.00395414036743
-0.0702489561104 0.0039561149799
-0.0696380956224 0.00395816458198
-0.0690272351345 0.00396028926542
-0.0684163746466 0.00396248912001
-0.0678055141587 0.00396476423355
-0.0671946536708 0.00396711469176
-0.0665837931829 0.00396954057832
-0.0659729326949 0.00397204197472
-0.065362072207 0.00397461896027
-0.0647512117191 0.00397727161206
-0.0641403512312 0.00398000000485
-0.0635294907433 0.00398280421108
-0.0629186302554 0.00398568430078
-0.0623077697674 0.00398864034151
-0.0616969092795 0.00399167239834
-0.0610860487916 0.00399478053378
-0.0604751883037 0.0039979648077
-0.0598643278158 0.0040012252773
-0.0592534673279 0.00400456199703
-0.0586426068399 0.00400797501854
-0.058031746352 0.00401146439062
-0.0574208858641 0.00401503015915
-0.0568100253762 0.00401867236701
-0.0561991648883 0.00402239105401
-0.0555883044004 0.00402618625687
-0.0549774439124 0.00403005800911
-0.0543665834245 0.00403400634099
-0.0537557229366 0.00403803127947
-0.0531448624487 0.00404213284808
-0.0525340019608 0.00404631106692
-0.0519231414729 0.00405056595253
-0.051312280985 0.00405489751784
-0.050701420497 0.0040593057721
-0.0500905600091 0.00406379072077
-0.0494796995212 0.00406835236549
-0.0488688390333 0.00407299070396
-0.0482579785454 0.00407770572989
-0.0476471180575 0.00408249743288
-0.0470362575695 0.00408736579838
-0.0464253970816 0.00409231080755
-0.0458145365937 0.00409733243724
-0.0452036761058 0.00410243065985
-0.0445928156179 0.00410760544325
-0.04398195513 0.00411285675069
-0.043371094642 0.00411818454074
-0.0427602341541 0.00412358876714
-0.0421493736662 0.00412906937874
-0.0415385131783 0.00413462631937
-0.0409276526904 0.0041402595278
-0.0403167922025 0.00414596893757
-0.0397059317145 0.00415175447693
-0.0390950712266 0.00415761606871
-0.0384842107387 0.00416355363024
-0.0378733502508 0.0041695670732
-0.0372624897629 0.00417565630357
-0.036651629275 0.00418182122145
-0.0360407687871 0.004188061721
-0.0354299082991 0.00419437769028
-0.0348190478112 0.00420076901118
-0.0342081873233 0.00420723555925
-0.0335973268354 0.00421377720361
-0.0329864663475 0.0042203938068
-0.0323756058596 0.0042270852247
-0.0317647453716 0.00423385130634
-0.0311538848837 0.0042406918938
-0.0305430243958 0.0042476068221
-0.0299321639079 0.00425459591901
-0.02932130342 0.00426165900497
-0.0287104429321 0.00426879589288
-0.0280995824441 0.00427600638805
-0.0274887219562 0.00428329028797
-0.0268778614683 0.00429064738219
-0.0262670009804 0.00429807745221
-0.0256561404925 0.00430558027127
-0.0250452800046 0.00431315560421
-0.0244344195166 0.00432080320734
-0.0238235590287 0.00432852282826
-0.0232126985408 0.00433631420569
-0.0226018380529 0.0043441770693
-0.021990977565 0.00435211113959
-0.0213801170771 0.00436011612764
-0.0207692565891 0.004368191735
-0.0201583961012 0.00437633765348
-0.0195475356133 0.00438455356501
-0.0189366751254 0.00439283914138
-0.0183258146375 0.00440119404413
-0.0177149541496 0.00440961792433
-0.0171040936617 0.00441811042238
-0.0164932331737 0.00442667116784
-0.0158823726858 0.00443529977919
-0.0152715121979 0.00444399586367
-0.01466065171 0.00445275901705
-0.0140497912221 0.00446158882342
-0.0134389307342 0.00447048485502
-0.0128280702462 0.00447944667193
-0.0122172097583 0.00448847382196
-0.0116063492704 0.00449756584036
-0.0109954887825 0.0045067222496
-0.0103846282946 0.00451594255915
-0.00977376780666 0.00452522626525
-0.00916290731874 0.00453457285068
-0.00855204683083 0.00454398178446
-0.00794118634291 0.00455345252169
-0.00733032585499 0.00456298450324
-0.00671946536708 0.0045725771555
-0.00610860487916 0.00458222989015
-0.00549774439124 0.00459194210387
-0.00488688390333 0.00460171317809
-0.00427602341541 0.00461154247869
-0.0036651629275 0.00462142935578
-0.00305430243958 0.00463137314335
-0.00244344195166 0.00464137315904
-0.00183258146375 0.00465142870382
-0.00122172097583 0.0046615390617
-0.000610860487916 0.00467170349944
0.0 0.00468192126623
0.00160529707243 0.00470892667676
0.00321059414487 0.00473610179344
0.0048158912173 0.00476344781115
0.00642118828974 0.00479096593441
0.00802648536217 0.00481865737752
0.00963178243461 0.0048465233646
0.011237079507 0.00487456512972
0.0128423765795 0.00490278391694
0.0144476736519 0.00493118098049
0.0160529707243 0.00495975758477
0.0176582677968 0.00498851500453
0.0192635648692 0.00501745452492
0.0208688619416 0.00504657744159
0.0224741590141 0.00507588506082
0.0240794560865 0.00510537869959
0.025684753159 0.00513505968569
0.0272900502314 0.00516492935786
0.0288953473038 0.00519498906582
0.0305006443763 0.00522524017046
0.0321059414487 0.00525568404387
0.0337112385211 0.00528632206952
0.0353165355936 0.00531715564231
0.036921832666 0.00534818616872
0.0385271297384 0.0053794150669
0.0401324268109 0.00541084376678
0.0417377238833 0.00544247371023
0.0433430209557 0.00547430635111
0.0449483180282 0.00550634315543
0.0465536151006 0.00553858560145
0.048158912173 0.00557103517982
0.0497642092455 0.00560369339369
0.0513695063179 0.0056365617588
0.0529748033903 0.00566964180368
0.0545801004628 0.00570293506971
0.0561853975352 0.00573644311125
0.0577906946076 0.00577016749582
0.0593959916801 0.00580410980417
0.0610012887525 0.00583827163045
0.0626065858249 0.00587265458233
0.0642118828974 0.00590726028114
0.0658171799698 0.00594209036198
0.0674224770423 0.00597714647391
0.0690277741147 0.00601243028002
0.0706330711871 0.00604794345765
0.0722383682596 0.00608368769847
0.073843665332 0.00611966470863
0.0754489624044 0.00615587620896
0.0770542594769 0.00619232393505
0.0786595565493 0.00622900963743
0.0802648536217 0.00626593508174
0.0818701506942 0.00630310204885
0.0834754477666 0.00634051233502
0.085080744839 0.00637816775207
0.0866860419115 0.00641607012754
0.0882913389839 0.00645422130483
0.0898966360563 0.0064926231434
0.0915019331288 0.00653127751887
0.0931072302012 0.00657018632327
0.0947125272736 0.00660935146513
0.0963178243461 0.0066487748697
0.0979231214185 0.0066884584791
0.0995284184909 0.00672840425251
0.101133715563 0.00676861416633
0.102739012636 0.00680909021437
0.104344309708 0.00684983440802
0.105949606781 0.00689084877645
0.107554903853 0.00693213536677
0.109160200926 0.00697369624427
0.110765497998 0.00701553349252
0.11237079507 0.00705764921366
0.113976092143 0.00710004552852
0.115581389215 0.00714272457686
0.117186686288 0.00718568851756
0.11879198336 0.00722893952882
0.120397280433 0.00727247980833
0.122002577505 0.00731631157356
0.123607874577 0.00736043706188
0.12521317165 0.00740485853082
0.126818468722 0.00744957825829
0.128423765795 0.00749459854278
0.130029062867 0.00753992170356
0.13163435994 0.00758555008095
0.133239657012 0.00763148603652
0.134844954085 0.00767773195331
0.136450251157 0.00772429023609
0.138055548229 0.00777116331157
0.139660845302 0.00781835362863
0.141266142374 0.00786586365859
0.142871439447 0.00791369589545
0.144476736519 0.00796185285611
0.146082033592 0.00801033708063
0.147687330664 0.0080591511325
0.149292627736 0.0081082975989
0.150897924809 0.00815777909091
0.152503221881 0.00820759824383
0.154108518954 0.00825775771743
0.155713816026 0.00830826019621
0.157319113099 0.00835910838967
0.158924410171 0.00841030503259
0.160529707243 0.00846185288535
0.162135004316 0.00851375473415
0.163740301388 0.00856601339132
0.165345598461 0.00861863169566
0.166950895533 0.00867161251266
0.168556192606 0.00872495873485
0.170161489678 0.0087786732821
0.171766786751 0.0088327591019
0.173372083823 0.00888721916969
0.174977380895 0.0089420564892
0.176582677968 0.0089972740927
0.17818797504 0.00905287504142
0.179793272113 0.0091088624258
0.181398569185 0.00916523936585
0.183003866258 0.00922200901151
0.18460916333 0.00927917454295
0.186214460402 0.00933673917095
0.187819757475 0.00939470613725
0.189425054547 0.00945307871488
0.19103035162 0.00951186020855
0.192635648692 0.00957105395499
0.194240945765 0.00963066332337
0.195846242837 0.0096906917156
0.197451539909 0.00975114256679
0.199056836982 0.00981201934558
0.200662134054 0.00987332555457
0.202267431127 0.00993506473067
0.203872728199 0.00999724044558
0.205478025272 0.0100598563061
0.207083322344 0.0101229159547
0.208688619416 0.0101864230697
0.210293916489 0.0102503813659
0.211899213561 0.010314794595
0.213504510634 0.0103796665458
0.215109807706 0.0104450010451
0.216715104779 0.0105108019578
0.218320401851 0.0105770731872
0.219925698924 0.0106438186759
0.221530995996 0.0107110424062
0.223136293068 0.0107787484003
0.224741590141 0.0108469407207
0.226346887213 0.0109156234714
0.227952184286 0.0109848007976
0.229557481358 0.0110544768866
0.231162778431 0.0111246559682
0.232768075503 0.0111953423154
0.234373372575 0.0112665402447
0.235978669648 0.0113382541166
0.23758396672 0.0114104883364
0.239189263793 0.0114832473547
0.240794560865 0.0115565356677
0.242399857938 0.011630357818
0.24400515501 0.0117047183951
0.245610452082 0.0117796220362
0.247215749155 0.0118550734262
0.248821046227 0.011931077299
0.2504263433 0.0120076384378
0.252031640372 0.0120847616755
0.253636937445 0.0121624518959
0.255242234517 0.0122407140337
0.25684753159 0.0123195530755
0.258452828662 0.0123989740605
0.260058125734 0.012478982081
0.261663422807 0.0125595822831
0.263268719879 0.0126407798676
0.264874016952 0.0127225800903
0.266479314024 0.0128049882632
0.268084611097 0.0128880097547
0.269689908169 0.0129716499908
0.271295205241 0.0130559144555
0.272900502314 0.0131408086918
0.274505799386 0.0132263383022
0.276111096459 0.0133125089499
0.277716393531 0.013399326359
0.279321690604 0.0134867963159
0.280926987676 0.0135749246697
0.282532284748 0.0136637173332
0.284137581821 0.0137531802837
0.285742878893 0.0138433195638
0.287348175966 0.0139341412825
0.288953473038 0.0140256516158
0.290558770111 0.0141178568077
0.292164067183 0.0142107631711
0.293769364256 0.0143043770889
0.295374661328 0.0143987050145
0.2969799584 0.0144937534734
0.298585255473 0.0145895290634
0.300190552545 0.0146860384563
0.301795849618 0.0147832883984
0.30340114669 0.0148812857119
0.305006443763 0.0149800372956
0.306611740835 0.0150795501261
0.308217037907 0.0151798312588
0.30982233498 0.0152808878293
0.311427632052 0.015382727054
0.313032929125 0.0154853562315
0.314638226197 0.0155887827438
0.31624352327 0.0156930140575
0.317848820342 0.0157980577245
0.319454117414 0.0159039213838
0.321059414487 0.0160106127626
0.322664711559 0.016118139677
0.324270008632 0.016226510034
0.325875305704 0.0163357318323
0.327480602777 0.016445813164
0.329085899849 0.0165567622153
0.330691196922 0.0166685872686
0.332296493994 0.0167812967033
0.333901791066 0.0168948989973
0.335507088139 0.0170094027288
0.337112385211 0.0171248165774
0.338717682284 0.0172411493254
0.340322979356 0.0173584098597
0.341928276429 0.0174766071732
0.343533573501 0.0175957503662
0.345138870573 0.0177158486482
0.346744167646 0.0178369113391
0.348349464718 0.0179589478714
0.349954761791 0.0180819677915
0.351560058863 0.0182059807613
0.353165355936 0.0183309965602
0.354770653008 0.0184570250867
0.35637595008 0.0185840763603
0.357981247153 0.018712160523
0.359586544225 0.0188412878416
0.361191841298 0.0189714687092
0.36279713837 0.0191027136474
0.364402435443 0.0192350333079
0.366007732515 0.0193684384749
0.367613029588 0.0195029400668
0.36921832666 0.0196385491385
0.370823623732 0.0197752768833
0.372428920805 0.019913134635
0.374034217877 0.0200521338705
0.37563951495 0.0201922862114
0.377244812022 0.0203336034267
0.378850109095 0.0204760974349
0.380455406167 0.0206197803065
0.382060703239 0.0207646642663
0.383666000312 0.0209107616957
0.385271297384 0.0210580851355
0.386876594457 0.0212066472881
0.388481891529 0.0213564610203
0.390087188602 0.0215075393657
0.391692485674 0.0216598955278
0.393297782746 0.0218135428821
0.394903079819 0.0219684949796
0.396508376891 0.0221247655489
0.398113673964 0.0222823684999
0.399718971036 0.0224413179258
0.401324268109 0.022601628107
0.402929565181 0.0227633135137
0.404534862254 0.022926388809
0.406140159326 0.0230908688524
0.407745456398 0.0232567687026
0.409350753471 0.0234241036213
0.410956050543 0.0235928890763
0.412561347616 0.023763140745
0.414166644688 0.023934874518
0.415771941761 0.0241081065025
0.417377238833 0.0242828530263
0.418982535905 0.0244591306413
0.420587832978 0.0246369561273
0.42219313005 0.0248163464961
0.423798427123 0.0249973189954
0.425403724195 0.0251798911128
0.427009021268 0.0253640805798
0.42861431834 0.0255499053766
0.430219615412 0.0257373837359
0.431824912485 0.0259265341474
0.433430209557 0.0261173753626
0.43503550663 0.0263099263989
0.436640803702 0.0265042065451
0.438246100775 0.0267002353653
0.439851397847 0.0268980327045
0.44145669492 0.0270976186934
0.443061991992 0.0272990137534
0.444667289064 0.027502238602
0.446272586137 0.0277073142582
0.447877883209 0.0279142620477
0.449483180282 0.028123103609
0.451088477354 0.0283338608986
0.452693774427 0.0285465561972
0.454299071499 0.0287612121156
0.455904368571 0.0289778516005
0.457509665644 0.0291964979414
0.459114962716 0.0294171747764
0.460720259789 0.0296399060992
0.462325556861 0.0298647162654
0.463930853934 0.0300916299996
0.465536151006 0.0303206724023
0.467141448078 0.0305518689571
0.468746745151 0.0307852455382
0.470352042223 0.0310208284175
0.471957339296 0.0312586442728
0.473562636368 0.0314987201952
0.475167933441 0.0317410836974
0.476773230513 0.031985762722
0.478378527586 0.0322327856497
0.479983824658 0.0324821813083
0.48158912173 0.032733978981
0.483194418803 0.0329882084161
0.484799715875 0.0332448998359
0.486405012948 0.0335040839464
0.48801031002 0.0337657919467
0.489615607093 0.0340300555396
0.491220904165 0.0342969069412
0.492826201237 0.0345663788919
0.49443149831 0.0348385046668
0.496036795382 0.0351133180868
0.497642092455 0.0353908535303
0.499247389527 0.0356711459441
0.5008526866 0.0359542308558
0.502457983672 0.036240144386
0.504063280744 0.0365289232604
0.505668577817 0.0368206048229
0.507273874889 0.0371152270491
0.508879171962 0.037412828559
0.510484469034 0.0377134486317
0.512089766107 0.038017127219
0.513695063179 0.0383239049604
0.515300360252 0.0386338231981
0.516905657324 0.0389469239919
0.518510954396 0.0392632501358
0.520116251469 0.0395828451735
0.521721548541 0.0399057534157
0.523326845614 0.0402320199568
0.524932142686 0.0405616906928
0.526537439759 0.040894812339
0.528142736831 0.0412314324494
0.529748033903 0.0415715994349
0.531353330976 0.0419153625836
0.532958628048 0.0422627720807
0.534563925121 0.0426138790296
0.536169222193 0.0429687354728
0.537774519266 0.0433273944146
0.539379816338 0.043689909843
0.54098511341 0.0440563367535
0.542590410483 0.0444267311731
0.544195707555 0.0448011501846
0.545801004628 0.0451796519523
0.5474063017 0.0455622957481
0.549011598773 0.0459491419786
0.550616895845 0.0463402522126
0.552222192917 0.0467356892098
0.55382748999 0.0471355169504
0.555432787062 0.0475398006655
0.557038084135 0.0479486068681
0.558643381207 0.0483620033857
0.56024867828 0.0487800593934
0.561853975352 0.0492028454484
0.563459272425 0.0496304335253
0.565064569497 0.0500628970527
0.566669866569 0.0505003109507
0.568275163642 0.0509427516702
0.569880460714 0.0513902972329
0.571485757787 0.0518430272725
0.573091054859 0.052301023078
0.574696351932 0.0527643676379
0.576301649004 0.0532331456855
0.577906946076 0.0537074437465
0.579512243149 0.0541873501881
0.581117540221 0.0546729552688
0.582722837294 0.0551643511912
0.584328134366 0.0556616321558
0.585933431439 0.0561648944169
0.587538728511 0.0566742363405
0.589144025583 0.0571897584637
0.590749322656 0.0577115635575
0.592354619728 0.0582397566901
0.593959916801 0.0587744452939
0.595565213873 0.0593157392341
0.597170510946 0.0598637508801
0.598775808018 0.0604185951793
0.600381105091 0.0609803897342
0.601986402163 0.0615492548814
0.603591699235 0.0621253137742
0.605196996308 0.0627086924686
0.60680229338 0.0632995200116
0.608407590453 0.0638979285337
0.610012887525 0.0645040533445
0.611618184598 0.0651180330324
0.61322348167 0.065740009568
0.614828778742 0.0663701284112
0.616434075815 0.0670085386234
0.618039372887 0.0676553929833
0.61964466996 0.068310848108
0.621249967032 0.0689750645791
0.622855264105 0.0696482070728
0.624460561177 0.0703304444973
0.626065858249 0.0710219501344
0.627671155322 0.0717229017874
0.629276452394 0.0724334819361
0.630881749467 0.0731538778969
0.632487046539 0.0738842819914
0.634092343612 0.0746248917216
0.635697640684 0.0753759099524
0.637302937757 0.076137545103
0.638908234829 0.0769100113464
0.640513531901 0.0776935288183
0.642118828974 0.0784883238346
0.643724126046 0.0792946291204
0.645329423119 0.0801126840482
0.646934720191 0.0809427348879
0.648540017264 0.081785035069
0.650145314336 0.0826398454548
0.651750611408 0.0835074346296
0.653355908481 0.0843880792009
0.654961205553 0.0852820641156
0.656566502626 0.0861896829924
0.658171799698 0.0871112384703
0.659777096771 0.088047042576
0.661382393843 0.0889974171089
0.662987690915 0.0899626940469
0.664592987988 0.0909432159731
0.66619828506 0.0919393365251
0.667803582133 0.0929514208691
0.669408879205 0.0939798461988
0.671014176278 0.0950250022619
0.67261947335 0.0960872919164
0.674224770423 0.0971671317176
0.675830067495 0.0982649525382
0.677435364567 0.099381200225
0.67904066164 0.100516336293
0.680645958712 0.10167083866
0.682251255785 0.102845202427
0.683856552857 0.104039940703
0.68546184993 0.105255585482
0.687067147002 0.106492688576
0.688672444074 0.1077518226
0.690277741147 0.109033582029
0.691883038219 0.110338584316
0.693488335292 0.111667471086
0.695093632364 0.113020909408
0.696698929437 0.114399593155
0.698304226509 0.115804244453
0.699909523581 0.117235615234
0.701514820654 0.118694488894
0.703120117726 0.120181682076
0.704725414799 0.121698046572
0.706330711871 0.123244471376
0.707936008944 0.124821884881
0.709541306016 0.126431257249
0.711146603089 0.128073602962
0.712751900161 0.129749983574
0.714357197233 0.131461510675
0.715962494306 0.133209349114
0.717567791378 0.134994720467
0.719173088451 0.13681890681
0.720778385523 0.138683254814
0.722383682596 0.140589180194
0.723988979668 0.142538172555
0.72559427674 0.144531800682
0.727199573813 0.146571718313
0.728804870885 0.14865967046
0.730410167958 0.150797500347
0.73201546503 0.152987157016
0.733620762103 0.155230703715
0.735226059175 0.157530327141
0.736831356247 0.159888347655
0.73843665332 0.162307230604
0.740041950392 0.164789598891
0.741647247465 0.167338246963
0.743252544537 0.16995615643
0.74485784161 0.172646513536
0.746463138682 0.175412728772
0.748068435755 0.178258458955
0.749673732827 0.181187632153
0.751279029899 0.184204475936
0.752884326972 0.187313549501
0.754489624044 0.19051978033
0.756094921117 0.19382850622
0.757700218189 0.197245523639
0.759305515262 0.200777143649
0.760910812334 0.204430256878
0.762516109406 0.2082124094
0.764121406479 0.212131891873
0.765726703551 0.216197844856
0.767332000624 0.220420384089
0.768937297696 0.224810750559
0.770542594769 0.229381491653
0.772147891841 0.234146681693
0.773753188913 0.239122192889
0.775358485986 0.244326031642
0.776963783058 0.249778760683
0.778569080131 0.255504035607
0.780174377203 0.261529296448
0.781779674276 0.267886673258
0.783384971348 0.274614193415
0.784990268421 0.281757424669
0.786595565493 0.289371765201
0.788200862565 0.297525726167
0.789806159638 0.306305796458
0.79141145671 0.315823949899
0.793016753783 0.326229825915
0.794622050855 0.337731798116
0.796227347928 0.350636638072
0.797832645 0.365433578851
0.799437942072 0.383007696634
0.801043239145 0.405387867449


==> figuresAndData/dataForConditionalVarianceLaplaceProb0pt4.tex <==
-13.5 0.111453299026
-13.473 0.111453299026
-13.446 0.111453299026
-13.419 0.111453299026
-13.392 0.111453299026
-13.365 0.111453299026
-13.338 0.111453299026
-13.311 0.111453299026
-13.284 0.111453299026
-13.257 0.111453299026
-13.23 0.111453299026
-13.203 0.111453299026
-13.176 0.111453299026
-13.149 0.111453299026
-13.122 0.111453299026
-13.095 0.111453299026
-13.068 0.111453299026
-13.041 0.111453299026
-13.014 0.111453299026
-12.987 0.111453299026
-12.96 0.111453299026
-12.933 0.111453299026
-12.906 0.111453299026
-12.879 0.111453299026
-12.852 0.111453299026
-12.825 0.111453299026
-12.798 0.111453299026
-12.771 0.111453299026
-12.744 0.111453299026
-12.717 0.111453299026
-12.69 0.111453299026
-12.663 0.111453299026
-12.636 0.111453299026
-12.609 0.111453299026
-12.582 0.111453299026
-12.555 0.111453299026
-12.528 0.111453299026
-12.501 0.111453299026
-12.474 0.111453299026
-12.447 0.111453299026
-12.42 0.111453299026
-12.393 0.111453299026
-12.366 0.111453299026
-12.339 0.111453299026
-12.312 0.111453299026
-12.285 0.111453299026
-12.258 0.111453299026
-12.231 0.111453299026
-12.204 0.111453299026
-12.177 0.111453299026
-12.15 0.111453299026
-12.123 0.111453299026
-12.096 0.111453299026
-12.069 0.111453299026
-12.042 0.111453299026
-12.015 0.111453299026
-11.988 0.111453299026
-11.961 0.111453299026
-11.934 0.111453299026
-11.907 0.111453299026
-11.88 0.111453299026
-11.853 0.111453299026
-11.826 0.111453299026
-11.799 0.111453299026
-11.772 0.111453299026
-11.745 0.111453299026
-11.718 0.111453299026
-11.691 0.111453299026
-11.664 0.111453299026
-11.637 0.111453299026
-11.61 0.111453299026
-11.583 0.111453299026
-11.556 0.111453299026
-11.529 0.111453299026
-11.502 0.111453299026
-11.475 0.111453299026
-11.448 0.111453299026
-11.421 0.111453299026
-11.394 0.111453299026
-11.367 0.111453299026
-11.34 0.111453299026
-11.313 0.111453299026
-11.286 0.111453299026
-11.259 0.111453299026
-11.232 0.111453299026
-11.205 0.111453299026
-11.178 0.111453299026
-11.151 0.111453299026
-11.124 0.111453299026
-11.097 0.111453299026
-11.07 0.111453299026
-11.043 0.111453299026
-11.016 0.111453299026
-10.989 0.111453299026
-10.962 0.111453299026
-10.935 0.111453299026
-10.908 0.111453299026
-10.881 0.111453299026
-10.854 0.111453299026
-10.827 0.111453299026
-10.8 0.111453299026
-10.773 0.111453299025
-10.746 0.111453299025
-10.719 0.111453299025
-10.692 0.111453299025
-10.665 0.111453299025
-10.638 0.111453299025
-10.611 0.111453299025
-10.584 0.111453299025
-10.557 0.111453299025
-10.53 0.111453299025
-10.503 0.111453299024
-10.476 0.111453299024
-10.449 0.111453299024
-10.422 0.111453299024
-10.395 0.111453299024
-10.368 0.111453299024
-10.341 0.111453299023
-10.314 0.111453299023
-10.287 0.111453299023
-10.26 0.111453299023
-10.233 0.111453299022
-10.206 0.111453299022
-10.179 0.111453299022
-10.152 0.111453299021
-10.125 0.111453299021
-10.098 0.11145329902
-10.071 0.11145329902
-10.044 0.111453299019
-10.017 0.111453299019
-9.99 0.111453299018
-9.963 0.111453299018
-9.936 0.111453299017
-9.909 0.111453299016
-9.882 0.111453299015
-9.855 0.111453299015
-9.828 0.111453299014
-9.801 0.111453299013
-9.774 0.111453299012
-9.747 0.11145329901
-9.72 0.111453299009
-9.693 0.111453299008
-9.666 0.111453299006
-9.639 0.111453299005
-9.612 0.111453299003
-9.585 0.111453299001
-9.558 0.111453298999
-9.531 0.111453298997
-9.504 0.111453298995
-9.477 0.111453298992
-9.45 0.11145329899
-9.423 0.111453298987
-9.396 0.111453298984
-9.369 0.11145329898
-9.342 0.111453298977
-9.315 0.111453298973
-9.288 0.111453298969
-9.261 0.111453298964
-9.234 0.111453298959
-9.207 0.111453298954
-9.18 0.111453298948
-9.153 0.111453298942
-9.126 0.111453298936
-9.099 0.111453298929
-9.072 0.111453298921
-9.045 0.111453298913
-9.018 0.111453298904
-8.991 0.111453298895
-8.964 0.111453298884
-8.937 0.111453298873
-8.91 0.111453298861
-8.883 0.111453298848
-8.856 0.111453298835
-8.829 0.11145329882
-8.802 0.111453298804
-8.775 0.111453298786
-8.748 0.111453298768
-8.721 0.111453298747
-8.694 0.111453298726
-8.667 0.111453298702
-8.64 0.111453298677
-8.613 0.11145329865
-8.586 0.111453298621
-8.559 0.111453298589
-8.532 0.111453298556
-8.505 0.111453298519
-8.478 0.11145329848
-8.451 0.111453298437
-8.424 0.111453298392
-8.397 0.111453298342
-8.37 0.111453298289
-8.343 0.111453298232
-8.316 0.111453298171
-8.289 0.111453298105
-8.262 0.111453298033
-8.235 0.111453297957
-8.208 0.111453297874
-8.181 0.111453297785
-8.154 0.111453297689
-8.127 0.111453297585
-8.1 0.111453297474
-8.073 0.111453297354
-8.046 0.111453297225
-8.019 0.111453297086
-7.992 0.111453296937
-7.965 0.111453296776
-7.938 0.111453296602
-7.911 0.111453296415
-7.884 0.111453296214
-7.857 0.111453295997
-7.83 0.111453295764
-7.803 0.111453295513
-7.776 0.111453295243
-7.749 0.111453294952
-7.722 0.111453294639
-7.695 0.111453294301
-7.668 0.111453293938
-7.641 0.111453293548
-7.614 0.111453293127
-7.587 0.111453292674
-7.56 0.111453292187
-7.533 0.111453291662
-7.506 0.111453291097
-7.479 0.11145329049
-7.452 0.111453289836
-7.425 0.111453289132
-7.398 0.111453288374
-7.371 0.111453287559
-7.344 0.111453286682
-7.317 0.111453285738
-7.29 0.111453284722
-7.263 0.111453283629
-7.236 0.111453282452
-7.209 0.111453281187
-7.182 0.111453279825
-7.155 0.11145327836
-7.128 0.111453276784
-7.101 0.111453275088
-7.074 0.111453273263
-7.047 0.111453271301
-7.02 0.11145326919
-6.993 0.111453266919
-6.966 0.111453264476
-6.939 0.111453261848
-6.912 0.111453259022
-6.885 0.111453255982
-6.858 0.111453252712
-6.831 0.111453249196
-6.804 0.111453245414
-6.777 0.111453241347
-6.75 0.111453236974
-6.723 0.111453232271
-6.696 0.111453227214
-6.669 0.111453221776
-6.642 0.111453215929
-6.615 0.111453209643
-6.588 0.111453202884
-6.561 0.111453195617
-6.534 0.111453187805
-6.507 0.111453179407
-6.48 0.111453170379
-6.453 0.111453160674
-6.426 0.111453150242
-6.399 0.11145313903
-6.372 0.111453126978
-6.345 0.111453114025
-6.318 0.111453100104
-6.291 0.111453085143
-6.264 0.111453069065
-6.237 0.111453051788
-6.21 0.111453033222
-6.183 0.111453013273
-6.156 0.111452991838
-6.129 0.111452968807
-6.102 0.111452944064
-6.075 0.111452917481
-6.048 0.111452888923
-6.021 0.111452858245
-5.994 0.111452825291
-5.967 0.111452789893
-5.94 0.111452751872
-5.913 0.111452711036
-5.886 0.111452667177
-5.859 0.111452620076
-5.832 0.111452569493
-5.805 0.111452515175
-5.778 0.111452456849
-5.751 0.11145239422
-5.724 0.111452326977
-5.697 0.111452254782
-5.67 0.111452177274
-5.643 0.111452094067
-5.616 0.111452004745
-5.589 0.111451908866
-5.562 0.111451805951
-5.535 0.111451695493
-5.508 0.111451576942
-5.481 0.111451449714
-5.454 0.111451313181
-5.427 0.111451166669
-5.4 0.11145100946
-5.373 0.11145084078
-5.346 0.111450659803
-5.319 0.111450465644
-5.292 0.111450257355
-5.265 0.11145003392
-5.238 0.111449794253
-5.211 0.111449537188
-5.184 0.111449261481
-5.157 0.111448965796
-5.13 0.111448648707
-5.103 0.111448308685
-5.076 0.111447944093
-5.049 0.111447553183
-5.022 0.11144713408
-4.995 0.111446684782
-4.968 0.111446203144
-4.941 0.111445686872
-4.914 0.111445133515
-4.887 0.111444540449
-4.86 0.111443904867
-4.833 0.11144322377
-4.806 0.111442493951
-4.779 0.111441711979
-4.752 0.111440874189
-4.725 0.111439976663
-4.698 0.111439015213
-4.671 0.111437985362
-4.644 0.11143688233
-4.617 0.111435701008
-4.59 0.111434435936
-4.563 0.111433081286
-4.536 0.11143163083
-4.509 0.111430077919
-4.482 0.111428415453
-4.455 0.111426635851
-4.428 0.111424731021
-4.401 0.111422692324
-4.374 0.111420510543
-4.347 0.11141817584
-4.32 0.11141567772
-4.293 0.111413004985
-4.266 0.111410145691
-4.239 0.111407087101
-4.212 0.111403815632
-4.185 0.111400316799
-4.158 0.111396575164
-4.131 0.111392574269
-4.104 0.111388296577
-4.077 0.111383723398
-4.05 0.111378834822
-4.023 0.111373609641
-3.996 0.111368025265
-3.969 0.111362057641
-3.942 0.111355681159
-3.915 0.111348868558
-3.888 0.111341590824
-3.861 0.111333817082
-3.834 0.111325514486
-3.807 0.111316648094
-3.78 0.111307180749
-3.753 0.111297072938
-3.726 0.11128628266
-3.699 0.11127476527
-3.672 0.111262473328
-3.645 0.111249356436
-3.618 0.111235361058
-3.591 0.111220430347
-3.564 0.111204503945
-3.537 0.111187517788
-3.51 0.111169403893
-3.483 0.111150090133
-3.456 0.111129500009
-3.429 0.1111075524
-3.402 0.111084161311
-3.375 0.111059235604
-3.348 0.111032678716
-3.321 0.111004388366
-3.294 0.110974256248
-3.267 0.110942167709
-3.24 0.110908001417
-3.213 0.110871629012
-3.186 0.11083291474
-3.159 0.110791715077
-3.132 0.110747878338
-3.105 0.110701244266
-3.078 0.110651643609
-3.051 0.110598897686
-3.024 0.110542817926
-2.997 0.110483205408
-2.97 0.110419850372
-2.943 0.110352531722
-2.916 0.110281016515
-2.889 0.110205059437
-2.862 0.110124402259
-2.835 0.110038773294
-2.808 0.109947886827
-2.781 0.10985144255
-2.754 0.109749124977
-2.727 0.109640602861
-2.7 0.109525528597
-2.673 0.109403537628
-2.646 0.109274247852
-2.619 0.109137259022
-2.592 0.108992152161
-2.565 0.10883848898
-2.538 0.108675811307
-2.511 0.108503640539
-2.484 0.108321477105
-2.457 0.108128799964
-2.43 0.107925066132
-2.403 0.10770971024
-2.376 0.107482144148
-2.349 0.107241756601
-2.322 0.106987912949
-2.295 0.106719954935
-2.268 0.106437200556
-2.241 0.106138944021
-2.214 0.10582445579
-2.187 0.105492982744
-2.16 0.105143748456
-2.133 0.104775953606
-2.106 0.104388776548
-2.079 0.103981374027
-2.052 0.103552882084
-2.025 0.103102417152
-1.998 0.102629077354
-1.971 0.102131944044
-1.944 0.101610083573
-1.917 0.101062549337
-1.89 0.100488384095
-1.863 0.0998866225905
-1.836 0.0992562944944
-1.809 0.0985964276852
-1.782 0.097906051887
-1.755 0.0971842026833
-1.728 0.0964299259234
-1.701 0.095642282538
-1.674 0.0948203537802
-1.647 0.0939632469024
-1.62 0.0930701012828
-1.593 0.0921400950074
-1.566 0.0911724519146
-1.539 0.0901664491018
-1.512 0.0891214248925
-1.485 0.088036787255
-1.458 0.0869120226602
-1.431 0.0857467053582
-1.404 0.0845405070473
-1.377 0.0832932069024
-1.35 0.0820047019197
-1.323 0.0806750175283
-1.296 0.0793043184073
-1.269 0.0778929194418
-1.242 0.0764412967367
-1.215 0.0749500986006
-1.188 0.0734201564017
-1.161 0.0718524951887
-1.134 0.0702483439608
-1.107 0.0686091454651
-1.08 0.0669365653943
-1.053 0.0652325008541
-1.026 0.063499087972
-0.999 0.061738708521
-0.972 0.0599539954435
-0.945 0.0581478371743
-0.918 0.0563233806823
-0.891 0.0544840331839
-0.864 0.0526334625165
-0.837 0.0507755962162
-0.81 0.0489146194017
-0.783 0.0470549716521
-0.756 0.0452013431555
-0.729 0.043358670526
-0.702 0.0415321328245
-0.675 0.0397271484865
-0.648 0.0379493740597
-0.621 0.0362047058994
-0.594 0.0344992862608
-0.567 0.0328395155916
-0.54 0.031232073274
-0.513 0.0296839496355
-0.486 0.02820249277
-0.459 0.0267954746583
-0.432 0.0254711823185
-0.405 0.0242385413806
-0.378 0.0231072817196
-0.351 0.0220881578227
-0.324 0.0211932407326
-0.297 0.0204363041312
-0.27 0.0198333350529
-0.243 0.019403210767
-0.216 0.0191685989761
-0.189 0.0191571609483
-0.162 0.0194031705657
-0.135 0.0199497140962
-0.108 0.0208517211697
-0.081 0.0221802304607
-0.054 0.0240285916123
-0.027 0.026521938745
0.0 0.0298327381143
0.000681100831688 0.0299286288128
0.00136220166338 0.0300248994533
0.00204330249506 0.0301215519528
0.00272440332675 0.0302185882405
0.00340550415844 0.0303160102581
0.00408660499013 0.03041381996
0.00476770582182 0.030512019313
0.0054488066535 0.0306106102967
0.00612990748519 0.0307095949037
0.00681100831688 0.0308089751394
0.00749210914857 0.0309087530223
0.00817320998026 0.0310089305842
0.00885431081194 0.03110950987
0.00953541164363 0.031210492938
0.0102165124753 0.0313118818602
0.010897613307 0.031413678722
0.0115787141387 0.0315158856225
0.0122598149704 0.0316185046748
0.0129409158021 0.0317215380059
0.0136220166338 0.0318249877567
0.0143031174654 0.0319288560825
0.0149842182971 0.0320331451527
0.0156653191288 0.0321378571513
0.0163464199605 0.0322429942767
0.0170275207922 0.032348558742
0.0177086216239 0.0324545527751
0.0183897224556 0.0325609786188
0.0190708232873 0.0326678385308
0.019751924119 0.0327751347843
0.0204330249506 0.0328828696674
0.0211141257823 0.0329910454838
0.021795226614 0.0330996645526
0.0224763274457 0.0332087292089
0.0231574282774 0.0333182418032
0.0238385291091 0.0334282047022
0.0245196299408 0.0335386202886
0.0252007307725 0.0336494909614
0.0258818316041 0.0337608191358
0.0265629324358 0.0338726072436
0.0272440332675 0.0339848577332
0.0279251340992 0.0340975730697
0.0286062349309 0.0342107557354
0.0292873357626 0.0343244082294
0.0299684365943 0.034438533068
0.030649537426 0.0345531327851
0.0313306382576 0.0346682099319
0.0320117390893 0.0347837670774
0.032692839921 0.0348998068084
0.0333739407527 0.0350163317296
0.0340550415844 0.0351333444639
0.0347361424161 0.0352508476526
0.0354172432478 0.0353688439552
0.0360983440795 0.0354873360501
0.0367794449112 0.0356063266342
0.0374605457428 0.0357258184237
0.0381416465745 0.0358458141536
0.0388227474062 0.0359663165784
0.0395038482379 0.0360873284718
0.0401849490696 0.0362088526276
0.0408660499013 0.0363308918588
0.041547150733 0.0364534489989
0.0422282515647 0.0365765269013
0.0429093523963 0.0367001284398
0.043590453228 0.0368242565088
0.0442715540597 0.0369489140234
0.0449526548914 0.0370741039193
0.0456337557231 0.0371998291539
0.0463148565548 0.0373260927052
0.0469959573865 0.0374528975732
0.0476770582182 0.0375802467794
0.0483581590498 0.037708143367
0.0490392598815 0.0378365904015
0.0497203607132 0.0379655909706
0.0504014615449 0.0380951481844
0.0510825623766 0.0382252651758
0.0517636632083 0.0383559451005
0.05244476404 0.0384871911374
0.0531258648717 0.0386190064885
0.0538069657034 0.0387513943797
0.054488066535 0.0388843580603
0.0551691673667 0.0390179008037
0.0558502681984 0.0391520259076
0.0565313690301 0.039286736694
0.0572124698618 0.0394220365096
0.0578935706935 0.039557928726
0.0585746715252 0.0396944167398
0.0592557723569 0.0398315039732
0.0599368731885 0.0399691938737
0.0606179740202 0.0401074899149
0.0612990748519 0.0402463955962
0.0619801756836 0.0403859144437
0.0626612765153 0.0405260500098
0.063342377347 0.0406668058738
0.0640234781787 0.0408081856422
0.0647045790104 0.0409501929487
0.065385679842 0.0410928314546
0.0660667806737 0.0412361048494
0.0667478815054 0.0413800168504
0.0674289823371 0.0415245712034
0.0681100831688 0.0416697716831
0.0687911840005 0.0418156220929
0.0694722848322 0.0419621262656
0.0701533856639 0.0421092880637
0.0708344864956 0.0422571113793
0.0715155873272 0.0424056001346
0.0721966881589 0.0425547582826
0.0728777889906 0.0427045898066
0.0735588898223 0.0428550987212
0.074239990654 0.0430062890721
0.0749210914857 0.043158164937
0.0756021923174 0.0433107304253
0.0762832931491 0.0434639896786
0.0769643939807 0.0436179468715
0.0776454948124 0.0437726062111
0.0783265956441 0.043927971938
0.0790076964758 0.0440840483263
0.0796887973075 0.0442408396842
0.0803698981392 0.0443983503539
0.0810509989709 0.0445565847126
0.0817320998026 0.0447155471721
0.0824132006342 0.0448752421797
0.0830943014659 0.0450356742185
0.0837754022976 0.0451968478075
0.0844565031293 0.0453587675022
0.085137603961 0.0455214378948
0.0858187047927 0.0456848636149
0.0864998056244 0.0458490493294
0.0871809064561 0.0460139997434
0.0878620072878 0.0461797196002
0.0885431081194 0.0463462136819
0.0892242089511 0.0465134868097
0.0899053097828 0.0466815438444
0.0905864106145 0.0468503896868
0.0912675114462 0.047020029278
0.0919486122779 0.0471904676
0.0926297131096 0.047361709676
0.0933108139413 0.047533760571
0.0939919147729 0.047706625392
0.0946730156046 0.0478803092886
0.0953541164363 0.0480548174534
0.096035217268 0.0482301551226
0.0967163180997 0.0484063275762
0.0973974189314 0.0485833401387
0.0980785197631 0.0487611981796
0.0987596205948 0.0489399071135
0.0994407214264 0.0491194724013
0.100121822258 0.0492998995499
0.10080292309 0.0494811941132
0.101484023922 0.0496633616925
0.102165124753 0.049846407937
0.102846225585 0.0500303385444
0.103527326417 0.0502151592613
0.104208427248 0.0504008758837
0.10488952808 0.0505874942577
0.105570628912 0.0507750202802
0.106251729743 0.0509634598989
0.106932830575 0.0511528191136
0.107613931407 0.0513431039761
0.108295032238 0.0515343205913
0.10897613307 0.0517264751174
0.109657233902 0.0519195737668
0.110338334733 0.0521136228067
0.111019435565 0.0523086285593
0.111700536397 0.052504597403
0.112381637229 0.0527015357726
0.11306273806 0.0528994501603
0.113743838892 0.0530983471161
0.114424939724 0.0532982332483
0.115106040555 0.0534991152247
0.115787141387 0.0537009997729
0.116468242219 0.053903893681
0.11714934305 0.0541078037983
0.117830443882 0.0543127370364
0.118511544714 0.0545187003693
0.119192645545 0.0547257008345
0.119873746377 0.0549337455337
0.120554847209 0.0551428416337
0.12123594804 0.0553529963666
0.121917048872 0.0555642170313
0.122598149704 0.0557765109938
0.123279250536 0.0559898856883
0.123960351367 0.0562043486176
0.124641452199 0.0564199073545
0.125322553031 0.056636569542
0.126003653862 0.0568543428947
0.126684754694 0.0570732351993
0.127365855526 0.0572932543156
0.128046956357 0.0575144081773
0.128728057189 0.0577367047932
0.129409158021 0.0579601522476
0.130090258852 0.0581847587016
0.130771359684 0.0584105323941
0.131452460516 0.0586374816423
0.132133561347 0.0588656148433
0.132814662179 0.0590949404744
0.133495763011 0.0593254670947
0.134176863843 0.0595572033457
0.134857964674 0.0597901579525
0.135539065506 0.0600243397249
0.136220166338 0.0602597575583
0.136901267169 0.0604964204349
0.137582368001 0.0607343374248
0.138263468833 0.0609735176869
0.138944569664 0.0612139704703
0.139625670496 0.0614557051154
0.140306771328 0.0616987310549
0.140987872159 0.061943057815
0.141668972991 0.062188695017
0.142350073823 0.0624356523777
0.143031174654 0.0626839397117
0.143712275486 0.0629335669316
0.144393376318 0.06318454405
0.14507447715 0.0634368811807
0.145755577981 0.0636905885398
0.146436678813 0.0639456764469
0.147117779645 0.0642021553271
0.147798880476 0.0644600357118
0.148479981308 0.0647193282402
0.14916108214 0.0649800436611
0.149842182971 0.0652421928338
0.150523283803 0.0655057867301
0.151204384635 0.0657708364355
0.151885485466 0.0660373531507
0.152566586298 0.0663053481934
0.15324768713 0.0665748329998
0.153928787961 0.066845819126
0.154609888793 0.0671183182499
0.155290989625 0.0673923421727
0.155972090457 0.0676679028206
0.156653191288 0.0679450122467
0.15733429212 0.0682236826325
0.158015392952 0.06850392629
0.158696493783 0.0687857556629
0.159377594615 0.0690691833294
0.160058695447 0.0693542220031
0.160739796278 0.0696408845355
0.16142089711 0.0699291839178
0.162101997942 0.0702191332828
0.162783098773 0.070510745907
0.163464199605 0.0708040352126
0.164145300437 0.0710990147697
0.164826401268 0.071395698298
0.1655075021 0.0716940996697
0.166188602932 0.0719942329109
0.166869703764 0.0722961122043
0.167550804595 0.0725997518916
0.168231905427 0.0729051664753
0.168913006259 0.0732123706215
0.16959410709 0.0735213791621
0.170275207922 0.0738322070973
0.170956308754 0.0741448695983
0.171637409585 0.0744593820093
0.172318510417 0.0747757598506
0.172999611249 0.0750940188211
0.17368071208 0.0754141748008
0.174361812912 0.0757362438537
0.175042913744 0.0760602422308
0.175724014576 0.0763861863722
0.176405115407 0.076714092911
0.177086216239 0.0770439786753
0.177767317071 0.077375860692
0.178448417902 0.0777097561891
0.179129518734 0.0780456825997
0.179810619566 0.0783836575642
0.180491720397 0.0787236989343
0.181172821229 0.0790658247759
0.181853922061 0.0794100533729
0.182535022892 0.07975640323
0.183216123724 0.0801048930768
0.183897224556 0.0804555418708
0.184578325387 0.0808083688018
0.185259426219 0.0811633932949
0.185940527051 0.0815206350146
0.186621627883 0.0818801138687
0.187302728714 0.0822418500123
0.187983829546 0.0826058638515
0.188664930378 0.0829721760479
0.189346031209 0.0833408075225
0.190027132041 0.0837117794604
0.190708232873 0.0840851133145
0.191389333704 0.0844608308107
0.192070434536 0.0848389539517
0.192751535368 0.0852195050224
0.193432636199 0.0856025065941
0.194113737031 0.0859879815296
0.194794837863 0.0863759529882
0.195475938694 0.0867664444304
0.196157039526 0.0871594796234
0.196838140358 0.0875550826465
0.19751924119 0.087953277896
0.198200342021 0.0883540900912
0.198881442853 0.0887575442795
0.199562543685 0.0891636658428
0.200243644516 0.0895724805028
0.200924745348 0.0899840143274
0.20160584618 0.0903982937367
0.202286947011 0.090815345509
0.202968047843 0.0912351967877
0.203649148675 0.0916578750877
0.204330249506 0.0920834083017
0.205011350338 0.0925118247079
0.20569245117 0.0929431529762
0.206373552001 0.0933774221757
0.207054652833 0.0938146617823
0.207735753665 0.0942549016857
0.208416854497 0.0946981721975
0.209097955328 0.095144504059
0.20977905616 0.0955939284491
0.210460156992 0.0960464769928
0.211141257823 0.0965021817691
0.211822358655 0.0969610753206
0.212503459487 0.0974231906612
0.213184560318 0.0978885612863
0.21386566115 0.0983572211811
0.214546761982 0.0988292048307
0.215227862813 0.0993045472299
0.215908963645 0.0997832838925
0.216590064477 0.100265450863
0.217271165308 0.100751084724
0.21795226614 0.101240222611
0.218633366972 0.101732902222
0.219314467804 0.102229161826
0.219995568635 0.102729040278
0.220676669467 0.10323257703
0.221357770299 0.103739812142
0.22203887113 0.104250786297
0.222719971962 0.104765540809
0.223401072794 0.105284117644
0.224082173625 0.105806559425
0.224763274457 0.106332909452
0.225444375289 0.106863211712
0.22612547612 0.107397510897
0.226806576952 0.107935852417
0.227487677784 0.108478282416
0.228168778615 0.109024847788
0.228849879447 0.109575596192
0.229530980279 0.110130576072
0.230212081111 0.110689836669
0.230893181942 0.111253428044
0.231574282774 0.111821401091
0.232255383606 0.112393807561
0.232936484437 0.112970700076
0.233617585269 0.113552132153
0.234298686101 0.114138158221
0.234979786932 0.114728833643
0.235660887764 0.11532421474
0.236341988596 0.115924358809
0.237023089427 0.116529324146
0.237704190259 0.117139170074
0.238385291091 0.117753956961
0.239066391922 0.118373746251
0.239747492754 0.118998600483
0.240428593586 0.119628583323
0.241109694418 0.120263759588
0.241790795249 0.120904195274
0.242471896081 0.121549957587
0.243152996913 0.12220111497
0.243834097744 0.122857737136
0.244515198576 0.123519895098
0.245196299408 0.124187661203
0.245877400239 0.124861109163
0.246558501071 0.125540314093
0.247239601903 0.126225352545
0.247920702734 0.126916302546
0.248601803566 0.127613243636
0.249282904398 0.128316256904
0.249964005229 0.129025425038
0.250645106061 0.129740832355
0.251326206893 0.130462564855
0.252007307725 0.13119071026
0.252688408556 0.131925358064
0.253369509388 0.132666599579
0.25405061022 0.133414527985
0.254731711051 0.134169238384
0.255412811883 0.134930827851
0.256093912715 0.135699395491
0.256775013546 0.136475042495
0.257456114378 0.1372578722
0.25813721521 0.138047990152
0.258818316041 0.138845504169
0.259499416873 0.139650524404
0.260180517705 0.140463163421
0.260861618536 0.141283536259
0.261542719368 0.142111760509
0.2622238202 0.142947956392
0.262904921032 0.143792246839
0.263586021863 0.144644757568
0.264267122695 0.14550561718
0.264948223527 0.146374957238
0.265629324358 0.147252912371
0.26631042519 0.14813962036
0.266991526022 0.149035222247
0.267672626853 0.149939862435
0.268353727685 0.150853688801
0.269034828517 0.151776852807
0.269715929348 0.152709509618
0.27039703018 0.15365181823
0.271078131012 0.154603941594
0.271759231844 0.155566046753
0.272440332675 0.156538304982
0.273121433507 0.157520891932
0.273802534339 0.15851398779
0.27448363517 0.15951777743
0.275164736002 0.160532450587
0.275845836834 0.161558202028
0.276526937665 0.162595231738
0.277208038497 0.163643745106
0.277889139329 0.164703953135
0.27857024016 0.165776072641
0.279251340992 0.166860326483
0.279932441824 0.167956943786
0.280613542655 0.169066160191
0.281294643487 0.170188218104
0.281975744319 0.171323366963
0.282656845151 0.172471863526
0.283337945982 0.173633972156
0.284019046814 0.174809965142
0.284700147646 0.176000123018
0.285381248477 0.177204734914
0.286062349309 0.178424098915
0.286743450141 0.179658522449
0.287424550972 0.180908322684
0.288105651804 0.182173826963
0.288786752636 0.183455373251
0.289467853467 0.184753310614
0.290148954299 0.186067999721
0.290830055131 0.187399813385
0.291511155962 0.188749137123
0.292192256794 0.190116369761
0.292873357626 0.191501924073
0.293554458458 0.192906227455
0.294235559289 0.19432972265
0.294916660121 0.195772868511
0.295597760953 0.197236140819
0.296278861784 0.198720033156
0.296959962616 0.200225057829
0.297641063448 0.201751746864
0.298322164279 0.203300653066
0.299003265111 0.204872351155
0.299684365943 0.206467438977
0.300365466774 0.208086538813
0.301046567606 0.20973029877
0.301727668438 0.211399394291
0.302408769269 0.213094529773
0.303089870101 0.214816440302
0.303770970933 0.216565893542
0.304452071765 0.218343691762
0.305133172596 0.220150674033
0.305814273428 0.221987718608
0.30649537426 0.2238557455
0.307176475091 0.225755719292
0.307857575923 0.227688652184
0.308538676755 0.22965560732
0.309219777586 0.23165770242
0.309900878418 0.233696113752
0.31058197925 0.235772080485
0.311263080081 0.237886909465
0.311944180913 0.240041980478
0.312625281745 0.242238752042
0.313306382576 0.244478767817
0.313987483408 0.246763663697
0.31466858424 0.249095175687
0.315349685072 0.251475148676
0.316030785903 0.253905546216
0.316711886735 0.256388461485
0.317392987567 0.258926129579
0.318074088398 0.261520941366
0.31875518923 0.264175459136
0.319436290062 0.266892434349
0.320117390893 0.269674827838
0.320798491725 0.272525832895
0.321479592557 0.275448901766
0.322160693388 0.278447776202
0.32284179422 0.281526522837
0.323522895052 0.284689574405
0.324203995883 0.287941777989
0.324885096715 0.291288451868
0.325566197547 0.29473545292
0.326247298379 0.298289257113
0.32692839921 0.301957056348
0.327609500042 0.305746875975
0.328290600874 0.309667718687
0.328971701705 0.313729742516
0.329652802537 0.31794448347
0.330333903369 0.322325137504
0.3310150042 0.326886922627
0.331696105032 0.331647551286
0.332377205864 0.336627857701
0.333058306695 0.341852648195
0.333739407527 0.347351881479
0.334420508359 0.353162353155
0.33510160919 0.359330180941
0.335782710022 0.365914621695
0.336463810854 0.372994233639
0.337144911686 0.380677477901
0.337826012517 0.389122560895
0.338507113349 0.39857921643
0.339188214181 0.409493969698
0.339869315012 0.422875621575


==> figuresAndData/dataForConditionalVarianceLaplaceProb0pt5.tex <==
-13.5 0.115161735767
-13.473 0.115161735767
-13.446 0.115161735767
-13.419 0.115161735767
-13.392 0.115161735767
-13.365 0.115161735767
-13.338 0.115161735767
-13.311 0.115161735767
-13.284 0.115161735767
-13.257 0.115161735767
-13.23 0.115161735767
-13.203 0.115161735767
-13.176 0.115161735767
-13.149 0.115161735767
-13.122 0.115161735767
-13.095 0.115161735767
-13.068 0.115161735767
-13.041 0.115161735767
-13.014 0.115161735767
-12.987 0.115161735767
-12.96 0.115161735767
-12.933 0.115161735767
-12.906 0.115161735767
-12.879 0.115161735767
-12.852 0.115161735767
-12.825 0.115161735767
-12.798 0.115161735767
-12.771 0.115161735767
-12.744 0.115161735767
-12.717 0.115161735767
-12.69 0.115161735767
-12.663 0.115161735767
-12.636 0.115161735767
-12.609 0.115161735767
-12.582 0.115161735767
-12.555 0.115161735767
-12.528 0.115161735767
-12.501 0.115161735767
-12.474 0.115161735767
-12.447 0.115161735767
-12.42 0.115161735767
-12.393 0.115161735767
-12.366 0.115161735767
-12.339 0.115161735767
-12.312 0.115161735767
-12.285 0.115161735767
-12.258 0.115161735767
-12.231 0.115161735767
-12.204 0.115161735767
-12.177 0.115161735767
-12.15 0.115161735767
-12.123 0.115161735767
-12.096 0.115161735767
-12.069 0.115161735767
-12.042 0.115161735767
-12.015 0.115161735767
-11.988 0.115161735767
-11.961 0.115161735767
-11.934 0.115161735767
-11.907 0.115161735767
-11.88 0.115161735767
-11.853 0.115161735767
-11.826 0.115161735767
-11.799 0.115161735767
-11.772 0.115161735767
-11.745 0.115161735767
-11.718 0.115161735767
-11.691 0.115161735767
-11.664 0.115161735767
-11.637 0.115161735767
-11.61 0.115161735767
-11.583 0.115161735767
-11.556 0.115161735767
-11.529 0.115161735767
-11.502 0.115161735767
-11.475 0.115161735767
-11.448 0.115161735767
-11.421 0.115161735767
-11.394 0.115161735767
-11.367 0.115161735767
-11.34 0.115161735767
-11.313 0.115161735767
-11.286 0.115161735767
-11.259 0.115161735767
-11.232 0.115161735767
-11.205 0.115161735767
-11.178 0.115161735767
-11.151 0.115161735767
-11.124 0.115161735767
-11.097 0.115161735767
-11.07 0.115161735767
-11.043 0.115161735767
-11.016 0.115161735767
-10.989 0.115161735767
-10.962 0.115161735767
-10.935 0.115161735767
-10.908 0.115161735767
-10.881 0.115161735767
-10.854 0.115161735767
-10.827 0.115161735767
-10.8 0.115161735766
-10.773 0.115161735766
-10.746 0.115161735766
-10.719 0.115161735766
-10.692 0.115161735766
-10.665 0.115161735766
-10.638 0.115161735766
-10.611 0.115161735766
-10.584 0.115161735766
-10.557 0.115161735766
-10.53 0.115161735766
-10.503 0.115161735766
-10.476 0.115161735765
-10.449 0.115161735765
-10.422 0.115161735765
-10.395 0.115161735765
-10.368 0.115161735765
-10.341 0.115161735765
-10.314 0.115161735765
-10.287 0.115161735764
-10.26 0.115161735764
-10.233 0.115161735764
-10.206 0.115161735764
-10.179 0.115161735763
-10.152 0.115161735763
-10.125 0.115161735763
-10.098 0.115161735762
-10.071 0.115161735762
-10.044 0.115161735762
-10.017 0.115161735761
-9.99 0.115161735761
-9.963 0.11516173576
-9.936 0.115161735759
-9.909 0.115161735759
-9.882 0.115161735758
-9.855 0.115161735758
-9.828 0.115161735757
-9.801 0.115161735756
-9.774 0.115161735755
-9.747 0.115161735754
-9.72 0.115161735753
-9.693 0.115161735752
-9.666 0.115161735751
-9.639 0.11516173575
-9.612 0.115161735748
-9.585 0.115161735747
-9.558 0.115161735745
-9.531 0.115161735743
-9.504 0.115161735741
-9.477 0.115161735739
-9.45 0.115161735737
-9.423 0.115161735735
-9.396 0.115161735732
-9.369 0.11516173573
-9.342 0.115161735727
-9.315 0.115161735724
-9.288 0.11516173572
-9.261 0.115161735717
-9.234 0.115161735713
-9.207 0.115161735708
-9.18 0.115161735704
-9.153 0.115161735699
-9.126 0.115161735693
-9.099 0.115161735688
-9.072 0.115161735682
-9.045 0.115161735675
-9.018 0.115161735668
-8.991 0.11516173566
-8.964 0.115161735651
-8.937 0.115161735642
-8.91 0.115161735633
-8.883 0.115161735622
-8.856 0.115161735611
-8.829 0.115161735599
-8.802 0.115161735586
-8.775 0.115161735572
-8.748 0.115161735556
-8.721 0.11516173554
-8.694 0.115161735522
-8.667 0.115161735503
-8.64 0.115161735483
-8.613 0.115161735461
-8.586 0.115161735437
-8.559 0.115161735411
-8.532 0.115161735384
-8.505 0.115161735354
-8.478 0.115161735322
-8.451 0.115161735287
-8.424 0.11516173525
-8.397 0.11516173521
-8.37 0.115161735167
-8.343 0.11516173512
-8.316 0.11516173507
-8.289 0.115161735016
-8.262 0.115161734958
-8.235 0.115161734895
-8.208 0.115161734828
-8.181 0.115161734755
-8.154 0.115161734677
-8.127 0.115161734592
-8.1 0.115161734501
-8.073 0.115161734404
-8.046 0.115161734298
-8.019 0.115161734185
-7.992 0.115161734063
-7.965 0.115161733931
-7.938 0.115161733789
-7.911 0.115161733637
-7.884 0.115161733473
-7.857 0.115161733296
-7.83 0.115161733105
-7.803 0.1151617329
-7.776 0.11516173268
-7.749 0.115161732442
-7.722 0.115161732186
-7.695 0.11516173191
-7.668 0.115161731614
-7.641 0.115161731295
-7.614 0.115161730951
-7.587 0.115161730581
-7.56 0.115161730182
-7.533 0.115161729754
-7.506 0.115161729292
-7.479 0.115161728795
-7.452 0.115161728261
-7.425 0.115161727685
-7.398 0.115161727066
-7.371 0.115161726399
-7.344 0.115161725682
-7.317 0.115161724909
-7.29 0.115161724079
-7.263 0.115161723184
-7.236 0.115161722222
-7.209 0.115161721187
-7.182 0.115161720073
-7.155 0.115161718874
-7.128 0.115161717584
-7.101 0.115161716196
-7.074 0.115161714703
-7.047 0.115161713096
-7.02 0.115161711368
-6.993 0.115161709509
-6.966 0.115161707508
-6.939 0.115161705357
-6.912 0.115161703042
-6.885 0.115161700553
-6.858 0.115161697875
-6.831 0.115161694994
-6.804 0.115161691896
-6.777 0.115161688564
-6.75 0.115161684981
-6.723 0.115161681127
-6.696 0.115161676982
-6.669 0.115161672525
-6.642 0.115161667733
-6.615 0.115161662579
-6.588 0.115161657037
-6.561 0.115161651079
-6.534 0.115161644673
-6.507 0.115161637785
-6.48 0.11516163038
-6.453 0.11516162242
-6.426 0.115161613862
-6.399 0.115161604662
-6.372 0.115161594773
-6.345 0.115161584143
-6.318 0.115161572717
-6.291 0.115161560437
-6.264 0.115161547238
-6.237 0.115161533053
-6.21 0.115161517809
-6.183 0.115161501426
-6.156 0.115161483822
-6.129 0.115161464905
-6.102 0.115161444578
-6.075 0.115161422738
-6.048 0.115161399272
-6.021 0.115161374061
-5.994 0.115161346976
-5.967 0.11516131788
-5.94 0.115161286623
-5.913 0.115161253047
-5.886 0.115161216983
-5.859 0.115161178246
-5.832 0.115161136641
-5.805 0.115161091958
-5.778 0.115161043971
-5.751 0.115160992438
-5.724 0.1151609371
-5.697 0.115160877679
-5.67 0.115160813876
-5.643 0.115160745373
-5.616 0.115160671825
-5.589 0.115160592867
-5.562 0.115160508103
-5.535 0.115160417112
-5.508 0.115160319441
-5.481 0.115160214605
-5.454 0.115160102086
-5.427 0.115159981325
-5.4 0.115159851727
-5.373 0.115159712651
-5.346 0.115159563415
-5.319 0.115159403282
-5.292 0.115159231469
-5.265 0.115159047133
-5.238 0.115158849374
-5.211 0.115158637224
-5.184 0.115158409652
-5.157 0.11515816555
-5.13 0.115157903733
-5.103 0.115157622933
-5.076 0.115157321792
-5.049 0.115156998856
-5.022 0.115156652569
-4.995 0.115156281267
-4.968 0.115155883168
-4.941 0.115155456365
-4.914 0.11515499882
-4.887 0.11515450835
-4.86 0.115153982621
-4.833 0.115153419137
-4.806 0.115152815228
-4.779 0.115152168039
-4.752 0.115151474516
-4.725 0.115150731396
-4.698 0.11514993519
-4.671 0.115149082166
-4.644 0.115148168337
-4.617 0.115147189444
-4.59 0.115146140933
-4.563 0.115145017937
-4.536 0.11514381526
-4.509 0.115142527349
-4.482 0.115141148274
-4.455 0.115139671699
-4.428 0.115138090862
-4.401 0.11513639854
-4.374 0.115134587022
-4.347 0.115132648078
-4.32 0.115130572924
-4.293 0.115128352183
-4.266 0.115125975853
-4.239 0.115123433259
-4.212 0.115120713017
-4.185 0.115117802981
-4.158 0.115114690201
-4.131 0.115111360866
-4.104 0.115107800252
-4.077 0.115103992664
-4.05 0.115099921372
-4.023 0.115095568549
-3.996 0.115090915199
-3.969 0.115085941087
-3.942 0.115080624657
-3.915 0.115074942955
-3.888 0.115068871537
-3.861 0.115062384383
-3.834 0.115055453793
-3.807 0.115048050291
-3.78 0.115040142511
-3.753 0.115031697087
-3.726 0.115022678528
-3.699 0.115013049095
-3.672 0.11500276866
-3.645 0.11499179457
-3.618 0.114980081494
-3.591 0.114967581265
-3.564 0.114954242716
-3.537 0.114940011503
-3.51 0.114924829923
-3.483 0.114908636718
-3.456 0.114891366874
-3.429 0.114872951406
-3.402 0.114853317135
-3.375 0.11483238645
-3.348 0.114810077067
-3.321 0.114786301764
-3.294 0.114760968114
-3.267 0.114733978204
-3.24 0.114705228333
-3.213 0.114674608709
-3.186 0.114642003122
-3.159 0.114607288612
-3.132 0.114570335113
-3.105 0.114531005092
-3.078 0.114489153166
-3.051 0.114444625714
-3.024 0.114397260459
-2.997 0.114346886051
-2.97 0.114293321626
-2.943 0.114236376351
-2.916 0.114175848956
-2.889 0.114111527253
-2.862 0.114043187638
-2.835 0.113970594581
-2.808 0.113893500102
-2.781 0.113811643236
-2.754 0.113724749489
-2.727 0.113632530276
-2.7 0.113534682362
-2.673 0.113430887284
-2.646 0.113320810775
-2.619 0.113204102182
-2.592 0.113080393883
-2.565 0.112949300703
-2.538 0.112810419337
-2.511 0.112663327781
-2.484 0.11250758477
-2.457 0.112342729235
-2.43 0.112168279776
-2.403 0.111983734163
-2.376 0.111788568865
-2.349 0.11158223861
-2.322 0.111364176
-2.295 0.11113379116
-2.268 0.110890471453
-2.241 0.11063358126
-2.214 0.110362461832
-2.187 0.110076431228
-2.16 0.109774784343
-2.133 0.109456793053
-2.106 0.109121706463
-2.079 0.108768751301
-2.052 0.108397132442
-2.025 0.108006033608
-1.998 0.107594618224
-1.971 0.10716203048
-1.944 0.106707396591
-1.917 0.106229826287
-1.89 0.105728414544
-1.863 0.105202243582
-1.836 0.104650385136
-1.809 0.104071903041
-1.782 0.103465856132
-1.755 0.10283130149
-1.728 0.102167298051
-1.701 0.101472910603
-1.674 0.100747214185
-1.647 0.0999892989079
-1.62 0.0991982752305
-1.593 0.0983732796825
-1.566 0.0975134810731
-1.539 0.0966180871888
-1.512 0.0956863519942
-1.485 0.0947175833449
-1.458 0.093711151218
-1.431 0.0926664964633
-1.404 0.0915831400716
-1.377 0.0904606929544
-1.35 0.0892988662222
-1.323 0.0880974819448
-1.296 0.0868564843683
-1.269 0.0855759515604
-1.242 0.0842561074465
-1.215 0.0828973341933
-1.188 0.0815001848911
-1.161 0.0800653964774
-1.134 0.078593902843
-1.107 0.0770868480531
-1.08 0.0755455996175
-1.053 0.0739717617398
-1.026 0.0723671884829
-0.999 0.0707339967896
-0.972 0.0690745793138
-0.945 0.0673916170328
-0.918 0.0656880916384
-0.891 0.0639672977425
-0.864 0.0622328549797
-0.837 0.0604887201559
-0.81 0.0587391996745
-0.783 0.0569889625817
-0.756 0.0552430547076
-0.729 0.0535069145595
-0.702 0.0517863918421
-0.675 0.0500877697673
-0.648 0.0484177926749
-0.621 0.0467837009482
-0.594 0.0451932758061
-0.567 0.0436548973207
-0.54 0.042177620025
-0.513 0.0407712718078
-0.486 0.0394465835744
-0.459 0.0382153595682
-0.432 0.0370907015455
-0.405 0.0360873045771
-0.378 0.0352218487023
-0.351 0.0345135198864
-0.324 0.0339847071651
-0.297 0.0336619427996
-0.27 0.0335771825306
-0.243 0.0337695701258
-0.216 0.0342879058873
-0.189 0.0351941637479
-0.162 0.0365686164231
-0.135 0.038517513503
-0.108 0.0411849830142
-0.081 0.0447722703979
-0.054 0.04957048755
-0.027 0.0560200272119
0.0 0.0648272482622
0.000383576096602 0.0649742333259
0.000767152193205 0.0651216730413
0.00115072828981 0.0652695693632
0.00153430438641 0.065417924258
0.00191788048301 0.0655667397032
0.00230145657961 0.0657160176881
0.00268503267622 0.0658657602136
0.00306860877282 0.0660159692922
0.00345218486942 0.0661666469484
0.00383576096602 0.0663177952185
0.00421933706263 0.0664694161507
0.00460291315923 0.0666215118055
0.00498648925583 0.0667740842553
0.00537006535243 0.0669271355851
0.00575364144904 0.067080667892
0.00613721754564 0.0672346832857
0.00652079364224 0.0673891838884
0.00690436973884 0.0675441718348
0.00728794583545 0.0676996492727
0.00767152193205 0.0678556183625
0.00805509802865 0.0680120812775
0.00843867412525 0.0681690402043
0.00882225022185 0.0683264973425
0.00920582631846 0.0684844549048
0.00958940241506 0.0686429151175
0.00997297851166 0.0688018802202
0.0103565546083 0.0689613524663
0.0107401307049 0.0691213341226
0.0111237068015 0.0692818274698
0.0115072828981 0.0694428348025
0.0118908589947 0.0696043584293
0.0122744350913 0.0697664006729
0.0126580111879 0.0699289638701
0.0130415872845 0.0700920503723
0.0134251633811 0.0702556625452
0.0138087394777 0.070419802769
0.0141923155743 0.0705844734388
0.0145758916709 0.0707496769641
0.0149594677675 0.0709154157698
0.0153430438641 0.0710816922956
0.0157266199607 0.0712485089962
0.0161101960573 0.071415868342
0.0164937721539 0.0715837728184
0.0168773482505 0.0717522249266
0.0172609243471 0.0719212271832
0.0176445004437 0.072090782121
0.0180280765403 0.0722608922882
0.0184116526369 0.0724315602495
0.0187952287335 0.0726027885856
0.0191788048301 0.0727745798933
0.0195623809267 0.0729469367862
0.0199459570233 0.0731198618942
0.0203295331199 0.0732933578641
0.0207131092165 0.0734674273596
0.0210966853131 0.0736420730611
0.0214802614097 0.0738172976663
0.0218638375063 0.0739931038904
0.0222474136029 0.0741694944657
0.0226309896995 0.0743464721422
0.0230145657961 0.0745240396876
0.0233981418927 0.0747021998875
0.0237817179893 0.0748809555455
0.0241652940859 0.0750603094832
0.0245488701826 0.0752402645409
0.0249324462792 0.075420823577
0.0253160223758 0.0756019894687
0.0256995984724 0.0757837651121
0.026083174569 0.0759661534219
0.0264667506656 0.0761491573323
0.0268503267622 0.0763327797966
0.0272339028588 0.0765170237875
0.0276174789554 0.0767018922975
0.028001055052 0.0768873883385
0.0283846311486 0.0770735149428
0.0287682072452 0.0772602751625
0.0291517833418 0.0774476720702
0.0295353594384 0.0776357087588
0.029918935535 0.0778243883419
0.0303025116316 0.0780137139541
0.0306860877282 0.0782036887507
0.0310696638248 0.0783943159085
0.0314532399214 0.0785855986255
0.031836816018 0.0787775401213
0.0322203921146 0.0789701436373
0.0326039682112 0.0791634124368
0.0329875443078 0.0793573498054
0.0333711204044 0.0795519590507
0.033754696501 0.0797472435033
0.0341382725976 0.0799432065162
0.0345218486942 0.0801398514655
0.0349054247908 0.0803371817503
0.0352890008874 0.0805352007933
0.035672576984 0.0807339120406
0.0360561530806 0.0809333189621
0.0364397291772 0.0811334250518
0.0368233052738 0.0813342338277
0.0372068813704 0.0815357488325
0.037590457467 0.0817379736333
0.0379740335636 0.0819409118223
0.0383576096602 0.0821445670167
0.0387411857568 0.0823489428591
0.0391247618534 0.0825540430176
0.03950833795 0.082759871186
0.0398919140466 0.0829664310845
0.0402754901432 0.0831737264593
0.0406590662399 0.0833817610832
0.0410426423365 0.0835905387556
0.0414262184331 0.0838000633034
0.0418097945297 0.0840103385802
0.0421933706263 0.0842213684676
0.0425769467229 0.0844331568747
0.0429605228195 0.0846457077388
0.0433440989161 0.0848590250255
0.0437276750127 0.0850731127288
0.0441112511093 0.0852879748718
0.0444948272059 0.0855036155066
0.0448784033025 0.0857200387147
0.0452619793991 0.0859372486075
0.0456455554957 0.0861552493259
0.0460291315923 0.0863740450415
0.0464127076889 0.0865936399563
0.0467962837855 0.0868140383031
0.0471798598821 0.0870352443457
0.0475634359787 0.0872572623797
0.0479470120753 0.0874800967322
0.0483305881719 0.0877037517623
0.0487141642685 0.0879282318616
0.0490977403651 0.0881535414543
0.0494813164617 0.0883796849976
0.0498648925583 0.0886066669821
0.0502484686549 0.0888344919319
0.0506320447515 0.0890631644053
0.0510156208481 0.0892926889948
0.0513991969447 0.0895230703274
0.0517827730413 0.0897543130653
0.0521663491379 0.089986421906
0.0525499252345 0.0902194015828
0.0529335013311 0.0904532568648
0.0533170774277 0.0906879925578
0.0537006535243 0.0909236135043
0.0540842296209 0.0911601245838
0.0544678057175 0.0913975307135
0.0548513818141 0.0916358368486
0.0552349579107 0.0918750479823
0.0556185340073 0.0921151691468
0.0560021101039 0.0923562054132
0.0563856862005 0.0925981618922
0.0567692622972 0.0928410437343
0.0571528383938 0.0930848561303
0.0575364144904 0.0933296043118
0.057919990587 0.0935752935514
0.0583035666836 0.0938219291635
0.0586871427802 0.0940695165044
0.0590707188768 0.0943180609726
0.0594542949734 0.0945675680098
0.05983787107 0.0948180431009
0.0602214471666 0.0950694917746
0.0606050232632 0.0953219196038
0.0609885993598 0.0955753322062
0.0613721754564 0.0958297352447
0.061755751553 0.0960851344277
0.0621393276496 0.0963415355099
0.0625229037462 0.0965989442927
0.0629064798428 0.0968573666246
0.0632900559394 0.0971168084016
0.063673632036 0.097377275568
0.0640572081326 0.0976387741169
0.0644407842292 0.0979013100905
0.0648243603258 0.0981648895807
0.0652079364224 0.0984295187298
0.065591512519 0.0986952037308
0.0659750886156 0.0989619508283
0.0663586647122 0.0992297663188
0.0667422408088 0.0994986565511
0.0671258169054 0.0997686279275
0.067509393002 0.100039686904
0.0678929690986 0.10031183999
0.0682765451952 0.100585093751
0.0686601212918 0.100859454808
0.0690436973884 0.101134929837
0.069427273485 0.101411525572
0.0698108495816 0.101689248804
0.0701944256782 0.101968106381
0.0705780017748 0.102248105211
0.0709615778714 0.102529252262
0.071345153968 0.10281155456
0.0717287300646 0.103095019194
0.0721123061612 0.103379653312
0.0724958822578 0.103665464126
0.0728794583545 0.103952458911
0.0732630344511 0.104240645004
0.0736466105477 0.104530029808
0.0740301866443 0.10482062079
0.0744137627409 0.105112425484
0.0747973388375 0.105405451489
0.0751809149341 0.105699706472
0.0755644910307 0.105995198169
0.0759480671273 0.106291934385
0.0763316432239 0.106589922994
0.0767152193205 0.10688917194
0.0770987954171 0.10718968924
0.0774823715137 0.107491482983
0.0778659476103 0.107794561331
0.0782495237069 0.108098932519
0.0786330998035 0.10840460486
0.0790166759001 0.10871158674
0.0794002519967 0.109019886623
0.0797838280933 0.109329513049
0.0801674041899 0.109640474641
0.0805509802865 0.109952780097
0.0809345563831 0.110266438198
0.0813181324797 0.110581457807
0.0817017085763 0.110897847868
0.0820852846729 0.11121561741
0.0824688607695 0.111534775547
0.0828524368661 0.111855331477
0.0832360129627 0.112177294487
0.0836195890593 0.11250067395
0.0840031651559 0.11282547933
0.0843867412525 0.11315172018
0.0847703173491 0.113479406144
0.0851538934457 0.11380854696
0.0855374695423 0.114139152459
0.0859210456389 0.114471232566
0.0863046217355 0.114804797303
0.0866881978321 0.115139856789
0.0870717739287 0.115476421243
0.0874553500253 0.115814500982
0.0878389261219 0.116154106426
0.0882225022185 0.116495248095
0.0886060783151 0.116837936615
0.0889896544118 0.117182182717
0.0893732305084 0.117527997239
0.089756806605 0.117875391125
0.0901403827016 0.118224375431
0.0905239587982 0.118574961324
0.0909075348948 0.11892716008
0.0912911109914 0.119280983094
0.091674687088 0.119636441872
0.0920582631846 0.119993548041
0.0924418392812 0.120352313343
0.0928254153778 0.120712749643
0.0932089914744 0.121074868928
0.093592567571 0.121438683306
0.0939761436676 0.121804205012
0.0943597197642 0.12217144641
0.0947432958608 0.122540419991
0.0951268719574 0.122911138375
0.095510448054 0.123283614317
0.0958940241506 0.123657860706
0.0962776002472 0.124033890567
0.0966611763438 0.124411717062
0.0970447524404 0.124791353496
0.097428328537 0.125172813313
0.0978119046336 0.125556110102
0.0981954807302 0.125941257601
0.0985790568268 0.126328269693
0.0989626329234 0.126717160412
0.09934620902 0.127107943947
0.0997297851166 0.12750063464
0.100113361213 0.127895246991
0.10049693731 0.128291795658
0.100880513406 0.128690295464
0.101264089503 0.129090761394
0.1016476656 0.1294932086
0.102031241696 0.129897652404
0.102414817793 0.130304108299
0.102798393889 0.130712591954
0.103181969986 0.131123119212
0.103565546083 0.131535706099
0.103949122179 0.131950368821
0.104332698276 0.132367123772
0.104716274372 0.132785987531
0.105099850469 0.13320697687
0.105483426566 0.133630108756
0.105867002662 0.134055400349
0.106250578759 0.134482869014
0.106634154855 0.134912532316
0.107017730952 0.135344408027
0.107401307049 0.13577851413
0.107784883145 0.136214868821
0.108168459242 0.13665349051
0.108552035338 0.13709439783
0.108935611435 0.137537609636
0.109319187532 0.13798314501
0.109702763628 0.138431023265
0.110086339725 0.13888126395
0.110469915821 0.139333886851
0.110853491918 0.139788911996
0.111237068015 0.14024635966
0.111620644111 0.140706250369
0.112004220208 0.141168604903
0.112387796304 0.141633444302
0.112771372401 0.142100789867
0.113154948498 0.142570663168
0.113538524594 0.14304308605
0.113922100691 0.14351808063
0.114305676788 0.14399566931
0.114689252884 0.144475874778
0.115072828981 0.144958720014
0.115456405077 0.145444228293
0.115839981174 0.145932423193
0.116223557271 0.1464233286
0.116607133367 0.14691696871
0.116990709464 0.147413368039
0.11737428556 0.147912551427
0.117757861657 0.148414544043
0.118141437754 0.14891937139
0.11852501385 0.149427059315
0.118908589947 0.149937634012
0.119292166043 0.150451122028
0.11967574214 0.150967550272
0.120059318237 0.15148694602
0.120442894333 0.152009336921
0.12082647043 0.152534751007
0.121210046526 0.153063216696
0.121593622623 0.153594762804
0.12197719872 0.154129418547
0.122360774816 0.154667213554
0.122744350913 0.155208177873
0.123127927009 0.155752341975
0.123511503106 0.15629973677
0.123895079203 0.156850393609
0.124278655299 0.157404344296
0.124662231396 0.157961621093
0.125045807492 0.158522256737
0.125429383589 0.159086284439
0.125812959686 0.159653737901
0.126196535782 0.160224651325
0.126580111879 0.16079905942
0.126963687975 0.161376997413
0.127347264072 0.161958501063
0.127730840169 0.162543606668
0.128114416265 0.163132351077
0.128497992362 0.163724771704
0.128881568458 0.164320906536
0.129265144555 0.164920794146
0.129648720652 0.16552447371
0.130032296748 0.166131985013
0.130415872845 0.166743368464
0.130799448941 0.167358665114
0.131183025038 0.167977916663
0.131566601135 0.16860116548
0.131950177231 0.169228454612
0.132333753328 0.169859827806
0.132717329424 0.170495329517
0.133100905521 0.171135004929
0.133484481618 0.171778899968
0.133868057714 0.172427061323
0.134251633811 0.173079536459
0.134635209907 0.173736373635
0.135018786004 0.174397621927
0.135402362101 0.175063331241
0.135785938197 0.175733552335
0.136169514294 0.17640833684
0.13655309039 0.177087737279
0.136936666487 0.177771807089
0.137320242584 0.17846060064
0.13770381868 0.179154173265
0.138087394777 0.179852581272
0.138470970873 0.18055588198
0.13885454697 0.181264133734
0.139238123067 0.181977395935
0.139621699163 0.182695729066
0.14000527526 0.18341919472
0.140388851356 0.184147855624
0.140772427453 0.184881775672
0.14115600355 0.185621019954
0.141539579646 0.186365654785
0.141923155743 0.18711574774
0.142306731839 0.187871367683
0.142690307936 0.188632584804
0.143073884033 0.189399470655
0.143457460129 0.190172098181
0.143841036226 0.190950541766
0.144224612322 0.191734877263
0.144608188419 0.192525182042
0.144991764516 0.193321535028
0.145375340612 0.194124016743
0.145758916709 0.194932709355
0.146142492806 0.195747696721
0.146526068902 0.196569064435
0.146909644999 0.197396899882
0.147293221095 0.198231292285
0.147676797192 0.19907233276
0.148060373289 0.199920114374
0.148443949385 0.200774732201
0.148827525482 0.201636283381
0.149211101578 0.202504867186
0.149594677675 0.203380585079
0.149978253772 0.204263540788
0.150361829868 0.205153840372
0.150745405965 0.206051592295
0.151128982061 0.206956907502
0.151512558158 0.207869899496
0.151896134255 0.208790684424
0.152279710351 0.20971938116
0.152663286448 0.210656111394
0.153046862544 0.211600999727
0.153430438641 0.212554173764
0.153814014738 0.213515764222
0.154197590834 0.214485905027
0.154581166931 0.215464733433
0.154964743027 0.21645239013
0.155348319124 0.217449019369
0.155731895221 0.218454769084
0.156115471317 0.219469791028
0.156499047414 0.220494240907
0.15688262351 0.221528278527
0.157266199607 0.222572067943
0.157649775704 0.223625777618
0.1580333518 0.224689580588
0.158416927897 0.225763654638
0.158800503993 0.226848182484
0.15918408009 0.227943351963
0.159567656187 0.229049356238
0.159951232283 0.230166394006
0.16033480838 0.231294669725
0.160718384476 0.232434393844
0.161101960573 0.233585783056
0.16148553667 0.234749060552
0.161869112766 0.235924456299
0.162252688863 0.237112207331
0.162636264959 0.238312558052
0.163019841056 0.239525760559
0.163403417153 0.240752074988
0.163786993249 0.24199176987
0.164170569346 0.243245122517
0.164554145442 0.244512419427
0.164937721539 0.245793956715
0.165321297636 0.247090040567
0.165704873732 0.248400987728
0.166088449829 0.249727126015
0.166472025925 0.251068794867
0.166855602022 0.25242634593
0.167239178119 0.253800143677
0.167622754215 0.255190566073
0.168006330312 0.256598005287
0.168389906408 0.258022868447
0.168773482505 0.259465578455
0.169157058602 0.260926574855
0.169540634698 0.262406314764
0.169924210795 0.263905273878
0.170307786891 0.265423947542
0.170691362988 0.266962851917
0.171074939085 0.268522525222
0.171458515181 0.270103529083
0.171842091278 0.271706449994
0.172225667374 0.273331900886
0.172609243471 0.274980522839
0.172992819568 0.276652986935
0.173376395664 0.278349996269
0.173759971761 0.28007228815
0.174143547857 0.281820636487
0.174527123954 0.283595854406
0.174910700051 0.285398797115
0.175294276147 0.287230365038
0.175677852244 0.289091507267
0.17606142834 0.290983225364
0.176445004437 0.292906577552
0.176828580534 0.294862683357
0.17721215663 0.296852728753
0.177595732727 0.298877971887
0.177979308824 0.300939749453
0.17836288492 0.303039483831
0.178746461017 0.30517869108
0.179130037113 0.307358989937
0.17951361321 0.309582111973
0.179897189307 0.311849913094
0.180280765403 0.314164386616
0.1806643415 0.31652767819
0.181047917596 0.31894210291
0.181431493693 0.321410165012
0.18181506979 0.323934580661
0.182198645886 0.326518304458
0.182582221983 0.329164560433
0.182965798079 0.331876878511
0.183349374176 0.334659137689
0.183732950273 0.337515617527
0.184116526369 0.340451060007
0.184500102466 0.343470744495
0.184883678562 0.346580579382
0.185267254659 0.349787215284
0.185650830756 0.353098186399
0.186034406852 0.356522089255
0.186417982949 0.360068811882
0.186801559045 0.363749832255
0.187185135142 0.367578613951
0.187568711239 0.371571141449
0.187952287335 0.375746661743
0.188335863432 0.380128740651
0.188719439528 0.384746817987
0.189103015625 0.389638590818
0.189486591722 0.394853851923
0.189870167818 0.40046107662
0.190253743915 0.406559716451
0.190637320011 0.41330600435
0.191020896108 0.420977726304
0.191404472205 0.430198038241


==> figuresAndData/dataForConditionalVarianceLaplaceProb0pt6.tex <==
-13.5 0.125052621402
-13.473 0.125052621402
-13.446 0.125052621402
-13.419 0.125052621402
-13.392 0.125052621402
-13.365 0.125052621402
-13.338 0.125052621402
-13.311 0.125052621402
-13.284 0.125052621402
-13.257 0.125052621402
-13.23 0.125052621402
-13.203 0.125052621402
-13.176 0.125052621402
-13.149 0.125052621402
-13.122 0.125052621402
-13.095 0.125052621402
-13.068 0.125052621402
-13.041 0.125052621402
-13.014 0.125052621402
-12.987 0.125052621402
-12.96 0.125052621402
-12.933 0.125052621402
-12.906 0.125052621402
-12.879 0.125052621402
-12.852 0.125052621402
-12.825 0.125052621402
-12.798 0.125052621402
-12.771 0.125052621402
-12.744 0.125052621402
-12.717 0.125052621402
-12.69 0.125052621402
-12.663 0.125052621402
-12.636 0.125052621402
-12.609 0.125052621402
-12.582 0.125052621402
-12.555 0.125052621402
-12.528 0.125052621402
-12.501 0.125052621402
-12.474 0.125052621402
-12.447 0.125052621402
-12.42 0.125052621402
-12.393 0.125052621402
-12.366 0.125052621402
-12.339 0.125052621402
-12.312 0.125052621402
-12.285 0.125052621402
-12.258 0.125052621402
-12.231 0.125052621402
-12.204 0.125052621402
-12.177 0.125052621402
-12.15 0.125052621402
-12.123 0.125052621402
-12.096 0.125052621402
-12.069 0.125052621402
-12.042 0.125052621402
-12.015 0.125052621402
-11.988 0.125052621402
-11.961 0.125052621402
-11.934 0.125052621402
-11.907 0.125052621402
-11.88 0.125052621402
-11.853 0.125052621401
-11.826 0.125052621401
-11.799 0.125052621401
-11.772 0.125052621401
-11.745 0.125052621401
-11.718 0.125052621401
-11.691 0.125052621401
-11.664 0.125052621401
-11.637 0.125052621401
-11.61 0.125052621401
-11.583 0.125052621401
-11.556 0.125052621401
-11.529 0.125052621401
-11.502 0.125052621401
-11.475 0.125052621401
-11.448 0.125052621401
-11.421 0.125052621401
-11.394 0.125052621401
-11.367 0.125052621401
-11.34 0.125052621401
-11.313 0.125052621401
-11.286 0.125052621401
-11.259 0.125052621401
-11.232 0.125052621401
-11.205 0.125052621401
-11.178 0.125052621401
-11.151 0.125052621401
-11.124 0.125052621401
-11.097 0.125052621401
-11.07 0.125052621401
-11.043 0.125052621401
-11.016 0.125052621401
-10.989 0.125052621401
-10.962 0.125052621401
-10.935 0.125052621401
-10.908 0.125052621401
-10.881 0.125052621401
-10.854 0.125052621401
-10.827 0.125052621401
-10.8 0.125052621401
-10.773 0.125052621401
-10.746 0.125052621401
-10.719 0.125052621401
-10.692 0.125052621401
-10.665 0.125052621401
-10.638 0.125052621401
-10.611 0.125052621401
-10.584 0.1250526214
-10.557 0.1250526214
-10.53 0.1250526214
-10.503 0.1250526214
-10.476 0.1250526214
-10.449 0.1250526214
-10.422 0.1250526214
-10.395 0.1250526214
-10.368 0.1250526214
-10.341 0.125052621399
-10.314 0.125052621399
-10.287 0.125052621399
-10.26 0.125052621399
-10.233 0.125052621399
-10.206 0.125052621398
-10.179 0.125052621398
-10.152 0.125052621398
-10.125 0.125052621398
-10.098 0.125052621397
-10.071 0.125052621397
-10.044 0.125052621397
-10.017 0.125052621396
-9.99 0.125052621396
-9.963 0.125052621396
-9.936 0.125052621395
-9.909 0.125052621395
-9.882 0.125052621394
-9.855 0.125052621393
-9.828 0.125052621393
-9.801 0.125052621392
-9.774 0.125052621391
-9.747 0.125052621391
-9.72 0.12505262139
-9.693 0.125052621389
-9.666 0.125052621388
-9.639 0.125052621387
-9.612 0.125052621385
-9.585 0.125052621384
-9.558 0.125052621383
-9.531 0.125052621381
-9.504 0.12505262138
-9.477 0.125052621378
-9.45 0.125052621376
-9.423 0.125052621374
-9.396 0.125052621372
-9.369 0.12505262137
-9.342 0.125052621367
-9.315 0.125052621365
-9.288 0.125052621362
-9.261 0.125052621359
-9.234 0.125052621355
-9.207 0.125052621352
-9.18 0.125052621348
-9.153 0.125052621344
-9.126 0.125052621339
-9.099 0.125052621334
-9.072 0.125052621329
-9.045 0.125052621323
-9.018 0.125052621317
-8.991 0.125052621311
-8.964 0.125052621304
-8.937 0.125052621296
-8.91 0.125052621288
-8.883 0.125052621279
-8.856 0.125052621269
-8.829 0.125052621259
-8.802 0.125052621248
-8.775 0.125052621236
-8.748 0.125052621223
-8.721 0.125052621209
-8.694 0.125052621194
-8.667 0.125052621178
-8.64 0.125052621161
-8.613 0.125052621142
-8.586 0.125052621122
-8.559 0.1250526211
-8.532 0.125052621076
-8.505 0.125052621051
-8.478 0.125052621024
-8.451 0.125052620995
-8.424 0.125052620963
-8.397 0.125052620929
-8.37 0.125052620892
-8.343 0.125052620853
-8.316 0.12505262081
-8.289 0.125052620765
-8.262 0.125052620715
-8.235 0.125052620662
-8.208 0.125052620605
-8.181 0.125052620543
-8.154 0.125052620477
-8.127 0.125052620405
-8.1 0.125052620328
-8.073 0.125052620245
-8.046 0.125052620156
-8.019 0.12505262006
-7.992 0.125052619956
-7.965 0.125052619844
-7.938 0.125052619724
-7.911 0.125052619594
-7.884 0.125052619455
-7.857 0.125052619305
-7.83 0.125052619143
-7.803 0.125052618969
-7.776 0.125052618781
-7.749 0.12505261858
-7.722 0.125052618362
-7.695 0.125052618128
-7.668 0.125052617876
-7.641 0.125052617605
-7.614 0.125052617313
-7.587 0.125052616999
-7.56 0.12505261666
-7.533 0.125052616296
-7.506 0.125052615904
-7.479 0.125052615481
-7.452 0.125052615027
-7.425 0.125052614538
-7.398 0.125052614011
-7.371 0.125052613445
-7.344 0.125052612835
-7.317 0.125052612178
-7.29 0.125052611472
-7.263 0.125052610711
-7.236 0.125052609893
-7.209 0.125052609013
-7.182 0.125052608065
-7.155 0.125052607045
-7.128 0.125052605948
-7.101 0.125052604768
-7.074 0.125052603497
-7.047 0.12505260213
-7.02 0.12505260066
-6.993 0.125052599078
-6.966 0.125052597375
-6.939 0.125052595544
-6.912 0.125052593574
-6.885 0.125052591455
-6.858 0.125052589175
-6.831 0.125052586723
-6.804 0.125052584085
-6.777 0.125052581248
-6.75 0.125052578196
-6.723 0.125052574914
-6.696 0.125052571384
-6.669 0.125052567588
-6.642 0.125052563505
-6.615 0.125052559115
-6.588 0.125052554393
-6.561 0.125052549317
-6.534 0.125052543857
-6.507 0.125052537988
-6.48 0.125052531676
-6.453 0.125052524891
-6.426 0.125052517595
-6.399 0.125052509752
-6.372 0.125052501321
-6.345 0.125052492257
-6.318 0.125052482513
-6.291 0.12505247204
-6.264 0.125052460782
-6.237 0.125052448682
-6.21 0.125052435677
-6.183 0.125052421699
-6.156 0.125052406678
-6.129 0.125052390535
-6.102 0.125052373187
-6.075 0.125052354546
-6.048 0.125052334515
-6.021 0.125052312992
-5.994 0.125052289867
-5.967 0.125052265022
-5.94 0.125052238329
-5.913 0.125052209654
-5.886 0.125052178848
-5.859 0.125052145757
-5.832 0.125052110212
-5.805 0.125052072033
-5.778 0.125052031026
-5.751 0.125051986984
-5.724 0.125051939685
-5.697 0.12505188889
-5.67 0.125051834343
-5.643 0.125051775771
-5.616 0.125051712878
-5.589 0.12505164535
-5.562 0.125051572848
-5.535 0.125051495011
-5.508 0.125051411449
-5.481 0.125051321746
-5.454 0.125051225457
-5.427 0.125051122102
-5.4 0.125051011169
-5.373 0.125050892108
-5.346 0.125050764332
-5.319 0.12505062721
-5.292 0.125050480065
-5.265 0.125050322175
-5.238 0.125050152763
-5.211 0.125049971001
-5.184 0.125049775997
-5.157 0.1250495668
-5.13 0.12504934239
-5.103 0.125049101675
-5.076 0.125048843485
-5.049 0.125048566569
-5.022 0.125048269586
-4.995 0.125047951103
-4.968 0.125047609584
-4.941 0.125047243385
-4.914 0.12504685075
-4.887 0.125046429795
-4.86 0.125045978509
-4.833 0.125045494738
-4.806 0.125044976178
-4.779 0.125044420366
-4.752 0.125043824665
-4.725 0.125043186258
-4.698 0.12504250213
-4.671 0.125041769061
-4.644 0.125040983605
-4.617 0.125040142079
-4.59 0.125039240548
-4.563 0.125038274806
-4.536 0.125037240356
-4.509 0.125036132396
-4.482 0.125034945794
-4.455 0.125033675068
-4.428 0.125032314361
-4.401 0.12503085742
-4.374 0.125029297567
-4.347 0.125027627669
-4.32 0.125025840113
-4.293 0.125023926772
-4.266 0.125021878971
-4.239 0.125019687451
-4.212 0.125017342334
-4.185 0.125014833078
-4.158 0.12501214844
-4.131 0.125009276425
-4.104 0.125006204242
-4.077 0.125002918252
-4.05 0.124999403912
-4.023 0.124995645719
-3.996 0.124991627149
-3.969 0.124987330594
-3.942 0.124982737291
-3.915 0.124977827251
-3.888 0.124972579183
-3.861 0.124966970409
-3.834 0.124960976786
-3.807 0.124954572608
-3.78 0.124947730511
-3.753 0.124940421376
-3.726 0.124932614218
-3.699 0.124924276073
-3.672 0.124915371878
-3.645 0.124905864349
-3.618 0.124895713842
-3.591 0.124884878217
-3.564 0.124873312688
-3.537 0.124860969666
-3.51 0.1248477986
-3.483 0.124833745797
-3.456 0.124818754247
-3.429 0.124802763426
-3.402 0.1247857091
-3.375 0.124767523113
-3.348 0.124748133162
-3.321 0.124727462569
-3.294 0.124705430036
-3.267 0.124681949392
-3.24 0.12465692932
-3.213 0.124630273087
-3.186 0.124601878242
-3.159 0.12457163632
-3.132 0.124539432518
-3.105 0.124505145367
-3.078 0.124468646381
-3.051 0.124429799706
-3.024 0.124388461738
-2.997 0.124344480738
-2.97 0.124297696432
-2.943 0.124247939589
-2.916 0.124195031593
-2.889 0.124138783995
-2.862 0.124078998055
-2.835 0.124015464267
-2.808 0.123947961871
-2.781 0.123876258356
-2.754 0.123800108944
-2.727 0.12371925607
-2.7 0.123633428845
-2.673 0.123542342515
-2.646 0.12344569791
-2.619 0.123343180886
-2.592 0.123234461763
-2.565 0.123119194765
-2.538 0.122997017449
-2.511 0.122867550151
-2.484 0.12273039543
-2.457 0.122585137519
-2.43 0.122431341794
-2.403 0.122268554258
-2.376 0.12209630105
-2.349 0.121914087977
-2.322 0.121721400079
-2.295 0.121517701236
-2.268 0.121302433822
-2.241 0.121075018405
-2.214 0.120834853519
-2.187 0.120581315495
-2.16 0.120313758386
-2.133 0.120031513966
-2.106 0.119733891846
-2.079 0.119420179693
-2.052 0.11908964358
-2.025 0.118741528476
-1.998 0.118375058892
-1.971 0.117989439692
-1.944 0.1175838571
-1.917 0.117157479905
-1.89 0.116709460893
-1.863 0.11623893852
-1.836 0.115745038847
-1.809 0.115226877766
-1.782 0.114683563521
-1.755 0.11411419957
-1.728 0.113517887794
-1.701 0.112893732082
-1.674 0.112240842322
-1.647 0.111558338815
-1.62 0.110845357143
-1.593 0.110101053513
-1.566 0.109324610602
-1.539 0.108515243934
-1.512 0.107672208801
-1.485 0.106794807758
-1.458 0.105882398725
-1.431 0.104934403689
-1.404 0.103950318056
-1.377 0.102929720651
-1.35 0.101872284384
-1.323 0.100777787604
-1.296 0.0996461261415
-1.269 0.0984773260582
-1.242 0.097271557104
-1.215 0.0960291468928
-1.188 0.0947505958002
-1.161 0.0934365925926
-1.134 0.0920880307944
-1.107 0.0907060258091
-1.08 0.0892919328151
-1.053 0.0878473654707
-1.026 0.086374215477
-0.999 0.0848746730746
-0.972 0.08335124858
-0.945 0.0818067951111
-0.918 0.080244532711
-0.891 0.0786680741527
-0.864 0.0770814528086
-0.837 0.0754891530951
-0.81 0.0738961441721
-0.783 0.0723079177898
-0.756 0.0707305314565
-0.729 0.0691706584604
-0.702 0.0676356467504
-0.675 0.066133589291
-0.648 0.0646734093118
-0.621 0.0632649649349
-0.594 0.0619191790746
-0.567 0.0606482024067
-0.54 0.0594656197779
-0.513 0.0583867139691
-0.486 0.0574288056384
-0.459 0.0566116952071
-0.432 0.0559582423655
-0.405 0.0554951333096
-0.378 0.055253907206
-0.351 0.0552723457264
-0.324 0.0555963795239
-0.297 0.0562827448643
-0.27 0.0574027530526
-0.243 0.0590477531894
-0.216 0.0613372490757
-0.189 0.0644313226617
-0.162 0.068550335656
-0.135 0.0740075428477
-0.108 0.081265997037
-0.081 0.0910446065426
-0.054 0.10453338002
-0.027 0.123883728994
0.0 0.153530967875
0.000140480687544 0.153726280949
0.000280961375088 0.153922012094
0.000421442062631 0.154118162763
0.000561922750175 0.154314734417
0.000702403437719 0.154511728526
0.000842884125263 0.154709146566
0.000983364812806 0.154906990021
0.00112384550035 0.155105260383
0.00126432618789 0.155303959153
0.00140480687544 0.155503087836
0.00154528756298 0.155702647949
0.00168576825053 0.155902641015
0.00182624893807 0.156103068565
0.00196672962561 0.156303932138
0.00210721031316 0.156505233281
0.0022476910007 0.156706973549
0.00238817168824 0.156909154507
0.00252865237579 0.157111777725
0.00266913306333 0.157314844785
0.00280961375088 0.157518357274
0.00295009443842 0.15772231679
0.00309057512596 0.157926724937
0.00323105581351 0.15813158333
0.00337153650105 0.158336893591
0.00351201718859 0.158542657352
0.00365249787614 0.158748876252
0.00379297856368 0.15895555194
0.00393345925123 0.159162686074
0.00407393993877 0.15937028032
0.00421442062631 0.159578336354
0.00435490131386 0.15978685586
0.0044953820014 0.159995840532
0.00463586268894 0.160205292074
0.00477634337649 0.160415212197
0.00491682406403 0.160625602622
0.00505730475158 0.160836465081
0.00519778543912 0.161047801314
0.00533826612666 0.161259613071
0.00547874681421 0.161471902111
0.00561922750175 0.161684670204
0.00575970818929 0.161897919129
0.00590018887684 0.162111650673
0.00604066956438 0.162325866637
0.00618115025193 0.162540568829
0.00632163093947 0.162755759067
0.00646211162701 0.16297143918
0.00660259231456 0.163187611007
0.0067430730021 0.163404276399
0.00688355368964 0.163621437213
0.00702403437719 0.163839095321
0.00716451506473 0.164057252603
0.00730499575228 0.16427591095
0.00744547643982 0.164495072265
0.00758595712736 0.164714738459
0.00772643781491 0.164934911457
0.00786691850245 0.165155593193
0.00800739918999 0.165376785612
0.00814787987754 0.165598490671
0.00828836056508 0.165820710339
0.00842884125263 0.166043446592
0.00856932194017 0.166266701423
0.00870980262771 0.166490476833
0.00885028331526 0.166714774836
0.0089907640028 0.166939597456
0.00913124469034 0.16716494673
0.00927172537789 0.167390824707
0.00941220606543 0.167617233447
0.00955268675298 0.167844175023
0.00969316744052 0.168071651519
0.00983364812806 0.168299665032
0.00997412881561 0.168528217671
0.0101146095032 0.168757311558
0.0102550901907 0.168986948826
0.0103955708782 0.169217131622
0.0105360515658 0.169447862105
0.0106765322533 0.169679142448
0.0108170129409 0.169910974834
0.0109574936284 0.170143361463
0.011097974316 0.170376304544
0.0112384550035 0.170609806303
0.011378935691 0.170843868976
0.0115194163786 0.171078494815
0.0116598970661 0.171313686084
0.0118003777537 0.171549445062
0.0119408584412 0.17178577404
0.0120813391288 0.172022675324
0.0122218198163 0.172260151235
0.0123623005039 0.172498204105
0.0125027811914 0.172736836283
0.0126432618789 0.172976050131
0.0127837425665 0.173215848027
0.012924223254 0.173456232362
0.0130647039416 0.173697205542
0.0132051846291 0.173938769988
0.0133456653167 0.174180928137
0.0134861460042 0.174423682439
0.0136266266917 0.174667035361
0.0137671073793 0.174910989384
0.0139075880668 0.175155547005
0.0140480687544 0.175400710738
0.0141885494419 0.17564648311
0.0143290301295 0.175892866666
0.014469510817 0.176139863967
0.0146099915046 0.176387477589
0.0147504721921 0.176635710124
0.0148909528796 0.176884564181
0.0150314335672 0.177134042388
0.0151719142547 0.177384147385
0.0153123949423 0.177634881832
0.0154528756298 0.177886248407
0.0155933563174 0.178138249801
0.0157338370049 0.178390888726
0.0158743176924 0.17864416791
0.01601479838 0.178898090099
0.0161552790675 0.179152658056
0.0162957597551 0.179407874564
0.0164362404426 0.179663742421
0.0165767211302 0.179920264446
0.0167172018177 0.180177443474
0.0168576825053 0.180435282361
0.0169981631928 0.18069378398
0.0171386438803 0.180952951224
0.0172791245679 0.181212787003
0.0174196052554 0.18147329425
0.017560085943 0.181734475914
0.0177005666305 0.181996334964
0.0178410473181 0.182258874391
0.0179815280056 0.182522097204
0.0181220086931 0.182786006433
0.0182624893807 0.183050605127
0.0184029700682 0.183315896357
0.0185434507558 0.183581883215
0.0186839314433 0.183848568813
0.0188244121309 0.184115956283
0.0189648928184 0.18438404878
0.019105373506 0.18465284948
0.0192458541935 0.184922361581
0.019386334881 0.185192588303
0.0195268155686 0.185463532886
0.0196672962561 0.185735198595
0.0198077769437 0.186007588716
0.0199482576312 0.186280706559
0.0200887383188 0.186554555455
0.0202292190063 0.18682913876
0.0203696996938 0.187104459853
0.0205101803814 0.187380522134
0.0206506610689 0.187657329032
0.0207911417565 0.187934883995
0.020931622444 0.188213190499
0.0210721031316 0.188492252041
0.0212125838191 0.188772072146
0.0213530645067 0.189052654363
0.0214935451942 0.189334002265
0.0216340258817 0.189616119452
0.0217745065693 0.189899009549
0.0219149872568 0.190182676207
0.0220554679444 0.190467123104
0.0221959486319 0.190752353943
0.0223364293195 0.191038372456
0.022476910007 0.1913251824
0.0226173906945 0.19161278756
0.0227578713821 0.191901191749
0.0228983520696 0.192190398807
0.0230388327572 0.192480412604
0.0231793134447 0.192771237036
0.0233197941323 0.193062876028
0.0234602748198 0.193355333537
0.0236007555074 0.193648613545
0.0237412361949 0.193942720068
0.0238817168824 0.194237657148
0.02402219757 0.194533428859
0.0241626782575 0.194830039306
0.0243031589451 0.195127492623
0.0244436396326 0.195425792978
0.0245841203202 0.195724944568
0.0247246010077 0.196024951623
0.0248650816952 0.196325818404
0.0250055623828 0.196627549206
0.0251460430703 0.196930148356
0.0252865237579 0.197233620215
0.0254270044454 0.197537969175
0.025567485133 0.197843199665
0.0257079658205 0.198149316147
0.0258484465081 0.198456323117
0.0259889271956 0.198764225106
0.0261294078831 0.199073026681
0.0262698885707 0.199382732445
0.0264103692582 0.199693347037
0.0265508499458 0.200004875131
0.0266913306333 0.20031732144
0.0268318113209 0.200630690712
0.0269722920084 0.200944987735
0.0271127726959 0.201260217335
0.0272532533835 0.201576384373
0.027393734071 0.201893493755
0.0275342147586 0.20221155042
0.0276746954461 0.202530559351
0.0278151761337 0.202850525571
0.0279556568212 0.203171454142
0.0280961375088 0.203493350168
0.0282366181963 0.203816218795
0.0283770988838 0.20414006521
0.0285175795714 0.204464894645
0.0286580602589 0.204790712371
0.0287985409465 0.205117523708
0.028939021634 0.205445334014
0.0290795023216 0.205774148697
0.0292199830091 0.206103973207
0.0293604636966 0.20643481304
0.0295009443842 0.206766673739
0.0296414250717 0.207099560892
0.0297819057593 0.207433480137
0.0299223864468 0.207768437156
0.0300628671344 0.208104437684
0.0302033478219 0.2084414875
0.0303438285095 0.208779592436
0.030484309197 0.209118758372
0.0306247898845 0.20945899124
0.0307652705721 0.209800297023
0.0309057512596 0.210142681755
0.0310462319472 0.210486151523
0.0311867126347 0.210830712468
0.0313271933223 0.211176370782
0.0314676740098 0.211523132716
0.0316081546973 0.211871004572
0.0317486353849 0.212219992709
0.0318891160724 0.212570103542
0.03202959676 0.212921343546
0.0321700774475 0.21327371925
0.0323105581351 0.213627237243
0.0324510388226 0.213981904174
0.0325915195102 0.214337726751
0.0327320001977 0.214694711744
0.0328724808852 0.215052865982
0.0330129615728 0.21541219636
0.0331534422603 0.215772709834
0.0332939229479 0.216134413423
0.0334344036354 0.216497314212
0.033574884323 0.216861419351
0.0337153650105 0.217226736058
0.033855845698 0.217593271616
0.0339963263856 0.217961033378
0.0341368070731 0.218330028763
0.0342772877607 0.218700265265
0.0344177684482 0.219071750443
0.0345582491358 0.219444491932
0.0346987298233 0.219818497438
0.0348392105109 0.220193774741
0.0349796911984 0.220570331695
0.0351201718859 0.220948176231
0.0352606525735 0.221327316355
0.035401133261 0.221707760152
0.0355416139486 0.222089515785
0.0356820946361 0.222472591497
0.0358225753237 0.222856995612
0.0359630560112 0.223242736536
0.0361035366987 0.223629822757
0.0362440173863 0.22401826285
0.0363844980738 0.224408065471
0.0365249787614 0.224799239368
0.0366654594489 0.225191793372
0.0368059401365 0.225585736406
0.036946420824 0.225981077483
0.0370869015116 0.226377825705
0.0372273821991 0.226775990269
0.0373678628866 0.227175580468
0.0375083435742 0.227576605686
0.0376488242617 0.227979075408
0.0377893049493 0.228382999215
0.0379297856368 0.228788386787
0.0380702663244 0.229195247909
0.0382107470119 0.229603592463
0.0383512276994 0.230013430441
0.038491708387 0.230424771936
0.0386321890745 0.230837627151
0.0387726697621 0.231252006396
0.0389131504496 0.231667920092
0.0390536311372 0.232085378774
0.0391941118247 0.232504393087
0.0393345925123 0.232924973795
0.0394750731998 0.233347131777
0.0396155538873 0.233770878032
0.0397560345749 0.23419622368
0.0398965152624 0.234623179963
0.04003699595 0.235051758247
0.0401774766375 0.235481970025
0.0403179573251 0.235913826921
0.0404584380126 0.236347340685
0.0405989187001 0.236782523203
0.0407393993877 0.237219386494
0.0408798800752 0.237657942714
0.0410203607628 0.238098204159
0.0411608414503 0.238540183263
0.0413013221379 0.238983892608
0.0414418028254 0.239429344918
0.041582283513 0.239876553066
0.0417227642005 0.240325530076
0.041863244888 0.240776289126
0.0420037255756 0.241228843548
0.0421442062631 0.241683206832
0.0422846869507 0.242139392628
0.0424251676382 0.242597414752
0.0425656483258 0.243057287184
0.0427061290133 0.243519024074
0.0428466097008 0.243982639742
0.0429870903884 0.244448148684
0.0431275710759 0.244915565574
0.0432680517635 0.245384905266
0.043408532451 0.245856182798
0.0435490131386 0.246329413395
0.0436894938261 0.246804612472
0.0438299745137 0.24728179564
0.0439704552012 0.247760978702
0.0441109358887 0.248242177667
0.0442514165763 0.248725408745
0.0443918972638 0.249210688355
0.0445323779514 0.249698033126
0.0446728586389 0.250187459903
0.0448133393265 0.250678985753
0.044953820014 0.251172627961
0.0450943007015 0.251668404044
0.0452347813891 0.252166331749
0.0453752620766 0.252666429058
0.0455157427642 0.253168714194
0.0456562234517 0.253673205625
0.0457967041393 0.254179922068
0.0459371848268 0.254688882495
0.0460776655144 0.255200106137
0.0462181462019 0.255713612487
0.0463586268894 0.25622942131
0.046499107577 0.256747552643
0.0466395882645 0.257268026805
0.0467800689521 0.257790864397
0.0469205496396 0.258316086315
0.0470610303272 0.258843713747
0.0472015110147 0.259373768188
0.0473419917022 0.259906271439
0.0474824723898 0.260441245616
0.0476229530773 0.260978713158
0.0477634337649 0.261518696829
0.0479039144524 0.262061219732
0.04804439514 0.262606305307
0.0481848758275 0.263153977346
0.0483253565151 0.263704259996
0.0484658372026 0.264257177766
0.0486063178901 0.26481275554
0.0487467985777 0.265371018578
0.0488872792652 0.265931992528
0.0490277599528 0.266495703436
0.0491682406403 0.267062177749
0.0493087213279 0.267631442331
0.0494492020154 0.268203524465
0.049589682703 0.268778451869
0.0497301633905 0.269356252701
0.049870644078 0.269936955569
0.0500111247656 0.270520589546
0.0501516054531 0.271107184175
0.0502920861407 0.271696769482
0.0504325668282 0.272289375989
0.0505730475158 0.272885034723
0.0507135282033 0.273483777228
0.0508540088908 0.274085635578
0.0509944895784 0.274690642392
0.0511349702659 0.275298830841
0.0512754509535 0.275910234668
0.051415931641 0.276524888196
0.0515564123286 0.277142826348
0.0516968930161 0.277764084656
0.0518373737037 0.278388699283
0.0519778543912 0.27901670703
0.0521183350787 0.27964814536
0.0522588157663 0.280283052411
0.0523992964538 0.280921467014
0.0525397771414 0.281563428711
0.0526802578289 0.282208977773
0.0528207385165 0.28285815522
0.052961219204 0.283511002841
0.0531016998915 0.284167563212
0.0532421805791 0.28482787972
0.0533826612666 0.285491996583
0.0535231419542 0.286159958876
0.0536636226417 0.286831812549
0.0538041033293 0.287507604455
0.0539445840168 0.288187382377
0.0540850647044 0.288871195049
0.0542255453919 0.289559092188
0.0543660260794 0.290251124517
0.054506506767 0.290947343801
0.0546469874545 0.29164780287
0.0547874681421 0.292352555657
0.0549279488296 0.293061657226
0.0550684295172 0.293775163807
0.0552089102047 0.294493132834
0.0553493908922 0.295215622976
0.0554898715798 0.295942694183
0.0556303522673 0.296674407717
0.0557708329549 0.2974108262
0.0559113136424 0.298152013655
0.05605179433 0.298898035548
0.0561922750175 0.29964895884
0.0563327557051 0.30040485203
0.0564732363926 0.30116578521
0.0566137170801 0.301931830115
0.0567541977677 0.302703060181
0.0568946784552 0.303479550599
0.0570351591428 0.30426137838
0.0571756398303 0.305048622413
0.0573161205179 0.305841363534
0.0574566012054 0.306639684593
0.0575970818929 0.307443670529
0.0577375625805 0.308253408442
0.057878043268 0.309068987673
0.0580185239556 0.309890499887
0.0581590046431 0.310718039161
0.0582994853307 0.311551702074
0.0584399660182 0.312391587801
0.0585804467058 0.313237798217
0.0587209273933 0.314090438
0.0588614080808 0.314949614742
0.0590018887684 0.315815439067
0.0591423694559 0.316688024754
0.0592828501435 0.317567488865
0.059423330831 0.318453951883
0.0595638115186 0.319347537855
0.0597042922061 0.320248374544
0.0598447728936 0.321156593592
0.0599852535812 0.322072330686
0.0601257342687 0.32299572574
0.0602662149563 0.323926923085
0.0604066956438 0.32486607167
0.0605471763314 0.325813325274
0.0606876570189 0.326768842736
0.0608281377065 0.327732788194
0.060968618394 0.328705331337
0.0611090990815 0.329686647684
0.0612495797691 0.330676918871
0.0613900604566 0.331676332955
0.0615305411442 0.332685084754
0.0616710218317 0.333703376187
0.0618115025193 0.334731416659
0.0619519832068 0.335769423462
0.0620924638943 0.336817622202
0.0622329445819 0.337876247266
0.0623734252694 0.338945542319
0.062513905957 0.340025760837
0.0626543866445 0.341117166681
0.0627948673321 0.342220034718
0.0629353480196 0.343334651493
0.0630758287072 0.344461315948
0.0632163093947 0.345600340207
0.0633567900822 0.346752050425
0.0634972707698 0.347916787712
0.0636377514573 0.349094909129
0.0637782321449 0.350286788788
0.0639187128324 0.35149281904
0.06405919352 0.352713411777
0.0641996742075 0.353948999863
0.064340154895 0.355200038701
0.0644806355826 0.356467007954
0.0646211162701 0.357750413449
0.0647615969577 0.359050789277
0.0649020776452 0.360368700116
0.0650425583328 0.36170474382
0.0651830390203 0.363059554289
0.0653235197079 0.364433804687
0.0654640003954 0.365828211034
0.0656044810829 0.36724353625
0.0657449617705 0.368680594708
0.065885442458 0.370140257383
0.0660259231456 0.371623457707
0.0661664038331 0.373131198227
0.0663068845207 0.374664558237
0.0664473652082 0.376224702554
0.0665878458957 0.377812891643
0.0667283265833 0.379430493391
0.0668688072708 0.381078996845
0.0670092879584 0.382760028346
0.0671497686459 0.384475370613
0.0672902493335 0.386226985455
0.067430730021 0.38801704101
0.0675712107086 0.389847944703
0.0677116913961 0.391722383459
0.0678521720836 0.393643373287
0.0679926527712 0.395614321087
0.0681331334587 0.397639102642
0.0682736141463 0.399722162418
0.0684140948338 0.401868643264
0.0685545755214 0.404084557976
0.0686950562089 0.406377020899
0.0688355368964 0.408754568029
0.068976017584 0.411227611819
0.0691164982715 0.413809109004
0.0692569789591 0.416515581171
0.0693974596466 0.419368753508
0.0695379403342 0.422398357697
0.0696784210217 0.425647344198
0.0698189017093 0.429182777899
0.0699593823968 0.433123051956
0.0700998630843 0.437731317613


==> figuresAndData/dataForConditionalVarianceLaplaceProb0pt8.tex <==
-13.5 0.18006620585
-13.4733405504 0.18006620585
-13.4466811008 0.18006620585
-13.4200216512 0.18006620585
-13.3933622017 0.18006620585
-13.3667027521 0.18006620585
-13.3400433025 0.18006620585
-13.3133838529 0.18006620585
-13.2867244033 0.18006620585
-13.2600649537 0.18006620585
-13.2334055042 0.18006620585
-13.2067460546 0.18006620585
-13.180086605 0.18006620585
-13.1534271554 0.18006620585
-13.1267677058 0.18006620585
-13.1001082562 0.18006620585
-13.0734488067 0.18006620585
-13.0467893571 0.18006620585
-13.0201299075 0.18006620585
-12.9934704579 0.18006620585
-12.9668110083 0.18006620585
-12.9401515587 0.18006620585
-12.9134921091 0.18006620585
-12.8868326596 0.18006620585
-12.86017321 0.18006620585
-12.8335137604 0.18006620585
-12.8068543108 0.18006620585
-12.7801948612 0.18006620585
-12.7535354116 0.18006620585
-12.7268759621 0.18006620585
-12.7002165125 0.18006620585
-12.6735570629 0.18006620585
-12.6468976133 0.18006620585
-12.6202381637 0.18006620585
-12.5935787141 0.18006620585
-12.5669192646 0.18006620585
-12.540259815 0.18006620585
-12.5136003654 0.18006620585
-12.4869409158 0.18006620585
-12.4602814662 0.18006620585
-12.4336220166 0.18006620585
-12.406962567 0.18006620585
-12.3803031175 0.18006620585
-12.3536436679 0.18006620585
-12.3269842183 0.18006620585
-12.3003247687 0.18006620585
-12.2736653191 0.18006620585
-12.2470058695 0.18006620585
-12.22034642 0.18006620585
-12.1936869704 0.18006620585
-12.1670275208 0.18006620585
-12.1403680712 0.18006620585
-12.1137086216 0.18006620585
-12.087049172 0.18006620585
-12.0603897225 0.18006620585
-12.0337302729 0.18006620585
-12.0070708233 0.18006620585
-11.9804113737 0.18006620585
-11.9537519241 0.18006620585
-11.9270924745 0.18006620585
-11.900433025 0.18006620585
-11.8737735754 0.18006620585
-11.8471141258 0.18006620585
-11.8204546762 0.18006620585
-11.7937952266 0.18006620585
-11.767135777 0.18006620585
-11.7404763274 0.18006620585
-11.7138168779 0.18006620585
-11.6871574283 0.18006620585
-11.6604979787 0.18006620585
-11.6338385291 0.18006620585
-11.6071790795 0.18006620585
-11.5805196299 0.18006620585
-11.5538601804 0.18006620585
-11.5272007308 0.18006620585
-11.5005412812 0.18006620585
-11.4738818316 0.18006620585
-11.447222382 0.18006620585
-11.4205629324 0.18006620585
-11.3939034829 0.18006620585
-11.3672440333 0.18006620585
-11.3405845837 0.18006620585
-11.3139251341 0.18006620585
-11.2872656845 0.18006620585
-11.2606062349 0.18006620585
-11.2339467853 0.18006620585
-11.2072873358 0.18006620585
-11.1806278862 0.18006620585
-11.1539684366 0.18006620585
-11.127308987 0.180066205849
-11.1006495374 0.180066205849
-11.0739900878 0.180066205849
-11.0473306383 0.180066205849
-11.0206711887 0.180066205849
-10.9940117391 0.180066205849
-10.9673522895 0.180066205849
-10.9406928399 0.180066205849
-10.9140333903 0.180066205849
-10.8873739408 0.180066205849
-10.8607144912 0.180066205849
-10.8340550416 0.180066205849
-10.807395592 0.180066205849
-10.7807361424 0.180066205849
-10.7540766928 0.180066205849
-10.7274172432 0.180066205849
-10.7007577937 0.180066205849
-10.6740983441 0.180066205849
-10.6474388945 0.180066205849
-10.6207794449 0.180066205849
-10.5941199953 0.180066205849
-10.5674605457 0.180066205849
-10.5408010962 0.180066205849
-10.5141416466 0.180066205849
-10.487482197 0.180066205849
-10.4608227474 0.180066205849
-10.4341632978 0.180066205848
-10.4075038482 0.180066205848
-10.3808443987 0.180066205848
-10.3541849491 0.180066205848
-10.3275254995 0.180066205848
-10.3008660499 0.180066205848
-10.2742066003 0.180066205848
-10.2475471507 0.180066205848
-10.2208877011 0.180066205847
-10.1942282516 0.180066205847
-10.167568802 0.180066205847
-10.1409093524 0.180066205847
-10.1142499028 0.180066205847
-10.0875904532 0.180066205846
-10.0609310036 0.180066205846
-10.0342715541 0.180066205846
-10.0076121045 0.180066205846
-9.98095265489 0.180066205845
-9.95429320531 0.180066205845
-9.92763375572 0.180066205845
-9.90097430614 0.180066205844
-9.87431485655 0.180066205844
-9.84765540697 0.180066205843
-9.82099595739 0.180066205843
-9.7943365078 0.180066205842
-9.76767705822 0.180066205842
-9.74101760863 0.180066205841
-9.71435815905 0.18006620584
-9.68769870947 0.18006620584
-9.66103925988 0.180066205839
-9.6343798103 0.180066205838
-9.60772036071 0.180066205837
-9.58106091113 0.180066205836
-9.55440146154 0.180066205835
-9.52774201196 0.180066205834
-9.50108256238 0.180066205833
-9.47442311279 0.180066205831
-9.44776366321 0.18006620583
-9.42110421362 0.180066205828
-9.39444476404 0.180066205827
-9.36778531446 0.180066205825
-9.34112586487 0.180066205823
-9.31446641529 0.180066205821
-9.2878069657 0.180066205819
-9.26114751612 0.180066205817
-9.23448806654 0.180066205814
-9.20782861695 0.180066205811
-9.18116916737 0.180066205808
-9.15450971778 0.180066205805
-9.1278502682 0.180066205802
-9.10119081861 0.180066205798
-9.07453136903 0.180066205794
-9.04787191945 0.18006620579
-9.02121246986 0.180066205785
-8.99455302028 0.18006620578
-8.96789357069 0.180066205775
-8.94123412111 0.180066205769
-8.91457467153 0.180066205763
-8.88791522194 0.180066205756
-8.86125577236 0.180066205749
-8.83459632277 0.180066205741
-8.80793687319 0.180066205733
-8.7812774236 0.180066205724
-8.75461797402 0.180066205714
-8.72795852444 0.180066205703
-8.70129907485 0.180066205692
-8.67463962527 0.18006620568
-8.64798017568 0.180066205667
-8.6213207261 0.180066205653
-8.59466127652 0.180066205638
-8.56800182693 0.180066205622
-8.54134237735 0.180066205604
-8.51468292776 0.180066205585
-8.48802347818 0.180066205565
-8.46136402859 0.180066205543
-8.43470457901 0.18006620552
-8.40804512943 0.180066205494
-8.38138567984 0.180066205467
-8.35472623026 0.180066205438
-8.32806678067 0.180066205406
-8.30140733109 0.180066205372
-8.27474788151 0.180066205336
-8.24808843192 0.180066205296
-8.22142898234 0.180066205254
-8.19476953275 0.180066205208
-8.16811008317 0.180066205159
-8.14145063358 0.180066205107
-8.114791184 0.18006620505
-8.08813173442 0.180066204989
-8.06147228483 0.180066204923
-8.03481283525 0.180066204852
-8.00815338566 0.180066204776
-7.98149393608 0.180066204694
-7.9548344865 0.180066204606
-7.92817503691 0.180066204511
-7.90151558733 0.180066204409
-7.87485613774 0.180066204299
-7.84819668816 0.180066204181
-7.82153723857 0.180066204053
-7.79487778899 0.180066203917
-7.76821833941 0.180066203769
-7.74155888982 0.180066203611
-7.71489944024 0.180066203441
-7.68823999065 0.180066203257
-7.66158054107 0.18006620306
-7.63492109149 0.180066202848
-7.6082616419 0.18006620262
-7.58160219232 0.180066202374
-7.55494274273 0.18006620211
-7.52828329315 0.180066201826
-7.50162384356 0.180066201521
-7.47496439398 0.180066201192
-7.4483049444 0.180066200839
-7.42164549481 0.180066200459
-7.39498604523 0.18006620005
-7.36832659564 0.180066199611
-7.34166714606 0.180066199138
-7.31500769648 0.180066198629
-7.28834824689 0.180066198083
-7.26168879731 0.180066197495
-7.23502934772 0.180066196863
-7.20836989814 0.180066196183
-7.18171044856 0.180066195452
-7.15505099897 0.180066194666
-7.12839154939 0.180066193821
-7.1017320998 0.180066192913
-7.07507265022 0.180066191936
-7.04841320063 0.180066190886
-7.02175375105 0.180066189758
-6.99509430147 0.180066188544
-6.96843485188 0.180066187239
-6.9417754023 0.180066185837
-6.91511595271 0.18006618433
-6.88845650313 0.180066182709
-6.86179705355 0.180066180968
-6.83513760396 0.180066179096
-6.80847815438 0.180066177083
-6.78181870479 0.180066174921
-6.75515925521 0.180066172597
-6.72849980562 0.180066170099
-6.70184035604 0.180066167415
-6.67518090646 0.18006616453
-6.64852145687 0.18006616143
-6.62186200729 0.1800661581
-6.5952025577 0.18006615452
-6.56854310812 0.180066150675
-6.54188365854 0.180066146542
-6.51522420895 0.180066142103
-6.48856475937 0.180066137333
-6.46190530978 0.180066132208
-6.4352458602 0.180066126703
-6.40858641061 0.180066120789
-6.38192696103 0.180066114436
-6.35526751145 0.180066107611
-6.32860806186 0.18006610028
-6.30194861228 0.180066092406
-6.27528916269 0.180066083949
-6.24862971311 0.180066074865
-6.22197026353 0.18006606511
-6.19531081394 0.180066054632
-6.16865136436 0.180066043381
-6.14199191477 0.180066031298
-6.11533246519 0.180066018323
-6.0886730156 0.18006600439
-6.06201356602 0.18006598943
-6.03535411644 0.180065973367
-6.00869466685 0.180065956121
-5.98203521727 0.180065937605
-5.95537576768 0.180065917727
-5.9287163181 0.180065896387
-5.90205686852 0.180065873479
-5.87539741893 0.180065848889
-5.84873796935 0.180065822493
-5.82207851976 0.180065794161
-5.79541907018 0.180065763752
-5.76875962059 0.180065731116
-5.74210017101 0.18006569609
-5.71544072143 0.180065658501
-5.68878127184 0.180065618164
-5.66212182226 0.18006557488
-5.63546237267 0.180065528435
-5.60880292309 0.180065478601
-5.58214347351 0.180065425133
-5.55548402392 0.180065367768
-5.52882457434 0.180065306227
-5.50216512475 0.180065240207
-5.47550567517 0.180065169386
-5.44884622558 0.18006509342
-5.422186776 0.180065011937
-5.39552732642 0.180064924542
-5.36886787683 0.180064830812
-5.34220842725 0.18006473029
-5.31554897766 0.180064622492
-5.28888952808 0.180064506896
-5.2622300785 0.180064382944
-5.23557062891 0.180064250041
-5.20891117933 0.180064107546
-5.18225172974 0.180063954777
-5.15559228016 0.180063791001
-5.12893283058 0.180063615435
-5.10227338099 0.180063427242
-5.07561393141 0.180063225523
-5.04895448182 0.18006300932
-5.02229503224 0.180062777605
-4.99563558265 0.180062529282
-4.96897613307 0.180062263174
-4.94231668349 0.180061978026
-4.9156572339 0.180061672493
-4.88899778432 0.180061345139
-4.86233833473 0.180060994426
-4.83567888515 0.180060618713
-4.80901943557 0.180060216241
-4.78235998598 0.180059785133
-4.7557005364 0.180059323382
-4.72904108681 0.180058828843
-4.70238163723 0.180058299221
-4.67572218764 0.180057732068
-4.64906273806 0.180057124763
-4.62240328848 0.180056474511
-4.59574383889 0.180055778323
-4.56908438931 0.180055033006
-4.54242493972 0.180054235151
-4.51576549014 0.180053381116
-4.48910604056 0.180052467013
-4.46244659097 0.18005148869
-4.43578714139 0.180050441713
-4.4091276918 0.180049321352
-4.38246824222 0.180048122555
-4.35580879263 0.180046839931
-4.32914934305 0.180045467727
-4.30248989347 0.180043999807
-4.27583044388 0.180042429621
-4.2491709943 0.180040750183
-4.22251154471 0.180038954043
-4.19585209513 0.180037033254
-4.16919264555 0.180034979343
-4.14253319596 0.180032783275
-4.11587374638 0.180030435419
-4.08921429679 0.18002792551
-4.06255484721 0.180025242605
-4.03589539762 0.180022375046
-4.00923594804 0.180019310412
-3.98257649846 0.18001603547
-3.95591704887 0.180012536124
-3.92925759929 0.180008797363
-3.9025981497 0.180004803205
-3.87593870012 0.180000536633
-3.84927925054 0.179995979534
-3.82261980095 0.179991112629
-3.79596035137 0.179985915406
-3.76930090178 0.179980366038
-3.7426414522 0.179974441312
-3.71598200261 0.179968116535
-3.68932255303 0.179961365452
-3.66266310345 0.179954160151
-3.63600365386 0.179946470962
-3.60934420428 0.179938266353
-3.58268475469 0.179929512822
-3.55602530511 0.179920174778
-3.52936585553 0.179910214422
-3.50270640594 0.179899591617
-3.47604695636 0.179888263751
-3.44938750677 0.179876185598
-3.42272805719 0.179863309165
-3.3960686076 0.179849583539
-3.36940915802 0.179834954718
-3.34274970844 0.17981936544
-3.31609025885 0.179802755002
-3.28943080927 0.179785059069
-3.26277135968 0.179766209475
-3.2361119101 0.179746134012
-3.20945246052 0.179724756219
-3.18279301093 0.179701995146
-3.15613356135 0.179677765124
-3.12947411176 0.179651975509
-3.10281466218 0.179624530432
-3.0761552126 0.179595328523
-3.04949576301 0.179564262635
-3.02283631343 0.179531219553
-2.99617686384 0.17949607969
-2.96951741426 0.179458716776
-2.94285796467 0.179418997537
-2.91619851509 0.179376781353
-2.88953906551 0.179331919921
-2.86287961592 0.179284256893
-2.83622016634 0.179233627512
-2.80956071675 0.179179858237
-2.78290126717 0.179122766355
-2.75624181759 0.179062159589
-2.729582368 0.178997835693
-2.70292291842 0.178929582048
-2.67626346883 0.178857175241
-2.64960401925 0.178780380648
-2.62294456966 0.178698952009
-2.59628512008 0.178612631007
-2.5696256705 0.178521146838
-2.54296622091 0.178424215791
-2.51630677133 0.178321540833
-2.48964732174 0.178212811193
-2.46298787216 0.178097701971
-2.43632842258 0.177975873746
-2.40966897299 0.177846972214
-2.38300952341 0.177710627842
-2.35635007382 0.177566455552
-2.32969062424 0.177414054436
-2.30303117465 0.177253007512
-2.27637172507 0.177082881523
-2.24971227549 0.176903226788
-2.2230528259 0.176713577118
-2.19639337632 0.176513449793
-2.16973392673 0.176302345627
-2.14307447715 0.176079749112
-2.11641502757 0.175845128671
-2.08975557798 0.17559793702
-2.0630961284 0.175337611652
-2.03643667881 0.175063575474
-2.00977722923 0.174775237587
-1.98311777964 0.174471994251
-1.95645833006 0.174153230035
-1.92979888048 0.173818319191
-1.90313943089 0.17346662725
-1.87647998131 0.17309751289
-1.84982053172 0.17271033008
-1.82316108214 0.172304430546
-1.79650163256 0.171879166567
-1.76984218297 0.171433894163
-1.74318273339 0.170967976678
-1.7165232838 0.17048078882
-1.68986383422 0.169971721186
-1.66320438463 0.169440185324
-1.63654493505 0.168885619368
-1.60988548547 0.168307494311
-1.58322603588 0.167705320966
-1.5565665863 0.167078657671
-1.52990713671 0.16642711881
-1.50324768713 0.165750384224
-1.47658823755 0.165048209592
-1.44992878796 0.164320437852
-1.42326933838 0.163567011796
-1.39660988879 0.162787987905
-1.36995043921 0.161983551579
-1.34329098962 0.161154033884
-1.31663154004 0.160299929963
-1.28997209046 0.159421919319
-1.26331264087 0.158520888136
-1.23665319129 0.157597953909
-1.2099937417 0.156654492644
-1.18333429212 0.155692168961
-1.15667484254 0.154712969489
-1.13001539295 0.153719240024
-1.10335594337 0.152713727004
-1.07669649378 0.151699623988
-1.0500370442 0.150680623968
-1.02337759461 0.149660978534
-0.996718145031 0.148645565156
-0.970058695447 0.147639964151
-0.943399245863 0.146650547295
-0.916739796278 0.145684580559
-0.890080346694 0.144750344086
-0.86342089711 0.143857273416
-0.836761447526 0.143016127072
-0.810101997942 0.142239187137
-0.783442548358 0.141540501462
-0.756783098773 0.140936178848
-0.730123649189 0.140444752269
-0.703464199605 0.140087630298
-0.676804750021 0.139889664056
-0.650145300437 0.139879867132
-0.623485850853 0.14009234051
-0.596826401268 0.140567475868
-0.570166951684 0.141353542451
-0.5435075021 0.142508811166
-0.516848052516 0.144104445094
-0.490188602932 0.146228506482
-0.463529153348 0.148991629637
-0.436869703764 0.15253524941
-0.410210254179 0.157043879486
-0.383550804595 0.162764060506
-0.356891355011 0.170034816141
-0.330231905427 0.179339137067
-0.303572455843 0.191396786496
-0.276913006259 0.207346459256
-0.250253556674 0.229148590088
-0.22359410709 0.260653857373
-0.196934657506 0.311535299056


==> figuresAndData/dataForGaussianSigma1.tex <==
0.998404231942 2.1954407823e-09
0.996808470268 1.71569571284e-08
0.995212721359 5.76503182146e-08
0.993616991599 1.36440680462e-07
0.992021287371 2.66292281172e-07
0.990425615056 4.59968132197e-07
0.988829981037 7.30229713657e-07
0.987234391695 1.08983666768e-06
0.985638853412 1.55154649222e-06
0.984043372566 2.12811423492e-06
0.982447955539 2.83229218707e-06
0.980852608708 3.67682957764e-06
0.979257338452 4.67447226737e-06
0.977662151148 5.83796244303e-06
0.976067053172 7.18003831172e-06
0.974472050899 8.71343379536e-06
0.972877150702 1.04508782252e-05
0.971282358956 1.24050960367e-05
0.96968768203 1.45888064641e-05
0.968093126294 1.70147232357e-05
0.966498698118 1.96955542691e-05
0.964904403869 2.26440013662e-05
0.963310249911 2.5872759909e-05
0.961716242608 2.93945185555e-05
0.960122388323 3.32219589353e-05
0.958528693415 3.73677553459e-05
0.956935164243 4.1844574449e-05
0.955341807163 4.66650749672e-05
0.953748628528 5.18419073808e-05
0.952155634692 5.73877136249e-05
0.950562832003 6.33151267866e-05
0.948970226809 6.96367708028e-05
0.947377825456 7.6365260158e-05
0.945785634286 8.35131995824e-05
0.944193659639 9.10931837503e-05
0.942601907853 9.91177969792e-05
0.941010385262 0.000107599612928
0.939419098199 0.000116551194299
0.937828052994 0.000125985092532
0.936237255972 0.000135913847511
0.934646713457 0.000146349987261
0.93305643177 0.000157306027649
0.931466417227 0.000168794472084
0.929876676144 0.000180827811223
0.92828721483 0.000193418522667
0.926698039593 0.000206579070666
0.925109156737 0.000220321905825
0.923520572564 0.0002346594648
0.921932293369 0.000249604170008
0.920344325446 0.000265168429326
0.918756675085 0.000281364635798
0.917169348571 0.00029820516734
0.915582352187 0.000315702386445
0.913995692211 0.000333868639887
0.912409374915 0.000352716258429
0.910823406571 0.000372257556528
0.909237793445 0.000392504832046
0.907652541796 0.000413470365951
0.906067657883 0.000435166422033
0.904483147959 0.000457605246605
0.902899018271 0.000480799068219
0.901315275063 0.000504760097369
0.899731924575 0.000529500526208
0.898148973041 0.000555032528254
0.896566426691 0.000581368258103
0.894984291749 0.000608519851141
0.893402574435 0.000636499423257
0.891821280965 0.000665319070553
0.890240417547 0.000694990869063
0.888659990388 0.000725526874463
0.887080005686 0.000756939121787
0.885500469636 0.000789239625142
0.883921388427 0.000822440377426
0.882342768242 0.000856553350043
0.88076461526 0.000891590492622
0.879186935652 0.000927563732731
0.877609735585 0.000964484975601
0.876033021221 0.00100236610384
0.874456798715 0.00104121897717
0.872881074217 0.0010810554321
0.87130585387 0.00112188728172
0.869731143811 0.00116372631537
0.868156950172 0.00120658429836
0.866583279079 0.00125047297173
0.86501013665 0.00129540405195
0.863437528998 0.00134138923065
0.861865462231 0.00138844017435
0.860293942447 0.00143656852416
0.85872297574 0.00148578589556
0.857152568198 0.00153610387808
0.855582725901 0.00158753403504
0.854013454922 0.0016400879033
0.852444761329 0.00169377699297
0.85087665118 0.00174861278714
0.84930913053 0.00180460674162
0.847742205425 0.00186177028469
0.846175881903 0.0019201148168
0.844610165997 0.0019796517103
0.84304506373 0.00204039230923
0.841480581122 0.002102347929
0.839916724181 0.00216552985615
0.83835349891 0.00222994934809
0.836790911305 0.00229561763283
0.835228967353 0.00236254590872
0.833667673035 0.0024307453442
0.832107034322 0.00250022707753
0.83054705718 0.00257100221653
0.828987747565 0.00264308183836
0.827429111426 0.00271647698919
0.825871154704 0.00279119868402
0.824313883331 0.00286725790638
0.822757303234 0.0029446656081
0.821201420328 0.00302343270904
0.819646240522 0.00310357009686
0.818091769716 0.00318508862675
0.816538013802 0.00326799912117
0.814984978663 0.00335231236965
0.813432670175 0.00343803912848
0.811881094202 0.00352519012053
0.810330256604 0.00361377603493
0.80878016323 0.0037038075269
0.807230819918 0.00379529521745
0.805682232502 0.00388824969316
0.804134406802 0.00398268150593
0.802587348634 0.00407860117278
0.801041063801 0.00417601917552
0.799495558099 0.00427494596063
0.797950837315 0.00437539193891
0.796406907225 0.00447736748533
0.794863773596 0.00458088293872
0.793321442189 0.00468594860162
0.791779918751 0.00479257473997
0.790239209023 0.00490077158292
0.788699318733 0.00501054932257
0.787160253604 0.0051219181138
0.785622019345 0.00523488807395
0.784084621658 0.00534946928268
0.782548066233 0.00546567178168
0.781012358753 0.00558350557448
0.779477504888 0.0057029806262
0.777943510301 0.00582410686337
0.776410380643 0.00594689417366
0.774878121554 0.00607135240567
0.773346738667 0.00619749136873
0.771816237602 0.00632532083267
0.77028662397 0.00645485052759
0.768757903372 0.00658609014368
0.767230081396 0.00671904933095
0.765703163623 0.00685373769907
0.764177155622 0.0069901648171
0.762652062951 0.00712834021336
0.761127891157 0.00726827337512
0.759604645777 0.00740997374848
0.758082332339 0.00755345073809
0.756560956356 0.00769871370701
0.755040523334 0.00784577197644
0.753521038765 0.00799463482556
0.752002508133 0.00814531149131
0.750484936909 0.0082978111682
0.748968330553 0.00845214300807
0.747452694515 0.00860831611996
0.745938034231 0.00876633956983
0.744424355129 0.00892622238044
0.742911662623 0.00908797353109
0.741399962119 0.00925160195748
0.739889259007 0.00941711655147
0.738379558668 0.00958452616091
0.736870866473 0.00975383958945
0.735363187777 0.00992506559636
0.733856527928 0.0100982128963
0.732350892259 0.0102732901592
0.730846286092 0.01045030601
0.729342714737 0.0106292690286
0.727840183494 0.0108101877494
0.726338697649 0.0109930706614
0.724838262475 0.011177926208
0.723338883236 0.0113647627866
0.721840565181 0.0115535887487
0.720343313548 0.0117444123993
0.718847133564 0.0119372419974
0.717352030441 0.0121320857551
0.715858009381 0.0123289518381
0.714365075572 0.0125278483648
0.71287323419 0.0127287834068
0.711382490399 0.0129317649884
0.70989284935 0.0131368010864
0.708404316181 0.0133438996301
0.706916896019 0.0135530685011
0.705430593976 0.0137643155329
0.703945415152 0.0139776485112
0.702461364634 0.0141930751733
0.700978447498 0.0144106032081
0.699496668805 0.014630240256
0.698016033603 0.0148519939087
0.696536546928 0.0150758717091
0.695058213802 0.015301881151
0.693581039235 0.015530029679
0.692105028222 0.0157603246886
0.690630185747 0.0159927735257
0.689156516779 0.0162273834865
0.687684026275 0.0164641618175
0.686212719176 0.0167031157155
0.684742600413 0.0169442523271
0.683273674902 0.0171875787486
0.681805947545 0.0174331020261
0.68033942323 0.0176808291553
0.678874106833 0.0179307670812
0.677410003216 0.0181829226981
0.675947117225 0.0184373028494
0.674485453696 0.0186939143275
0.673025017449 0.0189527638737
0.671565813289 0.0192138581781
0.67010784601 0.0194772038791
0.668651120389 0.0197428075639
0.667195641191 0.0200106757679
0.665741413167 0.0202808149748
0.664288441053 0.0205532316164
0.662836729571 0.0208279320723
0.661386283429 0.0211049226702
0.659937107321 0.0213842096854
0.658489205927 0.0216657993408
0.657042583912 0.021949697807
0.655597245926 0.0222359112018
0.654153196607 0.0225244455903
0.652710440576 0.0228153069848
0.651268982441 0.0231085013448
0.649828826794 0.0234040345764
0.648389978215 0.0237019125329
0.646952441268 0.0240021410142
0.645516220501 0.0243047257668
0.644081320449 0.0246096724837
0.642647745631 0.0249169868045
0.641215500554 0.025226674315
0.639784589707 0.0255387405472
0.638355017565 0.0258531909793
0.636926788589 0.0261700310355
0.635499907225 0.0264892660861
0.634074377903 0.026810901447
0.632650205039 0.0271349423801
0.631227393032 0.0274613940928
0.62980594627 0.0277902617382
0.628385869121 0.0281215504148
0.626967165942 0.0284552651667
0.625549841071 0.0287914109831
0.624133898835 0.0291299927987
0.622719343541 0.0294710154932
0.621306179485 0.0298144838913
0.619894410945 0.030160402763
0.618484042185 0.0305087768232
0.617075077452 0.0308596107313
0.615667520979 0.031212909092
0.614261376983 0.0315686764544
0.612856649666 0.0319269173123
0.611453343213 0.0322876361043
0.610051461795 0.0326508372132
0.608651009567 0.0330165249665
0.607251990667 0.033384703636
0.605854409219 0.0337553774378
0.604458269331 0.0341285505324
0.603063575094 0.0345042270245
0.601670330585 0.0348824109627
0.600278539863 0.03526310634
0.598888206974 0.0356463170933
0.597499335945 0.0360320471037
0.59611193079 0.0364203001958
0.594725995504 0.0368110801386
0.593341534069 0.0372043906447
0.591958550449 0.0376002353704
0.590577048592 0.0379986179159
0.589197032431 0.0383995418252
0.587818505883 0.0388030105858
0.586441472848 0.0392090276288
0.585065937209 0.0396175963291
0.583691902835 0.040028720005
0.582319373577 0.0404424019183
0.58094835327 0.0408586452744
0.579578845735 0.0412774532221
0.578210854772 0.0416988288535
0.57684438417 0.0421227752042
0.575479437698 0.0425492952532
0.57411601911 0.0429783919229
0.572754132142 0.0434100680787
0.571393780517 0.0438443265296
0.570034967938 0.0442811700277
0.568677698093 0.0447206012685
0.567321974653 0.0451626228904
0.565967801274 0.0456072374755
0.564615181593 0.0460544475486
0.563264119233 0.046504255578
0.561914617797 0.046956663975
0.560566680875 0.0474116750942
0.559220312039 0.0478692912331
0.557875514842 0.0483295146326
0.556532292825 0.0487923474766
0.555190649507 0.0492577918922
0.553850588394 0.0497258499494
0.552512112974 0.0501965236615
0.551175226719 0.0506698149849
0.549839933081 0.0511457258192
0.5485062355 0.0516242580069
0.547174137396 0.0521054133337
0.545843642172 0.0525891935286
0.544514753215 0.0530756002634
0.543187473895 0.0535646351534
0.541861807566 0.0540562997568
0.540537757563 0.0545505955751
0.539215327205 0.0550475240528
0.537894519795 0.0555470865777
0.536575338616 0.056049284481
0.535257786938 0.0565541190367
0.533941868011 0.0570615914623
0.532627585068 0.0575717029186
0.531314941328 0.0580844545096
0.530003939988 0.0585998472825
0.528694584231 0.059117882228
0.527386877224 0.05963856028
0.526080822113 0.0601618823159
0.52477642203 0.0606878491566
0.523473680089 0.061216461566
0.522172599386 0.0617477202521
0.520873183 0.0622816258658
0.519575433993 0.062818179002
0.518279355411 0.0633573801989
0.51698495028 0.0638992299384
0.515692221612 0.0644437286461
0.514401172398 0.0649908766911
0.513111805614 0.0655406743866
0.51182412422 0.0660931219891
0.510538131155 0.0666482196993
0.509253829343 0.0672059676616
0.50797122169 0.0677663659643
0.506690311086 0.0683294146397
0.505411100402 0.0688951136642
0.504133592491 0.0694634629581
0.502857790191 0.070034462386
0.50158369632 0.0706081117564
0.500311313681 0.0711844108223
0.499040645057 0.0717633592809
0.497771693216 0.0723449567737
0.496504460907 0.0729292028865
0.495238950862 0.0735160971499
0.493975165796 0.0741056390387
0.492713108404 0.0746978279724
0.491452781368 0.0752926633152
0.490194187349 0.075890144376
0.48893732899 0.0764902704085
0.48768220892 0.0770930406112
0.486428829748 0.0776984541276
0.485177194065 0.0783065100462
0.483927304446 0.0789172074006
0.482679163448 0.0795305451695
0.481432773609 0.0801465222769
0.480188137452 0.0807651375921
0.47894525748 0.0813863899296
0.47770413618 0.0820102780497
0.476464776021 0.082636800658
0.475227179455 0.0832659564059
0.473991348914 0.0838977438903
0.472757286816 0.0845321616542
0.471524995559 0.0851692081863
0.470294477523 0.0858088819212
0.469065735072 0.0864511812399
0.467838770553 0.0870961044692
0.466613586293 0.0877436498824
0.465390184602 0.088393815699
0.464168567774 0.0890466000851
0.462948738083 0.0897020011531
0.461730697789 0.0903600169624
0.46051444913 0.0910206455187
0.45929999433 0.0916838847749
0.458087335592 0.0923497326307
0.456876475105 0.0930181869327
0.455667415038 0.093689245475
0.454460157543 0.0943629059986
0.453254704754 0.0950391661921
0.452051058788 0.0957180236913
0.450849221745 0.0963994760799
0.449649195705 0.097083520889
0.448450982733 0.0977701555977
0.447254584875 0.0984593776329
0.44606000416 0.0991511843695
0.444867242599 0.0998455731307
0.443676302185 0.100542541188
0.442487184894 0.10124208576
0.441299892685 0.101944204017
0.440114427498 0.102648893074
0.438930791257 0.103356149997
0.437748985866 0.1040659718
0.436569013214 0.104778355448
0.435390875171 0.105493297851
0.434214573591 0.106210795873
0.433040110307 0.106930846324
0.431867487138 0.107653445965
0.430696705884 0.108378591505
0.429527768327 0.109106279605
0.428360676233 0.109836506874
0.427195431349 0.110569269873
0.426032035404 0.11130456511
0.424870490112 0.112042389047
0.423710797167 0.112782738094
0.422552958246 0.113525608612
0.42139697501 0.114270996912
0.4202428491 0.115018899258
0.419090582142 0.115769311863
0.417940175743 0.116522230892
0.416791631493 0.11727765246
0.415644950965 0.118035572636
0.414500135713 0.118795987438
0.413357187275 0.119558892836
0.412216107172 0.120324284753
0.411076896905 0.121092159064
0.409939557961 0.121862511595
0.408804091808 0.122635338124
0.407670499895 0.123410634384
0.406538783656 0.124188396057
0.405408944507 0.124968618781
0.404280983847 0.125751298144
0.403154903056 0.12653642969
0.402030703499 0.127324008914
0.400908386521 0.128114031265
0.399787953452 0.128906492145
0.398669405604 0.129701386911
0.397552744272 0.130498710874
0.396437970732 0.131298459296
0.395325086245 0.132100627396
0.394214092054 0.132905210347
0.393104989385 0.133712203276
0.391997779445 0.134521601264
0.390892463427 0.135333399348
0.389789042504 0.13614759252
0.388687517832 0.136964175725
0.387587890553 0.137783143867
0.386490161788 0.138604491802
0.385394332644 0.139428214344
0.384300404207 0.140254306261
0.383208377551 0.141082762278
0.382118253729 0.141913577078
0.381030033778 0.142746745296
0.379943718718 0.143582261527
0.378859309553 0.144420120322
0.37777680727 0.145260316188
0.376696212836 0.14610284359
0.375617527205 0.146947696949
0.374540751312 0.147794870646
0.373465886074 0.148644359017
0.372392932395 0.149496156356
0.371321891158 0.150350256916
0.370252763231 0.151206654909
0.369185549464 0.152065344502
0.368120250694 0.152926319824
0.367056867735 0.15378957496
0.365995401389 0.154655103957
0.36493585244 0.155522900818
0.363878221655 0.156392959506
0.362822509784 0.157265273945
0.36176871756 0.158139838017
0.3607168457 0.159016645564
0.359666894906 0.159895690389
0.35861886586 0.160776966255
0.357572759229 0.161660466884
0.356528575664 0.16254618596
0.355486315798 0.163434117127
0.35444598025 0.16432425399
0.353407569619 0.165216590116
0.352371084491 0.166111119033
0.351336525432 0.16700783423
0.350303892994 0.167906729159
0.349273187713 0.168807797232
0.348244410107 0.169711031824
0.347217560677 0.170616426274
0.346192639911 0.171523973881
0.345169648276 0.172433667908
0.344148586227 0.173345501582
0.343129454201 0.17425946809
0.342112252617 0.175175560586
0.341096981881 0.176093772185
0.340083642381 0.177014095968
0.339072234488 0.177936524977
0.338062758559 0.178861052221
0.337055214934 0.179787670671
0.336049603935 0.180716373265
0.335045925872 0.181647152904
0.334044181035 0.182580002455
0.3330443697 0.183514914749
0.332046492127 0.184451882584
0.331050548559 0.185390898722
0.330056539224 0.186331955892
0.329064464334 0.187275046788
0.328074324084 0.188220164073
0.327086118655 0.189167300372
0.326099848212 0.19011644828
0.325115512902 0.191067600357
0.324133112858 0.192020749133
0.323152648197 0.192975887102
0.322174119022 0.193933006727
0.321197525416 0.194892100439
0.320222867451 0.195853160635
0.31925014518 0.196816179684
0.318279358643 0.197781149919
0.317310507863 0.198748063645
0.316343592847 0.199716913135
0.315378613588 0.200687690628
0.314415570063 0.201660388337
0.313454462232 0.202634998442
0.312495290043 0.203611513091
0.311538053425 0.204589924407
0.310582752293 0.205570224477
0.309629386549 0.206552405362
0.308677956077 0.207536459094
0.307728460745 0.208522377673
0.30678090041 0.209510153073
0.305835274908 0.210499777237
0.304891584066 0.21149124208
0.30394982769 0.212484539489
0.303010005577 0.213479661324
0.302072117503 0.214476599414
0.301136163233 0.215475345563
0.300202142517 0.216475891547
0.299270055086 0.217478229114
0.298339900662 0.218482349986
0.297411678947 0.219488245857
0.296485389632 0.220495908397
0.29556103239 0.221505329245
0.294638606882 0.222516500019
0.293718112752 0.223529412307
0.292799549631 0.224544057675
0.291882917134 0.225560427661
0.290968214863 0.226578513778
0.290055442403 0.227598307516
0.289144599328 0.228619800337
0.288235685194 0.229642983681
0.287328699544 0.230667848963
0.286423641906 0.231694387574
0.285520511796 0.23272259088
0.284619308712 0.233752450226
0.28372003214 0.234783956931
0.28282268155 0.235817102292
0.281927256401 0.236851877583
0.281033756134 0.237888274056
0.280142180178 0.238926282937
0.279252527946 0.239965895436
0.27836479884 0.241007102734
0.277478992245 0.242049895996
0.276595107534 0.243094266362
0.275713144064 0.244140204952
0.27483310118 0.245187702865
0.273954978211 0.246236751177
0.273078774474 0.247287340947
0.272204489272 0.248339463211
0.271332121893 0.249393108984
0.270461671612 0.250448269264
0.26959313769 0.251504935028
0.268726519374 0.252563097231
0.2678618159 0.253622746813
0.266999026485 0.254683874692
0.266138150339 0.255746471769
0.265279186652 0.256810528924
0.264422134606 0.25787603702
0.263566993366 0.258942986904
0.262713762085 0.260011369401
0.261862439903 0.26108117532
0.261013025945 0.262152395455
0.260165519324 0.26322502058
0.259319919141 0.264299041452
0.25847622448 0.265374448812
0.257634434416 0.266451233386
0.256794548008 0.26752938588
0.255956564303 0.268608896987
0.255120482335 0.269689757384
0.254286301126 0.270771957732
0.253454019682 0.271855488674
0.252623636999 0.272940340842
0.25179515206 0.274026504851
0.250968563833 0.275113971302
0.250143871274 0.27620273078
0.249321073329 0.277292773857
0.248500168927 0.278384091092
0.247681156987 0.279476673028
0.246864036414 0.280570510197
0.246048806103 0.281665593115
0.245235464933 0.282761912286
0.244424011772 0.283859458203
0.243614445477 0.284958221343
0.24280676489 0.286058192173
0.242000968842 0.287159361148
0.241197056152 0.288261718709
0.240395025626 0.289365255288
0.239594876058 0.290469961303
0.238796606229 0.291575827162
0.23800021491 0.292682843261
0.237205700858 0.293790999988
0.236413062818 0.294900287717
0.235622299524 0.296010696814
0.234833409697 0.297122217633
0.234046392046 0.29823484052
0.23326124527 0.29934855581
0.232477968053 0.300463353829
0.231696559071 0.301579224894
0.230917016984 0.302696159312
0.230139340443 0.303814147384
0.229363528088 0.304933179399
0.228589578545 0.306053245639
0.22781749043 0.30717433638
0.227047262347 0.308296441886
0.226278892888 0.309419552418
0.225512380634 0.310543658226
0.224747724156 0.311668749553
0.22398492201 0.312794816639
0.223223972745 0.313921849712
0.222464874896 0.315049838996
0.221707626987 0.31617877471
0.220952227531 0.317308647065
0.220198675031 0.318439446267
0.219446967978 0.319571162515
0.218697104851 0.320703786004
0.21794908412 0.321837306924
0.217202904243 0.32297171546
0.216458563666 0.324107001791
0.215716060827 0.325243156092
0.214975394149 0.326380168534
0.214236562049 0.327518029285
0.213499562929 0.328656728508
0.212764395183 0.329796256361
0.212031057194 0.330936603001
0.211299547334 0.33207775858
0.210569863963 0.333219713249
0.209842005434 0.334362457155
0.209115970085 0.335505980441
0.208391756248 0.336650273251
0.207669362243 0.337795325723
0.206948786377 0.338941127997
0.206230026952 0.340087670209
0.205513082254 0.341234942493
0.204797950564 0.342382934983
0.20408463015 0.343531637813
0.203373119269 0.344681041113
0.202663416172 0.345831135015
0.201955519095 0.34698190965
0.201249426268 0.348133355149
0.200545135909 0.349285461642
0.199842646227 0.35043821926
0.19914195542 0.351591618134
0.198443061679 0.352745648396
0.197745963182 0.35390030018
0.197050658099 0.355055563618
0.196357144591 0.356211428846
0.195665420808 0.357367886002
0.194975484891 0.358524925222
0.194287334971 0.359682536648
0.193600969171 0.360840710421
0.192916385604 0.361999436688
0.192233582373 0.363158705593
0.191552557572 0.364318507289
0.190873309286 0.365478831926
0.19019583559 0.366639669663
0.189520134553 0.367801010657
0.188846204229 0.368962845071
0.188174042669 0.370125163073
0.187503647912 0.371287954834
0.186835017987 0.372451210526
0.186168150917 0.373614920331
0.185503044714 0.374779074431
0.184839697381 0.375943663014
0.184178106915 0.377108676275
0.183518271301 0.378274104412
0.182860188516 0.379439937628
0.182203856531 0.380606166133
0.181549273304 0.381772780142
0.180896436789 0.382939769876
0.180245344929 0.384107125563
0.179595995658 0.385274837435
0.178948386903 0.386442895734
0.178302516582 0.387611290705
0.177658382606 0.388780012602
0.177015982875 0.389949051687
0.176375315283 0.391118398228
0.175736377716 0.392288042499
0.175099168051 0.393457974784
0.174463684157 0.394628185375
0.173829923894 0.395798664571
0.173197885117 0.396969402678
0.17256756567 0.398140390014
0.17193896339 0.399311616902
0.171312076108 0.400483073676
0.170686901644 0.401654750678
0.170063437813 0.402826638259
0.169441682421 0.403998726781
0.168821633268 0.405171006615
0.168203288143 0.406343468139
0.16758664483 0.407516101745
0.166971701106 0.408688897832
0.166358454739 0.409861846811
0.16574690349 0.411034939103
0.165137045113 0.41220816514
0.164528877355 0.413381515364
0.163922397955 0.414554980228
0.163317604645 0.415728550197
0.16271449515 0.416902215747
0.162113067187 0.418075967366
0.161513318468 0.419249795552
0.160915246695 0.420423690817
0.160318849567 0.421597643684
0.159724124772 0.422771644689
0.159131069993 0.423945684378
0.158539682907 0.425119753314
0.157949961182 0.426293842068
0.157361902482 0.427467941227
0.156775504462 0.428642041391
0.156190764772 0.42981613317
0.155607681053 0.430990207193
0.155026250942 0.432164254097
0.154446472069 0.433338264536
0.153868342057 0.434512229178
0.153291858521 0.435686138703
0.152717019073 0.436859983807
0.152143821317 0.438033755201
0.15157226285 0.439207443608
0.151002341264 0.440381039769
0.150434054144 0.441554534436
0.149867399069 0.442727918381
0.149302373612 0.443901182387
0.148738975341 0.445074317254
0.148177201816 0.446247313798
0.147617050592 0.447420162849
0.147058519219 0.448592855257
0.146501605241 0.449765381882
0.145946306194 0.450937733605
0.14539261961 0.452109901322
0.144840543016 0.453281875944
0.144290073932 0.4544536484
0.143741209872 0.455625209637
0.143193948347 0.456796550616
0.142648286859 0.457967662317
0.142104222907 0.459138535738
0.141561753983 0.460309161892
0.141020877576 0.461479531812
0.140481591166 0.462649636547
0.139943892231 0.463819467165
0.139407778243 0.46498901475
0.138873246667 0.466158270407
0.138340294964 0.467327225258
0.137808920591 0.468495870443
0.137279120998 0.46966419712
0.136750893632 0.470832196467
0.136224235933 0.471999859681
0.135699145338 0.473167177977
0.135175619277 0.474334142589
0.134653655176 0.475500744772
0.134133250457 0.476666975799
0.133614402538 0.477832826961
0.133097108829 0.478998289573
0.132581366738 0.480163354966
0.132067173668 0.481328014492
0.131554527016 0.482492259523
0.131043424178 0.483656081453
0.130533862541 0.484819471694
0.13002583949 0.485982421679
0.129519352406 0.487144922862
0.129014398665 0.488306966718
0.128510975638 0.489468544743
0.128009080692 0.490629648452
0.127508711192 0.491790269385
0.127009864495 0.492950399099
0.126512537957 0.494110029175
0.126016728928 0.495269151215
0.125522434755 0.496427756842
0.125029652782 0.497585837702
0.124538380346 0.49874338546
0.124048614783 0.499900391808
0.123560353424 0.501056848454
0.123073593595 0.502212747134
0.122588332621 0.503368079601
0.122104567821 0.504522837636
0.121622296511 0.505677013038
0.121141516004 0.50683059763
0.120662223608 0.50798358326
0.120184416629 0.509135961795
0.119708092368 0.510287725129
0.119233248123 0.511438865177
0.11875988119 0.512589373876
0.118287988859 0.51373924319
0.117817568419 0.514888465103
0.117348617155 0.516037031624
0.116881132348 0.517184934787
0.116415111277 0.518332166647
0.115950551216 0.519478719285
0.115487449439 0.520624584806
0.115025803212 0.521769755337
0.114565609804 0.522914223032
0.114106866476 0.524057980068
0.113649570488 0.525201018645
0.113193719097 0.526343330991
0.112739309559 0.527484909355
0.112286339123 0.528625746014
0.111834805039 0.529765833267
0.111384704552 0.530905163438
0.110936034905 0.53204372888
0.11048879334 0.533181521965
0.110042977093 0.534318535096
0.109598583399 0.535454760697
0.109155609492 0.536590191219
0.108714052602 0.53772481914
0.108273909956 0.53885863696
0.10783517878 0.539991637209
0.107397856296 0.541123812439
0.106961939726 0.54225515523
0.106527426287 0.543385658187
0.106094313196 0.544515313942
0.105662597665 0.545644115151
0.105232276909 0.546772054499
0.104803348134 0.547899124694
0.10437580855 0.549025318474
0.103949655361 0.550150628601
0.10352488577 0.551275047864
0.10310149698 0.552398569079
0.10267948619 0.553521185088
0.102258850596 0.55464288876
0.101839587396 0.555763672992
0.101421693783 0.556883530705
0.101005166948 0.558002454851
0.100590004083 0.559120438405
0.100176202376 0.560237474372
0.0997637590147 0.561353555784
0.0993526711837 0.562468675697
0.0989429360673 0.5635828272
0.0985345508477 0.564696003404
0.0981275127059 0.56580819745
0.0977218188212 0.566919402507
0.0973174663715 0.568029611771
0.0969144525334 0.569138818465
0.0965127744823 0.570247015841
0.0961124293919 0.571354197177
0.0957134144349 0.572460355782
0.0953157267829 0.573565484989
0.0949193636059 0.574669578163
0.0945243220731 0.575772628694
0.0941305993525 0.576874630001
0.093738192611 0.577975575532
0.0933470990143 0.579075458762
0.0929573157274 0.580174273197
0.0925688399142 0.581272012367
0.0921816687375 0.582368669834
0.0917957993594 0.583464239187
0.0914112289411 0.584558714044
0.0910279546431 0.585652088051
0.0906459736249 0.586744354884
0.0902652830454 0.587835508246
0.0898858800627 0.58892554187
0.0895077618343 0.590014449517
0.0891309255171 0.591102224978
0.0887553682673 0.592188862071
0.0883810872406 0.593274354644
0.0880080795921 0.594358696574
0.0876363424765 0.595441881768
0.0872658730481 0.596523904161
0.0868966684605 0.597604757716
0.0865287258673 0.598684436428
0.0861620424215 0.599762934319
0.0857966152758 0.600840245441
0.0854324415827 0.601916363876
0.0850695184944 0.602991283732
0.0847078431629 0.604064999152
0.0843474127401 0.605137504304
0.0839882243776 0.606208793387
0.0836302752272 0.607278860629
0.0832735624402 0.608347700288
0.0829180831683 0.609415306651
0.0825638345628 0.610481674037
0.0822108137754 0.61154679679
0.0818590179576 0.612610669288
0.0815084442611 0.613673285937
0.0811590898378 0.614734641172
0.0808109518396 0.615794729459
0.0804640274187 0.616853545294
0.0801183137276 0.6179110832
0.079773807919 0.618967337734
0.079430507146 0.620022303481
0.0790884085617 0.621075975054
0.07874750932 0.622128347099
0.078407806575 0.62317941429
0.0780692974811 0.624229171333
0.0777319791935 0.625277612961
0.0773958488676 0.626324733939
0.0770609036595 0.627370529062
0.0767271407257 0.628414993155
0.0763945572236 0.629458121073
0.0760631503108 0.6304999077
0.0757329171458 0.631540347951
0.075403854888 0.632579436772
0.075075960697 0.633617169139
0.0747492317337 0.634653540056
0.0744236651594 0.63568854456
0.0740992581364 0.636722177715
0.0737760078277 0.63775443462
0.0734539113975 0.638785310399
0.0731329660104 0.63981480021
0.0728131688324 0.640842899239
0.0724945170303 0.641869602703
0.0721770077718 0.64289490585
0.0718606382259 0.643918803958
0.0715454055622 0.644941292334
0.071231306952 0.645962366317
0.0709183395672 0.646982021276
0.0706065005811 0.648000252609
0.0702957871681 0.649017055745
0.0699861965039 0.650032426144
0.0696777257654 0.651046359296
0.0693703721306 0.652058850721
0.0690641327792 0.653069895969
0.0687590048918 0.654079490621
0.0684549856506 0.655087630289
0.068152072239 0.656094310614
0.0678502618421 0.657099527268
0.0675495516463 0.658103275953
0.0672499388393 0.659105552401
0.0669514206105 0.660106352375
0.0666539941507 0.661105671668
0.0663576566525 0.662103506105
0.0660624053098 0.663099851537
0.0657682373183 0.66409470385
0.0654751498752 0.665088058958
0.0651831401795 0.666079912806
0.0648922054317 0.667070261368
0.0646023428343 0.668059100649
0.0643135495912 0.669046426685
0.0640258229085 0.670032235543
0.0637391599937 0.671016523317
0.0634535580564 0.671999286133
0.0631690143079 0.672980520149
0.0628855259615 0.673960221551
0.0626030902323 0.674938386556
0.0623217043374 0.67591501141
0.0620413654959 0.676890092391
0.0617620709287 0.677863625806
0.0614838178589 0.678835607993
0.0612066035117 0.679806035319
0.0609304251141 0.680774904181
0.0606552798955 0.681742211008
0.0603811650871 0.682707952257
0.0601080779224 0.683672124416
0.0598360156372 0.684634724003
0.0595649754692 0.685595747565
0.0592949546586 0.686555191681
0.0590259504476 0.687513052958
0.0587579600808 0.688469328035
0.0584909808051 0.689424013577
0.0582250098697 0.690377106284
0.0579600445261 0.691328602882
0.0576960820281 0.692278500128
0.057433119632 0.69322679481
0.0571711545965 0.694173483745
0.0569101841827 0.695118563778
0.0566502056542 0.696062031786
0.0563912162769 0.697003884675
0.0561332133195 0.697944119381
0.0558761940531 0.698882732869
0.0556201557512 0.699819722133
0.05536509569 0.700755084198
0.0551110111484 0.701688816119
0.0548578994077 0.702620914978
0.054605757752 0.703551377888
0.054354583468 0.704480201993
0.0541043738452 0.705407384463
0.0538551261756 0.7063329225
0.0536068377541 0.707256813334
0.0533595058783 0.708179054226
0.0531131278484 0.709099642464
0.0528677009678 0.710018575367
0.0526232225424 0.710935850282
0.0523796898809 0.711851464585
0.0521371002951 0.712765415684
0.0518954510995 0.713677701012
0.0516547396116 0.714588318033
0.0514149631518 0.71549726424
0.0511761190433 0.716404537156
0.0509382046125 0.717310134331
0.0507012171886 0.718214053344
0.0504651541039 0.719116291804
0.0502300126937 0.720016847348
0.0499957902964 0.720915717643
0.0497624842534 0.721812900382
0.0495300919091 0.72270839329
0.0492986106112 0.723602194118
0.0490680377103 0.724494300646
0.0488383705604 0.725384710684
0.0486096065185 0.726273422069
0.0483817429448 0.727160432667
0.0481547772027 0.728045740373
0.0479287066588 0.728929343108
0.047703528683 0.729811238824
0.0474792406485 0.730691425499
0.0472558399316 0.731569901142
0.0470333239121 0.732446663787
0.0468116899729 0.733321711498
0.0465909355004 0.734195042366
0.0463710578844 0.73506665451
0.0461520545178 0.735936546079
0.0459339227971 0.736804715247
0.0457166601222 0.737671160217
0.0455002638964 0.73853587922
0.0452847315263 0.739398870514
0.0450700604221 0.740260132386
0.0448562479974 0.74111966315
0.0446432916695 0.741977461145
0.0444311888589 0.742833524742
0.0442199369897 0.743687852336
0.0440095334897 0.74454044235
0.0437999757902 0.745391293236
0.0435912613259 0.746240403472
0.0433833875353 0.747087771562
0.0431763518604 0.747933396039
0.0429701517468 0.748777275463
0.0427647846439 0.749619408419
0.0425602480045 0.750459793522
0.0423565392853 0.751298429411
0.0421536559466 0.752135314754
0.0419515954524 0.752970448243
0.0417503552703 0.753803828601
0.0415499328718 0.754635454574
0.0413503257321 0.755465324935
0.0411515313302 0.756293438486
0.0409535471488 0.757119794052
0.0407563706743 0.757944390487
0.0405599993971 0.75876722667
0.0403644308114 0.759588301507
0.0401696624151 0.76040761393
0.0399756917101 0.761225162897
0.039782516202 0.762040947391
0.0395901334004 0.762854966423
0.0393985408188 0.763667219028
0.0392077359744 0.764477704269
0.0390177163887 0.765286421233
0.0388284795868 0.766093369034
0.0386400230979 0.76689854681
0.038452344455 0.767701953725
0.0382654411954 0.768503588971
0.0380793108599 0.769303451762
0.0378939509938 0.770101541339
0.0377093591461 0.770897856969
0.0375255328699 0.771692397943
0.0373424697223 0.772485163577
0.0371601672646 0.773276153213
0.0369786230619 0.774065366218
0.0367978346837 0.774852801983
0.0366177997033 0.775638459925
0.0364385156983 0.776422339486
0.0362599802501 0.77720444013
0.0360821909447 0.77798476135
0.0359051453719 0.77876330266
0.0357288411256 0.7795400636
0.0355532758041 0.780315043734
0.0353784470097 0.781088242651
0.035204352349 0.781859659963
0.0350309894325 0.782629295309
0.0348583558753 0.783397148348
0.0346864492965 0.784163218767
0.0345152673194 0.784927506274
0.0343448075715 0.785690010603
0.0341750676848 0.786450731511
0.0340060452953 0.787209668777
0.0338377380433 0.787966822208
0.0336701435734 0.788722191631
0.0335032595346 0.789475776897
0.03333708358 0.790227577881
0.0331716133672 0.790977594483
0.0330068465579 0.791725826622
0.0328427808184 0.792472274245
0.032679413819 0.793216937319
0.0325167432346 0.793959815836
0.0323547667443 0.794700909808
0.0321934820318 0.795440219274
0.0320328867848 0.796177744293
0.0318729786957 0.796913484947
0.0317137554611 0.797647441342
0.0315552147822 0.798379613604
0.0313973543643 0.799110001885
0.0312401719174 0.799838606356
0.0310836651558 0.800565427213
0.0309278317982 0.801290464673
0.0307726695679 0.802013718975
0.0306181761923 0.80273519038
0.0304643494037 0.803454879172
0.0303111869386 0.804172785656
0.030158686538 0.804888910159
0.0300068459475 0.80560325303
0.0298556629169 0.80631581464
0.0297051352008 0.80702659538
0.0295552605582 0.807735595665
0.0294060367526 0.808442815929
0.029257461552 0.809148256628
0.0291095327289 0.809851918241
0.0289622480604 0.810553801267
0.0288156053281 0.811253906224
0.0286696023182 0.811952233654
0.0285242368213 0.812648784118
0.0283795066328 0.8133435582
0.0282354095524 0.814036556503
0.0280919433846 0.81472777965
0.0279491059383 0.815417228286
0.027806895027 0.816104903077
0.027665308469 0.816790804707
0.0275243440869 0.817474933882
0.0273839997081 0.818157291329
0.0272442731646 0.818837877794
0.0271051622928 0.819516694043
0.0269666649341 0.820193740861
0.0268287789341 0.820869019056
0.0266915021434 0.821542529453
0.026554832417 0.822214272897
0.0264187676145 0.822884250254
0.0262833056004 0.823552462408
0.0261484442436 0.824218910264
0.0260141814179 0.824883594745
0.0258805150014 0.825546516793
0.0257474428772 0.826207677372
0.025614962933 0.826867077462
0.025483073061 0.827524718063
0.0253517711582 0.828180600195
0.0252210551264 0.828834724894
0.0250909228719 0.829487093219
0.0249613723057 0.830137706243
0.0248324013437 0.830786565061
0.0247040079062 0.831433670785
0.0245761899183 0.832079024546
0.0244489453101 0.832722627493
0.024322272016 0.833364480794
0.0241961679752 0.834004585633
0.0240706311319 0.834642943214
0.0239456594347 0.835279554759
0.0238212508371 0.835914421506
0.0236974032972 0.836547544713
0.0235741147779 0.837178925655
0.0234513832469 0.837808565623
0.0233292066765 0.838436465928
0.0232075830438 0.839062627897
0.0230865103307 0.839687052874
0.0229659865238 0.840309742222
0.0228460096143 0.840930697318
0.0227265775985 0.84154991956
0.0226076884771 0.84216741036
0.0224893402557 0.842783171148
0.0223715309447 0.843397203371
0.0222542585592 0.844009508492
0.022137521119 0.844620087991
0.0220213166488 0.845228943365
0.021905643178 0.845836076126
0.0217904987407 0.846441487805
0.0216758813759 0.847045179946
0.0215617891273 0.847647154111
0.0214482200434 0.848247411878
0.0213351721773 0.84884595484
0.0212226435871 0.849442784609
0.0211106323356 0.850037902808
0.0209991364905 0.85063131108
0.0208881541239 0.851223011081
0.0207776833131 0.851813004483
0.02066772214 0.852401292974
0.0205582686912 0.852987878258
0.0204493210583 0.853572762054
0.0203408773374 0.854155946093
0.0202329356297 0.854737432127
0.0201254940409 0.855317221917
0.0200185506817 0.855895317244
0.0199121036675 0.8564717199
0.0198061511183 0.857046431693
0.0197006911593 0.857619454447
0.0195957219201 0.858190789998
0.0194912415352 0.8587604402
0.0193872481441 0.859328406918
0.0192837398907 0.859894692032
0.0191807149241 0.860459297438
0.0190781713978 0.861022225044
0.0189761074703 0.861583476773
0.0188745213049 0.862143054562
0.0187734110697 0.862700960361
0.0186727749374 0.863257196136
0.0185726110856 0.863811763863
0.0184729176967 0.864364665536
0.0183736929579 0.864915903158
0.0182749350611 0.865465478749
0.0181766422032 0.86601339434
0.0180788125854 0.866559651976
0.0179814444143 0.867104253715
0.0178845359007 0.867647201629
0.0177880852607 0.868188497802
0.0176920907147 0.868728144331
0.0175965504882 0.869266143326
0.0175014628113 0.869802496909
0.017406825919 0.870337207214
0.017312638051 0.870870276391
0.0172188974518 0.871401706599
0.0171256023705 0.87193150001
0.0170327510613 0.872459658809
0.0169403417828 0.872986185192
0.0168483727987 0.873511081369
0.0167568423771 0.874034349561
0.0166657487912 0.874555991999
0.0165750903188 0.875076010929
0.0164848652423 0.875594408606
0.0163950718492 0.876111187299
0.0163057084314 0.876626349288
0.0162167732859 0.877139896862
0.016128264714 0.877651832324
0.0160401810222 0.878162157989
0.0159525205215 0.878670876179
0.0158652815275 0.879177989232
0.0157784623609 0.879683499494
0.0156920613469 0.880187409324
0.0156060768154 0.880689721089
0.0155205071011 0.881190437169
0.0154353505435 0.881689559954
0.0153506054866 0.882187091845
0.0152662702793 0.882683035253
0.0151823432752 0.8831773926
0.0150988228326 0.883670166318
0.0150157073145 0.884161358848
0.0149329950884 0.884650972644
0.014850684527 0.885139010168
0.0147687740071 0.885625473892
0.0146872619107 0.886110366299
0.0146061466242 0.88659368988
0.0145254265387 0.887075447138
0.0144451000501 0.887555640585
0.014365165559 0.88803427274
0.0142856214705 0.888511346137
0.0142064661946 0.888986863313
0.0141276981458 0.889460826819
0.0140493157432 0.889933239213
0.0139713174109 0.890404103063
0.0138937015772 0.890873420946
0.0138164666755 0.891341195447
0.0137396111436 0.891807429162
0.0136631334238 0.892272124694
0.0135870319635 0.892735284655
0.0135113052143 0.893196911666
0.0134359516326 0.893657008356
0.0133609696795 0.894115577365
0.0132863578206 0.894572621337
0.0132121145261 0.895028142928
0.0131382382711 0.8954821448
0.0130647275349 0.895934629626
0.0129915808017 0.896385600083
0.0129187965601 0.89683505886
0.0128463733036 0.89728300865
0.0127743095299 0.897729452159
0.0127026037415 0.898174392095
0.0126312544456 0.898617831178
0.0125602601537 0.899059772133
0.0124896193821 0.899500217694
0.0124193306516 0.899939170602
0.0123493924874 0.900376633605
0.0122798034195 0.900812609458
0.0122105619823 0.901247100925
0.0121416667149 0.901680110775
0.0120731161608 0.902111641786
0.0120049088681 0.902541696741
0.0119370433893 0.90297027843
0.0118695182816 0.903397389652
0.0118023321067 0.90382303321
0.0117354834307 0.904247211916
0.0116689708243 0.904669928587
0.0116027928627 0.905091186047
0.0115369481256 0.905510987126
0.0114714351971 0.905929334661
0.0114062526659 0.906346231495
0.0113413991252 0.906761680478
0.0112768731725 0.907175684463
0.01121267341 0.907588246314
0.0111487984442 0.907999368896
0.0110852468862 0.908409055083
0.0110220173513 0.908817307754
0.0109591084595 0.909224129793
0.0108965188351 0.909629524091
0.0108342471069 0.910033493544
0.0107722919081 0.910436041052
0.0107106518764 0.910837169522
0.0106493256538 0.911236881868
0.0105883118868 0.911635181005
0.0105276092261 0.912032069857
0.0104672163271 0.91242755135
0.0104071318494 0.912821628419
0.0103473544571 0.913214304
0.0102878828185 0.913605581037
0.0102287156064 0.913995462476
0.010169851498 0.914383951269
0.0101112891747 0.914771050375
0.0100530273225 0.915156762753
0.00999506463147 0.91554109137
0.0099373997962 0.915924039197
0.00988003151554 0.916305609209
0.00982295849269 0.916685804384
0.00976617943517 0.917064627706
0.00970969305479 0.917442082162
0.00965349806767 0.917818170745
0.00959759319425 0.918192896451
0.00954197715924 0.918566262278
0.00948664869165 0.918938271231
0.00943160652474 0.919308926317
0.00937684939606 0.919678230547
0.00932237604744 0.920046186936
0.00926818522493 0.920412798503
0.00921427567884 0.92077806827
0.00916064616375 0.921141999262
0.00910729543844 0.921504594509
0.00905422226593 0.921865857042
0.00900142541347 0.922225789898
0.00894890365251 0.922584396115
0.00889665575872 0.922941678734
0.00884468051194 0.923297640802
0.00879297669624 0.923652285367
0.00874154309985 0.924005615478
0.00869037851519 0.92435763419
0.00863948173883 0.92470834456
0.00858885157153 0.925057749647
0.00853848681818 0.925405852514
0.00848838628783 0.925752656224
0.00843854879366 0.926098163845
0.00838897315299 0.926442378447
0.00833965818728 0.926785303102
0.00829060272207 0.927126940885
0.00824180558704 0.927467294872
0.00819326561596 0.927806368142
0.0081449816467 0.928144163777
0.00809695252121 0.928480684859
0.00804917708552 0.928815934475
0.00800165418973 0.92914991571
0.00795438268801 0.929482631655
0.00790736143858 0.929814085401
0.00786058930371 0.930144280039
0.00781406514971 0.930473218666
0.00776778784692 0.930800904376
0.0077217562697 0.931127340268
0.00767596929645 0.93145252944
0.00763042580954 0.931776474995
0.00758512469537 0.932099180033
0.00754006484433 0.932420647659
0.00749524515077 0.932740880977
0.00745066451306 0.933059883093
0.00740632183349 0.933377657115
0.00736221601835 0.933694206151
0.00731834597786 0.93400953331
0.00727471062619 0.934323641702
0.00723130888144 0.93463653444
0.00718813966566 0.934948214635
0.0071452019048 0.9352586854
0.00710249452872 0.935567949849
0.0070600164712 0.935876011097
0.00701776666991 0.936182872258
0.00697574406639 0.936488536449
0.00693394760608 0.936793006785
0.00689237623829 0.937096286384
0.00685102891617 0.937398378362
0.00680990459676 0.937699285838
0.00676900224091 0.937999011928
0.00672832081334 0.938297559751
0.00668785928257 0.938594932425
0.00664761662096 0.938891133069
0.00660759180468 0.939186164802
0.0065677838137 0.939480030741
0.00652819163178 0.939772734005
0.00648881424649 0.940064277712
0.00644965064915 0.940354664982
0.00641069983487 0.940643898932
0.00637196080252 0.94093198268
0.00633343255472 0.941218919343
0.00629511409782 0.941504712039
0.00625700444195 0.941789363885
0.00621910260092 0.942072877997
0.00618140759228 0.942355257491
0.0061439184373 0.942636505483
0.00610663416094 0.942916625086
0.00606955379186 0.943195619416
0.00603267636241 0.943473491586
0.00599600090859 0.943750244708
0.00595952647011 0.944025881895
0.0059232520903 0.944300406256
0.00588717681618 0.944573820903
0.00585129969837 0.944846128945
0.00581561979116 0.945117333489
0.00578013615245 0.945387437643
0.00574484784375 0.945656444512
0.00570975393019 0.945924357202
0.0056748534805 0.946191178817
0.00564014556698 0.946456912458
0.00560562926553 0.946721561227
0.00557130365563 0.946985128223
0.0055371678203 0.947247616546
0.00550322084614 0.947509029291
0.00546946182328 0.947769369554
0.0054358898454 0.94802864043
0.0054025040097 0.948286845011
0.00536930341691 0.948543986387
0.00533628717125 0.948800067648
0.00530345438047 0.949055091881
0.00527080415581 0.949309062171
0.00523833561198 0.949561981603
0.00520604786718 0.949813853258
0.00517394004306 0.950064680217
0.00514201126477 0.950314465558
0.00511026066086 0.950563212356
0.00507868736335 0.950810923687
0.00504729050769 0.951057602622
0.00501606923275 0.951303252231
0.00498502268081 0.951547875583
0.00495414999757 0.951791475742
0.00492345033212 0.952034055773
0.00489292283693 0.952275618736
0.00486256666787 0.952516167691
0.00483238098415 0.952755705693
0.00480236494838 0.952994235798
0.00477251772649 0.953231761056
0.00474283848776 0.953468284518
0.00471332640483 0.953703809229
0.00468398065364 0.953938338233
0.00465480041346 0.954171874573
0.00462578486686 0.954404421287
0.00459693319972 0.954635981412
0.0045682446012 0.95486655798
0.00453971826375 0.955096154024
0.00451135338308 0.95532477257
0.0044831491582 0.955552416643
0.00445510479132 0.955779089267
0.00442721948795 0.95600479346
0.0043994924568 0.956229532239
0.00437192290983 0.956453308617
0.0043445100622 0.956676125605
0.00431725313231 0.956897986209
0.00429015134173 0.957118893436
0.00426320391524 0.957338850284
0.00423641008081 0.957557859753
0.00420976906957 0.957775924837
0.00418328011582 0.957993048528
0.00415694245703 0.958209233814
0.0041307553338 0.95842448368
0.00410471798988 0.958638801108
0.00407882967215 0.958852189075
0.00405308963061 0.959064650557
0.00402749711838 0.959276188526
0.00400205139167 0.959486805949
0.00397675170979 0.95969650579
0.00395159733514 0.959905291011
0.00392658753321 0.960113164568
0.00390172157252 0.960320129417
0.00387699872469 0.960526188506
0.00385241826438 0.960731344781
0.00382797946926 0.960935601187
0.00380368162009 0.961138960661
0.0037795240006 0.96134142614
0.00375550589757 0.961543000554
0.00373162660077 0.96174368683
0.00370788540297 0.961943487894
0.00368428159993 0.962142406664
0.00366081449039 0.962340446056
0.00363748337606 0.962537608983
0.00361428756161 0.962733898353
0.00359122635467 0.962929317068
0.00356829906581 0.963123868031
0.00354550500853 0.963317554135
0.00352284349926 0.963510378274
0.00350031385735 0.963702343335
0.00347791540506 0.9638934522
0.00345564746755 0.964083707751
0.00343350937286 0.964273112861
0.00341150045193 0.964461670402
0.00338962003855 0.964649383241
0.00336786746941 0.964836254239
0.00334624208403 0.965022286255
0.00332474322477 0.965207482143
0.00330337023685 0.965391844752
0.00328212246831 0.965575376926
0.00326099927002 0.965758081507
0.00323999999564 0.96593996133
0.00321912400165 0.966121019227
0.00319837064733 0.966301258025
0.00317773929473 0.966480680547
0.00315722930869 0.966659289611
0.0031368400568 0.966837088031
0.00311657090944 0.967014078614
0.00309642123971 0.967190264167
0.00307639042348 0.967365647487
0.00305647783932 0.96754023137
0.00303668286856 0.967714018607
0.00301700489522 0.967887011983
0.00299744330605 0.968059214279
0.00297799749047 0.96823062827
0.00295866684063 0.968401256729
0.00293945075131 0.968571102422
0.00292034862001 0.96874016811
0.00290135984686 0.968908456551
0.00288248383468 0.969075970495
0.0028637199889 0.969242712691
0.00284506771762 0.969408685881
0.00282652643155 0.969573892802
0.00280809554402 0.969738336185
0.00278977447098 0.96990201876
0.002771562631 0.970064943246
0.00275345944521 0.970227112364
0.00273546433735 0.970388528823
0.00271757673374 0.970549195333
0.00269979606326 0.970709114594
0.00268212175735 0.970868289305
0.00266455325002 0.971026722156
0.0026470899778 0.971184415836
0.00262973137977 0.971341373025
0.00261247689754 0.9714975964
0.00259532597523 0.971653088633
0.00257827805947 0.97180785239
0.0025613325994 0.971961890332
0.00254448904666 0.972115205115
0.00252774685534 0.972267799388
0.00251110548206 0.972419675798
0.00249456438585 0.972570836985
0.00247812302825 0.972721285582
0.00246178087323 0.97287102422
0.00244553738718 0.973020055522
0.00242939203898 0.973168382107
0.00241334429988 0.973316006589
0.00239739364359 0.973462931574
0.00238153954619 0.973609159667
0.00236578148621 0.973754693464
0.00235011894453 0.973899535556
0.00233455140443 0.97404368853
0.00231907835157 0.974187154967
0.00230369927398 0.974329937442
0.00228841366205 0.974472038525
0.0022732210085 0.974613460781
0.00225812080843 0.974754206768
0.00224311255924 0.974894279039
0.00222819576068 0.975033680142
0.00221336991482 0.97517241262
0.00219863452602 0.97531047901
0.00218398910096 0.975447881842
0.00216943314862 0.975584623642
0.00215496618024 0.97572070693
0.00214058770936 0.97585613422
0.00212629725178 0.975990908021
0.00211209432558 0.976125030836
0.00209797845106 0.976258505163
0.00208394915081 0.976391333492
0.00207000594961 0.976523518312
0.0020561483745 0.976655062101
0.00204237595474 0.976785967334
0.00202868822179 0.976916236481
0.00201508470933 0.977045872005
0.00200156495323 0.977174876363
0.00198812849155 0.977303252008
0.00197477486453 0.977431001385
0.00196150361459 0.977558126934
0.00194831428631 0.977684631092
0.00193520642644 0.977810516285
0.00192217958385 0.977935784938
0.00190923330959 0.978060439467
0.00189636715682 0.978184482285
0.00188358068083 0.978307915796
0.00187087343903 0.9784307424
0.00185824499095 0.978552964493
0.0018456948982 0.978674584461
0.00183322272452 0.978795604687
0.00182082803571 0.978916027548
0.00180851039964 0.979035855415
0.00179626938629 0.979155090651
0.00178410456768 0.979273735617
0.00177201551788 0.979391792665
0.00176000181302 0.979509264142
0.00174806303126 0.97962615239
0.00173619875282 0.979742459743
0.00172440855992 0.979858188532
0.00171269203679 0.979973341081
0.00170104876971 0.980087919706
0.00168947834692 0.980201926719
0.00167798035868 0.980315364427
0.00166655439722 0.980428235128
0.00165520005678 0.980540541118
0.00164391693354 0.980652284684
0.00163270462566 0.980763468108
0.00162156273325 0.980874093666
0.00161049085838 0.980984163629
0.00159948860506 0.98109368026
0.00158855557923 0.981202645818
0.00157769138875 0.981311062555
0.00156689564342 0.981418932717
0.00155616795494 0.981526258544
0.00154550793691 0.981633042271
0.00153491520485 0.981739286127
0.00152438937613 0.981844992333
0.00151393007005 0.981950163106
0.00150353690776 0.982054800655
0.00149320951227 0.982158907186
0.00148294750848 0.982262484897
0.00147275052311 0.98236553598
0.00146261818475 0.982468062622
0.00145255012382 0.982570067002
0.00144254597258 0.982671551295
0.00143260536511 0.982772517669
0.00142272793729 0.982872968286
0.00141291332684 0.982972905303
0.00140316117328 0.983072330871
0.00139347111789 0.983171247132
0.00138384280378 0.983269656225
0.00137427587583 0.983367560283
0.00136476998068 0.983464961431
0.00135532476676 0.983561861789
0.00134593988424 0.983658263472
0.00133661498505 0.983754168588
0.00132734972288 0.983849579238
0.00131814375314 0.983944497518
0.00130899673298 0.984038925519
0.00129990832127 0.984132865324
0.00129087817862 0.984226319011
0.00128190596732 0.984319288652
0.00127299135139 0.984411776313
0.00126413399653 0.984503784053
0.00125533357014 0.984595313926
0.0012465897413 0.98468636798
0.00123790218077 0.984776948256
0.00122927056099 0.984867056791
0.00122069455603 0.984956695613
0.00121217384165 0.985045866746
0.00120370809525 0.985134572207
0.00119529699587 0.985222814009
0.00118694022418 0.985310594157
0.00117863746249 0.98539791465
0.00117038839473 0.985484777481
0.00116219270644 0.985571184638
0.00115405008478 0.985657138103
0.0011459602185 0.98574263985
0.00113792279796 0.985827691849
0.00112993751509 0.985912296064
0.00112200406342 0.985996454451
0.00111412213805 0.986080168963
0.00110629143565 0.986163441543
0.00109851165444 0.986246274133
0.00109078249423 0.986328668664
0.00108310365634 0.986410627065
0.00107547484366 0.986492151256
0.0010678957606 0.986573243154
0.00106036611312 0.986653904666
0.00105288560868 0.986734137698
0.00104545395628 0.986813944145
0.00103807086641 0.9868933259
0.00103073605109 0.986972284847
0.0010234492238 0.987050822868
0.00101621009955 0.987128941833
0.00100901839482 0.987206643613
0.00100187382757 0.987283930067
0.000994776117227 0.987360803052
0.000987724984689 0.987437264416
0.000980720152318 0.987513316005
0.000973761343923 0.987588959656
0.000966848284768 0.9876641972
0.000959980701551 0.987739030464
0.000953158322411 0.987813461267
0.000946380876913 0.987887491424
0.000939648096046 0.987961122742
0.000932959712215 0.988034357024
0.000926315459236 0.988107196067
0.000919715072329 0.98817964166
0.000913158288113 0.988251695588
0.000906644844599 0.988323359631
0.000900174481184 0.988394635559
0.000893746938645 0.988465525142
0.000887361959134 0.988536030139
0.000881019286169 0.988606152305
0.000874718664633 0.98867589339
0.000868459840763 0.988745255138
0.000862242562147 0.988814239286
0.000856066577717 0.988882847565
0.000849931637743 0.988951081701
0.000843837493828 0.989018943416
0.000837783898901 0.989086434422
0.000831770607212 0.989153556428
0.000825797374325 0.989220311137
0.000819863957115 0.989286700246
0.000813970113758 0.989352725445
0.000808115603728 0.98941838842
0.000802300187791 0.98948369085
0.000796523627998 0.98954863441
0.00079078568768 0.989613220766
0.000785086131444 0.98967745158
0.000779424725164 0.989741328511
0.000773801235978 0.989804853207
0.000768215432279 0.989868027314
0.000762667083715 0.98993085247
0.000757155961178 0.98999333031
0.0007516818368 0.990055462461
0.000746244483949 0.990117250545
0.000740843677221 0.990178696179
0.000735479192438 0.990239800972
0.000730150806635 0.99030056653
0.000724858298066 0.990360994452
0.000719601446187 0.990421086331
0.000714380031659 0.990480843756
0.000709193836336 0.990540268309
0.000704042643264 0.990599361566
0.000698926236676 0.990658125098
0.000693844401982 0.990716560471
0.000688796925766 0.990774669244
0.000683783595785 0.990832452972
0.000678804200955 0.990889913202
0.000673858531354 0.990947051479
0.000668946378209 0.991003869338
0.000664067533898 0.991060368313
0.00065922179194 0.991116549928
0.00065440894699 0.991172415705
0.000649628794838 0.991227967159
0.000644881132396 0.991283205799
0.000640165757701 0.991338133129
0.000635482469904 0.991392750648
0.000630831069269 0.991447059849
0.000626211357162 0.991501062219
0.000621623136054 0.99155475924
0.000617066209509 0.991608152389
0.000612540382181 0.991661243136
0.000608045459811 0.991714032947
0.000603581249217 0.991766523283
0.000599147558296 0.991818715597
0.000594744196013 0.99187061134
0.000590370972396 0.991922211954
0.000586027698538 0.991973518879
0.000581714186581 0.992024533547
0.000577430249723 0.992075257386
0.000573175702201 0.992125691817
0.000568950359297 0.992175838258
0.000564754037326 0.992225698121
0.000560586553632 0.99227527281
0.000556447726588 0.992324563728
0.000552337375583 0.992373572269
0.000548255321026 0.992422299823
0.000544201384332 0.992470747776
0.000540175387927 0.992518917506
0.000536177155234 0.992566810387
0.000532206510675 0.99261442779
0.000528263279662 0.992661771077
0.000524347288595 0.992708841606
0.000520458364855 0.992755640731
0.0005165963368 0.992802169799
0.000512761033763 0.992848430154
0.000508952286043 0.992894423132
0.000505169924902 0.992940150065
0.000501413782561 0.992985612282
0.000497683692196 0.993030811103
0.000493979487933 0.993075747845
0.000490301004839 0.993120423819
0.000486648078925 0.993164840333
0.000483020547136 0.993208998686
0.000479418247348 0.993252900175
0.000475841018365 0.993296546092
0.00047228869991 0.993339937721
0.000468761132627 0.993383076344
0.000465258158071 0.993425963236
0.000461779618706 0.993468599668
0.000458325357899 0.993510986904
0.000454895219919 0.993553126206
0.000451489049929 0.99359501883
0.000448106693982 0.993636666024
0.000444747999019 0.993678069035
0.000441412812862 0.993719229103
0.00043810098421 0.993760147464
0.000434812362639 0.993800825347
0.000431546798589 0.993841263978
0.00042830414337 0.993881464577
0.000425084249147 0.993921428361
0.000421886968946 0.993961156538
0.000418712156643 0.994000650316
0.000415559666961 0.994039910895
0.000412429355468 0.99407893947
0.00040932107857 0.994117737233
0.000406234693509 0.994156305369
0.000403170058357 0.994194645059
0.000400127032015 0.994232757481
0.000397105474203 0.994270643804
0.000394105245463 0.994308305197
0.00039112620715 0.994345742821
0.000388168221429 0.994382957832
0.000385231151271 0.994419951383
0.000382314860451 0.994456724622
0.00037941921354 0.994493278691
0.000376544075903 0.994529614727
0.000373689313698 0.994565733865
0.000370854793867 0.994601637232
0.000368040384132 0.994637325952
0.000365245952998 0.994672801145
0.000362471369741 0.994708063924
0.000359716504407 0.994743115399
0.00035698122781 0.994777956675
0.000354265411525 0.994812588852
0.000351568927887 0.994847013026
0.000348891649984 0.994881230287
0.000346233451657 0.994915241723
0.000343594207492 0.994949048415
0.000340973792819 0.994982651439
0.000338372083706 0.995016051869
0.00033578895696 0.995049250773
0.000333224290117 0.995082249213
0.00033067796144 0.99511504825
0.00032814984992 0.995147648936
0.000325639835265 0.995180052322
0.000323147797901 0.995212259453
0.000320673618968 0.995244271371
0.000318217180315 0.99527608911
0.000315778364496 0.995307713703
0.000313357054768 0.995339146178
0.000310953135085 0.995370387557
0.000308566490098 0.995401438859
0.000306197005148 0.995432301097
0.000303844566262 0.995462975282
0.000301509060155 0.995493462419
0.000299190374219 0.995523763508
0.000296888396525 0.995553879545
0.000294603015815 0.995583811524
0.000292334121503 0.995613560432
0.000290081603669 0.995643127251
0.000287845353055 0.995672512962
0.000285625261064 0.995701718539
0.000283421219752 0.995730744952
0.00028123312183 0.995759593167
0.000279060860657 0.995788264147
0.000276904330239 0.99581675885
0.000274763425222 0.995845078227
0.000272638040892 0.99587322323
0.00027052807317 0.995901194802
0.000268433418609 0.995928993884
0.000266353974392 0.995956621413
0.000264289638326 0.995984078321
0.000262240308841 0.996011365537
0.000260205884984 0.996038483983
0.000258186266419 0.996065434581
0.000256181353422 0.996092218246
0.000254191046878 0.996118835889
0.000252215248277 0.996145288418
0.000250253859712 0.996171576736
0.000248306783874 0.996197701742
0.000246373924053 0.996223664333
0.000244455184128 0.996249465398
0.000242550468571 0.996275105825
0.000240659682437 0.996300586497
0.000238782731368 0.996325908294
0.000236919521583 0.996351072089
0.00023506995988 0.996376078755
0.000233233953631 0.996400929158
0.000231411410777 0.996425624161
0.000229602239828 0.996450164624
0.000227806349859 0.996474551401
0.000226023650506 0.996498785344
0.000224254051964 0.996522867301
0.000222497464984 0.996546798114
0.000220753800867 0.996570578623
0.000219022971467 0.996594209664
0.000217304889182 0.996617692068
0.000215599466955 0.996641026664
0.000213906618268 0.996664214276
0.000212226257144 0.996687255723
0.000210558298136 0.996710151823
0.000208902656332 0.996732903387
0.000207259247348 0.996755511224
0.000205627987327 0.996777976141
0.000204008792932 0.996800298937
0.000202401581351 0.99682248041
0.000200806270285 0.996844521355
0.000199222777952 0.996866422561
0.00019765102308 0.996888184814
0.000196090924908 0.996909808897
0.000194542403178 0.996931295589
0.000193005378139 0.996952645666
0.000191479770538 0.996973859898
0.00018996550162 0.996994939053
0.000188462493125 0.997015883897
0.000186970667285 0.997036695189
0.000185489946824 0.997057373686
0.000184020254948 0.997077920142
0.000182561515352 0.997098335307
0.000181113652208 0.997118619927
0.000179676590171 0.997138774744
0.000178250254368 0.997158800498
0.000176834570402 0.997178697924
0.000175429464345 0.997198467754
0.000174034862738 0.997218110717
0.000172650692589 0.997237627537
0.000171276881365 0.997257018937
0.000169913356996 0.997276285634
0.00016856004787 0.997295428342
0.000167216882828 0.997314447773
0.000165883791166 0.997333344634
0.000164560702627 0.99735211963
0.000163247547405 0.997370773461
0.000161944256136 0.997389306825
0.0001606507599 0.997407720416
0.000159366990216 0.997426014924
0.000158092879041 0.997444191036
0.000156828358767 0.997462249437
0.000155573362218 0.997480190806
0.000154327822648 0.997498015822
0.00015309167374 0.997515725157
0.0001518648496 0.997533319483
0.000150647284757 0.997550799466
0.000149438914163 0.997568165771
0.000148239673186 0.997585419058
0.000147049497608 0.997602559985
0.000145868323627 0.997619589205
0.00014469608785 0.99763650737
0.000143532727294 0.997653315128
0.00014237817938 0.997670013123
0.000141232381935 0.997686601995
0.000140095273186 0.997703082384
0.00013896679176 0.997719454924
0.00013784687668 0.997735720247
0.000136735467365 0.997751878982
0.000135632503624 0.997767931753
0.00013453792566 0.997783879184
0.000133451674059 0.997799721893
0.000132373689797 0.997815460497
0.00013130391423 0.997831095608
0.000130242289097 0.997846627837
0.000129188756514 0.99786205779
0.000128143258978 0.997877386071
0.000127105739355 0.99789261328
0.000126076140888 0.997907740016
0.000125054407186 0.997922766873
0.000124040482231 0.997937694443
0.000123034310367 0.997952523315
0.000122035836302 0.997967254073
0.000121045005108 0.997981887301
0.000120061762215 0.997996423579
0.000119086053411 0.998010863482
0.000118117824838 0.998025207586
0.000117157022993 0.998039456461
0.000116203594724 0.998053610675
0.000115257487226 0.998067670792
0.000114318648045 0.998081637376
0.000113387025068 0.998095510985
0.000112462566529 0.998109292176
0.000111545220998 0.998122981502
0.00011063493739 0.998136579514
0.000109731664951 0.99815008676
0.000108835353267 0.998163503784
0.000107945952255 0.99817683113
0.000107063412161 0.998190069336
0.000106187683565 0.99820321894
0.000105318717369 0.998216280474
0.000104456464804 0.998229254469
0.000103600877422 0.998242141456
0.000102751907097 0.998254941957
0.000101909506024 0.998267656498
0.000101073626713 0.998280285596
0.000100244221992 0.998292829771
9.94212450016e-05 0.998305289536
9.86046491939e-05 0.998317665404
9.77943883318e-05 0.998329957883
9.69904164865e-05 0.998342167481
9.61926880352e-05 0.998354294701
9.54011576598e-05 0.998366340044
9.46157803451e-05 0.99837830401
9.38365113763e-05 0.998390187094
9.30633063381e-05 0.998401989789
9.22961211124e-05 0.998413712587
9.15349118766e-05 0.998425355976
9.07796351018e-05 0.99843692044
9.00302475513e-05 0.998448406464
8.92867062781e-05 0.998459814527
8.85489686241e-05 0.998471145108
8.78169922178e-05 0.998482398682
8.70907349727e-05 0.998493575722
8.63701550855e-05 0.998504676698
8.56552110343e-05 0.998515702078
8.49458615775e-05 0.998526652327
8.42420657512e-05 0.998537527908
8.35437828681e-05 0.998548329282
8.28509725157e-05 0.998559056906
8.21635945547e-05 0.998569711236
8.14816091171e-05 0.998580292724
8.08049766047e-05 0.998590801822
8.01336576876e-05 0.998601238977
7.94676133021e-05 0.998611604636
7.880680465e-05 0.99862189924
7.81511931955e-05 0.998632123232
7.75007406654e-05 0.99864227705
7.68554090458e-05 0.99865236113
7.62151605816e-05 0.998662375906
7.55799577747e-05 0.998672321808
7.49497633822e-05 0.998682199268
7.43245404147e-05 0.99869200871
7.37042521353e-05 0.998701750559
7.30888620575e-05 0.998711425239
7.24783339443e-05 0.998721033167
7.18726318057e-05 0.998730574763
7.12717198982e-05 0.998740050441
7.06755627224e-05 0.998749460614
7.00841250223e-05 0.998758805693
6.94973717831e-05 0.998768086086
6.89152682301e-05 0.9987773022
6.83377798272e-05 0.998786454438
6.77648722753e-05 0.998795543203
6.71965115108e-05 0.998804568894
6.66326637042e-05 0.998813531907
6.60732952588e-05 0.99882243264
6.5518372809e-05 0.998831271483
6.4967863219e-05 0.998840048829
6.44217335813e-05 0.998848765066
6.38799512154e-05 0.99885742058
6.33424836662e-05 0.998866015756
6.28092987028e-05 0.998874550975
6.2280364317e-05 0.998883026619
6.17556487217e-05 0.998891443064
6.12351203499e-05 0.998899800688
6.07187478532e-05 0.998908099863
6.02065001002e-05 0.998916340961
5.96983461755e-05 0.998924524352
5.91942553778e-05 0.998932650403
5.86941972194e-05 0.998940719481
5.81981414238e-05 0.998948731947
5.77060579257e-05 0.998956688165
5.7217916868e-05 0.998964588493
5.6733688602e-05 0.998972433288
5.62533436855e-05 0.998980222906
5.57768528812e-05 0.9989879577
5.53041871556e-05 0.998995638022
5.48353176781e-05 0.99900326422
5.43702158193e-05 0.999010836643
5.39088531498e-05 0.999018355636
5.3451201439e-05 0.999025821541
5.29972326537e-05 0.999033234702
5.25469189571e-05 0.999040595456
5.21002327072e-05 0.999047904143
5.16571464561e-05 0.999055161097
5.12176329481e-05 0.999062366653
5.0781665119e-05 0.999069521142
5.03492160944e-05 0.999076624895
4.99202591893e-05 0.999083678239
4.94947679058e-05 0.999090681501
4.90727159328e-05 0.999097635006
4.86540771445e-05 0.999104539075
4.82388255989e-05 0.99911139403
4.78269355372e-05 0.999118200189
4.74183813821e-05 0.99912495787
4.70131377371e-05 0.999131667388
4.66111793851e-05 0.999138329055
4.6212481287e-05 0.999144943185
4.58170185811e-05 0.999151510086
4.54247665814e-05 0.999158030066
4.50357007771e-05 0.999164503432
4.46497968306e-05 0.999170930489
4.42670305776e-05 0.999177311538
4.38873780245e-05 0.999183646881
4.35108153486e-05 0.999189936818
4.31373188964e-05 0.999196181644
4.27668651823e-05 0.999202381658
4.23994308881e-05 0.999208537151
4.20349928615e-05 0.999214648417
4.1673528115e-05 0.999220715747
4.13150138251e-05 0.999226739428
4.09594273311e-05 0.999232719749
4.06067461337e-05 0.999238656995
4.0256947895e-05 0.99924455145
3.99100104359e-05 0.999250403396
3.95659117365e-05 0.999256213114
3.92246299341e-05 0.999261980882
3.88861433227e-05 0.999267706978
3.85504303519e-05 0.999273391677
3.82174696255e-05 0.999279035254
3.78872399011e-05 0.999284637981
3.75597200886e-05 0.999290200128
3.72348892492e-05 0.999295721966
3.69127265951e-05 0.999301203761
3.65932114874e-05 0.99930664578
3.62763234363e-05 0.999312048287
3.5962042099e-05 0.999317411545
3.56503472796e-05 0.999322735815
3.53412189277e-05 0.999328021357
3.50346371376e-05 0.99933326843
3.47305821472e-05 0.99933847729
3.44290343373e-05 0.999343648193
3.41299742302e-05 0.999348781391
3.38333824895e-05 0.999353877138
3.35392399184e-05 0.999358935683
3.32475274593e-05 0.999363957277
3.29582261924e-05 0.999368942166
3.26713173355e-05 0.999373890597
3.23867822423e-05 0.999378802814
3.21046024019e-05 0.999383679062
3.18247594382e-05 0.999388519581
3.15472351082e-05 0.999393324612
3.12720113019e-05 0.999398094394
3.09990700411e-05 0.999402829164
3.07283934782e-05 0.999407529158
3.04599638959e-05 0.999412194612
3.01937637062e-05 0.999416825758
2.99297754491e-05 0.999421422827
2.96679817922e-05 0.999425986051
2.94083655298e-05 0.999430515658
2.91509095818e-05 0.999435011877
2.88955969929e-05 0.999439474932
2.86424109325e-05 0.999443905049
2.83913346925e-05 0.999448302452
2.81423516875e-05 0.999452667362
2.78954454538e-05 0.999457000001
2.76505996484e-05 0.999461300587
2.74077980482e-05 0.99946556934
2.71670245495e-05 0.999469806475
2.69282631667e-05 0.999474012208
2.66914980318e-05 0.999478186754
2.64567133936e-05 0.999482330324
2.62238936171e-05 0.999486443132
2.5993023182e-05 0.999490525386
2.57640866828e-05 0.999494577295
2.55370688275e-05 0.999498599068
2.53119544371e-05 0.999502590911
2.50887284446e-05 0.999506553029
2.48673758945e-05 0.999510485626
2.46478819415e-05 0.999514388904
2.44302318505e-05 0.999518263064
2.42144109954e-05 0.999522108307
2.40004048586e-05 0.999525924832
2.37881990298e-05 0.999529712836
2.35777792058e-05 0.999533472516
2.33691311894e-05 0.999537204066
2.31622408891e-05 0.999540907682
2.29570943178e-05 0.999544583555
2.27536775925e-05 0.999548231877
2.25519769338e-05 0.999551852839
2.23519786643e-05 0.999555446629
2.21536692088e-05 0.999559013437
2.19570350933e-05 0.999562553448
2.17620629445e-05 0.999566066849
2.15687394881e-05 0.999569553823
2.13770515499e-05 0.999573014555
2.11869860534e-05 0.999576449226
2.09985300202e-05 0.999579858019
2.0811670569e-05 0.999583241111
2.06263949146e-05 0.999586598683
2.04426903679e-05 0.999589930913
2.02605443348e-05 0.999593237976
2.00799443155e-05 0.999596520048
1.9900877904e-05 0.999599777304
1.97233327875e-05 0.999603009917
1.95472967458e-05 0.99960621806
1.93727576503e-05 0.999609401902
1.91997034639e-05 0.999612561615
1.90281222396e-05 0.999615697367
1.8858002121e-05 0.999618809326
1.86893313404e-05 0.999621897659
1.85220982193e-05 0.999624962532
1.83562911671e-05 0.999628004109
1.81918986805e-05 0.999631022554
1.80289093433e-05 0.99963401803
1.78673118256e-05 0.999636990699
1.7707094883e-05 0.99963994072
1.75482473563e-05 0.999642868254
1.73907581706e-05 0.999645773459
1.72346163351e-05 0.999648656493
1.7079810942e-05 0.999651517511
1.69263311666e-05 0.99965435667
1.67741662659e-05 0.999657174125
1.66233055789e-05 0.999659970028
1.64737385254e-05 0.999662744532
1.63254546055e-05 0.999665497789
1.61784433993e-05 0.999668229949
1.60326945662e-05 0.999670941162
1.58881978441e-05 0.999673631578
1.57449430495e-05 0.999676301342
1.56029200762e-05 0.999678950603
1.54621188952e-05 0.999681579506
1.53225295542e-05 0.999684188196
1.51841421766e-05 0.999686776816
1.50469469614e-05 0.999689345511
1.49109341827e-05 0.999691894421
1.47760941888e-05 0.999694423689
1.46424174019e-05 0.999696933454
1.45098943176e-05 0.999699423856
1.43785155043e-05 0.999701895033
1.4248271603e-05 0.999704347123
1.41191533261e-05 0.999706780262
1.39911514574e-05 0.999709194587
1.38642568517e-05 0.999711590232
1.37384604338e-05 0.999713967331
1.36137531986e-05 0.999716326017
1.34901262102e-05 0.999718666423
1.33675706013e-05 0.999720988679
1.3246077573e-05 0.999723292918
1.31256383945e-05 0.999725579267
1.3006244402e-05 0.999727847856
1.28878869986e-05 0.999730098814
1.27705576539e-05 0.999732332267
1.26542479035e-05 0.999734548341
1.25389493482e-05 0.999736747162
1.24246536538e-05 0.999738928856
1.23113525508e-05 0.999741093544
1.21990378334e-05 0.999743241352
1.208770136e-05 0.9997453724
1.19773350513e-05 0.99974748681
1.18679308913e-05 0.999749584704
1.17594809259e-05 0.9997516662
1.16519772629e-05 0.999753731418
1.15454120715e-05 0.999755780476
1.14397775816e-05 0.999757813492
1.13350660836e-05 0.999759830581
1.12312699281e-05 0.999761831861
1.11283815251e-05 0.999763817447
1.10263933436e-05 0.999765787452
1.09252979117e-05 0.99976774199
1.08250878154e-05 0.999769681174
1.07257556989e-05 0.999771605117
1.06272942638e-05 0.999773513929
1.05296962685e-05 0.999775407722
1.04329545283e-05 0.999777286605
1.03370619144e-05 0.999779150687
1.02420113544e-05 0.999781000077
1.01477958304e-05 0.999782834882
1.00544083804e-05 0.99978465521
9.96184209656e-06 0.999786461167
9.8700901251e-06 0.999788252858
9.77914566636e-06 0.999790030388
9.68900197384e-06 0.999791793861
9.59965235448e-06 0.999793543382
9.51109016722e-06 0.999795279051
9.42330882381e-06 0.999797000972
9.33630178757e-06 0.999798709247
9.25006257346e-06 0.999800403974
9.16458474742e-06 0.999802085256
9.07986192633e-06 0.99980375319
8.99588777714e-06 0.999805407876
8.9126560171e-06 0.999807049412
8.83016041286e-06 0.999808677895
8.7483947806e-06 0.999810293421
8.6673529851e-06 0.999811896087
8.58702893991e-06 0.999813485988
8.50741660674e-06 0.999815063219
8.42850999494e-06 0.999816627873
8.35030316149e-06 0.999818180045
8.27279021065e-06 0.999819719827
8.19596529322e-06 0.999821247311
8.11982260662e-06 0.99982276259
8.04435639412e-06 0.999824265752
7.96956094506e-06 0.99982575689
7.89543059398e-06 0.999827236093
7.8219597206e-06 0.999828703449
7.74914274926e-06 0.999830159048
7.67697414883e-06 0.999831602977
7.60544843226e-06 0.999833035323
7.53456015634e-06 0.999834456173
7.46430392107e-06 0.999835865614
7.39467436972e-06 0.999837263729
7.32566618822e-06 0.999838650606
7.25727410533e-06 0.999840026327
7.18949289147e-06 0.999841390977
7.12231735922e-06 0.999842744638
7.05574236259e-06 0.999844087394
6.98976279689e-06 0.999845419325
6.92437359817e-06 0.999846740515
6.85956974333e-06 0.999848051043
6.79534624948e-06 0.99984935099
6.73169817356e-06 0.999850640435
6.66862061238e-06 0.999851919459
6.60610870218e-06 0.999853188139
6.54415761825e-06 0.999854446553
6.48276257476e-06 0.99985569478
6.42191882416e-06 0.999856932896
6.36162165768e-06 0.999858160978
6.30186640382e-06 0.999859379101
6.2426484293e-06 0.999860587342
6.1839631379e-06 0.999861785774
6.1258059707e-06 0.999862974474
6.06817240534e-06 0.999864153513
6.01105795639e-06 0.999865322966
5.95445817431e-06 0.999866482906
5.89836864573e-06 0.999867633405
5.84278499316e-06 0.999868774534
5.78770287418e-06 0.999869906366
5.7331179818e-06 0.99987102897
5.67902604409e-06 0.999872142418
5.62542282345e-06 0.999873246779
5.57230411691e-06 0.999874342122
5.51966575546e-06 0.999875428516
5.46750360408e-06 0.99987650603
5.41581356139e-06 0.999877574732
5.36459155931e-06 0.999878634689
5.31383356284e-06 0.999879685967
5.26353556984e-06 0.999880728634
5.21369361106e-06 0.999881762756
5.16430374897e-06 0.999882788397
5.11536207892e-06 0.999883805624
5.06686472745e-06 0.9998848145
5.01880785331e-06 0.99988581509
4.97118764609e-06 0.999886807458
4.92400032681e-06 0.999887791666
4.87724214759e-06 0.999888767778
4.83090939074e-06 0.999889735856
4.78499836942e-06 0.999890695961
4.73950542679e-06 0.999891648156
4.69442693596e-06 0.999892592502
4.64975929992e-06 0.999893529058
4.60549895098e-06 0.999894457886
4.56164235108e-06 0.999895379044
4.51818599079e-06 0.999896292593
4.47512638968e-06 0.999897198591
4.43246009618e-06 0.999898097097
4.39018368692e-06 0.999898988168
4.3482937665e-06 0.999899871862
4.30678696772e-06 0.999900748237
4.26565995126e-06 0.999901617349
4.22490940499e-06 0.999902479256
4.18453204443e-06 0.999903334011
4.14452461184e-06 0.999904181673
4.1048838767e-06 0.999905022295
4.06560663513e-06 0.999905855932
4.02668970967e-06 0.999906682639
3.98812994895e-06 0.99990750247
3.94992422803e-06 0.999908315478
3.91206944772e-06 0.999909121717
3.87456253437e-06 0.99990992124
3.83740043997e-06 0.999910714098
3.8005801416e-06 0.999911500345
3.76409864167e-06 0.999912280032
3.72795296733e-06 0.99991305321
3.69214017026e-06 0.99991381993
3.65665732704e-06 0.999914580244
3.62150153821e-06 0.9999153342
3.58666992861e-06 0.999916081849
3.55215964698e-06 0.999916823241
3.51796786557e-06 0.999917558424
3.48409178064e-06 0.999918287448
3.4505286115e-06 0.99991901036
3.41727560083e-06 0.99991972721
3.38433001401e-06 0.999920438044
3.35168913967e-06 0.99992114291
3.31935028874e-06 0.999921841856
3.28731079491e-06 0.999922534928
3.25556801395e-06 0.999923222171
3.22411932385e-06 0.999923903633
3.1929621247e-06 0.999924579359
3.16209383799e-06 0.999925249394
3.13151190712e-06 0.999925913784
3.10121379676e-06 0.999926572573
3.07119699317e-06 0.999927225805
3.04145900332e-06 0.999927873524
3.0119973552e-06 0.999928515774
2.98280959776e-06 0.9999291526
2.95389330041e-06 0.999929784042
2.92524605294e-06 0.999930410145
2.89686546573e-06 0.999931030951
2.86874916888e-06 0.999931646502
2.84089481262e-06 0.99993225684
2.81330006713e-06 0.999932862005
2.78596262204e-06 0.999933462041
2.75888018653e-06 0.999934056986
2.73205048917e-06 0.999934646883
2.70547127779e-06 0.999935231771
2.67914031893e-06 0.99993581169
2.65305539826e-06 0.99993638668
2.62721432032e-06 0.999936956781
2.60161490784e-06 0.999937522031
2.57625500233e-06 0.999938082469
2.5511324635e-06 0.999938638134
2.52624516905e-06 0.999939189065
2.50159101489e-06 0.999939735298
2.47716791468e-06 0.999940276872
2.45297379975e-06 0.999940813824
2.42900661918e-06 0.999941346192
2.40526433914e-06 0.999941874011
2.38174494349e-06 0.99994239732
2.35844643304e-06 0.999942916153
2.33536682559e-06 0.999943430547
2.31250415583e-06 0.999943940538
2.28985647532e-06 0.999944446162
2.26742185216e-06 0.999944947452
2.24519837089e-06 0.999945444446
2.22318413234e-06 0.999945937176
2.20137725371e-06 0.999946425678
2.17977586825e-06 0.999946909985
2.15837812501e-06 0.999947390132
2.13718218911e-06 0.999947866153
2.11618624113e-06 0.99994833808
2.0953884774e-06 0.999948805948
2.07478710956e-06 0.999949269788
2.05438036471e-06 0.999949729633
2.03416648514e-06 0.999950185516
2.01414372802e-06 0.99995063747
1.99431036574e-06 0.999951085525
1.97466468532e-06 0.999951529714
1.95520498869e-06 0.999951970068
1.93592959208e-06 0.999952406619
1.91683682649e-06 0.999952839396
1.89792503724e-06 0.999953268432
1.87919258365e-06 0.999953693756
1.86063783947e-06 0.999954115399
1.84225919231e-06 0.999954533391
1.82405504379e-06 0.999954947762
1.80602380906e-06 0.999955358541
1.78816391716e-06 0.999955765757
1.77047381078e-06 0.99995616944
1.75295194582e-06 0.999956569619
1.73559679173e-06 0.999956966322
1.71840683105e-06 0.999957359578
1.70138055955e-06 0.999957749415
1.68451648597e-06 0.999958135862
1.66781313182e-06 0.999958518945
1.65126903184e-06 0.999958898692
1.63488273297e-06 0.999959275132
1.61865279513e-06 0.999959648291
1.60257779058e-06 0.999960018196
1.5866563039e-06 0.999960384874
1.5708869322e-06 0.999960748352
1.55526828449e-06 0.999961108655
1.53979898221e-06 0.99996146581
1.52447765833e-06 0.999961819844
1.50930295828e-06 0.999962170781
1.49427353879e-06 0.999962518647
1.47938806871e-06 0.999962863469
1.4646452281e-06 0.99996320527
1.45004370877e-06 0.999963544076
1.43558221388e-06 0.999963879911
1.42125945801e-06 0.999964212801
1.40707416685e-06 0.99996454277
1.39302507718e-06 0.999964869841
1.37911093701e-06 0.999965194039
1.3653305051e-06 0.999965515388
1.35168255133e-06 0.999965833912
1.3381658559e-06 0.999966149633
1.32477921033e-06 0.999966462575
1.31152141614e-06 0.999966772762
1.29839128571e-06 0.999967080216
1.28538764177e-06 0.99996738496
1.27250931725e-06 0.999967687016
1.25975515541e-06 0.999967986407
1.24712400984e-06 0.999968283156
1.23461474399e-06 0.999968577283
1.22222623145e-06 0.999968868812
1.20995735542e-06 0.999969157764
1.19780700947e-06 0.99996944416
1.18577409636e-06 0.999969728021
1.17385752896e-06 0.99997000937
1.16205622935e-06 0.999970288226
1.15036912951e-06 0.999970564612
1.13879517039e-06 0.999970838547
1.12733330282e-06 0.999971110052
1.11598248642e-06 0.999971379147
1.10474169024e-06 0.999971645853
1.09360989253e-06 0.99997191019
1.08258608034e-06 0.999972172178
1.07166924979e-06 0.999972431836
1.0608584059e-06 0.999972689184
1.05015256269e-06 0.999972944241
1.0395507426e-06 0.999973197028
1.02905197696e-06 0.999973447562
1.01865530555e-06 0.999973695863
1.00835977668e-06 0.99997394195
9.9816444743e-07 0.999974185841
9.88068382779e-07 0.999974427555
9.78070656243e-07 0.999974667111
9.6817034978e-07 0.999974904526
9.58366553228e-07 0.999975139819
9.4865836453e-07 0.999975373008
9.39044889847e-07 0.99997560411
9.29525243221e-07 0.999975833143
9.20098546575e-07 0.999976060125
9.10763929718e-07 0.999976285073
9.01520530117e-07 0.999976508005
8.92367493011e-07 0.999976728936
8.83303971411e-07 0.999976947886
8.74329125655e-07 0.99997716487
8.65442123743e-07 0.999977379904
8.56642141001e-07 0.999977593007
8.47928360304e-07 0.999977804193
8.39299971744e-07 0.99997801348
8.30756172743e-07 0.999978220883
8.22296167713e-07 0.999978426419
8.13919168396e-07 0.999978630104
8.05624393529e-07 0.999978831953
7.97411069065e-07 0.999979031982
7.89278427504e-07 0.999979230206
7.81225708679e-07 0.999979426642
7.73252158859e-07 0.999979621304
7.65357031418e-07 0.999979814208
7.57539586282e-07 0.999980005368
7.49799090038e-07 0.999980194799
7.42134815934e-07 0.999980382517
7.34546043768e-07 0.999980568536
7.27032059888e-07 0.99998075287
7.19592156861e-07 0.999980935535
7.12225633914e-07 0.999981116544
7.0493179638e-07 0.999981295912
6.97709955921e-07 0.999981473652
6.90559430638e-07 0.999981649779
6.83479544517e-07 0.999981824307
6.76469627758e-07 0.999981997249
6.69529016561e-07 0.999982168619
6.62657053341e-07 0.999982338431
6.55853086173e-07 0.999982506698
6.49116469353e-07 0.999982673433
6.42446562837e-07 0.99998283865
6.35842732355e-07 0.999983002362
6.29304349631e-07 0.999983164582
6.22830791719e-07 0.999983325322
6.16421441779e-07 0.999983484596
6.1007568819e-07 0.999983642415
6.03792924991e-07 0.999983798794
5.97572552108e-07 0.999983953744
5.91413974238e-07 0.999984107277
5.85316602186e-07 0.999984259407
5.79279851531e-07 0.999984410145
5.73303143736e-07 0.999984559502
5.67385905148e-07 0.999984707492
5.61527567444e-07 0.999984854127
5.5572756763e-07 0.999984999417
5.49985347598e-07 0.999985143374
5.44300354566e-07 0.999985286011
5.38672040751e-07 0.999985427339
5.33099863254e-07 0.999985567368
5.27583284282e-07 0.999985706111
5.2212177104e-07 0.999985843579
5.16714795284e-07 0.999985979783
5.11361833988e-07 0.999986114733
5.06062368677e-07 0.999986248441
5.00815885762e-07 0.999986380918
4.95621876317e-07 0.999986512175
4.90479836079e-07 0.999986642221
4.85389265448e-07 0.999986771068
4.80349669374e-07 0.999986898726
4.75360557362e-07 0.999987025206
4.70421443466e-07 0.999987150518
4.65531846072e-07 0.999987274673
4.6069128834e-07 0.999987397679
4.55899297425e-07 0.999987519548
4.51155405146e-07 0.99998764029
4.4645914743e-07 0.999987759914
4.41810064533e-07 0.99998787843
4.37207701043e-07 0.999987995848
4.32651605653e-07 0.999988112178
4.28141331388e-07 0.999988227429
4.23676435157e-07 0.999988341611
4.1925647809e-07 0.999988454733
4.14881025312e-07 0.999988566805
4.10549646279e-07 0.999988677835
4.06261913888e-07 0.999988787833
4.02017405587e-07 0.999988896809
3.97815702158e-07 0.999989004771
3.9365638882e-07 0.999989111727
3.89539054235e-07 0.999989217688
3.85463291064e-07 0.999989322662
3.81428695739e-07 0.999989426657
3.77434868359e-07 0.999989529683
3.73481412796e-07 0.999989631748
3.69567936587e-07 0.99998973286
3.65694051041e-07 0.999989833028
3.61859370801e-07 0.99998993226
3.58063514505e-07 0.999990030564
3.543061039e-07 0.99999012795
3.50586764619e-07 0.999990224424
3.46905125626e-07 0.999990319996
3.43260819213e-07 0.999990414673
3.39653481451e-07 0.999990508463
3.36082751407e-07 0.999990601374
3.3254827192e-07 0.999990693414
3.29049688719e-07 0.999990784591
3.25586651417e-07 0.999990874912
3.22158812294e-07 0.999990964385
3.18765827179e-07 0.999991053017
3.15407355345e-07 0.999991140817
3.1208305884e-07 0.999991227791
3.08792603043e-07 0.999991313947
3.05535656553e-07 0.999991399293
3.02311891076e-07 0.999991483835
2.99120981206e-07 0.999991567581
2.95962604868e-07 0.999991650537
2.9283644265e-07 0.999991732712
2.89742178583e-07 0.999991814112
2.86679499362e-07 0.999991894743
2.83648094679e-07 0.999991974614
2.80647657114e-07 0.99999205373
2.77677882354e-07 0.999992132098
2.74738468753e-07 0.999992209726
2.71829117438e-07 0.99999228662
2.68949532645e-07 0.999992362786
2.66099421053e-07 0.999992438232
2.63278492452e-07 0.999992512963
2.60486459069e-07 0.999992586985
2.57723036023e-07 0.999992660307
2.54987941095e-07 0.999992732933
2.5228089473e-07 0.99999280487
2.49601619928e-07 0.999992876124
2.46949842464e-07 0.999992946702
2.44325290666e-07 0.999993016609
2.41727695194e-07 0.999993085852
2.39156789705e-07 0.999993154437
2.36612310078e-07 0.999993222369
2.34093994744e-07 0.999993289655
2.31601584577e-07 0.9999933563
2.29134823004e-07 0.99999342231
2.26693455896e-07 0.999993487691
2.24277231453e-07 0.999993552449
2.21885900209e-07 0.99999361659
2.19519215361e-07 0.999993680118
2.17176932105e-07 0.99999374304
2.1485880819e-07 0.999993805361
2.12564603586e-07 0.999993867086
2.10294080594e-07 0.999993928222
2.08047003736e-07 0.999993988772
2.05823139754e-07 0.999994048744
2.03622257722e-07 0.999994108141
2.01444128711e-07 0.99999416697
1.99288526348e-07 0.999994225235
1.97155226034e-07 0.999994282942
1.95044005502e-07 0.999994340095
1.92954644596e-07 0.9999943967
1.90886925266e-07 0.999994452761
1.88840631465e-07 0.999994508285
1.86815549363e-07 0.999994563275
1.84811467019e-07 0.999994617737
1.82828174711e-07 0.999994671675
1.80865464605e-07 0.999994725094
1.78923130756e-07 0.999994777999
1.77000969326e-07 0.999994830395
1.75098778588e-07 0.999994882286
1.73216358368e-07 0.999994933677
1.71353510825e-07 0.999994984573
1.69510039671e-07 0.999995034978
1.6768575084e-07 0.999995084897
1.65880451708e-07 0.999995134334
1.64093951871e-07 0.999995183293
1.62326062703e-07 0.999995231779
1.60576597241e-07 0.999995279797
1.58845370413e-07 0.999995327351
1.57132198919e-07 0.999995374444
1.5543690135e-07 0.999995421082
1.5375929785e-07 0.999995467268
1.52099210338e-07 0.999995513006
1.50456462511e-07 0.999995558302
1.48830879843e-07 0.999995603158
1.47222289359e-07 0.999995647579
1.45630519865e-07 0.99999569157
1.44055401607e-07 0.999995735133
1.42496766831e-07 0.999995778273
1.40954449002e-07 0.999995820994
1.39428283585e-07 0.999995863299
1.37918107379e-07 0.999995905194
1.36423758845e-07 0.99999594668
1.34945078001e-07 0.999995987763
1.33481906528e-07 0.999996028446
1.32034087441e-07 0.999996068732
1.30601465309e-07 0.999996108626
1.29183886477e-07 0.999996148131
1.27781198511e-07 0.99999618725
1.26393250643e-07 0.999996225988
1.25019893216e-07 0.999996264348
1.23660978568e-07 0.999996302332
1.2231635993e-07 0.999996339946
1.20985892416e-07 0.999996377192
1.19669432364e-07 0.999996414074
1.18366837443e-07 0.999996450595
1.17077966766e-07 0.999996486758
1.15802680778e-07 0.999996522567
1.14540841478e-07 0.999996558026
1.13292312087e-07 0.999996593137
1.12056957047e-07 0.999996627903
1.10834642242e-07 0.999996662329
1.09625235001e-07 0.999996696416
1.0842860354e-07 0.999996730169
1.07244617964e-07 0.999996763591
1.06073149042e-07 0.999996796684
1.0491406921e-07 0.999996829452
1.03767252013e-07 0.999996861897
1.0263257233e-07 0.999996894023
1.01509906036e-07 0.999996925833
1.00399130565e-07 0.99999695733
9.93001241234e-08 0.999996988517
9.82127666971e-08 0.999997019396
9.71369388258e-08 0.99999704997
9.6072522604e-08 0.999997080243
9.50194013472e-08 0.999997110217
9.3977459148e-08 0.999997139895
9.29465815425e-08 0.99999716928
9.19266550659e-08 0.999997198375
9.09175675856e-08 0.999997227182
8.99192077464e-08 0.999997255704
8.8931465525e-08 0.999997283944
8.79542318977e-08 0.999997311905
8.69873988396e-08 0.999997339588
8.60308596584e-08 0.999997366997
8.50845084388e-08 0.999997394135
8.41482404867e-08 0.999997421003
8.32219518854e-08 0.999997447605
8.23055401611e-08 0.999997473943
8.13989035064e-08 0.99999750002
8.05019412242e-08 0.999997525837
7.96145536164e-08 0.999997551398
7.87366420951e-08 0.999997576705
7.78681089608e-08 0.99999760176
7.7008857291e-08 0.999997626566
7.61587914955e-08 0.999997651125
7.53178165391e-08 0.999997675439
7.44858387192e-08 0.999997699511
7.36627649989e-08 0.999997723344
7.28485032297e-08 0.999997746938
7.20429624845e-08 0.999997770297
7.12460523911e-08 0.999997793423
7.04576836874e-08 0.999997816319
6.96777679998e-08 0.999997838985
6.89062177317e-08 0.999997861425
6.81429461746e-08 0.999997883641
6.73878676194e-08 0.999997905635
6.66408970229e-08 0.999997927408
6.59019502303e-08 0.999997948964
6.51709440858e-08 0.999997970304
6.44477960998e-08 0.99999799143
6.37324246711e-08 0.999998012344
6.30247490863e-08 0.999998033049
6.23246891873e-08 0.999998053546
6.16321658153e-08 0.999998073837
6.09471006996e-08 0.999998093925
6.02694162355e-08 0.999998113811
5.95990353736e-08 0.999998133497
5.89358822856e-08 0.999998152985
5.82798815874e-08 0.999998172277
5.7630958672e-08 0.999998191375
5.69890398205e-08 0.999998210281
5.63540519805e-08 0.999998228997
5.57259227651e-08 0.999998247524
5.51045805652e-08 0.999998265865
5.44899545485e-08 0.99999828402
5.38819746598e-08 0.999998301993
5.32805711773e-08 0.999998319784
5.26856756e-08 0.999998337395
5.20972197604e-08 0.999998354829
5.15151362679e-08 0.999998372087
5.09393583981e-08 0.99999838917
5.03698200927e-08 0.99999840608
4.98064560706e-08 0.99999842282
4.92492017168e-08 0.99999843939
4.86979927494e-08 0.999998455792
4.81527658858e-08 0.999998472029
4.76134582872e-08 0.9999984881
4.70800080032e-08 0.999998504009
4.65523533055e-08 0.999998519757
4.60304335759e-08 0.999998535344
4.55141883071e-08 0.999998550774
4.50035578803e-08 0.999998566047
4.44984833425e-08 0.999998581165
4.39989062961e-08 0.999998596129
4.35047686764e-08 0.999998610941
4.30160133069e-08 0.999998625602
4.25325835662e-08 0.999998640115
4.20544232771e-08 0.999998654479
4.15814769283e-08 0.999998668698
4.11136894529e-08 0.999998682771
4.06510065609e-08 0.999998696701
4.01933742955e-08 0.999998710489
3.97407392549e-08 0.999998724137
3.92930488147e-08 0.999998737645
3.88502506832e-08 0.999998751015
3.84122931241e-08 0.999998764249
3.79791249561e-08 0.999998777347
3.7550695553e-08 0.999998790312
3.71269546218e-08 0.999998803144
3.67078527574e-08 0.999998815845
3.62933406661e-08 0.999998828416
3.58833698311e-08 0.999998840858
3.54778920686e-08 0.999998853173
3.50768597501e-08 0.999998865362
3.46802256912e-08 0.999998877425
3.42879432624e-08 0.999998889365
3.38999662786e-08 0.999998901183
3.35162489984e-08 0.999998912879
3.31367461248e-08 0.999998924455
3.27614129159e-08 0.999998935913
3.23902051846e-08 0.999998947252
3.20230787443e-08 0.999998958475
3.16599904071e-08 0.999998969583
3.13008972075e-08 0.999998980576
3.09457565129e-08 0.999998991456
3.05945262458e-08 0.999999002224
3.02471646618e-08 0.999999012881
2.99036306828e-08 0.999999023429
2.95638833414e-08 0.999999033868
2.92278823366e-08 0.999999044199
2.88955877004e-08 0.999999054423
2.85669597977e-08 0.999999064542
2.82419594377e-08 0.999999074556
2.79205479847e-08 0.999999084467
2.7602687025e-08 0.999999094276
2.72883385888e-08 0.999999103983
2.69774650397e-08 0.99999911359
2.66700292961e-08 0.999999123097
2.63659944988e-08 0.999999132506
2.60653242323e-08 0.999999141818
2.57679824145e-08 0.999999151033
2.54739335181e-08 0.999999160152
2.51831421272e-08 0.999999169177
2.48955733806e-08 0.999999178109
2.46111925284e-08 0.999999186947
2.43299654867e-08 0.999999195694
2.40518585048e-08 0.999999204351
2.37768378319e-08 0.999999212917
2.35048703834e-08 0.999999221394
2.32359234076e-08 0.999999229783
2.2969964486e-08 0.999999238085
2.27069612002e-08 0.9999992463
2.24468820198e-08 0.99999925443
2.21896953034e-08 0.999999262475
2.19353700759e-08 0.999999270437
2.16838752509e-08 0.999999278315
2.14351805194e-08 0.999999286111
2.11892555724e-08 0.999999293826
2.09460706557e-08 0.999999301461
2.07055961265e-08 0.999999309016
2.0467802675e-08 0.999999316491
2.02326615462e-08 0.999999323889
2.00001438744e-08 0.99999933121
1.97702213489e-08 0.999999338453
1.95428659922e-08 0.999999345622
1.93180500485e-08 0.999999352715
1.90957458734e-08 0.999999359733
1.88759264885e-08 0.999999366679
1.86585649153e-08 0.999999373551
1.84436345085e-08 0.999999380352
1.82311089558e-08 0.999999387081
1.8020962167e-08 0.99999939374
1.78131683848e-08 0.999999400328
1.76077019631e-08 0.999999406848
1.7404537811e-08 0.999999413299
1.72036509483e-08 0.999999419682
1.7005016395e-08 0.999999425999
1.68086099483e-08 0.999999432249
1.66144072944e-08 0.999999438433
1.64223844523e-08 0.999999444552
1.62325177744e-08 0.999999450606
1.60447837239e-08 0.999999456597
1.58591590971e-08 0.999999462525
1.56756210234e-08 0.99999946839
1.54941466324e-08 0.999999474193
1.53147136084e-08 0.999999479935
1.5137299525e-08 0.999999485617
1.49618823997e-08 0.999999491239
1.47884405832e-08 0.999999496801
1.46169524262e-08 0.999999502304
1.44473966124e-08 0.999999507749
1.42797519365e-08 0.999999513137
1.41139977483e-08 0.999999518468
1.39501130647e-08 0.999999523742
1.37880777906e-08 0.999999528961
1.36278714979e-08 0.999999534124
1.34694742027e-08 0.999999539232
1.33128661428e-08 0.999999544287
1.31580276674e-08 0.999999549287
1.30049394587e-08 0.999999554235
1.28535823096e-08 0.99999955913
1.27039372355e-08 0.999999563973
1.25559853625e-08 0.999999568765
1.2409708372e-08 0.999999573506
1.22650877232e-08 0.999999578197
1.21221050975e-08 0.999999582837
1.19807428423e-08 0.999999587428
1.18409828609e-08 0.999999591971
1.17028076119e-08 0.999999596465
1.15661997757e-08 0.999999600911
1.14311420329e-08 0.99999960531
1.12976173972e-08 0.999999609662
1.11656088819e-08 0.999999613967
1.10350998339e-08 0.999999618227
1.09060737108e-08 0.999999622441
1.07785143033e-08 0.99999962661
1.06524052912e-08 0.999999630735
1.05277307982e-08 0.999999634815
1.04044749483e-08 0.999999638852
1.02826220871e-08 0.999999642846
1.01621566717e-08 0.999999646797
1.00430634919e-08 0.999999650706
9.92532722677e-09 0.999999654573
9.8089331102e-09 0.999999658399
9.69386604321e-09 0.999999662183
9.58011159291e-09 0.999999665927
9.46765510434e-09 0.999999669631
9.35648225564e-09 0.999999673295
9.24657872492e-09 0.99999967692
9.1379306344e-09 0.999999680506
9.03052388423e-09 0.999999684053
8.92434492972e-09 0.999999687563
8.81938000408e-09 0.999999691034
8.71561556259e-09 0.999999694469
8.61303850463e-09 0.999999697866
8.51163550752e-09 0.999999701227
8.41139358165e-09 0.999999704551
8.31229984843e-09 0.99999970784
8.21434142928e-09 0.999999711094
8.11750588969e-09 0.999999714312
8.02178057313e-09 0.999999717496
7.92715326714e-09 0.999999720645
7.83361164824e-09 0.99999972376
7.74114361501e-09 0.999999726842
7.64973728806e-09 0.99999972989
7.55938089902e-09 0.999999732906
7.47006256852e-09 0.999999735889
7.38177075021e-09 0.99999973884
7.29449423087e-09 0.999999741758
7.20822135314e-09 0.999999744646
7.12294112581e-09 0.999999747502
7.03864244667e-09 0.999999750327
6.95531421346e-09 0.999999753121
6.87294576807e-09 0.999999755885
6.79152634131e-09 0.99999975862
6.71104516403e-09 0.999999761324
6.63149191116e-09 0.999999763999
6.55285614659e-09 0.999999766646
6.47512765628e-09 0.999999769263
6.39829611515e-09 0.999999771852
6.32235164222e-09 0.999999774413
6.24728424548e-09 0.999999776946
6.17308404394e-09 0.999999779452
6.09974137866e-09 0.99999978193
6.02724659071e-09 0.999999784382
5.95559024319e-09 0.999999786806
5.88476278818e-09 0.999999789204
5.8147548998e-09 0.999999791577
5.74555758526e-09 0.999999793923
5.67716151867e-09 0.999999796244
5.60955781825e-09 0.999999798539
5.54273760223e-09 0.999999800809
5.47669187778e-09 0.999999803055
5.4114120962e-09 0.999999805276
5.34688959775e-09 0.999999807473
5.28311572268e-09 0.999999809646
5.22008225534e-09 0.999999811795
5.15778064702e-09 0.99999981392
5.0962027931e-09 0.999999816023
5.03534047791e-09 0.999999818102
4.97518548581e-09 0.999999820158
4.91573015626e-09 0.999999822192
4.85696627361e-09 0.999999824204
4.79888617733e-09 0.999999826194
4.74148220686e-09 0.999999828162
4.68474647963e-09 0.999999830108
4.62867166817e-09 0.999999832033
4.57325022296e-09 0.999999833937
4.51847481653e-09 0.99999983582
4.46433789936e-09 0.999999837682
4.41083247704e-09 0.999999839524
4.35795144416e-09 0.999999841345
4.30568747323e-09 0.999999843147
4.25403368087e-09 0.999999844928
4.20298318371e-09 0.99999984669
4.15252920938e-09 0.999999848433
4.10266487449e-09 0.999999850156
4.0533834067e-09 0.999999851861
4.0046783667e-09 0.999999853546
3.95654309315e-09 0.999999855214
3.90897114677e-09 0.999999856862
3.86195619928e-09 0.999999858493
3.81549181139e-09 0.999999860105
3.76957165482e-09 0.9999998617
3.72418973438e-09 0.999999863277
3.67933972178e-09 0.999999864837
3.63501573286e-09 0.999999866379
3.59121166138e-09 0.999999867904
3.54792162316e-09 0.999999869413
3.50513973402e-09 0.999999870905
3.46286022079e-09 0.99999987238
3.42107731033e-09 0.999999873839
3.37978534048e-09 0.999999875281
3.33897887117e-09 0.999999876708
3.29865212922e-09 0.999999878119
3.25879967455e-09 0.999999879514
3.21941617809e-09 0.999999880894
3.18049619974e-09 0.999999882259
3.14203452145e-09 0.999999883608
3.10402581416e-09 0.999999884942
3.06646497084e-09 0.999999886262
3.02934677343e-09 0.999999887567
2.99266622594e-09 0.999999888857
2.95641833237e-09 0.999999890133
2.92059798568e-09 0.999999891395
2.88520041192e-09 0.999999892642
2.8502207261e-09 0.999999893876
2.81565415428e-09 0.999999895096
2.7814960335e-09 0.999999896302
2.74774147879e-09 0.999999897495
2.71438593824e-09 0.999999898675
2.68142485993e-09 0.999999899842
2.64885369194e-09 0.999999900995
2.61666799339e-09 0.999999902136
2.58486332338e-09 0.999999903264
2.55343513e-09 0.999999904379
2.52237930543e-09 0.999999905482
2.49169151978e-09 0.999999906572
2.46136733217e-09 0.99999990765
2.43140285683e-09 0.999999908717
2.40179365285e-09 0.999999909771
2.37253583446e-09 0.999999910813
2.34362529383e-09 0.999999911844
2.31505803416e-09 0.999999912863
2.28682994763e-09 0.999999913871
2.25893737049e-09 0.999999914867
2.23137619493e-09 0.999999915853
2.2041427572e-09 0.999999916827
2.17723317153e-09 0.99999991779
2.15064366316e-09 0.999999918742
2.12437067937e-09 0.999999919684
2.09841033438e-09 0.999999920615
2.07275929753e-09 0.999999921536
2.04741368304e-09 0.999999922446
2.02237016023e-09 0.999999923346
1.99762517639e-09 0.999999924236
1.97317528983e-09 0.999999925116
1.94901705886e-09 0.999999925986
1.92514704178e-09 0.999999926846
1.90156190794e-09 0.999999927697
1.87825843767e-09 0.999999928538
1.85523330032e-09 0.999999929369
1.83248327623e-09 0.999999930191
1.81000514576e-09 0.999999931004
1.78779568927e-09 0.999999931807
1.76585190914e-09 0.999999932602
1.74417069676e-09 0.999999933387
1.7227489435e-09 0.999999934164
1.70158365176e-09 0.999999934932
1.68067182393e-09 0.999999935691
1.66001046242e-09 0.999999936441
1.63959679167e-09 0.999999937183
1.61942781407e-09 0.999999937917
1.59950064305e-09 0.999999938642
1.57981250304e-09 0.999999939359
1.56036061849e-09 0.999999940068
1.54114232487e-09 0.999999940769
1.52215462457e-09 0.999999941462
1.5033950751e-09 0.999999942147
1.4848609009e-09 0.999999942824
1.46654954847e-09 0.999999943494
1.44845835326e-09 0.999999944156
1.43058465074e-09 0.99999994481
1.41292610945e-09 0.999999945457
1.39548006484e-09 0.999999946097
1.3782439634e-09 0.999999946729
1.36121547367e-09 0.999999947355
1.34439215316e-09 0.999999947973
1.32777155937e-09 0.999999948583
1.31135124981e-09 0.999999949188
1.29512900404e-09 0.999999949785
1.27910249059e-09 0.999999950375
1.26326937799e-09 0.999999950958
1.24762722375e-09 0.999999951535
1.2321741405e-09 0.999999952106
1.21690757471e-09 0.999999952669
1.20182552799e-09 0.999999953227
1.18692566886e-09 0.999999953778
1.17220599893e-09 0.999999954322
1.15766440878e-09 0.999999954861
1.14329867795e-09 0.999999955393
1.12910691907e-09 0.999999955919
1.11508680067e-09 0.999999956439
1.1012365464e-09 0.999999956954
1.08755415784e-09 0.999999957462
1.07403741456e-09 0.999999957964
1.06068465122e-09 0.999999958461
1.0474937584e-09 0.999999958952
1.03446284871e-09 0.999999959437
1.02159003479e-09 0.999999959917
1.00887354026e-09 0.999999960392
9.96311366741e-10 0.99999996086
9.83901848883e-10 0.999999961324
9.71643099312e-10 0.999999961782
9.59533230649e-10 0.999999962235
9.47570688581e-10 0.999999962682
9.35753585729e-10 0.999999963125
9.24080256759e-10 0.999999963562
9.12548925314e-10 0.999999963994
9.01158037081e-10 0.999999964422
8.89905815704e-10 0.999999964844
8.78790706871e-10 0.999999965262
8.67811045246e-10 0.999999965674
8.56965165497e-10 0.999999966082
8.46251513309e-10 0.999999966486
8.35668645394e-10 0.999999966884
8.25214785394e-10 0.999999967278
8.14888601042e-10 0.999999967668
8.04688427003e-10 0.999999968053
7.94612819988e-10 0.999999968433
7.84660336706e-10 0.999999968809
7.74829422845e-10 0.999999969181
7.65118746138e-10 0.999999969548
7.55526863294e-10 0.999999969911
7.46052220002e-10 0.99999997027
7.36693595016e-10 0.999999970625
7.27449434024e-10 0.999999970976
7.1831851578e-10 0.999999971322
7.09299396995e-10 0.999999971665
7.00390856423e-10 0.999999972003
6.91591450774e-10 0.999999972338
6.82899958804e-10 0.999999972669
6.74315048244e-10 0.999999972996
6.65835386826e-10 0.999999973319
6.57459864328e-10 0.999999973638
6.49187148483e-10 0.999999973954
6.41016018044e-10 0.999999974266
6.32945251766e-10 0.999999974574
6.24973628405e-10 0.999999974879
6.17100037736e-10 0.99999997518
6.09323258516e-10 0.999999975478
6.0164218052e-10 0.999999975772
5.94055471481e-10 0.999999976063
5.86562243221e-10 0.99999997635
5.79161274494e-10 0.999999976634
5.71851455078e-10 0.999999976915
5.64631563726e-10 0.999999977192
5.57500823284e-10 0.999999977467
5.50457901483e-10 0.999999977738
5.43501799122e-10 0.999999978005
5.36631517001e-10 0.99999997827
5.29846055919e-10 0.999999978532
5.23144305653e-10 0.99999997879
5.16525267003e-10 0.999999979046
5.09988051789e-10 0.999999979298
5.03531549789e-10 0.999999979548
4.97154872825e-10 0.999999979794
4.90857021695e-10 0.999999980038
4.84637108222e-10 0.999999980279
4.78494022182e-10 0.999999980517
4.72427097442e-10 0.999999980752
4.66435223778e-10 0.999999980985
4.60517513012e-10 0.999999981215
4.54673076966e-10 0.999999981442
4.48901138483e-10 0.999999981666
4.43200698363e-10 0.999999981888
4.37570868428e-10 0.999999982107
4.32010982543e-10 0.999999982323
4.26520041508e-10 0.999999982538
4.21097157144e-10 0.999999982749
4.15741663318e-10 0.999999982958
4.10452671851e-10 0.999999983165
4.05229405587e-10 0.999999983369
4.00070976347e-10 0.99999998357
3.94976717999e-10 0.99999998377
3.89945853385e-10 0.999999983967
3.84977494328e-10 0.999999984161
3.80070974693e-10 0.999999984354
3.75225517324e-10 0.999999984544
3.70440345066e-10 0.999999984731
3.65714791783e-10 0.999999984917
3.61048080322e-10 0.9999999851
3.56439544547e-10 0.999999985282
3.51888518324e-10 0.999999985461
3.47394224498e-10 0.999999985638
3.42955885912e-10 0.999999985813
3.38573058478e-10 0.999999985985
3.34244854017e-10 0.999999986156
3.29970717416e-10 0.999999986325
3.25749982544e-10 0.999999986492
3.21581872242e-10 0.999999986656
3.17465942423e-10 0.999999986819
3.13401526952e-10 0.99999998698
3.09387848674e-10 0.999999987139
3.05424352476e-10 0.999999987296
3.01510483247e-10 0.999999987451
2.97645685876e-10 0.999999987605
2.93829183207e-10 0.999999987756
2.9006053115e-10 0.999999987906
2.86339063571e-10 0.999999988054
2.82664225359e-10 0.9999999882
2.79035461404e-10 0.999999988344
2.75452216592e-10 0.999999988487
2.71913935812e-10 0.999999988628
2.68420063954e-10 0.999999988767
2.64970045905e-10 0.999999988905
2.61563326553e-10 0.999999989041
2.58199350789e-10 0.999999989176
2.54877674521e-10 0.999999989308
2.51597853662e-10 0.99999998944
2.48359111055e-10 0.999999989569
2.45161224655e-10 0.999999989697
2.42003528328e-10 0.999999989824
2.38885466963e-10 0.999999989949
2.35806818516e-10 0.999999990072
2.3276680583e-10 0.999999990195
2.29765206861e-10 0.999999990315
2.26801355474e-10 0.999999990434
2.23874807581e-10 0.999999990552
2.20985230115e-10 0.999999990668
2.18132067964e-10 0.999999990783
2.15314877039e-10 0.999999990897
2.12533324273e-10 0.999999991009
2.09786854555e-10 0.99999999112
2.07075023795e-10 0.999999991229
2.04397498926e-10 0.999999991338
2.01753724838e-10 0.999999991445
1.99143479485e-10 0.99999999155
1.96566096733e-10 0.999999991655
1.9402146556e-10 0.999999991758
1.91508919833e-10 0.999999991859
1.89028237507e-10 0.99999999196
1.8657886347e-10 0.99999999206
1.84160575678e-10 0.999999992158
1.81772930041e-10 0.999999992255
1.79415482471e-10 0.999999992351
1.77088010922e-10 0.999999992445
1.74789960283e-10 0.999999992539
1.7252110851e-10 0.999999992631
1.70281011513e-10 0.999999992723
1.68069336226e-10 0.999999992813
1.65885749581e-10 0.999999992902
1.63729918512e-10 0.99999999299
1.61601398929e-10 0.999999993077
1.59499968788e-10 0.999999993163
1.57425295022e-10 0.999999993248
1.55376933542e-10 0.999999993332
1.53354662302e-10 0.999999993415
1.51358148237e-10 0.999999993497
1.49386947257e-10 0.999999993577
1.47440948339e-10 0.999999993657
1.45519596373e-10 0.999999993736
1.43622891358e-10 0.999999993814
1.4175016716e-10 0.999999993891
1.39901423779e-10 0.999999993967
1.38076217127e-10 0.999999994042
1.36274325158e-10 0.999999994117
1.34495414805e-10 0.99999999419
1.32739153003e-10 0.999999994262
1.31005428727e-10 0.999999994334
1.29293686868e-10 0.999999994405
1.27603927425e-10 0.999999994475
1.25935706308e-10 0.999999994544
1.24288912495e-10 0.999999994612
1.22662990876e-10 0.999999994679
1.21058052471e-10 0.999999994746
1.19473542171e-10 0.999999994811
1.17909237929e-10 0.999999994876
1.16365139746e-10 0.99999999494
1.14840692511e-10 0.999999995004
1.13335785201e-10 0.999999995066
1.11850195772e-10 0.999999995128
1.10383591156e-10 0.999999995189
1.08935860332e-10 0.999999995249
1.0750655921e-10 0.999999995309
1.06095687791e-10 0.999999995368
1.04703024029e-10 0.999999995426
1.03328123835e-10 0.999999995483
1.01970876187e-10 0.99999999554
1.00631059041e-10 0.999999995596
9.9308450352e-11 0.999999995651
9.80029390973e-11 0.999999995706
9.67140811881e-11 0.99999999576
9.54418766241e-11 0.999999995813
9.41859923387e-11 0.999999995866
9.29463173094e-11 0.999999995918
9.17226294916e-11 0.999999995969
9.05145958185e-11 0.99999999602
8.93222162901e-11 0.99999999607
8.81451578394e-11 0.999999996119
8.69833094441e-11 0.999999996168
8.58363380374e-11 0.999999996217
8.47042436192e-11 0.999999996264
8.35866931226e-11 0.999999996311
8.24836865476e-11 0.999999996358
8.13947798051e-11 0.999999996404
8.03199728949e-11 0.999999996449
7.92591547949e-11 0.999999996494
7.82118814158e-11 0.999999996538
7.71782637798e-11 0.999999996582
7.61579688202e-11 0.999999996625
7.51507744923e-11 0.999999996668
7.4156680796e-11 0.99999999671
7.31754656869e-11 0.999999996752
7.22070181425e-11 0.999999996793
7.1251005096e-11 0.999999996833
7.03074265473e-11 0.999999996874
6.9376060452e-11 0.999999996913
6.84566847653e-11 0.999999996952
6.75492994873e-11 0.999999996991
6.66536825733e-11 0.999999997029
6.57697230011e-11 0.999999997067
6.4897198726e-11 0.999999997104
6.40359987258e-11 0.999999997141
6.31859009559e-11 0.999999997177
6.23469054162e-11 0.999999997213
6.15187900621e-11 0.999999997248
6.07015548937e-11 0.999999997283
5.98947558217e-11 0.999999997318
5.90986148907e-11 0.999999997352
5.83126880116e-11 0.999999997386
5.75370862066e-11 0.999999997419
5.67715874311e-11 0.999999997452
5.60159696406e-11 0.999999997484
5.52702328349e-11 0.999999997516
5.45341549696e-11 0.999999997548
5.38077360446e-11 0.999999997579
5.30908650376e-11 0.99999999761
5.23832088817e-11 0.99999999764
5.16847675769e-11 0.999999997671
5.09955411232e-11 0.9999999977
5.0315307476e-11 0.99999999773
4.96438445907e-11 0.999999997759
4.89812634896e-11 0.999999997787
4.83272311058e-11 0.999999997816
4.76818584616e-11 0.999999997843
4.70448124901e-11 0.999999997871
4.64162042135e-11 0.999999997898
4.57957005651e-11 0.999999997925
4.5183412567e-11 0.999999997952
4.45791181747e-11 0.999999997978
4.39827063659e-11 0.999999998004
4.33940661182e-11 0.999999998029
4.28131974317e-11 0.999999998055
4.22398782618e-11 0.99999999808
4.16741086084e-11 0.999999998104
4.11157774494e-11 0.999999998128
4.05647737622e-11 0.999999998152
4.00209865248e-11 0.999999998176
3.94843047147e-11 0.9999999982
3.89546173096e-11 0.999999998223
3.84320353319e-11 0.999999998246
3.79162257147e-11 0.999999998268
3.74071884579e-11 0.99999999829
3.69048125393e-11 0.999999998312
3.64090979588e-11 0.999999998334
3.59199336941e-11 0.999999998355
3.54370977007e-11 0.999999998377
3.49607010008e-11 0.999999998398
3.44905215499e-11 0.999999998418
3.40265593479e-11 0.999999998439
3.35687033726e-11 0.999999998459
3.31168426015e-11 0.999999998479
3.26709770349e-11 0.999999998498
3.22309956502e-11 0.999999998518
3.17967874253e-11 0.999999998537
3.13683523601e-11 0.999999998556
3.094546841e-11 0.999999998574
3.05282465973e-11 0.999999998593
3.01165758998e-11 0.999999998611
2.97102342728e-11 0.999999998629
2.93093327386e-11 0.999999998646
2.89136492526e-11 0.999999998664
2.85232948372e-11 0.999999998681
2.81380474476e-11 0.999999998698
2.7757907084e-11 0.999999998715
2.7382762724e-11 0.999999998732
2.70126143675e-11 0.999999998748
2.66473509924e-11 0.999999998764
2.62869725987e-11 0.99999999878
2.59312571416e-11 0.999999998796
2.55803156435e-11 0.999999998812
2.52340370821e-11 0.999999998827
2.48923104351e-11 0.999999998842
2.45552467248e-11 0.999999998857
2.42225128844e-11 0.999999998872
2.3894219936e-11 0.999999998887
2.35702568574e-11 0.999999998901
2.32507346709e-11 0.999999998916
2.29353203096e-11 0.99999999893
2.26241247958e-11 0.999999998944
2.23170371072e-11 0.999999998957
2.20140572438e-11 0.999999998971
2.17151852056e-11 0.999999998984
2.14201989479e-11 0.999999998998
2.11290984709e-11 0.999999999011
2.08419947967e-11 0.999999999024
2.05585548585e-11 0.999999999036
2.02790007009e-11 0.999999999049
2.00032213016e-11 0.999999999061
1.97309946159e-11 0.999999999073
1.94624316663e-11 0.999999999086
1.91974214303e-11 0.999999999098
1.89360749303e-11 0.999999999109
1.86780590994e-11 0.999999999121
1.84235959821e-11 0.999999999132
1.8172463534e-11 0.999999999144
1.79246617549e-11 0.999999999155
1.76801906449e-11 0.999999999166
1.74390502039e-11 0.999999999177
1.72011294097e-11 0.999999999188
1.696631724e-11 0.999999999198
1.67346136948e-11 0.999999999209
1.65061297963e-11 0.999999999219
1.62806435e-11 0.999999999229
1.60581548059e-11 0.999999999239
1.58386637139e-11 0.999999999249
1.56220592018e-11 0.999999999259
1.54084522919e-11 0.999999999269
1.51976209395e-11 0.999999999279
1.4989676167e-11 0.999999999288
1.4784506952e-11 0.999999999297
1.45821132946e-11 0.999999999307
1.43823841725e-11 0.999999999316
1.41853195856e-11 0.999999999325
1.3990919534e-11 0.999999999334
1.37991840177e-11 0.999999999342
1.36100020143e-11 0.999999999351
1.34232625015e-11 0.99999999936
1.32391875241e-11 0.999999999368
1.30574440149e-11 0.999999999376
1.28782540187e-11 0.999999999385
1.27013954909e-11 0.999999999393
1.25269794538e-11 0.999999999401
1.23548948849e-11 0.999999999409
1.21850307622e-11 0.999999999416
1.20176091301e-11 0.999999999424
1.18522969217e-11 0.999999999432
1.16893161817e-11 0.999999999439
1.15285558877e-11 0.999999999447
1.13699050175e-11 0.999999999454
1.1213363571e-11 0.999999999461
1.10589315483e-11 0.999999999468
1.09066089493e-11 0.999999999475
1.07563957741e-11 0.999999999482
1.06081810003e-11 0.999999999489
1.0461964628e-11 0.999999999496
1.03176356347e-11 0.999999999502
1.0175305043e-11 0.999999999509
1.00349728527e-11 0.999999999515
9.89652804151e-12 0.999999999522
9.75985958718e-12 0.999999999528
9.62507851199e-12 0.999999999534
9.49218481594e-12 0.999999999541
9.36106747673e-12 0.999999999547
9.23161547206e-12 0.999999999553
9.10405084653e-12 0.999999999559
8.97815155554e-12 0.999999999565
8.85402862139e-12 0.99999999957
8.73145999947e-12 0.999999999576
8.61066773439e-12 0.999999999582
8.49142978154e-12 0.999999999587
8.37385716324e-12 0.999999999593
8.25794987946e-12 0.999999999598
8.14348588563e-12 0.999999999603
8.03068722632e-12 0.999999999609
7.91933185695e-12 0.999999999614
7.80953079982e-12 0.999999999619
7.70117303261e-12 0.999999999624
7.59436957765e-12 0.999999999629
7.48900941261e-12 0.999999999634
7.3849815152e-12 0.999999999639
7.28250793003e-12 0.999999999644
7.18125559018e-12 0.999999999649
7.08155756257e-12 0.999999999653
6.98308078029e-12 0.999999999658
6.88604728794e-12 0.999999999662
6.79034606321e-12 0.999999999667
6.69586608382e-12 0.999999999671
6.60271837205e-12 0.999999999676
6.51079190561e-12 0.99999999968
6.4201977068e-12 0.999999999684
6.33082475332e-12 0.999999999689
6.24267304516e-12 0.999999999693
6.15563156003e-12 0.999999999697
6.06992234253e-12 0.999999999701
5.98521232575e-12 0.999999999705
5.9018345766e-12 0.999999999709
5.81945602818e-12 0.999999999713
5.73829872508e-12 0.999999999717
5.658251645e-12 0.99999999972
5.57920376565e-12 0.999999999724
5.50137713162e-12 0.999999999728
5.42454969832e-12 0.999999999732
5.34872146574e-12 0.999999999735
5.27400345618e-12 0.999999999739
5.20028464734e-12 0.999999999742
5.12756503923e-12 0.999999999746
5.05584463184e-12 0.999999999749
4.98512342517e-12 0.999999999752
4.91529039692e-12 0.999999999756
4.8465675917e-12 0.999999999759
4.77873296489e-12 0.999999999762
4.71178651651e-12 0.999999999766
4.64572824654e-12 0.999999999769
4.5806691773e-12 0.999999999772
4.51638726418e-12 0.999999999775
4.45310455177e-12 0.999999999778
4.39071001779e-12 0.999999999781
4.32909263992e-12 0.999999999784
4.26836344047e-12 0.999999999787
4.20841139714e-12 0.99999999979
4.14934753223e-12 0.999999999792
4.09106082344e-12 0.999999999795
4.03355127077e-12 0.999999999798
3.97692989651e-12 0.999999999801
3.92097465607e-12 0.999999999803
3.86590759405e-12 0.999999999806
3.81150666584e-12 0.999999999809
3.75788289375e-12 0.999999999811
3.70503627778e-12 0.999999999814
3.65285579562e-12 0.999999999816
3.60145246958e-12 0.999999999819
3.55071527736e-12 0.999999999821
3.50064421895e-12 0.999999999824
3.45135031665e-12 0.999999999826
3.40272254817e-12 0.999999999828
3.35476091351e-12 0.999999999831
3.30746541266e-12 0.999999999833
3.26083604563e-12 0.999999999835
3.2147617901e-12 0.999999999838
3.1694646907e-12 0.99999999984
3.12461168051e-12 0.999999999842
3.08053582643e-12 0.999999999844
3.03701508386e-12 0.999999999846
2.99416047511e-12 0.999999999848
2.95174995557e-12 0.99999999985
2.91011659215e-12 0.999999999852
2.86892731793e-12 0.999999999854
2.82829315523e-12 0.999999999856
2.78832512635e-12 0.999999999858
2.74891220897e-12 0.99999999986
2.70994338081e-12 0.999999999862
2.67152966416e-12 0.999999999864
2.63378208132e-12 0.999999999866
2.59636756539e-12 0.999999999868
2.55961918327e-12 0.99999999987
2.52331489037e-12 0.999999999871
2.48756570898e-12 0.999999999873
2.45226061679e-12 0.999999999875
2.41751063612e-12 0.999999999877
2.38320474466e-12 0.999999999878
2.34934294241e-12 0.99999999988
2.31603625167e-12 0.999999999882
2.28306262784e-12 0.999999999883
2.25064411552e-12 0.999999999885
2.21866969241e-12 0.999999999886
2.18713935851e-12 0.999999999888
2.15605311382e-12 0.999999999889
2.12541095834e-12 0.999999999891
2.09510186977e-12 0.999999999892
2.06534789271e-12 0.999999999894
2.03592698256e-12 0.999999999895
2.00695016161e-12 0.999999999897
1.97841742988e-12 0.999999999898
1.95021776506e-12 0.9999999999
1.92235116714e-12 0.999999999901
1.89503968073e-12 0.999999999902
1.86795023893e-12 0.999999999904
1.84130488634e-12 0.999999999905
1.81510362296e-12 0.999999999906
1.78912440418e-12 0.999999999908
1.76358927462e-12 0.999999999909
1.73849823426e-12 0.99999999991
1.71362923851e-12 0.999999999911
1.68920433197e-12 0.999999999913
1.66500147003e-12 0.999999999914
1.6412426973e-12 0.999999999915
1.61781699148e-12 0.999999999916
1.59461333027e-12 0.999999999917
1.57185375826e-12 0.999999999918
1.54931623086e-12 0.99999999992
1.52711177037e-12 0.999999999921
1.50535139909e-12 0.999999999922
1.48370205011e-12 0.999999999923
1.46249679034e-12 0.999999999924
1.44151357517e-12 0.999999999925
1.42086342692e-12 0.999999999926
1.40054634556e-12 0.999999999927
1.38045130882e-12 0.999999999928
1.36068933898e-12 0.999999999929
1.34114941375e-12 0.99999999993
1.32183153312e-12 0.999999999931
1.3028467194e-12 0.999999999932
1.28419497258e-12 0.999999999933
1.26576527038e-12 0.999999999934
1.24755761277e-12 0.999999999935
1.22968302207e-12 0.999999999936
1.21191945368e-12 0.999999999936
1.19448895219e-12 0.999999999937
1.17739151761e-12 0.999999999938
1.16040510534e-12 0.999999999939
1.14375175997e-12 0.99999999994
1.1273204592e-12 0.999999999941
1.11100018074e-12 0.999999999942
1.09501296919e-12 0.999999999942
1.07924780224e-12 0.999999999943
1.06370467989e-12 0.999999999944
1.04838360215e-12 0.999999999945
1.03328456902e-12 0.999999999946
1.01840758049e-12 0.999999999946
1.00364161426e-12 0.999999999947
9.89208714941e-13 0.999999999948
9.74886837923e-13 0.999999999948
9.60898027813e-13 0.999999999949
9.47020240005e-13 0.99999999995
9.33364496802e-13 0.999999999951
9.19819775902e-13 0.999999999951
9.06497099606e-13 0.999999999952
8.93396467916e-13 0.999999999953
8.8051788083e-13 0.999999999953
8.67750316047e-13 0.999999999954
8.55204795869e-13 0.999999999955
8.42881320295e-13 0.999999999955
8.30668867025e-13 0.999999999956
8.18678458359e-13 0.999999999956
8.06799071995e-13 0.999999999957
7.95030707934e-13 0.999999999958
7.8359541078e-13 0.999999999958
7.72160113627e-13 0.999999999959
7.61057883381e-13 0.999999999959
7.49955653134e-13 0.99999999996
7.39075467493e-13 0.999999999961
7.28417326457e-13 0.999999999961
7.1775918542e-13 0.999999999962
7.07434111291e-13 0.999999999962
6.97109037162e-13 0.999999999963
6.87006007638e-13 0.999999999963
6.77014000416e-13 0.999999999964
6.67133015497e-13 0.999999999964
6.57474075183e-13 0.999999999965
6.47926157171e-13 0.999999999965
6.38489261462e-13 0.999999999966
6.29163388055e-13 0.999999999966
6.20059559253e-13 0.999999999967
6.11066752754e-13 0.999999999967
6.02073946254e-13 0.999999999968
5.9330318436e-13 0.999999999968
5.8475446707e-13 0.999999999969
5.7620574978e-13 0.999999999969
5.67768054793e-13 0.999999999969
5.59552404411e-13 0.99999999997
5.51336754029e-13 0.99999999997
5.43343148252e-13 0.999999999971
5.35349542474e-13 0.999999999971
5.27577981302e-13 0.999999999971
5.19917442432e-13 0.999999999972
5.12256903562e-13 0.999999999972
5.04818409297e-13 0.999999999973
4.97379915032e-13 0.999999999973
4.90163465372e-13 0.999999999973
4.82947015712e-13 0.999999999974
4.75952610657e-13 0.999999999974
4.68958205602e-13 0.999999999975
4.62074822849e-13 0.999999999975
4.55302462399e-13 0.999999999975
4.48641124251e-13 0.999999999976
4.42090808406e-13 0.999999999976
4.35651514863e-13 0.999999999976
4.2921222132e-13 0.999999999977
4.22994972382e-13 0.999999999977
4.16777723444e-13 0.999999999977
4.10671496809e-13 0.999999999978
4.04676292476e-13 0.999999999978
3.98681088143e-13 0.999999999978
3.92907928415e-13 0.999999999979
3.87134768687e-13 0.999999999979
3.81361608959e-13 0.999999999979
3.75810493836e-13 0.999999999979
3.70259378712e-13 0.99999999998
3.64819285892e-13 0.99999999998
3.59490215374e-13 0.99999999998
3.54161144855e-13 0.999999999981
3.4894309664e-13 0.999999999981
3.43836070726e-13 0.999999999981
3.38840067116e-13 0.999999999981
3.33844063505e-13 0.999999999982
3.28959082196e-13 0.999999999982
3.24074100888e-13 0.999999999982
3.19300141882e-13 0.999999999982
3.14637205179e-13 0.999999999983
3.09974268475e-13 0.999999999983
3.05422354074e-13 0.999999999983
3.00870439673e-13 0.999999999983
2.96429547575e-13 0.999999999984
2.92099677779e-13 0.999999999984
2.87769807983e-13 0.999999999984
2.83550960489e-13 0.999999999984
2.79332112996e-13 0.999999999985
2.75224287805e-13 0.999999999985
2.71116462613e-13 0.999999999985
2.67119659725e-13 0.999999999985
2.63233879139e-13 0.999999999985
2.59348098552e-13 0.999999999986
2.55462317966e-13 0.999999999986
2.51687559683e-13 0.999999999986
2.48023823701e-13 0.999999999986
2.44249065418e-13 0.999999999986
2.40696351739e-13 0.999999999987
2.3714363806e-13 0.999999999987
2.33590924381e-13 0.999999999987
2.30149233005e-13 0.999999999987
2.26707541628e-13 0.999999999987
2.23376872555e-13 0.999999999988
2.20046203481e-13 0.999999999988
2.16826556709e-13 0.999999999988
2.13606909938e-13 0.999999999988
2.10387263166e-13 0.999999999988
2.07278638698e-13 0.999999999988
2.04281036531e-13 0.999999999989
2.01172412062e-13 0.999999999989
1.98174809896e-13 0.999999999989
1.95288230032e-13 0.999999999989
1.92401650168e-13 0.999999999989
1.89515070304e-13 0.999999999989
1.86739512742e-13 0.99999999999
1.8396395518e-13 0.99999999999
1.81188397619e-13 0.99999999999
1.7852386236e-13 0.99999999999
1.75859327101e-13 0.99999999999
1.73194791842e-13 0.99999999999
1.70641278885e-13 0.99999999999
1.68087765928e-13 0.999999999991
1.65534252972e-13 0.999999999991
1.63091762317e-13 0.999999999991
1.60649271663e-13 0.999999999991
1.58317803312e-13 0.999999999991
1.55875312657e-13 0.999999999991
1.53654866608e-13 0.999999999991
1.51323398256e-13 0.999999999991
1.49102952207e-13 0.999999999992
1.46882506158e-13 0.999999999992
1.44662060109e-13 0.999999999992
1.42441614059e-13 0.999999999992
1.40332190313e-13 0.999999999992
1.38222766566e-13 0.999999999992
1.36224365122e-13 0.999999999992
1.34114941375e-13 0.999999999992
1.3211653993e-13 0.999999999992
1.30118138486e-13 0.999999999993
1.28230759344e-13 0.999999999993
1.26343380202e-13 0.999999999993
1.2445600106e-13 0.999999999993
1.22568621919e-13 0.999999999993
1.20681242777e-13 0.999999999993
1.18904885937e-13 0.999999999993
1.17128529098e-13 0.999999999993
1.15352172259e-13 0.999999999993
1.13686837722e-13 0.999999999994
1.11910480882e-13 0.999999999994
1.10245146345e-13 0.999999999994
1.08579811808e-13 0.999999999994
1.06914477271e-13 0.999999999994
1.05360165037e-13 0.999999999994
1.03805852802e-13 0.999999999994
1.02251540568e-13 0.999999999994
1.00697228334e-13 0.999999999994
9.9142916099e-14 0.999999999994
9.7699626167e-14 0.999999999994
9.6256336235e-14 0.999999999994
9.4813046303e-14 0.999999999995
9.3369756371e-14 0.999999999995
9.1926466439e-14 0.999999999995
9.05941988094e-14 0.999999999995
8.91509088774e-14 0.999999999995
8.78186412478e-14 0.999999999995
8.64863736183e-14 0.999999999995
8.52651282912e-14 0.999999999995
8.39328606617e-14 0.999999999995
8.27116153346e-14 0.999999999995
8.1379347705e-14 0.999999999995
8.01581023779e-14 0.999999999995
7.89368570508e-14 0.999999999995
7.78266340262e-14 0.999999999996
7.66053886991e-14 0.999999999996
7.54951656745e-14 0.999999999996
7.42739203474e-14 0.999999999996
7.31636973228e-14 0.999999999996
7.20534742982e-14 0.999999999996
7.1054273576e-14 0.999999999996
6.99440505514e-14 0.999999999996
6.88338275268e-14 0.999999999996
6.78346268046e-14 0.999999999996
6.68354260824e-14 0.999999999996
6.58362253603e-14 0.999999999996
6.48370246381e-14 0.999999999996
6.38378239159e-14 0.999999999996
6.28386231938e-14 0.999999999996
6.19504447741e-14 0.999999999996
6.09512440519e-14 0.999999999996
6.00630656322e-14 0.999999999996
5.91748872125e-14 0.999999999997
5.81756864904e-14 0.999999999997
5.73985303731e-14 0.999999999997
5.65103519534e-14 0.999999999997
5.56221735337e-14 0.999999999997
5.4733995114e-14 0.999999999997
5.39568389968e-14 0.999999999997
5.31796828795e-14 0.999999999997
5.22915044598e-14 0.999999999997
5.15143483426e-14 0.999999999997
5.07371922254e-14 0.999999999997
4.99600361081e-14 0.999999999997
4.91828799909e-14 0.999999999997
4.84057238737e-14 0.999999999997
4.77395900589e-14 0.999999999997
4.69624339416e-14 0.999999999997
4.62963001269e-14 0.999999999997
4.56301663121e-14 0.999999999997
4.48530101949e-14 0.999999999997
4.41868763801e-14 0.999999999997
4.35207425653e-14 0.999999999997
4.28546087505e-14 0.999999999997
4.21884749358e-14 0.999999999998
4.1522341121e-14 0.999999999998
4.09672296087e-14 0.999999999998
4.03010957939e-14 0.999999999998
3.97459842816e-14 0.999999999998
3.90798504668e-14 0.999999999998
3.85247389545e-14 0.999999999998
3.78586051397e-14 0.999999999998
3.73034936274e-14 0.999999999998
3.67483821151e-14 0.999999999998
3.61932706028e-14 0.999999999998
3.56381590905e-14 0.999999999998
3.50830475782e-14 0.999999999998
3.45279360658e-14 0.999999999998
3.39728245535e-14 0.999999999998
3.35287353437e-14 0.999999999998
3.29736238314e-14 0.999999999998
3.25295346215e-14 0.999999999998
3.19744231092e-14 0.999999999998
3.15303338994e-14 0.999999999998
3.0975222387e-14 0.999999999998
3.05311331772e-14 0.999999999998
3.00870439673e-14 0.999999999998
2.96429547575e-14 0.999999999998
2.91988655476e-14 0.999999999998
2.87547763378e-14 0.999999999998
2.83106871279e-14 0.999999999998
2.78665979181e-14 0.999999999998
2.74225087082e-14 0.999999999998
2.69784194984e-14 0.999999999998
2.65343302885e-14 0.999999999998
2.62012633812e-14 0.999999999998
2.57571741713e-14 0.999999999998
2.53130849615e-14 0.999999999998
2.49800180541e-14 0.999999999998
2.46469511467e-14 0.999999999999
2.42028619368e-14 0.999999999999
2.38697950294e-14 0.999999999999
2.34257058196e-14 0.999999999999
2.30926389122e-14 0.999999999999
2.27595720048e-14 0.999999999999
2.24265050974e-14 0.999999999999
2.209343819e-14 0.999999999999
2.17603712827e-14 0.999999999999
2.14273043753e-14 0.999999999999
2.10942374679e-14 0.999999999999
2.07611705605e-14 0.999999999999
2.04281036531e-14 0.999999999999
2.00950367457e-14 0.999999999999
1.97619698383e-14 0.999999999999
1.94289029309e-14 0.999999999999
1.9206858326e-14 0.999999999999
1.88737914186e-14 0.999999999999
1.85407245112e-14 0.999999999999
1.83186799063e-14 0.999999999999
1.79856129989e-14 0.999999999999
1.7763568394e-14 0.999999999999
1.74305014866e-14 0.999999999999
1.72084568817e-14 0.999999999999
1.69864122768e-14 0.999999999999
1.66533453694e-14 0.999999999999
1.64313007645e-14 0.999999999999
1.62092561595e-14 0.999999999999
1.58761892521e-14 0.999999999999
1.56541446472e-14 0.999999999999
1.54321000423e-14 0.999999999999
1.52100554374e-14 0.999999999999
1.49880108324e-14 0.999999999999
1.47659662275e-14 0.999999999999
1.44328993201e-14 0.999999999999
1.42108547152e-14 0.999999999999
1.39888101103e-14 0.999999999999
1.37667655054e-14 0.999999999999
1.36557432029e-14 0.999999999999
1.3433698598e-14 0.999999999999
1.3211653993e-14 0.999999999999
1.29896093881e-14 0.999999999999
1.27675647832e-14 0.999999999999
1.25455201783e-14 0.999999999999
1.24344978758e-14 0.999999999999
1.22124532709e-14 0.999999999999
1.1990408666e-14 0.999999999999
1.1768364061e-14 0.999999999999
1.16573417586e-14 0.999999999999
1.14352971536e-14 0.999999999999
1.13242748512e-14 0.999999999999
1.11022302463e-14 0.999999999999
1.08801856413e-14 0.999999999999
1.07691633389e-14 0.999999999999
1.05471187339e-14 0.999999999999
1.04360964315e-14 0.999999999999
1.02140518266e-14 0.999999999999
1.01030295241e-14 0.999999999999
9.99200722163e-15 0.999999999999
9.7699626167e-15 0.999999999999
9.65894031424e-15 0.999999999999
9.43689570931e-15 0.999999999999
9.32587340685e-15 0.999999999999
9.21485110439e-15 0.999999999999
8.99280649946e-15 0.999999999999
8.881784197e-15 0.999999999999
8.77076189454e-15 0.999999999999
8.65973959208e-15 0.999999999999
8.43769498715e-15 0.999999999999
8.32667268469e-15 0.999999999999
8.21565038223e-15 0.999999999999
8.10462807976e-15 0.999999999999
7.9936057773e-15 1.0
7.88258347484e-15 1.0
7.77156117238e-15 1.0
7.54951656745e-15 1.0
7.43849426499e-15 1.0
7.32747196253e-15 1.0
7.21644966006e-15 1.0
7.1054273576e-15 1.0
6.99440505514e-15 1.0
6.88338275268e-15 1.0
6.77236045021e-15 1.0
6.66133814775e-15 1.0
6.55031584529e-15 1.0
6.43929354283e-15 1.0
6.43929354283e-15 1.0
6.32827124036e-15 1.0
6.2172489379e-15 1.0
6.10622663544e-15 1.0
5.99520433298e-15 1.0
5.88418203051e-15 1.0
5.77315972805e-15 1.0
5.77315972805e-15 1.0
5.66213742559e-15 1.0
5.55111512313e-15 1.0
5.44009282066e-15 1.0
5.3290705182e-15 1.0
5.3290705182e-15 1.0
5.21804821574e-15 1.0
5.10702591328e-15 1.0
4.99600361081e-15 1.0
4.99600361081e-15 1.0
4.88498130835e-15 1.0
4.77395900589e-15 1.0
4.77395900589e-15 1.0
4.66293670343e-15 1.0
4.55191440096e-15 1.0
4.55191440096e-15 1.0
4.4408920985e-15 1.0
4.32986979604e-15 1.0
4.32986979604e-15 1.0
4.21884749358e-15 1.0
4.10782519111e-15 1.0
4.10782519111e-15 1.0
3.99680288865e-15 1.0
3.99680288865e-15 1.0
3.88578058619e-15 1.0
3.88578058619e-15 1.0
3.77475828373e-15 1.0
3.77475828373e-15 1.0
3.66373598126e-15 1.0
3.5527136788e-15 1.0
3.5527136788e-15 1.0
3.44169137634e-15 1.0
3.44169137634e-15 1.0
3.33066907388e-15 1.0
3.33066907388e-15 1.0
3.21964677141e-15 1.0
3.21964677141e-15 1.0
3.21964677141e-15 1.0
3.10862446895e-15 1.0
3.10862446895e-15 1.0
2.99760216649e-15 1.0
2.99760216649e-15 1.0
2.88657986403e-15 1.0
2.88657986403e-15 1.0
2.88657986403e-15 1.0
2.77555756156e-15 1.0
2.77555756156e-15 1.0
2.6645352591e-15 1.0
2.6645352591e-15 1.0
2.6645352591e-15 1.0
2.55351295664e-15 1.0
2.55351295664e-15 1.0
2.44249065418e-15 1.0
2.44249065418e-15 1.0
2.44249065418e-15 1.0
2.33146835171e-15 1.0
2.33146835171e-15 1.0
2.33146835171e-15 1.0
2.22044604925e-15 1.0
2.22044604925e-15 1.0
2.22044604925e-15 1.0
2.10942374679e-15 1.0
2.10942374679e-15 1.0
2.10942374679e-15 1.0
2.10942374679e-15 1.0
1.99840144433e-15 1.0
1.99840144433e-15 1.0
1.99840144433e-15 1.0
1.88737914186e-15 1.0
1.88737914186e-15 1.0
1.88737914186e-15 1.0
1.88737914186e-15 1.0
1.7763568394e-15 1.0
1.7763568394e-15 1.0
1.7763568394e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.66533453694e-15 1.0
1.55431223448e-15 1.0
1.55431223448e-15 1.0
1.55431223448e-15 1.0
1.55431223448e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.44328993201e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.33226762955e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.22124532709e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
1.11022302463e-15 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
9.99200722163e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
8.881784197e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
7.77156117238e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
6.66133814775e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
5.55111512313e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
4.4408920985e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
3.33066907388e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
2.22044604925e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
1.11022302463e-16 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0
0.0 1.0


==> figuresAndData/dataForPeriodicSigma1initialPart.tex <==
2.0 -1.0
1.0 0.0
0.666666666667 0.333333333333
0.5 0.5
0.4 0.6
0.333333333333 0.666666666667
0.285714285714 0.714285714286
0.25 0.75
0.222222222222 0.777777777778
0.2 0.8
0.181818181818 0.818181818182
0.166666666667 0.833333333333
0.153846153846 0.846153846154
0.142857142857 0.857142857143
0.133333333333 0.866666666667
0.125 0.875
0.117647058824 0.882352941176
0.111111111111 0.888888888889
0.105263157895 0.894736842105
0.1 0.9
0.0952380952381 0.904761904762
0.0909090909091 0.909090909091
0.0869565217391 0.913043478261
0.0833333333333 0.916666666667
0.08 0.92
0.0769230769231 0.923076923077
0.0740740740741 0.925925925926
0.0714285714286 0.928571428571
0.0689655172414 0.931034482759
0.0666666666667 0.933333333333
0.0645161290323 0.935483870968
0.0625 0.9375
0.0606060606061 0.939393939394
0.0588235294118 0.941176470588
0.0571428571429 0.942857142857
0.0555555555556 0.944444444444
0.0540540540541 0.945945945946
0.0526315789474 0.947368421053
0.0512820512821 0.948717948718
0.05 0.95
0.0487804878049 0.951219512195
0.047619047619 0.952380952381
0.046511627907 0.953488372093
0.0454545454545 0.954545454545
0.0444444444444 0.955555555556
0.0434782608696 0.95652173913
0.0425531914894 0.957446808511
0.0416666666667 0.958333333333
0.0408163265306 0.959183673469
0.04 0.96
0.0392156862745 0.960784313725
0.0384615384615 0.961538461538
0.0377358490566 0.962264150943
0.037037037037 0.962962962963
0.0363636363636 0.963636363636
0.0357142857143 0.964285714286
0.0350877192982 0.964912280702
0.0344827586207 0.965517241379
0.0338983050847 0.966101694915
0.0333333333333 0.966666666667
0.0327868852459 0.967213114754
0.0322580645161 0.967741935484
0.031746031746 0.968253968254
0.03125 0.96875
0.0307692307692 0.969230769231
0.030303030303 0.969696969697
0.0298507462687 0.970149253731
0.0294117647059 0.970588235294
0.0289855072464 0.971014492754
0.0285714285714 0.971428571429
0.0281690140845 0.971830985915
0.0277777777778 0.972222222222
0.027397260274 0.972602739726
0.027027027027 0.972972972973
0.0266666666667 0.973333333333
0.0263157894737 0.973684210526
0.025974025974 0.974025974026
0.025641025641 0.974358974359
0.0253164556962 0.974683544304
0.025 0.975
0.0246913580247 0.975308641975
0.0243902439024 0.975609756098
0.0240963855422 0.975903614458
0.0238095238095 0.97619047619
0.0235294117647 0.976470588235
0.0232558139535 0.976744186047
0.0229885057471 0.977011494253
0.0227272727273 0.977272727273
0.0224719101124 0.977528089888
0.0222222222222 0.977777777778
0.021978021978 0.978021978022
0.0217391304348 0.978260869565
0.0215053763441 0.978494623656
0.0212765957447 0.978723404255
0.0210526315789 0.978947368421
0.0208333333333 0.979166666667
0.020618556701 0.979381443299
0.0204081632653 0.979591836735
0.020202020202 0.979797979798
0.02 0.98
0.019801980198 0.980198019802
0.0196078431373 0.980392156863
0.0194174757282 0.980582524272
0.0192307692308 0.980769230769
0.0190476190476 0.980952380952
0.0188679245283 0.981132075472
0.018691588785 0.981308411215
0.0185185185185 0.981481481481
0.0183486238532 0.981651376147
0.0181818181818 0.981818181818
0.018018018018 0.981981981982
0.0178571428571 0.982142857143
0.0176991150442 0.982300884956
0.0175438596491 0.982456140351
0.0173913043478 0.982608695652
0.0172413793103 0.98275862069
0.017094017094 0.982905982906
0.0169491525424 0.983050847458
0.0168067226891 0.983193277311
0.0166666666667 0.983333333333
0.0165289256198 0.98347107438
0.016393442623 0.983606557377
0.0162601626016 0.983739837398
0.0161290322581 0.983870967742
0.016 0.984
0.015873015873 0.984126984127
0.0157480314961 0.984251968504
0.015625 0.984375
0.015503875969 0.984496124031
0.0153846153846 0.984615384615
0.0152671755725 0.984732824427
0.0151515151515 0.984848484848
0.015037593985 0.984962406015
0.0149253731343 0.985074626866
0.0148148148148 0.985185185185
0.0147058823529 0.985294117647
0.014598540146 0.985401459854
0.0144927536232 0.985507246377
0.0143884892086 0.985611510791
0.0142857142857 0.985714285714
0.0141843971631 0.985815602837
0.0140845070423 0.985915492958
0.013986013986 0.986013986014
0.0138888888889 0.986111111111
0.0137931034483 0.986206896552
0.013698630137 0.986301369863
0.0136054421769 0.986394557823
0.0135135135135 0.986486486486
0.0134228187919 0.986577181208
0.0133333333333 0.986666666667
0.0132450331126 0.986754966887
0.0131578947368 0.986842105263
0.0130718954248 0.986928104575
0.012987012987 0.987012987013
0.0129032258065 0.987096774194
0.0128205128205 0.987179487179
0.0127388535032 0.987261146497
0.0126582278481 0.987341772152
0.0125786163522 0.987421383648
0.0125 0.9875
0.0124223602484 0.987577639752
0.0123456790123 0.987654320988
0.0122699386503 0.98773006135
0.0121951219512 0.987804878049
0.0121212121212 0.987878787879
0.0120481927711 0.987951807229
0.0119760479042 0.988023952096
0.0119047619048 0.988095238095
0.0118343195266 0.988165680473
0.0117647058824 0.988235294118
0.0116959064327 0.988304093567
0.0116279069767 0.988372093023
0.0115606936416 0.988439306358
0.0114942528736 0.988505747126
0.0114285714286 0.988571428571
0.0113636363636 0.988636363636
0.0112994350282 0.988700564972
0.0112359550562 0.988764044944
0.0111731843575 0.988826815642
0.0111111111111 0.988888888889
0.0110497237569 0.988950276243
0.010989010989 0.989010989011
0.0109289617486 0.989071038251
0.0108695652174 0.989130434783
0.0108108108108 0.989189189189
0.010752688172 0.989247311828
0.0106951871658 0.989304812834
0.0106382978723 0.989361702128
0.010582010582 0.989417989418
0.0105263157895 0.989473684211
0.0104712041885 0.989528795812
0.0104166666667 0.989583333333
0.0103626943005 0.989637305699
0.0103092783505 0.989690721649
0.0102564102564 0.989743589744
0.0102040816327 0.989795918367
0.010152284264 0.989847715736
0.010101010101 0.989898989899
0.0100502512563 0.989949748744
0.01 0.99
0.00995024875622 0.990049751244
0.00990099009901 0.990099009901
0.00985221674877 0.990147783251
0.00980392156863 0.990196078431
0.00975609756098 0.990243902439
0.00970873786408 0.990291262136
0.00966183574879 0.990338164251
0.00961538461538 0.990384615385
0.00956937799043 0.99043062201
0.00952380952381 0.990476190476
0.00947867298578 0.990521327014
0.00943396226415 0.990566037736
0.0093896713615 0.990610328638
0.00934579439252 0.990654205607
0.0093023255814 0.990697674419
0.00925925925926 0.990740740741
0.00921658986175 0.990783410138
0.00917431192661 0.990825688073
0.00913242009132 0.990867579909
0.00909090909091 0.990909090909
0.00904977375566 0.990950226244
0.00900900900901 0.990990990991
0.00896860986547 0.991031390135
0.00892857142857 0.991071428571
0.00888888888889 0.991111111111
0.00884955752212 0.991150442478
0.00881057268722 0.991189427313
0.00877192982456 0.991228070175
0.00873362445415 0.991266375546
0.00869565217391 0.991304347826
0.00865800865801 0.991341991342
0.00862068965517 0.991379310345
0.00858369098712 0.991416309013
0.00854700854701 0.991452991453
0.00851063829787 0.991489361702
0.00847457627119 0.991525423729
0.0084388185654 0.991561181435
0.00840336134454 0.991596638655
0.00836820083682 0.991631799163
0.00833333333333 0.991666666667
0.00829875518672 0.991701244813
0.00826446280992 0.99173553719
0.0082304526749 0.991769547325
0.00819672131148 0.991803278689
0.00816326530612 0.991836734694
0.00813008130081 0.991869918699
0.0080971659919 0.991902834008
0.00806451612903 0.991935483871
0.00803212851406 0.991967871486
0.008 0.992
0.00796812749004 0.99203187251
0.00793650793651 0.992063492063
0.00790513833992 0.99209486166
0.00787401574803 0.992125984252
0.0078431372549 0.992156862745
0.0078125 0.9921875
0.00778210116732 0.992217898833
0.0077519379845 0.992248062016
0.00772200772201 0.992277992278
0.00769230769231 0.992307692308
0.00766283524904 0.992337164751
0.00763358778626 0.992366412214
0.00760456273764 0.992395437262
0.00757575757576 0.992424242424
0.00754716981132 0.992452830189
0.00751879699248 0.992481203008
0.00749063670412 0.992509363296
0.00746268656716 0.992537313433
0.00743494423792 0.992565055762
0.00740740740741 0.992592592593
0.00738007380074 0.992619926199
0.00735294117647 0.992647058824
0.00732600732601 0.992673992674
0.00729927007299 0.992700729927
0.00727272727273 0.992727272727
0.00724637681159 0.992753623188
0.0072202166065 0.992779783394
0.00719424460432 0.992805755396
0.00716845878136 0.992831541219
0.00714285714286 0.992857142857
0.00711743772242 0.992882562278
0.00709219858156 0.992907801418
0.00706713780919 0.992932862191
0.00704225352113 0.992957746479
0.00701754385965 0.99298245614
0.00699300699301 0.993006993007
0.00696864111498 0.993031358885
0.00694444444444 0.993055555556
0.00692041522491 0.993079584775
0.00689655172414 0.993103448276
0.00687285223368 0.993127147766
0.00684931506849 0.993150684932
0.00682593856655 0.993174061433
0.00680272108844 0.993197278912
0.00677966101695 0.993220338983
0.00675675675676 0.993243243243
0.00673400673401 0.993265993266
0.00671140939597 0.993288590604
0.0066889632107 0.993311036789
0.00666666666667 0.993333333333
0.00664451827243 0.993355481728
0.00662251655629 0.993377483444
0.00660066006601 0.993399339934
0.00657894736842 0.993421052632
0.00655737704918 0.993442622951
0.00653594771242 0.993464052288
0.00651465798046 0.99348534202
0.00649350649351 0.993506493506
0.00647249190939 0.993527508091
0.00645161290323 0.993548387097
0.0064308681672 0.993569131833
0.00641025641026 0.99358974359
0.00638977635783 0.993610223642
0.00636942675159 0.993630573248
0.00634920634921 0.993650793651
0.00632911392405 0.993670886076
0.00630914826498 0.993690851735
0.0062893081761 0.993710691824
0.00626959247649 0.993730407524
0.00625 0.99375
0.00623052959502 0.993769470405
0.00621118012422 0.993788819876
0.0061919504644 0.993808049536
0.00617283950617 0.993827160494
0.00615384615385 0.993846153846
0.00613496932515 0.993865030675
0.00611620795107 0.993883792049
0.00609756097561 0.993902439024
0.00607902735562 0.993920972644
0.00606060606061 0.993939393939
0.00604229607251 0.993957703927
0.00602409638554 0.993975903614
0.00600600600601 0.993993993994
0.0059880239521 0.994011976048
0.00597014925373 0.994029850746
0.00595238095238 0.994047619048
0.00593471810089 0.994065281899
0.00591715976331 0.994082840237
0.00589970501475 0.994100294985
0.00588235294118 0.994117647059
0.0058651026393 0.994134897361
0.00584795321637 0.994152046784
0.00583090379009 0.99416909621
0.00581395348837 0.994186046512
0.00579710144928 0.994202898551
0.00578034682081 0.994219653179
0.00576368876081 0.994236311239
0.00574712643678 0.994252873563
0.00573065902579 0.994269340974
0.00571428571429 0.994285714286
0.00569800569801 0.994301994302
0.00568181818182 0.994318181818
0.0056657223796 0.99433427762
0.00564971751412 0.994350282486
0.0056338028169 0.994366197183
0.00561797752809 0.994382022472
0.00560224089636 0.994397759104
0.00558659217877 0.994413407821
0.00557103064067 0.994428969359
0.00555555555556 0.994444444444
0.00554016620499 0.994459833795
0.00552486187845 0.994475138122
0.00550964187328 0.994490358127
0.00549450549451 0.994505494505
0.00547945205479 0.994520547945
0.00546448087432 0.994535519126
0.00544959128065 0.994550408719
0.0054347826087 0.994565217391
0.00542005420054 0.994579945799
0.00540540540541 0.994594594595
0.00539083557951 0.99460916442
0.00537634408602 0.994623655914
0.00536193029491 0.994638069705
0.00534759358289 0.994652406417
0.00533333333333 0.994666666667
0.00531914893617 0.994680851064
0.0053050397878 0.994694960212
0.00529100529101 0.994708994709
0.00527704485488 0.994722955145
0.00526315789474 0.994736842105
0.00524934383202 0.994750656168
0.00523560209424 0.994764397906
0.00522193211488 0.994778067885
0.00520833333333 0.994791666667
0.00519480519481 0.994805194805
0.00518134715026 0.99481865285
0.00516795865633 0.994832041344
0.00515463917526 0.994845360825
0.00514138817481 0.994858611825
0.00512820512821 0.994871794872
0.00511508951407 0.994884910486
0.00510204081633 0.994897959184
0.00508905852417 0.994910941476
0.00507614213198 0.994923857868
0.00506329113924 0.994936708861
0.00505050505051 0.994949494949
0.00503778337531 0.994962216625
0.00502512562814 0.994974874372
0.00501253132832 0.994987468672
0.005 0.995
0.00498753117207 0.995012468828
0.00497512437811 0.995024875622
0.00496277915633 0.995037220844
0.0049504950495 0.99504950495
0.00493827160494 0.995061728395
0.00492610837438 0.995073891626
0.004914004914 0.995085995086
0.00490196078431 0.995098039216
0.00488997555012 0.99511002445
0.00487804878049 0.99512195122
0.00486618004866 0.995133819951
0.00485436893204 0.995145631068
0.00484261501211 0.995157384988
0.0048309178744 0.995169082126
0.00481927710843 0.995180722892
0.00480769230769 0.995192307692
0.00479616306954 0.99520383693
0.00478468899522 0.995215311005
0.00477326968974 0.99522673031
0.0047619047619 0.995238095238
0.00475059382423 0.995249406176
0.00473933649289 0.995260663507
0.00472813238771 0.995271867612
0.00471698113208 0.995283018868
0.00470588235294 0.995294117647
0.00469483568075 0.995305164319
0.00468384074941 0.995316159251
0.00467289719626 0.995327102804
0.004662004662 0.995337995338
0.0046511627907 0.995348837209
0.0046403712297 0.99535962877
0.00462962962963 0.99537037037
0.00461893764434 0.995381062356
0.00460829493088 0.995391705069
0.00459770114943 0.995402298851
0.0045871559633 0.995412844037
0.0045766590389 0.995423340961
0.00456621004566 0.995433789954
0.00455580865604 0.995444191344
0.00454545454545 0.995454545455
0.00453514739229 0.995464852608
0.00452488687783 0.995475113122
0.00451467268623 0.995485327314
0.0045045045045 0.995495495495
0.00449438202247 0.995505617978
0.00448430493274 0.995515695067
0.00447427293065 0.995525727069
0.00446428571429 0.995535714286
0.00445434298441 0.995545657016
0.00444444444444 0.995555555556
0.00443458980044 0.9955654102
0.00442477876106 0.995575221239
0.00441501103753 0.995584988962
0.00440528634361 0.995594713656
0.0043956043956 0.995604395604
0.00438596491228 0.995614035088
0.00437636761488 0.995623632385
0.00436681222707 0.995633187773
0.00435729847495 0.995642701525
0.00434782608696 0.995652173913
0.00433839479393 0.995661605206
0.004329004329 0.995670995671
0.00431965442765 0.995680345572
0.00431034482759 0.995689655172
0.00430107526882 0.995698924731
0.00429184549356 0.995708154506
0.00428265524625 0.995717344754
0.0042735042735 0.995726495726
0.00426439232409 0.995735607676
0.00425531914894 0.995744680851
0.00424628450106 0.995753715499
0.00423728813559 0.995762711864
0.00422832980973 0.99577167019
0.0042194092827 0.995780590717
0.00421052631579 0.995789473684
0.00420168067227 0.995798319328
0.0041928721174 0.995807127883
0.00418410041841 0.995815899582
0.00417536534447 0.995824634656
0.00416666666667 0.995833333333
0.004158004158 0.995841995842
0.00414937759336 0.995850622407
0.00414078674948 0.995859213251
0.00413223140496 0.995867768595
0.00412371134021 0.99587628866
0.00411522633745 0.995884773663
0.0041067761807 0.995893223819
0.00409836065574 0.995901639344
0.0040899795501 0.99591002045
0.00408163265306 0.995918367347
0.0040733197556 0.995926680244
0.00406504065041 0.99593495935
0.00405679513185 0.995943204868
0.00404858299595 0.995951417004
0.0040404040404 0.99595959596
0.00403225806452 0.995967741935
0.00402414486922 0.995975855131
0.00401606425703 0.995983935743
0.00400801603206 0.995991983968
0.004 0.996
0.00399201596806 0.996007984032
0.00398406374502 0.996015936255
0.00397614314115 0.996023856859
0.00396825396825 0.996031746032
0.0039603960396 0.99603960396
0.00395256916996 0.99604743083
0.00394477317554 0.996055226824
0.00393700787402 0.996062992126
0.00392927308448 0.996070726916
0.00392156862745 0.996078431373
0.00391389432485 0.996086105675
0.00390625 0.99609375
0.00389863547758 0.996101364522
0.00389105058366 0.996108949416
0.00388349514563 0.996116504854
0.00387596899225 0.996124031008
0.00386847195358 0.996131528046
0.003861003861 0.996138996139
0.00385356454721 0.996146435453
0.00384615384615 0.996153846154
0.00383877159309 0.996161228407
0.00383141762452 0.996168582375
0.0038240917782 0.996175908222
0.00381679389313 0.996183206107
0.00380952380952 0.99619047619
0.00380228136882 0.996197718631
0.00379506641366 0.996204933586
0.00378787878788 0.996212121212
0.00378071833648 0.996219281664
0.00377358490566 0.996226415094
0.00376647834275 0.996233521657
0.00375939849624 0.996240601504
0.00375234521576 0.996247654784
0.00374531835206 0.996254681648
0.00373831775701 0.996261682243
0.00373134328358 0.996268656716
0.00372439478585 0.996275605214
0.00371747211896 0.996282527881
0.00371057513915 0.996289424861
0.0037037037037 0.996296296296
0.00369685767098 0.996303142329
0.00369003690037 0.9963099631
0.0036832412523 0.996316758748
0.00367647058824 0.996323529412
0.00366972477064 0.996330275229
0.003663003663 0.996336996337
0.0036563071298 0.99634369287
0.0036496350365 0.996350364964
0.00364298724954 0.99635701275
0.00363636363636 0.996363636364
0.00362976406534 0.996370235935
0.0036231884058 0.996376811594
0.00361663652803 0.996383363472
0.00361010830325 0.996389891697
0.0036036036036 0.996396396396
0.00359712230216 0.996402877698
0.00359066427289 0.996409335727
0.00358422939068 0.996415770609
0.00357781753131 0.996422182469
0.00357142857143 0.996428571429
0.00356506238859 0.996434937611
0.00355871886121 0.996441281139
0.00355239786856 0.996447602131
0.00354609929078 0.996453900709
0.00353982300885 0.996460176991
0.00353356890459 0.996466431095
0.00352733686067 0.996472663139
0.00352112676056 0.996478873239
0.00351493848858 0.996485061511
0.00350877192982 0.99649122807
0.00350262697023 0.99649737303
0.0034965034965 0.996503496503
0.00349040139616 0.996509598604
0.00348432055749 0.996515679443
0.00347826086957 0.99652173913
0.00347222222222 0.996527777778
0.00346620450607 0.996533795494
0.00346020761246 0.996539792388
0.00345423143351 0.996545768566
0.00344827586207 0.996551724138
0.00344234079174 0.996557659208
0.00343642611684 0.996563573883
0.00343053173242 0.996569468268
0.00342465753425 0.996575342466
0.0034188034188 0.996581196581
0.00341296928328 0.996587030717
0.00340715502555 0.996592844974
0.00340136054422 0.996598639456
0.00339558573854 0.996604414261
0.00338983050847 0.996610169492
0.00338409475465 0.996615905245
0.00337837837838 0.996621621622
0.00337268128162 0.996627318718
0.003367003367 0.996632996633
0.00336134453782 0.996638655462
0.00335570469799 0.996644295302
0.00335008375209 0.996649916248
0.00334448160535 0.996655518395
0.00333889816361 0.996661101836
0.00333333333333 0.996666666667
0.00332778702163 0.996672212978
0.00332225913621 0.996677740864
0.00331674958541 0.996683250415
0.00331125827815 0.996688741722
0.00330578512397 0.996694214876
0.003300330033 0.996699669967
0.00329489291598 0.996705107084
0.00328947368421 0.996710526316
0.00328407224959 0.99671592775
0.00327868852459 0.996721311475
0.00327332242226 0.996726677578
0.00326797385621 0.996732026144
0.00326264274062 0.996737357259
0.00325732899023 0.99674267101
0.00325203252033 0.99674796748
0.00324675324675 0.996753246753
0.0032414910859 0.996758508914
0.00323624595469 0.996763754045
0.0032310177706 0.996768982229
0.00322580645161 0.996774193548
0.00322061191626 0.996779388084
0.0032154340836 0.996784565916
0.00321027287319 0.996789727127
0.00320512820513 0.996794871795
0.0032 0.9968
0.00319488817891 0.996805111821
0.00318979266348 0.996810207337
0.0031847133758 0.996815286624
0.00317965023847 0.996820349762
0.0031746031746 0.996825396825
0.00316957210777 0.996830427892
0.00316455696203 0.996835443038
0.00315955766193 0.996840442338
0.00315457413249 0.996845425868
0.00314960629921 0.996850393701
0.00314465408805 0.996855345912
0.00313971742543 0.996860282575
0.00313479623824 0.996865203762
0.00312989045383 0.996870109546
0.003125 0.996875
0.00312012480499 0.996879875195
0.00311526479751 0.996884735202
0.00311041990669 0.996889580093
0.00310559006211 0.996894409938
0.0031007751938 0.996899224806
0.0030959752322 0.996904024768
0.00309119010819 0.996908809892
0.00308641975309 0.996913580247
0.00308166409861 0.996918335901
0.00307692307692 0.996923076923
0.00307219662058 0.996927803379
0.00306748466258 0.996932515337
0.00306278713629 0.996937212864
0.00305810397554 0.996941896024
0.0030534351145 0.996946564885
0.0030487804878 0.996951219512
0.00304414003044 0.99695585997
0.00303951367781 0.996960486322
0.00303490136571 0.996965098634
0.0030303030303 0.99696969697
0.00302571860817 0.996974281392
0.00302114803625 0.996978851964
0.00301659125189 0.996983408748
0.00301204819277 0.996987951807
0.00300751879699 0.996992481203
0.003003003003 0.996996996997
0.00299850074963 0.99700149925
0.00299401197605 0.997005988024
0.00298953662182 0.997010463378
0.00298507462687 0.997014925373
0.00298062593145 0.997019374069
0.00297619047619 0.997023809524
0.00297176820208 0.997028231798
0.00296735905045 0.99703264095
0.00296296296296 0.997037037037
0.00295857988166 0.997041420118
0.00295420974889 0.997045790251
0.00294985250737 0.997050147493
0.00294550810015 0.9970544919
0.00294117647059 0.997058823529
0.00293685756241 0.997063142438
0.00293255131965 0.99706744868
0.00292825768668 0.997071742313
0.00292397660819 0.997076023392
0.0029197080292 0.997080291971
0.00291545189504 0.997084548105
0.00291120815138 0.997088791849
0.00290697674419 0.997093023256
0.00290275761974 0.99709724238
0.00289855072464 0.997101449275
0.00289435600579 0.997105643994
0.0028901734104 0.99710982659
0.002886002886 0.997113997114
0.0028818443804 0.99711815562
0.00287769784173 0.997122302158
0.00287356321839 0.997126436782
0.00286944045911 0.997130559541
0.00286532951289 0.997134670487
0.00286123032904 0.997138769671
0.00285714285714 0.997142857143
0.00285306704708 0.997146932953
0.002849002849 0.997150997151
0.00284495021337 0.997155049787
0.00284090909091 0.997159090909
0.00283687943262 0.997163120567
0.0028328611898 0.99716713881
0.002828854314 0.997171145686
0.00282485875706 0.997175141243
0.00282087447109 0.997179125529
0.00281690140845 0.997183098592
0.0028129395218 0.997187060478
0.00280898876404 0.997191011236
0.00280504908836 0.997194950912
0.00280112044818 0.997198879552
0.0027972027972 0.997202797203
0.00279329608939 0.997206703911
0.00278940027894 0.997210599721
0.00278551532033 0.99721448468
0.00278164116829 0.997218358832
0.00277777777778 0.997222222222
0.00277392510402 0.997226074896
0.00277008310249 0.997229916898
0.00276625172891 0.997233748271
0.00276243093923 0.997237569061
0.00275862068966 0.99724137931
0.00275482093664 0.997245179063
0.00275103163686 0.997248968363
0.00274725274725 0.997252747253
0.00274348422497 0.997256515775
0.0027397260274 0.997260273973
0.00273597811218 0.997264021888
0.00273224043716 0.997267759563
0.00272851296044 0.99727148704
0.00272479564033 0.99727520436
0.00272108843537 0.997278911565
0.00271739130435 0.997282608696
0.00271370420624 0.997286295794
0.00271002710027 0.9972899729
0.00270635994587 0.997293640054
0.0027027027027 0.997297297297
0.00269905533063 0.997300944669
0.00269541778976 0.99730458221
0.00269179004038 0.99730820996
0.00268817204301 0.997311827957
0.00268456375839 0.997315436242
0.00268096514745 0.997319034853
0.00267737617135 0.997322623829
0.00267379679144 0.997326203209
0.00267022696929 0.997329773031
0.00266666666667 0.997333333333
0.00266311584554 0.997336884154
0.00265957446809 0.997340425532
0.00265604249668 0.997343957503
0.0026525198939 0.997347480106
0.00264900662252 0.997350993377
0.0026455026455 0.997354497354
0.00264200792602 0.997357992074
0.00263852242744 0.997361477573
0.00263504611331 0.997364953887
0.00263157894737 0.997368421053
0.00262812089356 0.997371879106
0.00262467191601 0.997375328084
0.00262123197903 0.997378768021
0.00261780104712 0.997382198953
0.00261437908497 0.997385620915
0.00261096605744 0.997389033943
0.0026075619296 0.99739243807
0.00260416666667 0.997395833333
0.00260078023407 0.997399219766
0.0025974025974 0.997402597403
0.00259403372244 0.997405966278
0.00259067357513 0.997409326425
0.0025873221216 0.997412677878
0.00258397932817 0.997416020672
0.00258064516129 0.997419354839
0.00257731958763 0.997422680412
0.002574002574 0.997425997426
0.0025706940874 0.997429305913
0.00256739409499 0.997432605905
0.0025641025641 0.997435897436
0.00256081946223 0.997439180538
0.00255754475703 0.997442455243
0.00255427841635 0.997445721584
0.00255102040816 0.997448979592
0.00254777070064 0.997452229299
0.00254452926209 0.997455470738
0.00254129606099 0.997458703939
0.00253807106599 0.997461928934
0.00253485424588 0.997465145754
0.00253164556962 0.99746835443
0.00252844500632 0.997471554994
0.00252525252525 0.997474747475
0.00252206809584 0.997477931904
0.00251889168766 0.997481108312
0.00251572327044 0.99748427673
0.00251256281407 0.997487437186
0.00250941028858 0.997490589711
0.00250626566416 0.997493734336
0.00250312891114 0.997496871089
0.0025 0.9975
0.00249687890137 0.997503121099
0.00249376558603 0.997506234414
0.00249066002491 0.997509339975
0.00248756218905 0.997512437811
0.00248447204969 0.99751552795
0.00248138957816 0.997518610422
0.00247831474597 0.997521685254
0.00247524752475 0.997524752475
0.00247218788628 0.997527812114
0.00246913580247 0.997530864198
0.00246609124538 0.997533908755
0.00246305418719 0.997536945813
0.00246002460025 0.9975399754
0.002457002457 0.997542997543
0.00245398773006 0.99754601227
0.00245098039216 0.997549019608
0.00244798041616 0.997552019584
0.00244498777506 0.997555012225
0.002442002442 0.997557997558
0.00243902439024 0.99756097561
0.00243605359318 0.997563946407
0.00243309002433 0.997566909976
0.00243013365735 0.997569866343
0.00242718446602 0.997572815534
0.00242424242424 0.997575757576
0.00242130750605 0.997578692494
0.00241837968561 0.997581620314
0.0024154589372 0.997584541063
0.00241254523522 0.997587454765
0.00240963855422 0.997590361446
0.00240673886883 0.997593261131
0.00240384615385 0.997596153846
0.00240096038415 0.997599039616
0.00239808153477 0.997601918465
0.00239520958084 0.997604790419
0.00239234449761 0.997607655502
0.00238948626045 0.99761051374
0.00238663484487 0.997613365155
0.00238379022646 0.997616209774
0.00238095238095 0.997619047619
0.00237812128419 0.997621878716
0.00237529691211 0.997624703088
0.00237247924081 0.997627520759
0.00236966824645 0.997630331754
0.00236686390533 0.997633136095
0.00236406619385 0.997635933806
0.00236127508855 0.997638724911
0.00235849056604 0.997641509434
0.00235571260306 0.997644287397
0.00235294117647 0.997647058824
0.00235017626322 0.997649823737
0.00234741784038 0.99765258216
0.00234466588511 0.997655334115
0.00234192037471 0.997658079625
0.00233918128655 0.997660818713
0.00233644859813 0.997663551402
0.00233372228705 0.997666277713
0.002331002331 0.997668997669
0.0023282887078 0.997671711292
0.00232558139535 0.997674418605
0.00232288037166 0.997677119628
0.00232018561485 0.997679814385
0.00231749710313 0.997682502897
0.00231481481481 0.997685185185
0.00231213872832 0.997687861272
0.00230946882217 0.997690531178
0.00230680507497 0.997693194925
0.00230414746544 0.997695852535
0.00230149597238 0.997698504028
0.00229885057471 0.997701149425
0.00229621125144 0.997703788749
0.00229357798165 0.997706422018
0.00229095074456 0.997709049255
0.00228832951945 0.997711670481
0.00228571428571 0.997714285714
0.00228310502283 0.997716894977
0.00228050171038 0.99771949829
0.00227790432802 0.997722095672
0.00227531285552 0.997724687144
0.00227272727273 0.997727272727
0.00227014755959 0.99772985244
0.00226757369615 0.997732426304
0.00226500566251 0.997734994337
0.00226244343891 0.997737556561
0.00225988700565 0.997740112994
0.00225733634312 0.997742663657
0.00225479143179 0.997745208568
0.00225225225225 0.997747747748
0.00224971878515 0.997750281215
0.00224719101124 0.997752808989
0.00224466891134 0.997755331089
0.00224215246637 0.997757847534
0.00223964165733 0.997760358343
0.00223713646532 0.997762863535
0.00223463687151 0.997765363128
0.00223214285714 0.997767857143
0.00222965440357 0.997770345596
0.0022271714922 0.997772828508
0.00222469410456 0.997775305895
0.00222222222222 0.997777777778
0.00221975582686 0.997780244173
0.00221729490022 0.9977827051
0.00221483942414 0.997785160576
0.00221238938053 0.997787610619
0.00220994475138 0.997790055249
0.00220750551876 0.997792494481
0.00220507166483 0.997794928335
0.00220264317181 0.997797356828
0.002200220022 0.997799779978
0.0021978021978 0.997802197802
0.00219538968167 0.997804610318
0.00219298245614 0.997807017544
0.00219058050383 0.997809419496
0.00218818380744 0.997811816193
0.00218579234973 0.99781420765
0.00218340611354 0.997816593886
0.00218102508179 0.997818974918
0.00217864923747 0.997821350763
0.00217627856366 0.997823721436
0.00217391304348 0.997826086957
0.00217155266015 0.99782844734
0.00216919739696 0.997830802603
0.00216684723727 0.997833152763
0.0021645021645 0.997835497835
0.00216216216216 0.997837837838
0.00215982721382 0.997840172786
0.00215749730313 0.997842502697
0.00215517241379 0.997844827586
0.0021528525296 0.99784714747
0.00215053763441 0.997849462366
0.00214822771214 0.997851772288
0.00214592274678 0.997854077253
0.0021436227224 0.997856377278
0.00214132762313 0.997858672377
0.00213903743316 0.997860962567
0.00213675213675 0.997863247863
0.00213447171825 0.997865528282
0.00213219616205 0.997867803838
0.00212992545261 0.997870074547
0.00212765957447 0.997872340426
0.00212539851222 0.997874601488
0.00212314225053 0.997876857749
0.00212089077413 0.997879109226
0.0021186440678 0.997881355932
0.0021164021164 0.997883597884
0.00211416490486 0.997885835095
0.00211193241816 0.997888067582
0.00210970464135 0.997890295359
0.00210748155954 0.99789251844
0.00210526315789 0.997894736842
0.00210304942166 0.997896950578
0.00210084033613 0.997899159664
0.00209863588667 0.997901364113
0.0020964360587 0.997903563941
0.0020942408377 0.997905759162
0.00209205020921 0.997907949791
0.00208986415883 0.997910135841
0.00208768267223 0.997912317328
0.00208550573514 0.997914494265
0.00208333333333 0.997916666667
0.00208116545265 0.997918834547
0.002079002079 0.997920997921
0.00207684319834 0.997923156802
0.00207468879668 0.997925311203
0.0020725388601 0.99792746114
0.00207039337474 0.997929606625
0.00206825232678 0.997931747673
0.00206611570248 0.997933884298
0.00206398348813 0.997936016512
0.0020618556701 0.99793814433
0.00205973223481 0.997940267765
0.00205761316872 0.997942386831
0.00205549845838 0.997944501542
0.00205338809035 0.99794661191
0.00205128205128 0.997948717949
0.00204918032787 0.997950819672
0.00204708290686 0.997952917093
0.00204498977505 0.997955010225
0.00204290091931 0.997957099081
0.00204081632653 0.997959183673
0.00203873598369 0.997961264016
0.0020366598778 0.997963340122
0.00203458799593 0.997965412004
0.0020325203252 0.997967479675
0.00203045685279 0.997969543147
0.00202839756592 0.997971602434
0.00202634245187 0.997973657548
0.00202429149798 0.997975708502
0.00202224469161 0.997977755308
0.0020202020202 0.99797979798
0.00201816347124 0.997981836529
0.00201612903226 0.997983870968
0.00201409869084 0.997985901309
0.00201207243461 0.997987927565
0.00201005025126 0.997989949749
0.00200803212851 0.997991967871
0.00200601805416 0.997993981946
0.00200400801603 0.997995991984
0.002002002002 0.997997997998


==> figuresAndData/dataForRayleigh-conditionalMean-sigma1.tex <==
0.0 0.212431330344
0.00488 0.212506831159
0.00976 0.212730293452
0.01464 0.213097220759
0.01952 0.213603218529
0.0244 0.214243994385
0.02928 0.21501535823
0.03416 0.215913222196
0.03904 0.216933600442
0.04392 0.218072608804
0.0488 0.219326464296
0.05368 0.220691484482
0.05856 0.222164086705
0.06344 0.223740787195
0.06832 0.225418200055
0.0732 0.227193036133
0.07808 0.229062101789
0.08296 0.231022297557
0.08784 0.233070616729
0.09272 0.235204143837
0.0976 0.237420053077
0.10248 0.239715606649
0.10736 0.24208815305
0.11224 0.244535125302
0.11712 0.247054039144
0.122 0.249642491178
0.12688 0.252298156987
0.13176 0.25501878923
0.13664 0.257802215712
0.14152 0.260646337451
0.1464 0.263549126729
0.15128 0.266508625145
0.15616 0.269522941677
0.16104 0.272590250747
0.16592 0.275708790297
0.1708 0.278876859891
0.17568 0.282092818826
0.18056 0.285355084278
0.18544 0.288662129468
0.19032 0.292012481858
0.1952 0.295404721382
0.20008 0.298837478708
0.20496 0.302309433541
0.20984 0.305819312952
0.21472 0.309365889759
0.2196 0.312947980939
0.22448 0.316564446082
0.22936 0.320214185885
0.23424 0.32389614069
0.23912 0.327609289061
0.244 0.331352646404
0.24888 0.335125263625
0.25376 0.338926225833
0.25864 0.342754651083
0.26352 0.346609689156
0.2684 0.350490520387
0.27328 0.354396354519
0.27816 0.358326429611
0.28304 0.362280010969
0.28792 0.366256390127
0.2928 0.370254883858
0.29768 0.374274833214
0.30256 0.378315602616
0.30744 0.382376578964
0.31232 0.386457170785
0.3172 0.390556807413
0.32208 0.394674938199
0.32696 0.398811031749
0.33184 0.402964575194
0.33672 0.407135073489
0.3416 0.411322048731
0.34648 0.415525039513
0.35136 0.4197436003
0.35624 0.423977300823
0.36112 0.428225725508
0.366 0.432488472918
0.37088 0.436765155221
0.37576 0.441055397678
0.38064 0.445358838153
0.38552 0.449675126639
0.3904 0.454003924805
0.39528 0.458344905565
0.40016 0.462697752652
0.40504 0.467062160224
0.40992 0.471437832475
0.4148 0.475824483265
0.41968 0.480221835765
0.42456 0.484629622118
0.42944 0.489047583107
0.43432 0.493475467844
0.4392 0.497913033467
0.44408 0.502360044849
0.44896 0.50681627432
0.45384 0.511281501399
0.45872 0.515755512537
0.4636 0.520238100872
0.46848 0.524729065987
0.47336 0.529228213688
0.47824 0.533735355781
0.48312 0.538250309863
0.488 0.542772899122
0.49288 0.547302952137
0.49776 0.551840302698
0.50264 0.556384789623
0.50752 0.560936256584
0.5124 0.565494551946
0.51728 0.570059528604
0.52216 0.574631043831
0.52704 0.579208959127
0.53192 0.583793140085
0.5368 0.588383456247
0.54168 0.592979780976
0.54656 0.59758199133
0.55144 0.60218996794
0.55632 0.606803594893
0.5612 0.611422759619
0.56608 0.616047352783
0.57096 0.620677268183
0.57584 0.625312402645
0.58072 0.62995265593
0.5856 0.634597930639
0.59048 0.639248132126
0.59536 0.643903168408
0.60024 0.648562950084
0.60512 0.653227390253
0.61 0.65789640444
0.61488 0.662569910517
0.61976 0.667247828637
0.62464 0.671930081157
0.62952 0.676616592579
0.6344 0.681307289482
0.63928 0.686002100458
0.64416 0.690700956056
0.64904 0.695403788723
0.65392 0.700110532747
0.6588 0.704821124203
0.66368 0.709535500905
0.66856 0.71425360235
0.67344 0.718975369675
0.67832 0.723700745607
0.6832 0.728429674419
0.68808 0.733162101888
0.69296 0.737897975249
0.69784 0.742637243159
0.70272 0.747379855656
0.7076 0.752125764119
0.71248 0.756874921234
0.71736 0.76162728096
0.72224 0.76638279849
0.72712 0.771141430222
0.732 0.775903133727
0.73688 0.780667867716
0.74176 0.785435592012
0.74664 0.790206267519
0.75152 0.794979856197
0.7564 0.799756321034
0.76128 0.804535626019
0.76616 0.809317736118
0.77104 0.814102617247
0.77592 0.818890236254
0.7808 0.82368056089
0.78568 0.828473559792
0.79056 0.833269202456
0.79544 0.838067459223
0.80032 0.842868301255
0.8052 0.847671700514
0.81008 0.852477629749
0.81496 0.857286062472
0.81984 0.862096972945
0.82472 0.86691033616
0.8296 0.871726127824
0.83448 0.876544324343
0.83936 0.881364902806
0.84424 0.88618784097
0.84912 0.891013117249
0.854 0.895840710694
0.85888 0.900670600984
0.86376 0.905502768412
0.86864 0.910337193872
0.87352 0.915173858846
0.8784 0.920012745395
0.88328 0.924853836144
0.88816 0.929697114271
0.89304 0.934542563501
0.89792 0.939390168091
0.9028 0.944239912821
0.90768 0.949091782984
0.91256 0.953945764378
0.91744 0.958801843297
0.92232 0.963660006521
0.9272 0.968520241305
0.93208 0.973382535378
0.93696 0.978246876928
0.94184 0.983113254598
0.94672 0.987981657476
0.9516 0.992852075092
0.95648 0.997724497406
0.96136 1.00259891481
0.96624 1.0074753181
0.97112 1.0123536985
0.976 1.01723404764
0.98088 1.02211635754
0.98576 1.02700062064
0.99064 1.03188682974
0.99552 1.03677497804
1.0004 1.04166505912
1.00528 1.04655706694
1.01016 1.05145099581
1.01504 1.05634684045
1.01992 1.06124459588
1.0248 1.06614425754
1.02968 1.07104582118
1.03456 1.07594928292
1.03944 1.08085463923
1.04432 1.0857618869
1.0492 1.09067102309
1.05408 1.09558204527
1.05896 1.10049495126
1.06384 1.10540973922
1.06872 1.1103264076
1.0736 1.11524495523
1.07848 1.12016538121
1.08336 1.125087685
1.08824 1.13001186635
1.09312 1.13493792535
1.098 1.13986586239
1.10288 1.14479567819
1.10776 1.14972737375
1.11264 1.1546609504
1.11752 1.15959640979
1.1224 1.16453375386
1.12728 1.16947298485
1.13216 1.17441410533
1.13704 1.17935711814
1.14192 1.18430202645
1.1468 1.18924883372
1.15168 1.19419754372
1.15656 1.1991481605
1.16144 1.20410068844
1.16632 1.2090551322
1.1712 1.21401149675
1.17608 1.21896978734
1.18096 1.22393000955
1.18584 1.22889216924
1.19072 1.23385627258
1.1956 1.23882232602
1.20048 1.24379033634
1.20536 1.24876031061
1.21024 1.25373225618
1.21512 1.25870618074
1.22 1.26368209226
1.22488 1.26865999902
1.22976 1.2736399096
1.23464 1.27862183289
1.23952 1.2836057781
1.2444 1.28859175473
1.24928 1.2935797726
1.25416 1.29856984184
1.25904 1.30356197289
1.26392 1.30855617652
1.2688 1.31355246379
1.27368 1.31855084611
1.27856 1.32355133518
1.28344 1.32855394305
1.28832 1.33355868207
1.2932 1.33856556496
1.29808 1.34357460471
1.30296 1.34858581469
1.30784 1.35359920859
1.31272 1.35861480044
1.3176 1.3636326046
1.32248 1.36865263578
1.32736 1.37367490905
1.33224 1.37869943981
1.33712 1.38372624383
1.342 1.38875533723
1.34688 1.39378673649
1.35176 1.39882045845
1.35664 1.40385652032
1.36152 1.40889493969
1.3664 1.41393573453
1.37128 1.41897892317
1.37616 1.42402452433
1.38104 1.42907255713
1.38592 1.43412304108
1.3908 1.43917599609
1.39568 1.44423144246
1.40056 1.44928940091
1.40544 1.45434989256
1.41032 1.45941293898
1.4152 1.46447856212
1.42008 1.46954678439
1.42496 1.47461762863
1.42984 1.47969111811
1.43472 1.48476727657
1.4396 1.48984612816
1.44448 1.49492769754
1.44936 1.5000120098
1.45424 1.50509909053
1.45912 1.51018896577
1.464 1.51528166207
1.46888 1.52037720647
1.47376 1.52547562649
1.47864 1.5305769502
1.48352 1.53568120615
1.4884 1.54078842343
1.49328 1.54589863166
1.49816 1.55101186101
1.50304 1.55612814219
1.50792 1.56124750647
1.5128 1.5663699857
1.51768 1.57149561229
1.52256 1.57662441924
1.52744 1.58175644017
1.53232 1.58689170929
1.5372 1.59203026141
1.54208 1.597172132
1.54696 1.60231735716
1.55184 1.60746597362
1.55672 1.6126180188
1.5616 1.61777353078
1.56648 1.62293254833
1.57136 1.6280951109
1.57624 1.63326125869
1.58112 1.63843103257
1.586 1.6436044742
1.59088 1.64878162597
1.59576 1.65396253101
1.60064 1.65914723327
1.60552 1.66433577747
1.6104 1.66952820914
1.61528 1.67472457465
1.62016 1.6799249212
1.62504 1.68512929685
1.62992 1.69033775053
1.6348 1.69555033207
1.63968 1.7007670922
1.64456 1.70598808258
1.64944 1.71121335583
1.65432 1.71644296553
1.6592 1.72167696623
1.66408 1.7269154135
1.66896 1.73215836394
1.67384 1.7374058752
1.67872 1.74265800598
1.6836 1.7479148161
1.68848 1.7531763665
1.69336 1.75844271922
1.69824 1.76371393751
1.70312 1.7689900858
1.708 1.77427122973
1.71288 1.77955743617
1.71776 1.78484877331
1.72264 1.79014531058
1.72752 1.79544711879
1.7324 1.80075427009
1.73728 1.80606683802
1.74216 1.81138489754
1.74704 1.81670852507
1.75192 1.82203779854
1.7568 1.82737279737
1.76168 1.83271360258
1.76656 1.83806029675
1.77144 1.84341296412
1.77632 1.84877169061
1.7812 1.85413656385
1.78608 1.85950767322
1.79096 1.86488510992
1.79584 1.87026896699
1.80072 1.87565933937
1.8056 1.88105632392
1.81048 1.88646001953
1.81536 1.89187052708
1.82024 1.8972879496
1.82512 1.90271239223
1.83 1.90814396233
1.83488 1.91358276952
1.83976 1.91902892573
1.84464 1.92448254531
1.84952 1.92994374501
1.8544 1.93541264414
1.85928 1.94088936456
1.86416 1.94637403082
1.86904 1.95186677016
1.87392 1.95736771265
1.8788 1.96287699124
1.88368 1.96839474184
1.88856 1.97392110342
1.89344 1.97945621808
1.89832 1.98500023115
1.9032 1.99055329129
1.90808 1.99611555058
1.91296 2.00168716463
1.91784 2.00726829267
1.92272 2.01285909769
1.9276 2.01845974652
1.93248 2.02407040997
1.93736 2.02969126294
1.94224 2.03532248457
1.94712 2.04096425836
1.952 2.0466167723
1.95688 2.05228021902
1.96176 2.05795479598
1.96664 2.06364070555
1.97152 2.06933815525
1.9764 2.07504735788
1.98128 2.0807685317
1.98616 2.08650190063
1.99104 2.09224769445
1.99592 2.09800614897
2.0008 2.1037775063
2.00568 2.109562015
2.01056 2.11535993038
2.01544 2.1211715147
2.02032 2.12699703744
2.0252 2.13283677557
2.03008 2.13869101382
2.03496 2.14456004499
2.03984 2.15044417023
2.04472 2.15634369941
2.0496 2.16225895141
2.05448 2.1681902545
2.05936 2.1741379467
2.06424 2.18010237622
2.06912 2.18608390182
2.074 2.19208289327
2.07888 2.19809973184
2.08376 2.20413481072
2.08864 2.2101885356
2.09352 2.21626132519
2.0984 2.22235361177
2.10328 2.22846584185
2.10816 2.23459847675
2.11304 2.24075199333
2.11792 2.24692688468
2.1228 2.25312366092
2.12768 2.25934284997
2.13256 2.26558499845
2.13744 2.27185067259
2.14232 2.27814045918
2.1472 2.28445496668
2.15208 2.29079482625
2.15696 2.29716069301
2.16184 2.30355324727
2.16672 2.3099731959
2.1716 2.31642127378
2.17648 2.3228982454
2.18136 2.32940490647
2.18624 2.33594208578
2.19112 2.34251064712
2.196 2.34911149136
2.20088 2.35574555873
2.20576 2.36241383127
2.21064 2.36911733542
2.21552 2.37585714493
2.2204 2.38263438396
2.22528 2.38945023045
2.23016 2.39630591981
2.23504 2.40320274894
2.23992 2.41014208063
2.2448 2.41712534835
2.24968 2.42415406158
2.25456 2.43122981158
2.25944 2.43835427782
2.26432 2.44552923508
2.2692 2.45275656128
2.27408 2.46003824619
2.27896 2.46737640117
2.28384 2.47477327001
2.28872 2.48223124107
2.2936 2.48975286094
2.29848 2.49734084987
2.30336 2.50499811922
2.30824 2.51272779125
2.31312 2.52053322174
2.318 2.52841802595
2.32288 2.53638610843
2.32776 2.54444169758
2.33264 2.55258938583
2.33752 2.56083417668
2.3424 2.56918154012
2.34728 2.57763747832
2.35216 2.58620860414
2.35704 2.59490223572
2.36192 2.60372651143
2.3668 2.61269053105
2.37168 2.62180453092
2.37656 2.63108010418
2.38144 2.64053048126
2.38632 2.65017089296
2.3912 2.66001904882
2.39608 2.67009578041
2.40096 2.68042592752
2.40584 2.69103959377
2.41072 2.70197398722
2.4156 2.71327623281
2.42048 2.72500789892
2.42536 2.73725278996
2.43024 2.75013163718
2.43512 2.76383366104


==> figuresAndData/dataForRayleigh-conditionalMean-sigma1prob0pt1.tex <==
0.0 0.302797401727
0.004276 0.3028391063
0.008552 0.302963191086
0.012828 0.303168122132
0.017104 0.303452385467
0.02138 0.303814487236
0.025656 0.304252953814
0.029932 0.304766331913
0.034208 0.305353188661
0.038484 0.306012111684
0.04276 0.306741709154
0.047036 0.307540609837
0.051312 0.308407463115
0.055588 0.309340939005
0.059864 0.310339728154
0.06414 0.311402541828
0.068416 0.312528111878
0.072692 0.313715190706
0.076968 0.314962551204
0.081244 0.316268986691
0.08552 0.317633310834
0.089796 0.319054357556
0.094072 0.320530980936
0.098348 0.322062055093
0.102624 0.323646474065
0.1069 0.325283151674
0.111176 0.326971021384
0.115452 0.328709036148
0.119728 0.330496168244
0.124004 0.332331409111
0.12828 0.334213769164
0.132556 0.336142277616
0.136832 0.338115982279
0.141108 0.34013394937
0.145384 0.342195263306
0.14966 0.344299026489
0.153936 0.346444359093
0.158212 0.348630398845
0.162488 0.350856300796
0.166764 0.353121237093
0.17104 0.355424396746
0.175316 0.357764985393
0.179592 0.360142225058
0.183868 0.362555353913
0.188144 0.365003626031
0.19242 0.367486311142
0.196696 0.370002694386
0.200972 0.372552076065
0.205248 0.375133771393
0.209524 0.377747110248
0.2138 0.380391436921
0.218076 0.383066109868
0.222352 0.385770501458
0.226628 0.388503997729
0.230904 0.391265998135
0.23518 0.394055915301
0.239456 0.39687317478
0.243732 0.399717214805
0.248008 0.402587486048
0.252284 0.40548345138
0.25656 0.408404585631
0.260836 0.411350375356
0.265112 0.414320318595
0.269388 0.417313924648
0.273664 0.420330713843
0.27794 0.423370217305
0.282216 0.42643197674
0.286492 0.429515544206
0.290768 0.432620481903
0.295044 0.435746361948
0.29932 0.438892766172
0.303596 0.442059285905
0.307872 0.445245521774
0.312148 0.448451083498
0.316424 0.451675589687
0.3207 0.454918667653
0.324976 0.458179953207
0.329252 0.461459090479
0.333528 0.464755731727
0.337804 0.468069537153
0.34208 0.471400174729
0.346356 0.474747320016
0.350632 0.478110655993
0.354908 0.481489872887
0.359184 0.484884668009
0.36346 0.488294745589
0.367736 0.491719816618
0.372012 0.495159598689
0.376288 0.498613815849
0.380564 0.502082198444
0.38484 0.505564482975
0.389116 0.509060411955
0.393392 0.512569733766
0.397668 0.516092202526
0.401944 0.519627577948
0.40622 0.523175625215
0.410496 0.526736114849
0.414772 0.530308822585
0.419048 0.533893529247
0.423324 0.537490020633
0.4276 0.541098087392
0.431876 0.544717524913
0.436152 0.548348133212
0.440428 0.551989716823
0.444704 0.555642084693
0.44898 0.559305050074
0.453256 0.562978430424
0.457532 0.56666204731
0.461808 0.570355726305
0.466084 0.5740592969
0.47036 0.577772592406
0.474636 0.581495449871
0.478912 0.585227709984
0.483188 0.588969216994
0.487464 0.592719818629
0.49174 0.596479366007
0.496016 0.600247713563
0.500292 0.60402471897
0.504568 0.60781024306
0.508844 0.611604149755
0.51312 0.615406305991
0.517396 0.619216581651
0.521672 0.623034849495
0.525948 0.626860985094
0.530224 0.630694866764
0.5345 0.634536375503
0.538776 0.63838539493
0.543052 0.642241811225
0.547328 0.646105513067
0.551604 0.649976391582
0.55588 0.653854340283
0.560156 0.657739255017
0.564432 0.661631033912
0.568708 0.665529577325
0.572984 0.669434787795
0.57726 0.673346569986
0.581536 0.677264830648
0.585812 0.681189478565
0.590088 0.68512042451
0.594364 0.689057581204
0.59864 0.693000863268
0.602916 0.696950187185
0.607192 0.700905471257
0.611468 0.704866635566
0.615744 0.708833601933
0.62002 0.712806293883
0.624296 0.716784636607
0.628572 0.720768556923
0.632848 0.724757983245
0.637124 0.728752845548
0.6414 0.732753075333
0.645676 0.736758605595
0.649952 0.74076937079
0.654228 0.74478530681
0.658504 0.748806350944
0.66278 0.752832441855
0.667056 0.75686351955
0.671332 0.760899525353
0.675608 0.764940401872
0.679884 0.768986092983
0.68416 0.773036543794
0.688436 0.777091700627
0.692712 0.781151510988
0.696988 0.785215923549
0.701264 0.789284888119
0.70554 0.793358355625
0.709816 0.797436278089
0.714092 0.801518608606
0.718368 0.805605301323
0.722644 0.809696311421
0.72692 0.813791595089
0.731196 0.817891109513
0.735472 0.821994812849
0.739748 0.826102664211
0.744024 0.830214623648
0.7483 0.834330652129
0.752576 0.838450711529
0.756852 0.842574764605
0.761128 0.846702774985
0.765404 0.850834707152
0.76968 0.854970526427
0.773956 0.859110198956
0.778232 0.863253691693
0.782508 0.867400972387
0.786784 0.871552009569
0.79106 0.875706772536
0.795336 0.879865231343
0.799612 0.884027356783
0.803888 0.88819312038
0.808164 0.892362494376
0.81244 0.896535451717
0.816716 0.900711966044
0.820992 0.904892011681
0.825268 0.909075563622
0.829544 0.913262597524
0.83382 0.917453089695
0.838096 0.921647017083
0.842372 0.925844357268
0.846648 0.930045088451
0.850924 0.934249189446
0.8552 0.93845663967
0.859476 0.942667419136
0.863752 0.946881508441
0.868028 0.951098888762
0.872304 0.955319541845
0.87658 0.959543449999
0.880856 0.963770596086
0.885132 0.968000963517
0.889408 0.972234536242
0.893684 0.976471298745
0.89796 0.980711236036
0.902236 0.984954333644
0.906512 0.989200577614
0.910788 0.993449954496
0.915064 0.997702451343
0.91934 1.0019580557
0.923616 1.00621675562
0.927892 1.0104785396
0.932168 1.01474339667
0.936444 1.01901131629
0.94072 1.02328228842
0.944996 1.02755630346
0.949272 1.03183335229
0.953548 1.03611342623
0.957824 1.04039651707
0.9621 1.04468261704
0.966376 1.0489717188
0.970652 1.05326381547
0.974928 1.05755890059
0.979204 1.06185696816
0.98348 1.06615801257
0.987756 1.07046202867
0.992032 1.07476901171
0.996308 1.07907895739
1.000584 1.08339186178
1.00486 1.08770772142
1.009136 1.09202653323
1.013412 1.09634829453
1.017688 1.10067300308
1.021964 1.10500065703
1.02624 1.10933125493
1.030516 1.11366479574
1.034792 1.11800127881
1.039068 1.1223407039
1.043344 1.12668307116
1.04762 1.13102838114
1.051896 1.13537663477
1.056172 1.1397278334
1.060448 1.14408197875
1.064724 1.14843907295
1.069 1.1527991185
1.073276 1.1571621183
1.077552 1.16152807564
1.081828 1.16589699421
1.086104 1.17026887806
1.09038 1.17464373166
1.094656 1.17902155985
1.098932 1.18340236786
1.103208 1.18778616131
1.107484 1.19217294622
1.11176 1.19656272899
1.116036 1.2009555164
1.120312 1.20535131563
1.124588 1.20975013427
1.128864 1.21415198026
1.13314 1.21855686197
1.137416 1.22296478814
1.141692 1.22737576793
1.145968 1.23178981088
1.150244 1.23620692692
1.15452 1.24062712639
1.158796 1.24505042004
1.163072 1.24947681901
1.167348 1.25390633484
1.171624 1.25833897949
1.1759 1.26277476533
1.180176 1.26721370513
1.184452 1.27165581207
1.188728 1.27610109977
1.193004 1.28054958223
1.19728 1.28500127392
1.201556 1.28945618969
1.205832 1.29391434485
1.210108 1.29837575511
1.214384 1.30284043664
1.21866 1.30730840603
1.222936 1.31177968032
1.227212 1.316254277
1.231488 1.32073221398
1.235764 1.32521350966
1.24004 1.32969818286
1.244316 1.33418625289
1.248592 1.33867773951
1.252868 1.34317266295
1.257144 1.34767104392
1.26142 1.3521729036
1.265696 1.35667826366
1.269972 1.36118714626
1.274248 1.36569957404
1.278524 1.37021557017
1.2828 1.37473515829
1.287076 1.37925836258
1.291352 1.38378520771
1.295628 1.38831571892
1.299904 1.39284992192
1.30418 1.39738784299
1.308456 1.40192950897
1.312732 1.40647494721
1.317008 1.41102418564
1.321284 1.41557725276
1.32556 1.42013417763
1.329836 1.4246949899
1.334112 1.42925971979
1.338388 1.43382839814
1.342664 1.43840105639
1.34694 1.44297772657
1.351216 1.44755844137
1.355492 1.45214323408
1.359768 1.45673213864
1.364044 1.46132518966
1.36832 1.46592242239
1.372596 1.47052387275
1.376872 1.47512957736
1.381148 1.47973957351
1.385424 1.48435389921
1.3897 1.48897259318
1.393976 1.49359569486
1.398252 1.49822324445
1.402528 1.50285528287
1.406804 1.50749185182
1.41108 1.51213299379
1.415356 1.51677875204
1.419632 1.52142917064
1.423908 1.52608429447
1.428184 1.53074416927
1.43246 1.5354088416
1.436736 1.54007835889
1.441012 1.54475276946
1.445288 1.5494321225
1.449564 1.55411646814
1.45384 1.55880585742
1.458116 1.56350034234
1.462392 1.56819997584
1.466668 1.57290481188
1.470944 1.57761490539
1.47522 1.58233031233
1.479496 1.58705108971
1.483772 1.59177729559
1.488048 1.59650898913
1.492324 1.60124623058
1.4966 1.60598908133
1.500876 1.61073760392
1.505152 1.61549186205
1.509428 1.62025192064
1.513704 1.62501784584
1.51798 1.62978970503
1.522256 1.63456756687
1.526532 1.63935150135
1.530808 1.64414157978
1.535084 1.64893787483
1.53936 1.65374046057
1.543636 1.6585494125
1.547912 1.66336480756
1.552188 1.6681867242
1.556464 1.67301524239
1.56074 1.67785044366
1.565016 1.68269241113
1.569292 1.68754122955
1.573568 1.69239698537
1.577844 1.69725976672
1.58212 1.7021296635
1.586396 1.7070067674
1.590672 1.71189117196
1.594948 1.71678297258
1.599224 1.72168226662
1.6035 1.7265891534
1.607776 1.73150373428
1.612052 1.73642611271
1.616328 1.74135639424
1.620604 1.74629468665
1.62488 1.75124109994
1.629156 1.75619574643
1.633432 1.7611587408
1.637708 1.76613020016
1.641984 1.77111024411
1.64626 1.77609899483
1.650536 1.78109657711
1.654812 1.78610311846
1.659088 1.79111874917
1.663364 1.79614360239
1.66764 1.80117781421
1.671916 1.80622152373
1.676192 1.81127487318
1.680468 1.81633800798
1.684744 1.82141107684
1.68902 1.8264942319
1.693296 1.83158762874
1.697572 1.83669142657
1.701848 1.84180578832
1.706124 1.84693088073
1.7104 1.85206687446
1.714676 1.85721394427
1.718952 1.86237226911
1.723228 1.86754203223
1.727504 1.87272342136
1.73178 1.87791662887
1.736056 1.88312185185
1.740332 1.88833929233
1.744608 1.89356915743
1.748884 1.89881165952
1.75316 1.90406701643
1.757436 1.90933545157
1.761712 1.91461719422
1.765988 1.91991247967
1.770264 1.92522154944
1.77454 1.93054465153
1.778816 1.93588204065
1.783092 1.94123397844
1.787368 1.94660073377
1.791644 1.95198258298
1.79592 1.95737981018
1.800196 1.96279270754
1.804472 1.96822157561
1.808748 1.97366672365
1.813024 1.97912847
1.8173 1.98460714239
1.821576 1.99010307838
1.825852 1.99561662575
1.830128 2.00114814293
1.834404 2.00669799942
1.83868 2.01226657633
1.842956 2.01785426685
1.847232 2.02346147675
1.851508 2.02908862503
1.855784 2.03473614445
1.86006 2.04040448217
1.864336 2.04609410047
1.868612 2.05180547743
1.872888 2.05753910767
1.877164 2.06329550321
1.88144 2.06907519431
1.885716 2.07487873038
1.889992 2.08070668094
1.894268 2.08655963674
1.898544 2.09243821077
1.90282 2.09834303957
1.907096 2.10427478443
1.911372 2.11023413277
1.915648 2.11622179969
1.919924 2.12223852946
1.9242 2.12828509729
1.928476 2.13436231118
1.932752 2.14047101386
1.937028 2.14661208497
1.941304 2.1527864434
1.94558 2.1589950498
1.949856 2.16523890931
1.954132 2.17151907457
1.958408 2.17783664898
1.962684 2.18419279019
1.96696 2.19058871406
1.971236 2.19702569889
1.975512 2.20350509007
1.979788 2.21002830528
1.984064 2.21659684015
1.98834 2.22321227454
1.992616 2.22987627953
1.996892 2.23659062517
2.001168 2.2433571891
2.005444 2.25017796628
2.00972 2.25705507977
2.013996 2.26399079301
2.018272 2.27098752358
2.022548 2.27804785886
2.026824 2.28517457385
2.0311 2.29237065156
2.035376 2.29963930642
2.039652 2.3069840113
2.043928 2.31440852888
2.048204 2.32191694828
2.05248 2.32951372804
2.056756 2.33720374702
2.061032 2.34499236493
2.065308 2.35288549506
2.069584 2.36088969236
2.07386 2.36901226114
2.078136 2.37726138819
2.082412 2.38564630931
2.086688 2.3941775204
2.090964 2.40286704906
2.09524 2.41172881024
2.099516 2.42077908106
2.103792 2.43003714953
2.108068 2.43952622495
2.112344 2.44927475749
2.11662 2.45931842697
2.120896 2.46970328991
2.125172 2.48049107966
2.129448 2.49176890652
2.133724 2.50366921695


==> figuresAndData/dataForRayleigh-conditionalMean-sigma1prob0pt1pt5prob0pt5.tex <==
0.0 0.212431330344
0.004276 0.212457201831
0.008552 0.212534209276
0.012828 0.212661443745
0.017104 0.212838008132
0.02138 0.21306301719
0.025656 0.213335597555
0.029932 0.213654887758
0.034208 0.214020038238
0.038484 0.214430211347
0.04276 0.214884581346
0.047036 0.215382334397
0.051312 0.21592266855
0.055588 0.21650479372
0.059864 0.217127931664
0.06414 0.217791315947
0.068416 0.218494191906
0.072692 0.219235816606
0.076968 0.220015458792
0.081244 0.220832398836
0.08552 0.22168592868
0.089796 0.222575351769
0.094072 0.223499982986
0.098348 0.224459148576
0.102624 0.225452186074
0.1069 0.226478444217
0.111176 0.227537282865
0.115452 0.228628072905
0.119728 0.229750196164
0.124004 0.230903045305
0.12828 0.232086023735
0.132556 0.233298545496
0.136832 0.234540035158
0.141108 0.235809927713
0.145384 0.237107668461
0.14966 0.238432712897
0.153936 0.239784526592
0.158212 0.241162585074
0.162488 0.242566373709
0.166764 0.243995387576
0.17104 0.245449131347
0.175316 0.246927119152
0.179592 0.248428874463
0.183868 0.249953929955
0.188144 0.251501827387
0.19242 0.253072117461
0.196696 0.2546643597
0.200972 0.256278122312
0.205248 0.257912982058
0.209524 0.259568524122
0.2138 0.261244341975
0.218076 0.262940037249
0.222352 0.264655219595
0.226628 0.266389506562
0.230904 0.268142523455
0.23518 0.269913903211
0.239456 0.271703286264
0.243732 0.273510320416
0.248008 0.275334660707
0.252284 0.277175969286
0.25656 0.279033915284
0.260836 0.280908174687
0.265112 0.282798430209
0.269388 0.284704371166
0.273664 0.286625693355
0.27794 0.288562098929
0.282216 0.290513296279
0.286492 0.292478999908
0.290768 0.294458930319
0.295044 0.296452813892
0.29932 0.298460382772
0.303596 0.300481374753
0.307872 0.302515533167
0.312148 0.304562606767
0.316424 0.306622349624
0.3207 0.308694521015
0.324976 0.310778885317
0.329252 0.312875211903
0.333528 0.314983275035
0.337804 0.317102853767
0.34208 0.319233731842
0.346356 0.321375697593
0.350632 0.323528543847
0.354908 0.325692067831
0.359184 0.327866071076
0.36346 0.330050359326
0.367736 0.332244742448
0.372012 0.334449034343
0.376288 0.336663052859
0.380564 0.338886619705
0.38484 0.341119560369
0.389116 0.343361704033
0.393392 0.345612883494
0.397668 0.347872935085
0.401944 0.350141698596
0.40622 0.352419017201
0.410496 0.354704737379
0.414772 0.356998708846
0.419048 0.359300784479
0.423324 0.36161082025
0.4276 0.363928675153
0.431876 0.366254211143
0.436152 0.368587293062
0.440428 0.370927788583
0.444704 0.373275568142
0.44898 0.375630504878
0.453256 0.377992474571
0.457532 0.380361355586
0.461808 0.382737028813
0.466084 0.385119377611
0.47036 0.387508287755
0.474636 0.389903647377
0.478912 0.392305346918
0.483188 0.394713279075
0.487464 0.39712733875
0.49174 0.399547423001
0.496016 0.401973430992
0.500292 0.404405263951
0.504568 0.406842825117
0.508844 0.409286019701
0.51312 0.411734754838
0.517396 0.414188939547
0.521672 0.416648484687
0.525948 0.419113302917
0.530224 0.421583308654
0.5345 0.424058418036
0.538776 0.426538548885
0.543052 0.429023620666
0.547328 0.431513554451
0.551604 0.434008272888
0.55588 0.436507700159
0.560156 0.439011761953
0.564432 0.441520385427
0.568708 0.444033499177
0.572984 0.446551033207
0.57726 0.449072918893
0.581536 0.451599088959
0.585812 0.454129477444
0.590088 0.456664019674
0.594364 0.459202652232
0.59864 0.461745312935
0.602916 0.464291940802
0.607192 0.466842476032
0.611468 0.469396859974
0.615744 0.471955035108
0.62002 0.474516945014
0.624296 0.477082534352
0.628572 0.47965174884
0.632848 0.482224535227
0.637124 0.484800841274
0.6414 0.487380615731
0.645676 0.489963808315
0.649952 0.492550369693
0.654228 0.495140251457
0.658504 0.497733406109
0.66278 0.500329787036
0.667056 0.502929348496
0.671332 0.5055320456
0.675608 0.508137834288
0.679884 0.51074667132
0.68416 0.51335851425
0.688436 0.515973321418
0.692712 0.518591051926
0.696988 0.521211665627
0.701264 0.523835123108
0.70554 0.526461385673
0.709816 0.529090415331
0.714092 0.531722174781
0.718368 0.534356627395
0.722644 0.536993737206
0.72692 0.539633468897
0.731196 0.542275787783
0.735472 0.544920659801
0.739748 0.547568051496
0.744024 0.550217930011
0.7483 0.552870263071
0.752576 0.555525018976
0.756852 0.558182166585
0.761128 0.560841675308
0.765404 0.563503515091
0.76968 0.566167656412
0.773956 0.568834070263
0.778232 0.571502728144
0.782508 0.574173602052
0.786784 0.576846664473
0.79106 0.579521888367
0.795336 0.582199247166
0.799612 0.584878714758
0.803888 0.587560265483
0.808164 0.590243874122
0.81244 0.592929515888
0.816716 0.595617166418
0.820992 0.598306801767
0.825268 0.600998398396
0.829544 0.603691933167
0.83382 0.606387383336
0.838096 0.609084726543
0.842372 0.611783940804
0.846648 0.614485004509
0.850924 0.617187896409
0.8552 0.619892595614
0.859476 0.62259908158
0.863752 0.625307334112
0.868028 0.628017333347
0.872304 0.630729059756
0.87658 0.633442494134
0.880856 0.636157617593
0.885132 0.638874411558
0.889408 0.641592857764
0.893684 0.644312938244
0.89796 0.647034635327
0.902236 0.649757931634
0.906512 0.652482810071
0.910788 0.655209253822
0.915064 0.657937246348
0.91934 0.660666771379
0.923616 0.66339781291
0.927892 0.666130355197
0.932168 0.668864382751
0.936444 0.671599880335
0.94072 0.674336832958
0.944996 0.677075225871
0.949272 0.679815044564
0.953548 0.682556274762
0.957824 0.685298902416
0.9621 0.688042913707
0.966376 0.690788295036
0.970652 0.693535033023
0.974928 0.6962831145
0.979204 0.699032526512
0.98348 0.70178325631
0.987756 0.70453529135
0.992032 0.707288619286
0.996308 0.710043227969
1.000584 0.712799105445
1.00486 0.715556239948
1.009136 0.718314619901
1.013412 0.721074233908
1.017688 0.723835070757
1.021964 0.72659711941
1.02624 0.729360369008
1.030516 0.732124808861
1.034792 0.734890428449
1.039068 0.737657217418
1.043344 0.740425165578
1.04762 0.7431942629
1.051896 0.745964499513
1.056172 0.748735865703
1.060448 0.751508351907
1.064724 0.754281948715
1.069 0.757056646866
1.073276 0.759832437243
1.077552 0.762609310873
1.081828 0.765387258928
1.086104 0.768166272714
1.09038 0.77094634368
1.094656 0.773727463405
1.098932 0.776509623604
1.103208 0.779292816122
1.107484 0.782077032934
1.11176 0.78486226614
1.116036 0.787648507966
1.120312 0.790435750763
1.124588 0.793223987
1.128864 0.796013209269
1.13314 0.798803410276
1.137416 0.801594582846
1.141692 0.804386719917
1.145968 0.807179814539
1.150244 0.809973859875
1.15452 0.812768849196
1.158796 0.815564775879
1.163072 0.818361633411
1.167348 0.821159415381
1.171624 0.823958115482
1.1759 0.826757727507
1.180176 0.829558245353
1.184452 0.832359663012
1.188728 0.835161974575
1.193004 0.837965174231
1.19728 0.84076925626
1.201556 0.843574215038
1.205832 0.846380045033
1.210108 0.849186740803
1.214384 0.851994296997
1.21866 0.854802708352
1.222936 0.85761196969
1.227212 0.860422075923
1.231488 0.863233022046
1.235764 0.866044803138
1.24004 0.86885741436
1.244316 0.871670850957
1.248592 0.874485108251
1.252868 0.877300181648
1.257144 0.880116066629
1.26142 0.882932758754
1.265696 0.885750253659
1.269972 0.888568547058
1.274248 0.891387634736
1.278524 0.894207512554
1.2828 0.897028176446
1.287076 0.899849622417
1.291352 0.902671846544
1.295628 0.905494844973
1.299904 0.90831861392
1.30418 0.911143149671
1.308456 0.913968448577
1.312732 0.916794507057
1.317008 0.919621321599
1.321284 0.922448888751
1.32556 0.925277205131
1.329836 0.928106267418
1.334112 0.930936072353
1.338388 0.933766616744
1.342664 0.936597897456
1.34694 0.939429911419
1.351216 0.942262655619
1.355492 0.945096127107
1.359768 0.947930322989
1.364044 0.950765240432
1.36832 0.953600876659
1.372596 0.956437228953
1.376872 0.95927429465
1.381148 0.962112071145
1.385424 0.964950555888
1.3897 0.967789746383
1.393976 0.970629640189
1.398252 0.97347023492
1.402528 0.976311528241
1.406804 0.979153517871
1.41108 0.981996201583
1.415356 0.984839577199
1.419632 0.987683642594
1.423908 0.990528395694
1.428184 0.993373834475
1.43246 0.996219956962
1.436736 0.999066761231
1.441012 1.00191424541
1.445288 1.00476240766
1.449564 1.00761124622
1.45384 1.01046075934
1.458116 1.01331094536
1.462392 1.01616180262
1.466668 1.01901332954
1.470944 1.02186552458
1.47522 1.02471838623
1.479496 1.02757191305
1.483772 1.03042610363
1.488048 1.03328095661
1.492324 1.03613647066
1.4966 1.03899264452
1.500876 1.04184947695
1.505152 1.04470696677
1.509428 1.04756511284
1.513704 1.05042391404
1.51798 1.05328336933
1.522256 1.05614347769
1.526532 1.05900423814
1.530808 1.06186564975
1.535084 1.06472771164
1.53936 1.06759042295
1.543636 1.07045378287
1.547912 1.07331779064
1.552188 1.07618244552
1.556464 1.07904774683
1.56074 1.08191369393
1.565016 1.0847802862
1.569292 1.08764752307
1.573568 1.09051540402
1.577844 1.09338392856
1.58212 1.09625309624
1.586396 1.09912290663
1.590672 1.10199335938
1.594948 1.10486445414
1.599224 1.10773619061
1.6035 1.11060856854
1.607776 1.11348158771
1.612052 1.11635524792
1.616328 1.11922954904
1.620604 1.12210449095
1.62488 1.12498007359
1.629156 1.1278562969
1.633432 1.13073316091
1.637708 1.13361066564
1.641984 1.13648881117
1.64626 1.13936759762
1.650536 1.14224702512
1.654812 1.14512709387
1.659088 1.14800780408
1.663364 1.15088915601
1.66764 1.15377114995
1.671916 1.15665378623
1.676192 1.15953706521
1.680468 1.1624209873
1.684744 1.16530555293
1.68902 1.16819076256
1.693296 1.17107661671
1.697572 1.17396311591
1.701848 1.17685026075
1.706124 1.17973805183
1.7104 1.1826264898
1.714676 1.18551557535
1.718952 1.18840530919
1.723228 1.19129569207
1.727504 1.19418672479
1.73178 1.19707840815
1.736056 1.19997074303
1.740332 1.20286373032
1.744608 1.20575737093
1.748884 1.20865166584
1.75316 1.21154661604
1.757436 1.21444222256
1.761712 1.21733848648
1.765988 1.22023540888
1.770264 1.22313299092
1.77454 1.22603123376
1.778816 1.2289301386
1.783092 1.2318297067
1.787368 1.23472993932
1.791644 1.23763083778
1.79592 1.24053240343
1.800196 1.24343463764
1.804472 1.24633754184
1.808748 1.24924111747
1.813024 1.25214536603
1.8173 1.25505028903
1.821576 1.25795588803
1.825852 1.26086216463
1.830128 1.26376912046
1.834404 1.26667675718
1.83868 1.26958507648
1.842956 1.27249408011
1.847232 1.27540376984
1.851508 1.27831414746
1.855784 1.28122521483
1.86006 1.28413697383
1.864336 1.28704942636
1.868612 1.28996257438
1.872888 1.29287641987
1.877164 1.29579096487
1.88144 1.29870621142
1.885716 1.30162216163
1.889992 1.30453881762
1.894268 1.30745618158
1.898544 1.3103742557
1.90282 1.31329304223
1.907096 1.31621254345
1.911372 1.31913276168
1.915648 1.32205369927
1.919924 1.32497535863
1.9242 1.32789774217
1.928476 1.33082085238
1.932752 1.33374469175
1.937028 1.33666926284
1.941304 1.33959456822
1.94558 1.34252061053
1.949856 1.34544739242
1.954132 1.34837491659
1.958408 1.35130318578
1.962684 1.35423220278
1.96696 1.3571619704
1.971236 1.36009249149
1.975512 1.36302376897
1.979788 1.36595580576
1.984064 1.36888860485
1.98834 1.37182216926
1.992616 1.37475650204
1.996892 1.37769160629
2.001168 1.38062748517
2.005444 1.38356414184
2.00972 1.38650157955
2.013996 1.38943980156
2.018272 1.39237881117
2.022548 1.39531861174
2.026824 1.39825920666
2.0311 1.40120059938
2.035376 1.40414279337
2.039652 1.40708579216
2.043928 1.41002959932
2.048204 1.41297421846
2.05248 1.41591965323
2.056756 1.41886590734
2.061032 1.42181298454
2.065308 1.42476088862
2.069584 1.42770962342
2.07386 1.43065919281
2.078136 1.43360960073
2.082412 1.43656085116
2.086688 1.43951294811
2.090964 1.44246589567
2.09524 1.44541969794
2.099516 1.44837435909
2.103792 1.45132988334
2.108068 1.45428627495
2.112344 1.45724353823
2.11662 1.46020167754
2.120896 1.46316069729
2.125172 1.46612060195
2.129448 1.46908139602
2.133724 1.47204308406


==> figuresAndData/dataForRayleigh-conditionalMean-sigma1pt5.tex <==
0.0 0.302797401727
0.0064 0.302838924999
0.0128 0.302962472597
0.0192 0.303166520526
0.0256 0.3034495646
0.032 0.30381012057
0.0384 0.304246724243
0.0448 0.304757931581
0.0512 0.305342318789
0.0576 0.305998482385
0.064 0.306725039257
0.0704 0.307520626704
0.0768 0.308383902466
0.0832 0.309313544735
0.0896 0.310308252153
0.096 0.311366743803
0.1024 0.312487759176
0.1088 0.313670058135
0.1152 0.314912420859
0.1216 0.316213647777
0.128 0.317572559492
0.1344 0.318987996693
0.1408 0.320458820051
0.1472 0.321983910111
0.1536 0.323562167168
0.16 0.325192511137
0.1664 0.32687388141
0.1728 0.328605236709
0.1792 0.33038555492
0.1856 0.332213832934
0.192 0.334089086466
0.1984 0.336010349874
0.2048 0.337976675968
0.2112 0.339987135816
0.2176 0.34204081854
0.224 0.344136831109
0.2304 0.346274298125
0.2368 0.348452361604
0.2432 0.350670180755
0.2496 0.352926931753
0.256 0.35522180751
0.2624 0.357554017437
0.2688 0.359922787213
0.2752 0.362327358544
0.2816 0.364766988923
0.288 0.367240951384
0.2944 0.369748534262
0.3008 0.372289040947
0.3072 0.374861789634
0.3136 0.37746611308
0.32 0.380101358359
0.3264 0.382766886607
0.3328 0.385462072786
0.3392 0.388186305429
0.3456 0.3909389864
0.352 0.393719530648
0.3584 0.396527365962
0.3648 0.399361932733
0.3712 0.402222683713
0.3776 0.405109083773
0.384 0.408020609671
0.3904 0.410956749817
0.3968 0.413917004039
0.4032 0.416900883354
0.4096 0.419907909741
0.416 0.422937615919
0.4224 0.425989545119
0.4288 0.429063250871
0.4352 0.432158296784
0.4416 0.435274256335
0.448 0.438410712657
0.4544 0.441567258333
0.4608 0.444743495189
0.4672 0.447939034099
0.4736 0.45115349478
0.48 0.454386505606
0.4864 0.457637703407
0.4928 0.46090673329
0.4992 0.464193248447
0.5056 0.467496909982
0.512 0.470817386723
0.5184 0.474154355056
0.5248 0.477507498748
0.5312 0.480876508784
0.5376 0.484261083195
0.544 0.487660926904
0.5504 0.491075751563
0.5568 0.494505275398
0.5632 0.49794922306
0.5696 0.501407325472
0.576 0.504879319689
0.5824 0.508364948749
0.5888 0.511863961539
0.5952 0.515376112654
0.6016 0.518901162266
0.608 0.522438875996
0.6144 0.525989024779
0.6208 0.529551384746
0.6272 0.5331257371
0.6336 0.536711867997
0.64 0.540309568425
0.6464 0.543918634099
0.6528 0.547538865342
0.6592 0.551170066981
0.6656 0.554812048237
0.672 0.558464622628
0.6784 0.562127607859
0.6848 0.565800825731
0.6912 0.56948410204
0.6976 0.573177266488
0.704 0.576880152583
0.7104 0.580592597559
0.7168 0.58431444228
0.7232 0.588045531162
0.7296 0.591785712086
0.736 0.595534836315
0.7424 0.59929275842
0.7488 0.603059336198
0.7552 0.606834430602
0.7616 0.610617905662
0.768 0.614409628415
0.7744 0.618209468838
0.7808 0.622017299776
0.7872 0.62583299688
0.7936 0.629656438538
0.8 0.633487505813
0.8064 0.637326082383
0.8128 0.64117205448
0.8192 0.645025310832
0.8256 0.648885742604
0.832 0.652753243346
0.8384 0.656627708935
0.8448 0.660509037525
0.8512 0.664397129495
0.8576 0.668291887396
0.864 0.672193215907
0.8704 0.676101021783
0.8768 0.68001521381
0.8832 0.683935702762
0.8896 0.687862401353
0.896 0.691795224195
0.9024 0.69573408776
0.9088 0.699678910332
0.9152 0.703629611973
0.9216 0.707586114483
0.928 0.711548341359
0.9344 0.715516217764
0.9408 0.719489670484
0.9472 0.723468627897
0.9536 0.727453019942
0.96 0.731442778077
0.9664 0.735437835255
0.9728 0.739438125889
0.9792 0.743443585818
0.9856 0.747454152284
0.992 0.751469763896
0.9984 0.755490360607
1.0048 0.759515883682
1.0112 0.763546275672
1.0176 0.76758148039
1.024 0.771621442881
1.0304 0.7756661094
1.0368 0.779715427389
1.0432 0.783769345448
1.0496 0.787827813317
1.056 0.791890781848
1.0624 0.795958202991
1.0688 0.800030029763
1.0752 0.804106216234
1.0816 0.808186717503
1.088 0.812271489682
1.0944 0.81636048987
1.1008 0.820453676141
1.1072 0.824551007522
1.1136 0.828652443975
1.12 0.832757946381
1.1264 0.836867476522
1.1328 0.840980997064
1.1392 0.845098471543
1.1456 0.849219864347
1.152 0.853345140699
1.1584 0.857474266649
1.1648 0.86160720905
1.1712 0.865743935552
1.1776 0.869884414584
1.184 0.87402861534
1.1904 0.878176507769
1.1968 0.882328062559
1.2032 0.886483251126
1.2096 0.890642045604
1.216 0.894804418828
1.2224 0.898970344328
1.2288 0.903139796314
1.2352 0.907312749667
1.2416 0.911489179928
1.248 0.915669063287
1.2544 0.919852376575
1.2608 0.924039097251
1.2672 0.928229203395
1.2736 0.932422673698
1.28 0.936619487453
1.2864 0.940819624547
1.2928 0.945023065451
1.2992 0.949229791212
1.3056 0.953439783447
1.312 0.957653024333
1.3184 0.961869496599
1.3248 0.966089183521
1.3312 0.970312068914
1.3376 0.974538137124
1.344 0.97876737302
1.3504 0.982999761993
1.3568 0.987235289944
1.3632 0.991473943278
1.3696 0.995715708904
1.376 0.999960574222
1.3824 1.00420852712
1.3888 1.00845955597
1.3952 1.01271364963
1.4016 1.01697079742
1.408 1.02123098912
1.4144 1.025494215
1.4208 1.02976046576
1.4272 1.03402973257
1.4336 1.03830200705
1.44 1.04257728126
1.4464 1.0468555477
1.4528 1.05113679933
1.4592 1.0554210295
1.4656 1.05970823204
1.472 1.06399840117
1.4784 1.06829153156
1.4848 1.07258761828
1.4912 1.07688665683
1.4976 1.08118864313
1.504 1.08549357351
1.5104 1.0898014447
1.5168 1.09411225384
1.5232 1.09842599849
1.5296 1.1027426766
1.536 1.10706228652
1.5424 1.11138482701
1.5488 1.11571029722
1.5552 1.1200386967
1.5616 1.12437002539
1.568 1.12870428362
1.5744 1.13304147213
1.5808 1.13738159203
1.5872 1.14172464482
1.5936 1.14607063241
1.6 1.15041955707
1.6064 1.15477142148
1.6128 1.1591262287
1.6192 1.16348398216
1.6256 1.16784468569
1.632 1.17220834351
1.6384 1.17657496021
1.6448 1.18094454079
1.6512 1.1853170906
1.6576 1.1896926154
1.664 1.19407112134
1.6704 1.19845261493
1.6768 1.2028371031
1.6832 1.20722459314
1.6896 1.21161509273
1.696 1.21600860997
1.7024 1.2204051533
1.7088 1.2248047316
1.7152 1.22920735412
1.7216 1.23361303048
1.728 1.23802177075
1.7344 1.24243358534
1.7408 1.24684848511
1.7472 1.25126648127
1.7536 1.25568758546
1.76 1.26011180973
1.7664 1.26453916653
1.7728 1.26896966869
1.7792 1.27340332951
1.7856 1.27784016264
1.792 1.28228018218
1.7984 1.28672340266
1.8048 1.291169839
1.8112 1.29561950656
1.8176 1.30007242114
1.824 1.30452859895
1.8304 1.30898805664
1.8368 1.31345081131
1.8432 1.31791688049
1.8496 1.32238628216
1.856 1.32685903474
1.8624 1.33133515712
1.8688 1.33581466864
1.8752 1.3402975891
1.8816 1.34478393877
1.888 1.34927373839
1.8944 1.35376700919
1.9008 1.35826377284
1.9072 1.36276405155
1.9136 1.36726786799
1.92 1.37177524534
1.9264 1.37628620726
1.9328 1.38080077795
1.9392 1.38531898212
1.9456 1.38984084498
1.952 1.39436639228
1.9584 1.39889565031
1.9648 1.40342864589
1.9712 1.4079654064
1.9776 1.41250595977
1.984 1.41705033449
1.9904 1.42159855961
1.9968 1.42615066478
2.0032 1.43070668022
2.0096 1.43526663675
2.016 1.43983056579
2.0224 1.44439849937
2.0288 1.44897047015
2.0352 1.4535465114
2.0416 1.45812665704
2.048 1.46271094165
2.0544 1.46729940044
2.0608 1.47189206932
2.0672 1.47648898485
2.0736 1.48109018429
2.08 1.48569570563
2.0864 1.49030558752
2.0928 1.49491986936
2.0992 1.49953859131
2.1056 1.50416179422
2.112 1.50878951977
2.1184 1.51342181035
2.1248 1.51805870917
2.1312 1.52270026025
2.1376 1.5273465084
2.144 1.53199749927
2.1504 1.53665327937
2.1568 1.54131389603
2.1632 1.5459793975
2.1696 1.55064983288
2.176 1.55532525222
2.1824 1.56000570647
2.1888 1.56469124752
2.1952 1.56938192823
2.2016 1.57407780243
2.208 1.57877892497
2.2144 1.58348535169
2.2208 1.58819713948
2.2272 1.59291434628
2.2336 1.59763703114
2.24 1.60236525417
2.2464 1.60709907664
2.2528 1.61183856093
2.2592 1.61658377063
2.2656 1.6213347705
2.272 1.62609162652
2.2784 1.63085440595
2.2848 1.63562317727
2.2912 1.64039801031
2.2976 1.6451789762
2.304 1.64996614745
2.3104 1.65475959793
2.3168 1.65955940296
2.3232 1.66436563929
2.3296 1.66917838518
2.336 1.67399772038
2.3424 1.6788237262
2.3488 1.68365648557
2.3552 1.688496083
2.3616 1.6933426047
2.368 1.69819613857
2.3744 1.70305677427
2.3808 1.70792460323
2.3872 1.71279971873
2.3936 1.71768221591
2.4 1.72257219183
2.4064 1.72746974556
2.4128 1.73237497815
2.4192 1.73728799273
2.4256 1.74220889457
2.432 1.74713779111
2.4384 1.75207479203
2.4448 1.7570200093
2.4512 1.76197355725
2.4576 1.76693555265
2.464 1.77190611471
2.4704 1.77688536522
2.4768 1.7818734286
2.4832 1.78687043195
2.4896 1.79187650512
2.496 1.79689178085
2.5024 1.80191639476
2.5088 1.80695048552
2.5152 1.81199419487
2.5216 1.81704766776
2.528 1.82211105239
2.5344 1.82718450037
2.5408 1.83226816675
2.5472 1.83736221022
2.5536 1.8424667931
2.56 1.84758208155
2.5664 1.85270824565
2.5728 1.85784545952
2.5792 1.86299390145
2.5856 1.86815375405
2.592 1.87332520435
2.5984 1.87850844401
2.6048 1.88370366938
2.6112 1.88891108174
2.6176 1.89413088743
2.624 1.899363298
2.6304 1.90460853043
2.6368 1.90986680729
2.6432 1.91513835694
2.6496 1.92042341375
2.656 1.92572221827
2.6624 1.93103501752
2.6688 1.93636206515
2.6752 1.94170362176
2.6816 1.9470599551
2.688 1.95243134035
2.6944 1.95781806044
2.7008 1.9632204063
2.7072 1.96863867719
2.7136 1.97407318106
2.72 1.97952423483
2.7264 1.98499216481
2.7328 1.99047730707
2.7392 1.99598000782
2.7456 2.00150062387
2.752 2.00703952305
2.7584 2.01259708471
2.7648 2.0181737002
2.7712 2.0237697734
2.7776 2.02938572131
2.784 2.03502197462
2.7904 2.04067897833
2.7968 2.04635719246
2.8032 2.0520570927
2.8096 2.05777917123
2.816 2.06352393747
2.8224 2.06929191897
2.8288 2.0750836623
2.8352 2.08089973402
2.8416 2.08674072173
2.848 2.09260723517
2.8544 2.09849990741
2.8608 2.10441939612
2.8672 2.11036638493
2.8736 2.11634158489
2.88 2.12234573606
2.8864 2.12837960918
2.8928 2.13444400751
2.8992 2.14053976879
2.9056 2.1466677674
2.912 2.15282891661
2.9184 2.15902417114
2.9248 2.16525452983
2.9312 2.17152103862
2.9376 2.17782479374
2.944 2.18416694526
2.9504 2.19054870092
2.9568 2.19697133031
2.9632 2.20343616953
2.9696 2.2099446263
2.976 2.21649818551
2.9824 2.22309841551
2.9888 2.22974697492
2.9952 2.23644562037
3.0016 2.24319621495
3.008 2.25000073781
3.0144 2.25686129487
3.0208 2.26378013081
3.0272 2.27075964275
3.0336 2.27780239559
3.04 2.28491113965
3.0464 2.29208883067
3.0528 2.29933865288
3.0592 2.3066640456
3.0656 2.31406873402
3.072 2.32155676528
3.0784 2.32913255059
3.0848 2.33680091521
3.0912 2.34456715779
3.0976 2.35243712167
3.104 2.36041728101
3.1104 2.3685148462
3.1168 2.37673789383
3.1232 2.38509552917
3.1296 2.39359809182
3.136 2.40225741992
3.1424 2.41108719547
3.1488 2.42010340443
3.1552 2.42932496378
3.1616 2.43877459912
3.168 2.44848011221
3.1744 2.45847628348
3.1808 2.46880786649
3.1872 2.47953459676
3.1936 2.49074027328


==> figuresAndData/dataForRayleigh-conditionalMean-sigma1pt5prob0pt05.tex <==
0.0 0.212431330344
0.004276 0.212457201831
0.008552 0.212534209276
0.012828 0.212661443745
0.017104 0.212838008132
0.02138 0.21306301719
0.025656 0.213335597555
0.029932 0.213654887758
0.034208 0.214020038238
0.038484 0.214430211347
0.04276 0.214884581346
0.047036 0.215382334397
0.051312 0.21592266855
0.055588 0.21650479372
0.059864 0.217127931664
0.06414 0.217791315947
0.068416 0.218494191906
0.072692 0.219235816606
0.076968 0.220015458792
0.081244 0.220832398836
0.08552 0.22168592868
0.089796 0.222575351769
0.094072 0.223499982986
0.098348 0.224459148576
0.102624 0.225452186074
0.1069 0.226478444217
0.111176 0.227537282865
0.115452 0.228628072905
0.119728 0.229750196164
0.124004 0.230903045305
0.12828 0.232086023735
0.132556 0.233298545496
0.136832 0.234540035158
0.141108 0.235809927713
0.145384 0.237107668461
0.14966 0.238432712897
0.153936 0.239784526592
0.158212 0.241162585074
0.162488 0.242566373709
0.166764 0.243995387576
0.17104 0.245449131347
0.175316 0.246927119152
0.179592 0.248428874463
0.183868 0.249953929955
0.188144 0.251501827387
0.19242 0.253072117461
0.196696 0.2546643597
0.200972 0.256278122312
0.205248 0.257912982058
0.209524 0.259568524122
0.2138 0.261244341975
0.218076 0.262940037249
0.222352 0.264655219595
0.226628 0.266389506562
0.230904 0.268142523455
0.23518 0.269913903211
0.239456 0.271703286264
0.243732 0.273510320416
0.248008 0.275334660707
0.252284 0.277175969286
0.25656 0.279033915284
0.260836 0.280908174687
0.265112 0.282798430209
0.269388 0.284704371166
0.273664 0.286625693355
0.27794 0.288562098929
0.282216 0.290513296279
0.286492 0.292478999908
0.290768 0.294458930319
0.295044 0.296452813892
0.29932 0.298460382772
0.303596 0.300481374753
0.307872 0.302515533167
0.312148 0.304562606767
0.316424 0.306622349624
0.3207 0.308694521015
0.324976 0.310778885317
0.329252 0.312875211903
0.333528 0.314983275035
0.337804 0.317102853767
0.34208 0.319233731842
0.346356 0.321375697593
0.350632 0.323528543847
0.354908 0.325692067831
0.359184 0.327866071076
0.36346 0.330050359326
0.367736 0.332244742448
0.372012 0.334449034343
0.376288 0.336663052859
0.380564 0.338886619705
0.38484 0.341119560369
0.389116 0.343361704033
0.393392 0.345612883494
0.397668 0.347872935085
0.401944 0.350141698596
0.40622 0.352419017201
0.410496 0.354704737379
0.414772 0.356998708846
0.419048 0.359300784479
0.423324 0.36161082025
0.4276 0.363928675153
0.431876 0.366254211143
0.436152 0.368587293062
0.440428 0.370927788583
0.444704 0.373275568142
0.44898 0.375630504878
0.453256 0.377992474571
0.457532 0.380361355586
0.461808 0.382737028813
0.466084 0.385119377611
0.47036 0.387508287755
0.474636 0.389903647377
0.478912 0.392305346918
0.483188 0.394713279075
0.487464 0.39712733875
0.49174 0.399547423001
0.496016 0.401973430992
0.500292 0.404405263951
0.504568 0.406842825117
0.508844 0.409286019701
0.51312 0.411734754838
0.517396 0.414188939547
0.521672 0.416648484687
0.525948 0.419113302917
0.530224 0.421583308654
0.5345 0.424058418036
0.538776 0.426538548885
0.543052 0.429023620666
0.547328 0.431513554451
0.551604 0.434008272888
0.55588 0.436507700159
0.560156 0.439011761953
0.564432 0.441520385427
0.568708 0.444033499177
0.572984 0.446551033207
0.57726 0.449072918893
0.581536 0.451599088959
0.585812 0.454129477444
0.590088 0.456664019674
0.594364 0.459202652232
0.59864 0.461745312935
0.602916 0.464291940802
0.607192 0.466842476032
0.611468 0.469396859974
0.615744 0.471955035108
0.62002 0.474516945014
0.624296 0.477082534352
0.628572 0.47965174884
0.632848 0.482224535227
0.637124 0.484800841274
0.6414 0.487380615731
0.645676 0.489963808315
0.649952 0.492550369693
0.654228 0.495140251457
0.658504 0.497733406109
0.66278 0.500329787036
0.667056 0.502929348496
0.671332 0.5055320456
0.675608 0.508137834288
0.679884 0.51074667132
0.68416 0.51335851425
0.688436 0.515973321418
0.692712 0.518591051926
0.696988 0.521211665627
0.701264 0.523835123108
0.70554 0.526461385673
0.709816 0.529090415331
0.714092 0.531722174781
0.718368 0.534356627395
0.722644 0.536993737206
0.72692 0.539633468897
0.731196 0.542275787783
0.735472 0.544920659801
0.739748 0.547568051496
0.744024 0.550217930011
0.7483 0.552870263071
0.752576 0.555525018976
0.756852 0.558182166585
0.761128 0.560841675308
0.765404 0.563503515091
0.76968 0.566167656412
0.773956 0.568834070263
0.778232 0.571502728144
0.782508 0.574173602052
0.786784 0.576846664473
0.79106 0.579521888367
0.795336 0.582199247166
0.799612 0.584878714758
0.803888 0.587560265483
0.808164 0.590243874122
0.81244 0.592929515888
0.816716 0.595617166418
0.820992 0.598306801767
0.825268 0.600998398396
0.829544 0.603691933167
0.83382 0.606387383336
0.838096 0.609084726543
0.842372 0.611783940804
0.846648 0.614485004509
0.850924 0.617187896409
0.8552 0.619892595614
0.859476 0.62259908158
0.863752 0.625307334112
0.868028 0.628017333347
0.872304 0.630729059756
0.87658 0.633442494134
0.880856 0.636157617593
0.885132 0.638874411558
0.889408 0.641592857764
0.893684 0.644312938244
0.89796 0.647034635327
0.902236 0.649757931634
0.906512 0.652482810071
0.910788 0.655209253822
0.915064 0.657937246348
0.91934 0.660666771379
0.923616 0.66339781291
0.927892 0.666130355197
0.932168 0.668864382751
0.936444 0.671599880335
0.94072 0.674336832958
0.944996 0.677075225871
0.949272 0.679815044564
0.953548 0.682556274762
0.957824 0.685298902416
0.9621 0.688042913707
0.966376 0.690788295036
0.970652 0.693535033023
0.974928 0.6962831145
0.979204 0.699032526512
0.98348 0.70178325631
0.987756 0.70453529135
0.992032 0.707288619286
0.996308 0.710043227969
1.000584 0.712799105445
1.00486 0.715556239948
1.009136 0.718314619901
1.013412 0.721074233908
1.017688 0.723835070757
1.021964 0.72659711941
1.02624 0.729360369008
1.030516 0.732124808861
1.034792 0.734890428449
1.039068 0.737657217418
1.043344 0.740425165578
1.04762 0.7431942629
1.051896 0.745964499513
1.056172 0.748735865703
1.060448 0.751508351907
1.064724 0.754281948715
1.069 0.757056646866
1.073276 0.759832437243
1.077552 0.762609310873
1.081828 0.765387258928
1.086104 0.768166272714
1.09038 0.77094634368
1.094656 0.773727463405
1.098932 0.776509623604
1.103208 0.779292816122
1.107484 0.782077032934
1.11176 0.78486226614
1.116036 0.787648507966
1.120312 0.790435750763
1.124588 0.793223987
1.128864 0.796013209269
1.13314 0.798803410276
1.137416 0.801594582846
1.141692 0.804386719917
1.145968 0.807179814539
1.150244 0.809973859875
1.15452 0.812768849196
1.158796 0.815564775879
1.163072 0.818361633411
1.167348 0.821159415381
1.171624 0.823958115482
1.1759 0.826757727507
1.180176 0.829558245353
1.184452 0.832359663012
1.188728 0.835161974575
1.193004 0.837965174231
1.19728 0.84076925626
1.201556 0.843574215038
1.205832 0.846380045033
1.210108 0.849186740803
1.214384 0.851994296997
1.21866 0.854802708352
1.222936 0.85761196969
1.227212 0.860422075923
1.231488 0.863233022046
1.235764 0.866044803138
1.24004 0.86885741436
1.244316 0.871670850957
1.248592 0.874485108251
1.252868 0.877300181648
1.257144 0.880116066629
1.26142 0.882932758754
1.265696 0.885750253659
1.269972 0.888568547058
1.274248 0.891387634736
1.278524 0.894207512554
1.2828 0.897028176446
1.287076 0.899849622417
1.291352 0.902671846544
1.295628 0.905494844973
1.299904 0.90831861392
1.30418 0.911143149671
1.308456 0.913968448577
1.312732 0.916794507057
1.317008 0.919621321599
1.321284 0.922448888751
1.32556 0.925277205131
1.329836 0.928106267418
1.334112 0.930936072353
1.338388 0.933766616744
1.342664 0.936597897456
1.34694 0.939429911419
1.351216 0.942262655619
1.355492 0.945096127107
1.359768 0.947930322989
1.364044 0.950765240432
1.36832 0.953600876659
1.372596 0.956437228953
1.376872 0.95927429465
1.381148 0.962112071145
1.385424 0.964950555888
1.3897 0.967789746383
1.393976 0.970629640189
1.398252 0.97347023492
1.402528 0.976311528241
1.406804 0.979153517871
1.41108 0.981996201583
1.415356 0.984839577199
1.419632 0.987683642594
1.423908 0.990528395694
1.428184 0.993373834475
1.43246 0.996219956962
1.436736 0.999066761231
1.441012 1.00191424541
1.445288 1.00476240766
1.449564 1.00761124622
1.45384 1.01046075934
1.458116 1.01331094536
1.462392 1.01616180262
1.466668 1.01901332954
1.470944 1.02186552458
1.47522 1.02471838623
1.479496 1.02757191305
1.483772 1.03042610363
1.488048 1.03328095661
1.492324 1.03613647066
1.4966 1.03899264452
1.500876 1.04184947695
1.505152 1.04470696677
1.509428 1.04756511284
1.513704 1.05042391404
1.51798 1.05328336933
1.522256 1.05614347769
1.526532 1.05900423814
1.530808 1.06186564975
1.535084 1.06472771164
1.53936 1.06759042295
1.543636 1.07045378287
1.547912 1.07331779064
1.552188 1.07618244552
1.556464 1.07904774683
1.56074 1.08191369393
1.565016 1.0847802862
1.569292 1.08764752307
1.573568 1.09051540402
1.577844 1.09338392856
1.58212 1.09625309624
1.586396 1.09912290663
1.590672 1.10199335938
1.594948 1.10486445414
1.599224 1.10773619061
1.6035 1.11060856854
1.607776 1.11348158771
1.612052 1.11635524792
1.616328 1.11922954904
1.620604 1.12210449095
1.62488 1.12498007359
1.629156 1.1278562969
1.633432 1.13073316091
1.637708 1.13361066564
1.641984 1.13648881117
1.64626 1.13936759762
1.650536 1.14224702512
1.654812 1.14512709387
1.659088 1.14800780408
1.663364 1.15088915601
1.66764 1.15377114995
1.671916 1.15665378623
1.676192 1.15953706521
1.680468 1.1624209873
1.684744 1.16530555293
1.68902 1.16819076256
1.693296 1.17107661671
1.697572 1.17396311591
1.701848 1.17685026075
1.706124 1.17973805183
1.7104 1.1826264898
1.714676 1.18551557535
1.718952 1.18840530919
1.723228 1.19129569207
1.727504 1.19418672479
1.73178 1.19707840815
1.736056 1.19997074303
1.740332 1.20286373032
1.744608 1.20575737093
1.748884 1.20865166584
1.75316 1.21154661604
1.757436 1.21444222256
1.761712 1.21733848648
1.765988 1.22023540888
1.770264 1.22313299092
1.77454 1.22603123376
1.778816 1.2289301386
1.783092 1.2318297067
1.787368 1.23472993932
1.791644 1.23763083778
1.79592 1.24053240343
1.800196 1.24343463764
1.804472 1.24633754184
1.808748 1.24924111747
1.813024 1.25214536603
1.8173 1.25505028903
1.821576 1.25795588803
1.825852 1.26086216463
1.830128 1.26376912046
1.834404 1.26667675718
1.83868 1.26958507648
1.842956 1.27249408011
1.847232 1.27540376984
1.851508 1.27831414746
1.855784 1.28122521483
1.86006 1.28413697383
1.864336 1.28704942636
1.868612 1.28996257438
1.872888 1.29287641987
1.877164 1.29579096487
1.88144 1.29870621142
1.885716 1.30162216163
1.889992 1.30453881762
1.894268 1.30745618158
1.898544 1.3103742557
1.90282 1.31329304223
1.907096 1.31621254345
1.911372 1.31913276168
1.915648 1.32205369927
1.919924 1.32497535863
1.9242 1.32789774217
1.928476 1.33082085238
1.932752 1.33374469175
1.937028 1.33666926284
1.941304 1.33959456822
1.94558 1.34252061053
1.949856 1.34544739242
1.954132 1.34837491659
1.958408 1.35130318578
1.962684 1.35423220278
1.96696 1.3571619704
1.971236 1.36009249149
1.975512 1.36302376897
1.979788 1.36595580576
1.984064 1.36888860485
1.98834 1.37182216926
1.992616 1.37475650204
1.996892 1.37769160629
2.001168 1.38062748517
2.005444 1.38356414184
2.00972 1.38650157955
2.013996 1.38943980156
2.018272 1.39237881117
2.022548 1.39531861174
2.026824 1.39825920666
2.0311 1.40120059938
2.035376 1.40414279337
2.039652 1.40708579216
2.043928 1.41002959932
2.048204 1.41297421846
2.05248 1.41591965323
2.056756 1.41886590734
2.061032 1.42181298454
2.065308 1.42476088862
2.069584 1.42770962342
2.07386 1.43065919281
2.078136 1.43360960073
2.082412 1.43656085116
2.086688 1.43951294811
2.090964 1.44246589567
2.09524 1.44541969794
2.099516 1.44837435909
2.103792 1.45132988334
2.108068 1.45428627495
2.112344 1.45724353823
2.11662 1.46020167754
2.120896 1.46316069729
2.125172 1.46612060195
2.129448 1.46908139602
2.133724 1.47204308406


==> figuresAndData/dataForRayleigh-conditionalMean-sigma2.tex <==
0.0 0.302797401727
0.00853 0.302838892665
0.01706 0.302962344457
0.02559 0.303166234883
0.03412 0.303449061498
0.04265 0.303809341765
0.05118 0.304245613172
0.05971 0.304756433327
0.06824 0.305340380053
0.07677 0.305996051452
0.0853 0.306722065965
0.09383 0.307517062411
0.10236 0.308379700019
0.11089 0.309308658437
0.11942 0.310302637733
0.12795 0.311360358381
0.13648 0.312480561235
0.14501 0.313662007486
0.15354 0.314903478613
0.16207 0.316203776311
0.1706 0.31756172242
0.17913 0.318976158834
0.18766 0.3204459474
0.19619 0.321969969808
0.20472 0.323547127468
0.21325 0.32517634138
0.22178 0.326856551995
0.23031 0.328586719061
0.23884 0.330365821467
0.24737 0.332192857074
0.2559 0.334066842541
0.26443 0.335986813145
0.27296 0.337951822587
0.28149 0.339960942801
0.29002 0.342013263746
0.29855 0.344107893207
0.30708 0.346243956575
0.31561 0.348420596631
0.32414 0.350636973327
0.33267 0.352892263555
0.3412 0.355185660923
0.34973 0.357516375516
0.35826 0.359883633666
0.36679 0.362286677708
0.37532 0.364724765745
0.38385 0.367197171403
0.39238 0.369703183585
0.40091 0.372242106231
0.40944 0.374813258071
0.41797 0.377415972375
0.4265 0.380049596712
0.43503 0.382713492699
0.44356 0.385407035759
0.45209 0.388129614872
0.46062 0.390880632331
0.46915 0.3936595035
0.47768 0.396465656568
0.48621 0.399298532312
0.49474 0.402157583853
0.50327 0.405042276422
0.5118 0.40795208712
0.52033 0.410886504689
0.52886 0.413845029275
0.53739 0.416827172203
0.54592 0.419832455748
0.55445 0.42286041291
0.56298 0.425910587197
0.57151 0.4289825324
0.58004 0.43207581238
0.58857 0.435190000857
0.5971 0.438324681197
0.60563 0.441479446205
0.61416 0.444653897924
0.62269 0.447847647434
0.63122 0.45106031465
0.63975 0.454291528134
0.64828 0.457540924901
0.65681 0.46080815023
0.66534 0.464092857483
0.67387 0.467394707922
0.6824 0.470713370531
0.69093 0.474048521842
0.69946 0.477399845765
0.70799 0.480767033417
0.71652 0.484149782962
0.72505 0.487547799444
0.73358 0.490960794633
0.74211 0.494388486871
0.75064 0.497830600915
0.75917 0.501286867793
0.7677 0.504757024657
0.77623 0.508240814641
0.78476 0.51173798672
0.79329 0.515248295577
0.80182 0.518771501466
0.81035 0.522307370085
0.81888 0.525855672444
0.82741 0.529416184745
0.83594 0.532988688259
0.84447 0.536572969204
0.853 0.540168818633
0.86153 0.543776032315
0.87006 0.547394410631
0.87859 0.551023758459
0.88712 0.554663885071
0.89565 0.558314604029
0.90418 0.561975733087
0.91271 0.565647094085
0.92124 0.56932851286
0.92977 0.573019819151
0.9383 0.576720846503
0.94683 0.580431432182
0.95536 0.584151417085
0.96389 0.587880645656
0.97242 0.591618965803
0.98095 0.595366228818
0.98948 0.599122289295
0.99801 0.602887005054
1.00654 0.606660237069
1.01507 0.610441849388
1.0236 0.614231709069
1.03213 0.618029686104
1.04066 0.621835653355
1.04919 0.625649486486
1.05772 0.629471063898
1.06625 0.633300266666
1.07478 0.63713697848
1.08331 0.64098108558
1.09184 0.644832476703
1.10037 0.648691043022
1.1089 0.652556678093
1.11743 0.656429277798
1.12596 0.660308740298
1.13449 0.664194965972
1.14302 0.668087857378
1.15155 0.671987319194
1.16008 0.675893258178
1.16861 0.679805583117
1.17714 0.683724204784
1.18567 0.687649035892
1.1942 0.691579991052
1.20273 0.695516986733
1.21126 0.699459941218
1.21979 0.703408774564
1.22832 0.707363408568
1.23685 0.711323766722
1.24538 0.715289774183
1.25391 0.719261357733
1.26244 0.723238445744
1.27097 0.727220968146
1.2795 0.731208856392
1.28803 0.735202043427
1.29656 0.739200463655
1.30509 0.743204052908
1.31362 0.747212748418
1.32215 0.751226488786
1.33068 0.755245213954
1.33921 0.759268865177
1.34774 0.763297384996
1.35627 0.767330717212
1.3648 0.77136880686
1.37333 0.775411600184
1.38186 0.779459044613
1.39039 0.783511088734
1.39892 0.787567682275
1.40745 0.791628776078
1.41598 0.795694322075
1.42451 0.799764273272
1.43304 0.803838583725
1.44157 0.807917208519
1.4501 0.812000103751
1.45863 0.816087226506
1.46716 0.820178534843
1.47569 0.824273987773
1.48422 0.828373545243
1.49275 0.832477168118
1.50128 0.836584818164
1.50981 0.840696458032
1.51834 0.844812051239
1.52687 0.848931562157
1.5354 0.853054955993
1.54393 0.857182198778
1.55246 0.861313257349
1.56099 0.865448099338
1.56952 0.869586693155
1.57805 0.873729007976
1.58658 0.877875013731
1.59511 0.882024681089
1.60364 0.886177981449
1.61217 0.890334886924
1.6207 0.89449537033
1.62923 0.898659405176
1.63776 0.902826965653
1.64629 0.906998026622
1.65482 0.911172563602
1.66335 0.915350552765
1.67188 0.919531970917
1.68041 0.923716795498
1.68894 0.927905004567
1.69747 0.932096576793
1.706 0.936291491446
1.71453 0.940489728391
1.72306 0.944691268076
1.73159 0.948896091526
1.74012 0.953104180335
1.74865 0.957315516656
1.75718 0.961530083195
1.76571 0.965747863204
1.77424 0.969968840473
1.78277 0.974192999323
1.7913 0.978420324601
1.79983 0.982650801671
1.80836 0.986884416408
1.81689 0.991121155195
1.82542 0.99536100491
1.83395 0.999603952931
1.84248 1.00384998712
1.85101 1.00809909582
1.85954 1.01235126786
1.86807 1.01660649253
1.8766 1.02086475959
1.88513 1.02512605928
1.89366 1.02939038227
1.90219 1.0336577197
1.91072 1.03792806316
1.91925 1.04220140469
1.92778 1.04647773676
1.93631 1.05075705228
1.94484 1.05503934459
1.95337 1.05932460748
1.9619 1.06361283514
1.97043 1.0679040222
1.97896 1.07219816372
1.98749 1.07649525516
1.99602 1.08079529239
2.00455 1.08509827172
2.01308 1.08940418985
2.02161 1.09371304388
2.03014 1.09802483133
2.03867 1.10233955013
2.0472 1.10665719858
2.05573 1.11097777542
2.06426 1.11530127975
2.07279 1.11962771108
2.08132 1.12395706933
2.08985 1.12828935478
2.09838 1.13262456813
2.10691 1.13696271046
2.11544 1.14130378323
2.12397 1.14564778831
2.1325 1.14999472792
2.14103 1.15434460471
2.14956 1.15869742169
2.15809 1.16305318225
2.16662 1.16741189019
2.17515 1.17177354967
2.18368 1.17613816525
2.19221 1.18050574187
2.20074 1.18487628486
2.20927 1.18924979991
2.2178 1.19362629313
2.22633 1.198005771
2.23486 1.20238824037
2.24339 1.20677370851
2.25192 1.21116218305
2.26045 1.21555367202
2.26898 1.21994818384
2.27751 1.2243457273
2.28604 1.22874631163
2.29457 1.23314994639
2.3031 1.23755664158
2.31163 1.24196640759
2.32016 1.24637925519
2.32869 1.25079519555
2.33722 1.25521424027
2.34575 1.25963640131
2.35428 1.26406169108
2.36281 1.26849012236
2.37134 1.27292170836
2.37987 1.2773564627
2.3884 1.28179439941
2.39693 1.28623553294
2.40546 1.29067987816
2.41399 1.29512745038
2.42252 1.2995782653
2.43105 1.30403233909
2.43958 1.30848968833
2.44811 1.31295033004
2.45664 1.31741428168
2.46517 1.32188156116
2.4737 1.32635218684
2.48223 1.33082617753
2.49076 1.33530355249
2.49929 1.33978433145
2.50782 1.3442685346
2.51635 1.3487561826
2.52488 1.35324729658
2.53341 1.35774189818
2.54194 1.36224000949
2.55047 1.36674165309
2.559 1.37124685209
2.56753 1.37575563008
2.57606 1.38026801114
2.58459 1.3847840199
2.59312 1.38930368148
2.60165 1.39382702155
2.61018 1.39835406629
2.61871 1.40288484243
2.62724 1.40741937725
2.63577 1.41195769857
2.6443 1.4164998348
2.65283 1.42104581487
2.66136 1.42559566833
2.66989 1.4301494253
2.67842 1.43470711648
2.68695 1.43926877318
2.69548 1.44383442733
2.70401 1.44840411145
2.71254 1.45297785872
2.72107 1.45755570293
2.7296 1.46213767852
2.73813 1.46672382061
2.74666 1.47131416496
2.75519 1.47590874802
2.76372 1.4805076069
2.77225 1.48511077946
2.78078 1.48971830422
2.78931 1.49433022045
2.79784 1.49894656814
2.80637 1.50356738803
2.8149 1.50819272162
2.82343 1.51282261118
2.83196 1.51745709975
2.84049 1.5220962312
2.84902 1.52674005017
2.85755 1.53138860217
2.86608 1.53604193351
2.87461 1.54070009139
2.88314 1.54536312386
2.89167 1.55003107987
2.9002 1.55470400927
2.90873 1.55938196282
2.91726 1.56406499224
2.92579 1.56875315019
2.93432 1.57344649032
2.94285 1.57814506725
2.95138 1.58284893664
2.95991 1.58755815518
2.96844 1.59227278059
2.97697 1.59699287168
2.9855 1.60171848837
2.99403 1.60644969168
3.00256 1.61118654378
3.01109 1.61592910801
3.01962 1.62067744889
3.02815 1.62543163217
3.03668 1.63019172482
3.04521 1.63495779509
3.05374 1.63972991254
3.06227 1.64450814803
3.0708 1.64929257378
3.07933 1.6540832634
3.08786 1.6588802919
3.09639 1.66368373575
3.10492 1.66849367289
3.11345 1.67331018277
3.12198 1.67813334638
3.13051 1.68296324632
3.13904 1.68779996677
3.14757 1.69264359359
3.1561 1.69749421435
3.16463 1.70235191832
3.17316 1.70721679659
3.18169 1.71208894204
3.19022 1.71696844943
3.19875 1.72185541544
3.20728 1.72674993871
3.21581 1.73165211988
3.22434 1.73656206166
3.23287 1.74147986886
3.2414 1.74640564849
3.24993 1.75133950976
3.25846 1.75628156416
3.26699 1.76123192555
3.27552 1.76619071015
3.28405 1.77115803671
3.29258 1.77613402647
3.30111 1.78111880329
3.30964 1.78611249371
3.31817 1.79111522704
3.3267 1.79612713539
3.33523 1.80114835379
3.34376 1.80617902028
3.35229 1.81121927596
3.36082 1.8162692651
3.36935 1.82132913523
3.37788 1.82639903725
3.38641 1.8314791255
3.39494 1.83656955789
3.40347 1.841670496
3.412 1.84678210519
3.42053 1.85190455472
3.42906 1.85703801786
3.43759 1.86218267203
3.44612 1.86733869895
3.45465 1.87250628471
3.46318 1.87768562001
3.47171 1.88287690023
3.48024 1.8880803256
3.48877 1.89329610142
3.4973 1.89852443814
3.50583 1.90376555162
3.51436 1.90901966324
3.52289 1.91428700016
3.53142 1.9195677955
3.53995 1.92486228851
3.54848 1.93017072485
3.55701 1.9354933568
3.56554 1.9408304435
3.57407 1.9461822512
3.5826 1.95154905353
3.59113 1.95693113179
3.59966 1.96232877525
3.60819 1.96774228142
3.61672 1.97317195643
3.62525 1.97861811533
3.63378 1.98408108247
3.64231 1.98956119186
3.65084 1.99505878761
3.65937 2.0005742243
3.6679 2.00610786746
3.67643 2.01166009402
3.68496 2.01723129283
3.69349 2.02282186515
3.70202 2.02843222524
3.71055 2.03406280091
3.71908 2.03971403418
3.72761 2.04538638192
3.73614 2.05108031656
3.74467 2.05679632682
3.7532 2.06253491852
3.76173 2.06829661541
3.77026 2.07408196009
3.77879 2.07989151494
3.78732 2.08572586317
3.79585 2.09158560988
3.80438 2.09747138327
3.81291 2.10338383586
3.82144 2.10932364587
3.82997 2.1152915186
3.8385 2.12128818807
3.84703 2.12731441858
3.85556 2.13337100662
3.86409 2.13945878272
3.87262 2.1455786136
3.88115 2.1517314044
3.88968 2.15791810118
3.89821 2.16413969356
3.90674 2.17039721764
3.91527 2.17669175914
3.9238 2.18302445688
3.93233 2.18939650654
3.94086 2.19580916479
3.94939 2.20226375383
3.95792 2.2087616664
3.96645 2.21530437125
3.97498 2.22189341928
3.98351 2.22853045023
3.99204 2.23521720022
4.00057 2.24195551005
4.0091 2.2487473346
4.01763 2.25559475321
4.02616 2.26249998151
4.03469 2.26946538464
4.04322 2.27649349234
4.05175 2.28358701601
4.06028 2.29074886824
4.06881 2.29798218527
4.07734 2.30529035274
4.08587 2.31267703569
4.0944 2.32014621337
4.10293 2.32770222018
4.11146 2.3353497939
4.11999 2.34309413299
4.12852 2.3509409653
4.13705 2.358896631
4.14558 2.36696818371
4.15411 2.37516351512
4.16264 2.38349151024
4.17117 2.39196224345
4.1797 2.40058722963
4.18823 2.40937975111
4.19676 2.41835529169
4.20529 2.42753212527
4.21382 2.43693213509
4.22235 2.44658198918
4.23088 2.45651489019
4.23941 2.46677330155
4.24794 2.47741344742
4.25647 2.48851332698


==> figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt05.tex <==
0.0 0.212431330344
0.008276 0.212485700302
0.016552 0.212646953884
0.024828 0.212912335474
0.033104 0.213279142092
0.04138 0.213744723529
0.049656 0.214306482438
0.057932 0.214961874351
0.066208 0.215708407653
0.074484 0.216543643486
0.08276 0.217465195606
0.091036 0.218470730187
0.099312 0.219557965566
0.107588 0.220724671943
0.115864 0.221968671031
0.12414 0.223287835657
0.132416 0.224680089321
0.140692 0.226143405712
0.148968 0.227675808182
0.157244 0.229275369184
0.16552 0.23094020967
0.173796 0.232668498465
0.182072 0.234458451601
0.190348 0.236308331623
0.198624 0.23821644688
0.2069 0.240181150775
0.215176 0.242200841011
0.223452 0.244273958806
0.231728 0.246398988098
0.240004 0.248574454734
0.24828 0.250798925645
0.256556 0.253071008015
0.264832 0.255389348438
0.273108 0.257752632076
0.281384 0.260159581802
0.28966 0.262608957351
0.297936 0.265099554466
0.306212 0.267630204046
0.314488 0.270199771296
0.322764 0.272807154881
0.33104 0.275451286088
0.339316 0.278131127991
0.347592 0.280845674625
0.355868 0.28359395017
0.364144 0.286375008146
0.37242 0.289187930611
0.380696 0.292031827382
0.388972 0.294905835259
0.397248 0.297809117266
0.405524 0.300740861901
0.4138 0.303700282409
0.422076 0.306686616059
0.430352 0.309699123438
0.438628 0.312737087766
0.446904 0.315799814217
0.45518 0.318886629264
0.463456 0.32199688003
0.471732 0.325129933663
0.480008 0.328285176721
0.488284 0.331462014574
0.49656 0.334659870822
0.504836 0.337878186728
0.513112 0.341116420663
0.521388 0.344374047574
0.529664 0.347650558456
0.53794 0.350945459849
0.546216 0.354258273343
0.554492 0.357588535098
0.562768 0.360935795382
0.571044 0.364299618117
0.57932 0.367679580443
0.587596 0.371075272296
0.595872 0.37448629599
0.604148 0.377912265826
0.612424 0.381352807703
0.6207 0.384807558741
0.628976 0.388276166924
0.637252 0.391758290743
0.645528 0.395253598865
0.653804 0.398761769796
0.66208 0.402282491568
0.670356 0.40581546143
0.678632 0.40936038555
0.686908 0.412916978729
0.695184 0.416484964121
0.70346 0.420064072965
0.711736 0.423654044325
0.720012 0.427254624837
0.728288 0.430865568467
0.736564 0.434486636278
0.74484 0.438117596198
0.753116 0.441758222807
0.761392 0.445408297118
0.769668 0.449067606379
0.777944 0.452735943869
0.78622 0.456413108712
0.794496 0.460098905687
0.802772 0.463793145053
0.811048 0.467495642377
0.819324 0.471206218362
0.8276 0.474924698694
0.835876 0.478650913878
0.844152 0.482384699095
0.852428 0.486125894051
0.860704 0.48987434284
0.86898 0.493629893808
0.877256 0.497392399421
0.885532 0.501161716137
0.893808 0.504937704289
0.902084 0.50872022796
0.91036 0.512509154874
0.918636 0.516304356283
0.926912 0.520105706859
0.935188 0.523913084596
0.943464 0.527726370705
0.95174 0.531545449519
0.960016 0.535370208403
0.968292 0.539200537658
0.976568 0.543036330442
0.984844 0.546877482676
0.99312 0.550723892971
1.001396 0.554575462547
1.009672 0.558432095152
1.017948 0.562293696997
1.026224 0.566160176676
1.0345 0.570031445105
1.042776 0.573907415449
1.051052 0.577788003062
1.059328 0.581673125421
1.067604 0.58556270207
1.07588 0.589456654558
1.084156 0.593354906382
1.092432 0.597257382937
1.100708 0.601164011459
1.108984 0.605074720973
1.11726 0.608989442247
1.125536 0.612908107743
1.133812 0.616830651568
1.142088 0.620757009431
1.150364 0.624687118599
1.15864 0.628620917857
1.166916 0.632558347461
1.175192 0.636499349106
1.183468 0.640443865881
1.191744 0.644391842238
1.20002 0.648343223949
1.208296 0.652297958077
1.216572 0.65625599294
1.224848 0.660217278078
1.233124 0.66418176422
1.2414 0.668149403255
1.249676 0.672120148204
1.257952 0.676093953185
1.266228 0.680070773391
1.274504 0.68405056506
1.28278 0.688033285447
1.291056 0.692018892803
1.299332 0.696007346345
1.307608 0.699998606236
1.315884 0.703992633559
1.32416 0.707989390296
1.332436 0.711988839304
1.340712 0.715990944295
1.348988 0.719995669816
1.357264 0.724002981226
1.36554 0.72801284468
1.373816 0.732025227109
1.382092 0.736040096198
1.390368 0.740057420375
1.398644 0.744077168785
1.40692 0.748099311282
1.415196 0.752123818406
1.423472 0.75615066137
1.431748 0.760179812046
1.440024 0.764211242944
1.4483 0.768244927206
1.456576 0.772280838585
1.464852 0.776318951433
1.473128 0.780359240689
1.481404 0.784401681866
1.48968 0.788446251036
1.497956 0.79249292482
1.506232 0.796541680376
1.514508 0.800592495386
1.522784 0.804645348047
1.53106 0.808700217055
1.539336 0.812757081602
1.547612 0.81681592136
1.555888 0.820876716471
1.564164 0.824939447542
1.57244 0.829004095628
1.580716 0.833070642231
1.588992 0.837139069285
1.597268 0.84120935915
1.605544 0.8452814946
1.61382 0.849355458822
1.622096 0.8534312354
1.630372 0.857508808313
1.638648 0.861588161921
1.646924 0.865669280966
1.6552 0.869752150559
1.663476 0.873836756173
1.671752 0.877923083638
1.680028 0.882011119136
1.688304 0.886100849189
1.69658 0.89019226066
1.704856 0.894285340739
1.713132 0.898380076946
1.721408 0.902476457116
1.729684 0.906574469401
1.73796 0.910674102258
1.746236 0.914775344451
1.754512 0.91887818504
1.762788 0.922982613376
1.771064 0.927088619101
1.77934 0.931196192139
1.787616 0.935305322692
1.795892 0.939416001238
1.804168 0.943528218522
1.812444 0.947641965556
1.82072 0.951757233614
1.828996 0.955874014227
1.837272 0.959992299179
1.845548 0.964112080503
1.853824 0.968233350479
1.8621 0.97235610163
1.870376 0.976480326716
1.878652 0.980606018735
1.886928 0.984733170915
1.895204 0.988861776713
1.90348 0.992991829815
1.911756 0.997123324126
1.920032 1.00125625377
1.928308 1.0053906131
1.936584 1.00952639667
1.94486 1.01366359925
1.953136 1.01780221582
1.961412 1.02194224156
1.969688 1.02608367187
1.977964 1.03022650234
1.98624 1.03437072875
1.994516 1.03851634711
2.002792 1.04266335359
2.011068 1.04681174458
2.019344 1.05096151663
2.02762 1.05511266652
2.035896 1.05926519118
2.044172 1.06341908775
2.052448 1.06757435354
2.060724 1.07173098604
2.069 1.07588898295
2.077276 1.08004834211
2.085552 1.08420906155
2.093828 1.0883711395
2.102104 1.09253457432
2.11038 1.09669936459
2.118656 1.10086550903
2.126932 1.10503300654
2.135208 1.10920185619
2.143484 1.11337205722
2.15176 1.11754360903
2.160036 1.12171651121
2.168312 1.12589076348
2.176588 1.13006636575
2.184864 1.13424331808
2.19314 1.1384216207
2.201416 1.14260127401
2.209692 1.14678227855
2.217968 1.15096463503
2.226244 1.15514834433
2.23452 1.15933340748
2.242796 1.16351982566
2.251072 1.16770760023
2.259348 1.17189673268
2.267624 1.17608722469
2.2759 1.18027907807
2.284176 1.18447229479
2.292452 1.18866687699
2.300728 1.19286282695
2.309004 1.19706014712
2.31728 1.20125884009
2.325556 1.20545890862
2.333832 1.20966035562
2.342108 1.21386318415
2.350384 1.21806739742
2.35866 1.22227299882
2.366936 1.22647999187
2.375212 1.23068838025
2.383488 1.2348981678
2.391764 1.23910935853
2.40004 1.24332195656
2.408316 1.24753596622
2.416592 1.25175139197
2.424868 1.25596823841
2.433144 1.26018651033
2.44142 1.26440621266
2.449696 1.26862735049
2.457972 1.27284992906
2.466248 1.27707395378
2.474524 1.28129943021
2.4828 1.28552636408
2.491076 1.28975476128
2.499352 1.29398462783
2.507628 1.29821596997
2.515904 1.30244879404
2.52418 1.30668310658
2.532456 1.3109189143
2.540732 1.31515622403
2.549008 1.31939504282
2.557284 1.32363537786
2.56556 1.32787723649
2.573836 1.33212062625
2.582112 1.33636555483
2.590388 1.34061203009
2.598664 1.34486006009
2.60694 1.34910965302
2.615216 1.35336081727
2.623492 1.35761356139
2.631768 1.36186789413
2.640044 1.36612382438
2.64832 1.37038136126
2.656596 1.37464051402
2.664872 1.37890129211
2.673148 1.38316370518
2.681424 1.38742776305
2.6897 1.39169347571
2.697976 1.39596085337
2.706252 1.40022990641
2.714528 1.4045006454
2.722804 1.40877308111
2.73108 1.4130472245
2.739356 1.41732308674
2.747632 1.42160067918
2.755908 1.42588001337
2.764184 1.43016110108
2.77246 1.43444395427
2.780736 1.43872858511
2.789012 1.44301500598
2.797288 1.44730322947
2.805564 1.45159326838
2.81384 1.45588513573
2.822116 1.46017884475
2.830392 1.46447440891
2.838668 1.46877184187
2.846944 1.47307115754
2.85522 1.47737237005
2.863496 1.48167549377
2.871772 1.48598054327
2.880048 1.4902875334
2.888324 1.49459647922
2.8966 1.49890739603
2.904876 1.50322029939
2.913152 1.5075352051
2.921428 1.51185212921
2.929704 1.51617108802
2.93798 1.52049209809
2.946256 1.52481517624
2.954532 1.52914033955
2.962808 1.53346760538
2.971084 1.53779699134
2.97936 1.54212851533
2.987636 1.54646219552
2.995912 1.55079805035
3.004188 1.55513609858
3.012464 1.55947635922
3.02074 1.56381885159
3.029016 1.56816359532
3.037292 1.5725106103
3.045568 1.57685991678
3.053844 1.58121153528
3.06212 1.58556548665
3.070396 1.58992179205
3.078672 1.59428047297
3.086948 1.59864155123
3.095224 1.60300504898
3.1035 1.60737098871
3.111776 1.61173939324
3.120052 1.61611028576
3.128328 1.62048368979
3.136604 1.62485962924
3.14488 1.62923812834
3.153156 1.63361921174
3.161432 1.63800290442
3.169708 1.64238923177
3.177984 1.64677821957
3.18626 1.65116989397
3.194536 1.65556428153
3.202812 1.65996140924
3.211088 1.66436130447
3.219364 1.66876399502
3.22764 1.67316950912
3.235916 1.67757787544
3.244192 1.68198912308
3.252468 1.68640328159
3.260744 1.69082038098
3.26902 1.69524045173
3.277296 1.69966352476
3.285572 1.70408963151
3.293848 1.70851880388
3.302124 1.71295107427
3.3104 1.7173864756
3.318676 1.72182504129
3.326952 1.72626680528
3.335228 1.73071180204
3.343504 1.7351600666
3.35178 1.73961163452
3.360056 1.74406654192
3.368332 1.74852482551
3.376608 1.75298652256
3.384884 1.75745167095
3.39316 1.76192030914
3.401436 1.76639247623
3.409712 1.77086821191
3.417988 1.77534755655
3.426264 1.77983055113
3.43454 1.78431723731
3.442816 1.78880765743
3.451092 1.79330185449
3.459368 1.79779987221
3.467644 1.80230175502
3.47592 1.80680754808
3.484196 1.81131729727
3.492472 1.81583104925
3.500748 1.82034885144
3.509024 1.82487075205
3.5173 1.82939680008
3.525576 1.83392704536
3.533852 1.83846153855
3.542128 1.84300033116
3.550404 1.84754347556
3.55868 1.85209102503
3.566956 1.85664303373
3.575232 1.86119955675
3.583508 1.86576065013
3.591784 1.87032637087
3.60006 1.87489677695
3.608336 1.87947192736
3.616612 1.8840518821
3.624888 1.88863670224
3.633164 1.89322644991
3.64144 1.89782118832
3.649716 1.90242098182
3.657992 1.90702589589
3.666268 1.91163599719
3.674544 1.91625135356
3.68282 1.92087203407
3.691096 1.92549810904
3.699372 1.93012965005
3.707648 1.93476673002
3.715924 1.93940942317
3.7242 1.94405780512
3.732476 1.94871195287
3.740752 1.95337194486
3.749028 1.95803786099
3.757304 1.96270978268
3.76558 1.96738779288
3.773856 1.9720719761
3.782132 1.97676241849
3.790408 1.98145920783
3.798684 1.98616243362
3.80696 1.99087218708
3.815236 1.9955885612
3.823512 2.00031165083
3.831788 2.00504155265
3.840064 2.0097783653
3.84834 2.01452218936
3.856616 2.01927312745
3.864892 2.02403128424
3.873168 2.02879676655
3.881444 2.03356968338
3.88972 2.03835014597
3.897996 2.04313826787
3.906272 2.04793416497
3.914548 2.05273795563
3.922824 2.05754976069
3.9311 2.06236970354
3.939376 2.06719791025
3.947652 2.07203450957
3.955928 2.07687963305
3.964204 2.08173341512
3.97248 2.08659599316
3.980756 2.09146750759
3.989032 2.09634810196
3.997308 2.10123792306
4.005584 2.10613712096
4.01386 2.11104584921
4.022136 2.11596426482
4.030412 2.12089252849
4.038688 2.12583080463
4.046964 2.13077926153
4.05524 2.13573807146
4.063516 2.1407074108
4.071792 2.14568746018
4.080068 2.15067840461
4.088344 2.15568043361
4.09662 2.16069374141
4.104896 2.16571852704
4.113172 2.17075499455
4.121448 2.17580335312
4.129724 2.18086381732


==> figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt1.tex <==
0.0 0.605594803453
0.0841218682305 0.613235310435
0.168243736461 0.634361835277
0.252365604692 0.666569449344
0.336487472922 0.707827951057
0.420609341153 0.756455185036
0.504731209383 0.811077930808
0.588853077614 0.87058740455
0.672974945844 0.934094898218
0.757096814075 1.00089109379
0.841218682305 1.07041079889
0.925340550536 1.14220355546
1.00946241877 1.2159097971
1.093584287 1.29124185818
1.17770615523 1.36796902637
1.26182802346 1.44590586331
1.34594989169 1.52490311557
1.43007175992 1.60484065494
1.51419362815 1.68562199873
1.59831549638 1.76717005797
1.68243736461 1.84942384149
1.76655923284 1.93233590749
1.85068110107 2.01587040448
1.9348029693 2.10000158212
2.01892483753 2.18471268268
2.10304670576 2.26999514747
2.18716857399 2.35584809115
2.27129044222 2.44227801205
2.35541231046 2.52929871959
2.43953417869 2.61693147127
2.52365604692 2.70520532317
2.60777791515 2.79415770932
2.69189978338 2.88383527882
2.77602165161 2.97429503606
2.86014351984 3.06560585041
2.94426538807 3.15785043081
3.0283872563 3.25112790156
3.11250912453 3.34555717486
3.19663099276 3.44128140503
3.28075286099 3.5384739467
3.36487472922 3.63734645869
3.44899659745 3.73816015646
3.53311846568 3.8412418354
3.61724033391 3.94700739859
3.70136220214 4.05599772794
3.78548407037 4.16893600065
3.8696059386 4.28682492682
3.95372780684 4.41112533599
4.03784967507 4.54412255633
4.1219715433 4.6898152272


==> figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt3.tex <==
0.0 1.08570849158
0.0608288216233 1.08825086988
0.121657643247 1.0956356355
0.18248646487 1.10751169183
0.243315286493 1.12354569781
0.304144108116 1.14342311879
0.36497292974 1.1668488905
0.425801751363 1.19354772739
0.486630572986 1.22326411521
0.54745939461 1.25576203277
0.608288216233 1.2908244506
0.669117037856 1.32825265423
0.72994585948 1.36786543744
0.790774681103 1.40949820728
0.851603502726 1.45300203818
0.912432324349 1.49824270655
0.973261145973 1.54509973272
1.0340899676 1.59346545139
1.09491878922 1.64324412736
1.15574761084 1.69435112928
1.21657643247 1.74671217083
1.27740525409 1.80026262613
1.33823407571 1.85494692423
1.39906289734 1.91071802632
1.45989171896 1.96753698869
1.52072054058 2.02537261429
1.58154936221 2.08420119664
1.64237818383 2.14400636048
1.70320700545 2.20477900588
1.76403582708 2.2665173648
1.8248646487 2.32922718281
1.88569347032 2.39292204339
1.94652229195 2.45762385887
2.00735111357 2.5233635609
2.06817993519 2.59018203573
2.12900875682 2.65813136692
2.18983757844 2.72727647306
2.25066640006 2.79769726443
2.31149522169 2.86949149729
2.37232404331 2.9427785886
2.43315286493 3.01770478695
2.49398168656 3.09445031383
2.55481050818 3.17323946063
2.6156393298 3.25435528802
2.67646815143 3.33816181825
2.73729697305 3.42513910868
2.79812579467 3.51594204339
2.85895461629 3.61150690545
2.91978343792 3.71326691868
2.98061225954 3.82366697785


==> figuresAndData/dataForRayleigh-conditionalMean-sigma2prob0pt6.tex <==
0.0 1.63820438154
0.0396220919817 1.63908128563
0.0792441839634 1.64167785387
0.118866275945 1.64594353725
0.158488367927 1.65182877612
0.198110459909 1.65928510572
0.23773255189 1.66826525469
0.277354643872 1.67872323684
0.316976735854 1.69061443623
0.356598827835 1.7038956858
0.396220919817 1.71852533991
0.435843011799 1.73446334133
0.475465103781 1.75167128304
0.515087195762 1.77011246577
0.554709287744 1.78975195175
0.594331379726 1.81055661574
0.633953471707 1.83249519419
0.673575563689 1.85553833357
0.713197655671 1.87965863919
0.752819747653 1.90483072568
0.792441839634 1.93103127066
0.832063931616 1.95823907341
0.871686023598 1.98643512017
0.911308115579 2.01560265855
0.950930207561 2.04572728332
0.990552299543 2.07679703678
1.03017439152 2.10880252714
1.06979648351 2.14173706919
1.10941857549 2.17559685262
1.14904066747 2.21038114423
1.18866275945 2.2460925324
1.22828485143 2.28273722394
1.26790694341 2.32032540663
1.3075290354 2.35887169484
1.34715112738 2.39839568097
1.38677321936 2.43892262372
1.42639531134 2.48048431521
1.46601740332 2.5231201858
1.50563949531 2.56687873004
1.54526158729 2.61181937537
1.58488367927 2.65801497506
1.62450577125 2.70555520467
1.66412786323 2.75455130708
1.70374995521 2.80514292455
1.7433720472 2.85750830585
1.78299413918 2.91188027362
1.82261623116 2.96857271847
1.86223832314 3.02802813457
1.90186041512 3.09091275886
1.9414825071 3.15834132813


==> figuresAndData/dataForRayleigh-conditionalMean-sigma2pt01.tex <==
0.0 0.605594803453
0.0841218682305 0.613235310435
0.168243736461 0.634361835277
0.252365604692 0.666569449344
0.336487472922 0.707827951057
0.420609341153 0.756455185036
0.504731209383 0.811077930808
0.588853077614 0.87058740455
0.672974945844 0.934094898218
0.757096814075 1.00089109379
0.841218682305 1.07041079889
0.925340550536 1.14220355546
1.00946241877 1.2159097971
1.093584287 1.29124185818
1.17770615523 1.36796902637
1.26182802346 1.44590586331
1.34594989169 1.52490311557
1.43007175992 1.60484065494
1.51419362815 1.68562199873
1.59831549638 1.76717005797
1.68243736461 1.84942384149
1.76655923284 1.93233590749
1.85068110107 2.01587040448
1.9348029693 2.10000158212
2.01892483753 2.18471268268
2.10304670576 2.26999514747
2.18716857399 2.35584809115
2.27129044222 2.44227801205
2.35541231046 2.52929871959
2.43953417869 2.61693147127
2.52365604692 2.70520532317
2.60777791515 2.79415770932
2.69189978338 2.88383527882
2.77602165161 2.97429503606
2.86014351984 3.06560585041
2.94426538807 3.15785043081
3.0283872563 3.25112790156
3.11250912453 3.34555717486
3.19663099276 3.44128140503
3.28075286099 3.5384739467
3.36487472922 3.63734645869
3.44899659745 3.73816015646
3.53311846568 3.8412418354
3.61724033391 3.94700739859
3.70136220214 4.05599772794
3.78548407037 4.16893600065
3.8696059386 4.28682492682
3.95372780684 4.41112533599
4.03784967507 4.54412255633
4.1219715433 4.6898152272


==> figuresAndData/dataForRayleigh-conditionalMean-sigma4prob0pt3.tex <==
0.0 2.17141698317
0.121657643247 2.17650173976
0.243315286493 2.19127127099
0.36497292974 2.21502338366
0.486630572986 2.24709139562
0.608288216233 2.28684623758
0.72994585948 2.33369778099
0.851603502726 2.38709545478
0.973261145973 2.44652823043
1.09491878922 2.51152406553
1.21657643247 2.58164890119
1.33823407571 2.65650530847
1.45989171896 2.73573087487
1.58154936221 2.81899641457
1.70320700545 2.90600407636
1.8248646487 2.9964854131
1.94652229195 3.09019946544
2.06817993519 3.18693090279
2.18983757844 3.28648825473
2.31149522169 3.38870225856
2.43315286493 3.49342434165
2.55481050818 3.60052525225
2.67646815143 3.70989384846
2.79812579467 3.82143605265
2.91978343792 3.93507397737
3.04144108116 4.05074522858
3.16309872441 4.16840239329
3.28475636766 4.28801272096
3.4064140109 4.40955801176
3.52807165415 4.5330347296
3.6497292974 4.65845436562
3.77138694064 4.78584408678
3.89304458389 4.91524771775
4.01470222714 5.0467271218
4.13635987038 5.18036407146
4.25801751363 5.31626273384
4.37967515688 5.45455294613
4.50133280012 5.59539452886
4.62299044337 5.73898299459
4.74464808662 5.88555717721
4.86630572986 6.0354095739
4.98796337311 6.18890062767
5.10962101636 6.34647892127
5.2312786596 6.50871057604
5.35293630285 6.6763236365
5.4745939461 6.85027821737
5.59625158934 7.03188408677
5.71790923259 7.2230138109
5.83956687584 7.42653383736
5.96122451908 7.6473339557


==> figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt3.tex <==
0.0 4.34283396634
0.243315286493 4.35300347952
0.486630572986 4.38254254198
0.72994585948 4.43004676732
0.973261145973 4.49418279124
1.21657643247 4.57369247516
1.45989171896 4.66739556198
1.70320700545 4.77419090956
1.94652229195 4.89305646085
2.18983757844 5.02304813106
2.43315286493 5.16329780239
2.67646815143 5.31301061694
2.91978343792 5.47146174974
3.16309872441 5.63799282914
3.4064140109 5.81200815273
3.6497292974 5.9929708262
3.89304458389 6.18039893089
4.13635987038 6.37386180558
4.37967515688 6.57297650946
4.62299044337 6.77740451712
4.86630572986 6.98684868331
5.10962101636 7.20105050451
5.35293630285 7.41978769691
5.59625158934 7.6428721053
5.83956687584 7.87014795475
6.08288216233 8.10149045717
6.32619744882 8.33680478657
6.56951273532 8.57602544193
6.81282802181 8.81911602352
7.0561433083 9.0660694592
7.2994585948 9.31690873124
7.54277388129 9.57168817357
7.78608916778 9.83049543549
8.02940445428 10.0934542436
8.27271974077 10.3607281429
8.51603502726 10.6325254677
8.75935031375 10.9091058923
9.00266560025 11.1907890577
9.24598088674 11.4779659892
9.48929617323 11.7711143544
9.73261145973 12.0708191478
9.97592674622 12.3778012553
10.2192420327 12.6929578425
10.4625573192 13.0174211521
10.7058726057 13.352647273
10.9491878922 13.7005564347
11.1925031787 14.0637681735
11.4358184652 14.4460276218
11.6791337517 14.8530676747
11.9224490382 15.2946679114


==> figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt6.tex <==
0.0 6.55281752616
0.158488367927 6.55632514251
0.316976735854 6.5667114155
0.475465103781 6.58377414899
0.633953471707 6.60731510449
0.792441839634 6.63714042289
0.950930207561 6.67306101876
1.10941857549 6.71489294736
1.26790694341 6.76245774493
1.42639531134 6.81558274319
1.58488367927 6.87410135965
1.7433720472 6.93785336531
1.90186041512 7.00668513216
2.06034878305 7.08044986307
2.21883715098 7.15900780699
2.3773255189 7.24222646296
2.53581388683 7.32998077675
2.69430225476 7.42215333429
2.85279062268 7.51863455678
3.01127899061 7.6193229027
3.16976735854 7.72412508263
3.32825572646 7.83295629362
3.48674409439 7.94574048069
3.64523246232 8.06241063421
3.80372083024 8.18290913329
3.96220919817 8.30718814714
4.1206975661 8.43521010855
4.27918593403 8.56694827678
4.43767430195 8.70238741049
4.59616266988 8.84152457693
4.75465103781 8.98437012961
4.91313940573 9.13094889574
5.07162777366 9.28130162652
5.23011614159 9.43548677935
5.38860450951 9.59358272387
5.54709287744 9.75569049486
5.70558124537 9.92193726084
5.86406961329 10.0924807432
6.02255798122 10.2675149202
6.18104634915 10.4472775015
6.33953471707 10.6320599002
6.498023085 10.8222208187
6.65651145293 11.0182052283
6.81499982086 11.2205716982
6.97348818878 11.4300332234
7.13197655671 11.6475210945
7.29046492464 11.8742908739
7.44895329256 12.1121125383
7.60744166049 12.3636510354
7.76593002842 12.6333653125


==> figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt7.tex <==
0.0 7.2741317407
0.132433347565 7.27654448121
0.26486669513 7.28371439829
0.397300042696 7.29554031459
0.529733390261 7.31192292338
0.662166737826 7.33276495201
0.794600085391 7.35797132256
0.927033432956 7.38744930949
1.05946678052 7.42110869487
1.19190012809 7.45886192129
1.32433347565 7.50062424321
1.45676682322 7.54631387722
1.58920017078 7.59585215231
1.72163351835 7.64916366101
1.85406686591 7.70617641277
1.98650021348 7.76682199095
2.11893356104 7.83103571529
2.25136690861 7.89875681174
2.38380025617 7.96992859213
2.51623360374 8.04449864641
2.6486669513 8.12241905066
2.78110029887 8.20364659477
2.91353364643 8.28814303423
3.045966994 8.37587537146
3.17840034157 8.46681617308
3.31083368913 8.56094393085
3.4432670367 8.65824347582
3.57570038426 8.75870645713
3.70813373183 8.8623318999
3.84056707939 8.96912685998
3.97300042696 9.07910719826
4.10543377452 9.19229850326
4.23786712209 9.30873719923
4.37030046965 9.42847188842
4.50273381722 9.55156499178
4.63516716478 9.67809477499
4.76760051235 9.80815787798
4.90003385991 9.94187251297
5.03246720748 10.0793825651
5.16490055504 10.2208629362
5.29733390261 10.3665266386
5.42976725017 10.5166344194
5.56220059774 10.6715081561
5.6946339453 10.8315500793
5.82706729287 10.9972714042
5.95950064043 11.169336996
6.091933988 11.3486392867
6.22436733556 11.5364305719
6.35680068313 11.7345871752
6.4892340307 11.9462321295


==> figuresAndData/dataForRayleigh-conditionalMean-sigma8prob0pt8.tex <==
0.0 8.03256415469
0.104749805795 8.03409467573
0.20949961159 8.03865676714
0.314249417386 8.04620690425
0.418999223181 8.0567025351
0.523749028976 8.07010213233
0.628498834771 8.08636524743
0.733248640566 8.10545256746
0.837998446361 8.12732597447
0.942748252157 8.1519486077
1.04749805795 8.17928492919
1.15224786375 8.20930079279
1.25699766954 8.24196351731
1.36174747534 8.27724196437
1.46649728113 8.31510662138
1.57124708693 8.35552969073
1.67599689272 8.398485186
1.78074669852 8.44394903626
1.88549650431 8.49189919989
1.99024631011 8.54231578942
2.0949961159 8.5951812092
2.1997459217 8.65048030826
2.30449572749 8.70820055087
2.40924553329 8.768332208
2.51399533908 8.83086857362
2.61874514488 8.89580621048
2.72349495067 8.963145231
2.82824475647 9.0328896206
2.93299456226 9.10504761195
3.03774436806 9.17963212148
3.14249417386 9.2566612618
3.24724397965 9.33615894817
3.35199378545 9.41815562178
3.45674359124 9.5026891202
3.56149339704 9.58980573483
3.66624320283 9.67956150906
3.77099300863 9.77202385052
3.87574281442 9.86727355948
3.98049262022 9.96540741822
4.08524242601 10.0665415516
4.18999223181 10.1708158721
4.2947420376 10.2784000905
4.3994918434 10.3895020555
4.50424164919 10.5043796894
4.60899145499 10.62335872
4.71374126078 10.7468602778
4.81849106658 10.8754464697
4.92324087237 11.0099017872
5.02799067817 11.1513953717
5.13274048396 11.3018629034


==> figuresAndData/dataForRayleigh-conditionalMean.tex <==
0.0 0.302797401727
0.00853 0.302838892665
0.01706 0.302962344457
0.02559 0.303166234883
0.03412 0.303449061498
0.04265 0.303809341765
0.05118 0.304245613172
0.05971 0.304756433327
0.06824 0.305340380053
0.07677 0.305996051452
0.0853 0.306722065965
0.09383 0.307517062411
0.10236 0.308379700019
0.11089 0.309308658437
0.11942 0.310302637733
0.12795 0.311360358381
0.13648 0.312480561235
0.14501 0.313662007486
0.15354 0.314903478613
0.16207 0.316203776311
0.1706 0.31756172242
0.17913 0.318976158834
0.18766 0.3204459474
0.19619 0.321969969808
0.20472 0.323547127468
0.21325 0.32517634138
0.22178 0.326856551995
0.23031 0.328586719061
0.23884 0.330365821467
0.24737 0.332192857074
0.2559 0.334066842541
0.26443 0.335986813145
0.27296 0.337951822587
0.28149 0.339960942801
0.29002 0.342013263746
0.29855 0.344107893207
0.30708 0.346243956575
0.31561 0.348420596631
0.32414 0.350636973327
0.33267 0.352892263555
0.3412 0.355185660923
0.34973 0.357516375516
0.35826 0.359883633666
0.36679 0.362286677708
0.37532 0.364724765745
0.38385 0.367197171403
0.39238 0.369703183585
0.40091 0.372242106231
0.40944 0.374813258071
0.41797 0.377415972375
0.4265 0.380049596712
0.43503 0.382713492699
0.44356 0.385407035759
0.45209 0.388129614872
0.46062 0.390880632331
0.46915 0.3936595035
0.47768 0.396465656568
0.48621 0.399298532312
0.49474 0.402157583853
0.50327 0.405042276422
0.5118 0.40795208712
0.52033 0.410886504689
0.52886 0.413845029275
0.53739 0.416827172203
0.54592 0.419832455748
0.55445 0.42286041291
0.56298 0.425910587197
0.57151 0.4289825324
0.58004 0.43207581238
0.58857 0.435190000857
0.5971 0.438324681197
0.60563 0.441479446205
0.61416 0.444653897924
0.62269 0.447847647434
0.63122 0.45106031465
0.63975 0.454291528134
0.64828 0.457540924901
0.65681 0.46080815023
0.66534 0.464092857483
0.67387 0.467394707922
0.6824 0.470713370531
0.69093 0.474048521842
0.69946 0.477399845765
0.70799 0.480767033417
0.71652 0.484149782962
0.72505 0.487547799444
0.73358 0.490960794633
0.74211 0.494388486871
0.75064 0.497830600915
0.75917 0.501286867793
0.7677 0.504757024657
0.77623 0.508240814641
0.78476 0.51173798672
0.79329 0.515248295577
0.80182 0.518771501466
0.81035 0.522307370085
0.81888 0.525855672444
0.82741 0.529416184745
0.83594 0.532988688259
0.84447 0.536572969204
0.853 0.540168818633
0.86153 0.543776032315
0.87006 0.547394410631
0.87859 0.551023758459
0.88712 0.554663885071
0.89565 0.558314604029
0.90418 0.561975733087
0.91271 0.565647094085
0.92124 0.56932851286
0.92977 0.573019819151
0.9383 0.576720846503
0.94683 0.580431432182
0.95536 0.584151417085
0.96389 0.587880645656
0.97242 0.591618965803
0.98095 0.595366228818
0.98948 0.599122289295
0.99801 0.602887005054
1.00654 0.606660237069
1.01507 0.610441849388
1.0236 0.614231709069
1.03213 0.618029686104
1.04066 0.621835653355
1.04919 0.625649486486
1.05772 0.629471063898
1.06625 0.633300266666
1.07478 0.63713697848
1.08331 0.64098108558
1.09184 0.644832476703
1.10037 0.648691043022
1.1089 0.652556678093
1.11743 0.656429277798
1.12596 0.660308740298
1.13449 0.664194965972
1.14302 0.668087857378
1.15155 0.671987319194
1.16008 0.675893258178
1.16861 0.679805583117
1.17714 0.683724204784
1.18567 0.687649035892
1.1942 0.691579991052
1.20273 0.695516986733
1.21126 0.699459941218
1.21979 0.703408774564
1.22832 0.707363408568
1.23685 0.711323766722
1.24538 0.715289774183
1.25391 0.719261357733
1.26244 0.723238445744
1.27097 0.727220968146
1.2795 0.731208856392
1.28803 0.735202043427
1.29656 0.739200463655
1.30509 0.743204052908
1.31362 0.747212748418
1.32215 0.751226488786
1.33068 0.755245213954
1.33921 0.759268865177
1.34774 0.763297384996
1.35627 0.767330717212
1.3648 0.77136880686
1.37333 0.775411600184
1.38186 0.779459044613
1.39039 0.783511088734
1.39892 0.787567682275
1.40745 0.791628776078
1.41598 0.795694322075
1.42451 0.799764273272
1.43304 0.803838583725
1.44157 0.807917208519
1.4501 0.812000103751
1.45863 0.816087226506
1.46716 0.820178534843
1.47569 0.824273987773
1.48422 0.828373545243
1.49275 0.832477168118
1.50128 0.836584818164
1.50981 0.840696458032
1.51834 0.844812051239
1.52687 0.848931562157
1.5354 0.853054955993
1.54393 0.857182198778
1.55246 0.861313257349
1.56099 0.865448099338
1.56952 0.869586693155
1.57805 0.873729007976
1.58658 0.877875013731
1.59511 0.882024681089
1.60364 0.886177981449
1.61217 0.890334886924
1.6207 0.89449537033
1.62923 0.898659405176
1.63776 0.902826965653
1.64629 0.906998026622
1.65482 0.911172563602
1.66335 0.915350552765
1.67188 0.919531970917
1.68041 0.923716795498
1.68894 0.927905004567
1.69747 0.932096576793
1.706 0.936291491446
1.71453 0.940489728391
1.72306 0.944691268076
1.73159 0.948896091526
1.74012 0.953104180335
1.74865 0.957315516656
1.75718 0.961530083195
1.76571 0.965747863204
1.77424 0.969968840473
1.78277 0.974192999323
1.7913 0.978420324601
1.79983 0.982650801671
1.80836 0.986884416408
1.81689 0.991121155195
1.82542 0.99536100491
1.83395 0.999603952931
1.84248 1.00384998712
1.85101 1.00809909582
1.85954 1.01235126786
1.86807 1.01660649253
1.8766 1.02086475959
1.88513 1.02512605928
1.89366 1.02939038227
1.90219 1.0336577197
1.91072 1.03792806316
1.91925 1.04220140469
1.92778 1.04647773676
1.93631 1.05075705228
1.94484 1.05503934459
1.95337 1.05932460748
1.9619 1.06361283514
1.97043 1.0679040222
1.97896 1.07219816372
1.98749 1.07649525516
1.99602 1.08079529239
2.00455 1.08509827172
2.01308 1.08940418985
2.02161 1.09371304388
2.03014 1.09802483133
2.03867 1.10233955013
2.0472 1.10665719858
2.05573 1.11097777542
2.06426 1.11530127975
2.07279 1.11962771108
2.08132 1.12395706933
2.08985 1.12828935478
2.09838 1.13262456813
2.10691 1.13696271046
2.11544 1.14130378323
2.12397 1.14564778831
2.1325 1.14999472792
2.14103 1.15434460471
2.14956 1.15869742169
2.15809 1.16305318225
2.16662 1.16741189019
2.17515 1.17177354967
2.18368 1.17613816525
2.19221 1.18050574187
2.20074 1.18487628486
2.20927 1.18924979991
2.2178 1.19362629313
2.22633 1.198005771
2.23486 1.20238824037
2.24339 1.20677370851
2.25192 1.21116218305
2.26045 1.21555367202
2.26898 1.21994818384
2.27751 1.2243457273
2.28604 1.22874631163
2.29457 1.23314994639
2.3031 1.23755664158
2.31163 1.24196640759
2.32016 1.24637925519
2.32869 1.25079519555
2.33722 1.25521424027
2.34575 1.25963640131
2.35428 1.26406169108
2.36281 1.26849012236
2.37134 1.27292170836
2.37987 1.2773564627
2.3884 1.28179439941
2.39693 1.28623553294
2.40546 1.29067987816
2.41399 1.29512745038
2.42252 1.2995782653
2.43105 1.30403233909
2.43958 1.30848968833
2.44811 1.31295033004
2.45664 1.31741428168
2.46517 1.32188156116
2.4737 1.32635218684
2.48223 1.33082617753
2.49076 1.33530355249
2.49929 1.33978433145
2.50782 1.3442685346
2.51635 1.3487561826
2.52488 1.35324729658
2.53341 1.35774189818
2.54194 1.36224000949
2.55047 1.36674165309
2.559 1.37124685209
2.56753 1.37575563008
2.57606 1.38026801114
2.58459 1.3847840199
2.59312 1.38930368148
2.60165 1.39382702155
2.61018 1.39835406629
2.61871 1.40288484243
2.62724 1.40741937725
2.63577 1.41195769857
2.6443 1.4164998348
2.65283 1.42104581487
2.66136 1.42559566833
2.66989 1.4301494253
2.67842 1.43470711648
2.68695 1.43926877318
2.69548 1.44383442733
2.70401 1.44840411145
2.71254 1.45297785872
2.72107 1.45755570293
2.7296 1.46213767852
2.73813 1.46672382061
2.74666 1.47131416496
2.75519 1.47590874802
2.76372 1.4805076069
2.77225 1.48511077946
2.78078 1.48971830422
2.78931 1.49433022045
2.79784 1.49894656814
2.80637 1.50356738803
2.8149 1.50819272162
2.82343 1.51282261118
2.83196 1.51745709975
2.84049 1.5220962312
2.84902 1.52674005017
2.85755 1.53138860217
2.86608 1.53604193351
2.87461 1.54070009139
2.88314 1.54536312386
2.89167 1.55003107987
2.9002 1.55470400927
2.90873 1.55938196282
2.91726 1.56406499224
2.92579 1.56875315019
2.93432 1.57344649032
2.94285 1.57814506725
2.95138 1.58284893664
2.95991 1.58755815518
2.96844 1.59227278059
2.97697 1.59699287168
2.9855 1.60171848837
2.99403 1.60644969168
3.00256 1.61118654378
3.01109 1.61592910801
3.01962 1.62067744889
3.02815 1.62543163217
3.03668 1.63019172482
3.04521 1.63495779509
3.05374 1.63972991254
3.06227 1.64450814803
3.0708 1.64929257378
3.07933 1.6540832634
3.08786 1.6588802919
3.09639 1.66368373575
3.10492 1.66849367289
3.11345 1.67331018277
3.12198 1.67813334638
3.13051 1.68296324632
3.13904 1.68779996677
3.14757 1.69264359359
3.1561 1.69749421435
3.16463 1.70235191832
3.17316 1.70721679659
3.18169 1.71208894204
3.19022 1.71696844943
3.19875 1.72185541544
3.20728 1.72674993871
3.21581 1.73165211988
3.22434 1.73656206166
3.23287 1.74147986886
3.2414 1.74640564849
3.24993 1.75133950976
3.25846 1.75628156416
3.26699 1.76123192555
3.27552 1.76619071015
3.28405 1.77115803671
3.29258 1.77613402647
3.30111 1.78111880329
3.30964 1.78611249371
3.31817 1.79111522704
3.3267 1.79612713539
3.33523 1.80114835379
3.34376 1.80617902028
3.35229 1.81121927596
3.36082 1.8162692651
3.36935 1.82132913523
3.37788 1.82639903725
3.38641 1.8314791255
3.39494 1.83656955789
3.40347 1.841670496
3.412 1.84678210519
3.42053 1.85190455472
3.42906 1.85703801786
3.43759 1.86218267203
3.44612 1.86733869895
3.45465 1.87250628471
3.46318 1.87768562001
3.47171 1.88287690023
3.48024 1.8880803256
3.48877 1.89329610142
3.4973 1.89852443814
3.50583 1.90376555162
3.51436 1.90901966324
3.52289 1.91428700016
3.53142 1.9195677955
3.53995 1.92486228851
3.54848 1.93017072485
3.55701 1.9354933568
3.56554 1.9408304435
3.57407 1.9461822512
3.5826 1.95154905353
3.59113 1.95693113179
3.59966 1.96232877525
3.60819 1.96774228142
3.61672 1.97317195643
3.62525 1.97861811533
3.63378 1.98408108247
3.64231 1.98956119186
3.65084 1.99505878761
3.65937 2.0005742243
3.6679 2.00610786746
3.67643 2.01166009402
3.68496 2.01723129283
3.69349 2.02282186515
3.70202 2.02843222524
3.71055 2.03406280091
3.71908 2.03971403418
3.72761 2.04538638192
3.73614 2.05108031656
3.74467 2.05679632682
3.7532 2.06253491852
3.76173 2.06829661541
3.77026 2.07408196009
3.77879 2.07989151494
3.78732 2.08572586317
3.79585 2.09158560988
3.80438 2.09747138327
3.81291 2.10338383586
3.82144 2.10932364587
3.82997 2.1152915186
3.8385 2.12128818807
3.84703 2.12731441858
3.85556 2.13337100662
3.86409 2.13945878272
3.87262 2.1455786136
3.88115 2.1517314044
3.88968 2.15791810118
3.89821 2.16413969356
3.90674 2.17039721764
3.91527 2.17669175914
3.9238 2.18302445688
3.93233 2.18939650654
3.94086 2.19580916479
3.94939 2.20226375383
3.95792 2.2087616664
3.96645 2.21530437125
3.97498 2.22189341928
3.98351 2.22853045023
3.99204 2.23521720022
4.00057 2.24195551005
4.0091 2.2487473346
4.01763 2.25559475321
4.02616 2.26249998151
4.03469 2.26946538464
4.04322 2.27649349234
4.05175 2.28358701601
4.06028 2.29074886824
4.06881 2.29798218527
4.07734 2.30529035274
4.08587 2.31267703569
4.0944 2.32014621337
4.10293 2.32770222018
4.11146 2.3353497939
4.11999 2.34309413299
4.12852 2.3509409653
4.13705 2.358896631
4.14558 2.36696818371
4.15411 2.37516351512
4.16264 2.38349151024
4.17117 2.39196224345
4.1797 2.40058722963
4.18823 2.40937975111
4.19676 2.41835529169
4.20529 2.42753212527
4.21382 2.43693213509
4.22235 2.44658198918
4.23088 2.45651489019
4.23941 2.46677330155
4.24794 2.47741344742
4.25647 2.48851332698


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1.tex <==
0.0 0.23451626127
0.00488 0.234567541235
0.00976 0.23474276739
0.01464 0.234992242008
0.01952 0.235329247628
0.0244 0.235766127298
0.02928 0.236314681523
0.03416 0.236953280993
0.03904 0.237659176776
0.04392 0.238476341162
0.0488 0.239382015299
0.05368 0.240352571364
0.05856 0.24143406032
0.06344 0.242604062975
0.06832 0.243875958703
0.0732 0.245190726867
0.07808 0.24663709355
0.08296 0.248157560755
0.08784 0.249730573232
0.09272 0.251414128952
0.0976 0.253190590188
0.10248 0.25504213292
0.10736 0.256950674281
0.11224 0.258941668008
0.11712 0.261044483212
0.122 0.263200737445
0.12688 0.26539470928
0.13176 0.267707469761
0.13664 0.270080809563
0.14152 0.272502642126
0.1464 0.27501350327
0.15128 0.277605783396
0.15616 0.280272228613
0.16104 0.282948682417
0.16592 0.285741412103
0.1708 0.288527891352
0.17568 0.291421800181
0.18056 0.294358701078
0.18544 0.297399780254
0.19032 0.300409630976
0.1952 0.303518697528
0.20008 0.306656879739
0.20496 0.309895701567
0.20984 0.313162013977
0.21472 0.316453576915
0.2196 0.319768623142
0.22448 0.323190531462
0.22936 0.326551874631
0.23424 0.330024541029
0.23912 0.333524453525
0.244 0.337052771289
0.24888 0.340709973832
0.25376 0.344304092779
0.25864 0.347933907554
0.26352 0.351603140091
0.2684 0.355316212204
0.27328 0.359078269757
0.27816 0.362895206912
0.28304 0.366651595407
0.28792 0.370469571743
0.2928 0.374357131213
0.29768 0.378189596996
0.30256 0.382102179952
0.30744 0.386105170073
0.31232 0.39006395455
0.3172 0.393977763149
0.32208 0.398000675967
0.32696 0.402146129151
0.33184 0.406101319441
0.33672 0.410190073439
0.3416 0.414255092519
0.34648 0.418476554819
0.35136 0.422505932574
0.35624 0.426707562517
0.36112 0.430907159969
0.366 0.435108959141
0.37088 0.439317672055
0.37576 0.443538499571
0.38064 0.447777142149
0.38552 0.451818536679
0.3904 0.456106064359
0.39528 0.460431497823
0.40016 0.464802637604
0.40504 0.468982299762
0.40992 0.473464111836
0.4148 0.477759907302
0.41968 0.482124926906
0.42456 0.486297855331
0.42944 0.49082597386
0.43432 0.495170515425
0.4392 0.499614814985
0.44408 0.503871702436
0.44896 0.508239111879
0.45384 0.512730271282
0.45872 0.517359035462
0.4636 0.521810619015
0.46848 0.526076949851
0.47336 0.530494747333
0.47824 0.535079718674
0.48312 0.539487322303
0.488 0.544079066469
0.49288 0.548494851529
0.49776 0.553113196393
0.50264 0.557557987725
0.50752 0.562225234235
0.5124 0.566722351744
0.51728 0.571042570112
0.52216 0.575608851565
0.52704 0.580002872981
0.53192 0.58466627477
0.5368 0.589163118325
0.54168 0.593954193188
0.54656 0.598585486469
0.55144 0.603051111163
0.55632 0.607841283009
0.5612 0.612473848343
0.56608 0.616943224632
0.57096 0.621243820215
0.57584 0.625906588551
0.58072 0.630957098724
0.5856 0.635306695126
0.59048 0.640054716618
0.59536 0.644649277237
0.60024 0.649085433683
0.60512 0.65395880838
0.61 0.65868600366
0.61488 0.663262409231
0.61976 0.667683418623
0.62464 0.672589855656
0.62952 0.677354665742
0.6344 0.681973580121
0.63928 0.686442337605
0.64416 0.691448666492
0.64904 0.695616262957
0.65392 0.700336960451
0.6588 0.70564284535
0.66368 0.710086261359
0.66856 0.714379198432
0.67344 0.719282660988
0.67832 0.724052904995
0.6832 0.728686379476
0.68808 0.733982197413
0.69296 0.73834432057
0.69784 0.743387509917
0.70272 0.747464640695
0.7076 0.752241997747
0.71248 0.756888102661
0.71736 0.762280497125
0.72224 0.766667961567
0.72712 0.771822267259
0.732 0.775938953407
0.73688 0.780843450101
0.74176 0.785625522444
0.74664 0.790282380315
0.75152 0.794811253342
0.7564 0.800198983842
0.76128 0.804477631474
0.76616 0.809637794845
0.77104 0.814687422476
0.77592 0.819624073641
0.7808 0.824445327159
0.78568 0.829148782182
0.79056 0.833732058974
0.79544 0.838192799682
0.80032 0.842528669105
0.8052 0.847869863037
0.81008 0.853110900814
0.81496 0.857087823293
0.81984 0.862107551696
0.82472 0.867020883691
0.8296 0.87182580042
0.83448 0.876520304328
0.83936 0.881102419774
0.84424 0.886821551699
0.84912 0.891188149622
0.854 0.895436617409
0.85888 0.900861852294
0.86376 0.906195676119
0.86864 0.910109103926
0.87352 0.915239696268
0.8784 0.920273778917
0.88328 0.925209706558
0.88816 0.930045854436
0.89304 0.934780618816
0.89792 0.939412417439
0.9028 0.943939689971
0.90768 0.949811657019
0.91256 0.954140859346
0.91744 0.958361015202
0.92232 0.963968197045
0.9272 0.967981515209
0.93208 0.973410305399
0.93696 0.978755679868
0.94184 0.982456118863
0.94672 0.987614999415
0.9516 0.992686525476
0.95648 0.99766942699
0.96136 1.00256245303
0.96624 1.00736437211
0.97112 1.01207397249
0.976 1.01669006249
0.98088 1.02289746833
0.98576 1.02733878195
0.99064 1.0316831297
0.99552 1.03592940104
1.0004 1.04182541591
1.00528 1.04588800055
1.01016 1.051629606
1.01504 1.05550427342
1.01992 1.06108726659
1.0248 1.06659724353
1.02968 1.07019026193
1.03456 1.07553556965
1.03944 1.08080488156
1.04432 1.08599723009
1.0492 1.09111166374
1.05408 1.09614724726
1.05896 1.10110306181
1.06384 1.1059782052
1.06872 1.11077179203
1.0736 1.11548295389
1.07848 1.12011083951
1.08336 1.12465461491
1.08824 1.12911346362
1.09312 1.13552999819
1.098 1.13983176766
1.10288 1.14404621937
1.10776 1.1502613166
1.11264 1.15431391345
1.11752 1.16039560144
1.1224 1.16428328356
1.12728 1.17022834649
1.13216 1.17394817972
1.13704 1.17975351368
1.14192 1.18330269158
1.1468 1.18896530661
1.15168 1.19456273033
1.15656 1.19785817431
1.16144 1.20330854258
1.16632 1.20869151072
1.1712 1.21400634461
1.17608 1.21925232254
1.18096 1.22442873532
1.18584 1.22953488636
1.19072 1.23457009181
1.1956 1.23953368062
1.20048 1.24442499466
1.20536 1.24924338881
1.21024 1.25398823103
1.21512 1.25865890245
1.22 1.26325479749
1.22488 1.26777532387
1.22976 1.27221990272
1.23464 1.27904423004
1.23952 1.28334823694
1.2444 1.2875745416
1.24928 1.29421757647
1.25416 1.29829961489
1.25904 1.30230230988
1.26392 1.3087579081
1.2688 1.31261285736
1.27368 1.31894431282
1.27856 1.32264924494
1.28344 1.32885389522
1.28832 1.33240663297
1.2932 1.3384818985
1.29808 1.34188035982
1.30296 1.3478237451
1.30784 1.35370600761
1.31272 1.35687503873
1.3176 1.36262171677
1.32248 1.36830528486
1.32736 1.37392505866
1.33224 1.37948036285
1.33712 1.38226430073
1.342 1.38767809401
1.34688 1.39302557636
1.35176 1.39830611063
1.35664 1.40351906912
1.36152 1.40866383358
1.3664 1.41373979536
1.37128 1.4187463554
1.37616 1.42368292438
1.38104 1.42854892272
1.38592 1.43334378068
1.3908 1.43806693841
1.39568 1.44271784597
1.40056 1.44729596347
1.40544 1.45464291764
1.41032 1.4590825376
1.4152 1.46344766307
1.42008 1.46773779368
1.42496 1.47482834214
1.42984 1.47897509842
1.43472 1.48304527147
1.4396 1.48993805531
1.44448 1.49386131826
1.44936 1.50062122421
1.45424 1.50439521278
1.45912 1.5080901164
1.464 1.5146417296
1.46888 1.51818410652
1.47376 1.5245957872
1.47864 1.53093972186
1.48352 1.5342524502
1.4884 1.54045218121
1.49328 1.54360693152
1.49816 1.54965980503
1.50304 1.55564114145
1.50792 1.56155014471
1.5128 1.56438850538
1.51768 1.57014524247
1.52256 1.5758274713
1.52744 1.58143443081
1.53232 1.58696536878
1.5372 1.59241954192
1.54208 1.59476962755
1.54696 1.60006380982
1.55184 1.60527921644
1.55672 1.61041514108
1.5616 1.61547088677
1.56648 1.62044576591
1.57136 1.62838881878
1.57624 1.63320321513
1.58112 1.63793457281
1.586 1.64258224228
1.59088 1.64714558376
1.59576 1.65162396728
1.60064 1.65908360889
1.60552 1.66339249888
1.6104 1.6676144327
1.61528 1.67482194055
1.62016 1.67886997047
1.62504 1.68282913547
1.62992 1.68977676915
1.6348 1.69355779946
1.63968 1.7003283721
1.64456 1.70392843663
1.64944 1.71051848559
1.65432 1.71393483554
1.6592 1.7203409811
1.66408 1.72665404668
1.66896 1.72978989753
1.67384 1.73591398041
1.67872 1.74194224014
1.6836 1.74479137617
1.68848 1.75062576757
1.69336 1.75636169101
1.69824 1.76199823145
1.70312 1.76753448519
1.708 1.77296955994
1.71288 1.77830257492
1.71776 1.78353266086
1.72264 1.78865896012
1.72752 1.79368062673
1.7324 1.7985968264
1.73728 1.80340673662
1.74216 1.80810954667
1.74704 1.81576589128
1.75192 1.82024935316
1.7568 1.82462319076
1.76168 1.83193926864
1.76656 1.83608833054
1.77144 1.84012535382
1.77632 1.84709197483
1.7812 1.85089901921
1.78608 1.85762642788
1.79096 1.86120004327
1.79584 1.86768420139
1.80072 1.87404305395
1.8056 1.87725801518
1.81048 1.88336760171
1.81536 1.88934869963
1.82024 1.8952002236
1.82512 1.90092110251
1.83 1.9065102795
1.83488 1.91196671191
1.83976 1.91728937129
1.84464 1.92247724338
1.84952 1.92752932809
1.8544 1.93244463942
1.85928 1.93722220548
1.86416 1.94186106836
1.86904 1.94930446067
1.87392 1.95365640462
1.8788 1.95786670762
1.88368 1.96485809801
1.88856 1.96877529286
1.89344 1.97545723312
1.89832 1.98197899543
1.9032 1.98544513529
1.90808 1.99165045527
1.91296 1.99769195701
1.91784 2.0035684116
1.92272 2.00927860603
1.9276 2.0148213431
1.93248 2.02019544117
1.93736 2.02539973402
1.94224 2.03043307062
1.94712 2.03529431489
1.952 2.0427929975
1.95688 2.04729760891
1.96176 2.05162667484
1.96664 2.05856206601
1.97152 2.06252732855
1.9764 2.06907754725
1.98128 2.07542835128
1.98616 2.08157833454
1.99104 2.08752610675
1.99592 2.09054625936
2.0008 2.0960957587
2.00568 2.10414248208
2.01056 2.10926780783
2.01544 2.11418419238
2.02032 2.11889033047
2.0252 2.12604558528
2.03008 2.13031638257
2.03496 2.13701155017
2.03984 2.14346882582
2.04472 2.14968661659
2.0496 2.15305873647
2.05448 2.15880437618
2.05936 2.16688733101
2.06424 2.17213148742
2.06912 2.17712836193
2.074 2.1818764218
2.07888 2.18890782239
2.08376 2.19566297622
2.08864 2.19963084742
2.09352 2.20584041532
2.0984 2.21176836413
2.10328 2.21741287616
2.10816 2.22277213478
2.11304 2.23029056762
2.11792 2.23506097554
2.1228 2.24196096245
2.12768 2.24854216679
2.13256 2.25240828247
2.13744 2.25835878717
2.14232 2.26635181014
2.1472 2.27163655492
2.15208 2.27659178721
2.15696 2.28354240797
2.16184 2.29013175245
2.16672 2.29405761295
2.1716 2.30221654903
2.17648 2.30770688935
2.18136 2.31282572037
2.18624 2.31981432431
2.19112 2.32639778594
2.196 2.33257309937
2.20088 2.33833719669
2.20576 2.34368694062
2.21064 2.3507917756
2.21552 2.35528858469
2.2204 2.36150469479
2.22528 2.36939283111
2.23016 2.37467626297
2.23504 2.38159449555
2.23992 2.38801408563
2.2448 2.39393054271
2.24968 2.39933920021
2.25456 2.40627566841
2.25944 2.41266443782
2.26432 2.41849998612
2.2692 2.42577204866
2.27408 2.43244881504
2.27896 2.43852367264
2.28384 2.44398964132
2.28872 2.45077431726
2.2936 2.45690431872
2.29848 2.46427564874
2.30336 2.47094400127
2.30824 2.4768994043
2.31312 2.48398984376
2.318 2.49031430009
2.32288 2.49768814524
2.32776 2.50423876814
2.33264 2.50995102537
2.33752 2.51659020614
2.3424 2.52409177889
2.34728 2.53063809822
2.35216 2.53794226553
2.35704 2.54421244118
2.36192 2.55112513375
2.3668 2.5569125185
2.37168 2.56488618666
2.37656 2.57159454881
2.38144 2.57863257329
2.38632 2.58589780136
2.3912 2.5932778437
2.39608 2.5990505007
2.40096 2.60628417714
2.40584 2.61476983995
2.41072 2.62116702131
2.4156 2.62835977495
2.42048 2.63600809181
2.42536 2.6436786068
2.43024 2.65227116445
2.43512 2.66086021886


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1prob0pt1.tex <==
0.0 0.333808418527
0.004276 0.333806678676
0.008552 0.333886857632
0.012828 0.334043537963
0.017104 0.334226406958
0.02138 0.334473912959
0.025656 0.334779752126
0.029932 0.335137345056
0.034208 0.335539832531
0.038484 0.336025459752
0.04276 0.336541843354
0.047036 0.337081315517
0.051312 0.337682021462
0.055588 0.338336533252
0.059864 0.339083948193
0.06414 0.339823337986
0.068416 0.340640477
0.072692 0.341480446707
0.076968 0.34238299242
0.081244 0.343340691854
0.08552 0.344395050862
0.089796 0.345440733852
0.094072 0.346518504612
0.098348 0.347670887348
0.102624 0.348891311484
0.1069 0.350121512903
0.111176 0.351405276125
0.115452 0.352788622628
0.119728 0.354159585116
0.124004 0.355563392688
0.12828 0.357047773541
0.132556 0.358607644528
0.136832 0.360181653109
0.141108 0.361762460796
0.145384 0.36345829857
0.14966 0.36514909003
0.153936 0.366886714552
0.158212 0.36866597531
0.162488 0.370542963661
0.166764 0.372390757816
0.17104 0.374327689303
0.175316 0.376287229849
0.179592 0.378264116912
0.183868 0.380319295195
0.188144 0.382450637498
0.19242 0.384519259691
0.196696 0.386725187302
0.200972 0.388928489748
0.205248 0.391123835336
0.209524 0.393379003871
0.2138 0.395692312682
0.218076 0.398062196736
0.222352 0.40041014042
0.226628 0.402887588014
0.230904 0.405337764213
0.23518 0.407836544425
0.239456 0.410300140501
0.243732 0.412891531401
0.248008 0.415442892394
0.252284 0.418036125005
0.25656 0.420670540151
0.260836 0.423345574535
0.265112 0.426060792632
0.269388 0.428815888806
0.273664 0.431610689534
0.27794 0.434347711495
0.282216 0.437220122758
0.286492 0.440031381176
0.290768 0.442879197187
0.295044 0.445763980508
0.29932 0.448686287122
0.303596 0.451646822065
0.307872 0.454646442258
0.312148 0.457686159386
0.316424 0.460651984436
0.3207 0.463656082832
0.324976 0.466819347652
0.329252 0.469906520713
0.333528 0.472912589153
0.337804 0.476085191451
0.34208 0.479304622242
0.346356 0.482441988965
0.350632 0.485625940973
0.354908 0.48885894896
0.359184 0.492005095884
0.36346 0.495341805022
0.367736 0.498592316258
0.372012 0.501898305167
0.376288 0.505263070175
0.380564 0.508538286851
0.38484 0.511873922448
0.389116 0.515273750637
0.393392 0.518581476023
0.397668 0.52195575413
0.401944 0.525400853933
0.40622 0.528752144975
0.410496 0.532177371435
0.414772 0.535681316592
0.419048 0.53909064598
0.423324 0.542582595744
0.4276 0.546162481176
0.431876 0.549647890465
0.436152 0.553225957083
0.440428 0.556707965081
0.444704 0.560287827695
0.44898 0.563770356753
0.453256 0.567356424976
0.457532 0.571052560431
0.461808 0.574653614559
0.466084 0.578155793539
0.47036 0.5817744302
0.474636 0.585516738665
0.478912 0.589163606635
0.483188 0.592711409916
0.487464 0.596390660545
0.49174 0.600209276521
0.496016 0.603933497432
0.500292 0.607559884935
0.504568 0.61133484649
0.508844 0.615013119928
0.51312 0.618591350794
0.517396 0.622328268836
0.521672 0.626232989271
0.525948 0.630044402407
0.530224 0.633759362886
0.5345 0.637374714965
0.538776 0.641170650077
0.543052 0.645157135647
0.547328 0.648760065587
0.551604 0.652556361856
0.55588 0.656556480575
0.560156 0.66046544082
0.564432 0.664280416513
0.568708 0.667998576602
0.572984 0.671936672853
0.57726 0.675781714333
0.581536 0.679530983919
0.585812 0.683515624747
0.590088 0.687408734217
0.594364 0.691207712431
0.59864 0.695258464819
0.602916 0.698866339968
0.607192 0.703089262164
0.611468 0.706864347077
0.615744 0.710911176871
0.62002 0.714868922806
0.624296 0.71873522774
0.628572 0.722507736641
0.632848 0.726573403904
0.637124 0.730551123556
0.6414 0.734438665099
0.645676 0.738233801645
0.649952 0.742344940045
0.654228 0.746370081052
0.658504 0.750307122928
0.66278 0.75415396878
0.667056 0.758341067984
0.671332 0.762444929897
0.675608 0.766463582171
0.679884 0.770395058266
0.68416 0.774237397969
0.688436 0.778449372666
0.692712 0.782579791127
0.696988 0.786626816374
0.701264 0.79058861841
0.70554 0.794463374701
0.709816 0.798739018335
0.714092 0.802440150762
0.718368 0.806550433736
0.722644 0.810578425531
0.72692 0.815035976827
0.731196 0.818900361801
0.735472 0.823203066275
0.739748 0.826897291998
0.744024 0.831038751673
0.7483 0.835100281176
0.752576 0.839080337025
0.756852 0.843533683279
0.761128 0.847352420376
0.765404 0.85165390068
0.76968 0.855880401459
0.773956 0.860030507213
0.778232 0.864102811958
0.782508 0.868095919574
0.786784 0.87200844415
0.79106 0.876445758956
0.795336 0.880199418108
0.799612 0.884488021844
0.803888 0.888703546132
0.808164 0.892844725435
0.81244 0.896910304383
0.816716 0.900899038074
0.820992 0.905461771485
0.825268 0.909299680785
0.829544 0.913722301706
0.83382 0.918076409595
0.838096 0.922360868679
0.842372 0.925889528974
0.846648 0.930716347692
0.850924 0.934785147215
0.8552 0.938779857625
0.859476 0.942699395818
0.863752 0.947261056639
0.868028 0.951033759288
0.872304 0.955459920115
0.87658 0.95982017286
0.880856 0.964113527841
0.885132 0.968339005509
0.889408 0.972495636659
0.893684 0.976582462643
0.89796 0.980598535573
0.902236 0.985322045301
0.906512 0.989200611623
0.910788 0.993798378977
0.915064 0.997535809558
0.91934 1.00200427575
0.923616 1.00641019031
0.927892 1.01075269937
0.932168 1.01503095893
0.936444 1.01924413498
0.94072 1.02339140366
0.944996 1.02747195148
0.949272 1.0314849754
0.953548 1.03629064041
0.957824 1.04017308539
0.9621 1.04486027831
0.966376 1.04860905915
0.970652 1.05317473198
0.974928 1.05768193524
0.979204 1.06122802798
0.98348 1.06560928238
0.987756 1.06992989173
0.992032 1.07418914857
0.996308 1.07838635496
1.000584 1.08345673237
1.00486 1.08753456476
1.009136 1.09154830333
1.013412 1.09549728872
1.017688 1.100343848
1.021964 1.10416813635
1.02624 1.10890219094
1.030516 1.11358238352
1.034792 1.11721821086
1.039068 1.121782068
1.043344 1.12629016872
1.04762 1.13074189408
1.051896 1.13513663348
1.056172 1.13947378474
1.060448 1.14375275418
1.064724 1.14797295673
1.069 1.15213381601
1.073276 1.15623476443
1.077552 1.16133129973
1.081828 1.16531728412
1.086104 1.16924168852
1.09038 1.17417953635
1.094656 1.1779856564
1.098932 1.18281705029
1.103208 1.18650274206
1.107484 1.19122548255
1.11176 1.19589626895
1.116036 1.20051455038
1.120312 1.20395954632
1.124588 1.20846491346
1.128864 1.21291619209
1.13314 1.21731286058
1.137416 1.22165440461
1.141692 1.22594031724
1.145968 1.23017009899
1.150244 1.23550687471
1.15452 1.23962900727
1.158796 1.24369352484
1.163072 1.24888170556
1.167348 1.25283557792
1.171624 1.25673041655
1.1759 1.26176536326
1.180176 1.26554668743
1.184452 1.27047893298
1.188728 1.275361982
1.193004 1.27897244688
1.19728 1.28374981416
1.201556 1.28847646882
1.205832 1.29191196147
1.210108 1.29653006928
1.214384 1.30109600415
1.21866 1.30560927877
1.222936 1.31006941181
1.227212 1.314475928
1.231488 1.31882835818
1.235764 1.32312623931
1.24004 1.32865281973
1.244316 1.33284552146
1.248592 1.33698227894
1.252868 1.34106265357
1.257144 1.34639076491
1.26142 1.35036218943
1.265696 1.35427590806
1.269972 1.3594512163
1.274248 1.36325325655
1.278524 1.3683258961
1.2828 1.37334888858
1.287076 1.37698247858
1.291352 1.38189983173
1.295628 1.38676600279
1.299904 1.39022712104
1.30418 1.39498477588
1.308456 1.39968975882
1.312732 1.40434156635
1.317008 1.40893969983
1.321284 1.41348366551
1.32556 1.41797297462
1.329836 1.42240714333
1.334112 1.42678569286
1.338388 1.43110814947
1.342664 1.4353740445
1.34694 1.44098400958
1.351216 1.4451394125
1.355492 1.44923682289
1.359768 1.45468874255
1.364044 1.45867267543
1.36832 1.46401779072
1.372596 1.46788626524
1.376872 1.47312238438
1.381148 1.47687345738
1.385424 1.48199842341
1.3897 1.48563018994
1.393976 1.49064188129
1.398252 1.49559782675
1.402528 1.5004974491
1.406804 1.50388830162
1.41108 1.50867039277
1.415356 1.51339451495
1.419632 1.51806010765
1.423908 1.52266661458
1.428184 1.52721348364
1.43246 1.531700167
1.436736 1.53612612113
1.441012 1.54196629753
1.445288 1.54627184878
1.449564 1.55051500221
1.45384 1.55469523143
1.458116 1.56029776675
1.462392 1.56435299736
1.466668 1.56983416647
1.470944 1.57376208535
1.47522 1.57911933029
1.479496 1.58291765714
1.483772 1.588148451
1.488048 1.59181493879
1.492324 1.59691678614
1.4966 1.60195416103
1.500876 1.60692638446
1.505152 1.61183278116
1.509428 1.61516258415
1.513704 1.61993373331
1.51798 1.62463712057
1.522256 1.62927208605
1.526532 1.63535399405
1.530808 1.63985146213
1.535084 1.64427848328
1.53936 1.64863441298
1.543636 1.6529186106
1.547912 1.6586522925
1.552188 1.6627920852
1.556464 1.66838186166
1.56074 1.67237445612
1.565016 1.67781727064
1.569292 1.68165990348
1.573568 1.6869527286
1.577844 1.69216969078
1.58212 1.69578250386
1.586396 1.70084491986
1.590672 1.7058291055
1.594948 1.71073425529
1.599224 1.71555956724
1.6035 1.72030424287
1.607776 1.7249674872
1.612052 1.7295485087
1.616328 1.73404651931
1.620604 1.73998904596
1.62488 1.74431842436
1.629156 1.74856237731
1.633432 1.75424741891
1.637708 1.75831772797
1.641984 1.76382646912
1.64626 1.7692453762
1.650536 1.77304859242
1.654812 1.7782856974
1.659088 1.78343012508
1.663364 1.78848091008
1.66764 1.79343708991
1.671916 1.79829770491
1.676192 1.80306179818
1.680468 1.80772841543
1.684744 1.81229660498
1.68902 1.8182806777
1.693296 1.82264774403
1.697572 1.82691347137
1.701848 1.8325876701
1.706124 1.83664626019
1.7104 1.84210800639
1.714676 1.8474610084
1.718952 1.85270412061
1.723228 1.85783619903
1.727504 1.86285610106
1.73178 1.86776268534
1.736056 1.87255481151
1.740332 1.87723134001
1.744608 1.88179113183
1.748884 1.88772168666
1.75316 1.89204216222
1.757436 1.89772610658
1.761712 1.90180243426
1.765988 1.90723466036
1.770264 1.91253774737
1.77454 1.91771034749
1.778816 1.92275111137
1.783092 1.92765868763
1.787368 1.93243172251
1.791644 1.93852993764
1.79592 1.9430266859
1.800196 1.94883947392
1.804472 1.9530542111
1.808748 1.95857556387
1.813024 1.963947225
1.8173 1.96916761048
1.821576 1.97423512963
1.825852 1.97914818428
1.830128 1.98390516799
1.834404 1.98993107684
1.83868 1.99436725342
1.842956 2.00006132985
1.847232 2.00558485297
1.851508 2.01093596856
1.855784 2.01611280826
1.86006 2.0211134883
1.864336 2.02593610801
1.868612 2.03197298321
1.872888 2.03642937472
1.877164 2.04208732419
1.88144 2.04755042705
1.885716 2.05281648841
1.889992 2.05788328601
1.894268 2.06411583069
1.898544 2.06877260461
1.90282 2.07458097786
1.907096 2.08017115168
1.911372 2.08554054943
1.915648 2.09068655031
1.919924 2.09560648559
1.9242 2.10163065048
1.928476 2.10608510971
1.932752 2.11162781176
1.937028 2.11692266412
1.941304 2.12327867738
1.94558 2.12806295158
1.949856 2.13389102683
1.954132 2.13944717426
1.958408 2.14472772386
1.962684 2.1510137344
1.96696 2.15572600366
1.971236 2.16142444793
1.975512 2.16681989823
1.979788 2.17316989575
1.984064 2.17793989366
1.98834 2.1836431729
1.992616 2.19025689664
1.996892 2.19528086342
2.001168 2.20119211435
2.005444 2.20674014816
2.00972 2.21191855544
2.013996 2.21793463839
2.018272 2.22355480219
2.022548 2.22997296756
2.026824 2.23477145769
2.0311 2.24152742277
2.035376 2.24664547236
2.039652 2.25248705645
2.043928 2.25902197308
2.048204 2.26389235249
2.05248 2.27057509015
2.056756 2.27671646142
2.061032 2.28230094997
2.065308 2.28844850795
2.069584 2.29399002153
2.07386 2.30002809822
2.078136 2.30651905869
2.082412 2.31230595665
2.086688 2.31846187642
2.090964 2.32383527885
2.09524 2.33056519702
2.099516 2.33639799407
2.103792 2.34342927054
2.108068 2.34941252619
2.112344 2.35532684997
2.11662 2.36210188614
2.120896 2.36851338587
2.125172 2.37539981457
2.129448 2.38246312906
2.133724 2.38927212064


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1prob0pt1pt5prob0pt5.tex <==
0.0 0.147880225764
0.004276 0.147933398943
0.008552 0.148091744473
0.012828 0.14835361007
0.017104 0.148717501834
0.02138 0.14918207647
0.025656 0.149746133931
0.029932 0.150408610421
0.034208 0.151168571768
0.038484 0.152025207133
0.04276 0.152977823035
0.047036 0.154025837684
0.051312 0.155168775599
0.055588 0.156406262492
0.059864 0.157738020408
0.06414 0.159163863114
0.068416 0.160683691702
0.072692 0.162297490416
0.076968 0.164005322678
0.081244 0.16580732731
0.08552 0.167703714927
0.089796 0.16969476451
0.094072 0.171780820137
0.098348 0.173962287865
0.102624 0.176239632754
0.1069 0.178613376036
0.111176 0.181084092396
0.115452 0.183652407393
0.119728 0.186318994981
0.124004 0.189084575146
0.12828 0.191949911643
0.132556 0.194915809832
0.136832 0.197983114604
0.141108 0.201152708394
0.145384 0.20442550928
0.14966 0.207802469156
0.153936 0.211284571979
0.158212 0.21244039093
0.162488 0.212459953312
0.166764 0.212501794379
0.17104 0.21258452889
0.175316 0.212684522909
0.179592 0.212799190165
0.183868 0.212925972056
0.188144 0.213106094685
0.19242 0.213293934288
0.196696 0.213509239194
0.200972 0.21375008214
0.205248 0.214014580467
0.209524 0.214300893259
0.2138 0.214607218638
0.218076 0.214954949576
0.222352 0.215319611636
0.226628 0.215699523974
0.230904 0.216116838727
0.23518 0.216570617695
0.239456 0.21701145167
0.243732 0.217510612176
0.248008 0.218018542443
0.252284 0.218558790594
0.25656 0.219105414672
0.260836 0.219682558692
0.265112 0.220289666053
0.269388 0.220926241637
0.273664 0.221565430759
0.27794 0.222259397286
0.282216 0.222927631937
0.286492 0.223650031223
0.290768 0.224399656059
0.295044 0.225148332353
0.29932 0.225923298292
0.303596 0.226724497897
0.307872 0.227551937678
0.312148 0.22837623714
0.316424 0.229256049891
0.3207 0.230132276763
0.324976 0.231034604056
0.329252 0.231932313125
0.333528 0.23288739952
0.337804 0.233837825313
0.34208 0.234782795814
0.346356 0.235787004774
0.350632 0.236786021911
0.354908 0.237812805301
0.359184 0.238833968081
0.36346 0.239883483645
0.367736 0.240962211118
0.372012 0.242035488503
0.376288 0.243138907168
0.380564 0.244236901212
0.38484 0.245366185888
0.389116 0.246527961009
0.393392 0.24768525271
0.397668 0.248837742344
0.401944 0.250024530151
0.40622 0.251207121128
0.410496 0.252425877131
0.414772 0.253641252975
0.419048 0.254894920396
0.423324 0.256103823545
0.4276 0.257395197639
0.431876 0.258641777749
0.436152 0.259930389275
0.440428 0.261218071663
0.444704 0.262504959116
0.44898 0.263837641175
0.453256 0.265171315834
0.457532 0.266506260237
0.461808 0.267842790089
0.466084 0.269181260529
0.47036 0.27052206701
0.474636 0.271916479306
0.478912 0.273315696843
0.483188 0.274667876407
0.487464 0.27607761962
0.49174 0.277493962606
0.496016 0.278917598671
0.500292 0.280349268257
0.504568 0.281733229047
0.508844 0.283182516445
0.51312 0.284642338158
0.517396 0.286113632446
0.521672 0.287537328656
0.525948 0.289033675875
0.530224 0.29048270959
0.5345 0.292008444415
0.538776 0.293487315626
0.543052 0.294982448845
0.547328 0.296495124266
0.551604 0.297959944212
0.55588 0.299510770301
0.560156 0.301014554569
0.564432 0.30253950927
0.568708 0.304087172184
0.572984 0.305659143529
0.57726 0.307184107086
0.581536 0.308734591792
0.585812 0.310312347371
0.590088 0.311842902903
0.594364 0.313402164915
0.59864 0.314992039012
0.602916 0.316614499026
0.607192 0.318190694241
0.611468 0.319719174695
0.615744 0.321365034611
0.62002 0.3229650943
0.624296 0.324517942203
0.628572 0.326196095491
0.632848 0.327740975171
0.637124 0.329415907985
0.6414 0.331045611232
0.645676 0.33262873202
0.649952 0.334257322531
0.654228 0.335934004328
0.658504 0.337565374455
0.66278 0.339150116886
0.667056 0.340785746628
0.671332 0.342475104785
0.675608 0.344119464351
0.679884 0.34582062381
0.68416 0.347477104442
0.688436 0.349087654887
0.692712 0.350758452978
0.696988 0.352383758369
0.701264 0.354072762142
0.70554 0.355828770778
0.709816 0.357428209675
0.714092 0.359095318408
0.718368 0.360833560981
0.722644 0.362528308725
0.72692 0.364178404844
0.731196 0.365904073461
0.735472 0.367586008507
0.739748 0.369347739857
0.744024 0.371066780503
0.7483 0.372742025076
0.752576 0.374372360601
0.756852 0.376088076787
0.761128 0.377893225778
0.765404 0.379522183285
0.76968 0.381241908283
0.773956 0.383056626901
0.778232 0.384690228388
0.782508 0.386420311166
0.786784 0.388251278758
0.79106 0.389896236922
0.795336 0.391643725068
0.799612 0.393348893822
0.803888 0.395162065905
0.808164 0.396934725642
0.81244 0.398665906119
0.816716 0.400354634734
0.820992 0.402159007229
0.825268 0.403922922849
0.829544 0.405645441955
0.83382 0.407325619616
0.838096 0.409129600041
0.842372 0.4108934282
0.846648 0.412616193952
0.850924 0.414470274532
0.8552 0.41611026446
0.859476 0.417883958573
0.863752 0.419796832544
0.868028 0.421490862529
0.872304 0.423326642275
0.87658 0.424937526637
0.880856 0.426881145325
0.885132 0.42859817498
0.889408 0.430273920743
0.893684 0.432102611442
0.89796 0.433892851484
0.902236 0.435643827932
0.906512 0.437556694554
0.910788 0.439229019008
0.915064 0.441066284237
0.91934 0.442865744651
0.923616 0.444626621693
0.927892 0.446348133419
0.932168 0.44824571479
0.936444 0.45010723228
0.94072 0.451710831803
0.944996 0.453495528126
0.949272 0.45546799886
0.953548 0.457177842986
0.957824 0.459079020023
0.9621 0.460711080099
0.966376 0.462538091545
0.970652 0.464328227933
0.974928 0.466322199267
0.979204 0.468039077314
0.98348 0.469963642457
0.987756 0.471604480282
0.992032 0.473456919425
0.996308 0.475273616296
1.000584 0.47705390183
1.00486 0.478797104673
1.009136 0.480765443523
1.013412 0.482435224045
1.017688 0.484334357313
1.021964 0.486199325567
1.02624 0.488029501342
1.030516 0.489824255191
1.034792 0.491582955721
1.039068 0.493587621232
1.043344 0.495275209255
1.04762 0.497213320446
1.051896 0.498827321341
1.056172 0.500696469887
1.060448 0.502531715308
1.064724 0.504332468844
1.069 0.506401459971
1.073276 0.508134483555
1.077552 0.509831257938
1.081828 0.511803644548
1.086104 0.513744756016
1.09038 0.515335407893
1.094656 0.517209219896
1.098932 0.51905010693
1.103208 0.520857522571
1.107484 0.522630919133
1.11176 0.524704177303
1.116036 0.526411100791
1.120312 0.528423249258
1.124588 0.530061568628
1.128864 0.532010545909
1.13314 0.533928806202
1.137416 0.535815849458
1.141692 0.537671174623
1.145968 0.539494279669
1.150244 0.541284661619
1.15452 0.543041816577
1.158796 0.544765239752
1.163072 0.546828652395
1.167348 0.548486531282
1.171624 0.550490298502
1.1759 0.552465274655
1.180176 0.554022915879
1.184452 0.55593543684
1.188728 0.557817786292
1.193004 0.559669508856
1.19728 0.5614901485
1.201556 0.563685086915
1.205832 0.56544579513
1.210108 0.567174067107
1.214384 0.56886944443
1.21866 0.570951838608
1.222936 0.572583728121
1.227212 0.574609110864
1.231488 0.576607211229
1.235764 0.57857762359
1.24004 0.58008098837
1.244316 0.581991034106
1.248592 0.583872154015
1.252868 0.585723940823
1.257144 0.587545986898
1.26142 0.589795880951
1.265696 0.591561084891
1.269972 0.593295341539
1.274248 0.594998242033
1.278524 0.597142938652
1.2828 0.598785835802
1.287076 0.600877620517
1.291352 0.602458948943
1.295628 0.60449632821
1.299904 0.606507949146
1.30418 0.608493455877
1.308456 0.609950990036
1.312732 0.611879135934
1.317008 0.613780081012
1.321284 0.615653468823
1.32556 0.617498942822
1.329836 0.619316146381
1.334112 0.621630879348
1.338388 0.62339464368
1.342664 0.625129085253
1.34694 0.626833847286
1.351216 0.629051524059
1.355492 0.630700099705
1.359768 0.632869398519
1.364044 0.634460431945
1.36832 0.636580067847
1.372596 0.63811220352
1.376872 0.640180891752
1.381148 0.642225799062
1.385424 0.644246621954
1.3897 0.645661281986
1.393976 0.647628624304
1.398252 0.649570954714
1.402528 0.651487970061
1.406804 0.653379367311
1.41108 0.655244843561
1.415356 0.657084096057
1.419632 0.658896822216
1.423908 0.660682719634
1.428184 0.663063496922
1.43246 0.664799386991
1.436736 0.666507559398
1.441012 0.668823443951
1.445288 0.670479884105
1.449564 0.67210771965
1.45384 0.674356254047
1.458116 0.675930636416
1.462392 0.678134466368
1.466668 0.679654262051
1.470944 0.681812322002
1.47522 0.683949460178
1.479496 0.685387626143
1.483772 0.687477416323
1.488048 0.689545521682
1.492324 0.691591693854
1.4966 0.692918755024
1.500876 0.694915493961
1.505152 0.696889539972
1.509428 0.698840645835
1.513704 0.700768564635
1.51798 0.702673049774
1.522256 0.704553854987
1.526532 0.706410734352
1.530808 0.708243442306
1.535084 0.710051733653
1.53936 0.711835363582
1.543636 0.714344951477
1.547912 0.716083523997
1.552188 0.717796718707
1.556464 0.719484292394
1.56074 0.721916951589
1.565016 0.723557615747
1.569292 0.725171947356
1.573568 0.727545880288
1.577844 0.729111929339
1.58212 0.731447340118
1.586396 0.732964205628
1.590672 0.735260255505
1.594948 0.736727039952
1.599224 0.738982893234
1.6035 0.740398702742
1.607776 0.742613526961
1.612052 0.744810137753
1.616328 0.746150437567
1.620604 0.74830479162
1.62488 0.750440342212
1.629156 0.752556898286
1.633432 0.753795261029
1.637708 0.755867945272
1.641984 0.75792104995
1.64626 0.759954385658
1.650536 0.761967763408
1.654812 0.763960994644
1.659088 0.765933891246
1.663364 0.767886265542
1.66764 0.769817930316
1.671916 0.77172869882
1.676192 0.773618384779
1.680468 0.775486802403
1.684744 0.777333766395
1.68902 0.779159091963
1.693296 0.780962594824
1.697572 0.782744091218
1.701848 0.784503397913
1.706124 0.787191513487
1.7104 0.788911436104
1.714676 0.790608635555
1.718952 0.792282930742
1.723228 0.794907568551
1.727504 0.79654110837
1.73178 0.79815121675
1.736056 0.800727959771
1.740332 0.802296301186
1.744608 0.803840688915
1.748884 0.806368120347
1.75316 0.807869738868
1.757436 0.81036540756
1.761712 0.811823602182
1.765988 0.813256988253
1.770264 0.815701024106
1.77454 0.817090000416
1.778816 0.819500757918
1.783092 0.821897527225
1.787368 0.823221565161
1.791644 0.825584176838
1.79592 0.826862215875
1.800196 0.829190080899
1.804472 0.831503255558
1.808748 0.832714022284
1.813024 0.834991585505
1.8173 0.837254044728
1.821576 0.838396165994
1.825852 0.840622158071
1.830128 0.842832636746
1.834404 0.845027470023
1.83868 0.846077920539
1.842956 0.848235167395
1.847232 0.850376365266
1.851508 0.852501384024
1.855784 0.854610093998
1.86006 0.856702365983
1.864336 0.858778071244
1.868612 0.859666950062
1.872888 0.861703166475
1.877164 0.863722423259
1.88144 0.865724593714
1.885716 0.867709551638
1.889992 0.869677171334
1.894268 0.871627327615
1.898544 0.873559895811
1.90282 0.875474751774
1.907096 0.87737177188
1.911372 0.87925083304
1.915648 0.881111812702
1.919924 0.882954588857
1.9242 0.886027516068
1.928476 0.887839609598
1.932752 0.889633145236
1.937028 0.891408003098
1.941304 0.893164063873
1.94558 0.894901208822
1.949856 0.896619319785
1.954132 0.899609538652
1.958408 0.901295373891
1.962684 0.902961831829
1.96696 0.904608796573
1.971236 0.906236152838
1.975512 0.909165836778
1.979788 0.910759814133
1.984064 0.91233384795
1.98834 0.915228435788
1.992616 0.916768446862
1.996892 0.918288184342
2.001168 0.921146769127
2.005444 0.92263184923
2.00972 0.924096330803
2.013996 0.926918017236
2.018272 0.928347216232
2.022548 0.929755497007
2.026824 0.932539401764
2.0311 0.933911784423
2.035376 0.936672103064
2.039652 0.938008186586
2.043928 0.940744543207
2.048204 0.942043930748
2.05248 0.943321678796
2.056756 0.946018251755
2.061032 0.947258711266
2.065308 0.94993039217
2.069584 0.952592641158
2.07386 0.953779602384
2.078136 0.956416419877
2.082412 0.957565140742
2.086688 0.960176168189
2.090964 0.961286273645
2.09524 0.963871156134
2.099516 0.964942275672
2.103792 0.967500661983
2.108068 0.970048840076
2.112344 0.971063972343
2.11662 0.973585138242
2.120896 0.976095845534
2.125172 0.977054193987
2.129448 0.979537381004
2.133724 0.982009862537


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1pt5.tex <==
0.0 0.208916205288
0.0064 0.208999387658
0.0128 0.209247010917
0.0192 0.209656385231
0.0256 0.210225085186
0.032 0.210950936208
0.0384 0.211832001658
0.0448 0.212866570567
0.0512 0.21405314599
0.0576 0.215390433933
0.064 0.216877332828
0.0704 0.21851292353
0.0768 0.220296459801
0.0832 0.222227359258
0.0896 0.224305194765
0.096 0.226529686229
0.1024 0.228900692799
0.1088 0.231418205427
0.1152 0.234082339783
0.1216 0.236893329496
0.128 0.239851519712
0.1344 0.242957360941
0.1408 0.246211403185
0.1472 0.249614290334
0.1536 0.253166754798
0.16 0.256869612389
0.1664 0.26072375741
0.1728 0.264730157969
0.1792 0.268889851482
0.1856 0.273203940364
0.192 0.277673587907
0.1984 0.282300014318
0.2048 0.287084492921
0.2112 0.29202834651
0.2176 0.297132943849
0.224 0.302399696305
0.2304 0.302813240164
0.2368 0.302855187534
0.2432 0.302956564474
0.2496 0.303083782785
0.256 0.303262496441
0.2624 0.303458848998
0.2688 0.303729523719
0.2752 0.304010357504
0.2816 0.304359135701
0.288 0.304710867717
0.2944 0.305124492757
0.3008 0.305597655568
0.3072 0.306096042896
0.3136 0.306616616677
0.32 0.307189078981
0.3264 0.307811455643
0.3328 0.308481875518
0.3392 0.309198567639
0.3456 0.309925795644
0.352 0.310695303563
0.3584 0.311540386167
0.3648 0.312390380738
0.3712 0.313278382573
0.3776 0.314203143322
0.384 0.315199962954
0.3904 0.316195289946
0.3968 0.317261527081
0.4032 0.318323527981
0.4096 0.319455688748
0.416 0.320581168662
0.4224 0.321776458494
0.4288 0.323002744711
0.4352 0.32425960717
0.4416 0.32554671595
0.448 0.32686383239
0.4544 0.328210810253
0.4608 0.329587597038
0.4672 0.330994235413
0.4736 0.332430864767
0.48 0.333897722882
0.4864 0.335350034936
0.4928 0.336877807234
0.4992 0.338437115365
0.5056 0.340028609256
0.512 0.341605209376
0.5184 0.343262739882
0.5248 0.344905757812
0.5312 0.346583150076
0.5376 0.348296082741
0.544 0.349994257064
0.5504 0.351729071688
0.5568 0.353502008997
0.5632 0.355314677786
0.5696 0.357113953078
0.576 0.358954845097
0.5824 0.360782708548
0.5888 0.362654443916
0.5952 0.364572227568
0.6016 0.366479051604
0.608 0.368434815577
0.6144 0.370380846958
0.6208 0.37231691916
0.6272 0.374306049009
0.6336 0.376351138155
0.64 0.378324773531
0.6464 0.380356456318
0.6528 0.382449453557
0.6592 0.384538772117
0.6656 0.386555189919
0.672 0.388707625473
0.6784 0.390787937857
0.6848 0.39293904952
0.6912 0.395090924443
0.6976 0.397244227996
0.704 0.399399693027
0.7104 0.401558121245
0.7168 0.403799335822
0.7232 0.405967638212
0.7296 0.408223246934
0.736 0.410488357576
0.7424 0.412680082614
0.7488 0.414966606659
0.7552 0.417266517029
0.7616 0.419493096188
0.768 0.421822845698
0.7744 0.424079604028
0.7808 0.426445614026
0.7872 0.428739231555
0.7936 0.43105326239
0.8 0.433389616122
0.8064 0.435750291314
0.8128 0.438137376748
0.8192 0.440451633867
0.8256 0.442896602384
0.832 0.445270202126
0.8384 0.447676252491
0.8448 0.450117249947
0.8512 0.452486321262
0.8576 0.454892284217
0.864 0.457337867381
0.8704 0.459825899369
0.8768 0.462243043061
0.8832 0.464705093421
0.8896 0.467095334477
0.896 0.469654724421
0.9024 0.472145134644
0.9088 0.474564450271
0.9152 0.47703761753
0.9216 0.479568108943
0.928 0.482028657503
0.9344 0.484549967088
0.9408 0.487135772718
0.9472 0.489653261272
0.9536 0.492100452326
0.96 0.494756621176
0.9664 0.49720391332
0.9728 0.499723702066
0.9792 0.502320200683
0.9856 0.504848893454
0.992 0.507458855317
0.9984 0.510001505036
1.0048 0.512630230354
1.0112 0.515192301673
1.0176 0.517845506249
1.024 0.520432882843
1.0304 0.522952681702
1.0368 0.52556941946
1.0432 0.528119599838
1.0496 0.530772354965
1.056 0.533359748517
1.0624 0.536055615589
1.0688 0.538687495214
1.0752 0.541253765612
1.0816 0.54393544734
1.088 0.546553102346
1.0944 0.549105150248
1.1008 0.5517799919
1.1072 0.554583500633
1.1136 0.557131693168
1.12 0.559810536575
1.1264 0.56242606721
1.1328 0.565179443555
1.1392 0.567871711998
1.1456 0.570501434274
1.152 0.573277671108
1.1584 0.575780626591
1.1648 0.578648406518
1.1712 0.581240122138
1.1776 0.583988816571
1.184 0.586677303935
1.1904 0.589304241705
1.1968 0.592097863643
1.2032 0.594832860643
1.2096 0.597507942787
1.216 0.60012181693
1.2224 0.602914137466
1.2288 0.605648445649
1.2352 0.608323502672
1.2416 0.611187769394
1.248 0.613743556212
1.2544 0.616492023136
1.2608 0.619182282235
1.2672 0.622074812624
1.2736 0.624912845283
1.28 0.627427475436
1.2864 0.630150038348
1.2928 0.633088658953
1.2992 0.635697394466
1.3056 0.638526215392
1.312 0.641300079294
1.3184 0.644017910701
1.3248 0.646968447208
1.3312 0.649574214135
1.3376 0.652417033955
1.344 0.655206075
1.3504 0.65794031903
1.3568 0.660618747202
1.3632 0.663549849752
1.3696 0.666429805378
1.376 0.669257654921
1.3824 0.672032438922
1.3888 0.674753197732
1.3952 0.677418971613
1.4016 0.680358736678
1.408 0.683248546591
1.4144 0.685750597298
1.4208 0.68887470281
1.4272 0.691609250519
1.4336 0.694290246086
1.44 0.697267869878
1.4464 0.69984265944
1.4528 0.702719506369
1.4592 0.705546493875
1.4656 0.708322784515
1.472 0.711416775359
1.4784 0.714092851757
1.4848 0.717092372542
1.4912 0.719664971025
1.4976 0.722566837846
1.504 0.725420567975
1.5104 0.728225387174
1.5168 0.730980522268
1.5232 0.734084469614
1.5296 0.736741760047
1.536 0.739754034779
1.5424 0.742721312305
1.5488 0.745228152802
1.5552 0.748099391288
1.5616 0.750923482481
1.568 0.754126230222
1.5744 0.756857868298
1.5808 0.759540257569
1.5872 0.762611148952
1.5936 0.765639417876
1.6 0.768177915664
1.6064 0.77111494889
1.6128 0.774007404041
1.6192 0.776854638199
1.6256 0.77965601013
1.632 0.782877798327
1.6384 0.785589663229
1.6448 0.788728969866
1.6512 0.791348851048
1.6576 0.79440327273
1.664 0.797416453676
1.6704 0.799895855849
1.6768 0.802820590013
1.6832 0.805702335112
1.6896 0.80904521128
1.696 0.811843535691
1.7024 0.814597171567
1.7088 0.817305551225
1.7152 0.820489997883
1.7216 0.823110508365
1.728 0.826214663415
1.7344 0.82928006003
1.7408 0.832306185844
1.7472 0.835292530428
1.7536 0.838238585343
1.76 0.841143844185
1.7664 0.844007802645
1.7728 0.846829958554
1.7792 0.849609811937
1.7856 0.852917228932
1.792 0.855615477371
1.7984 0.858269950475
1.8048 0.861464030169
1.8112 0.864622412615
1.8176 0.867151712308
1.824 0.870232809149
1.8304 0.873276861081
1.8368 0.876283427298
1.8432 0.879252069107
1.8496 0.882182349966
1.856 0.885073835528
1.8624 0.88792609368
1.8688 0.891368394048
1.8752 0.89414555896
1.8816 0.896882225387
1.888 0.900221644767
1.8944 0.902880730443
1.9008 0.90615111185
1.9072 0.908730988361
1.9136 0.911930755742
1.92 0.91509699017
1.9264 0.918229314431
1.9328 0.920650707422
1.9392 0.923709338615
1.9456 0.926732930701
1.952 0.929721114994
1.9584 0.932673524985
1.9648 0.935589796373
1.9712 0.93917485078
1.9776 0.942022565999
1.984 0.944833071982
1.9904 0.948325730828
1.9968 0.951065585207
2.0032 0.953767179727
2.0096 0.957164391932
2.016 0.959793278737
2.0224 0.963126810721
2.0288 0.966430443446
2.0352 0.968950194442
2.0416 0.972188204318
2.048 0.97539536357
2.0544 0.978571361337
2.0608 0.981715888711
2.0672 0.984050518777
2.0736 0.987126278318
2.08 0.99016964679
2.0864 0.993180323507
2.0928 0.996955797483
2.0992 0.999905127699
2.1056 1.00282088179
2.112 1.00570276731
2.1184 1.00855049396
2.1248 1.0121862557
2.1312 1.01496975714
2.1376 1.01855063247
2.144 1.02126879049
2.1504 1.02395137901
2.1568 1.02744539735
2.1632 1.03091323172
2.1696 1.03349741155
2.176 1.0369071205
2.1824 1.03942269798
2.1888 1.0427732314
2.1952 1.04609627685
2.2016 1.0493915797
2.208 1.05265888697
2.2144 1.05500587845
2.2208 1.05821145722
2.2272 1.06138829017
2.2336 1.06453613125
2.24 1.06765473615
2.2464 1.07074386226
2.2528 1.07380326876
2.2592 1.07775970251
2.2656 1.08076394468
2.272 1.08373775523
2.2784 1.08668090022
2.2848 1.08959314746
2.2912 1.09342619004
2.2976 1.0962809407
2.304 1.09910410698
2.3104 1.10286233564
2.3168 1.10562664404
2.3232 1.10933552255
2.3296 1.1120400804
2.336 1.11569871479
2.3424 1.11834264182
2.3488 1.12195014893
2.3552 1.1255342433
2.3616 1.12808808494
2.368 1.13161974455
2.3744 1.13512733874
2.3808 1.13758917493
2.3872 1.14104305032
2.3936 1.14447221839
2.4 1.14787646612
2.4064 1.15125558155
2.4128 1.15460935378
2.4192 1.15793757295
2.4256 1.16124003027
2.432 1.16451651801
2.4384 1.16776682947
2.4448 1.17099075899
2.4512 1.17418810196
2.4576 1.17735865481
2.464 1.18050221497
2.4704 1.1836185809
2.4768 1.18670755208
2.4832 1.19086881911
2.4896 1.19390725023
2.496 1.19691768334
2.5024 1.19989992164
2.5088 1.20397298399
2.5152 1.20690306105
2.5216 1.21093316912
2.528 1.21381027432
2.5344 1.21665819683
2.5408 1.22061991192
2.5472 1.2234136645
2.5536 1.22733033121
2.56 1.23122652574
2.5664 1.23393989576
2.5728 1.23778977648
2.5792 1.24044697467
2.5856 1.24424970643
2.592 1.2480308899
2.5984 1.25060469044
2.6048 1.25433746248
2.6112 1.25804803745
2.6176 1.2617361946
2.624 1.26540171279
2.6304 1.26904437039
2.6368 1.27145056906
2.6432 1.27504225984
2.6496 1.27861043553
2.656 1.28215487246
2.6624 1.28567534628
2.6688 1.28917163188
2.6752 1.2926435033
2.6816 1.29609073375
2.688 1.30076270941
2.6944 1.30416443719
2.7008 1.30754082203
2.7072 1.31089163265
2.7136 1.31421663651
2.72 1.31751559975
2.7264 1.32206442254
2.7328 1.32531496338
2.7392 1.32853873597
2.7456 1.33302466019
2.752 1.33619848708
2.7584 1.34064254844
2.7648 1.34376538028
2.7712 1.34686018548
2.7776 1.35123721343
2.784 1.35427942971
2.7904 1.358611738
2.7968 1.36292331886
2.8032 1.36588665413
2.8096 1.37015168995
2.816 1.37439503733
2.8224 1.37727685294
2.8288 1.38147175632
2.8352 1.38564396923
2.8416 1.38979314006
2.848 1.39256329939
2.8544 1.39666134409
2.8608 1.40073527941
2.8672 1.40478472929
2.8736 1.4088093106
2.88 1.41280863286
2.8864 1.4167822978
2.8928 1.42072989894
2.8992 1.42465102119
2.9056 1.42854524031
2.912 1.43241212244
2.9184 1.43764909541
2.9248 1.44146364756
2.9312 1.44524947008
2.9376 1.44900608424
2.944 1.45414542406
2.9504 1.45784570691
2.9568 1.46151523573
2.9632 1.46657650559
2.9696 1.47018638725
2.976 1.47519376682
2.9824 1.47874159802
2.9888 1.48369248047
2.9952 1.48861574678
3.0016 1.4920672993
3.008 1.49692978615
3.0144 1.50176234922
3.0208 1.5065641491
3.0272 1.5113343131
3.0336 1.51607193261
3.04 1.52077606033
3.0464 1.52544570707
3.0528 1.53007983822
3.0592 1.53467736989
3.0656 1.53923716445
3.072 1.54375802566
3.0784 1.54971869907
3.0848 1.55416063212
3.0912 1.56004509856
3.0976 1.56440227684
3.104 1.57020417327
3.1104 1.57447002782
3.1168 1.58018215587
3.1232 1.58584761826
3.1296 1.59146414989
3.136 1.59702930747
3.1424 1.60254044488
3.1488 1.60950238493
3.1552 1.61489875621
3.1616 1.62174352207
3.168 1.62701099224
3.1744 1.63372272175
3.1808 1.64036181697
3.1872 1.64844236018
3.1936 1.65492088809


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma1pt5prob0pt05.tex <==
0.0 0.147880225764
0.004276 0.147933398943
0.008552 0.148091744473
0.012828 0.14835361007
0.017104 0.148717501834
0.02138 0.14918207647
0.025656 0.149746133931
0.029932 0.150408610421
0.034208 0.151168571768
0.038484 0.152025207133
0.04276 0.152977823035
0.047036 0.154025837684
0.051312 0.155168775599
0.055588 0.156406262492
0.059864 0.157738020408
0.06414 0.159163863114
0.068416 0.160683691702
0.072692 0.162297490416
0.076968 0.164005322678
0.081244 0.16580732731
0.08552 0.167703714927
0.089796 0.16969476451
0.094072 0.171780820137
0.098348 0.173962287865
0.102624 0.176239632754
0.1069 0.178613376036
0.111176 0.181084092396
0.115452 0.183652407393
0.119728 0.186318994981
0.124004 0.189084575146
0.12828 0.191949911643
0.132556 0.194915809832
0.136832 0.197983114604
0.141108 0.201152708394
0.145384 0.20442550928
0.14966 0.207802469156
0.153936 0.211284571979
0.158212 0.21244039093
0.162488 0.212459953312
0.166764 0.212501794379
0.17104 0.21258452889
0.175316 0.212684522909
0.179592 0.212799190165
0.183868 0.212925972056
0.188144 0.213106094685
0.19242 0.213293934288
0.196696 0.213509239194
0.200972 0.21375008214
0.205248 0.214014580467
0.209524 0.214300893259
0.2138 0.214607218638
0.218076 0.214954949576
0.222352 0.215319611636
0.226628 0.215699523974
0.230904 0.216116838727
0.23518 0.216570617695
0.239456 0.21701145167
0.243732 0.217510612176
0.248008 0.218018542443
0.252284 0.218558790594
0.25656 0.219105414672
0.260836 0.219682558692
0.265112 0.220289666053
0.269388 0.220926241637
0.273664 0.221565430759
0.27794 0.222259397286
0.282216 0.222927631937
0.286492 0.223650031223
0.290768 0.224399656059
0.295044 0.225148332353
0.29932 0.225923298292
0.303596 0.226724497897
0.307872 0.227551937678
0.312148 0.22837623714
0.316424 0.229256049891
0.3207 0.230132276763
0.324976 0.231034604056
0.329252 0.231932313125
0.333528 0.23288739952
0.337804 0.233837825313
0.34208 0.234782795814
0.346356 0.235787004774
0.350632 0.236786021911
0.354908 0.237812805301
0.359184 0.238833968081
0.36346 0.239883483645
0.367736 0.240962211118
0.372012 0.242035488503
0.376288 0.243138907168
0.380564 0.244236901212
0.38484 0.245366185888
0.389116 0.246527961009
0.393392 0.24768525271
0.397668 0.248837742344
0.401944 0.250024530151
0.40622 0.251207121128
0.410496 0.252425877131
0.414772 0.253641252975
0.419048 0.254894920396
0.423324 0.256103823545
0.4276 0.257395197639
0.431876 0.258641777749
0.436152 0.259930389275
0.440428 0.261218071663
0.444704 0.262504959116
0.44898 0.263837641175
0.453256 0.265171315834
0.457532 0.266506260237
0.461808 0.267842790089
0.466084 0.269181260529
0.47036 0.27052206701
0.474636 0.271916479306
0.478912 0.273315696843
0.483188 0.274667876407
0.487464 0.27607761962
0.49174 0.277493962606
0.496016 0.278917598671
0.500292 0.280349268257
0.504568 0.281733229047
0.508844 0.283182516445
0.51312 0.284642338158
0.517396 0.286113632446
0.521672 0.287537328656
0.525948 0.289033675875
0.530224 0.29048270959
0.5345 0.292008444415
0.538776 0.293487315626
0.543052 0.294982448845
0.547328 0.296495124266
0.551604 0.297959944212
0.55588 0.299510770301
0.560156 0.301014554569
0.564432 0.30253950927
0.568708 0.304087172184
0.572984 0.305659143529
0.57726 0.307184107086
0.581536 0.308734591792
0.585812 0.310312347371
0.590088 0.311842902903
0.594364 0.313402164915
0.59864 0.314992039012
0.602916 0.316614499026
0.607192 0.318190694241
0.611468 0.319719174695
0.615744 0.321365034611
0.62002 0.3229650943
0.624296 0.324517942203
0.628572 0.326196095491
0.632848 0.327740975171
0.637124 0.329415907985
0.6414 0.331045611232
0.645676 0.33262873202
0.649952 0.334257322531
0.654228 0.335934004328
0.658504 0.337565374455
0.66278 0.339150116886
0.667056 0.340785746628
0.671332 0.342475104785
0.675608 0.344119464351
0.679884 0.34582062381
0.68416 0.347477104442
0.688436 0.349087654887
0.692712 0.350758452978
0.696988 0.352383758369
0.701264 0.354072762142
0.70554 0.355828770778
0.709816 0.357428209675
0.714092 0.359095318408
0.718368 0.360833560981
0.722644 0.362528308725
0.72692 0.364178404844
0.731196 0.365904073461
0.735472 0.367586008507
0.739748 0.369347739857
0.744024 0.371066780503
0.7483 0.372742025076
0.752576 0.374372360601
0.756852 0.376088076787
0.761128 0.377893225778
0.765404 0.379522183285
0.76968 0.381241908283
0.773956 0.383056626901
0.778232 0.384690228388
0.782508 0.386420311166
0.786784 0.388251278758
0.79106 0.389896236922
0.795336 0.391643725068
0.799612 0.393348893822
0.803888 0.395162065905
0.808164 0.396934725642
0.81244 0.398665906119
0.816716 0.400354634734
0.820992 0.402159007229
0.825268 0.403922922849
0.829544 0.405645441955
0.83382 0.407325619616
0.838096 0.409129600041
0.842372 0.4108934282
0.846648 0.412616193952
0.850924 0.414470274532
0.8552 0.41611026446
0.859476 0.417883958573
0.863752 0.419796832544
0.868028 0.421490862529
0.872304 0.423326642275
0.87658 0.424937526637
0.880856 0.426881145325
0.885132 0.42859817498
0.889408 0.430273920743
0.893684 0.432102611442
0.89796 0.433892851484
0.902236 0.435643827932
0.906512 0.437556694554
0.910788 0.439229019008
0.915064 0.441066284237
0.91934 0.442865744651
0.923616 0.444626621693
0.927892 0.446348133419
0.932168 0.44824571479
0.936444 0.45010723228
0.94072 0.451710831803
0.944996 0.453495528126
0.949272 0.45546799886
0.953548 0.457177842986
0.957824 0.459079020023
0.9621 0.460711080099
0.966376 0.462538091545
0.970652 0.464328227933
0.974928 0.466322199267
0.979204 0.468039077314
0.98348 0.469963642457
0.987756 0.471604480282
0.992032 0.473456919425
0.996308 0.475273616296
1.000584 0.47705390183
1.00486 0.478797104673
1.009136 0.480765443523
1.013412 0.482435224045
1.017688 0.484334357313
1.021964 0.486199325567
1.02624 0.488029501342
1.030516 0.489824255191
1.034792 0.491582955721
1.039068 0.493587621232
1.043344 0.495275209255
1.04762 0.497213320446
1.051896 0.498827321341
1.056172 0.500696469887
1.060448 0.502531715308
1.064724 0.504332468844
1.069 0.506401459971
1.073276 0.508134483555
1.077552 0.509831257938
1.081828 0.511803644548
1.086104 0.513744756016
1.09038 0.515335407893
1.094656 0.517209219896
1.098932 0.51905010693
1.103208 0.520857522571
1.107484 0.522630919133
1.11176 0.524704177303
1.116036 0.526411100791
1.120312 0.528423249258
1.124588 0.530061568628
1.128864 0.532010545909
1.13314 0.533928806202
1.137416 0.535815849458
1.141692 0.537671174623
1.145968 0.539494279669
1.150244 0.541284661619
1.15452 0.543041816577
1.158796 0.544765239752
1.163072 0.546828652395
1.167348 0.548486531282
1.171624 0.550490298502
1.1759 0.552465274655
1.180176 0.554022915879
1.184452 0.55593543684
1.188728 0.557817786292
1.193004 0.559669508856
1.19728 0.5614901485
1.201556 0.563685086915
1.205832 0.56544579513
1.210108 0.567174067107
1.214384 0.56886944443
1.21866 0.570951838608
1.222936 0.572583728121
1.227212 0.574609110864
1.231488 0.576607211229
1.235764 0.57857762359
1.24004 0.58008098837
1.244316 0.581991034106
1.248592 0.583872154015
1.252868 0.585723940823
1.257144 0.587545986898
1.26142 0.589795880951
1.265696 0.591561084891
1.269972 0.593295341539
1.274248 0.594998242033
1.278524 0.597142938652
1.2828 0.598785835802
1.287076 0.600877620517
1.291352 0.602458948943
1.295628 0.60449632821
1.299904 0.606507949146
1.30418 0.608493455877
1.308456 0.609950990036
1.312732 0.611879135934
1.317008 0.613780081012
1.321284 0.615653468823
1.32556 0.617498942822
1.329836 0.619316146381
1.334112 0.621630879348
1.338388 0.62339464368
1.342664 0.625129085253
1.34694 0.626833847286
1.351216 0.629051524059
1.355492 0.630700099705
1.359768 0.632869398519
1.364044 0.634460431945
1.36832 0.636580067847
1.372596 0.63811220352
1.376872 0.640180891752
1.381148 0.642225799062
1.385424 0.644246621954
1.3897 0.645661281986
1.393976 0.647628624304
1.398252 0.649570954714
1.402528 0.651487970061
1.406804 0.653379367311
1.41108 0.655244843561
1.415356 0.657084096057
1.419632 0.658896822216
1.423908 0.660682719634
1.428184 0.663063496922
1.43246 0.664799386991
1.436736 0.666507559398
1.441012 0.668823443951
1.445288 0.670479884105
1.449564 0.67210771965
1.45384 0.674356254047
1.458116 0.675930636416
1.462392 0.678134466368
1.466668 0.679654262051
1.470944 0.681812322002
1.47522 0.683949460178
1.479496 0.685387626143
1.483772 0.687477416323
1.488048 0.689545521682
1.492324 0.691591693854
1.4966 0.692918755024
1.500876 0.694915493961
1.505152 0.696889539972
1.509428 0.698840645835
1.513704 0.700768564635
1.51798 0.702673049774
1.522256 0.704553854987
1.526532 0.706410734352
1.530808 0.708243442306
1.535084 0.710051733653
1.53936 0.711835363582
1.543636 0.714344951477
1.547912 0.716083523997
1.552188 0.717796718707
1.556464 0.719484292394
1.56074 0.721916951589
1.565016 0.723557615747
1.569292 0.725171947356
1.573568 0.727545880288
1.577844 0.729111929339
1.58212 0.731447340118
1.586396 0.732964205628
1.590672 0.735260255505
1.594948 0.736727039952
1.599224 0.738982893234
1.6035 0.740398702742
1.607776 0.742613526961
1.612052 0.744810137753
1.616328 0.746150437567
1.620604 0.74830479162
1.62488 0.750440342212
1.629156 0.752556898286
1.633432 0.753795261029
1.637708 0.755867945272
1.641984 0.75792104995
1.64626 0.759954385658
1.650536 0.761967763408
1.654812 0.763960994644
1.659088 0.765933891246
1.663364 0.767886265542
1.66764 0.769817930316
1.671916 0.77172869882
1.676192 0.773618384779
1.680468 0.775486802403
1.684744 0.777333766395
1.68902 0.779159091963
1.693296 0.780962594824
1.697572 0.782744091218
1.701848 0.784503397913
1.706124 0.787191513487
1.7104 0.788911436104
1.714676 0.790608635555
1.718952 0.792282930742
1.723228 0.794907568551
1.727504 0.79654110837
1.73178 0.79815121675
1.736056 0.800727959771
1.740332 0.802296301186
1.744608 0.803840688915
1.748884 0.806368120347
1.75316 0.807869738868
1.757436 0.81036540756
1.761712 0.811823602182
1.765988 0.813256988253
1.770264 0.815701024106
1.77454 0.817090000416
1.778816 0.819500757918
1.783092 0.821897527225
1.787368 0.823221565161
1.791644 0.825584176838
1.79592 0.826862215875
1.800196 0.829190080899
1.804472 0.831503255558
1.808748 0.832714022284
1.813024 0.834991585505
1.8173 0.837254044728
1.821576 0.838396165994
1.825852 0.840622158071
1.830128 0.842832636746
1.834404 0.845027470023
1.83868 0.846077920539
1.842956 0.848235167395
1.847232 0.850376365266
1.851508 0.852501384024
1.855784 0.854610093998
1.86006 0.856702365983
1.864336 0.858778071244
1.868612 0.859666950062
1.872888 0.861703166475
1.877164 0.863722423259
1.88144 0.865724593714
1.885716 0.867709551638
1.889992 0.869677171334
1.894268 0.871627327615
1.898544 0.873559895811
1.90282 0.875474751774
1.907096 0.87737177188
1.911372 0.87925083304
1.915648 0.881111812702
1.919924 0.882954588857
1.9242 0.886027516068
1.928476 0.887839609598
1.932752 0.889633145236
1.937028 0.891408003098
1.941304 0.893164063873
1.94558 0.894901208822
1.949856 0.896619319785
1.954132 0.899609538652
1.958408 0.901295373891
1.962684 0.902961831829
1.96696 0.904608796573
1.971236 0.906236152838
1.975512 0.909165836778
1.979788 0.910759814133
1.984064 0.91233384795
1.98834 0.915228435788
1.992616 0.916768446862
1.996892 0.918288184342
2.001168 0.921146769127
2.005444 0.92263184923
2.00972 0.924096330803
2.013996 0.926918017236
2.018272 0.928347216232
2.022548 0.929755497007
2.026824 0.932539401764
2.0311 0.933911784423
2.035376 0.936672103064
2.039652 0.938008186586
2.043928 0.940744543207
2.048204 0.942043930748
2.05248 0.943321678796
2.056756 0.946018251755
2.061032 0.947258711266
2.065308 0.94993039217
2.069584 0.952592641158
2.07386 0.953779602384
2.078136 0.956416419877
2.082412 0.957565140742
2.086688 0.960176168189
2.090964 0.961286273645
2.09524 0.963871156134
2.099516 0.964942275672
2.103792 0.967500661983
2.108068 0.970048840076
2.112344 0.971063972343
2.11662 0.973585138242
2.120896 0.976095845534
2.125172 0.977054193987
2.129448 0.979537381004
2.133724 0.982009862537


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2.tex <==
0.0 0.0900282553096
0.00853 0.0900645934754
0.01706 0.090172769951
0.02559 0.0903516162454
0.03412 0.0906000831503
0.04265 0.0909172346294
0.05118 0.0913022420318
0.05971 0.0917543786124
0.06824 0.0922730143419
0.07677 0.0928576109899
0.0853 0.0935077174666
0.09383 0.0942229654065
0.10236 0.0950030649831
0.11089 0.0958478009388
0.11942 0.0967570288196
0.12795 0.0977306714007
0.13648 0.0987687152947
0.14501 0.0998712077291
0.15354 0.101038253486
0.16207 0.10227001199
0.1706 0.103566694546
0.17913 0.104928561701
0.18766 0.106355920743
0.19619 0.107849123312
0.20472 0.10940856313
0.21325 0.111034673827
0.22178 0.112727926882
0.23031 0.114488829646
0.23884 0.116317923459
0.24737 0.118215781851
0.2559 0.120183008826
0.26443 0.122220237213
0.27296 0.124328127098
0.28149 0.126507364313
0.29002 0.128758659001
0.29855 0.131082744228
0.30708 0.133480374663
0.31561 0.135952325305
0.32414 0.138499390266
0.33267 0.141122381601
0.3412 0.143822128183
0.34973 0.146599474623
0.35826 0.149455280234
0.36679 0.152390418031
0.37532 0.155405773772
0.38385 0.15850224503
0.39238 0.16168074031
0.40091 0.164942178185
0.40944 0.168287486473
0.41797 0.171717601441
0.4265 0.175233467038
0.43503 0.178836034151
0.44356 0.182526259894
0.45209 0.186305106917
0.46062 0.19017354274
0.46915 0.194132539111
0.47768 0.198183071385
0.48621 0.202326117922
0.49474 0.206562659507
0.50327 0.210893678792
0.5118 0.215320159751
0.52033 0.219843087155
0.52886 0.224463446067
0.53739 0.229182221348
0.54592 0.234000397183
0.55445 0.238918956622
0.56298 0.243938881131
0.57151 0.249061150164
0.58004 0.25428674074
0.58857 0.259616627045
0.5971 0.265051780033
0.60563 0.270593167048
0.61416 0.276241751458
0.62269 0.281998492292
0.63122 0.287864343897
0.63975 0.293840255602
0.64828 0.299927171391
0.65681 0.302793805764
0.66534 0.302867249126
0.67387 0.302943870435
0.6824 0.303082513628
0.69093 0.303283863577
0.69946 0.303518435722
0.70799 0.303786374453
0.71652 0.304118675545
0.72505 0.304485358715
0.73358 0.304886786418
0.74211 0.305323389329
0.75064 0.305795667791
0.75917 0.306304193363
0.7677 0.306849610486
0.77623 0.307465462797
0.78476 0.30808721985
0.79329 0.308748265715
0.80182 0.30941573574
0.81035 0.310157957034
0.81888 0.310908048022
0.82741 0.31170101014
0.83594 0.312502852185
0.84447 0.313349432856
0.853 0.314242179531
0.86153 0.315109748203
0.87006 0.316061831095
0.87859 0.317026828498
0.88712 0.318005254452
0.89565 0.318997673104
0.90418 0.320043258637
0.91271 0.321105023458
0.92124 0.322183716334
0.92977 0.323280142323
0.9383 0.324395164275
0.94683 0.32552970436
0.95536 0.32672615208
0.96389 0.327903246131
0.97242 0.329103005827
0.98095 0.330369561773
0.98948 0.3316187809
0.99801 0.332850370544
1.00654 0.334153227805
1.01507 0.335440165747
1.0236 0.336802441393
1.03213 0.338104455861
1.04066 0.339485032081
1.04919 0.340852673113
1.05772 0.342255463845
1.06625 0.343646528556
1.07478 0.34507527979
1.08331 0.346493705084
1.09184 0.347952588316
1.10037 0.349402745653
1.1089 0.350896376893
1.11743 0.352383091386
1.12596 0.353863186144
1.13449 0.355391053536
1.14302 0.3569144106
1.15155 0.358489178331
1.16008 0.360005543477
1.16861 0.361575747675
1.17714 0.363202574707
1.18567 0.364771919269
1.1942 0.366341384827
1.20273 0.367971687713
1.21126 0.369605069437
1.21979 0.371242303489
1.22832 0.372884203547
1.23685 0.374531624208
1.24538 0.376185461728
1.25391 0.377846654753
1.26244 0.379516185053
1.27097 0.381261795291
1.2795 0.38295200306
1.28803 0.384653770518
1.29656 0.386368259304
1.30509 0.388096677812
1.31362 0.389840281909
1.32215 0.391528202453
1.33068 0.393305189835
1.33921 0.395027330408
1.34774 0.396843265784
1.35627 0.398605345667
1.3648 0.400389170778
1.37333 0.402118283342
1.38186 0.40394935187
1.39039 0.405726956068
1.39892 0.407530822786
1.40745 0.409362703245
1.41598 0.41122440384
1.42451 0.41303348801
1.43304 0.414874000845
1.44157 0.416661402076
1.4501 0.418569536551
1.45863 0.420337661201
1.46716 0.422230612001
1.47569 0.424071954753
1.48422 0.425952553077
1.49275 0.427874623891
1.50128 0.429745960098
1.50981 0.431565326085
1.51834 0.433525227979
1.52687 0.435337422978
1.5354 0.437294988334
1.54393 0.439203001405
1.55246 0.441060282097
1.56099 0.442968710898
1.56952 0.444930913435
1.57805 0.446843946998
1.58658 0.448813598483
1.59511 0.450734405483
1.60364 0.452605242848
1.61217 0.454535879203
1.6207 0.456529216761
1.62923 0.458474612723
1.63776 0.460370982809
1.64629 0.462333603904
1.65482 0.464365569453
1.66335 0.466350862999
1.67188 0.468288444407
1.68041 0.47017726768
1.68894 0.47226324202
1.69747 0.474179242026
1.706 0.476172686977
1.71453 0.478119097078
1.72306 0.480146864358
1.73159 0.482128602448
1.74012 0.484195762467
1.74865 0.486084035892
1.75718 0.488194366069
1.76571 0.490123900012
1.77424 0.492144287468
1.78277 0.494119085034
1.7913 0.496189189709
1.79983 0.498215052136
1.80836 0.500195765124
1.81689 0.502277123142
1.82542 0.504314803555
1.83395 0.506307923509
1.84248 0.508407291608
1.85101 0.510463697951
1.85954 0.512476285089
1.86807 0.514444191897
1.8766 0.516525080936
1.88513 0.518563035441
1.89366 0.520557220936
1.90219 0.522670586997
1.91072 0.5247420623
1.91925 0.526770839993
1.92778 0.528925275337
1.93631 0.530868041936
1.94484 0.53293849824
1.95337 0.535141357402
1.9619 0.537128372788
1.97043 0.53924996047
1.97896 0.541330709201
1.98749 0.543369864729
1.99602 0.545550748515
2.00455 0.547506366432
2.01308 0.549606062215
2.02161 0.551665031498
2.03014 0.55387439482
2.03867 0.555851698284
2.0472 0.55798190862
2.05573 0.560072480245
2.06426 0.562322545037
2.07279 0.564333768483
2.08132 0.566507163787
2.08985 0.568642234158
2.09838 0.570738311538
2.10691 0.572794725995
2.11544 0.574810805744
2.12397 0.577000182416
2.1325 0.579152116071
2.14103 0.581265968658
2.14956 0.583341100487
2.15809 0.585599738402
2.16662 0.587597676265
2.17515 0.589782206204
2.18368 0.591929853342
2.19221 0.594040009535
2.20074 0.596112065244
2.20927 0.598381518332
2.2178 0.600377791632
2.22633 0.602574768891
2.23486 0.604735765909
2.24339 0.606860206057
2.25192 0.608947511547
2.26045 0.611246929877
2.26898 0.613260560418
2.27751 0.615489834213
2.28604 0.617684382144
2.29457 0.619843660537
2.3031 0.62196712477
2.31163 0.624054229295
2.32016 0.626370860873
2.32869 0.62838603081
2.33722 0.630634509298
2.34575 0.632849353658
2.35428 0.635030053662
2.36281 0.637176098343
2.37134 0.639286976028
2.37987 0.641645862772
2.3884 0.643687386414
2.39693 0.645980954504
2.40546 0.648242403844
2.41399 0.650177420011
2.42252 0.652370634669
2.43105 0.654829283217
2.43958 0.656957498789
2.44811 0.659051213685
2.45664 0.661416773773
2.46517 0.663442689754
2.4737 0.665744793064
2.48223 0.668015820371
2.49076 0.670255331691
2.49929 0.67246288671
2.50782 0.674638044804
2.51635 0.676780365061
2.52488 0.678889406299
2.53341 0.681295750283
2.54194 0.683339663378
2.55047 0.685685530436
2.559 0.688001925464
2.56753 0.689946327139
2.57606 0.692199762729
2.58459 0.694422503934
2.59312 0.696614147408
2.60165 0.699127711737
2.61018 0.701258807902
2.61871 0.703357608877
2.62724 0.705785747113
2.63577 0.707821644521
2.6443 0.710191892503
2.65283 0.71253409041
2.66136 0.714847873668
2.66989 0.717132877749
2.67842 0.719388738191
2.68695 0.721615090608
2.69548 0.723811570714
2.70401 0.725977814333
2.71254 0.728113457422
2.72107 0.730612750004
2.7296 0.732689139762
2.73813 0.735134554811
2.74666 0.737150288682
2.75519 0.739540475913
2.76372 0.741904088098
2.77225 0.744240801145
2.78078 0.746550291202
2.78931 0.748832234677
2.79784 0.751086308251
2.80637 0.753312188894
2.8149 0.755509553882
2.82343 0.757678080807
2.83196 0.760252557327
2.84049 0.762365646815
2.84902 0.764890475546
2.85755 0.766946893219
2.86608 0.769420892155
2.87461 0.771870660618
2.88314 0.773841396923
2.89167 0.776238581174
2.9002 0.778610678633
2.90873 0.780957408954
2.91726 0.783278492255
2.92579 0.785573649132
2.93432 0.787842600671
2.94285 0.790085068467
2.95138 0.792781878241
2.95991 0.794973925165
2.96844 0.797138668916
2.97697 0.799767111132
2.9855 0.801879837884
2.99403 0.804462569668
3.00256 0.806522229481
3.01109 0.809058253449
3.01962 0.811572283373
3.02815 0.813552125005
3.03668 0.816017972931
3.04521 0.818461111389
3.05374 0.820881307413
3.06227 0.82327832874
3.0708 0.825651943822
3.07933 0.82800192185
3.08786 0.830328032761
3.09639 0.832630047262
3.10492 0.834907736839
3.11345 0.837708289782
3.12198 0.839940261364
3.13051 0.842147239804
3.13904 0.844887291864
3.14757 0.847047260732
3.1561 0.849747179259
3.16463 0.851859294516
3.17316 0.854518288701
3.18169 0.856581713633
3.19022 0.859199000176
3.19875 0.861797002462
3.20728 0.863787709118
3.21581 0.866342855977
3.22434 0.86887816788
3.23287 0.871393467515
3.2414 0.873888578679
3.24993 0.876363326299
3.25846 0.878817536457
3.26699 0.881251036418
3.27552 0.883663654649
3.28405 0.88605522085
3.29258 0.88842556598
3.30111 0.891404246883
3.30964 0.893735531148
3.31817 0.896045107559
3.3267 0.898332812402
3.33523 0.901243810574
3.34376 0.903491220151
3.35229 0.906369489014
3.36082 0.908576016104
3.36935 0.911421024746
3.37788 0.913586094553
3.38641 0.916397324994
3.39494 0.91852037575
3.40347 0.921297323583
3.412 0.924058959593
3.42053 0.926119982273
3.42906 0.928846618783
3.43759 0.931557612656
3.44612 0.934252861885
3.45465 0.936230774285
3.46318 0.938890131513
3.47171 0.941533438087
3.48024 0.944160600788
3.48877 0.946771528766
3.4973 0.949366133608
3.50583 0.951944329411
3.51436 0.954506032858
3.52289 0.957051163298
3.53142 0.960318552287
3.53995 0.962834529465
3.54848 0.965333721987
3.55701 0.9678160608
3.56554 0.970281479972
3.57407 0.973490071976
3.5826 0.975925758746
3.59113 0.978344361742
3.59966 0.981518892426
3.60819 0.983907508256
3.61672 0.986278908904
3.62525 0.989419152014
3.63378 0.991760380633
3.64231 0.994879155629
3.65084 0.997190141451
3.65937 1.00028745388
3.6679 1.00337626243
3.67643 1.00564405955
3.68496 1.00871150529
3.69349 1.0117705443
3.70202 1.01399526577
3.71055 1.01703314505
3.71908 1.02006277048
3.72761 1.02224469124
3.73614 1.02525347755
3.74467 1.02825422648
3.7532 1.03124703131
3.76173 1.03423199398
3.77026 1.03720922551
3.77879 1.04017884642
3.78732 1.04226927026
3.79585 1.04521940623
3.80438 1.04816233782
3.81291 1.05109822878
3.82144 1.05402725522
3.82997 1.05694960635
3.8385 1.06076546944
3.84703 1.06367987045
3.85556 1.06658826987
3.86409 1.06949091793
3.87262 1.07238808249
3.88115 1.07528005012
3.88968 1.07816712737
3.89821 1.08198347476
3.90674 1.08486669947
3.91527 1.08774611
3.9238 1.0915707619
3.93233 1.09444876839
3.94086 1.09732427673
3.94939 1.10116146736
3.95792 1.10403856002
3.96645 1.10691476936
3.97498 1.11076965344
3.98351 1.11365111315
3.99204 1.11752293959
4.00057 1.12041257964
4.0091 1.12430461315
4.01763 1.12720582218
4.02616 1.13112183731
4.03469 1.1340385552
4.04322 1.13798294219
4.05175 1.14091977883
4.06028 1.14489768012
4.06881 1.14786006996
4.07734 1.15187755938
4.08587 1.15592024976
4.0944 1.15893628831
4.10293 1.16303001667
4.11146 1.16715560562
4.11999 1.17131577345
4.12852 1.17443677378
4.13705 1.17866966537
4.14558 1.18294726742
4.15411 1.18727386008
4.16264 1.19055369793
4.17117 1.19498743649
4.1797 1.19948694816
4.18823 1.20405971805
4.19676 1.20871456253
4.20529 1.21232977173
4.21382 1.21717588683
4.22235 1.2221428803
4.23088 1.22725050413
4.23941 1.23252433471
4.24794 1.23799868254
4.25647 1.24372181311


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt05.tex <==
0.0 0.063045006828
0.008276 0.0630929904667
0.016552 0.0632354443447
0.024828 0.0634703466344
0.033104 0.0637959686838
0.04138 0.0642108544897
0.049656 0.0647138017242
0.057932 0.0653038441889
0.066208 0.0659802355847
0.074484 0.0667424344872
0.08276 0.0675900904331
0.091036 0.068523031026
0.099312 0.0695412499786
0.107588 0.070644896016
0.115864 0.0718342625686
0.12414 0.0731097781919
0.132416 0.0744719976537
0.140692 0.0759215936348
0.148968 0.0774593489937
0.157244 0.0790861495514
0.16552 0.0808029773532
0.173796 0.082610904371
0.182072 0.0845110866125
0.190348 0.086504758603
0.198624 0.0885932282147
0.2069 0.0907778718145
0.215176 0.0930601297069
0.223452 0.0954415018518
0.231728 0.0979235438341
0.240004 0.10050786307
0.24828 0.103196115229
0.256556 0.105990000863
0.264832 0.108891262221
0.273108 0.111901680239
0.281384 0.115023071697
0.28966 0.118257286525
0.297936 0.121606205258
0.306212 0.125071736616
0.314488 0.128655815218
0.322764 0.132360399404
0.33104 0.136187469179
0.339316 0.140139024244
0.347592 0.14421708214
0.355868 0.148423676473
0.364144 0.152760855224
0.37242 0.157230679148
0.380696 0.161835220241
0.388972 0.166576560278
0.397248 0.171456789427
0.405524 0.176478004915
0.4138 0.181642309765
0.422076 0.186951811581
0.430352 0.192408621392
0.438628 0.198014852543
0.446904 0.203772619636
0.45518 0.209684037519
0.463456 0.212450042882
0.471732 0.212503564887
0.480008 0.212630779006
0.488284 0.212811034847
0.49656 0.213044783834
0.504836 0.213332660738
0.513112 0.213675487716
0.521388 0.214074279036
0.529664 0.214507348379
0.53794 0.215021612386
0.546216 0.21554908769
0.554492 0.216137343875
0.562768 0.216764238301
0.571044 0.217430981572
0.57932 0.218138951783
0.587596 0.218889700516
0.595872 0.219684959207
0.604148 0.220500712929
0.612424 0.221364217278
0.6207 0.222251015722
0.628976 0.223189484925
0.637252 0.224154704804
0.645528 0.225148227731
0.653804 0.226171759
0.66208 0.227227162512
0.670356 0.228316466643
0.678632 0.229411966324
0.686908 0.230544934876
0.695184 0.23171789067
0.70346 0.232902090903
0.711736 0.234098812578
0.720012 0.235341996185
0.728288 0.236601756286
0.736564 0.237879786547
0.74484 0.239177916262
0.753116 0.240498114867
0.761392 0.24184249652
0.769668 0.243213324746
0.777944 0.244576227336
0.78622 0.245969247312
0.794496 0.247395080919
0.802772 0.248817777757
0.811048 0.250277779646
0.819324 0.251738019879
0.8276 0.253199650545
0.835876 0.254705630565
0.844152 0.256217119382
0.852428 0.257735613111
0.860704 0.259262714822
0.86898 0.260844976112
0.877256 0.262395363996
0.885532 0.263959855129
0.893808 0.265540509932
0.902084 0.267139510515
0.91036 0.268759163664
0.918636 0.270401903818
0.926912 0.272019404457
0.935188 0.273663401841
0.943464 0.275283923996
0.95174 0.276988453438
0.960016 0.278618861217
0.968292 0.280339454001
0.976568 0.281986455602
0.984844 0.283730305565
0.99312 0.285401396874
1.001396 0.287116707356
1.009672 0.288880002702
1.017948 0.29057129733
1.026224 0.292314167418
1.0345 0.294048579085
1.042776 0.295840743362
1.051052 0.297562145337
1.059328 0.299345629734
1.067604 0.301127027398
1.07588 0.302907553069
1.084156 0.30468849215
1.092432 0.306471202
1.100708 0.308257113241
1.108984 0.310122758727
1.11726 0.311920956153
1.125536 0.313727117031
1.133812 0.31554297801
1.142088 0.317370355395
1.150364 0.319211146416
1.15864 0.321067330481
1.166916 0.322856520378
1.175192 0.324748344446
1.183468 0.326574681506
1.191744 0.328422245704
1.20002 0.330293388971
1.208296 0.33219055228
1.216572 0.334023031535
1.224848 0.335883624852
1.233124 0.337774989293
1.2414 0.339699875218
1.249676 0.341561662142
1.257952 0.343459543802
1.266228 0.34529380503
1.274504 0.347271261847
1.28278 0.349082021642
1.291056 0.351042303168
1.299332 0.352941702541
1.307608 0.354889571106
1.315884 0.356776522111
1.32416 0.358715434065
1.332436 0.360593526915
1.340712 0.36252728625
1.348988 0.364400462824
1.357264 0.366333229971
1.36554 0.368329487321
1.373816 0.370267666713
1.382092 0.372146184502
1.390368 0.374092836674
1.398644 0.376111832535
1.40692 0.37807419884
1.415196 0.379978423605
1.423472 0.38196025655
1.431748 0.383884932117
1.440024 0.385750966511
1.4483 0.387843658356
1.456576 0.389737558686
1.464852 0.391720132543
1.473128 0.39364658018
1.481404 0.395667343491
1.48968 0.397633479437
1.497956 0.39954361974
1.506232 0.401554802777
1.514508 0.403511685064
1.522784 0.405412934829
1.53106 0.407422378634
1.539336 0.409378086537
1.547612 0.411448539983
1.555888 0.413467334395
1.564164 0.415433224369
1.57244 0.417344957619
1.580716 0.419380521543
1.588992 0.421364245196
1.597268 0.423294919054
1.605544 0.425357904267
1.61382 0.427370373694
1.622096 0.429331162511
1.630372 0.431433203979
1.638648 0.433289664363
1.646924 0.435290164918
1.6552 0.437441304649
1.663476 0.439340917908
1.671752 0.441394185959
1.680028 0.443398206916
1.688304 0.445351900688
1.69658 0.447469320637
1.704856 0.449321827395
1.713132 0.451341375893
1.721408 0.453535185442
1.729684 0.455458229026
1.73796 0.457559087677
1.746236 0.459613388369
1.754512 0.461620145632
1.762788 0.463578369951
1.771064 0.465487067831
1.77934 0.467588672162
1.787616 0.469644655206
1.795892 0.471654078437
1.804168 0.47361599975
1.812444 0.475784850693
1.82072 0.477651969672
1.828996 0.47973024701
1.837272 0.481763416749
1.845548 0.483750586957
1.853824 0.48596168237
1.8621 0.487857321129
1.870376 0.489981444314
1.878652 0.492062395686
1.886928 0.494099336018
1.895204 0.496091423372
1.90348 0.498037813153
1.911756 0.500231054373
1.920032 0.50208682042
1.928308 0.50419441417
1.936584 0.50625965276
1.94486 0.508281747241
1.953136 0.510570116236
1.961412 0.512506977542
1.969688 0.514398337317
1.977964 0.516563970378
1.98624 0.518689504665
1.994516 0.520774206886
2.002792 0.522817341852
2.011068 0.524818172528
2.019344 0.526775960071
2.02762 0.529031885852
2.035896 0.530905001577
2.044172 0.533082092541
2.052448 0.535220559842
2.060724 0.537319725017
2.069 0.539378908108
2.077276 0.541397427707
2.085552 0.543374600995
2.093828 0.545309743782
2.102104 0.547577672693
2.11038 0.549430542375
2.118656 0.551622562113
2.126932 0.553777609315
2.135208 0.555895062384
2.143484 0.557974298612
2.15176 0.560014694215
2.160036 0.562015624375
2.168312 0.563976463274
2.176588 0.566307535958
2.184864 0.568190364552
2.19314 0.570450324681
2.201416 0.572252720311
2.209692 0.574439233415
2.217968 0.576590218687
2.226244 0.578705113008
2.23452 0.580783352532
2.242796 0.582824372719
2.251072 0.584827608368
2.259348 0.58679249365
2.267624 0.589175272764
2.2759 0.591066063639
2.284176 0.593382272741
2.292452 0.595196790359
2.300728 0.597444339637
2.309004 0.599658973174
2.31728 0.601357196984
2.325556 0.603500051658
2.333832 0.605608463244
2.342108 0.607681929427
2.350384 0.609719947556
2.35866 0.611722014672
2.366936 0.614197621159
2.375212 0.616130855536
2.383488 0.618026651022
2.391764 0.620408303323
2.40004 0.622232355915
2.408316 0.624550596175
2.416592 0.62683878745
2.424868 0.628553969339
2.433144 0.630776013884
2.44142 0.63296667507
2.449696 0.635125515339
2.457972 0.637252097055
2.466248 0.639345982533
2.474524 0.64140673406
2.4828 0.643433913924
2.491076 0.645427084436
2.499352 0.647385807954
2.507628 0.649900540968
2.515904 0.65179401676
2.52418 0.654252589128
2.532456 0.656079155769
2.540732 0.658479994285
2.549008 0.660237991196
2.557284 0.662579523393
2.56556 0.664267291206
2.573836 0.666547945714
2.582112 0.668800139401
2.590388 0.671023501647
2.598664 0.673217662006
2.60694 0.675382250225
2.615216 0.677516896271
2.623492 0.679621230343
2.631768 0.6816948829
2.640044 0.683737484676
2.64832 0.685748666703
2.656596 0.687728060329
2.664872 0.68967529724
2.673148 0.692284211456
2.681424 0.694171421949
2.6897 0.696025394114
2.697976 0.698556197271
2.706252 0.700348046404
2.714528 0.702826942706
2.722804 0.70455528882
2.73108 0.706980983435
2.739356 0.709382360691
2.747632 0.711015650899
2.755908 0.713361910587
2.764184 0.715682927732
2.77246 0.717978401564
2.780736 0.719482129617
2.789012 0.721719956606
2.797288 0.723931320026
2.805564 0.726115920811
2.81384 0.728273460343
2.822116 0.730403640471
2.830392 0.732506163529
2.838668 0.734580732347
2.846944 0.736627050268
2.85522 0.739462385777
2.863496 0.741457154465
2.871772 0.743422805326
2.880048 0.74535904385
2.888324 0.747265576117
2.8966 0.749989071161
2.904876 0.75184125032
2.913152 0.75452172221
2.921428 0.7563184578
2.929704 0.758084065613
2.93798 0.760695101949
2.946256 0.762403619724
2.954532 0.764969094913
2.962808 0.767514450069
2.971084 0.769138358018
2.97936 0.771636672744
2.987636 0.773200822194
2.995912 0.77565110337
3.004188 0.778080079698
3.012464 0.780487523345
3.02074 0.781935168693
3.029016 0.784292644427
3.037292 0.786627888876
3.045568 0.788940676496
3.053844 0.791230782328
3.06212 0.793497982008
3.070396 0.794766409404
3.078672 0.796980795718
3.086948 0.799171588536
3.095224 0.801338566063
3.1035 0.803481507154
3.111776 0.806607664391
3.120052 0.808708291199
3.128328 0.810784239726
3.136604 0.812835291468
3.14488 0.814861228627
3.153156 0.816861834122
3.161432 0.818836891598
3.169708 0.821838956966
3.177984 0.82376881299
3.18626 0.825672493432
3.194536 0.827549784871
3.202812 0.830479507309
3.211088 0.832309991924
3.219364 0.83411346871
3.22764 0.836988631315
3.235916 0.838744120502
3.244192 0.841584222878
3.252468 0.843290955519
3.260744 0.846095297186
3.26902 0.847752510132
3.277296 0.850520395853
3.285572 0.852127331898
3.293848 0.854858071822
3.302124 0.856413979851
3.3104 0.85910688966
3.318676 0.860611024793
3.326952 0.863265425838
3.335228 0.865903742849
3.343504 0.86733226902
3.35178 0.869931085654
3.360056 0.872513348789
3.368332 0.873864672576
3.376608 0.876406456787
3.384884 0.878931224325
3.39316 0.881438827216
3.401436 0.883929118165
3.409712 0.885152947892
3.417988 0.887601178988
3.426264 0.890031645796
3.43454 0.8924442039
3.442816 0.894838709609
3.451092 0.897215019959
3.459368 0.899572992723
3.467644 0.901912486421
3.47592 0.902927972114
3.484196 0.905222974558
3.492472 0.907499064057
3.500748 0.909756102274
3.509024 0.911993951657
3.5173 0.91421247545
3.525576 0.9164115377
3.533852 0.919946464518
3.542128 0.922113407093
3.550404 0.924260498615
3.55868 0.926387606347
3.566956 0.928494598399
3.575232 0.930581343729
3.583508 0.93264771216
3.591784 0.934693574382
3.60006 0.938132292941
3.608336 0.94014407175
3.616612 0.942134974564
3.624888 0.944104875558
3.633164 0.946053649818
3.64144 0.949431352051
3.649716 0.951344878641
3.657992 0.953236921789
3.666268 0.956579699541
3.674544 0.958435827014
3.68282 0.960270122421
3.691096 0.962082467322
3.699372 0.965374805371
3.707648 0.967150360513
3.715924 0.970420618321
3.7242 0.972158969633
3.732476 0.973874816873
3.740752 0.977107525041
3.749028 0.978785549361
3.757304 0.981995271442
3.76558 0.983635077487
3.773856 0.986821468246
3.782132 0.9884226684
3.790408 0.990000633021
3.798684 0.993147604516
3.80696 0.994686385436
3.815236 0.99780918391
3.823512 1.00092358371
3.831788 1.00240672073
3.840064 1.00549648373
3.84834 1.00693954561
3.856616 1.01000436539
3.864892 1.01140700613
3.873168 1.01444658471
3.881444 1.01747727948
3.88972 1.01882251539
3.897996 1.02182754903
3.906272 1.02313154927
3.914548 1.02611064596
3.922824 1.02908054594
3.9311 1.03032599018
3.939376 1.03326956762
3.947652 1.03620377664
3.955928 1.03912856588
3.964204 1.04029754708
3.97248 1.04319554092
3.980756 1.0460839582
3.989032 1.0489627527
3.997308 1.05005424237
4.005584 1.05290581041
4.01386 1.05574761503
4.022136 1.05857961558
4.030412 1.05959267326
4.038688 1.06239706141
4.046964 1.06519152239
4.05524 1.06797602163
4.063516 1.07075052617
4.071792 1.0735150047
4.080068 1.07441283562
4.088344 1.07714922614
4.09662 1.07987549691
4.104896 1.08259162364
4.113172 1.08529758388
4.121448 1.0879933571
4.129724 1.09067892476


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt1.tex <==
0.0 0.667616837054
0.0841218682305 0.672852075515
0.168243736461 0.688044582385
0.252365604692 0.712701125396
0.336487472922 0.746158671838
0.420609341153 0.787679970271
0.504731209383 0.836219008942
0.588853077614 0.890833907482
0.672974945844 0.950212032527
0.757096814075 1.01377162623
0.841218682305 1.0810332708
0.925340550536 1.15075696393
1.00946241877 1.22293118237
1.093584287 1.29677003707
1.17770615523 1.37245400874
1.26182802346 1.44965750716
1.34594989169 1.5279938986
1.43007175992 1.60713440563
1.51419362815 1.68703332162
1.59831549638 1.76825759909
1.68243736461 1.84967668353
1.76655923284 1.93213604894
1.85068110107 2.01636548398
1.9348029693 2.09934671387
2.01892483753 2.18428424866
2.10304670576 2.26898060596
2.18716857399 2.3546113305
2.27129044222 2.44011892237
2.35541231046 2.52636666536
2.43953417869 2.6141897773
2.52365604692 2.70172631064
2.60777791515 2.78932522965
2.69189978338 2.88002720961
2.77602165161 2.96840581225
2.86014351984 3.06004366061
2.94426538807 3.14885446937
3.0283872563 3.24328274545
3.11250912453 3.33362000864
3.19663099276 3.42797363904
3.28075286099 3.52506993351
3.36487472922 3.62016798946
3.44899659745 3.7172212282
3.53311846568 3.81648788735
3.61724033391 3.91743145217
3.70136220214 4.01855051764
3.78548407037 4.12265104793
3.8696059386 4.23030852394
3.95372780684 4.33917717162
4.03784967507 4.45010006914
4.1219715433 4.56498180311


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt3.tex <==
0.0 1.18705533876
0.0608288216233 1.18878960072
0.121657643247 1.1938197879
0.18248646487 1.20219676905
0.243315286493 1.21354510197
0.304144108116 1.22801966935
0.36497292974 1.24571095471
0.425801751363 1.26638778559
0.486630572986 1.28999358549
0.54745939461 1.31635415887
0.608288216233 1.34554259515
0.669117037856 1.3775324817
0.72994585948 1.41169043461
0.790774681103 1.44843553006
0.851603502726 1.48728824882
0.912432324349 1.52839953683
0.973261145973 1.57128270743
1.0340899676 1.61578679094
1.09491878922 1.6621974226
1.15574761084 1.70991858466
1.21657643247 1.75942198422
1.27740525409 1.81015198404
1.33823407571 1.86188038039
1.39906289734 1.91528329884
1.45989171896 1.96926658294
1.52072054058 2.02506503537
1.58154936221 2.08146756031
1.64237818383 2.13869973711
1.70320700545 2.19702944566
1.76403582708 2.25612387324
1.8248646487 2.31622107609
1.88569347032 2.3768818732
1.94652229195 2.43899619488
2.00735111357 2.5013203355
2.06817993519 2.5654661761
2.12900875682 2.62924282069
2.18983757844 2.69422500026
2.25066640006 2.76044309863
2.31149522169 2.82700014782
2.37232404331 2.8954761347
2.43315286493 2.96391994636
2.49398168656 3.03286217469
2.55481050818 3.10366991147
2.6156393298 3.17484528048
2.67646815143 3.24743244809
2.73729697305 3.32038373172
2.79812579467 3.39508464724
2.85895461629 3.47055376252
2.91978343792 3.54777289321
2.98061225954 3.62714100814


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2prob0pt6.tex <==
0.0 1.74826716143
0.0396220919817 1.74879512228
0.0792441839634 1.75029653747
0.118866275945 1.75306628167
0.158488367927 1.75666139316
0.198110459909 1.76149461
0.23773255189 1.76724158239
0.277354643872 1.77400758023
0.316976735854 1.78189769123
0.356598827835 1.79071424281
0.396220919817 1.80071656853
0.435843011799 1.81170894849
0.475465103781 1.82381040736
0.515087195762 1.83682846183
0.554709287744 1.85106610502
0.594331379726 1.86617998573
0.633953471707 1.88250574517
0.673575563689 1.89971017531
0.713197655671 1.91817054003
0.752819747653 1.93738344301
0.792441839634 1.95776346673
0.832063931616 1.97899997229
0.871686023598 2.00136470466
0.911308115579 2.02455641797
0.950930207561 2.04867602809
0.990552299543 2.0736325817
1.03017439152 2.09955819706
1.06979648351 2.126383822
1.10941857549 2.15381230109
1.14904066747 2.18223725718
1.18866275945 2.21137227531
1.22828485143 2.2414068084
1.26790694341 2.27204696169
1.3075290354 2.3034962295
1.34715112738 2.33571596055
1.38677321936 2.36839627566
1.42639531134 2.40203254425
1.46601740332 2.43603507492
1.50563949531 2.47091510746
1.54526158729 2.5063451711
1.58488367927 2.54226795163
1.62450577125 2.57891958918
1.66412786323 2.61623906891
1.70374995521 2.65415296521
1.7433720472 2.69257345162
1.78299413918 2.7317116917
1.82261623116 2.77113496945
1.86223832314 2.81166060198
1.90186041512 2.85314223671
1.9414825071 2.89574201706


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma2pt01.tex <==
0.0 0.667616837054
0.0841218682305 0.672852075515
0.168243736461 0.688044582385
0.252365604692 0.712701125396
0.336487472922 0.746158671838
0.420609341153 0.787679970271
0.504731209383 0.836219008942
0.588853077614 0.890833907482
0.672974945844 0.950212032527
0.757096814075 1.01377162623
0.841218682305 1.0810332708
0.925340550536 1.15075696393
1.00946241877 1.22293118237
1.093584287 1.29677003707
1.17770615523 1.37245400874
1.26182802346 1.44965750716
1.34594989169 1.5279938986
1.43007175992 1.60713440563
1.51419362815 1.68703332162
1.59831549638 1.76825759909
1.68243736461 1.84967668353
1.76655923284 1.93213604894
1.85068110107 2.01636548398
1.9348029693 2.09934671387
2.01892483753 2.18428424866
2.10304670576 2.26898060596
2.18716857399 2.3546113305
2.27129044222 2.44011892237
2.35541231046 2.52636666536
2.43953417869 2.6141897773
2.52365604692 2.70172631064
2.60777791515 2.78932522965
2.69189978338 2.88002720961
2.77602165161 2.96840581225
2.86014351984 3.06004366061
2.94426538807 3.14885446937
3.0283872563 3.24328274545
3.11250912453 3.33362000864
3.19663099276 3.42797363904
3.28075286099 3.52506993351
3.36487472922 3.62016798946
3.44899659745 3.7172212282
3.53311846568 3.81648788735
3.61724033391 3.91743145217
3.70136220214 4.01855051764
3.78548407037 4.12265104793
3.8696059386 4.23030852394
3.95372780684 4.33917717162
4.03784967507 4.45010006914
4.1219715433 4.56498180311


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma4prob0pt3.tex <==
0.0 2.37411067752
0.121657643247 2.37757920143
0.243315286493 2.3876395758
0.36497292974 2.40439353809
0.486630572986 2.42709020395
0.608288216233 2.4560393387
0.72994585948 2.49142190942
0.851603502726 2.53277557117
0.973261145973 2.57998717097
1.09491878922 2.63270831774
1.21657643247 2.69108519031
1.33823407571 2.7550649634
1.45989171896 2.82338086923
1.58154936221 2.89687106012
1.70320700545 2.97457649765
1.8248646487 3.05679907367
1.94652229195 3.14256541486
2.06817993519 3.23157358187
2.18983757844 3.32439484521
2.31149522169 3.41983716933
2.43315286493 3.51884396844
2.55481050818 3.62030396808
2.67646815143 3.72376076078
2.79812579467 3.83056659767
2.91978343792 3.93853316587
3.04144108116 4.05013007075
3.16309872441 4.16293512062
3.28475636766 4.27739947422
3.4064140109 4.39405889132
3.52807165415 4.51224774648
3.6497292974 4.63244215218
3.77138694064 4.7537637464
3.89304458389 4.87799238976
4.01470222714 5.002640671
4.13635987038 5.13093235221
4.25801751363 5.25848564139
4.37967515688 5.38845000052
4.50133280012 5.52088619727
4.62299044337 5.65400029565
4.74464808662 5.7909522694
4.86630572986 5.92783989273
4.98796337311 6.06572434938
5.10962101636 6.20733982293
5.2312786596 6.34969056096
5.35293630285 6.49486489618
5.4745939461 6.64076746344
5.59625158934 6.79016929448
5.71790923259 6.94110752504
5.83956687584 7.09554578643
5.96122451908 7.25428201627


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt3.tex <==
0.0 4.74822135504
0.243315286493 4.75515840287
0.486630572986 4.77527915161
0.72994585948 4.80878707619
0.973261145973 4.85418040789
1.21657643247 4.91207867741
1.45989171896 4.98284381883
1.70320700545 5.06555114234
1.94652229195 5.15997434194
2.18983757844 5.26541663549
2.43315286493 5.38217038061
2.67646815143 5.5101299268
2.91978343792 5.64676173845
3.16309872441 5.79374212024
3.4064140109 5.9491529953
3.6497292974 6.11359814733
3.89304458389 6.28513082972
4.13635987038 6.46314716375
4.37967515688 6.64878969041
4.62299044337 6.83967433865
4.86630572986 7.03768793689
5.10962101636 7.24060793616
5.35293630285 7.44752152156
5.59625158934 7.66113319534
5.83956687584 7.87706633174
6.08288216233 8.10026014149
6.32619744882 8.32587024124
6.56951273532 8.55479894844
6.81282802181 8.78811778265
7.0561433083 9.02449549295
7.2994585948 9.26488430437
7.54277388129 9.50752749281
7.78608916778 9.75598477952
8.02940445428 10.005281342
8.27271974077 10.2618647044
8.51603502726 10.5169712828
8.75935031375 10.776900001
9.00266560025 11.0417723945
9.24598088674 11.3080005913
9.48929617323 11.5819045388
9.73261145973 11.8556797855
9.97592674622 12.1314486988
10.2192420327 12.4146796459
10.4625573192 12.6993811219
10.7058726057 12.9897297924
10.9491878922 13.2815349269
11.1925031787 13.580338589
11.4358184652 13.8822150501
11.6791337517 14.1910915729
11.9224490382 14.5085640325


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt6.tex <==
0.0 6.9930686457
0.158488367927 6.99518048911
0.316976735854 7.00118614987
0.475465103781 7.01226512668
0.633953471707 7.02664557265
0.792441839634 7.04597843998
0.950930207561 7.06896632957
1.10941857549 7.09603032094
1.26790694341 7.12759076492
1.42639531134 7.16285697123
1.58488367927 7.20286627411
1.7433720472 7.24683579396
1.90186041512 7.29524162945
2.06034878305 7.34731384731
2.21883715098 7.40426442008
2.3773255189 7.4647199429
2.53581388683 7.53002298067
2.69430225476 7.59884070123
2.85279062268 7.67268216014
3.01127899061 7.74953377203
3.16976735854 7.83105386691
3.32825572646 7.91599988915
3.48674409439 8.00545881862
3.64523246232 8.09822567189
3.80372083024 8.19470411235
3.96220919817 8.29453032679
4.1206975661 8.39823278822
4.27918593403 8.505535288
4.43767430195 8.61524920438
4.59616266988 8.72894902873
4.75465103781 8.84548910123
4.91313940573 8.9656272336
5.07162777366 9.08818784677
5.23011614159 9.21398491799
5.38860450951 9.34286384218
5.54709287744 9.47358510264
5.70558124537 9.60813017699
5.86406961329 9.74414029969
6.02255798122 9.88366042983
6.18104634915 10.0253806844
6.33953471707 10.1690718065
6.498023085 10.3156783567
6.65651145293 10.4649562757
6.81499982086 10.6166118608
6.97348818878 10.7702938065
7.13197655671 10.9268467668
7.29046492464 11.0845398778
7.44895329256 11.2466424079
7.60744166049 11.4125689468
7.76593002842 11.5829680682


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt7.tex <==
0.0 7.65201087312
0.132433347565 7.6531464162
0.26486669513 7.65746418317
0.397300042696 7.66421160717
0.529733390261 7.67365991293
0.662166737826 7.68553077287
0.794600085391 7.70005456047
0.927033432956 7.71745018199
1.05946678052 7.73792988816
1.19190012809 7.76061554826
1.32433347565 7.78569238657
1.45676682322 7.81390069692
1.58920017078 7.84488971493
1.72163351835 7.8788625844
1.85406686591 7.91546472808
1.98650021348 7.95491058722
2.11893356104 7.99743383461
2.25136690861 8.04269816381
2.38380025617 8.09036218181
2.51623360374 8.14129831812
2.6486669513 8.19520719663
2.78110029887 8.25178841964
2.91353364643 8.31074040403
3.045966994 8.3730538349
3.17840034157 8.4378284088
3.31083368913 8.50545905448
3.4432670367 8.57570586206
3.57570038426 8.64833087311
3.70813373183 8.72379768971
3.84056707939 8.80190553544
3.97300042696 8.88245615199
4.10543377452 8.96598704051
4.23786712209 9.05084844584
4.37030046965 9.1390827778
4.50273381722 9.22903176285
4.63516716478 9.32128407036
4.76760051235 9.41647353208
4.90003385991 9.51287430377
5.03246720748 9.61191908506
5.16490055504 9.71347967087
5.29733390261 9.81659239816
5.42976725017 9.92109275674
5.56220059774 10.0285157813
5.6946339453 10.1378890822
5.82706729287 10.2490729826
5.95950064043 10.3628089042
6.091933988 10.4790052959
6.22436733556 10.5976164282
6.35680068313 10.718708677
6.4892340307 10.8444235348


==> figuresAndData/dataForRayleigh-conditionalMeanCentered-sigma8prob0pt8.tex <==
0.0 8.28210551064
0.104749805795 8.28296816209
0.20949961159 8.28507141802
0.314249417386 8.28877666826
0.418999223181 8.29356066033
0.523749028976 8.30020983205
0.628498834771 8.30774580214
0.733248640566 8.3173868775
0.837998446361 8.32814082025
0.942748252157 8.34033459756
1.04749805795 8.35384829079
1.15224786375 8.36900579755
1.25699766954 8.3856825972
1.36174747534 8.4042036063
1.46649728113 8.42398657421
1.57124708693 8.4458122949
1.67599689272 8.46909425076
1.78074669852 8.4936964547
1.88549650431 8.52041542574
1.99024631011 8.54865703801
2.0949961159 8.57876123772
2.1997459217 8.61012365507
2.30449572749 8.64356915539
2.40924553329 8.67849414828
2.51399533908 8.71574723229
2.61874514488 8.75423408987
2.72349495067 8.79432037374
2.82824475647 8.83638751247
2.93299456226 8.88032775262
3.03774436806 8.92552351195
3.14249417386 8.97288370583
3.24724397965 9.0217959509
3.35199378545 9.07215443656
3.45674359124 9.12438179951
3.56149339704 9.17838739751
3.66624320283 9.23354581606
3.77099300863 9.29083762914
3.87574281442 9.34964560116
3.98049262022 9.40988718076
4.08524242601 9.47148347587
4.18999223181 9.53491704005
4.2947420376 9.60013171097
4.3994918434 9.66651598546
4.50424164919 9.73515817835
4.60899145499 9.80491061376
4.71374126078 9.87634834087
4.81849106658 9.9501039022
4.92324087237 10.0257428669
5.02799067817 10.1041289961
5.13274048396 10.1852940748


==> figuresAndData/dataForRayleigh-conditionalMeanCentered.tex <==
0.0 0.0900282553096
0.00853 0.0900645934754
0.01706 0.090172769951
0.02559 0.0903516162454
0.03412 0.0906000831503
0.04265 0.0909172346294
0.05118 0.0913022420318
0.05971 0.0917543786124
0.06824 0.0922730143419
0.07677 0.0928576109899
0.0853 0.0935077174666
0.09383 0.0942229654065
0.10236 0.0950030649831
0.11089 0.0958478009388
0.11942 0.0967570288196
0.12795 0.0977306714007
0.13648 0.0987687152947
0.14501 0.0998712077291
0.15354 0.101038253486
0.16207 0.10227001199
0.1706 0.103566694546
0.17913 0.104928561701
0.18766 0.106355920743
0.19619 0.107849123312
0.20472 0.10940856313
0.21325 0.111034673827
0.22178 0.112727926882
0.23031 0.114488829646
0.23884 0.116317923459
0.24737 0.118215781851
0.2559 0.120183008826
0.26443 0.122220237213
0.27296 0.124328127098
0.28149 0.126507364313
0.29002 0.128758659001
0.29855 0.131082744228
0.30708 0.133480374663
0.31561 0.135952325305
0.32414 0.138499390266
0.33267 0.141122381601
0.3412 0.143822128183
0.34973 0.146599474623
0.35826 0.149455280234
0.36679 0.152390418031
0.37532 0.155405773772
0.38385 0.15850224503
0.39238 0.16168074031
0.40091 0.164942178185
0.40944 0.168287486473
0.41797 0.171717601441
0.4265 0.175233467038
0.43503 0.178836034151
0.44356 0.182526259894
0.45209 0.186305106917
0.46062 0.19017354274
0.46915 0.194132539111
0.47768 0.198183071385
0.48621 0.202326117922
0.49474 0.206562659507
0.50327 0.210893678792
0.5118 0.215320159751
0.52033 0.219843087155
0.52886 0.224463446067
0.53739 0.229182221348
0.54592 0.234000397183
0.55445 0.238918956622
0.56298 0.243938881131
0.57151 0.249061150164
0.58004 0.25428674074
0.58857 0.259616627045
0.5971 0.265051780033
0.60563 0.270593167048
0.61416 0.276241751458
0.62269 0.281998492292
0.63122 0.287864343897
0.63975 0.293840255602
0.64828 0.299927171391
0.65681 0.302793805764
0.66534 0.302867249126
0.67387 0.302943870435
0.6824 0.303082513628
0.69093 0.303283863577
0.69946 0.303518435722
0.70799 0.303786374453
0.71652 0.304118675545
0.72505 0.304485358715
0.73358 0.304886786418
0.74211 0.305323389329
0.75064 0.305795667791
0.75917 0.306304193363
0.7677 0.306849610486
0.77623 0.307465462797
0.78476 0.30808721985
0.79329 0.308748265715
0.80182 0.30941573574
0.81035 0.310157957034
0.81888 0.310908048022
0.82741 0.31170101014
0.83594 0.312502852185
0.84447 0.313349432856
0.853 0.314242179531
0.86153 0.315109748203
0.87006 0.316061831095
0.87859 0.317026828498
0.88712 0.318005254452
0.89565 0.318997673104
0.90418 0.320043258637
0.91271 0.321105023458
0.92124 0.322183716334
0.92977 0.323280142323
0.9383 0.324395164275
0.94683 0.32552970436
0.95536 0.32672615208
0.96389 0.327903246131
0.97242 0.329103005827
0.98095 0.330369561773
0.98948 0.3316187809
0.99801 0.332850370544
1.00654 0.334153227805
1.01507 0.335440165747
1.0236 0.336802441393
1.03213 0.338104455861
1.04066 0.339485032081
1.04919 0.340852673113
1.05772 0.342255463845
1.06625 0.343646528556
1.07478 0.34507527979
1.08331 0.346493705084
1.09184 0.347952588316
1.10037 0.349402745653
1.1089 0.350896376893
1.11743 0.352383091386
1.12596 0.353863186144
1.13449 0.355391053536
1.14302 0.3569144106
1.15155 0.358489178331
1.16008 0.360005543477
1.16861 0.361575747675
1.17714 0.363202574707
1.18567 0.364771919269
1.1942 0.366341384827
1.20273 0.367971687713
1.21126 0.369605069437
1.21979 0.371242303489
1.22832 0.372884203547
1.23685 0.374531624208
1.24538 0.376185461728
1.25391 0.377846654753
1.26244 0.379516185053
1.27097 0.381261795291
1.2795 0.38295200306
1.28803 0.384653770518
1.29656 0.386368259304
1.30509 0.388096677812
1.31362 0.389840281909
1.32215 0.391528202453
1.33068 0.393305189835
1.33921 0.395027330408
1.34774 0.396843265784
1.35627 0.398605345667
1.3648 0.400389170778
1.37333 0.402118283342
1.38186 0.40394935187
1.39039 0.405726956068
1.39892 0.407530822786
1.40745 0.409362703245
1.41598 0.41122440384
1.42451 0.41303348801
1.43304 0.414874000845
1.44157 0.416661402076
1.4501 0.418569536551
1.45863 0.420337661201
1.46716 0.422230612001
1.47569 0.424071954753
1.48422 0.425952553077
1.49275 0.427874623891
1.50128 0.429745960098
1.50981 0.431565326085
1.51834 0.433525227979
1.52687 0.435337422978
1.5354 0.437294988334
1.54393 0.439203001405
1.55246 0.441060282097
1.56099 0.442968710898
1.56952 0.444930913435
1.57805 0.446843946998
1.58658 0.448813598483
1.59511 0.450734405483
1.60364 0.452605242848
1.61217 0.454535879203
1.6207 0.456529216761
1.62923 0.458474612723
1.63776 0.460370982809
1.64629 0.462333603904
1.65482 0.464365569453
1.66335 0.466350862999
1.67188 0.468288444407
1.68041 0.47017726768
1.68894 0.47226324202
1.69747 0.474179242026
1.706 0.476172686977
1.71453 0.478119097078
1.72306 0.480146864358
1.73159 0.482128602448
1.74012 0.484195762467
1.74865 0.486084035892
1.75718 0.488194366069
1.76571 0.490123900012
1.77424 0.492144287468
1.78277 0.494119085034
1.7913 0.496189189709
1.79983 0.498215052136
1.80836 0.500195765124
1.81689 0.502277123142
1.82542 0.504314803555
1.83395 0.506307923509
1.84248 0.508407291608
1.85101 0.510463697951
1.85954 0.512476285089
1.86807 0.514444191897
1.8766 0.516525080936
1.88513 0.518563035441
1.89366 0.520557220936
1.90219 0.522670586997
1.91072 0.5247420623
1.91925 0.526770839993
1.92778 0.528925275337
1.93631 0.530868041936
1.94484 0.53293849824
1.95337 0.535141357402
1.9619 0.537128372788
1.97043 0.53924996047
1.97896 0.541330709201
1.98749 0.543369864729
1.99602 0.545550748515
2.00455 0.547506366432
2.01308 0.549606062215
2.02161 0.551665031498
2.03014 0.55387439482
2.03867 0.555851698284
2.0472 0.55798190862
2.05573 0.560072480245
2.06426 0.562322545037
2.07279 0.564333768483
2.08132 0.566507163787
2.08985 0.568642234158
2.09838 0.570738311538
2.10691 0.572794725995
2.11544 0.574810805744
2.12397 0.577000182416
2.1325 0.579152116071
2.14103 0.581265968658
2.14956 0.583341100487
2.15809 0.585599738402
2.16662 0.587597676265
2.17515 0.589782206204
2.18368 0.591929853342
2.19221 0.594040009535
2.20074 0.596112065244
2.20927 0.598381518332
2.2178 0.600377791632
2.22633 0.602574768891
2.23486 0.604735765909
2.24339 0.606860206057
2.25192 0.608947511547
2.26045 0.611246929877
2.26898 0.613260560418
2.27751 0.615489834213
2.28604 0.617684382144
2.29457 0.619843660537
2.3031 0.62196712477
2.31163 0.624054229295
2.32016 0.626370860873
2.32869 0.62838603081
2.33722 0.630634509298
2.34575 0.632849353658
2.35428 0.635030053662
2.36281 0.637176098343
2.37134 0.639286976028
2.37987 0.641645862772
2.3884 0.643687386414
2.39693 0.645980954504
2.40546 0.648242403844
2.41399 0.650177420011
2.42252 0.652370634669
2.43105 0.654829283217
2.43958 0.656957498789
2.44811 0.659051213685
2.45664 0.661416773773
2.46517 0.663442689754
2.4737 0.665744793064
2.48223 0.668015820371
2.49076 0.670255331691
2.49929 0.67246288671
2.50782 0.674638044804
2.51635 0.676780365061
2.52488 0.678889406299
2.53341 0.681295750283
2.54194 0.683339663378
2.55047 0.685685530436
2.559 0.688001925464
2.56753 0.689946327139
2.57606 0.692199762729
2.58459 0.694422503934
2.59312 0.696614147408
2.60165 0.699127711737
2.61018 0.701258807902
2.61871 0.703357608877
2.62724 0.705785747113
2.63577 0.707821644521
2.6443 0.710191892503
2.65283 0.71253409041
2.66136 0.714847873668
2.66989 0.717132877749
2.67842 0.719388738191
2.68695 0.721615090608
2.69548 0.723811570714
2.70401 0.725977814333
2.71254 0.728113457422
2.72107 0.730612750004
2.7296 0.732689139762
2.73813 0.735134554811
2.74666 0.737150288682
2.75519 0.739540475913
2.76372 0.741904088098
2.77225 0.744240801145
2.78078 0.746550291202
2.78931 0.748832234677
2.79784 0.751086308251
2.80637 0.753312188894
2.8149 0.755509553882
2.82343 0.757678080807
2.83196 0.760252557327
2.84049 0.762365646815
2.84902 0.764890475546
2.85755 0.766946893219
2.86608 0.769420892155
2.87461 0.771870660618
2.88314 0.773841396923
2.89167 0.776238581174
2.9002 0.778610678633
2.90873 0.780957408954
2.91726 0.783278492255
2.92579 0.785573649132
2.93432 0.787842600671
2.94285 0.790085068467
2.95138 0.792781878241
2.95991 0.794973925165
2.96844 0.797138668916
2.97697 0.799767111132
2.9855 0.801879837884
2.99403 0.804462569668
3.00256 0.806522229481
3.01109 0.809058253449
3.01962 0.811572283373
3.02815 0.813552125005
3.03668 0.816017972931
3.04521 0.818461111389
3.05374 0.820881307413
3.06227 0.82327832874
3.0708 0.825651943822
3.07933 0.82800192185
3.08786 0.830328032761
3.09639 0.832630047262
3.10492 0.834907736839
3.11345 0.837708289782
3.12198 0.839940261364
3.13051 0.842147239804
3.13904 0.844887291864
3.14757 0.847047260732
3.1561 0.849747179259
3.16463 0.851859294516
3.17316 0.854518288701
3.18169 0.856581713633
3.19022 0.859199000176
3.19875 0.861797002462
3.20728 0.863787709118
3.21581 0.866342855977
3.22434 0.86887816788
3.23287 0.871393467515
3.2414 0.873888578679
3.24993 0.876363326299
3.25846 0.878817536457
3.26699 0.881251036418
3.27552 0.883663654649
3.28405 0.88605522085
3.29258 0.88842556598
3.30111 0.891404246883
3.30964 0.893735531148
3.31817 0.896045107559
3.3267 0.898332812402
3.33523 0.901243810574
3.34376 0.903491220151
3.35229 0.906369489014
3.36082 0.908576016104
3.36935 0.911421024746
3.37788 0.913586094553
3.38641 0.916397324994
3.39494 0.91852037575
3.40347 0.921297323583
3.412 0.924058959593
3.42053 0.926119982273
3.42906 0.928846618783
3.43759 0.931557612656
3.44612 0.934252861885
3.45465 0.936230774285
3.46318 0.938890131513
3.47171 0.941533438087
3.48024 0.944160600788
3.48877 0.946771528766
3.4973 0.949366133608
3.50583 0.951944329411
3.51436 0.954506032858
3.52289 0.957051163298
3.53142 0.960318552287
3.53995 0.962834529465
3.54848 0.965333721987
3.55701 0.9678160608
3.56554 0.970281479972
3.57407 0.973490071976
3.5826 0.975925758746
3.59113 0.978344361742
3.59966 0.981518892426
3.60819 0.983907508256
3.61672 0.986278908904
3.62525 0.989419152014
3.63378 0.991760380633
3.64231 0.994879155629
3.65084 0.997190141451
3.65937 1.00028745388
3.6679 1.00337626243
3.67643 1.00564405955
3.68496 1.00871150529
3.69349 1.0117705443
3.70202 1.01399526577
3.71055 1.01703314505
3.71908 1.02006277048
3.72761 1.02224469124
3.73614 1.02525347755
3.74467 1.02825422648
3.7532 1.03124703131
3.76173 1.03423199398
3.77026 1.03720922551
3.77879 1.04017884642
3.78732 1.04226927026
3.79585 1.04521940623
3.80438 1.04816233782
3.81291 1.05109822878
3.82144 1.05402725522
3.82997 1.05694960635
3.8385 1.06076546944
3.84703 1.06367987045
3.85556 1.06658826987
3.86409 1.06949091793
3.87262 1.07238808249
3.88115 1.07528005012
3.88968 1.07816712737
3.89821 1.08198347476
3.90674 1.08486669947
3.91527 1.08774611
3.9238 1.0915707619
3.93233 1.09444876839
3.94086 1.09732427673
3.94939 1.10116146736
3.95792 1.10403856002
3.96645 1.10691476936
3.97498 1.11076965344
3.98351 1.11365111315
3.99204 1.11752293959
4.00057 1.12041257964
4.0091 1.12430461315
4.01763 1.12720582218
4.02616 1.13112183731
4.03469 1.1340385552
4.04322 1.13798294219
4.05175 1.14091977883
4.06028 1.14489768012
4.06881 1.14786006996
4.07734 1.15187755938
4.08587 1.15592024976
4.0944 1.15893628831
4.10293 1.16303001667
4.11146 1.16715560562
4.11999 1.17131577345
4.12852 1.17443677378
4.13705 1.17866966537
4.14558 1.18294726742
4.15411 1.18727386008
4.16264 1.19055369793
4.17117 1.19498743649
4.1797 1.19948694816
4.18823 1.20405971805
4.19676 1.20871456253
4.20529 1.21232977173
4.21382 1.21717588683
4.22235 1.2221428803
4.23088 1.22725050413
4.23941 1.23252433471
4.24794 1.23799868254
4.25647 1.24372181311


==> figuresAndData/dataForRayleigh-leftEnd-sigma2prob0pt1.tex <==
0.0 0.0
0.0841218682305 0.0841218682305
0.168243736461 0.168243736461
0.252365604692 0.252365604692
0.336487472922 0.336487472922
0.420609341153 0.420609341153
0.504731209383 0.504731209383
0.588853077614 0.588853077614
0.672974945844 0.672974945844
0.757096814075 0.757096814075
0.841218682305 0.841218682305
0.925340550536 0.925340550536
1.00946241877 1.00946241877
1.093584287 1.093584287
1.17770615523 1.17770615523
1.26182802346 1.26182802346
1.34594989169 1.34594989169
1.43007175992 1.43007175992
1.51419362815 1.51419362815
1.59831549638 1.59831549638
1.68243736461 1.68243736461
1.76655923284 1.76655923284
1.85068110107 1.85068110107
1.9348029693 1.9348029693
2.01892483753 2.01892483753
2.10304670576 2.10304670576
2.18716857399 2.18716857399
2.27129044222 2.27129044222
2.35541231046 2.35541231046
2.43953417869 2.43953417869
2.52365604692 2.52365604692
2.60777791515 2.60777791515
2.69189978338 2.69189978338
2.77602165161 2.77602165161
2.86014351984 2.86014351984
2.94426538807 2.94426538807
3.0283872563 3.0283872563
3.11250912453 3.11250912453
3.19663099276 3.19663099276
3.28075286099 3.28075286099
3.36487472922 3.36487472922
3.44899659745 3.44899659745
3.53311846568 3.53311846568
3.61724033391 3.61724033391
3.70136220214 3.70136220214
3.78548407037 3.78548407037
3.8696059386 3.8696059386
3.95372780684 3.95372780684
4.03784967507 4.03784967507
4.1219715433 4.1219715433


==> figuresAndData/dataForRayleigh-leftEnd-sigma2prob0pt3.tex <==
0.0 0.0
0.0608288216233 0.0608288216233
0.121657643247 0.121657643247
0.18248646487 0.18248646487
0.243315286493 0.243315286493
0.304144108116 0.304144108116
0.36497292974 0.36497292974
0.425801751363 0.425801751363
0.486630572986 0.486630572986
0.54745939461 0.54745939461
0.608288216233 0.608288216233
0.669117037856 0.669117037856
0.72994585948 0.72994585948
0.790774681103 0.790774681103
0.851603502726 0.851603502726
0.912432324349 0.912432324349
0.973261145973 0.973261145973
1.0340899676 1.0340899676
1.09491878922 1.09491878922
1.15574761084 1.15574761084
1.21657643247 1.21657643247
1.27740525409 1.27740525409
1.33823407571 1.33823407571
1.39906289734 1.39906289734
1.45989171896 1.45989171896
1.52072054058 1.52072054058
1.58154936221 1.58154936221
1.64237818383 1.64237818383
1.70320700545 1.70320700545
1.76403582708 1.76403582708
1.8248646487 1.8248646487
1.88569347032 1.88569347032
1.94652229195 1.94652229195
2.00735111357 2.00735111357
2.06817993519 2.06817993519
2.12900875682 2.12900875682
2.18983757844 2.18983757844
2.25066640006 2.25066640006
2.31149522169 2.31149522169
2.37232404331 2.37232404331
2.43315286493 2.43315286493
2.49398168656 2.49398168656
2.55481050818 2.55481050818
2.6156393298 2.6156393298
2.67646815143 2.67646815143
2.73729697305 2.73729697305
2.79812579467 2.79812579467
2.85895461629 2.85895461629
2.91978343792 2.91978343792
2.98061225954 2.98061225954


==> figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt3.tex <==
0.0 0.0
0.243315286493 0.243315286493
0.486630572986 0.486630572986
0.72994585948 0.72994585948
0.973261145973 0.973261145973
1.21657643247 1.21657643247
1.45989171896 1.45989171896
1.70320700545 1.70320700545
1.94652229195 1.94652229195
2.18983757844 2.18983757844
2.43315286493 2.43315286493
2.67646815143 2.67646815143
2.91978343792 2.91978343792
3.16309872441 3.16309872441
3.4064140109 3.4064140109
3.6497292974 3.6497292974
3.89304458389 3.89304458389
4.13635987038 4.13635987038
4.37967515688 4.37967515688
4.62299044337 4.62299044337
4.86630572986 4.86630572986
5.10962101636 5.10962101636
5.35293630285 5.35293630285
5.59625158934 5.59625158934
5.83956687584 5.83956687584
6.08288216233 6.08288216233
6.32619744882 6.32619744882
6.56951273532 6.56951273532
6.81282802181 6.81282802181
7.0561433083 7.0561433083
7.2994585948 7.2994585948
7.54277388129 7.54277388129
7.78608916778 7.78608916778
8.02940445428 8.02940445428
8.27271974077 8.27271974077
8.51603502726 8.51603502726
8.75935031375 8.75935031375
9.00266560025 9.00266560025
9.24598088674 9.24598088674
9.48929617323 9.48929617323
9.73261145973 9.73261145973
9.97592674622 9.97592674622
10.2192420327 10.2192420327
10.4625573192 10.4625573192
10.7058726057 10.7058726057
10.9491878922 10.9491878922
11.1925031787 11.1925031787
11.4358184652 11.4358184652
11.6791337517 11.6791337517
11.9224490382 11.9224490382


==> figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt6.tex <==
0.0 0.0
0.158488367927 0.158488367927
0.316976735854 0.316976735854
0.475465103781 0.475465103781
0.633953471707 0.633953471707
0.792441839634 0.792441839634
0.950930207561 0.950930207561
1.10941857549 1.10941857549
1.26790694341 1.26790694341
1.42639531134 1.42639531134
1.58488367927 1.58488367927
1.7433720472 1.7433720472
1.90186041512 1.90186041512
2.06034878305 2.06034878305
2.21883715098 2.21883715098
2.3773255189 2.3773255189
2.53581388683 2.53581388683
2.69430225476 2.69430225476
2.85279062268 2.85279062268
3.01127899061 3.01127899061
3.16976735854 3.16976735854
3.32825572646 3.32825572646
3.48674409439 3.48674409439
3.64523246232 3.64523246232
3.80372083024 3.80372083024
3.96220919817 3.96220919817
4.1206975661 4.1206975661
4.27918593403 4.27918593403
4.43767430195 4.43767430195
4.59616266988 4.59616266988
4.75465103781 4.75465103781
4.91313940573 4.91313940573
5.07162777366 5.07162777366
5.23011614159 5.23011614159
5.38860450951 5.38860450951
5.54709287744 5.54709287744
5.70558124537 5.70558124537
5.86406961329 5.86406961329
6.02255798122 6.02255798122
6.18104634915 6.18104634915
6.33953471707 6.33953471707
6.498023085 6.498023085
6.65651145293 6.65651145293
6.81499982086 6.81499982086
6.97348818878 6.97348818878
7.13197655671 7.13197655671
7.29046492464 7.29046492464
7.44895329256 7.44895329256
7.60744166049 7.60744166049
7.76593002842 7.76593002842


==> figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt7.tex <==
0.0 0.0
0.132433347565 0.132433347565
0.26486669513 0.26486669513
0.397300042696 0.397300042696
0.529733390261 0.529733390261
0.662166737826 0.662166737826
0.794600085391 0.794600085391
0.927033432956 0.927033432956
1.05946678052 1.05946678052
1.19190012809 1.19190012809
1.32433347565 1.32433347565
1.45676682322 1.45676682322
1.58920017078 1.58920017078
1.72163351835 1.72163351835
1.85406686591 1.85406686591
1.98650021348 1.98650021348
2.11893356104 2.11893356104
2.25136690861 2.25136690861
2.38380025617 2.38380025617
2.51623360374 2.51623360374
2.6486669513 2.6486669513
2.78110029887 2.78110029887
2.91353364643 2.91353364643
3.045966994 3.045966994
3.17840034157 3.17840034157
3.31083368913 3.31083368913
3.4432670367 3.4432670367
3.57570038426 3.57570038426
3.70813373183 3.70813373183
3.84056707939 3.84056707939
3.97300042696 3.97300042696
4.10543377452 4.10543377452
4.23786712209 4.23786712209
4.37030046965 4.37030046965
4.50273381722 4.50273381722
4.63516716478 4.63516716478
4.76760051235 4.76760051235
4.90003385991 4.90003385991
5.03246720748 5.03246720748
5.16490055504 5.16490055504
5.29733390261 5.29733390261
5.42976725017 5.42976725017
5.56220059774 5.56220059774
5.6946339453 5.6946339453
5.82706729287 5.82706729287
5.95950064043 5.95950064043
6.091933988 6.091933988
6.22436733556 6.22436733556
6.35680068313 6.35680068313
6.4892340307 6.4892340307


==> figuresAndData/dataForRayleigh-leftEnd-sigma8prob0pt8.tex <==
0.0 0.0
0.104749805795 0.104749805795
0.20949961159 0.20949961159
0.314249417386 0.314249417386
0.418999223181 0.418999223181
0.523749028976 0.523749028976
0.628498834771 0.628498834771
0.733248640566 0.733248640566
0.837998446361 0.837998446361
0.942748252157 0.942748252157
1.04749805795 1.04749805795
1.15224786375 1.15224786375
1.25699766954 1.25699766954
1.36174747534 1.36174747534
1.46649728113 1.46649728113
1.57124708693 1.57124708693
1.67599689272 1.67599689272
1.78074669852 1.78074669852
1.88549650431 1.88549650431
1.99024631011 1.99024631011
2.0949961159 2.0949961159
2.1997459217 2.1997459217
2.30449572749 2.30449572749
2.40924553329 2.40924553329
2.51399533908 2.51399533908
2.61874514488 2.61874514488
2.72349495067 2.72349495067
2.82824475647 2.82824475647
2.93299456226 2.93299456226
3.03774436806 3.03774436806
3.14249417386 3.14249417386
3.24724397965 3.24724397965
3.35199378545 3.35199378545
3.45674359124 3.45674359124
3.56149339704 3.56149339704
3.66624320283 3.66624320283
3.77099300863 3.77099300863
3.87574281442 3.87574281442
3.98049262022 3.98049262022
4.08524242601 4.08524242601
4.18999223181 4.18999223181
4.2947420376 4.2947420376
4.3994918434 4.3994918434
4.50424164919 4.50424164919
4.60899145499 4.60899145499
4.71374126078 4.71374126078
4.81849106658 4.81849106658
4.92324087237 4.92324087237
5.02799067817 5.02799067817
5.13274048396 5.13274048396


==> figuresAndData/dataForRayleigh-lowerEnd-sigma2prob0pt1.tex <==
0.0 0.0
0.0841218682305 0.0841218682305
0.168243736461 0.168243736461
0.252365604692 0.252365604692
0.336487472922 0.336487472922
0.420609341153 0.420609341153
0.504731209383 0.504731209383
0.588853077614 0.588853077614
0.672974945844 0.672974945844
0.757096814075 0.757096814075
0.841218682305 0.841218682305
0.925340550536 0.925340550536
1.00946241877 1.00946241877
1.093584287 1.093584287
1.17770615523 1.17770615523
1.26182802346 1.26182802346
1.34594989169 1.34594989169
1.43007175992 1.43007175992
1.51419362815 1.51419362815
1.59831549638 1.59831549638
1.68243736461 1.68243736461
1.76655923284 1.76655923284
1.85068110107 1.85068110107
1.9348029693 1.9348029693
2.01892483753 2.01892483753
2.10304670576 2.10304670576
2.18716857399 2.18716857399
2.27129044222 2.27129044222
2.35541231046 2.35541231046
2.43953417869 2.43953417869
2.52365604692 2.52365604692
2.60777791515 2.60777791515
2.69189978338 2.69189978338
2.77602165161 2.77602165161
2.86014351984 2.86014351984
2.94426538807 2.94426538807
3.0283872563 3.0283872563
3.11250912453 3.11250912453
3.19663099276 3.19663099276
3.28075286099 3.28075286099
3.36487472922 3.36487472922
3.44899659745 3.44899659745
3.53311846568 3.53311846568
3.61724033391 3.61724033391
3.70136220214 3.70136220214
3.78548407037 3.78548407037
3.8696059386 3.8696059386
3.95372780684 3.95372780684
4.03784967507 4.03784967507
4.1219715433 4.1219715433


==> figuresAndData/dataForRayleigh-midPoint-sigma1.tex <==
0.0 0.160145706136
0.00488 0.162605271339
0.00976 0.165103952687
0.01464 0.167641707448
0.01952 0.170218464577
0.0244 0.172834124972
0.02928 0.175488561835
0.03416 0.17818162113
0.03904 0.180913122131
0.04392 0.18368285806
0.0488 0.186490596817
0.05368 0.189336081773
0.05856 0.192219032649
0.06344 0.195139146451
0.06832 0.19809609847
0.0732 0.201089543327
0.07808 0.204119116062
0.08296 0.207184433267
0.08784 0.210285094233
0.09272 0.213420682134
0.0976 0.216590765212
0.10248 0.219794897976
0.10736 0.223032622402
0.11224 0.226303469121
0.11712 0.229606958601
0.122 0.232942602311
0.12688 0.23630990386
0.13176 0.239708360111
0.13664 0.243137462266
0.14152 0.24659669691
0.1464 0.25008554703
0.15128 0.253603492981
0.15616 0.257150013416
0.16104 0.260724586172
0.16592 0.264326689114
0.1708 0.267955800923
0.17568 0.27161140185
0.18056 0.275292974415
0.18544 0.279000004064
0.19032 0.282731979776
0.1952 0.286488394628
0.20008 0.290268746315
0.20496 0.294072537626
0.20984 0.297899276879
0.21472 0.301748478312
0.2196 0.30561966244
0.22448 0.309512356371
0.22936 0.313426094085
0.23424 0.317360416684
0.23912 0.321314872604
0.244 0.325289017799
0.24888 0.329282415895
0.25376 0.333294638319
0.25864 0.337325264399
0.26352 0.341373881445
0.2684 0.3454400848
0.27328 0.349523477881
0.27816 0.353623672193
0.28304 0.357740287325
0.28792 0.36187295094
0.2928 0.366021298735
0.29768 0.370184974404
0.30256 0.374363629571
0.30744 0.378556923733
0.31232 0.38276452417
0.3172 0.386986105869
0.32208 0.39122135142
0.32696 0.395469950918
0.33184 0.399731601857
0.33672 0.404006009013
0.3416 0.408292884328
0.34648 0.412591946786
0.35136 0.416902922294
0.35624 0.421225543545
0.36112 0.425559549898
0.366 0.429904687242
0.37088 0.434260707861
0.37576 0.438627370306
0.38064 0.443004439258
0.38552 0.447391685399
0.3904 0.45178888527
0.39528 0.456195821149
0.40016 0.460612280909
0.40504 0.465038057897
0.40992 0.469472950797
0.4148 0.473916763505
0.41968 0.478369305001
0.42456 0.482830389227
0.42944 0.487299834963
0.43432 0.491777465702
0.4392 0.496263109538
0.44408 0.500756599045
0.44896 0.505257771161
0.45384 0.50976646708
0.45872 0.514282532139
0.4636 0.518805815709
0.46848 0.523336171093
0.47336 0.527873455421
0.47824 0.532417529546
0.48312 0.536968257952
0.488 0.541525508652
0.49288 0.546089153097
0.49776 0.550659066083
0.50264 0.555235125663
0.50752 0.559817213059
0.5124 0.564405212575
0.51728 0.568999011519
0.52216 0.57359850012
0.52704 0.578203571448
0.53192 0.58281412134
0.5368 0.587430048324
0.54168 0.59205125355
0.54656 0.596677640714
0.55144 0.601309115995
0.55632 0.605945587988
0.5612 0.610586967635
0.56608 0.615233168166
0.57096 0.619884105039
0.57584 0.624539695877
0.58072 0.629199860412
0.5856 0.63386452043
0.59048 0.638533599717
0.59536 0.643207024003
0.60024 0.647884720915
0.60512 0.652566619922
0.61 0.657252652292
0.61488 0.661942751043
0.61976 0.666636850895
0.62464 0.671334888231
0.62952 0.676036801047
0.6344 0.680742528918
0.63928 0.685452012951
0.64416 0.69016519575
0.64904 0.694882021376
0.65392 0.699602435309
0.6588 0.704326384416
0.66368 0.709053816911
0.66856 0.713784682325
0.67344 0.718518931471
0.67832 0.723256516414
0.6832 0.727997390439
0.68808 0.732741508019
0.69296 0.737488824791
0.69784 0.742239297523
0.70272 0.746992884087
0.7076 0.751749543437
0.71248 0.756509235575
0.71736 0.761271921536
0.72224 0.766037563354
0.72712 0.770806124046
0.732 0.775577567583
0.73688 0.780351858873
0.74176 0.785128963737
0.74664 0.789908848886
0.75152 0.794691481905
0.7564 0.79947683123
0.76128 0.804264866132
0.76616 0.809055556694
0.77104 0.813848873797
0.77592 0.8186447891
0.7808 0.823443275026
0.78568 0.828244304741
0.79056 0.833047852145
0.79544 0.837853891847
0.80032 0.842662399159
0.8052 0.847473350076
0.81008 0.852286721265
0.81496 0.857102490049
0.81984 0.861920634394
0.82472 0.866741132899
0.8296 0.871563964778
0.83448 0.876389109854
0.83936 0.881216548543
0.84424 0.886046261844
0.84912 0.890878231328
0.854 0.895712439127
0.85888 0.900548867926
0.86376 0.905387500948
0.86864 0.910228321947
0.87352 0.915071315202
0.8784 0.9199164655
0.88328 0.924763758135
0.88816 0.929613178894
0.89304 0.934464714053
0.89792 0.939318350364
0.9028 0.944174075051
0.90768 0.949031875801
0.91256 0.953891740759
0.91744 0.958753658516
0.92232 0.963617618107
0.9272 0.968483609002
0.93208 0.973351621101
0.93696 0.978221644726
0.94184 0.983093670616
0.94672 0.987967689924
0.9516 0.992843694205
0.95648 0.997721675417
0.96136 1.00260162591
0.96624 1.00748353844
0.97112 1.01236740612
0.976 1.01725322246
0.98088 1.02214098136
0.98576 1.02703067707
0.99064 1.03192230422
0.99552 1.03681585781
1.0004 1.04171133317
1.00528 1.04660872603
1.01016 1.05150803245
1.01504 1.05640924884
1.01992 1.06131237197
1.0248 1.06621739893
1.02968 1.07112432718
1.03456 1.0760331545
1.03944 1.08094387901
1.04432 1.08585649918
1.0492 1.09077101378
1.05408 1.09568742194
1.05896 1.1006057231
1.06384 1.10552591702
1.06872 1.11044800382
1.0736 1.11537198389
1.07848 1.12029785798
1.08336 1.12522562714
1.08824 1.13015529275
1.09312 1.1350868565
1.098 1.1400203204
1.10288 1.14495568676
1.10776 1.14989295823
1.11264 1.15483213775
1.11752 1.1597732286
1.1224 1.16471623433
1.12728 1.16966115885
1.13216 1.17460800635
1.13704 1.17955678135
1.14192 1.18450748866
1.1468 1.18946013343
1.15168 1.19441472111
1.15656 1.19937125745
1.16144 1.20432974853
1.16632 1.20929020074
1.1712 1.21425262079
1.17608 1.21921701569
1.18096 1.22418339277
1.18584 1.22915175969
1.19072 1.23412212442
1.1956 1.23909449525
1.20048 1.24406888079
1.20536 1.24904528998
1.21024 1.25402373206
1.21512 1.25900421663
1.22 1.26398675359
1.22488 1.26897135318
1.22976 1.27395802599
1.23464 1.2789467829
1.23952 1.28393763516
1.2444 1.28893059435
1.24928 1.29392567238
1.25416 1.29892288153
1.25904 1.3039222344
1.26392 1.30892374395
1.2688 1.31392742349
1.27368 1.31893328667
1.27856 1.32394134754
1.28344 1.32895162046
1.28832 1.33396412018
1.2932 1.33897886184
1.29808 1.34399586091
1.30296 1.34901513326
1.30784 1.35403669514
1.31272 1.35906056319
1.3176 1.36408675441
1.32248 1.36911528624
1.32736 1.37414617647
1.33224 1.37917944332
1.33712 1.38421510541
1.342 1.38925318178
1.34688 1.39429369188
1.35176 1.39933665559
1.35664 1.4043820932
1.36152 1.40943002546
1.3664 1.41448047355
1.37128 1.41953345908
1.37616 1.42458900415
1.38104 1.42964713128
1.38592 1.43470786348
1.3908 1.43977122422
1.39568 1.44483723745
1.40056 1.44990592763
1.40544 1.45497731967
1.41032 1.46005143903
1.4152 1.46512831164
1.42008 1.47020796396
1.42496 1.47529042299
1.42984 1.48037571625
1.43472 1.48546387181
1.4396 1.49055491827
1.44448 1.49564888483
1.44936 1.50074580123
1.45424 1.50584569779
1.45912 1.51094860545
1.464 1.51605455571
1.46888 1.52116358072
1.47376 1.52627571321
1.47864 1.53139098659
1.48352 1.53650943488
1.4884 1.54163109276
1.49328 1.5467559956
1.49816 1.55188417942
1.50304 1.55701568096
1.50792 1.56215053765
1.5128 1.56728878765
1.51768 1.57243046985
1.52256 1.57757562388
1.52744 1.58272429015
1.53232 1.58787650983
1.5372 1.5930323249
1.54208 1.59819177813
1.54696 1.60335491314
1.55184 1.60852177436
1.55672 1.61369240712
1.5616 1.61886685758
1.56648 1.62404517284
1.57136 1.62922740089
1.57624 1.63441359066
1.58112 1.63960379202
1.586 1.64479805583
1.59088 1.64999643395
1.59576 1.65519897924
1.60064 1.66040574561
1.60552 1.66561678802
1.6104 1.67083216253
1.61528 1.6760519263
1.62016 1.68127613762
1.62504 1.68650485597
1.62992 1.69173814197
1.6348 1.6969760575
1.63968 1.70221866565
1.64456 1.7074660308
1.64944 1.71271821863
1.65432 1.71797529613
1.6592 1.72323733169
1.66408 1.72850439507
1.66896 1.73377655748
1.67384 1.73905389157
1.67872 1.74433647152
1.6836 1.74962437304
1.68848 1.7549176734
1.69336 1.76021645151
1.69824 1.76552078792
1.70312 1.77083076489
1.708 1.77614646643
1.71288 1.78146797831
1.71776 1.78679538817
1.72264 1.7921287855
1.72752 1.79746826175
1.7324 1.80281391033
1.73728 1.80816582671
1.74216 1.81352410843
1.74704 1.81888885519
1.75192 1.82426016888
1.7568 1.82963815369
1.76168 1.8350229161
1.76656 1.84041456502
1.77144 1.8458132118
1.77632 1.85121897033
1.7812 1.8566319571
1.78608 1.8620522913
1.79096 1.86748009485
1.79584 1.87291549251
1.80072 1.87835861199
1.8056 1.88380958397
1.81048 1.88926854226
1.81536 1.89473562383
1.82024 1.90021096897
1.82512 1.90569472134
1.83 1.9111870281
1.83488 1.91668803999
1.83976 1.9221979115
1.84464 1.92771680094
1.84952 1.93324487055
1.8544 1.93878228668
1.85928 1.94432921988
1.86416 1.94988584506
1.86904 1.95545234161
1.87392 1.96102889359
1.8788 1.96661568982
1.88368 1.97221292411
1.88856 1.9778207954
1.89344 1.98343950792
1.89832 1.9890692714
1.9032 1.99471030126
1.90808 2.0003628188
1.91296 2.0060270514
1.91784 2.01170323277
1.92272 2.01739160316
1.9276 2.02309240959
1.93248 2.02880590613
1.93736 2.03453235412
1.94224 2.04027202249
1.94712 2.04602518803
1.952 2.05179213568
1.95688 2.05757315886
1.96176 2.0633685598
1.96664 2.06917864989
1.97152 2.07500375003
1.9764 2.08084419105
1.98128 2.08670031409
1.98616 2.09257247103
1.99104 2.09846102491
1.99592 2.10436635048
2.0008 2.1102888346
2.00568 2.11622887684
2.01056 2.12218688998
2.01544 2.12816330063
2.02032 2.13415854982
2.0252 2.14017309367
2.03008 2.14620740407
2.03496 2.15226196938
2.03984 2.15833729524
2.04472 2.16443390539
2.0496 2.17055234247
2.05448 2.17669316902
2.05936 2.18285696839
2.06424 2.1890443458
2.06912 2.19525592944
2.074 2.20149237163
2.07888 2.20775435006
2.08376 2.21404256915
2.08864 2.22035776141
2.09352 2.22670068898
2.0984 2.23307214526
2.10328 2.2394729566
2.10816 2.24590398415
2.11304 2.25236612585
2.11792 2.25886031856
2.1228 2.26538754031
2.12768 2.27194881274
2.13256 2.27854520375
2.13744 2.28517783035
2.14232 2.29184786164
2.1472 2.29855652219
2.15208 2.30530509553
2.15696 2.31209492806
2.16184 2.31892743317
2.16672 2.3258040958
2.1716 2.33272647733
2.17648 2.33969622096
2.18136 2.34671505751
2.18624 2.35378481178
2.19112 2.36090740948
2.196 2.36808488488
2.20088 2.37531938909
2.20576 2.38261319922
2.21064 2.3899687285
2.21552 2.39738853731
2.2204 2.40487534549
2.22528 2.4124320459
2.23016 2.42006171947
2.23504 2.42776765193
2.23992 2.43555335246
2.2448 2.44342257454
2.24968 2.45137933924
2.25456 2.45942796142
2.25944 2.46757307923
2.26432 2.4758196874
2.2692 2.48417317494
2.27408 2.49263936807
2.27896 2.501224579
2.28384 2.50993566199
2.28872 2.51878007752
2.2936 2.52776596647
2.29848 2.53690223601
2.30336 2.54619865948
2.30824 2.5556659933
2.31312 2.56531611425
2.318 2.57516218182
2.32288 2.58521883116
2.32776 2.59550240391
2.33264 2.60603122623
2.33752 2.6168259462
2.3424 2.62790994645
2.34728 2.63930985312
2.35216 2.65105616979
2.35704 2.66318407502
2.36192 2.6757344371
2.3668 2.68875512166
2.37168 2.70230269985
2.37656 2.71644471472
2.38144 2.7312627411
2.38632 2.74685659853
2.3912 2.76335028415
2.39608 2.78090054676
2.40096 2.79970965864
2.40584 2.82004513296
2.41072 2.84227150079
2.4156 2.86690429499
2.42048 2.8947080431
2.42536 2.92689014648
2.43024 2.96553216795
2.43512 3.01472789297


==> figuresAndData/dataForRayleigh-midPoint-sigma1prob0pt1.tex <==
0.0 0.229521802513
0.004276 0.231670866425
0.008552 0.233842055028
0.012828 0.236035358932
0.017104 0.238250762499
0.02138 0.24048824387
0.025656 0.242747774992
0.029932 0.245029321663
0.034208 0.247332843578
0.038484 0.249658294386
0.04276 0.252005621759
0.047036 0.254374767465
0.051312 0.256765667447
0.055588 0.259178251916
0.059864 0.261612445446
0.06414 0.26406816708
0.068416 0.266545330439
0.072692 0.269043843837
0.076968 0.271563610408
0.081244 0.274104528233
0.08552 0.276666490473
0.089796 0.279249385508
0.094072 0.281853097082
0.098348 0.284477504447
0.102624 0.287122482517
0.1069 0.28978790202
0.111176 0.292473629658
0.115452 0.295179528263
0.119728 0.297905456959
0.124004 0.300651271327
0.12828 0.30341682357
0.132556 0.306201962675
0.136832 0.30900653458
0.141108 0.311830382343
0.145384 0.314673346302
0.14966 0.317535264246
0.153936 0.320415971573
0.158212 0.323315301461
0.162488 0.326233085022
0.166764 0.329169151467
0.17104 0.332123328259
0.175316 0.335095441275
0.179592 0.338085314953
0.183868 0.341092772446
0.188144 0.344117635769
0.19242 0.347159725942
0.196696 0.350218863132
0.200972 0.353294866791
0.205248 0.35638755579
0.209524 0.35949674855
0.2138 0.36262226317
0.218076 0.365763917547
0.222352 0.368921529497
0.226628 0.372094916871
0.230904 0.375283897666
0.23518 0.378488290131
0.239456 0.381707912871
0.243732 0.384942584948
0.248008 0.388192125974
0.252284 0.3914563562
0.25656 0.39473509661
0.260836 0.398028168997
0.265112 0.401335396046
0.269388 0.404656601409
0.273664 0.407991609775
0.27794 0.411340246941
0.282216 0.414702339872
0.286492 0.418077716764
0.290768 0.421466207099
0.295044 0.424867641702
0.29932 0.428281852787
0.303596 0.431708674004
0.307872 0.435147940488
0.312148 0.438599488889
0.316424 0.442063157421
0.3207 0.445538785888
0.324976 0.449026215717
0.329252 0.452525289991
0.333528 0.456035853471
0.337804 0.459557752619
0.34208 0.463090835623
0.346356 0.466634952413
0.350632 0.470189954677
0.354908 0.473755695877
0.359184 0.47733203126
0.36346 0.48091881787
0.367736 0.484515914552
0.372012 0.488123181963
0.376288 0.491740482576
0.380564 0.495367680681
0.38484 0.499004642387
0.389116 0.502651235624
0.393392 0.506307330139
0.397668 0.509972797494
0.401944 0.513647511065
0.40622 0.517331346032
0.410496 0.521024179375
0.414772 0.524725889868
0.419048 0.528436358068
0.423324 0.532155466307
0.4276 0.535883098682
0.431876 0.539619141045
0.436152 0.543363480989
0.440428 0.547116007835
0.444704 0.550876612625
0.44898 0.5546451881
0.453256 0.558421628691
0.457532 0.562205830504
0.461808 0.565997691304
0.466084 0.569797110497
0.47036 0.573603989118
0.474636 0.577418229814
0.478912 0.581239736824
0.483188 0.585068415967
0.487464 0.58890417462
0.49174 0.592746921704
0.496016 0.596596567666
0.500292 0.60045302446
0.504568 0.60431620553
0.508844 0.608186025793
0.51312 0.612062401618
0.517396 0.615945250812
0.521672 0.619834492598
0.525948 0.623730047602
0.530224 0.627631837827
0.5345 0.631539786645
0.538776 0.635453818769
0.543052 0.639373860242
0.547328 0.643299838417
0.551604 0.647231681938
0.55588 0.651169320723
0.560156 0.655112685948
0.564432 0.659061710025
0.568708 0.663016326591
0.572984 0.666976470487
0.57726 0.670942077738
0.581536 0.674913085543
0.585812 0.678889432254
0.590088 0.682871057358
0.594364 0.686857901463
0.59864 0.690849906284
0.602916 0.694847014621
0.607192 0.698849170346
0.611468 0.70285631839
0.615744 0.706868404724
0.62002 0.710885376344
0.624296 0.714907181257
0.628572 0.718933768465
0.632848 0.722965087952
0.637124 0.727001090669
0.6414 0.731041728517
0.645676 0.735086954338
0.649952 0.739136721895
0.654228 0.743190985865
0.658504 0.74724970182
0.66278 0.751312826217
0.667056 0.755380316383
0.671332 0.759452130505
0.675608 0.763528227613
0.679884 0.767608567574
0.68416 0.771693111074
0.688436 0.775781819606
0.692712 0.779874655466
0.696988 0.783971581731
0.701264 0.788072562256
0.70554 0.792177561657
0.709816 0.796286545305
0.714092 0.800399479312
0.718368 0.804516330522
0.722644 0.8086370665
0.72692 0.812761655523
0.731196 0.816890066568
0.735472 0.821022269305
0.739748 0.825158234085
0.744024 0.829297931934
0.7483 0.83344133454
0.752576 0.837588414247
0.756852 0.841739144044
0.761128 0.845893497559
0.765404 0.850051449049
0.76968 0.854212973392
0.773956 0.858378046079
0.778232 0.862546643207
0.782508 0.866718741471
0.786784 0.870894318155
0.79106 0.875073351127
0.795336 0.879255818832
0.799612 0.883441700282
0.803888 0.887630975051
0.808164 0.891823623272
0.81244 0.896019625623
0.816716 0.900218963327
0.820992 0.904421618145
0.825268 0.908627572365
0.829544 0.912836808804
0.83382 0.917049310796
0.838096 0.921265062189
0.842372 0.92548404734
0.846648 0.92970625111
0.850924 0.933931658856
0.8552 0.93816025643
0.859476 0.942392030173
0.863752 0.946626966907
0.868028 0.950865053937
0.872304 0.95510627904
0.87658 0.959350630467
0.880856 0.963598096933
0.885132 0.967848667616
0.889408 0.972102332156
0.893684 0.976359080644
0.89796 0.980618903627
0.902236 0.984881792097
0.906512 0.989147737494
0.910788 0.993416731698
0.915064 0.997688767029
0.91934 1.00196383624
0.923616 1.00624193253
0.927892 1.01052304951
0.932168 1.01480718123
0.936444 1.01909432216
0.94072 1.0233844672
0.944996 1.02767761168
0.949272 1.03197375132
0.953548 1.03627288229
0.957824 1.04057500116
0.9621 1.0448801049
0.966376 1.04918819092
0.970652 1.05349925703
0.974928 1.05781330145
0.979204 1.0621303228
0.98348 1.06645032011
0.987756 1.07077329284
0.992032 1.07509924081
0.996308 1.0794281643
1.000584 1.08376006394
1.00486 1.0880949408
1.009136 1.09243279634
1.013412 1.09677363243
1.017688 1.10111745133
1.021964 1.10546425573
1.02624 1.10981404868
1.030516 1.11416683367
1.034792 1.11852261458
1.039068 1.12288139569
1.043344 1.1272431817
1.04762 1.13160797769
1.051896 1.13597578917
1.056172 1.14034662205
1.060448 1.14472048264
1.064724 1.14909737765
1.069 1.15347731424
1.073276 1.15786029994
1.077552 1.16224634272
1.081828 1.16663545094
1.086104 1.1710276334
1.09038 1.1754228993
1.094656 1.17982125828
1.098932 1.18422272038
1.103208 1.18862729609
1.107484 1.19303499631
1.11176 1.19744583237
1.116036 1.20185981604
1.120312 1.20627695952
1.124588 1.21069727545
1.128864 1.21512077692
1.13314 1.21954747745
1.137416 1.22397739101
1.141692 1.22841053203
1.145968 1.2328469154
1.150244 1.23728655645
1.15452 1.24172947098
1.158796 1.24617567527
1.163072 1.25062518607
1.167348 1.25507802058
1.171624 1.25953419651
1.1759 1.26399373204
1.180176 1.26845664585
1.184452 1.2729229571
1.188728 1.27739268547
1.193004 1.28186585114
1.19728 1.28634247479
1.201556 1.29082257763
1.205832 1.29530618139
1.210108 1.29979330834
1.214384 1.30428398127
1.21866 1.30877822351
1.222936 1.31327605897
1.227212 1.31777751208
1.231488 1.32228260787
1.235764 1.32679137191
1.24004 1.33130383037
1.244316 1.33582001
1.248592 1.34033993814
1.252868 1.34486364275
1.257144 1.34939115239
1.26142 1.35392249625
1.265696 1.35845770414
1.269972 1.36299680652
1.274248 1.3675398345
1.278524 1.37208681984
1.2828 1.37663779499
1.287076 1.38119279306
1.291352 1.38575184787
1.295628 1.39031499393
1.299904 1.39488226646
1.30418 1.39945370144
1.308456 1.40402933555
1.312732 1.40860920624
1.317008 1.41319335173
1.321284 1.417781811
1.32556 1.42237462384
1.329836 1.42697183084
1.334112 1.4315734734
1.338388 1.43617959377
1.342664 1.44079023504
1.34694 1.44540544117
1.351216 1.450025257
1.355492 1.45464972828
1.359768 1.45927890166
1.364044 1.46391282474
1.36832 1.46855154605
1.372596 1.47319511512
1.376872 1.47784358245
1.381148 1.48249699955
1.385424 1.48715541897
1.3897 1.4918188943
1.393976 1.49648748021
1.398252 1.50116123248
1.402528 1.50584020797
1.406804 1.51052446471
1.41108 1.5152140619
1.415356 1.51990905992
1.419632 1.52460952035
1.423908 1.52931550605
1.428184 1.53402708112
1.43246 1.53874431097
1.436736 1.54346726233
1.441012 1.54819600331
1.445288 1.55293060339
1.449564 1.55767113346
1.45384 1.56241766589
1.458116 1.56717027452
1.462392 1.57192903471
1.466668 1.57669402339
1.470944 1.58146531907
1.47522 1.58624300191
1.479496 1.59102715372
1.483772 1.59581785804
1.488048 1.60061520017
1.492324 1.6054192672
1.4966 1.61023014805
1.500876 1.61504793357
1.505152 1.6198727165
1.509428 1.62470459161
1.513704 1.62954365568
1.51798 1.6343900076
1.522256 1.63924374839
1.526532 1.6441049813
1.530808 1.64897381182
1.535084 1.65385034775
1.53936 1.65873469932
1.543636 1.66362697917
1.547912 1.66852730247
1.552188 1.67343578699
1.556464 1.67835255314
1.56074 1.68327772407
1.565016 1.68821142575
1.569292 1.69315378702
1.573568 1.69810493973
1.577844 1.70306501876
1.58212 1.70803416215
1.586396 1.71301251119
1.590672 1.71800021049
1.594948 1.72299740814
1.599224 1.72800425572
1.6035 1.73302090851
1.607776 1.73804752552
1.612052 1.74308426967
1.616328 1.74813130785
1.620604 1.7531888111
1.62488 1.7582569547
1.629156 1.76333591836
1.633432 1.76842588629
1.637708 1.77352704741
1.641984 1.77863959545
1.64626 1.78376372918
1.650536 1.7888996525
1.654812 1.79404757467
1.659088 1.79920771049
1.663364 1.80438028043
1.66764 1.8095655109
1.671916 1.81476363443
1.676192 1.81997488989
1.680468 1.82519952268
1.684744 1.83043778502
1.68902 1.83568993619
1.693296 1.84095624273
1.697572 1.84623697878
1.701848 1.85153242634
1.706124 1.85684287555
1.7104 1.86216862501
1.714676 1.86750998213
1.718952 1.87286726344
1.723228 1.87824079495
1.727504 1.88363091256
1.73178 1.88903796241
1.736056 1.89446230134
1.740332 1.8999042973
1.744608 1.90536432981
1.748884 1.91084279047
1.75316 1.91634008344
1.757436 1.92185662599
1.761712 1.92739284909
1.765988 1.93294919795
1.770264 1.93852613272
1.77454 1.94412412912
1.778816 1.94974367914
1.783092 1.95538529181
1.787368 1.96104949396
1.791644 1.96673683109
1.79592 1.97244786823
1.800196 1.97818319089
1.804472 1.98394340606
1.808748 1.98972914325
1.813024 1.99554105563
1.8173 2.00137982124
1.821576 2.00724614423
1.825852 2.01314075624
1.830128 2.01906441784
1.834404 2.02501792008
1.83868 2.03100208612
1.842956 2.03701777301
1.847232 2.04306587357
1.851508 2.04914731839
1.855784 2.05526307802
1.86006 2.06141416528
1.864336 2.06760163774
1.868612 2.07382660043
1.872888 2.08009020868
1.877164 2.08639367127
1.88144 2.09273825377
1.885716 2.09912528217
1.889992 2.10555614676
1.894268 2.11203230642
1.898544 2.11855529321
1.90282 2.12512671731
1.907096 2.13174827253
1.911372 2.13842174217
1.915648 2.14514900546
1.919924 2.15193204463
1.9242 2.1587729526
1.928476 2.16567394138
1.932752 2.17263735139
1.937028 2.17966566159
1.941304 2.18676150074
1.94558 2.19392765972
1.949856 2.20116710532
1.954132 2.20848299531
1.958408 2.21587869537
1.962684 2.22335779787
1.96696 2.23092414275
1.971236 2.23858184104
1.975512 2.24633530112
1.979788 2.25418925828
1.984064 2.26214880814
1.98834 2.2702194444
1.992616 2.27840710169
1.996892 2.28671820442
2.001168 2.29515972262
2.005444 2.30373923597
2.00972 2.31246500758
2.013996 2.32134606939
2.018272 2.33039232128
2.022548 2.33961464696
2.026824 2.34902504976
2.0311 2.358636813
2.035376 2.36846469019
2.039652 2.37852513216
2.043928 2.38883656004
2.048204 2.39941969572
2.05248 2.41029796508
2.056756 2.42149799404
2.061032 2.43305022454
2.065308 2.44498968708
2.069584 2.45735698037
2.07386 2.47019952875
2.078136 2.48357321802
2.082412 2.49754455559
2.086688 2.51219357155
2.090964 2.52761778937
2.09524 2.54393777949
2.099516 2.56130512271
2.103792 2.57991416411
2.108068 2.60001996329
2.112344 2.62196684798
2.11662 2.64623614777
2.120896 2.67353109548
2.125172 2.70494037594
2.129448 2.74228875552
2.133724 2.78901262453


==> figuresAndData/dataForRayleigh-midPoint-sigma1pt5.tex <==
0.0 0.302797401727
0.0064 0.302838924999
0.0128 0.302962472597
0.0192 0.303166520526
0.0256 0.3034495646
0.032 0.30381012057
0.0384 0.304246724243
0.0448 0.304757931581
0.0512 0.305342318789
0.0576 0.305998482385
0.064 0.306725039257
0.0704 0.307520626704
0.0768 0.308383902466
0.0832 0.309313544735
0.0896 0.310308252153
0.096 0.311366743803
0.1024 0.312487759176
0.1088 0.313670058135
0.1152 0.314912420859
0.1216 0.316213647777
0.128 0.317572559492
0.1344 0.318987996693
0.1408 0.320458820051
0.1472 0.321983910111
0.1536 0.323562167168
0.16 0.325192511137
0.1664 0.32687388141
0.1728 0.328605236709
0.1792 0.33038555492
0.1856 0.332213832934
0.192 0.334089086466
0.1984 0.336010349874
0.2048 0.337976675968
0.2112 0.339987135816
0.2176 0.34204081854
0.224 0.344136831109
0.2304 0.346274298125
0.2368 0.348452361604
0.2432 0.350670180755
0.2496 0.352926931753
0.256 0.35522180751
0.2624 0.357554017437
0.2688 0.359922787213
0.2752 0.362327358544
0.2816 0.364766988923
0.288 0.367240951384
0.2944 0.369748534262
0.3008 0.372289040947
0.3072 0.374861789634
0.3136 0.37746611308
0.32 0.380101358359
0.3264 0.382766886607
0.3328 0.385462072786
0.3392 0.388186305429
0.3456 0.3909389864
0.352 0.393719530648
0.3584 0.396527365962
0.3648 0.399361932733
0.3712 0.402222683713
0.3776 0.405109083773
0.384 0.408020609671
0.3904 0.410956749817
0.3968 0.413917004039
0.4032 0.416900883354
0.4096 0.419907909741
0.416 0.422937615919
0.4224 0.425989545119
0.4288 0.429063250871
0.4352 0.432158296784
0.4416 0.435274256335
0.448 0.438410712657
0.4544 0.441567258333
0.4608 0.444743495189
0.4672 0.447939034099
0.4736 0.45115349478
0.48 0.454386505606
0.4864 0.457637703407
0.4928 0.46090673329
0.4992 0.464193248447
0.5056 0.467496909982
0.512 0.470817386723
0.5184 0.474154355056
0.5248 0.477507498748
0.5312 0.480876508784
0.5376 0.484261083195
0.544 0.487660926904
0.5504 0.491075751563
0.5568 0.494505275398
0.5632 0.49794922306
0.5696 0.501407325472
0.576 0.504879319689
0.5824 0.508364948749
0.5888 0.511863961539
0.5952 0.515376112654
0.6016 0.518901162266
0.608 0.522438875996
0.6144 0.525989024779
0.6208 0.529551384746
0.6272 0.5331257371
0.6336 0.536711867997
0.64 0.540309568425
0.6464 0.543918634099
0.6528 0.547538865342
0.6592 0.551170066981
0.6656 0.554812048237
0.672 0.558464622628
0.6784 0.562127607859
0.6848 0.565800825731
0.6912 0.56948410204
0.6976 0.573177266488
0.704 0.576880152583
0.7104 0.580592597559
0.7168 0.58431444228
0.7232 0.588045531162
0.7296 0.591785712086
0.736 0.595534836315
0.7424 0.59929275842
0.7488 0.603059336198
0.7552 0.606834430602
0.7616 0.610617905662
0.768 0.614409628415
0.7744 0.618209468838
0.7808 0.622017299776
0.7872 0.62583299688
0.7936 0.629656438538
0.8 0.633487505813
0.8064 0.637326082383
0.8128 0.64117205448
0.8192 0.645025310832
0.8256 0.648885742604
0.832 0.652753243346
0.8384 0.656627708935
0.8448 0.660509037525
0.8512 0.664397129495
0.8576 0.668291887396
0.864 0.672193215907
0.8704 0.676101021783
0.8768 0.68001521381
0.8832 0.683935702762
0.8896 0.687862401353
0.896 0.691795224195
0.9024 0.69573408776
0.9088 0.699678910332
0.9152 0.703629611973
0.9216 0.707586114483
0.928 0.711548341359
0.9344 0.715516217764
0.9408 0.719489670484
0.9472 0.723468627897
0.9536 0.727453019942
0.96 0.731442778077
0.9664 0.735437835255
0.9728 0.739438125889
0.9792 0.743443585818
0.9856 0.747454152284
0.992 0.751469763896
0.9984 0.755490360607
1.0048 0.759515883682
1.0112 0.763546275672
1.0176 0.76758148039
1.024 0.771621442881
1.0304 0.7756661094
1.0368 0.779715427389
1.0432 0.783769345448
1.0496 0.787827813317
1.056 0.791890781848
1.0624 0.795958202991
1.0688 0.800030029763
1.0752 0.804106216234
1.0816 0.808186717503
1.088 0.812271489682
1.0944 0.81636048987
1.1008 0.820453676141
1.1072 0.824551007522
1.1136 0.828652443975
1.12 0.832757946381
1.1264 0.836867476522
1.1328 0.840980997064
1.1392 0.845098471543
1.1456 0.849219864347
1.152 0.853345140699
1.1584 0.857474266649
1.1648 0.86160720905
1.1712 0.865743935552
1.1776 0.869884414584
1.184 0.87402861534
1.1904 0.878176507769
1.1968 0.882328062559
1.2032 0.886483251126
1.2096 0.890642045604
1.216 0.894804418828
1.2224 0.898970344328
1.2288 0.903139796314
1.2352 0.907312749667
1.2416 0.911489179928
1.248 0.915669063287
1.2544 0.919852376575
1.2608 0.924039097251
1.2672 0.928229203395
1.2736 0.932422673698
1.28 0.936619487453
1.2864 0.940819624547
1.2928 0.945023065451
1.2992 0.949229791212
1.3056 0.953439783447
1.312 0.957653024333
1.3184 0.961869496599
1.3248 0.966089183521
1.3312 0.970312068914
1.3376 0.974538137124
1.344 0.97876737302
1.3504 0.982999761993
1.3568 0.987235289944
1.3632 0.991473943278
1.3696 0.995715708904
1.376 0.999960574222
1.3824 1.00420852712
1.3888 1.00845955597
1.3952 1.01271364963
1.4016 1.01697079742
1.408 1.02123098912
1.4144 1.025494215
1.4208 1.02976046576
1.4272 1.03402973257
1.4336 1.03830200705
1.44 1.04257728126
1.4464 1.0468555477
1.4528 1.05113679933
1.4592 1.0554210295
1.4656 1.05970823204
1.472 1.06399840117
1.4784 1.06829153156
1.4848 1.07258761828
1.4912 1.07688665683
1.4976 1.08118864313
1.504 1.08549357351
1.5104 1.0898014447
1.5168 1.09411225384
1.5232 1.09842599849
1.5296 1.1027426766
1.536 1.10706228652
1.5424 1.11138482701
1.5488 1.11571029722
1.5552 1.1200386967
1.5616 1.12437002539
1.568 1.12870428362
1.5744 1.13304147213
1.5808 1.13738159203
1.5872 1.14172464482
1.5936 1.14607063241
1.6 1.15041955707
1.6064 1.15477142148
1.6128 1.1591262287
1.6192 1.16348398216
1.6256 1.16784468569
1.632 1.17220834351
1.6384 1.17657496021
1.6448 1.18094454079
1.6512 1.1853170906
1.6576 1.1896926154
1.664 1.19407112134
1.6704 1.19845261493
1.6768 1.2028371031
1.6832 1.20722459314
1.6896 1.21161509273
1.696 1.21600860997
1.7024 1.2204051533
1.7088 1.2248047316
1.7152 1.22920735412
1.7216 1.23361303048
1.728 1.23802177075
1.7344 1.24243358534
1.7408 1.24684848511
1.7472 1.25126648127
1.7536 1.25568758546
1.76 1.26011180973
1.7664 1.26453916653
1.7728 1.26896966869
1.7792 1.27340332951
1.7856 1.27784016264
1.792 1.28228018218
1.7984 1.28672340266
1.8048 1.291169839
1.8112 1.29561950656
1.8176 1.30007242114
1.824 1.30452859895
1.8304 1.30898805664
1.8368 1.31345081131
1.8432 1.31791688049
1.8496 1.32238628216
1.856 1.32685903474
1.8624 1.33133515712
1.8688 1.33581466864
1.8752 1.3402975891
1.8816 1.34478393877
1.888 1.34927373839
1.8944 1.35376700919
1.9008 1.35826377284
1.9072 1.36276405155
1.9136 1.36726786799
1.92 1.37177524534
1.9264 1.37628620726
1.9328 1.38080077795
1.9392 1.38531898212
1.9456 1.38984084498
1.952 1.39436639228
1.9584 1.39889565031
1.9648 1.40342864589
1.9712 1.4079654064
1.9776 1.41250595977
1.984 1.41705033449
1.9904 1.42159855961
1.9968 1.42615066478
2.0032 1.43070668022
2.0096 1.43526663675
2.016 1.43983056579
2.0224 1.44439849937
2.0288 1.44897047015
2.0352 1.4535465114
2.0416 1.45812665704
2.048 1.46271094165
2.0544 1.46729940044
2.0608 1.47189206932
2.0672 1.47648898485
2.0736 1.48109018429
2.08 1.48569570563
2.0864 1.49030558752
2.0928 1.49491986936
2.0992 1.49953859131
2.1056 1.50416179422
2.112 1.50878951977
2.1184 1.51342181035
2.1248 1.51805870917
2.1312 1.52270026025
2.1376 1.5273465084
2.144 1.53199749927
2.1504 1.53665327937
2.1568 1.54131389603
2.1632 1.5459793975
2.1696 1.55064983288
2.176 1.55532525222
2.1824 1.56000570647
2.1888 1.56469124752
2.1952 1.56938192823
2.2016 1.57407780243
2.208 1.57877892497
2.2144 1.58348535169
2.2208 1.58819713948
2.2272 1.59291434628
2.2336 1.59763703114
2.24 1.60236525417
2.2464 1.60709907664
2.2528 1.61183856093
2.2592 1.61658377063
2.2656 1.6213347705
2.272 1.62609162652
2.2784 1.63085440595
2.2848 1.63562317727
2.2912 1.64039801031
2.2976 1.6451789762
2.304 1.64996614745
2.3104 1.65475959793
2.3168 1.65955940296
2.3232 1.66436563929
2.3296 1.66917838518
2.336 1.67399772038
2.3424 1.6788237262
2.3488 1.68365648557
2.3552 1.688496083
2.3616 1.6933426047
2.368 1.69819613857
2.3744 1.70305677427
2.3808 1.70792460323
2.3872 1.71279971873
2.3936 1.71768221591
2.4 1.72257219183
2.4064 1.72746974556
2.4128 1.73237497815
2.4192 1.73728799273
2.4256 1.74220889457
2.432 1.74713779111
2.4384 1.75207479203
2.4448 1.7570200093
2.4512 1.76197355725
2.4576 1.76693555265
2.464 1.77190611471
2.4704 1.77688536522
2.4768 1.7818734286
2.4832 1.78687043195
2.4896 1.79187650512
2.496 1.79689178085
2.5024 1.80191639476
2.5088 1.80695048552
2.5152 1.81199419487
2.5216 1.81704766776
2.528 1.82211105239
2.5344 1.82718450037
2.5408 1.83226816675
2.5472 1.83736221022
2.5536 1.8424667931
2.56 1.84758208155
2.5664 1.85270824565
2.5728 1.85784545952
2.5792 1.86299390145
2.5856 1.86815375405
2.592 1.87332520435
2.5984 1.87850844401
2.6048 1.88370366938
2.6112 1.88891108174
2.6176 1.89413088743
2.624 1.899363298
2.6304 1.90460853043
2.6368 1.90986680729
2.6432 1.91513835694
2.6496 1.92042341375
2.656 1.92572221827
2.6624 1.93103501752
2.6688 1.93636206515
2.6752 1.94170362176
2.6816 1.9470599551
2.688 1.95243134035
2.6944 1.95781806044
2.7008 1.9632204063
2.7072 1.96863867719
2.7136 1.97407318106
2.72 1.97952423483
2.7264 1.98499216481
2.7328 1.99047730707
2.7392 1.99598000782
2.7456 2.00150062387
2.752 2.00703952305
2.7584 2.01259708471
2.7648 2.0181737002
2.7712 2.0237697734
2.7776 2.02938572131
2.784 2.03502197462
2.7904 2.04067897833
2.7968 2.04635719246
2.8032 2.0520570927
2.8096 2.05777917123
2.816 2.06352393747
2.8224 2.06929191897
2.8288 2.0750836623
2.8352 2.08089973402
2.8416 2.08674072173
2.848 2.09260723517
2.8544 2.09849990741
2.8608 2.10441939612
2.8672 2.11036638493
2.8736 2.11634158489
2.88 2.12234573606
2.8864 2.12837960918
2.8928 2.13444400751
2.8992 2.14053976879
2.9056 2.1466677674
2.912 2.15282891661
2.9184 2.15902417114
2.9248 2.16525452983
2.9312 2.17152103862
2.9376 2.17782479374
2.944 2.18416694526
2.9504 2.19054870092
2.9568 2.19697133031
2.9632 2.20343616953
2.9696 2.2099446263
2.976 2.21649818551
2.9824 2.22309841551
2.9888 2.22974697492
2.9952 2.23644562037
3.0016 2.24319621495
3.008 2.25000073781
3.0144 2.25686129487
3.0208 2.26378013081
3.0272 2.27075964275
3.0336 2.27780239559
3.04 2.28491113965
3.0464 2.29208883067
3.0528 2.29933865288
3.0592 2.3066640456
3.0656 2.31406873402
3.072 2.32155676528
3.0784 2.32913255059
3.0848 2.33680091521
3.0912 2.34456715779
3.0976 2.35243712167
3.104 2.36041728101
3.1104 2.3685148462
3.1168 2.37673789383
3.1232 2.38509552917
3.1296 2.39359809182
3.136 2.40225741992
3.1424 2.41108719547
3.1488 2.42010340443
3.1552 2.42932496378
3.1616 2.43877459912
3.168 2.44848011221
3.1744 2.45847628348
3.1808 2.46880786649
3.1872 2.47953459676
3.1936 2.49074027328


==> figuresAndData/dataForRayleigh-midPoint-sigma1pt5prob0pt05.tex <==
0.0 0.240218559204
0.004276 0.242366574095
0.008552 0.244534616277
0.012828 0.246722678277
0.017104 0.24893074765
0.02138 0.251158806998
0.025656 0.253406833986
0.029932 0.255674801375
0.034208 0.25796267705
0.038484 0.260270424067
0.04276 0.262598000692
0.047036 0.264945360456
0.051312 0.26731245221
0.055588 0.269699220186
0.059864 0.272105604069
0.06414 0.274531539063
0.068416 0.276976955971
0.072692 0.279441781279
0.076968 0.281925937237
0.081244 0.284429341953
0.08552 0.286951909485
0.089796 0.28949354994
0.094072 0.292054169574
0.098348 0.294633670899
0.102624 0.297231952785
0.1069 0.299848910577
0.111176 0.3024844362
0.115452 0.305138418279
0.119728 0.307810742253
0.124004 0.310501290492
0.12828 0.313209942418
0.132556 0.315936574626
0.136832 0.318681061001
0.141108 0.321443272847
0.145384 0.324223079002
0.14966 0.327020345964
0.153936 0.329834938013
0.158212 0.332666717333
0.162488 0.335515544134
0.166764 0.338381276769
0.17104 0.341263771859
0.175316 0.344162884408
0.179592 0.347078467925
0.183868 0.350010374533
0.188144 0.35295845509
0.19242 0.355922559298
0.196696 0.358902535815
0.200972 0.361898232364
0.205248 0.364909495841
0.209524 0.367936172416
0.2138 0.370978107638
0.218076 0.374035146535
0.222352 0.377107133712
0.226628 0.38019391344
0.230904 0.383295329758
0.23518 0.386411226554
0.239456 0.389541447657
0.243732 0.392685836919
0.248008 0.395844238296
0.252284 0.399016495929
0.25656 0.402202454219
0.260836 0.405401957898
0.265112 0.408614852102
0.269388 0.411840982439
0.273664 0.41508019505
0.27794 0.418332336676
0.282216 0.421597254714
0.286492 0.424874797275
0.290768 0.428164813238
0.295044 0.4314671523
0.29932 0.434781665028
0.303596 0.438108202903
0.307872 0.441446618365
0.312148 0.444796764851
0.316424 0.448158496841
0.3207 0.451531669887
0.324976 0.454916140653
0.329252 0.458311766945
0.333528 0.461718407741
0.337804 0.46513592322
0.34208 0.468564174785
0.346356 0.472003025092
0.350632 0.475452338068
0.354908 0.478911978932
0.359184 0.482381814213
0.36346 0.48586171177
0.367736 0.489351540802
0.372012 0.492851171863
0.376288 0.496360476878
0.380564 0.499879329146
0.38484 0.503407603355
0.389116 0.506945175585
0.393392 0.510491923319
0.397668 0.514047725443
0.401944 0.517612462253
0.40622 0.521186015456
0.410496 0.524768268172
0.414772 0.528359104933
0.419048 0.531958411687
0.423324 0.535566075789
0.4276 0.539181986006
0.431876 0.542806032507
0.436152 0.546438106866
0.440428 0.55007810205
0.444704 0.553725912418
0.44898 0.557381433714
0.453256 0.561044563058
0.457532 0.56471519894
0.461808 0.568393241214
0.466084 0.572078591083
0.47036 0.575771151098
0.474636 0.579470825142
0.478912 0.583177518423
0.483188 0.586891137461
0.487464 0.590611590082
0.49174 0.594338785403
0.496016 0.598072633819
0.500292 0.601813046997
0.504568 0.605559937859
0.508844 0.60931322057
0.51312 0.61307281053
0.517396 0.616838624355
0.521672 0.620610579869
0.525948 0.62438859609
0.530224 0.628172593215
0.5345 0.631962492608
0.538776 0.635758216787
0.543052 0.63955968941
0.547328 0.643366835263
0.551604 0.647179580242
0.55588 0.650997851346
0.560156 0.654821576658
0.564432 0.658650685334
0.568708 0.662485107587
0.572984 0.666324774678
0.57726 0.670169618897
0.581536 0.674019573553
0.585812 0.677874572959
0.590088 0.681734552419
0.594364 0.685599448214
0.59864 0.689469197589
0.602916 0.693343738741
0.607192 0.697223010802
0.611468 0.701106953832
0.615744 0.704995508799
0.62002 0.708888617572
0.624296 0.712786222902
0.628572 0.716688268417
0.632848 0.720594698603
0.637124 0.724505458794
0.6414 0.728420495158
0.645676 0.732339754688
0.649952 0.736263185187
0.654228 0.740190735256
0.658504 0.744122354283
0.66278 0.748057992431
0.667056 0.751997600628
0.671332 0.755941130552
0.675608 0.759888534621
0.679884 0.763839765984
0.68416 0.767794778506
0.688436 0.771753526762
0.692712 0.775715966019
0.696988 0.779682052234
0.701264 0.783651742035
0.70554 0.787624992718
0.709816 0.79160176223
0.714092 0.795582009164
0.718368 0.799565692746
0.722644 0.803552772829
0.72692 0.807543209875
0.731196 0.811536964957
0.735472 0.815533999738
0.739748 0.819534276471
0.744024 0.823537757983
0.7483 0.827544407671
0.752576 0.831554189489
0.756852 0.835567067943
0.761128 0.839583008078
0.765404 0.843601975475
0.76968 0.847623936236
0.773956 0.851648856983
0.778232 0.855676704842
0.782508 0.859707447442
0.786784 0.863741052904
0.79106 0.867777489833
0.795336 0.871816727308
0.799612 0.875858734883
0.803888 0.879903482569
0.808164 0.883950940833
0.81244 0.888001080591
0.816716 0.892053873197
0.820992 0.89610929044
0.825268 0.900167304535
0.829544 0.904227888116
0.83382 0.908291014233
0.838096 0.91235665634
0.842372 0.916424788293
0.846648 0.920495384341
0.850924 0.924568419122
0.8552 0.928643867655
0.859476 0.932721705337
0.863752 0.936801907932
0.868028 0.940884451571
0.872304 0.944969312741
0.87658 0.949056468284
0.880856 0.95314589539
0.885132 0.957237571588
0.889408 0.961331474748
0.893684 0.965427583068
0.89796 0.969525875076
0.902236 0.973626329617
0.906512 0.977728925857
0.910788 0.981833643272
0.915064 0.985940461643
0.91934 0.990049361056
0.923616 0.994160321892
0.927892 0.998273324828
0.932168 1.00238835083
0.936444 1.00650538114
0.94072 1.01062439729
0.944996 1.01474538108
0.949272 1.01886831459
0.953548 1.02299318016
0.957824 1.0271199604
0.9621 1.03124863816
0.966376 1.03537919658
0.970652 1.03951161902
0.974928 1.04364588911
0.979204 1.0477819907
0.98348 1.05191990791
0.987756 1.05605962507
0.992032 1.06020112676
0.996308 1.06434439779
1.000584 1.06848942319
1.00486 1.07263618822
1.009136 1.07678467834
1.013412 1.08093487926
1.017688 1.08508677689
1.021964 1.08924035733
1.02624 1.09339560691
1.030516 1.09755251217
1.034792 1.10171105984
1.039068 1.10587123685
1.043344 1.11003303032
1.04762 1.11419642757
1.051896 1.11836141612
1.056172 1.12252798366
1.060448 1.12669611808
1.064724 1.13086580744
1.069 1.13503703999
1.073276 1.13920980416
1.077552 1.14338408853
1.081828 1.1475598819
1.086104 1.15173717318
1.09038 1.1559159515
1.094656 1.16009620613
1.098932 1.16427792651
1.103208 1.16846110224
1.107484 1.17264572308
1.11176 1.17683177895
1.116036 1.18101925991
1.120312 1.18520815618
1.124588 1.18939845815
1.128864 1.19359015634
1.13314 1.1977832414
1.137416 1.20197770417
1.141692 1.20617353559
1.145968 1.21037072677
1.150244 1.21456926894
1.15452 1.21876915347
1.158796 1.22297037188
1.163072 1.22717291581
1.167348 1.23137677703
1.171624 1.23558194746
1.1759 1.23978841913
1.180176 1.2439961842
1.184452 1.24820523497
1.188728 1.25241556383
1.193004 1.25662716334
1.19728 1.26084002615
1.201556 1.26505414503
1.205832 1.26926951288
1.210108 1.27348612272
1.214384 1.27770396765
1.21866 1.28192304094
1.222936 1.28614333593
1.227212 1.29036484608
1.231488 1.29458756497
1.235764 1.29881148629
1.24004 1.30303660383
1.244316 1.30726291147
1.248592 1.31149040323
1.252868 1.31571907321
1.257144 1.31994891562
1.26142 1.32417992477
1.265696 1.32841209507
1.269972 1.33264542104
1.274248 1.33687989726
1.278524 1.34111551847
1.2828 1.34535227944
1.287076 1.34959017509
1.291352 1.3538292004
1.295628 1.35806935045
1.299904 1.36231062042
1.30418 1.36655300558
1.308456 1.37079650129
1.312732 1.37504110298
1.317008 1.37928680619
1.321284 1.38353360655
1.32556 1.38778149976
1.329836 1.39203048162
1.334112 1.39628054801
1.338388 1.40053169489
1.342664 1.4047839183
1.34694 1.40903721437
1.351216 1.41329157932
1.355492 1.41754700943
1.359768 1.42180350108
1.364044 1.42606105072
1.36832 1.43031965488
1.372596 1.43457931016
1.376872 1.43884001325
1.381148 1.4431017609
1.385424 1.44736454997
1.3897 1.45162837736
1.393976 1.45589324006
1.398252 1.46015913513
1.402528 1.4644260597
1.406804 1.46869401098
1.41108 1.47296298626
1.415356 1.47723298288
1.419632 1.48150399827
1.423908 1.48577602992
1.428184 1.49004907539
1.43246 1.49432313232
1.436736 1.49859819841
1.441012 1.50287427142
1.445288 1.5071513492
1.449564 1.51142942966
1.45384 1.51570851076
1.458116 1.51998859054
1.462392 1.52426966711
1.466668 1.52855173864
1.470944 1.53283480337
1.47522 1.5371188596
1.479496 1.54140390569
1.483772 1.54568994007
1.488048 1.54997696123
1.492324 1.55426496774
1.4966 1.55855395821
1.500876 1.56284393131
1.505152 1.5671348858
1.509428 1.57142682048
1.513704 1.57571973422
1.51798 1.58001362594
1.522256 1.58430849463
1.526532 1.58860433935
1.530808 1.59290115919
1.535084 1.59719895333
1.53936 1.601497721
1.543636 1.60579746149
1.547912 1.61009817413
1.552188 1.61439985835
1.556464 1.6187025136
1.56074 1.6230061394
1.565016 1.62731073533
1.569292 1.63161630104
1.573568 1.63592283622
1.577844 1.64023034063
1.58212 1.64453881406
1.586396 1.6488482564
1.590672 1.65315866756
1.594948 1.65747004753
1.599224 1.66178239634
1.6035 1.66609571409
1.607776 1.67041000093
1.612052 1.67472525706
1.616328 1.67904148274
1.620604 1.6833586783
1.62488 1.68767684411
1.629156 1.69199598059
1.633432 1.69631608823
1.637708 1.70063716756
1.641984 1.70495921919
1.64626 1.70928224376
1.650536 1.71360624198
1.654812 1.7179312146
1.659088 1.72225716245
1.663364 1.72658408638
1.66764 1.73091198732
1.671916 1.73524086625
1.676192 1.73957072421
1.680468 1.74390156228
1.684744 1.7482333816
1.68902 1.75256618337
1.693296 1.75689996884
1.697572 1.76123473931
1.701848 1.76557049616
1.706124 1.76990724078
1.7104 1.77424497465
1.714676 1.7785836993
1.718952 1.78292341629
1.723228 1.78726412728
1.727504 1.79160583393
1.73178 1.79594853799
1.736056 1.80029224127
1.740332 1.80463694561
1.744608 1.80898265292
1.748884 1.81332936515
1.75316 1.81767708433
1.757436 1.82202581253
1.761712 1.82637555187
1.765988 1.83072630453
1.770264 1.83507807276
1.77454 1.83943085884
1.778816 1.84378466512
1.783092 1.84813949401
1.787368 1.85249534796
1.791644 1.85685222949
1.79592 1.86121014118
1.800196 1.86556908564
1.804472 1.86992906557
1.808748 1.87429008371
1.813024 1.87865214284
1.8173 1.88301524583
1.821576 1.8873793956
1.825852 1.89174459509
1.830128 1.89611084736
1.834404 1.90047815547
1.83868 1.90484652256
1.842956 1.90921595185
1.847232 1.91358644659
1.851508 1.91795801009
1.855784 1.92233064572
1.86006 1.92670435694
1.864336 1.93107914722
1.868612 1.93545502012
1.872888 1.93983197926
1.877164 1.94421002831
1.88144 1.948589171
1.885716 1.95296941112
1.889992 1.95735075254
1.894268 1.96173319917
1.898544 1.96611675498
1.90282 1.97050142402
1.907096 1.97488721039
1.911372 1.97927411825
1.915648 1.98366215184
1.919924 1.98805131544
1.9242 1.9924416134
1.928476 1.99683305015
1.932752 2.00122563017
1.937028 2.005619358
1.941304 2.01001423826
1.94558 2.01441027562
1.949856 2.01880747484
1.954132 2.02320584071
1.958408 2.02760537812
1.962684 2.03200609201
1.96696 2.03640798739
1.971236 2.04081106934
1.975512 2.04521534302
1.979788 2.04962081362
1.984064 2.05402748645
1.98834 2.05843536686
1.992616 2.06284446027
1.996892 2.06725477218
2.001168 2.07166630816
2.005444 2.07607907385
2.00972 2.08049307497
2.013996 2.0849083173
2.018272 2.08932480669
2.022548 2.09374254909
2.026824 2.0981615505
2.0311 2.102581817
2.035376 2.10700335475
2.039652 2.11142616999
2.043928 2.11585026904
2.048204 2.12027565827
2.05248 2.12470234416
2.056756 2.12913033325
2.061032 2.13355963218
2.065308 2.13799024765
2.069584 2.14242218644
2.07386 2.14685545542
2.078136 2.15129006155
2.082412 2.15572601186
2.086688 2.16016331346
2.090964 2.16460197357
2.09524 2.16904199946
2.099516 2.1734833985
2.103792 2.17792617817
2.108068 2.182370346
2.112344 2.18681590962
2.11662 2.19126287677
2.120896 2.19571125526
2.125172 2.20016105298
2.129448 2.20461227795
2.133724 2.20906493823


==> figuresAndData/dataForRayleigh-midPoint-sigma1pt5prob0pt5.tex <==
0.0 0.240218559204
0.004276 0.242366574095
0.008552 0.244534616277
0.012828 0.246722678277
0.017104 0.24893074765
0.02138 0.251158806998
0.025656 0.253406833986
0.029932 0.255674801375
0.034208 0.25796267705
0.038484 0.260270424067
0.04276 0.262598000692
0.047036 0.264945360456
0.051312 0.26731245221
0.055588 0.269699220186
0.059864 0.272105604069
0.06414 0.274531539063
0.068416 0.276976955971
0.072692 0.279441781279
0.076968 0.281925937237
0.081244 0.284429341953
0.08552 0.286951909485
0.089796 0.28949354994
0.094072 0.292054169574
0.098348 0.294633670899
0.102624 0.297231952785
0.1069 0.299848910577
0.111176 0.3024844362
0.115452 0.305138418279
0.119728 0.307810742253
0.124004 0.310501290492
0.12828 0.313209942418
0.132556 0.315936574626
0.136832 0.318681061001
0.141108 0.321443272847
0.145384 0.324223079002
0.14966 0.327020345964
0.153936 0.329834938013
0.158212 0.332666717333
0.162488 0.335515544134
0.166764 0.338381276769
0.17104 0.341263771859
0.175316 0.344162884408
0.179592 0.347078467925
0.183868 0.350010374533
0.188144 0.35295845509
0.19242 0.355922559298
0.196696 0.358902535815
0.200972 0.361898232364
0.205248 0.364909495841
0.209524 0.367936172416
0.2138 0.370978107638
0.218076 0.374035146535
0.222352 0.377107133712
0.226628 0.38019391344
0.230904 0.383295329758
0.23518 0.386411226554
0.239456 0.389541447657
0.243732 0.392685836919
0.248008 0.395844238296
0.252284 0.399016495929
0.25656 0.402202454219
0.260836 0.405401957898
0.265112 0.408614852102
0.269388 0.411840982439
0.273664 0.41508019505
0.27794 0.418332336676
0.282216 0.421597254714
0.286492 0.424874797275
0.290768 0.428164813238
0.295044 0.4314671523
0.29932 0.434781665028
0.303596 0.438108202903
0.307872 0.441446618365
0.312148 0.444796764851
0.316424 0.448158496841
0.3207 0.451531669887
0.324976 0.454916140653
0.329252 0.458311766945
0.333528 0.461718407741
0.337804 0.46513592322
0.34208 0.468564174785
0.346356 0.472003025092
0.350632 0.475452338068
0.354908 0.478911978932
0.359184 0.482381814213
0.36346 0.48586171177
0.367736 0.489351540802
0.372012 0.492851171863
0.376288 0.496360476878
0.380564 0.499879329146
0.38484 0.503407603355
0.389116 0.506945175585
0.393392 0.510491923319
0.397668 0.514047725443
0.401944 0.517612462253
0.40622 0.521186015456
0.410496 0.524768268172
0.414772 0.528359104933
0.419048 0.531958411687
0.423324 0.535566075789
0.4276 0.539181986006
0.431876 0.542806032507
0.436152 0.546438106866
0.440428 0.55007810205
0.444704 0.553725912418
0.44898 0.557381433714
0.453256 0.561044563058
0.457532 0.56471519894
0.461808 0.568393241214
0.466084 0.572078591083
0.47036 0.575771151098
0.474636 0.579470825142
0.478912 0.583177518423
0.483188 0.586891137461
0.487464 0.590611590082
0.49174 0.594338785403
0.496016 0.598072633819
0.500292 0.601813046997
0.504568 0.605559937859
0.508844 0.60931322057
0.51312 0.61307281053
0.517396 0.616838624355
0.521672 0.620610579869
0.525948 0.62438859609
0.530224 0.628172593215
0.5345 0.631962492608
0.538776 0.635758216787
0.543052 0.63955968941
0.547328 0.643366835263
0.551604 0.647179580242
0.55588 0.650997851346
0.560156 0.654821576658
0.564432 0.658650685334
0.568708 0.662485107587
0.572984 0.666324774678
0.57726 0.670169618897
0.581536 0.674019573553
0.585812 0.677874572959
0.590088 0.681734552419
0.594364 0.685599448214
0.59864 0.689469197589
0.602916 0.693343738741
0.607192 0.697223010802
0.611468 0.701106953832
0.615744 0.704995508799
0.62002 0.708888617572
0.624296 0.712786222902
0.628572 0.716688268417
0.632848 0.720594698603
0.637124 0.724505458794
0.6414 0.728420495158
0.645676 0.732339754688
0.649952 0.736263185187
0.654228 0.740190735256
0.658504 0.744122354283
0.66278 0.748057992431
0.667056 0.751997600628
0.671332 0.755941130552
0.675608 0.759888534621
0.679884 0.763839765984
0.68416 0.767794778506
0.688436 0.771753526762
0.692712 0.775715966019
0.696988 0.779682052234
0.701264 0.783651742035
0.70554 0.787624992718
0.709816 0.79160176223
0.714092 0.795582009164
0.718368 0.799565692746
0.722644 0.803552772829
0.72692 0.807543209875
0.731196 0.811536964957
0.735472 0.815533999738
0.739748 0.819534276471
0.744024 0.823537757983
0.7483 0.827544407671
0.752576 0.831554189489
0.756852 0.835567067943
0.761128 0.839583008078
0.765404 0.843601975475
0.76968 0.847623936236
0.773956 0.851648856983
0.778232 0.855676704842
0.782508 0.859707447442
0.786784 0.863741052904
0.79106 0.867777489833
0.795336 0.871816727308
0.799612 0.875858734883
0.803888 0.879903482569
0.808164 0.883950940833
0.81244 0.888001080591
0.816716 0.892053873197
0.820992 0.89610929044
0.825268 0.900167304535
0.829544 0.904227888116
0.83382 0.908291014233
0.838096 0.91235665634
0.842372 0.916424788293
0.846648 0.920495384341
0.850924 0.924568419122
0.8552 0.928643867655
0.859476 0.932721705337
0.863752 0.936801907932
0.868028 0.940884451571
0.872304 0.944969312741
0.87658 0.949056468284
0.880856 0.95314589539
0.885132 0.957237571588
0.889408 0.961331474748
0.893684 0.965427583068
0.89796 0.969525875076
0.902236 0.973626329617
0.906512 0.977728925857
0.910788 0.981833643272
0.915064 0.985940461643
0.91934 0.990049361056
0.923616 0.994160321892
0.927892 0.998273324828
0.932168 1.00238835083
0.936444 1.00650538114
0.94072 1.01062439729
0.944996 1.01474538108
0.949272 1.01886831459
0.953548 1.02299318016
0.957824 1.0271199604
0.9621 1.03124863816
0.966376 1.03537919658
0.970652 1.03951161902
0.974928 1.04364588911
0.979204 1.0477819907
0.98348 1.05191990791
0.987756 1.05605962507
0.992032 1.06020112676
0.996308 1.06434439779
1.000584 1.06848942319
1.00486 1.07263618822
1.009136 1.07678467834
1.013412 1.08093487926
1.017688 1.08508677689
1.021964 1.08924035733
1.02624 1.09339560691
1.030516 1.09755251217
1.034792 1.10171105984
1.039068 1.10587123685
1.043344 1.11003303032
1.04762 1.11419642757
1.051896 1.11836141612
1.056172 1.12252798366
1.060448 1.12669611808
1.064724 1.13086580744
1.069 1.13503703999
1.073276 1.13920980416
1.077552 1.14338408853
1.081828 1.1475598819
1.086104 1.15173717318
1.09038 1.1559159515
1.094656 1.16009620613
1.098932 1.16427792651
1.103208 1.16846110224
1.107484 1.17264572308
1.11176 1.17683177895
1.116036 1.18101925991
1.120312 1.18520815618
1.124588 1.18939845815
1.128864 1.19359015634
1.13314 1.1977832414
1.137416 1.20197770417
1.141692 1.20617353559
1.145968 1.21037072677
1.150244 1.21456926894
1.15452 1.21876915347
1.158796 1.22297037188
1.163072 1.22717291581
1.167348 1.23137677703
1.171624 1.23558194746
1.1759 1.23978841913
1.180176 1.2439961842
1.184452 1.24820523497
1.188728 1.25241556383
1.193004 1.25662716334
1.19728 1.26084002615
1.201556 1.26505414503
1.205832 1.26926951288
1.210108 1.27348612272
1.214384 1.27770396765
1.21866 1.28192304094
1.222936 1.28614333593
1.227212 1.29036484608
1.231488 1.29458756497
1.235764 1.29881148629
1.24004 1.30303660383
1.244316 1.30726291147
1.248592 1.31149040323
1.252868 1.31571907321
1.257144 1.31994891562
1.26142 1.32417992477
1.265696 1.32841209507
1.269972 1.33264542104
1.274248 1.33687989726
1.278524 1.34111551847
1.2828 1.34535227944
1.287076 1.34959017509
1.291352 1.3538292004
1.295628 1.35806935045
1.299904 1.36231062042
1.30418 1.36655300558
1.308456 1.37079650129
1.312732 1.37504110298
1.317008 1.37928680619
1.321284 1.38353360655
1.32556 1.38778149976
1.329836 1.39203048162
1.334112 1.39628054801
1.338388 1.40053169489
1.342664 1.4047839183
1.34694 1.40903721437
1.351216 1.41329157932
1.355492 1.41754700943
1.359768 1.42180350108
1.364044 1.42606105072
1.36832 1.43031965488
1.372596 1.43457931016
1.376872 1.43884001325
1.381148 1.4431017609
1.385424 1.44736454997
1.3897 1.45162837736
1.393976 1.45589324006
1.398252 1.46015913513
1.402528 1.4644260597
1.406804 1.46869401098
1.41108 1.47296298626
1.415356 1.47723298288
1.419632 1.48150399827
1.423908 1.48577602992
1.428184 1.49004907539
1.43246 1.49432313232
1.436736 1.49859819841
1.441012 1.50287427142
1.445288 1.5071513492
1.449564 1.51142942966
1.45384 1.51570851076
1.458116 1.51998859054
1.462392 1.52426966711
1.466668 1.52855173864
1.470944 1.53283480337
1.47522 1.5371188596
1.479496 1.54140390569
1.483772 1.54568994007
1.488048 1.54997696123
1.492324 1.55426496774
1.4966 1.55855395821
1.500876 1.56284393131
1.505152 1.5671348858
1.509428 1.57142682048
1.513704 1.57571973422
1.51798 1.58001362594
1.522256 1.58430849463
1.526532 1.58860433935
1.530808 1.59290115919
1.535084 1.59719895333
1.53936 1.601497721
1.543636 1.60579746149
1.547912 1.61009817413
1.552188 1.61439985835
1.556464 1.6187025136
1.56074 1.6230061394
1.565016 1.62731073533
1.569292 1.63161630104
1.573568 1.63592283622
1.577844 1.64023034063
1.58212 1.64453881406
1.586396 1.6488482564
1.590672 1.65315866756
1.594948 1.65747004753
1.599224 1.66178239634
1.6035 1.66609571409
1.607776 1.67041000093
1.612052 1.67472525706
1.616328 1.67904148274
1.620604 1.6833586783
1.62488 1.68767684411
1.629156 1.69199598059
1.633432 1.69631608823
1.637708 1.70063716756
1.641984 1.70495921919
1.64626 1.70928224376
1.650536 1.71360624198
1.654812 1.7179312146
1.659088 1.72225716245
1.663364 1.72658408638
1.66764 1.73091198732
1.671916 1.73524086625
1.676192 1.73957072421
1.680468 1.74390156228
1.684744 1.7482333816
1.68902 1.75256618337
1.693296 1.75689996884
1.697572 1.76123473931
1.701848 1.76557049616
1.706124 1.76990724078
1.7104 1.77424497465
1.714676 1.7785836993
1.718952 1.78292341629
1.723228 1.78726412728
1.727504 1.79160583393
1.73178 1.79594853799
1.736056 1.80029224127
1.740332 1.80463694561
1.744608 1.80898265292
1.748884 1.81332936515
1.75316 1.81767708433
1.757436 1.82202581253
1.761712 1.82637555187
1.765988 1.83072630453
1.770264 1.83507807276
1.77454 1.83943085884
1.778816 1.84378466512
1.783092 1.84813949401
1.787368 1.85249534796
1.791644 1.85685222949
1.79592 1.86121014118
1.800196 1.86556908564
1.804472 1.86992906557
1.808748 1.87429008371
1.813024 1.87865214284
1.8173 1.88301524583
1.821576 1.8873793956
1.825852 1.89174459509
1.830128 1.89611084736
1.834404 1.90047815547
1.83868 1.90484652256
1.842956 1.90921595185
1.847232 1.91358644659
1.851508 1.91795801009
1.855784 1.92233064572
1.86006 1.92670435694
1.864336 1.93107914722
1.868612 1.93545502012
1.872888 1.93983197926
1.877164 1.94421002831
1.88144 1.948589171
1.885716 1.95296941112
1.889992 1.95735075254
1.894268 1.96173319917
1.898544 1.96611675498
1.90282 1.97050142402
1.907096 1.97488721039
1.911372 1.97927411825
1.915648 1.98366215184
1.919924 1.98805131544
1.9242 1.9924416134
1.928476 1.99683305015
1.932752 2.00122563017
1.937028 2.005619358
1.941304 2.01001423826
1.94558 2.01441027562
1.949856 2.01880747484
1.954132 2.02320584071
1.958408 2.02760537812
1.962684 2.03200609201
1.96696 2.03640798739
1.971236 2.04081106934
1.975512 2.04521534302
1.979788 2.04962081362
1.984064 2.05402748645
1.98834 2.05843536686
1.992616 2.06284446027
1.996892 2.06725477218
2.001168 2.07166630816
2.005444 2.07607907385
2.00972 2.08049307497
2.013996 2.0849083173
2.018272 2.08932480669
2.022548 2.09374254909
2.026824 2.0981615505
2.0311 2.102581817
2.035376 2.10700335475
2.039652 2.11142616999
2.043928 2.11585026904
2.048204 2.12027565827
2.05248 2.12470234416
2.056756 2.12913033325
2.061032 2.13355963218
2.065308 2.13799024765
2.069584 2.14242218644
2.07386 2.14685545542
2.078136 2.15129006155
2.082412 2.15572601186
2.086688 2.16016331346
2.090964 2.16460197357
2.09524 2.16904199946
2.099516 2.1734833985
2.103792 2.17792617817
2.108068 2.182370346
2.112344 2.18681590962
2.11662 2.19126287677
2.120896 2.19571125526
2.125172 2.20016105298
2.129448 2.20461227795
2.133724 2.20906493823


==> figuresAndData/dataForRayleigh-midPoint-sigma2.tex <==
0.0 0.459043605026
0.00853 0.463330619152
0.01706 0.467661655327
0.02559 0.472036694963
0.03412 0.476455707107
0.04265 0.480918648484
0.05118 0.485425463566
0.05971 0.489976084645
0.06824 0.494570431933
0.07677 0.499208413674
0.0853 0.503889926274
0.09383 0.508614854449
0.10236 0.513383071382
0.11089 0.518194438903
0.11942 0.523048807679
0.12795 0.527946017418
0.13648 0.532885897088
0.14501 0.537868265146
0.15354 0.542892929783
0.16207 0.547959689173
0.1706 0.553068331743
0.17913 0.55821863644
0.18766 0.563410373019
0.19619 0.568643302329
0.20472 0.573917176614
0.21325 0.579231739813
0.22178 0.584586727875
0.23031 0.58998186907
0.23884 0.595416884306
0.24737 0.600891487458
0.2559 0.606405385684
0.26443 0.611958279756
0.27296 0.617549864385
0.28149 0.623179828554
0.29002 0.628847855835
0.29855 0.634553624726
0.30708 0.640296808968
0.31561 0.64607707787
0.32414 0.65189409663
0.33267 0.657747526646
0.3412 0.663637025834
0.34973 0.669562248931
0.35826 0.675522847802
0.36679 0.681518471732
0.37532 0.687548767724
0.38385 0.693613380779
0.39238 0.699711954181
0.40091 0.705844129765
0.40944 0.712009548187
0.41797 0.718207849178
0.4265 0.724438671802
0.43503 0.730701654695
0.44356 0.736996436301
0.45209 0.743322655105
0.46062 0.74967994985
0.46915 0.756067959751
0.47768 0.762486324701
0.48621 0.768934685467
0.49474 0.775412683879
0.50327 0.781919963009
0.5118 0.78845616735
0.52033 0.795020942976
0.52886 0.801613937701
0.53739 0.808234801231
0.54592 0.814883185304
0.55445 0.821558743824
0.56298 0.828261132995
0.57151 0.834990011431
0.58004 0.841745040281
0.58857 0.848525883327
0.5971 0.855332207087
0.60563 0.862163680908
0.61416 0.869019977053
0.62269 0.875900770784
0.63122 0.882805740431
0.63975 0.889734567467
0.64828 0.896686936569
0.65681 0.903662535672
0.66534 0.91066105603
0.67387 0.917682192256
0.6824 0.924725642366
0.69093 0.931791107821
0.69946 0.938878293556
0.70799 0.94598690801
0.71652 0.953116663153
0.72505 0.960267274504
0.73358 0.967438461151
0.74211 0.97462994576
0.75064 0.981841454591
0.75917 0.989072717501
0.7677 0.996323467948
0.77623 1.00359344299
0.78476 1.0108823833
0.79329 1.01819003311
0.80182 1.02551614029
0.81035 1.03286045624
0.81888 1.04022273596
0.82741 1.04760273799
0.83594 1.0550002244
0.84447 1.06241496079
0.853 1.06984671626
0.86153 1.07729526336
0.87006 1.08476037813
0.87859 1.09224184002
0.88712 1.0997394319
0.89565 1.10725293999
0.90418 1.1147821539
0.91271 1.12232686654
0.92124 1.1298868741
0.92977 1.13746197605
0.9383 1.14505197509
0.94683 1.1526566771
0.95536 1.16027589116
0.96389 1.16790942945
0.97242 1.17555710726
0.98095 1.18321874294
0.98948 1.19089415787
0.99801 1.19858317644
1.00654 1.20628562599
1.01507 1.21400133677
1.0236 1.22173014194
1.03213 1.2294718775
1.04066 1.23722638228
1.04919 1.24499349788
1.05772 1.25277306866
1.06625 1.26056494168
1.07478 1.26836896667
1.08331 1.27618499601
1.09184 1.28401288468
1.10037 1.29185249024
1.1089 1.29970367276
1.11743 1.30756629483
1.12596 1.3154402215
1.13449 1.32332532024
1.14302 1.33122146092
1.15155 1.33912851579
1.16008 1.34704635939
1.16861 1.3549748686
1.17714 1.36291392252
1.18567 1.37086340251
1.1942 1.37882319212
1.20273 1.38679317704
1.21126 1.39477324514
1.21979 1.40276328636
1.22832 1.41076319271
1.23685 1.41877285826
1.24538 1.42679217907
1.25391 1.43482105322
1.26244 1.44285938069
1.27097 1.45090706343
1.2795 1.45896400525
1.28803 1.46703011186
1.29656 1.47510529078
1.30509 1.48318945137
1.31362 1.49128250476
1.32215 1.49938436384
1.33068 1.50749494325
1.33921 1.51561415931
1.34774 1.52374193005
1.35627 1.53187817515
1.3648 1.54002281593
1.37333 1.54817577532
1.38186 1.55633697782
1.39039 1.56450634953
1.39892 1.57268381806
1.40745 1.58086931255
1.41598 1.58906276367
1.42451 1.59726410352
1.43304 1.60547326568
1.44157 1.61369018517
1.4501 1.62191479842
1.45863 1.63014704326
1.46716 1.6383868589
1.47569 1.6466341859
1.48422 1.65488896616
1.49275 1.66315114292
1.50128 1.6714206607
1.50981 1.67969746533
1.51834 1.68798150389
1.52687 1.69627272472
1.5354 1.70457107741
1.54393 1.71287651275
1.55246 1.72118898274
1.56099 1.72950844059
1.56952 1.73783484067
1.57805 1.7461681385
1.58658 1.75450829077
1.59511 1.76285525529
1.60364 1.77120899099
1.61217 1.7795694579
1.6207 1.78793661716
1.62923 1.79631043097
1.63776 1.80469086262
1.64629 1.81307787644
1.65482 1.82147143782
1.66335 1.82987151316
1.67188 1.8382780699
1.68041 1.8466910765
1.68894 1.8551105024
1.69747 1.86353631804
1.706 1.87196849484
1.71453 1.8804070052
1.72306 1.88885182248
1.73159 1.89730292098
1.74012 1.90576027596
1.74865 1.91422386361
1.75718 1.92269366105
1.76571 1.93116964632
1.77424 1.93965179837
1.78277 1.94814009707
1.7913 1.95663452316
1.79983 1.96513505829
1.80836 1.97364168499
1.81689 1.98215438668
1.82542 1.99067314764
1.83395 1.99919795301
1.84248 2.0077287888
1.85101 2.01626564189
1.85954 2.02480849998
1.86807 2.03335735163
1.8766 2.04191218625
1.88513 2.05047299408
1.89366 2.05903976618
1.90219 2.06761249446
1.91072 2.07619117163
1.91925 2.08477579125
1.92778 2.09336634767
1.93631 2.10196283608
1.94484 2.11056525246
1.95337 2.11917359361
1.9619 2.12778785715
1.97043 2.13640804149
1.97896 2.14503414585
1.98749 2.15366617024
1.99602 2.16230411548
2.00455 2.17094798321
2.01308 2.17959777583
2.02161 2.18825349656
2.03014 2.19691514942
2.03867 2.20558273923
2.0472 2.21425627159
2.05573 2.22293575291
2.06426 2.2316211904
2.07279 2.24031259206
2.08132 2.2490099667
2.08985 2.25771332392
2.09838 2.26642267414
2.10691 2.27513802857
2.11544 2.28385939922
2.12397 2.29258679892
2.1325 2.30132024132
2.14103 2.31005974086
2.14956 2.3188053128
2.15809 2.32755697324
2.16662 2.33631473909
2.17515 2.34507862806
2.18368 2.35384865874
2.19221 2.36262485052
2.20074 2.37140722363
2.20927 2.38019579915
2.2178 2.38899059901
2.22633 2.39779164598
2.23486 2.40659896371
2.24339 2.41541257669
2.25192 2.42423251029
2.26045 2.43305879077
2.26898 2.44189144523
2.27751 2.45073050172
2.28604 2.45957598913
2.29457 2.46842793729
2.3031 2.47728637692
2.31163 2.48615133967
2.32016 2.49502285812
2.32869 2.50390096578
2.33722 2.5127856971
2.34575 2.5216770875
2.35428 2.53057517334
2.36281 2.53947999197
2.37134 2.54839158173
2.37987 2.55730998194
2.3884 2.56623523293
2.39693 2.57516737605
2.40546 2.58410645368
2.41399 2.59305250922
2.42252 2.60200558716
2.43105 2.61096573301
2.43958 2.6199329934
2.44811 2.62890741604
2.45664 2.63788904973
2.46517 2.6468779444
2.4737 2.65587415113
2.48223 2.66487772214
2.49076 2.67388871081
2.49929 2.68290717171
2.50782 2.69193316062
2.51635 2.70096673452
2.52488 2.71000795164
2.53341 2.71905687146
2.54194 2.72811355472
2.55047 2.73717806346
2.559 2.74625046105
2.56753 2.75533081216
2.57606 2.76441918284
2.58459 2.7735156405
2.59312 2.78262025395
2.60165 2.79173309342
2.61018 2.8008542306
2.61871 2.80998373862
2.62724 2.81912169213
2.63577 2.82826816727
2.6443 2.83742324176
2.65283 2.84658699487
2.66136 2.85575950748
2.66989 2.86494086209
2.67842 2.87413114286
2.68695 2.88333043566
2.69548 2.89253882805
2.70401 2.90175640936
2.71254 2.91098327072
2.72107 2.92021950504
2.7296 2.92946520713
2.73813 2.93872047366
2.74666 2.94798540324
2.75519 2.95726009646
2.76372 2.96654465588
2.77225 2.97583918614
2.78078 2.98514379395
2.78931 2.99445858817
2.79784 3.00378367981
2.80637 3.01311918211
2.8149 3.02246521059
2.82343 3.03182188307
2.83196 3.04118931975
2.84049 3.05056764321
2.84902 3.05995697855
2.85755 3.06935745336
2.86608 3.0787691978
2.87461 3.08819234471
2.88314 3.09762702957
2.89167 3.10707339066
2.9002 3.11653156906
2.90873 3.12600170874
2.91726 3.13548395662
2.92579 3.14497846264
2.93432 3.15448537983
2.94285 3.16400486439
2.95138 3.17353707577
2.95991 3.18308217672
2.96844 3.1926403334
2.97697 3.20221171546
2.9855 3.21179649612
2.99403 3.22139485225
3.00256 3.23100696447
3.01109 3.24063301727
3.01962 3.25027319906
3.02815 3.2599277023
3.03668 3.26959672361
3.04521 3.27928046385
3.05374 3.28897912829
3.06227 3.29869292665
3.0708 3.30842207327
3.07933 3.31816678722
3.08786 3.32792729243
3.09639 3.33770381783
3.10492 3.34749659748
3.11345 3.3573058707
3.12198 3.36713188225
3.13051 3.37697488245
3.13904 3.38683512736
3.14757 3.39671287894
3.1561 3.4066084052
3.16463 3.41652198043
3.17316 3.42645388532
3.18169 3.4364044072
3.19022 3.44637384019
3.19875 3.45636248547
3.20728 3.46637065143
3.21581 3.47639865393
3.22434 3.48644681651
3.23287 3.49651547065
3.2414 3.506604956
3.24993 3.51671562065
3.25846 3.52684782139
3.26699 3.53700192401
3.27552 3.54717830358
3.28405 3.55737734473
3.29258 3.56759944201
3.30111 3.57784500021
3.30964 3.58811443468
3.31817 3.5984081717
3.3267 3.60872664889
3.33523 3.61907031553
3.34376 3.62943963305
3.35229 3.63983507539
3.36082 3.65025712949
3.36935 3.66070629572
3.37788 3.67118308841
3.38641 3.68168803632
3.39494 3.69222168319
3.40347 3.7027845883
3.412 3.71337732707
3.42053 3.72400049164
3.42906 3.73465469153
3.43759 3.74534055433
3.44612 3.75605872636
3.45465 3.76680987348
3.46318 3.77759468183
3.47171 3.78841385864
3.48024 3.79926813311
3.48877 3.81015825733
3.4973 3.82108500721
3.50583 3.83204918348
3.51436 3.8430516128
3.52289 3.85409314881
3.53142 3.86517467335
3.53995 3.87629709768
3.54848 3.88746136383
3.55701 3.89866844594
3.56554 3.90991935175
3.57407 3.92121512416
3.5826 3.93255684286
3.59113 3.94394562609
3.59966 3.95538263244
3.60819 3.96686906286
3.61672 3.97840616273
3.62525 3.98999522405
3.63378 4.00163758778
3.64231 4.01333464638
3.65084 4.02508784645
3.65937 4.03689869155
3.6679 4.04876874526
3.67643 4.06069963438
3.68496 4.07269305242
3.69349 4.08475076325
3.70202 4.0968746051
3.71055 4.10906649474
3.71908 4.12132843209
3.72761 4.13366250505
3.73614 4.14607089478
3.74467 4.15855588131
3.7532 4.17111984964
3.76173 4.18376529631
3.77026 4.19649483644
3.77879 4.20931121144
3.78732 4.22221729723
3.79585 4.23521611328
3.80438 4.24831083229
3.81291 4.26150479085
3.82144 4.27480150089
3.82997 4.28820466232
3.8385 4.30171817666
3.84703 4.3153461621
3.85556 4.32909296987
3.86409 4.34296320228
3.87262 4.35696173252
3.88115 4.37109372641
3.88968 4.38536466649
3.89821 4.3997803786
3.90674 4.41434706125
3.91527 4.4290713184
3.9238 4.44396019574
3.93233 4.45902122125
3.94086 4.4742624506
3.94939 4.48969251787
3.95792 4.50532069277
3.96645 4.52115694494
3.97498 4.53721201681
3.98351 4.5534975061
3.99204 4.57002595982
4.00057 4.5868109815
4.0091 4.60386735416
4.01763 4.62121118177
4.02616 4.63886005268
4.03469 4.6568332293
4.04322 4.6751518692
4.05175 4.69383928422
4.06028 4.71292124555
4.06881 4.73242634526
4.07734 4.75238642702
4.08587 4.77283710287
4.0944 4.79381837736
4.10293 4.81537540732
4.11146 4.83755943424
4.11999 4.86042893876
4.12852 4.88405108427
4.13705 4.90850354133
4.14558 4.93387682079
4.15411 4.96027729656
4.16264 4.9878311791
4.17117 5.01668982419
4.1797 5.0470369568
4.18823 5.07909870749
4.19676 5.1131578933
4.20529 5.1495749075
4.21382 5.18881928405
4.22235 5.23151926853
4.23088 5.27854339456
4.23941 5.33114273535
4.24794 5.39121795535
4.25647 5.46187206455


==> figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt05.tex <==
0.0 0.320291412272
0.008276 0.32445754832
0.016552 0.328679941716
0.024828 0.332958548254
0.033104 0.337293294386
0.04138 0.341684077413
0.049656 0.34613076576
0.057932 0.35063319931
0.066208 0.355191189826
0.074484 0.359804521428
0.08276 0.364472951148
0.091036 0.369196209541
0.099312 0.37397400136
0.107588 0.378806006282
0.115864 0.383691879692
0.12414 0.388631253511
0.132416 0.393623737066
0.140692 0.398668918
0.148968 0.40376636322
0.157244 0.408915619862
0.16552 0.414116216299
0.173796 0.419367663149
0.182072 0.424669454312
0.190348 0.430021068012
0.198624 0.435421967844
0.2069 0.440871603831
0.215176 0.446369413464
0.223452 0.451914822753
0.231728 0.457507247255
0.240004 0.463146093099
0.24828 0.468830757985
0.256556 0.474560632173
0.264832 0.480335099444
0.273108 0.486153538042
0.281384 0.492015321584
0.28966 0.497919819947
0.297936 0.503866400123
0.306212 0.509854427041
0.314488 0.515883264364
0.322764 0.521952275241
0.33104 0.528060823038
0.339316 0.534208272026
0.347592 0.540393988038
0.355868 0.54661733909
0.364144 0.55287769597
0.37242 0.559174432788
0.380696 0.565506927497
0.388972 0.571874562375
0.397248 0.578276724483
0.405524 0.58471280608
0.4138 0.591182205014
0.422076 0.597684325079
0.430352 0.604218576344
0.438628 0.610784375454
0.446904 0.6173811459
0.45518 0.624008318268
0.463456 0.630665330454
0.471732 0.637351627864
0.480008 0.644066663586
0.488284 0.650809898538
0.49656 0.6575808016
0.504836 0.66437884972
0.513112 0.671203528008
0.521388 0.678054329804
0.529664 0.684930756739
0.53794 0.691832318769
0.546216 0.698758534206
0.554492 0.705708929725
0.562768 0.712683040363
0.571044 0.719680409508
0.57932 0.726700588871
0.587596 0.733743138454
0.595872 0.740807626504
0.604148 0.747893629459
0.612424 0.755000731889
0.6207 0.762128526425
0.628976 0.769276613686
0.637252 0.776444602197
0.645528 0.783632108303
0.653804 0.790838756077
0.66208 0.798064177223
0.670356 0.805308010979
0.678632 0.812569904011
0.686908 0.819849510311
0.695184 0.827146491083
0.70346 0.834460514639
0.711736 0.841791256279
0.720012 0.849138398183
0.728288 0.856501629293
0.736564 0.8638806452
0.74484 0.87127514802
0.753116 0.878684846288
0.761392 0.88610945483
0.769668 0.893548694655
0.777944 0.901002292831
0.78622 0.908469982374
0.794496 0.915951502128
0.802772 0.923446596653
0.811048 0.93095501611
0.819324 0.938476516147
0.8276 0.946010857789
0.835876 0.953557807322
0.844152 0.961117136192
0.852428 0.968688620888
0.860704 0.976272042841
0.86898 0.983867188316
0.877256 0.991473848309
0.885532 0.999091818444
0.893808 1.00672089887
0.902084 1.01436089418
0.91036 1.02201161328
0.918636 1.02967286932
0.926912 1.03734447959
0.935188 1.04502626544
0.943464 1.05271805217
0.95174 1.06041966895
0.960016 1.06813094874
0.968292 1.0758517282
0.976568 1.0835818476
0.984844 1.09132115075
0.99312 1.09906948491
1.001396 1.1068267007
1.009672 1.11459265208
1.017948 1.12236719619
1.026224 1.13015019334
1.0345 1.13794150692
1.042776 1.14574100332
1.051052 1.15354855188
1.059328 1.1613640248
1.067604 1.16918729709
1.07588 1.17701824652
1.084156 1.18485675351
1.092432 1.19270270113
1.100708 1.20055597498
1.108984 1.20841646318
1.11726 1.2162840563
1.125536 1.22415864728
1.133812 1.23204013141
1.142088 1.23992840625
1.150364 1.2478233716
1.15864 1.25572492944
1.166916 1.26363298387
1.175192 1.27154744109
1.183468 1.27946820931
1.191744 1.28739519875
1.20002 1.29532832158
1.208296 1.30326749185
1.216572 1.3112126255
1.224848 1.31916364026
1.233124 1.32712045565
1.2414 1.33508299294
1.249676 1.34305117509
1.257952 1.35102492671
1.266228 1.35900417407
1.274504 1.36698884499
1.28278 1.37497886889
1.291056 1.38297417668
1.299332 1.39097470077
1.307608 1.39898037505
1.315884 1.40699113479
1.32416 1.4150069167
1.332436 1.42302765884
1.340712 1.4310533006
1.348988 1.43908378268
1.357264 1.44711904709
1.36554 1.45515903705
1.373816 1.46320369704
1.382092 1.47125297273
1.390368 1.47930681098
1.398644 1.48736515978
1.40692 1.49542796828
1.415196 1.50349518672
1.423472 1.51156676643
1.431748 1.51964265979
1.440024 1.52772282023
1.4483 1.53580720221
1.456576 1.54389576118
1.464852 1.55198845357
1.473128 1.56008523677
1.481404 1.56818606912
1.48968 1.57629090988
1.497956 1.58439971921
1.506232 1.59251245816
1.514508 1.60062908866
1.522784 1.60874957349
1.53106 1.61687387627
1.539336 1.62500196144
1.547612 1.63313379425
1.555888 1.64126934074
1.564164 1.64940856773
1.57244 1.65755144281
1.580716 1.66569793432
1.588992 1.67384801133
1.597268 1.68200164362
1.605544 1.69015880172
1.61382 1.69831945681
1.622096 1.70648358081
1.630372 1.71465114626
1.638648 1.7228221264
1.646924 1.73099649511
1.6552 1.73917422691
1.663476 1.74735529695
1.671752 1.755539681
1.680028 1.76372735544
1.688304 1.77191829725
1.69658 1.78011248399
1.704856 1.78830989382
1.713132 1.79651050545
1.721408 1.80471429817
1.729684 1.81292125182
1.73796 1.82113134677
1.746236 1.82934456395
1.754512 1.83756088481
1.762788 1.84578029131
1.771064 1.85400276595
1.77934 1.8622282917
1.787616 1.87045685206
1.795892 1.87868843101
1.804168 1.88692301302
1.812444 1.89516058304
1.82072 1.90340112648
1.828996 1.91164462924
1.837272 1.91989107765
1.845548 1.92814045852
1.853824 1.9363927591
1.8621 1.94464796708
1.870376 1.95290607059
1.878652 1.96116705819
1.886928 1.96943091887
1.895204 1.97769764205
1.90348 1.98596721756
1.911756 1.99423963565
1.920032 2.00251488695
1.928308 2.01079296254
1.936584 2.01907385387
1.94486 2.02735755278
1.953136 2.03564405154
1.961412 2.04393334276
1.969688 2.05222541948
1.977964 2.06052027508
1.98624 2.06881790334
1.994516 2.07711829842
2.002792 2.08542145484
2.011068 2.09372736748
2.019344 2.10203603161
2.02762 2.11034744284
2.035896 2.11866159714
2.044172 2.12697849085
2.052448 2.13529812066
2.060724 2.14362048361
2.069 2.15194557708
2.077276 2.16027339882
2.085552 2.1686039469
2.093828 2.17693721974
2.102104 2.18527321613
2.11038 2.19361193515
2.118656 2.20195337626
2.126932 2.21029753923
2.135208 2.21864442419
2.143484 2.22699403156
2.15176 2.23534636215
2.160036 2.24370141705
2.168312 2.25205919771
2.176588 2.26041970589
2.184864 2.26878294369
2.19314 2.27714891354
2.201416 2.28551761818
2.209692 2.29388906068
2.217968 2.30226324445
2.226244 2.31064017321
2.23452 2.31901985099
2.242796 2.32740228218
2.251072 2.33578747146
2.259348 2.34417542384
2.267624 2.35256614467
2.2759 2.36095963961
2.284176 2.36935591463
2.292452 2.37775497605
2.300728 2.38615683049
2.309004 2.3945614849
2.31728 2.40296894655
2.325556 2.41137922306
2.333832 2.41979232234
2.342108 2.42820825264
2.350384 2.43662702254
2.35866 2.44504864095
2.366936 2.45347311708
2.375212 2.46190046051
2.383488 2.47033068112
2.391764 2.47876378913
2.40004 2.4871997951
2.408316 2.49563870991
2.416592 2.50408054478
2.424868 2.51252531127
2.433144 2.52097302127
2.44142 2.52942368702
2.449696 2.53787732109
2.457972 2.5463339364
2.466248 2.55479354622
2.474524 2.56325616416
2.4828 2.57172180417
2.491076 2.58019048056
2.499352 2.588662208
2.507628 2.59713700151
2.515904 2.60561487646
2.52418 2.6140958486
2.532456 2.62257993401
2.540732 2.63106714918
2.549008 2.63955751093
2.557284 2.64805103647
2.56556 2.65654774338
2.573836 2.66504764962
2.582112 2.67355077353
2.590388 2.68205713383
2.598664 2.69056674963
2.60694 2.69907964044
2.615216 2.70759582615
2.623492 2.71611532704
2.631768 2.72463816383
2.640044 2.73316435761
2.64832 2.74169392988
2.656596 2.75022690258
2.664872 2.75876329805
2.673148 2.76730313905
2.681424 2.77584644877
2.6897 2.78439325084
2.697976 2.79294356931
2.706252 2.8014974287
2.714528 2.81005485393
2.722804 2.81861587041
2.73108 2.827180504
2.739356 2.835748781
2.747632 2.8443207282
2.755908 2.85289637285
2.764184 2.86147574268
2.77246 2.87005886591
2.780736 2.87864577125
2.789012 2.88723648789
2.797288 2.89583104554
2.805564 2.90442947441
2.81384 2.91303180523
2.822116 2.92163806925
2.830392 2.93024829826
2.838668 2.93886252457
2.846944 2.94748078103
2.85522 2.95610310106
2.863496 2.96472951863
2.871772 2.97336006827
2.880048 2.9819947851
2.888324 2.9906337048
2.8966 2.99927686367
2.904876 3.00792429857
2.913152 3.016576047
2.921428 3.02523214708
2.929704 3.03389263752
2.93798 3.0425575577
2.946256 3.05122694764
2.954532 3.05990084801
2.962808 3.06857930012
2.971084 3.077262346
2.97936 3.08595002834
2.987636 3.09464239053
2.995912 3.10333947666
3.004188 3.11204133156
3.012464 3.12074800076
3.02074 3.12945953055
3.029016 3.13817596798
3.037292 3.14689736086
3.045568 3.15562375776
3.053844 3.16435520807
3.06212 3.17309176197
3.070396 3.18183347046
3.078672 3.19058038537
3.086948 3.19933255939
3.095224 3.20809004606
3.1035 3.21685289979
3.111776 3.22562117588
3.120052 3.23439493056
3.128328 3.24317422097
3.136604 3.25195910517
3.14488 3.2607496422
3.153156 3.26954589206
3.161432 3.27834791576
3.169708 3.28715577529
3.177984 3.29596953368
3.18626 3.30478925501
3.194536 3.31361500442
3.202812 3.32244684815
3.211088 3.33128485351
3.219364 3.34012908897
3.22764 3.34897962413
3.235916 3.35783652977
3.244192 3.36669987786
3.252468 3.37556974157
3.260744 3.38444619534
3.26902 3.39332931483
3.277296 3.40221917702
3.285572 3.41111586019
3.293848 3.42001944398
3.302124 3.42893000935
3.3104 3.43784763871
3.318676 3.44677241585
3.326952 3.45570442602
3.335228 3.46464375596
3.343504 3.47359049392
3.35178 3.48254472968
3.360056 3.49150655461
3.368332 3.50047606168
3.376608 3.50945334549
3.384884 3.51843850235
3.39316 3.52743163023
3.401436 3.53643282891
3.409712 3.5454421999
3.417988 3.55445984658
3.426264 3.56348587416
3.43454 3.57252038979
3.442816 3.58156350255
3.451092 3.59061532351
3.459368 3.59967596578
3.467644 3.60874554456
3.47592 3.61782417718
3.484196 3.62691198313
3.492472 3.63600908416
3.500748 3.64511560428
3.509024 3.65423166984
3.5173 3.66335740957
3.525576 3.67249295465
3.533852 3.68163843877
3.542128 3.69079399818
3.550404 3.69995977174
3.55868 3.709135901
3.566956 3.71832253029
3.575232 3.72751980672
3.583508 3.73672788032
3.591784 3.74594690407
3.60006 3.75517703397
3.608336 3.76441842916
3.616612 3.77367125194
3.624888 3.78293566791
3.633164 3.79221184599
3.64144 3.80149995858
3.649716 3.81080018158
3.657992 3.82011269453
3.666268 3.82943768066
3.674544 3.83877532707
3.68282 3.84812582471
3.691096 3.85748936862
3.699372 3.86686615792
3.707648 3.87625639599
3.715924 3.8856602906
3.7242 3.89507805395
3.732476 3.9045099029
3.740752 3.913956059
3.749028 3.92341674868
3.757304 3.93289220341
3.76558 3.94238265976
3.773856 3.95188835964
3.782132 3.96140955038
3.790408 3.97094648496
3.798684 3.9804994221
3.80696 3.99006862649
3.815236 3.99965436894
3.823512 4.0092569266
3.831788 4.01887658308
3.840064 4.02851362872
3.84834 4.03816836077
3.856616 4.04784108361
3.864892 4.05753210897
3.873168 4.06724175614
3.881444 4.07697035226
3.88972 4.08671823254
3.897996 4.09648574053
3.906272 4.10627322839
3.914548 4.11608105716
3.922824 4.12590959709
3.9311 4.13575922791
3.939376 4.1456303392
3.947652 4.15552333066
3.955928 4.16543861251
3.964204 4.17537660584
3.97248 4.18533774298
3.980756 4.19532246793
3.989032 4.20533123673
3.997308 4.21536451791
4.005584 4.22542279298
4.01386 4.23550655686
4.022136 4.24561631838
4.030412 4.25575260082
4.038688 4.26591594246
4.046964 4.27610689712
4.05524 4.28632603479
4.063516 4.29657394224
4.071792 4.30685122366
4.080068 4.31715850141
4.088344 4.32749641668
4.09662 4.3378656303
4.104896 4.3482668235
4.113172 4.35870069881
4.121448 4.36916798087
4.129724 4.37966941745


==> figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt1.tex <==
0.0 0.459043605026
0.0841218682305 0.5032407464
0.168243736461 0.55165298416
0.252365604692 0.604115959843
0.336487472922 0.660378844751
0.420609341153 0.720132324207
0.504731209383 0.78303758718
0.588853077614 0.848751351875
0.672974945844 0.916944410345
0.757096814075 0.987313382263
0.841218682305 1.0595867203
0.925340550536 1.13352651328
1.00946241877 1.20892758045
1.093584287 1.28561504554
1.17770615523 1.36344122559
1.26182802346 1.44228236604
1.34594989169 1.52203552842
1.43007175992 1.60261578634
1.51419362815 1.68395379188
1.59831549638 1.76599372116
1.68243736461 1.84869158003
1.76655923284 1.93201383942
1.85068110107 2.01593636734
1.9348029693 2.10044362735
2.01892483753 2.18552811884
2.10304670576 2.27119004145
2.18716857399 2.35743717377
2.27129044222 2.44428496535
2.35541231046 2.53175685052
2.43953417869 2.61988480413
2.52365604692 2.70871017309
2.60777791515 2.79828483543
2.69189978338 2.88867276235
2.77602165161 2.97995209153
2.86014351984 3.07221786644
2.94426538807 3.16558566499
3.0283872563 3.26019644251
3.11250912453 3.35622307211
3.19663099276 3.45387931399
3.28075286099 3.55343235203
3.36487472922 3.65522072098
3.44899659745 3.75968064908
3.53311846568 3.86738604338
3.61724033391 3.97911159929
3.70136220214 4.09593726876
3.78548407037 4.21943176773
3.8696059386 4.35200039994
3.95372780684 4.49761463232
4.03784967507 4.66357732911
4.1219715433 4.86584665822


==> figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt3.tex <==
0.0 0.844600430901
0.0608288216233 0.875796868305
0.121657643247 0.908553958713
0.18248646487 0.942861602995
0.243315286493 0.978703301404
0.304144108116 1.01605663158
0.36497292974 1.05489387958
0.425801751363 1.09518279066
0.486630572986 1.13688740278
0.54745939461 1.17996892581
0.608288216233 1.22438663168
0.669117037856 1.27009872561
0.72994585948 1.31706317466
0.790774681103 1.36523847652
0.851603502726 1.41458435838
0.912432324349 1.46506240175
0.973261145973 1.51663659452
1.0340899676 1.56927381589
1.09491878922 1.62294426299
1.15574761084 1.67762183088
1.21657643247 1.73328445899
1.27740525409 1.78991445859
1.33823407571 1.84749883713
1.39906289734 1.90602963609
1.45989171896 1.9655043007
1.52072054058 2.02592610158
1.58154936221 2.08730463114
1.64237818383 2.14965640171
1.70320700545 2.21300557768
1.76403582708 2.27738488225
1.8248646487 2.3428367303
1.88569347032 2.4094146551
1.94652229195 2.47718511908
2.00735111357 2.54622983154
2.06817993519 2.61664874379
2.12900875682 2.68856396273
2.18983757844 2.76212493044
2.25066640006 2.83751538225
2.31149522169 2.91496285684
2.37232404331 2.9947519584
2.43315286493 3.07724328967
2.49398168656 3.16290123453
2.55481050818 3.25233607653
2.6156393298 3.34637039366
2.67646815143 3.44614882434
2.73729697305 3.55333061841
2.79812579467 3.67045406284
2.85895461629 3.80169963955
2.91978343792 3.95473315531
2.98061225954 4.14625281077


==> figuresAndData/dataForRayleigh-midPoint-sigma2prob0pt6.tex <==
0.0 1.35372872606
0.0396220919817 1.37390218105
0.0792441839634 1.39480051277
0.118866275945 1.4164239019
0.158488367927 1.43877266481
0.198110459909 1.46184727641
0.23773255189 1.48564840232
0.277354643872 1.51017694034
0.316976735854 1.5354340715
0.356598827835 1.56142132095
0.396220919817 1.58814062891
0.435843011799 1.61559443227
0.475465103781 1.64378575747
0.515087195762 1.67271832529
0.554709287744 1.70239666892
0.594331379726 1.73282626632
0.633953471707 1.76401368885
0.673575563689 1.79596676813
0.713197655671 1.82869478404
0.752819747653 1.86220867702
0.792441839634 1.89652128914
0.832063931616 1.93164763903
0.871686023598 1.96760523743
0.911308115579 2.00441445163
0.950930207561 2.04209892927
0.990552299543 2.08068609481
1.03017439152 2.12020773549
1.06979648351 2.16070069871
1.10941857549 2.20220772872
1.14904066747 2.24477847966
1.18866275945 2.2884707533
1.22828485143 2.3333520265
1.26790694341 2.37950135629
1.3075290354 2.42701178276
1.34715112738 2.47599339794
1.38677321936 2.52657731819
1.42639531134 2.57892090366
1.46601740332 2.63321473114
1.50563949531 2.68969208476
1.54526158729 2.74864215034
1.58488367927 2.8104288091
1.62450577125 2.8755181705
1.66412786323 2.94452026243
1.70374995521 3.0182546941
1.7433720472 3.09785914402
1.78299413918 3.1849795823
1.82261623116 3.28213017087
1.86223832314 3.39344677598
1.90186041512 3.52650657882
1.9414825071 3.69780434443


==> figuresAndData/dataForRayleigh-midPoint-sigma2pt01.tex <==
0.0 0.459043605026
0.0841218682305 0.5032407464
0.168243736461 0.55165298416
0.252365604692 0.604115959843
0.336487472922 0.660378844751
0.420609341153 0.720132324207
0.504731209383 0.78303758718
0.588853077614 0.848751351875
0.672974945844 0.916944410345
0.757096814075 0.987313382263
0.841218682305 1.0595867203
0.925340550536 1.13352651328
1.00946241877 1.20892758045
1.093584287 1.28561504554
1.17770615523 1.36344122559
1.26182802346 1.44228236604
1.34594989169 1.52203552842
1.43007175992 1.60261578634
1.51419362815 1.68395379188
1.59831549638 1.76599372116
1.68243736461 1.84869158003
1.76655923284 1.93201383942
1.85068110107 2.01593636734
1.9348029693 2.10044362735
2.01892483753 2.18552811884
2.10304670576 2.27119004145
2.18716857399 2.35743717377
2.27129044222 2.44428496535
2.35541231046 2.53175685052
2.43953417869 2.61988480413
2.52365604692 2.70871017309
2.60777791515 2.79828483543
2.69189978338 2.88867276235
2.77602165161 2.97995209153
2.86014351984 3.07221786644
2.94426538807 3.16558566499
3.0283872563 3.26019644251
3.11250912453 3.35622307211
3.19663099276 3.45387931399
3.28075286099 3.55343235203
3.36487472922 3.65522072098
3.44899659745 3.75968064908
3.53311846568 3.86738604338
3.61724033391 3.97911159929
3.70136220214 4.09593726876
3.78548407037 4.21943176773
3.8696059386 4.35200039994
3.95372780684 4.49761463232
4.03784967507 4.66357732911
4.1219715433 4.86584665822


==> figuresAndData/dataForRayleigh-midPoint-sigma4prob0pt3.tex <==
0.0 1.6892008618
0.121657643247 1.75159373661
0.243315286493 1.81710791743
0.36497292974 1.88572320599
0.486630572986 1.95740660281
0.608288216233 2.03211326315
0.72994585948 2.10978775916
0.851603502726 2.19036558132
0.973261145973 2.27377480557
1.09491878922 2.35993785162
1.21657643247 2.44877326335
1.33823407571 2.54019745122
1.45989171896 2.63412634932
1.58154936221 2.73047695304
1.70320700545 2.82916871675
1.8248646487 2.93012480349
1.94652229195 3.03327318905
2.06817993519 3.13854763178
2.18983757844 3.24588852597
2.31149522169 3.35524366176
2.43315286493 3.46656891798
2.55481050818 3.57982891718
2.67646815143 3.69499767426
2.79812579467 3.81205927218
2.91978343792 3.93100860141
3.04144108116 4.05185220316
3.16309872441 4.17460926228
3.28475636766 4.29931280341
3.4064140109 4.42601115536
3.52807165415 4.5547697645
3.6497292974 4.6856734606
3.77138694064 4.81882931021
3.89304458389 4.95437023817
4.01470222714 5.09245966308
4.13635987038 5.23329748758
4.25801751363 5.37712792546
4.37967515688 5.52424986088
4.50133280012 5.6750307645
4.62299044337 5.82992571367
4.74464808662 5.9895039168
4.86630572986 6.15448657934
4.98796337311 6.32580246906
5.10962101636 6.50467215307
5.2312786596 6.69274078732
5.35293630285 6.89229764867
5.4745939461 7.10666123681
5.59625158934 7.34090812567
5.71790923259 7.60339927909
5.83956687584 7.90946631063
5.96122451908 8.29250562155


==> figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt3.tex <==
0.0 3.3784017236
0.243315286493 3.50318747322
0.486630572986 3.63421583485
0.72994585948 3.77144641198
0.973261145973 3.91481320562
1.21657643247 4.0642265263
1.45989171896 4.21957551832
1.70320700545 4.38073116265
1.94652229195 4.54754961113
2.18983757844 4.71987570324
2.43315286493 4.89754652671
2.67646815143 5.08039490244
2.91978343792 5.26825269865
3.16309872441 5.46095390608
3.4064140109 5.65833743351
3.6497292974 5.86024960698
3.89304458389 6.0665463781
4.13635987038 6.27709526355
4.37967515688 6.49177705194
4.62299044337 6.71048732353
4.86630572986 6.93313783596
5.10962101636 7.15965783437
5.35293630285 7.38999534851
5.59625158934 7.62411854435
5.83956687584 7.86201720281
6.08288216233 8.10370440632
6.32619744882 8.34921852456
6.56951273532 8.59862560682
6.81282802181 8.85202231072
7.0561433083 9.109539529
7.2994585948 9.37134692121
7.54277388129 9.63765862042
7.78608916778 9.90874047634
8.02940445428 10.1849193262
8.27271974077 10.4665949752
8.51603502726 10.7542558509
8.75935031375 11.0484997218
9.00266560025 11.350061529
9.24598088674 11.6598514273
9.48929617323 11.9790078336
9.73261145973 12.3089731587
9.97592674622 12.6516049381
10.2192420327 13.0093443061
10.4625573192 13.3854815746
10.7058726057 13.7845952973
10.9491878922 14.2133224736
11.1925031787 14.6818162513
11.4358184652 15.2067985582
11.6791337517 15.8189326213
11.9224490382 16.5850112431


==> figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt6.tex <==
0.0 5.41491490422
0.158488367927 5.49560872421
0.316976735854 5.5792020511
0.475465103781 5.66569560762
0.633953471707 5.75509065924
0.792441839634 5.84738910565
0.950930207561 5.94259360928
1.10941857549 6.04070776134
1.26790694341 6.141736286
1.42639531134 6.2456852838
1.58488367927 6.35256251563
1.7433720472 6.4623777291
1.90186041512 6.57514302986
2.06034878305 6.69087330115
2.21883715098 6.80958667567
2.3773255189 6.93130506529
2.53581388683 7.05605475538
2.69430225476 7.18386707252
2.85279062268 7.31477913614
3.01127899061 7.44883470809
3.16976735854 7.58608515657
3.32825572646 7.72659055612
3.48674409439 7.87042094971
3.64523246232 8.01765780651
3.80372083024 8.1683957171
3.96220919817 8.32274437924
4.1206975661 8.48083094197
4.27918593403 8.64280279482
4.43767430195 8.80883091488
4.59616266988 8.97911391865
4.75465103781 9.15388301318
4.91313940573 9.33340810602
5.07162777366 9.51800542516
5.23011614159 9.70804713105
5.38860450951 9.90397359176
5.54709287744 10.1063092728
5.70558124537 10.3156836147
5.86406961329 10.5328589246
6.02255798122 10.758768339
6.18104634915 10.9945686014
6.33953471707 11.2417152364
6.498023085 11.502072682
6.65651145293 11.7780810497
6.81499982086 12.0730187764
6.97348818878 12.3914365761
7.13197655671 12.7399183292
7.29046492464 13.1285206835
7.44895329256 13.5737871039
7.60744166049 14.1060263153
7.76593002842 14.7912173777


==> figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt7.tex <==
0.0 6.20702261462
0.132433347565 6.27441670023
0.26486669513 6.34416653012
0.397300042696 6.41627487851
0.529733390261 6.49074641043
0.662166737826 6.56758774411
0.794600085391 6.64680753949
0.927033432956 6.72841661375
1.05946678052 6.81242808543
1.19190012809 6.89885754889
1.32433347565 6.98772328155
1.45676682322 7.07904648675
1.58920017078 7.17285157575
1.72163351835 7.26916649329
1.85406686591 7.36802309189
1.98650021348 7.46945756134
2.11893356104 7.57351092122
2.25136690861 7.68022958575
2.38380025617 7.78966601274
2.51623360374 7.90187945062
2.6486669513 8.01693680094
2.78110029887 8.13491361774
2.91353364643 8.25589527027
3.045966994 8.37997830215
3.17840034157 8.50727202824
3.31083368913 8.63790042156
3.4432670367 8.77200435681
3.57570038426 8.90974429553
3.70813373183 9.05130352339
3.84056707939 9.19689208359
3.97300042696 9.34675159675
4.10543377452 9.50116122153
4.23786712209 9.6604451001
4.37030046965 9.82498176054
4.50273381722 9.99521613404
4.63516716478 10.1716751194
4.76760051235 10.3549880411
4.90003385991 10.5459139873
5.03246720748 10.7453790262
5.16490055504 10.9545279528
5.29733390261 11.1747980055
5.42976725017 11.408026873
5.56220059774 11.6566162605
5.6946339453 11.9237895492
5.82706729287 12.2140175782
5.95950064043 12.5337653717
6.091933988 12.8929053239
6.22436733556 13.3076769061
6.35680068313 13.8078368023
6.4892340307 14.4581893519


==> figuresAndData/dataForRayleigh-midPoint-sigma8prob0pt8.tex <==
0.0 7.17649031198
0.104749805795 7.22982091121
0.20949961159 7.28506410738
0.314249417386 7.34222352366
0.418999223181 7.40130523353
0.523749028976 7.46231781353
0.628498834771 7.52527241828
0.733248640566 7.59018287889
0.837998446361 7.6570658262
0.942748252157 7.72594084094
1.04749805795 7.79683063308
1.15224786375 7.86976125357
1.25699766954 7.94476234184
1.36174747534 8.02186741382
1.46649728113 8.10111419545
1.57124708693 8.18254500831
1.67599689272 8.26620721522
1.78074669852 8.3521537349
1.88549650431 8.44044363742
1.99024631011 8.53114283418
2.0949961159 8.62432487933
2.1997459217 8.72007190376
2.30449572749 8.81847570725
2.40924553329 8.91963904095
2.51399533908 9.02367712055
2.61874514488 9.13071942058
2.72349495067 9.24091181447
2.82824475647 9.35441914283
2.93299456226 9.47142831679
3.03774436806 9.59215209587
3.14249417386 9.71683372475
3.24724397965 9.84575267483
3.35199378545 9.97923182392
3.45674359124 10.117646531
3.56149339704 10.2614362433
3.66624320283 10.411119538
3.77099300863 10.5673139043
3.87574281442 10.7307621881
3.98049262022 10.9023686074
4.08524242601 11.0832488462
4.18999223181 11.2748014405
4.2947420376 11.4788124068
4.3994918434 11.6976137473
4.50424164919 11.9343332306
4.60899145499 12.1933073222
4.71374126078 12.480805707
4.81849106658 12.8064031607
4.92324087237 13.1858544743
5.02799067817 13.6480448071
5.13274048396 14.2559377466


==> figuresAndData/dataForRayleigh-midPoint.tex <==
0.0 0.459043605026
0.00853 0.463330619152
0.01706 0.467661655327
0.02559 0.472036694963
0.03412 0.476455707107
0.04265 0.480918648484
0.05118 0.485425463566
0.05971 0.489976084645
0.06824 0.494570431933
0.07677 0.499208413674
0.0853 0.503889926274
0.09383 0.508614854449
0.10236 0.513383071382
0.11089 0.518194438903
0.11942 0.523048807679
0.12795 0.527946017418
0.13648 0.532885897088
0.14501 0.537868265146
0.15354 0.542892929783
0.16207 0.547959689173
0.1706 0.553068331743
0.17913 0.55821863644
0.18766 0.563410373019
0.19619 0.568643302329
0.20472 0.573917176614
0.21325 0.579231739813
0.22178 0.584586727875
0.23031 0.58998186907
0.23884 0.595416884306
0.24737 0.600891487458
0.2559 0.606405385684
0.26443 0.611958279756
0.27296 0.617549864385
0.28149 0.623179828554
0.29002 0.628847855835
0.29855 0.634553624726
0.30708 0.640296808968
0.31561 0.64607707787
0.32414 0.65189409663
0.33267 0.657747526646
0.3412 0.663637025834
0.34973 0.669562248931
0.35826 0.675522847802
0.36679 0.681518471732
0.37532 0.687548767724
0.38385 0.693613380779
0.39238 0.699711954181
0.40091 0.705844129765
0.40944 0.712009548187
0.41797 0.718207849178
0.4265 0.724438671802
0.43503 0.730701654695
0.44356 0.736996436301
0.45209 0.743322655105
0.46062 0.74967994985
0.46915 0.756067959751
0.47768 0.762486324701
0.48621 0.768934685467
0.49474 0.775412683879
0.50327 0.781919963009
0.5118 0.78845616735
0.52033 0.795020942976
0.52886 0.801613937701
0.53739 0.808234801231
0.54592 0.814883185304
0.55445 0.821558743824
0.56298 0.828261132995
0.57151 0.834990011431
0.58004 0.841745040281
0.58857 0.848525883327
0.5971 0.855332207087
0.60563 0.862163680908
0.61416 0.869019977053
0.62269 0.875900770784
0.63122 0.882805740431
0.63975 0.889734567467
0.64828 0.896686936569
0.65681 0.903662535672
0.66534 0.91066105603
0.67387 0.917682192256
0.6824 0.924725642366
0.69093 0.931791107821
0.69946 0.938878293556
0.70799 0.94598690801
0.71652 0.953116663153
0.72505 0.960267274504
0.73358 0.967438461151
0.74211 0.97462994576
0.75064 0.981841454591
0.75917 0.989072717501
0.7677 0.996323467948
0.77623 1.00359344299
0.78476 1.0108823833
0.79329 1.01819003311
0.80182 1.02551614029
0.81035 1.03286045624
0.81888 1.04022273596
0.82741 1.04760273799
0.83594 1.0550002244
0.84447 1.06241496079
0.853 1.06984671626
0.86153 1.07729526336
0.87006 1.08476037813
0.87859 1.09224184002
0.88712 1.0997394319
0.89565 1.10725293999
0.90418 1.1147821539
0.91271 1.12232686654
0.92124 1.1298868741
0.92977 1.13746197605
0.9383 1.14505197509
0.94683 1.1526566771
0.95536 1.16027589116
0.96389 1.16790942945
0.97242 1.17555710726
0.98095 1.18321874294
0.98948 1.19089415787
0.99801 1.19858317644
1.00654 1.20628562599
1.01507 1.21400133677
1.0236 1.22173014194
1.03213 1.2294718775
1.04066 1.23722638228
1.04919 1.24499349788
1.05772 1.25277306866
1.06625 1.26056494168
1.07478 1.26836896667
1.08331 1.27618499601
1.09184 1.28401288468
1.10037 1.29185249024
1.1089 1.29970367276
1.11743 1.30756629483
1.12596 1.3154402215
1.13449 1.32332532024
1.14302 1.33122146092
1.15155 1.33912851579
1.16008 1.34704635939
1.16861 1.3549748686
1.17714 1.36291392252
1.18567 1.37086340251
1.1942 1.37882319212
1.20273 1.38679317704
1.21126 1.39477324514
1.21979 1.40276328636
1.22832 1.41076319271
1.23685 1.41877285826
1.24538 1.42679217907
1.25391 1.43482105322
1.26244 1.44285938069
1.27097 1.45090706343
1.2795 1.45896400525
1.28803 1.46703011186
1.29656 1.47510529078
1.30509 1.48318945137
1.31362 1.49128250476
1.32215 1.49938436384
1.33068 1.50749494325
1.33921 1.51561415931
1.34774 1.52374193005
1.35627 1.53187817515
1.3648 1.54002281593
1.37333 1.54817577532
1.38186 1.55633697782
1.39039 1.56450634953
1.39892 1.57268381806
1.40745 1.58086931255
1.41598 1.58906276367
1.42451 1.59726410352
1.43304 1.60547326568
1.44157 1.61369018517
1.4501 1.62191479842
1.45863 1.63014704326
1.46716 1.6383868589
1.47569 1.6466341859
1.48422 1.65488896616
1.49275 1.66315114292
1.50128 1.6714206607
1.50981 1.67969746533
1.51834 1.68798150389
1.52687 1.69627272472
1.5354 1.70457107741
1.54393 1.71287651275
1.55246 1.72118898274
1.56099 1.72950844059
1.56952 1.73783484067
1.57805 1.7461681385
1.58658 1.75450829077
1.59511 1.76285525529
1.60364 1.77120899099
1.61217 1.7795694579
1.6207 1.78793661716
1.62923 1.79631043097
1.63776 1.80469086262
1.64629 1.81307787644
1.65482 1.82147143782
1.66335 1.82987151316
1.67188 1.8382780699
1.68041 1.8466910765
1.68894 1.8551105024
1.69747 1.86353631804
1.706 1.87196849484
1.71453 1.8804070052
1.72306 1.88885182248
1.73159 1.89730292098
1.74012 1.90576027596
1.74865 1.91422386361
1.75718 1.92269366105
1.76571 1.93116964632
1.77424 1.93965179837
1.78277 1.94814009707
1.7913 1.95663452316
1.79983 1.96513505829
1.80836 1.97364168499
1.81689 1.98215438668
1.82542 1.99067314764
1.83395 1.99919795301
1.84248 2.0077287888
1.85101 2.01626564189
1.85954 2.02480849998
1.86807 2.03335735163
1.8766 2.04191218625
1.88513 2.05047299408
1.89366 2.05903976618
1.90219 2.06761249446
1.91072 2.07619117163
1.91925 2.08477579125
1.92778 2.09336634767
1.93631 2.10196283608
1.94484 2.11056525246
1.95337 2.11917359361
1.9619 2.12778785715
1.97043 2.13640804149
1.97896 2.14503414585
1.98749 2.15366617024
1.99602 2.16230411548
2.00455 2.17094798321
2.01308 2.17959777583
2.02161 2.18825349656
2.03014 2.19691514942
2.03867 2.20558273923
2.0472 2.21425627159
2.05573 2.22293575291
2.06426 2.2316211904
2.07279 2.24031259206
2.08132 2.2490099667
2.08985 2.25771332392
2.09838 2.26642267414
2.10691 2.27513802857
2.11544 2.28385939922
2.12397 2.29258679892
2.1325 2.30132024132
2.14103 2.31005974086
2.14956 2.3188053128
2.15809 2.32755697324
2.16662 2.33631473909
2.17515 2.34507862806
2.18368 2.35384865874
2.19221 2.36262485052
2.20074 2.37140722363
2.20927 2.38019579915
2.2178 2.38899059901
2.22633 2.39779164598
2.23486 2.40659896371
2.24339 2.41541257669
2.25192 2.42423251029
2.26045 2.43305879077
2.26898 2.44189144523
2.27751 2.45073050172
2.28604 2.45957598913
2.29457 2.46842793729
2.3031 2.47728637692
2.31163 2.48615133967
2.32016 2.49502285812
2.32869 2.50390096578
2.33722 2.5127856971
2.34575 2.5216770875
2.35428 2.53057517334
2.36281 2.53947999197
2.37134 2.54839158173
2.37987 2.55730998194
2.3884 2.56623523293
2.39693 2.57516737605
2.40546 2.58410645368
2.41399 2.59305250922
2.42252 2.60200558716
2.43105 2.61096573301
2.43958 2.6199329934
2.44811 2.62890741604
2.45664 2.63788904973
2.46517 2.6468779444
2.4737 2.65587415113
2.48223 2.66487772214
2.49076 2.67388871081
2.49929 2.68290717171
2.50782 2.69193316062
2.51635 2.70096673452
2.52488 2.71000795164
2.53341 2.71905687146
2.54194 2.72811355472
2.55047 2.73717806346
2.559 2.74625046105
2.56753 2.75533081216
2.57606 2.76441918284
2.58459 2.7735156405
2.59312 2.78262025395
2.60165 2.79173309342
2.61018 2.8008542306
2.61871 2.80998373862
2.62724 2.81912169213
2.63577 2.82826816727
2.6443 2.83742324176
2.65283 2.84658699487
2.66136 2.85575950748
2.66989 2.86494086209
2.67842 2.87413114286
2.68695 2.88333043566
2.69548 2.89253882805
2.70401 2.90175640936
2.71254 2.91098327072
2.72107 2.92021950504
2.7296 2.92946520713
2.73813 2.93872047366
2.74666 2.94798540324
2.75519 2.95726009646
2.76372 2.96654465588
2.77225 2.97583918614
2.78078 2.98514379395
2.78931 2.99445858817
2.79784 3.00378367981
2.80637 3.01311918211
2.8149 3.02246521059
2.82343 3.03182188307
2.83196 3.04118931975
2.84049 3.05056764321
2.84902 3.05995697855
2.85755 3.06935745336
2.86608 3.0787691978
2.87461 3.08819234471
2.88314 3.09762702957
2.89167 3.10707339066
2.9002 3.11653156906
2.90873 3.12600170874
2.91726 3.13548395662
2.92579 3.14497846264
2.93432 3.15448537983
2.94285 3.16400486439
2.95138 3.17353707577
2.95991 3.18308217672
2.96844 3.1926403334
2.97697 3.20221171546
2.9855 3.21179649612
2.99403 3.22139485225
3.00256 3.23100696447
3.01109 3.24063301727
3.01962 3.25027319906
3.02815 3.2599277023
3.03668 3.26959672361
3.04521 3.27928046385
3.05374 3.28897912829
3.06227 3.29869292665
3.0708 3.30842207327
3.07933 3.31816678722
3.08786 3.32792729243
3.09639 3.33770381783
3.10492 3.34749659748
3.11345 3.3573058707
3.12198 3.36713188225
3.13051 3.37697488245
3.13904 3.38683512736
3.14757 3.39671287894
3.1561 3.4066084052
3.16463 3.41652198043
3.17316 3.42645388532
3.18169 3.4364044072
3.19022 3.44637384019
3.19875 3.45636248547
3.20728 3.46637065143
3.21581 3.47639865393
3.22434 3.48644681651
3.23287 3.49651547065
3.2414 3.506604956
3.24993 3.51671562065
3.25846 3.52684782139
3.26699 3.53700192401
3.27552 3.54717830358
3.28405 3.55737734473
3.29258 3.56759944201
3.30111 3.57784500021
3.30964 3.58811443468
3.31817 3.5984081717
3.3267 3.60872664889
3.33523 3.61907031553
3.34376 3.62943963305
3.35229 3.63983507539
3.36082 3.65025712949
3.36935 3.66070629572
3.37788 3.67118308841
3.38641 3.68168803632
3.39494 3.69222168319
3.40347 3.7027845883
3.412 3.71337732707
3.42053 3.72400049164
3.42906 3.73465469153
3.43759 3.74534055433
3.44612 3.75605872636
3.45465 3.76680987348
3.46318 3.77759468183
3.47171 3.78841385864
3.48024 3.79926813311
3.48877 3.81015825733
3.4973 3.82108500721
3.50583 3.83204918348
3.51436 3.8430516128
3.52289 3.85409314881
3.53142 3.86517467335
3.53995 3.87629709768
3.54848 3.88746136383
3.55701 3.89866844594
3.56554 3.90991935175
3.57407 3.92121512416
3.5826 3.93255684286
3.59113 3.94394562609
3.59966 3.95538263244
3.60819 3.96686906286
3.61672 3.97840616273
3.62525 3.98999522405
3.63378 4.00163758778
3.64231 4.01333464638
3.65084 4.02508784645
3.65937 4.03689869155
3.6679 4.04876874526
3.67643 4.06069963438
3.68496 4.07269305242
3.69349 4.08475076325
3.70202 4.0968746051
3.71055 4.10906649474
3.71908 4.12132843209
3.72761 4.13366250505
3.73614 4.14607089478
3.74467 4.15855588131
3.7532 4.17111984964
3.76173 4.18376529631
3.77026 4.19649483644
3.77879 4.20931121144
3.78732 4.22221729723
3.79585 4.23521611328
3.80438 4.24831083229
3.81291 4.26150479085
3.82144 4.27480150089
3.82997 4.28820466232
3.8385 4.30171817666
3.84703 4.3153461621
3.85556 4.32909296987
3.86409 4.34296320228
3.87262 4.35696173252
3.88115 4.37109372641
3.88968 4.38536466649
3.89821 4.3997803786
3.90674 4.41434706125
3.91527 4.4290713184
3.9238 4.44396019574
3.93233 4.45902122125
3.94086 4.4742624506
3.94939 4.48969251787
3.95792 4.50532069277
3.96645 4.52115694494
3.97498 4.53721201681
3.98351 4.5534975061
3.99204 4.57002595982
4.00057 4.5868109815
4.0091 4.60386735416
4.01763 4.62121118177
4.02616 4.63886005268
4.03469 4.6568332293
4.04322 4.6751518692
4.05175 4.69383928422
4.06028 4.71292124555
4.06881 4.73242634526
4.07734 4.75238642702
4.08587 4.77283710287
4.0944 4.79381837736
4.10293 4.81537540732
4.11146 4.83755943424
4.11999 4.86042893876
4.12852 4.88405108427
4.13705 4.90850354133
4.14558 4.93387682079
4.15411 4.96027729656
4.16264 4.9878311791
4.17117 5.01668982419
4.1797 5.0470369568
4.18823 5.07909870749
4.19676 5.1131578933
4.20529 5.1495749075
4.21382 5.18881928405
4.22235 5.23151926853
4.23088 5.27854339456
4.23941 5.33114273535
4.24794 5.39121795535
4.25647 5.46187206455


==> figuresAndData/dataForRayleigh-rightEnd-sigma2prob0pt1.tex <==
0.0 0.918087210053
0.0841218682305 0.922359624569
0.168243736461 0.935062231858
0.252365604692 0.955866314995
0.336487472922 0.98427021658
0.420609341153 1.01965530726
0.504731209383 1.06134396498
0.588853077614 1.10864962614
0.672974945844 1.16091387485
0.757096814075 1.21752995045
0.841218682305 1.2779547583
0.925340550536 1.34171247602
1.00946241877 1.40839274214
1.093584287 1.47764580409
1.17770615523 1.54917629596
1.26182802346 1.62273670863
1.34594989169 1.69812116516
1.43007175992 1.77515981275
1.51419362815 1.8537139556
1.59831549638 1.93367194593
1.68243736461 2.01494579545
1.76655923284 2.097468446
1.85068110107 2.18119163361
1.9348029693 2.26608428539
2.01892483753 2.35213140015
2.10304670576 2.43933337714
2.18716857399 2.52770577355
2.27129044222 2.61727948848
2.35541231046 2.70810139059
2.43953417869 2.80023542958
2.52365604692 2.89376429926
2.60777791515 2.98879175571
2.69189978338 3.08544574133
2.77602165161 3.18388253145
2.86014351984 3.28429221304
2.94426538807 3.3869059419
3.0283872563 3.49200562872
3.11250912453 3.59993701969
3.19663099276 3.71112763521
3.28075286099 3.82611184307
3.36487472922 3.94556671273
3.44899659745 4.07036470071
3.53311846568 4.20165362107
3.61724033391 4.34098286467
3.70136220214 4.49051233537
3.78548407037 4.65337946509
3.8696059386 4.83439486127
3.95372780684 5.04150145781
4.03784967507 5.28930498316
4.1219715433 5.60972177315


==> figuresAndData/dataForRayleigh-rightEnd-sigma2prob0pt3.tex <==
0.0 1.6892008618
0.0608288216233 1.69076491499
0.121657643247 1.69545027418
0.18248646487 1.70323674112
0.243315286493 1.71409131631
0.304144108116 1.72796915503
0.36497292974 1.74481482942
0.425801751363 1.76456382996
0.486630572986 1.78714423258
0.54745939461 1.81247845701
0.608288216233 1.84048504712
0.669117037856 1.87108041337
0.72994585948 1.90418048984
0.790774681103 1.93970227194
0.851603502726 1.97756521403
0.912432324349 2.01769247914
0.973261145973 2.06001204308
1.0340899676 2.10445766418
1.09491878922 2.15096973675
1.15574761084 2.19949605092
1.21657643247 2.24999248551
1.27740525409 2.3024236631
1.33823407571 2.35676359854
1.39906289734 2.41299637484
1.45989171896 2.47111688245
1.52072054058 2.53113166258
1.58154936221 2.59305990008
1.64237818383 2.65693461958
1.70320700545 2.72280414991
1.76403582708 2.79073393743
1.8248646487 2.86080881191
1.88569347032 2.93313583989
1.94652229195 3.00784794622
2.00735111357 3.08510854951
2.06817993519 3.16511755239
2.12900875682 3.24811916864
2.18983757844 3.33441228245
2.25066640006 3.42436436443
2.31149522169 3.51843049199
2.37232404331 3.61717987349
2.43315286493 3.72133371441
2.49398168656 3.83182078251
2.55481050818 3.94986164489
2.6156393298 4.07710145752
2.67646815143 4.21582949725
2.73729697305 4.36936426376
2.79812579467 4.542782331
2.85895461629 4.7444446628
2.91978343792 4.98968287271
2.98061225954 5.311893362


==> figuresAndData/dataForRayleigh-rightEnd-sigma2prob0pt6.tex <==
0.0 2.70745745211
0.0396220919817 2.70818227013
0.0792441839634 2.71035684158
0.118866275945 2.71398152786
0.158488367927 2.71905696169
0.198110459909 2.72558409292
0.23773255189 2.73356425275
0.277354643872 2.7429992368
0.316976735854 2.75389140715
0.356598827835 2.76624381407
0.396220919817 2.780060338
0.435843011799 2.79534585275
0.475465103781 2.81210641115
0.515087195762 2.83034945482
0.554709287744 2.85008405009
0.594331379726 2.87132115292
0.633953471707 2.89407390598
0.673575563689 2.91835797257
0.713197655671 2.9441919124
0.752819747653 2.97159760639
0.792441839634 3.00060073865
0.832063931616 3.03123134644
0.871686023598 3.06352445126
0.911308115579 3.09752078768
0.950930207561 3.13326765099
0.990552299543 3.17081989008
1.03017439152 3.21024107946
1.06979648351 3.2516049139
1.10941857549 3.29499688195
1.14904066747 3.34051629185
1.18866275945 3.38827874714
1.22828485143 3.43841920158
1.26790694341 3.49109576917
1.3075290354 3.54649453013
1.34715112738 3.6048356685
1.38677321936 3.66638141702
1.42639531134 3.73144649599
1.46601740332 3.80041205896
1.50563949531 3.87374467422
1.54526158729 3.95202271339
1.58488367927 4.03597393892
1.62450577125 4.12653056974
1.66412786323 4.22491266162
1.70374995521 4.33275943298
1.7433720472 4.45234624085
1.78299413918 4.58696502543
1.82261623116 4.74164411059
1.86223832314 4.92465522882
1.90186041512 5.15115274251
1.9414825071 5.45412618175


==> figuresAndData/dataForRayleigh-rightEnd-sigma2pt01.tex <==
0.0 0.918087210053
0.0841218682305 0.922359624569
0.168243736461 0.935062231858
0.252365604692 0.955866314995
0.336487472922 0.98427021658
0.420609341153 1.01965530726
0.504731209383 1.06134396498
0.588853077614 1.10864962614
0.672974945844 1.16091387485
0.757096814075 1.21752995045
0.841218682305 1.2779547583
0.925340550536 1.34171247602
1.00946241877 1.40839274214
1.093584287 1.47764580409
1.17770615523 1.54917629596
1.26182802346 1.62273670863
1.34594989169 1.69812116516
1.43007175992 1.77515981275
1.51419362815 1.8537139556
1.59831549638 1.93367194593
1.68243736461 2.01494579545
1.76655923284 2.097468446
1.85068110107 2.18119163361
1.9348029693 2.26608428539
2.01892483753 2.35213140015
2.10304670576 2.43933337714
2.18716857399 2.52770577355
2.27129044222 2.61727948848
2.35541231046 2.70810139059
2.43953417869 2.80023542958
2.52365604692 2.89376429926
2.60777791515 2.98879175571
2.69189978338 3.08544574133
2.77602165161 3.18388253145
2.86014351984 3.28429221304
2.94426538807 3.3869059419
3.0283872563 3.49200562872
3.11250912453 3.59993701969
3.19663099276 3.71112763521
3.28075286099 3.82611184307
3.36487472922 3.94556671273
3.44899659745 4.07036470071
3.53311846568 4.20165362107
3.61724033391 4.34098286467
3.70136220214 4.49051233537
3.78548407037 4.65337946509
3.8696059386 4.83439486127
3.95372780684 5.04150145781
4.03784967507 5.28930498316
4.1219715433 5.60972177315


==> figuresAndData/dataForRayleigh-rightEnd-sigma4prob0pt3.tex <==
0.0 3.3784017236
0.121657643247 3.38152982998
0.243315286493 3.39090054836
0.36497292974 3.40647348224
0.486630572986 3.42818263263
0.608288216233 3.45593831007
0.72994585948 3.48962965884
0.851603502726 3.52912765992
0.973261145973 3.57428846516
1.09491878922 3.62495691402
1.21657643247 3.68097009424
1.33823407571 3.74216082673
1.45989171896 3.80836097969
1.58154936221 3.87940454387
1.70320700545 3.95513042805
1.8248646487 4.03538495828
1.94652229195 4.12002408615
2.06817993519 4.20891532836
2.18983757844 4.3019394735
2.31149522169 4.39899210184
2.43315286493 4.49998497103
2.55481050818 4.60484732619
2.67646815143 4.71352719709
2.79812579467 4.82599274968
2.91978343792 4.94223376489
3.04144108116 5.06226332516
3.16309872441 5.18611980015
3.28475636766 5.31386923917
3.4064140109 5.44560829981
3.52807165415 5.58146787485
3.6497292974 5.72161762381
3.77138694064 5.86627167978
3.89304458389 6.01569589245
4.01470222714 6.17021709903
4.13635987038 6.33023510478
4.25801751363 6.49623833729
4.37967515688 6.66882456489
4.50133280012 6.84872872887
4.62299044337 7.03686098397
4.74464808662 7.23435974698
4.86630572986 7.44266742881
4.98796337311 7.66364156502
5.10962101636 7.89972328978
5.2312786596 8.15420291504
5.35293630285 8.43165899449
5.4745939461 8.73872852753
5.59625158934 9.085564662
5.71790923259 9.48888932559
5.83956687584 9.97936574542
5.96122451908 10.623786724


==> figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt3.tex <==
0.0 6.7568034472
0.243315286493 6.76305965995
0.486630572986 6.78180109672
0.72994585948 6.81294696448
0.973261145973 6.85636526526
1.21657643247 6.91187662014
1.45989171896 6.97925931769
1.70320700545 7.05825531985
1.94652229195 7.14857693032
2.18983757844 7.24991382805
2.43315286493 7.36194018848
2.67646815143 7.48432165346
2.91978343792 7.61672195937
3.16309872441 7.75880908775
3.4064140109 7.91026085611
3.6497292974 8.07076991657
3.89304458389 8.2400481723
4.13635987038 8.41783065672
4.37967515688 8.60387894701
4.62299044337 8.79798420368
4.86630572986 8.99996994206
5.10962101636 9.20969465238
5.35293630285 9.42705439418
5.59625158934 9.65198549936
5.83956687584 9.88446752979
6.08288216233 10.1245266503
6.32619744882 10.3722396003
6.56951273532 10.6277384783
6.81282802181 10.8912165996
7.0561433083 11.1629357497
7.2994585948 11.4432352476
7.54277388129 11.7325433596
7.78608916778 12.0313917849
8.02940445428 12.3404341981
8.27271974077 12.6604702096
8.51603502726 12.9924766746
8.75935031375 13.3376491298
9.00266560025 13.6974574577
9.24598088674 14.0737219679
9.48929617323 14.468719494
9.73261145973 14.8853348576
9.97592674622 15.32728313
10.2192420327 15.7994465796
10.4625573192 16.3084058301
10.7058726057 16.863317989
10.9491878922 17.4774570551
11.1925031787 18.171129324
11.4358184652 18.9777786512
11.6791337517 19.9587314908
11.9224490382 21.247573448


==> figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt6.tex <==
0.0 10.8298298084
0.158488367927 10.8327290805
0.316976735854 10.8414273663
0.475465103781 10.8559261115
0.633953471707 10.8762278468
0.792441839634 10.9023363717
0.950930207561 10.934257011
1.10941857549 10.9719969472
1.26790694341 11.0155656286
1.42639531134 11.0649752563
1.58488367927 11.120241352
1.7433720472 11.181383411
1.90186041512 11.2484256446
2.06034878305 11.3213978193
2.21883715098 11.4003362004
2.3773255189 11.4852846117
2.53581388683 11.5762956239
2.69430225476 11.6734318903
2.85279062268 11.7767676496
3.01127899061 11.8863904256
3.16976735854 12.0024029546
3.32825572646 12.1249253858
3.48674409439 12.254097805
3.64523246232 12.3900831507
3.80372083024 12.5330706039
3.96220919817 12.6832795603
4.1206975661 12.8409643178
4.27918593403 13.0064196556
4.43767430195 13.1799875278
4.59616266988 13.3620651674
4.75465103781 13.5531149886
4.91313940573 13.7536768063
5.07162777366 13.9643830767
5.23011614159 14.1859781205
5.38860450951 14.419342674
5.54709287744 14.6655256681
5.70558124537 14.9257859839
5.86406961329 15.2016482359
6.02255798122 15.4949786969
6.18104634915 15.8080908536
6.33953471707 16.1438957557
6.498023085 16.506122279
6.65651145293 16.8996506465
6.81499982086 17.3310377319
6.97348818878 17.8093849634
7.13197655671 18.3478601017
7.29046492464 18.9665764423
7.44895329256 19.6986209153
7.60744166049 20.60461097
7.76593002842 21.816504727


==> figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt7.tex <==
0.0 12.4140452292
0.132433347565 12.4164000529
0.26486669513 12.4234663651
0.397300042696 12.4352497143
0.529733390261 12.4517594306
0.662166737826 12.4730087504
0.794600085391 12.4990149936
0.927033432956 12.5297997945
1.05946678052 12.5653893903
1.19190012809 12.6058149697
1.32433347565 12.6511130874
1.45676682322 12.7013261503
1.58920017078 12.7565029807
1.72163351835 12.8166994682
1.85406686591 12.8819793179
1.98650021348 12.9524149092
2.11893356104 13.0280882814
2.25136690861 13.1090922629
2.38380025617 13.1955317693
2.51623360374 13.2875252975
2.6486669513 13.3852066506
2.78110029887 13.4887269366
2.91353364643 13.5982568941
3.045966994 13.7139896103
3.17840034157 13.8361437149
3.31083368913 13.964967154
3.4432670367 14.1007416769
3.57570038426 14.2437882068
3.70813373183 14.394473315
3.84056707939 14.5532170878
3.97300042696 14.7205027665
4.10543377452 14.8968886685
4.23786712209 15.0830230781
4.37030046965 15.2796630514
4.50273381722 15.4876984509
4.63516716478 15.708183074
4.76760051235 15.9423755699
4.90003385991 16.1917941147
5.03246720748 16.4582908448
5.16490055504 16.7441553506
5.29733390261 17.0522621084
5.42976725017 17.3862864957
5.56220059774 17.7510319232
5.6946339453 18.1529451532
5.82706729287 18.6009678635
5.95950064043 19.1080301031
6.091933988 19.6938766597
6.22436733556 20.3909864766
6.35680068313 21.2588729216
6.4892340307 22.4271446731


==> figuresAndData/dataForRayleigh-rightEnd-sigma8prob0pt8.tex <==
0.0 14.352980624
0.104749805795 14.3548920166
0.20949961159 14.3606286032
0.314249417386 14.3701976299
0.418999223181 14.3836112439
0.523749028976 14.4008865981
0.628498834771 14.4220460018
0.733248640566 14.4471171172
0.837998446361 14.476133206
0.942748252157 14.5091334297
1.04749805795 14.5461632082
1.15224786375 14.5872746434
1.25699766954 14.6325270141
1.36174747534 14.6819873523
1.46649728113 14.7357311098
1.57124708693 14.7938429297
1.67599689272 14.8564175377
1.78074669852 14.9235607713
1.88549650431 14.9953907705
1.99024631011 15.0720393582
2.0949961159 15.1536536428
2.1997459217 15.2403978858
2.30449572749 15.332455687
2.40924553329 15.4300325486
2.51399533908 15.533358902
2.61874514488 15.6426936963
2.72349495067 15.7583286783
2.82824475647 15.8805935292
2.93299456226 16.0098620713
3.03774436806 16.1465598237
3.14249417386 16.2911732756
3.24724397965 16.44426137
3.35199378545 16.6064698624
3.45674359124 16.7785494708
3.56149339704 16.9613790895
3.66624320283 17.1559958731
3.77099300863 17.3636347999
3.87574281442 17.5857815618
3.98049262022 17.8242445946
4.08524242601 18.0812552664
4.18999223181 18.3596106492
4.2947420376 18.662882776
4.3994918434 18.9957356513
4.50424164919 19.3644248119
4.60899145499 19.7776231894
4.71374126078 20.2478701531
4.81849106658 20.7943152547
4.92324087237 21.4484680762
5.02799067817 22.2680989361
5.13274048396 23.3791350092


==> figuresAndData/dataForRayleigh-upperEnd-sigma1prob0pt1.tex <==
0.0 0.459043605026
0.004276 0.45906573285
0.008552 0.459132110057
0.012828 0.459242717864
0.017104 0.459397524999
0.02138 0.45959648774
0.025656 0.459839549984
0.029932 0.460126643326
0.034208 0.460457687155
0.038484 0.460832588772
0.04276 0.461251243519
0.047036 0.46171353493
0.051312 0.462219334894
0.055588 0.462768503831
0.059864 0.463360890892
0.06414 0.463996334161
0.068416 0.464674660878
0.072692 0.465395687674
0.076968 0.466159220816
0.081244 0.466965056466
0.08552 0.467812980946
0.089796 0.468702771017
0.094072 0.469634194164
0.098348 0.470607008894
0.102624 0.471620965034
0.1069 0.472675804041
0.111176 0.473771259317
0.115452 0.474907056525
0.119728 0.476082913917
0.124004 0.477298542654
0.12828 0.47855364714
0.132556 0.47984792535
0.136832 0.481181069161
0.141108 0.482552764686
0.145384 0.483962692604
0.14966 0.485410528491
0.153936 0.486895943147
0.158212 0.488418602923
0.162488 0.489978170045
0.166764 0.491574302933
0.17104 0.493206656518
0.175316 0.49487488255
0.179592 0.496578629906
0.183868 0.498317544893
0.188144 0.500091271538
0.19242 0.501899451884
0.196696 0.503741726263
0.200972 0.505617733581
0.205248 0.50752711158
0.209524 0.509469497101
0.2138 0.511444526341
0.218076 0.513451835094
0.222352 0.515491058994
0.226628 0.517561833742
0.230904 0.519663795331
0.23518 0.521796580261
0.239456 0.523959825742
0.243732 0.526153169897
0.248008 0.528376251948
0.252284 0.530628712401
0.25656 0.53291019322
0.260836 0.535220337994
0.265112 0.537558792092
0.269388 0.539925202818
0.273664 0.542319219551
0.27794 0.544740493883
0.282216 0.547188679744
0.286492 0.549663433527
0.290768 0.552164414198
0.295044 0.554691283404
0.29932 0.557243705573
0.303596 0.559821348009
0.307872 0.562423880975
0.312148 0.565050977779
0.316424 0.567702314842
0.3207 0.570377571775
0.324976 0.573076431434
0.329252 0.575798579982
0.333528 0.578543706942
0.337804 0.581311505238
0.34208 0.584101671247
0.346356 0.586913904826
0.350632 0.589747909354
0.354908 0.592603391754
0.359184 0.595480062521
0.36346 0.59837763574
0.367736 0.601295829103
0.372012 0.604234363927
0.376288 0.607192965153
0.380564 0.610171361363
0.38484 0.613169284775
0.389116 0.616186471248
0.393392 0.619222660278
0.397668 0.622277594989
0.401944 0.625351022131
0.40622 0.628442692064
0.410496 0.631552358751
0.414772 0.634679779736
0.419048 0.637824716136
0.423324 0.640986932614
0.4276 0.644166197365
0.431876 0.647362282091
0.436152 0.650574961977
0.440428 0.653804015671
0.444704 0.65704922525
0.44898 0.6603103762
0.453256 0.663587257382
0.457532 0.666879661009
0.461808 0.670187382607
0.466084 0.673510220993
0.47036 0.676847978236
0.474636 0.680200459627
0.478912 0.683567473648
0.483188 0.686948831933
0.487464 0.690344349239
0.49174 0.693753843408
0.496016 0.697177135332
0.500292 0.70061404892
0.504568 0.704064411061
0.508844 0.707528051586
0.51312 0.711004803236
0.517396 0.714494501623
0.521672 0.717996985196
0.525948 0.721512095203
0.530224 0.725039675655
0.5345 0.72857957329
0.538776 0.732131637538
0.543052 0.735695720485
0.547328 0.739271676835
0.551604 0.742859363877
0.55588 0.746458641447
0.560156 0.750069371895
0.564432 0.75369142005
0.568708 0.757324653183
0.572984 0.760968940973
0.57726 0.764624155476
0.581536 0.768290171087
0.585812 0.771966864507
0.590088 0.775654114715
0.594364 0.779351802927
0.59864 0.783059812568
0.602916 0.786778029241
0.607192 0.790506340692
0.611468 0.794244636781
0.615744 0.797992809449
0.62002 0.801750752688
0.624296 0.805518362513
0.628572 0.80929553693
0.632848 0.813082175904
0.637124 0.816878181338
0.6414 0.820683457034
0.645676 0.824497908676
0.649952 0.82832144379
0.654228 0.83215397173
0.658504 0.83599540364
0.66278 0.839845652433
0.667056 0.843704632766
0.671332 0.847572261009
0.675608 0.851448455227
0.679884 0.855333135149
0.68416 0.859226222147
0.688436 0.863127639213
0.692712 0.867037310932
0.696988 0.870955163462
0.701264 0.874881124511
0.70554 0.878815123314
0.709816 0.88275709061
0.714092 0.886706958624
0.718368 0.890664661044
0.722644 0.894630133
0.72692 0.898603311046
0.731196 0.902584133136
0.735472 0.906572538609
0.739748 0.91056846817
0.744024 0.914571863868
0.7483 0.91858266908
0.752576 0.922600828493
0.756852 0.926626288087
0.761128 0.930658995118
0.765404 0.934698898097
0.76968 0.938745946783
0.773956 0.942800092157
0.778232 0.946861286414
0.782508 0.950929482941
0.786784 0.95500463631
0.79106 0.959086702255
0.795336 0.963175637664
0.799612 0.967271400563
0.803888 0.971373950103
0.808164 0.975483246544
0.81244 0.979599251246
0.816716 0.983721926655
0.820992 0.98785123629
0.825268 0.99198714473
0.829544 0.996129617608
0.83382 1.00027862159
0.838096 1.00443412438
0.842372 1.00859609468
0.846648 1.01276450222
0.850924 1.01693931771
0.8552 1.02112051286
0.859476 1.02530806035
0.863752 1.02950193381
0.868028 1.03370210787
0.872304 1.03790855808
0.87658 1.04212126093
0.880856 1.04634019387
0.885132 1.05056533523
0.889408 1.05479666431
0.893684 1.05903416129
0.89796 1.06327780725
0.902236 1.06752758419
0.906512 1.07178347499
0.910788 1.0760454634
0.915064 1.08031353406
0.91934 1.08458767249
0.923616 1.08886786506
0.927892 1.09315409902
0.932168 1.09744636245
0.936444 1.10174464432
0.94072 1.10604893441
0.944996 1.11035922336
0.949272 1.11467550265
0.953548 1.11899776458
0.957824 1.12332600231
0.9621 1.1276602098
0.966376 1.13200038185
0.970652 1.13634651407
0.974928 1.1406986029
0.979204 1.1450566456
0.98348 1.14942064023
0.987756 1.15379058568
0.992032 1.15816648163
0.996308 1.16254832859
1.000584 1.16693612788
1.00486 1.1713298816
1.009136 1.17572959268
1.013412 1.18013526486
1.017688 1.18454690267
1.021964 1.18896451145
1.02624 1.19338809736
1.030516 1.19781766734
1.034792 1.20225322916
1.039068 1.20669479138
1.043344 1.21114236339
1.04762 1.21559595538
1.051896 1.22005557835
1.056172 1.2245212441
1.060448 1.22899296527
1.064724 1.23347075531
1.069 1.23795462849
1.073276 1.24244459989
1.077552 1.24694068544
1.081828 1.25144290188
1.086104 1.25595126679
1.09038 1.2604657986
1.094656 1.26498651655
1.098932 1.26951344076
1.103208 1.27404659218
1.107484 1.27858599262
1.11176 1.28313166474
1.116036 1.28768363208
1.120312 1.29224191904
1.124588 1.29680655091
1.128864 1.30137755384
1.13314 1.30595495489
1.137416 1.31053878202
1.141692 1.31512906406
1.145968 1.31972583079
1.150244 1.32432911289
1.15452 1.32893894196
1.158796 1.33355535055
1.163072 1.33817837213
1.167348 1.34280804116
1.171624 1.34744439301
1.1759 1.35208746408
1.180176 1.35673729169
1.184452 1.3613939142
1.188728 1.36605737094
1.193004 1.37072770228
1.19728 1.37540494958
1.201556 1.38008915526
1.205832 1.38478036279
1.210108 1.38947861668
1.214384 1.39418396253
1.21866 1.39889644702
1.222936 1.40361611794
1.227212 1.40834302417
1.231488 1.41307721574
1.235764 1.41781874382
1.24004 1.42256766074
1.244316 1.42732402
1.248592 1.43208787629
1.252868 1.43685928551
1.257144 1.44163830479
1.26142 1.4464249925
1.265696 1.45121940828
1.269972 1.45602161305
1.274248 1.460831669
1.278524 1.46564963969
1.2828 1.47047558998
1.287076 1.47530958612
1.291352 1.48015169574
1.295628 1.48500198785
1.299904 1.48986053293
1.30418 1.49472740288
1.308456 1.4996026711
1.312732 1.50448641248
1.317008 1.50937870346
1.321284 1.51427962201
1.32556 1.51918924769
1.329836 1.52410766168
1.334112 1.5290349468
1.338388 1.53397118754
1.342664 1.53891647008
1.34694 1.54387088234
1.351216 1.54883451401
1.355492 1.55380745656
1.359768 1.55878980333
1.364044 1.56378164948
1.36832 1.56878309211
1.372596 1.57379423024
1.376872 1.5788151649
1.381148 1.5838459991
1.385424 1.58888683793
1.3897 1.59393778859
1.393976 1.59899896042
1.398252 1.60407046495
1.402528 1.60915241594
1.406804 1.61424492943
1.41108 1.61934812381
1.415356 1.62446211984
1.419632 1.62958704071
1.423908 1.6347230121
1.428184 1.63987016223
1.43246 1.64502862193
1.436736 1.65019852467
1.441012 1.65538000663
1.445288 1.66057320678
1.449564 1.66577826693
1.45384 1.67099533179
1.458116 1.67622454904
1.462392 1.68146606943
1.466668 1.68672004678
1.470944 1.69198663815
1.47522 1.69726600381
1.479496 1.70255830744
1.483772 1.70786371608
1.488048 1.71318240034
1.492324 1.71851453439
1.4966 1.7238602961
1.500876 1.72921986713
1.505152 1.734593433
1.509428 1.73998118322
1.513704 1.74538331136
1.51798 1.7508000152
1.522256 1.75623149679
1.526532 1.7616779626
1.530808 1.76713962363
1.535084 1.77261669551
1.53936 1.77810939864
1.543636 1.78361795834
1.547912 1.78914260495
1.552188 1.79468357398
1.556464 1.80024110628
1.56074 1.80581544814
1.565016 1.81140685149
1.569292 1.81701557405
1.573568 1.82264187946
1.577844 1.82828603752
1.58212 1.8339483243
1.586396 1.83962902237
1.590672 1.84532842099
1.594948 1.85104681627
1.599224 1.85678451145
1.6035 1.86254181702
1.607776 1.86831905105
1.612052 1.87411653934
1.616328 1.87993461569
1.620604 1.88577362219
1.62488 1.89163390941
1.629156 1.89751583673
1.633432 1.90341977259
1.637708 1.90934609481
1.641984 1.9152951909
1.64626 1.92126745835
1.650536 1.927263305
1.654812 1.93328314935
1.659088 1.93932742097
1.663364 1.94539656085
1.66764 1.9514910218
1.671916 1.95761126887
1.676192 1.96375777977
1.680468 1.96993104536
1.684744 1.97613157005
1.68902 1.98235987237
1.693296 1.98861648545
1.697572 1.99490195756
1.701848 2.00121685268
1.706124 2.00756175109
1.7104 2.01393725003
1.714676 2.02034396427
1.718952 2.02678252688
1.723228 2.0332535899
1.727504 2.03975782512
1.73178 2.04629592482
1.736056 2.05286860268
1.740332 2.05947659459
1.744608 2.06612065962
1.748884 2.07280158094
1.75316 2.07952016688
1.757436 2.08627725199
1.761712 2.09307369818
1.765988 2.0999103959
1.770264 2.10678826545
1.77454 2.11370825825
1.778816 2.12067135828
1.783092 2.12767858361
1.787368 2.13473098792
1.791644 2.14182966218
1.79592 2.14897573646
1.800196 2.15617038179
1.804472 2.16341481212
1.808748 2.1707102865
1.813024 2.17805811126
1.8173 2.18545964248
1.821576 2.19291628846
1.825852 2.20042951247
1.830128 2.20800083568
1.834404 2.21563184016
1.83868 2.22332417224
1.842956 2.23107954603
1.847232 2.23889974714
1.851508 2.24678663678
1.855784 2.25474215604
1.86006 2.26276833056
1.864336 2.27086727549
1.868612 2.27904120085
1.872888 2.28729241735
1.877164 2.29562334254
1.88144 2.30403650755
1.885716 2.31253456434
1.889992 2.32112029352
1.894268 2.32979661285
1.898544 2.33856658641
1.90282 2.34743343462
1.907096 2.35640054506
1.911372 2.36547148433
1.915648 2.37465001092
1.919924 2.38394008927
1.9242 2.3933459052
1.928476 2.40287188277
1.932752 2.41252270278
1.937028 2.42230332319
1.941304 2.43221900147
1.94558 2.44227531945
1.949856 2.45247821063
1.954132 2.46283399061
1.958408 2.47334939075
1.962684 2.48403159574
1.96696 2.49488828551
1.971236 2.50592768209
1.975512 2.51715860223
1.979788 2.52859051656
1.984064 2.54023361628
1.98834 2.5520988888
1.992616 2.56419820337
1.996892 2.57654440884
2.001168 2.58915144524
2.005444 2.60203447193
2.00972 2.61521001517
2.013996 2.62869613877
2.018272 2.64251264257
2.022548 2.65668129391
2.026824 2.67122609951
2.0311 2.68617362599
2.035376 2.70155338038
2.039652 2.71739826433
2.043928 2.73374512008
2.048204 2.75063539144
2.05248 2.76811593016
2.056756 2.78623998808
2.061032 2.80506844908
2.065308 2.82467137416
2.069584 2.84512996074
2.07386 2.86653905751
2.078136 2.88901043604
2.082412 2.91267711118
2.086688 2.9376991431
2.090964 2.96427157874
2.09524 2.99263555898
2.099516 3.02309424542
2.103792 3.05603632821
2.108068 3.09197192658
2.112344 3.13158969596
2.11662 3.17585229553
2.120896 3.22616619096
2.125172 3.28470875188
2.129448 3.35512951105
2.133724 3.44430124906


==> figuresAndData/dataForRayleigh-upperEnd-sigma1pt5prob0pt05.tex <==
0.0 0.480437118408
0.004276 0.48045714819
0.008552 0.480517232554
0.012828 0.480617356553
0.017104 0.480757495301
0.02138 0.480937613996
0.025656 0.481157667973
0.029932 0.481417602749
0.034208 0.4817173541
0.038484 0.482056848134
0.04276 0.482436001384
0.047036 0.482854720912
0.051312 0.483312904419
0.055588 0.483810440372
0.059864 0.484347208138
0.06414 0.484923078126
0.068416 0.485537911943
0.072692 0.486191562559
0.076968 0.486883874475
0.081244 0.487614683906
0.08552 0.48838381897
0.089796 0.489191099879
0.094072 0.490036339148
0.098348 0.490919341798
0.102624 0.491839905571
0.1069 0.492797821154
0.111176 0.493792872401
0.115452 0.494824836559
0.119728 0.495893484506
0.124004 0.496998580984
0.12828 0.498139884836
0.132556 0.499317149251
0.136832 0.500530122003
0.141108 0.501778545694
0.145384 0.503062158004
0.14966 0.504380691928
0.153936 0.505733876026
0.158212 0.507121434667
0.162488 0.508543088267
0.166764 0.509998553537
0.17104 0.511487543717
0.175316 0.513009768817
0.179592 0.51456493585
0.183868 0.516152749067
0.188144 0.51777291018
0.19242 0.519425118596
0.196696 0.52110907163
0.200972 0.522824464729
0.205248 0.524570991682
0.209524 0.526348344831
0.2138 0.528156215276
0.218076 0.529994293071
0.222352 0.531862267423
0.226628 0.533759826881
0.230904 0.535686659516
0.23518 0.537642453109
0.239456 0.539626895315
0.243732 0.541639673838
0.248008 0.543680476592
0.252284 0.545748991858
0.25656 0.547844908438
0.260836 0.549967915795
0.265112 0.552117704204
0.269388 0.554293964878
0.273664 0.5564963901
0.27794 0.558724673352
0.282216 0.560978509428
0.286492 0.56325759455
0.290768 0.565561626475
0.295044 0.5678903046
0.29932 0.570243330056
0.303596 0.572620405807
0.307872 0.575021236729
0.312148 0.577445529702
0.316424 0.579892993681
0.3207 0.582363339774
0.324976 0.584856281306
0.329252 0.58737153389
0.333528 0.589908815483
0.337804 0.59246784644
0.34208 0.59504834957
0.346356 0.597650050185
0.350632 0.600272676136
0.354908 0.602915957864
0.359184 0.605579628427
0.36346 0.60826342354
0.367736 0.610967081603
0.372012 0.613690343726
0.376288 0.616432953756
0.380564 0.619194658292
0.38484 0.621975206709
0.389116 0.62477435117
0.393392 0.627591846638
0.397668 0.630427450887
0.401944 0.633280924507
0.40622 0.636152030912
0.410496 0.639040536344
0.414772 0.641946209867
0.419048 0.644868823374
0.423324 0.647808151578
0.4276 0.650763972011
0.431876 0.653736065014
0.436152 0.656724213731
0.440428 0.659728204099
0.444704 0.662747824836
0.44898 0.665782867427
0.453256 0.668833126115
0.457532 0.671898397881
0.461808 0.674978482428
0.466084 0.678073182167
0.47036 0.681182302197
0.474636 0.684305650284
0.478912 0.687443036845
0.483188 0.690594274922
0.487464 0.693759180165
0.49174 0.696937570806
0.496016 0.700129267639
0.500292 0.703334093995
0.504568 0.706551875718
0.508844 0.70978244114
0.51312 0.713025621059
0.517396 0.716281248709
0.521672 0.719549159738
0.525948 0.72282919218
0.530224 0.72612118643
0.5345 0.729424985216
0.538776 0.732740433574
0.543052 0.736067378821
0.547328 0.739405670526
0.551604 0.742755160485
0.55588 0.746115702693
0.560156 0.749487153317
0.564432 0.752869370668
0.568708 0.756262215175
0.572984 0.759665549357
0.57726 0.763079237795
0.581536 0.766503147107
0.585812 0.769937145919
0.590088 0.773381104838
0.594364 0.776834896428
0.59864 0.780298395178
0.602916 0.783771477481
0.607192 0.787254021605
0.611468 0.790745907664
0.615744 0.794247017599
0.62002 0.797757235143
0.624296 0.801276445804
0.628572 0.804804536835
0.632848 0.808341397207
0.637124 0.811886917588
0.6414 0.815440990316
0.645676 0.819003509377
0.649952 0.822574370374
0.654228 0.826153470511
0.658504 0.829740708565
0.66278 0.833335984863
0.667056 0.836939201257
0.671332 0.840550261104
0.675608 0.844169069242
0.679884 0.847795531968
0.68416 0.851429557013
0.688436 0.855071053524
0.692712 0.858719932039
0.696988 0.862376104468
0.701264 0.866039484071
0.70554 0.869709985435
0.709816 0.873387524459
0.714092 0.877072018327
0.718368 0.880763385493
0.722644 0.884461545657
0.72692 0.888166419751
0.731196 0.891877929913
0.735472 0.895595999476
0.739748 0.899320552941
0.744024 0.903051515966
0.7483 0.906788815341
0.752576 0.910532378978
0.756852 0.914282135885
0.761128 0.918038016156
0.765404 0.92179995095
0.76968 0.925567872473
0.773956 0.929341713965
0.778232 0.933121409684
0.782508 0.936906894885
0.786784 0.940698105809
0.79106 0.944494979665
0.795336 0.948297454617
0.799612 0.952105469766
0.803888 0.955918965138
0.808164 0.959737881667
0.81244 0.963562161182
0.816716 0.967391746394
0.820992 0.97122658088
0.825268 0.975066609069
0.829544 0.978911776233
0.83382 0.982762028466
0.838096 0.98661731268
0.842372 0.990477576585
0.846648 0.994342768681
0.850924 0.998212838243
0.8552 1.00208773531
0.859476 1.00596741067
0.863752 1.00985181586
0.868028 1.01374090314
0.872304 1.01763462548
0.87658 1.02153293657
0.880856 1.02543579078
0.885132 1.02934314318
0.889408 1.0332549495
0.893684 1.03717116614
0.89796 1.04109175015
0.902236 1.04501665923
0.906512 1.04894585171
0.910788 1.05287928654
0.915064 1.05681692329
0.91934 1.06075872211
0.923616 1.06470464378
0.927892 1.06865464966
0.932168 1.07260870166
0.936444 1.07656676228
0.94072 1.08052879458
0.944996 1.08449476216
0.949272 1.08846462918
0.953548 1.09243836032
0.957824 1.09641592079
0.9621 1.10039727633
0.966376 1.10438239316
0.970652 1.10837123805
0.974928 1.11236377822
0.979204 1.1163599814
0.98348 1.12035981582
0.987756 1.12436325014
0.992032 1.12837025353
0.996308 1.13238079559
1.000584 1.13639484638
1.00486 1.14041237643
1.009136 1.14443335668
1.013412 1.14845775853
1.017688 1.15248555377
1.021964 1.15651671465
1.02624 1.16055121383
1.030516 1.16458902435
1.034792 1.16863011968
1.039068 1.1726744737
1.043344 1.17672206063
1.04762 1.18077285514
1.051896 1.18482683224
1.056172 1.18888396732
1.060448 1.19294423616
1.064724 1.19700761488
1.069 1.20107407999
1.073276 1.20514360832
1.077552 1.20921617707
1.081828 1.21329176379
1.086104 1.21737034636
1.09038 1.221451903
1.094656 1.22553641227
1.098932 1.22962385303
1.103208 1.23371420449
1.107484 1.23780744617
1.11176 1.24190355789
1.116036 1.24600251981
1.120312 1.25010431236
1.124588 1.2542089163
1.128864 1.25831631267
1.13314 1.26242648281
1.137416 1.26653940834
1.141692 1.27065507119
1.145968 1.27477345354
1.150244 1.27889453787
1.15452 1.28301830694
1.158796 1.28714474375
1.163072 1.29127383161
1.167348 1.29540555406
1.171624 1.29953989492
1.1759 1.30367683826
1.180176 1.3078163684
1.184452 1.31195846993
1.188728 1.31610312767
1.193004 1.32025032669
1.19728 1.3244000523
1.201556 1.32855229007
1.205832 1.33270702577
1.210108 1.33686424543
1.214384 1.34102393531
1.21866 1.34518608188
1.222936 1.34935067185
1.227212 1.35351769216
1.231488 1.35768712995
1.235764 1.36185897258
1.24004 1.36603320765
1.244316 1.37020982294
1.248592 1.37438880646
1.252868 1.37857014643
1.257144 1.38275383125
1.26142 1.38693984955
1.265696 1.39112819015
1.269972 1.39531884207
1.274248 1.39951179453
1.278524 1.40370703693
1.2828 1.40790455888
1.287076 1.41210435018
1.291352 1.4163064008
1.295628 1.4205107009
1.299904 1.42471724085
1.30418 1.42892601117
1.308456 1.43313700257
1.312732 1.43735020595
1.317008 1.44156561238
1.321284 1.4457832131
1.32556 1.45000299953
1.329836 1.45422496325
1.334112 1.45844909602
1.338388 1.46267538977
1.342664 1.46690383659
1.34694 1.47113442874
1.351216 1.47536715864
1.355492 1.47960201887
1.359768 1.48383900217
1.364044 1.48807810144
1.36832 1.49231930975
1.372596 1.49656262031
1.376872 1.50080802649
1.381148 1.50505552181
1.385424 1.50930509995
1.3897 1.51355675472
1.393976 1.51781048012
1.398252 1.52206627025
1.402528 1.5263241194
1.406804 1.53058402197
1.41108 1.53484597252
1.415356 1.53910996576
1.419632 1.54337599654
1.423908 1.54764405984
1.428184 1.55191415078
1.43246 1.55618626464
1.436736 1.56046039681
1.441012 1.56473654284
1.445288 1.56901469841
1.449564 1.57329485931
1.45384 1.57757702151
1.458116 1.58186118108
1.462392 1.58614733422
1.466668 1.59043547729
1.470944 1.59472560674
1.47522 1.5990177192
1.479496 1.60331181138
1.483772 1.60760788014
1.488048 1.61190592247
1.492324 1.61620593548
1.4966 1.62050791641
1.500876 1.62481186263
1.505152 1.62911777161
1.509428 1.63342564097
1.513704 1.63773546844
1.51798 1.64204725188
1.522256 1.64636098927
1.526532 1.65067667869
1.530808 1.65499431838
1.535084 1.65931390666
1.53936 1.663635442
1.543636 1.66795892297
1.547912 1.67228434827
1.552188 1.6766117167
1.556464 1.68094102719
1.56074 1.6852722788
1.565016 1.68960547067
1.569292 1.69394060209
1.573568 1.69827767245
1.577844 1.70261668125
1.58212 1.70695762812
1.586396 1.71130051279
1.590672 1.71564533512
1.594948 1.71999209505
1.599224 1.72434079268
1.6035 1.72869142818
1.607776 1.73304400185
1.612052 1.73739851411
1.616328 1.74175496549
1.620604 1.7461133566
1.62488 1.75047368822
1.629156 1.75483596118
1.633432 1.75920017645
1.637708 1.76356633513
1.641984 1.76793443839
1.64626 1.77230448753
1.650536 1.77667648396
1.654812 1.78105042921
1.659088 1.78542632489
1.663364 1.78980417275
1.66764 1.79418397464
1.671916 1.79856573251
1.676192 1.80294944842
1.680468 1.80733512455
1.684744 1.81172276319
1.68902 1.81611236673
1.693296 1.82050393767
1.697572 1.82489747863
1.701848 1.82929299231
1.706124 1.83369048156
1.7104 1.8380899493
1.714676 1.84249139859
1.718952 1.84689483259
1.723228 1.85130025455
1.727504 1.85570766786
1.73178 1.86011707599
1.736056 1.86452848254
1.740332 1.86894189122
1.744608 1.87335730583
1.748884 1.8777747303
1.75316 1.88219416866
1.757436 1.88661562506
1.761712 1.89103910373
1.765988 1.89546460906
1.770264 1.89989214552
1.77454 1.90432171768
1.778816 1.90875333024
1.783092 1.91318698801
1.787368 1.91762269592
1.791644 1.92206045898
1.79592 1.92650028235
1.800196 1.93094217128
1.804472 1.93538613114
1.808748 1.93983216741
1.813024 1.94428028568
1.8173 1.94873049167
1.821576 1.95318279119
1.825852 1.95763719019
1.830128 1.96209369471
1.834404 1.96655231093
1.83868 1.97101304513
1.842956 1.9754759037
1.847232 1.97994089317
1.851508 1.98440802017
1.855784 1.98887729145
1.86006 1.99334871388
1.864336 1.99782229444
1.868612 2.00229804025
1.872888 2.00677595852
1.877164 2.01125605662
1.88144 2.01573834199
1.885716 2.02022282225
1.889992 2.02470950508
1.894268 2.02919839834
1.898544 2.03368950996
1.90282 2.03818284804
1.907096 2.04267842078
1.911372 2.04717623651
1.915648 2.05167630368
1.919924 2.05617863087
1.9242 2.0606832268
1.928476 2.0651901003
1.932752 2.06969926033
1.937028 2.07421071599
1.941304 2.07872447651
1.94558 2.08324055124
1.949856 2.08775894967
1.954132 2.09227968142
1.958408 2.09680275624
1.962684 2.10132818402
1.96696 2.10585597478
1.971236 2.11038613869
1.975512 2.11491868603
1.979788 2.11945362724
1.984064 2.1239909729
1.98834 2.12853073371
1.992616 2.13307292053
1.996892 2.13761754436
2.001168 2.14216461632
2.005444 2.14671414771
2.00972 2.15126614994
2.013996 2.15582063459
2.018272 2.16037761338
2.022548 2.16493709818
2.026824 2.16949910099
2.0311 2.174063634
2.035376 2.1786307095
2.039652 2.18320033999
2.043928 2.18777253807
2.048204 2.19234731654
2.05248 2.19692468832
2.056756 2.20150466651
2.061032 2.20608726436
2.065308 2.21067249529
2.069584 2.21526037287
2.07386 2.21985091084
2.078136 2.2244441231
2.082412 2.22904002372
2.086688 2.23363862693
2.090964 2.23823994713
2.09524 2.24284399891
2.099516 2.24745079701
2.103792 2.25206035633
2.108068 2.25667269199
2.112344 2.26128781924
2.11662 2.26590575354
2.120896 2.27052651052
2.125172 2.27515010597
2.129448 2.27977655589
2.133724 2.28440587647


==> figuresAndData/dataForRayleigh-upperEnd-sigma1pt5prob0pt5.tex <==
0.0 0.480437118408
0.004276 0.48045714819
0.008552 0.480517232554
0.012828 0.480617356553
0.017104 0.480757495301
0.02138 0.480937613996
0.025656 0.481157667973
0.029932 0.481417602749
0.034208 0.4817173541
0.038484 0.482056848134
0.04276 0.482436001384
0.047036 0.482854720912
0.051312 0.483312904419
0.055588 0.483810440372
0.059864 0.484347208138
0.06414 0.484923078126
0.068416 0.485537911943
0.072692 0.486191562559
0.076968 0.486883874475
0.081244 0.487614683906
0.08552 0.48838381897
0.089796 0.489191099879
0.094072 0.490036339148
0.098348 0.490919341798
0.102624 0.491839905571
0.1069 0.492797821154
0.111176 0.493792872401
0.115452 0.494824836559
0.119728 0.495893484506
0.124004 0.496998580984
0.12828 0.498139884836
0.132556 0.499317149251
0.136832 0.500530122003
0.141108 0.501778545694
0.145384 0.503062158004
0.14966 0.504380691928
0.153936 0.505733876026
0.158212 0.507121434667
0.162488 0.508543088267
0.166764 0.509998553537
0.17104 0.511487543717
0.175316 0.513009768817
0.179592 0.51456493585
0.183868 0.516152749067
0.188144 0.51777291018
0.19242 0.519425118596
0.196696 0.52110907163
0.200972 0.522824464729
0.205248 0.524570991682
0.209524 0.526348344831
0.2138 0.528156215276
0.218076 0.529994293071
0.222352 0.531862267423
0.226628 0.533759826881
0.230904 0.535686659516
0.23518 0.537642453109
0.239456 0.539626895315
0.243732 0.541639673838
0.248008 0.543680476592
0.252284 0.545748991858
0.25656 0.547844908438
0.260836 0.549967915795
0.265112 0.552117704204
0.269388 0.554293964878
0.273664 0.5564963901
0.27794 0.558724673352
0.282216 0.560978509428
0.286492 0.56325759455
0.290768 0.565561626475
0.295044 0.5678903046
0.29932 0.570243330056
0.303596 0.572620405807
0.307872 0.575021236729
0.312148 0.577445529702
0.316424 0.579892993681
0.3207 0.582363339774
0.324976 0.584856281306
0.329252 0.58737153389
0.333528 0.589908815483
0.337804 0.59246784644
0.34208 0.59504834957
0.346356 0.597650050185
0.350632 0.600272676136
0.354908 0.602915957864
0.359184 0.605579628427
0.36346 0.60826342354
0.367736 0.610967081603
0.372012 0.613690343726
0.376288 0.616432953756
0.380564 0.619194658292
0.38484 0.621975206709
0.389116 0.62477435117
0.393392 0.627591846638
0.397668 0.630427450887
0.401944 0.633280924507
0.40622 0.636152030912
0.410496 0.639040536344
0.414772 0.641946209867
0.419048 0.644868823374
0.423324 0.647808151578
0.4276 0.650763972011
0.431876 0.653736065014
0.436152 0.656724213731
0.440428 0.659728204099
0.444704 0.662747824836
0.44898 0.665782867427
0.453256 0.668833126115
0.457532 0.671898397881
0.461808 0.674978482428
0.466084 0.678073182167
0.47036 0.681182302197
0.474636 0.684305650284
0.478912 0.687443036845
0.483188 0.690594274922
0.487464 0.693759180165
0.49174 0.696937570806
0.496016 0.700129267639
0.500292 0.703334093995
0.504568 0.706551875718
0.508844 0.70978244114
0.51312 0.713025621059
0.517396 0.716281248709
0.521672 0.719549159738
0.525948 0.72282919218
0.530224 0.72612118643
0.5345 0.729424985216
0.538776 0.732740433574
0.543052 0.736067378821
0.547328 0.739405670526
0.551604 0.742755160485
0.55588 0.746115702693
0.560156 0.749487153317
0.564432 0.752869370668
0.568708 0.756262215175
0.572984 0.759665549357
0.57726 0.763079237795
0.581536 0.766503147107
0.585812 0.769937145919
0.590088 0.773381104838
0.594364 0.776834896428
0.59864 0.780298395178
0.602916 0.783771477481
0.607192 0.787254021605
0.611468 0.790745907664
0.615744 0.794247017599
0.62002 0.797757235143
0.624296 0.801276445804
0.628572 0.804804536835
0.632848 0.808341397207
0.637124 0.811886917588
0.6414 0.815440990316
0.645676 0.819003509377
0.649952 0.822574370374
0.654228 0.826153470511
0.658504 0.829740708565
0.66278 0.833335984863
0.667056 0.836939201257
0.671332 0.840550261104
0.675608 0.844169069242
0.679884 0.847795531968
0.68416 0.851429557013
0.688436 0.855071053524
0.692712 0.858719932039
0.696988 0.862376104468
0.701264 0.866039484071
0.70554 0.869709985435
0.709816 0.873387524459
0.714092 0.877072018327
0.718368 0.880763385493
0.722644 0.884461545657
0.72692 0.888166419751
0.731196 0.891877929913
0.735472 0.895595999476
0.739748 0.899320552941
0.744024 0.903051515966
0.7483 0.906788815341
0.752576 0.910532378978
0.756852 0.914282135885
0.761128 0.918038016156
0.765404 0.92179995095
0.76968 0.925567872473
0.773956 0.929341713965
0.778232 0.933121409684
0.782508 0.936906894885
0.786784 0.940698105809
0.79106 0.944494979665
0.795336 0.948297454617
0.799612 0.952105469766
0.803888 0.955918965138
0.808164 0.959737881667
0.81244 0.963562161182
0.816716 0.967391746394
0.820992 0.97122658088
0.825268 0.975066609069
0.829544 0.978911776233
0.83382 0.982762028466
0.838096 0.98661731268
0.842372 0.990477576585
0.846648 0.994342768681
0.850924 0.998212838243
0.8552 1.00208773531
0.859476 1.00596741067
0.863752 1.00985181586
0.868028 1.01374090314
0.872304 1.01763462548
0.87658 1.02153293657
0.880856 1.02543579078
0.885132 1.02934314318
0.889408 1.0332549495
0.893684 1.03717116614
0.89796 1.04109175015
0.902236 1.04501665923
0.906512 1.04894585171
0.910788 1.05287928654
0.915064 1.05681692329
0.91934 1.06075872211
0.923616 1.06470464378
0.927892 1.06865464966
0.932168 1.07260870166
0.936444 1.07656676228
0.94072 1.08052879458
0.944996 1.08449476216
0.949272 1.08846462918
0.953548 1.09243836032
0.957824 1.09641592079
0.9621 1.10039727633
0.966376 1.10438239316
0.970652 1.10837123805
0.974928 1.11236377822
0.979204 1.1163599814
0.98348 1.12035981582
0.987756 1.12436325014
0.992032 1.12837025353
0.996308 1.13238079559
1.000584 1.13639484638
1.00486 1.14041237643
1.009136 1.14443335668
1.013412 1.14845775853
1.017688 1.15248555377
1.021964 1.15651671465
1.02624 1.16055121383
1.030516 1.16458902435
1.034792 1.16863011968
1.039068 1.1726744737
1.043344 1.17672206063
1.04762 1.18077285514
1.051896 1.18482683224
1.056172 1.18888396732
1.060448 1.19294423616
1.064724 1.19700761488
1.069 1.20107407999
1.073276 1.20514360832
1.077552 1.20921617707
1.081828 1.21329176379
1.086104 1.21737034636
1.09038 1.221451903
1.094656 1.22553641227
1.098932 1.22962385303
1.103208 1.23371420449
1.107484 1.23780744617
1.11176 1.24190355789
1.116036 1.24600251981
1.120312 1.25010431236
1.124588 1.2542089163
1.128864 1.25831631267
1.13314 1.26242648281
1.137416 1.26653940834
1.141692 1.27065507119
1.145968 1.27477345354
1.150244 1.27889453787
1.15452 1.28301830694
1.158796 1.28714474375
1.163072 1.29127383161
1.167348 1.29540555406
1.171624 1.29953989492
1.1759 1.30367683826
1.180176 1.3078163684
1.184452 1.31195846993
1.188728 1.31610312767
1.193004 1.32025032669
1.19728 1.3244000523
1.201556 1.32855229007
1.205832 1.33270702577
1.210108 1.33686424543
1.214384 1.34102393531
1.21866 1.34518608188
1.222936 1.34935067185
1.227212 1.35351769216
1.231488 1.35768712995
1.235764 1.36185897258
1.24004 1.36603320765
1.244316 1.37020982294
1.248592 1.37438880646
1.252868 1.37857014643
1.257144 1.38275383125
1.26142 1.38693984955
1.265696 1.39112819015
1.269972 1.39531884207
1.274248 1.39951179453
1.278524 1.40370703693
1.2828 1.40790455888
1.287076 1.41210435018
1.291352 1.4163064008
1.295628 1.4205107009
1.299904 1.42471724085
1.30418 1.42892601117
1.308456 1.43313700257
1.312732 1.43735020595
1.317008 1.44156561238
1.321284 1.4457832131
1.32556 1.45000299953
1.329836 1.45422496325
1.334112 1.45844909602
1.338388 1.46267538977
1.342664 1.46690383659
1.34694 1.47113442874
1.351216 1.47536715864
1.355492 1.47960201887
1.359768 1.48383900217
1.364044 1.48807810144
1.36832 1.49231930975
1.372596 1.49656262031
1.376872 1.50080802649
1.381148 1.50505552181
1.385424 1.50930509995
1.3897 1.51355675472
1.393976 1.51781048012
1.398252 1.52206627025
1.402528 1.5263241194
1.406804 1.53058402197
1.41108 1.53484597252
1.415356 1.53910996576
1.419632 1.54337599654
1.423908 1.54764405984
1.428184 1.55191415078
1.43246 1.55618626464
1.436736 1.56046039681
1.441012 1.56473654284
1.445288 1.56901469841
1.449564 1.57329485931
1.45384 1.57757702151
1.458116 1.58186118108
1.462392 1.58614733422
1.466668 1.59043547729
1.470944 1.59472560674
1.47522 1.5990177192
1.479496 1.60331181138
1.483772 1.60760788014
1.488048 1.61190592247
1.492324 1.61620593548
1.4966 1.62050791641
1.500876 1.62481186263
1.505152 1.62911777161
1.509428 1.63342564097
1.513704 1.63773546844
1.51798 1.64204725188
1.522256 1.64636098927
1.526532 1.65067667869
1.530808 1.65499431838
1.535084 1.65931390666
1.53936 1.663635442
1.543636 1.66795892297
1.547912 1.67228434827
1.552188 1.6766117167
1.556464 1.68094102719
1.56074 1.6852722788
1.565016 1.68960547067
1.569292 1.69394060209
1.573568 1.69827767245
1.577844 1.70261668125
1.58212 1.70695762812
1.586396 1.71130051279
1.590672 1.71564533512
1.594948 1.71999209505
1.599224 1.72434079268
1.6035 1.72869142818
1.607776 1.73304400185
1.612052 1.73739851411
1.616328 1.74175496549
1.620604 1.7461133566
1.62488 1.75047368822
1.629156 1.75483596118
1.633432 1.75920017645
1.637708 1.76356633513
1.641984 1.76793443839
1.64626 1.77230448753
1.650536 1.77667648396
1.654812 1.78105042921
1.659088 1.78542632489
1.663364 1.78980417275
1.66764 1.79418397464
1.671916 1.79856573251
1.676192 1.80294944842
1.680468 1.80733512455
1.684744 1.81172276319
1.68902 1.81611236673
1.693296 1.82050393767
1.697572 1.82489747863
1.701848 1.82929299231
1.706124 1.83369048156
1.7104 1.8380899493
1.714676 1.84249139859
1.718952 1.84689483259
1.723228 1.85130025455
1.727504 1.85570766786
1.73178 1.86011707599
1.736056 1.86452848254
1.740332 1.86894189122
1.744608 1.87335730583
1.748884 1.8777747303
1.75316 1.88219416866
1.757436 1.88661562506
1.761712 1.89103910373
1.765988 1.89546460906
1.770264 1.89989214552
1.77454 1.90432171768
1.778816 1.90875333024
1.783092 1.91318698801
1.787368 1.91762269592
1.791644 1.92206045898
1.79592 1.92650028235
1.800196 1.93094217128
1.804472 1.93538613114
1.808748 1.93983216741
1.813024 1.94428028568
1.8173 1.94873049167
1.821576 1.95318279119
1.825852 1.95763719019
1.830128 1.96209369471
1.834404 1.96655231093
1.83868 1.97101304513
1.842956 1.9754759037
1.847232 1.97994089317
1.851508 1.98440802017
1.855784 1.98887729145
1.86006 1.99334871388
1.864336 1.99782229444
1.868612 2.00229804025
1.872888 2.00677595852
1.877164 2.01125605662
1.88144 2.01573834199
1.885716 2.02022282225
1.889992 2.02470950508
1.894268 2.02919839834
1.898544 2.03368950996
1.90282 2.03818284804
1.907096 2.04267842078
1.911372 2.04717623651
1.915648 2.05167630368
1.919924 2.05617863087
1.9242 2.0606832268
1.928476 2.0651901003
1.932752 2.06969926033
1.937028 2.07421071599
1.941304 2.07872447651
1.94558 2.08324055124
1.949856 2.08775894967
1.954132 2.09227968142
1.958408 2.09680275624
1.962684 2.10132818402
1.96696 2.10585597478
1.971236 2.11038613869
1.975512 2.11491868603
1.979788 2.11945362724
1.984064 2.1239909729
1.98834 2.12853073371
1.992616 2.13307292053
1.996892 2.13761754436
2.001168 2.14216461632
2.005444 2.14671414771
2.00972 2.15126614994
2.013996 2.15582063459
2.018272 2.16037761338
2.022548 2.16493709818
2.026824 2.16949910099
2.0311 2.174063634
2.035376 2.1786307095
2.039652 2.18320033999
2.043928 2.18777253807
2.048204 2.19234731654
2.05248 2.19692468832
2.056756 2.20150466651
2.061032 2.20608726436
2.065308 2.21067249529
2.069584 2.21526037287
2.07386 2.21985091084
2.078136 2.2244441231
2.082412 2.22904002372
2.086688 2.23363862693
2.090964 2.23823994713
2.09524 2.24284399891
2.099516 2.24745079701
2.103792 2.25206035633
2.108068 2.25667269199
2.112344 2.26128781924
2.11662 2.26590575354
2.120896 2.27052651052
2.125172 2.27515010597
2.129448 2.27977655589
2.133724 2.28440587647


==> figuresAndData/dataForRayleigh-upperEnd-sigma2prob0pt05.tex <==
0.0 0.640582824544
0.008276 0.64063909664
0.016552 0.640807883433
0.024828 0.641089096509
0.033104 0.641482588771
0.04138 0.641988154827
0.049656 0.64260553152
0.057932 0.643334398621
0.066208 0.644174379652
0.074484 0.645125042856
0.08276 0.646185902295
0.091036 0.647356419082
0.099312 0.648636002719
0.107588 0.650024012564
0.115864 0.651519759384
0.12414 0.653122507022
0.132416 0.654831474132
0.140692 0.656645836001
0.148968 0.658564726439
0.157244 0.660587239725
0.16552 0.662712432599
0.173796 0.664939326299
0.182072 0.667266908625
0.190348 0.669694136024
0.198624 0.672219935689
0.2069 0.674843207662
0.215176 0.677562826928
0.223452 0.680377645505
0.231728 0.68328649451
0.240004 0.686288186198
0.24828 0.68938151597
0.256556 0.692565264345
0.264832 0.695838198888
0.273108 0.699199076084
0.281384 0.702646643168
0.28966 0.706179639895
0.297936 0.709796800246
0.306212 0.713496854083
0.314488 0.717278528728
0.322764 0.721140550481
0.33104 0.725081646075
0.339316 0.729100544052
0.347592 0.733195976076
0.355868 0.737366678181
0.364144 0.741611391941
0.37242 0.745928865576
0.380696 0.750317854993
0.388972 0.75477712475
0.397248 0.759305448966
0.405524 0.76390161216
0.4138 0.768564410028
0.422076 0.773292650157
0.430352 0.778085152687
0.438628 0.782940750907
0.446904 0.7878582918
0.45518 0.792836636535
0.463456 0.797874660907
0.471732 0.802971255728
0.480008 0.808125327172
0.488284 0.813335797076
0.49656 0.8186016032
0.504836 0.82392169944
0.513112 0.829295056015
0.521388 0.834720659608
0.529664 0.840197513477
0.53794 0.845724637538
0.546216 0.851301068412
0.554492 0.856925859449
0.562768 0.862598080725
0.571044 0.868316819015
0.57932 0.874081177742
0.587596 0.879890276909
0.595872 0.885743253009
0.604148 0.891639258919
0.612424 0.897577463778
0.6207 0.90355705285
0.628976 0.909577227372
0.637252 0.915637204395
0.645528 0.921736216607
0.653804 0.927873512154
0.66208 0.934048354446
0.670356 0.940260021957
0.678632 0.946507808022
0.686908 0.952791020622
0.695184 0.959108982167
0.70346 0.965461029278
0.711736 0.971846512558
0.720012 0.978264796366
0.728288 0.984715258587
0.736564 0.991197290399
0.74484 0.997710296041
0.753116 1.00425369258
0.761392 1.01082690966
0.769668 1.01742938931
0.777944 1.02406058566
0.78622 1.03071996475
0.794496 1.03740700426
0.802772 1.04412119331
0.811048 1.05086203222
0.819324 1.05762903229
0.8276 1.06442171558
0.835876 1.07123961464
0.844152 1.07808227238
0.852428 1.08494924178
0.860704 1.09184008568
0.86898 1.09875437663
0.877256 1.10569169662
0.885532 1.11265163689
0.893808 1.11963379775
0.902084 1.12663778837
0.91036 1.13366322656
0.918636 1.14070973864
0.926912 1.14777695919
0.935188 1.15486453089
0.943464 1.16197210434
0.95174 1.1690993379
0.960016 1.17624589749
0.968292 1.18341145641
0.976568 1.19059569521
0.984844 1.1977983015
0.99312 1.20501896981
1.001396 1.21225740141
1.009672 1.21951330416
1.017948 1.22678639238
1.026224 1.23407638668
1.0345 1.24138301384
1.042776 1.24870600664
1.051052 1.25604510376
1.059328 1.2634000496
1.067604 1.27077059419
1.07588 1.27815649304
1.084156 1.28555750702
1.092432 1.29297340225
1.100708 1.30040394995
1.108984 1.30784892636
1.11726 1.3153081126
1.125536 1.32278129456
1.133812 1.33026826282
1.142088 1.33776881251
1.150364 1.34528274321
1.15864 1.35280985889
1.166916 1.36034996775
1.175192 1.36790288217
1.183468 1.37546841861
1.191744 1.3830463975
1.20002 1.39063664315
1.208296 1.3982389837
1.216572 1.405853251
1.224848 1.41347928052
1.233124 1.42111691131
1.2414 1.42876598589
1.249676 1.43642635018
1.257952 1.44409785342
1.266228 1.45178034813
1.274504 1.45947368998
1.28278 1.46717773778
1.291056 1.47489235336
1.299332 1.48261740155
1.307608 1.49035275009
1.315884 1.49809826958
1.32416 1.5058538334
1.332436 1.51361931768
1.340712 1.52139460119
1.348988 1.52917956537
1.357264 1.53697409417
1.36554 1.5447780741
1.373816 1.55259139407
1.382092 1.56041394546
1.390368 1.56824562195
1.398644 1.57608631957
1.40692 1.58393593657
1.415196 1.59179437345
1.423472 1.59966153286
1.431748 1.60753731957
1.440024 1.61542164046
1.4483 1.62331440443
1.456576 1.63121552236
1.464852 1.63912490714
1.473128 1.64704247355
1.481404 1.65496813825
1.48968 1.66290181976
1.497956 1.67084343841
1.506232 1.67879291632
1.514508 1.68675017732
1.522784 1.69471514698
1.53106 1.70268775254
1.539336 1.71066792287
1.547612 1.71865558849
1.555888 1.72665068147
1.564164 1.73465313546
1.57244 1.74266288563
1.580716 1.75067986864
1.588992 1.75870402265
1.597268 1.76673528724
1.605544 1.77477360343
1.61382 1.78281891363
1.622096 1.79087116161
1.630372 1.79893029252
1.638648 1.8069962528
1.646924 1.81506899022
1.6552 1.82314845382
1.663476 1.8312345939
1.671752 1.839327362
1.680028 1.84742671088
1.688304 1.85553259449
1.69658 1.86364496797
1.704856 1.87176378763
1.713132 1.8798890109
1.721408 1.88802059634
1.729684 1.89615850364
1.73796 1.90430269355
1.746236 1.91245312791
1.754512 1.92060976962
1.762788 1.92877258263
1.771064 1.93694153189
1.77934 1.9451165834
1.787616 1.95329770412
1.795892 1.96148486202
1.804168 1.96967802605
1.812444 1.97787716608
1.82072 1.98608225297
1.828996 1.99429325848
1.837272 2.0025101553
1.845548 2.01073291704
1.853824 2.0189615182
1.8621 2.02719593415
1.870376 2.03543614117
1.878652 2.04368211637
1.886928 2.05193383774
1.895204 2.06019128411
1.90348 2.06845443513
1.911756 2.07672327129
1.920032 2.0849977739
1.928308 2.09327792508
1.936584 2.10156370773
1.94486 2.10985510557
1.953136 2.11815210308
1.961412 2.12645468553
1.969688 2.13476283895
1.977964 2.14307655015
1.98624 2.15139580668
1.994516 2.15972059684
2.002792 2.16805090968
2.011068 2.17638673497
2.019344 2.18472806322
2.02762 2.19307488568
2.035896 2.20142719428
2.044172 2.20978498171
2.052448 2.21814824133
2.060724 2.22651696722
2.069 2.23489115417
2.077276 2.24327079764
2.085552 2.25165589379
2.093828 2.26004643949
2.102104 2.26844243226
2.11038 2.2768438703
2.118656 2.28525075252
2.126932 2.29366307847
2.135208 2.30208084837
2.143484 2.31050406313
2.15176 2.3189327243
2.160036 2.3273668341
2.168312 2.33580639541
2.176588 2.34425141178
2.184864 2.35270188739
2.19314 2.36115782708
2.201416 2.36961923636
2.209692 2.37808612137
2.217968 2.3865584889
2.226244 2.39503634641
2.23452 2.40351970198
2.242796 2.41200856436
2.251072 2.42050294291
2.259348 2.42900284769
2.267624 2.43750828935
2.2759 2.44601927922
2.284176 2.45453582927
2.292452 2.4630579521
2.300728 2.47158566097
2.309004 2.48011896979
2.31728 2.48865789311
2.325556 2.49720244612
2.333832 2.50575264468
2.342108 2.51430850528
2.350384 2.52287004509
2.35866 2.53143728189
2.366936 2.54001023417
2.375212 2.54858892102
2.383488 2.55717336224
2.391764 2.56576357827
2.40004 2.5743595902
2.408316 2.58296141982
2.416592 2.59156908956
2.424868 2.60018262253
2.433144 2.60880204254
2.44142 2.61742737403
2.449696 2.62605864218
2.457972 2.63469587281
2.466248 2.64333909245
2.474524 2.65198832832
2.4828 2.66064360833
2.491076 2.66930496112
2.499352 2.67797241601
2.507628 2.68664600302
2.515904 2.69532575293
2.52418 2.7040116972
2.532456 2.71270386803
2.540732 2.72140229836
2.549008 2.73010702186
2.557284 2.73881807294
2.56556 2.74753548676
2.573836 2.75625929924
2.582112 2.76498954706
2.590388 2.77372626766
2.598664 2.78246949927
2.60694 2.79121928088
2.615216 2.79997565229
2.623492 2.80873865409
2.631768 2.81750832766
2.640044 2.82628471521
2.64832 2.83506785976
2.656596 2.84385780516
2.664872 2.85265459609
2.673148 2.86145827809
2.681424 2.87026889754
2.6897 2.87908650168
2.697976 2.88791113863
2.706252 2.89674285739
2.714528 2.90558170786
2.722804 2.91442774083
2.73108 2.923281008
2.739356 2.932141562
2.747632 2.9410094564
2.755908 2.9498847457
2.764184 2.95876748537
2.77246 2.96765773183
2.780736 2.97655554249
2.789012 2.98546097577
2.797288 2.99437409107
2.805564 3.00329494881
2.81384 3.01222361046
2.822116 3.02116013851
2.830392 3.03010459652
2.838668 3.03905704913
2.846944 3.04801756206
2.85522 3.05698620212
2.863496 3.06596303726
2.871772 3.07494813655
2.880048 3.0839415702
2.888324 3.09294340961
2.8966 3.10195372733
2.904876 3.11097259714
2.913152 3.12000009401
2.921428 3.12903629415
2.929704 3.13808127504
2.93798 3.14713511541
2.946256 3.15619789529
2.954532 3.16526969601
2.962808 3.17435060025
2.971084 3.18344069201
2.97936 3.19254005669
2.987636 3.20164878106
2.995912 3.21076695333
3.004188 3.21989466312
3.012464 3.22903200152
3.02074 3.23817906111
3.029016 3.24733593597
3.037292 3.25650272171
3.045568 3.26567951552
3.053844 3.27486641614
3.06212 3.28406352394
3.070396 3.29327094092
3.078672 3.30248877075
3.086948 3.31171711879
3.095224 3.32095609212
3.1035 3.33020579957
3.111776 3.33946635177
3.120052 3.34873786113
3.128328 3.35802044194
3.136604 3.36731421034
3.14488 3.3766192844
3.153156 3.38593578413
3.161432 3.39526383152
3.169708 3.40460355057
3.177984 3.41395506736
3.18626 3.42331851002
3.194536 3.43269400885
3.202812 3.44208169629
3.211088 3.45148170702
3.219364 3.46089417794
3.22764 3.47031924826
3.235916 3.47975705955
3.244192 3.48920775572
3.252468 3.49867148315
3.260744 3.50814839067
3.26902 3.51763862965
3.277296 3.52714235404
3.285572 3.53665972039
3.293848 3.54619088795
3.302124 3.55573601871
3.3104 3.56529527742
3.318676 3.57486883169
3.326952 3.58445685204
3.335228 3.59405951192
3.343504 3.60367698784
3.35178 3.61330945936
3.360056 3.62295710922
3.368332 3.63262012336
3.376608 3.64229869099
3.384884 3.65199300469
3.39316 3.66170326047
3.401436 3.67142965781
3.409712 3.6811723998
3.417988 3.69093169315
3.426264 3.70070774833
3.43454 3.71050077958
3.442816 3.7203110051
3.451092 3.73013864701
3.459368 3.73998393156
3.467644 3.74984708912
3.47592 3.75972835435
3.484196 3.76962796627
3.492472 3.77954616833
3.500748 3.78948320857
3.509024 3.79943933968
3.5173 3.80941481914
3.525576 3.8194099093
3.533852 3.82942487755
3.542128 3.83945999635
3.550404 3.84951554347
3.55868 3.85959180201
3.566956 3.86968906058
3.575232 3.87980761345
3.583508 3.88994776065
3.591784 3.90010980814
3.60006 3.91029406794
3.608336 3.92050085832
3.616612 3.93073050388
3.624888 3.94098333581
3.633164 3.95125969199
3.64144 3.96155991716
3.649716 3.97188436316
3.657992 3.98223338905
3.666268 3.99260736133
3.674544 4.00300665413
3.68282 4.01343164943
3.691096 4.02388273723
3.699372 4.03436031583
3.707648 4.04486479199
3.715924 4.0553965812
3.7242 4.06595610791
3.732476 4.0765438058
3.740752 4.08716011799
3.749028 4.09780549737
3.757304 4.10848040682
3.76558 4.11918531952
3.773856 4.12992071927
3.782132 4.14068710077
3.790408 4.15148496991
3.798684 4.16231484419
3.80696 4.17317725297
3.815236 4.18407273789
3.823512 4.19500185319
3.831788 4.20596516615
3.840064 4.21696325744
3.84834 4.22799672154
3.856616 4.23906616723
3.864892 4.25017221793
3.873168 4.26131551228
3.881444 4.27249670452
3.88972 4.28371646509
3.897996 4.29497548107
3.906272 4.30627445678
3.914548 4.31761411432
3.922824 4.32899519417
3.9311 4.34041845583
3.939376 4.35188467839
3.947652 4.36339466131
3.955928 4.37494922501
3.964204 4.38654921167
3.97248 4.39819548597
3.980756 4.40988893586
3.989032 4.42163047345
3.997308 4.43342103583
4.005584 4.44526158597
4.01386 4.45715311372
4.022136 4.46909663675
4.030412 4.48109320164
4.038688 4.49314388492
4.046964 4.50524979424
4.05524 4.51741206958
4.063516 4.52963188447
4.071792 4.54191044732
4.080068 4.55424900282
4.088344 4.56664883337
4.09662 4.5791112606
4.104896 4.59163764701
4.113172 4.60422939761
4.121448 4.61688796174
4.129724 4.62961483489


==> figuresAndData/dataForRayleigh-upperEnd-sigma2prob0pt1.tex <==
0.0 0.918087210053
0.00856 0.918131548535
0.01712 0.918264551407
0.02568 0.918486180962
0.03424 0.91879637442
0.0428 0.919195044011
0.05136 0.919682077111
0.05992 0.920257336397
0.06848 0.920920660047
0.07704 0.921671861972
0.0856 0.922510732081
0.09416 0.923437036577
0.10272 0.924450518291
0.11128 0.925550897035
0.11984 0.926737869998
0.1284 0.928011112163
0.13696 0.929370276749
0.14552 0.930814995681
0.15408 0.932344880091
0.16264 0.933959520828
0.1712 0.935658488998
0.17976 0.937441336525
0.18832 0.939307596725
0.19688 0.941256784896
0.20544 0.943288398928
0.214 0.945401919922
0.22256 0.947596812819
0.23112 0.949872527045
0.23968 0.952228497157
0.24824 0.954664143501
0.2568 0.957178872869
0.26536 0.959772079169
0.27392 0.962443144087
0.28248 0.965191437754
0.29104 0.968016319412
0.2996 0.970917138082
0.30816 0.973893233214
0.31672 0.976943935355
0.32528 0.980068566785
0.33384 0.983266442172
0.3424 0.986536869194
0.35096 0.989879149175
0.35952 0.993292577689
0.36808 0.996776445175
0.37664 1.00033003752
0.3852 1.00395263664
0.39376 1.00764352106
0.40232 1.01140196645
0.41088 1.01522724617
0.41944 1.01911863178
0.428 1.02307539361
0.43656 1.02709680115
0.44512 1.03118212363
0.45368 1.03533063043
0.46224 1.03954159152
0.4708 1.04381427792
0.47936 1.0481479621
0.48792 1.05254191837
0.49648 1.05699542329
0.50504 1.06150775599
0.5136 1.06607819856
0.52216 1.07070603636
0.53072 1.07539055836
0.53928 1.0801310574
0.54784 1.08492683054
0.5564 1.08977717927
0.56496 1.0946814098
0.57352 1.09963883328
0.58208 1.10464876608
0.59064 1.10971052992
0.5992 1.11482345214
0.60776 1.11998686586
0.61632 1.12520011015
0.62488 1.13046253021
0.63344 1.1357734775
0.642 1.14113230986
0.65056 1.1465383917
0.65912 1.15199109405
0.66768 1.1574897947
0.67624 1.16303387827
0.6848 1.16862273631
0.69336 1.17425576739
0.70192 1.17993237712
0.71048 1.18565197824
0.71904 1.19141399068
0.7276 1.19721784156
0.73616 1.20306296526
0.74472 1.20894880342
0.75328 1.21487480498
0.76184 1.22084042616
0.7704 1.2268451305
0.77896 1.23288838886
0.78752 1.23896967937
0.79608 1.24508848746
0.80464 1.25124430583
0.8132 1.25743663444
0.82176 1.26366498047
0.83032 1.26992885829
0.83888 1.27622778942
0.84744 1.28256130252
0.856 1.28892893334
0.86456 1.29533022464
0.87312 1.30176472618
0.88168 1.30823199468
0.89024 1.31473159371
0.8988 1.32126309371
0.90736 1.32782607188
0.91592 1.33442011211
0.92448 1.341044805
0.93304 1.34769974768
0.9416 1.35438454386
0.95016 1.36109880367
0.95872 1.36784214366
0.96728 1.3746141867
0.97584 1.38141456191
0.9844 1.38824290461
0.99296 1.39509885623
1.00152 1.40198206424
1.01008 1.4088921821
1.01864 1.41582886916
1.0272 1.4227917906
1.03576 1.42978061737
1.04432 1.43679502608
1.05288 1.44383469898
1.06144 1.45089932384
1.07 1.45798859391
1.07856 1.46510220782
1.08712 1.47223986954
1.09568 1.47940128827
1.10424 1.4865861784
1.1128 1.49379425944
1.12136 1.5010252559
1.12992 1.50827889729
1.13848 1.515554918
1.14704 1.52285305726
1.1556 1.53017305905
1.16416 1.53751467203
1.17272 1.54487764951
1.18128 1.55226174933
1.18984 1.55966673383
1.1984 1.56709236978
1.20696 1.5745384283
1.21552 1.58200468482
1.22408 1.589490919
1.23264 1.59699691465
1.2412 1.60452245972
1.24976 1.6120673462
1.25832 1.61963137007
1.26688 1.62721433122
1.27544 1.63481603344
1.284 1.64243628433
1.29256 1.65007489523
1.30112 1.65773168122
1.30968 1.66540646098
1.31824 1.67309905682
1.3268 1.6808092946
1.33536 1.68853700362
1.34392 1.69628201668
1.35248 1.70404416992
1.36104 1.71182330284
1.3696 1.71961925824
1.37816 1.72743188213
1.38672 1.73526102375
1.39528 1.74310653547
1.40384 1.75096827276
1.4124 1.75884609417
1.42096 1.76673986124
1.42952 1.77464943849
1.43808 1.7825746934
1.44664 1.79051549629
1.4552 1.79847172037
1.46376 1.80644324164
1.47232 1.81442993889
1.48088 1.8224316936
1.48944 1.83044839001
1.498 1.83847991496
1.50656 1.84652615794
1.51512 1.85458701105
1.52368 1.8626623689
1.53224 1.87075212866
1.5408 1.87885618996
1.54936 1.8869744549
1.55792 1.89510682802
1.56648 1.90325321623
1.57504 1.91141352882
1.5836 1.9195876774
1.59216 1.92777557592
1.60072 1.93597714057
1.60928 1.94419228981
1.61784 1.95242094435
1.6264 1.96066302705
1.63496 1.968918463
1.64352 1.97718717939
1.65208 1.98546910558
1.66064 1.99376417301
1.6692 2.0020723152
1.67776 2.01039346773
1.68632 2.01872756824
1.69488 2.02707455635
1.70344 2.03543437371
1.712 2.04380696393
1.72056 2.05219227257
1.72912 2.06059024715
1.73768 2.0690008371
1.74624 2.07742399375
1.7548 2.08585967033
1.76336 2.09430782193
1.77192 2.1027684055
1.78048 2.11124137982
1.78904 2.11972670552
1.7976 2.12822434502
1.80616 2.13673426253
1.81472 2.14525642408
1.82328 2.15379079745
1.83184 2.16233735217
1.8404 2.17089605953
1.84896 2.17946689256
1.85752 2.18804982603
1.86608 2.19664483639
1.87464 2.20525190183
1.8832 2.21387100223
1.89176 2.22250211916
1.90032 2.23114523586
1.90888 2.23980033728
1.91744 2.24846740998
1.926 2.25714644224
1.93456 2.26583742395
1.94312 2.27454034669
1.95168 2.28325520363
1.96024 2.29198198964
1.9688 2.30072070118
1.97736 2.30947133635
1.98592 2.31823389489
1.99448 2.32700837817
2.00304 2.33579478915
2.0116 2.34459313245
2.02016 2.35340341428
2.02872 2.36222564249
2.03728 2.37105982652
2.04584 2.37990597745
2.0544 2.38876410798
2.06296 2.39763423241
2.07152 2.40651636669
2.08008 2.41541052835
2.08864 2.42431673658
2.0972 2.43323501219
2.10576 2.4421653776
2.11432 2.4511078569
2.12288 2.46006247578
2.13144 2.4690292616
2.14 2.47800824337
2.14856 2.48699945172
2.15712 2.49600291899
2.16568 2.50501867915
2.17424 2.51404676786
2.1828 2.52308722245
2.19136 2.53214008196
2.19992 2.5412053871
2.20848 2.55028318033
2.21704 2.55937350579
2.2256 2.56847640936
2.23416 2.57759193867
2.24272 2.58672014308
2.25128 2.59586107374
2.25984 2.60501478356
2.2684 2.61418132723
2.27696 2.62336076127
2.28552 2.63255314398
2.29408 2.64175853551
2.30264 2.65097699788
2.3112 2.66020859493
2.31976 2.66945339241
2.32832 2.67871145796
2.33688 2.68798286113
2.34544 2.69726767342
2.354 2.70656596826
2.36256 2.71587782107
2.37112 2.72520330927
2.37968 2.73454251228
2.38824 2.74389551157
2.3968 2.75326239066
2.40536 2.76264323518
2.41392 2.77203813283
2.42248 2.78144717349
2.43104 2.79087044916
2.4396 2.80030805406
2.44816 2.80976008461
2.45672 2.81922663947
2.46528 2.82870781959
2.47384 2.83820372821
2.4824 2.84771447091
2.49096 2.85724015565
2.49952 2.86678089276
2.50808 2.87633679503
2.51664 2.88590797773
2.5252 2.8954945586
2.53376 2.90509665797
2.54232 2.91471439871
2.55088 2.92434790633
2.55944 2.93399730901
2.568 2.94366273763
2.57656 2.95334432581
2.58512 2.96304220996
2.59368 2.97275652934
2.60224 2.98248742608
2.6108 2.99223504526
2.61936 3.00199953493
2.62792 3.01178104616
2.63648 3.02157973314
2.64504 3.03139575316
2.6536 3.04122926673
2.66216 3.0510804376
2.67072 3.06094943284
2.67928 3.07083642289
2.68784 3.08074158161
2.6964 3.09066508637
2.70496 3.10060711809
2.71352 3.11056786134
2.72208 3.12054750437
2.73064 3.1305462392
2.7392 3.14056426172
2.74776 3.15060177172
2.75632 3.16065897299
2.76488 3.17073607339
2.77344 3.18083328498
2.782 3.19095082402
2.79056 3.20108891113
2.79912 3.21124777135
2.80768 3.22142763424
2.81624 3.23162873397
2.8248 3.24185130941
2.83336 3.25209560426
2.84192 3.26236186713
2.85048 3.27265035166
2.85904 3.28296131661
2.8676 3.29329502602
2.87616 3.30365174926
2.88472 3.31403176121
2.89328 3.32443534238
2.90184 3.33486277898
2.9104 3.34531436314
2.91896 3.35579039298
2.92752 3.36629117278
2.93608 3.37681701313
2.94464 3.38736823104
2.9532 3.39794515018
2.96176 3.40854810093
2.97032 3.41917742066
2.97888 3.42983345379
2.98744 3.44051655207
2.996 3.45122707468
3.00456 3.46196538846
3.01312 3.47273186811
3.02168 3.48352689636
3.03024 3.49435086421
3.0388 3.50520417113
3.04736 3.51608722527
3.05592 3.52700044373
3.06448 3.53794425275
3.07304 3.54891908799
3.0816 3.55992539476
3.09016 3.57096362832
3.09872 3.58203425412
3.10728 3.59313774807
3.11584 3.60427459691
3.1244 3.6154452984
3.13296 3.62665036175
3.14152 3.63789030786
3.15008 3.6491656697
3.15864 3.66047699265
3.1672 3.67182483487
3.17576 3.68320976766
3.18432 3.6946323759
3.19288 3.70609325839
3.20144 3.71759302832
3.21 3.72913231369
3.21856 3.74071175779
3.22712 3.75233201965
3.23568 3.76399377453
3.24424 3.77569771446
3.2528 3.78744454876
3.26136 3.79923500459
3.26992 3.81106982754
3.27848 3.82294978223
3.28704 3.83487565293
3.2956 3.84684824422
3.30416 3.8588683817
3.31272 3.87093691263
3.32128 3.88305470676
3.32984 3.89522265703
3.3384 3.90744168045
3.34696 3.91971271888
3.35552 3.93203673994
3.36408 3.94441473794
3.37264 3.95684773484
3.3812 3.96933678126
3.38976 3.98188295752
3.39832 3.99448737477
3.40688 4.00715117613
3.41544 4.01987553791
3.424 4.03266167089
3.43256 4.04551082163
3.44112 4.05842427392
3.44968 4.07140335016
3.45824 4.08444941301
3.4668 4.09756386693
3.47536 4.11074815992
3.48392 4.12400378531
3.49248 4.13733228365
3.50104 4.15073524467
3.5096 4.1642143094
3.51816 4.17777117238
3.52672 4.19140758397
3.53528 4.20512535281
3.54384 4.2189263484
3.5524 4.23281250387
3.56096 4.24678581887
3.56952 4.26084836259
3.57808 4.27500227706
3.58664 4.28924978055
3.5952 4.30359317125
3.60376 4.31803483108
3.61232 4.33257722983
3.62088 4.34722292949
3.62944 4.36197458894
3.638 4.37683496878
3.64656 4.39180693667
3.65512 4.40689347286
3.66368 4.4220976762
3.67224 4.43742277045
3.6808 4.45287211113
3.68936 4.46844919278
3.69792 4.48415765671
3.70648 4.50000129938
3.71504 4.51598408132
3.7236 4.53211013675
3.73216 4.54838378386
3.74072 4.56480953593
3.74928 4.58139211329
3.75784 4.59813645618
3.7664 4.61504773867
3.77496 4.63213138369
3.78352 4.64939307928
3.79208 4.66683879624
3.80064 4.68447480722
3.8092 4.70230770751
3.81776 4.72034443759
3.82632 4.73859230782
3.83488 4.75705902524
3.84344 4.77575272297
3.852 4.79468199233
3.86056 4.8138559181
3.86912 4.83328411724
3.87768 4.8529767815
3.88624 4.87294472437
3.8948 4.89319943308
3.90336 4.91375312598
3.91192 4.93461881636
3.92048 4.95581038338
3.92904 4.97734265103
3.9376 4.99923147653
3.94616 5.02149384921
3.95472 5.04414800166
3.96328 5.0672135349
3.97184 5.09071155981
3.9804 5.11466485736
3.98896 5.1390980609
3.99752 5.164037864
4.00608 5.18951325857
4.01464 5.21555580849
4.0232 5.24219996552
4.03176 5.2694834354
4.04032 5.29744760431
4.04888 5.3261380378
4.05744 5.35560506781
4.066 5.38590448698
4.07456 5.41709837495
4.08312 5.44925608791
4.09168 5.48245545192
4.10024 5.51678421269
4.1088 5.55234181129
4.11736 5.58924157799
4.12592 5.62761346892
4.13448 5.66760751571
4.14304 5.70939822411
4.1516 5.75319025456
4.16016 5.79922586283
4.16872 5.84779480106
4.17728 5.89924772954
4.18584 5.95401475412
4.1944 6.01263164623
4.20296 6.07577793231
4.21152 6.14433397835
4.22008 6.21946976626
4.22864 6.30278925457
4.2372 6.39657838242
4.24576 6.50426177906
4.25432 6.63132393347
4.26288 6.78741494
4.27144 6.99214594989


==> figuresAndData/dataForSingleLaplace-conditionalMean-lambda1.tex <==
0.0 0.484011655289
0.0069908289012 0.496075388345
0.0139816578024 0.508220129963
0.0209724867036 0.520448129349
0.0279633156048 0.532761738418
0.034954144506 0.545163418632
0.0419449734072 0.557655748446
0.0489358023084 0.570241431442
0.0559266312096 0.582923305208
0.0629174601108 0.595704351067
0.069908289012 0.608587704758
0.0768991179132 0.621576668172
0.0838899468144 0.634674722298
0.0908807757156 0.64788554152
0.0978716046168 0.661213009451
0.104862433518 0.674661236511
0.111853262419 0.688234579511
0.11884409132 0.701937663498
0.125834920222 0.715775406241
0.132825749123 0.729753045728
0.139816578024 0.74387617117
0.146807406925 0.758150758074
0.153798235826 0.772583208081
0.160789064728 0.787180394386
0.167779893629 0.801949713767
0.17477072253 0.816899146436
0.181761551431 0.832037325257
0.188752380332 0.847373616207
0.195743209234 0.862918212453
0.202734038135 0.878682245028
0.209724867036 0.894677913932
0.216715695937 0.910918644547
0.223706524838 0.927419275766
0.23069735374 0.944196288265
0.237688182641 0.961268084154
0.244679011542 0.978655333278
0.251669840443 0.996381407176
0.258660669344 1.01447293019
0.265651498246 1.03296048993
0.272642327147 1.05187956905
0.279633156048 1.07127179135
0.286623984949 1.09118662668
0.29361481385 1.11168378656
0.300605642752 1.13283669912
0.307596471653 1.15473774764
0.314587300554 1.17750655365
0.321578129455 1.20130389618
0.328568958356 1.22635706317
0.335559787258 1.25301151686
0.342550616159 1.28185574633


==> figuresAndData/dataForSingleLaplace-conditionalMean-lambda1prob0pt5.tex <==
0.0 0.30685281944
0.013585684739 0.325743799658
0.0271713694779 0.344751622427
0.0407570542169 0.363880012679
0.0543427389559 0.383132874209
0.0679284236949 0.402514301906
0.0815141084338 0.422028595084
0.0950997931728 0.441680272047
0.108685477912 0.461474086033
0.122271162651 0.481415042708
0.13585684739 0.501508419375
0.149442532129 0.521759786148
0.163028216868 0.542175029313
0.176613901607 0.562760377176
0.190199586346 0.583522428734
0.203785271085 0.604468185558
0.217370955824 0.625605087344
0.230956640563 0.646941051661
0.244542325302 0.668484518548
0.258128010041 0.690244500687
0.271713694779 0.71223064005
0.285299379518 0.734453272104
0.298885064257 0.756923498825
0.312470748996 0.779653272107
0.326056433735 0.802655489433
0.339642118474 0.825944104133
0.353227803213 0.849534253094
0.366813487952 0.873442405463
0.380399172691 0.897686536804
0.39398485743 0.922286334343
0.407570542169 0.947263440483
0.421156226908 0.972641743855
0.434741911647 0.998447729991
0.448327596386 1.02471090755
0.461913281125 1.05146433145
0.475498965864 1.07874525177
0.489084650603 1.10659592845
0.502670335342 1.13506466776
0.516256020081 1.16420716097
0.52984170482 1.1940882433
0.543427389559 1.22478425063
0.557013074298 1.25638625014
0.570598759037 1.28900458861
0.584184443776 1.32277550276
0.597770128515 1.35787110428
0.611355813254 1.39451520002
0.624941497993 1.43300993132
0.638527182732 1.47378439486
0.652112867471 1.51749394376
0.66569855221 1.56526069445


==> figuresAndData/dataForSingleLaplace-conditionalMean-lambda1prob0pt75.tex <==
0.0 0.537901879627
0.00563856862005 0.548358668405
0.0112771372401 0.558885674637
0.0169157058602 0.569484782273
0.0225542744802 0.580157960215
0.0281928431003 0.590907267935
0.0338314117203 0.6017348616
0.0394699803404 0.612643000739
0.0451085489604 0.62363405554
0.0507471175805 0.634710514833
0.0563856862005 0.645874994845
0.0620242548206 0.657130248832
0.0676628234407 0.66847917769
0.0733013920607 0.679924841663
0.0789399606808 0.691470473325
0.0845785293008 0.70311949197
0.0902170979209 0.714875519639
0.0958556665409 0.726742399005
0.101494235161 0.738724213399
0.107132803781 0.750825309292
0.112771372401 0.763050321646
0.118409941021 0.775404202571
0.124048509641 0.787892253862
0.129687078261 0.8005201641
0.135325646881 0.813294051105
0.140964215501 0.826220510785
0.146602784121 0.839306673589
0.152241352741 0.852560270109
0.157879921362 0.865989707757
0.163518489982 0.879604160944
0.169157058602 0.893413677841
0.174795627222 0.907429307724
0.180434195842 0.921663254074
0.186072764462 0.936129060267
0.191711333082 0.950841836979
0.197349901702 0.965818543673
0.202988470322 0.981078341196
0.208627038942 0.996643039388
0.214265607562 1.01253767389
0.219904176182 1.0287912623
0.225542744802 1.04543781503
0.231181313422 1.06251771773
0.236819882042 1.08007967307
0.242458450662 1.09818351603
0.248097019282 1.11690445637
0.253735587902 1.13633978374
0.259374156523 1.15662013038
0.265012725143 1.17792997499
0.270651293763 1.20054941002
0.276289862383 1.2249550274


==> figuresAndData/dataForSingleLaplace-conditionalMean-lambda1prob0pt85.tex <==
0.0 0.665214120314
0.00318537101816 0.672346248907
0.00637074203631 0.679524479528
0.00955611305447 0.686749960165
0.0127414840726 0.694023889198
0.0159268550908 0.701347518684
0.0191122261089 0.708722157943
0.0222975971271 0.716149177451
0.0254829681453 0.723630013102
0.0286683391634 0.731166170867
0.0318537101816 0.738759231901
0.0350390811997 0.746410858159
0.0382244522179 0.75412279857
0.041409823236 0.761896895859
0.0445951942542 0.769735094096
0.0477805652723 0.777639447057
0.0509659362905 0.78561212754
0.0541513073087 0.793655437743
0.0573366783268 0.801771820881
0.060522049345 0.809963874222
0.0637074203631 0.818234363767
0.0668927913813 0.826586240846
0.0700781623994 0.835022660936
0.0732635334176 0.843547005107
0.0764489044358 0.852162904551
0.0796342754539 0.860874268776
0.0828196464721 0.869685318174
0.0860050174902 0.878600621835
0.0891903885084 0.887625141716
0.0923757595265 0.896764284551
0.0955611305447 0.906023963255
0.0987465015628 0.915410670123
0.101931872581 0.924931564762
0.105117243599 0.934594580664
0.108302614617 0.94440855563
0.111487985635 0.954383393077
0.114673356654 0.964530263962
0.117858727672 0.974861862909
0.12104409869 0.98539273803
0.124229469708 0.996139722952
0.127414840726 1.00712251394
0.130600211744 1.01836445855
0.133785582763 1.0298936625
0.136970953781 1.04174459327
0.140156324799 1.05396049464
0.143341695817 1.06659719987
0.146527066835 1.07972953153
0.149712437853 1.09346294299
0.152897808872 1.10795721286
0.15608317989 1.12348362781


==> figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1.tex <==
0.0 0.484011655289
0.0069908289012 0.484011655289
0.0139816578024 0.484011655289
0.0209724867036 0.484011655289
0.0279633156048 0.484011655289
0.034954144506 0.484011655289
0.0419449734072 0.484011655289
0.0489358023084 0.484011655289
0.0559266312096 0.484011655289
0.0629174601108 0.484011655289
0.069908289012 0.489245099459
0.0768991179132 0.499502303469
0.0838899468144 0.509790905262
0.0908807757156 0.520111639781
0.0978716046168 0.530465293538
0.104862433518 0.540852709976
0.111853262419 0.551274795506
0.11884409132 0.561732526334
0.125834920222 0.572226956189
0.132825749123 0.58275922511
0.139816578024 0.593330569459
0.146807406925 0.603942333372
0.153798235826 0.614595981909
0.160789064728 0.625293116215
0.167779893629 0.636035491056
0.17477072253 0.646825035216
0.181761551431 0.657663875329
0.188752380332 0.668554363866
0.195743209234 0.679499112197
0.202734038135 0.690501029879
0.209724867036 0.701563371678
0.216715695937 0.712689794231
0.223706524838 0.723884424899
0.23069735374 0.735151946161
0.237688182641 0.746497700063
0.244679011542 0.757927818902
0.251669840443 0.769449390687
0.258660669344 0.781070671494
0.265651498246 0.792801362146
0.272642327147 0.80465297501
0.279633156048 0.816639329978
0.286623984949 0.828777240724
0.29361481385 0.841087490197
0.300605642752 0.85359626249
0.307596471653 0.866337328008
0.314587300554 0.879355542931
0.321578129455 0.892712808453
0.328568958356 0.906499077532
0.335559787258 0.920855123724
0.342550616159 0.936028467717


==> figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1prob0pt5.tex <==
0.0 0.30685281944
0.013585684739 0.30685281944
0.0271713694779 0.30685281944
0.0407570542169 0.322826487276
0.0543427389559 0.340546682936
0.0679284236949 0.358330362932
0.0815141084338 0.376178593432
0.0950997931728 0.394092467349
0.108685477912 0.412073106348
0.122271162651 0.430121663125
0.13585684739 0.448239324032
0.149442532129 0.466427312083
0.163028216868 0.484686890418
0.176613901607 0.503019366299
0.190199586346 0.521426095727
0.203785271085 0.539908488785
0.217370955824 0.558468015845
0.230956640563 0.577106214781
0.244542325302 0.595824699386
0.258128010041 0.614625169198
0.271713694779 0.633509421015
0.285299379518 0.652479362425
0.298885064257 0.671537027735
0.312470748996 0.690684596808
0.326056433735 0.709924417382
0.339642118474 0.72925903164
0.353227803213 0.748691207952
0.366813487952 0.768223978954
0.380399172691 0.78786068747
0.39398485743 0.807605042155
0.407570542169 0.827461185327
0.421156226908 0.84743377618
0.434741911647 0.8675280936
0.448327596386 0.887750164196
0.461913281125 0.908106923179
0.475498965864 0.928606418501
0.489084650603 0.949258072849
0.502670335342 0.970073024171
0.516256020081 0.991064574785
0.52984170482 1.01224879363
0.543427389559 1.03364533969
0.557013074298 1.05527861339
0.570598759037 1.07717941024
0.584184443776 1.09938737266
0.597770128515 1.12195476909
0.611355813254 1.14495260686
0.624941497993 1.16848114782
0.638527182732 1.19268953575
0.652112867471 1.21781685047
0.66569855221 1.2442941738


==> figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1prob0pt75.tex <==
0.0 0.537901879627
0.00563856862005 0.537901879627
0.0112771372401 0.537901879627
0.0169157058602 0.537901879627
0.0225542744802 0.537901879627
0.0281928431003 0.537901879627
0.0338314117203 0.537901879627
0.0394699803404 0.537901879627
0.0451085489604 0.537901879627
0.0507471175805 0.537901879627
0.0563856862005 0.537901879627
0.0620242548206 0.537901879627
0.0676628234407 0.537901879627
0.0733013920607 0.537901879627
0.0789399606808 0.537901879627
0.0845785293008 0.545256752409
0.0902170979209 0.553880075434
0.0958556665409 0.562532559225
0.101494235161 0.571215184589
0.107132803781 0.579929011551
0.112771372401 0.588675188118
0.118409941021 0.597454960273
0.124048509641 0.606269683424
0.129687078261 0.615120835553
0.135325646881 0.624010032395
0.140964215501 0.632939045046
0.146602784121 0.641909820472
0.152241352741 0.650924505546
0.157879921362 0.659985475369
0.163518489982 0.66909536685
0.169157058602 0.678257118798
0.174795627222 0.687474020133
0.180434195842 0.696749768345
0.186072764462 0.706088540988
0.191711333082 0.715495083989
0.197349901702 0.724974821912
0.202988470322 0.734533997285
0.208627038942 0.744179849052
0.214265607562 0.753920844631
0.219904176182 0.763766986937
0.225542744802 0.773730228715
0.231181313422 0.783825044678
0.236819882042 0.794069243112
0.242458450662 0.804485154723
0.248097019282 0.815101443038
0.253735587902 0.825955997306
0.259374156523 0.837100847465
0.265012725143 0.848611220123
0.270651293763 0.860604223466
0.276289862383 0.873284612311


==> figuresAndData/dataForSingleLaplace-conditionalMeanCentered-lambda1prob0pt85.tex <==
0.0 0.665214120314
0.00318537101816 0.665214120314
0.00637074203631 0.665214120314
0.00955611305447 0.665214120314
0.0127414840726 0.665214120314
0.0159268550908 0.665214120314
0.0191122261089 0.665214120314
0.0222975971271 0.665214120314
0.0254829681453 0.665214120314
0.0286683391634 0.665214120314
0.0318537101816 0.665214120314
0.0350390811997 0.665214120314
0.0382244522179 0.665214120314
0.041409823236 0.665214120314
0.0445951942542 0.665214120314
0.0477805652723 0.665214120314
0.0509659362905 0.665214120314
0.0541513073087 0.665214120314
0.0573366783268 0.665214120314
0.060522049345 0.665214120314
0.0637074203631 0.665214120314
0.0668927913813 0.665214120314
0.0700781623994 0.665214120314
0.0732635334176 0.665214120314
0.0764489044358 0.665214120314
0.0796342754539 0.665214120314
0.0828196464721 0.665214120314
0.0860050174902 0.665214120314
0.0891903885084 0.665214120314
0.0923757595265 0.665214120314
0.0955611305447 0.665214120314
0.0987465015628 0.665214120314
0.101931872581 0.665214120314
0.105117243599 0.665214120314
0.108302614617 0.665214120314
0.111487985635 0.668597139454
0.114673356654 0.674455573811
0.117858727672 0.680373266856
0.12104409869 0.686355795245
0.124229469708 0.692409690705
0.127414840726 0.698542691075
0.130600211744 0.704764085607
0.133785582763 0.711085202796
0.136970953781 0.717520121989
0.140156324799 0.724086752371
0.143341695817 0.730808549421
0.146527066835 0.737717417545
0.149712437853 0.744859032021
0.152897808872 0.752303762103
0.15608317989 0.7601732722


==> figuresAndData/dataForSingleLaplace-leftEnd-lambda1.tex <==
0.0 0.0
0.0069908289012 0.0069908289012
0.0139816578024 0.0139816578024
0.0209724867036 0.0209724867036
0.0279633156048 0.0279633156048
0.034954144506 0.034954144506
0.0419449734072 0.0419449734072
0.0489358023084 0.0489358023084
0.0559266312096 0.0559266312096
0.0629174601108 0.0629174601108
0.069908289012 0.069908289012
0.0768991179132 0.0768991179132
0.0838899468144 0.0838899468144
0.0908807757156 0.0908807757156
0.0978716046168 0.0978716046168
0.104862433518 0.104862433518
0.111853262419 0.111853262419
0.11884409132 0.11884409132
0.125834920222 0.125834920222
0.132825749123 0.132825749123
0.139816578024 0.139816578024
0.146807406925 0.146807406925
0.153798235826 0.153798235826
0.160789064728 0.160789064728
0.167779893629 0.167779893629
0.17477072253 0.17477072253
0.181761551431 0.181761551431
0.188752380332 0.188752380332
0.195743209234 0.195743209234
0.202734038135 0.202734038135
0.209724867036 0.209724867036
0.216715695937 0.216715695937
0.223706524838 0.223706524838
0.23069735374 0.23069735374
0.237688182641 0.237688182641
0.244679011542 0.244679011542
0.251669840443 0.251669840443
0.258660669344 0.258660669344
0.265651498246 0.265651498246
0.272642327147 0.272642327147
0.279633156048 0.279633156048
0.286623984949 0.286623984949
0.29361481385 0.29361481385
0.300605642752 0.300605642752
0.307596471653 0.307596471653
0.314587300554 0.314587300554
0.321578129455 0.321578129455
0.328568958356 0.328568958356
0.335559787258 0.335559787258
0.342550616159 0.342550616159


==> figuresAndData/dataForSingleLaplace-leftEnd-lambda1prob0pt5.tex <==
0.0 0.0
0.013585684739 0.013585684739
0.0271713694779 0.0271713694779
0.0407570542169 0.0407570542169
0.0543427389559 0.0543427389559
0.0679284236949 0.0679284236949
0.0815141084338 0.0815141084338
0.0950997931728 0.0950997931728
0.108685477912 0.108685477912
0.122271162651 0.122271162651
0.13585684739 0.13585684739
0.149442532129 0.149442532129
0.163028216868 0.163028216868
0.176613901607 0.176613901607
0.190199586346 0.190199586346
0.203785271085 0.203785271085
0.217370955824 0.217370955824
0.230956640563 0.230956640563
0.244542325302 0.244542325302
0.258128010041 0.258128010041
0.271713694779 0.271713694779
0.285299379518 0.285299379518
0.298885064257 0.298885064257
0.312470748996 0.312470748996
0.326056433735 0.326056433735
0.339642118474 0.339642118474
0.353227803213 0.353227803213
0.366813487952 0.366813487952
0.380399172691 0.380399172691
0.39398485743 0.39398485743
0.407570542169 0.407570542169
0.421156226908 0.421156226908
0.434741911647 0.434741911647
0.448327596386 0.448327596386
0.461913281125 0.461913281125
0.475498965864 0.475498965864
0.489084650603 0.489084650603
0.502670335342 0.502670335342
0.516256020081 0.516256020081
0.52984170482 0.52984170482
0.543427389559 0.543427389559
0.557013074298 0.557013074298
0.570598759037 0.570598759037
0.584184443776 0.584184443776
0.597770128515 0.597770128515
0.611355813254 0.611355813254
0.624941497993 0.624941497993
0.638527182732 0.638527182732
0.652112867471 0.652112867471
0.66569855221 0.66569855221


==> figuresAndData/dataForSingleLaplace-leftEnd-lambda1prob0pt75.tex <==
0.0 0.0
0.00563856862005 0.00563856862005
0.0112771372401 0.0112771372401
0.0169157058602 0.0169157058602
0.0225542744802 0.0225542744802
0.0281928431003 0.0281928431003
0.0338314117203 0.0338314117203
0.0394699803404 0.0394699803404
0.0451085489604 0.0451085489604
0.0507471175805 0.0507471175805
0.0563856862005 0.0563856862005
0.0620242548206 0.0620242548206
0.0676628234407 0.0676628234407
0.0733013920607 0.0733013920607
0.0789399606808 0.0789399606808
0.0845785293008 0.0845785293008
0.0902170979209 0.0902170979209
0.0958556665409 0.0958556665409
0.101494235161 0.101494235161
0.107132803781 0.107132803781
0.112771372401 0.112771372401
0.118409941021 0.118409941021
0.124048509641 0.124048509641
0.129687078261 0.129687078261
0.135325646881 0.135325646881
0.140964215501 0.140964215501
0.146602784121 0.146602784121
0.152241352741 0.152241352741
0.157879921362 0.157879921362
0.163518489982 0.163518489982
0.169157058602 0.169157058602
0.174795627222 0.174795627222
0.180434195842 0.180434195842
0.186072764462 0.186072764462
0.191711333082 0.191711333082
0.197349901702 0.197349901702
0.202988470322 0.202988470322
0.208627038942 0.208627038942
0.214265607562 0.214265607562
0.219904176182 0.219904176182
0.225542744802 0.225542744802
0.231181313422 0.231181313422
0.236819882042 0.236819882042
0.242458450662 0.242458450662
0.248097019282 0.248097019282
0.253735587902 0.253735587902
0.259374156523 0.259374156523
0.265012725143 0.265012725143
0.270651293763 0.270651293763
0.276289862383 0.276289862383


==> figuresAndData/dataForSingleLaplace-leftEnd-lambda1prob0pt85.tex <==
0.0 0.0
0.00318537101816 0.00318537101816
0.00637074203631 0.00637074203631
0.00955611305447 0.00955611305447
0.0127414840726 0.0127414840726
0.0159268550908 0.0159268550908
0.0191122261089 0.0191122261089
0.0222975971271 0.0222975971271
0.0254829681453 0.0254829681453
0.0286683391634 0.0286683391634
0.0318537101816 0.0318537101816
0.0350390811997 0.0350390811997
0.0382244522179 0.0382244522179
0.041409823236 0.041409823236
0.0445951942542 0.0445951942542
0.0477805652723 0.0477805652723
0.0509659362905 0.0509659362905
0.0541513073087 0.0541513073087
0.0573366783268 0.0573366783268
0.060522049345 0.060522049345
0.0637074203631 0.0637074203631
0.0668927913813 0.0668927913813
0.0700781623994 0.0700781623994
0.0732635334176 0.0732635334176
0.0764489044358 0.0764489044358
0.0796342754539 0.0796342754539
0.0828196464721 0.0828196464721
0.0860050174902 0.0860050174902
0.0891903885084 0.0891903885084
0.0923757595265 0.0923757595265
0.0955611305447 0.0955611305447
0.0987465015628 0.0987465015628
0.101931872581 0.101931872581
0.105117243599 0.105117243599
0.108302614617 0.108302614617
0.111487985635 0.111487985635
0.114673356654 0.114673356654
0.117858727672 0.117858727672
0.12104409869 0.12104409869
0.124229469708 0.124229469708
0.127414840726 0.127414840726
0.130600211744 0.130600211744
0.133785582763 0.133785582763
0.136970953781 0.136970953781
0.140156324799 0.140156324799
0.143341695817 0.143341695817
0.146527066835 0.146527066835
0.149712437853 0.149712437853
0.152897808872 0.152897808872
0.15608317989 0.15608317989


==> figuresAndData/dataForSingleLaplace-midPoint-lambda1.tex <==
0.0 0.601986402163
0.0069908289012 0.61722949998
0.0139816578024 0.632670450647
0.0209724867036 0.648317493409
0.0279633156048 0.664179387773
0.034954144506 0.680265458256
0.0419449734072 0.696585644037
0.0489358023084 0.713150554195
0.0559266312096 0.729971529291
0.0629174601108 0.747060710197
0.069908289012 0.76443111521
0.0768991179132 0.78209672669
0.0838899468144 0.800072588659
0.0908807757156 0.818374917075
0.0978716046168 0.837021224803
0.104862433518 0.856030463704
0.111853262419 0.87542318673
0.11884409132 0.895221733515
0.125834920222 0.915450443643
0.132825749123 0.936135902742
0.139816578024 0.957307227617
0.146807406925 0.978996398125
0.153798235826 1.00123864529
0.160789064728 1.0240729075
0.167779893629 1.04754236962
0.17477072253 1.07169510388
0.181761551431 1.09658483627
0.188752380332 1.12227186952
0.195743209234 1.14882420231
0.202734038135 1.17631889721
0.209724867036 1.20484376681
0.216715695937 1.23449947111
0.223706524838 1.26540215269
0.23069735374 1.29768678435
0.237688182641 1.33151147339
0.244679011542 1.36706307071
0.251669840443 1.40456459023
0.258660669344 1.44428518828
0.265651498246 1.48655384218
0.272642327147 1.531778506
0.279633156048 1.58047360643
0.286623984949 1.63330065497
0.29361481385 1.69113028467
0.300605642752 1.7551408907
0.307596471653 1.82698330288
0.314587300554 1.90907285225
0.321578129455 2.00514912516
0.328568958356 2.12146535528
0.335559787258 2.26971137305
0.342550616159 2.47600583887


==> figuresAndData/dataForSingleLaplace-midPoint-lambda1prob0pt5.tex <==
0.0 0.34657359028
0.013585684739 0.367045675311
0.0271713694779 0.387710121052
0.0407570542169 0.408575160455
0.0543427389559 0.42964954685
0.0679284236949 0.450942598697
0.0815141084338 0.472464249234
0.0950997931728 0.494225101721
0.108685477912 0.516236491021
0.122271162651 0.538510552425
0.13585684739 0.561060298772
0.149442532129 0.583899707086
0.163028216868 0.607043816175
0.176613901607 0.630508836904
0.190199586346 0.654312277168
0.203785271085 0.678473083982
0.217370955824 0.703011805578
0.230956640563 0.727950776988
0.244542325302 0.753314333327
0.258128010041 0.779129055872
0.271713694779 0.805424057206
0.285299379518 0.832231313088
0.298885064257 0.859586050572
0.312470748996 0.887527204199
0.326056433735 0.916097955128
0.339642118474 0.945346371975
0.353227803213 0.975326177293
0.366813487952 1.00609767047
0.380399172691 1.03772884696
0.39398485743 1.07029676628
0.407570542169 1.10388923807
0.421156226908 1.13860691949
0.434741911647 1.17456595044
0.448327596386 1.21190130117
0.461913281125 1.25077107653
0.475498965864 1.29136212513
0.489084650603 1.33389745871
0.502670335342 1.37864623156
0.516256020081 1.42593741909
0.52984170482 1.4761789736
0.543427389559 1.52988532012
0.557013074298 1.58771796865
0.570598759037 1.65054755084
0.584184443776 1.7195524606
0.597770128515 1.79638352663
0.611355813254 1.88345607899
0.624941497993 1.98450970316
0.638527182732 2.10579763208
0.652112867471 2.2590096956
0.66569855221 2.47026455365


==> figuresAndData/dataForSingleLaplace-midPoint-lambda1prob0pt75.tex <==
0.0 0.69314718056
0.00563856862005 0.707340256107
0.0112771372401 0.72173188896
0.0169157058602 0.736330318642
0.0225542744802 0.75114430494
0.0281928431003 0.766183172637
0.0338314117203 0.781456861177
0.0394699803404 0.796975979898
0.0451085489604 0.812751869615
0.0507471175805 0.828796671446
0.0563856862005 0.845123403931
0.0620242548206 0.861746049666
0.0676628234407 0.878679652904
0.0733013920607 0.895940429827
0.0789399606808 0.913545893521
0.0845785293008 0.931514996059
0.0902170979209 0.949868290605
0.0958556665409 0.96862811699
0.101494235161 0.987818815
0.107132803781 1.00746697045
0.112771372401 1.02760170034
0.118409941021 1.04825498469
0.124048509641 1.06946205472
0.129687078261 1.09126184897
0.135325646881 1.11369755248
0.140964215501 1.13681723761
0.146602784121 1.16067463054
0.152241352741 1.18533003413
0.157879921362 1.21085144719
0.163518489982 1.23731593244
0.169157058602 1.26481130259
0.174795627222 1.29343821777
0.180434195842 1.32331282067
0.186072764462 1.3545700842
0.191711333082 1.38736811578
0.197349901702 1.4218937664
0.202988470322 1.45837005007
0.208627038942 1.49706612322
0.214265607562 1.53831096324
0.219904176182 1.5825125243
0.225542744802 1.63018523314
0.231181313422 1.68199060134
0.236819882042 1.738799262
0.242458450662 1.80178961035
0.248097019282 1.87261247625
0.253735587902 1.9536831908
0.259374156523 2.04874134039
0.265012725143 2.16404015869
0.270651293763 2.31126947619
0.276289862383 2.51654795332


==> figuresAndData/dataForSingleLaplace-midPoint-lambda1prob0pt85.tex <==
0.0 0.948559992443
0.00318537101816 0.960867683898
0.00637074203631 0.973374829895
0.00955611305447 0.986089670144
0.0127414840726 0.999020964612
0.0159268550908 1.01217803826
0.0191122261089 1.02557083072
0.0222975971271 1.03920995148
0.0254829681453 1.05310674154
0.0286683391634 1.06727334217
0.0318537101816 1.08172277207
0.0350390811997 1.09646901401
0.0382244522179 1.11152711237
0.041409823236 1.1269132835
0.0445951942542 1.14264504062
0.0477805652723 1.15874133596
0.0509659362905 1.1752227228
0.0541513073087 1.19211154112
0.0573366783268 1.20943213083
0.060522049345 1.22721107788
0.0637074203631 1.24547749938
0.0668927913813 1.26426337548
0.0700781623994 1.2836039375
0.0732635334176 1.3035381241
0.0764489044358 1.32410912044
0.0796342754539 1.34536499897
0.0828196464721 1.36735948598
0.0860050174902 1.39015288441
0.0891903885084 1.41381319317
0.0923757595265 1.43841747507
0.0955611305447 1.46405354292
0.0987465015628 1.4908220569
0.101931872581 1.5188391598
0.105117243599 1.54823982461
0.108302614617 1.57918215879
0.111487985635 1.61185301343
0.114673356654 1.64647540259
0.117858727672 1.68331848274
0.12104409869 1.72271123135
0.124229469708 1.76506160263
0.127414840726 1.81088402337
0.130600211744 1.86084000519
0.133785582763 1.91580018124
0.136970953781 1.97694294677
0.140156324799 2.04591913169
0.143341695817 2.12514406711
0.146527066835 2.21835733945
0.149712437853 2.33181218242
0.152897808872 2.47719842651
0.15608317989 2.68063473215


==> figuresAndData/dataForSingleLaplace-rightEnd-lambda1.tex <==
0.0 1.20397280433
0.0069908289012 1.22746817106
0.0139816578024 1.25135924349
0.0209724867036 1.27566250011
0.0279633156048 1.30039545994
0.034954144506 1.32557677201
0.0419449734072 1.35122631467
0.0489358023084 1.37736530608
0.0559266312096 1.40401642737
0.0629174601108 1.43120396028
0.069908289012 1.45895394141
0.0768991179132 1.48729433547
0.0838899468144 1.5162552305
0.0908807757156 1.54586905844
0.0978716046168 1.57617084499
0.104862433518 1.60719849389
0.111853262419 1.63899311104
0.11884409132 1.67159937571
0.125834920222 1.70506596706
0.132825749123 1.73944605636
0.139816578024 1.77479787721
0.146807406925 1.81118538933
0.153798235826 1.84867905475
0.160789064728 1.88735675027
0.167779893629 1.92730484562
0.17477072253 1.96861948522
0.181761551431 2.01140812111
0.188752380332 2.05579135871
0.195743209234 2.10190519538
0.202734038135 2.14990375628
0.209724867036 2.19996266659
0.216715695937 2.25228324628
0.223706524838 2.30709778054
0.23069735374 2.36467621496
0.237688182641 2.42533476414
0.244679011542 2.48944712989
0.251669840443 2.55745934003
0.258660669344 2.62990970722
0.265651498246 2.70745618611
0.272642327147 2.79091468486
0.279633156048 2.8813140568
0.286623984949 2.97997732499
0.29361481385 3.08864575549
0.300605642752 3.20967613865
0.307596471653 3.3463701341
0.314587300554 3.50355840394
0.321578129455 3.68872012087
0.328568958356 3.91436175221
0.335559787258 4.20386295884
0.342550616159 4.60946106158


==> figuresAndData/dataForSingleLaplace-rightEnd-lambda1prob0pt5.tex <==
0.0 0.69314718056
0.013585684739 0.720505665882
0.0271713694779 0.748248872626
0.0407570542169 0.776393266692
0.0543427389559 0.804956354745
0.0679284236949 0.833956773698
0.0815141084338 0.863414390034
0.0950997931728 0.893350410269
0.108685477912 0.92378750413
0.122271162651 0.954749942198
0.13585684739 0.986263750154
0.149442532129 1.01835688204
0.163028216868 1.05105941548
0.176613901607 1.0844037722
0.190199586346 1.11842496799
0.203785271085 1.15316089688
0.217370955824 1.18865265533
0.230956640563 1.22494491341
0.244542325302 1.26208634135
0.258128010041 1.3001301017
0.271713694779 1.33913441963
0.285299379518 1.37916324666
0.298885064257 1.42028703689
0.312470748996 1.4625836594
0.326056433735 1.50613947652
0.339642118474 1.55105062548
0.353227803213 1.59742455137
0.366813487952 1.64538185298
0.380399172691 1.69505852123
0.39398485743 1.74660867513
0.407570542169 1.80020793397
0.421156226908 1.85605761207
0.434741911647 1.91438998924
0.448327596386 1.97547500595
0.461913281125 2.03962887193
0.475498965864 2.10722528439
0.489084650603 2.17871026681
0.502670335342 2.25462212778
0.516256020081 2.3356188181
0.52984170482 2.42251624239
0.543427389559 2.51634325069
0.557013074298 2.618422863
0.570598759037 2.73049634264
0.584184443776 2.85492047742
0.597770128515 2.99499692475
0.611355813254 3.15555634472
0.624941497993 3.34407790833
0.638527182732 3.57306808143
0.652112867471 3.86590652372
0.66569855221 4.27483055509


==> figuresAndData/dataForSingleLaplace-rightEnd-lambda1prob0pt75.tex <==
0.0 1.38629436112
0.00563856862005 1.40904194359
0.0112771372401 1.43218664068
0.0169157058602 1.45574493142
0.0225542744802 1.4797343354
0.0281928431003 1.50417350217
0.0338314117203 1.52908231063
0.0394699803404 1.55448197946
0.0451085489604 1.58039519027
0.0507471175805 1.60684622531
0.0563856862005 1.63386112166
0.0620242548206 1.66146784451
0.0676628234407 1.68969648237
0.0733013920607 1.71857946759
0.0789399606808 1.74815182636
0.0845785293008 1.77845146282
0.0902170979209 1.80951948329
0.0958556665409 1.84140056744
0.101494235161 1.87414339484
0.107132803781 1.90780113712
0.112771372401 1.94243202828
0.118409941021 1.97810002837
0.124048509641 2.0148755998
0.129687078261 2.05283661967
0.135325646881 2.09206945807
0.140964215501 2.13267025972
0.146602784121 2.17474647696
0.152241352741 2.21841871552
0.157879921362 2.26382297302
0.163518489982 2.31111337489
0.169157058602 2.36046554659
0.174795627222 2.41208080831
0.180434195842 2.46619144549
0.186072764462 2.52306740394
0.191711333082 2.58302489847
0.197349901702 2.6464376311
0.202988470322 2.71375162982
0.208627038942 2.7855052075
0.214265607562 2.86235631892
0.219904176182 2.94512087242
0.225542744802 3.03482772147
0.231181313422 3.13279988925
0.236819882042 3.24077864196
0.242458450662 3.36112077004
0.248097019282 3.49712793323
0.253735587902 3.6536307937
0.259374156523 3.83810852425
0.265012725143 4.06306759224
0.270651293763 4.35188765863
0.276289862383 4.75680604425


==> figuresAndData/dataForSingleLaplace-rightEnd-lambda1prob0pt85.tex <==
0.0 1.89711998489
0.00318537101816 1.91854999678
0.00637074203631 1.94037891775
0.00955611305447 1.96262322723
0.0127414840726 1.98530044515
0.0159268550908 2.00842922144
0.0191122261089 2.03202943532
0.0222975971271 2.05612230583
0.0254829681453 2.08073051493
0.0286683391634 2.10587834517
0.0318537101816 2.13159183396
0.0350390811997 2.15789894681
0.0382244522179 2.18482977252
0.041409823236 2.21241674377
0.0445951942542 2.24069488699
0.0477805652723 2.26970210664
0.0509659362905 2.29947950931
0.0541513073087 2.33007177493
0.0573366783268 2.36152758334
0.060522049345 2.39390010642
0.0637074203631 2.42724757839
0.0668927913813 2.46163395958
0.0700781623994 2.4971297126
0.0732635334176 2.53381271479
0.0764489044358 2.57176933644
0.0796342754539 2.61109572249
0.0828196464721 2.65189932548
0.0860050174902 2.69430075132
0.0891903885084 2.73843599783
0.0923757595265 2.78445919062
0.0955611305447 2.83254595529
0.0987465015628 2.88289761224
0.101931872581 2.93574644702
0.105117243599 2.99136240562
0.108302614617 3.05006170297
0.111487985635 3.11221804122
0.114673356654 3.17827744852
0.117858727672 3.24877823781
0.12104409869 3.32437836401
0.124229469708 3.40589373555
0.127414840726 3.49435320601
0.130600211744 3.59107979863
0.133785582763 3.69781477971
0.136970953781 3.81691493976
0.140156324799 3.95168193858
0.143341695817 4.1069464384
0.146527066835 4.29018761207
0.149712437853 4.51391192699
0.152897808872 4.80149904414
0.15608317989 5.20518628441


==> figuresAndData/dataForUniformSigma1.tex <==
0.998 4e-06
0.996 1.6e-05
0.994 3.6e-05
0.992 6.4e-05
0.99 0.0001
0.988 0.000144
0.986 0.000196
0.984 0.000256
0.982 0.000324
0.98 0.0004
0.978 0.000484
0.976 0.000576
0.974 0.000676
0.972 0.000784
0.97 0.0009
0.968 0.001024
0.966 0.001156
0.964 0.001296
0.962 0.001444
0.96 0.0016
0.958 0.001764
0.956 0.001936
0.954 0.002116
0.952 0.002304
0.95 0.0025
0.948 0.002704
0.946 0.002916
0.944 0.003136
0.942 0.003364
0.94 0.0036
0.938 0.003844
0.936 0.004096
0.934 0.004356
0.932 0.004624
0.93 0.0049
0.928 0.005184
0.926 0.005476
0.924 0.005776
0.922 0.006084
0.92 0.0064
0.918 0.006724
0.916 0.007056
0.914 0.007396
0.912 0.007744
0.91 0.0081
0.908 0.008464
0.906 0.008836
0.904 0.009216
0.902 0.009604
0.9 0.01
0.898 0.010404
0.896 0.010816
0.894 0.011236
0.892 0.011664
0.89 0.0121
0.888 0.012544
0.886 0.012996
0.884 0.013456
0.882 0.013924
0.88 0.0144
0.878 0.014884
0.876 0.015376
0.874 0.015876
0.872 0.016384
0.87 0.0169
0.868 0.017424
0.866 0.017956
0.864 0.018496
0.862 0.019044
0.86 0.0196
0.858 0.020164
0.856 0.020736
0.854 0.021316
0.852 0.021904
0.85 0.0225
0.848 0.023104
0.846 0.023716
0.844 0.024336
0.842 0.024964
0.84 0.0256
0.838 0.026244
0.836 0.026896
0.834 0.027556
0.832 0.028224
0.83 0.0289
0.828 0.029584
0.826 0.030276
0.824 0.030976
0.822 0.031684
0.82 0.0324
0.818 0.033124
0.816 0.033856
0.814 0.034596
0.812 0.035344
0.81 0.0361
0.808 0.036864
0.806 0.037636
0.804 0.038416
0.802 0.039204
0.8 0.04
0.798 0.040804
0.796 0.041616
0.794 0.042436
0.792 0.043264
0.79 0.0441
0.788 0.044944
0.786 0.045796
0.784 0.046656
0.782 0.047524
0.78 0.0484
0.778 0.049284
0.776 0.050176
0.774 0.051076
0.772 0.051984
0.77 0.0529
0.768 0.053824
0.766 0.054756
0.764 0.055696
0.762 0.056644
0.76 0.0576
0.758 0.058564
0.756 0.059536
0.754 0.060516
0.752 0.061504
0.75 0.0625
0.748 0.063504
0.746 0.064516
0.744 0.065536
0.742 0.066564
0.74 0.0676
0.738 0.068644
0.736 0.069696
0.734 0.070756
0.732 0.071824
0.73 0.0729
0.728 0.073984
0.726 0.075076
0.724 0.076176
0.722 0.077284
0.72 0.0784
0.718 0.079524
0.716 0.080656
0.714 0.081796
0.712 0.082944
0.71 0.0841
0.708 0.085264
0.706 0.086436
0.704 0.087616
0.702 0.088804
0.7 0.09
0.698 0.091204
0.696 0.092416
0.694 0.093636
0.692 0.094864
0.69 0.0961
0.688 0.097344
0.686 0.098596
0.684 0.099856
0.682 0.101124
0.68 0.1024
0.678 0.103684
0.676 0.104976
0.674 0.106276
0.672 0.107584
0.67 0.1089
0.668 0.110224
0.666 0.111556
0.664 0.112896
0.662 0.114244
0.66 0.1156
0.658 0.116964
0.656 0.118336
0.654 0.119716
0.652 0.121104
0.65 0.1225
0.648 0.123904
0.646 0.125316
0.644 0.126736
0.642 0.128164
0.64 0.1296
0.638 0.131044
0.636 0.132496
0.634 0.133956
0.632 0.135424
0.63 0.1369
0.628 0.138384
0.626 0.139876
0.624 0.141376
0.622 0.142884
0.62 0.1444
0.618 0.145924
0.616 0.147456
0.614 0.148996
0.612 0.150544
0.61 0.1521
0.608 0.153664
0.606 0.155236
0.604 0.156816
0.602 0.158404
0.6 0.16
0.598 0.161604
0.596 0.163216
0.594 0.164836
0.592 0.166464
0.59 0.1681
0.588 0.169744
0.586 0.171396
0.584 0.173056
0.582 0.174724
0.58 0.1764
0.578 0.178084
0.576 0.179776
0.574 0.181476
0.572 0.183184
0.57 0.1849
0.568 0.186624
0.566 0.188356
0.564 0.190096
0.562 0.191844
0.56 0.1936
0.558 0.195364
0.556 0.197136
0.554 0.198916
0.552 0.200704
0.55 0.2025
0.548 0.204304
0.546 0.206116
0.544 0.207936
0.542 0.209764
0.54 0.2116
0.538 0.213444
0.536 0.215296
0.534 0.217156
0.532 0.219024
0.53 0.2209
0.528 0.222784
0.526 0.224676
0.524 0.226576
0.522 0.228484
0.52 0.2304
0.518 0.232324
0.516 0.234256
0.514 0.236196
0.512 0.238144
0.51 0.2401
0.508 0.242064
0.506 0.244036
0.504 0.246016
0.502 0.248004
0.5 0.25
0.498 0.252004
0.496 0.254016
0.494 0.256036
0.492 0.258064
0.49 0.2601
0.488 0.262144
0.486 0.264196
0.484 0.266256
0.482 0.268324
0.48 0.2704
0.478 0.272484
0.476 0.274576
0.474 0.276676
0.472 0.278784
0.47 0.2809
0.468 0.283024
0.466 0.285156
0.464 0.287296
0.462 0.289444
0.46 0.2916
0.458 0.293764
0.456 0.295936
0.454 0.298116
0.452 0.300304
0.45 0.3025
0.448 0.304704
0.446 0.306916
0.444 0.309136
0.442 0.311364
0.44 0.3136
0.438 0.315844
0.436 0.318096
0.434 0.320356
0.432 0.322624
0.43 0.3249
0.428 0.327184
0.426 0.329476
0.424 0.331776
0.422 0.334084
0.42 0.3364
0.418 0.338724
0.416 0.341056
0.414 0.343396
0.412 0.345744
0.41 0.3481
0.408 0.350464
0.406 0.352836
0.404 0.355216
0.402 0.357604
0.4 0.36
0.398 0.362404
0.396 0.364816
0.394 0.367236
0.392 0.369664
0.39 0.3721
0.388 0.374544
0.386 0.376996
0.384 0.379456
0.382 0.381924
0.38 0.3844
0.378 0.386884
0.376 0.389376
0.374 0.391876
0.372 0.394384
0.37 0.3969
0.368 0.399424
0.366 0.401956
0.364 0.404496
0.362 0.407044
0.36 0.4096
0.358 0.412164
0.356 0.414736
0.354 0.417316
0.352 0.419904
0.35 0.4225
0.348 0.425104
0.346 0.427716
0.344 0.430336
0.342 0.432964
0.34 0.4356
0.338 0.438244
0.336 0.440896
0.334 0.443556
0.332 0.446224
0.33 0.4489
0.328 0.451584
0.326 0.454276
0.324 0.456976
0.322 0.459684
0.32 0.4624
0.318 0.465124
0.316 0.467856
0.314 0.470596
0.312 0.473344
0.31 0.4761
0.308 0.478864
0.306 0.481636
0.304 0.484416
0.302 0.487204
0.3 0.49
0.298 0.492804
0.296 0.495616
0.294 0.498436
0.292 0.501264
0.29 0.5041
0.288 0.506944
0.286 0.509796
0.284 0.512656
0.282 0.515524
0.28 0.5184
0.278 0.521284
0.276 0.524176
0.274 0.527076
0.272 0.529984
0.27 0.5329
0.268 0.535824
0.266 0.538756
0.264 0.541696
0.262 0.544644
0.26 0.5476
0.258 0.550564
0.256 0.553536
0.254 0.556516
0.252 0.559504
0.25 0.5625
0.248 0.565504
0.246 0.568516
0.244 0.571536
0.242 0.574564
0.24 0.5776
0.238 0.580644
0.236 0.583696
0.234 0.586756
0.232 0.589824
0.23 0.5929
0.228 0.595984
0.226 0.599076
0.224 0.602176
0.222 0.605284
0.22 0.6084
0.218 0.611524
0.216 0.614656
0.214 0.617796
0.212 0.620944
0.21 0.6241
0.208 0.627264
0.206 0.630436
0.204 0.633616
0.202 0.636804
0.2 0.64
0.198 0.643204
0.196 0.646416
0.194 0.649636
0.192 0.652864
0.19 0.6561
0.188 0.659344
0.186 0.662596
0.184 0.665856
0.182 0.669124
0.18 0.6724
0.178 0.675684
0.176 0.678976
0.174 0.682276
0.172 0.685584
0.17 0.6889
0.168 0.692224
0.166 0.695556
0.164 0.698896
0.162 0.702244
0.16 0.7056
0.158 0.708964
0.156 0.712336
0.154 0.715716
0.152 0.719104
0.15 0.7225
0.148 0.725904
0.146 0.729316
0.144 0.732736
0.142 0.736164
0.14 0.7396
0.138 0.743044
0.136 0.746496
0.134 0.749956
0.132 0.753424
0.13 0.7569
0.128 0.760384
0.126 0.763876
0.124 0.767376
0.122 0.770884
0.12 0.7744
0.118 0.777924
0.116 0.781456
0.114 0.784996
0.112 0.788544
0.11 0.7921
0.108 0.795664
0.106 0.799236
0.104 0.802816
0.102 0.806404
0.1 0.81
0.098 0.813604
0.096 0.817216
0.094 0.820836
0.092 0.824464
0.09 0.8281
0.088 0.831744
0.086 0.835396
0.084 0.839056
0.082 0.842724
0.08 0.8464
0.078 0.850084
0.076 0.853776
0.074 0.857476
0.072 0.861184
0.07 0.8649
0.068 0.868624
0.066 0.872356
0.064 0.876096
0.062 0.879844
0.06 0.8836
0.058 0.887364
0.056 0.891136
0.054 0.894916
0.052 0.898704
0.05 0.9025
0.048 0.906304
0.046 0.910116
0.044 0.913936
0.042 0.917764
0.04 0.9216
0.038 0.925444
0.036 0.929296
0.034 0.933156
0.032 0.937024
0.03 0.9409
0.028 0.944784
0.026 0.948676
0.024 0.952576
0.022 0.956484
0.02 0.9604
0.018 0.964324
0.016 0.968256
0.014 0.972196
0.012 0.976144
0.01 0.9801
0.008 0.984064
0.006 0.988036
0.004 0.992016
0.002 0.996004

